Space- and Computationally-Efficient Set Reconciliation via Parity Bitmap Sketch (PBS)

Set reconciliation is a fundamental algorithmic problem that arises in many networking, system, and database applications. In this problem, two large sets A and B of objects (bitcoins, files, records, etc.) are stored respectively at two different network-connected hosts, which we name Alice and Bob respectively. Alice and Bob communicate with each other to learn $A\Delta B$, the difference between A and B, and as a result the reconciled set $A\bigcup B$. Current set reconciliation schemes are based on either Invertible Bloom Filters (IBF) or Error-Correction Codes (ECC). The former has a low computational complexity of O(d), where d is the cardinality of $A\Delta B$, but has a high communication overhead that is several times larger than the theoretical minimum. The latter has a low communication overhead close to the theoretical minimum, but has a much higher computational complexity of $O(d^2)$. In this work, we propose Parity Bitmap Sketch (PBS), an ECC- based set reconciliation scheme that gets the better of both worlds: PBS has both a low computational complexity of O(d) just like IBF-based solutions and a low communication overhead of roughly twice the theoretical minimum. A separate contribution of this work is a novel rigorous analytical framework that can be used for the precise calculation of various performance metrics and for the near-optimal parameter tuning of PBS.

==> section/abstract_copy.tex <==
\begin{abstract}
Set reconciliation is a fundamental algorithmic problem that arises in many networking, systems, and database applications. Current set reconciliation schemes are based on either Invertible Bloom Filters (IBF) or Error-Correction Codes (ECC). The former has a high communication overhead that is several times larger than the theoretical optimal. The later has a high computational complexity when the cardinality of the set difference is large. 

In this paper, we propose Parity Bitmap Sketch (PBS), an ECC-based set reconciliation scheme that achieves a much better tradeoff between communication overhead and computational complexity than existing solutions: PBS has both a low computational complexity of $O(d)$ just like IBF-based solutions and a low communication overhead of roughly $2$ times the theoretical optimal. Compare to other ECC-based schemes, PBS uses a hash-partition technique to reduce computational complexity by paying small additional communication overhead. Although this technique may reduce the computational complexity of other ECC-based schemes (e.g., PinSketch), the additional communication overhead is much larger. 
\end{abstract}

==> section/applications_of_theoretical_analysis0222.tex <==
\section{Applications of the analytical framework}\label{sec:application_analysis}

In this section, we describe three main applications of the analytical framework described in \autoref{sec:tail_bound}, which are (1) parameter settings; (2) analyzing the affect of the target number of round $r$; (3) analyzing the affect of ``piecewise decodability''. 

\subsection{Parameter Settings}\label{sec:parameter_settings}

In this section, we elaborate how to set the parameters $n$, $t$, and $g$ given the target success probability $p_0$ within $r$ rounds (the probability that PBS successfully reconciles all distinct elements within $r$ rounds to be larger than $p_0$) in PBS. We continue to assume $d$ is precisely known. First, as explained in \autoref{subsec:protocol2}, $\delta$ should be a small number, so we fix $\delta=5$ and therefore $g=d/\delta$ is also fixed. 
Given the target success probability $p_0$ within $r$ rounds
%(i.e., set reconciliation is complete in $r$ rounds with probability $p_0$) 
%depend on the requirement of specific applications)
, the parameter setting problem aims to find the optimal parameter settings of $n,t$ that minimizes the overall communication overhead, under the constraint that the tail bound of the success probability of $r$ rounds is larger than $p_0$. Note that the overall communication overhead is only slightly larger than the communication overhead in the first round (to be explained in \autoref{sec:piecewise_decodability}), so we minimize the later instead of the former in the parameter setting problem. Furthermore, the later (i.e., the communication overhead in the first round) for each group pair (described in \autoref{sec:multi-rounds}) contains only two terms $t\log n+\delta\log n$ that depend on parameter settings. So we only need to minimize $t\log n+\delta\log n$ in the parameter setting problem, which can be formalized as the following optimization problem:

% \begin{equation}
% \min\limits_{n,t} t\log n+\delta\log n \quad \mbox{s.t.}\quad 1-2(1-\alpha^g(n,t))>p_0
% \end{equation}

\begin{align}
\mbox{minimize} \quad
&
t\log n+\delta\log n \nonumber
\\
\mbox{subject to} \quad 
&
1-2(1-\alpha^g(n,t))>p_0,\quad n,t\in \mathbb{N}^+ \nonumber
% \\
% &
% n,t\in \mathbb{N}^+ \label{eq:row_sum_requirement}
\end{align}

This optimization problem is not as daunting as it looks, since we can narrow down its solution space into only a few combinations and traverse all these combinations to find the optimal parameter settings as follows: First, since $n$ is the ``code length'' of BCH code, we select $n$ to be $2^m-1$ for some integer $m$ for BCH coding efficiency. Then the range of $n$ is narrowed down to $\{63,127,255,511,1023,2047\}$ (recall that $n=\Omega(\delta^2)$). Second, we select $t$ in the range from $1.5\delta$ to $3.5\delta$, since any smaller $t$ will cause a high probability of BCH decoding failure (explained in \autoref{subsec:protocol2}) and therefore a low success probability (below $50\%$), and any higher $t$ incurs significant additional communication overhead on transmitting BCH codeword (explained in \autoref{subsec:protocol2}) while barely increases the success probability.

% This optimization problem seems to be difficult to solve, since the constraint is a very comprehensive function of the parameters (remind that $\alpha=\alpha(n,t)$ is a function of $n$ and $t$ for arbitrary $r$, $d$, and $g$). However, we can narrow down the solution space into only a few combinations and traverse all these combinations to find the optimal parameter settings as follows: First, for BCH coding efficiency, we select $n$ to be $2^m-1$ for some integer $m$ and therefore narrow its range down to $\{63,127,255,511,1023\}$ (recall that $n=\Omega(\delta^2)$). Second, we select $t$ in the range from $1.5\delta$ to $3\delta$, as we suggested in \autoref{subsec:protocol2}. 

Here we use an example to show how we set parameters: Given $d=\num{1000}$ distinct elements, $r=3$ rounds, $p_0=99\%$, for each $(n,t)$ combination in $\{63,127,255,511,1023,2047\}\times \{8,9,...,16,17\}$, we compute the tail bound of the success probability under the parameter settings and obtain \autoref{tab:success_prob}.

\begin{table}[h]
\setlength{\tabcolsep}{3.2pt}
\centering
\caption{Tail bounds of the success probability under different parameter settings ($d=\num{1000}$, $r=3$)}\label{tab:success_prob}
\begin{tabular}{@{}|c|c|c|c|c|c|c|@{}}
\hline 
\diagbox{$t$}{$n$}    & $63$ & $127$ & $255$ & $511$ & $1023$ & $2047$ \\ \hline 
8   & 0 & 25.5\% & 32.7\% & 34.3\% & 34.9\% & 35.0\% \\ \hline
9   & 52.1\% & 78.0\% & 84.2\% & 85.7\% & 86.1\% & 86.2\% \\ \hline
10  & 75.1\% & 92.7\% & 96.5\% & 97.4\% & 97.6\% & 97.7\% \\ \hline
11  & 85.9\% & 96.9\% & \cellcolor{blue!25}99.1\% & \cellcolor{blue!25}99.5\% & \cellcolor{blue!25}99.6\% & \cellcolor{blue!25}99.6\% \\ \hline
12  & 91.3\% & 98.5\% & \cellcolor{blue!25}99.7\% & \cellcolor{blue!25}99.9\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% \\ \hline
13  & 93.9\% & \cellcolor{blue!60}99.1\% & \cellcolor{blue!25}99.8\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% \\ \hline
14  & 95.1\% & \cellcolor{blue!25}99.4\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% \\ \hline
15  & 95.6\% & \cellcolor{blue!25}99.5\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% \\ \hline
16  & 95.7\% & \cellcolor{blue!25}99.6\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% \\ \hline
17  & 95.8\% & \cellcolor{blue!25}99.6\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% \\ \hline
\end{tabular}
\end{table}

In \autoref{tab:success_prob}, all $(n,t)$ combinations in the highlighted cells satisfy the success probability requirement. Among them, $(127,13)$ has the lowest communication overhead (w.r.t. $t\log n+\delta\log n$). So we set $n=127, t=13$ in this case. For the case of the set difference cardinality $d$ is not precisely known, we use the scaled estimation of $d$ (described in \autoref{subsec:ToW}) for parameter settings, which is larger than the actual $d$ with high probability. The computed optimal parameter $n$ and $t$ based on an overestimation of $d$ is always sufficient to achieve the success probability. {\bf Note that calculating the probabilities in this table is very fast, since each entry in the table can be computed in $O(1)$ time given $M^r$, and $M^r$ for each $n\in\{63,127,255,511,1023,2047\}$ ($M$ is a function of $n$) can be precomputed in $O(t^3)$ time.}

\subsection{What if the target number of rounds $r$ changes?}\label{sec:vary_r}

Note that for each possible target number of rounds $r$ (while keeping the same target success probability $p_0=99\%$), we can also compute a success probability table that is similar to \autoref{tab:success_prob} to obtain the corresponding optimal $n$ and $t$. 
%For example, when $r=1$, the optimal parameter setting is $n=524287$ and $t=16$; when $r=2$, the optimal parameter setting is $n=1023$ and $t=16$. 
The results are shown in \autoref{tab:vary_r} for $r=1,2,3,4$ using the same example above ($p_0=99\%, d=1000$). \autoref{tab:vary_r} also compares the {\it communication overhead per group pair} for each $r$, which accounts both the `constant' communication overhead that does not depend on the parameter settings (i.e., $\delta\log |\mathcal{U}|+32=192$ bits) and the `tunable' communication overhead that does depend on the parameter settings (i.e., the objective function $t\log n+\delta\log n$). The {\it communication overhead per distinct element}, which is simply equal to the communication overhead per group pair divided by $\delta$ (since each group pair contains $\delta$ distinct elements on average), is also compared in \autoref{tab:vary_r}. It shows that if we increase the target number of rounds $r$ while keeping the same target probability $p_0$ and therefore `loosen' the parameter setting requirement, the communication overhead (per distinct element) that is needed to achieve this requirement decreases. For instance, the communication overhead per distinct element is reduced by $32\%$ from $r=1$ to $r=2$, and that number from $r=2$ to $r=3$ and from $r=3$ to $r=4$ is $21\%$ and $10\%$ respectively. This ``saving'' on the communication overhead decreases as $r$ increases, so we set $r$ to the tune of $3$, which is a `sweet spot' that achieves the most ``saving'' on the communication overhead while not taking too many rounds to reconcile all distinct elements. 

\autoref{tab:vary_r} also shows that the optimal $n$ decreases as $r$ increases. Recall that the computational complexity per finite field operations in BCH decoding is $O(\log^2 n)$ (quadratic to the ``width" of the Galois field), which means the BCH decoding complexity also decreases as $r$ increases. Here $r=3$ is also a `sweet spot' that achieves the most `savings' on BCH decoding complexity (the complexity decreases as $O(19^2)\rightarrow O(10^2)\rightarrow O(7^2)\rightarrow O(6^2)$ when $r$ increases from $1$ to $4$). Note that the above analysis only shows that $r=3$ is a `sweet spot' when the target success probability is $p_0=99\%$. The `sweet spot' of $r$ could be different for various target success probabilities. However, we fix $r$ to be $3$ in our evaluation, since it is the `sweet spot' for the two target success probabilities to be used in our evaluation, which are $p_0=99\%$ and $p_0=99.58\%$ $(239/240)$, using the same analysis above.
%The communication overhead per group pair is $220$ bits, $210$ bits parameter settings when $r=3$ ($n=127, t=13$), this optimal parameter settings ($n=1023, t=16$) are much larger (more expensive) and incur additional communication overhead of $84$ bits per group pair. It shows that to achieve the same target success probability using fewer rounds (smaller $r$), PBS need more resources (e.g., larger $n$, $t$). Note that the optimal parameter settings when $r=1$ are even larger ($n=2047, t=15$) and incur even more additional communication overhead ($94$ bits comparing to the optimal parameter settings when $r=3$), which shows that running PBS for multiple rounds saves a considerate amount of communication overhead comparing to running PBS for only $1$ round when achieving the same target success probability.}

\begin{table}[h]
\centering
\caption{Vary $r$ ($p_0=99\%, d=1000$)}\label{tab:vary_r}
\begin{tabular}{@{}|c|c|c|c|c|@{}}
\hline 
$r$   & $1$ & $2$ & $3$ & $4$ \\ \hline 
Optimal $n$   & $524287$ & $1023$ & $127$ & $63$ \\ \hline
Optimal $t$   & $16$ & $16$ & $13$ & $11$ \\ \hline
\makecell{Objective function \\$t\log n+\delta\log n$}  & $399$ & $210$ & $126$ & $96$ \\ \hline
\makecell{Communication overhead \\per group pair (bits)}  & $591$ & $402$ & $318$ & $288$ \\ \hline
\makecell{Communication overhead \\per distinct element (bits)} & $118.2$ & $80.4$ & $63.6$ & $57.6$ \\ \hline
\end{tabular}
\end{table}

% Hidden table for d=10000
% \begin{table}[h]
% \centering
% \caption{Vary the target number of round $r$}\label{tab:vary_r}
% \begin{tabular}{@{}|c|c|c|c|@{}}
% \hline 
% $r$   & $1$ & $2$ & $3$ \\ \hline 
% Optimal $(n,t)$   & $(4096,14)$ & $(4095,17)$ & $(255,14)$ \\ \hline
% Objective function $t\log n+\delta\log n$  & $220$ & $210$ & $126$ \\ \hline
% Communication overhead per group pair (bits)  & $412$ & $402$ & $318$ \\ \hline
% Communication overhead per distinct element (bits) & $82.4$ & $80.4$ & $63.6$ \\ \hline
% \end{tabular}
% \end{table}

% {\bf (change r)} If we reduce the number of rounds $r$ from $3$ to $2$ while keeping the same target success probability $p_0=99\%$, we can also compute a success probability table that is similar to \autoref{tab:success_prob} to obtain the optimal parameter setting, which is $n=1023, t=16$. Compare to the previous optimal parameter settings when $r=3$ ($n=127, t=13$), this optimal parameter settings ($n=1023, t=16$) are much larger (more expensive) and incur additional communication overhead of $84$ bits per group pair. It shows that to achieve the same target success probability using fewer rounds (smaller $r$), PBS need more resources (e.g., larger $n$, $t$). Note that the optimal parameter settings when $r=1$ are even larger ($n=2047, t=15$) and incur even more additional communication overhead ($94$ bits comparing to the optimal parameter settings when $r=3$), which shows that running PBS for multiple rounds saves a considerate amount of communication overhead comparing to running PBS for only $1$ round when achieving the same target success probability.}

% {\bf Readers may think we can further increase $r$ (keeping the same target success probability) to reduce communication overhead. However, it could make PBS taking too many rounds to reconcile all distinct elements.} 
%Also, further increasing $r$ does not save much communication overhead. For example, if we increase $r$ from $3$ to $4$ (rounds), the optimal parameter setting becomes $n=63,t=11$, which only saves communication overhead of $30$ bits per group pair. }

\subsection{Analysis on ``Piecewise Decodability''}\label{sec:piecewise_decodability}

{\bf Note that PBS reconciles the distinct elements gradually round by round. The distinct elements that have been reconciled in the first round are no longer needed to be reconciled again and only the remaining distinct elements will be reconciled in the second round. This is the ``piecewise decodability'' mentioned in \autoref{sec:intro_oursolution}. Using the transition matrix $M$ (of the Markov chain described in \autoref{sec:single_markov}), we can theoretically analyze this ``piecewise decodability'' by computing the expected value of how many distinct elements would be reconciled in the each round as follows. 

Define $Z_i$ as the number of distinct elements that would be reconciled in the $i$-th round in an arbitrary group pair for $i=1,2,...$, and $X$ as the number of distinct elements in the group pair. $\mathbb{E}[Z_1|X=x]$, the expectation of $Z_1$ when the group pair contains exactly $x$ distinct elements, can be computed as $\sum_{y=0}^x y\cdot Pr[x\!\xrsquigarrow{1}\! y]$, where $Pr[x\!\xrsquigarrow{1}\! y]$ denotes the probability that starting with state $x$, the Markov chain (described in \autoref{sec:single_markov}) reaches state $y$ in $1$ transition, which is equal to $M(x,y)$. Recall that $X$ follows the Binomial distribution $Binomial(d,1/g)$, we can compute $\mathbb{E}[Z_1]$ given $d$, $g$, and $n$. $\mathbb{E}[Z_2]$, $\mathbb{E}[Z_3]$, ..., can also be computed (e.g., $\mathbb{E}[Z_2]$ can be computed based on $\mathbb{E}[Z_1+Z_2|X=x]=\sum_{y=0}^x y\cdot Pr[x\!\xrsquigarrow{2}\! y]$ and $\mathbb{E}[Z_1]$, where $Pr[x\!\xrsquigarrow{2}\! y]=\big{(}M^2\big{)}(x,y)$). We omit the details about the computation and only show results of the expected percentage of distinct elements are reconciled in each round (i.e., $Z_1/\delta$, $Z_2/\delta$, $Z_3/\delta$, and $Z_4/\delta$) under the optimal parameter settings above when $r=3$ and $p_0=0.99$ ($d=1000$, $g=200$, $n=127$, $t=13$) in \autoref{tab:reconcile_ratio}.
} %% added by long to prevent the all-bold issue
% Using the transition matrix $M$, we can compute the expected value of how many distinct elements are reconciled in each round. 
% From the transition matrix $M$, we can theoretically analyze this ``piecewise decodability'' by computing the expected value of how many distinct elements are reconciled in the each round. 
% $\mathbb{E}[Z|X=x]=\sum_{y=0}^x y\cdot Pr[x\!\xrsquigarrow{1}\! y]=\sum_{y=0}^x y\cdot M(x,y)$
% For example, $\sum_{l=0}^x l\cdot Pr[x\!\xrsquigarrow{1}\! l]$ is the average number of the distinct elements that are reconciled in the first round (for an arbitrary group pair with $x$ distinct elements). 
% Although this expected value in any scenario (given $d$, $n$, and $t$) is computable, we only show the `general' results in \autoref{tab:reconcile_ratio}, in which we assume $\delta_1,\delta_2,...,\delta_g$ follow the Poisson distribution with mean of $\delta$ (this is a tiny approximation for relatively large $d$, since the Poisson distribution is a limiting case of the Binomial distribution with the same expectation), and $t$ is sufficiently large. }
\begin{table}[h]
\centering
\caption{The expected percentage of the distinct elements would be reconciled in each round}\label{tab:reconcile_ratio}
\begin{tabular}{@{}|c|c|c|c|@{}}
\hline 
Round $1$ & Round $2$ & Round $3$ & Round $4$ \\ \hline 
0.962 & 0.0380 & $3.61\times 10^{-4}$ & $2.86\times 10^{-6}$ \\ \hline
% $127$  & 0.961 & 0.0382 & $3.7\times 10^{-4}$ & $2.9\times 10^{-6}$ \\ \hline
% $255$  & 0.981 & 0.0193 & $8.4\times 10^{-5}$ & $3.3\times 10^{-7}$ \\ \hline
% $511$ & 0.990 & 0.00972 & $2.0\times 10^{-5}$ & $3.9\times 10^{-8}$ \\ \hline
% $1023$ & 0.995 & 0.00487 & $4.9\times 10^{-6}$ & $4.8\times 10^{-9}$ \\ \hline
% \begin{table}[h]
% \centering
% \caption{Average percentage of distinct elements are reconciled per round}\label{tab:reconcile_ratio}
% \begin{tabular}{@{}|c|c|c|c|c|@{}}
% \hline 
% $n$   & Round $1$ & Round $2$ & Round $3$ & Round $4$ \\ \hline 
% $63$   & 0.924 & 0.0746 & $1.7\times 10^{-3}$ & $2.7\times 10^{-5}$ \\ \hline
% $127$  & 0.961 & 0.0382 & $3.7\times 10^{-4}$ & $2.9\times 10^{-6}$ \\ \hline
% $255$  & 0.981 & 0.0193 & $8.4\times 10^{-5}$ & $3.3\times 10^{-7}$ \\ \hline
% $511$ & 0.990 & 0.00972 & $2.0\times 10^{-5}$ & $3.9\times 10^{-8}$ \\ \hline
% $1023$ & 0.995 & 0.00487 & $4.9\times 10^{-6}$ & $4.8\times 10^{-9}$ \\ \hline
% $63$   & 0.924 & 0.0746 & 0.00167 & 0.0000274 \\ \hline
% $127$   & 0.961 & 0.0382 & 0.000365 & 0.00000289 \\ \hline
% $255$  & 0.981 & 0.0193 & 0.0000839 & 0.000000330 \\ \hline
% $511$ & 0.990 & 0.00972 & 0.0000200 & 0.0000000392 \\ \hline
% $1023$ & 0.995 & 0.00487 & 0.00000489 & 0.00000000478 \\ \hline
% \begin{tabular}{@{}|c|c|c|c|c|c|c|@{}}
% \hline 
% \diagbox{$r$}{$n$}    & $63$ & $127$ & $255$ & $511$ & $1023$ & $2047$ \\ \hline 
% 1   & 92.4\% & 96.1\% & 98.1\% & 99.0\% & 99.5\% & 99.8\% \\ \hline
% 2   & 7.46\% & 3.82\% & 1.93\% & 0.97\% & 0.49\% & 0.24\% \\ \hline
% 3  & $1.7\times 10^{-3}$ & $3.7\times 10^{-4}$ & $8.4\times 10^{-5}$ & $2.0\times 10^{-5}$ & $4.9\times 10^{-6}$ & $1.2\times 10^{-6}$ \\ \hline
% 4  & $2.7\times 10^{-5}$ & $2.9\times 10^{-6}$ & $3.3\times 10^{-7}$ & $3.9\times 10^{-8}$ & $4.8\times 10^{-9}$ & $5.9\times 10^{-10}$ \\ \hline
\end{tabular}
\end{table}

{\bf \autoref{tab:reconcile_ratio} shows that the majority of the distinct elements ($96.2\%$) are reconciled in the first round. Therefore, the communication overhead (roughly proportional to the number of distinct elements that are reconciled) in the first round is the major part of the overall communication overhead. This property can be similarily proved for other set reconciliation circumstances that have various number of distinct elements $d$ and various requirements (i.e., various $r$, and $p_0$).}  
%In other words, the overall communication overhead of all rounds is only slightly larger than that in the first round. 
Due to this reason, we use the communication overhead in the first round (described in \autoref{sec:communication_overhead_single_PBS}) to approximate the overall communication overhead of all rounds in parameter settings in \autoref{sec:parameter_settings}. {\bf \autoref{tab:reconcile_ratio} also shows that the number of remaining distinct elements (the ones that have not been reconciled) decreases exponentially round after round. }

==> section/applications_of_theoretical_analysis0224.tex <==
\section{Applications of the analytical framework}\label{sec:application_analysis}

In this section, we describe three main applications of the analytical framework described in \autoref{sec:tail_bound}, which are (1) parameter settings; (2) analyzing the affect of the target number of round $r$; (3) analyzing the affect of ``piecewise reconciliability''. 

\subsection{Parameter Settings}\label{sec:parameter_settings}

In this section, we elaborate how to set the parameters $n$, $t$, and $g$ given the target success probability $p_0$ and the target number of rounds $r$. 
%In other words, the probability that PBS successfully reconciles all distinct elements within $r$ rounds to be larger than $p_0$) in PBS. 
We continue to assume $d$ is precisely known. First, as explained in \autoref{subsec:protocol2}, $\delta$ should be a small number, so we fix $\delta=5$ and therefore $g=d/\delta$ is also fixed. 
Given the target success probability $p_0$ within $r$ rounds
%(i.e., set reconciliation is complete in $r$ rounds with probability $p_0$) 
%depend on the requirement of specific applications)
, the parameter setting problem aims to find the optimal parameter settings of $n,t$ that minimizes the overall communication overhead, under the constraint that the tail bound of the success probability within $r$ rounds (described in \autoref{sec:times2bound}) is at least $p_0$. Since the overall communication overhead is only slightly larger than the communication overhead in the first round (we will show in \autoref{sec:piecewise_decodability}), so we minimize the later instead of the former in the parameter setting problem. Note that the latter (i.e., the communication overhead in the first round) for each group pair (described in \autoref{sec:multi-rounds}) contains only two terms $t\log n+\delta\log n$ that depend on parameter settings. So we only need to minimize $t\log n+\delta\log n$ in the parameter setting problem, which can be formalized as the follows:

% \begin{equation}
% \min\limits_{n,t} t\log n+\delta\log n \quad \mbox{s.t.}\quad 1-2(1-\alpha^g(n,t))>p_0
% \end{equation}

\begin{align}
\mbox{minimize} \quad
&
t\log n+\delta\log n \nonumber
\\
\mbox{subject to} \quad 
&
1-2(1-\alpha^g(n,t))\geq p_0,\quad n,t\in \mathbb{N}^+ \nonumber
% \\
% &
% n,t\in \mathbb{N}^+ \label{eq:row_sum_requirement}
\end{align}

This optimization problem is not as daunting as it might look, since there are only a few practical combinations of $(n,t)$. 
%we can narrow down its solution space into only a few combinations and traverse all these combinations to find the optimal parameter settings as follows: 
First, since $n$ is the ``code length'' of BCH code, we select $n$ to be $2^m-1$ for some integer $m$ that has ``no waste'' on decodability of the BCH codeword and maximizes the coding efficiency. Then the range of $n$ is narrowed down to $\{63,127,255,511,1023,2047\}$, since $n=\Omega(\delta^2)$ as explained in \autoref{sec:hash_partition}. Second, we select $t$ in the range from $1.5\delta$ to $3.5\delta$, since any smaller $t$ will cause a high probability of BCH decoding failure (explained in \autoref{subsec:protocol2}) and therefore a low success probability (below $50\%$), and any higher $t$ incurs significant additional communication overhead on transmitting BCH codeword (explained in \autoref{subsec:protocol2}) while barely increases the success probability.

% This optimization problem seems to be difficult to solve, since the constraint is a very comprehensive function of the parameters (remind that $\alpha=\alpha(n,t)$ is a function of $n$ and $t$ for arbitrary $r$, $d$, and $g$). However, we can narrow down the solution space into only a few combinations and traverse all these combinations to find the optimal parameter settings as follows: First, for BCH coding efficiency, we select $n$ to be $2^m-1$ for some integer $m$ and therefore narrow its range down to $\{63,127,255,511,1023\}$ (recall that $n=\Omega(\delta^2)$). Second, we select $t$ in the range from $1.5\delta$ to $3\delta$, as we suggested in \autoref{subsec:protocol2}. 

Here we use an example to show how we set parameters: Given $d=1000$ distinct elements, $r=3$ rounds, $p_0=99\%$, for each $(n,t)$ combination in $\{63,127,255,511,1023,2047\}\times \{8,9,...,16,17\}$, we compute the tail bound of the success probability under the parameter settings and obtain \autoref{tab:success_prob}.

\begin{table}[h]
\setlength{\tabcolsep}{3.2pt}
\centering
\caption{Tail bounds of the success probability under different parameter settings ($d=1000$, $r=3$)}\label{tab:success_prob}
\begin{tabular}{@{}|c|c|c|c|c|c|c|@{}}
\hline 
\diagbox{$t$}{$n$}    & $63$ & $127$ & $255$ & $511$ & $1023$ & $2047$ \\ \hline 
8   & 0 & 25.5\% & 32.7\% & 34.3\% & 34.9\% & 35.0\% \\ \hline
9   & 52.1\% & 78.0\% & 84.2\% & 85.7\% & 86.1\% & 86.2\% \\ \hline
10  & 75.1\% & 92.7\% & 96.5\% & 97.4\% & 97.6\% & 97.7\% \\ \hline
11  & 85.9\% & 96.9\% & \cellcolor{blue!25}99.1\% & \cellcolor{blue!25}99.5\% & \cellcolor{blue!25}99.6\% & \cellcolor{blue!25}99.6\% \\ \hline
12  & 91.3\% & 98.5\% & \cellcolor{blue!25}99.7\% & \cellcolor{blue!25}99.9\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% \\ \hline
13  & 93.9\% & \cellcolor{blue!60}99.1\% & \cellcolor{blue!25}99.8\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% \\ \hline
14  & 95.1\% & \cellcolor{blue!25}99.4\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% \\ \hline
15  & 95.6\% & \cellcolor{blue!25}99.5\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% \\ \hline
16  & 95.7\% & \cellcolor{blue!25}99.6\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% \\ \hline
17  & 95.8\% & \cellcolor{blue!25}99.6\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% \\ \hline
\end{tabular}
\end{table}

In \autoref{tab:success_prob}, all $(n,t)$ combinations in the highlighted cells satisfy the success probability requirement. Among them, $(127,13)$ has the lowest communication overhead (w.r.t. $t\log n+\delta\log n$). So we set $n=127, t=13$ in this case. For the case of the set difference cardinality $d$ is not precisely known, we use the scaled estimation of $d$ (described in \autoref{subsec:ToW}) for parameter settings, as explained in \autoref{subsec:ToW}. 
%which is larger than the actual $d$ with high probability. The computed optimal parameter $n$ and $t$ based on an overestimation of $d$ is always sufficient to achieve the success probability. 
{\bf Note that calculating the probabilities in this table is very fast, since each entry in the table can be computed in $O(1)$ time given $M^r$. $M^r$ for each $n\in\{63,127,255,511,1023,2047\}$ ($M$ is a function of $n$), in turn, can be precomputed in $O(t^3)$ time.}

\subsection{What if the target number of rounds $r$ changes?}\label{sec:vary_r}
In this section, we analyze the affect of the target number of rounds $r$ on parameter settings, communication overhead, and decoding complexity.
Note that for each possible target number of rounds $r$ (while keeping the same target success probability $p_0=99\%$), we can also compute a success probability table that is similar to \autoref{tab:success_prob} to obtain the corresponding optimal $n$ and $t$. 
%For example, when $r=1$, the optimal parameter setting is $n=524287$ and $t=16$; when $r=2$, the optimal parameter setting is $n=1023$ and $t=16$. 
The results are shown in \autoref{tab:vary_r} for $r=1,2,3,4$ using the same example above ($p_0=99\%, d=1000$). \autoref{tab:vary_r} also compares the {\it communication overhead per group pair} for each $r$, which accounts both the `constant' communication overhead that does not depend on the parameter settings (i.e., $\delta\log |\mathcal{U}|+32=192$ bits) and the `tunable' communication overhead that does depend on the parameter settings (i.e., the objective function $t\log n+\delta\log n$). The {\it communication overhead per distinct element}, which is simply equal to the communication overhead per group pair divided by $\delta$ (since each group pair contains $\delta$ distinct elements on average), is also compared in \autoref{tab:vary_r}. 

It shows that if we increase the target number of rounds $r$ while keeping the same target probability $p_0$ (`loosen' the parameter setting requirement), the communication overhead (per distinct element) that is needed to achieve this requirement decreases. For instance, the communication overhead per distinct element is reduced by $32\%$ from $r=1$ to $r=2$, and that number from $r=2$ to $r=3$ and from $r=3$ to $r=4$ is $21\%$ and $10\%$ respectively. This ``saving'' on the communication overhead decreases as $r$ increases, so we set $r$ to the tune of $3$, which is a `sweet spot' that achieves the most ``saving'' on the communication overhead while not taking too many rounds to reconcile all distinct elements. 

\autoref{tab:vary_r} also shows that the optimal $n$ decreases as $r$ increases. Recall that the computational complexity per finite field operations in BCH decoding is $O(\log^2 n)$ (quadratic to the ``width" of the Galois field), which means the BCH decoding complexity also decreases as $r$ increases. Here $r=3$ is also a `sweet spot' that achieves the most `savings' on BCH decoding complexity (the complexity decreases as $O(19^2)\rightarrow O(10^2)\rightarrow O(7^2)\rightarrow O(6^2)$ when $r$ increases from $1$ to $4$). Note that the above analysis only shows that $r=3$ is a `sweet spot' when the target success probability is $p_0=99\%$. The `sweet spot' of $r$ could be different for various target success probabilities. However, we fix $r$ to be $3$ in our evaluation, since it is the `sweet spot' for the two target success probabilities to be used in our evaluation, which are $p_0=99\%$ and $p_0=99.58\%$ $(239/240)$, using the same analysis above.
%The communication overhead per group pair is $220$ bits, $210$ bits parameter settings when $r=3$ ($n=127, t=13$), this optimal parameter settings ($n=1023, t=16$) are much larger (more expensive) and incur additional communication overhead of $84$ bits per group pair. It shows that to achieve the same target success probability using fewer rounds (smaller $r$), PBS need more resources (e.g., larger $n$, $t$). Note that the optimal parameter settings when $r=1$ are even larger ($n=2047, t=15$) and incur even more additional communication overhead ($94$ bits comparing to the optimal parameter settings when $r=3$), which shows that running PBS for multiple rounds saves a considerate amount of communication overhead comparing to running PBS for only $1$ round when achieving the same target success probability.}

\begin{table}[h]
\centering
\caption{Vary $r$ ($p_0=99\%, d=1000$)}\label{tab:vary_r}
\begin{tabular}{@{}|c|c|c|c|c|@{}}
\hline 
$r$   & $1$ & $2$ & $3$ & $4$ \\ \hline 
Optimal $n$   & $524287$ & $1023$ & $127$ & $63$ \\ \hline
Optimal $t$   & $16$ & $16$ & $13$ & $11$ \\ \hline
\makecell{Objective function \\$t\log n+\delta\log n$ (bits)}  & $399$ & $210$ & $126$ & $96$ \\ \hline
\makecell{Communication overhead \\per group pair (bits)}  & $591$ & $402$ & $318$ & $288$ \\ \hline
\makecell{Communication overhead \\per distinct element (bits)} & $118.2$ & $80.4$ & $63.6$ & $57.6$ \\ \hline
\end{tabular}
\end{table}

% Hidden table for d=10000
% \begin{table}[h]
% \centering
% \caption{Vary the target number of round $r$}\label{tab:vary_r}
% \begin{tabular}{@{}|c|c|c|c|@{}}
% \hline 
% $r$   & $1$ & $2$ & $3$ \\ \hline 
% Optimal $(n,t)$   & $(4096,14)$ & $(4095,17)$ & $(255,14)$ \\ \hline
% Objective function $t\log n+\delta\log n$  & $220$ & $210$ & $126$ \\ \hline
% Communication overhead per group pair (bits)  & $412$ & $402$ & $318$ \\ \hline
% Communication overhead per distinct element (bits) & $82.4$ & $80.4$ & $63.6$ \\ \hline
% \end{tabular}
% \end{table}

% {\bf (change r)} If we reduce the number of rounds $r$ from $3$ to $2$ while keeping the same target success probability $p_0=99\%$, we can also compute a success probability table that is similar to \autoref{tab:success_prob} to obtain the optimal parameter setting, which is $n=1023, t=16$. Compare to the previous optimal parameter settings when $r=3$ ($n=127, t=13$), this optimal parameter settings ($n=1023, t=16$) are much larger (more expensive) and incur additional communication overhead of $84$ bits per group pair. It shows that to achieve the same target success probability using fewer rounds (smaller $r$), PBS need more resources (e.g., larger $n$, $t$). Note that the optimal parameter settings when $r=1$ are even larger ($n=2047, t=15$) and incur even more additional communication overhead ($94$ bits comparing to the optimal parameter settings when $r=3$), which shows that running PBS for multiple rounds saves a considerate amount of communication overhead comparing to running PBS for only $1$ round when achieving the same target success probability.}

% {\bf Readers may think we can further increase $r$ (keeping the same target success probability) to reduce communication overhead. However, it could make PBS taking too many rounds to reconcile all distinct elements.} 
%Also, further increasing $r$ does not save much communication overhead. For example, if we increase $r$ from $3$ to $4$ (rounds), the optimal parameter setting becomes $n=63,t=11$, which only saves communication overhead of $30$ bits per group pair. }

\subsection{Analysis on ``Piecewise Reconciliability''}\label{sec:piecewise_decodability}

{\bf Note that PBS reconciles the distinct elements gradually round by round. The distinct elements that have been reconciled in the first round are no longer needed to be reconciled again and only the remaining distinct elements will be reconciled in the second round. This is the ``piecewise reconciliability'' mentioned in \autoref{sec:intro_oursolution}. Using the transition matrix $M$ (of the Markov chain described in \autoref{sec:single_markov}), we can theoretically analyze this ``piecewise reconciliability'' by computing the expected value of how many distinct elements would be reconciled in each round as follows. 

Fix a group pair, and define $Z_i$ as the number of distinct elements that would be reconciled in the $i$-th round in the group pair for $i=1,2,...$, and $X$ as the number of distinct elements in the group pair. $\mathbb{E}[Z_1|X=x]$, the expectation of $Z_1$ when the group pair contains exactly $x$ distinct elements, can be computed as $\sum_{y=0}^x y\cdot Pr[x\!\xrsquigarrow{1}\! y]$, where $Pr[x\!\xrsquigarrow{1}\! y]$ denotes the probability that starting with state $x$, the Markov chain (described in \autoref{sec:single_markov}) reaches state $y$ in $1$ transition, which is equal to $M(x,y)$. Recall that $X$ follows the Binomial distribution $Binomial(d,1/g)$, we can compute $\mathbb{E}[Z_1]$ given $d$, $g$, and $n$. $\mathbb{E}[Z_2]$, $\mathbb{E}[Z_3]$, ..., can also be computed, since for $k=1,2,...$, we have

\begin{equation}\label{eq:piecewise}
\mathbb{E}[Z_1+Z_2+\cdots+Z_k|X=x]=\sum_{y=0}^x y\cdot Pr[x\!\xrsquigarrow{k}\! y]
\end{equation}

Both sides of \autoref{eq:piecewise} are the expectation of the number of distinct elements that would be reconciled within the $k$-th round, in which the left-hand side is by the definition of $Z_i$ and the right-hand side is derived from the Markov chain. Based on the linearity of the expectation, we can easily compute $\mathbb{E}[Z_2]$, $\mathbb{E}[Z_3]$, ... (e.g., $\mathbb{E}[Z_2] = \mathbb{E}[Z_1+Z_2]-\mathbb{E}[Z_1]$).
%(e.g., $\mathbb{E}[Z_2]$ can be computed based on $\mathbb{E}[Z_1+Z_2|X=x]=\sum_{y=0}^x y\cdot Pr[x\!\xrsquigarrow{2}\! y]$ and $\mathbb{E}[Z_1]$, where $Pr[x\!\xrsquigarrow{2}\! y]=\big{(}M^2\big{)}(x,y)$). 
We omit the details about the computation and only show results of the expected percentage of distinct elements are reconciled in each round (i.e., $\mathbb{E}[Z_1]/\delta$, $\mathbb{E}[Z_2]/\delta$, $\mathbb{E}[Z_3]/\delta$, and $\mathbb{E}[Z_4]/\delta$) under the optimal parameter settings above when $r=3$ and $p_0=0.99$ ($d=1000$, $g=200$, $n=127$, $t=13$) in \autoref{tab:reconcile_ratio}.
} %% added by long to prevent the all-bold issue
% Using the transition matrix $M$, we can compute the expected value of how many distinct elements are reconciled in each round. 
% From the transition matrix $M$, we can theoretically analyze this ``piecewise decodability'' by computing the expected value of how many distinct elements are reconciled in the each round. 
% $\mathbb{E}[Z|X=x]=\sum_{y=0}^x y\cdot Pr[x\!\xrsquigarrow{1}\! y]=\sum_{y=0}^x y\cdot M(x,y)$
% For example, $\sum_{l=0}^x l\cdot Pr[x\!\xrsquigarrow{1}\! l]$ is the average number of the distinct elements that are reconciled in the first round (for an arbitrary group pair with $x$ distinct elements). 
% Although this expected value in any scenario (given $d$, $n$, and $t$) is computable, we only show the `general' results in \autoref{tab:reconcile_ratio}, in which we assume $\delta_1,\delta_2,...,\delta_g$ follow the Poisson distribution with mean of $\delta$ (this is a tiny approximation for relatively large $d$, since the Poisson distribution is a limiting case of the Binomial distribution with the same expectation), and $t$ is sufficiently large. }
\begin{table}[h]
\centering
\caption{The expected percentage of the distinct elements would be reconciled in each round}\label{tab:reconcile_ratio}
\begin{tabular}{@{}|c|c|c|c|@{}}
\hline 
Round $1$ & Round $2$ & Round $3$ & Round $4$ \\ \hline 
0.962 & 0.0380 & $3.61\times 10^{-4}$ & $2.86\times 10^{-6}$ \\ \hline
% $127$  & 0.961 & 0.0382 & $3.7\times 10^{-4}$ & $2.9\times 10^{-6}$ \\ \hline
% $255$  & 0.981 & 0.0193 & $8.4\times 10^{-5}$ & $3.3\times 10^{-7}$ \\ \hline
% $511$ & 0.990 & 0.00972 & $2.0\times 10^{-5}$ & $3.9\times 10^{-8}$ \\ \hline
% $1023$ & 0.995 & 0.00487 & $4.9\times 10^{-6}$ & $4.8\times 10^{-9}$ \\ \hline
% \begin{table}[h]
% \centering
% \caption{Average percentage of distinct elements are reconciled per round}\label{tab:reconcile_ratio}
% \begin{tabular}{@{}|c|c|c|c|c|@{}}
% \hline 
% $n$   & Round $1$ & Round $2$ & Round $3$ & Round $4$ \\ \hline 
% $63$   & 0.924 & 0.0746 & $1.7\times 10^{-3}$ & $2.7\times 10^{-5}$ \\ \hline
% $127$  & 0.961 & 0.0382 & $3.7\times 10^{-4}$ & $2.9\times 10^{-6}$ \\ \hline
% $255$  & 0.981 & 0.0193 & $8.4\times 10^{-5}$ & $3.3\times 10^{-7}$ \\ \hline
% $511$ & 0.990 & 0.00972 & $2.0\times 10^{-5}$ & $3.9\times 10^{-8}$ \\ \hline
% $1023$ & 0.995 & 0.00487 & $4.9\times 10^{-6}$ & $4.8\times 10^{-9}$ \\ \hline
% $63$   & 0.924 & 0.0746 & 0.00167 & 0.0000274 \\ \hline
% $127$   & 0.961 & 0.0382 & 0.000365 & 0.00000289 \\ \hline
% $255$  & 0.981 & 0.0193 & 0.0000839 & 0.000000330 \\ \hline
% $511$ & 0.990 & 0.00972 & 0.0000200 & 0.0000000392 \\ \hline
% $1023$ & 0.995 & 0.00487 & 0.00000489 & 0.00000000478 \\ \hline
% \begin{tabular}{@{}|c|c|c|c|c|c|c|@{}}
% \hline 
% \diagbox{$r$}{$n$}    & $63$ & $127$ & $255$ & $511$ & $1023$ & $2047$ \\ \hline 
% 1   & 92.4\% & 96.1\% & 98.1\% & 99.0\% & 99.5\% & 99.8\% \\ \hline
% 2   & 7.46\% & 3.82\% & 1.93\% & 0.97\% & 0.49\% & 0.24\% \\ \hline
% 3  & $1.7\times 10^{-3}$ & $3.7\times 10^{-4}$ & $8.4\times 10^{-5}$ & $2.0\times 10^{-5}$ & $4.9\times 10^{-6}$ & $1.2\times 10^{-6}$ \\ \hline
% 4  & $2.7\times 10^{-5}$ & $2.9\times 10^{-6}$ & $3.3\times 10^{-7}$ & $3.9\times 10^{-8}$ & $4.8\times 10^{-9}$ & $5.9\times 10^{-10}$ \\ \hline
\end{tabular}
\end{table}

\autoref{tab:reconcile_ratio} shows that $96.2\%$ of the distinct elements are reconciled in the first round. Therefore, the communication overhead (roughly proportional to the number of distinct elements that are reconciled) in the first round is the major part of the overall communication overhead. This property can also hold for other set reconciliation circumstances that have various number of distinct elements $d$ and various requirements (i.e., various $r$, and $p_0$).
%In other words, the overall communication overhead of all rounds is only slightly larger than that in the first round. 
Due to this reason, we use the communication overhead in the first round (described in \autoref{sec:communication_overhead_single_PBS}) to approximate the overall communication overhead of all rounds in parameter settings in \autoref{sec:parameter_settings}. 
%{\bf \autoref{tab:reconcile_ratio} also shows that the number of remaining distinct elements (the ones that have not been reconciled) decreases exponentially round after round. 

==> section/closely_related_work.tex <==
% \section{Closely Related Work}\label{sec:closely-related}
\section{Related Work}\label{sec:closely-related}

% In this section, we describe several highly-related research work: three set-difference reconciliation algorithms (\autoref{subsec:recon-bench}) and two set-difference size estimation algorithms (\autoref{subsec:est-bench}), which we will evaluate our reconciliation algorithm and our ToW estimator against in ~\autoref{subsec:recon-perf} and~\autoref{subsec:est-perf} respectively. 
% In this section, we first provide, in~\autoref{subsec:recon-bench}, a brief survey of related set reconciliation algorithms, 
% including those we have already 
% briefly described earlier ({\it e.g.,} PinSketch~\cite{Dodis_PinSketch_2008}), focusing on those 
% directly related to PBS and the state-of-the-art algorithms which we will compare PBS against 
% in~\autoref{sec:evaluation}. Then, we briefly describe, in~\autoref{subsec:est-bench}, 
% some related research work on set-difference cardinality estimation. 
In this section, we first provide, in~\autoref{subsec:recon-bench}, a brief survey of related set reconciliation algorithms, 
besides those we have already described earlier ({\it e.g.,} PinSketch~\cite{Dodis_PinSketch_2008}), focusing on those 
directly related to PBS and the state-of-the-art algorithms which we will compare PBS against 
in~\autoref{sec:evaluation}. Then, we briefly describe, in~\autoref{subsec:est-bench}, 
some related research work on set-difference cardinality estimation. 
%
% {=== Here, we first describe set reconciliation algorithms because the Strata estimator requires the knowledge of IBT. Whereas, in the evaluation section, we first evaluate the set-difference size estimator as the evaluation of the 
% set reconciliation depends on it.}
%
\subsection{Set Reconciliation Algorithms}\label{subsec:recon-bench}

% Several set reconciliation algorithms have been proposed. In this section, we only describe those
% that are highly related to our scheme. 

As mentioned in~\autoref{sec:intro}, we only consider the unidirectional set reconciliation in which 
Alice learns $A\Delta B$ in this work. 

% We first describe set reconciliation algorithms that are based on 
% Bloom Filters (BFs)~\cite{Bloom_Space/TimeTradeoffs_1970} and 
% its variants ({\it e.g.,} Invertible Bloom Filters (IBFs)~\cite{Goodrich_InvertibleBloomLookup_2011}).
We first describe set reconciliation algorithms that are based on 
Bloom Filters (BFs)~\cite{Bloom_Space/TimeTradeoffs_1970} and 
Invertible Bloom Filters (IBFs)~\cite{Goodrich_InvertibleBloomLookup_2011}.  
\begin{comment}
A BF is a space-efficient approximate representation of a set $S$, which, given any element $x$, 
allows for the membership query ``$x\in S$?''. Yet, false positive answers are possible. 
Given a set $S$ with $n$ elements, a BF represents it as a table with $m$ cells (each with $1$ bit) as follows. 
For each element $x \in S$, the BF uses $k$ independent hash functions to hash $x$ into $k$ different cells and 
set those cells to $1$. For testing the membership of an arbitrary element $y$, the BF  
uses the same $k$ hash functions to hash $y$ to $k$ distinct cells and returns ``YES'' if all those 
cells are set; Otherwise, it returns ``NO''. 
\end{comment}
% A straightforward idea of using BFs for set reconciliation
% A straightforward BF-based set reconciliation scheme  
% is as follows. Alice %represents 
% encodes set $A$ as a BF, and then sends it to Bob. 
% Using this BF, Bob can tell which elements belong to the intersection $A\cap B$, 
% thus inferring those belong to $B\setminus A$.  
% % ({\it i.e.,} the elements that set 
% % $B$ has but set $A$ does not).  
% Similarly, Alice can tell which elements belong to $A\setminus B$. 
% Finally, Bob sends $B\setminus A$ to Alice so that Alice can infer $A\Delta B$=$(A\setminus B)\bigcup(B\setminus A)$.
Set difference can be learned by simply exchanging the BFs for sets $A$ and $B$ between Alice and Bob. 
This scheme, however, has a flaw: 
Alice may not learn the exact set difference
$A\Delta B$ because of the false positive errors of BFs, which is not desirable in many applications. 
\begin{comment}
However, there are two main disadvantages. First, some elements belonging to the set 
difference $A\Delta B$ (=$(A\setminus B)\cup (B\setminus A)$) might be missing because 
of the aforementioned false positiveness of BFs. 
Second, a BF requires $m=-\frac{n \ln p}{(\ln 2)^2}$ cells (bits) to ensure a false positive rate of $p$ 
for a set with $n$ elements. Thus, this scheme has a communication overhead of $O(|A| + |B|)$, which is too high when the 
set sizes $|A|$ and/or $|B|$ are large. 
\end{comment}
% To overcome its disadvantages, 
To resolve this flaw, 
several advanced BF-based set reconciliation algorithms~\cite{Byers_Informedcontentdelivery_2004,Guo_SetReconciliationvia_2013,Eppstein_WhatsDifference?Efficient_2011,Ozisik2019,Fan_CuckooFilterPractically_2014} have been proposed. Here we describe two of them: Difference Digest and Graphene. 
% The ideas for other set reconciliation algorithms that are based on BFs and its variants are similar.

++++ {\bf Concise Version }

D.Digest~\cite{Eppstein_WhatsDifference?Efficient_2011} is an IBF~\cite{Goodrich_InvertibleBloomLookup_2011} 
based set reconciliation algorithm. Like in BFs, 
each element (from a set) is inserted into $k$ cells indexed by $k$ independent hash functions in IBFs. 
Instead of having a single bit as in a BF, each cell in an IBF has three fields, each of which requires a single memory word. 
Therefore, IBFs are much more powerful than BFs: The set difference of two sets (say $A$ and $B$) can be decoded from the 
``difference'' of the their encoded IBFs. However, as shown in~\cite{Eppstein_WhatsDifference?Efficient_2011}, 
the number of cells should be as twice as the estimate of the set difference cardinality to roughly ensure a success rate of 
$0.99$, %(with a probability of 0.99, all distinct elements can be successfully decoded), 
which results in a communication overhead of 6d words, {\it i.e.,} 6 times of the minimum. As we will show in~\autoref{sec:evaluation}, 
PBS is much more space-efficient, whose communication overhead is only 2.15 to 2.67 times of the minimum. 
% when ensuring the same 
% success rate. 

++++ {\bf Old Version }
\noindent
{\bf Difference Digest (D.Digest)}. D.Digest~\cite{Eppstein_WhatsDifference?Efficient_2011} 
is an IBF~\cite{Goodrich_InvertibleBloomLookup_2011} based set reconciliation algorithm. 
Like in BFs, 
% elements are inserted in a table of cells using $k$ independent hash functions in IBFs. 
each element (from a set) is inserted into $k$ cells indexed by $k$ independent hash functions in IBFs. 
% Unlike in BFs, 
Each cell in IBFs has three fields: A {\it count} 
field records the number of elements 
hashed to this cell; an {\it idSum} field records the \code{XOR} sum of all the elements hashed to 
this cell; and a {\it hashSum} field 
% {\bf \lbrack NOT USE checksum simplification\rbrack 
records the \code{XOR} sum of the hash values (by an additional hash function) of all the elements 
hashed to this cell. 
% } 
Given a cell with exact one element hashed to it, it is clear that the {\it idSum} should be equal to  
the element and the {\it hashSum} should be the hash value of the element.  
% if exact one element is hashed into a cell. 
Using such a property, 
% Unlike standard BFs, which can only be used for membership test, 
a set can be decoded from its encoded IBF (with high probability) when the number of 
cells is large enough, the decoding process will be elaborated very soon. 
In~\cite{Eppstein_WhatsDifference?Efficient_2011},  
% Besides, a 
a subtract operator %(which is not available in standard BFs) 
of two IBFs (say \code{IBF}$_A$ and \code{IBF}$_B$ for sets A and B respectively)  
is added 
so that the resulting IBF \code{IBF}$_D\triangleq$\code{IBF}$_A-$
\code{IBF}$_B$ can be viewed as the encoded IBF for set $D\triangleq A\Delta B$. 
To decode $D$ from \code{IBF}$_D$, an iterative decoding algorithm % proposed in~\cite{Eppstein_WhatsDifference?Efficient_2011} to recover elements within the set difference, by 
was used. 
This algorithm is also referred to as a ``peeling process'', which  
is similar to the decoding algorithms for some erasure-correcting codes, such as Tornado codes~\cite{luby1998tornado}. 
%
It iteratively decodes element located in pure cells, 
{\it i.e.,} cells whose \code{count} field is $\pm 1$ and \code{hashSum} equals 
to the hash value of its \code{idSum}, and then removes each of them from the $k$ cells indexed by the $k$ hash functions.  
The decoding succeeds if eventually 
all cells are empty, {\it i.e.,} the IBF corresponds to an empty set; otherwise, it fails. 
% This standard ``peeling process'' 
% is similar to the decoding algorithms for some erasure-correcting codes, such as Tornado codes. 
% The iterative peeling succeeds if eventually 
% all cells are empty; otherwise, it fails. 
%to support the removal of a set from the IBF 
% so that the difference $D\triangleq A\Delta B$ of sets $A$ and $B$ can 
% be recovered from the resulting IBF \code{IBF}$_D\triangleq$\code{IBF}$_A-$
% \code{IBF}$_B$ where \code{IBF}$_X$ is the IBF for set $X$. 
% An iterative peeling decoding algorithm was 
% proposed in~\cite{Eppstein_WhatsDifference?Efficient_2011} to recover elements within the set difference, by 
% attractively finding pure cells, {\it i.e.,} cells whose \code{count} field is $\pm 1$ and \code{hashSum} equals 
% to the hash value of its \code{idSum}, and removing them from the IBF. The iterative peeling succeeds if eventually 
% all cells are empty; otherwise, it fails. 
To ensure a high enough probability of successfully decoding, 
it was suggested in~\cite{Eppstein_WhatsDifference?Efficient_2011} that 
roughly $2|D|$ cells should be used,  
% for accurate estimation and decoding 
% (note that the number of cells can be smaller if $|D|$ is known a prior), 
which results in a communication overhead of 
around $6|D|$ ``words'' (assuming each of the three field takes one ``word''), {\it i.e.,} $6$ times of that of the minimum.  

++++ {\bf Concise Version }

Graphene~\cite{Ozisik2019} is a hybrid algorithm that combines BFs and IBFs, in which IBFs are used to recover the elements 
that are ``missing'' because of the false positive errors of BFs. It was shown in~\cite{Gabrys2019} that Graphene is generally more space-efficient than  
IBF-only schemes ({\it e.g.,} D.Digest). However, when $|A\Delta B|\!\ll\! |A\cap B|$ that is common in many application scenarios, 
Graphene would reduce to an ``IBF-only scheme'', because now Graphene can not afford to create a BF that has low false positive rate (otherwise, the 
BF alone could incur a larger communication overhead than the IBF-only schemes). 
As observed in our experiments in~\autoref{sec:evaluation}, the false positive rate 
is very close to 1 in such scenarios. Therefore, Graphene is also not as space-efficient as PBS. 

++++ {\bf Old Version }
\noindent 
{\bf Graphene}. Graphene~\cite{Ozisik2019} is a hybrid algorithm that combines BF- and 
IBF- based solutions. 
% Like the aforementioned naive BF-based scheme, Graphene uses BFs to %allow one host (say Bob) 
% to find the elements in the set difference $A\Delta B$, yet, missing a few because of the false positiveness of BFs. 
% To compensate the false positive effects of BFs, Graphene uses IBFs to recover these missing elements.  
Here, we only describe the simplest version ({\it i.e.,} Protocol I in~\cite{Ozisik2019}) of Grapheme, 
which only works for the scenario where one set is a subset of the other. 
% Note that the ideas of more powerful versions ({\it e.g.,} Protocol II in~\cite{Ozisik2019}) are similar. 
Without loss of generality, 
% in the following description of Graphene, 
we assume $B\subset A$. 
In Graphene, Bob encodes a BF \code{BF}$_B$ and an IBF \code{IBF}$_B$ for $B$ and sends them to Alice. 
Alice then decodes a set from \code{BF}$_B$, denoting as $\tilde{B}$, which contains elements 
(in $A$) that pass the membership test of \code{BF}$_B$. 
$\tilde{B}$ should be the same as $B$ if there is no false positive error in BFs, and then Bob can obtain 
the set difference $A\Delta B = A\!\setminus\! B \!=\! A\!\setminus\! \tilde{B}$. However, because of the false positiveness,  %of BFs, 
$\tilde{B}$ also contains a few elements from $A\Delta B$. In Graphene, these elements were then decoded from 
the resulting IBF of \code{IBF}$_{\tilde{A}}$-\code{IBF}$_A$, which, together with those in $B\!\setminus\! \tilde{A}$,  
compose the set difference $A\Delta B$. 
% Clearly, $\tilde{Z}$ contains all elements in
% $(A\cap B)$ ($=\!A$) and a few elements in $(B\setminus A)$ ($=\!A\Delta B$) because of the false positiveness of BFs. 
% Unlike in the IBF-only solution ({\it e.g.,} D.Digest), where the 
% IBF should have enough number of cells ({\it e.g.,} $2|B\setminus A|$ cells) to ensure that all elements in 
% the set difference ($B\setminus A$ in this case) can be recovered with high probability, 
% Unlike in D.Digest, 
% the IBF in Graphene is used to recover the elements in $Z\setminus (A\cap B)$, {\it i.e.,} 
% a few elements in $B\setminus A$ that passes the mem.
% The latter, elements in $\tilde{Z}\setminus A$, which is then ``identified'' by decoding the subtracted IBF of the received IBF and that of $\tilde{Z}$, 
% together with those in $B\setminus \tilde{Z}$ ({\it i.e.,} elements do not pass the membership test of the BF) make up $A\Delta B$. 
%
% The number of 
% % such elements 
% elements ({\it i.e.,} elements in $\tilde{Z}\setminus A$) needed to be decoded from the IBF  
% % are 
% is less than $|B\setminus A|$, %the size of the set $B\setminus A$, and 
% and much less when the false positive rate of the BF is low. Hence, the required number of 
% cells for the IBF can be less than that in IBF-only schemes. 
We note that 
more complicated versions ({\it e.g.,} Protocol II in~\cite{Ozisik2019}) of Graphene are required in general scenarios, in 
which at least an additional BF and an additional IBF are required to be transmitted between Alice and Bob. 
% , thus incurring 
% higher communication overhead. 
It was shown in~\cite{Gabrys2019} that Graphene is generally more space-efficient than  
IBF-only schemes. However, when $|A\Delta B|\!\ll\! |A\cap B|$ which is common in many application scenarios, 
Graphene would reduce to an ``IBF-only scheme'', because now Graphene can not afford to create a BF that has low false positive rate (otherwise, the 
BF alone could incur a larger communication overhead than the IBF-only schemes). As observed in our experiments in~\autoref{sec:evaluation}, the false positive rate 
is very close to 1 in such scenarios. 
\begin{comment}
Graphene performs extremely well when $|A\Delta B|\!\approx\! |A\cap B|$ because the BF can 
help significantly reduce the number of cells required by the IBF, yet, 
the BF itself needs only $O(|A|)\!=\!O(|A\Delta B|)$ (with a small constant factor) 
bits to guarantee a low enough false positive rate. 
Unfortunately, in most of the scenarios that are considered in this work, $|A\Delta B|\!\ll\! |A\cap B|$, 
Graphene can not afford to create a BF that has low false positive rate (otherwise, the 
BF alone could incur a larger communication overhead than the IBF-only solutions) 
because now $|A|\!\gg\! |A\Delta B|$. 
In other words, Graphene almost reduces to an IBF-only solution when $|A\Delta B|\!\ll\! |A\cap B|$ 
as the false positive rate of the BF is so high (close to $1$) 
that the BF can not help much in reducing the number of cells in the IBF.
\end{comment}

Then, we describe algorithms~\cite{Minsky2003,Dodis_PinSketch_2008,naumenko2019bandwidth,Karpovsky_eccreconciliation_2003} that 
are based on error-correction codes (ECCs). 
The basic ideas of these algorithms are similar to that of PinSketch~\cite{Dodis_PinSketch_2008}. 
Like PinSketch~\cite{Dodis_PinSketch_2008}, they have communication overhead close to the minimum, yet have 
high decoding computational complexity of up to $O(d^3)$, which is much higher than that of PBS, {\it i.e.,} $O(d)$.  
% here we only describe the PinSketch algorithm~\cite{Dodis_PinSketch_2008}, a representative one among them. 

++++++++
{\bf Old Version }

\noindent 
{\bf PinSketch}. 
% PinSketch~\cite{Dodis_PinSketch_2008} is an error-correction code (ECC) based set reconciliation algorithm.  
As mentioned in~\autoref{sec:intro}, given any set $S$ from a universe $\mathcal{U}$, %with $|\mathcal{U}|=u$, 
PinSketch 
% (and other ECC-based set reconciliation algorithms) represents 
encodes $S$ as a %is viewed 
% as a characteristic vector (binary string) $s$ in $\{0,1\}^n$.  
$|\mathcal{U}|$-bit-long bitmap $S[1..|\mathcal{U}|]$: $S[i]$ (the $i^{th}$ bit of $S[1..|\mathcal{U}|]$) 
is $1$ if $i\in S$; otherwise, $S[i]=0$. 
% For example, $s_x=1$ for $x\in \mathcal{U}$ if 
% $x\in S$; otherwise $s_x=0$. 
% Using such a representation, 
% With such encoding, 
% set reconciliation problems can be converted into 
% error-correcting problems in Hamming space. More precisely, 
With this encoding, reconciling two 
sets $A$ and $B$ whose difference $A\Delta B$ has $d$ elements is equivalent to recovering 
from $B[1..|\mathcal{U}|]$ (viewed as a corrupted version of $A[1..|\mathcal{U}|]$ with $d$ corrupted bit positions) 
to $A[1..|\mathcal{U}|]$. 
% from a corrupted binary string in $\{0,1\}^{|\mathcal{U}|}$ where the number of errors is at most $d$. 
% With a suitable error-correcting code, ECC-based set reconciliation algorithms can achieve the 
% optimal communication overhead $t\log n$ (assuming $t$ is known a prior). 
% Unfortunately, as mentioned in~\autoref{sec:intro}, their 
% decoding computational complexity can be as high as $O(t^3)$. % where $t$ is the set-difference size. 
PinSketch uses BCH codes~\cite{Lin_ErrorControlCoding_1983} with a decoding capacity $t=d$ (assuming $d$ is known a prior) 
to solve this error-correcting problem. 
However, the decoding algorithm of BCH codes has a computational complexity of 
$O(d^2)$ finite field operations with the recent optimized implementation~\cite{Wuille_Minisketchoptimizedlibrary_2019}, 
% $O(d^3)$ finite field operations 
% in general 
% (can be reduced to $O(d^2)$ by exploiting the algebraic structures of certain 
% codes~\cite{Dodis_SyndromeEncodingDecoding_2006,Wuille_Minisketchoptimizedlibrary_2019}). 
% % as it requires to solve 
% % systems of linear equations in the form of $Mx=y$ where $M$ is a $d\times d$ matrix with Gaussian elimination. 
% % has a communication complexity of $t \log n$ and a 
% % (decoding) computational complexity of $O(d^3)$ using the implementation 
% % of the standard BCH decoding algorithm proposed in~\cite{Dodis_SyndromeEncodingDecoding_2006}. 
% Recently, 
% an optimized implementation of the PinSketch algorithm, 
% called Minisketch~\cite{Wuille_Minisketchoptimizedlibrary_2019}, was designed and open-sourced by the authors 
% of~\cite{naumenko2019bandwidth}. %Minisketch 
% This implementation has a computational complexity of $O(d^2)$ (instead of $O(d^3)$), 
which, however, is too high when $d$ is large. For example, we will show in~\autoref{subsec:recon-perf}, 
on a workstation with an Intel Core i7-9800X processor, PinSketch needs around 20\,\si{\second} 
when $d\!=\!$\num{10000}, whereas 
PBS only requires around $10^{-2}$\,\si{\second} (three orders of magnitude lower). 
% In the sequel, we still use ``PinSketch'' (not Minisketch) with the understanding that 
% the optimized implementation is used. 
% To avoid any confusions, only Minisketch (not PinSketch) will be used in the sequel.


+++++++
{\bf New Version (Copied from intro); I do not think it is proper to move the following paragraph here. 
It is more proper to move it to somewhere in the scheme section. 
So that we just remove the description on PinSketch in the related work section. } 

{\bf PinSketch.} 
As mentioned in~\autoref{sec:intro}, like PBS, PinSketch also uses BCH coding, yet in a very different manner. 
% We emphasize that BCH coding is used in PBS in a very different and much more efficient manner than that in PinSketch~\cite{Dodis_PinSketch_2008}.  
In PinSketch, each bit encodes only a single element in the universe $\mathcal{U}$, 
so the size of the bitmap is equal to the size of the universe $\mathcal{U}$.  
For example, when $|\mathcal{U}| \!=\! 2^{32}$ as assumed in most existing works, 
%in the set reconciliation problem we usually assume each element is ``indexed" by a $32$-bit-long (hash) signature, so the universe contains a total of $2^{32}$ elements. In this case, 
the bitmap encoding for any set in PinSketch is $2^{32}$ bits long, and the Galois field involved in its BCH decoding is the ``$32$-bit-wide" $GF(2^{32})$.  
In contrast, as explained earlier, in PBS 
%since each bit encodes the oddness or evenness of the cardinality of a subset,   
the size $n$ of a bitmap is dependent only on $d$, and not on the size of the universe or on the cardinality of the set the bitmap encodes.   For example, as shown in the example in~\autoref{}, $n \!=\! 255$ is large enough for $d \!=\! 5$.  In this case, 
the BCH decoding operates in the much shorter
``8-bit-wide" $GF(2^{8})$.  This shorter ``width" alone in theory translates into roughly $16$ times shorter BCH decoding time, 
% which as will be explained in \autoref{sec:BCH_code} 
which as have be explained in \autoref{sec:BCH_code} 
grows quadratically with the ``width" of the underlying Galois field.  This shorter ``width" also implies four times shorter BCH codeword in PBS than in PinSketch, making it 
much more costly
for PinSketch to adopt the same BCH-decoding time reduction technique that we will describe next for the general case where $d$ can be very large, as will be elaborated 
in \autoref{subsec:protocol2}.  

+++{\bf Suggest to keep}
% \noindent
% {\bf Summary}. 
\autoref{tab:sum-recon} summarizes the above set reconciliation algorithms (including PinSketch that we have described earlier) and 
PBS, where ``GF($2^x$) ops'' (in the second column, {\it i.e.,} the column for ``Decoding time complexity'') 
stands for Galois field operations in a GF($2^x$) finite field. 

Not shown are their encoding computational complexity and communication complexity, each of which is  
the same for the four algorithms with an exception for 
the encoding computational complexity of PinSketch. 
More precisely, the former is $O(|A|\!+\!|B|)$ (the total encoding computational 
complexity at both Alice and Bob) except for that of PinSketch which is 
$O(d(|A|\!+\!|B|))$ and the later is $O(d)$. 


+++++ {\bf The following paragraph can actually be removed.}

Like in most literature, we decompose the computational complexity into the encoding and decoding complexities, 
since encoding  
is usually (and possibly simultaneously) conducted by both Alice and Bob, 
whereas decoding is usually performed by only 
one of them, {\it e.g.,} Alice or Bob. Though for some algorithms ({\it e.g.,} PinSketch), this decomposition is 
straightforward, we explicitly explain it for all the four algorithms. 
For D.Digest, the encoding is 
the constructions of \code{IBF}$_A$ (by Alice) and \code{IBF}$_B$ (by Bob), and decoding is the 
calculation of \code{IBF}$_D$ (=\code{IBF}$_A$-\code{IBF}$_B$) and the procedure ({\it i.e.,} 
the ``peeling process'') of decoding elements from \code{IBF}$_D$. For PinSketch, 
the encoding and decoding are the encoding 
and decoding of BCH codes respectively. 
For PBS, we consider hash-partition and parity bitmap encoding (\autoref{sec:hash_partition}) together with 
BCH and XOR encodings (\autoref{sec:BCH_code})
as encoding, whereas the 
decoding of BCH and XORs (\autoref{sec:BCH_code}) as decoding. 
For Graphene, we consider the constructions of BFs and IBFs are encoding, and 
the procedures of passing elements through the received BFs, {\it i.e.,} membership test, 
and subtraction and decoding of the IBFs as decoding. 
% Unlike the previous three algorithms, the encoding of procedures in Graphene, 
% {\it i.e.}, the constructions of the BFs and IBFs, 
% can only be conducted sequentially. Take Protocol I of Graphene for instance, 
% the receiver (say Bob) can create the IBF only after Bob receives the BF sent by Alice as the construction of the IBF for set 
% $Z$ depends on this BF. 
\begin{comment}
Finally, we emphasize that the number of rounds shown in the last column of~\autoref{tab:sum-recon} 
includes the round for the set-difference size estimation (if necessary). Though our scheme requires 
3 or 4 rounds of message exchanges between Alice and Bob, in other words, 
our set reconciliation scheme requires 2 to 3 rounds (excluding the estimation 
round), this is not a weakness because we will show in~\autoref{subsec:recon-perf} that 
more than 95\% of elements can be recovered after the first round of our reconciliation algorithm and the 
underlying synchronization of data objects ({\it e.g.,} files in cloud storage systems) can be started 
immediately after the first round of our reconciliation algorithm. 
\end{comment}



\noindent
{\bf Others.} 
Recently, a Cuckoo Filter (CF)~\cite{Fan_CuckooFilterPractically_2014} based set reconciliation 
algorithm was proposed in~\cite{Luo_SetReconciliationCuckoo_2019}. Though empirically CFs 
can have lower space overhead than BFs, 
this CF-based set reconciliation algorithm still suffers from the two major weaknesses 
described in~\autoref{sec:closely-related} as BF-based schemes do. 

Besides the standard set reconciliation problem, many researchers considered its variants. 
For example,  Gabrys {\it et al} considered in~\cite{Gabrys2019} the variant of reconciling two {\it similar sets}, in which 
elements in the symmetric difference $A\Delta B$ are similar (more precisely, 
they are related through the Hamming distance metric). Luo {\it et al} considered 
in~\cite{Luo_accurateMultisetReconciliation_2019a} the variant of 
reconciling multisets, in which elements can have multiple replicas. 

\begin{table}
\centering
\caption{Summary of set reconciliation algorithms.}\label{tab:sum-recon}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{@{}|l|c|c|@{}}  
\hline
Algorithms & \shortstack{Decoding time complexity} & \# of rounds \\ 
\hline\hline
D.Digest & O(d) & 1\\ \hline
Graphene & $O(|A|+|B|)$ & 2 or 3 \\ \hline 
PinSketch & $O(d^2)$ GF($2^{32}$) ops & 1 \\ \hline
% PBS & $O(d)$ GF($2^{6}$) to GF($2^{10}$) ops & 2 or 3\\
PBS & $O(d)$ GF($2^{6\text{ to } 10}$) ops & 2 or 3\\
\hline
\end{tabular}
\end{table}
% \begin{table}
% \centering
% \caption{Summary of set reconciliation algorithms.}\label{tab:sum-recon}
% \setlength{\tabcolsep}{3pt}
% \begin{tabular}{@{}|l|c|c|c|@{}}  
% \hline
% Algorithms & \shortstack{Estimator\\ required?} & \shortstack{Decoding comput-\\ational complexity} & \# of rounds \\ 
% \hline\hline
% D.Digest & YES & O(t) & 2\\ \hline
% Graphene & NO  & $O(|A|+|B|)$ & 2 or 3 \\ \hline 
% Minisketch & YES & $O(t^2)$ & 2 \\ \hline
% Our scheme & YES &$O(t)$ & 3 or 4\\
% \hline
% \end{tabular}
% \end{table}

% It was shown in~\cite{Eppstein_WhatsDifference?Efficient_2011} roughly 
% $1.5t$ cells were required to make sure that the iterative peeling algorithm succeed with a high enough probability, 
% which results in a communication cost more than $3$ times of the optimal one. Note that besides the IBF, many 
% other variants of Bloom filters can also be used for set reconciliation, such as counting Bloom filters~\cite{counting}, and 
% Invertible Bloom Lookup Table (IBLT)~\cite{Goodrich_InvertibleBloomLookup_2011}. However, the communication cost 
% is similar or even higher than that of IBFs based set reconciliation. Recently, a set reconciliation scheme,  
% which uses a combination of a Bloom filter and an IBLT, was proposed in~\cite{Ozisik2019}. ...

\subsection{Set-Difference Size Estimators}\label{subsec:est-bench}

% Recall that in real-life applications, the set-difference size $d$ might not be known a prior. In such a scenario, 
% Most set reconciliation algorithms rely on an accurate estimation of $d$ to set their parameters 
% so that they avoid unnecessary bandwidth waste, yet ensure that failure rarely happens. 

Besides the ToW estimator described in~\autoref{subsec:ToW}, the min-wise estimator and the Strata estimator are 
two-well known ones. The min-wise estimator is based on Min-wise hashing~\cite{Broder_MinWiseIndependent_2000} 
that is commonly used to estimate set similarity~\cite{Broder_minwise_1997}, 
more precisely, the Jaccard similarity $J(A,B)\triangleq \frac{|A\cap B|}{|A \cup B |}$. %Whereas, 
The Strata estimator is an IBF-based set difference cardinality estimator using the 
idea of Flajolet and Martin (FM) sketch~\cite{Flajolet_Strata_1985}.  
However, these two estimators are much less space-efficient than the ToW estimator. %as shown in~\autoref{}. 

We note that, the algorithm, which was proposed in~\cite{Feigenbaum_AppL1Difference_2003} and designed for 
more general $L_1$ difference, can also be 
used for the estimation of set difference cardinality. It has similar space-efficiency, in theory, as the ToW estimator. 
However, it is much more complicated. %than the ToW estimator. 

\begin{comment}
As mentioned earlier, set-difference size estimation is a critical sub-problem for set-difference reconciliation. Most 
set reconciliation algorithms rely on an accuracy estimation of the size of the set difference to set their parameters 
so that they avoid unnecessary bandwidth waste. 

\noindent
{\bf Min-wise hashing}. Min-wise hashing~\cite{Broder_MinWiseIndependent_2000} is commonly used to estimate set similarity~\cite{Broder_minwise_1997}, 
more precisely, the Jaccard similarity $J(A,B)\triangleq \frac{|A\cap B|}{|A \cup B |}$. 
Using the relation between the Jaccard similarity $J(A,B)$ and the set-difference size $t$: $t\!=\!\frac{1-J(A,B)}{1 + J(A,B)}(|A| + |B|)$, we can use min-wise hashing to estimate the set-difference size $t$. 
Min-wise hashing uses the property of min-wise independent permutation: Given a min-wise 
independent permutation family $\mathcal{F}$ on the universe $\mathcal{U}$, and a permutation $\pi$ uniformly randomly selected 
from $\mathcal{F}$, then $\mathbf{P}[\min\{\pi(A)\} \!=\! \min\{\pi(B)\}]=J(A,B)$. 
More precisely, min-wise hashing uses $k$ random permutations $\pi_1,\pi_2,\cdots,\pi_k$ from a 
min-wise independent permutation family on the universe $\mathcal{U}$. Define a hash function $h_i(S)=\min\{\pi_i(S)\}$ 
for any $S\subseteq \mathcal{U}$, then 
min-wise hashing uses $\hat{J}\!=\!\frac{|\{i \in \{1,2,\cdots, k\}|h_i(A)=h_i(B)\}|}{k}$ to estimate $J(A,B)$. Given $\hat{J}$, 
we can then estimate the set-difference size with $\hat{t}=g(\hat{J})=\frac{1-\hat{J}}{1 + \hat{J}}(|A| + |B|)$. 
% Given a random variable $X$ with a finite mean $E[X]$ and variance $Var[X]$, the variance of the random variance $f(X)$, where $f(\cdot)$ is a twice differentiable function, can be approximated with the first-order delta method as,
% \[
% Var[f(X)]\approx \big{(}f'(E[X])\big{)}^2Var[X].
% \]
It is easy to check that, using the first-order Taylor expansion method~\cite{Papanicolaou_Taylorapproximationdelta_2009}, 
the variance of min-wise estimator with $k$ hash functions for the set-difference 
size is approximately $\frac{4t|A\cup B|}{k\big{(}1+(|A\cup B|-t)/|A\cup B|\big{)}^2}$. 
When $t\!\ll\! |A\cup B|$, the scenarios that are mainly considered in this work and common in many applications, 
the variance can be further approximated as $\frac{t|A\cup B|}{k}\!\gg\!\frac{2t(t-1)}{k}$, the variance of 
our ToW estimator with $k$ sketches. 
% \[
% \big{(}g'(E[\hat{J}])\big{)}^2Var[\hat{J}]=\big{(}g'(J)\big{)}^2\frac{J(1-J)}{k}=\frac{4J(1-J)(|A|+|B|)^2}{k(1+J)^2}.
% \]
% Besides the standard min-wise sketches described above, many more efficient variants of min-wise sketches~\cite{Li_bBitMinwise_2009} are 
% proposed to estimate the Jaccard similarity or the extended Jaccard similarity. 
Therefore, to guarantee a high enough accuracy, the min-wise estimator (for the set-difference size) 
has to use a prohibitively large (much larger than the number of sketches required by our ToW estimator) $k$ 
when $t\!\ll\! |A\cup B|$, which results in too high communication cost. 

\noindent
{\bf Strata}. Strata Estimator~\cite{Eppstein_WhatsDifference?Efficient_2011} is an IBF 
based set-difference size estimator using the idea of Flajolet and Martin (FM) sketch~\cite{Flajolet_Strata_1985}. 
Given two sets $A$ and $B$ from a universe $\mathcal{U}$, 
Strata Estimator stratifies each set into $\ell\!=\!1+\log |\mathcal{U}|$ partitions (or strata), and 
encodes each partition with an IBF. 
Here we only describe the procedure 
(of Strata Estimator) for set $A$; the procedure for set $B$ is identical. 
Strata Estimator inserts element $x\in A$ into the $i$-th 
IBF (for $A$), denoting as \code{IBF}$_{A_i}$, if $x$ has $i$ trailing zeros so that \code{IBF}$_{A_i}$ contains $t/2^{i+1}$ elements from the set difference 
on average.
In the decoding stage, Strata Estimator maintains a counter $c$ that is 
the number of all elements in the IBFs that are successfully decoded, 
while traversing the IBFs \code{IBF}$_{D_i}\triangleq$\code{IBF}$_{A_i}$-\code{IBF}$_{B_i}$ for $i=0,1,2,\cdots,\ell$ 
from \code{IBF}$_{D_\ell}$ to \code{IBF}$_{D_0}$ until encountering any IBF that cannot be 
decoded successfully. 
If the $i$-th IBF, {\it i.e.,} \code{IBF}$_{D_i}$, fails to decode, Strata Estimator estimates with $2^{i+1}c$, otherwise if 
all IBFs decode successfully, it estimates with $c$. Though it is much more communication-efficient than the min-wise 
estimator when $t\!\ll\! |A\cup B|$, it is still much more expensive than our ToW estimator for achieving the same level of 
accuracy. For example, as will be shown in~\autoref{subsec:est-perf}, 
Strata Estimator using 16 strata ({\it i.e.,} $\ell\!=\!16$) of 80 cells, the settings suggested in~\cite{Eppstein_WhatsDifference?Efficient_2011}, needs around 15 KB of space, whereas our ToW estimator 
only requires around 300 bytes to achieve the same accuracy.

\noindent
{\bf Summary}. \autoref{tab:estimators} summarizes the above two estimators together with our ToW estimator. 
Note that for the space shown in the second column, we assume each element in the universe takes $u$ bytes and 
the largest possible set-difference size $t_{max}$ is known. 

\begin{table}
\setlength{\tabcolsep}{0pt}
\newcolumntype{V}{>{\centering\arraybackslash} m{2.5cm} }
\newcolumntype{Q}{>{\centering\arraybackslash} m{3.2cm} }
\newcolumntype{M}{>{\centering\arraybackslash} m{2.8cm} }
    \centering
    \caption{Summary of set-difference size estimators.}\label{tab:estimators}
\begin{tabular}{@{}|M|V|Q|@{}}
\hline
Estimators &  Space (bytes) & Variance \\
\hline \hline
\shortstack{Min-wise\\ ($k$ hashes)}  & $ku$ & $\frac{4t|A\cup B|}{k\big{(}1+(|A\cup B|-t)/|A\cup B|\big{)}^2}$\\\hline 
\shortstack{Strata \\($m$ cells per strata)} & $3um\lfloor \log_2 t_{max}\rfloor $ & - \\ \hline 
\shortstack{ToW \\($k$ sketches)} &  $k\lceil \log_2 (2t_{max}\!+\!1)\rceil$ & $\frac{2t^2-2t}{k}$\\\hline
\end{tabular}
\end{table}
\end{comment}


==> section/closely_related_work_OLD.tex <==
\section{Closely Related Work}\label{sec:closely-related}

In this section, we describe several highly-related research work: three set-difference reconciliation algorithms (\autoref{subsec:recon-bench}) and two set-difference size estimation algorithms (\autoref{subsec:est-bench}), which we will evaluate our reconciliation algorithm and our ToW estimator against in ~\autoref{subsec:recon-perf} and~\autoref{subsec:est-perf} respectively. 

%
{=== Here, we first describe set reconciliation algorithms because the Strata estimator requires the knowledge of IBT. Whereas, in the evaluation section, we first evaluate the set-difference size estimator as the evaluation of the 
set reconciliation depends on it.}
%
\subsection{Set Reconciliation Algorithms}\label{subsec:recon-bench}

% Several set reconciliation algorithms have been proposed. In this section, we only describe those
% that are highly related to our scheme. 


First, we describe set reconciliation algorithms that are based on 
Bloom filters (BFs)~\cite{Bloom_Space/TimeTradeoffs_1970} and its 
variants ({\it e.g.,} Invertible Bloom Filters (IBFs)~\cite{Goodrich_InvertibleBloomLookup_2011}). 
A BF is a space-efficient approximate representation of a set $S$, which, given any element $x$, 
allows for the membership query ``$x\in S$?''. Yet, false positive answers are possible. 
Given a set $S$ with $n$ elements, a BF represents it as a table with $m$ cells (each with $1$ bit) as follows. 
For each element $x \in S$, the BF uses $k$ independent hash functions to hash $x$ into $k$ different cells and 
set those cells to $1$. For testing the membership of an arbitrary element $y$, the BF  
uses the same $k$ hash functions to hash $y$ to $k$ distinct cells and returns ``YES'' if all those 
cells are set; Otherwise, it returns ``NO''. 
A straightforward idea of using BFs for set reconciliation 
is that Alice represents set $A$ as a BF, and then sends it to Bob. 
Using this BF, Bob can tell which elements belong to the intersection $A\cap B$, 
thus inferring those belong to $B\setminus A$ ({\it i.e.,} the elements that set B has but set A does not).  
Similarly, Alice can tell which elements belong to $A\setminus B$. 
However, there are two main disadvantages. First, some elements belonging to the set 
difference $A\Delta B$ (=$(A\setminus B)\cup (B\setminus A)$) might be missing because 
of the aforementioned false positiveness of BFs. 
Second, a BF requires $m=-\frac{n \ln p}{(\ln 2)^2}$ cells (bits) to ensure a false positive rate of $p$ 
for a set with $n$ elements. Thus, this scheme has a communication overhead of $O(|A| + |B|)$, which is too high when the 
set sizes $|A|$ and/or $|B|$ are large. To overcome its disadvantages, several advanced BF-based set reconciliation algorithms~\cite{Byers_Informedcontentdelivery_2004,Guo_SetReconciliationvia_2013,Eppstein_WhatsDifference?Efficient_2011,Ozisik2019,Fan_CuckooFilterPractically_2014} have been proposed. Here we describe two of them: Difference Digest and Graphene. The ideas for other set reconciliation algorithms that are based on BFs and its variants are similar.

\noindent
{\bf Difference Digest (D.Digest)}. D.Digest~\cite{Eppstein_WhatsDifference?Efficient_2011} 
is an IBF~\cite{Goodrich_InvertibleBloomLookup_2011} based set reconciliation algorithm. Like in BFs, elements are inserted in a table of cells using $k$ independent hash functions in IBFs. 
Unlike in BFs, each cell in IBFs has three fields (instead of a single bit): A {\it count} 
field records the number of elements 
hashed in this cell; A {\it idSum} field records the \code{XOR} sum of all the elements hashed into 
this cell; And a {\it hashSum} field records the \code{XOR} sum of the hash value of all the elements 
hashed into this cell. Besides, a subtract operator (which is not available in the standard BFs) 
is added 
%to support the removal of a set from the IBF 
so that the difference $D\triangleq A\Delta B$ of sets $A$ and $B$ can 
be recovered from the resulting IBF \code{IBF}$_D\triangleq$\code{IBF}$_A-$
\code{IBF}$_B$ where \code{IBF}$_X$ is the IBF for set $X$. 
% An iterative peeling decoding algorithm was 
% proposed in~\cite{Eppstein_WhatsDifference?Efficient_2011} to recover elements within the set difference, by 
% attractively finding pure cells, {\it i.e.,} cells whose \code{count} field is $\pm 1$ and \code{hashSum} equals 
% to the hash value of its \code{idSum}, and removing them from the IBF. The iterative peeling succeeds if eventually 
% all cells are empty; otherwise, it fails. 
To ensure a high enough success rate ($\ge 0.99$), {\it i.e.,} all elements in $A\Delta B$ 
being successfully recovered from \code{IBF}$_D$, the number of cells should be large enough. 
It was suggested in~\cite{Eppstein_WhatsDifference?Efficient_2011} that 
empirically $2|D|$ cells should be used (to ensure a success rate of 0.99), 
which results in a communication overhead of 
around $24|D|$ bytes (assuming each of the three field takes $4$ bytes, 
or in other words, a cell takes $12$ bytes). 

\noindent 
{\bf Graphene}. Graphene~\cite{Ozisik2019} is a hybrid algorithm for set reconciliation that combines BFs and 
IBFs. Like the aforementioned naive BF-based scheme, Graphene uses BFs to %allow one host (say Bob) 
to find the elements in the set difference $A\Delta B$, yet, missing a few because of the false positiveness of BFs. 
To compensate the false positive effects of BFs, Graphene uses IBFs to recover these missing elements.  
Here, we only describe the simplest version ({\it i.e.,} Protocol I in~\cite{Ozisik2019}) of Grapheme, 
which only works for the scenarios where one set is a subset of the other. Note that the ideas of more powerful versions ({\it e.g.,} Protocol II in~\cite{Ozisik2019}) are similar. 
Without loss of generality, in the following description of Graphene, we assume $A\subset B$. 
In Graphene, Alice creates a BF and an IBF for $A$ and sends them to Bob. 
Using the received BF, Bob can obtain a set, denoting as $Z$, which contains all the elements in 
the set intersection $A\cap B$ and a few elements in $B\setminus A$ because of the false positiveness of BFs. 
Unlike in the IBF-only solution ({\it e.g.,} D.Digest), where the 
IBF should have enough number of cells ({\it e.g.,} $2|B\setminus A|$ cells) to ensure that all elements in 
the set difference ($B\setminus A$ in this case) can be recovered with high probability, 
the IBF in Graphene only requires to recover the elements in $B\setminus A$ which are falsely 
included in $Z$. 
The number of such elements are less than $B\setminus A$, %the size of the set $B\setminus A$, and 
and much less when the false positive rate of the BF is low. 
Graphene performs extremely well when $|A\Delta B|\!\approx\! |A\cap B|$ because the BF can 
help significantly reduce the number of cells required by the IBF, yet, 
the BF itself needs only $O(|A|)\!=\!O(|A\Delta B|)$ (with a small constant factor) 
bits to guarantee a low enough false positive rate. 
Unfortunately, in most of the scenarios that are considered in this work, $|A\Delta B|\!\ll\! |A\cap B|$, 
Graphene can not afford to create a BF that has low false positive rate (otherwise, the 
BF alone could incur a larger communication overhead than the IBF-only solutions) 
because now $|A|\!\gg\! |A\Delta B|$. 
In other words, Graphene almost reduces to an IBF-only solution when $|A\Delta B|\!\ll\! |A\cap B|$ 
as the false positive rate of the BF is so high (close to $1$) 
that the BF can not help much in reducing the number of cells in the IBF.


Then, we describe algorithms~\cite{Minsky2003,Dodis_PinSketch_2008,naumenko2019bandwidth,Karpovsky_eccreconciliation_2003} that are based on error-correction codes (ECCs). The basic ideas of these algorithms are similar, 
here we only describe the PinSketch algorithm~\cite{Dodis_PinSketch_2008}, a representative one among them. 


\noindent 
{\bf PinSketch}. 
% PinSketch~\cite{Dodis_PinSketch_2008} is an error-correction code (ECC) based set reconciliation algorithm.  
Given any set $S$ from a universe $\mathcal{U}$ with $|\mathcal{U}|=n$, 
PinSketch (and other ECC-based set reconciliation algorithms) represents $S$ %is viewed 
as a characteristic vector (binary string) $s$ in $\{0,1\}^n$.  
For example, $s_x=1$ for $x\in \mathcal{U}$ if 
$x\in S$; otherwise $s_x=0$. Using such a representation, set reconciliation problems can be converted into 
error-correcting problems in Hamming space. More precisely, under this representation, reconciling two 
sets $A$ and $B$ whose difference $A\Delta B$ has at most $t$ elements is equivalent to recovering 
from a corrupted binary string in $\{0,1\}^n$ where the number of errors is at most $t$. 
With a suitable error-correcting code, ECC-based set reconciliation algorithms can achieve the 
optimal communication overhead $t\log n$ (assuming $t$ is known a prior). 
Unfortunately, as mentioned in~\autoref{sec:intro}, their 
decoding computational complexity can be as high as $O(t^3)$. % where $t$ is the set-difference size. 
PinSketch uses the BCH codes~\cite{Lin_ErrorControlCoding_1983}, and has a communication complexity of $t \log n$ and a 
(decoding) computational complexity of $O(t^3)$ using the implementation 
of the standard BCH decoding algorithm proposed in~\cite{Dodis_SyndromeEncodingDecoding_2006}. Recently, 
an optimized implementation of the PinSketch algorithm, 
called Minisketch~\cite{Wuille_Minisketchoptimizedlibrary_2019}, was designed and open-sourced by the authors 
of~\cite{naumenko2019bandwidth}. Minisketch reduces this computational complexity from $O(t^3)$ to $O(t^2)$, 
which, however, is still too high when $t$ is large. For example, we will show in~\autoref{subsec:recon-perf}, 
on a workstation with an Intel Core i7-9800X processor, Minisketch needs around 20\,\si{\second} 
when $t\!=\!$\num{10000}, whereas 
our scheme only requires around 10\,\si{\milli\second}. To avoid any confusions, only Minisketch (not PinSketch) will be used in the sequel.


\noindent
{\bf Summary}. \autoref{tab:sum-recon} summarizes the above set reconciliation algorithms and 
our scheme. 

Not shown are their encoding computational complexity and communication complexity, each of which is  
the same for the four algorithms with an exception for 
the encoding computational complexity of Minisketch. 
More precisely, the former is $O(|A|\!+\!|B|)$ (the total encoding computational 
complexity for both Alice and Bob) except for that of Minisketch which is 
$O(t(|A|\!+\!|B|))$ and the later is $O(t)$. 
We decompose the computational complexity into the encoding and decoding complexities, 
since the encoding procedures 
are usually (and possibly simultaneously) conducted by both Alice and Bob, 
whereas the decoding procedures are usually performed by only 
one of them, {\it e.g.,} Alice or Bob. Though for some algorithms ({\it e.g.,} Minisketch), this decomposition is 
straightforward, we explicitly explain it for all the four algorithms. For D.Digest, the encoding procedure is 
the constructions of \code{IBF}$_A$ (by Alice) and \code{IBF}$_B$ (by Bob), and the decoding procedure is the 
calculation of \code{IBF}$_D$ (=\code{IBF}$_A$-\code{IBF}$_B$) and the procedure of recovering elements from 
(or the decoding of) \code{IBF}$_D$. For Minisketch, the encoding and decoding procedures are the encoding and decoding of BCH codes respectively. 
For our scheme, we consider the partition procedure and the BCH and XOR encoding 
for each subset as the encoding procedure, whereas the 
decoding of the BCH codes and the XORs for each subset as the decoding procedure. For Graphene, we consider the constructions of the BFs and the IBFs are the encoding procedure, and 
the procedures of passing elements through the received BFs and the subtraction and decoding of the IBFs as 
the decoding procedure. 
% Unlike the previous three algorithms, the encoding of procedures in Graphene, 
% {\it i.e.}, the constructions of the BFs and IBFs, 
% can only be conducted sequentially. Take Protocol I of Graphene for instance, 
% the receiver (say Bob) can create the IBF only after Bob receives the BF sent by Alice as the construction of the IBF for set 
% $Z$ depends on this BF. 

Finally, we emphasize that the number of rounds shown in the last column of~\autoref{tab:sum-recon} 
includes the round for the set-difference size estimation (if necessary). Though our scheme requires 
3 or 4 rounds of message exchanges between Alice and Bob, in other words, 
our set reconciliation scheme requires 2 to 3 rounds (excluding the estimation 
round), this is not a weakness because we will show in~\autoref{subsec:recon-perf} that 
more than 95\% of elements can be recovered after the first round of our reconciliation algorithm and the 
underlying synchronization of data objects ({\it e.g.,} files in cloud storage systems) can be started 
immediately after the first round of our reconciliation algorithm. 

We note that the number of rounds for our schemes can be reduced by one in practice by 
a simple trick: After receiving ToW sketches from Alice, 
instead of just sending the estimate back to Alice, 
Bob starts the set reconciliation process by sending to Alice
the BCH codes for all the subsets together with the estimate. Clearly, such a trick 
also applies to D.Digest and Minisketch. However, in the sequel, for ease of presentation, 
we still assume that our scheme (and D.Digest and Minisketch) uses 
a separate round for set-difference size estimation. 


\begin{table}
\centering
\caption{Summary of set reconciliation algorithms.}\label{tab:sum-recon}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{@{}|l|c|c|c|@{}}  
\hline
Algorithms & \shortstack{Estimator\\ required?} & \shortstack{Decoding comput-\\ational complexity} & \# of rounds \\ 
\hline\hline
D.Digest & YES & O(t) & 2\\ \hline
Graphene & NO  & $O(|A|+|B|)$ & 2 or 3 \\ \hline 
Minisketch & YES & $O(t^2)$ & 2 \\ \hline
Our scheme & YES &$O(t)$ & 3 or 4\\
\hline
\end{tabular}
\end{table}

% It was shown in~\cite{Eppstein_WhatsDifference?Efficient_2011} roughly 
% $1.5t$ cells were required to make sure that the iterative peeling algorithm succeed with a high enough probability, 
% which results in a communication cost more than $3$ times of the optimal one. Note that besides the IBF, many 
% other variants of Bloom filters can also be used for set reconciliation, such as counting Bloom filters~\cite{counting}, and 
% Invertible Bloom Lookup Table (IBLT)~\cite{Goodrich_InvertibleBloomLookup_2011}. However, the communication cost 
% is similar or even higher than that of IBFs based set reconciliation. Recently, a set reconciliation scheme,  
% which uses a combination of a Bloom filter and an IBLT, was proposed in~\cite{Ozisik2019}. ...

\subsection{Set-Difference Size Estimators}\label{subsec:est-bench}

As mentioned earlier, set-difference size estimation is a critical sub-problem for set-difference reconciliation. Most 
set reconciliation algorithms rely on an accuracy estimation of the size of the set difference to set their parameters 
so that they avoid unnecessary bandwidth waste. 

\noindent
{\bf Min-wise hashing}. Min-wise hashing~\cite{Broder_MinWiseIndependent_2000} is commonly used to estimate set similarity~\cite{Broder_minwise_1997}, 
more precisely, the Jaccard similarity $J(A,B)\triangleq \frac{|A\cap B|}{|A \cup B |}$. 
Using the relation between the Jaccard similarity $J(A,B)$ and the set-difference size $t$: $t\!=\!\frac{1-J(A,B)}{1 + J(A,B)}(|A| + |B|)$, we can use min-wise hashing to estimate the set-difference size $t$. 
Min-wise hashing uses the property of min-wise independent permutation: Given a min-wise 
independent permutation family $\mathcal{F}$ on the universe $\mathcal{U}$, and a permutation $\pi$ uniformly randomly selected 
from $\mathcal{F}$, then $\mathbf{P}[\min\{\pi(A)\} \!=\! \min\{\pi(B)\}]=J(A,B)$. 
More precisely, min-wise hashing uses $k$ random permutations $\pi_1,\pi_2,\cdots,\pi_k$ from a 
min-wise independent permutation family on the universe $\mathcal{U}$. Define a hash function $h_i(S)=\min\{\pi_i(S)\}$ 
for any $S\subseteq \mathcal{U}$, then 
min-wise hashing uses $\hat{J}\!=\!\frac{|\{i \in \{1,2,\cdots, k\}|h_i(A)=h_i(B)\}|}{k}$ to estimate $J(A,B)$. Given $\hat{J}$, 
we can then estimate the set-difference size with $\hat{t}=g(\hat{J})=\frac{1-\hat{J}}{1 + \hat{J}}(|A| + |B|)$. 
% Given a random variable $X$ with a finite mean $E[X]$ and variance $Var[X]$, the variance of the random variance $f(X)$, where $f(\cdot)$ is a twice differentiable function, can be approximated with the first-order delta method as,
% \[
% Var[f(X)]\approx \big{(}f'(E[X])\big{)}^2Var[X].
% \]
It is easy to check that, using the first-order Taylor expansion method~\cite{Papanicolaou_Taylorapproximationdelta_2009}, 
the variance of min-wise estimator with $k$ hash functions for the set-difference 
size is approximately $\frac{4t|A\cup B|}{k\big{(}1+(|A\cup B|-t)/|A\cup B|\big{)}^2}$. 
When $t\!\ll\! |A\cup B|$, the scenarios that are mainly considered in this work and common in many applications, 
the variance can be further approximated as $\frac{t|A\cup B|}{k}\!\gg\!\frac{2t(t-1)}{k}$, the variance of 
our ToW estimator with $k$ sketches. 
% \[
% \big{(}g'(E[\hat{J}])\big{)}^2Var[\hat{J}]=\big{(}g'(J)\big{)}^2\frac{J(1-J)}{k}=\frac{4J(1-J)(|A|+|B|)^2}{k(1+J)^2}.
% \]
% Besides the standard min-wise sketches described above, many more efficient variants of min-wise sketches~\cite{Li_bBitMinwise_2009} are 
% proposed to estimate the Jaccard similarity or the extended Jaccard similarity. 
Therefore, to guarantee a high enough accuracy, the min-wise estimator (for the set-difference size) 
has to use a prohibitively large (much larger than the number of sketches required by our ToW estimator) $k$ 
when $t\!\ll\! |A\cup B|$, which results in too high communication cost. 

\noindent
{\bf Strata}. Strata Estimator~\cite{Eppstein_WhatsDifference?Efficient_2011} is an IBF 
based set-difference size estimator using the idea of Flajolet and Martin (FM) sketch~\cite{Flajolet_Strata_1985}. 
Given two sets $A$ and $B$ from a universe $\mathcal{U}$, 
Strata Estimator stratifies each set into $\ell\!=\!1+\log |\mathcal{U}|$ partitions (or strata), and 
encodes each partition with an IBF. 
Here we only describe the procedure 
(of Strata Estimator) for set $A$; the procedure for set $B$ is identical. 
Strata Estimator inserts element $x\in A$ into the $i$-th 
IBF (for $A$), denoting as \code{IBF}$_{A_i}$, if $x$ has $i$ trailing zeros so that \code{IBF}$_{A_i}$ contains $t/2^{i+1}$ elements from the set difference 
on average.
In the decoding stage, Strata Estimator maintains a counter $c$ that is 
the number of all elements in the IBFs that are successfully decoded, 
while traversing the IBFs \code{IBF}$_{D_i}\triangleq$\code{IBF}$_{A_i}$-\code{IBF}$_{B_i}$ for $i=0,1,2,\cdots,\ell$ 
from \code{IBF}$_{D_\ell}$ to \code{IBF}$_{D_0}$ until encountering any IBF that cannot be 
decoded successfully. 
If the $i$-th IBF, {\it i.e.,} \code{IBF}$_{D_i}$, fails to decode, Strata Estimator estimates with $2^{i+1}c$, otherwise if 
all IBFs decode successfully, it estimates with $c$. Though it is much more communication-efficient than the min-wise 
estimator when $t\!\ll\! |A\cup B|$, it is still much more expensive than our ToW estimator for achieving the same level of 
accuracy. For example, as will be shown in~\autoref{subsec:est-perf}, 
Strata Estimator using 16 strata ({\it i.e.,} $\ell\!=\!16$) of 80 cells, the settings suggested in~\cite{Eppstein_WhatsDifference?Efficient_2011}, needs around 15 KB of space, whereas our ToW estimator 
only requires around 300 bytes to achieve the same accuracy.

\noindent
{\bf Summary}. \autoref{tab:estimators} summarizes the above two estimators together with our ToW estimator. 
Note that for the space shown in the second column, we assume each element in the universe takes $u$ bytes and 
the largest possible set-difference size $t_{max}$ is known. 

\begin{table}
\setlength{\tabcolsep}{0pt}
\newcolumntype{V}{>{\centering\arraybackslash} m{2.5cm} }
\newcolumntype{Q}{>{\centering\arraybackslash} m{3.2cm} }
\newcolumntype{M}{>{\centering\arraybackslash} m{2.8cm} }
    \centering
    \caption{Summary of set-difference size estimators.}\label{tab:estimators}
\begin{tabular}{@{}|M|V|Q|@{}}
\hline
Estimators &  Space (bytes) & Variance \\
\hline \hline
\shortstack{Min-wise\\ ($k$ hashes)}  & $ku$ & $\frac{4t|A\cup B|}{k\big{(}1+(|A\cup B|-t)/|A\cup B|\big{)}^2}$\\\hline 
\shortstack{Strata \\($m$ cells per strata)} & $3um\lfloor \log_2 t_{max}\rfloor $ & - \\ \hline 
\shortstack{ToW \\($k$ sketches)} &  $k\lceil \log_2 (2t_{max}\!+\!1)\rceil$ & $\frac{2t^2-2t}{k}$\\\hline
\end{tabular}
\end{table}



==> section/conflicts/schemes_new__Liu_Liang_s_conflicted_copy_2020-02-12_.tex <==
\section{PBS for small $d$}\label{sec:scheme}

%\section{Set Reconciliation}\label{sec:scheme}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%     Writing Guideline for This Section     %%%%%%%%%%
% “balls – elements in the symmetric difference of the two sets” 

% Protocol 0 (reconcile two sets whose set difference has at most one ball)

% Protocol I.I (partition elements into a sufficiently large number of subsets such that each subset has at most one ball with high probability and use Protocol 0 to reconcile each of them) 

% Protocol I.II (a two-step refinement of Protocol I.I: first use BCH to identify good bins, i.e., bins/subsets have exactly one ball, and then use Protocol 0 to reconcile each good bin) 

% Protocol II (a two-layer refinement of Protocol I.II: in the first layer, we partition elements into t/c subsets, where t is the size of set difference and c is a small constant, then each subset has c balls on average. In the second layer, we further partition each subset into large enough number of bins/subsets such that with high probability each bin has at most one ball, then use Protocol I.II to reconcile them one by one) 

% Protocol III/IV (mainly fix certain exceptions in Protocol II，e.g., how to address bad bins, how to handle the cases where BCH fails to decode and etc)

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% In this section, we describe our set reconciliation scheme in details. First, we give a formal problem statement in \autoref{sec:model}. In \autoref{subsec:protocol0}, we introduce a basic scheme for the trivial case, in which the two sets $A$ and $B$ has at most one distinct element. Building upon the basic scheme, we propose the preliminary version of scheme in \autoref{sucsec:our-scheme} that targets to the cases where the total number of distinct elements $d$ is small. Then we extend the preliminary version and propose the final version of our scheme in \autoref{subsec:protocol2} for general cases (i.e., any arbitrary $d$). We assume $d$ is precisely known throughout this section except in \autoref{subsec:ToW}, where we will describe how to estimate $d$ using a Tug-of-War Estimator. 

\subsection{Problem Statement}\label{sec:model}

In this work, we adopt the commonly used model for the set reconciliation problem. 
Two remote sets $A$ and $B$ are stored at hosts Alice and Bob respectively. Each element in $A$ and $B$ is a hash signiture with signiture width $w$ in the key space (universe) $\mathcal{U}$, which is the set of all $w$-bit binary strings (i.e., $|\mathcal{U}|=2^w$). 
%We use $\mathcal{U}$ to denote the set of all $w$-bit binary strings and name it the universe of signitures. 
The set reconciliation problem is to compute the symmetric set difference between $A$ and $B$, 
{\it i.e.,} $A\Delta B\triangleq (A\!\setminus\! B) \bigcup (B\!\setminus\! A)$. 
Let $d\!=\!|A\Delta B|$ be the cardinality of this difference.
%We denote $d\!=\!|A\Delta B|$. 
Throughout this paper, we call each element in $A\Delta B$ a \textit{distinct element}, and each element in $A\bigcap B$ a \textit{common element}.
{\bf Like in all existing solutions, we describe only {\it unidirectional} set reconciliation, in which Alice or Bob learns the set difference $A\Delta B$. Since the performance of our scheme does not depend on who learns the set difference, we assume Bob learns the set difference $A\Delta B$ in the rest of the paper, as mentioned in \autoref{sec:psea}.}
% As mentioned in \autoref{sec:psea}, we describe {\it unidirectional} set reconciliation that Bob learns the set difference $A\Delta B$. 
%In \autoref{sec:evaluation}, we use the same semantic to measure the communication cost of our scheme and other compared set reconciliation schemes. 

In the rest of this section, we build up our scheme gradually as follows: We start with the trivial case where $d\leq 1$ in \autoref{subsec:protocol0}. Then we generalize our scheme to the case where $d$ is a small number in \autoref{sucsec:our-scheme}. 
%After that, we further generalize our scheme to the case that $d$ is a large number in \autoref{subsec:protocol2}. 
Throughout this section, we assume $d$ is precisely known.
%except in \autoref{subsec:ToW}, where we will describe how to estimate $d$ using a Tug-of-War Estimator. 

%The rest of this section is organized as follows: In \autoref{subsec:protocol0}, we introduce a basic scheme for the trivial case, in which the two sets $A$ and $B$ has at most one distinct element. In \autoref{sucsec:our-scheme} and \autoref{subsec:protocol2}, we elaborate the two versions of our solution that are introduced in \autoref{sec:smalld} and \autoref{sec:larged} respectively. Throughout this section, we assume $d$ is precisely known except in \autoref{subsec:ToW}, where we will describe how to estimate $d$ using a Tug-of-War Estimator. 

\subsection{The Trivial Case of $d\leq 1$}\label{subsec:protocol0}

%We start with the trivial case, in which $A$ and $B$ have at most one distinct element ({\it i.e.,} $d\leq 1$), we have a simple set reconciliation scheme showed in \autoref{alg:trivial_case}:

\autoref{alg:trivial_case} shows the reconciliation scheme for the trivial case, in which $A$ and $B$ differ by at most one distinct element:

\begin{algorithm}
\caption{Set reconciliation when $d\le 1$}
\label{alg:trivial_case}

{\it Alice}: $s_A\leftarrow\underset{a\in A}{\oplus} a$; Send $s_A$ to Bob\; \label{alg1:sender}

{\it Bob}: $s_B\leftarrow\underset{b\in B}{\oplus} b$; $s\leftarrow s_A \oplus s_B$\; \label{alg1:receiver}
\end{algorithm}

First, Alice calculates $s_A$, the bitwise \code{XOR} of all elements in $A$, and send it to Bob. 
Second, Bob also calculates $s_B$, the bitwise \code{XOR} of all elements of $B$. Upon receiving $s_A$, Bob computes $s\!\triangleq\! s_A \!\oplus\! s_B$, and we have

\begin{itemize}
	\item If $A$ and $B$ are identical sets (i.e., $d=0$), we have $s_A=s_B$ and $s=\mathbf{0}$;
	\item If $A$ and $B$ has one distinct element (i.e., $d=1$), the computed $s$, the bitwise \code{XOR} of $s_A$ and $s_B$, will cancel out all common elements and remain the distinct element. In other words, we have $A\Delta B=\{s\}$. 
	%And $s$ is the missing element of $A$ (i.e., $s\in B\!\setminus\! A$) if $s\in B$, or the missing element of $B$ (i.e., $s\in A\!\setminus\! B$) otherwise;
	% \item If $A$ and $B$ has more than one distinct elements (i.e., $d>1$), the bitwise \code{XOR} of $s_A$ and $s_B$ will still cancel out all common elements and remain the \code{XOR} of the distinct elements, i.e., $s$ is the \code{XOR} of all distinct elements;
\end{itemize}

Like most works on set reconciliation, we assume $\mathbf{0}$ is excluded from $\mathcal{U}$, as \autoref{alg:trivial_case} does not work when $\mathbf{0}\in A\bigcap B$ for the following reason: When $s=\mathbf{0}$, \autoref{alg:trivial_case} cannot tell whether $A$ and $B$ are identical, or they have a distinct element of value $\mathbf{0}$. 
%However, we can extend our scheme to support $\mathbf{0}$. For example, we let Alice send to Bob a single bit to indicate whether Alice has element $\mathbf{0}$, so Bob will know whether $\mathbf{0}\in A\Delta B$ or not. 
\autoref{alg:trivial_case} also does not work when there are more than one distinct elements in $A\Delta B$ (i.e., $d>1$), since the computed $s$ is the \code{XOR} of all these distinct elements.

% Note that \autoref{alg:trivial_case} works if and only if $|A\Delta B|\!\leq\! 1$ and $0\!\notin\! (A\!\cup\! B)$ (which we have explained in~\autoref{sec:model}). 

%\subsection{PBS: When $d$ is small}\label{sucsec:our-scheme}

%In this section, we generalize PBS to the case when $d$ is a small number, as we described in \autoref{sec:smalld}. 
%First, we describe each step of single-round PBS from \autoref{sec:hash_partition} to \autoref{sec:reconcile_by_trivial} and summarize it in \autoref{sec:single_round_pbs}. Second, we discuss the exceptions in single-round PBS in \autoref{subsec:exception_hash_partition}. Third, we propose multi-round PBS to handle the exceptions.

\subsection{Hash Partition and Parity Bitmap Encoding}\label{sec:hash_partition}
% \medskip
% \noindent{\bf Hash Partition} 

Here we formalize the process of partitioning $A$ into $\{A_i\}_{i=1}^n$, $B$ into $\{B_i\}_{i=1}^n$, and $A\Delta B$ into $\{A_i\Delta B_i\}_{i=1}^n$ as described in \autoref{sec:smalld} by introducing the concept of {\it sub-universes}. Given a hash function $h(\cdot): \mathcal{U}\rightarrow \{1,2,\cdots,n\}$, we define {\it sub-universe} $\mathcal{U}_i$ as the set of elements in $\mathcal{U}$ that are hashed into value $i$. More precisely, $\mathcal{U}_i\triangleq\{s\!\mid\! s\in \mathcal{U} \mbox{ and } h(s)=i\}$ for $i=1,2,...,n$. Then defining $A_i\triangleq A\bigcap\mathcal{U}_i$ and $B_i\triangleq B\bigcap\mathcal{U}_i$ for $i=1,2,...,n$ induces the partitioning of $A$, $B$, and $A\Delta B$, as mentioned in \autoref{sec:smalld}. 

For the moment, we assume the following {\bf ideal case} happens: Every subset pair difference $A_i\Delta B_i$ contains at most one distinct element. The nonideal case of a subset pair difference containing more than $1$ distinct elements will be discussed in \autoref{subsec:exception_hash_partition}. 

%In this section, we give a detailed description on how to partition $A$ and $B$ (as introduced in \autoref{sec:smalld}) by introducing {\it sub-universes}, which is defined as follows: Given a hash function $h(\cdot): \mathcal{U}\rightarrow \{1,2,\cdots,n\}$, we define {\it sub-universes} $\{\mathcal{U}_i\}_{i=1}^n$, a partition of the universe $\mathcal{U}$, as $\mathcal{U}_i=\{s\!\mid\! s\in \mathcal{U} \mbox{ and } h(s)=i\}$ for $i=1,2,...,n$. Based on $\{\mathcal{U}_i\}_{i=1}^n$, we define $\{A_i\}_{i=1}^n$, the partition of $A$ introduced in \autoref{sec:smalld}, as $A_i\! \triangleq\! A\bigcap \mathcal{U}_i$ for $i=1,2,...,n$. $\{B_i\}_{i=1}^n$ is similarly defined. By this definition, the set difference $A\Delta B$ is partitioned into $n$ set differences of the partitioned subset pairs (i.e., $\{(A_i, B_i)\}_{i=1}^n$). From \autoref{sec:hash_partition} to \autoref{sec:reconcile_by_trivial}, we assume the following {\bf ideal case} happens: Each subset pair $(A_i, B_i)$ contains at most one distinct element ({\it i.e.,} $|A_i\Delta B_i|\!\leq\!1$). The nonideal case of a subset pair contains more than $1$ distinct elements will be discussed in \autoref{subsec:exception_hash_partition}. 

% Here we describe the hash-partition step introduced in \autoref{sec:smalld} in details. First, we use a hash function $h(\cdot): \mathcal{U}\rightarrow \{1,2,\cdots,n\}$ to partition the universe $\mathcal{U}$ into $n$ sub-universes: $\mathcal{U}_i=\{s\!\mid\! s\in \mathcal{U} \mbox{ and } h(s)=i\}$ for $\forall i=1,2,\cdots,n$. The hash function $h(\cdot)$ can be predetermined between Alice and Bob and does not require additional communication cost. Define $A_i\! \triangleq\! A\bigcap \mathcal{U}_i$ and $B_i\! \triangleq\! B\bigcap \mathcal{U}_i$ for $i=1,2,\cdots,n$. Then $\{A_i\}_{i=1}^n$ and $\{B_i\}_{i=1}^n$ are partitions of $A$ and $B$ respectively. Furthermore, $\{A_i\Delta B_i\}_{i=1}^n$ is a partition of $A\Delta B$. From \autoref{sec:hash_partition} to \autoref{sec:reconcile_by_trivial}, we assume the following {\bf ideal case} happens: Each subset pair $(A_i, B_i)$ contains at most one distinct element ({\it i.e.,} $|A_i\Delta B_i|\!\leq\!1$). The nonideal case of a subset pair contains more than $1$ distinct elements will be discussed in \autoref{subsec:exception_hash_partition}. 

How the $d$ distinct elements (balls) in $A\Delta B$ are distributed into the $n$ subset pair differences $\{A_i\Delta B_i\}_{i=1}^n$ (bins) 
can be viewed as throwing $d$ balls each uniformly and randomly into one of the $n$ bins. 
%follows the familiar {\it balls-into-bins} probability model. 
%The distinct elements are viewed as balls and the subset pairs are viewed as bins. 
%Each of the $d$ balls is uniformly and randomly thrown by the hash function $h(\cdot)$ into one of the $n$ bins. 
The aforementioned ideal case that corresponds to the $d$ balls ending up in $d$ distinct bins happens with probability $\prod_{k=1}^{d - 1}(1 - \frac{k}{n})$, which is on the order of $1-O(d^2/n)$ when $d\!\ll\!n$.
%approximately $e^{-\frac{d(d-1)}{2n}}$ when $d\!\ll\!n$. 
Hence, $n$ must be $\Omega(d^2)$ to ensure the ideal case happens with a nontrivial probability, as mentioned in \autoref{sec:smalld}.


%in which the distinct elements are viewed as balls and the subset pairs are viewed as bins. The hash-parition basically throws (hashes) $d$ balls (distinct elements) uniformly and randomly into $n$ bins (subset pairs). The aforementioned ideal case in this context becomes, after throwing $d$ balls uniformly and randomly into $n$ bins, each bin receives at most $1$ ball (i.e., $d$ nonempty bins have $1$ ball in each and the rest $n-d$ bins are empty). The number of balls in each bin is a Binomial random variable $Binomial(d,1/n)$.
%{\bf It may remind readers about the Birthday problem. And the ideal case can be analogous to the case that no people share the same birthday.} 
% The ideal case happens with a probability of $p\!=\!\prod_{k=1}^{d - 1}(1 - \frac{k}{n})\!\approx\! e^{-\frac{d(d-1)}{2n}}$ when $d\!\ll\!n$. In other words, $n$ must be at least $O(d^2)$ to ensure the ideal case happens with a nontrivial probability, as described in \autoref{sec:smalld}.  

% Note that the ideal case does not always happen. However, we can ensure that the ideal case happens with high probability by properly setting $n$ based on $d$ (i.e., $n=\Omega(d^2)$). Furthermore, as we will describe in \autoref{subsec:nonideal}, even if the ideal case does not happen (i.e., some distinct elements are hashed into the same subset pair), most of the distinct elements should be distributed into different subset pairs and therefore can be reconciled. So the scheme, even cannot reconcile all of the distinct elements, can still reconcile the majority of them (i.e., piecewise decodability in \autoref{sec:intro_oursolution}). Based on this property, we will extend our scheme from single-round to multi-rounds in \autoref{subsec:nonideal} to further increase the probability of reconciling all distinct elements. 

% \medskip
% \noindent{\bf Parity Bitmap Encoding} 

We encode $\{A_i\}_{i=1}^n$ into an $n$-bit-long parity bitmap $A[1..n]$, in which $A[i]$, the $i^{th}$ bit of the parity bitmap, is equal to the oddness / evenness (parity) of the cardinality of $A_i$ (i.e., $A[i]=1$ if $|A_i|$ is odd; otherwise $A[i]=0$). In the ideal case, the two bitmaps $A[1..n]$, $B[1..n]$ differ in exactly $d$ bit positions $i_1,i_2,...,i_d$, each of which corresponds to a subset pair that contains $1$ distinct element. The next step is to let Alice and Bob know these bit positions.
%Once the $d$ bit positions are known, Alice and Bob can start to reconcile $(A_{i_1},B_{i_1}), (A_{i_2},B_{i_2}),...,(A_{i_d},B_{i_d})$ using \autoref{alg:trivial_case} and obtain the $d$ distinct elements (i.e., $A\Delta B$). 

% \subsubsection{Parity Bitmap Encoding}\label{sec:parity_bitmap_encoding}

% %After hash-partitioning $A$ and $B$ into partitions $\{A_i\}_{i=1}^n$ and $\{B_i\}_{i=1}^n$, 
% As introduced in \autoref{sec:smalld}, we encode each partition into an $n$-bit-long parity bitmap and denote them as $A[1..n]$ and $B[1..n]$ respectively, as introduced in \autoref{sec:smalld}. For $i=1,2,...,n$, $A[i]$ (the $i^{th}$ bit of the parity bitmap $A[i]$) is equal to $1$ if $A_i$ contains an odd number of elements, and is equal to $0$ otherwise.
% % More specifically, for $i=1,2,...,n$, $A[i]$ (the $i^{th}$ bit of the parity bitmap $A[i]$) is defined as follows: $A[i]=1$ if $A_i$ contains an odd number of elements, and $A[i]=0$ otherwise. In this way, each bit $A[i]$ encodes the oddness / evenness (parity) of the cardinality of $A_i$. The $n$-bit-long parity bitmap $B[1..n]$ and $B[i]$ (the $i^{th}$ bit of $B[1..n]$) are similarly defined. 
% In the ideal case, 
% %$A[i]$ and $B[i]$ differ if and only if $A_i$ and $B_i$ have exactly $1$ distinct element, and $A[i]$ and $B[i]$ are the same if and only if $A_i=B_i$. Meanwhile, the $d$ distinct elements are hashed into $d$ different subset pairs. So 
% the two bitmaps $A[1..n]$, $B[1..n]$ differ in exactly $d$ bit positions, each of which corresponds to a subset pair that contains $1$ distinct element. Once the $d$ bit positions are known, Alice starts to reconcile each of the $d$ corresponding subset pairs by \autoref{alg:trivial_case} and gets the $d$ distinct elements (i.e., $A\Delta B$). 
% %If knowing the $d$ bit positions (i.e., the $d$ corresponding subset pairs), we can use \autoref{alg:trivial_case} to reconcile the $d$ subset pairs respectively to obtain all the $d$ distinct elements (i.e., $A\Delta B$). 
% In \autoref{sec:BCH_code}, we will describe how to find the $d$ bit positions using BCH code~\cite{Lint_IntroductionCodingTheory_1998}. 

% \medskip
% \noindent{\bf Find the $d$ Bit Positions Using ECC} 

%\subsubsection{Find the $d$ Bit Positions Using ECC}\label{sec:BCH_code}
\subsection{Find and Reconcile the $d$ subset pairs}\label{sec:BCH_code}

We view $A[1..n]$ as a corrupted message of $B[1..n]$ sent ({\bf not actually being sent}) from Bob to Alice through an {\it unreliable} commnunication channel that flips $d$ bits. To locate these $d$ bit positions, we let Bob also send an {\it error-correction code} that encodes $B[1..n]$ to Alice, such that Alice can recover $B[1..n]$ (original message) and obtain the $d$ bit positions $i_1,i_2,...,i_d$. In PBS, we choose BCH code~\cite{bch1} as the error-correction code.

There are two different BCH encoding techniques: {\it systematic} and {\it unsystematic}. The difference is, the message appears as the prefix of the codeword (i.e., codeword = [message net-codeword]) in systematic BCH encoding, whereas it does not appear as a substring of the codeword in unsystematic BCH encoding. In PBS, we choose systematic BCH encoding because we are not actually sending the ``message'', and only the net-codeword is transmitted from Bob to Alice. 

To correct $d$ bit errors, the length of the net-codeword only is no more than $d\log n$ bits. We use the term `codeword' to refer to the net-codeword in the rest of this paper.
%The computational complexity of the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} is $O(d^2\log^2 n)$.
The systematic BCH encoding is also used in other ECC-based set reconciliation works, such as PinSketch \cite{Wuille_Minisketchoptimizedlibrary_2019}, {\bf while} PinSketch encodes a much longer message (e.g., $2^{32}$ bits) than in ours (hundreds of bits).  

%\subsubsection{Find the $d$ Bit Positions Using ECC}\label{sec:BCH_code}

% A straightforward approach to find the $d$ bit positions is to let Bob send the complete parity bitmap $B[1..n]$ to Alice, then Alice compares $A[1..n]$ with $B[1..n]$ locally. This approach has a communication overhead of $n$ bits, which is quite wasteful. As we discussed in~\autoref{sec:hash_partition}, $d$ is usually much smaller than $n$. It means $A[1..n]$ and $B[1..n]$ differ only at a tiny portion of bits. Therefore, we can view $A[1..n]$ as a corrupted message of $B[1..n]$ with $d$ bit errors, and the bit positions of the $d$ bit errors basically correspond to the $d$ subset pairs that contain distinct elements. The detection of bit errors, on the other hand, can be solved by Error-Correction Code (ECC)~\cite{Lin_ErrorControlCoding_1983}. 

% Since $A[1..n]$ and $B[1..n]$ differ at $d$ bit positions, we can view $A[1..n]$ as a corrupted message of $B[1..n]$ from Bob to Alice through an {\it unreliable} commnunication channel with $d$ corrupted bits, which are located on the $d$ bit positions. Therefore, to find the $d$ bit position, we only need to correct the $d$ corrupted bits in $A[1..n]$, which is done by transmitting a ``code'' that can correct upto $d$ bit errors from Bob to Alice through a {\it reliable} communication channel. 

% In PBS, we use {\it systematic} BCH code to generate the ``code'' by encoding the message $B[1..n]$. The codeword of the systematic BCH code is in the form of [message, net-codeword], since the message appears as the prefix of the codeword in systematic BCH code. The ``code'' is simply the net-codeword in the BCH codeword. We choose {\it systematic} BCH code because the (corrupted) message is already transmitted and we only need to pay a small communication overhead on transmitting ``code'' (i.e., net-codeword). To correct upto $d$ bit errors, the length of the net-codeword is no more than $d\log n$ bits, which is much smaller than the message when $d\!\ll\! n$. The computational complexity of the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} is $O(d^2\log^2 n)$. This type of BCH code is also used in other ECC-based set reconciliation works, such as PinSketch \cite{Wuille_Minisketchoptimizedlibrary_2019}. 

% Different from {\it unsystematic} BCH code
% The ``code'' is generated by {\it systematic} BCH code, which encodes the message $B[1..n]$ into a BCH codeword in the form of [message, net-codeword]. The ``code'' transmitted on the reliable channel is the net-codeword of the BCH codeword. In {\it systematic} BCH code, the message appears as the prefix of the codeword. 

% More specifically, PBS uses {\it systematic} BCH code~\cite{Lint_IntroductionCodingTheory_1998} that can correct upto $d$ bit errors to encode the parity bitmaps. In the {\it systematic} BCH code \footnote{In unsystematic BCH code, message does not appear to be the prefix of the codeword}, the message (i.e., the parity bitmap) appears as the prefix of the raw codeword, which in the form of [message, net codeword]. Normally, to correct upto $d$ errors, the length of the net codeword is $2n\log d$, where $n$ is the length of the message (i.e., parity bitmap). However, our case is special in the sense that the net codeword is error-free (all $d$ bit errors are in the message), so the length of the net codeword can be reduced to $n\log d$. This type of BCH code is also used in other ECC-based set reconciliation works, such as PinSketch \cite{Wuille_Minisketchoptimizedlibrary_2019}. 

% Now we can formally describe how to find the $d$ bit positions: First, Bob uses a $d$-error-correcting systematic BCH code to encode $B[1..n]$ and sends the net codeword ($d\log n$ bits) to Alice. Upon receiving the net codeword and combining it with the corrupted message $A[1..n]$, Alice uses the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} to decode the $d$ bit errors in $A[1..n]$. The communication overhead of transmitting the net codeword is $d\log n$ bits. The computational complexity of the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} is $O(d^2\log^2 n)$. Both the communication overhead and the computational complexity here are relatively small when $d$ is small.

% \medskip
% \noindent{\bf Reconcile the $d$ subset pairs using \autoref{alg:trivial_case}} 

%Once the $d$ bit positions are known, Alice can start to reconcile $(A_{i_1},B_{i_1}), (A_{i_2},B_{i_2}),...,(A_{i_d},B_{i_d})$ using \autoref{alg:trivial_case} and obtain the $d$ distinct elements (i.e., $A\Delta B$). 
Once Alice decodes $i_1,i_2,...,i_d$, the corresponding subset pairs $(A_{i_1},B_{i_1}), (A_{i_2},B_{i_2}),...,(A_{i_d},B_{i_d})$ each can be reconciled using \autoref{alg:trivial_case}. To do so, Alice needs to send not only the corresponding \code{XOR} sums $S_{A_{i_1}}$, $S_{A_{i_2}}$, ...,$S_{A_{i_d}}$, but also the subset pair indices $i_1,i_2,...,i_d$, to Bob, since Bob does not know which of the $d$ subset pairs are being reconciled. Each index needs to be encoded into $\log n$ bits, so the additional communication overhead on transmitting the indices is $d\log n$ bits. 
% When reconciling $(A_{i_1},B_{i_1}), (A_{i_2},B_{i_2}),...,(A_{i_d},B_{i_d})$ using \autoref{alg:trivial_case}, Alice needs to send not only the bitwise \code{XOR} of $A_{i_1}, A_{i_2},..., A_{i_d}$, but also the indices of the subset pairs ($i_1,i_2,...,i_d$), since Bob does not know which of the $d$ subset pairs are being reconciled. Each index is an integer between $1$ and $n$ and can be encoded into $\log n$ bits, So the additional communication overhead on transmitting the indices is $d\log n$ bits. 



% \subsubsection{Reconcile the $d$ subset pairs using \autoref{alg:trivial_case}}\label{sec:reconcile_by_trivial}

% After decoding the $d$ bit errors that corresponds to the $d$ subset pairs, Alice starts to reconcile them using \autoref{alg:trivial_case}. For each of the $d$ subset pairs, Alice needs to send not only the bitwise \code{XOR} of the subset pair, but also the index of the subset pair (since Bob does not know the $d$ subset pairs to reconcile). So the communication overhead on \autoref{alg:trivial_case} is $d\log |\mathcal{U}|+d\log n$ bits. 
%Plus the communication overhead on transmitting the net codeword of parity bitmap ($d\log n$, as we explained in \autoref{sec:BCH_code}), the overall communication overhead of single-round PBS is $d\log u+2d\log n$ bits.

% \medskip
% \noindent{\bf Check if set reconciliation is complete} 

After reconciling the subset pairs and obtaining the reconciled set difference (denoted as $\hat{D}$), PBS needs to check if set reconciliation is complete (or whether $\hat{D}=A\Delta B$), since the reconciled set difference $\hat{D}$ is not the actual set difference $A\Delta B$ in the nonideal case (to be discussed in \autoref{subsec:exception_hash_partition}). Hence, we add a verfication step after obtaining $\hat{D}$ to check if $\hat{D}=A\Delta B$. In PBS, we check an equivalent condition, $A=B\Delta\hat{D}$, instead of $\hat{D}=A\Delta B$, since $B$ and $\hat{D}$ are both known by Bob and their set difference $B\Delta\hat{D}$ can be locally computed. More specifically, to check if the remote sets $A$ and $B\Delta\hat{D}$ are equal, we let Alice compute a $32$-bit checksum of $A$ and send it to Bob. {\bf Then Bob computes the $32$-bit checksum of $B\Delta\hat{D}$ using the same checksum algorithm and compare the two checksums. In PBS, we select {\it longitudinal parity check} (i.e., bitwise \code{XOR} of all elements in the set) as the checksum algorithm, so that the checksum $B\Delta\hat{D}$ can be efficiently computed as the bitwise \code{XOR} between the checksum of $B$ (can be pre-computed) and that of $\hat{D}$. Other checksum algorithms that are {\it linear} to the set difference operator (i.e., $\Delta$) also work for PBS. }
% Then Bob checks if $B\Delta\hat{D}$ satisfies the receiving checksum. 

The condition $A=B\Delta\hat{D}$ can be almost surely verified by a $32$-bit checksum, albeit it could mistakenly believe two different sets as identical ones with probability $2^{-32}\approx 2.3\times 10^{-10}$. This probability should be small enough for most applications.
%and such an event (i.e., mistaken $A$ and $B\Delta\hat{D}$ are identical when they are different) never happens in our evaluation. For some super critical applications, we can certainly use a $64$-bit checksum to reduce this probability to $5.4\times 10^{-20}$ if needed.

% When the ideal case does not happen, set reconciliation cannot accomplish in one round, as we will explain in \autoref{subsec:exception_hash_partition}. Hence, we add a verfication step to check if set reconciliation is complete. Let $\hat{D}$ denote the set of reconciled elements. The idea of this verification is basically to compare $A$ with $B\Delta \hat{D}$: If $A=B\Delta \hat{D}$ (i.e., $\hat{D}=A\Delta B$), we know the set reconciliation is complete; Otherwise, the set reconciliation is incomplete.  using a $32$-bit checksum. 

\subsection{Communication overhead of PBS (First Round)}\label{sec:communication_overhead_single_PBS}

All the steps of PBS in the first round are summarized in \autoref{alg:single_round_pbs}. The overall communication overhead consists of three components: (1) the BCH codeword of $d\log n$ bits in \autoref{step:BCH_encode}; (2) the subset pair indices $i_1,i_2,...,i_d$ and the corresponding bitwise \code{XOR}s of $d\log n+d\log |\mathcal{U}|$ bits in \autoref{step:trivial_reconcile}; and (3) the $32$-bit checksum of $A$ in \autoref{step:terminate_condition}. 

\begin{algorithm}
\caption{Single-round PBS}
\label{alg:single_round_pbs}

%Hash-partition $A$, $B$ into $\{A_i\}_{i=1}^n$, $\{B_i\}_{i=1}^n$\; \label{step:hash_partition}

%Parity encode $\{A_i\}_{i=1}^n$, $\{B_i\}_{i=1}^n$ into $A[1..n]$, $B[1..n]$\; \label{step:parity_encode}

{\it Bob}: BCH-Encodeing $B[1..n]$ and send the codeword to Alice\; \label{step:BCH_encode}

{\it Alice}: Upon receiving the codeword, decode the bit errors between $A[1..n]$ and $B[1..n]$\; \label{step:BCH_decode}

{\it Alice}: For each bit error, start reconciling the corresponding subset pair by \autoref{alg:trivial_case}\; \label{step:trivial_reconcile}

{\it Bob}: Upon receiving the reconciled set difference $\hat{D}$, check whether $A=B\Delta \hat{D}$ via checksum\; \label{step:terminate_condition}
\end{algorithm}


% \subsubsection{Single-round PBS}\label{sec:single_round_pbs}

% Here we summarize all the steps of single-round PBS and represent it by pseudocode in \autoref{alg:single_round_pbs}. \autoref{step:hash_partition} and \autoref{step:parity_encode} operates at both hosts (i.e., Alice and Bob). \autoref{step:hash_partition} to \autoref{step:trivial_reconcile} have been elaborated from \autoref{sec:hash_partition} to \autoref{sec:reconcile_by_trivial}. The last step in \autoref{step:terminate_condition} aims to check whether reconciliation is complete (i.e., $\mathcal{D}=A\Delta B$). More specifically, Alice calculates the checksum (e.g., CRC-$32$) of $A$ and send it to Bob. Then Bob calculates the checksum of $B\Delta \mathcal{D}$ and compares it to the receiving checksum of $A$. If the two checksums are the same, we believe $A=B\Delta \mathcal{D}$ and therefore $\mathcal{D}=A\Delta B$ (i.e., reconciliation is complete); Else, we know some elements are reconciled incorrectly. We classify those elements (i.e., the ones in the set difference between $A\Delta B$ and $\mathcal{D}$) into two subsets $A\Delta B\!\setminus\!\mathcal{D}$ and $\mathcal{D}\!\setminus\!(A\Delta B)$ and refer the elements in the former as {\it false-negatives}, and refer the elements in the later as {\it false-positives}. 

% In the ideal case, neither false-positives nor false-negatives will happen and the two checksums always equal. However, in real life, the ideal case does not always happen. We will discuss the nonideal case in \autoref{subsec:exception_hash_partition}. In our evaluation, we use a $32$-bit checksum for comparing $A$ to $B\Delta \mathcal{D}$ that has {\bf an error probability} roughly $10^{-9}$. This error (i.e., mistake $A=B\Delta \mathcal{D}$) incurs false-negatives. All set reconciliation schemes have the same problem on their termination conditions (i.e., check whether $\mathcal{D}=A\Delta B$). For some super critical applications, we can certainly decrease the error probability by using more powerful checksums (i.e., $64-$bit). Using a $32$-bit checksum, this kind of false-negatives never happen in the evaluation. 
% %For simplification, we assume no error happens when checking $\mathcal{D}=A\Delta B$ in the rest of the paper.

% \begin{algorithm}
% \caption{Single-round PBS}
% \label{alg:single_round_pbs}

% Hash-partition $A$, $B$ into $\{A_i\}_{i=1}^n$, $\{B_i\}_{i=1}^n$\; \label{step:hash_partition}

% Parity encode $\{A_i\}_{i=1}^n$, $\{B_i\}_{i=1}^n$ into $A[1..n]$, $B[1..n]$\; \label{step:parity_encode}

% {\it Bob}: Encode $B[1..n]$ by BCH code, then send the codeword to Alice\; \label{step:BCH_encode}

% {\it Alice}: Upon receiving the codeword, decode the bit errors between $A[1..n]$ and $B[1..n]$\; \label{step:BCH_decode}

% {\it Alice}: For each bit error, reconcile the corresponding subset pair by \autoref{alg:trivial_case}\; \label{step:trivial_reconcile}

% {\it Bob}: Upon the reconciled distinct elements $\mathcal{D}$, check whether $A=B\Delta \mathcal{D}$ via checksum\; \label{step:terminate_condition}
% \end{algorithm}

\subsection{Exception Handling}\label{subsec:exception_hash_partition}

When the ideal case does not happen, some subset pair may contain more than $1$ distinct elements and cannot be successfully reconciled by \autoref{alg:trivial_case}. Due to the parity encoding, we can classify such a subset pair into the following two types: 

\noindent {\bf Type (\Romannum{1})}: Subset pair $(A_i, B_i)$ contains even number ($\geq 2$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be the same and PBS will not reconcile the subset pair yet in this round. It happens with a small but nontrivial probability: For example, $d=5$ and $n=255$ (i.e., throwing $5$ balls uniformly and randomly into $255$ bins), the probability that some bin has $2$ or $4$ balls is roughly $0.04$. Note that when a Type (\Romannum{1}) subset pair exists, the $32$-bit checksum (\autoref{step:terminate_condition} in \autoref{alg:single_round_pbs}) can almost surely detect that the set reconciliation is incomplete. If this is the case (i.e., the checksum is verified to be incorrect), PBS will start another round of set reconciliation to reconcile the remaining distinct elements (e.g., the ``hidden'' distinct elements in Type (\Romannum{1}) subset pairs), so on so force, until all distinct elements are reconciled and the checksum is verified to be correct, as we will describe in \autoref{sec:multi-rounds}. 

\noindent {\bf Type (\Romannum{2})}: Subset pair $(A_i, B_i)$ contains odd number ($\geq 3$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be different and PBS will reconcile the subset pair using \autoref{alg:trivial_case}. The reconciled element (i.e., $s$ in \autoref{alg:trivial_case}) is however a ``fake'' distinct element, which is actually the bitwise \code{XOR} of all distinct elements in $(A_i, B_i)$ (explained in \autoref{subsec:protocol0}).
%, which will be mistakenly believed as the distinct element of $(A_i, B_i)$. 
It happens with a much smaller probability than Type (\Romannum{1}): Use the same example ($d=5$ and $n=255$), the probability that some bin has $3$ or $5$ balls is roughly $1.52\times 10^{-4}$ ({\bf was miscalculated}). Similarly, the $32$-bit checksum can also almost surely detect that the set reconciliation is incomplete when a Type (\Romannum{2}) subset pair exists, and both the ``hidden'' and the ``fake'' distinct elements in Type (\Romannum{2}) subset pairs will also be reconciled in later rounds. 

Note that those ``fake'' distinct elements will become new distinct elements and therefore incur additional communication overhead in the next round. To filter out (the majority of) those ``fake'' distinct elements from later-round set reconciliation, we add a verification on each reconciled element of \autoref{alg:trivial_case} with no additional communication cost, which can detect ``fake'' distinct elements with high probability: 

\begin{algorithm}
\caption{Verify reconciled element $s$ of $(A_i, B_i)$}
\label{alg:verification}
\If{$h(s)\neq i$} {Discard the reconciled element $s$;}
\end{algorithm}

Although a distinct element of $(A_i, B_i)$ must be in sub-universe $\mathcal{U}_i$ (i.e., the hash value of the element under $h$ equals to $i$), a ``fake'' distinct element could be in any sub-universe with probability $1/n$, since it is the bitwise \code{XOR} of all distinct elements of $(A_i, B_i)$. Therefore, \autoref{alg:verification} only fails to identify a ``fake'' distinct element with probability $1/n$, which is roughly $3.9\times 10^{-3}$ when $n=255$. In other words, a ``fake'' distinct element that cannot be identified by \autoref{alg:verification} appears with probability $6\times 10^{-7}$. {\bf I feel that defining $\tilde{a}_4=a_1\oplus a_2\oplus a_3$ does not help much.}

{\bf Readers may wonder encoding the exact subset sizes (i.e., $|A_i|, |B_i|$) instead of their oddness / evenness (parity) (described in \autoref{sec:hash_partition}) could help to identify Type (\Romannum{1}), (\Romannum{2}) subset pairs. However, encoding the exact subset sizes not only incurs much more additional communication overhead comparing to the parity bits, but also does not help much on identify Type (\Romannum{1}), (\Romannum{2}) subset pairs, since we cannot precisely derive $|A_i\Delta B_i|$, the total number of distinct elements in $(A_i, B_i)$, even knowing $|A_i|, |B_i|$: For instance, when $|A_i|\!=\!|B_i|\!=\!50, |A_i\Delta B_i|$ could be any even number ($\leq 100$) if the distinct elements are evenly splitted and assigned between $A_i$ and $B_i$. }

% As we have described in \autoref{sec:hash_partition}, the ideal case does not always happen, which means some subset pair may contain more than $1$ distinct elements and cannot be successfully reconciled by \autoref{alg:trivial_case}. Due to the parity encoding, we can classify such subset pair into the following two scenarios:

% \begin{itemize}
%     \item Scenario 1: If a subset pair $(A_i, B_i)$ contains even number ($\geq 2$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be the same and PBS will not reconcile the subset pair yet in this round;
%     \item Scenario 2: If a subset pair $(A_i, B_i)$ contains odd number ($\geq 3$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be different and PBS will reconcile the subset pair using \autoref{alg:trivial_case}. The reconciled element (i.e., $s$ in \autoref{alg:trivial_case}) is however the bitwise \code{XOR} of all distinct elements in $(A_i, B_i)$ (explained in \autoref{subsec:protocol0}), which will be mistakenly believed as the distinct element of $(A_i, B_i)$. 
%     %However, as described in \autoref{subsec:protocol0}, when a subset pair contains more than $1$ distinct elements, \autoref{alg:trivial_case} will output the bitwise \code{XOR} of them as the `distinct element', which is not an actual distinct element with high probability;
% \end{itemize}

% In both scenarios, the distinct elements in the subset pair will not be reconciled in this round. As we will describe in \autoref{sec:multi-rounds}, we generalize PBS into multi-round, so that the distinct elements that have not been reconciled in the first round will be reconciled in later rounds. On the other hand, the second scenario could result in incorrectly reconciled distinct elements, which will become new distinct elements in the next round in multi-round PBS. 

% % In both scenarios, the distinct elements in the subset pair cannot be successfully reconciled in this round and will remain in the set difference (i.e., $(A\Delta B)\!\setminus\!\hat{D}$). On the other hand, the incorrectly reconciled distinct element in the second scenario will appear as a new distinct element (i.e., $\hat{D}\!\setminus\!(A\Delta B)$) in the next round if we generalize PBS into multi-round (to be elaborated in \autoref{sec:multi-rounds}). Both scenarios can be almost surely detected by the 32-bit checksum (\autoref{step:terminate_condition} in \autoref{alg:single_round_pbs}). The set difference after the reconciliation in this round, $D\Delta\hat{D}$, can be reconciled in later rounds, as we will describe in \autoref{sec:multi-rounds}. 

% Naturally, we do not want to generate new distinct elements in the process of set reconciliation, even though it happens with a tiny probability when $n=\Omega(d^2)$: For instance, when $d=5$ and $n=255$ (i.e., throwing $5$ balls uniformly and randomly into $255$ bins), the probability (i.e., some bin has $3$ or $5$ balls) is only $7.6\times 10^{-6}$. Therefore, we add a verification with no additional communication cost on each reconciled element of \autoref{alg:trivial_case}, such that each incorrect dinstinct element can be identified with high probability. The verfication is shown in \autoref{alg:verification}. 

% \begin{algorithm}
% \caption{Verify reconciled element $s$ of $(A_i, B_i)$}
% \label{alg:verification}
% \If{$h(s)\neq i$} {Discard the reconciled element $s$;}
% \end{algorithm}

% Although any distinct element of $(A_i, B_i)$ must be in sub-universe $\mathcal{U}_i$ (i.e., the hash value of the element under $h$ equals to $i$), the bitwise \code{XOR} of multiple distinct elements of $(A_i, B_i)$ could be in any sub-universe with probability $1/n$. Therefore, \autoref{alg:verification} fails to identify an incorrectly reconciled distinct element in the second scenario with probability $1/n$ that is roughly $3.9\times 10^{-3}$ when $n=255$. In other words, an incorrectly reconciled distinct element that cannot be identified by \autoref{alg:verification} appears with probability $3\times 10^{-8}$. {\bf I feel that defining $\tilde{a}_4=a_1\oplus a_2\oplus a_3$ does not help much.}

% In both scenarios, the distinct elements in the subset pair cannot be successfully reconciled in this round. These distinct elements can be reconciled in later rounds if needed, as we will describe in \autoref{sec:multi-rounds}. In this section, we only discuss how to identify the {\it incorrect} distinct element in the second scenario. Let us use an example to elaborate the second scenario: Assume $(A_i, B_i)$ contains $3$ distinct elements $a_1, a_2, a_3$, then Bob computes $\tilde{s}=a_1\oplus a_2\oplus a_3$ using \autoref{alg:trivial_case} and mistakes it as the distinct element in $(A_i, B_i)$. 

% In both scenarios, the distinct elements in the subset pair cannot be successfully reconciled (i.e., false-negatives defined in \autoref{sec:single_round_pbs}. The distinct elements that are not successfully reconciled in this round, if needed, can be reconciled in later rounds as we will describe in \autoref{sec:multi-rounds}. In this section, we only discuss how to identify the {\it incorrect} distinct elements in the second scenario. Let us use an example to elaborate the second scenario: Assume $(A_i, B_i)$ contains $3$ distinct elements $a_1, a_2, a_3$, then Bob computes $\tilde{s}=a_1\oplus a_2\oplus a_3$ using \autoref{alg:trivial_case} and mistakes it as the distinct element in $(A_i, B_i)$. 

\begin{comment}
============================================

We add a no-communication-cost verification step to check whether a reconciled element is an actual distinct element or not. Note that an actual distinct element of $(A_i, B_i)$ must be in sub-universe $\mathcal{U}_i$. On the other hand, an incorrectly reconciled element (e.g., $\tilde{s}$) can be in any sub-universe with probability $1/n$. So at the end \autoref{subsec:protocol0}, we check whether the reconciled element is in $\mathcal{U}_i$ by the hash function $h$ in hash-partition:

This verfication cannot completely eliminate false-positives, since an incorrectly reconciled element (e.g., $\tilde{s}$) can coincidentally end up in $\mathcal{U}_i$ with probability $1/n$. The chance of false-positives is extremely small using the verification. For instance, if $d=5$ and $n=255$, the probability of the second scenario is only $7.6\times 10^{-6}$. The probability of false-positives using the verfication is $1/n$ times this small probability, which is roughly $3\times 10^{-8}$. {\bf Note that a small probability of false-positives only costs a little waste on set reconciliation when synchronizing objectives (e.g., files), which is acceptable for most applications.}

Even worse, in the second scenario, the false-positives defined in \autoref{sec:single_round_pbs} could happen. For example, if subset pair $(A_i, B_i)$ contains $3$ distinct elements $s_1, s_2, s_3$, then \autoref{alg:trivial_case} computes $\tilde{s}=s_1\oplus s_2\oplus s_3$ and Bob mistakes $\tilde{s}$ as an actual distinct element. The good thing is, the probability of this kind of false-positives is extremely small for small $d$. For instance, if $d=5$ and $n=255$, the probability of the false-positives is only $7.6\times 10^{-6}$. To further reduce the chance of false-positives, we add a no-communication-cost verification step at the end of \autoref{subsec:protocol0} to check whether $\tilde{s}$ is an actual distinct element or not. The verification step works as follows: Given the output $s$ of subset pair $(A_i,B_i)$, if $s\in\mathcal{U}_i$ (i.e., $h(s)=i$), we consider $s$ as an actual distinct element; Otherwise, we consider $s$ as an incorrect output and discard it. 

Note that if $\tilde{s}\in A_i\Delta B_i$, $\tilde{s}$ must be in sub-universe $\mathcal{U}_i$. However, if $\tilde{s}$ is the bitwise \code{XOR} of the distinct elements in $(A_i,B_i)$ (i.e., the second scenario happens), it ends up in $\mathcal{U}_i$ with probablity of only $1/n$. 
%In fact, if we assume the hash-partition described in \autoref{sec:hash_partition} hashes the elements of $\mathcal{U}$ uniformly, independently, and randomly into $n$ sub-universes, the output $s$ in the second scenario will be in a different sub-universe $\mathcal{U}_j (j\neq i)$ with a high probability of $1-\frac{1}{n}$. Hence, this verfication method can further reduce the probability of false-positives by a factor of $\frac{1}{n}$. 
Use the same example (i.e., $d=5$, $n=255$), the probability of this kind of false-positives is reduced from $7.6\times 10^{-6}$ to $3\times 10^{-8}$ by this verification method. 
%{\bf This probability can be further reduced in \autoref{subsec:protocol2}, where PBS does two tiers of hash-partitions. So we can do verification on both of the two hash functions.}

%In some super critical cases (i.e., no false-positive is allowed), we can use a more powerful verification method to completely eliminate false-positives. That is, to check if the output $s$ exists in exactly one of the two sets (i.e., $s\in A\!\setminus\! B$ or $s\in B\!\setminus\! A$). To do so, Bob transmits $s$ along with an identification bit $\mathbbm{1}_{\{s\in B\}}$ to Alice, then Alice checks if $s\in (A\!\setminus\! B)\bigcup (B\!\setminus\! A)$ . This method verification costs additional $d(\log u+1)$ bits of communication overhead. In most applications, this rigorous $0\%$ probability guarantee of false-positives is unnecessary and the probability of the former verification method is small enough, so we use the former in the evaluation. Based on our observation, this kind of false-positives do not happen even once in the evaluation using the former verfication method. In the rest of this paper, we assume Scenario 2 is always correctly verified. 

============================================
\end{comment}

\subsection{Running PBS for Multiple Rounds}\label{sec:multi-rounds}

When the ideal case does not happen (i.e., Type (\Romannum{1}) or Type (\Romannum{2}) subset pairs exist), PBS will know the set reconciliation is incomplete by the $32$-bit checksum (\autoref{step:terminate_condition} in \autoref{alg:single_round_pbs}). To reconcile those distinct elements that have not been reconciled yet in the first round, we rule out all reconciled elements and run another round of PBS. This procedure replicates until the checksum is verified to be correct.

More specifically, in the second round, we run PBS to reconcile $A$ and $B\Delta \hat{D}$ instead of $A$ and $B$ to rule out all elements that have been reconciled, where $\hat{D}$ is the set of reconciled distinct elements in the first round. On the other hand, we use a different hash function for hash-partition in the second round to avoid the exceptions (i.e., Type (\Romannum{1}) or Type (\Romannum{2}) subset pairs described in \autoref{subsec:exception_hash_partition}) that happened in the first round happen again. The later rounds are similarly operated. 

Although PBS may need to run many rounds to reconcile all distinct elements, the communication overhead mostly happens in the first round, since the majority of the distinct elements should be reconciled in the first round. Use the same example ($d=5, n=255$), on average $4.81$ out of $5$ distinct elements should be reconciled in the first round. So the total communication overhead in all rounds is only slightly larger ($1.03$ to $1.08$ times of {\bf refer to the evaluation result.}) than that in the first round. Due to this reason, we use the communication overhead in the first round (described in \autoref{sec:communication_overhead_single_PBS}) to approximate the total communication overhead (all rounds) in parameter settings (to be elaborated in \autoref{sec:parameter_settings}).

When running PBS for multiple rounds, we set an objective $(r,p_0)$ that the set reconciliation will be complete in $r$ round with probability $p_0$. This objective is needed for parameter settings and it ensures the set reconciliation completes in a few rounds. For example, when we set an objective of $(3,0.99)$ (i.e., the set reconciliation completes in $3$ round with probability $0.99$), PBS should run at most $5$ rounds to complete set reconciliation with extremely high probability (say $0.999999$). 

For the moment, we assume no ``fake'' distinct element fails to be detected in PBS, which happens with overwhelming probability as explained in \autoref{subsec:exception_hash_partition}. Then PBS reconciles the distinct elements gradually round by round. This is the ``piecewise decodability'' mentioned in \autoref{sec:intro_oursolution}. We use the following example to describe it in details: Given two sets $A$, $B$ with $10$ distinct elements (i.e., $d=10$), in the first round, PBS hashes them into $7$ distinct subset pairs. $6$ distinct elements are hashed into $6$ distinct subset pairs, and the other $4$ distinct elements are hashed into the same subset pair. Then the former $6$ distinct elements are successfully reconciled in the first round and the later $4$ distinct elements remain to be reconciled in the second round, which are hashed into $3$ distinct subset pairs (under a different hash function). $2$ remaining distinct elements are hashed into $2$ distinct subset pairs, and the other $2$ remaining distinct elements are hashed into the same subset pair. Then the former $2$ remaining distinct elements are successfully reconciled in the second round and the later $2$ remaining distinct elements remain to be reconciled in the third round, so on so force. The dynamics of the number of remaining distinct elements (i.e., $10\leadsto 4\leadsto 2\leadsto \cdots$ in the example) is in nature a Markov chain, which will be elaborated and analyzed in \autoref{sec:tail_bound_per_group} to derive a tail bound of success probability (i.e., all distinct elements are reconciled in $r$ rounds) for paramenter settings.

% Even if the ideal case does not happen, most of the distinct elements should be distributed into different subset pairs, one distinct element in each, and therefore can be successfully reconciled. So in the first round, even if PBS cannot reconcile all distinct elements, it can reconcile the majority of them.
% % (piecewise decodability mentioned in \autoref{sec:intro_oursolution})
% Based on this intuition, we generalize PBS to multi-round, so that the distinct elements that are not reconciled yet in the first round can be reconciled in later rounds.  

% Without loss of generality, we only describe the second round of multi-round PBS, the reconciliation in the later rounds are similar. Let $\hat{D}_1$ denote the set of reconciled elements in the first round. If set reconciliation is not complete in the first round (i.e., the checksum infers $A\neq B\Delta \hat{D}_1$), then multi-round PBS saves $\hat{D}_1$, which includes correctly and incorrectly reconciled elements as described in \autoref{subsec:exception_hash_partition}, and starts the second round to find (1) the remaining distinct elements; (2) the incorrectly reconciled distinct elements in the first round. In the second round, multi-round PBS reconciles $A$ and $B\Delta \hat{D}_1$ instead of $A$ and $B$ (i.e., $B\leftarrow B\Delta\hat{D}_1$) to rule out all elements that have been reconciled. {\bf It uses a hash function that is different from the one used in the first round for hash-partition, otherwise every remaining distinct element will be hashed into the same subset pair and cause the same exception (described in \autoref{subsec:exception_hash_partition}) that happened in the first round.}

% If set reconciliation is complete in the second round, the set of reconciled elements in the second round (denoted as $\hat{D}_2$) should be the union of (1) all distinct elements that have not been reconciled in the first round (i.e., $(A\Delta B)\!\setminus\!\hat{D}_1$); and (2) all incorrectly reconciled elements in the first round (i.e., $\hat{D}_1\!\setminus\!(A\Delta B)$), which is by definition the set difference between $A\Delta B$ and $\hat{D}_1$. Therefore, the overall set difference $A\Delta B$ equals to the set difference between $\hat{D}_1$ and $\hat{D}_2$; Else, multiround PBS saves $\hat{D}_2$ and starts the third round, so on so force. 

% {\bf May need this algorithm to show the dynamics, if so, the earlier algorithm needs to change accordingly.}
% \IncMargin{1em}
% \begin{algorithm}
% \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
% \Input{$A$ and $B$}
% \Input{Maximum number of rounds $r$}
% \Output{$D$}

% $\hat{D},\mbox{ complete} \leftarrow PBS(A,B)$\;

% $D \leftarrow \hat{D}$\;

% \While{!complete and $r>0$}{
	
% 	$B \leftarrow B\Delta\hat{D}$\;

% 	$\hat{D},\mbox{ complete} \leftarrow PBS(A,B)$\;

% 	$D \leftarrow D\Delta\hat{D}$\;

% 	$r \leftarrow r-1$\;
% }

% \caption{Multi-round PBS} \label{proto:multirounds}
% \end{algorithm}\DecMargin{1em}

% The idea of multi-round PBS is quite simple: In each round, we discard the reconciled distinct elements in the previous rounds and aim to find the rest distinct elements from the remaining elements. More specifically, the first round of multi-round PBS is just the same as single-round PBS in \autoref{alg:single_round_pbs}. The second round has the same procedures as the first round. One difference is, we update $B$ by $B\leftarrow B\Delta\mathcal{D}$ in the second round, so that (1) Reconciled distinct elements in $\mathcal{D}$ that were contained in $A\Delta B$ are not longer contained in $A\Delta (B\Delta\mathcal{D})$; and (2) The other distinct elements remain in $A\Delta (B\Delta\mathcal{D})$ and can be reconciled later. The other difference is, we use a different hash function for partition (\autoref{step:hash_partition}) in the second round. Later rounds update $B$ in the same way and also use different hash functions. Multi-round terminates if the check in \autoref{step:termination} is correct. The overall set difference $A\Delta B$ is simply the union of reconciled distinct elements in all rounds. 

% A straightforward approach to discard reconciled distinct elements is to remove them from both $A$ and $B$. This approach however incurs additional communication overhead to update $A$, since only Bob learns the partial set difference in \autoref{step:reconcile}. Therefore, we use the approach in \autoref{step:updateb} that only updates $B$. It has another benefit in \autoref{step:termination}, which only needs to transmit the CRC of $A$ from Alice to Bob in the first round. In the later rounds, \autoref{step:termination} can be checked locally by Bob and does not require any additional communication overhead;

% Note that the communication overhead in the first round accounts for a large percentage of the total communication overhead in multi-round PBS, since most of the distinct elements (over $95\%$ as we will show in {\bf point to the figure}) should be reconciled in the first round. Therefore, we use the same parameter $n$ in later rounds because otherwise we have to compute a new parameter that can only save tiny communication overhead, even though the number of remaining distinct elements is small and can be reconciled using smaller $n$ with high probability. {\bf Due to the same reason, we can the same expression of the communication overhead in single-round PBS to approximate the communication overhead in multi-round PBS.}

% The natural termination condition of multi-round PBS is that all distinct elements are reconciled, which could require a large number of rounds and incur large additional communication overhead (each additional round incurs $d\log n$ bits of additional communication overhead on transmitting BCH codeword). To control the amount of additional communication overhead, we set another termination condition that multi-round PBS runs for at most $r$ rounds (typically $2$ or $3$). This termination condition could cause an `early' termination when some distinct elements have not been reconciled. However, under proper parameter settings (to be discussed in \autoref{sec:parameter_settings}), we can prove that the probability of an `early' termination (i.e., set reconciliation is incomplete in $r$ round) is very small
% %, and even if an `early' termination happens, an overwhelming percentage of distinct elements should have been reconciled, which is sufficient for most applications
% . For example, when $d=5, n=255, r=2$, an `early' termination happens with probability $4.8\times 10^{-4}$ (how to compute this probability will be elaborated in \autoref{sec:tail_bound}).

% For the moment, we assume no incorrectly reconciled distinct elements appears in multi-round PBS, which happens with overwhelming probability as explained in \autoref{subsec:exception_hash_partition}. Then multi-round PBS reconciles the distinct elements gradually round by round. This is the ``piecewise decodability'' mentioned in \autoref{sec:intro_oursolution}. We use the following example to describe it in details: Given two sets $A$, $B$ with $10$ distinct elements (i.e., $d=10$), in the first round, multi-round PBS hashes them into $7$ distinct subset pairs. $6$ distinct elements are hashed into $6$ distinct subset pairs, and the other $4$ distinct elements are hashed into the same subset pair. Then the former $6$ distinct elements are successfully reconciled in the first round and the later $4$ distinct elements remain to be reconciled in the second round, which are hashed into $3$ distinct subset pairs (under a different hash function). $2$ remaining distinct elements are hashed into $2$ distinct subset pairs, and the other $2$ remaining distinct elements are hashed into the same subset pair. Then the former $2$ remaining distinct elements are successfully reconciled in the second round and the later $2$ remaining distinct elements remain to be reconciled in the third round, so on so force. The dynamics of the number of remaining distinct elements (i.e., $10\leadsto 4\leadsto 2\leadsto \cdots$ in the example) is in nature a Markov chain, which will be elaborated and analyzed in \autoref{sec:tail_bound_per_group} to derive a tail bound of success probability (i.e., all distinct elements are reconciled in $r$ rounds) for paramenter settings. 

% In most applications, a high percentage of reconciliation (e.g., $>99\%$ distinct elements are reconciled) is good enough. Therefore, we add another termination condition on the maximum number of rounds (denoted as $r$). The larger $r$ is, the higher percentage of distinct elements will be reconciled. How to set parameters based on $r$ will be elaborated in \autoref{sec:parameter_settings};

% Readers may think the communication overhead of multi-round PBS is proportional to the number of rounds. In fact, the majority of the communication overhead is spent in the first round, since most of the distinct elements (over $95\%$ as we will show in {\bf point to the figure}) are reconciled in the first round. Each additional round only incurs a small amount of additional communication overhead. For example, when $d=10, n=255, |\mathcal{U}|=2^{32}$, assume $8$ distinct elements are reconciled in the first round and the rest $2$ distinct elements are reconciled in the second round. Then the communication overhead in the first round is $432$ bits. That number of the second round is only $160$


%the communication overhead of single-round PBS of $272$ ($2d\log n+d\log |\mathcal{U}|+32$) bits, and each additional round incurs $40$ ($d\log n$) bits of additional communication overhead. 

%among the three components of the communication overhead mentioned in \autoref{sec:communication_overhead_single_PBS}, only the first component (i.e., the BCH codeword) is proportional to the number of rounds. The other two components does not depend on the number of rounds.

% The second component only depends on the total number reconciled elements, which is roughly equal to $d$. The third component, the checksum of $A$, only needs to be sent once in the first round.
%Therefore, the communication overhead of multi-round PBS is only slightly larger than that of single-round PBS when the number of rounds is small (say $3$). For example, when $d=5, n=255, |\mathcal{U}|=2^{32}$, the communication overhead of multi-round PBS of $3$ rounds is $352$ bits, which is roughly $1.3$ times of the communication overhead of single-round PBS ($272$ bits).

% Therefore, each additional round of multi-round PBS only incurs a small amount of additional communication overhead. For example, when $d=5, n=255, |\mathcal{U}|=2^{32}$, the communication overhead of single-round PBS of $272$ ($2d\log n+d\log |\mathcal{U}|+32$) bits, and each additional round incurs $40$ ($d\log n$) bits of additional communication overhead. 

% As we explained in \autoref{sec:reconcile_by_trivial}, the communication overhead in each round is proportional to the number of (remaining) distinct elements, which decreases exponentially as the number of round increase (i.e., the first round reconciles $90\%$ of distinct elements, the second round reconciles $90\%$ of the remaining $10\%$ distinct elements, etc.). So the majority of the communication overhead (i.e., $\approx 90\%$) is in the first round. Therefore, we do not bother to optimize parameters (i.e., smaller $n$) in later rounds to save tiny communication overhead, even though remaining distinct elements become fewer and can be reconciled using smaller $n$;

% The termination condition of multi-round PBS is that all distinct elements are reconciled, which may require many rounds. In most applications, a high percentage of reconciliation (e.g., $>99\%$ distinct elements are reconciled) is good enough. Therefore, we add another termination condition on the maximum number of rounds (denoted as $r$). The larger $r$ is, the higher percentage of distinct elements will be reconciled. How to set parameters based on $r$ will be elaborated in \autoref{sec:parameter_settings};

% Multi-round means multiple round-trip delays. {\bf Thanks for the piecewise decodability of PBS, in almost all practical application scenarios, this tradeoff does not lead to longer response time because the reconciliation of objects identified by the successfully decodable codewords, which constitute the vast majority of all codewords, can run in parallel with the transmissions and decodings of the rest.  In other words, the piecewise decodability effective masks the slightly larger number of communication rounds as far as the response time is concerned.}

\begin{comment}
==============================

The pseudocode of set reconciliation operations in each round is shown as follows:

\IncMargin{1em}
\begin{algorithm}
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
\Input{$A$ and $B^{(in)}$}
\Input{Set of reconciled distinct elements $D^{(in)}$}
\Output{$B^{(out)}$}
\Output{Set of reconciled distinct elements $D^{(out)}$}

% Hash-partition $A^{(in)}$, $B^{(in)}$ into $\{A^{(in)}_i\}_{i=1}^n$, $\{B^{(in)}_i\}_{i=1}^n$ (\autoref{sec:hash_partition})\label{step:hash_partition}\;

% Encode $\{A^{(in)}_i\}_{i=1}^n$, $\{B^{(in)}_i\}_{i=1}^n$ into parity bitmaps (\autoref{sec:parity_bitmap_encoding})\;


% Find those subset pairs (denoted them as $(A^{(in)}_{i_1}, B^{(in)}_{i_1}), ...,(A^{(in)}_{i_k}, B^{(in)}_{i_k})$) that parity bits differ (\autoref{sec:BCH_code})\;

Run single-round PBS on $A$ and $B^{(in)}$ to obtain the (partial) set difference $\mathcal{D}$\label{step:reconcile} \;

$D^{(out)} \leftarrow D^{(in)}\bigcup \mathcal{D}$\label{step:updated}\;

$B^{(out)} \leftarrow B^{(in)}\Delta\mathcal{D}$\label{step:updateb}\;

Check whether the set reconciliation is complete by comparing $A$ to $B^{(out)}$ (via CRC)\label{step:termination}\;

\caption{Set reconciliation operations of PBS in each round} \label{proto:multirounds}
\end{algorithm}\DecMargin{1em}

In \autoref{proto:multirounds}, the output $B^{(out)}$ in the $r^{th}$ round is the input $B^{(in)}$ in the $(r+1)^{th}$ round. $D^{(in)}$ and $D^{(out)}$ have the same relationship, and they denote the set of reconciled distinct elements before and after a round. $B^{(in)}$ and $D^{(in)}$ are initialized as $B$ and $\emptyset$ respectively. We omit the currect number of round $r$ in \autoref{proto:multirounds}, since the operations in different rounds are exactly the same. Due to the same reason, we only elaborate the operations in the first round: First, Alice and Bob reconcile $A$ and $B^{(in)}$ $(=B)$ using single-round PBS and Bob obtains the (partial) set difference $\mathcal{D}$ (\autoref{step:reconcile}); Second, Bob updates the set of reconciled distinct elements by merging it with $\mathcal{D}$ (\autoref{step:updated}); Third, Bob updates $B^{(in)}$ $(=B)$ to $B^{(out)}$ as \autoref{step:updateb} shows, such that (1) The reconciled distinct elements in $\mathcal{D}$ that are contained in $A\Delta B^{(in)}$ are not longer contained in $A\Delta B^{(out)}$; and (2) The distinct elements that are not successfully reconciled remain in $A\Delta B^{(out)}$ and can be reconciled in later rounds; Finally, we check whether all distinct elements are reconciled. Note that if it is true, $B^{(out)}$ should be the same as $A$ and multi-round PBS should terminate. We use a $32$-bit CRC (Cyclic Reduncancy Check) to check if $B^{(out)}=A$ in our evaluation. {\bf To achieve higher confidence, we can certainly use longer CRC (e.g., 64-bit). }

{\bf Remarks:}

(1) In each round, hash-partition in \autoref{sec:hash_partition} uses different hash functions, so that the remaining distinct elements from the last round will be hashed into different subset pairs with high probability;

(2) A straightforward approach to discard reconciled distinct elements is to remove them from both $A$ and $B$. This approach however incurs additional communication overhead to update $A$, since only Bob learns the partial set difference in \autoref{step:reconcile}. Therefore, we use the approach in \autoref{step:updateb} that only updates $B$. It has another benefit in \autoref{step:termination}, which only needs to transmit the CRC of $A$ from Alice to Bob in the first round. In the later rounds, \autoref{step:termination} can be checked locally by Bob and does not require any additional communication overhead;

(3) As we explained in \autoref{sec:reconcile_by_trivial}, the communication overhead in each round is proportional to the number of remaining distinct elements, which decreases exponentially as the number of round increase (i.e., the first round reconciles $90\%$ of distinct elements, the second round reconciles $90\%$ of the remaining $10\%$ distinct elements, etc.). So the majority of the communication overhead (i.e., $\approx 90\%$) is in the first round. Therefore, we do not bother to optimize parameters (i.e., smaller $n$) in later rounds to save tiny communication overhead, even though remaining distinct elements become fewer and can be reconciled using smaller $n$;

(4) One termination condition of Multi-round PBS is $B^{(out)}=A$, which refers that all distinct elements are reconciled. In most applications, a high percentage of reconciliation (e.g., $>99\%$ distinct elements are reconciled) is good enough. Therefore, we add another termination condition of the maximum number of rounds (denoted as $r$). The larger $r$ is, the higher percentage distinct elements will be reconciled, and the smaller $n$ is required. How to set parameters (e.g., $n$) based on $r$ will be elaborated in \autoref{sec:parameter_settings};

(5) Multi-round means multiple round-trip delays. {\bf Thanks for the piecewise decodability of PBS, in almost all practical application scenarios, this tradeoff does not lead to longer response time because the reconciliation of objects identified by the successfully decodable codewords, which constitute the vast majority of all codewords, can run in parallel with the transmissions and decodings of the rest.  In other words, the piecewise decodability effective masks the slightly larger number of communication rounds as far as the response time is concerned.}

==============================

\end{comment}

% (3) Readers may wonder in the later rounds, most distinct elements should be reconciled, and the rest distinct elements could be reconciled using degraded parameters (i.e., smaller $n$ and $t$). In fact, degrade parameters in later rounds cannot save much communication overhead, since the majority of it is spent in the first round (i.e., $>90\%$). Therefore, we use the same parameters (i.e., $n,t$) among all rounds in multi-rounds PBS;

% (4) The number of remaining distinct elements decreases exponentially as the number of round increase (i.e., the first round reconciles $90\%$ of distinct elements, the second round reconciles $90\%$ of the remaining $10\%$ distinct elements, etc.). 
% (4) The termination condition of Multi-rounds PBS is $B^{(out)}=A$ to reconcile all distinct elements. In some applications,  


% The output $B^{(out)}$ in the $r^{th}$ round is the input $B^{(in)}$ in the $(r+1)^{th}$ round. $D^{(in)}$ and $D^{(out)}$ are similarly defined. $B^{(in)}$ and $D^{(in)}$ are initialized as $B$ and $\emptyset$ respectively. Since and $D$ are updated in each round, so we use $B^{(in)}$ to denote the input and $B^{(out)}$ to denote the output respectively.  Specifically, in the first round, we initialize $B^{(in)}$ and $D^{(in)}$ as $B$ and $\emptyset$ respectively. we first use the single-round scheme 

% Then we run our (single-round) scheme on the updated two sets (i.e., after removing reconciled distinct elements) using a different (independent) hash-partition function from previous rounds, so that the rest distinct elements are hashed into different subset pairs (i.e., the ideal case) with high probability. At the end of each round, we check whether the set reconciliation is complete (i.e., all distinct elements are found) by computing the bitwise \code{XOR} of the remaining elements in $A$ and $B$ 
 

% This {\bf multi-rounds} scheme can significantly increase the success probability (i.e., the probability that all distinct elements are reconciled). Readers may wonder in the later rounds, most distinct elements should be reconciled, and the rest distinct elements could be reconciled using degraded parameters (i.e., smaller $n$ and $t$). In fact, degrade parameters in later rounds cannot save much communication overhead, since the majority of it is spent in the first round (i.e., $>90\%$). Therefore, we use the same parameters (i.e., $n,t$) among all rounds in our evaluation. 
% %The tradeoff between the number of rounds and the communication overhead per rounds will be elaborated in \autoref{sec:tail_bound}. In our evaluation, $r=2,3$ rounds are enough to achieve an extremely high success probability. 

% Readers may think the cost (i.e., communication overhead and the computational complexity) of this multi-rounds scheme is proportional to the number of rounds (denoted as $r$) and increases linearly with $r$. In fact, the cost of each round is roughly proportional to the number of remaining distinct elements, which decreases exponentially as $r$ increases (i.e., the first round reconciles $99\%$ of distinct elements, the second round reconciles $99\%$ of the remaining $1\%$ distinct elements, etc.). So the cost of this multi-rounds scheme is only slightly larger than that of the single-round scheme. Furthermore, as we explained in \autoref{sec:intro}, {\bf from intro thanks for the piecewise decodability of our solution, in almost all practical application scenarios, this tradeoff does not lead to longer response time because the reconciliation of objects identified by the successfully decodable codewords, which constitute the vast majority of all codewords, can run in parallel with the transmissions and decodings of the rest.  In other words, the piecewise decodability effective masks the slightly larger number of communication rounds as far as the response time is concerned.} 

\begin{comment}

\subsection{Baseline Scheme}\label{subsec:protocol1} 

Note that the set difference $A\Delta B$ can contain more than 1 elements (i.e., $d>1$), and \autoref{alg:trivial_case} cannot reconcile $A$ and $B$ directly in this case. Therefore, we propose a baseline scheme building upon~\autoref{alg:trivial_case} that also works when $d>1$: First, we partition the element universe $\mathcal{U}$ into $n$ sub-universes $\mathcal{U}_1, \mathcal{U}_2, \cdots, \mathcal{U}_n$. Denote $A_i \triangleq A\bigcap \mathcal{U}_i$ and $B_i \triangleq B\bigcap \mathcal{U}_i$ for $i=1,2,\cdots,n$. Then $\{A_i\}_{i=1}^n$ and $\{B_i\}_{i=1}^n$ are partitions of $A$ and $B$ respectively. Furthermore, $\Phi\triangleq\{A_i\Delta B_i\}_{i=1}^n$ is a partition of $A\Delta B$. 

Assume the {\bf ideal case} happens, in which each subset pair $(A_i, B_i)$ contains at most one distinct element ({\it i.e.,} $|A_i\Delta B_i|\!\leq\!1$), we use \autoref{alg:trivial_case} to reconcile each subset pair and obtain $A_i\Delta B_i$ for $i=1,2,\cdots,n$. The overall set difference $A\Delta B$ is simply their union $\bigcup_{i=1}^n \big{(}A_i\Delta B_i\big{)}$. 

In the first step of the baseline scheme, we can use a hash function $h(\cdot): \mathcal{U}\rightarrow \{1,2,\cdots,n\}$ to partition the universe $\mathcal{U}$ into $n$ sub-universes: $\mathcal{U}_i=\{s\mid s\in \mathcal{U} \mbox{ and } h(s)=i\}$ for $\forall i=1,2,\cdots,n$. And the hash function $h(\cdot)$ can be predetermined between Alice and Bob and does not require additional communication cost.

This hash-partition can be modeled as a {\it balls-into-bins problem}, in which the distinct elements are viewed as balls and the subset pairs are viewed as bins. The hash-parition basically throws (hashes) $d$ balls (distinct elements) uniformly and randomly into $n$ bins (subset pairs). The aforementioned ideal case in this context becomes, after throwing $d$ balls uniformly and randomly into $n$ bins, each bin receives at most 1 ball (i.e., $d$ nonempty bins have 1 ball in each and the rest $n-d$ bins are empty). {\bf It may remind readers about the Birthday problem. And the ideal case can be analogous to the case that no people share the same birthday.} The ideal case happens with a probability of $p=\frac{n\,!}{(n-d)\,!n^d}\!=\!\prod_{k=1}^{d - 1}(1 - \frac{k}{n})\!\approx\! e^{-\frac{d(d-1)}{2n}}$ when $d\!\ll\!n$. In other words, $n$ must be $\Omega(d^2)$ to ensure the ideal case happens with a nontrivial probability.  Note that the communication overhead of the baseline scheme is proportional to $n$, as each subset pair requires communication of a bitwise \code{XOR} in \autoref{alg:trivial_case}. So this communication overhead increases at least quadratically as $d$ increases. 

In fact, this communication overhead can be significantly reduced: In the ideal case, $n-d$ out of $n$ subset pairs are identical ones, and only $d (\ll n)$ out of $n$ subset pairs contain distinct elements (one distinct element in each of the $d$ subset pairs) and need to be reconciled. If we can identify these $d$ subset pairs (with a tiny additional communication overhead) and only reconcile them, the overall communication overhead will be significantly reduced from $\Omega(d^2)$ to $O(d)$. Based on this intuition, we propose our scheme in \autoref{sucsec:our-scheme}, which uses Parity Bitmap Sketch (PBS) and Error Correction Coding (ECC) to identify those subset pairs with a tiny additional communication overhead. 

Note that the ideal case does not always happen. However, we can ensure that the ideal case happens with high probability by properly selecting $n$ based on $d$ (i.e., $n=\Omega(d^2)$). Furthermore, as we will describe in \autoref{subsec:nonideal}, even if the ideal case does not happen (i.e., some distinct elements are hashed into the same subset pair), most of the distinct elements should be distributed into different subset pairs and therefore can be reconciled. So the baseline scheme, even cannot reconcile all of the distinct elements, can still reconcile the majority of them. Based on this property, we will extend our scheme from single-round to multi-rounds in \autoref{subsec:nonideal} to further increase the probability of reconciling all distinct elements. 

For general cases ({\it i.e.,} $t=|A\Delta B|$ is an arbitrary number), we have a straightforward strawman scheme building upon~\autoref{alg:trivial_case}, which works as follows: First, Alice and Bob choose some hash function $h(s): \mathcal{U} \rightarrow \{0,1,\cdots,2^{32}-1\}$ to partition $A$ and $B$ into $m$ subsets $A_1,A_2,\cdots,A_m$ and $B_1,B_2,\cdots,B_m$ respectively:

\begin{align}
s\in A_i & \mbox{ iff } s\in A \mbox{ and } h(s)=i\!\mod m, \nonu{}mber\\
s\in B_i & \mbox{ iff } s\in B \mbox{ and } h(s)=i\!\mod m. \nonumber
\end{align} 

{\bf call a subset pair -> partition?} Since Alice and Bob use the same hash function for partition, common elements (i.e., elements in $A\cap B$) are always hashed into the same subset pair $(A_i, B_i)$. And the set difference of each subset pair only contains distinct elements (i.e., elements in $A\Delta B$): $A_i\Delta B_i \subset A\Delta B$. In the ideal case, with a sufficient large $m$, each subset pair $(A_i, B_i)$ contains at most one distinct element ({\it i.e.,} $|A_i\Delta B_i|\!\leq\!1$). Then \autoref{alg:trivial_case} can reconcile each subset pair and obtain $A_i\Delta B_i$ for $i=1,2,\cdots,m$. The overall set difference $A\Delta B$ is simply their union $\bigcup_{i=1}^m \big{(}A_i\Delta B_i\big{)}$. The selection of hash function $h(s)$ can be predetermined between Alice and Bob and it does not require additional communication cost.

%To make sure Alice and Bob use the same hash function for partition, we let them pre-agree on some universal hash family (e.g., \code{xxHash}~\cite{Collet_xxHashExtremelyfast_}) and a common selection order, and each time they choose a hash function from the family in the same order. Note that we can also let Alice generates a hash function and send it to Bob. The hash function that Alice and Bob choose for partition can be either generated by 

This hash-partition is in nature a {\it balls-into-bins model}. We can view the distinct elements as balls and the subset pairs as bins. The hash-parition basically throws (hashes) $t$ balls (distinct elements) uniformly and randomly into $m$ bins (subset pairs). The aforementioned ideal case in this context is, with a sufficient large number of bins, each bin receives at most 1 ball. The strawman scheme works correctly if and only if the ideal case happens, which has a probability of $\frac{m\,!}{(m-t)\,!m^t}\!=\!\prod_{k=1}^{t - 1}(1 - \frac{k}{m})\!\approx\! e^{-\frac{t(t-1)}{2m}}$. In other words, to ensure the strawman scheme works correctly with a probability of $p$, it roughly requires $m \!=\!\lceil \frac{t(t-1)}{-2\ln p}\rceil$ subset pairs. 

Note that the communication overhead of this strawman scheme is proportional to the number of subset pairs $m$, as each subset pair requires communication of an \code{XOR} sum in \autoref{alg:trivial_case} during the reconciliation. When $t$ is small, a small communication cost can guarantee that the strawman scheme works correctly with high probability. For instance, when $t=5$, $m=95$ subset pairs are sufficient for the strawman scheme to work correctly with a probability of $90\%$. However, when $t$ is relatively large, it requires a huge communication cost to ensure the strawman scheme works correctly. For instance, when $t=1,000$, it requires $m=4,740,865$ subset pairs to guarantee a success probability of $90\%$. 

In fact, the majority of subset pairs are identical ones and do not need to reconcile. And only a small portion of them contain distinct elements. If we can identify those subset pairs that contain distinct elements and only reconcile them, the communication cost could be significantly reduced. Our scheme is based on this intuition and uses parity bitmap sketch and BCH code to identify the subset pairs, which we will elaborate in \autoref{sucsec:our-scheme}. 

%To distribute balls as uniformly as possible and maximize the probability of the ideal case, we choose a uniform hashing function $h$ that throws balls uniformly and randomly into bins: $$\mathbb{P}[h(s)=i]=\frac{1}{m} \mbox{ for } \forall i=1,2,\cdots,m, \forall s\in U$$.

%Note that the probability of the ideal case is $\frac{m\,!}{(m-t)\,!m^t}\!=\!\prod_{k=1}^{t - 1}(1 - \frac{k}{m})\!\approx\! e^{-\frac{t(t-1)}{2m}}$. Hence, at least $\lceil \frac{t(t-1)}{-2\ln p}\rceil$ bins are required to ensure that this probability is at least $p$. In other words, to ensure that the ideal case happens with a probability of $p$, the strawman scheme roughly requires $m \!=\!\lceil \frac{t(t-1)}{-2\ln p}\rceil$. For example, suppose $t\!=\!$\num{1000}, %and $p\!=\!0.01$, this strawman scheme roughly requires $m\!=\!$\num{720626} bins (partitions) to ensure that $|A_i\Delta B_i|\!\leq\!1$ (for any $i=1,2,\cdots,m$) holds with probability $50\%$.  

% A straightforward strawman scheme building upon~\autoref{alg:trivial_case} 
% to reconcile two sets $A$ and $B$ in general 
% ({\it i.e.,} $|A\Delta B|$ is an arbitrary number) is the following: 
% Uniformly randomly partition $A$ and $B$ into $m$ subsets ($A_1,A_2,\cdots,A_m$ 
% and $B_1,B_2,\cdots,B_m$) so that the set difference 
% $A_i\Delta B_i$ of each subset pair $(A_i, B_i)$ contains at most one element 
% ({\it i.e.,} $|A_i\Delta B_i|\!\leq\!1$) {\it w.h.p.} ({\it i.e.,} with high probability), 
% and then reconcile each subset pair with~\autoref{alg:trivial_case}. 

% Now let us analyze this strawman scheme using the {\it balls-into-bins model}. 
% Assume that sets $A$ and $B$ have $t$ elements in their set difference, {\it i.e.,} $|A\Delta B|\!=\!t$. 
% These $t$ elements can be viewed as $t$ balls and the $m$ partitions (subset pairs) can be viewed as 
% $m$ bins. The random partition process in this strawman scheme can be modeled as throwing 
% $t$ balls into $m$ bins in the following manner: Each ball goes into a 
% uniformly random bin and independently of other balls. %so that each bin contains at most one ball, {\it w.h.p.}  
% The probability that each bin contains at most one ball is  
% $\frac{m\,!}{(m-t)\,!m^t}\!=\!\prod_{k=1}^{t - 1}(1 - \frac{k}{m})\!\approx\! e^{-\frac{t(t-1)}{2m}}$. 
% Hence, at least $\lceil \frac{t(t-1)}{-2\ln p}\rceil$ bins are required 
% to ensure that this probability is at least $p$. In other words, to ensure 
% that each bin contains at most one ball with a probability of $p$, 
% the strawman scheme roughly requires $m \!=\!\lceil \frac{t(t-1)}{-2\ln p}\rceil$. 
% For example, suppose $t\!=\!$\num{1000}, %and $p\!=\!0.01$, 
% this scheme roughly requires $m\!=\!$\num{108469} bins (partitions) to 
% ensure that $|A_i\Delta B_i|\!\leq\!1$ (for any $i=1,2,\cdots,m$) holds with probability $0.01$.  

% We note that the communication overhead of this strawman scheme is proportional to 
% $m$ ($\!\gg\! t$), as each partition (subset pair) requires communication of an \code{XOR} sum during the reconciliation. 
% This communication overhead is much higher than that of the optimal scheme, which only requires 
% to exchange the elements in the set difference (assuming an oracle tells it which elements belong to 
% the set difference), {\it i.e.,} proportional to $t$. In the example above, assuming each element takes 4 bytes, 
% the communication overhead of the strawman scheme is $4m$ bytes ($\!\approx\! \num{423.71}\,$KB) to ensure 
% a success rate of only 0.01 ({\it i.e.,} with a probability of $0.0.1$, all elements in 
% the set difference are successfully reconciled), 
% which is approximately 2 orders of magnitude higher than $4t$ bytes ($\!=\!\num{3.90}\,$KB), the communication 
% overhead of the optimal scheme. 

\subsection{Our Scheme: The Preliminary Version}\label{sucsec:our-scheme}

Like the baseline scheme, our scheme also hash-partitions the two sets $A$ and $B$ into $n$ subset pairs. The difference is, instead of reconciling all subset pairs using \autoref{alg:trivial_case}, our scheme identifies the subset pairs that contains distinct elements and only reconciles them. Since the hash-partition and set reconciliation on each subset pair using \autoref{alg:trivial_case} have been described in \autoref{subsec:protocol1}, we only elaborate how to identify the subset pairs that contain distinct elements in this section. 

The general idea of identification is very simple: First, we {\bf encode} each subset into $1$ bit, such that in the ideal case, for $\forall i=1,2,\cdots,n$:

\begin{itemize}
	\item The codewords (bits) of $A_i$ and $B_i$ are different if and only if subset pair $(A_i, B_i)$ contains $1$ distinct element;
	\item The codewords (bits) of $A_i$ and $B_i$ are the same if and only if subset pair $(A_i, B_i)$ contains no distinct element;
\end{itemize}

Second, we {\bf compare} the codewords of each subset pair. And the subset pairs that contain distinct elements are the ones with different codewords (bits). We will describe the two steps in details in \autoref{sec:parity_bitmap_encoding} and \autoref{sec:BCH_code} respectively.

\subsubsection{Parity Bitmap Encoding}\label{sec:parity_bitmap_encoding}

In our scheme, we use {\it parity encoding} to encode each subset into a parity bit. More specific, it encodes a subset as ``1'' if it contains odd number of elements, and as ``0'' otherwise. And it satisfies the aforementioned requirements in the ideal case:

\begin{itemize}
	\item If subset pair $(A_i, B_i)$ contains $1$ distinct element, the corresponding two subsets $A_i$ and $B_i$ differ exactly one element, which implies that $||A_i|\!-\!|B_i||\!=\!1$. Hence, if $|A_i|$ ({\it i.e.,} number of elements in $A_i$) is odd (or even), then $|B_i|$ must be even (or odd). And the parity bits of $A_i$ and $B_i$ will be different;
	\item If subset pair $(A_i, B_i)$ contains no distinct element, the corresponding two subsets $A_i$ and $B_i$ should be the same and therefore contain the same number of elements. Hence, if $|A_i|$ is odd (or even), then $|B_i|$ must be odd (or even). And the parity bits of $A_i$ and $B_i$ will be the same;
\end{itemize}

Using parity encoding, the $n$ subsets of $A$ are encoded as a bit string $A[1..n]$ in $\{0,1\}^n$, 
where the $i$-th bit $A[i]$ in $A[1..n]$ corresponds to the parity encoding bit of $A_i$. Similarly, the $n$ subsets of $B$ are similarly 
encoded as a bit string $B[1..n]$. We call $A[1..n]$ ($B[1..n]$) the {\it parity bitmap} of $\{A_i\}_{i=1}^n$ ($\{B_i\}_{i=1}^n$). In the ideal case, $A[1..n]$ and $B[1..n]$ differ at $d$ different bit-positions, which corresponds to the $d$ subset pairs that contain distinct elements. And our scheme only reconciles those subset pairs that the parity bits are different. We will describe the nonideal case (i.e., some subset pair contains more than 1 distinct elements) in \autoref{subsec:nonideal}.

\subsubsection{Parity Bitmap Comparison Using BCH Code}\label{sec:BCH_code}

A straightforward approach to compare the parity bitmaps is to let Bob send the complete parity bitmap $B[1..n]$ to Alice, then Alice compares $A[1..n]$ with $B[1..n]$ locally. This approach has a communication overhead of $n$ bits, which is unnecessarily high. As we discussed in~\autoref{subsec:protocol0}, $d$ is usually much smaller than $n$. It means $A[1..n]$ and $B[1..n]$ differ only at a tiny portion of bits. Therefore, we can view $A[1..n]$ as a corrupted message of $B[1..n]$ with $d$ corrupted bits, and the bit-positions of the $d$ corrupted bits basically correspond to the $d$ subset pairs that contain distinct elements. The detection of corrupted bits, on the other hand, can be solved by Error-Correction Code (ECC)~\cite{Lin_ErrorControlCoding_1983}. And our scheme uses BCH code~\cite{Lint_IntroductionCodingTheory_1998} to encode the parity bitmap and detect the $d$ corrupted bits.

More specific, after the parity bitmap encoding, Bob uses a $d$-error-correcting systematic BCH code to encode $B[1..n]$ into an $n+d\log n$ codeword, in which the first $n$ bits are $B[1..n]$ (property of systematic BCH code). Then Bob sends the rest $d\log n$ bits, which we denote as {\it parity bitmap sketch (PBS)}, to Alice. Upon the received PBS and $A[1..n]$ (corrupted message), Alice uses the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} to detect the $d$ corrupted bits in $A[1..n]$. The communication overhead of this approach is $d\log n$ bits (i.e., length of PBS), which is much smaller than that of the straightforward approach ($n$ bits, when $d\!\ll\!n$). On the other hand, the computational complexity of the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} is $O(d^2\log^2 n)$. 

\subsubsection{Exceptional Handling and Multi-rounds}\label{subsec:nonideal}

As we described in \autoref{subsec:protocol1}, the ideal case does not always happen, which means some subset pair may contain more than 1 distinct elements and cannot be successfully reconciled by \autoref{alg:trivial_case}. Due to the parity encoding, we can classify such subset pair into the following two scenarios:

\begin{itemize}
    \item Scenario 1: If a subset pair $(A_i, B_i)$ contains even number ($\geq 2$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be the same and our scheme will not reconcile the subset pair. Hence, the distinct elements in the subset pair will not be reconciled;
    \item Scenario 2: If a subset pair $(A_i, B_i)$ contains odd number ($\geq 3$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be different and our scheme will reconcile the subset pair using \autoref{alg:trivial_case}. However, as we described in \autoref{subsec:protocol0}, when a subset pair contains more than 1 distinct elements, \autoref{alg:trivial_case} will output the bitwise \code{XOR} of them as the `distinct element', which is not a real distinct element with high probability;
\end{itemize}

In both scenarios, the distinct elements in the subset pair cannot be reconciled. Even worse, in the second scenario, a false-positive could happen (i.e., the output of \autoref{subsec:protocol0} is not a real distinct element). However, as we will analyze in \autoref{sec:tail_bound} and show in {\bf the evaluation section}, the second scenario barely happens both theoretically and empirically. To further reduce the chance of false-positives, we add a verification step at the end of \autoref{subsec:protocol0} to check whether the output of \autoref{subsec:protocol0} $s$ is a real distinct element or not. The verification step works as follows: Given the output $s$ of subset pair $(A_i,B_i)$, if $s\in\mathcal{U}_i$ (i.e., $h(s)=i$), we consider $s$ as a real distinct element; Otherwise, we consider $s$ as an incorrect output and discard it. 

Note that if $s$ is a real distinct element of $(A_i,B_i)$, $s$ must be in sub-universe $\mathcal{U}_i$. However, if $s$ is the bitwise \code{XOR} of the distinct elements in $(A_i,B_i)$ (i.e., the second scenario happens), $s$ could be in any sub-universe other than $\mathcal{U}_i$. In fact, if we assume the hash-partition described in \autoref{subsec:protocol1} hashes the elements of $\mathcal{U}$ uniformly, independently, and randomly into $n$ sub-universes, the output $s$ in the second scenario will be in a different sub-universe $\mathcal{U}_j (j\neq i)$ with a high probability of $1-\frac{1}{n}$. Hence, this verfication step can reduce the chance of false-positives by a factor of $\frac{1}{n}$. 

Even if the ideal case does not happen, most of the distinct elements should be distributed into different subset pairs and therefore can be reconciled. So our scheme, even cannot reconcile all of the distinct elements, can still reconcile the majority of them (piecewise decodability). To reconcile the rest distinct elements, we can just run our scheme for another round under a different hash-partition function, so on so force. This {\bf multi-rounds} scheme can significantly increase the success probability (i.e., the probability that all distinct elements are reconciled). Readers may wonder in the later rounds, most distinct elements should be reconciled, and the remaining could be reconciled using degraded parameters (i.e., smaller $n$ and $t$). In fact, degrade parameters in later rounds cannot save much communication overhead, since the majority of it is spent in the first round (i.e., $>90\%$). Therefore, we use the same parameters (i.e., $n,t$) among all rounds in our evaluation.
%The tradeoff between the number of rounds and the communication overhead per rounds will be elaborated in \autoref{sec:tail_bound}. In our evaluation, $r=2,3$ rounds are enough to achieve an extremely high success probability. 

Readers may think the cost (i.e., communication overhead and the computational complexity) of this multi-rounds scheme is proportional to the number of rounds (denoted as $r$) and increases linearly with $r$. In fact, the cost of each round is roughly proportional to the number of remaining distinct elements, which decreases exponentially as $r$ increases (i.e., the first round reconciles $99\%$ of distinct elements, the second round reconciles $99\%$ of the remaining $1\%$ distinct elements, etc.). So the cost of this multi-rounds scheme is only slightly larger than that of the single-round scheme. Furthermore, as we explained in \autoref{sec:intro}, {\bf from intro thanks for the piecewise decodability of our solution, in almost all practical application scenarios, this tradeoff does not lead to longer response time because the reconciliation of objects identified by the successfully decodable codewords, which constitute the vast majority of all codewords, can run in parallel with the transmissions and decodings of the rest.  In other words, the piecewise decodability effective masks the slightly larger number of communication rounds as far as the response time is concerned.} 

\end{comment}

\section{PBS: When $d$ is large}\label{subsec:protocol2}

Note that the BCH decoding computational complexity is $O(d^2)$ of finite field operations in GF($2^{8}$) using the state-of-the-art decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019}, which is too expensive for large $d$. To overcome this drawback, we first hash-partition sets $A$ and $B$ each into $d/\delta$ subsets (which we call {\it groups} to distinguish from subsets), just like what we did in \autoref{sec:hash_partition}, for some small integer $\delta$ (say $5$) and reconcile each of the group pairs by the PBS we described in \autoref{sec:scheme}. After the partition, each group has $\delta$ distinct elements on average. The BCH decoding computational complexity of each group pair can be considered as $O(1)$, since $\delta$ is a small number. As a result, the overall computational complexity of PBS is reduced from $O(d^2)$ to $O(d)$. 

To differentiate from the PBS described in \autoref{sec:scheme}, we refer it as PBS-basic in this section. Same as in \autoref{sec:scheme}, we assume that the number of distinct elements $d$ is precisely known. Even so, due to the randomness of hash-partition, $d_i$, the number of distinct elements in the $i^{th}$ group pair, is a Binomial random variable with mean of $\delta$ $(=d/g)$ for $i=1,2,...,g$, which cannot be precisely known without a huge amount of additional communication overhead. Hence, we can no longer set the error-correction capability of the BCH code for each group pair based on the exact number of distinct element in it, as we did in \autoref{sucsec:our-scheme}. Instead, we set a conservative error-correction capability $t$ (say $2.5\delta$) for all group pairs, which is sufficient for all group pairs (i.e., $t\geq d_i$ for $i=1,2,...,g$) with high probability. We will discuss the case that $d_i>t$ in \autoref{sec:BCH_exception}.



% ===============================
% To differentiate from the PBS described in \autoref{sucsec:our-scheme}, we refer it as PBS-basic in this section. Note that the BCH decoding computational complexity is $O(d^2\log ^2 n)$, which is $\Omega(d^2\log^2 d)$ when $n=\Omega(d^2)$, with the state-of-the-art decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019}. It is too large in PBS-basic for large $d$. To overcome this drawback and generalize PBS-basic for large $d$, we partition sets $A$ and $B$ each into $d/\delta$ subsets (which we call {\it groups} to distinguish from subsets) for some small integer $\delta$ (say $5$) and reconcile the $d/\delta$ group pairs respectively using PBS-basic. After this partition, each group has $\delta$ distinct elements on average. The BCH decoding computational complexity of each group pair can be considered as $O(1)$, since $\delta$ is a small number. As a result, the overall computational complexity of PBS is reduced from $O(d^2\log ^2 n)$ to $O(d)$. 

% % To differentiate from the PBS described in \autoref{sucsec:our-scheme}, we refer it as PBS-basic in this section. PBS-basic is not suitable for large $d$ for two reasons: First, its communication overhead is asymptotically $O(d\log n)\!=\!O(d\log d)$ (since $n=\Omega(d^2)$), which is not asymptotically optimal. Second, the decoding computational complexity is proportional to $d^2$ with the state-of-the-art decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} for BCH codes, which is too high when $d$ is large. To overcome these two drawbacks, we use a simple algorithmic trick to (1) reduce the communication overhead from $O(d\log d)$ to $d\log u \!+\! O(d)$; (2) reduce the decoding computational complexity from $O(d^2)$ to $O(d)$. 

% Now, we describe the generalized PBS in details: In the first step, we hash-partition $A$ and $B$ (by some hash function $h_1(\cdot)$) into $g$ group pairs, just like what we did in \autoref{sucsec:our-scheme}. The objective of this partition is however different: In \autoref{sucsec:our-scheme}, we aim to ensure each subset pair contains at most $1$ distinct element (i.e., the ideal case) with high probability; Here we aim to make each group pair contains roughly $\delta$ distinct elements for some small constant $\delta$ (say $5$) by setting $g=d/\delta$. 
% %To differentiate the $g$ subset pairs here from those in \autoref{sec:hash_partition}, we call them the $g$ {\bf groups} in the sequel. 
% In the second step, we just apply PBS-basic (described in \autoref{sucsec:our-scheme}) to reconcile each group pair and obtain the distinct elements. 
% ================================

% To differentiate from the PBS described in \autoref{sucsec:our-scheme}, we refer it as PBS-basic in this section. When $d$ is large (more than several), we hash-partition set $A$ and $B$ into groups, such that each group pair contains $\delta$ distinct elements on average for small $\delta$ (say $5$), as described in \autoref{sec:larged}. Then each group pair can be reconciled by PBS-basic.

% When describing the PBS-basic in \autoref{sucsec:our-scheme}, we assume that the number of distinct elements is precisely known. We set the error-correction capability of the BCH code (denoted as $t$) just enough to correct $d$ errors (i.e., $t=d$). However, due to the randomness of hash-partition, $d_i$, the number of distinct elements in the $i^{th}$ group pair, is a Binomial random variable $Binomial(d,1/g)$ with expectation of $\delta$ $(=d/g)$ for $i=1,2,...,g$, which cannot be precisely known without a huge amount of additional communication overhead. Hence, we can no longer set the error-correction capability of the BCH code for each group pair based on the exact number of distinct element in it, as we did in \autoref{sucsec:our-scheme}. Instead, we set a universal error-correction capability $t$ (say $2.5\delta$) for all group pairs, which is sufficient for all group pairs (i.e., $t\geq d_i$ for $i=1,2,...,g$) with high probability. We will discuss the case that $d_i>t$ in \autoref{sec:BCH_exception}.

%This assumption in general does not hold: 
% Let $d_i$ denote the number of distinct elements in Group $i$. Due to the property of hash-partition, each $d_i$ is a Binomial random variable $Binomial(d,1/g)$ with expectation of $\delta$ $(=d/g)$. Even if $d$ is precisely known, each $d_i$ is not. To ensure the error-correction capability $t$ is sufficient for each group (i.e., $d_i\leq t$) with high probability, we leave some safety margin for the randomness of $d_i$ and conservatively set $t$ roughly $2.5\delta$ (the factor $2.5$ varies depend on other parameters, which will be discussed in \autoref{sec:parameter_settings}), so that $Pr[d_i>t]$ is tiny. We will discuss the case that $d_i>t$ in \autoref{sec:BCH_exception}.

Note that the `safety margin' between $t$ and $\delta$ (i.e., the average number of distinct elements in a group pair) incurs additional communication overhead on transmitting BCH codeword: In the perfect scenario (i.e., $\{d_i\}_{i=1}^g$ is precisely known), the average communication overhead on transmitting BCH codeword per group pair is $\delta\log n$; On the other hand, when we set $t$ to be the error-correction capability for each group pair, then the average overhead becomes $t\log n$, which is roughly $2.5$ times of that in the perfect scenario (when $t$ is roughly $2.5\delta$). Readers may wonder if we can reduce this additional communication overhead by using some technique to estimate $\{d_i\}_{i=1}^g$ (e.g., ToW estimator in \autoref{subsec:ToW}), so that we can set the error-correction capability of each group more wisely and save some waste on the safety margin. However, to achieve that, the estimation on $\{d_i\}_{i=1}^g$ must be in extremely high precision (since $\{d_i\}_{i=1}^g$ are small numbers with mean of $\delta$), which requires a much higher communication overhead than the savings. Due to the same reason (i.e., estimate $\{d_i\}_{i=1}^g$ is costly), we set the number of subset pairs for each group pair to be all equal (denoted as $n$) based on $\delta$. The detail about how to set $n$ and $t$ will be elaborated in \autoref{sec:parameter_settings}. 

% Note that this safety margin incurs additional communication overhead on transmitting BCH codeword: In the perfect scenario (i.e., $\{d_i\}_{i=1}^g$ is precisely known), the average communication overhead on transmitting BCH codeword per group is $\delta\log n$; On the other hand, when we set $t$ to be the error-correction capability for each group, then the average overhead becomes $t\log n$, which is roughly $2.5$ times of that in the perfect scenario (when $t$ is roughly $2.5\delta$). Readers may wonder if we can reduce this additional communication overhead by using some technique to estimate $\{d_i\}_{i=1}^g$ (e.g., ToW estimator in \autoref{subsec:ToW}), so that we can set the error-correction capability of each group more wisely and save some waste on the safety margin. However, to achieve that, the estimation on $\{d_i\}_{i=1}^g$ must be in high precision, which requires a much higher communication overhead than the savings. 

\subsection{What if PinSketch also uses partitions?}

The same algorithmic trick (i.e., hash-partition two sets each into groups) can also be implemented in PinSketch~\cite{Dodis_PinSketch_2008} to reduce it computational complexity from $O(d^2\log^2 |\mathcal{U}|)$ to $O(d)$. However, it will encounter the same randomness problem and have to set up a safety margin on the error-correction capability. This safety margin will incur much more additional communication overhead on PinSketch than on our scheme: Considering the average communication overhead per group pair, the additional overhead caused by the safety margin is $(t-\delta)\log n$ in PBS and $(t-\delta)\log |\mathcal{U}|$ in PinSketch. The later is roughly $4$ times of the former under the default setting ($n=255, |\mathcal{U}|=2^{32}$). Note that the optimal communication overhead to reconcile $d$ distinct elements is $\delta\log |\mathcal{U}|$. Use the same example in \autoref{sec:intro}, when $\delta=5, n=255, u=2^{32}, t=2.5\delta$, the overhead of PinSketch using the algorithmic trick is $2.5$ times of the optimal, while that of PBS is $2.075$ times of the optimal (as we mentioned in \autoref{sec:intro_oursolution}). It means PBS could have a lower communication overhead than PinSketch if they both use the algorithmic trick. Furthermore, as the signiture width $\log |\mathcal{U}|$ increases, the advantage of PBS over PinSketch becomes more significant, which we will show in \autoref{subsec:mini-partition}.

% The same algorithmic trick can also be implemented in PinSketch~\cite{Dodis_PinSketch_2008} to reduce it computational complexity from $O(d^2)$ to $O(d)$. However, it will encounter the same randomness problem and have to set up a safety margin on the error-correction capability. This safety margin will incur much more communication overhead on PinSketch than on our scheme: Considering the average communication overhead per group, in our scheme, this overhead can be expressed as $t\log n+\delta\log n+\delta \log u+32$, in which $t\log n$ accounts for the BCH codeword, $\delta\log n$ accounts for the index of the subset pairs, $\delta \log u$ accounts for the bitwise \code{XOR} in \autoref{alg:trivial_case}, and $32$ accounts for the $32$-bit CRC in \autoref{proto:multirounds}. In PinSketch, this overhead increases from $O(\delta\log u)$ (optimal) to $O(t\log u)$ (PinSketch does not need to transmit bitwise \code{XOR}) if it uses the same algorithmic trick. Use the same example in \autoref{sec:intro}, when $\delta=5, n=255, u=2^{32}, t=2.5\delta$, the overhead of PinSketch using the trick is $2.5$ times of the optimal, while that of our scheme is $2.075$ times of the optimal (as we introduced in \autoref{sec:intro_oursolution}). That means our scheme has a lower communication overhead than PinSketch if they both use the algorithmic trick. Furthermore, as the signiture size $\log u$ increases, the advantage of our scheme over PinSketch becomes more significantly, which we will show in \autoref{subsec:mini-partition}.

% In PinSketch, each bit encodes only a single element in the universe, so the size of the bitmap is equal to the size of the universe.  
% For example, in the set reconciliation problem we usually assume each element is ``indexed" by a $32$-bit-long (hash) signature, so the universe contains a total of $2^{32}$ elements. In this case, the bitmap encoding for any set in PinSketch is $2^{32}$ bits long, and the Galois field involved in its BCH decoding is the ``$32$-bit-wide" $GF(2^{32})$.  In contrast, as explained earlier, in PBS 
% %since each bit encodes the oddness or evenness of the cardinality of a subset,   
% the size $n$ of a bitmap is dependent only on $d$, and not on the size of the universe or on the cardinality of the set the bitmap encodes.   For example, as shown in the example above, $n = 255$ is large enough for $d = 5$.  In this case, the BCH decoding operates in the much shorter
% ``8-bit-wide" $GF(2^{8})$.  This shorter ``width" alone in theory translates into roughly $16$ times shorter BCH decoding time, which as will be explained in~\ref{} grows quadratically with the ``width" of the underlying Galois field.  This shorter ``width" also implies four times shorter BCH codeword in PBS than in PinSketch, resulting in lower communication complexity as will be shown in~\autoref{}.

% Note that our scheme only takes 1 round trip delay to both identify the $d$ subset pairs and reconcile them: In the first half, Bob computes and sends PBS to Alice. Then Alice locally identifies the $d$ subset pairs and then initiates the reconciliation ({\it i.e.,} \autoref{alg:trivial_case}) for them, {\it i.e.,} computes the bitwise \code{XOR} of the corresponded $d$ subsets. In the second half, Alice sends the bitwise \code{XOR} of the $d$ subsets with their indexes to Bob. Then Bob can compute the set difference $A\Delta B$ locally.


% We can certainly use some communication-efficient technique to estimate $d_i$ (e.g., \autoref{subsec:ToW}). However, to obtain $d_i$ precisely will require a communication cost almost as large as to reconcile Group $i$. So instead of obtaining $d_i$ and set $c_i$ (i.e., the error-correction capability of Group $i$) equal to $d_i$, we leave the randomness of $d_i$ and set $c_i$ neither too conservative, nor too libertive in the following sense: (1) $c_i$ is not too big (conservative, i.e., $10\delta$) to make the total size of PBS unnecessarily large and incur too much extra communication overhead; (2) $c_i$ is not too small (libertive, i.e., $\delta$) to incur a high probability of insufficient decode capability, which can result in hefty penalties in the latter case of incorrect decoding (will be elaborated in \autoref{sec:BCH_exception}). In our scheme, we set $c_i$ to be $2-3$ times of $\delta$, which will be shown in \autoref{sec:tail_bound} that it is just enough to make the probability of decode failure very small. Meanwhile, we set the error-correction capability of each group ($c_1,c_2,...,c_k$) to be all equal and denote it as $c$. 

%Since the decoding capacity $t$ and the number of subset pairs for each group $n$ are both small constants independent of $d$, therefore, the communication overhead per group is $t\cdot\log n \!=\!O(1)$, which implies a total communication overhead of $O(d)$. Similarly, the total decoding computational complexity is also $O(d)$. 

% \subsection{Exception Handling}\label{sec:exceptions}

% \subsubsection{Exception Handling on Hash-Partition}\label{subsec:exception_hash_partition}

% As we have described in \autoref{sec:hash_partition}, the ideal case does not always happen, which means some subset pair may contain more than 1 distinct elements and cannot be successfully reconciled by \autoref{alg:trivial_case}. Due to the parity encoding, we can classify such subset pair into the following two scenarios:

% \begin{itemize}
%     \item Scenario 1: If a subset pair $(A_i, B_i)$ contains even number ($\geq 2$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be the same and our scheme will not reconcile the subset pair. Hence, the distinct elements in the subset pair will not be reconciled;
%     \item Scenario 2: If a subset pair $(A_i, B_i)$ contains odd number ($\geq 3$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be different and our scheme will reconcile the subset pair using \autoref{alg:trivial_case}. However, as we described in \autoref{subsec:protocol0}, when a subset pair contains more than 1 distinct elements, \autoref{alg:trivial_case} will output the bitwise \code{XOR} of them as the `distinct element', which is not a real distinct element with high probability;
% \end{itemize}

% In both scenarios, the distinct elements in the subset pair cannot be reconciled. Even worse, in the second scenario, a false-positive could happen (i.e., the output of \autoref{subsec:protocol0} is not a real distinct element). For example, if subset pair $(A_i, B_i)$ contains $3$ distinct elements $s_1, s_2, s_3$, then the output of \autoref{alg:trivial_case} is $\tilde{s}_4=s_1\oplus s_2\oplus s_3$, which is normally not a distinct element. The good thing is, the probability of the false-positive is extremely small for small $d$. For instance, if $d=5$ and $n=255$, the probability of the false-positive is $7.6\times 10^{-6}$, which is very small. To further reduce the chance of false-positives, we add a verification step at the end of \autoref{subsec:protocol0} to check whether the output of \autoref{subsec:protocol0} $s$ is a real distinct element or not. The verification step works as follows: Given the output $s$ of subset pair $(A_i,B_i)$, if $s\in\mathcal{U}_i$ (i.e., $h(s)=i$), we consider $s$ as a real distinct element; Otherwise, we consider $s$ as an incorrect output and discard it. 

% Note that if $s$ is a real distinct element of $(A_i,B_i)$, $s$ must be in sub-universe $\mathcal{U}_i$. However, if $s$ is the bitwise \code{XOR} of the distinct elements in $(A_i,B_i)$ (i.e., the second scenario happens), $s$ could be in any sub-universe other than $\mathcal{U}_i$. In fact, if we assume the hash-partition described in \autoref{sec:hash_partition} hashes the elements of $\mathcal{U}$ uniformly, independently, and randomly into $n$ sub-universes, the output $s$ in the second scenario will be in a different sub-universe $\mathcal{U}_j (j\neq i)$ with a high probability of $1-\frac{1}{n}$. Hence, this verfication method can further reduce the probability of false-positives by a factor of $\frac{1}{n}$. Use the same example (i.e., $d=5$, $n=255$), the probability is reduced from $7.6\times 10^{-6}$ to $3\times 10^{-8}$ by this verification method. 

% In some super critical cases (i.e., no false-positive is allowed), we can use a more powerful verification method to completely eliminate false-positives. That is, to check if the output $s$ exists in exactly one of the two sets (i.e., $s\in A\setminus B$ or $s\in B\setminus A$). To do so, Bob transmits $s$ along with an identification bit $\mathbb{1}_{\{s\in B\}}$ to Alice, then Alice checks if $s$ . This method verification costs $d(\log u+1)$ bits of additional communication overhead. In most applications, rigorously $0\%$ probability of false-positives is unnecessary and the probability of the former verification method is small enough, so we use the former verfication method in our evaluation. Based on our observation, the false-positive does not happen even once in our evaluation using the former verfication method.

\subsubsection{Exception Handling on BCH Decoding}\label{sec:BCH_exception}

The exceptions that happens within PBS-basic have been discussed and handled in \autoref{subsec:exception_hash_partition} and \autoref{sec:multi-rounds}. In this section, we only discuss the exceptions that the error-correction capability $t$ is insufficient for some group $i$. More specifically, when $d_i$ (i.e., the number of distinct elements in group $i$) is larger than the error-correction capability $t$, the BCH codewords of group $i$ differ at $d_i$ bit positions in the ideal case, which exceeds the error-correction capability $t$. If so, the BCH decoder cannot decode the bit errors correctly (\autoref{step:BCH_decode} in \autoref{alg:single_round_pbs}). This exception happens with a small probability in each group pair: For example, when $d=1000, g=200 (\delta=5), t=13$, the probability that this exception happens is only $6.7\times 10^{-4}$. 


and report a failure. 

To handle this type of exceptions, we use the same algorithm trick in \autoref{subsec:protocol2} to partition each problematic group into $3$ sub-groups and reconcile them respectively using PBS-basic. Note that $d_i$, if is not smaller, should be only slightly larger than $t$ with high probability. Hence, partitioning into $3$ sub-groups is enough to make sure each sub-group has no more than $t$ distinct elements. Then in the next round, each subgroup does not encounter this type of expections and can be reconciled by PBS-basic respectively. More specifically, we add a termination condition of \autoref{alg:3_way_partition} after \autoref{step:BCH_decode} in \autoref{alg:single_round_pbs}:

\begin{algorithm}
\caption{Termination condition when BCH decoding fails}
\label{alg:3_way_partition}

\If{BCH decoding fails\label{step:if1}}
{Hash-partition the group into $3$ sub-groups and do PBS for each of them in the next round; Break;}\label{step:term1} 

\end{algorithm}

% Back to the \autoref{proto:multirounds}, which shows the set reconciliation operations in each round of PBS-basic, this kind of exceptions only affect \autoref{step:reconcile} in \autoref{proto:multirounds}. Now this step needs to check whether BCH decoding is successful or not: If successful, all the operations remain the same; Else, we hash-partition the group ($A$ and $B$) into $3$ sub-groups and reconcile them respectively using \autoref{proto:multirounds}. 

Another type of exceptions that happens when $d_i>t$ is, the BCH decoder mistakes the decoding is successful and returns $t$ incorrectly decoded bit errors (i.e., subset pairs). The probability of this type of exceptions is very small. For instance, when $d=1000, \delta=5, t=13$ $(2.5\delta)$, $d_i>t$ happens with probability roughly $6.7\times 10^{-5}$, and the probability that the BCH decoder mistakes the decoding is successful when $d_i>t$ is in order of $10^{-7}$ \cite{kim1996undetected}. So the probability that this type of exceptions happens in each group is in order of $10^{-12}$. On the other hand, the impact of this type of exceptions is insignificant. Assume an incorrectly decoded bit error corresponds to a random subset pair, which could contain (1) no distinct element; (2) exactly $1$ distinct element; or (3) more than $1$ distinct elements. Reconcile the subset pair using \autoref{alg:trivial_case} could (1) get nothing and waste $\log |\mathcal{U}|$ bits of communication overhead; (2) get an actual distinct elements; or (3) trigger the exceptions that were discussed and handled in \autoref{subsec:exception_hash_partition}. 

% We handle this type of exceptions by the same method (i.e., hash-partition into $3$ sub-groups) as above. To detect them, on the other hand, is simple: Note that incorrect decoded bit errors correspond to the subset pairs that do not contain distinct elements. When we reconcile those subset pairs in \autoref{sec:reconcile_by_trivial}, the output (i.e., reconciled elements) will be $\mathbf{0}$, which is abnormal (since $\mathbf{0}\notin A\bigcup B$, as we described in \autoref{subsec:protocol0}). Hence, this type of exceptions happen if and only if one of the reconciled distinct elements is $\mathbf{0}$. 
%Hence, we consider BCH decoding is successful by two criteria: (1) the BCH decoder reports a successful decode; and (2) None of the reconciled elements is $\mathbf{0}$. 
========================
In fact, even if $d_i>t$, PBS-basic is still possible to reconcile group $i$ in some nonideal cases. For example, when $t=10$ and $d_i=11$, if the $11$ distinct elements are distributed in $10$ subset pairs, such that $1$ subset pair contains $2$ distinct elements and $9$ subset pairs contain $1$ distinct element in each, the two parity bitmaps differ at only $9$ bit positions. So BCH decoder is able to decode the later $9$ subset pairs and the corresponding $9$ distinct elements can be reconciled. In the second round, only $2$ distinct elements remain and BCH decoding certainly works. In this case, we do not need to partition the group into sub-groups, and this case does not trigger \autoref{alg:3_way_partition} in PBS. 
========================
% Instead, it will either (1) report a failure about exceeding the error-correction capability; or (2) mistake the decoding is successful and return incorrect decoded bit errors. 

% The second case happens with a very small probability (in order of $10^{-7}$ \cite{kim1996undetected}) and is very simple to detect : 

% The first case is easy to handle: We can simply adapt the same algorithmic trick to partition the group into smaller groups and reconcile them respectively. In our scheme, we set the number of smaller groups to be $3$, which is big enough because $d_i$, if not smaller, only slightly larger than $t$ with high probability. The second case on the other hand, although theoretically possible, happens with a very small probability when $d_i>t$ (in order of $10^{-7}$ \cite{kim1996undetected}). Besides, the probability of $d_i>t$ is also very small (e.g., when $t=15$ and $\delta=5$, this probability is about $2.3\times 10^{-4}$), so the overall probability of the second case, which is the multiplication of these two small numbers, is negligible (e.g., in order of $10^{-11}$).

% \subsection{Multi-rounds}

% Even if the ideal case does not happen, most of the distinct elements should be distributed into different subset pairs and therefore can be reconciled. So our scheme, even cannot reconcile all of the distinct elements, can still reconcile the majority of them (piecewise decodability). To reconcile the rest distinct elements, we can just run our scheme for multi-rounds under different hash-partition functions. For each round, our scheme works as follows: 

% \IncMargin{1em}
% \begin{algorithm}
% \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
% \Input{Two sets $A$ and $B$}
% \Input{Size of set difference $d$}
% \Input{The number of subset pairs $n$}
% \Input{BCH error-correction capability $t$}

% Hash-partition $A$ and $B$ into $n$ subset pairs $\{(A_i,B_i)\}_{i=1}^n$;

% \If{BCH decoding fails}
% 	Hash-partition $A$ and $B$ into $3$ subset pairs and reconcile them respectively in the next round\;
% \ElseIf{BCH decoding success}
	
% \Else{}

% $k \leftarrow \lceil \frac{t}{c}\rceil $\;

% Partition elements into $k$ subsets using~\autoref{alg:random-part}\;

% \For{$j = 0$ \KwTo $k-1$}{
%     Reconcile the $j$-th subset pair using the straw-man scheme with the BCH correcting capability $\tau$, number of smaller subsets $m$, and number of rounds $r$\;
% }

% \caption{PBS (per round)} \label{proto:II}
% \end{algorithm}\DecMargin{1em}

% This {\bf multi-rounds} scheme can significantly increase the success probability (i.e., the probability that all distinct elements are reconciled). Readers may wonder in the later rounds, most distinct elements should be reconciled, and the remaining could be reconciled using degraded parameters (i.e., smaller $n$ and $t$). In fact, degrade parameters in later rounds cannot save much communication overhead, since the majority of it is spent in the first round (i.e., $>90\%$). Therefore, we use the same parameters (i.e., $n,t$) among all rounds in our evaluation. 
% %The tradeoff between the number of rounds and the communication overhead per rounds will be elaborated in \autoref{sec:tail_bound}. In our evaluation, $r=2,3$ rounds are enough to achieve an extremely high success probability. 

% Readers may think the cost (i.e., communication overhead and the computational complexity) of this multi-rounds scheme is proportional to the number of rounds (denoted as $r$) and increases linearly with $r$. In fact, the cost of each round is roughly proportional to the number of remaining distinct elements, which decreases exponentially as $r$ increases (i.e., the first round reconciles $99\%$ of distinct elements, the second round reconciles $99\%$ of the remaining $1\%$ distinct elements, etc.). So the cost of this multi-rounds scheme is only slightly larger than that of the single-round scheme. Furthermore, as we explained in \autoref{sec:intro}, {\bf from intro thanks for the piecewise decodability of our solution, in almost all practical application scenarios, this tradeoff does not lead to longer response time because the reconciliation of objects identified by the successfully decodable codewords, which constitute the vast majority of all codewords, can run in parallel with the transmissions and decodings of the rest.  In other words, the piecewise decodability effective masks the slightly larger number of communication rounds as far as the response time is concerned.} 





\begin{comment}
\subsubsection{Random Partition}

\IncMargin{1em}
\begin{algorithm}
% \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
% \Input{Set $S$}
% \Input{The number of subsets $m$ for partition}
% \Output{Subsets $S_1, S_2, ..., S_m$}

% Generate hash function $h(\cdot)$ that maps each element into $\{1,2,...,m\}$;

\ForEach{$s \in S$}{
    $j \leftarrow h(s) \bmod m$\;    
    Insert $s$ into the $j$-th subset $S_j$\;
}

\caption{Partition using hash function $h(\cdot)$.} \label{alg:random-part}
\end{algorithm}\DecMargin{1em}

Like the strawman scheme, our scheme randomly partitions sets $A$ and $B$ into $m$ subsets. This random partition 
can be easily accomplished by using some hash function, $h(\cdot)$, and inserting each element $x$ into the subset 
corresponding to $h(x)$. \autoref{alg:random-part} presents the pseudo-code of this random partition using hash 
function $h(\cdot)$.  

% Unlike the strawman scheme, our scheme only reconciles those subset pairs that need to be reconciled, 
% because 



Like the strawman scheme, our scheme hash-partitions the two sets $A$ and $B$ into $m$ subset pairs $(A_i, B_i)$ for $i=1,2,\cdots,m$. 
We note that, among those $m$ bins (subset pairs), 
at most $t$ ($t\!\ll\!m$ as shown in our analysis in~\autoref{subsec:protocol1}) bins contain balls 
(elements belonging to the set difference), {\it i.e.,} requiring reconciliation.  
Motivated by this observation, we, therefore, propose to first detect those bins that 
contain balls and then only reconcile them. The detection is solved with a simple encoding approach that 
will be detailed in the next section.

\subsubsection{Detection before Reconciliation} 

In fact, identifying those non-empty bins is easy when each bin contains at most one ball. In this section, we assume that 
each bin after the random partition contains at most one ball, we will show later how to handle the cases when some 
bins contain more than one balls later in~\autoref{subsec:exceptions}. 

Given an arbitrary bin (say subset pair $(A_i, B_i)$) that contains one ball ({\it i.e.,} $A_i\Delta B_i$ contains exactly one element), 
the corresponding two subsets $A_i$ and $B_i$ differ exactly one element, which implies that 
$||A_i|\!-\!|B_i||\!=\!1$. Hence, if $|A_i|$ ({\it i.e.,} number of 
elements in $A_i$) is odd (or even), then $|B_i|$ must be even (or odd). In other words, the odevity of $|A_i|$ 
and $|B_i|$ are opposite. %differs if $|A_i\Delta B_i|\!=\!1$. 
Based on this property, we propose the {\it odevity encoding}: 
A subset is encoded as ``1'' if it contains odd number of elements, and as ``0'' otherwise. 
Using this odevity encoding, the $m$ subsets of $A$ can be encoded as a bit string $b_A$ in $\{0,1\}^m$, 
where the $i$-th bit in $b_A$ corresponds to the odevity encoding of $|A_i|$. Similarly, the $m$ subsets of $B$ can also 
be encoded as a bit string $b_B$. Clearly, $b_A$ and $b_B$ differ at $t$ different positions, or in other words, 
the Hamming distance of bit strings $b_A$ and $b_B$ is $t$. A straightforward approach is 
to let Alice send $b_A$ to Bob, and then Bob compares $b_B$ against $b_A$ to obtain those non-empty bins. 

This approach, however, has a communication overhead of $m$ bits, which is still unnecessarily high. As 
analyzed in~\autoref{subsec:protocol0}, $t$ is usually much smaller than $m$. 
That means $b_A$ and $b_B$ differ only at a tiny portion of bits. %have much more in common than differences. 
Therefore, if we view $b_B$ as a corrupted message of $b_A$ with $t$ corrupted bits, the detection of those $t$ bins can be converted to 
the detection of the positions of the $t$ corrupted bits. The latter can be solved using an Error-Correction Code (ECC)~\cite{Lin_ErrorControlCoding_1983} that can correct up to $t$ errors. In this work, we use the BCH code~\cite{Lint_IntroductionCodingTheory_1998}. 
More precisely, this ECC-based approach (with the BCH code) works as follows. 
Alice computes the parity bits for $b_A$ using a $t$-error-correcting BCH code with a block length of 
$(2^{\lceil \log m\rceil} -1)$ and sends the parity bits to Bob. Bob then decodes the positions of the $t$ corrupted bits 
using the BCH decoding algorithm with $b_B$ and those parity bits received from Alice. The communication overhead of 
this approach is roughly $t\lceil \log m\rceil$ ($=O(t\log t)$) bits. In the example above, this communication overhead is 
roughly $\num{17000}$ bits, which is approximately $6$ times lower 
than $m\!=\!\num{108469}$ bits, the communication overhead of the aforementioned straightforward approach. 

At first sight, it seems that the detection of non-empty bins and reconciliation of subsets in those bins require two rounds 
(or at least two round trip delays), {\it i.e.,} one round for detection and the other for reconciliation. In fact, 
it only requires one. After Bob receives the parity bits from Alice and decodes out those non-empty bins, it initiates 
the reconciliation ({\it i.e.,} \autoref{alg:trivial_case}) for each bin (subset pair) immediately, 
{\it i.e.,} sends the \code{XOR} sums of subsets in those bins together the indexes of those bins. 
After receiving those \code{XOR} sums and bin indexes, Alice can compute the set difference. 

% A naive way to combine the detection of non-empty bins and reconciliation of subset pairs in those bins is to first detect 
% those non-empty bins via one round of message exchanges between Alice and Bob and then to reconcile the corresponding 
% subset pairs in those bins with another round of message exchanges. This requires two rounds ({\it i.e.,} taking at least 
% two round trip delays). In fact, after Bob receives the parity bits from Alice and obtains those 

\subsubsection{Multiple Rounds}\label{sec:multiround}

{\bf This section was not clear enough. I need more time to think about and revise it.}


In the above section, we have assumed that each bin contains at most one ball. 
However, even with a sufficient large $m$, some bin might contain more than one balls though with tiny probability. 
We will show in~\autoref{subsec:exceptions}, how such rare events, {\it i.e.,} one bin contains more than one balls, 
can be easily detected.
To ensure our scheme can successfully reconcile all elements even when such rare events happen, 
we propose to use multiple rounds (of communication between Alice and Bob). More precisely, instead of 
selecting a prohibitively large $m$ to ensure that each bin contains at most one ball with a extremely high probability 
(say 0.99999), we select a reasonably large $m$ so that the communication overhead is not very high and very few bins contain 
more than one balls (or in other words, most bins contain at most one ball). Therefore, after running one round of 
our scheme, most elements in the set difference will be reconciled. Only those in the bins that contain more than one balls 
fail to be reconciled. For elements in the subsets corresponding to those bins, we run another round of our scheme. 
If some elements still fail to be reconcile, we can run one more round of our scheme. So on so forth,  
our scheme can keep running for more rounds until all elements are reconciled. 

With the same communication overhead, multiple rounds can significantly increase the success rate, 
{\it i.e.,} the probability that all elements in the set difference will be successfully reconciles, 
which will be elaborated in~\autoref{sec:tail_bound}. 

% % to be emphasized
% % say that too many rounds should be avoided (latency & communication overhead reduction is negligible when r is too large, 2 - 3 is good enough)
% % multiple rounds is not an issue when r is small

% We note that the number of rounds $r$, however, should not be large. On one hand, it results in large latency (at least $r$ round trip delays). 
% On the other hand, when $r$ is large, the reduction of communication overhead by the increase of $r$ gradually diminishes. 

We note that multiple rounds, when $r$ is small, would not really increase the ``latency'', as long as most elements in the 
set difference can be reconciled in the first rounds, since the underlying synchronization of data objects corresponding to 
those elements can start immediately after the first round of our scheme. Therefore, the actual latency is one round trip delay instead of 
$r$. 

As we mentioned, this straw-man protocol works correctly if each subset pair has at most one exclusive element (i.e., \autoref{eq:requirement_strawman} holds). On the other hand, if a subset pair has more than one exclusive elements, some of which will not be successfully reconciled:

\begin{itemize}
\item If a subset pair has even number of exclusive elements, Odevity coding will encode it as 0. Then the straw-man scheme will consider the subset pair having no exclusive element and all exclusive elements in this subset will not be reconciled;

\item If a subset pair has odd number ($\geq 3$) of exclusive elements, Odevity coding will encode it as 1 and consider the subset pair having only 1 exclusive element. Then the straw-man scheme will use \autoref{alg:trivial_case} to decode only one exclusive element and dismiss all others. Even worse, the only decoded element is probably not a real exclusive element, since the element computed by \autoref{alg:trivial_case} is the \code{XOR} sum of all exclusive elements, not one of them. 
\end{itemize}

In summary, if a subset pair has more than one exclusive elements, most of its exclusive elements cannot be reconciled, and the reconciled element is usually incorrect (i.e., false-positive). The false-positive however is easy to check, which will be elaborated in \autoref{subsec:exceptions}. The good thing is, even if not all subset pairs have at most one exclusive element and are successfully decoded, most of them will be w.h.p.. In other words, even if the straw-man protocol cannot reconcile all exclusive elements, it still can reconcile most of them. To reconcile all exclusive elements w.h.p., we can simply extend the single-round straw-man scheme to multi-round. And each round adapts the straw-man scheme to do set reconciliation using independent hashing functions $h(\cdot)$ for partition (i.e., in \autoref{alg:random-part}). This multi-round extension can significantly increase the probability of a successful reconciliation, which will be elaborated in \autoref{sec:tail_bound}. 



\subsection{Our Scheme: The Final Version}\label{subsec:protocol2}

{\bf Under revision~}

The preliminary version of our scheme suffers from two major drawbacks. 
First, its communication overhead is asymptotically 
$O(t\log m)\!=\!O(t\log t)$, which is not asymptotically optimal. 
Second, the decoding computational complexity is proportional to 
$t^2$ with the state-of-the-art decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} for BCH codes, 
which is too high when $t$ is large. 
To overcome these two drawbacks, we use a simple algorithmic trick: divide and conquer. With this algorithmic 
trick, the decoding computational complexity is reduced to $O(t)$, 
and the communication overhead is reduced to $t\cdot\frac{\log u}{8} \!+\! O(t)$ (with a small 
hidden constant roughly varying from 4 to 8) bytes which implies that 
our scheme has an additive communication overhead (compared to the optimal scheme) 
of 4 to 8 bytes per element in the 
set difference and this additive overhead is independent of the key size ({\it i.e.}, $\log u$). 
Recall that the IBF-based schemes usually have a communication overhead of roughly 6 times of the 
optimal scheme, which increases linearly as the key size. Therefore, our scheme is much more 
communication-efficient. 

Now, we describe in detail this algorithmic trick. We let Alice divide elements in $A$ into $\lceil\frac{t}{c}\rceil$ groups (subsets)  
for some small constant $c$ (say $5$) so that each group contains roughly $c$ elements from the set difference on average. We let Bob do the same operations on $B$. To ensure that any common element ({\it i.e.,} any element $x\!\in\! A\bigcup B$) goes into 
the same group ({\it i.e.,} groups at Alice and Bob with the same index), we can use the partition procedure with a hash function shown 
in~\autoref{alg:random-part}. Then, we can apply the preliminary version on each group with a constant $m$ (say $m\!=\!256$) independent of 
$t$. To ensure that each group can be reconciled with a high probability, we need to use BCH codes whose decoding capacity 
larger than $c$ (say $\tau\!=\!2c$), as exact number of elements to be reconciled could be larger than $c$. 
Since this decoding capacity $\tau$ is still a small constant independent of $t$, therefore, the communication 
overhead per group is $\tau\cdot\log m \!=\!O(1)$, which implies a total communication overhead of $O(t)$. 
Similarly, the total decoding computational complexity is also $O(t)$. 

\subsubsection{Parameter Configurations} 

Our scheme now has several parameters: $c$ (average number of elements from the set difference in each group), 
$\tau$ (the correcting capability of the BCH code), $m$ (number of bins for each group), and $r$ (maximum number of rounds). 
We note that the maximum number of rounds $r$ is usually associated with another parameter $p$ the desired success rate: With 
at most $r$ rounds, our scheme should guarantee that the success rate is at least $p$. 
%How to tune these parameters to achieve favorable performance will be detailed later in~\autoref{sec:tail_bound}. 
Here, we provide some guidances for the parameter configurations using our theoretical analysis, which gives the tail bound of 
the success probability of our scheme and will be shown in~\autoref{sec:tail_bound}. 

\noindent
{\bf Parameterizing $c$ and $r$.} The values of $c$ and $r$ are usually provided by users based on the requirements of 
applications. For the value of $c$, a larger $c$ results in a longer decoding time yet lower communication overhead.  
So if the decoding time is a big concern, then a smaller $c$ (say $c=5$) should be used; otherwise, a larger $c$ could be used. 
For the values of $r$, a larger $r$ leads to lower communication overhead and usually lower decoding time (as it allows to use 
a smaller $\tau$), however, the reduction is marginal when $r>3$. Therefore, we suggest users to configure $r$ to be $2$ or $3$. 
% The configuration of $c$ is relatively straightforward, as a larger $c$ will result in 
% a longer decoding time and a slightly lower communication overhead. The former is ..., The latter is slightly tricky. 


\noindent
{\bf Using $c$ and $r$ to parameterize other parameters.} After users specify the values for $c$ and $r$ (associated with a value for 
$p$), we can use our theoretical analysis in~\autoref{sec:tail_bound} to parameterize $\tau$ and $m$. 
Since in a BCH code, the block length is in the form of $2^q-1$, we only need to consider $m=2^q-1$. 

{\bf Liang, please revise the following algorithm!}

\begin{algorithm}
\SetKwProg{Proc}{}{}{end}
\SetKwFunction{algo}{\small Search}

\Proc{Search($c$, $r$, $p$)}{\label{search:entrance}

$\mbox{co}_{best}\leftarrow\infty$\tcc*{\small Best communication overhead}

\For{$\tau \leftarrow c\,\KwTo\, \infty$}{}



}
\end{algorithm}


% , unlike 
% the IBF-based schemes which have an multiplicative overhead of 6 
% The inspiration is from the famous 
% divide and conquer algorithm for the selection problem, in which, given an array with $n$ elements, we want to get the $k$-th largest 
% element. A straightforward idea for this problem is sorting. However, if using insertion-sorting, the complexity would be $O(n^2)$. 
% Then the famous divide and conquer trick comes. It first divides the array into $\lceil n/5\rceil$ groups so that the first 
% $\lfloor n/5\rfloor$ contains $5$ elements and at most one group contains the rest $n \mod 5$ elements, and find the median of each 
% group using the insertion-sorting and th


% This straw-man scheme still has a problem on decoding computational complexity. More specific, the complexity increases dramatically with the total number of corrupted bits $t$. Therefore, when $t$ is moderate or large, the decoding computational complexity could be very high. For instance, the decoding complexity of BCH codes~\cite{Lint_IntroductionCodingTheory_1998} is $O(t^3)$, which could be quite high for a large $t$. To keep the decoding complexity reasonably low, we design the following two-layer protocol: In the first layer, we use a hash function to partition the two sets into $\lceil\frac{t}{c}\rceil$ subsets for some small constant $c$ (say $5$), just like the first step of our straw-man scheme. The objective, which is however different from before, is to make each subset pair contains roughly $c$ exclusive elements on average. In the second layer, we use the straw-man scheme with the same configuration (number of subsets $m$, and error-correction capability $\tau$, number of rounds $r$) to reconcile each subset pair. 

% In fact, the straw-man scheme is a proper solution when $t$ is small. First, the decoding complexity will not be a problem for a small $t$; Second, we do not need an extremely large $m$ to guarantee \autoref{eq:requirement_strawman} w.h.p.. For instance, when $t=5$ and $m=1024$, \autoref{eq:requirement_strawman} holds with probability $\frac{m\,!}{(m-t)\,!m^t}\approx 99\%$. This motivates us to design the following two-layer protocol: In the first layer, we use a hash function to partition the two sets into $\lceil\frac{t}{c}\rceil$ subsets for some small constant $c$ (say $5$), just like the first step of our straw-man scheme. The objective, which is however different from before, is to make each subset pair contains roughly $c$ exclusive elements on average. In the second layer, we use the straw-man scheme with the same configuration (number of subsets $m$, and error-correction capability $\tau$) to reconcile each subset pair. 

\autoref{proto:II} shows the pseudocode of our scheme. It first uses the same hash-function based random partition algorithm as \autoref{alg:random-part} to partition elements into $k\triangleq\lceil \frac{t}{c} \rceil$ subsets. Note that the random partition only guarantees that each such subset 
contains $c$ exclusive elements on average, and the exact number is not known. Hence, our scheme uses a BCH code with a capability of 
correcting up to $\tau$ errors with $\tau > c$ to make sure that the BCH code has a high probability to decode successfully. We will describe how to deal with situation where the size of set difference exceeds $\tau$ later in~\autoref{subsec:exceptions}.

As the decoding of a $\tau$-error-correcting BCH code where $\tau$ is a small constant has a constant-time computational complexity, the decoding complexity of 
our scheme is $O(k)=O(t)$. We now have several parameters, average number of exclusive elements in each subset $c$, the correcting capability $\tau$ of BCH code, the number of smaller subsets $m$ for each subset to be divided to, and the number of rounds $r$. How to tune these parameters to achieve favorable performance will be detailed later in~\autoref{sec:tail_bound}. 

\IncMargin{1em}
\begin{algorithm}
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
\Input{Size of set difference $t$}
\Input{The number of subsets $m$ for each partition}
\Input{Average number of exclusive elements in each partition $c$}
\Input{BCH code capability $\tau$}

$k \leftarrow \lceil \frac{t}{c}\rceil $\;

Partition elements into $k$ subsets using~\autoref{alg:random-part}\;

\For{$j = 0$ \KwTo $k-1$}{
    Reconcile the $j$-th subset pair using the straw-man scheme with the BCH correcting capability $\tau$, number of smaller subsets $m$, and number of rounds $r$\;
}

\caption{Our Scheme} \label{proto:II}
\end{algorithm}\DecMargin{1em}




\subsection{Exceptional Handling}\label{subsec:exceptions}

{\bf To be revised~}

In this section, we will elaborate how to handle the following two types of exceptions that we mentioned in \autoref{sec:multiround} and \autoref{subsec:protocol2}:
\begin{itemize}
    \item Exception 1: A subset pair has odd number ($\geq 3$) of exclusive elements and causes false-positives (i.e., a decoded distinct element is not a real one);
    \item Exception 2: A subset pair contains too many exclusive elements, such that a BCH code with capability of correcting up to $\tau$ errors cannot decode it (i.e., $t>\tau$).
	\item Exception 3: A subset pair has even number ($\geq 2$) of exclusive elements and causes false-negatives(i.e., two or more distinct elements are neglected as the parity bit is 0);
\end{itemize}

To handle Exception 1, we need to check whether a computed exclusive element by \autoref{alg:trivial_case} is a real exclusive element or not. (The group index happens to come in handy if we use it as a fingerprint of the element we computed. If this element is truly an exclusive element, it should be hashed into the same group as before. Notably, We have two group indices available for this check, one is in the initial divide and conquer phase, the other is in the BCH code part) It can be easily done at the end of set reconciliation, during which two hosts exchange their exclusive elements. In fact, as we will elaborate in \autoref{sec:tail_bound}, Exception 1 hardly happens if we set parameters properly. 

On the other hand, when Exception 2 happens, the BCH decoder will report a failure about exceeding the error-correction capability. For such a subset pair, we can use the same approach as in \autoref{subsec:protocol2} to partition it into smaller subsets and use the straw-man scheme to reconcile them respectively. We set the number of small subsets to be 3. It is because, as we will elaborate in \autoref{sec:tail_bound}, the number of exclusive elements for each subset pair $t$ should be, if not smaller, only slightly larger than $\tau$ w.h.p.. Partitioning those exclusive elements into 3 small subsets is enough to guarentee that each of them has less than $\tau$ exclusive elements.

\end{comment}

==> section/db_application.bk.0719.tex <==
\subsubsection{Possible Applications of PBS}\label{subsec:db-app}

%% added 
{\color{red}
%% Maybe move to other section
%PBS is a solution for the set reconciliation problem in which tradeoffs exist among communication overhead, 
%computational complexity, and latency (in terms of round-trip delays). That said, PBS might not be suitable 
%for all applications that need set reconciliation. 
As explained earlier, elements in set difference $A \triangle B$ are the hash signatures of actual objects that need to be exchanged.  
When the size of an object is much larger than that of a hash signature,  
the communication cost of reconciling $A$ and $B$, using any existing set conciliation scheme except the naive scheme, 
is anyway negligible compared to that of 
exchanging the actual objects.   However, in many real-life applications, either
the actual object size is not significantly larger (e.g., in the transaction relay operation of a blockchain scheme), or the actual objects need to be 
synchronized mush less often than their hash signatures (e.g., in Dropbox under the smart sync mode).  In such applications, it makes a performance difference to 
reduce the communication cost of reconciling $A$ and $B$.
%, as we will elaborate using an example shortly.

For example, as measured in a blockchain work called Erlay~\cite{Naumenko_ErlayEfficientTransaction_2019}, 
this communication cost accounts for around $5\%$ of the total network bandwidth consumption of its transaction relay operation even when
PinSkech~\cite{Dodis_PinSketch_2008}, the most communication-efficient set reconciliation scheme, is used and 
the size of the hash signature (called {\it transaction ID} in blockchain schemes) is compressed from \SI{256}{bits} to \SI{64}{bits} 
(at cost of possible hash collisions among different transactions during the set reconciliation process).   This communication cost would
account for around $55\%$ of the total bandwidth consumption if IBF-based schemes were used instead and transaction ID's were not compressed.  

PBS is better suited, than any existing set reconciliation scheme, for such applications in general and blockchain schemes in particular, for two reasons.
First, although PinSketch, the state of the art ECC-based solution, has a slightly smaller communication overhead than PBS, its  
computational complexity 
is too high to scale to scenarios  
where $| A\triangle B  |$ is large. 
%In contrast, PBS is much more computationally 
%efficient and only has slightly higher communication overhead. 
Second, the communication overhead of IBF-based solutions, including the state of the art solution Graphene~\cite{Ozisik2019}, are generally much larger than that of PBS.

Therefore, in the following we will use the transaction relay operation in blockchain schemes as an example application for PBS.
Transaction relay (operation) refers to the synchronization (reconciliation) of the transaction databases (sets) across 
the peer-to-peer network of a blockchain scheme.  In this application, Alice and Bob are two peers engaging in a transaction relay,
and $A$ and $B$ are the sets of hash signatures of the transactions recorded at Alice and Bob respectively. 
The blockchain schemes and their transaction relay operations have recently 
received considerable research attention from the database community ({\it e.g.,} ProvenDB~\cite{_ProvenDB_}, 
BlockchainDB~\cite{ElHindi_BlockchainDBSharedDatabase_2019}, 
BigchainDB~\cite{McConaghy_Bigchaindbscalableblockchain_2016}, 
and SEBDB~\cite{Zhu_SEBDBSemanticsEmpowered_2019}), partly due to the semantic similarities between blockchains and 
distributed databases~\cite{Ruan_BlockchainsDistributedDatabases_2019,Sharma_BlurringLinesBlockchains_2019}.
}

%Graphene (and other ) is much 
%higher than . 
%These salient properties make PBS an excellent candidate algorithm that is bandwidth- and computationally-efficient 
%for transaction relay in blockchain. 


%Arguably, the performance benefit is more pronounced in applications (of set reconciliation) when 
%reducing the former communication cost still makes a performance difference for
%real-life applications where 


% incur much higher communication overheads resulting in much higher bandwidth consumption. 
% PBS could be a better alternative than both Graphene and PinSketch, since 
% PBS has a communication overhead much lower than Graphene and slightly higher than 
% PinSketch, and a computational complexity much lower than PinSketch, as will be shown in~\autoref{sec:evaluation}. 
%  in which both IBF-based set reconciliation techniques, 
% {\it e.g.,} Graphene~\cite{Ozisik2019} and ECC-based set reconciliation techniques, {\it e.g.,} 
% PinSketch in Erlay~\cite{Nakamoto_Bitcoinpeerpeer_2019}, can significantly reduce 
% the bandwidth consumption.
% the reconciliation of those hash signatures take a decent amount of bandwidth. 
% For example, as measured in Erlay~\cite{Naumenko_ErlayEfficientTransaction_2019}, a set-reconciliation based solution to 
% transaction relay in Bitcoin, the set reconciliation takes around $5\%$ of the total bandwidth even 
% when they compress the transaction ID from \SI{256}{bits} to \SI{64}{bits} at cost of possible collisions among different 
% transactions. 


% though a proper set reconciliation schemes is also 
% a promising solution to many other decentralized synchronization applications, 
% such as synchronizations of state ({\it e.g.,} game state) databases in named 
% data networking (NDN)~\cite{Zhu_LetsChronoSyncDecentralized_2013,Moll_InterServerGame_2019}. 

% As mentioned earlier, set reconciliation arises in various applications. 
% To better illustrate set reconciliation in the context of databases applications, we use %the application of 
% the synchronization of transaction databases in a peer-to-peer network in blockchain propagation~\cite{Ozisik2019,Naumenko_ErlayEfficientTransaction_2019} as an example throughout this paper, though a proper set reconciliation schemes is 
% a promising solution to many other decentralized database synchronization applications, such as synchronizations of   
% state ({\it e.g.,} game state) databases in named data networking (NDN)~\cite{Zhu_LetsChronoSyncDecentralized_2013,Moll_InterServerGame_2019}. For ease of presentation, we assume that the key-value databases are used. We note that our scheme and many other 
% set reconciliation schemes can be applied to other types of databases without modifications as well.  


% In the context of blockchain propagation, we can view the transaction ID, which is usually equal to its cryptographic hash, 
% as the key and the full transaction as the value. Every transaction needs to relay to all nodes 
% to achieve synchronization among all parties. In a blockchain propagation protocol, newly created and signed transactions 
% (key-value pairs in the databases), and newly mined blocks, each of which is a collection of transactions, at different peers are synchronized periodically. 
% % On one hand, too frequent synchronization could result in bandwidth waste. On the other hand, 
% % too infrequent synchronization could result in high latency of transaction propagation.  

\begin{comment}
A blockchain is a set of blocks, each of which consists of multiple cryptographically 
signed transactions. These blocks are kept consistent among all nodes in the peer-to-peer 
network. 
Each transaction contains a unique transaction ID, 
which is usually a cryptographic hash value. 
To achieve consistency among all nodes, every transaction, after created and signed at some node, 
needs to relay all other nodes. Usually, the relay process is initiated periodically (say every few seconds). 

During each relay process, each node might obtain a set of new transactions that are newly 
created and signed by itself or received from its neighbors. 
It can relay those transactions in its entirety to its neighbors, but this could result in unnecessary bandwidth waste because the receivers are likely to store some of them 
locally. Instead, a node can apply our solution to identify and relay only those 
transactions in the set difference to save bandwidth. 
More precisely, for each node pair, say Alice and Bob, 
the sets of transaction IDs of the newly obtained transactions are the two respective 
two sets at Alice and Bob. 
We refer to the sets at Alice and Bob as sets $A$ and 
$B$ respectively. As mentioned earlier, after reconciling sets $A$ and $B$ using our solution, 
both Alice and Bob learn $A\bigcup B$ and can infer what (transactions) are needed to relay 
to each other. 
% Finally, Alice and Bob exchange those transactions to reach the consistency. 
More precisely, Alice relays to 
Bob the transactions that Bob does not have and Bob relays to Alice the transactions that Alice does not have. 
\end{comment}

% ----Handle 
% Database applications that allow no incorrect verification. Fortunately, we can apply a one way hash function, $H$, to 
% both $A\triangle\hat{D}$ and $B$ and verify $H(A\triangle\hat{D})\!\stackrel{?}{=}\!H(B)$. Here, $H(S)$ for any ordered 
% set $S$ is to apply the one way hash function, $H$, to the string that is the concatenation of all strings in $S$ 
% according to the pre-determined ordering. Even though the function $H$ is applied to a very long string, the output is actually 
% very short (say $256$ bits long), therefore, the communication overhead of this extra verification is quite low. 
% We do not count this overhead in the calculation of the communication overhead in the sequel, since all schemes described in 
% this paper requires this extra verification process when using in database applications. We note that in some applications, 
% the system itself does provide methods to verify the consistency. For example, Ethereum~\cite{Wood_Ethereumsecuredecentralised_2014} 
% and Bitcoin~\cite{Nakamoto_Bitcoinpeerpeer_2019} both have fundamental component to verify the integrity and consistency of transactions based the Merkle tree~\cite{Merkle_merkle-tree_1980}. In a Merkle tree, each leaf node is a cryptographic hash of a transaction, 
% and each non-leaf node is the hash 
% of its two children, and its root validates the consistency of all transactions. 

% We note that even if the $c(A\triangle\hat{D})\!\stackrel{?}{=}\!c(B)$ verification is incorrect, we can still finish the 
% reconciliation process using this incorrect $\hat{D}$ so that the efforts are not wasted 
% and doing so will only result in ``underestimated'' unions. 
% The elements (transactions) that neither Alice nor Bob has will be eliminated if even they have ever 
% generated during the set reconciliation process, because Alice cannot send to Bob transactions she does not have and 
% vice versa. Then, we re-run the whole reconciliation process again, the communication overhead would be much less than that of 
% the previous run, since now $d$ is much smaller.


==> section/db_application_copy.tex <==
\subsubsection{Apply PBS in real-life applications}\label{subsec:db-app}

%% added 
{\color{red}
%% Maybe move to other section
PBS is a solution for the set reconciliation problem in which tradeoffs exist among communication overhead, 
computational complexity, and latency (in terms of round-trip delays). That said, PBS might not be suitable 
for all applications that need set reconciliation. 
PBS is more suitable for applications where the actual object size is not too large (relative to the hash signature) 
or the actual objects need to be 
synchronized mush less often than the their hash signatures. 
One example of such applications is transaction relay
in blockchain (to be described next), in which set reconciliation algorithms, 
as shown in Graphene~\cite{Ozisik2019} (an IBF-based technique) and Erlay~\cite{Nakamoto_Bitcoinpeerpeer_2019} (using PinSketch~\cite{Dodis_PinSketch_2008}, an ECC-based technique),  can help significantly reduce the bandwidth consumption. 
As measured in Erlay~\cite{Naumenko_ErlayEfficientTransaction_2019}, 
the set reconciliation step alone takes around $5\%$ of the total bandwidth in the transaction relay even 
when they use PinSkech, the most communication-efficient set reconciliation technique and compress the transaction ID (``hash signature'') from \SI{256}{bits} to \SI{64}{bits} 
at cost of possible collisions among different 
transactions during the set reconciliation. 
On one hand, 
as mentioned earlier, the computational complexity of PinSketch (and other ECC-based techniques) 
is too high to scale to scenarios  
where the cardinality of the set difference is large. 
In contrast, PBS is much more computationally 
efficient and only has slightly higher communication overhead. 
On the other hand, the communication overhead of Graphene (and other IBF-based techniques) is much 
higher than that of PBS. 
These salient properties make PBS an excellent candidate algorithm that is bandwidth- and computationally-efficient 
for transaction relay in blockchain. 
% incur much higher communication overheads resulting in much higher bandwidth consumption. 
% PBS could be a better alternative than both Graphene and PinSketch, since 
% PBS has a communication overhead much lower than Graphene and slightly higher than 
% PinSketch, and a computational complexity much lower than PinSketch, as will be shown in~\autoref{sec:evaluation}. 
%  in which both IBF-based set reconciliation techniques, 
% {\it e.g.,} Graphene~\cite{Ozisik2019} and ECC-based set reconciliation techniques, {\it e.g.,} 
% PinSketch in Erlay~\cite{Nakamoto_Bitcoinpeerpeer_2019}, can significantly reduce 
% the bandwidth consumption.
% the reconciliation of those hash signatures take a decent amount of bandwidth. 
% For example, as measured in Erlay~\cite{Naumenko_ErlayEfficientTransaction_2019}, a set-reconciliation based solution to 
% transaction relay in Bitcoin, the set reconciliation takes around $5\%$ of the total bandwidth even 
% when they compress the transaction ID from \SI{256}{bits} to \SI{64}{bits} at cost of possible collisions among different 
% transactions. 

To better illustrate how our solution (and other similar solutions) can 
be used in real-life applications, we use synchronization of transaction databases in 
a peer-to-peer network, more precisely transaction relay, in blockchain  
as an example throughout this paper. We note that some existing blockchain platforms, 
{\it e.g.,} Ethereum~\cite{Wood_Ethereumsecuredecentralised_2014} and Bitcoin~\cite{Nakamoto_Bitcoinpeerpeer_2019}, might not use database techniques directly. However, 
we still consider them as databases due to the similarities between blockchains and 
distributed databases~\cite{Ruan_BlockchainsDistributedDatabases_2019,Sharma_BlurringLinesBlockchains_2019}. Furthermore, because of these similarities, 
many blockchain databases, {\it e.g.,} ProvenDB~\cite{_ProvenDB_}, BlockchainDB~\cite{ElHindi_BlockchainDBSharedDatabase_2019}, BigchainDB~\cite{McConaghy_Bigchaindbscalableblockchain_2016}, SEBDB~\cite{Zhu_SEBDBSemanticsEmpowered_2019} and {\it etc}, 
have been proposed in both academia and industry. 
% though a proper set reconciliation schemes is also 
% a promising solution to many other decentralized synchronization applications, 
% such as synchronizations of state ({\it e.g.,} game state) databases in named 
% data networking (NDN)~\cite{Zhu_LetsChronoSyncDecentralized_2013,Moll_InterServerGame_2019}. 

% As mentioned earlier, set reconciliation arises in various applications. 
% To better illustrate set reconciliation in the context of databases applications, we use %the application of 
% the synchronization of transaction databases in a peer-to-peer network in blockchain propagation~\cite{Ozisik2019,Naumenko_ErlayEfficientTransaction_2019} as an example throughout this paper, though a proper set reconciliation schemes is 
% a promising solution to many other decentralized database synchronization applications, such as synchronizations of   
% state ({\it e.g.,} game state) databases in named data networking (NDN)~\cite{Zhu_LetsChronoSyncDecentralized_2013,Moll_InterServerGame_2019}. For ease of presentation, we assume that the key-value databases are used. We note that our scheme and many other 
% set reconciliation schemes can be applied to other types of databases without modifications as well.  

A blockchain is a set of blocks, each of which consists of multiple cryptographically 
signed transactions. These blocks are kept consistent among all nodes in a peer-to-peer 
network. Each transaction contains a unique transaction ID, 
which is usually a cryptographic hash value. 
To achieve consistency among all nodes, every transaction, after created and signed at some node, 
needs to relay all other nodes. Usually, the relay process is initiated periodically (say every few seconds). 

% In the context of blockchain propagation, we can view the transaction ID, which is usually equal to its cryptographic hash, 
% as the key and the full transaction as the value. Every transaction needs to relay to all nodes 
% to achieve synchronization among all parties. In a blockchain propagation protocol, newly created and signed transactions 
% (key-value pairs in the databases), and newly mined blocks, each of which is a collection of transactions, at different peers are synchronized periodically. 
% % On one hand, too frequent synchronization could result in bandwidth waste. On the other hand, 
% % too infrequent synchronization could result in high latency of transaction propagation.  
During each relay process, each node might obtain a set of new transactions that are newly 
created and signed by itself or received from its neighbors. 
It can relay those transactions in its entirety to its neighbors, but this could result in unnecessary bandwidth waste because the receivers are likely to store some of them 
locally. Instead, a node can apply our solution to identify and relay only those 
transactions in the set difference to save bandwidth. 
More precisely, for each node pair, say Alice and Bob, 
the sets of transaction IDs of the newly obtained transactions are the two respective 
two sets at Alice and Bob. 
We refer to the sets at Alice and Bob as sets $A$ and 
$B$ respectively. As mentioned earlier, after reconciling sets $A$ and $B$ using our solution, 
both Alice and Bob learn $A\bigcup B$ and can infer what (transactions) are needed to relay 
to each other. 
% Finally, Alice and Bob exchange those transactions to reach the consistency. 
More precisely, Alice relays to 
Bob the transactions that Bob does not have and Bob relays to Alice the transactions that Alice does not have. 

% ----Handle 
% Database applications that allow no incorrect verification. Fortunately, we can apply a one way hash function, $H$, to 
% both $A\triangle\hat{D}$ and $B$ and verify $H(A\triangle\hat{D})\!\stackrel{?}{=}\!H(B)$. Here, $H(S)$ for any ordered 
% set $S$ is to apply the one way hash function, $H$, to the string that is the concatenation of all strings in $S$ 
% according to the pre-determined ordering. Even though the function $H$ is applied to a very long string, the output is actually 
% very short (say $256$ bits long), therefore, the communication overhead of this extra verification is quite low. 
% We do not count this overhead in the calculation of the communication overhead in the sequel, since all schemes described in 
% this paper requires this extra verification process when using in database applications. We note that in some applications, 
% the system itself does provide methods to verify the consistency. For example, Ethereum~\cite{Wood_Ethereumsecuredecentralised_2014} 
% and Bitcoin~\cite{Nakamoto_Bitcoinpeerpeer_2019} both have fundamental component to verify the integrity and consistency of transactions based the Merkle tree~\cite{Merkle_merkle-tree_1980}. In a Merkle tree, each leaf node is a cryptographic hash of a transaction, 
% and each non-leaf node is the hash 
% of its two children, and its root validates the consistency of all transactions. 

% We note that even if the $c(A\triangle\hat{D})\!\stackrel{?}{=}\!c(B)$ verification is incorrect, we can still finish the 
% reconciliation process using this incorrect $\hat{D}$ so that the efforts are not wasted 
% and doing so will only result in ``underestimated'' unions. 
% The elements (transactions) that neither Alice nor Bob has will be eliminated if even they have ever 
% generated during the set reconciliation process, because Alice cannot send to Bob transactions she does not have and 
% vice versa. Then, we re-run the whole reconciliation process again, the communication overhead would be much less than that of 
% the previous run, since now $d$ is much smaller.
}

==> section/estimator_analysis.tex <==
\section{Estimator Variance}

minhash estimator $\hat{J}$:

\begin{equation}
    J = \frac{|A\cap B|}{|A \cup B|} 
\end{equation}

\begin{equation}
    \hat{t} = (1 - \hat{J})|A \cup B|.
\end{equation}

\begin{align}
    Var(\hat{t}) &= |A \cup B|^2 Var(\hat{J}) \\
                 &= |A \cup B|^2 \frac{J(1-J)}{m} \\
                 &= \frac{|A\cap B| \cdot |A\Delta B|}{m}.
\end{align}



ToW estimator $\hat{Y}$ (from Nan Hua's infocom):

\begin{equation}
    X_j = \sum_{k=1}^t s_k
\end{equation}

\begin{equation}
    s_k = \begin{cases}1& \mbox{ with probability } 1/2\\
    -1 & \mbox{ with probability } 1/2\\
    \end{cases}
\end{equation}

Let $Y_j=X_j^2$, then
\begin{align}
    \mathbb{E}[Y_j] &= \mathbb{E}[(\sum_{k=1}^t s_k)^2] \\
                    &= \mathbb{E}[\sum_k s_k^2 + 2\sum_{k}\sum_{k'\neq k}s_ks_{k'}]\\
                    &= t.
\end{align}

\begin{align}
    \mathbb{E}[Y_j^2] &= \mathbb{E}[(\sum_{k=1}^t s_k)^4] \\
                      &= t + 3t(t-1)\\
                      &= 3t^2 - 2t.
\end{align}

\begin{align}
    Var(Y_j) &= \mathbb{E}[Y_j^2] - (\mathbb{E}[Y_J])^2\\
             &= 3t^2 - 2 t - t^2\\
             &= 2t^2 - 2t.\\
\end{align}

\begin{align}
    Var(\hat{Y}) &= \frac{Var(Y)}{m}\\
                 &=\frac{2t^2-2t}{m}\\
                 &=\frac{2|A\Delta B|(|A \Delta B| - 1)}{m}.
\end{align}


To make sure that $\mathbb{P}[\beta \hat{Y}>t]\leq 0.99$, based on the \href{ http://sphweb.bumc.bu.edu/otlt/MPH-Modules/BS/BS704_Probability/BS704_Probability10.html}{table}, we have $\beta t \geq (t + 2.326 \sigma) \Rightarrow \beta \geq 1 + 2.326\sqrt{2/m}$. Therefore, when $m=256$, we have $\beta \approx 1.2$. (Which matches our simulation results)

% %
% %
% % 0.99, 1.39 ==> 71.14
% % 0.95, 1.39 ==> 35.58

==> section/estimator_without_comments.tex <==
% \subsection{Set difference size estimation}\label{subsec:ToW}
\subsection{Set Difference Cardinality Estimation}\label{subsec:ToW}

% Recall that in real-life applications, 
% % the cardinality of set difference $d$ 
% the set difference cardinality $d$ 
% might not be precisely known. In such a scenario,
For the case of the set difference cardinality $d$ so far is not precisely known, we need a relatively accurate estimation of $d$, 
just like most of other set reconciliation algorithms~\cite{Eppstein_WhatsDifference?Efficient_2011,Dodis_PinSketch_2008,Guo_SetReconciliationvia_2013}. 
In this work, 
% we propose a scheme to estimate the cardinality of set difference that is based on Tug-of-War (ToW) sketch~\cite{AlonMS99}.
we propose a new set difference cardinality estimator that is based on Tug-of-War (ToW) sketch~\cite{AlonMS99}.

++++ {\bf Revised by Long}
The ToW sketch was originally proposed in~\cite{AlonMS99} to estimate the second frequency moment of a data stream. 
Later, in~\cite{Hua_simplerbetterdesign_2012,Hua_TowardsOptimalError_2012,huang_eec_2014}, ToW was used for the 
estimation of the Hamming distance between two binary strings. We found that ToW can also be used for the estimation of the 
set difference cardinality. Given a universal $\mathcal{U}$, let $\mathcal{F}$ be a family of hash functions that maps each 
element in $\mathcal{U}$ to $+1$ or $-1$. The ToW sketch of a set $S\subset \mathcal{U}$ under hash function 
$f\in\mathcal{F}$ is defined as $\alpha_f(S)\triangleq \sum_{s \in S}f(s)$. 
Using similar proof as in~\cite{AlonMS99}, it can be proved that the ToW estimator with $k$ sketches, 
$\hat{d}\!\triangleq\! \sum_{i=1}^k(\alpha_{f_i}(A)\!-\!\alpha_{f_i}(B))^2/k$, is an unbiased estimator of   
$d\!=\!|A\Delta B|$, as long as the hash family $\mathcal{F}$ is four-wise independent and $f_1,f_2,\cdots,f_k$ are drawn uniformly randomly from $\mathcal{F}$. 
The variance of this estimator is $(2d^2\!-\!2d)/k$, which decreases as the number of ToW sketches $k$ increases. 
To achieve higher accuracy ({\it i.e.,} lower variance), 
we need more ToW sketches ({\it i.e.}, larger $k$) and therefore resulting in higher communication overhead, which is proportional to $k$.

% To obtain higher accuracy (lower variance), multiple (say $k$) sketches with $k$ independent hash functions 
% $f_1,f_2,...,f_k$ are usually used and the mean $\hat{d}\!=\!\sum_{i=1}^k (\alpha_{f_i}(A)-\alpha_{f_i}(B))^2/k$ of $k$ independent estimates is used as the final estimate. 
\begin{comment}

++++ {\bf Old version}
% The Tug-of-War (ToW) 
The ToW sketch is originally proposed in~\cite{AlonMS99} to estimate the second frequency moment of data streams. In~\cite{Feigenbaum_AppL1Difference_2003}, Feigenbaum {\it et al.} suggested to use ToW sketch to estimate the size of set difference. We substantiate the idea and propose an unbiased set difference size estimator based on ToW as follows: Given a universal $\mathcal{U}$, let $\mathcal{F}$ be a family of hash functions that maps each element in $\mathcal{U}$ to $+1$ or $-1$. The ToW sketch of a set $S\subset \mathcal{U}$ under hash function $f\in\mathcal{F}$ is defined as $\alpha_f(S)\triangleq \sum_{s \in S}f(s)$. It was proved in~\cite{AlonMS99}, $\hat{d}\triangleq \sum_{i=1}^k (\alpha_{f_i}(A)-\alpha_{f_i}(B))$ is an unbiased estimator on the size of set difference $d$, as long as the hash family $\mathcal{F}$ is four-wise independent and $f_1,f_2,...,f_k$ are drawn uniformly randomly from $\mathcal{F}$. The variance of this estimator is $(2d^2-2d)/k$, which decreases as the number of ToW sketches $k$ increases. To achieve higher estimation accuracy, we need more ToW sketches (i.e., larger $k$) and therefore more communication overhead, which is proportional to $k$.
%Each ToW sketch ranges in $[-|A\bigcup B|, |A\bigcup B|$ and can be represented in $\log |A\bigcup B|$ bits. Therefore, the communication overhead on transmitting ToW sketches is $k\log |A\bigcup B|$ bits. Note that the estimation accuracy  

++++ {\bf The following paragraph seems not necessary} 

For PBS, we do not need a very accurate estimation on $d$. It is because, in practice ({\it e.g.}, in \cite{Eppstein_WhatsDifference?Efficient_2011}), the estimate returned by the estimator is usually scaled up by a proper factor $\gamma$ to ensure that $d>\gamma\hat{d}$ (i.e., the actual number of distinct elements is more than estimation) rarely happens. In the evaluation in~\autoref{sec:evaluation}, we use \code{xxHash}~\cite{Collet_xxHashExtremelyfast_} as the hash family. 

{\bf MOVED from related work, may not necessary} 
We note that the extra round of message exchange resulting from the ToW estimator can be reduced in practice by 
a simple trick: After receiving ToW sketches from Alice, 
instead of just sending the estimates back to Alice, 
Bob starts the set reconciliation process by sending to Alice
the BCH codeword together with the estimates in~\autoref{step:BCH_encode} of~\autoref{alg:single_round_pbs}. 
Clearly, such a trick 
also applies to other set reconciliation algorithms that require an estimator ({\it e.g.,} PinSketch). 
% However, in the sequel, for ease of presentation, 
% we still assume that our scheme (and D.Digest and Minisketch) uses 
% a separate round for set-difference size estimation. 

==================================

Given a hash function $f:\mathcal{U}\rightarrow \{\}$ drawn uniformly randomly from such a hash family $\mathcal{F}$, we define the ToW sketch of a set $S\subset \mathcal{U}$ under $f$ as $\sum_{s \in S}f(s)$. It was proved in~\cite{AlonMS99},  as long as the hash family is four-wise independent, 
the ToW sketches generated using hash functions have the exact same statistical properties ({\it i.e.,} \autoref{eq:tow} holds) as those for binary vectors. 
As shown in~\autoref{subsec:est-bench}, the efficient hash family, 
\code{xxHash}~\cite{Collet_xxHashExtremelyfast_}, works extremely well in practice. 

The objective of an estimator for the set-difference size $d$ in the context of set reconciliation is to provide estimates with high-enough accuracy. On one hand, if the estimator over-estimates, the subsequent reconciliation will usually waste unnecessary bandwidth. 
On the other hand, if the estimator under-estimates, the reconciliation might fail. Hence, in practice (e.g., in \autoref{subsec:vs-prior}), the estimate returned by the estimator is usually scaled up by a proper factor to ensure that the failure rarely happens. 


As mentioned earlier, to make our reconciliation algorithm work efficiently, we must have a relatively 
accurate estimation of the set-difference size $t$. In this work, we propose an efficient estimator 
based on the Tug-of-War (ToW) sketch~\cite{AlonMS99}.  
% We use Tug-of-War(ToW) Sketch to estimate the size of set difference.
The ToW sketch was first introduced in \cite{AlonMS99} 
for estimating the second frequency moment (equivalently, the square of the $L_2$ norm) 
of a data stream~\cite{Muthukrishnan_DatastreamsAlgorithms_2005}. 
ToW is also a good estimator for Hamming distance in the two-party computation 
({\it e.g.,} \cite{Hua_simplerbetterdesign_2012,Hua_TowardsOptimalError_2012}) where Alice 
and Bob each has a binary vector $x$ and $y$ respectively and want to estimate their Hamming 
\code{Hamming}$(x,y)$ because \code{Hamming}$(x,y)=\|x-y\|_2^2$. 
Given a binary vector $x\in\{0,1\}^n$, a ToW sketch is defined as $\phi_R(x)=\langle x, R\rangle$, where $R$ is 
a $n$-dimensional vector whose $d$ scalars are {\it i.i.d.} random variables taking the values of $+1$ or $-1$ with 
equal probability ({\it i.e.,} 1/2). Given any two binary vectors $x,y\in\{0,1\}^n$ whose Hamming distance is $t$, 
define a random variable $X=\big{(}\phi_R(x)-\phi_R(y)\big{)}^2$, it was shown in~\cite{Hua_simplerbetterdesign_2012} that 
\begin{equation}\label{eq:tow}
\begin{cases}
\mathbf{E}[X] &= t.\\
{\mbox{\bf Var}}[X] & = 2t^2 - 2t. \\
\end{cases}
\end{equation}

A naive scheme of using the above ToW to estimating the set-difference size is to represent each set 
$S$ as an characteristic vector $s\in\{0,1\}^n$ (where $n$ is the size of the universe): 
$s_x=1$ if $x\in S$; Otherwise $s_x=0$. Using such a representation, we have converted the set-difference size to 
the Hamming distance of two binary vectors, since, given any two sets $A$ and 
$B$ and their characteristic vectors $a$ and $b$, we have \code{Hamming}$(a,b)\!=\!t=|A\Delta B|$ 
the set-difference size. In this naive scheme, Alice first represents $A$ as its characteristic vector $a$, 
computes $k$ ToW sketches, denoting as $\alpha_1,\alpha_2,\cdots,\alpha_k$, for $a$, and then sends them 
to Bob. Similarly, Bob computes $k$ ToW sketches, $\beta_1,\beta_2,\cdots,\beta_k$, for the characteristic vector 
of set $B$. Upon receiving the $k$ ToW sketches from Alice, Bob can estimate the set-difference size as 
$\hat{t}=\frac{1}{k}\sum_{i=1}^k(\alpha_i-\beta_i)^2$. Clearly, the variance of this estimator is $\frac{2t^2-2t}{k}$. 

This naive scheme is impractical since it needs Alice and Bob each to generate $k$ $n$-dimensional $\pm 1$ vectors 
where $n$ is usually huge (say $2^{32}$ or even larger). Fortunately, we do not need to explicitly 
represent sets as their characteristic vectors and generate those $\pm 1$ vectors for getting ToW sketches. 
Instead, we can simply use hash functions to achieve the same goal. 
Here it suffices to only describe how to use a hash function to generate a single ToW sketch. 
Given a universal $\mathcal{U}$, let $\mathcal{H}$ be a hash family in which each hash function maps 
any element $x\in\mathcal{U}$ to $+1$ or $-1$.
%  in such a way that, given any element $x\in \mathcal{U}$, 
% for a hash function $h$ that is drawn uniformly randomly from this family, we have $h(x)$ equals $1$ 
% or $-1$ each with probability $1/2$. 
Given a hash function $h$ drawn uniformly randomly from such 
a hash family $\mathcal{H}$, a ToW sketch of a set $S\subset \mathcal{U}$ is defined as $\sum_{s \in S}h(s)$. It was 
proved in~\cite{AlonMS99}, as long as the hash family is four-wise independent, 
the ToW sketches generated using hash functions 
have the exact same statistical properties ({\it i.e.,} \autoref{eq:tow} holds) as those for binary vectors. 
As shown in~\autoref{subsec:est-bench}, the efficient hash family, 
\code{xxHash}~\cite{Collet_xxHashExtremelyfast_}, works extremely well in practice. 

The objective of an estimator for the set-difference size $d$ in the context of set reconciliation is to provide estimates with high-enough accuracy. On one hand, if the estimator over-estimates, the subsequent reconciliation will usually waste unnecessary bandwidth. 
On the other hand, if the estimator under-estimates, the reconciliation might fail. Hence, in practice (e.g., in \autoref{subsec:vs-prior}), the estimate returned by the estimator is usually scaled up by a proper factor to ensure that the failure rarely happens. 

% Let $k$ be the cardinality of sequence $A$ and $m_i$ be the count for the $i$th distinguished element in $A$. Then the second frequency moment of sequence A is defined as
% \[F_2 = \sum_{i=1}^{k} {m_i}^2 \]
% In our context with set difference, every element only occurs once in a set. So the second frequency moment is also the size of this set. 

The ToW Sketch hashes every item in the sequence to $\{+1,-1\}$ with hash function $h$ and then sum up these hash values. The square of the sum is an unbiased estimate of the second frequency moment.
\[\hat F_2 = ({\sum_{i=0}^{n} {h(a_i)}})^2 \]
This method can then be altered to estimate set difference. Let $s_{A,B}$ denotes the sum of hash values of every element in $set_{A,B}$ using the same hash function. If we subtract $s_A$ from $s_B$, then the hash values of elements in set union $A \cap B$ are cancelled out. 
\[s_B - s_A = s_{B\setminus A} - s_{A\setminus B} \]
So the square of this difference is exactly the estimate of set difference(second frequency moment or the symmetric difference). Although it is $s_{B\setminus A} - s_{A\setminus B}$ instead of $s_{B\setminus A} + s_{A\setminus B}$, the estimate is still accurate since the probability of hashing into +1 and  the probability of hashing into -1 are both 0.5.
In practice, We will use $p$ ToW Sketches in order to increase the accuracy of our estimates.
%\subsection{Parity Bits and Binary BCH codes}\label{Two}
%In the second layer, the strategy we use is to partition each bin into much larger number of small bins. We want to ensure that all exclusive elements are distributed into different small bins. Under this assumption, we only need to compute the parity of each small bin's size on both A and B side and then compare them to find out which bins may contain only one exclusive element. If a small bin has the same value on A and B side, we call it a 0-bin. Otherwise, we call it a 1-bin. We only focus on the 1-bins to obtain the exclusive elements.

%We use binary BCH codes to further reduce communication cost. Suppose we scatter all elements into $n$ small bins. Normally, we would need to transmit all $n$ bits representing the parity of every small bin. With binary BCH codes, we only need to transmit $t \cdot log(n)$ bits to find out where the 1-bins are if there are no more than $t$ 1-bins.

%BCH codes \cite{bch1, bch2} is an error-correcting code constructed by using polynomials over a finite field. Similar to Hamming codes, it computes several check bits from the data bits, catenates it after the data bits to form a codeword and then transmits the codeword. The receiver can then recover the codeword if the corrupted one it received is not too far from the original codeword. An (n,k,t) BCH codes can correct all bit errors with an n-bit codeword containing k data bits if there is no more than t bit errors.

%In our context, we can view the bits we used to represent the parity of each subset on A side as original data bits and the ones on B side as corrupted data bits with $t$ bit errors. Thus, we only need to transmit the check bits from A to B in order to detect all $t$ bit errors on B side. The positions of these bit errors are exactly the indices of 1-bins. Furthermore, we can use all $n$ bits as data bits by XOR data bits with check bits instead of catenating check bits after data bits. Because in our context, bit errors only occur in data bits but not in check bits.

%\subsection{To Make It Robust}
%It is obvious that in the second layer, there is possibility that multiple exclusive elements are thrown into one bin. When even number of elements are in one bin, they will all be neglected because it forms a 0-bin. When odd number($\leq 3$) of elements are in one bin, their XOR sum will be obtained instead of themselves.

%To handle the first situation, along with the XOR sums of 1-bins, we send the XOR sum of all elements in 0-bins to see if we missed some exclusive elements in 0-bins. If so, after we obtain some of the exclusive elements from 1-bins, we can use the same scheme in the second layer to deal with the rest in the next round.

%To handle the second one, we need to check whether the XOR sum we get is truly an element. A simple method is to map the result we get with the same mapping function to see it will be thrown into the same small bin in the same big bin as before. If not, it is certain that the result we get is the XOR sum of multiple elements. And we  will use the same scheme to deal with the small bin it belongs to in the next round. There is still false positive with this validity check. But the possibility is extremely low with normal settings.

%Another kind of situation happens when the number of 1-bins exceeds the capacity $t$ of BCH code. With high probability, the BCH decoder will fail to decode. Then we need to divide the big bin into several big bins and apply the second layer scheme to each of them. It is possible that the BCH decoder will decode the corrupted codeword into another codeword when there is more than $t$ bit errors. However, when the BCH codes we use is long, the possibility is extremely low. Furthermore, the two mechanisms above can also deal with this situation.

% To make things clear for us. Not necessary for readers.
\subsection{Parameter Setting}
For the ToW estimator, the only one parameter we need to adjust is the number of ToW sketches $p$. It affects the accuracy of our estimation of set difference.
In the first layer, we have a parameter $\delta$, which is the ratio of number of big bins to the estimate of set difference. It correlate with the distribution of number of exclusive elements in a big bin,
In the second layer, we have $n$ as the number of small bins in each big bin and $t$ as the maximum number of errors that the BCH code can correct. They will affect the reconcile ability of each big bin.
These are the four major parameters that have large impact on the performance of our model.


To evaluate the performance, we also have four metrics, which are total bits transmitted, number of rounds, false negative rate and false positive rate. There is a lot of trade-offs between these four parameters and four metrics. We will further analyze and demonstrate the trade-offs in the analysis section and experiment section.
\end{comment}

==> section/evaluation-BK.tex <==
\section{Performance Evaluation}\label{sec:evaluation}
%% Experiments for estimators

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% Task 1.1: Experiments %%%%%%%%%%%%%%%%%%%%%%%%
%==> I will start (and hopefully complete) this experiments by the mid-night of Nov. 17, 2019. ---- Long
%%% Benchmark estimators: Strata Estimator/min-hash/Bagminhash 
%%% MSE (??) plus Correction overhead
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%% Experiments for Reconciliation

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% Task 1.2: Experiments %%%%%%%%%%%%%%%%%%%%%%%%
%==> I need some time to figure out how to use (or even modify) the source codes of Graphene ---- Long
%==> Hopefully, I can finish this part by the end of the next week (Nov. 22, 2019)
%%% Benchmark algorithms: minisketch/Graphene/KeyDiff
%%% 99% (??) reconciliation correction rate in one round (CO v.s. d) with roughly the same computational complexity 
%%% 95% (??) decoding rate in one round (CO v.s. d)
%%% multiple rounds for our scheme (maybe also for minisketch)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% Task 2.1: Writing %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%==> While conducting those experiments, I will also add the paragraphs for evaluation.   --- Long
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% Task 2.2: Writing %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%==> I have added a few more papers on this topic. If you (@ziheng) have  some time, you can help us add some sentences regarding them in the  related work section. I will also read them and try to produce some paragraphs.  --- Long
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%% To ZiHeng %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%==> If you have any suggestions of concerns regarding the above plan, please feel free to ``shoot'' to us. ---- Long
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% In this section, we evaluate the performances of our ToW estimator 
% and our set reconciliation algorithm.

% % 
In this section, we evaluate the performance of PBS, and compare 
it with Difference Digest (D.Digest)~\cite{Eppstein_WhatsDifference?Efficient_2011}, 
Graphene~\cite{Ozisik2019}, and Minisketch~\cite{naumenko2019bandwidth}, which we have 
described in detail in~\autoref{subsec:recon-bench}. 

\subsection{Methodologies}\label{subsec:exp-methodologies}

In our evaluation, we first fix key size $u$ (the length  
of each element in the universe $\mathcal{U}$) as $4$ bytes. 
Later, in~\autoref{sucsec:varying-key-sizes} we evaluate the performances under various values of $u$.   
Like in~\cite{Eppstein_WhatsDifference?Efficient_2011}, each pair of sets, $A$ and $B$, 
was created by exercising two degrees of freedom: the number of elements in $A$ and $B$, 
and the size $d$ of the set difference $A\Delta B$.  
First, elements in $A$ were chosen from the universe $\mathcal{U}$ uniformly at random. 
A subset of elements in $A$ were then selected also uniformly at random and copied to $B$. 
% % explain why we only exercise the above two degrees of freedom (need revision)
We did not exercise the degree of freedom in varying the sizes of $A\!\setminus\! B$ and $B\!\setminus\! A$ because 
all estimators compared in~\autoref{subsec:est-perf} are designed for the estimation of 
only $d$ (not the sizes of $A\setminus B$ and/or $B\setminus A$) %(the size of the set difference $A\Delta B$) 
% %
and the performances of all the algorithms we considered in~\autoref{subsec:recon-perf} are independent 
of the partitions of elements in $A\Delta B$ except for Graphene~\cite{Ozisik2019}, 
for which this is the best scenario. 

\begin{comment}


\subsection{Evaluation of Our ToW Estimator}\label{subsec:est-perf}

In this section, we compare our ToW estimator with two existing algorithms: Strata~\cite{Eppstein_WhatsDifference?Efficient_2011} and min-wise hashing~\cite{Broder_MinWiseIndependent_2000}, which we have described in~\autoref{subsec:est-bench} in detail. In the comparisons, we fix the size of the union $A\cup B$ to 100K and set the value of 
$t$ (the size of the set difference $A\Delta B$) varying from 10 to 10K (or in other words, $t/|A\cup B|$ varying from $10^{-4}$ to $10^{-1}$). 

For our ToW estimator and min-wise hashing, we used  \code{xxHash} hash functions~\cite{Collet_xxHashExtremelyfast_}. 
For Strata, we used the optimized open-source implementation of IBFs~\cite{Ozisik2019}. 

\subsubsection{ToW Estimator: Empirical vs. Analytical}

We first evaluate the empirical accuracy of our ToW estimator against its theoretical accuracy, since 
as mentioned in~\autoref{subsec:ToW} the hash family for calculating the ToW sketches should be 
four-wise independent to achieve the theoretical accuracy whereas \code{xxHash} might not be. 
We use the relative root mean square error (rRMSE) from the ground truth as the metric. 
%The accuracy is measured by the relative root mean square error (rRMSE) from the ground truth. 
For each value of $t$ (the set-difference size), 
we created $c=$1,000 different pairs of $A$ and $B$ and obtained estimates $\{\hat{t}_i\}_{i=1}^{c}$ using our ToW estimator. %For each estimate $\hat{t}_i$ ($i=1,2,\cdots,c$). 
We calculated the empirical rRMSE, which is defined as,
\begin{equation}
\mbox{\texttt{rRMSE}}(\hat{t})=\frac{1}{t}\sqrt{\frac{1}{c}\sum\limits_{i=1}^c(\hat{t}_i-t)^2}.
\end{equation}

% % Need to check whether "perfect" is the right word.
% In~\autoref{}, we have analyzed the accuracy (variance) of our ToW estimator assuming that the hash functions are perfect. 
% However, the hash functions used in practice are generally not perfect. 
As analyzed in~\autoref{subsec:ToW}, given the ground truth $t$ of the set-difference size, 
the variance of our ToW estimator with $k$ sketches is $\frac{2t^2-2t}{k}$. 
Therefore, the analytical rRMSE of our ToW estimator is $\frac{1}{t}\sqrt{\mbox{\bf Var}(\hat{t})}\!=\!\sqrt{\frac{2}{k}(1-\frac{1}{t})}$. 

\autoref{fig:rrmse} reports the empirical and analytical rRMSE of our ToW estimator. We only present the 
results for $t=10$ (\autoref{fig:rrmse-10}) and $t=\num{10000}$ (\autoref{fig:rrmse-10000}), since the 
empirical results are nearly identical to the analytical results under all different values of $t$,  
like what have been shown in \autoref{fig:rrmse-10} and \autoref{fig:rrmse-10000}. 

% \begin{figure}
% \centering
% \includegraphics[width=0.49\textwidth]{figures/estimator/rrmse}
% \caption{rRMSE of ToW.}\label{fig:rrmse}
% \end{figure}


\begin{figure}
\centering
\begin{subfigure}[t]{0.25\textwidth}
    \centering
    \includegraphics[width=1.0\textwidth]{figures/estimator/rrmse_10}
    \caption{t=10.}\label{fig:rrmse-10}
\end{subfigure}%
\begin{subfigure}[t]{0.25\textwidth}
    \centering
    \includegraphics[width=1.0\textwidth]{figures/estimator/rrmse_10000}
    \caption{t=\num{10000}.} \label{fig:rrmse-10000} %%%%%
\end{subfigure}
\caption{rRMSE of ToW.}\label{fig:rrmse}
\end{figure}

% 121	1.30000000000000
% 113	1.31000000000000
% 106	1.32000000000000
% 100	1.33000000000000
% 94	1.34000000000000
% 89	1.35000000000000
% 84	1.36000000000000
% 80	1.37000000000000
% 75	1.38000000000000
% 72	1.39000000000000
% 68	1.40000000000000
% 65	1.41000000000000
% 62	1.42000000000000
% 59	1.43000000000000
% 56	1.44000000000000
% 54	1.45000000000000
% 52	1.46000000000000
% 49	1.47000000000000
% 47	1.48000000000000
% 46	1.49000000000000
% 44	1.50000000000000

% \subsubsection{Correction Overheads}
\subsubsection{ToW Estimator vs. Prior Estimators}

The objective of an estimator for the set-difference size $t$ in the context of 
set reconciliation is to provide estimates with high-enough accuracy. 
On one hand, if the estimator over-estimates, the subsequent reconciliation will 
usually waste unnecessary bandwidth. 
On the other hand, if the estimator under-estimates, the reconciliation might fail. 
Hence, in practice, the estimate returned by the estimator is usually 
scaled up by a proper factor to ensure that the failure rarely happens. 


Now, we compare the scaling ratios, which we call the {\it correction overheads} like 
in~\cite{Eppstein_WhatsDifference?Efficient_2011}, of the three estimators. 
For each value of $t$, we created \num{10000} different pairs of $A$ and $B$, obtained 
estimates from the three estimators, and then calculated the required correction overhead 
for each estimator to ensure that 99\% estimates are larger than or equal to the ground 
truth. For Strata, we used the best parameters reported in~\cite{Eppstein_WhatsDifference?Efficient_2011} for 
our experimental configuration (the same as that in~\cite{Eppstein_WhatsDifference?Efficient_2011}): 
$3$ hash functions for each IBF, and $16$ strata each with $80$ cells. We note that this parameter 
setting assumes the approximate total set size ({\it i.e.,} 100K), or in other words the 
largest possible set-difference size $t_{max}$ is known a prior; Otherwise, more 
strata should be used. We assume that each ToW sketch takes $\lceil \log_2 (2t_{max} + 1)\rceil\!=\!18$ 
bits as each ToW sketch is an integer within the range of $[-t_{max},t_{max}]$. 
For our ToW estimator, we first calculate an approximate number of sketches required to achieve comparable 
correction overheads as Strata by using the central limit theorem (CLT) and then tune the exact number of 
sketches (we only tested the values of power of $2$ for saving time). For min-wise estimator, we use the 
same number of hashes as the number of sketches in our ToW estimator. 
The experimental results are reported in~\autoref{fig:co}. For ToW estimator and min-wise estimator, we only show the results for $k\!=\!128$ and $256$. 

\noindent
{\bf ToW vs. Strata}. As shown in~\autoref{fig:co}, our ToW estimator with $128$ sketches already 
achieves comparable correction overheads as Strata. Note that the estimates should be scaled up be a 
factor according to the worst case among all the points shown in~\autoref{fig:co} for each estimator. 
%as the ground truth of the set-difference size $t$ is not known a prior. 
That is, the estimates have 
to be scaled up by a factor (correction overhead) of $1.36$ and $1.38$ using Strata and 128-sketch ToW estimator 
respectively. If using 256 sketches, ToW estimator only requires this factor to be 
$1.25$. Now, we 
compare the space required by Strata and ToW estimator with 128 sketches. Our ToW estimator 
with 128 sketches only requires 288 bytes. As each cell in Strata 
requires 12 bytes (4 bytes for each field), the space required for Strata is 15 KB, which is around 
$53$ times of that of ToW estimator. 

\noindent
{\bf ToW vs. min-wise}. Now, we compare our ToW estimator with min-wise estimator. 
As shown in~\autoref{fig:co}, the correction overhead only becomes less than $3$ when 
$t$ gets larger than \num{7000} for the min-wise estimator with 128 hashes. Even when using 
256 hashes, min-wise estimator still requires this factor to be larger than 3 for most 
of the values (of $t$) we experimented. We note that for $t\leq 400$, 
most estimates returned from min-wise 
estimator is 0, which results in an infinite correction overhead. In fact, as reported in~\cite{Eppstein_WhatsDifference?Efficient_2011}, even when using thousands of hash functions (more precisely, 
\num{3840} hashes), 
min-wise estimator can still have an infinite correction overhead when $t\!<\!200$. 
Therefore, we conclude that min-wise estimator 
is not a feasible estimator for the set-difference size when $t\!\ll\! |A\cup B|$. 

\noindent
{\bf Summary}. Through the above comparisons with Strata and min-wise estimators, we conclude that 
our ToW estimator is much more space-efficient for achieving the same accuracy. Besides, the parameter 
setting for our ToW estimator is much easier. On one hand, 
our ToW estimator only has one parameter, 
{\it i.e.,} number of sketches, whereas Strata has 3 parameters ({\it i.e.,} number of 
strata, number of cells and number of hashes for each IBF). 
On the other hand, number of sketches (of ToW estimator) required for achieving a desired 
correction overhead is almost independent of $t$ and 
$|A|$ and $|B|$, whereas Strata should set the number of strata according to maximum possible 
set-difference size and number of hashes required by min-wise estimator 
for achieving a desired correction overhead is highly dependent on the ratio $t/|A\cup B|$. 



% \begin{figure}
% \centering
% \begin{subfigure}[t]{0.25\textwidth}
%     \centering
%     \includegraphics[width=0.99\textwidth]{figures/estimator/co_95}
%     \caption{95\%.}\label{fig:co95}
% \end{subfigure}%
% \begin{subfigure}[t]{0.25\textwidth}
%     \centering
%     \includegraphics[width=0.99\textwidth]{figures/estimator/co_99}
%     \caption{99\%.} \label{fig:co99} %%%%%
% \end{subfigure}
% \caption{Correction overheads of different estimators to ensure that at least 95\% and 99\% of the estimates are larger than or equal to the ground truth, respectively.}\label{fig:co}
% \end{figure}

\begin{figure}
\centering
    \centering
    \includegraphics[width=0.49\textwidth]{figures/estimator/co_99_with_minhash_v2}
\caption{Correction overheads of different estimators to ensure that at least 99\% of the estimates are larger than or equal to the ground truth.}\label{fig:co}
\end{figure}
\end{comment}

\subsection{Evaluation of Our Reconciliation Scheme}\label{subsec:recon-perf}

% % 
In this section, we evaluate the performance of our algorithm for set reconciliation, and compare 
it with Difference Digest (D.Digest)~\cite{Eppstein_WhatsDifference?Efficient_2011}, 
Graphene~\cite{Ozisik2019}, and Minisketch~\cite{naumenko2019bandwidth}, which we have 
described in detail in~\autoref{subsec:recon-bench}. 

Like in~\autoref{subsec:est-perf}, 
in the comparisons, we fix the size of the union $A\cup B$ to 100K and set the value of $t$ varying 
from 10 to 10K. For each value of $t$, we created \num{1000} different pairs of $A$ and $B$. 
All the experiments in this section were performed on a workstation with an Intel Core i7-9800X processor 
running Ubuntu 18.0.4.  


For D.Digest, as the authors of~\cite{Eppstein_WhatsDifference?Efficient_2011} did not 
release their source codes, we used the optimized open-source implementation of IBFs in C++ released by 
the authors of~\cite{Ozisik2019}. For Minisketch, we used its C++ implementation~\cite{Wuille_Minisketchoptimizedlibrary_2019}  
released by the authors of~\cite{naumenko2019bandwidth}. 
% Note that, Minisketch is just an optimized implementation of the PinSketch~\cite{Dodis_PinSketch_2008} 
% algorithm. 
For Graphene, we used the source codes provided by the authors of~\cite{Ozisik2019}. 
Note that, the implementation of Graphene is in Python. 
We implemented our scheme in C++: 
we used \texttt{xxHash}~\cite{Collet_xxHashExtremelyfast_} for the partition process 
and Minisketch for BCH encoding and decoding. 


\subsubsection{Our Scheme vs. Prior Work}\label{subsec:vs-prior}

% \begin{figure*}
% \centering
% \begin{subfigure}[t]{0.32\textwidth}
% \includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/communication_costs}
% \caption{Communication overheads.} %(excluding those of the ToW estimator).}
% \label{fig:communication-costs}
% \end{subfigure}%
% \begin{subfigure}[t]{0.32\textwidth}
% \includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/decoding_time}
% \caption{Decoding time.}
% \label{fig:decoding-time}
% \end{subfigure}%
% \begin{subfigure}[t]{0.32\textwidth}
% \includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/success_rate}
% \caption{Success rate.}
% \label{fig:success-rate}
% \end{subfigure}
% \caption{Comparisons our schemes against Minisketch and D.Digest.}% with at least 99\% success rate.}
% \label{fig:comp-old}
% \end{figure*}

\begin{figure*}
\centering
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/communication_costs}
\caption{Communication overheads.} %(excluding those of the ToW estimator).}
\label{fig:communication-costs}
\end{subfigure}%
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/encoding_time}
\caption{Encoding time.}
\label{fig:encoding-time}
\end{subfigure}%
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/decoding_time}
\caption{Decoding time.}
\label{fig:decoding-time}
\end{subfigure}%
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/success_rate}
\caption{Success rate.}
\label{fig:success-rate}
\end{subfigure}
\caption{Comparisons against Minisketch and D.Digest.}% with at least 99\% success rate.}
\label{fig:comp-old}
\end{figure*}

\noindent
{\bf Our Scheme vs. D.Digest and Minisketch}. We now compare our set reconciliation scheme 
against D.Digest and Minisketch. We used 128-sketch ToW estimator with 128 sketches for 
the estimation of $t$ for all these algorithms. 
For D.Digest, we used the parameter setting suggested by the authors of~\cite{Eppstein_WhatsDifference?Efficient_2011}: $2\hat{t}$ cells where $\hat{t}$ is the estimate of the set-difference size, 
and 3 hash functions for estimates less than 200; Otherwise we used 4 hash functions. 
Note that with this parameter setting, D.Digest can roughly ensure a success rate of 
at least 0.99, that is, for at least 99\% of the instances that we experimented, all elements should be successfully recovered. For Minisketch, we scaled up the estimates 
by 1.38 so that it can also ensure a success rate of 0.99. For our scheme, 
we set the average number of ``bad balls'' in each bin (elements in the set difference $A\Delta B$) 
to $5$ and whenever any bin fails to decode (which happens with tiny probability), 
we decomposed the bin in to three. We used the same BCH parameters 
(BCH code length and decoding capacity) for all bins, the 
values of which was obtained as follows. 
We first scaled up the estimates by 1.38. Then, based on the scaled estimates 
(assuming they are the true values), 
we computed the best parameters that can ensure a success rate of at least 
0.99 with 2 or 3 rounds (excluding the set-difference size estimation round) 
using our analytical results in~\autoref{sec:tail_bound}. Therefore, our scheme 
also roughly ensures a success rate of 0.99. 

% \autoref{fig:comp-old} presents the amount of data transfered (\autoref{fig:communication-costs}), the decoding time (\autoref{fig:decoding-time}), and the empirical 
% success rate (\autoref{fig:success-rate}) of Minisketch, D.Digest, and our scheme with 2 and 3 rounds. 

\autoref{fig:communication-costs} presents the amount of communication overheads of 
Minisketch, D.Digest, and our scheme (with 2 and 3 rounds). 
We note that the communication overhead of the estimator is excluded since 
it is constant (288 bytes) and the same for these algorithms. 
Results confirm that all these algorithms have the same 
asymptotic communication complexity, that is $O(t)$. However, the constant factors are different and do 
matter in practice. D.Digest is the worst, which requires 24 bytes per element in the set difference. 
Minisketch is the best, which only requires around 5.52 bytes per element. These values for 
our scheme with 2 and 3 rounds are 9.97 to 14.15 and 8.60 to 10.67 respectively. 

\autoref{fig:encoding-time} shows their encoding times. The results show that our scheme 
% (especially when using 3 rounds) 
has the lowest encoding time under all values of $t$. 
The results also show that the encoding time of our scheme increases as $t$ increases. 
This is because the encoding time mainly consists of two parts in our scheme: the partition process and 
the BCH encoding. The former is independent of $t$, which has a computational complexity 
of $O(|A|+|B|)$ (1 hash operation per element). The latter has a computational complexity 
proportional to $t$ as the number of bins (subset pairs) increases almost linearly as $t$ and 
the encoding of each subset pairs has a constant computational complexity.  

\autoref{fig:decoding-time} shows their decoding times. The results show that 
the decoding time of D.Digest and our scheme increase roughly linearly along with $t$, whereas 
that of Minisketch increases roughly quadratically with $t$. The decoding time of 
Minisketch is much higher than those of D.Digest and our scheme when $t$ is large (say $\ge$ \num{1000}). 
For example, when $t=$\num{10000}, the decoding time of Minisketch is more than two orders of magnitude 
larger than those of D.Digest and our scheme. 

\autoref{fig:success-rate} shows that all the algorithms achieve an empirical success rate for all 
the different values of $t$ except that the success rate of D.Digest are slightly lower than 0.99 when 
$t\!<\!100$. 


\noindent
{\bf Our Scheme vs. Graphene}. 
Then, we compare our scheme against Graphene. 
We separate the comparisons against Graphene from those against others for two reasons. 
First, Graphene does not require an estimator. 
Second, we only have the pre-computed parameters (provided by the authors of~\cite{Ozisik2019}) 
optimized for a success rate of 239/240 instead of 0.99. 
For fair comparisons, we set the parameters for our scheme to roughly ensure a success rate of 239/240, 
though, as shown in~\autoref{fig:success-rate}, our scheme already achieves this success rate empirically by 
using parameters calcluated for ensuring a success rate of 0.99. 
As shown~\autoref{fig:success-rate-vs-graphene}, both Graphene and our scheme have achieved success rates higher 
than 239/240 empirically. 

\autoref{fig:comm-cost-vs-graphene} presents the communication overheads of Graphene and our scheme (with 
2 and 3 rounds). For our scheme, we include those for our ToW estimator. 
The eesults show that our scheme has lower communication overheads than Graphene 
under almost values of $t$ except for those close to \num{10000} 
where our scheme has slightly higher communication overheads than Graphene. 
The results also show that the average 
communication per element in the set difference gets smaller for Graphene. 
For $t\!<\!$\num{1000}, it is mainly because the IBF requires less cells per 
element as $t$ gets larger to ensure the same success rate, as shown in Figure 7 
of~\cite{Eppstein_WhatsDifference?Efficient_2011}. When $t\ge 1000$, the average number of cells per 
element is almost independent of $t$ (remains the same as $t$ increases). The average communication 
per element (in the set difference) continues to decrease 
because when $t$ is large enough the BF in Graphene can help 
reduce the number of cells required by the IBFs thus resulting in a lower communication overhead per 
element in the set difference.  

We note that the scenarios (more precisely, the partition scenarios of elements in $A\Delta B$) are the best 
cases for Graphene. In more general cases ({\it i.e.,} $B$ is not a subset of $A$), the communication overheads 
of Graphene would be higher than those we reported in~\autoref{fig:comm-cost-vs-graphene}. 

We did not compare the encoding and decoding time of 
our scheme against Graphene because Graphene is implemented in Python, whereas our scheme is implemented in C++.  
% We note that the asymptotic encoding computational complexity is the same as that of our scheme and 
% its decoding computational complexity is 

% for two reasons. 
% First, asymptotically, 
% its decoding complexity is $O(|A|+|B|)$ which is much higher than $O(t)$, 
% the asymptotic decoding complexity. Second, 
% Graphene is implemented in Python, whereas our scheme is implemented in C++.  
% Though we found that the encoding and decoding time of our scheme is shorter than 
% those of Graphene, it is fair for Gra

% \begin{figure*}
% \centering
% \begin{minipage}{0.32\textwidth}
% \includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/communication_costs}
% \caption{Communication overheads.}
% \label{fig:communication-costs}
% \end{minipage}%
% \begin{minipage}{0.32\textwidth}
% \includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/decoding_time}
% \caption{Decoding time.}
% \label{fig:decoding-time}
% \end{minipage}%
% \begin{minipage}{0.32\textwidth}
% \includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/success_rate}
% \caption{Success rate.}
% \label{fig:success-rate}
% \end{minipage}
% \end{figure*}



\begin{figure}
\centering
\begin{subfigure}[t]{0.25\textwidth}
    \centering
    \includegraphics[width=1.0\textwidth]{figures/reconciliation/success-rate-239-240/communication_costs_vs_Graphene_v2}
    \caption{Communication overheads.}% (including those of the ToW estimator).}
    \label{fig:comm-cost-vs-graphene}
\end{subfigure}%
\begin{subfigure}[t]{0.25\textwidth}
    \centering
    \includegraphics[width=1.0\textwidth]{figures/reconciliation/success-rate-239-240/success_rate_vs_Graphene_v2}
    \caption{Success rate.} \label{fig:success-rate-vs-graphene} %%%%%
\end{subfigure}
\caption{Comparisons against Graphene.}\label{fig:vs-graphene}
\end{figure}

\begin{comment}
\noindent
{\bf Is multiple rounds a issue?} Readers might think that our scheme might have longer latency 
than D.Digest and Minisketch, as they only require 1 round whereas our scheme requires more 
than 1. However, multiple rounds will not increase the latency of our scheme. 
To support it, we present the ratio of the number of elements successfully recovered in each round 
of our scheme in~\autoref{fig:recovered-ratio}. For our scheme running 2 rounds (or 3 rounds), more than 97\% (or 95\%) of elements 
in the set difference are successfully recovered in the first round. Therefore, the underlying synchronization 
process ({\it e.g.,} file synchronization) can start immediately after the first round of our scheme and do not need to wait until our reconciliation algorithm finishes. 
\end{comment}

% \noindent
% {\bf Per-Round Performance of Our Scheme.} 
% % Readers might think that our scheme might have longer latency 
% % than D.Digest and Minisketch, as they only require 1 round whereas our scheme requires more 
% % than 1. However, multiple rounds will not increase the latency of our scheme. 
% Now, we investigate the per-round performance of our scheme. 
% We present the ratio of the number of elements successfully recovered in each round 
% of our scheme in~\autoref{fig:recovered-ratio}, which shows that 
% our scheme running 2 rounds (or 3 rounds) can successfully recover more than 97\% (or 95\%) of elements 
% in the set difference in the first round. Therefore, the underlying synchronization 
% process ({\it e.g.,} file synchronization) can start immediately after 
% the first round of our scheme and do not have to wait until the set reconciliation finishes. 

\noindent
% {\bf Per-Round Performance of PBS.} 
{\bf Piecewise Decodability of PBS.}
% Readers might think that our scheme might have longer latency 
% than D.Digest and Minisketch, as they only require 1 round whereas our scheme requires more 
% than 1. However, multiple rounds will not increase the latency of our scheme. 
% Now, we investigate the per-round performance of PBS. 
Recall from~\autoref{sec:intro} that the only minor tradeoff of PBS is that the number of 
rounds (of message exchanges) needed by PBS is slightly larger than existing solutions. \autoref{fig:avg-num-rounds} 
presents the average number of rounds required by PBS with $r\!=$ 2 or 3 respectively. 
However, thanks to the piecewise decodability (that existing solutions do not have), the vast majority 
of all distinct elements are successfully reconciled in the first round. 
The ratio is presented in~\autoref{fig:recovered-ratio}, which shows that 
PBS with $r\!=$ 2 (or 3) can successfully reconcile more than 97\% (or 95\%) of all the distinct elements 
in the first round. Therefore, this tradeoff does not lead to longer response time because the reconciliation of objects identified
the successfully decodable ``codewords'' (hash signatures) can run in parallel with the transmissions and decodings of the rest. 

% the underlying synchronization 
% process ({\it e.g.,} file synchronization) can start immediately after 
% the first round of our scheme and do not have to wait until the set reconciliation finishes. 


We note that only those instances in which all distinct elements are successfully 
reconciled are considered in~\autoref{fig:avg-num-rounds} and~\autoref{fig:recovered-ratio}. 
Unlike in the existing solutions where nothing can be reconciled in the failed instances\footnote{We note that ``piecewise decodability'' can be also achieved in IBF-based solutions, as IBF-based solutions can also decode part of the distinct elements when decoding fails. However, on one hand, no existing solutions even mention this. On the other hand, the ``piecewise decodability'' of IBF-based solutions is much less efficient than that of PBS.}, the vast majority of 
all distinct elements are successfully reconciled in those failed instances in PBS because of its piecewise decodability. 
Furthermore, through experiments, 
we found that the rest distinct elements in those failed instances can be successfully reconciled with one more round of message exchanges  
({\it i.e.,} running one more round of PBS), and only negligible communication overhead incurred (thanks to piecewise decodability). In other words, failed instances lead to 
negligible penalties in PBS, whereas, in all the existing solutions, failed instances would result in hefty penalties, as they do not have 
piecewise decodability.


% \begin{figure}
% \centering
% \begin{subfigure}[t]{0.25\textwidth}
%     \centering
%     \includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/portion_recovered_max_round2_curve}
%     \caption{r=2.}\label{fig:recovered-ratio-r2}
% \end{subfigure}%
% \begin{subfigure}[t]{0.25\textwidth}
%     \centering
%     \includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/portion_recovered_max_round3_curve}
%     \caption{r=3.} \label{fig:recovered-ratio-r3} %%%%%
% \end{subfigure}
% \caption{Recovered ratio in each round.}\label{fig:recovered-ratio}
% \end{figure}

\begin{figure}
\centering
\begin{minipage}[t]{0.23\textwidth}
    \centering
    \includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/pbs_avg_rounds_wrl}
    \caption{Average number of rounds.} \label{fig:avg-num-rounds} %%%%%
\end{minipage}
\hspace{0.01\textwidth}%
\begin{minipage}[t]{0.23\textwidth}
    \centering
    \includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/pbs_first_round}
    \caption{Recovered ratio in the first round.}\label{fig:recovered-ratio}
\end{minipage}%
% \caption{Recovered ratio in each round.}\label{fig:recovered-ratio}
\end{figure}

% \begin{figure}
% \centering 
% \includegraphics[width=0.5\textwidth]{figures/reconciliation/success-rate-99/communication_costs_verying_key_sizes_d10000}
% \caption{Communication overheads (excluding those of the ToW estimator) of Minisketch, D.Digest, and our schemes under various key sizes.}\label{fig:varying-key-sizes}
% \end{figure}
\subsubsection{Varying Key Sizes}\label{sucsec:varying-key-sizes}

In real applications, the key size (length of each element in the universe) might be much higher than 
4 bytes. For example, the transaction ID in Bitcoin applications could 
have 256 bytes~\cite{naumenko2019bandwidth}. 
We investigate how the communication overhead of each algorithm changes as the key size $u$ increases. 
We consider key sizes varying from 4 bytes to 256 bytes. 
Same as before, we separate the comparisons 
against D.Digest and Minisketch and those against Graphene. 
The results are shown in~\autoref{fig:cc-comp-vk} and~\autoref{fig:cc-comp-vk-vs-graphene} respectively. 

Same as before, for the results in~\autoref{fig:cc-comp-vk}, we make each algorithm ensure a success rate of 
0.99 and exclude the communication required by the estimator for all algorithms. For those in~\autoref{fig:cc-comp-vk-vs-graphene}, we make our scheme and Graphene ensure a success rate of 239/240 and include 
the communication required by the estimator for our scheme (note that Graphene does not require an estimator). 

As shown in~\autoref{fig:cc-comp-vk} and~\autoref{fig:cc-comp-vk-vs-graphene}, our scheme has the best 
scaling behavior among all these algorithms. For D.Digest and Minisketch, the communication overheads double 
as the key size doubles, whereas the communication overhead increases much slower in our scheme 
as the key size increases. 
For Graphene, when $t\!=\!$\num{100} and $t\!=\!$\num{1000}, its scaling behavior is almost the same as D.Digest, since as explained in~\autoref{subsec:recon-bench}, Graphene almost reduces to an IBF-only solution when $t\ll|A\cup B|$. When $t=$\num{10000}, the scaling behavior is very close to that of our scheme, as now the communication overheads resulting from IBFs in Graphene is around 40\% and those for the BFs do not increase as the key size. 

\begin{figure*}[!htbp]
\centering
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/communication_costs_verying_key_sizes_d100}
\caption{t=100.}
\label{fig:-d100}
\end{subfigure}%
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/communication_costs_verying_key_sizes_d1000}
\caption{t=\num{1000}.}
\label{-d1000}
\end{subfigure}%
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/communication_costs_verying_key_sizes_d10000}
\caption{t=\num{10000}.}
\label{fig:-d10000}
\end{subfigure}
\caption{Communication overheads of Minisketch, D.Digest, and our schemes under various key sizes.}% with at least 99\% success rate.}
\label{fig:cc-comp-vk}
\end{figure*}

\begin{figure*}[!htbp]
\centering
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-239-240/vs_graphene_verying_key_sizes_d100}
\caption{t=100.}
\label{fig:vs-graphene-d100}
\end{subfigure}%
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-239-240/vs_graphene_verying_key_sizes_d1000}
\caption{t=\num{1000}.}
\label{fig:vs-graphene-d1000}
\end{subfigure}%
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-239-240/vs_graphene_verying_key_sizes_d10000}
\caption{t=\num{10000}.}
\label{fig:vs-graphene-d10000}
\end{subfigure}
\caption{Communication overheads of Graphene and our schemes under various key sizes.}% with at least 99\% success rate.}
\label{fig:cc-comp-vk-vs-graphene}
\end{figure*}

\subsubsection{What If Minisketch Also Uses Partitions?}\label{subsec:mini-partition}

The success we have with our scheme leads readers to wonder what if we apply the partition 
idea to Minisketch. For example, like in our scheme, we partition all elements into several subsets 
so that each subset contains a few elements (say $5$) on average from the set difference. Then, for 
each subset we create BCH codes with a capacity large enough so that we can ensure a desired success rate. 
We refer to this new scheme as Minisketch With Partition, or Minisketch/WP for short. 

We compare the performances of our scheme with those of Minisketch/WP with a desired success rate of 
0.99. For Minisketch/WP, we set the average number of elements from the set difference to $5$ (same 
as our scheme) and use the same BCH decoding capacity for all subsets. We tune this capacity to the best: 
the one with the minimum communication overhead yet ensures a success rate of at least 0.99.    

\autoref{fig:cc-comp-vs-minisketchwp} presents the communication overheads under different key sizes varying 
from 4 bytes to 256 bytes for three different set-difference sizes \numlist{100;1000;10000}. 
The sesults show that Minisketch/WP has similar or 
slightly lower communication overheads than our scheme only when the key size is 4 bytes. This advantage 
diminishes as the key size gets larger and our scheme is consistently better when the key size is no less than 
$16$ bytes. Hence, we conclude that our scheme overall remains the best practical solution for the 
set reconciliation problem.




% \begin{figure*}[!htbp]
% \centering
% \begin{subfigure}[t]{0.32\textwidth}
% \includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/vs_minisketchwp_verying_key_sizes_d100}
% \caption{t=\num{100}.}
% \label{fig:vs-minisketchwp-d100}
% \end{subfigure}%
% \begin{subfigure}[t]{0.32\textwidth}
% \includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/vs_minisketchwp_verying_key_sizes_d1000}
% \caption{t=\num{1000}.}
% \label{fig:vs-minisketchwp-d1000}
% \end{subfigure}%
% \begin{subfigure}[t]{0.32\textwidth}
% \includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/vs_minisketchwp_verying_key_sizes_d10000}
% \caption{t=\num{10000}.}
% \label{fig:vs-minisketchwp-d10000}
% \end{subfigure}
% \caption{Communication overheads of our schemes against those of Minisketch/WP.}% with at least 99\% success rate.}
% \label{fig:cc-comp-vs-minisketchwp}
% \end{figure*}

\begin{figure*}[!htbp]
\centering
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/vs_minisketchwp_match_varying_key_sizes_d100}
\caption{t=\num{100}.}
\label{fig:vs-minisketchwp-d100}
\end{subfigure}%
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/vs_minisketchwp_match_varying_key_sizes_d1000}
\caption{t=\num{1000}.}
\label{fig:vs-minisketchwp-d1000}
\end{subfigure}%
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/vs_minisketchwp_match_varying_key_sizes_d10000}
\caption{t=\num{10000}.}
\label{fig:vs-minisketchwp-d10000}
\end{subfigure}
\caption{Communication overheads of our schemes against those of Minisketch/WP.}% with at least 99\% success rate.}
\label{fig:cc-comp-vs-minisketchwp}
\end{figure*}


==> section/evaluation-BK0220.tex <==
\section{Performance Evaluation}\label{sec:evaluation}
%% Experiments for estimators

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% Task 1.1: Experiments %%%%%%%%%%%%%%%%%%%%%%%%
%==> I will start (and hopefully complete) this experiments by the mid-night of Nov. 17, 2019. ---- Long
%%% Benchmark estimators: Strata Estimator/min-hash/Bagminhash 
%%% MSE (??) plus Correction overhead
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%% Experiments for Reconciliation

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% Task 1.2: Experiments %%%%%%%%%%%%%%%%%%%%%%%%
%==> I need some time to figure out how to use (or even modify) the source codes of Graphene ---- Long
%==> Hopefully, I can finish this part by the end of the next week (Nov. 22, 2019)
%%% Benchmark algorithms: minisketch/Graphene/KeyDiff
%%% 99% (??) reconciliation correction rate in one round (CO v.s. d) with roughly the same computational complexity 
%%% 95% (??) decoding rate in one round (CO v.s. d)
%%% multiple rounds for our scheme (maybe also for minisketch)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% Task 2.1: Writing %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%==> While conducting those experiments, I will also add the paragraphs for evaluation.   --- Long
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% Task 2.2: Writing %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%==> I have added a few more papers on this topic. If you (@ziheng) have  some time, you can help us add some sentences regarding them in the  related work section. I will also read them and try to produce some paragraphs.  --- Long
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%% To ZiHeng %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%==> If you have any suggestions of concerns regarding the above plan, please feel free to ``shoot'' to us. ---- Long
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% In this section, we evaluate the performances of our ToW estimator 
% and our set reconciliation algorithm.

% % 
In this section, we evaluate the performance of PBS, and compare 
it with Difference Digest (D.Digest)~\cite{Eppstein_WhatsDifference?Efficient_2011}, 
Graphene~\cite{Ozisik2019}, and PinSketch~\cite{Dodis_PinSketch_2008}, which we have 
described in detail in~\autoref{sec:related}. 

% {\bf A short paragraph summarizes the conclusions of the evaluation}

The following conclusions are drawn from this evaluation. 


First, PBS strikes much better balance between communication and overheads than all existing work. 
It has a communication overhead much lower than IBF-based techniques such as D.Digest and Graphene, 
but only slightly higher than that of PinSketch. 
In terms of computational overhead, it is the best. 
% Second, The piecewise decodability of PBS, 
% % which all existing set reconciliation algorithms do not have,  
% which none of existing set reconciliation algorithms has, 
% significantly reduces the penalty when failure happens. 

Second, results for communication overheads 
of these algorithms 
scaling {\it w.r.t.} signature width $\log|\mathcal{U}|$, shown in~\autoref{subsubsec:varying-sig-width} 
and \autoref{subsec:vs-graphene-sig}, conclusively demonstrated that PBS 
scales the best %{\it w.r.t.} signature width $\log |\mathcal{U}|$ 
making it an excellent candidate for applications that have large signature widths. 
% Fourth, To ensure the same success rate, less rounds (as low as 2 rounds) can be achieved in PBS by paying only marginal cost.  

% \subsection{Methodologies}\label{subsec:exp-methodologies}

\subsection{Experiment Setup}\label{subsec:exp-setup}

% In our evaluation, we first fix signature width $w$ (see~\autoref{sec:model}) 
% as $32$ bits. 

We first evaluate a key space (universe) $\mathcal{U}$ of $32$-bit binary strings, 
{\it i.e.,} $\log|\mathcal{U}|\!=\!32$, in the rest of~\autoref{sec:evaluation} 
except in~\autoref{subsubsec:varying-sig-width} and~\autoref{subsec:vs-graphene}, 
where we evaluate how the communication overheads 
of these algorithms 
scale with respect to $\log|\mathcal{U}|$.  
%
% Besides these two, a third 
% degree of freedom is how many distinct elements in $A\Delta B$ are from $A$ (or $B$).  
% We defer the explanation of why we do not exercise this degree of freedom later in~\autoref{subsubsec:discussion}. 
%
Like in~\cite{Eppstein_WhatsDifference?Efficient_2011}, each pair of sets, 
$A$ (stored at Alice) and $B$ (stored at Bob), was created as follows. 
% was created by exercising two degrees of freedom: the number of elements in $A$, 
% and the size $d$ of the set difference $A \Delta B$. 
% First, we drawn $10^5$ elements from the universe $\mathcal{U}$ 
% uniformly at random without replacement, 
% which made up the set $A$. 
First, elements in $A$ were drawn from %the universe 
$\mathcal{U}$ 
uniformly at random without replacement. 
A certain number %(more precisely, $|A|\!-\!d$) 
of elements in $A$ were then sampled also 
uniformly at random without replacement  
and made up set $B$ so that the set difference $A\Delta B$ 
contains exactly $d$ elements. 
In such a setting, 
% set $B$ contains no distinct elements, {\it i.e.,} 
we have $B\subset A$ and $A\Delta B\!=\!A\setminus B$.  
In other words, $A$ contains all distinct elements and $B$ contains none. 
As will be elaborated in~\autoref{subsubsec:discussion}, this scenario is enough for our evaluation. 
% We defer the explanation of why we do not consider the scenarios where 
% $B$ also contains some distinct elements later in~\autoref{subsubsec:discussion}. 
In all experiments, we fixed the cardinality of $A$ to $10^5$ and 
let the value of $d$ vary from $10$ to $10^4$. 
% 
For each value of $d$, we created \num{1000} mutually independent experiment instances (pairs of $A$, $B$). %, which are mutually independent.   
Each point in our plots in the evaluation results  
is the average of the corresponding \num{1000} independent experiment instances. 
%
All experiments were performed on a workstation with an Intel Core i7-9800X processor 
running Ubuntu 18.0.4. 
%
% ++++ {\bf The following sentence can be removed if we have defined success rate before.} 
%
Like in~\cite{Eppstein_WhatsDifference?Efficient_2011,Ozisik2019}, we consider an experiment instance for an algorithm 
successful only if Alice is able to correctly determine $A\Delta B$. 

Like in most set reconciliation literature, our evaluation mainly focused on 
two performance metrics: {\it communication overhead} and {\it computational overhead} (more precisely, encoding time and decoding time). 
As mentioned earlier in~\autoref{sec:intro}, 
we only considered the unidirectional set reconciliation in which Alice learns $A\Delta B$. %in all evaluated algorithms 
% except Graphene, in which we let Alice learn $A\Delta B$.  
Hence, communication overhead was measured by the total amount of data 
transmitted between Alice and Bob to ensure that Alice %Bob (or Alice in Graphene) 
learns $A\Delta B$. The computational overhead was measured similarly. 
We emphasize that, given sets $A$ and $B$, communication and computational overheads are independent 
of whom (Alice or Bob) learns $A\Delta B$ in the 
unidirectional set reconciliation in all evaluated algorithms except Graphene. 
As we will explain later in~\autoref{subsubsec:discussion}, this scenario 
({\it i.e.,} $B\subset A$ and Alice learns $A\Delta B$) is 
the best 
scenario for Graphene. Therefore, we have treated Graphene more than fairly. 

Note that for algorithms that need multiple rounds of message exchanges, including PBS, 
both communication overhead and computational overhead shown in the evaluation results %~\autoref{subsec:recon-perf} 
are the sum over all these rounds. 

\subsubsection{About Estimator}\label{subsubsec:est-setup}
Our evaluation assumed that the set difference cardinality $d$ is not known a prior, which is common in many applications. 
As mentioned in~\autoref{subsec:ToW}, we used the ToW estimator with 128 sketches whenever it is required. 
We note that all evaluated algorithms except Graphene require  
an estimator. For these algorithms, in all plots for their communication overheads shown in the evaluation results, 
% the amount of 
the overhead resulted from the ToW estimator, 
more precisely 288 bytes\footnote{We assume that each ToW sketch takes $\lceil \log_2 (2d_{max} + 1)\rceil\!=\!18$ 
bits as each ToW sketch is an integer within the range of $[-d_{max},d_{max}]$, where $d_{max}\!=\!10^5$ is the 
largest possible set difference cardinality,  
like in~\cite{Eppstein_WhatsDifference?Efficient_2011}, we assume it is known a prior.},  
was excluded. For fair comparison, we subtracted the same  
amount ({\it i.e.,} 288 bytes) from the communication overheads of Graphene. %as it does not require an estimator. 

\begin{comment}
\subsubsection{Parameter Configurations}\label{subsubsec:configuration}

Our evaluation assumed that the set difference cardinality $d$ is not known a prior, which is common in many applications. 
++++ {\bf Although Prof. Jim has suggested to write a similar short paragraph (to emphasize ToW is the best) in the estimator section, 
I still think it is more natural to mention it here, because we have to give necessary details on the experiments of estimators here.} 
We used a ToW estimator with 128 sketches ({\it i.e.,} $k\!=\!$128) to 
obtain an estimate $\hat{d}$ of $d$ in our evaluation 
whenever a set reconciliation algorithm requires an estimator, because 
the ToW estimator was shown, through experiments (the results were not shown here in the interest of space), 
to have the best overall performance among all commonly used estimators ({\it e.g.,} the Min-wise 
estimator~\cite{Broder_MinWiseIndependent_2000} and the Strata estimator~\cite{Eppstein_WhatsDifference?Efficient_2011}) 
in terms of space-efficiency, accuracy, and implementation complexity. 
Recall from~\autoref{subsec:ToW} that in many applications, the estimate $\hat{d}$ is usually scaled up 
by a proper factor $\gamma$ so that the scaled estimate $\gamma\hat{d}$ is no smaller than the ground 
truth $d$ with a high enough probability $\beta$, {\it i.e.,} $\mathbf{P}[\gamma \hat{d} \ge d]\ge\beta$. 
Through experiments, we investigated the smallest factors ($\gamma$'s) of ToW estimators for 
various assurance probabilities ($\beta$'s). For example, the smallest $\gamma$ is $1.38$ when $\beta\!=\!0.99$.  
% {\it i.e.,} $\mathbf{P}[1.38\hat{d}\!\ge\! d]\!\ge\!0.99$. % with a probability of at least 0.99. 
% For example, through experiments, we found to make $\beta\!=\!0.99$, 
% {\it i.e.,} $\alpha\hat{d}\!\ge\! d$ with a probability of at least 0.99, $\alpha$ 
% should be set to $1.38$. 
% Like in~\cite{Eppstein_WhatsDifference?Efficient_2011}, the estimate $\hat{d}$ is scaled up 
% by a proper factor (1.38 in our evaluation) so that the scaled estimate is no smaller than the ground 
% truth with a high enough probability (99\% in our evaluation). 
We note that all evaluated algorithms except Graphene require  
an estimator. For these algorithms, in all plots for their communication overheads shown in the evaluation results, 
% the amount of 
the overhead resulted from the ToW estimator, 
more precisely 288 bytes\footnote{We assume that each ToW sketch takes $\lceil \log_2 (2d_{max} + 1)\rceil\!=\!18$ 
bits as each ToW sketch is an integer within the range of $[-d_{max},d_{max}]$, where $d_{max}\!=\!10^5$ is the 
largest possible set difference cardinality,  
like in~\cite{Eppstein_WhatsDifference?Efficient_2011}, we assume it is known a prior.},  
was excluded. For fair comparison, we subtracted the same  
amount ({\it i.e.,} 288 bytes) from the communication overheads of Graphene, as it does not require an estimator. 


% We note that all of the evaluated algorithms might fail, {\it i.e.,} they cannot determine all 
% the distinct elements in some instances. 
% We note that e
Each of the evaluated algorithms might fail. 
% to determine all of the distinct elements in some 
% instances. 
For example, PinSketch fails if the true set difference cardinality $d$ is larger than its BCH decoding 
capacity $t$.  
% As explained earlier in~\autoref{subsec:ToW}, 
++++ {\bf The following sentence can be simplified, if we have defined and explained success rate in previous section.} 
In real applications, 
a set reconciliation algorithm should be properly configured 
so that it has a high enough {\it success rate} (say $0.99$): The fraction of successful experiment instances among all instances. 
Clearly, a higher success rate requires ``higher price'' ({\it e.g.,} higher communication overhead and/or more rounds of message exchanges).  
To fairly compare these set reconciliation algorithms, we should properly configure their 
parameters so that they roughly have the same success rate. 
Unfortunately, in the paper of D.Digest~\cite{Eppstein_WhatsDifference?Efficient_2011}, the authors 
only suggested the parameter setting tuned for a success rate of roughly 0.99, whereas 
we only have the pre-computed parameter tables (provided by the authors of~\cite{Ozisik2019}) 
tuned for a success rate of roughly 239/240 ($\!\approx\!0.9958$) instead of 0.99. 
Tuning parameters of these algorithms is out scope of this paper,  
hence we 
% used the parameters suggested or provided by the corresponding authors and 
% configured our 
tuned the parameters of PBS 
to match their success rates respectively. 
In~\autoref{subsec:recon-perf}, we first compared PBS against D.Digest and PinSketch with each of 
them %configuring to ensure 
tuning for a success rate of roughly 0.99, and then we compared PBS against 
Graphene with each of them %configuring to ensure 
tuning for a success rate of roughly 239/240. 
Now, we describe, in detail, the parameter settings for all of them. 

\noindent
{\bf D.Digest}. 
% Like in~\cite{Eppstein_WhatsDifference?Efficient_2011}, 
% we allocated $3\log|\mathcal{U}|$ bits for each IBF cell in D.Digest, with $\log|\mathcal{U}|$ bits given to each of the three fields in a cell. 
We used the parameter setting suggested in~\cite{Eppstein_WhatsDifference?Efficient_2011} to roughly ensure a success rate of 0.99: 
$2\hat{d}$ IBF cells, where $\hat{d}$ is the estimate of the set difference cardinality, 
and $3$ hash functions for estimates greater than $200$; otherwise we used $4$ hash functions. 
% Recall from~\autoref{subsec:ToW} that the ToW estimator is unbiased, {\it i.e.,}
% % shown in~\autoref{eq:tow}, 
% $\mathbf{E}[\hat{d}]\!=\!d$, 
Therefore, 
the communication overhead of D.Digest is roughly $6d\log|\mathcal{U}|$ bits, which is $6$ times of the minimum.  
% As mentioned earlier in this section, 
% As shown in~\cite{Eppstein_WhatsDifference?Efficient_2011}, with this parameter setting, 
% D.Digest ensures a success rate of roughly 0.99. 
% That is, for roughly 99\% of the experiment 
% instances, the reconciliation should succeed. 

\noindent
{\bf PinSketch}. 
% For PinSketch, we 
We set the decoding capacity of the BCH code, the only parameter in PinSketch, to $t\!=\!1.38\hat{d}$.  
% Recall from~\autoref{sec:scheme} that, i
It is not hard to check the communication overhead of PinSketch, under this parameter 
setting, is roughly $1.38d\log|\mathcal{U}|$ bits, which is $1.38$ times of the minimum. 
As explained earlier in this section, 
$\mathbf{P}[1.38\hat{d}\!\ge\! d]\!\ge\!0.99$, thus, 
$\mathbf{P}[t\!\ge\! d]\!\ge\!0.99$. 
% by scaling up by a factor of 1.38, 
% the scaled estimate $1.38\hat{d}$ is no smaller than 
% the ground truth (the true set-difference size $d$) with a probability of at least 0.99, 
% {\it i.e.,} $t\!=\!1.38\hat{d}\ge d$ with a probability of at least 0.99. 
% Therefore, the decoding capacity $t$ would be no smaller 
% than the set-difference size $d$ with a probability of 0.99. 
% As explained earlier, 
Therefore, 
% the reconciliation should succeed   
% with a probability of at least 0.99. In other words, with this parameter setting, 
PinSketch %also 
ensures a success rate of at least 0.99. 

\noindent
{\bf Graphene}.
% Like we did for D.Digest, 
% we allocated $3\log|\mathcal{U}|$ bits for each IBF cell in Graphene, 
% with $\log|\mathcal{U}|$ bits given to each of the three fields in a cell. 
% For Graphene, 
We used the pre-computed parameter settings ({\it e.g.,} how many hash 
functions and cells should be used in the IBF)
provided by the authors of~\cite{Ozisik2019} tuned for a success rate of 239/240. 

\noindent
{\bf PBS}.  
% We set the maximum number of rounds, $r\!=\!3$. 
% Later, in~\autoref{subsec:recon-perf}, we investigated how the performances of PBS 
% scale with respect to $r$. 
% We set $\delta\!=\!5$.  
We first let the target success probability $p_0$=0.99 within $r$=3 rounds. %, {\it i.e.,} we let PBS to 
Later, in~\autoref{subsec:less-rounds}, we investigated how performances of PBS 
scale with respect to $r$. 
% we set $\delta$, the average number of distinct elements in each group,  
% to $5$. 
% We used the same $n$ ({\it i.e.,} number of subset pairs in each group), 
% and $t$ ({\it i.e.,} the decoding capability of the BCH codes) for all groups, the 
% values of which was obtained using our analytical results as follows. 
The values of $n$, number of subset pairs in each group, and $t$, 
BCH decode capability in each group, are set 
based on the set difference cardinality estimate $\hat{d}$ (as $d$ is not known).   
% differently for different set-difference size $d$.   
For each $\hat{d}$, we used the parameter setting procedure described 
in~\autoref{sec:parameter_settings} to obtain the values of $n$ and $t$,  
% tuning for a success 
% rate of at least $0.99$ 
by letting the set difference cardinality be the scaled estimate, {\it i.e.,} $1.38\hat{d}$. 
% In other words, if the true set-difference size $d\le 1.38\hat{d}$, PBS (within 3 rounds) should succeed with a 
% probability of at least $0.99$. Therefore, w
It is not hard to check, with this parameter setting,  
PBS strictly ensures a success rate of at least $0.99\times 0.99\!=\!0.9801$: The 
first $0.99$ comes from the assurance from the scaled estimates, {\it i.e.,} $\mathbf{P}[1.38\hat{d}\ge d]\ge 0.99$; 
the second $0.99$ comes from 
the rigorous tail bound derived in~\autoref{sec:tail_bound}. As shown in~\autoref{subsec:recon-perf},   
empirically, the success rates of PBS are much higher than $0.99$ under all different values of $d$. 
We refer to this parameter setting as ``the default setting'' for PBS in the sequel of this section. 
% Need revision
% Later, in~\autoref{subsec:recon-perf}, we investigated how the communication overheads of PBS scale with respect to $r$, 
% more precisely, the communication overheads of PBS ensuring a success rate of $0.99$ within $r$ rounds scale with respect to $r$. 

Similarly, we then tuned PBS to roughly ensure a success rate of $239/240$ 
% ({\it i.e.,} only changing the target success rate from 0.99 to 239/240, the rest remains exactly the same as the default setting) 
when comparing against Graphene. 
\end{comment}


\begin{comment}
% seems not quite useful
\autoref{tab:param-pbs} summarizes the values for all parameters in PBS.

\begin{table}
\centering
\caption{Parameters for PBS.}\label{tab:param-pbs}
\begin{tabular}{@{}|c|c|c|c|c|@{}}
\hline 
success rate & $\delta$ & $r$ & $n$ & $t$ \\ \hline 
roughly 0.99     &  \num{5} & \num{3} & \numlist[list-separator = {, },list-final-separator = {, or }]{63;127;255;511} &  \numrange{8}{13} \\ \hline
roughly 239/240  &  \num{5} & \num{3} & \numlist[list-separator = {, },list-final-separator = {, or }]{63;127;255;511} &  \numrange{8}{14} \\ 
\hline 
\end{tabular}
\end{table}
\end{comment}
% We first scaled up the estimates by 1.38. Based on the scaled estimates, 
% we computed the best parameters that can ensure a success rate of at least 
% 0.99 with 3 rounds of PBS
% using our analytical results in~\autoref{sec:tail_bound}. Therefore, our scheme 
% also roughly ensures a success rate of 0.99. 


\subsubsection{Implementations}\label{subsubsec:impl}

%% no consisent conventions on how to decribe implementations was found, but the majority used ``past tense''
We implemented PBS in C++. We used \texttt{xxHash}~\cite{Collet_xxHashExtremelyfast_} for all hash functions in PBS. 
The Minisketch library~\cite{Wuille_Minisketchoptimizedlibrary_2019}, released by the authors of~\cite{naumenko2019bandwidth}, was used for the BCH encoding and decoding in both PBS and PinSketch~\cite{Dodis_PinSketch_2008}. 
As the authors of D.Digest~\cite{Eppstein_WhatsDifference?Efficient_2011} have not 
released their source codes, we coded it using the optimized open-source implementation of IBFs in C++ released by 
the authors of~\cite{Ozisik2019}. 
%
% Note that, Minisketch is just an optimized implementation of the PinSketch~\cite{Dodis_PinSketch_2008} 
% algorithm. 
For Graphene, we used the source codes provided by the authors of~\cite{Ozisik2019}. 
% Note that, the implementation of Graphene is in Python. 


\subsubsection{Discussions}\label{subsubsec:discussion}

% Recall from the experiment setup in~\autoref{subsec:exp-setup}, 
% in our evaluation, we only considered 
% the scenario where set $B$ contains no distinct elements ({\it i.e.,} $B\subset A$). 
% % explain why we only exercise the above two degrees of freedom (need revision)
% We did not exercise the degree of freedom in varying the sizes of 
% $A\!\setminus\! B$ and $B\!\setminus\! A$ 
% As mentioned earlier, we only considered the scenario 
% This is enough for 
In this section, we explain why the scenario where $B\subset A$ is sufficient for our evaluation.   
% all estimators compared in~\autoref{subsec:est-perf} are designed for the estimation of 
% only $d$ (not the sizes of $A\setminus B$ and/or $B\setminus A$) %(the size of the set difference $A\Delta B$) 
% % %
% and 
Given $A$ and $d$, communication overhead and decoding time 
of all algorithms except Graphene~\cite{Ozisik2019} 
considered in our evaluation are independent 
of how distinct elements are distributed in $A$ and $B$. 
%
% except 
% for Graphene~\cite{Ozisik2019}. 
% {\bf Revision Required!!} 
% The encoding times of these algorithms will change in the same manner if we 
% change how many distinct elements are distributed in $A$ (or $B$) when $A$ and $d$ are fixed,  
% since, as described in~\autoref{subsec:recon-bench}, the encoding times of all these algorithms are proportional to $|A|\!+\!|B|$. 
%
The communication overhead of Graphene usually depends on how many distinct elements are distributed in 
$A$ (or $B$). However, 
% as shown in~\cite{Ozisik2019}, 
when $A$ and $d$ are fixed, 
the scenario  considered in our evaluation, where set $B$ is a subset of $A$ 
and Alice learns $A\Delta B$ corresponds to the 
% ``simplest'' 
scenario shown in~\cite[Figure 1 (Left)]{Ozisik2019}:  
``the receiver's mempool contains the entire block''. As shown in~\cite{Ozisik2019}, it is
the best scenario (for Graphene) in terms of communication overhead and decoding time.  
% For encoding time, the distribution of distinct elements has slight impact. 
% However, none of the algorithms can benefit (in terms of encoding time) unfairly from this setup. 
% , 
% because the distribution affects $|B|$ slightly and, as described in~\autoref{sec:closely-related}, all algorithms have an encoding computational complexity proportional 
% to $|A|\!+\!|B|$. 
% However, this slight impact is the same for all algorithms. 

We note that the fact that set $B$ is always a subset of $A$ is not known to any algorithm in our evaluation and 
thus no algorithm takes advantage of this fact. 


\begin{comment}


\subsection{Evaluation of Our ToW Estimator}\label{subsec:est-perf}

In this section, we compare our ToW estimator with two existing algorithms: Strata~\cite{Eppstein_WhatsDifference?Efficient_2011} and min-wise hashing~\cite{Broder_MinWiseIndependent_2000}, which we have described in~\autoref{subsec:est-bench} in detail. In the comparisons, we fix the size of the union $A\cup B$ to 100K and set the value of 
$t$ (the size of the set difference $A\Delta B$) varying from 10 to 10K (or in other words, $t/|A\cup B|$ varying from $10^{-4}$ to $10^{-1}$). 

For our ToW estimator and min-wise hashing, we used  \code{xxHash} hash functions~\cite{Collet_xxHashExtremelyfast_}. 
For Strata, we used the optimized open-source implementation of IBFs~\cite{Ozisik2019}. 

\subsubsection{ToW Estimator: Empirical vs. Analytical}

We first evaluate the empirical accuracy of our ToW estimator against its theoretical accuracy, since 
as mentioned in~\autoref{subsec:ToW} the hash family for calculating the ToW sketches should be 
four-wise independent to achieve the theoretical accuracy whereas \code{xxHash} might not be. 
We use the relative root mean square error (rRMSE) from the ground truth as the metric. 
%The accuracy is measured by the relative root mean square error (rRMSE) from the ground truth. 
For each value of $t$ (the set-difference size), 
we created $c=$1,000 different pairs of $A$ and $B$ and obtained estimates $\{\hat{t}_i\}_{i=1}^{c}$ using our ToW estimator. %For each estimate $\hat{t}_i$ ($i=1,2,\cdots,c$). 
We calculated the empirical rRMSE, which is defined as,
\begin{equation}
\mbox{\texttt{rRMSE}}(\hat{t})=\frac{1}{t}\sqrt{\frac{1}{c}\sum\limits_{i=1}^c(\hat{t}_i-t)^2}.
\end{equation}

% % Need to check whether "perfect" is the right word.
% In~\autoref{}, we have analyzed the accuracy (variance) of our ToW estimator assuming that the hash functions are perfect. 
% However, the hash functions used in practice are generally not perfect. 
As analyzed in~\autoref{subsec:ToW}, given the ground truth $t$ of the set-difference size, 
the variance of our ToW estimator with $k$ sketches is $\frac{2t^2-2t}{k}$. 
Therefore, the analytical rRMSE of our ToW estimator is $\frac{1}{t}\sqrt{\mbox{\bf Var}(\hat{t})}\!=\!\sqrt{\frac{2}{k}(1-\frac{1}{t})}$. 

\autoref{fig:rrmse} reports the empirical and analytical rRMSE of our ToW estimator. We only present the 
results for $t=10$ (\autoref{fig:rrmse-10}) and $t=\num{10000}$ (\autoref{fig:rrmse-10000}), since the 
empirical results are nearly identical to the analytical results under all different values of $t$,  
like what have been shown in \autoref{fig:rrmse-10} and \autoref{fig:rrmse-10000}. 

% \begin{figure}
% \centering
% \includegraphics[width=0.49\textwidth]{figures/estimator/rrmse}
% \caption{rRMSE of ToW.}\label{fig:rrmse}
% \end{figure}


\begin{figure}
\centering
\begin{subfigure}[t]{0.25\textwidth}
    \centering
    \includegraphics[width=1.0\textwidth]{figures/estimator/rrmse_10}
    \caption{t=10.}\label{fig:rrmse-10}
\end{subfigure}%
\begin{subfigure}[t]{0.25\textwidth}
    \centering
    \includegraphics[width=1.0\textwidth]{figures/estimator/rrmse_10000}
    \caption{t=\num{10000}.} \label{fig:rrmse-10000} %%%%%
\end{subfigure}
\caption{rRMSE of ToW.}\label{fig:rrmse}
\end{figure}

% 121	1.30000000000000
% 113	1.31000000000000
% 106	1.32000000000000
% 100	1.33000000000000
% 94	1.34000000000000
% 89	1.35000000000000
% 84	1.36000000000000
% 80	1.37000000000000
% 75	1.38000000000000
% 72	1.39000000000000
% 68	1.40000000000000
% 65	1.41000000000000
% 62	1.42000000000000
% 59	1.43000000000000
% 56	1.44000000000000
% 54	1.45000000000000
% 52	1.46000000000000
% 49	1.47000000000000
% 47	1.48000000000000
% 46	1.49000000000000
% 44	1.50000000000000

% \subsubsection{Correction Overheads}
\subsubsection{ToW Estimator vs. Prior Estimators}

The objective of an estimator for the set-difference size $t$ in the context of 
set reconciliation is to provide estimates with high-enough accuracy. 
On one hand, if the estimator over-estimates, the subsequent reconciliation will 
usually waste unnecessary bandwidth. 
On the other hand, if the estimator under-estimates, the reconciliation might fail. 
Hence, in practice, the estimate returned by the estimator is usually 
scaled up by a proper factor to ensure that the failure rarely happens. 


Now, we compare the scaling ratios, which we call the {\it correction overheads} like 
in~\cite{Eppstein_WhatsDifference?Efficient_2011}, of the three estimators. 
For each value of $t$, we created \num{10000} different pairs of $A$ and $B$, obtained 
estimates from the three estimators, and then calculated the required correction overhead 
for each estimator to ensure that 99\% estimates are larger than or equal to the ground 
truth. For Strata, we used the best parameters reported in~\cite{Eppstein_WhatsDifference?Efficient_2011} for 
our experimental configuration (the same as that in~\cite{Eppstein_WhatsDifference?Efficient_2011}): 
$3$ hash functions for each IBF, and $16$ strata each with $80$ cells. We note that this parameter 
setting assumes the approximate total set size ({\it i.e.,} 100K), or in other words the 
largest possible set-difference size $t_{max}$ is known a prior; Otherwise, more 
strata should be used. We assume that each ToW sketch takes $\lceil \log_2 (2t_{max} + 1)\rceil\!=\!18$ 
bits as each ToW sketch is an integer within the range of $[-t_{max},t_{max}]$. 
For our ToW estimator, we first calculate an approximate number of sketches required to achieve comparable 
correction overheads as Strata by using the central limit theorem (CLT) and then tune the exact number of 
sketches (we only tested the values of power of $2$ for saving time). For min-wise estimator, we use the 
same number of hashes as the number of sketches in our ToW estimator. 
The experimental results are reported in~\autoref{fig:co}. For ToW estimator and min-wise estimator, we only show the results for $k\!=\!128$ and $256$. 

\noindent
{\bf ToW vs. Strata}. As shown in~\autoref{fig:co}, our ToW estimator with $128$ sketches already 
achieves comparable correction overheads as Strata. Note that the estimates should be scaled up be a 
factor according to the worst case among all the points shown in~\autoref{fig:co} for each estimator. 
%as the ground truth of the set-difference size $t$ is not known a prior. 
That is, the estimates have 
to be scaled up by a factor (correction overhead) of $1.36$ and $1.38$ using Strata and 128-sketch ToW estimator 
respectively. If using 256 sketches, ToW estimator only requires this factor to be 
$1.25$. Now, we 
compare the space required by Strata and ToW estimator with 128 sketches. Our ToW estimator 
with 128 sketches only requires 288 bytes. As each cell in Strata 
requires 12 bytes (4 bytes for each field), the space required for Strata is 15 KB, which is around 
$53$ times of that of ToW estimator. 

\noindent
{\bf ToW vs. min-wise}. Now, we compare our ToW estimator with min-wise estimator. 
As shown in~\autoref{fig:co}, the correction overhead only becomes less than $3$ when 
$t$ gets larger than \num{7000} for the min-wise estimator with 128 hashes. Even when using 
256 hashes, min-wise estimator still requires this factor to be larger than 3 for most 
of the values (of $t$) we experimented. We note that for $t\leq 400$, 
most estimates returned from min-wise 
estimator is 0, which results in an infinite correction overhead. In fact, as reported in~\cite{Eppstein_WhatsDifference?Efficient_2011}, even when using thousands of hash functions (more precisely, 
\num{3840} hashes), 
min-wise estimator can still have an infinite correction overhead when $t\!<\!200$. 
Therefore, we conclude that min-wise estimator 
is not a feasible estimator for the set-difference size when $t\!\ll\! |A\cup B|$. 

\noindent
{\bf Summary}. Through the above comparisons with Strata and min-wise estimators, we conclude that 
our ToW estimator is much more space-efficient for achieving the same accuracy. Besides, the parameter 
setting for our ToW estimator is much easier. On one hand, 
our ToW estimator only has one parameter, 
{\it i.e.,} number of sketches, whereas Strata has 3 parameters ({\it i.e.,} number of 
strata, number of cells and number of hashes for each IBF). 
On the other hand, number of sketches (of ToW estimator) required for achieving a desired 
correction overhead is almost independent of $t$ and 
$|A|$ and $|B|$, whereas Strata should set the number of strata according to maximum possible 
set-difference size and number of hashes required by min-wise estimator 
for achieving a desired correction overhead is highly dependent on the ratio $t/|A\cup B|$. 



% \begin{figure}
% \centering
% \begin{subfigure}[t]{0.25\textwidth}
%     \centering
%     \includegraphics[width=0.99\textwidth]{figures/estimator/co_95}
%     \caption{95\%.}\label{fig:co95}
% \end{subfigure}%
% \begin{subfigure}[t]{0.25\textwidth}
%     \centering
%     \includegraphics[width=0.99\textwidth]{figures/estimator/co_99}
%     \caption{99\%.} \label{fig:co99} %%%%%
% \end{subfigure}
% \caption{Correction overheads of different estimators to ensure that at least 95\% and 99\% of the estimates are larger than or equal to the ground truth, respectively.}\label{fig:co}
% \end{figure}

\begin{figure}
\centering
    \centering
    \includegraphics[width=0.49\textwidth]{figures/estimator/co_99_with_minhash_v2}
\caption{Correction overheads of different estimators to ensure that at least 99\% of the estimates are larger than or equal to the ground truth.}\label{fig:co}
\end{figure}
\end{comment}

%% comparisons against D.Digest and PinSketch
\input{section/evaluation_against_ddigest_etc}
%% comparisons against Graphene
\input{section/evaluation_against_graphene}

\begin{comment}
\subsection{Experiment Results}\label{subsec:recon-perf}

We report the experiment results in this section. Before diving into the detailed results for the two major performance 
metrics ({\it i.e.,} communication overhead and computational overhead),  %in~\autoref{}. 
we first present the empirical 
success rates of all these algorithms %, the results were presented 
in~\autoref{fig:success-rate}. \autoref{fig:success-rate} shows that all these algorithms have achieved empirical success rates 
at least as high as the corresponding target success rates under all 
different values of set difference cardinalities except that the empirical success rates of D.Digest are lower than 0.99, 
its target success rate, when $d\!\le\!30$. 

% The results mainly focused on the communication overheads 
% and decoding time of PBS against prior work
\begin{figure}
\centering
\begin{subfigure}[t]{0.25\textwidth}
\centering
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/success_rate}
% \caption{PBS vs. D.Digest and PinSketch (targeted success rate: 0.99).}
% \caption{Target success rate: 0.99.}
\caption{vs. D.Digest and PinSketch}
\label{fig:success-rate-99}
\end{subfigure}%
\begin{subfigure}[t]{0.25\textwidth}
\centering
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-239-240/success_rate_vs_Graphene_v2}
% \caption{PBS vs. Graphene.}\label{fig:success-rate-9958}
% \caption{Target success rate: 0.9958.}
\caption{vs. Graphene}
\label{fig:success-rate-9958}
\end{subfigure}
\caption{Success rate.}\label{fig:success-rate}
\end{figure}


% \subsubsection{Basic Results}\label{subsubsec:basic}

We now present the experiment results on communication overhead.


\begin{figure}
\centering
\begin{subfigure}[t]{0.25\textwidth}
\centering
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/communication_costs}
% \caption{PBS vs. D.Digest and PinSketch (targeted success rate: 0.99).}
% \caption{Target success rate: 0.99.}
\caption{vs. D.Digest and PinSketch}
\label{fig:co-99}
\end{subfigure}%
\begin{subfigure}[t]{0.25\textwidth}
\centering
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-239-240/communication_costs_vs_Graphene_v2}
% \caption{PBS vs. Graphene.}\label{fig:success-rate-9958}
% \caption{Target success rate: 0.9958.}
\caption{vs. Graphene}
\label{fig:co-9958}
\end{subfigure}
\caption{Communication overheads.}\label{fig:co}
\end{figure}

\smallskip
\noindent
{\bf Communication overhead}.
\autoref{fig:co-99} shows the communication overhead of 
PBS against those of D.Digest and PinSketch, with a target success rate of 0.99. 
% We note that the communication overhead of the estimator is excluded since 
% it is constant (288 bytes) and the same for these algorithms. 
% Results confirm that all these algorithms have the same 
% asymptotic communication complexity, that is $O(t)$. However, the constant factors are different and do 
% matter in practice. 
Results show that the communication overheads scale approximately linearly with respect to $d$ for all 
the three algorithms. More precisely, under any set difference cardinality $d$, the amount of communication per 
distinct element is roughly a constant. 
D.Digest is the worst. It requires around 6$\times$32 bits per distinct element, which is  
6 times of the minimum, 32 bits per distinct element. 
% Our PBS requires less than half of those of D.Digest. 
PBS is much better, which %only  
% requiring no more than 
% More precisely, PBS 
needs (2.15 to 2.67)$\times$32 bits per distinct element ({\it i.e.,} 2.15 to 2.67 times of the minimum). 
PinSketch is the best, which only requires around 1.38$\times$32 bits per distinct element ({\it i.e.,} 1.38 times of the minimum). 
However, as we will show very soon, its decoding time is significantly (up to 3 orders of magnitude) higher than those of the others, when 
$d$ is large. 
% \ These values for $($
% our scheme with 2 and 3 rounds are 9.97 to 14.15 and 8.60 to 10.67 respectively. 

% As mentioned earlier in~\autoref{sec:parameter_settings}, we separated the comparisons against 
\autoref{fig:co-9958} presents the communication overhead of PBS against that of Graphene, 
with a target success rate of 239/240. 
%  and our scheme (with 
% 2 and 3 rounds). 
% For our scheme, we include those for our ToW estimator. 
The results show that PBS has lower communication overhead than Graphene 
under all different set difference cardinalities except for those close to \num{10000} 
where PBS has slightly higher communication overheads than Graphene. 
PBS requires roughly (2.21 to 2.75)$\times$32 bits per distinct element (higher than those in~\autoref{fig:co-99} 
as the target success rate here is higher). 
Unlike in other algorithms, in Graphene, the average amount of 
communication per distinct element varies significantly as $d$ changes and %as shown in~\autoref{fig:co-9958}, 
it roughly decreases as $d$ increases.  
For example, Graphene requires approximately 7.33$\times$32 bits per distinct element when $d$=10, 
whereas it only requires 1.84$\times$32 bits when $d$=\num{10000}. 
% This phenomenon results from the parameter setting procedure of Graphene: 
% Given a target success rate, Graphene used the optimal sizes for the BFs and IBFs to 
% minimize the total communication overheads. 
% % not sure whether we have to explain
% Recall that Graphene is a hybrid algorithm that combines BFs and IBFs, its communication overheads 
% are mainly consisted of two components: the communication for the BFs and the communication for the IBFs. 

% % maybe adding a figure
% \autoref{} shows the fraction of the communication overheads resulted from the IBFs. 
% As shown in \autoref{}, when $d\!\le\!$\num{1000}, the communication of the IBFs covers more than 99\% of that of Graphene. 
% In these scenarios ({\it i.e.,} $d\!\le\!$\num{1000}), the average 
% communication per distinct element roughly decreases, because unlike in D.Digest, where a good enough parameter setting 
% was used, in Graphene, a procedure that can determine the optimal size (for a given target success rate) for an IBF was used. 

% The results also show that the average 
% communication per element in the set difference gets smaller for Graphene. 
% For $t\!<\!$\num{1000}, it is mainly because the IBF requires less cells per 
% element as $t$ gets larger to ensure the same success rate, as shown in Figure 7 
% of~\cite{Eppstein_WhatsDifference?Efficient_2011}. When $t\ge 1000$, the average number of cells per 
% element is almost independent of $t$ (remains the same as $t$ increases). The average communication 
% per element (in the set difference) continues to decrease 
% because when $t$ is large enough the BF in Graphene can help 
% reduce the number of cells required by the IBFs thus resulting in a lower communication overhead per 
% element in the set difference.  

As explained in~\autoref{subsubsec:discussion}, the scenario in our evaluation ({\it i.e.,} $B\subset A$) 
is the best for Graphene. In more general scenarios ({\it i.e.,} $B$ is not a subset of $A$), the communication overhead 
of Graphene would be higher than that shown in~\autoref{fig:co-9958}. 

\begin{figure}
\centering
\begin{minipage}[t]{0.25\textwidth}
\centering
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/encoding_time}
\caption{Encoding time.}
\label{fig:et-99}
\end{minipage}%
\begin{minipage}[t]{0.25\textwidth}
\centering
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/decoding_time}
\caption{Decoding time.}
\label{fig:dt-99}
\end{minipage}%
\end{figure}

% In real applications, the 
% % key size (length of each element in the universe) 
% hash signature width $w$ (width of each binary string in the universe $\mathcal{U}$) 
% might be much higher than 
% 32 bits. For example, the transaction ID in Bitcoin applications could 
% have 2048 bits~\cite{naumenko2019bandwidth}. 



We then present the experiment results on computational overhead, more precisely, encoding time and decoding time. Note that the results of 
PBS against Graphene are not presented for fairness consideration, because Graphene is implemented in Python, which 
is much slower than PBS that is implemented in C++.   

\smallskip
\noindent
{\bf Encoding time}.
\autoref{fig:et-99} shows the encoding time of PBS against those of D.Digest and PinSketch, 
with a target success rate of 0.99. 
As shown in~\autoref{fig:et-99}, PBS 
has the lowest encoding time under all different values of $d$ get larger. 
% Results of PinSketch and D.Digest match well with our theoretical analysis in~\autoref{sec:closely-related}: 
% The encoding time of PinSketch increases linearly as $d$, and that of D.Digest is 
% $O(|A|\!+\!|B|)$ (3 or 4 hash operations per element), independent of $d$.  
% We note that the encoding time of D.Digest is slightly higher when $d$ is small.  
% This is because, as described in~\autoref{subsubsec:configuration}, 
% D.Digest used 3 hash functions when $d\!>\!200$, and $4$ hash functions otherwise. 
\autoref{fig:et-99} also clearly shows that the encoding time of PBS increases slightly as $d$ increases. 
This is because the encoding time mainly consists of two parts in PBS: 
hash-partition and parity bitmap encoding (\autoref{sec:hash_partition}) and 
BCH encoding (\autoref{step:BCH_encode} of~\autoref{alg:single_round_pbs}). 
The former is independent of $d$, which has a computational complexity 
of $O(|A|\!+\!|B|)$ (1 hash operation per element). The latter has a computational complexity 
linear in $d$, because the number of groups is on average $1.38d/5$ 
% ,  
% which increases linearly as $d$ 
and BCH encoding time per group is roughly a constant (as $n$ and $t$ are the same for all groups). %the same.  

% The results also show that the encoding time of our scheme increases as $t$ increases. 
% This is because the encoding time mainly consists of two parts in our scheme: the partition process and 
% the BCH encoding. The former is independent of $t$, which has a computational complexity 
% of $O(|A|+|B|)$ (1 hash operation per element). The latter has a computational complexity 
% proportional to $t$ as the number of bins (subset pairs) increases almost linearly as $t$ and 
% the encoding of each subset pairs has a constant computational complexity.  

\smallskip
\noindent
{\bf Decoding time}.
\autoref{fig:dt-99} shows decoding time of PBS against those of D.Digest and PinSketch, 
with a target success rate of 0.99. 
% Results show that 
% the decoding times of D.Digest and PBS scale roughly linearly with respect to $d$, whereas 
% that of PinSketch scales roughly quadratically with $d$. 
As shown in~\autoref{fig:dt-99}, the decoding time of 
PinSketch is much higher than those of D.Digest and PBS when $d$ is large (say $\ge$ \num{1000}). 
For example, when $t\!=\!$\num{10000}, the decoding time of PinSketch is roughly three orders of magnitude 
higher than those of D.Digest and PBS. 
% As mentioned earlier in~\autoref{sec:scheme}, the substantially longer decoding time of PinSketch is because 
% the decoding computational complexity of BCH codes is quadratic in $t$, thus also quadratic in $d$ 
% (here we use the fact $\mathbf{E}[t]\!=\!$1.38d in our 
% evaluation). Though our PBS also uses BCH codes, as explained in~\autoref{sec:scheme}, PBS resolved this issue 
% by using BCH codes in a much more efficient manner so that its decoding computational complexity is linear in 
% $d$. 
\autoref{fig:dt-99} also shows clearly that D.Digest is the best, whose decoding time is 2 to 3 times shorter than that of PBS. 
However, as discussed earlier, its encoding time is much longer (up to one order of magnitude longer) 
than that of PBS, and encoding time (of 
PBS and D.Digest) is usually much longer than the corresponding decoding time. 
Therefore, PBS has the lowest overall computational overhead. 
\end{comment}

\begin{comment}
\subsection{Piecewise Decodability of PBS}\label{subsec:piecewise}

\begin{figure}
\centering 
\includegraphics[width=0.45\textwidth]{figures/reconciliation/success-rate-99/pbs_3_per_round_all_v3}
\caption{Fraction of communication overhead incurred in each round.}\label{fig:per-round-con}
\end{figure}

As mentioned earlier in~\autoref{subsubsec:configuration}, failure is inevasible (though usually with a tiny probability) 
in most set reconciliation algorithms.  
When failure happens, in most of existing set reconciliation algorithms, the process has to start from square one, 
thus the communication overhead doubles. 
% Recall from~\autoref{sec:intro}, 
However, failure only incurs very tiny additional communication 
overhead in PBS because of its piecewise decodability. 
In this section, we demonstrate, through experiments, the piecewise decodability of PBS. 

We use the default parameter setting described in~\autoref{subsubsec:configuration} except that now we 
% allow PBS to run as many 
% rounds as possible 
measure the communication overhead incurred in each round 
until PBS believes all distinct elements are successfully reconciled, {\it i.e.,} \autoref{proto:multirounds} 
stops because \code{complete} becomes \code{true}.   

\autoref{fig:per-round-con} shows per-round communication overhead, more precisely, 
the percentage of communication overhead incurred in each round. To clearly present the results, 
we use a separate axis for each round in~\autoref{fig:per-round-con}. 
%
As shown in~\autoref{fig:per-round-con}, 
PBS runs at most 4 rounds. 
% From \autoref{fig:per-round-con}, it is hard to read the percentages in round 3 and 4 clearly, because 
% the communication overhead incurred in these two rounds are so tiny ({\bf $<0.1$ percentage ??}). 
We note that 
% no error occurred in any experiment instance, that is, 
all distinct elements in all 
experiment instances were eventually successfully reconciled. 

% \autoref{fig:per-round-con} clearly shows that the vast majority ($>$93\%) of the communication overhead 
% is incurred in round 1 and the per-round communication overhead drops exponentially as the number of rounds increases. 
\autoref{fig:per-round-con} clearly shows that more than 93\%, 1\% to 7\%, less than 0.16\%, and less than 0.013\% of the communication overhead 
is incurred in round 1, 2, 3, and 4, respectively. 
% and the per-round communication overhead drops exponentially as the number of rounds increases. 
This confirms the piecewise decodability of PBS, which can be explained as follows. 
+++ {\bf The following explanation can be removed if we already explained this in scheme section.} 
After round 1, some distinct elements in a few groups fail to be reconciled because of 
the exceptions described in~\autoref{subsec:exception_hash_partition} and BCH decoding failure described in~\autoref{sec:BCH_exception}. 
% Though when the latter happens, one group is decomposed into $3$. The number of groups resulting 
% from such failure is tiny, as the probability that such failure occurs is extremely low (roughly at the order of $10^{-5}$), 
These events happen with tiny probability, 
thus only a tiny fraction of distinct elements remain un-reconciled and PBS only needs to reconcile them in round 2. 
Therefore, the communication overhead in round 2 is much lower than that incurred in round 1. If PBS does not reconcile 
all the remaining distinct elements in round 2, round 3 then comes. Similarly,  the communication overhead in round 3 is much 
lower than that incurred in round 2. And so on so forth until all distinct elements are successfully reconciled. 

% +++ {\bf The following can be added if we have space.}
% To reassure readers that the exponential drop of the per-round communication overhead as 
% the number of rounds increases is really because of the piecewise decodability instead of most of the experiment 
% instances being successfully reconciled (though it is also a reason when $d$ is small), we further measured 
% After the first round, most of the distinct elements were determined and the rest rounds only need to handle the remaining 
% tiny percentage 

% In this section, we demonstrate the piecewise decodability of PBS, an important feature for set reconciliation algorithms, 
% which all existing set reconciliation does not have. 

\begin{figure*}
\centering
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/communication_costs_verying_key_sizes_d100}
\caption{d=100}
\label{fig:-d100}
\end{subfigure}%
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/communication_costs_verying_key_sizes_d1000}
\caption{d=\num{1000}}
\label{-d1000}
\end{subfigure}%
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/communication_costs_verying_key_sizes_d10000}
\caption{d=\num{10000}}
\label{fig:-d10000}
\end{subfigure}
\caption{Communication overheads of PBS against those of PinSketch, D.Digest under various signature widths.}% with at least 99\% success rate.}
\label{fig:cc-comp-vk}
\end{figure*}
\end{comment}

\begin{comment}
\subsection{Varying Signature Width}\label{subsubsec:varying-sig-width}

In real applications, the 
% key size (length of each element in the universe) 
hash signature width $\log|\mathcal{U}|$ (width of each binary string in the universe $\mathcal{U}$) 
might be much higher than 
32 bits. For example, the transaction ID (``hash signature'') in Bitcoin applications could 
be as large as 2048 bits~\cite{naumenko2019bandwidth}. 
In this section, we investigate how the performance of each algorithm scales with respect to $\log|\mathcal{U}|$. 
We consider signature width $\log|\mathcal{U}|$ varying from 32 to 2048 bits. 
As the implementations of all the evaluated algorithms do not support signature width higher than $64$ bits (some of them only support 
32 bits), all results for $\log|\mathcal{U}|\!>\!$32 in this section were obtained by using simulations with a $32$-bit universe. 
Thus, we only present the results for communication overhead in this section. However, we note that PBS 
also has some superiority in computational overhead, more precisely, decoding time, over all the rest algorithms, 
because the BCH decoding computational complexity in PBS is independent of 
$\log|\mathcal{U}|$, whereas it grows linearly in $\log|\mathcal{U}|$ or even faster in all other algorithms.  
Like in~\autoref{subsec:recon-perf}, we separate the comparisons 
against D.Digest and PinSketch (with a target success rate 0.99) and those against Graphene (with a target success rate of 239/240).  
The results are shown in~\autoref{fig:cc-comp-vk} and~\autoref{fig:cc-comp-vk-vs-graphene} respectively. 

% Same as before, for the results in~\autoref{fig:cc-comp-vk}, we make each algorithm ensure a success rate of 
% 0.99 and exclude the communication required by the estimator for all algorithms. For those in~\autoref{fig:cc-comp-vk-vs-graphene}, we make our scheme and Graphene ensure a success rate of 239/240 and include 
% the communication required by the estimator for our scheme (note that Graphene does not require an estimator). 

We can see from \autoref{fig:cc-comp-vk} that the communication overhead increases for all algorithms when 
the signature width increases, under all 3 different set difference cardinalities, which is not surprising. 
However, \autoref{fig:cc-comp-vk} also clearly shows that PBS scales much better than D.Digest and PinSketch, as 
we will elaborate next. 

We make the following two observations from \autoref{fig:cc-comp-vk}. First, the communication overheads of D.Digest and PinSketch grow linearly as the signature width $\log|\mathcal{U}|$ increases, remaining $6$ and $1.38$ times of the minimum respectively, which matches well 
our rough estimates in~\autoref{subsubsec:configuration}.  
% Second, the gap between PBS and the minimum shrinks rapidly as the signature width becomes larger.  
Second, PBS overtakes PinSketch rapidly and becomes the one with the lowest communication overhead as the signature width $\log|\mathcal{U}|$ becomes larger. 
+++ {\bf The following explanation can be removed or at least simplified if we already explained it in the scheme section.}  
The reason is as follows. 
As described earlier in~\autoref{sec:communication_overhead_single_PBS}, the communication overhead of PBS is 
consisted of three parts: BCH codewords,  
XOR sums (together with subset pair indices), and checksums. 
Only the communication overhead resulting from  
XOR sums (excluding indices) in the the second part grows as $\log|\mathcal{U}|$ gets larger, which is approximately $d\log|\mathcal{U}|$ bits. 
The rest is independent of $\log|\mathcal{U}|$, which takes slightly more than 50\% in the total communication overhead when $\log|\mathcal{U}|\!=\!32$. 
Hence, as $\log|\mathcal{U}|$ increases, this part takes less and less fraction in the total communication overhead, and 
the communication overhead resulting from XOR sums, approximately $d\log|\mathcal{U}|$ bits, gradually dominates the communication overhead of PBS.  
% The former is independent of $w$. The latter 
% is roughly $wd$ bits. 
Therefore, when the signature width $\log|\mathcal{U}|$ increases, the communication overhead of PBS becomes increasingly closer to 
% $1\!\times\!$ 
% $wd$ bits (the ratio of the communication overhead for PBS to $wd$ bits gets closer to $1$),
the minimum ($d\log|\mathcal{U}|$ bits), 
outperforming PinSketch which requires $1.38d\log|\mathcal{U}|$ bits.   
% Our explanation for the first observation is as follows. D.Digest requires to allocate $w$ bits to each field in every IBF cell, 
% hence its communication overhead becomes approximately $6w$ bits per dist
% \autoref{fig:cc-comp-vk} shows that the communication overheads of D.Digest and PinSketch double 
% as the signature width $w$ doubles, requiring $6$ and $1.38$ times of the minimum, $w$ bits per distinct 
% element. \autoref{fig:cc-comp-vk} also shows that communication overhead of PBS increases much slower as $w$ increases. 


% As shown in~\autoref{fig:cc-comp-vk} and~\autoref{fig:cc-comp-vk-vs-graphene}, PBS has the best 
% scaling behavior (with respect to $w$) among all these algorithms. 
% For D.Digest and PinSketch, the communication overheads double 
% as the signature width $w$ doubles, whereas the communication overhead increases much slower in PBS.  
% as the key size increases. 
We can see from \autoref{fig:cc-comp-vk-vs-graphene} that the communication overhead of Graphene also grows 
linearly as the signature width $\log|\mathcal{U}|$ increases when $d\!=\!$\num{100} (\autoref{fig:vs-graphene-d100}) and $d\!=\!$\num{1000} (\autoref{fig:vs-graphene-d1000}). 
However, it grows much slower when $d\!=\!$\num{10000} (\autoref{fig:vs-graphene-d10000}). 
Our explanation for these observations is as follows. As described in~\autoref{sec:closely-related}, Graphene is 
a hybrid set reconciliation algorithm that combines BFs and IBFs. %BF- and IBF-based solutions. 
Its communication overhead 
mainly results from two parts: BFs and IBFs. Recall from~\autoref{sec:closely-related},  when $d\!=\!|A\Delta B|\!\ll\!|A\cup B|$ (the scenarios shown in 
\autoref{fig:vs-graphene-d100} and \autoref{fig:vs-graphene-d1000}), Graphene can not afford to create BFs with low false positive 
rate, thus the space for the IBFs dominates the communication overhead. This interpretation was later confirmed by detailed instruments: The false positive rates of the BFs are close to $1$ and the IBFs take more than $99\%$ of the communication 
overhead. The space of IBFs grows linearly as $\log|\mathcal{U}|$ gets larger. Therefore, the communication overhead of Graphene also grows 
linearly as the signature width $\log|\mathcal{U}|$ increases when $d\!=\!$\num{100} (\autoref{fig:vs-graphene-d100}) and $d\!=\!$\num{1000} (\autoref{fig:vs-graphene-d1000}). 

However, as $d$ gets larger, Graphene now can afford to create BFs with relatively low false positive rates and now the space 
of IBFs takes less fraction. Through detailed instruments, we found the fraction of communication overhead resulting from 
IBFs becomes roughly $39\%$ when $d\!=\!$\num{10000} and $\log|\mathcal{U}|\!=\!32$. The space of BFs 
is independent of $\log|\mathcal{U}|$. Therefore, just like that of PBS, the communication overhead of Graphene grows much slower when $d\!=\!$\num{10000} (\autoref{fig:vs-graphene-d10000}). 
% For Graphene, when $t\!=\!$\num{100} and $t\!=\!$\num{1000}, its scaling behavior is almost the same as D.Digest, since as explained in~\autoref{subsec:recon-bench}, Graphene almost reduces to an IBF-only solution when $t\ll|A\cup B|$. When $t=$\num{10000}, the scaling behavior is very close to that of our scheme, as now the communication overheads resulting from IBFs in Graphene is around 40\% and those for the BFs do not increase as the key size. 



\begin{figure*}[!htbp]
\centering
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-239-240/vs_graphene_verying_key_sizes_d100}
\caption{d=100}
\label{fig:vs-graphene-d100}
\end{subfigure}%
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-239-240/vs_graphene_verying_key_sizes_d1000}
\caption{d=\num{1000}}
\label{fig:vs-graphene-d1000}
\end{subfigure}%
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-239-240/vs_graphene_verying_key_sizes_d10000}
\caption{d=\num{10000}}
\label{fig:vs-graphene-d10000}
\end{subfigure}
\caption{Communication overheads of PBS against those of Graphene under various signature widths.}% with at least 99\% success rate.}
\label{fig:cc-comp-vk-vs-graphene}
\end{figure*}
\end{comment}

\begin{comment}

\subsection{What If PinSketch Also Uses Partitions?}\label{subsec:mini-partition}
+++ {\bf The following paragraph can be removed!} 
The success we have with PBS leads readers to wonder what if we apply the same  
idea to PinSketch. Like in PBS, we can partition $A$ into $\{A_i\}_{i=1}^g$ and $B$ into $\{B_i\}_{i=1}^g$ 
using the hash partition described in~\autoref{sec:hash_partition} so that each subset-pair-differences $\{A_i\Delta B_i\}_{i=1}^g$ 
contains $\delta =d/g$ distinct elements on average. Then, we use PinSketch with a high enough error-correction capability $t$ (say $2.5\delta$) 
to reconcile each subset pair 
independently. We refer to this new scheme as PinSketch With Partition, or PinSketch/WP for short.  
Clearly, by letting $\delta$ be a small constant (say $5$), PinSketch/WP also has a decoding computational 
complexity of $O(d)$ and communication complexity of $O(d)$. 

Now We compare the performance of PBS against that of PinSketch/WP. %, with a target success probability of $p_0$=0.99 within $r$=3 rounds. 
As performing rigorous theoretical analysis -- like we did for PBS in~\autoref{sec:tail_bound} -- for PinSketch/WP 
is out scope of this paper. We simply used the same parameter setting as which we used for PBS ({\it i.e.,} the default parameter setting), 
for PinSketch/WP. That is, PinSketch/WP uses the same $\delta$ and $t$ as PBS (note that 
there is no ``n'' in PinSketch/WP), with a target success probability of $p_0$=0.99 within $r$=3 rounds, in each experiment instance.  
% For example, like in our scheme, we partition all elements into several subsets 
% so that each subset contains a few elements (say $5$) on average from the set difference. Then, for 
% each subset we create BCH codes with a capacity large enough so that we can ensure a desired success rate. 


% We compare the performances of our scheme with those of Minisketch/WP with a desired success rate of 
% 0.99. For Minisketch/WP, we set the average number of elements from the set difference to $5$ (same 
% as our scheme) and use the same BCH decoding capacity for all subsets. We tune this capacity to the best: 
% the one with the minimum communication overhead yet ensures a success rate of at least 0.99.    

\autoref{fig:cc-comp-vs-minisketchwp} presents the communication overheads under different signature widths varying 
from 32 to \num{2048} bits for three different set difference cardinalities \numlist{100;1000;10000}. Like in~\autoref{subsubsec:varying-sig-width}, 
the results for signature widths higher than 32 bits were obtained through simulations with a $32$-bit universe.  
The results show that PinSketch/WP has %similar or 
slightly higher communication overhead than PBS when the signature width is 32 bits. 
The superiority of PBS  
gets outstanding as the signature width $\log|\mathcal{U}|$ gets larger: The gap between PinSketch/WP and PBS increases rapidly as 
the signature width $\log|\mathcal{U}|$ gets larger. Besides, PBS is also computationally 
more efficient than PinSketch/WP because of the shorter width of the Galois field as explained in~\autoref{}, 
which was further confirmed by experiments on encoding and decoding time of PBS against those of 
PinSketch/WP. These results are omitted here in the interest of space. 
% Therefore, we conclude that our scheme overall remains the best practical solution for the 
% set reconciliation problem.

% \begin{figure*}[!htbp]
% \centering
% \begin{subfigure}[t]{0.32\textwidth}
% \includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/co_vs_erlaywp_match}
% \label{fig:vs-minisketchwp-co}
% \end{subfigure}%
% \begin{subfigure}[t]{0.32\textwidth}
% \includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/decoding_time_vs_erlaywp_match}
% \caption{t=\num{1000}.}
% \label{fig:vs-minisketchwp-dt}
% \end{subfigure}%
% \begin{subfigure}[t]{0.32\textwidth}
% \includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/vs_minisketchwp_match_varying_key_sizes_d10000}
% \caption{t=\num{10000}.}
% \label{fig:vs-minisketchwp-et}
% \end{subfigure}
% \caption{Comparisons of PBS against PinSketch/WP, with a target success rate of 0.99.}% with at least 99\% success rate.}
% \label{fig:cc-comp-vs-minisketchwp}
% \end{figure*}

% % need to change
\begin{figure*}[!htbp]
\centering
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/vs_minisketchwp_match_varying_key_sizes_d100}
\caption{d=\num{100}}
\label{fig:vs-minisketchwp-d100}
\end{subfigure}%
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/vs_minisketchwp_match_varying_key_sizes_d1000}
\caption{d=\num{1000}}
\label{fig:vs-minisketchwp-d1000}
\end{subfigure}%
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/vs_minisketchwp_match_varying_key_sizes_d10000}
\caption{d=\num{10000}}
\label{fig:vs-minisketchwp-d10000}
\end{subfigure}
\caption{Communication overheads of PBS against those of PinSketch/WP.}% with at least 99\% success rate.}
\label{fig:cc-comp-vs-minisketchwp}
\end{figure*}


\subsection{Can We Use Less Rounds in PBS}\label{subsec:less-rounds}

In this section, we address one question: Is it possible to use less rounds in PBS without using significantly 
more resources ?


Like in~\autoref{subsubsec:configuration}, we configured PBS to achieve a target success rate of $p_0$=0.99 within $r$=1, 2, or  
3 rounds respectively and compared  
communication overhead and computational overhead. %({\it i.e.,} encoding time and decoding time). 
The experiment results are presented in \autoref{fig:2vs3}, which also include  
their empirical success rates (\autoref{subfig:success-rate}). As resources (both communication overhead and 
computational overhead) required for $r\!=\!1$ are 
significantly higher, we only presented the results for $r\!=2\!$ and $3$. 

We can see from~\autoref{fig:2vs3}, PBS with $r\!=\!2$ has both higher communication overhead and 
higher computational overhead than those of PBS with $r\!=\!3$, but only slightly. This is 
reasonable, as it is obvious that achieving the same success rate within 2 rounds is harder than within 3 rounds. 
Therefore, we consider PBS with $r\!=\!2$ is ``reasonably priced,'' {\it i.e.,} paying reasonably higher 
price (resources) for less rounds. In other words, those slightly additional resources by reducing from 
3 rounds to 2 rounds are only ``marginal cost''.

\def\WD{0.25}
\begin{figure*}[!htbp]
\centering
\begin{subfigure}[t]{\WD\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/success_rate_2vs3}
\caption{Empirical success rate}\label{subfig:success-rate}
\end{subfigure}%
\begin{subfigure}[t]{\WD\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/communication_costs_2vs3}
\caption{Communication overhead}\label{subfig:co}
\end{subfigure}%
\begin{subfigure}[t]{\WD\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/encoding_time_2vs3}
\caption{Encoding time}\label{subfig:et}
\end{subfigure}%
\begin{subfigure}[t]{\WD\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/decoding_time_2vs3}
\caption{Decoding time}\label{subfig:dt}
\end{subfigure}
\caption{PBS: 2 rounds vs. 3 rounds.}\label{fig:2vs3}
\end{figure*}

\end{comment}


\begin{comment}

\subsection{Evaluation of Our Reconciliation Scheme}\label{subsec:recon-perf}

% % 
In this section, we evaluate the performance of our algorithm for set reconciliation, and compare 
it with Difference Digest (D.Digest)~\cite{Eppstein_WhatsDifference?Efficient_2011}, 
Graphene~\cite{Ozisik2019}, and Minisketch~\cite{naumenko2019bandwidth}, which we have 
described in detail in~\autoref{subsec:recon-bench}. 

Like in~\autoref{subsec:est-perf}, 
in the comparisons, we fix the size of the union $A\cup B$ to 100K and set the value of $t$ varying 
from 10 to 10K. For each value of $t$, we created \num{1000} different pairs of $A$ and $B$. 
All the experiments in this section were performed on a workstation with an Intel Core i7-9800X processor 
running Ubuntu 18.0.4.  


For D.Digest, as the authors of~\cite{Eppstein_WhatsDifference?Efficient_2011} did not 
release their source codes, we used the optimized open-source implementation of IBFs in C++ released by 
the authors of~\cite{Ozisik2019}. For Minisketch, we used its C++ implementation~\cite{Wuille_Minisketchoptimizedlibrary_2019}  
released by the authors of~\cite{naumenko2019bandwidth}. 
% Note that, Minisketch is just an optimized implementation of the PinSketch~\cite{Dodis_PinSketch_2008} 
% algorithm. 
For Graphene, we used the source codes provided by the authors of~\cite{Ozisik2019}. 
Note that, the implementation of Graphene is in Python. 
We implemented our scheme in C++: 
we used \texttt{xxHash}~\cite{Collet_xxHashExtremelyfast_} for the partition process 
and Minisketch for BCH encoding and decoding. 


\subsubsection{Our Scheme vs. Prior Work}\label{subsec:vs-prior}

% \begin{figure*}
% \centering
% \begin{subfigure}[t]{0.32\textwidth}
% \includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/communication_costs}
% \caption{Communication overheads.} %(excluding those of the ToW estimator).}
% \label{fig:communication-costs}
% \end{subfigure}%
% \begin{subfigure}[t]{0.32\textwidth}
% \includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/decoding_time}
% \caption{Decoding time.}
% \label{fig:decoding-time}
% \end{subfigure}%
% \begin{subfigure}[t]{0.32\textwidth}
% \includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/success_rate}
% \caption{Success rate.}
% \label{fig:success-rate}
% \end{subfigure}
% \caption{Comparisons our schemes against Minisketch and D.Digest.}% with at least 99\% success rate.}
% \label{fig:comp-old}
% \end{figure*}

\begin{figure*}
\centering
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/communication_costs}
\caption{Communication overheads.} %(excluding those of the ToW estimator).}
\label{fig:communication-costs}
\end{subfigure}%
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/encoding_time}
\caption{Encoding time.}
\label{fig:encoding-time}
\end{subfigure}%
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/decoding_time}
\caption{Decoding time.}
\label{fig:decoding-time}
\end{subfigure}%
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/success_rate}
\caption{Success rate.}
\label{fig:success-rate}
\end{subfigure}
\caption{Comparisons against Minisketch and D.Digest.}% with at least 99\% success rate.}
\label{fig:comp-old}
\end{figure*}

\noindent
{\bf Our Scheme vs. D.Digest and Minisketch}. We now compare our set reconciliation scheme 
against D.Digest and Minisketch. We used 128-sketch ToW estimator with 128 sketches for 
the estimation of $t$ for all these algorithms. 
For D.Digest, we used the parameter setting suggested by the authors of~\cite{Eppstein_WhatsDifference?Efficient_2011}: $2\hat{t}$ cells where $\hat{t}$ is the estimate of the set-difference size, 
and 3 hash functions for estimates less than 200; Otherwise we used 4 hash functions. 
Note that with this parameter setting, D.Digest can roughly ensure a success rate of 
at least 0.99, that is, for at least 99\% of the instances that we experimented, all elements should be successfully recovered. For Minisketch, we scaled up the estimates 
by 1.38 so that it can also ensure a success rate of 0.99. For our scheme, 
we set the average number of ``bad balls'' in each bin (elements in the set difference $A\Delta B$) 
to $5$ and whenever any bin fails to decode (which happens with tiny probability), 
we decomposed the bin in to three. We used the same BCH parameters 
(BCH code length and decoding capacity) for all bins, the 
values of which was obtained as follows. 
We first scaled up the estimates by 1.38. Then, based on the scaled estimates 
(assuming they are the true values), 
we computed the best parameters that can ensure a success rate of at least 
0.99 with 2 or 3 rounds (excluding the set-difference size estimation round) 
using our analytical results in~\autoref{sec:tail_bound}. Therefore, our scheme 
also roughly ensures a success rate of 0.99. 

% \autoref{fig:comp-old} presents the amount of data transfered (\autoref{fig:communication-costs}), the decoding time (\autoref{fig:decoding-time}), and the empirical 
% success rate (\autoref{fig:success-rate}) of Minisketch, D.Digest, and our scheme with 2 and 3 rounds. 

\autoref{fig:communication-costs} presents the amount of communication overheads of 
Minisketch, D.Digest, and our scheme (with 2 and 3 rounds). 
We note that the communication overhead of the estimator is excluded since 
it is constant (288 bytes) and the same for these algorithms. 
Results confirm that all these algorithms have the same 
asymptotic communication complexity, that is $O(t)$. However, the constant factors are different and do 
matter in practice. D.Digest is the worst, which requires 24 bytes per element in the set difference. 
Minisketch is the best, which only requires around 5.52 bytes per element. These values for 
our scheme with 2 and 3 rounds are 9.97 to 14.15 and 8.60 to 10.67 respectively. 

\autoref{fig:encoding-time} shows their encoding times. The results show that our scheme 
% (especially when using 3 rounds) 
has the lowest encoding time under all values of $t$. 
The results also show that the encoding time of our scheme increases as $t$ increases. 
This is because the encoding time mainly consists of two parts in our scheme: the partition process and 
the BCH encoding. The former is independent of $t$, which has a computational complexity 
of $O(|A|+|B|)$ (1 hash operation per element). The latter has a computational complexity 
proportional to $t$ as the number of bins (subset pairs) increases almost linearly as $t$ and 
the encoding of each subset pairs has a constant computational complexity.  

\autoref{fig:decoding-time} shows their decoding times. The results show that 
the decoding time of D.Digest and our scheme increase roughly linearly along with $t$, whereas 
that of Minisketch increases roughly quadratically with $t$. The decoding time of 
Minisketch is much higher than those of D.Digest and our scheme when $t$ is large (say $\ge$ \num{1000}). 
For example, when $t=$\num{10000}, the decoding time of Minisketch is more than two orders of magnitude 
larger than those of D.Digest and our scheme. 

\autoref{fig:success-rate} shows that all the algorithms achieve an empirical success rate for all 
the different values of $t$ except that the success rate of D.Digest are slightly lower than 0.99 when 
$t\!<\!100$. 


\noindent
{\bf Our Scheme vs. Graphene}. 
Then, we compare our scheme against Graphene. 
We separate the comparisons against Graphene from those against others for two reasons. 
First, Graphene does not require an estimator. 
Second, we only have the pre-computed parameters (provided by the authors of~\cite{Ozisik2019}) 
optimized for a success rate of 239/240 instead of 0.99. 
For fair comparisons, we set the parameters for our scheme to roughly ensure a success rate of 239/240, 
though, as shown in~\autoref{fig:success-rate}, our scheme already achieves this success rate empirically by 
using parameters calcluated for ensuring a success rate of 0.99. 
As shown~\autoref{fig:success-rate-vs-graphene}, both Graphene and our scheme have achieved success rates higher 
than 239/240 empirically. 

\autoref{fig:comm-cost-vs-graphene} presents the communication overheads of Graphene and our scheme (with 
2 and 3 rounds). For our scheme, we include those for our ToW estimator. 
The eesults show that our scheme has lower communication overheads than Graphene 
under almost values of $t$ except for those close to \num{10000} 
where our scheme has slightly higher communication overheads than Graphene. 
The results also show that the average 
communication per element in the set difference gets smaller for Graphene. 
For $t\!<\!$\num{1000}, it is mainly because the IBF requires less cells per 
element as $t$ gets larger to ensure the same success rate, as shown in Figure 7 
of~\cite{Eppstein_WhatsDifference?Efficient_2011}. When $t\ge 1000$, the average number of cells per 
element is almost independent of $t$ (remains the same as $t$ increases). The average communication 
per element (in the set difference) continues to decrease 
because when $t$ is large enough the BF in Graphene can help 
reduce the number of cells required by the IBFs thus resulting in a lower communication overhead per 
element in the set difference.  

We note that the scenarios (more precisely, the partition scenarios of elements in $A\Delta B$) are the best 
cases for Graphene. In more general cases ({\it i.e.,} $B$ is not a subset of $A$), the communication overheads 
of Graphene would be higher than those we reported in~\autoref{fig:comm-cost-vs-graphene}. 

We did not compare the encoding and decoding time of 
our scheme against Graphene because Graphene is implemented in Python, whereas our scheme is implemented in C++.  
% We note that the asymptotic encoding computational complexity is the same as that of our scheme and 
% its decoding computational complexity is 

% for two reasons. 
% First, asymptotically, 
% its decoding complexity is $O(|A|+|B|)$ which is much higher than $O(t)$, 
% the asymptotic decoding complexity. Second, 
% Graphene is implemented in Python, whereas our scheme is implemented in C++.  
% Though we found that the encoding and decoding time of our scheme is shorter than 
% those of Graphene, it is fair for Gra

% \begin{figure*}
% \centering
% \begin{minipage}{0.32\textwidth}
% \includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/communication_costs}
% \caption{Communication overheads.}
% \label{fig:communication-costs}
% \end{minipage}%
% \begin{minipage}{0.32\textwidth}
% \includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/decoding_time}
% \caption{Decoding time.}
% \label{fig:decoding-time}
% \end{minipage}%
% \begin{minipage}{0.32\textwidth}
% \includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/success_rate}
% \caption{Success rate.}
% \label{fig:success-rate}
% \end{minipage}
% \end{figure*}



\begin{figure}
\centering
\begin{subfigure}[t]{0.25\textwidth}
    \centering
    \includegraphics[width=1.0\textwidth]{figures/reconciliation/success-rate-239-240/communication_costs_vs_Graphene_v2}
    \caption{Communication overheads.}% (including those of the ToW estimator).}
    \label{fig:comm-cost-vs-graphene}
\end{subfigure}%
\begin{subfigure}[t]{0.25\textwidth}
    \centering
    \includegraphics[width=1.0\textwidth]{figures/reconciliation/success-rate-239-240/success_rate_vs_Graphene_v2}
    \caption{Success rate.} \label{fig:success-rate-vs-graphene} %%%%%
\end{subfigure}
\caption{Comparisons against Graphene.}\label{fig:vs-graphene}
\end{figure}

\end{comment}
\begin{comment}
\noindent
{\bf Is multiple rounds a issue?} Readers might think that our scheme might have longer latency 
than D.Digest and Minisketch, as they only require 1 round whereas our scheme requires more 
than 1. However, multiple rounds will not increase the latency of our scheme. 
To support it, we present the ratio of the number of elements successfully recovered in each round 
of our scheme in~\autoref{fig:recovered-ratio}. For our scheme running 2 rounds (or 3 rounds), more than 97\% (or 95\%) of elements 
in the set difference are successfully recovered in the first round. Therefore, the underlying synchronization 
process ({\it e.g.,} file synchronization) can start immediately after the first round of our scheme and do not need to wait until our reconciliation algorithm finishes. 
\end{comment}

% \noindent
% {\bf Per-Round Performance of Our Scheme.} 
% % Readers might think that our scheme might have longer latency 
% % than D.Digest and Minisketch, as they only require 1 round whereas our scheme requires more 
% % than 1. However, multiple rounds will not increase the latency of our scheme. 
% Now, we investigate the per-round performance of our scheme. 
% We present the ratio of the number of elements successfully recovered in each round 
% of our scheme in~\autoref{fig:recovered-ratio}, which shows that 
% our scheme running 2 rounds (or 3 rounds) can successfully recover more than 97\% (or 95\%) of elements 
% in the set difference in the first round. Therefore, the underlying synchronization 
% process ({\it e.g.,} file synchronization) can start immediately after 
% the first round of our scheme and do not have to wait until the set reconciliation finishes. 

\begin{comment}

\noindent
% {\bf Per-Round Performance of PBS.} 
{\bf Piecewise Decodability of PBS.}
% Readers might think that our scheme might have longer latency 
% than D.Digest and Minisketch, as they only require 1 round whereas our scheme requires more 
% than 1. However, multiple rounds will not increase the latency of our scheme. 
% Now, we investigate the per-round performance of PBS. 
Recall from~\autoref{sec:intro} that the only minor tradeoff of PBS is that the number of 
rounds (of message exchanges) needed by PBS is slightly larger than existing solutions. \autoref{fig:avg-num-rounds} 
presents the average number of rounds required by PBS with $r\!=$ 2 or 3 respectively. 
However, thanks to the piecewise decodability (that existing solutions do not have), the vast majority 
of all distinct elements are successfully reconciled in the first round. 
The ratio is presented in~\autoref{fig:recovered-ratio}, which shows that 
PBS with $r\!=$ 2 (or 3) can successfully reconcile more than 97\% (or 95\%) of all the distinct elements 
in the first round. Therefore, this tradeoff does not lead to longer response time because the reconciliation of objects identified
the successfully decodable ``codewords'' (hash signatures) can run in parallel with the transmissions and decodings of the rest. 

% the underlying synchronization 
% process ({\it e.g.,} file synchronization) can start immediately after 
% the first round of our scheme and do not have to wait until the set reconciliation finishes. 


We note that only those instances in which all distinct elements are successfully 
reconciled are considered in~\autoref{fig:avg-num-rounds} and~\autoref{fig:recovered-ratio}. 
Unlike in the existing solutions where nothing can be reconciled in the failed instances\footnote{We note that ``piecewise decodability'' can be also achieved in IBF-based solutions, as IBF-based solutions can also decode part of the distinct elements when decoding fails. However, on one hand, no existing solutions even mention this. On the other hand, the ``piecewise decodability'' of IBF-based solutions is much less efficient than that of PBS.}, the vast majority of 
all distinct elements are successfully reconciled in those failed instances in PBS because of its piecewise decodability. 
Furthermore, through experiments, 
we found that the rest distinct elements in those failed instances can be successfully reconciled with one more round of message exchanges  
({\it i.e.,} running one more round of PBS), and only negligible communication overhead incurred (thanks to piecewise decodability). In other words, failed instances lead to 
negligible penalties in PBS, whereas, in all the existing solutions, failed instances would result in hefty penalties, as they do not have 
piecewise decodability.


% \begin{figure}
% \centering
% \begin{subfigure}[t]{0.25\textwidth}
%     \centering
%     \includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/portion_recovered_max_round2_curve}
%     \caption{r=2.}\label{fig:recovered-ratio-r2}
% \end{subfigure}%
% \begin{subfigure}[t]{0.25\textwidth}
%     \centering
%     \includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/portion_recovered_max_round3_curve}
%     \caption{r=3.} \label{fig:recovered-ratio-r3} %%%%%
% \end{subfigure}
% \caption{Recovered ratio in each round.}\label{fig:recovered-ratio}
% \end{figure}

\begin{figure}
\centering
\begin{minipage}[t]{0.23\textwidth}
    \centering
    \includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/pbs_avg_rounds_wrl}
    \caption{Average number of rounds.} \label{fig:avg-num-rounds} %%%%%
\end{minipage}
\hspace{0.01\textwidth}%
\begin{minipage}[t]{0.23\textwidth}
    \centering
    \includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/pbs_first_round}
    \caption{Recovered ratio in the first round.}\label{fig:recovered-ratio}
\end{minipage}%
% \caption{Recovered ratio in each round.}\label{fig:recovered-ratio}
\end{figure}

% \begin{figure}
% \centering 
% \includegraphics[width=0.5\textwidth]{figures/reconciliation/success-rate-99/communication_costs_verying_key_sizes_d10000}
% \caption{Communication overheads (excluding those of the ToW estimator) of Minisketch, D.Digest, and our schemes under various key sizes.}\label{fig:varying-key-sizes}
% \end{figure}
\subsubsection{Varying Key Sizes}\label{sucsec:varying-key-sizes}

In real applications, the key size (length of each element in the universe) might be much higher than 
4 bytes. For example, the transaction ID in Bitcoin applications could 
have 256 bytes~\cite{naumenko2019bandwidth}. 
We investigate how the communication overhead of each algorithm changes as the key size $u$ increases. 
We consider key sizes varying from 4 bytes to 256 bytes. 
Same as before, we separate the comparisons 
against D.Digest and Minisketch and those against Graphene. 
The results are shown in~\autoref{fig:cc-comp-vk} and~\autoref{fig:cc-comp-vk-vs-graphene} respectively. 

Same as before, for the results in~\autoref{fig:cc-comp-vk}, we make each algorithm ensure a success rate of 
0.99 and exclude the communication required by the estimator for all algorithms. For those in~\autoref{fig:cc-comp-vk-vs-graphene}, we make our scheme and Graphene ensure a success rate of 239/240 and include 
the communication required by the estimator for our scheme (note that Graphene does not require an estimator). 

As shown in~\autoref{fig:cc-comp-vk} and~\autoref{fig:cc-comp-vk-vs-graphene}, our scheme has the best 
scaling behavior among all these algorithms. For D.Digest and Minisketch, the communication overheads double 
as the key size doubles, whereas the communication overhead increases much slower in our scheme 
as the key size increases. 
For Graphene, when $t\!=\!$\num{100} and $t\!=\!$\num{1000}, its scaling behavior is almost the same as D.Digest, since as explained in~\autoref{subsec:recon-bench}, Graphene almost reduces to an IBF-only solution when $t\ll|A\cup B|$. When $t=$\num{10000}, the scaling behavior is very close to that of our scheme, as now the communication overheads resulting from IBFs in Graphene is around 40\% and those for the BFs do not increase as the key size. 

\begin{figure*}[!htbp]
\centering
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/communication_costs_verying_key_sizes_d100}
\caption{t=100.}
\label{fig:-d100}
\end{subfigure}%
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/communication_costs_verying_key_sizes_d1000}
\caption{t=\num{1000}.}
\label{-d1000}
\end{subfigure}%
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/communication_costs_verying_key_sizes_d10000}
\caption{t=\num{10000}.}
\label{fig:-d10000}
\end{subfigure}
\caption{Communication overheads of Minisketch, D.Digest, and our schemes under various key sizes.}% with at least 99\% success rate.}
\label{fig:cc-comp-vk}
\end{figure*}

\begin{figure*}[!htbp]
\centering
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-239-240/vs_graphene_verying_key_sizes_d100}
\caption{t=100.}
\label{fig:vs-graphene-d100}
\end{subfigure}%
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-239-240/vs_graphene_verying_key_sizes_d1000}
\caption{t=\num{1000}.}
\label{fig:vs-graphene-d1000}
\end{subfigure}%
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-239-240/vs_graphene_verying_key_sizes_d10000}
\caption{t=\num{10000}.}
\label{fig:vs-graphene-d10000}
\end{subfigure}
\caption{Communication overheads of Graphene and our schemes under various key sizes.}% with at least 99\% success rate.}
\label{fig:cc-comp-vk-vs-graphene}
\end{figure*}

\subsubsection{What If Minisketch Also Uses Partitions?}\label{subsec:mini-partition}

The success we have with our scheme leads readers to wonder what if we apply the partition 
idea to Minisketch. For example, like in our scheme, we partition all elements into several subsets 
so that each subset contains a few elements (say $5$) on average from the set difference. Then, for 
each subset we create BCH codes with a capacity large enough so that we can ensure a desired success rate. 
We refer to this new scheme as Minisketch With Partition, or Minisketch/WP for short. 

We compare the performances of our scheme with those of Minisketch/WP with a desired success rate of 
0.99. For Minisketch/WP, we set the average number of elements from the set difference to $5$ (same 
as our scheme) and use the same BCH decoding capacity for all subsets. We tune this capacity to the best: 
the one with the minimum communication overhead yet ensures a success rate of at least 0.99.    

\autoref{fig:cc-comp-vs-minisketchwp} presents the communication overheads under different key sizes varying 
from 4 bytes to 256 bytes for three different set-difference sizes \numlist{100;1000;10000}. 
The sesults show that Minisketch/WP has similar or 
slightly lower communication overheads than our scheme only when the key size is 4 bytes. This advantage 
diminishes as the key size gets larger and our scheme is consistently better when the key size is no less than 
$16$ bytes. Hence, we conclude that our scheme overall remains the best practical solution for the 
set reconciliation problem.




% \begin{figure*}[!htbp]
% \centering
% \begin{subfigure}[t]{0.32\textwidth}
% \includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/vs_minisketchwp_verying_key_sizes_d100}
% \caption{t=\num{100}.}
% \label{fig:vs-minisketchwp-d100}
% \end{subfigure}%
% \begin{subfigure}[t]{0.32\textwidth}
% \includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/vs_minisketchwp_verying_key_sizes_d1000}
% \caption{t=\num{1000}.}
% \label{fig:vs-minisketchwp-d1000}
% \end{subfigure}%
% \begin{subfigure}[t]{0.32\textwidth}
% \includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/vs_minisketchwp_verying_key_sizes_d10000}
% \caption{t=\num{10000}.}
% \label{fig:vs-minisketchwp-d10000}
% \end{subfigure}
% \caption{Communication overheads of our schemes against those of Minisketch/WP.}% with at least 99\% success rate.}
% \label{fig:cc-comp-vs-minisketchwp}
% \end{figure*}

\begin{figure*}[!htbp]
\centering
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/vs_minisketchwp_match_varying_key_sizes_d100}
\caption{t=\num{100}.}
\label{fig:vs-minisketchwp-d100}
\end{subfigure}%
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/vs_minisketchwp_match_varying_key_sizes_d1000}
\caption{t=\num{1000}.}
\label{fig:vs-minisketchwp-d1000}
\end{subfigure}%
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/vs_minisketchwp_match_varying_key_sizes_d10000}
\caption{t=\num{10000}.}
\label{fig:vs-minisketchwp-d10000}
\end{subfigure}
\caption{Communication overheads of our schemes against those of Minisketch/WP.}% with at least 99\% success rate.}
\label{fig:cc-comp-vs-minisketchwp}
\end{figure*}

\end{comment}

==> section/evaluation-BK2.tex <==
\section{Performance Evaluation}\label{sec:evaluation}
%% Experiments for estimators

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% Task 1.1: Experiments %%%%%%%%%%%%%%%%%%%%%%%%
%==> I will start (and hopefully complete) this experiments by the mid-night of Nov. 17, 2019. ---- Long
%%% Benchmark estimators: Strata Estimator/min-hash/Bagminhash 
%%% MSE (??) plus Correction overhead
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%% Experiments for Reconciliation

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% Task 1.2: Experiments %%%%%%%%%%%%%%%%%%%%%%%%
%==> I need some time to figure out how to use (or even modify) the source codes of Graphene ---- Long
%==> Hopefully, I can finish this part by the end of the next week (Nov. 22, 2019)
%%% Benchmark algorithms: minisketch/Graphene/KeyDiff
%%% 99% (??) reconciliation correction rate in one round (CO v.s. d) with roughly the same computational complexity 
%%% 95% (??) decoding rate in one round (CO v.s. d)
%%% multiple rounds for our scheme (maybe also for minisketch)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% Task 2.1: Writing %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%==> While conducting those experiments, I will also add the paragraphs for evaluation.   --- Long
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% Task 2.2: Writing %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%==> I have added a few more papers on this topic. If you (@ziheng) have  some time, you can help us add some sentences regarding them in the  related work section. I will also read them and try to produce some paragraphs.  --- Long
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%% To ZiHeng %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%==> If you have any suggestions of concerns regarding the above plan, please feel free to ``shoot'' to us. ---- Long
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% In this section, we evaluate the performances of our ToW estimator 
% and our set reconciliation algorithm.

% % 
In this section, we evaluate the performance of PBS, and compare 
it with Difference Digest (D.Digest)~\cite{Eppstein_WhatsDifference?Efficient_2011}, 
Graphene~\cite{Ozisik2019}, and PinSketch~\cite{Dodis_PinSketch_2008}, which we have 
described in detail in~\autoref{subsec:recon-bench}. 

% {\bf A short paragraph summarizes the conclusions of the evaluation}

The following conclusions are drawn from this evaluation:
\begin{sitemize}
% \item PBS strikes an excellent balance between communication overhead and computational overhead: It achieves communication overhead close to that of PinSketch (the best in terms of communication overhead), yet has the lowest computational overhead. 
\item PBS strikes much better balance between communication overhead and computational overhead than existing work: 
It has a communication overhead much lower than those of D.Digest and Graphene but slightly higher than that of PinSketch, yet has the lowest computational overhead which can be up to three orders of magnitude lower than that of PinSketch. 
\item The piecewise decodability of PBS, 
% which all existing set reconciliation algorithms do not have,  
which none of existing set reconciliation algorithms has, 
significantly reduces the penalty when failure happens. 
\item PBS scales the best with respect to the signature width $\log |\mathcal{U}|$, which makes it an excellent candidate for applications that 
have large signature widths.
\item To ensure the same success rate, less rounds (as low as 2 rounds) can be achieved in PBS by paying only marginal cost.  
\end{sitemize}
% \subsection{Methodologies}\label{subsec:exp-methodologies}

\subsection{Experiment Setup}\label{subsec:exp-setup}

% In our evaluation, we first fix signature width $w$ (see~\autoref{sec:model}) 
% as $32$ bits. 

We first evaluate a key space (universe) $\mathcal{U}$ of $32$-bit binary strings, 
{\it i.e.,} $\log|\mathcal{U}|\!=\!32$. 
Later, in~\autoref{subsubsec:varying-sig-width} we evaluate how the performances 
% of these algorithms 
scale with respect to $\log|\mathcal{U}|$.  
%
% Besides these two, a third 
% degree of freedom is how many distinct elements in $A\Delta B$ are from $A$ (or $B$).  
% We defer the explanation of why we do not exercise this degree of freedom later in~\autoref{subsubsec:discussion}. 
%
Like in~\cite{Eppstein_WhatsDifference?Efficient_2011}, each pair of sets, 
$A$ (stored at Alice) and $B$ (stored at Bob), was created as follows. 
% was created by exercising two degrees of freedom: the number of elements in $A$, 
% and the size $d$ of the set difference $A \Delta B$. 
% First, we drawn $10^5$ elements from the universe $\mathcal{U}$ 
% uniformly at random without replacement, 
% which made up the set $A$. 
First, elements in $A$ were drawn from %the universe 
$\mathcal{U}$ 
uniformly at random without replacement. 
A certain number %(more precisely, $|A|\!-\!d$) 
of elements in $A$ were then sampled also 
uniformly at random without replacement  
and made up set $B$ so that the set difference $A\Delta B$ 
contains exactly $d$ elements. 
In such a setting, set $B$ contains no distinct elements, {\it i.e.,} 
$B$ is a subset of $A$. 
We defer the explanation of why we do not consider the scenarios where 
$B$ also contains some distinct elements later in~\autoref{subsubsec:discussion}. 
In all experiments, we set the cardinality of $A$ to $10^5$ and 
let the value of $d$ vary from $10$ to $10^4$. 
% 
For each value of $d$, we created \num{1000} different pairs of $A$ and $B$, which are mutually independent.   
Each point in our plots in the evaluation results  
is the average of the corresponding \num{1000} independent experiment instances. 
%
All experiments were performed on a workstation with an Intel Core i7-9800X processor 
running Ubuntu 18.0.4. 

++++ {\bf The following sentence can be removed if we have defined success rate before.} 

Like in~\cite{Eppstein_WhatsDifference?Efficient_2011,Ozisik2019}, we consider an experiment instance for an algorithm 
successful only if the algorithm is able to successfully determine
all of the distinct elements, no more, no less. 

Like in most set reconciliation literature, our evaluation mainly focused on 
two performance metrics: {\it communication overhead} and {\it computational overhead} (more precisely, encoding time and decoding time). 
As mentioned earlier in~\autoref{sec:model}, 
% we only considered the unidirectional set reconciliation in which either Alice or Bob (not both) learns $A\Delta B$. 
% we only considered the unidirectional set reconciliation in which Bob learns $A\Delta B$ in all evaluated algorithms 
% except Graphene, in which we let Alice learn $A\Delta B$.  
we only considered the unidirectional set reconciliation in which Alice learns $A\Delta B$. %in all evaluated algorithms 
% except Graphene, in which we let Alice learn $A\Delta B$.  
Hence, communication overhead was measured by the total amount of data 
transmitted between Alice and Bob to ensure that Alice %Bob (or Alice in Graphene) 
learns $A\Delta B$. The computational overhead was measured similarly. 
We emphasize that, given sets $A$ and $B$, the communication overhead and computational overhead are independent 
of whom (Alice or Bob) learns $A\Delta B$ in the 
unidirectional set reconciliation in all evaluated algorithms except Graphene. 
% In Graphene, we let Alice to learn $A\Delta B$. 
% It is not unfair to 
% Graphene, a
As we will explain later in~\autoref{subsubsec:discussion}, this scenario 
({\it i.e.,} $B\subset A$ and Alice learns $A\Delta B$) is 
the best 
% (in terms of communication overhead) 
scenario for Graphene. Therefore, it is not unfair to Graphene. 
% In most set reconciliation algorithms, 
% ``this whom'' can be simply adapted by controlling whom initiating the 
% set reconciliation process. However, in some reconciliation algorithms, 
% ``this whom'' is determined whenever $A$ and $B$ are determined. For example, 
% in Graphene, ``this whom'' is always the one whose set size is larger. 

Note that for algorithms that need multiple rounds of message exchanges, like PBS, 
both communication overhead and computational overhead shown in the evaluation results %~\autoref{subsec:recon-perf} 
are the sum over all these rounds. 


\subsubsection{Parameter Configurations}\label{subsubsec:configuration}

Our evaluation assumed that the set difference cardinality $d$ is not known a prior, which is common in many applications. 
++++ {\bf Although Prof. Jim has suggested to write a similar short paragraph (to emphasize ToW is the best) in the estimator section, 
I still think it is more natural to mention it here, because we have to give necessary details on the experiments of estimators here.} 
We used a ToW estimator with 128 sketches ({\it i.e.,} $k\!=\!$128) to 
obtain an estimate $\hat{d}$ of $d$ in our evaluation 
whenever a set reconciliation algorithm requires an estimator, because 
the ToW estimator was shown, through experiments (the results were not shown here in the interest of space), 
to have the best overall performance among all commonly used estimators ({\it e.g.,} the Min-wise 
estimator~\cite{Broder_MinWiseIndependent_2000} and the Strata estimator~\cite{Eppstein_WhatsDifference?Efficient_2011}) 
in terms of space-efficiency, accuracy, and implementation complexity. 
Recall from~\autoref{subsec:ToW} that in many applications, the estimate $\hat{d}$ is usually scaled up 
by a proper factor $\gamma$ so that the scaled estimate $\gamma\hat{d}$ is no smaller than the ground 
truth $d$ with a high enough probability $\beta$, {\it i.e.,} $\mathbf{P}[\gamma \hat{d} \ge d]\ge\beta$. 
Through experiments, we investigated the smallest factors ($\gamma$'s) of ToW estimators for 
various assurance probabilities ($\beta$'s). For example, the smallest $\gamma$ is $1.38$ when $\beta\!=\!0.99$.  
% {\it i.e.,} $\mathbf{P}[1.38\hat{d}\!\ge\! d]\!\ge\!0.99$. % with a probability of at least 0.99. 
% For example, through experiments, we found to make $\beta\!=\!0.99$, 
% {\it i.e.,} $\alpha\hat{d}\!\ge\! d$ with a probability of at least 0.99, $\alpha$ 
% should be set to $1.38$. 
% Like in~\cite{Eppstein_WhatsDifference?Efficient_2011}, the estimate $\hat{d}$ is scaled up 
% by a proper factor (1.38 in our evaluation) so that the scaled estimate is no smaller than the ground 
% truth with a high enough probability (99\% in our evaluation). 
We note that all evaluated algorithms except Graphene require  
an estimator. For these algorithms, in all plots for their communication overheads shown in the evaluation results, 
% the amount of 
the overhead resulted from the ToW estimator, 
more precisely 288 bytes\footnote{We assume that each ToW sketch takes $\lceil \log_2 (2d_{max} + 1)\rceil\!=\!18$ 
bits as each ToW sketch is an integer within the range of $[-d_{max},d_{max}]$, where $d_{max}\!=\!10^5$ is the 
largest possible set difference cardinality,  
like in~\cite{Eppstein_WhatsDifference?Efficient_2011}, we assume it is known a prior.},  
was excluded. For fair comparison, we subtracted the same  
amount ({\it i.e.,} 288 bytes) from the communication overheads of Graphene, as it does not require an estimator. 


% We note that all of the evaluated algorithms might fail, {\it i.e.,} they cannot determine all 
% the distinct elements in some instances. 
% We note that e
Each of the evaluated algorithms might fail. 
% to determine all of the distinct elements in some 
% instances. 
For example, PinSketch fails if the true set difference cardinality $d$ is larger than its BCH decoding 
capacity $t$.  
% As explained earlier in~\autoref{subsec:ToW}, 
++++ {\bf The following sentence can be simplified, if we have defined and explained success rate in previous section.} 
In real applications, 
a set reconciliation algorithm should be properly configured 
so that it has a high enough {\it success rate} (say $0.99$): The fraction of successful experiment instances among all instances. 
Clearly, a higher success rate requires ``higher price'' ({\it e.g.,} higher communication overhead and/or more rounds of message exchanges).  
To fairly compare these set reconciliation algorithms, we should properly configure their 
parameters so that they roughly have the same success rate. 
Unfortunately, in the paper of D.Digest~\cite{Eppstein_WhatsDifference?Efficient_2011}, the authors 
only suggested the parameter setting tuned for a success rate of roughly 0.99, whereas 
we only have the pre-computed parameter tables (provided by the authors of~\cite{Ozisik2019}) 
tuned for a success rate of roughly 239/240 ($\!\approx\!0.9958$) instead of 0.99. 
Tuning parameters of these algorithms is out scope of this paper,  
hence we 
% used the parameters suggested or provided by the corresponding authors and 
% configured our 
tuned the parameters of PBS 
to match their success rates respectively. 
In~\autoref{subsec:recon-perf}, we first compared PBS against D.Digest and PinSketch with each of 
them %configuring to ensure 
tuning for a success rate of roughly 0.99, and then we compared PBS against 
Graphene with each of them %configuring to ensure 
tuning for a success rate of roughly 239/240. 
Now, we describe, in detail, the parameter settings for all of them. 

\noindent
{\bf D.Digest}. 
Like in~\cite{Eppstein_WhatsDifference?Efficient_2011}, 
we allocated $3\log|\mathcal{U}|$ bits for each IBF cell in D.Digest, with $\log|\mathcal{U}|$ bits given to each of the three fields in a cell. 
We used the parameter setting suggested in~\cite{Eppstein_WhatsDifference?Efficient_2011}: 
$2\hat{d}$ IBF cells, where $\hat{d}$ is the estimate of the set difference cardinality, 
and $3$ hash functions for estimates greater than $200$; otherwise we used $4$ hash functions. 
Recall from~\autoref{subsec:ToW} that the ToW estimator is unbiased, {\it i.e.,}
% shown in~\autoref{eq:tow}, 
$\mathbf{E}[\hat{d}]\!=\!d$, therefore, 
the communication overhead of D.Digest is on average $6d\log|\mathcal{U}|$ bits, which is $6$ times of the minimum.  
% As mentioned earlier in this section, 
As shown in~\cite{Eppstein_WhatsDifference?Efficient_2011}, with this parameter setting, 
D.Digest ensures a success rate of roughly 0.99. 
% That is, for roughly 99\% of the experiment 
% instances, the reconciliation should succeed. 

\noindent
{\bf PinSketch}. 
For PinSketch, we set the decoding capacity of the BCH code, the only parameter in PinSketch, to $t\!=\!1.38\hat{d}$.  
% Recall from~\autoref{sec:scheme} that, i
It is not hard to check the communication overhead of PinSketch, under this parameter 
setting, is on average $1.38d\log|\mathcal{U}|$ bits, which is $1.38$ times of the minimum. 
As explained earlier in this section, 
$\mathbf{P}[1.38\hat{d}\!\ge\! d]\!\ge\!0.99$, thus, 
$\mathbf{P}[t\!\ge\! d]\!\ge\!0.99$. 
% by scaling up by a factor of 1.38, 
% the scaled estimate $1.38\hat{d}$ is no smaller than 
% the ground truth (the true set-difference size $d$) with a probability of at least 0.99, 
% {\it i.e.,} $t\!=\!1.38\hat{d}\ge d$ with a probability of at least 0.99. 
% Therefore, the decoding capacity $t$ would be no smaller 
% than the set-difference size $d$ with a probability of 0.99. 
% As explained earlier, 
Therefore, the reconciliation should succeed   
with a probability of at least 0.99. In other words, with this parameter setting, PinSketch %also 
ensures a success rate of at least 0.99. 

\noindent
{\bf Graphene}.
Like we did for D.Digest, 
we allocated $3\log|\mathcal{U}|$ bits for each IBF cell in Graphene, 
with $\log|\mathcal{U}|$ bits given to each of the three fields in a cell. 
For Graphene, we used the pre-computed parameter settings ({\it e.g.,} how many hash 
functions and cells should be used in the IBF)
provided by the authors of~\cite{Ozisik2019} tuned for a success rate of 239/240. 

\noindent
{\bf PBS}.  
% We set the maximum number of rounds, $r\!=\!3$. 
% Later, in~\autoref{subsec:recon-perf}, we investigated how the performances of PBS 
% scale with respect to $r$. 
% We set $\delta\!=\!5$.  
We first let the target success probability $p_0$=0.99 within $r$=3 rounds. %, {\it i.e.,} we let PBS to 
Later, in~\autoref{subsec:less-rounds}, we investigated how performances of PBS 
scale with respect to $r$. 
% we set $\delta$, the average number of distinct elements in each group,  
% to $5$. 
% We used the same $n$ ({\it i.e.,} number of subset pairs in each group), 
% and $t$ ({\it i.e.,} the decoding capability of the BCH codes) for all groups, the 
% values of which was obtained using our analytical results as follows. 
The values of $n$, number of subset pairs in each group, and $t$, 
BCH decode capability in each group, are set 
based on the set difference cardinality estimate $\hat{d}$ (as $d$ is not known).   
% differently for different set-difference size $d$.   
For each $\hat{d}$, we used the parameter setting procedure described 
in~\autoref{sec:parameter_settings} to obtain the values of $n$ and $t$,  
% tuning for a success 
% rate of at least $0.99$ 
by letting the set difference cardinality be the scaled estimate, {\it i.e.,} $1.38\hat{d}$. 
% In other words, if the true set-difference size $d\le 1.38\hat{d}$, PBS (within 3 rounds) should succeed with a 
% probability of at least $0.99$. Therefore, w
It is not hard to check, with this parameter setting,  
PBS strictly ensures a success rate of at least $0.99\times 0.99\!=\!0.9801$: The 
first $0.99$ comes from the assurance from the scaled estimates, {\it i.e.,} $\mathbf{P}[1.38\hat{d}\ge d]\ge 0.99$; 
the second $0.99$ comes from 
the rigorous tail bound derived in~\autoref{sec:tail_bound}. As shown in~\autoref{subsec:recon-perf},   
empirically, the success rates of PBS are much higher than $0.99$ under all different values of $d$. 
We refer to this parameter setting as ``the default setting'' for PBS in the sequel of this section. 
% Need revision
% Later, in~\autoref{subsec:recon-perf}, we investigated how the communication overheads of PBS scale with respect to $r$, 
% more precisely, the communication overheads of PBS ensuring a success rate of $0.99$ within $r$ rounds scale with respect to $r$. 

Similarly, we then tuned PBS to roughly ensure a success rate of $239/240$ 
% ({\it i.e.,} only changing the target success rate from 0.99 to 239/240, the rest remains exactly the same as the default setting) 
when comparing against Graphene. 
\begin{comment}
% seems not quite useful
\autoref{tab:param-pbs} summarizes the values for all parameters in PBS.

\begin{table}
\centering
\caption{Parameters for PBS.}\label{tab:param-pbs}
\begin{tabular}{@{}|c|c|c|c|c|@{}}
\hline 
success rate & $\delta$ & $r$ & $n$ & $t$ \\ \hline 
roughly 0.99     &  \num{5} & \num{3} & \numlist[list-separator = {, },list-final-separator = {, or }]{63;127;255;511} &  \numrange{8}{13} \\ \hline
roughly 239/240  &  \num{5} & \num{3} & \numlist[list-separator = {, },list-final-separator = {, or }]{63;127;255;511} &  \numrange{8}{14} \\ 
\hline 
\end{tabular}
\end{table}
\end{comment}
% We first scaled up the estimates by 1.38. Based on the scaled estimates, 
% we computed the best parameters that can ensure a success rate of at least 
% 0.99 with 3 rounds of PBS
% using our analytical results in~\autoref{sec:tail_bound}. Therefore, our scheme 
% also roughly ensures a success rate of 0.99. 


\subsubsection{Implementations}\label{subsubsec:impl}

We implemented PBS in C++: We used \texttt{xxHash}~\cite{Collet_xxHashExtremelyfast_} for all hash functions needed by PBS 
and Minisketch library~\cite{Wuille_Minisketchoptimizedlibrary_2019} released by the authors of~\cite{naumenko2019bandwidth}, for the BCH encoding and decoding. The Minisketch library was also used in the implementation of PinSketch~\cite{Dodis_PinSketch_2008}.   
For D.Digest, as the authors of~\cite{Eppstein_WhatsDifference?Efficient_2011} did not 
release their source codes, we implemented their scheme by using the optimized open-source implementation of IBFs in C++ released by 
the authors of~\cite{Ozisik2019}. 
%
% Note that, Minisketch is just an optimized implementation of the PinSketch~\cite{Dodis_PinSketch_2008} 
% algorithm. 
For Graphene, we used the source codes provided by the authors of~\cite{Ozisik2019}. 
% Note that, the implementation of Graphene is in Python. 


\subsubsection{Discussions}\label{subsubsec:discussion}

Recall from the experiment setup in~\autoref{subsec:exp-setup}, 
in our evaluation, we only considered 
the scenario where set $B$ contains no distinct elements ({\it i.e.,} $B\subset A$). 
% % explain why we only exercise the above two degrees of freedom (need revision)
% We did not exercise the degree of freedom in varying the sizes of 
% $A\!\setminus\! B$ and $B\!\setminus\! A$ 
This is enough for our evaluation for the following reasons.  
% all estimators compared in~\autoref{subsec:est-perf} are designed for the estimation of 
% only $d$ (not the sizes of $A\setminus B$ and/or $B\setminus A$) %(the size of the set difference $A\Delta B$) 
% % %
% and 
Given $A$ and $d$, communication overhead and decoding time 
of all algorithms except Graphene~\cite{Ozisik2019} 
considered in our evaluation are independent 
of how distinct elements are distributed in $A$ and $B$. 
%
% except 
% for Graphene~\cite{Ozisik2019}. 
% {\bf Revision Required!!} 
% The encoding times of these algorithms will change in the same manner if we 
% change how many distinct elements are distributed in $A$ (or $B$) when $A$ and $d$ are fixed,  
% since, as described in~\autoref{subsec:recon-bench}, the encoding times of all these algorithms are proportional to $|A|\!+\!|B|$. 
%
The communication overhead of Graphene usually depends on how many distinct elements are distributed in 
$A$ (or $B$). However, 
% as shown in~\cite{Ozisik2019}, 
when $A$ and $d$ are fixed, 
the scenario  considered in our evaluation, where set $B$ is a subset of $A$ 
and Alice learns $A\Delta B$ corresponds to the 
% ``simplest'' 
scenario shown in~\cite[Figure 1 (Left)]{Ozisik2019}:  
``the receiver's mempool contains the entire block''. As shown in~\cite{Ozisik2019}, it is
arguably the best scenario (for Graphene) in terms of communication overhead and decoding time.  
For encoding time, the distribution of distinct elements has slight impact. 
However, none of the algorithms can benefit (in terms of encoding time) unfairly from this setup. 
% , 
% because the distribution affects $|B|$ slightly and, as described in~\autoref{sec:closely-related}, all algorithms have an encoding computational complexity proportional 
% to $|A|\!+\!|B|$. 
% However, this slight impact is the same for all algorithms. 

We note that the fact that set $B$ is always a subset of $A$ is not known to any algorithm in our evaluation and 
thus no algorithm takes advantage of this fact. 


\begin{comment}


\subsection{Evaluation of Our ToW Estimator}\label{subsec:est-perf}

In this section, we compare our ToW estimator with two existing algorithms: Strata~\cite{Eppstein_WhatsDifference?Efficient_2011} and min-wise hashing~\cite{Broder_MinWiseIndependent_2000}, which we have described in~\autoref{subsec:est-bench} in detail. In the comparisons, we fix the size of the union $A\cup B$ to 100K and set the value of 
$t$ (the size of the set difference $A\Delta B$) varying from 10 to 10K (or in other words, $t/|A\cup B|$ varying from $10^{-4}$ to $10^{-1}$). 

For our ToW estimator and min-wise hashing, we used  \code{xxHash} hash functions~\cite{Collet_xxHashExtremelyfast_}. 
For Strata, we used the optimized open-source implementation of IBFs~\cite{Ozisik2019}. 

\subsubsection{ToW Estimator: Empirical vs. Analytical}

We first evaluate the empirical accuracy of our ToW estimator against its theoretical accuracy, since 
as mentioned in~\autoref{subsec:ToW} the hash family for calculating the ToW sketches should be 
four-wise independent to achieve the theoretical accuracy whereas \code{xxHash} might not be. 
We use the relative root mean square error (rRMSE) from the ground truth as the metric. 
%The accuracy is measured by the relative root mean square error (rRMSE) from the ground truth. 
For each value of $t$ (the set-difference size), 
we created $c=$1,000 different pairs of $A$ and $B$ and obtained estimates $\{\hat{t}_i\}_{i=1}^{c}$ using our ToW estimator. %For each estimate $\hat{t}_i$ ($i=1,2,\cdots,c$). 
We calculated the empirical rRMSE, which is defined as,
\begin{equation}
\mbox{\texttt{rRMSE}}(\hat{t})=\frac{1}{t}\sqrt{\frac{1}{c}\sum\limits_{i=1}^c(\hat{t}_i-t)^2}.
\end{equation}

% % Need to check whether "perfect" is the right word.
% In~\autoref{}, we have analyzed the accuracy (variance) of our ToW estimator assuming that the hash functions are perfect. 
% However, the hash functions used in practice are generally not perfect. 
As analyzed in~\autoref{subsec:ToW}, given the ground truth $t$ of the set-difference size, 
the variance of our ToW estimator with $k$ sketches is $\frac{2t^2-2t}{k}$. 
Therefore, the analytical rRMSE of our ToW estimator is $\frac{1}{t}\sqrt{\mbox{\bf Var}(\hat{t})}\!=\!\sqrt{\frac{2}{k}(1-\frac{1}{t})}$. 

\autoref{fig:rrmse} reports the empirical and analytical rRMSE of our ToW estimator. We only present the 
results for $t=10$ (\autoref{fig:rrmse-10}) and $t=\num{10000}$ (\autoref{fig:rrmse-10000}), since the 
empirical results are nearly identical to the analytical results under all different values of $t$,  
like what have been shown in \autoref{fig:rrmse-10} and \autoref{fig:rrmse-10000}. 

% \begin{figure}
% \centering
% \includegraphics[width=0.49\textwidth]{figures/estimator/rrmse}
% \caption{rRMSE of ToW.}\label{fig:rrmse}
% \end{figure}


\begin{figure}
\centering
\begin{subfigure}[t]{0.25\textwidth}
    \centering
    \includegraphics[width=1.0\textwidth]{figures/estimator/rrmse_10}
    \caption{t=10.}\label{fig:rrmse-10}
\end{subfigure}%
\begin{subfigure}[t]{0.25\textwidth}
    \centering
    \includegraphics[width=1.0\textwidth]{figures/estimator/rrmse_10000}
    \caption{t=\num{10000}.} \label{fig:rrmse-10000} %%%%%
\end{subfigure}
\caption{rRMSE of ToW.}\label{fig:rrmse}
\end{figure}

% 121	1.30000000000000
% 113	1.31000000000000
% 106	1.32000000000000
% 100	1.33000000000000
% 94	1.34000000000000
% 89	1.35000000000000
% 84	1.36000000000000
% 80	1.37000000000000
% 75	1.38000000000000
% 72	1.39000000000000
% 68	1.40000000000000
% 65	1.41000000000000
% 62	1.42000000000000
% 59	1.43000000000000
% 56	1.44000000000000
% 54	1.45000000000000
% 52	1.46000000000000
% 49	1.47000000000000
% 47	1.48000000000000
% 46	1.49000000000000
% 44	1.50000000000000

% \subsubsection{Correction Overheads}
\subsubsection{ToW Estimator vs. Prior Estimators}

The objective of an estimator for the set-difference size $t$ in the context of 
set reconciliation is to provide estimates with high-enough accuracy. 
On one hand, if the estimator over-estimates, the subsequent reconciliation will 
usually waste unnecessary bandwidth. 
On the other hand, if the estimator under-estimates, the reconciliation might fail. 
Hence, in practice, the estimate returned by the estimator is usually 
scaled up by a proper factor to ensure that the failure rarely happens. 


Now, we compare the scaling ratios, which we call the {\it correction overheads} like 
in~\cite{Eppstein_WhatsDifference?Efficient_2011}, of the three estimators. 
For each value of $t$, we created \num{10000} different pairs of $A$ and $B$, obtained 
estimates from the three estimators, and then calculated the required correction overhead 
for each estimator to ensure that 99\% estimates are larger than or equal to the ground 
truth. For Strata, we used the best parameters reported in~\cite{Eppstein_WhatsDifference?Efficient_2011} for 
our experimental configuration (the same as that in~\cite{Eppstein_WhatsDifference?Efficient_2011}): 
$3$ hash functions for each IBF, and $16$ strata each with $80$ cells. We note that this parameter 
setting assumes the approximate total set size ({\it i.e.,} 100K), or in other words the 
largest possible set-difference size $t_{max}$ is known a prior; Otherwise, more 
strata should be used. We assume that each ToW sketch takes $\lceil \log_2 (2t_{max} + 1)\rceil\!=\!18$ 
bits as each ToW sketch is an integer within the range of $[-t_{max},t_{max}]$. 
For our ToW estimator, we first calculate an approximate number of sketches required to achieve comparable 
correction overheads as Strata by using the central limit theorem (CLT) and then tune the exact number of 
sketches (we only tested the values of power of $2$ for saving time). For min-wise estimator, we use the 
same number of hashes as the number of sketches in our ToW estimator. 
The experimental results are reported in~\autoref{fig:co}. For ToW estimator and min-wise estimator, we only show the results for $k\!=\!128$ and $256$. 

\noindent
{\bf ToW vs. Strata}. As shown in~\autoref{fig:co}, our ToW estimator with $128$ sketches already 
achieves comparable correction overheads as Strata. Note that the estimates should be scaled up be a 
factor according to the worst case among all the points shown in~\autoref{fig:co} for each estimator. 
%as the ground truth of the set-difference size $t$ is not known a prior. 
That is, the estimates have 
to be scaled up by a factor (correction overhead) of $1.36$ and $1.38$ using Strata and 128-sketch ToW estimator 
respectively. If using 256 sketches, ToW estimator only requires this factor to be 
$1.25$. Now, we 
compare the space required by Strata and ToW estimator with 128 sketches. Our ToW estimator 
with 128 sketches only requires 288 bytes. As each cell in Strata 
requires 12 bytes (4 bytes for each field), the space required for Strata is 15 KB, which is around 
$53$ times of that of ToW estimator. 

\noindent
{\bf ToW vs. min-wise}. Now, we compare our ToW estimator with min-wise estimator. 
As shown in~\autoref{fig:co}, the correction overhead only becomes less than $3$ when 
$t$ gets larger than \num{7000} for the min-wise estimator with 128 hashes. Even when using 
256 hashes, min-wise estimator still requires this factor to be larger than 3 for most 
of the values (of $t$) we experimented. We note that for $t\leq 400$, 
most estimates returned from min-wise 
estimator is 0, which results in an infinite correction overhead. In fact, as reported in~\cite{Eppstein_WhatsDifference?Efficient_2011}, even when using thousands of hash functions (more precisely, 
\num{3840} hashes), 
min-wise estimator can still have an infinite correction overhead when $t\!<\!200$. 
Therefore, we conclude that min-wise estimator 
is not a feasible estimator for the set-difference size when $t\!\ll\! |A\cup B|$. 

\noindent
{\bf Summary}. Through the above comparisons with Strata and min-wise estimators, we conclude that 
our ToW estimator is much more space-efficient for achieving the same accuracy. Besides, the parameter 
setting for our ToW estimator is much easier. On one hand, 
our ToW estimator only has one parameter, 
{\it i.e.,} number of sketches, whereas Strata has 3 parameters ({\it i.e.,} number of 
strata, number of cells and number of hashes for each IBF). 
On the other hand, number of sketches (of ToW estimator) required for achieving a desired 
correction overhead is almost independent of $t$ and 
$|A|$ and $|B|$, whereas Strata should set the number of strata according to maximum possible 
set-difference size and number of hashes required by min-wise estimator 
for achieving a desired correction overhead is highly dependent on the ratio $t/|A\cup B|$. 



% \begin{figure}
% \centering
% \begin{subfigure}[t]{0.25\textwidth}
%     \centering
%     \includegraphics[width=0.99\textwidth]{figures/estimator/co_95}
%     \caption{95\%.}\label{fig:co95}
% \end{subfigure}%
% \begin{subfigure}[t]{0.25\textwidth}
%     \centering
%     \includegraphics[width=0.99\textwidth]{figures/estimator/co_99}
%     \caption{99\%.} \label{fig:co99} %%%%%
% \end{subfigure}
% \caption{Correction overheads of different estimators to ensure that at least 95\% and 99\% of the estimates are larger than or equal to the ground truth, respectively.}\label{fig:co}
% \end{figure}

\begin{figure}
\centering
    \centering
    \includegraphics[width=0.49\textwidth]{figures/estimator/co_99_with_minhash_v2}
\caption{Correction overheads of different estimators to ensure that at least 99\% of the estimates are larger than or equal to the ground truth.}\label{fig:co}
\end{figure}
\end{comment}


\subsection{Experiment Results}\label{subsec:recon-perf}

We report the experiment results in this section. Before diving into the detailed results for the two major performance 
metrics ({\it i.e.,} communication overhead and computational overhead),  %in~\autoref{}. 
we first present the empirical 
success rates of all these algorithms %, the results were presented 
in~\autoref{fig:success-rate}. \autoref{fig:success-rate} shows that all these algorithms have achieved empirical success rates 
at least as high as the corresponding target success rates under all 
different values of set difference cardinalities except that the empirical success rates of D.Digest are lower than 0.99, 
its target success rate, when $d\!\le\!30$. 

% The results mainly focused on the communication overheads 
% and decoding time of PBS against prior work
\begin{figure}
\centering
\begin{subfigure}[t]{0.25\textwidth}
\centering
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/success_rate}
% \caption{PBS vs. D.Digest and PinSketch (targeted success rate: 0.99).}
% \caption{Target success rate: 0.99.}
\caption{vs. D.Digest and PinSketch}
\label{fig:success-rate-99}
\end{subfigure}%
\begin{subfigure}[t]{0.25\textwidth}
\centering
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-239-240/success_rate_vs_Graphene_v2}
% \caption{PBS vs. Graphene.}\label{fig:success-rate-9958}
% \caption{Target success rate: 0.9958.}
\caption{vs. Graphene}
\label{fig:success-rate-9958}
\end{subfigure}
\caption{Success rate.}\label{fig:success-rate}
\end{figure}


% \subsubsection{Basic Results}\label{subsubsec:basic}

We now present the experiment results on communication overhead.


\begin{figure}
\centering
\begin{subfigure}[t]{0.25\textwidth}
\centering
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/communication_costs}
% \caption{PBS vs. D.Digest and PinSketch (targeted success rate: 0.99).}
% \caption{Target success rate: 0.99.}
\caption{vs. D.Digest and PinSketch}
\label{fig:co-99}
\end{subfigure}%
\begin{subfigure}[t]{0.25\textwidth}
\centering
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-239-240/communication_costs_vs_Graphene_v2}
% \caption{PBS vs. Graphene.}\label{fig:success-rate-9958}
% \caption{Target success rate: 0.9958.}
\caption{vs. Graphene}
\label{fig:co-9958}
\end{subfigure}
\caption{Communication overheads.}\label{fig:co}
\end{figure}

\smallskip
\noindent
{\bf Communication overhead}.
\autoref{fig:co-99} shows the communication overhead of 
PBS against those of D.Digest and PinSketch, with a target success rate of 0.99. 
% We note that the communication overhead of the estimator is excluded since 
% it is constant (288 bytes) and the same for these algorithms. 
% Results confirm that all these algorithms have the same 
% asymptotic communication complexity, that is $O(t)$. However, the constant factors are different and do 
% matter in practice. 
Results show that the communication overheads scale approximately linearly with respect to $d$ for all 
the three algorithms. More precisely, under any set difference cardinality $d$, the amount of communication per 
distinct element is roughly a constant. 
D.Digest is the worst. It requires around 6$\times$32 bits per distinct element, which is  
6 times of the minimum, 32 bits per distinct element. 
% Our PBS requires less than half of those of D.Digest. 
PBS is much better, which %only  
% requiring no more than 
% More precisely, PBS 
needs (2.15 to 2.67)$\times$32 bits per distinct element ({\it i.e.,} 2.15 to 2.67 times of the minimum). 
PinSketch is the best, which only requires around 1.38$\times$32 bits per distinct element ({\it i.e.,} 1.38 times of the minimum). 
However, as we will show very soon, its decoding time is significantly (up to 3 orders of magnitude) higher than those of the others, when 
$d$ is large. 
% \ These values for $($
% our scheme with 2 and 3 rounds are 9.97 to 14.15 and 8.60 to 10.67 respectively. 

% As mentioned earlier in~\autoref{sec:parameter_settings}, we separated the comparisons against 
\autoref{fig:co-9958} presents the communication overhead of PBS against that of Graphene, 
with a target success rate of 239/240. 
%  and our scheme (with 
% 2 and 3 rounds). 
% For our scheme, we include those for our ToW estimator. 
The results show that PBS has lower communication overhead than Graphene 
under all different set difference cardinalities except for those close to \num{10000} 
where PBS has slightly higher communication overheads than Graphene. 
PBS requires roughly (2.21 to 2.75)$\times$32 bits per distinct element (higher than those in~\autoref{fig:co-99} 
as the target success rate here is higher). 
Unlike in other algorithms, in Graphene, the average amount of 
communication per distinct element varies significantly as $d$ changes and %as shown in~\autoref{fig:co-9958}, 
it roughly decreases as $d$ increases.  
For example, Graphene requires approximately 7.33$\times$32 bits per distinct element when $d$=10, 
whereas it only requires 1.84$\times$32 bits when $d$=\num{10000}. 
% This phenomenon results from the parameter setting procedure of Graphene: 
% Given a target success rate, Graphene used the optimal sizes for the BFs and IBFs to 
% minimize the total communication overheads. 
% % not sure whether we have to explain
% Recall that Graphene is a hybrid algorithm that combines BFs and IBFs, its communication overheads 
% are mainly consisted of two components: the communication for the BFs and the communication for the IBFs. 

% % maybe adding a figure
% \autoref{} shows the fraction of the communication overheads resulted from the IBFs. 
% As shown in \autoref{}, when $d\!\le\!$\num{1000}, the communication of the IBFs covers more than 99\% of that of Graphene. 
% In these scenarios ({\it i.e.,} $d\!\le\!$\num{1000}), the average 
% communication per distinct element roughly decreases, because unlike in D.Digest, where a good enough parameter setting 
% was used, in Graphene, a procedure that can determine the optimal size (for a given target success rate) for an IBF was used. 

% The results also show that the average 
% communication per element in the set difference gets smaller for Graphene. 
% For $t\!<\!$\num{1000}, it is mainly because the IBF requires less cells per 
% element as $t$ gets larger to ensure the same success rate, as shown in Figure 7 
% of~\cite{Eppstein_WhatsDifference?Efficient_2011}. When $t\ge 1000$, the average number of cells per 
% element is almost independent of $t$ (remains the same as $t$ increases). The average communication 
% per element (in the set difference) continues to decrease 
% because when $t$ is large enough the BF in Graphene can help 
% reduce the number of cells required by the IBFs thus resulting in a lower communication overhead per 
% element in the set difference.  

As explained in~\autoref{subsubsec:discussion}, the scenario in our evaluation ({\it i.e.,} $B\subset A$) 
is the best for Graphene. In more general scenarios ({\it i.e.,} $B$ is not a subset of $A$), the communication overhead 
of Graphene would be higher than that shown in~\autoref{fig:co-9958}. 

\begin{figure}
\centering
\begin{minipage}[t]{0.25\textwidth}
\centering
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/encoding_time}
\caption{Encoding time.}
\label{fig:et-99}
\end{minipage}%
\begin{minipage}[t]{0.25\textwidth}
\centering
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/decoding_time}
\caption{Decoding time.}
\label{fig:dt-99}
\end{minipage}%
\end{figure}

% In real applications, the 
% % key size (length of each element in the universe) 
% hash signature width $w$ (width of each binary string in the universe $\mathcal{U}$) 
% might be much higher than 
% 32 bits. For example, the transaction ID in Bitcoin applications could 
% have 2048 bits~\cite{naumenko2019bandwidth}. 



We then present the experiment results on computational overhead, more precisely, encoding time and decoding time. Note that the results of 
PBS against Graphene are not presented for fairness consideration, because Graphene is implemented in Python, which 
is much slower than PBS that is implemented in C++.   

\smallskip
\noindent
{\bf Encoding time}.
\autoref{fig:et-99} shows the encoding time of PBS against those of D.Digest and PinSketch, 
with a target success rate of 0.99. 
As shown in~\autoref{fig:et-99}, PBS 
has the lowest encoding time under all different values of $d$ get larger. 
% Results of PinSketch and D.Digest match well with our theoretical analysis in~\autoref{sec:closely-related}: 
% The encoding time of PinSketch increases linearly as $d$, and that of D.Digest is 
% $O(|A|\!+\!|B|)$ (3 or 4 hash operations per element), independent of $d$.  
% We note that the encoding time of D.Digest is slightly higher when $d$ is small.  
% This is because, as described in~\autoref{subsubsec:configuration}, 
% D.Digest used 3 hash functions when $d\!>\!200$, and $4$ hash functions otherwise. 
\autoref{fig:et-99} also clearly shows that the encoding time of PBS increases slightly as $d$ increases. 
This is because the encoding time mainly consists of two parts in PBS: 
hash-partition and parity bitmap encoding (\autoref{sec:hash_partition}) and 
BCH encoding (\autoref{step:BCH_encode} of~\autoref{alg:single_round_pbs}). 
The former is independent of $d$, which has a computational complexity 
of $O(|A|\!+\!|B|)$ (1 hash operation per element). The latter has a computational complexity 
linear in $d$, because the number of groups is on average $1.38d/5$ 
% ,  
% which increases linearly as $d$ 
and BCH encoding time per group is roughly a constant (as $n$ and $t$ are the same for all groups). %the same.  

% The results also show that the encoding time of our scheme increases as $t$ increases. 
% This is because the encoding time mainly consists of two parts in our scheme: the partition process and 
% the BCH encoding. The former is independent of $t$, which has a computational complexity 
% of $O(|A|+|B|)$ (1 hash operation per element). The latter has a computational complexity 
% proportional to $t$ as the number of bins (subset pairs) increases almost linearly as $t$ and 
% the encoding of each subset pairs has a constant computational complexity.  

\smallskip
\noindent
{\bf Decoding time}.
\autoref{fig:dt-99} shows decoding time of PBS against those of D.Digest and PinSketch, 
with a target success rate of 0.99. 
% Results show that 
% the decoding times of D.Digest and PBS scale roughly linearly with respect to $d$, whereas 
% that of PinSketch scales roughly quadratically with $d$. 
As shown in~\autoref{fig:dt-99}, the decoding time of 
PinSketch is much higher than those of D.Digest and PBS when $d$ is large (say $\ge$ \num{1000}). 
For example, when $t\!=\!$\num{10000}, the decoding time of PinSketch is roughly three orders of magnitude 
higher than those of D.Digest and PBS. 
% As mentioned earlier in~\autoref{sec:scheme}, the substantially longer decoding time of PinSketch is because 
% the decoding computational complexity of BCH codes is quadratic in $t$, thus also quadratic in $d$ 
% (here we use the fact $\mathbf{E}[t]\!=\!$1.38d in our 
% evaluation). Though our PBS also uses BCH codes, as explained in~\autoref{sec:scheme}, PBS resolved this issue 
% by using BCH codes in a much more efficient manner so that its decoding computational complexity is linear in 
% $d$. 
\autoref{fig:dt-99} also shows clearly that D.Digest is the best, whose decoding time is 2 to 3 times shorter than that of PBS. 
However, as discussed earlier, its encoding time is much longer (up to one order of magnitude longer) 
than that of PBS, and encoding time (of 
PBS and D.Digest) is usually much longer than the corresponding decoding time. 
Therefore, PBS has the lowest overall computational overhead. 


\subsection{Piecewise Decodability of PBS}\label{subsec:piecewise}

\begin{figure}
\centering 
\includegraphics[width=0.45\textwidth]{figures/reconciliation/success-rate-99/pbs_3_per_round_all_v3}
\caption{Fraction of communication overhead incurred in each round.}\label{fig:per-round-con}
\end{figure}

As mentioned earlier in~\autoref{subsubsec:configuration}, failure is inevasible (though usually with a tiny probability) 
in most set reconciliation algorithms.  
When failure happens, in most of existing set reconciliation algorithms, the process has to start from square one, 
thus the communication overhead doubles. 
% Recall from~\autoref{sec:intro}, 
However, failure only incurs very tiny additional communication 
overhead in PBS because of its piecewise decodability. 
In this section, we demonstrate, through experiments, the piecewise decodability of PBS. 

We use the default parameter setting described in~\autoref{subsubsec:configuration} except that now we 
% allow PBS to run as many 
% rounds as possible 
measure the communication overhead incurred in each round 
until PBS believes all distinct elements are successfully reconciled, {\it i.e.,} \autoref{proto:multirounds} 
stops because \code{complete} becomes \code{true}.   

\autoref{fig:per-round-con} shows per-round communication overhead, more precisely, 
the percentage of communication overhead incurred in each round. To clearly present the results, 
we use a separate axis for each round in~\autoref{fig:per-round-con}. 
%
As shown in~\autoref{fig:per-round-con}, 
PBS runs at most 4 rounds. 
% From \autoref{fig:per-round-con}, it is hard to read the percentages in round 3 and 4 clearly, because 
% the communication overhead incurred in these two rounds are so tiny ({\bf $<0.1$ percentage ??}). 
We note that 
% no error occurred in any experiment instance, that is, 
all distinct elements in all 
experiment instances were eventually successfully reconciled. 

% \autoref{fig:per-round-con} clearly shows that the vast majority ($>$93\%) of the communication overhead 
% is incurred in round 1 and the per-round communication overhead drops exponentially as the number of rounds increases. 
\autoref{fig:per-round-con} clearly shows that more than 93\%, 1\% to 7\%, less than 0.16\%, and less than 0.013\% of the communication overhead 
is incurred in round 1, 2, 3, and 4, respectively. 
% and the per-round communication overhead drops exponentially as the number of rounds increases. 
This confirms the piecewise decodability of PBS, which can be explained as follows. 
+++ {\bf The following explanation can be removed if we already explained this in scheme section.} 
After round 1, some distinct elements in a few groups fail to be reconciled because of 
the exceptions described in~\autoref{subsec:exception_hash_partition} and BCH decoding failure described in~\autoref{sec:BCH_exception}. 
% Though when the latter happens, one group is decomposed into $3$. The number of groups resulting 
% from such failure is tiny, as the probability that such failure occurs is extremely low (roughly at the order of $10^{-5}$), 
These events happen with tiny probability, 
thus only a tiny fraction of distinct elements remain un-reconciled and PBS only needs to reconcile them in round 2. 
Therefore, the communication overhead in round 2 is much lower than that incurred in round 1. If PBS does not reconcile 
all the remaining distinct elements in round 2, round 3 then comes. Similarly,  the communication overhead in round 3 is much 
lower than that incurred in round 2. And so on so forth until all distinct elements are successfully reconciled. 

% +++ {\bf The following can be added if we have space.}
% To reassure readers that the exponential drop of the per-round communication overhead as 
% the number of rounds increases is really because of the piecewise decodability instead of most of the experiment 
% instances being successfully reconciled (though it is also a reason when $d$ is small), we further measured 
% After the first round, most of the distinct elements were determined and the rest rounds only need to handle the remaining 
% tiny percentage 

% In this section, we demonstrate the piecewise decodability of PBS, an important feature for set reconciliation algorithms, 
% which all existing set reconciliation does not have. 

\begin{figure*}
\centering
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/communication_costs_verying_key_sizes_d100}
\caption{d=100}
\label{fig:-d100}
\end{subfigure}%
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/communication_costs_verying_key_sizes_d1000}
\caption{d=\num{1000}}
\label{-d1000}
\end{subfigure}%
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/communication_costs_verying_key_sizes_d10000}
\caption{d=\num{10000}}
\label{fig:-d10000}
\end{subfigure}
\caption{Communication overheads of PBS against those of PinSketch, D.Digest under various signature widths.}% with at least 99\% success rate.}
\label{fig:cc-comp-vk}
\end{figure*}


\subsection{Varying Signature Width}\label{subsubsec:varying-sig-width}

In real applications, the 
% key size (length of each element in the universe) 
hash signature width $\log|\mathcal{U}|$ (width of each binary string in the universe $\mathcal{U}$) 
might be much higher than 
32 bits. For example, the transaction ID (``hash signature'') in Bitcoin applications could 
be as large as 2048 bits~\cite{naumenko2019bandwidth}. 
In this section, we investigate how the performance of each algorithm scales with respect to $\log|\mathcal{U}|$. 
We consider signature width $\log|\mathcal{U}|$ varying from 32 to 2048 bits. 
As the implementations of all the evaluated algorithms do not support signature width higher than $64$ bits (some of them only support 
32 bits), all results for $\log|\mathcal{U}|\!>\!$32 in this section were obtained by using simulations with a $32$-bit universe. 
Thus, we only present the results for communication overhead in this section. However, we note that PBS 
also has some superiority in computational overhead, more precisely, decoding time, over all the rest algorithms, 
because the BCH decoding computational complexity in PBS is independent of 
$\log|\mathcal{U}|$, whereas it grows linearly in $\log|\mathcal{U}|$ or even faster in all other algorithms.  
Like in~\autoref{subsec:recon-perf}, we separate the comparisons 
against D.Digest and PinSketch (with a target success rate 0.99) and those against Graphene (with a target success rate of 239/240).  
The results are shown in~\autoref{fig:cc-comp-vk} and~\autoref{fig:cc-comp-vk-vs-graphene} respectively. 

% Same as before, for the results in~\autoref{fig:cc-comp-vk}, we make each algorithm ensure a success rate of 
% 0.99 and exclude the communication required by the estimator for all algorithms. For those in~\autoref{fig:cc-comp-vk-vs-graphene}, we make our scheme and Graphene ensure a success rate of 239/240 and include 
% the communication required by the estimator for our scheme (note that Graphene does not require an estimator). 

We can see from \autoref{fig:cc-comp-vk} that the communication overhead increases for all algorithms when 
the signature width increases, under all 3 different set difference cardinalities, which is not surprising. 
However, \autoref{fig:cc-comp-vk} also clearly shows that PBS scales much better than D.Digest and PinSketch, as 
we will elaborate next. 

We make the following two observations from \autoref{fig:cc-comp-vk}. First, the communication overheads of D.Digest and PinSketch grow linearly as the signature width $\log|\mathcal{U}|$ increases, remaining $6$ and $1.38$ times of the minimum respectively, which matches well 
our rough estimates in~\autoref{subsubsec:configuration}.  
% Second, the gap between PBS and the minimum shrinks rapidly as the signature width becomes larger.  
Second, PBS overtakes PinSketch rapidly and becomes the one with the lowest communication overhead as the signature width $\log|\mathcal{U}|$ becomes larger. 
+++ {\bf The following explanation can be removed or at least simplified if we already explained it in the scheme section.}  
The reason is as follows. 
As described earlier in~\autoref{sec:communication_overhead_single_PBS}, the communication overhead of PBS is 
consisted of three parts: BCH codewords,  
XOR sums (together with subset pair indices), and checksums. 
Only the communication overhead resulting from  
XOR sums (excluding indices) in the the second part grows as $\log|\mathcal{U}|$ gets larger, which is approximately $d\log|\mathcal{U}|$ bits. 
The rest is independent of $\log|\mathcal{U}|$, which takes slightly more than 50\% in the total communication overhead when $\log|\mathcal{U}|\!=\!32$. 
Hence, as $\log|\mathcal{U}|$ increases, this part takes less and less fraction in the total communication overhead, and 
the communication overhead resulting from XOR sums, approximately $d\log|\mathcal{U}|$ bits, gradually dominates the communication overhead of PBS.  
% The former is independent of $w$. The latter 
% is roughly $wd$ bits. 
Therefore, when the signature width $\log|\mathcal{U}|$ increases, the communication overhead of PBS becomes increasingly closer to 
% $1\!\times\!$ 
% $wd$ bits (the ratio of the communication overhead for PBS to $wd$ bits gets closer to $1$),
the minimum ($d\log|\mathcal{U}|$ bits), 
outperforming PinSketch which requires $1.38d\log|\mathcal{U}|$ bits.   
% Our explanation for the first observation is as follows. D.Digest requires to allocate $w$ bits to each field in every IBF cell, 
% hence its communication overhead becomes approximately $6w$ bits per dist
% \autoref{fig:cc-comp-vk} shows that the communication overheads of D.Digest and PinSketch double 
% as the signature width $w$ doubles, requiring $6$ and $1.38$ times of the minimum, $w$ bits per distinct 
% element. \autoref{fig:cc-comp-vk} also shows that communication overhead of PBS increases much slower as $w$ increases. 


% As shown in~\autoref{fig:cc-comp-vk} and~\autoref{fig:cc-comp-vk-vs-graphene}, PBS has the best 
% scaling behavior (with respect to $w$) among all these algorithms. 
% For D.Digest and PinSketch, the communication overheads double 
% as the signature width $w$ doubles, whereas the communication overhead increases much slower in PBS.  
% as the key size increases. 
We can see from \autoref{fig:cc-comp-vk-vs-graphene} that the communication overhead of Graphene also grows 
linearly as the signature width $\log|\mathcal{U}|$ increases when $d\!=\!$\num{100} (\autoref{fig:vs-graphene-d100}) and $d\!=\!$\num{1000} (\autoref{fig:vs-graphene-d1000}). 
However, it grows much slower when $d\!=\!$\num{10000} (\autoref{fig:vs-graphene-d10000}). 
Our explanation for these observations is as follows. As described in~\autoref{sec:closely-related}, Graphene is 
a hybrid set reconciliation algorithm that combines BFs and IBFs. %BF- and IBF-based solutions. 
Its communication overhead 
mainly results from two parts: BFs and IBFs. Recall from~\autoref{sec:closely-related},  when $d\!=\!|A\Delta B|\!\ll\!|A\cup B|$ (the scenarios shown in 
\autoref{fig:vs-graphene-d100} and \autoref{fig:vs-graphene-d1000}), Graphene can not afford to create BFs with low false positive 
rate, thus the space for the IBFs dominates the communication overhead. This interpretation was later confirmed by detailed instruments: The false positive rates of the BFs are close to $1$ and the IBFs take more than $99\%$ of the communication 
overhead. The space of IBFs grows linearly as $\log|\mathcal{U}|$ gets larger. Therefore, the communication overhead of Graphene also grows 
linearly as the signature width $\log|\mathcal{U}|$ increases when $d\!=\!$\num{100} (\autoref{fig:vs-graphene-d100}) and $d\!=\!$\num{1000} (\autoref{fig:vs-graphene-d1000}). 

However, as $d$ gets larger, Graphene now can afford to create BFs with relatively low false positive rates and now the space 
of IBFs takes less fraction. Through detailed instruments, we found the fraction of communication overhead resulting from 
IBFs becomes roughly $39\%$ when $d\!=\!$\num{10000} and $\log|\mathcal{U}|\!=\!32$. The space of BFs 
is independent of $\log|\mathcal{U}|$. Therefore, just like that of PBS, the communication overhead of Graphene grows much slower when $d\!=\!$\num{10000} (\autoref{fig:vs-graphene-d10000}). 
% For Graphene, when $t\!=\!$\num{100} and $t\!=\!$\num{1000}, its scaling behavior is almost the same as D.Digest, since as explained in~\autoref{subsec:recon-bench}, Graphene almost reduces to an IBF-only solution when $t\ll|A\cup B|$. When $t=$\num{10000}, the scaling behavior is very close to that of our scheme, as now the communication overheads resulting from IBFs in Graphene is around 40\% and those for the BFs do not increase as the key size. 



\begin{figure*}[!htbp]
\centering
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-239-240/vs_graphene_verying_key_sizes_d100}
\caption{d=100}
\label{fig:vs-graphene-d100}
\end{subfigure}%
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-239-240/vs_graphene_verying_key_sizes_d1000}
\caption{d=\num{1000}}
\label{fig:vs-graphene-d1000}
\end{subfigure}%
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-239-240/vs_graphene_verying_key_sizes_d10000}
\caption{d=\num{10000}}
\label{fig:vs-graphene-d10000}
\end{subfigure}
\caption{Communication overheads of PBS against those of Graphene under various signature widths.}% with at least 99\% success rate.}
\label{fig:cc-comp-vk-vs-graphene}
\end{figure*}


\subsection{What If PinSketch Also Uses Partitions?}\label{subsec:mini-partition}
+++ {\bf The following paragraph can be removed!} 
The success we have with PBS leads readers to wonder what if we apply the same  
idea to PinSketch. Like in PBS, we can partition $A$ into $\{A_i\}_{i=1}^g$ and $B$ into $\{B_i\}_{i=1}^g$ 
using the hash partition described in~\autoref{sec:hash_partition} so that each subset-pair-differences $\{A_i\Delta B_i\}_{i=1}^g$ 
contains $\delta =d/g$ distinct elements on average. Then, we use PinSketch with a high enough error-correction capability $t$ (say $2.5\delta$) 
to reconcile each subset pair 
independently. We refer to this new scheme as PinSketch With Partition, or PinSketch/WP for short.  
Clearly, by letting $\delta$ be a small constant (say $5$), PinSketch/WP also has a decoding computational 
complexity of $O(d)$ and communication complexity of $O(d)$. 

Now We compare the performance of PBS against that of PinSketch/WP. %, with a target success probability of $p_0$=0.99 within $r$=3 rounds. 
As performing rigorous theoretical analysis -- like we did for PBS in~\autoref{sec:tail_bound} -- for PinSketch/WP 
is out scope of this paper. We simply used the same parameter setting as which we used for PBS ({\it i.e.,} the default parameter setting), 
for PinSketch/WP. That is, PinSketch/WP uses the same $\delta$ and $t$ as PBS (note that 
there is no ``n'' in PinSketch/WP), with a target success probability of $p_0$=0.99 within $r$=3 rounds, in each experiment instance.  
% For example, like in our scheme, we partition all elements into several subsets 
% so that each subset contains a few elements (say $5$) on average from the set difference. Then, for 
% each subset we create BCH codes with a capacity large enough so that we can ensure a desired success rate. 


% We compare the performances of our scheme with those of Minisketch/WP with a desired success rate of 
% 0.99. For Minisketch/WP, we set the average number of elements from the set difference to $5$ (same 
% as our scheme) and use the same BCH decoding capacity for all subsets. We tune this capacity to the best: 
% the one with the minimum communication overhead yet ensures a success rate of at least 0.99.    

\autoref{fig:cc-comp-vs-minisketchwp} presents the communication overheads under different signature widths varying 
from 32 to \num{2048} bits for three different set difference cardinalities \numlist{100;1000;10000}. Like in~\autoref{subsubsec:varying-sig-width}, 
the results for signature widths higher than 32 bits were obtained through simulations with a $32$-bit universe.  
The results show that PinSketch/WP has %similar or 
slightly higher communication overhead than PBS when the signature width is 32 bits. 
The superiority of PBS  
gets outstanding as the signature width $\log|\mathcal{U}|$ gets larger: The gap between PinSketch/WP and PBS increases rapidly as 
the signature width $\log|\mathcal{U}|$ gets larger. Besides, PBS is also computationally 
more efficient than PinSketch/WP because of the shorter width of the Galois field as explained in~\autoref{}, 
which was further confirmed by experiments on encoding and decoding time of PBS against those of 
PinSketch/WP. These results are omitted here in the interest of space. 
% Therefore, we conclude that our scheme overall remains the best practical solution for the 
% set reconciliation problem.

% \begin{figure*}[!htbp]
% \centering
% \begin{subfigure}[t]{0.32\textwidth}
% \includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/co_vs_erlaywp_match}
% \label{fig:vs-minisketchwp-co}
% \end{subfigure}%
% \begin{subfigure}[t]{0.32\textwidth}
% \includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/decoding_time_vs_erlaywp_match}
% \caption{t=\num{1000}.}
% \label{fig:vs-minisketchwp-dt}
% \end{subfigure}%
% \begin{subfigure}[t]{0.32\textwidth}
% \includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/vs_minisketchwp_match_varying_key_sizes_d10000}
% \caption{t=\num{10000}.}
% \label{fig:vs-minisketchwp-et}
% \end{subfigure}
% \caption{Comparisons of PBS against PinSketch/WP, with a target success rate of 0.99.}% with at least 99\% success rate.}
% \label{fig:cc-comp-vs-minisketchwp}
% \end{figure*}

% % need to change
\begin{figure*}[!htbp]
\centering
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/vs_minisketchwp_match_varying_key_sizes_d100}
\caption{d=\num{100}}
\label{fig:vs-minisketchwp-d100}
\end{subfigure}%
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/vs_minisketchwp_match_varying_key_sizes_d1000}
\caption{d=\num{1000}}
\label{fig:vs-minisketchwp-d1000}
\end{subfigure}%
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/vs_minisketchwp_match_varying_key_sizes_d10000}
\caption{d=\num{10000}}
\label{fig:vs-minisketchwp-d10000}
\end{subfigure}
\caption{Communication overheads of PBS against those of PinSketch/WP.}% with at least 99\% success rate.}
\label{fig:cc-comp-vs-minisketchwp}
\end{figure*}


\subsection{Can We Use Less Rounds in PBS}\label{subsec:less-rounds}

In this section, we address one question: Is it possible to use less rounds in PBS without using significantly 
more resources ?


Like in~\autoref{subsubsec:configuration}, we configured PBS to achieve a target success rate of $p_0$=0.99 within $r$=1, 2, or  
3 rounds respectively and compared  
communication overhead and computational overhead. %({\it i.e.,} encoding time and decoding time). 
The experiment results are presented in \autoref{fig:2vs3}, which also include  
their empirical success rates (\autoref{subfig:success-rate}). As resources (both communication overhead and 
computational overhead) required for $r\!=\!1$ are 
significantly higher, we only presented the results for $r\!=2\!$ and $3$. 

We can see from~\autoref{fig:2vs3}, PBS with $r\!=\!2$ has both higher communication overhead and 
higher computational overhead than those of PBS with $r\!=\!3$, but only slightly. This is 
reasonable, as it is obvious that achieving the same success rate within 2 rounds is harder than within 3 rounds. 
Therefore, we consider PBS with $r\!=\!2$ is ``reasonably priced,'' {\it i.e.,} paying reasonably higher 
price (resources) for less rounds. In other words, those slightly additional resources by reducing from 
3 rounds to 2 rounds are only ``marginal cost''.

\def\WD{0.25}
\begin{figure*}[!htbp]
\centering
\begin{subfigure}[t]{\WD\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/success_rate_2vs3}
\caption{Empirical success rate}\label{subfig:success-rate}
\end{subfigure}%
\begin{subfigure}[t]{\WD\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/communication_costs_2vs3}
\caption{Communication overhead}\label{subfig:co}
\end{subfigure}%
\begin{subfigure}[t]{\WD\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/encoding_time_2vs3}
\caption{Encoding time}\label{subfig:et}
\end{subfigure}%
\begin{subfigure}[t]{\WD\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/decoding_time_2vs3}
\caption{Decoding time}\label{subfig:dt}
\end{subfigure}
\caption{PBS: 2 rounds vs. 3 rounds.}\label{fig:2vs3}
\end{figure*}
\begin{comment}

\subsection{Evaluation of Our Reconciliation Scheme}\label{subsec:recon-perf}

% % 
In this section, we evaluate the performance of our algorithm for set reconciliation, and compare 
it with Difference Digest (D.Digest)~\cite{Eppstein_WhatsDifference?Efficient_2011}, 
Graphene~\cite{Ozisik2019}, and Minisketch~\cite{naumenko2019bandwidth}, which we have 
described in detail in~\autoref{subsec:recon-bench}. 

Like in~\autoref{subsec:est-perf}, 
in the comparisons, we fix the size of the union $A\cup B$ to 100K and set the value of $t$ varying 
from 10 to 10K. For each value of $t$, we created \num{1000} different pairs of $A$ and $B$. 
All the experiments in this section were performed on a workstation with an Intel Core i7-9800X processor 
running Ubuntu 18.0.4.  


For D.Digest, as the authors of~\cite{Eppstein_WhatsDifference?Efficient_2011} did not 
release their source codes, we used the optimized open-source implementation of IBFs in C++ released by 
the authors of~\cite{Ozisik2019}. For Minisketch, we used its C++ implementation~\cite{Wuille_Minisketchoptimizedlibrary_2019}  
released by the authors of~\cite{naumenko2019bandwidth}. 
% Note that, Minisketch is just an optimized implementation of the PinSketch~\cite{Dodis_PinSketch_2008} 
% algorithm. 
For Graphene, we used the source codes provided by the authors of~\cite{Ozisik2019}. 
Note that, the implementation of Graphene is in Python. 
We implemented our scheme in C++: 
we used \texttt{xxHash}~\cite{Collet_xxHashExtremelyfast_} for the partition process 
and Minisketch for BCH encoding and decoding. 


\subsubsection{Our Scheme vs. Prior Work}\label{subsec:vs-prior}

% \begin{figure*}
% \centering
% \begin{subfigure}[t]{0.32\textwidth}
% \includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/communication_costs}
% \caption{Communication overheads.} %(excluding those of the ToW estimator).}
% \label{fig:communication-costs}
% \end{subfigure}%
% \begin{subfigure}[t]{0.32\textwidth}
% \includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/decoding_time}
% \caption{Decoding time.}
% \label{fig:decoding-time}
% \end{subfigure}%
% \begin{subfigure}[t]{0.32\textwidth}
% \includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/success_rate}
% \caption{Success rate.}
% \label{fig:success-rate}
% \end{subfigure}
% \caption{Comparisons our schemes against Minisketch and D.Digest.}% with at least 99\% success rate.}
% \label{fig:comp-old}
% \end{figure*}

\begin{figure*}
\centering
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/communication_costs}
\caption{Communication overheads.} %(excluding those of the ToW estimator).}
\label{fig:communication-costs}
\end{subfigure}%
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/encoding_time}
\caption{Encoding time.}
\label{fig:encoding-time}
\end{subfigure}%
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/decoding_time}
\caption{Decoding time.}
\label{fig:decoding-time}
\end{subfigure}%
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/success_rate}
\caption{Success rate.}
\label{fig:success-rate}
\end{subfigure}
\caption{Comparisons against Minisketch and D.Digest.}% with at least 99\% success rate.}
\label{fig:comp-old}
\end{figure*}

\noindent
{\bf Our Scheme vs. D.Digest and Minisketch}. We now compare our set reconciliation scheme 
against D.Digest and Minisketch. We used 128-sketch ToW estimator with 128 sketches for 
the estimation of $t$ for all these algorithms. 
For D.Digest, we used the parameter setting suggested by the authors of~\cite{Eppstein_WhatsDifference?Efficient_2011}: $2\hat{t}$ cells where $\hat{t}$ is the estimate of the set-difference size, 
and 3 hash functions for estimates less than 200; Otherwise we used 4 hash functions. 
Note that with this parameter setting, D.Digest can roughly ensure a success rate of 
at least 0.99, that is, for at least 99\% of the instances that we experimented, all elements should be successfully recovered. For Minisketch, we scaled up the estimates 
by 1.38 so that it can also ensure a success rate of 0.99. For our scheme, 
we set the average number of ``bad balls'' in each bin (elements in the set difference $A\Delta B$) 
to $5$ and whenever any bin fails to decode (which happens with tiny probability), 
we decomposed the bin in to three. We used the same BCH parameters 
(BCH code length and decoding capacity) for all bins, the 
values of which was obtained as follows. 
We first scaled up the estimates by 1.38. Then, based on the scaled estimates 
(assuming they are the true values), 
we computed the best parameters that can ensure a success rate of at least 
0.99 with 2 or 3 rounds (excluding the set-difference size estimation round) 
using our analytical results in~\autoref{sec:tail_bound}. Therefore, our scheme 
also roughly ensures a success rate of 0.99. 

% \autoref{fig:comp-old} presents the amount of data transfered (\autoref{fig:communication-costs}), the decoding time (\autoref{fig:decoding-time}), and the empirical 
% success rate (\autoref{fig:success-rate}) of Minisketch, D.Digest, and our scheme with 2 and 3 rounds. 

\autoref{fig:communication-costs} presents the amount of communication overheads of 
Minisketch, D.Digest, and our scheme (with 2 and 3 rounds). 
We note that the communication overhead of the estimator is excluded since 
it is constant (288 bytes) and the same for these algorithms. 
Results confirm that all these algorithms have the same 
asymptotic communication complexity, that is $O(t)$. However, the constant factors are different and do 
matter in practice. D.Digest is the worst, which requires 24 bytes per element in the set difference. 
Minisketch is the best, which only requires around 5.52 bytes per element. These values for 
our scheme with 2 and 3 rounds are 9.97 to 14.15 and 8.60 to 10.67 respectively. 

\autoref{fig:encoding-time} shows their encoding times. The results show that our scheme 
% (especially when using 3 rounds) 
has the lowest encoding time under all values of $t$. 
The results also show that the encoding time of our scheme increases as $t$ increases. 
This is because the encoding time mainly consists of two parts in our scheme: the partition process and 
the BCH encoding. The former is independent of $t$, which has a computational complexity 
of $O(|A|+|B|)$ (1 hash operation per element). The latter has a computational complexity 
proportional to $t$ as the number of bins (subset pairs) increases almost linearly as $t$ and 
the encoding of each subset pairs has a constant computational complexity.  

\autoref{fig:decoding-time} shows their decoding times. The results show that 
the decoding time of D.Digest and our scheme increase roughly linearly along with $t$, whereas 
that of Minisketch increases roughly quadratically with $t$. The decoding time of 
Minisketch is much higher than those of D.Digest and our scheme when $t$ is large (say $\ge$ \num{1000}). 
For example, when $t=$\num{10000}, the decoding time of Minisketch is more than two orders of magnitude 
larger than those of D.Digest and our scheme. 

\autoref{fig:success-rate} shows that all the algorithms achieve an empirical success rate for all 
the different values of $t$ except that the success rate of D.Digest are slightly lower than 0.99 when 
$t\!<\!100$. 


\noindent
{\bf Our Scheme vs. Graphene}. 
Then, we compare our scheme against Graphene. 
We separate the comparisons against Graphene from those against others for two reasons. 
First, Graphene does not require an estimator. 
Second, we only have the pre-computed parameters (provided by the authors of~\cite{Ozisik2019}) 
optimized for a success rate of 239/240 instead of 0.99. 
For fair comparisons, we set the parameters for our scheme to roughly ensure a success rate of 239/240, 
though, as shown in~\autoref{fig:success-rate}, our scheme already achieves this success rate empirically by 
using parameters calcluated for ensuring a success rate of 0.99. 
As shown~\autoref{fig:success-rate-vs-graphene}, both Graphene and our scheme have achieved success rates higher 
than 239/240 empirically. 

\autoref{fig:comm-cost-vs-graphene} presents the communication overheads of Graphene and our scheme (with 
2 and 3 rounds). For our scheme, we include those for our ToW estimator. 
The eesults show that our scheme has lower communication overheads than Graphene 
under almost values of $t$ except for those close to \num{10000} 
where our scheme has slightly higher communication overheads than Graphene. 
The results also show that the average 
communication per element in the set difference gets smaller for Graphene. 
For $t\!<\!$\num{1000}, it is mainly because the IBF requires less cells per 
element as $t$ gets larger to ensure the same success rate, as shown in Figure 7 
of~\cite{Eppstein_WhatsDifference?Efficient_2011}. When $t\ge 1000$, the average number of cells per 
element is almost independent of $t$ (remains the same as $t$ increases). The average communication 
per element (in the set difference) continues to decrease 
because when $t$ is large enough the BF in Graphene can help 
reduce the number of cells required by the IBFs thus resulting in a lower communication overhead per 
element in the set difference.  

We note that the scenarios (more precisely, the partition scenarios of elements in $A\Delta B$) are the best 
cases for Graphene. In more general cases ({\it i.e.,} $B$ is not a subset of $A$), the communication overheads 
of Graphene would be higher than those we reported in~\autoref{fig:comm-cost-vs-graphene}. 

We did not compare the encoding and decoding time of 
our scheme against Graphene because Graphene is implemented in Python, whereas our scheme is implemented in C++.  
% We note that the asymptotic encoding computational complexity is the same as that of our scheme and 
% its decoding computational complexity is 

% for two reasons. 
% First, asymptotically, 
% its decoding complexity is $O(|A|+|B|)$ which is much higher than $O(t)$, 
% the asymptotic decoding complexity. Second, 
% Graphene is implemented in Python, whereas our scheme is implemented in C++.  
% Though we found that the encoding and decoding time of our scheme is shorter than 
% those of Graphene, it is fair for Gra

% \begin{figure*}
% \centering
% \begin{minipage}{0.32\textwidth}
% \includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/communication_costs}
% \caption{Communication overheads.}
% \label{fig:communication-costs}
% \end{minipage}%
% \begin{minipage}{0.32\textwidth}
% \includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/decoding_time}
% \caption{Decoding time.}
% \label{fig:decoding-time}
% \end{minipage}%
% \begin{minipage}{0.32\textwidth}
% \includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/success_rate}
% \caption{Success rate.}
% \label{fig:success-rate}
% \end{minipage}
% \end{figure*}



\begin{figure}
\centering
\begin{subfigure}[t]{0.25\textwidth}
    \centering
    \includegraphics[width=1.0\textwidth]{figures/reconciliation/success-rate-239-240/communication_costs_vs_Graphene_v2}
    \caption{Communication overheads.}% (including those of the ToW estimator).}
    \label{fig:comm-cost-vs-graphene}
\end{subfigure}%
\begin{subfigure}[t]{0.25\textwidth}
    \centering
    \includegraphics[width=1.0\textwidth]{figures/reconciliation/success-rate-239-240/success_rate_vs_Graphene_v2}
    \caption{Success rate.} \label{fig:success-rate-vs-graphene} %%%%%
\end{subfigure}
\caption{Comparisons against Graphene.}\label{fig:vs-graphene}
\end{figure}

\end{comment}
\begin{comment}
\noindent
{\bf Is multiple rounds a issue?} Readers might think that our scheme might have longer latency 
than D.Digest and Minisketch, as they only require 1 round whereas our scheme requires more 
than 1. However, multiple rounds will not increase the latency of our scheme. 
To support it, we present the ratio of the number of elements successfully recovered in each round 
of our scheme in~\autoref{fig:recovered-ratio}. For our scheme running 2 rounds (or 3 rounds), more than 97\% (or 95\%) of elements 
in the set difference are successfully recovered in the first round. Therefore, the underlying synchronization 
process ({\it e.g.,} file synchronization) can start immediately after the first round of our scheme and do not need to wait until our reconciliation algorithm finishes. 
\end{comment}

% \noindent
% {\bf Per-Round Performance of Our Scheme.} 
% % Readers might think that our scheme might have longer latency 
% % than D.Digest and Minisketch, as they only require 1 round whereas our scheme requires more 
% % than 1. However, multiple rounds will not increase the latency of our scheme. 
% Now, we investigate the per-round performance of our scheme. 
% We present the ratio of the number of elements successfully recovered in each round 
% of our scheme in~\autoref{fig:recovered-ratio}, which shows that 
% our scheme running 2 rounds (or 3 rounds) can successfully recover more than 97\% (or 95\%) of elements 
% in the set difference in the first round. Therefore, the underlying synchronization 
% process ({\it e.g.,} file synchronization) can start immediately after 
% the first round of our scheme and do not have to wait until the set reconciliation finishes. 

\begin{comment}

\noindent
% {\bf Per-Round Performance of PBS.} 
{\bf Piecewise Decodability of PBS.}
% Readers might think that our scheme might have longer latency 
% than D.Digest and Minisketch, as they only require 1 round whereas our scheme requires more 
% than 1. However, multiple rounds will not increase the latency of our scheme. 
% Now, we investigate the per-round performance of PBS. 
Recall from~\autoref{sec:intro} that the only minor tradeoff of PBS is that the number of 
rounds (of message exchanges) needed by PBS is slightly larger than existing solutions. \autoref{fig:avg-num-rounds} 
presents the average number of rounds required by PBS with $r\!=$ 2 or 3 respectively. 
However, thanks to the piecewise decodability (that existing solutions do not have), the vast majority 
of all distinct elements are successfully reconciled in the first round. 
The ratio is presented in~\autoref{fig:recovered-ratio}, which shows that 
PBS with $r\!=$ 2 (or 3) can successfully reconcile more than 97\% (or 95\%) of all the distinct elements 
in the first round. Therefore, this tradeoff does not lead to longer response time because the reconciliation of objects identified
the successfully decodable ``codewords'' (hash signatures) can run in parallel with the transmissions and decodings of the rest. 

% the underlying synchronization 
% process ({\it e.g.,} file synchronization) can start immediately after 
% the first round of our scheme and do not have to wait until the set reconciliation finishes. 


We note that only those instances in which all distinct elements are successfully 
reconciled are considered in~\autoref{fig:avg-num-rounds} and~\autoref{fig:recovered-ratio}. 
Unlike in the existing solutions where nothing can be reconciled in the failed instances\footnote{We note that ``piecewise decodability'' can be also achieved in IBF-based solutions, as IBF-based solutions can also decode part of the distinct elements when decoding fails. However, on one hand, no existing solutions even mention this. On the other hand, the ``piecewise decodability'' of IBF-based solutions is much less efficient than that of PBS.}, the vast majority of 
all distinct elements are successfully reconciled in those failed instances in PBS because of its piecewise decodability. 
Furthermore, through experiments, 
we found that the rest distinct elements in those failed instances can be successfully reconciled with one more round of message exchanges  
({\it i.e.,} running one more round of PBS), and only negligible communication overhead incurred (thanks to piecewise decodability). In other words, failed instances lead to 
negligible penalties in PBS, whereas, in all the existing solutions, failed instances would result in hefty penalties, as they do not have 
piecewise decodability.


% \begin{figure}
% \centering
% \begin{subfigure}[t]{0.25\textwidth}
%     \centering
%     \includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/portion_recovered_max_round2_curve}
%     \caption{r=2.}\label{fig:recovered-ratio-r2}
% \end{subfigure}%
% \begin{subfigure}[t]{0.25\textwidth}
%     \centering
%     \includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/portion_recovered_max_round3_curve}
%     \caption{r=3.} \label{fig:recovered-ratio-r3} %%%%%
% \end{subfigure}
% \caption{Recovered ratio in each round.}\label{fig:recovered-ratio}
% \end{figure}

\begin{figure}
\centering
\begin{minipage}[t]{0.23\textwidth}
    \centering
    \includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/pbs_avg_rounds_wrl}
    \caption{Average number of rounds.} \label{fig:avg-num-rounds} %%%%%
\end{minipage}
\hspace{0.01\textwidth}%
\begin{minipage}[t]{0.23\textwidth}
    \centering
    \includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/pbs_first_round}
    \caption{Recovered ratio in the first round.}\label{fig:recovered-ratio}
\end{minipage}%
% \caption{Recovered ratio in each round.}\label{fig:recovered-ratio}
\end{figure}

% \begin{figure}
% \centering 
% \includegraphics[width=0.5\textwidth]{figures/reconciliation/success-rate-99/communication_costs_verying_key_sizes_d10000}
% \caption{Communication overheads (excluding those of the ToW estimator) of Minisketch, D.Digest, and our schemes under various key sizes.}\label{fig:varying-key-sizes}
% \end{figure}
\subsubsection{Varying Key Sizes}\label{sucsec:varying-key-sizes}

In real applications, the key size (length of each element in the universe) might be much higher than 
4 bytes. For example, the transaction ID in Bitcoin applications could 
have 256 bytes~\cite{naumenko2019bandwidth}. 
We investigate how the communication overhead of each algorithm changes as the key size $u$ increases. 
We consider key sizes varying from 4 bytes to 256 bytes. 
Same as before, we separate the comparisons 
against D.Digest and Minisketch and those against Graphene. 
The results are shown in~\autoref{fig:cc-comp-vk} and~\autoref{fig:cc-comp-vk-vs-graphene} respectively. 

Same as before, for the results in~\autoref{fig:cc-comp-vk}, we make each algorithm ensure a success rate of 
0.99 and exclude the communication required by the estimator for all algorithms. For those in~\autoref{fig:cc-comp-vk-vs-graphene}, we make our scheme and Graphene ensure a success rate of 239/240 and include 
the communication required by the estimator for our scheme (note that Graphene does not require an estimator). 

As shown in~\autoref{fig:cc-comp-vk} and~\autoref{fig:cc-comp-vk-vs-graphene}, our scheme has the best 
scaling behavior among all these algorithms. For D.Digest and Minisketch, the communication overheads double 
as the key size doubles, whereas the communication overhead increases much slower in our scheme 
as the key size increases. 
For Graphene, when $t\!=\!$\num{100} and $t\!=\!$\num{1000}, its scaling behavior is almost the same as D.Digest, since as explained in~\autoref{subsec:recon-bench}, Graphene almost reduces to an IBF-only solution when $t\ll|A\cup B|$. When $t=$\num{10000}, the scaling behavior is very close to that of our scheme, as now the communication overheads resulting from IBFs in Graphene is around 40\% and those for the BFs do not increase as the key size. 

\begin{figure*}[!htbp]
\centering
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/communication_costs_verying_key_sizes_d100}
\caption{t=100.}
\label{fig:-d100}
\end{subfigure}%
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/communication_costs_verying_key_sizes_d1000}
\caption{t=\num{1000}.}
\label{-d1000}
\end{subfigure}%
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/communication_costs_verying_key_sizes_d10000}
\caption{t=\num{10000}.}
\label{fig:-d10000}
\end{subfigure}
\caption{Communication overheads of Minisketch, D.Digest, and our schemes under various key sizes.}% with at least 99\% success rate.}
\label{fig:cc-comp-vk}
\end{figure*}

\begin{figure*}[!htbp]
\centering
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-239-240/vs_graphene_verying_key_sizes_d100}
\caption{t=100.}
\label{fig:vs-graphene-d100}
\end{subfigure}%
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-239-240/vs_graphene_verying_key_sizes_d1000}
\caption{t=\num{1000}.}
\label{fig:vs-graphene-d1000}
\end{subfigure}%
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-239-240/vs_graphene_verying_key_sizes_d10000}
\caption{t=\num{10000}.}
\label{fig:vs-graphene-d10000}
\end{subfigure}
\caption{Communication overheads of Graphene and our schemes under various key sizes.}% with at least 99\% success rate.}
\label{fig:cc-comp-vk-vs-graphene}
\end{figure*}

\subsubsection{What If Minisketch Also Uses Partitions?}\label{subsec:mini-partition}

The success we have with our scheme leads readers to wonder what if we apply the partition 
idea to Minisketch. For example, like in our scheme, we partition all elements into several subsets 
so that each subset contains a few elements (say $5$) on average from the set difference. Then, for 
each subset we create BCH codes with a capacity large enough so that we can ensure a desired success rate. 
We refer to this new scheme as Minisketch With Partition, or Minisketch/WP for short. 

We compare the performances of our scheme with those of Minisketch/WP with a desired success rate of 
0.99. For Minisketch/WP, we set the average number of elements from the set difference to $5$ (same 
as our scheme) and use the same BCH decoding capacity for all subsets. We tune this capacity to the best: 
the one with the minimum communication overhead yet ensures a success rate of at least 0.99.    

\autoref{fig:cc-comp-vs-minisketchwp} presents the communication overheads under different key sizes varying 
from 4 bytes to 256 bytes for three different set-difference sizes \numlist{100;1000;10000}. 
The sesults show that Minisketch/WP has similar or 
slightly lower communication overheads than our scheme only when the key size is 4 bytes. This advantage 
diminishes as the key size gets larger and our scheme is consistently better when the key size is no less than 
$16$ bytes. Hence, we conclude that our scheme overall remains the best practical solution for the 
set reconciliation problem.




% \begin{figure*}[!htbp]
% \centering
% \begin{subfigure}[t]{0.32\textwidth}
% \includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/vs_minisketchwp_verying_key_sizes_d100}
% \caption{t=\num{100}.}
% \label{fig:vs-minisketchwp-d100}
% \end{subfigure}%
% \begin{subfigure}[t]{0.32\textwidth}
% \includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/vs_minisketchwp_verying_key_sizes_d1000}
% \caption{t=\num{1000}.}
% \label{fig:vs-minisketchwp-d1000}
% \end{subfigure}%
% \begin{subfigure}[t]{0.32\textwidth}
% \includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/vs_minisketchwp_verying_key_sizes_d10000}
% \caption{t=\num{10000}.}
% \label{fig:vs-minisketchwp-d10000}
% \end{subfigure}
% \caption{Communication overheads of our schemes against those of Minisketch/WP.}% with at least 99\% success rate.}
% \label{fig:cc-comp-vs-minisketchwp}
% \end{figure*}

\begin{figure*}[!htbp]
\centering
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/vs_minisketchwp_match_varying_key_sizes_d100}
\caption{t=\num{100}.}
\label{fig:vs-minisketchwp-d100}
\end{subfigure}%
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/vs_minisketchwp_match_varying_key_sizes_d1000}
\caption{t=\num{1000}.}
\label{fig:vs-minisketchwp-d1000}
\end{subfigure}%
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[width=0.99\textwidth]{figures/reconciliation/success-rate-99/vs_minisketchwp_match_varying_key_sizes_d10000}
\caption{t=\num{10000}.}
\label{fig:vs-minisketchwp-d10000}
\end{subfigure}
\caption{Communication overheads of our schemes against those of Minisketch/WP.}% with at least 99\% success rate.}
\label{fig:cc-comp-vs-minisketchwp}
\end{figure*}

\end{comment}

==> section/introduction_copy.tex <==
\section{Introduction}\label{sec:intro}



Set reconciliation is a fundamental algorithmic problem that has received considerable research attention over the past two 
decades~\cite{Minsky2003,Guo_SetReconciliationvia_2013,Luo_SetReconciliationCuckoo_2019,Eppstein_WhatsDifference?Efficient_2011,Dodis_PinSketch_2008}. %% filled by long (but not quite sure)
In the simplest form of this problem, two large sets $A$ and $B$ of objects (bitcoins, files, records, etc.)
are stored respectively at two different network-connected hosts, which we name Alice and Bob respectively.
Alice and Bob communicate with each other to find out the 
%[define set difference] [define set reconciliation based on the former]
% % 
difference between $A$ and $B$, defined as $A\triangle B\triangleq (A\! \setminus\! B) \bigcup (B\! \setminus\! A)$,
% and often denoted as $A ??? B$,
so that both Alice and Bob obtain the set union $A\bigcup B$ $(=A\bigcup (A\triangle B)=B\bigcup (A\triangle B))$.  

Set reconciliation arises in many networking, system, and database applications.  
% % 
In cloud storage systems ({\it e.g.,} Dropbox, Microsoft OneDrive, Google Drive, and Apple iCloud), sets of files and directories 
need to be synchronized across the copies stored locally on different devices and in the cloud. 
In distributed database systems ({\it e.g.,} Spanner~\cite{Corbett_Spanner_2013} and Cassandra~\cite{Lakshman_Cassandra_2010}), 
an update at a single node has to get replicated across all other nodes eventually. 
In blockchains~\cite{Ozisik2019,Naumenko_ErlayEfficientTransaction_2019}, transactions need to be synchronized with some peers.

\subsection{Problem Formulation}\label{sec:intro_prob_formulation}

As is standard in the literature, in the rest of the paper we describe only unidirectional set reconciliation, in which Alice learns $A\triangle B$ and then infers $A\bigcup B$;
for bidirectional set reconciliation, Alice can simply infer $A\!\setminus\! B$ (from $A\triangle B$) and send it to Bob, from which Bob can infer $A\bigcup B$ as well. %$A\triangle B$.  
A simple but naive set reconciliation scheme is for Bob to send $B$, in its entirety, to Alice.  
%by exchanging the entire sets of data objects between the two hosts. 
This scheme, however, is grossly inefficient when
%$A$ and $B$ overlap significantly, or equivalently
%the set difference 
$A\triangle B$ is small (in cardinality) relative to their union $A \bigcup B$,
%overlap , or in other words when 
%the cardinality of $ ... $ is much smaller than that of    
% , {\it i.e.,} the set difference of the two sets is small relative to their union. 
which is indeed a usual situation in most applications. 
In this situation, it would be ideal if only the elements (objects) in $A\triangle B$ need to be transmitted.  In other words, 
Bob sends only $B\! \setminus\! A$ to Alice.

% and Bob sends only $B\! \setminus\! A$ to Alice.

% % 

In the set reconciliation problem, we usually assume each element is ``indexed" by a fixed-length (hash) signature, so the universe $\mathcal{U}$ contains all binary strings of this length.
%except the all-0 string.  
For example, when this length is $32$ bits, $\mathcal{U}$ contains
% $2^{32} - 1$ elements.  We denote this length as $\log |\mathcal{U}|$ (ignoring the slight numerical inaccuracy caused by the `-1') in the sequel.  
$2^{32}$ elements.  We denote this length as $\log |\mathcal{U}|$ in the sequel. 
% {\bf Throughout this paper, `$\log$' denotes the logarithm to base $2$.}
Let $d\triangleq |A\triangle B|$ denote the cardinality 
%(assuming for the moment that the size of each object is $1$) 
of the set difference.   It is not hard to prove (using information theory) that the theoretical minimum amount of communication between Alice and Bob for the {\it bidirectional} 
set reconciliation is the size of the set difference $d \log |\mathcal{U}|$~\cite{Minsky2003}.  Roughly speaking, this minimum applies also to the unidirectional case except in special situations 
such as $A \subset B$.  


\subsection{Existing Approaches}\label{sec:psea}



Although many techniques have been proposed for this problem, they all fall victim to a seemingly fundamental 
tradeoff between the communication overhead, of transmitting the codewords (in the general sense rather than in the narrow context of error-correction codes) needed for 
set reconciliation, and the computational complexity of decoding such codewords.  
The majority of such techniques are based on either invertible Bloom filters (IBF) or error-correction codes (ECC).  
% complexity
On one hand, IBF-based techniques incur a communication overhead that is several times  
(e.g., $6$ times in~\cite{Eppstein_WhatsDifference?Efficient_2011}) the theoretical minimum $d \log |\mathcal{U}|$,
but have a linear (i.e., $O(d)$) decoding computational complexity.  
%In other words, their overhead, in terms of the communication
%complexity, is a linear function of $d$ with a relatively large constant. 
On the other hand, the ECC-based techniques have a low communication overhead close to the theoretical minimum, but 
have a decoding computational complexity of $O(d^2)$ finite field operations,
%in general
%(can be reduced to $O(d^2)$) 
% by exploiting the algebraic structures of certain 
% codes~\cite{Dodis_SyndromeEncodingDecoding_2006,Wuille_Minisketchoptimizedlibrary_2019} such as BCH, 
which can be very high when $d$ is large (say $d \!=\! \num{10000}$).  


%and Bob only needs to send  to Bob and Bob only needs to be should only exchange the data objects 
%in the set difference. 

%, yet with communication overhead proportional to the size of the set difference to 
% %
%[One paragraph talking about myriad applications of set reconciliation.  Get good examples from the literature.]




\begin{comment}
Although many techniques have been proposed for this problem, they all fall victim to a seemingly fundamental 
tradeoff between the communication complexity, more precisely the cost of transmitting the codes needed for 
the set reconciliation, and the computational complexity of decoding such codes.  The majority of such techniques
are based on Bloom filters or counting Bloom filters.  These techniques generally need to transmit several times 
(e.g., 6.?? times in ...) of the size of the difference $d$.  In other words, their overhead, in terms of the communication
complexity, is a linear function of $d$.
\end{comment}



\begin{comment}
In this work, we propose a solution that strikes much better balance between the communication and computational complexities in 
the sense that if need to transmit exactly $d$ items plus 
some meta data that is of size roughly ? - ?, yet has a decoding computational complexity proportional to the size of 
the set difference. 
\end{comment}


\subsection{Our Solution}\label{sec:intro_oursolution}


In this work, we propose a solution, called Parity Bitmap Sketch (PBS), that mostly avoids this unfortunate tradeoff and gets the better of both worlds.  More specifically, PBS has both a low computational complexity of $O(d)$ just like IBF-based solutions and a low communication overhead of roughly twice the theoretical minimum.
%just like ECC-based solutions.   
PBS also has another advantage over all existing solutions in that it is ``piecewise reconciliable" in the following sense.  
In all existing solutions, decoding of the codewords to obtain $A\triangle B$ is an all-or-nothing process
in the sense that when the decoding failed 
(albeit usually with a small probability when the codewords are appropriately parameterized), 
little knowledge has been learned (so most of the communication, encoding, and decoding efforts are wasted) and the process starts from square one.  
%{\color{red}no knowledge has been learned (so all communication, encoding, and decoding efforts are wasted) and the process starts from square one.}  
In contrast, in PBS, the decoding of each codeword (also in the general sense) 
is independent of those of others, and the successful decoding of each codeword leads to a subset of 
{\it distinct elements} being reconciled;   here and in the sequel, we refer to each element in $A\triangle B$ a {\it distinct element}.  
This way,
%in our solution 
additional efforts are incurred only for the small percentage of codewords whose decodings failed earlier.  
 




%In any existing solution that runs for multiple rounds, all {\it distinct element}, defined as the elements in the set difference $A\triangle B$, will not be reconciled until in the last %round. In our solution, however, the majority of the distinct elements are expected to be reconciled in the first round, then in the next round, our solution only reconciles the %``remaining'' distinct elements that have not been reconciled yet, so on so force, until all distinct elements are reconciled.
%{\bf (Previous)} Our solution also has another advantage over all existing solutions in that it is ``piecewise reconciliable" in the following sense. 


%\footnote{We note that a recent technique called  Bisection proposed in~\cite{naumenko2019bandwidth} can make use of previously transmitted information. However, the total efforts when decoding fails are roughly doubled compared to the cases when decoding succeeds.}

%We will show that although
%some other tech

The only minor tradeoff of our solution is that the number of rounds of message exchanges needed for set reconciliation is slightly larger 
%(by a tiny fractional number on average) 
than some existing solutions.  However, in almost all practical application scenarios, this tradeoff is not expected to lead to longer response time 
for the following reason.  
Thanks to the piecewise reconciliability of PBS, the vast majority, if not all, of the distinct elements in $A\triangle B$ are successfully reconciled in the first round.  
The ``synchronization'' of the objects ``indexed" by these successfully reconciled distinct elements can then run in parallel with the reconciliation of the rest in $A\triangle B$.  
In other words, the piecewise reconciliability is expected to effectively mask the slightly larger number of communication rounds as far as the response time is concerned.

\begin{comment}
The only minor tradeoff of our solution is that the number of rounds of message exchanges needed for set reconciliation is slightly larger 
%(by a tiny fractional number on average) 
than some existing solutions. However, thanks to the piecewise reconciliability of our solution, in almost all practical application scenarios, this tradeoff is not expected to lead to longer response time because the reconciliation of objects identified by the successfully decodable codewords, which constitute the vast majority of all codewords, can run in parallel with the transmissions and decodings of the rest.  In other words, the piecewise decodability effective masks the slightly larger number of communication rounds as far as the response time is concerned.
\end{comment}







%The rough idea of (the non-crypto-part of) PinSketch is to view both A and B as gigantic (in the size of the universe for all these sets) bitmps (bit value is 1 if %the corresponding element is in the set and is 0 otherwise), and for Alice to send Bob only the BCH codewords needed to ?correct? B to A and vice versa.  


%has sublinear overhead in the sense it needs to transmit exactly $d$ items plus 
%some meta data that is of size $o(d)$ (i.e., sublinear of $d$).  Despite its extremely high communication efficiency, this solution %is also conceptually extremely simple, as we will describe shortly.  

\subsubsection{When \texorpdfstring{\larger\MakeLowercase{$d$}}{d} is small}\label{sec:smalld}

%Now we are ready to describe the rough idea of our solution. 

Here we sketch the main ideas of PBS.
%, and defer its details to \autoref{sec:scheme}. 
For the moment, we assume that the set difference cardinality $d$ is small (say no more than several elements), 
and the value of $d$ is precisely known.    
%We make no assumptions about the sizes of both sets A and B, which can be very large.
%These $d$ elements can be viewed as $d$ balls that will be ``thrown into $k >> d$ bins" as will be described next.
The first step of PBS is to partition $A$ and $B$ each into subsets in a consistent manner.
We partition the set $A$ into $n$ disjoint subsets $A_1$, $A_2$, ..., $A_n$ using a hash function $h$ as follows:
$A_1$ contains all elements in $A$ that are hashed to value $1$ (by $h$), $A_2$ contains all elements in $A$ that are hashed to value $2$, and so on.  
In the same manner, we partition $B$ into $B_1, B_2, \cdots, B_n$ using the same $h$. 
The use of the common hash function $h$ induces a hash-partitioning (also by $h$)
of the set-pair-difference $A\triangle B$ into $n$ disjoint subset-pair-differences $A_1 \triangle B_1$, $A_2 \triangle B_2$, ..., 
$A_n \triangle B_n$. We set this constant $n$ to be roughly an order of magnitude larger than $d^2$, so that  
%The objective of making $k > d^2$ is that, 
with high probability, the following {\it ideal situation} happens:
The $d$ distinct elements between $A$ and $B$ are hashed (by $h$) into $d$ distinct subset-pair-differences,
% The $d$ elements in $A\triangle B$ ({\bf we call them the {\it distinct elements} between $A$ and $B$ in the sequal}) are hashed (by $h$) into $d$ distinct subset-pair-differences,
% among $A_1 \triangle B_1$, $A_2 \triangle B_2$, ..., $A_n \triangle B_n$
so that each such subset-pair-difference contains exactly one distinct element.  This situation is ideal, because 
each such subset pair 
%each corresponding subset pair differs by 
% exactly
%at most  
%one element, and they 
can be easily reconciled as will be shown in \autoref{subsec:protocol0}. 
To guarantee that the ideal situation happens with high probability, the value of $n$ does not have to be very large when $d$ is small. 
%When $d$ is small, the appropriate $n$ value is quite moderate. 
For example, when $d = 5$ and $n$ is set to $255$, the probability for the ideal situation to occur is $0.96$.


%duplicated

The second step of PBS is to encode partitions $\{A_i\}_{i=1}^n$ and $\{B_i\}_{i=1}^n$ each into an $n$-bit-long {\it parity bitmap}.  
The $n$-bit-long parity bitmap encoding of $\{A_i\}_{i=1}^n$, denoted as $A[1..n]$, is defined as follows. 
For $i = 1, 2, ..., n$, $A[i]$, the $i^{th}$ bit of $A[1..n]$, is equal to $1$ if $A_i$ contains an odd number of elements,
and is equal to $0$ otherwise. 
%{\color{blue} This way each bit $A[i]$ encodes the oddness/evenness (parity) of the cardinality of the set $A_i$, and hence we call $A[1..n]$ a parity bitmap.} 
%{\color{green} From Mitsu: This sentence may be redundant and can be removed}
The $n$-bit-long parity bitmap of $\{B_i\}_{i=1}^n$, denoted as $B[1..n]$, is similarly defined. 
In the aforementioned ideal situation of the $d$ elements in $A\triangle B$ landing in $d$ distinct subset-pair-differences, the two bitmaps differ in exactly $d$ bit positions.  In this situation, if Bob knows these $d$ bit positions then the $d$ corresponding subset pairs, and hence the set pair $A$ and $B$, can be easily reconciled as we will describe in \autoref{sec:pbs_smalld}.  

While Alice can certainly send the $n$-bit-long parity bitmap $A[1..n]$ to Bob, this is quite wasteful since $n\! \gg\! d$.  
Instead, using the same error-correction coding trick used first in PinSkech~\cite{Dodis_PinSketch_2008}, Alice can achieve the same goal by sending to Bob a BCH~\cite{bch1} codeword of much shorter length
%roughly of length $d \log n$ 
that can ``correct'' $B[1..n]$ (which Bob already has locally) into $A[1..n]$ by viewing the $d$ bits where $A[1..n]$ and $B[1..n]$ differ as ``bit errors" that occurred during an imaginary transmission of $A[1..n]$ over a noisy communication channel.  
Referring to this BCH coding as sketching (as was done in~\cite{Dodis_PinSketch_2008}), we call our scheme Parity Bitmap Sketch (PBS).
%{\color{red} The ``Sketch'' in the name Parity Bitmap Sketch is a reference to this BCH coding as sketching (as was done in~\cite{Dodis_PinSketch_2008}).}



\subsubsection{When \texorpdfstring{\larger\MakeLowercase{$d$}}{d} is large}\label{sec:larged}

In general, $d$ can be much larger than several.  When $d$ is very large, it would be computationally too costly to decode all $d$ errors ``in one shot'' (i.e., in a single parity bitmap) using the
aforementioned $O(d^2)$ BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019}.
% that as explained earlier has a time complexity of $O(n^2)$ finite field operations.
%$ \log^2 d)$ (where the $\log^2 d$ term comes from the ``width" of the underlying Galois field to handle the aforementioned ``$d$ bit errors"), 
Instead, in this case we partition, consistently using a different hash function $h'$ (than the $h$ above), sets $A$ and $B$ each into $d/\delta$ smaller sets, where 
$\delta$ is a small number no larger than several (just like what we earlier assumed $d$ to be).  
We refer to these smaller sets as {\it groups} to distinguish them from the {\it subsets} $A_i$'s and $B_i$'s above.  
With this partitioning, on average only $\delta$ distinct elements are hashed to any group pair.
%With such a partitioning, each group pair on average contains $\delta$ is distinct elements.   
%Here $\delta$ is a small number no larger than several, just like what we earlier assumed $d$ to be.   
%Any such pair can then be reconciled using the first two steps of PBS explained earlier.  
Then, the PBS-for-small-$d$ scheme described above is used to reconcile each group pair. 
%Hence, the third step of PBS is to apply the first two steps to each group pair.
% which as just explained differ by 
%at most several elements like the set pair $(A, B)$ was earlier assumed to be.   s
The computational complexity of the BCH decoding involved in reconciling each group pair is only $O(\delta^2)$, which can be considered $O(1)$, since $\delta$ is a small constant. 
%(finite field operations).  
As a result, the total BCH and other decoding computational complexity of PBS (for all $d/\delta$ group pairs) is only $O(d)$.
%, just like IBF-based solutions as mentioned earlier.  


% which is 
%much smaller than between $O(d^2)$ and $O(d^3)$ for ECC-based solutions such as PinSketch.  

%We emphasize hash-partitioning appears to be the only practical partitioning technique for partitioning two sets consistently in the sense 
%every (common) element in $A\bigcap B$ is mapped to the same subset or group pair.  

%We fix such a group pair, denoted as $A^{(g)}$ and $B^{(g)}$, for discussing a potential issue or pitfall that PBS handles very well.  

% {\bf this paragraph has been moved to Section 3} The number of elements in the set difference between any group pair is in general not a constant.  Rather, it is a random variable that has roughly a Poisson distribution with mean $\delta$.  The potential issue arises from dealing with this randomness in setting a global parameter that corresponds to the error-correction capability of the BCH code used for reconciling every group pair.  This parameter, denoted as $t$ (consistent with other literatures on BCH code), is the maximum number of errors that the BCH code used by any group pair can correct, and the size of each such codeword is roughly $8t$ bits (assuming $n = 255$ as explained above). The issue is that, on one hand, if $t$ is too large (say several times larger than $\delta$), then the total size of the BCH codewords, which is the bulk of the extra communication cost, is unnecessarily large; but on the other hand, if $t$ is too small (say equal to $\delta$), then close to half of the BCH codewords cannot decode or worse decode incorrectly (unknown to Alice and Bob), which can result in hefty penalties in the latter case of incorrect decoding.   In PBS, we manage to make $t$ as small as possible (so that the total size of the BCH codewords is kept to a minimum) yet pay negligible penalties of incorrect BCH decoding.

% by exploiting the ``complementary relationship" between the Poisson distribution and the probability distribution of incorrect BCH decoding.  
% {\bf move to the comparison section
% Arguably this partitioning-into-groups strategy can be used by PinSketch to reduce its decoding time complexity to $O(d)$ as well.  However, to do so PinSketch
% would have to pay roughly $(t - \delta) * \log \mathcal{U}$ extra communication complexity per group.  
% }

% \subsubsection{Markov-chain-based modeling of PBS}

\subsubsection{Markov-chain modeling of PBS}

Another significant contribution of this work is a rigorous and accurate Markov-chain modeling of the multi-round set reconciliation process of PBS.  This model enables not only the
accurate analysis of various performance metrics, such as the probability that all distinct elements are successfully reconciled in $r$ rounds, but also the
tuning of the parameters of PBS for near-optimal performances.  In contrast, most existing solutions lack such a rigorous analytical framework. 

\begin{comment}

{\bf (Previous version)} A significant contribution of this work is a rigorous and precise analysis of various performance metrics, such as the total communication overhead and the average number of rounds needed for set reconciliation.   Through this analysis, we obtain exact values of the first moments (expectations) and extremely tight probability tail bounds that err by at most a factor of 2 in the probability value (e.g., the bound $p \ge 1-2 \times 10^{-10}$ implies that the actual probability $p \le 1-10^{-10}$).  In contrast, few existing solutions have rigorous analysis on such performance metrics.  

{\bf A separate contribution of this work is a novel Markov-chain-based analytical framework that can be used to precisely calculate various performance metrics and to near-optimally tune the parameters of PBS.}


Through this analysis, we obtain an extremely tight tail bound on the success probability given parameter settings. This tail bound guides us on parameter settings (to be elaborated in \autoref{sec:parameter_settings}) for various application requirements (e.g., success probability $>99\%$ within $3$ rounds). In contrast, few existing solutions have rigorous analysis on such performance metrics.  

\end{comment}


%% added during revision
\input{section/db_application}

The rest of the paper is organized as follows.  First, we describe the aforementioned PBS-for-small-$d$ and PBS-for-large-$d$ schemes in 
\autoref{sec:scheme} and~\autoref{sec:pbs-for-large-d}, respectively.
%{\bf ??? and ???, respectively}.  
%formally state the set reconciliation problem and describe our scheme (PBS) in \autoref{sec:scheme}. 
Then, we describe our analytical framework in \autoref{sec:tail_bound} and apply it to the performance analysis and the near-optimal parameter tuning of PBS in \autoref{sec:application_analysis}. After that, we present a new estimator for estimating the set difference cardinality in~\autoref{subsec:ToW}. 
%the rigorous and precise analysis and elaborate %parameter settings in \autoref{sec:tail_bound}. 
Finally, we survey existing set reconciliation schemes in \autoref{sec:related}, 
compare the performance of PBS with that of some of them in \autoref{sec:evaluation}, and conclude the paper in \autoref{sec:conclusion}.  



% === to move the following paragraph somewhere

% We emphasize that BCH coding is used in PBS in a very different and much more efficient manner than that in PinSketch~\cite{Dodis_PinSketch_2008}.  
% In PinSketch, each bit encodes only a single element in the universe $\mathcal{U}$, so the size of the bitmap is equal to the size of the universe $u$.  
% For example, when $|\mathcal{U}| = 2^{32}$ as assumed in most existing works, 
% %in the set reconciliation problem we usually assume each element is ``indexed" by a $32$-bit-long (hash) signature, so the universe contains a total of $2^{32}$ elements. In this case, 
% the bitmap encoding for any set in PinSketch is $2^{32}$ bits long, and the Galois field involved in its BCH decoding is the ``$32$-bit-wide" $GF(2^{32})$.  
% In contrast, as explained earlier, in PBS 
% %since each bit encodes the oddness or evenness of the cardinality of a subset,   
% the size $n$ of a bitmap is dependent only on $d$, and not on the size of the universe or on the cardinality of the set the bitmap encodes.   For example, as shown in the example above, $n = 255$ is large enough for $d = 5$.  In this case, the BCH decoding operates in the much shorter
% ``8-bit-wide" $GF(2^{8})$.  This shorter ``width" alone in theory translates into roughly $16$ times shorter BCH decoding time, which as will be explained in \autoref{sec:BCH_code} grows quadratically with the ``width" of the underlying Galois field.  This shorter ``width" also implies four times shorter BCH codeword in PBS than in PinSketch, making it 
% much more costly
% for PinSketch to adopt the same BCH-decoding time reduction technique that we will describe next for the general case where $d$ can be very large, as will be elaborated 
% in \autoref{subsec:protocol2}.  


\begin{comment}
================================ excess paragraphs below ===================

========= two paragraphs on PinSketch that may be useful later ===

Although our solution is not based on the hallmark ECC-based solution PinSketch,
it is very simple to describe on top of the core idea of PinSketch, because our solutions uses the 
BCH coding in a very different and arguably more 
cost-effective way than PinSketch.    Hence here we first provide a brief introduction to PinSketch.  In a nutshell, (the non-crypto-part of) PinSketch is to encode each set as a bitmap, in which each bit corresponds
to an element in the universe;  this bit takes value 1 if the corresponding element belongs to the set and 0 otherwise.  For example, in the set reconciliation
problem we usually assume each element is a 64-long-bit hash signature, so the universe contains a total of $2^{64}$ distinct 64-bit binary strings.
In this case, the set $A$ (that Alice has) 
corresponds to a bitmap that is $2^{64}$ bits long, and so does the set $B$ (that Bob has).  
With a slight and harmless abuse of notation, we denote the  two corresponding bitmaps also as A and B respectively.

With this bitmap encoding, the difference between sets A and B is simply the set of bits that the bitmaps A and B differs in.
Needless to say that the idea of PinSketch is not for 
Alice to send the entire  
bitmap $A$, roughly 16 billion billion bits long, to Bob.
%since Bob already knows bitmap B, which agrees with bitmap A in vast majority of the bits.   
Rather, Alice sends to Bob only the BCH codewords needed to ``correct" the bitmap B, 
which Bob already implicitly (i.e., does not explicitly keep a local copy) knows, to the bitmap A, and vice versa.  
The PinSketch solution is near-optimal in terms of space efficiency.  However, its  
main drawback is that, as mentioned earlier, its decoding computational complexity grows 
at least quadratically, if not cubically, with the number of ``errors" 
(size of set differences) $d$.

====================================================




Furthermore, unlike most IBF-based solutions, 
the performance of this solution, including a number of statistics 
such as the number of iterations needed to reconcile the two sets with a certain high probability (e.g., 0.99999999), 
can be precisely analyzed using a Markov chain.  



This parameter has to be global (same for all group pairs), because the total
cost of determining the appropriate ``capacity" value for each group pair is far higher than any savings from 

 

.   As we will explain 
We have to use th

For example, if we design the BCH code to 
be able to correct exactly 
 

, as used above in partitioning a set into subsets or groups, is the de facto partitioning technique
if consistency 

We discuss a subtle issue with hash-partitioning 





The value $d'$, the average number of 
distinct elements in $ ??? $ that are hashed to any group, 

as explained above, 

Then we hash-partition $A$ and $B$ each 
into $O(d)$ subsets, using a different random hash function $g$ (than the $h$ above),
such that on average each subset pair $A^i$ and $B^i$ (so denoted to distinguish them from $A_i$ and $B_i$ above)
differ by several elements.  


So far, we assume the value of $d$ is precisely known.  In this case, we first obtain an estimate of $d$
using a set difference estimation protocol such as~\cite{Feigenbaum's}.  





  This bit takes value 1 if the corresponding element belongs to $A$ and 0 otherwise.



As we will show, 

With such an encoding, $k$ only needs to be at least $\Omega(d^2)$

the $d$.  


and this cardinality can potentially be very large (e.g., millions).





{\bf Long and Liang:  Maybe we can add a hat to A and B to denote bitmaps in the following}.  
With a slight and harmless abuse of notation, we denote the  two corresponding bitmaps also as A and B respectively.



When $d$ is small 

 For example,
when $d$ is around 5, $k$ only needs to be $255$.  


In comparison, in the bitmap encoding of a set in each bit corresponds
to only a single element in the universe;  this bit takes value 1 if the corresponding element belongs to the set and 0 otherwise.  









whereas in PinSketch, each bit corresponds to 
whethe


, the ``$d$ balls" in the set difference are thrown independently uniformly randomly
into $k$ bins.  Since $k >> d$, with high probability, these $d$ balls fall into $d$ distinct bins.  Suppose this usual case 
happens.   
Then each such bin, say bin $i$, 
corresponds to subsets $A_i$ and $B_i$ differing by only one element (the ball that falls into it), in which case Alice and Bob
can reconcile $A_i$ and $B_i$ by exchanging only one element worth of content as will be shown in ...   Before Alice and Bob
can do so however, they need to first figure out the indices of the $d$ bins (the bit locations in the k-bit bitmap), that the balls
fall into (the bit values differ between the two $k$-bit bitmaps).  This can clearly be accomplished using 
the same BCH coding as above.  Note that the BCH encoding and decoding in our solution operates on 
a much smaller finite field of say GF($2^8$) (corresponding to $k = 255$ in the above example) than GF($2^{64}$) in 
PinSketch.   



(containing those elements hashed to value $1$ 
by $h$),  and the set B into 
$k$ subsets $B_1$, $B_2$, ..., $B_k$, both using the same hash function $h$.  The set $A$ is thus encoded as 
a $k$-bit bimtap in which, for any $i$ such that $1 \le i \le k$, the $i^{th}$ bit takes value 1 if the set $A_i$ contains an odd
number of elements, and takes value 0 otherwise;  the set $B$ is similarly encoded as a $k$-bit bitmap.  Note although this 
$k$ has to much larger than $d$ as hinted earlier, it is tiny compared with $2^{64}$, the size of the universe.  For example,
when $d$ is around 5, $k$ only needs to be $255$.  

With such a hash partition, the ``$d$ balls" in the set difference are thrown independently uniformly randomly
into $k$ bins.  Since $k >> d$, with high probability, these $d$ balls fall into $d$ distinct bins.  Suppose this usual case 
happens.   
Then each such bin, say bin $i$, 
corresponds to subsets $A_i$ and $B_i$ differing by only one element (the ball that falls into it), in which case Alice and Bob
can reconcile $A_i$ and $B_i$ by exchanging only one element worth of content as will be shown in ...   Before Alice and Bob
can do so however, they need to first figure out the indices of the $d$ bins (the bit locations in the k-bit bitmap), that the balls
fall into (the bit values differ between the two $k$-bit bitmaps).  This can clearly be accomplished using 
the same BCH coding as above.  Note that the BCH encoding and decoding in our solution operates on 
a much smaller finite field of say GF($2^8$) (corresponding to $k = 255$ in the above example) than GF($2^{64}$) in 
PinSketch.   




 using a hash function $h$,
and similarly partition the set B into $k$ subsets

and B each   
These $d$ differences can be viewed as $d$ balls.
Our idea is to uniformly randomly throw these $d$ balls into $k >> d$ bins, so that with fairly high probability the following ideal
situation happens:  no bin contains 
more than one balls.  The reason why this situation is ideal will become clear shortly.  We will show that, under this ideal situation,
sets $A$ and $B$ each can be encoded, without information loss, as a $k$-bit bitmap so that $A's$ bitmap differs with $B's$ in the i-th
bit if and only if a ball falls into the i-th bin.  

and is based on the following
idea.  Based on an estimation of $d$, we divide set $A$ into $O(d)$ subsets ... using a hash function $h$.  We similarly 
divide $b$ into subsets ... using the same hash function $h$.  


This balls-into-bins operation can be carried out by uniformly randomly dividing set $A$ into $k$
subsets ... and set $B$ also into $k$ subsets ..., both using the same hash function $g$.  If subsets $A_i$ and $B_i$ differ by exactly
one element, then we say exactly one ball falls into bin $i$, and in this case reconciliation between $A_i$ and $B_i$ can be 
accomplished in a straightforward manner (and hence it is a good case that makes the decoding easy), as will be elaborated in ...    
Suppose every pair of subsets $A_i$ and $B_i$ either agree 










==== the following two are legacy paragraphs emphasizing set-diff

and has rigorous 

approaches this problem from a unique angle:  to implicitly map
a set to a random walk using a hash function.  The encoding allows for a very communication-efficient way of comparing two sets for their 
differences.  For example, we can succinctly encode/represent the set as the end point of the random walk.  
With this representation, we can reasonably accurately estimate the size difference between A and B from 
the respective end points of their RW encodings. 
For example, when A and B differs by only one element, their RW encoding will differ by only 1, so observing the latter
suggests the former with a decent probability, and this probability could be strengthened through multiple independent mappings (hash functions).
 









[move the following paragraph somewhere]
Almost all recent work on set difference is based on min-hash.  The idea is to summarize the elements in a set by a min-hash value.  
Given a hash function h, the minimum among all the hash values of all elements, is called the min-hash value of the set A with respect to 
h.  More precisely [mathematical definition].  Then to find out the difference between set A and B, we examine if their min-hash values 
... and ... are the same.  It is not hard to prove that, given a uniform hash function, Pr[ ... = ...] = ...  Using multiple such hash functions h1, h2, ...,
we can estimate ... from examining how many such equations (inside the Pr[ ]) hold.

[maybe we should focus on the set reconciliation, and mention our resurrecting the ToW-based approach as a side contribution] 

==== the following two are legacy paragraphs emphasizing set-diff
\end{comment}

==> section/meeting-notes.tex <==
1. Further reduce communication overhead: It seems that we can save some communication overhead during the XOR step, for example, we randomly sample several bits from the 32 bit as the rule for partitioning subsets, and then we only need to transmit the remaining ones!

2. Advantages over minisketch (even if it also uses the partition approach): Unlike our scheme, minisketch does not support 
``partial decoding'' in the sense that minisketch can either decode all or decode nothing. When decoding fails, it has to ``increase 
the decoding capability'' (even with the recent proposed approach called bisection: randomly sample a portion and encoding those 
sampled portion with BCH ``high enough decoding capacity'') which results in higher communication (high penalty). However about ensure most graphs to be able to decode successfully 
w.h.p (give an example, we need much higher decode capacity than the average number of balls in each bin).

They cannot figure out where goes wrong when failure happens. 

3. Advantages over IBLT-based approaches: lower communication overheads yet similar computational complexity. Besides, IBLT-based 
approaches do not support effective ``partial decoding'' either, which means when failure happens, the communication overhead would 
increase significantly.

4. How about Graphene? It works extremely well when the set difference of the the two sets have comparable size as that of their intersection. Graphene is a hybrid approach that combines the Bloom filter (BF) based ones and Invertible Bloom filter based approaches. 

The basic idea is to send a BF which contains all elements in $A$ together with an IBLT that aims at compensating the false positive 
effects of the BF. However, we found that in our cases where $|A\Delta B|\ll |A\cup B|$, Graphene has to either use a BF with low 
false positive rate but requires even more space than the IBLT-only solution or use a useless BF with a very high false positive rate (say, 0.99). .... 

5. Discussion on multiple iterations: We donot think running multiple iterations (rounds) in our approach is a big issue, since 
the synchronization process (synchronization of the data objects between the two hosts) can start immediately after the 
first iteration (round) as we have shown in ... most elements in the set difference will be recovered in the first iteration. 

6. Advantages over all existing approach: Our approach have rigorous theoretical analysis, we can provide strong and tight theoretical guarantee.


==> section/misc_paragraphs.tex <==
%Note that $M(i, j)$ is originally an infinite matrix as $i$ and $j$ each can take any nonnegative integer values.  However, elements other than those $(t+1) \times (t+1)$ in the ``upper-left corner" of (the original) $M$
%are irrelevant when we assume $i \le t$.  

  For all practical matrices, however, it can be considered an $(t+1) \times (t+1)$ matrix, since under the 
assumption $i \le t$,   
In other words, we compute only the $(t+1) \times (t+1)$ elements in the ``upper-left corner" of $M$, and call that $M$ instead.  
 
 
==============
 
Note that $M$ is originally (i.e., before all but the $(t+1) \times (t+1)$ elements in the ``upper-left corner" is ``truncated out") 
an infinite matrix. 
 
It is clear from the three bases that the value of each term $ ??? (i, j, k)$ depends on only one parameter (other than the arguments $i$, $j$, $k$):  $n$.  
As a result, $n$ is the only parameter in the matrix $M$.  We will use this fact in {\bf ???}.  

%Hence, in using this analytical framework for optimal parameter tuning, 


Since $M$ is parameterized only by $n$ (mentioned at the end of ???), we can precompute a 
$(t+1) \times (t+1)$ matrix $M$ for each of these several possible $n$ values, where $t$ is a universal (for all values of $n$)
parameter that is set conservatively to a large value (to make $Pr[\delta_i > t]$ tiny) such as several times of $\delta$.
This way, the cost of computing $M$ can be excluded from that of set reconciliation.

=============


A universal $t$ value that is the maximum possible  

and use it for 

      
all possible parameter values (there are only several of them) of $n$ so that set reconciliation




 so $t$ is the ``bound" of the ``support" of (the infinite) $M$, 


==> section/model.tex <==
\section{Problem Statement}\label{sec:model}

In this work, we adopt the commonly used model for the set reconciliation problem. 
Two remote sets $A$ and $B$ are stored at hosts Alice and Bob respectively. The elements in $A$ and $B$
are from the same universe $\mathcal{U}=\{0, 1,\cdots,u-1\}$ and denoted as $\log u$-bit-long signitures.  
The set reconciliation problem is to compute the symmetric set difference between $A$ and $B$, 
{\it i.e.,} $A\Delta B\triangleq (A\!\setminus\! B) \bigcup (B\!\setminus\! A)$. We denote $d\!=\!|A\Delta B|$. Throught this paper, we call each element in $A\Delta B$ a \textit{distinct element}, and we call each element in $A\bigcap B$ a \textit{common element}.

Like most works on set reconciliation, we consider set reconciliation is {\it complete} if one of the two hosts knows the set difference $A\Delta B$. In \autoref{sec:evaluation}, we use the same semantic to measure the communication cost of our scheme and other compared set reconciliation schemes. {\bf a stronger semantic may not be necessary}

\begin{comment}
=== may not be the best location === 
We note that our scheme, which we will describe in~\autoref{sec:scheme}, does not work for $0$ as we will explain 
in~\autoref{subsec:protocol0}. However, we can extend our scheme to support 0. For example, 
we let Alice send to Bob a single bit to indicate whether Alice has element 0, so Bob will know whether 
$0\in D$ or not. In the sequel of this paper, we assume 0 is excluded from $\mathcal{U}$.  

\subsection{Performance Metrics}\label{subsec:metrics}
%% More references are needed here
% Like~\cite{Eppstein_WhatsDifference?Efficient_2011,Dodis_PinSketch_2008}, we assume that 
% sets $A$ and $B$ are stored at two distinct hosts. 
The research objective of set reconciliation is to compute $D$ with low cost, as 
measured by different performance metrics. Typically, set reconciliation algorithms are evaluated on the following three performance 
metrics: {\it communication}, {\it computation}, and {\it latency}. 
\end{comment}

==> section/more_related_work.tex <==
\section{More Related Work}\label{sec:more-related}

\subsection{Set Reconciliation Algorithms}

Recently, a Cuckoo Filter (CF)~\cite{Fan_CuckooFilterPractically_2014} based set reconciliation 
algorithm was proposed in~\cite{Luo_SetReconciliationCuckoo_2019}. Though empirically CFs 
can have lower space overhead than BFs, 
this CF-based set reconciliation algorithm still suffers from the two major weaknesses 
described in~\autoref{sec:closely-related} as BF-based schemes do. 

Besides the standard set reconciliation problem, many researchers considered its variants. 
For example,  Gabrys {\it et al} considered in~\cite{Gabrys2019} the variant of reconciling two {\it similar sets}, in which 
elements in the symmetric difference $A\Delta B$ are similar (more precisely, 
they are related through the Hamming distance metric). Luo {\it et al} considered 
in~\cite{Luo_accurateMultisetReconciliation_2019a} the variant of 
reconciling multisets, in which elements can have multiple replicas. 

\subsection{Set-Difference Size Estimators} 

Besides the min-wise estimator and Strata estimator describe in~\autoref{sec:closely-related}, 
the algorithm, which was proposed in~\cite{Feigenbaum_AppL1Difference_2003} and designed for 
more general $L_1$ difference, can also be 
used for the estimation of th set-difference size. Similar to our ToW estimator, 
it also achieves near-optimal communication overhead. 
However, it is much more complicated than our ToW based algorithm. 

==> section/motivation_analysis.tex <==
\subsection{Motivation (new section)}\label{sec:motivation_theoretical_analysis}

In this section, we establish an analytical framework for the set reconciliation process of PBS to reach the optimizable goal. Recall that the optimizable goal is to find the optimal parameter settings that minimize the overall communication overhead under the constraint that $Pr[R\leq r]$, the success probability of PBS within $r$ rounds, is at least $p_0$ {\bf (To Jim: success probability is defined in multi-group multi-round operations section)}. From the analytical framework, we can obtain a fairly accurate estimate (more precisely, a tight lower bound) of $Pr[R\leq r]$ under any given parameter settings and target number of rounds $r$. Using this estimate, we can verify if an arbitrary parameter setting satisfies the constraint by checking if the estimate of $Pr[R\leq r]$ is larger than or equal to $p_0$. Among all the parameter settings that satisfy the constraint, we select the ``best'' (near-optimal) parameter setting that has the lowest communication overhead. The details about parameter settings will be elaborated in \autoref{sec:parameter_settings}. 

This analytical framework also enables us to analyze two other performance metrics of PBS. The first one is the effect of the target number of rounds $r$ on parameter settings. Note that $Pr[R\leq r]$ is a function of the number of subsets per group $n$ and the BCH error-correction capability $t$. In general, to achieve the same target success probability $p_0$ (i.e., ensure $Pr[R\leq r]\geq p_0$) within a small target number of rounds $r$, we need $n$ and $t$ to be larger, so that in each group pair (1) the ideal case happens with higher probability; and (2) the BCH decoding succeeds with higher probability. The larger $n$ and $t$ lead to higher communication overhead and BCH decoding complexity. Due to this relation, we have a trade-off between the target number of rounds $r$ and the resulting communication overhead and BCH decoding complexity (under the corresponding optimal parameter setting). The analytical framework can help us to find the ``sweet spot'' of $r$ in this trade-off that achieves the most ``saving'' on both the communication overhead and the BCH decoding complexity while managing to make $r$ as small as possible, as will be elaborated in \autoref{sec:vary_r}. 

The second performance metric of PBS is ``piecewise reconciliability''. 
%Note that PBS reconciles the distinct elements gradually round by round: As we described in \autoref{subsec:protocol2}, each group pair is independently reconciled by PBS-for-small-$d$, in which some of the distinct elements in the group pair can be reconciled in each round. 
The analytical framework also helps us to analyze the aforementioned question that is related to ``piecewise reconciliability'', that is, ``what portion of the distinct elements are expected to be reconciled in the first round, in the second round, etc.''. The result shows that the vast majority of the distinct elements are reconciled in the first round, which induces that the communication overhead in the first round, which is roughly proportional to the number of distinct elements that are reconciled in the first round, is the bulk of the overall communication overhead. This property is useful for parameter settings. 
%All these three applications will be elaborate in \autoref{sec:application_analysis}.

===============================
The parameter settings are related to both the target success probability $p_0$ and the target number of rounds $r$. In general, to achieve the same target success probability, the smaller $r$ is, the larger $n$ and $t$ are needed to respectively ensure (1) the ideal case happens with higher probability; and (2) the BCH decoding in each group succeeds with higher probability, and therefore a higher communication overhead and BCH decoding complexity are required. In \autoref{sec:vary_r}, we will analyze the effect of $r$ in details using the analytical framework.

Note that PBS reconciles the distinct elements gradually round by round: As we described in \autoref{subsec:protocol2}, each group pair is independently reconciled by PBS-for-small-$d$, in which some of the distinct elements in the group pair can be reconciled in each round. This is the ``piecewise reconciliability'' mentioned in \autoref{sec:intro_oursolution}. In \autoref{sec:piecewise_decodability}, we will analyze ``what portion of the distinct elements are expected to be reconciled in the first round, in the second round, etc.'' using the analytical framework. The results, closely related (roughly proportional) to ``how much reconciliation works are expected to be done in the first round, in the second round, etc.'', show that the vast majority (over $95\%$) of the overall communication overhead is in the first round. This property will be used in our parameter settings, as we will describe shortly.

%, the probability that all group pairs are successfully reconciled within $r$ round, is at least $p_0$. 

{\bf (Copy from multiround-for-large-d)} This optimization goal is hard to achieve if not impossible, since the distribution of $R$ depends on many parameters, such as the number of groups $g$, the number of subset pairs per group $n$, etc. Instead, we propose a more optimizable goal, which is roughly the dual of the previous goal. In this optimizable goal, we set a {\it target success probability} $p_0$ combined with a {\it target number of rounds} $r$ to specify its constraint, that is, $Pr[R\leq r]$, the probability that all group pairs are successfully reconciled within $r$ round, is at least $p_0$. The optimizable goal itself is to find the optimal parameter settings that minimize the overall communication overhead under the above constraint. 

In PBS, the set reconciliation process of the group pairs are independent with each other, and each group pair runs as many rounds of PBS-for-small-$d$ as needed to reconcile all distinct elements in it. Therefore, different group pairs may take different number of rounds to be successfully reconciled. The total number of rounds to reconcile all group pairs, denoted as $R$, is their maximum.
An obvious goal related to $R$ is, given the total ``budget'' of communication overhead, find the optimal parameter settings for PBS that {\it stochastically minimize} $R$. 

This optimization is hard to achieve if not possible. Instead, we propose a more optimizable goal, which is roughly the dual of the previous optimization problem, as follows: Given a {\it target success probability} $p_0$ and a {\it target number of rounds} $r$, find the optimal parameter settings that minimize the overall communication overhead under the constraint that the {\it success probability}, the probability that all distinct elements are reconciled, within $r$ rounds is at least $p_0$. 

Towards this optimizable goal, we propose an analytical framework for the set reconciliation process of PBS. From this framework, we can obtain a fairly accurate estimation of the success probability within an arbitrary number of rounds under any given parameter settings. Based on it, we can reach the optimizable goal, as we will elaborate in \autoref{sec:parameter_settings}. This analytical framework also enables us to analyze other performance metrics of PBS, as we will show in \autoref{sec:vary_r} and \autoref{sec:piecewise_decodability}.
===============================


% In this section, we provide a theoretical analysis (analytical framework) for the set reconciliation process of PBS and establish a tight tail bound on the {\it success probability} within $r$ rounds under arbitrary parameter settings of $n$, $\delta$, and $t$. This analytical framework has several applications on parameter settings and analyzing the properties of PBS that we will elaborate in \autoref{sec:application_analysis}.

% Note that the set reconciliation process of the group pairs are independent with each other, and each group pair runs as many rounds of PBS-for-small-$d$ as needed to reconcile all distinct elements in it. Therefore, different group pairs may need different number of rounds to be successfully reconciled. Intuitively, we want all group pairs to be successfully reconciled in only a few rounds (say $3$) with high probability (say $99\%$). Hence, when tuning parameters (to be discussed in \autoref{sec:parameter_settings}), we set a {\it target success probability} $p_0$ combined with a {\it target number of rounds} $r$ as the {\it paramenter setting requirement}, which aims to ensure that the {\it success probability}, the probability that all distinct elements (of all group pairs) are reconciled, within $r$ rounds to be at least $p_0$. 

% {\bf Normally, to achieve the same target success probability within fewer rounds (smaller $r$), PBS need more resources (e.g., larger $n$, $t$) for the ideal case happening with higher probability (fewer exceptions happen and need to be handled in later rounds), as we will explain in \autoref{sec:vary_r}.}

% On one hand, this tail bound gives us a theoretical guarantee on the success probability under specific parameter settings. On the other hand, given a parameter setting requirement (i.e., a target success probability $p_0$ within $r$ rounds), we can use the tail bound to find all feasible parameter settings that satisfy the requirement, then select the optimal parameter settings among them that have the lowest communication overhead. {\bf This analysis also provides other theoretical results for PBS, such as the expected number (percentage) of the distinct elements would be reconciled in the each round (``piecewise decodability'', to be shown in \autoref{sec:piecewise_decodability})}%In this section, we continue to assume $d$ is precisely known. 

% For simplicity, we ignore the small probability event that a type (\RN{2}) event happens, in which the incurred ``fake'' distinct element is not successfully verified by \autoref{alg:verification} (mentioned in \autoref{subsec:exception_hash_partition}). As we discussed earlier, this event happens with a tiny probabilty that is in order of $10^{-7}$. Hence, ignoring this event barely compromises the accuracy of our analysis. 

==> section/multiround.bk.0719.tex <==
\subsection{Running PBS for Multiple Rounds}\label{sec:multi-rounds}

%{\bf (merged from the following two paragraphs)} 

As mentioned earlier, when the ideal case does not happen, Alice and Bob cannot successfully reconcile their respective sets $A$ and $B$ 
%in the first round, 
{\color{red}in a single round}, 
and Alice can tell this situation from the checksum verification
step {\color{red}({\it i.e.,}~\autoref{step:terminate_condition} of~\autoref{alg:single_round_pbs})}.  In this situation, Alice and Bob need to run additional rounds of \autoref{alg:single_round_pbs}, but with a different input set pair (than $(A, B)$) as follows. 
%To deal with the ``remaining'' distinct elements, 
Let $\hat{D}_1$ be the estimated set difference Alice obtained in the first round.
In the second round, Alice and Bob try to reconcile their respective sets $A\triangle \hat{D}_1$ and $B$, from which Alice obtains another estimated difference (between $A\triangle \hat{D}_1$ and $B$) that we denote
as $\hat{D}_2$.  If the set reconciliation is still not successfully completed, Alice and Bob run a third round to try to reconcile sets $(A\triangle \hat{D}_1)\triangle \hat{D}_2$ and $B$.  This process continues
until the set reconciliation is successfully completed as verified by the checksum. 

%{\color{red}The final result is $\hat{D}_1\triangle\hat{D}_2\triangle\cdots\triangle \hat{D}_r$, 
%where $r$ is the number of rounds this process runs 
%and $\hat{D}_i$ for $i=1,2,\cdots,r$ is the estimated set difference in the $i^{th}$ round. 
%}


In each subsequent round, a different and (mutually) independent hash function is used to perform the consistent hash partitioning of the two sets to be reconciled (e.g., $A\triangle \hat{D}_1$ and $B$ in the second
round), so that the same type (\RN{1}) and/or (\RN{2}) exceptions encountered in the previous round, which have so far prevented the set reconciliation from being successfully completed, can be avoided with 
overwhelming probability.  The use of independent hash functions in different rounds offers another significant benefit:  How the number of unreconciled distinct elements decreases one round after another (and 
eventually goes down to $0$) can now
be precisely modeled as a Markov chain, as will be elaborated in \autoref{sec:tail_bound}. 


\begin{comment}
We have shown in the previous section that a trouble-causing element $s$ resulting from a type (\RN{2}) exception in the first round will be mistakenly considered as a distinct element (between $A$ and $B$) 
and included in $\hat{D}_1$, by Alice. 
This will not lead to a reconciliation error, since $s$ will be detected in later rounds for the following reason. 
When $s\not\in A\triangle B$, there are two possible scenarios: (1) $s\!\in\! A$ \& $s\!\in\! B$; and (2) $s\!\not\in\! A$ \& $s\!\not\in\! B$. 
%{\bf (still think this sentence is unnecessary) The latter happens with much higher probability than the former, because $s$ is the \code{XOR} of multiple (distinct) elements and therefore can be considered as a random element. It coincidentally lands in $A\cap B$ with a tiny probability, since the size of the universe $\mathcal{U}$ is typically much larger than $|A\cap B|$.} 
If scenario (1) is the case, we have $s\!\in\! B$ whereas $s\!\not\in\! A\triangle \hat{D}_1$ (since $s\!\in\! \hat{D}_1$ and $s\!\in\! A$). Hence $s$ is a distinct element between $A\triangle \hat{D}_1$ and $B$.  In a later round, say the 
second round to make our presentation simple, $s$ will be reconciled and included in $\hat{D}_2$.  This is however a ``contradiction", since an actual distinct element should not be discover ``twice'' (once in $\hat{D}_1$ 
and another in $\hat{D}_2$).  From this ``contradiction", Alice concludes that $s$ is not an actual distinct element.
% incurred by a type (\RN{2}) exception.
%a trouble-causing element (i.e., a fake element). 
Similarly, Alice will detect the same ``contradiction" in the case of scenario (2).
\end{comment}
% is the case and the trouble-causing element will be detected.



%%%% added by Long
{\color{red}
The following theorem concerns the correctness of PBS.

\begin{theorem}\label{thm:corrctness}
Assuming that the verification in~\autoref{step:terminate_condition} of~\autoref{alg:single_round_pbs} is always correct. If PBS terminates after $r$ rounds, then 
% the result of PBS, $\hat{D}_1\triangle\hat{D}_2\triangle\cdots\triangle \hat{D}_r$ is correct, {\it i.e.,}
\[
\hat{D}_1\triangle\hat{D}_2\triangle\cdots\triangle \hat{D}_r=A\triangle B.
\]
\end{theorem}
\begin{proof}
Since PBS terminates after $r$ rounds, we have, the verification in~\autoref{step:terminate_condition} of~\autoref{alg:single_round_pbs} succeeds in the $r^{th}$ round, {\it i.e,} 
$c\big{(}(A\triangle\hat{D}_1\triangle\hat{D}_2\triangle\cdots\triangle \hat{D}_{r-1})\triangle \hat{D}_{r}\big{)}=c(B)$. 
Hence, 
$(A\triangle\hat{D}_1\triangle\hat{D}_2\triangle\cdots\triangle \hat{D}_{r-1})\triangle \hat{D}_{r}=B$. Therefore,
\[
\hat{D}_1\triangle\hat{D}_2\triangle\cdots\triangle \hat{D}_r=A\triangle B.
\]
\end{proof}

\noindent
{\bf Remarks.} We have shown in the previous section that some distinct elements might be 
excluded from $\hat{D}_1$ in the first round because of 
type (\RN{1}) exceptions, and
a fake distinct element resulting from a type (\RN{2}) exception in the first round 
will be mistakenly considered as a distinct element (between $A$ and $B$) 
and included in $\hat{D}_1$, by Alice. More complicated scenarios might happen if those missing distinct elements or 
fake distinct elements get involved in possible exceptions in the subsequent rounds. 
However, by the above theorem, PBS guarantees that all these exceptions will be fixed automatically, and outputs the correct 
reconciliation result, though their occurrence will result in more rounds required by PBS to terminate. 
We will show in~\autoref{sec:BCH_exception} that the number of rounds for PBS to correctly reconcile all distinct 
elements is small with overwhelming probability. 
}



\begin{comment}

Recall that a trouble-causing element $s$ incurred by a type (\RN{2}) exception will be mistakenly believed as a distinct element (between $A$ and $B$) and be contained in $\hat{D}_1$. %This is not an issue because $s$ 
It can be easily detected in the latter rounds for the following reason. Note that when $s\not\in A\triangle B$, there are two possible scenarios: (1) $s\in A$ \& $s\in B$; and (2) $s\not\in A$ \& $s\not\in B$. 
%{\bf (still think this sentence is unnecessary) The latter happens with much higher probability than the former, because $s$ is the \code{XOR} of multiple (distinct) elements and therefore can be considered as a random element. It coincidentally lands in $A\cap B$ with a tiny probability, since the size of the universe $\mathcal{U}$ is typically much larger than $|A\cap B|$.} 
If (1) is the case, we have $s\in B$ whereas $s\not\in A\triangle \hat{D}_1$ (since $s\in \hat{D}_1$ and $s\in A$). Hence $s$ is a distinct element between $A\triangle \hat{D}_1$ and $B$. In the second round, $s$ should be reconciled with high probability. If so, $s$ will be contained in $\hat{D}_2$. This is however a contradiction, since an actual distinct element should not be reconciled ``twice'' (i.e., $s\in \hat{D}_1$ and $s\in \hat{D}_2$) in this multi-round set reconciliation process. From this contradiction, we can deduct that $s$ is not an actual distinct element, but a trouble-causing element incurred by a type (\RN{2}) exception.
%a trouble-causing element (i.e., a fake element). 
Similarly, the same contradiction happens if (2) is the case and the trouble-causing element will be detected.

Alice remove (and save) all the distinct elements that has been reconciled in the first round, denoted as $\hat{D}_1$, and run another round of PBS. More precisely, in the second round, we try to reconcile $A\triangle \hat{D}_1$ and $B$ to obtain the estimated set difference between them, denoted as $\hat{D}_2$, by running the same procedure except for using a different and independent hash function (than $h$) to do hash-partition. 
%instead of reconciling $A$ and $B$ for both (1) removing all the distinct elements that have been reconciled; and (2) keeping all the distinct elements that have not been reconciled, which we will explain shortly. 
Here we use a different and independent hash function to avoid the same type (\RN{1}), (\RN{2}) exceptions happen again. If there are still some distinct elements remaining as verified by the checksum (\autoref{alg:single_round_pbs} of \autoref{step:terminate_condition}), we run another round of PBS (the third round) and try to reconcile $(A\triangle \hat{D}_1)\triangle \hat{D}_2$ and $B$ using another different and independent hash function, so on and so forth, until the set reconciliation is successfully completed as verified by the checksum.
% We use a different hash function for hash-partition in the second round to avoid the same exceptions (i.e., type (\RN{1}), (\RN{2}) events) that happened in the first round happen again. 
%PBS keeps running until the set reconciliation is successfully completed as verified by the checksum. 
The use of independent hash functions in different rounds naturally enables the Markov chain modeling of the reconciliation process, which will be elaborated in \autoref{sec:single_markov}. 


{\bf (previous)} Note that a fake distinct element $s$ (say is incurred in the first round), if is not detected by \autoref{alg:verification},
%{\bf () and does not coincidentally happens to be an actual distinct element (with negligible probability)}
will be mistakenly believed as a distinct element (between $A$ and $B$) and contained in $\hat{D}_1$. This is not an issue because $s$, if is not an actual distinct element, can be easily detected in latter rounds. Note that when $s\not\in A\triangle B$, there are two possible scenarios: (1) $s\in A$ and $s\in B$; and (2) $s\not\in A$ and $s\not\in B$. 
%{\bf (still think this sentence is unnecessary) The latter happens with much higher probability than the former, because $s$ is the \code{XOR} of multiple (distinct) elements and therefore can be considered as a random element. It coincidentally lands in $A\cap B$ with a tiny probability, since the size of the universe $\mathcal{U}$ is typically much larger than $|A\cap B|$.} 
If (1) is the case, we have $s\not\in A\triangle \hat{D}_1$ (since $s\in \hat{D}_1$). That means $s$ is a distinct element between $A\triangle \hat{D}_1$ and $B$ and would be reconciled in the second round with high probability. If this is the case, we have $s\in \hat{D}_2$. This is however a contradiction, since an actual distinct element should not be reconciled ``twice'' (i.e., $s\in \hat{D}_1$ and $s\in \hat{D}_2$) in this multi-round set reconciliation process. From this contradiction, we can deduct that $s$ is a fake distinct element. Similarly, the same contradiction can be detected in (2).  
%Assume in the second round, PBS reconciles $s$ and saves it in $\hat{D}_2$ (happens with high probability), then we find a contradiction that $s$ has been reconciled ``twice'' and is contained in both $\hat{D}_1$ and $\hat{D}_2$. and  is an actual distinct element between $A\triangle \hat{D}$ and $B$. Starting with the second round, PBS will try to reconcile $s$ and eventually ``correct'' this fake distinct element. 

\end{comment}

==> section/multiround_copy.tex <==
\subsection{Running PBS for Multiple Rounds}\label{sec:multi-rounds}

%{\bf (merged from the following two paragraphs)} 

As mentioned earlier, when the ideal case does not happen, Alice and Bob cannot successfully reconcile their respective sets $A$ and $B$ 
%in the first round, 
{\color{red}in a single round}, 
and Alice can tell this situation from the checksum verification
step {\color{red}({\it i.e.,}~\autoref{step:terminate_condition} of~\autoref{alg:single_round_pbs})}.  In this situation, Alice and Bob need to run additional rounds of \autoref{alg:single_round_pbs}, but with a different input set pair (than $(A, B)$) as follows. 
%To deal with the ``remaining'' distinct elements, 
Let $\hat{D}_1$ be the estimated set difference Alice obtained in the first round.
In the second round, Alice and Bob try to reconcile their respective sets $A\triangle \hat{D}_1$ and $B$, from which Alice obtains another estimated difference (between $A\triangle \hat{D}_1$ and $B$) that we denote
as $\hat{D}_2$.  If the set reconciliation is still not successfully completed, Alice and Bob run a third round to try to reconcile sets $(A\triangle \hat{D}_1)\triangle \hat{D}_2$ and $B$.  This process continues
until the set reconciliation is successfully completed as verified by the checksum. 
{\color{red}The final result is $\hat{D}_1\triangle\hat{D}_2\triangle\cdots\triangle \hat{D}_r$, 
where $r$ is the number of rounds this process runs 
and $\hat{D}_i$ for $i=1,2,\cdots,r$ is the estimated set difference in the $i^{th}$ round. 
}


In each subsequent round, a different and (mutually) independent hash function is used to perform the consistent hash partitioning of the two sets to be reconciled (e.g., $A\triangle \hat{D}_1$ and $B$ in the second
round), so that the same type (\RN{1}) and/or (\RN{2}) exceptions encountered in the previous round, which have so far prevented the set reconciliation from being successfully completed, can be avoided with 
overwhelming probability.  The use of independent hash functions in different rounds offers another significant benefit:  How the number of unreconciled distinct elements decreases one round after another (and 
eventually goes down to $0$) can now
be precisely modeled as a Markov chain, as will be elaborated in \autoref{sec:single_markov}. 


\begin{comment}
We have shown in the previous section that a trouble-causing element $s$ resulting from a type (\RN{2}) exception in the first round will be mistakenly considered as a distinct element (between $A$ and $B$) 
and included in $\hat{D}_1$, by Alice. 
This will not lead to a reconciliation error, since $s$ will be detected in later rounds for the following reason. 
When $s\not\in A\triangle B$, there are two possible scenarios: (1) $s\!\in\! A$ \& $s\!\in\! B$; and (2) $s\!\not\in\! A$ \& $s\!\not\in\! B$. 
%{\bf (still think this sentence is unnecessary) The latter happens with much higher probability than the former, because $s$ is the \code{XOR} of multiple (distinct) elements and therefore can be considered as a random element. It coincidentally lands in $A\cap B$ with a tiny probability, since the size of the universe $\mathcal{U}$ is typically much larger than $|A\cap B|$.} 
If scenario (1) is the case, we have $s\!\in\! B$ whereas $s\!\not\in\! A\triangle \hat{D}_1$ (since $s\!\in\! \hat{D}_1$ and $s\!\in\! A$). Hence $s$ is a distinct element between $A\triangle \hat{D}_1$ and $B$.  In a later round, say the 
second round to make our presentation simple, $s$ will be reconciled and included in $\hat{D}_2$.  This is however a ``contradiction", since an actual distinct element should not be discover ``twice'' (once in $\hat{D}_1$ 
and another in $\hat{D}_2$).  From this ``contradiction", Alice concludes that $s$ is not an actual distinct element.
% incurred by a type (\RN{2}) exception.
%a trouble-causing element (i.e., a fake element). 
Similarly, Alice will detect the same ``contradiction" in the case of scenario (2).
\end{comment}
% is the case and the trouble-causing element will be detected.



%%%% added by Long
{\color{red}
The following theorem concerns the correctness of PBS.

\begin{theorem}\label{thm:corrctness}
Assuming that the verification in~\autoref{step:terminate_condition} of~\autoref{alg:single_round_pbs} is always correct. If PBS terminates after $r$ rounds, then 
% the result of PBS, $\hat{D}_1\triangle\hat{D}_2\triangle\cdots\triangle \hat{D}_r$ is correct, {\it i.e.,}
\[
\hat{D}_1\triangle\hat{D}_2\triangle\cdots\triangle \hat{D}_r=A\triangle B.
\]
\end{theorem}
\begin{proof}
Since PBS terminates after $r$ rounds, we have, the verification in~\autoref{step:terminate_condition} of~\autoref{alg:single_round_pbs} succeeds in the $r^{th}$ round, {\it i.e,} 
$c\big{(}(A\triangle\hat{D}_1\triangle\hat{D}_2\triangle\cdots\triangle \hat{D}_{r-1})\triangle \hat{D}_{r}\big{)}=c(B)$. 
Hence, 
$(A\triangle\hat{D}_1\triangle\hat{D}_2\triangle\cdots\triangle \hat{D}_{r-1})\triangle \hat{D}_{r}=B$. Therefore,
\[
\hat{D}_1\triangle\hat{D}_2\triangle\cdots\triangle \hat{D}_r=A\triangle B.
\]
\end{proof}

\noindent
{\bf Remarks.} We have shown in the previous section that some distinct elements might be 
excluded from $\hat{D}_1$ in the first round because of 
type (\RN{1}) exceptions, and
a fake distinct element resulting from a type (\RN{2}) exception in the first round 
will be mistakenly considered as a distinct element (between $A$ and $B$) 
and included in $\hat{D}_1$, by Alice. More complicated scenarios might happen if those missing distinct elements or 
fake distinct elements get involved in possible exceptions in the subsequent rounds. 
However, by the above theorem, PBS guarantees that all these exceptions will be fixed automatically, and outputs the correct 
reconciliation result, though their occurrence will result in more rounds required by PBS to terminate. 
We will show in~\autoref{sec:BCH_exception} that the number of rounds for PBS to correctly reconcile all distinct 
elements is small with overwhelming probability. 
}



\begin{comment}

Recall that a trouble-causing element $s$ incurred by a type (\RN{2}) exception will be mistakenly believed as a distinct element (between $A$ and $B$) and be contained in $\hat{D}_1$. %This is not an issue because $s$ 
It can be easily detected in the latter rounds for the following reason. Note that when $s\not\in A\triangle B$, there are two possible scenarios: (1) $s\in A$ \& $s\in B$; and (2) $s\not\in A$ \& $s\not\in B$. 
%{\bf (still think this sentence is unnecessary) The latter happens with much higher probability than the former, because $s$ is the \code{XOR} of multiple (distinct) elements and therefore can be considered as a random element. It coincidentally lands in $A\cap B$ with a tiny probability, since the size of the universe $\mathcal{U}$ is typically much larger than $|A\cap B|$.} 
If (1) is the case, we have $s\in B$ whereas $s\not\in A\triangle \hat{D}_1$ (since $s\in \hat{D}_1$ and $s\in A$). Hence $s$ is a distinct element between $A\triangle \hat{D}_1$ and $B$. In the second round, $s$ should be reconciled with high probability. If so, $s$ will be contained in $\hat{D}_2$. This is however a contradiction, since an actual distinct element should not be reconciled ``twice'' (i.e., $s\in \hat{D}_1$ and $s\in \hat{D}_2$) in this multi-round set reconciliation process. From this contradiction, we can deduct that $s$ is not an actual distinct element, but a trouble-causing element incurred by a type (\RN{2}) exception.
%a trouble-causing element (i.e., a fake element). 
Similarly, the same contradiction happens if (2) is the case and the trouble-causing element will be detected.

Alice remove (and save) all the distinct elements that has been reconciled in the first round, denoted as $\hat{D}_1$, and run another round of PBS. More precisely, in the second round, we try to reconcile $A\triangle \hat{D}_1$ and $B$ to obtain the estimated set difference between them, denoted as $\hat{D}_2$, by running the same procedure except for using a different and independent hash function (than $h$) to do hash-partition. 
%instead of reconciling $A$ and $B$ for both (1) removing all the distinct elements that have been reconciled; and (2) keeping all the distinct elements that have not been reconciled, which we will explain shortly. 
Here we use a different and independent hash function to avoid the same type (\RN{1}), (\RN{2}) exceptions happen again. If there are still some distinct elements remaining as verified by the checksum (\autoref{alg:single_round_pbs} of \autoref{step:terminate_condition}), we run another round of PBS (the third round) and try to reconcile $(A\triangle \hat{D}_1)\triangle \hat{D}_2$ and $B$ using another different and independent hash function, so on and so forth, until the set reconciliation is successfully completed as verified by the checksum.
% We use a different hash function for hash-partition in the second round to avoid the same exceptions (i.e., type (\RN{1}), (\RN{2}) events) that happened in the first round happen again. 
%PBS keeps running until the set reconciliation is successfully completed as verified by the checksum. 
The use of independent hash functions in different rounds naturally enables the Markov chain modeling of the reconciliation process, which will be elaborated in \autoref{sec:single_markov}. 


{\bf (previous)} Note that a fake distinct element $s$ (say is incurred in the first round), if is not detected by \autoref{alg:verification},
%{\bf () and does not coincidentally happens to be an actual distinct element (with negligible probability)}
will be mistakenly believed as a distinct element (between $A$ and $B$) and contained in $\hat{D}_1$. This is not an issue because $s$, if is not an actual distinct element, can be easily detected in latter rounds. Note that when $s\not\in A\triangle B$, there are two possible scenarios: (1) $s\in A$ and $s\in B$; and (2) $s\not\in A$ and $s\not\in B$. 
%{\bf (still think this sentence is unnecessary) The latter happens with much higher probability than the former, because $s$ is the \code{XOR} of multiple (distinct) elements and therefore can be considered as a random element. It coincidentally lands in $A\cap B$ with a tiny probability, since the size of the universe $\mathcal{U}$ is typically much larger than $|A\cap B|$.} 
If (1) is the case, we have $s\not\in A\triangle \hat{D}_1$ (since $s\in \hat{D}_1$). That means $s$ is a distinct element between $A\triangle \hat{D}_1$ and $B$ and would be reconciled in the second round with high probability. If this is the case, we have $s\in \hat{D}_2$. This is however a contradiction, since an actual distinct element should not be reconciled ``twice'' (i.e., $s\in \hat{D}_1$ and $s\in \hat{D}_2$) in this multi-round set reconciliation process. From this contradiction, we can deduct that $s$ is a fake distinct element. Similarly, the same contradiction can be detected in (2).  
%Assume in the second round, PBS reconciles $s$ and saves it in $\hat{D}_2$ (happens with high probability), then we find a contradiction that $s$ has been reconciled ``twice'' and is contained in both $\hat{D}_1$ and $\hat{D}_2$. and  is an actual distinct element between $A\triangle \hat{D}$ and $B$. Starting with the second round, PBS will try to reconcile $s$ and eventually ``correct'' this fake distinct element. 

\end{comment}

==> section/multiround_pbs_large_d_copy.tex <==
\subsection{Multi-round Operations}\label{sec:multiround_large_d}

In PBS, the set reconciliation processes of the $g$ group pairs are independent of each other.  
Each group pair runs as many rounds of PBS-for-small-$d$ as needed to reconcile all distinct elements between them. 
Almost every set reconciliation scheme is designed and parameterized to provide the performance guarantee that 
the reconciliation process is successfully completed, {\color{red}{\it i.e.,} correctly reconciles all distinct elements,} with at least a target probability $p_0$.   
In PBS, this guarantee will involve an additional 
parameter $r$ that is the target number of rounds the scheme is allowed to run to reach this target success probability.     More precisely, 
the multi-group-pair multi-round operation of PBS must, with a probability that is at least $p_0$, be successfully completed 
in $r$ rounds.  
%Let $R_i$, $i=1,2,...,g$, be the actual number of rounds for the reconciliation of group pair $i$ to be completed.  Define $R\triangleq\max(R_1,R_2,...,R_g)$.  

Let $R$ be the number of rounds it takes for all $g$ group pairs, and hence the set pair, to be successfully reconciled.
This guarantee can then be succinctly written as $Pr[R\leq r] \ge p_0$.  Intuitively, we can always provide this guarantee by making the values of the two key parameters
$n$ (the size of the parity bitmap) and $t$ (the BCH error-correction capacity) very large, but doing so would 
result in a high communication overhead.  This apparent tradeoff leads us to study the following parameter optimization problem:
Among all parameter settings of $n$ and $t$ that can 
guarantee $Pr[R\leq r] \ge p_0$, which one results in the smallest communication overhead?  


To tackle this optimization problem, we need to first analyze the multi-group-pair
success probability $Pr[R\leq r]$.  
%Roughly speaking, 
The latter boils down roughly (but not exactly as we will explain in \autoref{sec:times2bound}) to analyzing the following single-group-pair success probability.
%analyzing the probability with which a single group pair are successfully reconciled within $r$ rounds.  
%In this section, we introduce a Markov-chain model for analyzing this probability.  
%an analytical framework for solving this much simpler problem that 
%The analysis of this probability can be precisely formulated as follows.    
Consider a single group pair that have
%In the following modeling, we assume that the group pair 
$x$ distinct elements between them before the first round starts.    For the moment, we assume $x \le t$
so that we do not have to worry about the BCH decoding failure.   Our problem is to derive the formula for the probability of the 
following event that we denote as $\{x\!\xrsquigarrow{r}\! 0\}$:  All the $x$ 
distinct elements, and hence the pair, are successfully reconciled in no more than $r$ rounds.   
Solving this problem is the sole topic of \autoref{sec:tail_bound}.  

%We will show in ??? that this formula serves as the basic building block for 
%not only for solving this parameter optimization problem, but for answering two other related questions concerning PBS
%design and parameterization.



% can be considered as imposing a stochastic upper bound on $R$.  

%It is certainly desirable for this random variable $R$ to be as small as possible stochastically.

\begin{comment}
Indeed, as we will explain soon, we can always make $R$ stochastically smaller by increasing the values of the 
two key parameters $n$ and $t$, but doing so would 
also increase the communication overhead.  This apparent tradeoff leads us to study the following optimization problem:
Among all parameter settings of $n$ and $t$ that can 
guarantee $Pr[R\leq r] \ge p_0$, which one results in the smallest communication overhead?  
\end{comment}



 

%for the set reconciliation process of PBS, as will be elaborated in \autoref{sec:tail_bound}. 


\begin{comment}
the probability that all group pairs are successfully reconciled within $r$ round, is at least $p_0$. We call $Pr[R\leq r]$ the {\it success probability} of PBS within $r$ rounds, and $Pr[R_i\leq r]$ the {\it success probability} of group pair $i$ for $i=1,2,...,g$, in the sequel. The optimizable goal itself is to find the optimal parameter settings that minimize the overall communication overhead under the above constraint. Towards this optimizable goal, we propose an analytical framework for the set reconciliation process of PBS, as will be elaborated in \autoref{sec:tail_bound}. 
\end{comment}

% denoted as $R$, is their maximum (i.e., $R=\max(R_1,R_2,...,R_g)$) and also a random variable. 


%$R_i$'s are random variables that are identically distributed, due to the ``symmetry'' of the set reconciliation process of PBS (among different group pairs). The overall number of rounds to reconcile all group pairs, denoted as $R$, is their maximum (i.e., $R=\max(R_1,R_2,...,R_g)$) and also a random variable. 
%Normally, we expect $R$ to be as small as possible, or in other words, all distinct elements to be reconciled within as few rounds as possible. It leads us to an obvious optimization goal: Given the total ``budget'' of communication %overhead, find the optimal parameter settings for PBS that {\it stochastically minimize} $R$. 

% Therefore, different group pairs may take different numbers of rounds to be successfully reconciled. The overall number of rounds to reconcile all group pairs, denoted as $R$, is their maximum. $R$ is a random variable. Normally, we expect $R$ to be as small as possible, or in other words, all distinct elements to be reconciled within as few rounds as possible. It leads us to an obvious optimization goal: Given the total ``budget'' of communication overhead, find the optimal parameter settings for PBS that {\it stochastically minimize} $R$. 
%$R$ is an important metric for PBS. 
% An obvious optimization goal related to $R$ is, given the total ``budget'' of communication overhead, find the optimal parameter settings for PBS that {\it stochastically minimize} $R$. 

%This optimization goal is hard to achieve if not impossible, since $R$ is the maximum of $g$ random variables $\{R_i\}_{i=1}^g$ that are not mutually independent, as we will explain in \autoref{sec:times2bound}. 
%the distribution of each $R_i$ is already depends on many parameters, such as the number of groups $g$, the number of subset pairs per group pair $n$, etc. 

\begin{comment}
Instead, we propose a more optimizable goal, which is roughly the dual of the previous goal. In this optimizable goal, we set a {\it target success probability} $p_0$ combined with a {\it target number of rounds} $r$ to specify its constraint, that is, $Pr[R\leq r]$, the probability that all group pairs are successfully reconciled within $r$ round, is at least $p_0$. We call $Pr[R\leq r]$ the {\it success probability} of PBS within $r$ rounds, and $Pr[R_i\leq r]$ the {\it success probability} of group pair $i$ for $i=1,2,...,g$, in the sequel. The optimizable goal itself is to find the optimal parameter settings that minimize the overall communication overhead under the above constraint. Towards this optimizable goal, we propose an analytical framework for the set reconciliation process of PBS, as will be elaborated in \autoref{sec:tail_bound}. 
\end{comment}

%this more optimizable goal is to find the optimal parameter settings that minimize the overall communication overhead under a specific constraint. The constraint of this goal  we set a {\it target success probability} $p_0$ combined with a {\it target number of rounds} $r$. The constraint of this goal is that $Pr[R\leq r]$, the probability that all group pairs are successfully reconciled within $r$ round, is at least $p_0$. The goal is to find the optimal parameter settings that minimize the overall communication overhead.

% The more optimizable goal is, as follows: Given a {\it target success probability} $p_0$ and a {\it target number of rounds} $r$, find the optimal parameter settings that minimize the overall communication overhead, under the constraint that $Pr[R\leq r]$, the probability that all group pairs are successfully reconciled within $r$ round, is at least $p_0$. 

% This optimization goal is hard to achieve if not impossible. Instead, we propose a more optimizable goal, which is roughly the dual of the previous goal. More specifically, we set a {\it target success probability} $p_0$ combined with a {\it target number of rounds} $r$. The more optimizable goal is, as follows: Given a {\it target success probability} $p_0$ and a {\it target number of rounds} $r$, find the optimal parameter settings that minimize the overall communication overhead, under the constraint that $Pr[R\leq r]$, the probability that all group pairs are successfully reconciled within $r$ round, is at least $p_0$. 

\begin{comment}
The independency of the set reconciliation processes of the group pairs also lead to the ``piecewise reconciliability'' of PBS, that is, the distinct elements are gradually reconciled one round after another. More precisely, in the first round, some group pairs (i.e., each group pair $i$ that satisfies $R_i=1$), and therefore the distinct elements in them, are successfully reconciled. Besides, even for a group pair that has not been successfully reconciled yet in the first round, some of the distinct elements in it (i.e., each distinct element in a subset pair that does not have a type (\RN{1}) or type (\RN{2}) exception) could be reconciled as well. In the second round, another portion of the distinct element (from the ``remaining'') will be reconciled, and so on. This ``piecewise reconciliability'' naturally leads to the following question (performance metric): ``What portion of the distinct elements are expected to be reconciled in the first round, in the second round, etc.''. This question will be thoroughly analyzed in \autoref{sec:piecewise_decodability} using the same analytical framework. 
\end{comment}

%The answer of this question is useful for parameter sett
%The conclusion of this analysis is that, the majority ($>95\%$) of the distinct elements are expected to be reconciled in the first round under typical parameter settings. This conclusion will be used for setting the objective function in parameter settings.

% Note that PBS reconciles the distinct elements gradually round by round: As we described in \autoref{subsec:protocol2}, each group pair is independently reconciled by PBS-for-small-$d$, in which some of the distinct elements in the group pair can be reconciled in each round.

%From this framework, we can obtain a fairly accurate estimation of the success probability within an arbitrary number of rounds under any given parameter settings. Based on it, we can reach the optimizable goal, as we will elaborate in \autoref{sec:parameter_settings}. This analytical framework also enables us to analyze other performance metrics of PBS, as we will show in \autoref{sec:vary_r} and \autoref{sec:piecewise_decodability}.

\begin{comment}
================================
{\bf (moved from the small d case)} Note that the set reconciliation process of the group pairs are independent with each other, and each group pair runs as many rounds of PBS-for-small-$d$ as needed to reconcile all distinct elements in it. Therefore, different group pairs may need different number of rounds to be successfully reconciled. Intuitively, we want all group pairs to be successfully reconciled in only a few rounds (say $3$) with high probability (say $99\%$). Hence, when tuning parameters (to be discussed in \autoref{sec:parameter_settings}), we set a {\it target success probability} $p_0$ combined with a {\it target number of rounds} $r$ as the {\it paramenter setting requirement}, which aims to ensure that the {\it success probability}, the probability that all distinct elements (of all group pairs) are reconciled, within $r$ rounds to be at least $p_0$. 
{\bf Normally, to achieve the same target success probability within fewer rounds (smaller $r$), PBS need more resources (e.g., larger $n$, $t$) for the ideal case happening with higher probability (fewer exceptions happen and need to be handled in later rounds), as we will explain in \autoref{sec:vary_r}.}

{\bf (moved from the small d case)} Although PBS runs as many rounds as needed to reconcile all distinct elements (in each group pair), we want PBS to successfully reconcile all distinct elements in only a few rounds (say $3$) with high probability (say $99\%$). Hence, when tuning parameters (to be discussed in \autoref{sec:parameter_settings}), we set a {\it target success probability} $p_0$ combined with a {\it target number of rounds} $r$ as the {\it paramenter setting requirement}, which aims to ensure that the {\it success probability}, the probability that all distinct elements are reconciled, within $r$ rounds to be larger than $p_0$. 
{\bf Normally, to achieve the same target success probability within fewer rounds (smaller $r$), PBS need more resources (e.g., larger $n$, $t$) for the ideal case happening with higher probability (fewer exceptions happen and need to be handled in later rounds), as we will explain in \autoref{sec:parameter_settings}.}

Like what we did in \autoref{sec:multi-rounds}, we set a paramenter setting requirement on the target success probability $p_0$ of $r$ rounds for all group pairs, which ensures the probability that all group pairs are completely reconciled in $r$ rounds to be larger than $p_0$. The detail about how to set $n$, $g$, and $t$ given such a success probability requirement will be elaborated in \autoref{sec:parameter_settings}. 

we set a {\it target success probability} $p_0$ of $r$ rounds as a paramenter setting requirement, which aims to ensure the probability that all distinct elements are reconciled in $r$ rounds to be larger than $p_0$. This requirement should also ensure the majority of the distinct elements are reconciled in the first round. Use the same example ($d=5, n=255$), on average $4.81$ out of $5$ distinct elements should be reconciled in the first round. So the total communication overhead in all rounds is only slightly larger than ($1.01$ to $1.07$ times of, as we will show in \autoref{fig:per-round-con}) that in the first round. Due to this reason, we use the communication overhead in the first round (described in \autoref{sec:communication_overhead_single_PBS}) to approximate the total communication overhead of all rounds in parameter settings (to be elaborated in \autoref{sec:parameter_settings}.
================================
\end{comment}

==> section/new_paragraphs_xu.tex <==
In a set reconciliation operation, the actual objects (files, database records, etc.) are each hashed into a signature.  Throughout this paper, 
we talk about reconciliating two sets $A$ and $B$ of such signatures.  Once $A ??? B$ is known, Alice will send the objects indexed by 
the signatures in ... to Bob, and Bob will the objects indexed by the signatures in ... to Alice.  

Planned experiment:  Two data sets derived from the 1B-point data set.  Most likely 32-bit signature will not work.  

Resizing the signature size is unthinkable!  Hence it is important to make this signature so large that the probability for resizing is minute.  

We had had this narrative in our original draft that the signature size has to be large enough for each signature to be unique for a large set.
However, for a large set with billions of elements in it, this would lead to a signature size that is at least 64 bits long.  Since every other paper
adopts 32 bits to be the signature size, and a larger signature gives our scheme more advantage over most other schemes except Graphene,
we decided to drop this line of description in our submission, because we wanted to avoid any appearance of our having an ulterior motive to 
increase the signature size.  Graphene will perform better than our scheme when the signature size increases, but as explained in our paper
this advantage can only be exploited when the set difference is large with respect to the two original sets;  when the set differences is small, 
the BF cannot be used, and Graphene becomes an IBF-only scheme and a larger signature size plays to its advantage.  


==> section/pbs_large_d.bk.0719.tex <==
\section{PBS for large \texorpdfstring{\larger\boldmath\MakeLowercase{$d$}}{d}}\label{subsec:protocol2}\label{sec:pbs-for-large-d}

In this section, we continue to assume that the number of distinct elements $d$ is precisely known in advance.
As explained in \autoref{sec:larged}, the PBS-for-small-$d$ scheme described in the previous section is no longer suitable when $d$ is very large, since its BCH decoding computational complexity is 
$O(d^2)$ finite field operations.  Instead, we first hash-partition sets $A$ and $B$ each into $g = d/\delta$ groups, and then apply PBS-for-small-$d$ to each of the $g$ group pairs.  
{\color{red}Here $\delta$ is a small constant, by which we can control the tradeoff between 
the communication and computational overheads of PBS. Generally, the larger $\delta$ is, 
the lower the communication overhead is and the higher the computational overhead. 
We will elaborate how 
$\delta$ controls this tradeoff in~\autoref{app:vs-delta}. 
Nonetheless, we have found that $\delta$=5 is a nice tradeoff point, and hence we fix $\delta$ at $5$ in this paper.}
Since each group pair contains on average $\delta = 5$ distinct elements, the BCH decoding computational complexity per group pair can be considered $O(1)$.  
As a result, the overall BCH decoding computational complexity is $O(d)$ for all $g = d/\delta$ group pairs.  We refer to this PBS-for-large-$d$ scheme as PBS in the sequel except in 
places where this abbreviation would result in ambiguity or confusion.


\begin{comment}
The scheme described above, which we refer to as PBS-for-small-$d$, can also do set reconciliation when $d$ is large. However, the BCH decoding computational complexity in it is $O(d^2)$ of finite field operations, 
%even using the state-of-the-art decoding algorithm~\cite{Dodis_SyndromeEncodingDecoding_2006}, 
which is too expensive for large $d$. To overcome this drawback, we first consistently partition sets $A$ and $B$ each into $d/\delta$ smaller subsets (which we call {\it groups} to distinguish from subsets) for some small integer $\delta$ (say $5$). In this way, each group pair contains roughly $\delta$ distinct elements. Then we apply PBS-for-small-$d$ to reconcile each group pair respectively. The BCH decoding computational complexity of each group pair is roughly $O(\delta^2)$, which can be considered as $O(1)$, since $\delta$ is a small number. As a result, the overall BCH decoding computational complexity is reduced from $O(d^2)$ to $O(d)$. 
\end{comment}

% To overcome this drawback, we use the same technique in \autoref{sec:hash_partition} to hash-partition sets $A$ and $B$ each into $d/\delta$ subsets (which we call {\it groups} to distinguish from subsets) for some small integer $\delta$ (say $5$), so that each of the group pairs contains roughly $\delta$ distinct elements and can be reconciled by PBS-for-small-$d$ respectively. The BCH decoding computational complexity of each group pair is roughly $O(\delta^2)$, which can be considered as $O(1)$, since $\delta$ is a small number. As a result, the overall computational complexity is reduced from $O(d^2)$ to $O(d)$. 
%{\bf In PBS, we set $\delta = 5$. }

%Note that the BCH decoding computational complexity is $O(d^2)$ of finite field operations (in GF($2^{8}$) when $n=255$) using the state-of-the-art decoding algorithm~\cite{Dodis_SyndromeEncodingDecoding_2006}, which is too expensive for large $d$. To overcome this drawback, we first hash-partition sets $A$ and $B$ each into $d/\delta$ subsets (which we call {\it groups} to distinguish from subsets), just like what we did in \autoref{sec:hash_partition}, for some small integer $\delta$ (say $5$), then reconcile each of the group pairs by the PBS we described in \autoref{sec:scheme}. After the partition, each group pair has $\delta$ distinct elements on average. So the BCH decoding computational complexity of each group pair is roughly $O(\delta^2)$, which can be considered as a constant, since $\delta$ is a small number. As a result, the overall computational complexity of PBS is reduced from $O(d^2)$ to $O(d)$. 

%To differentiate from the PBS described in \autoref{sec:scheme}, we refer to it as PBS-basic in this section. 

% \subsection{How to Set Parameters \texorpdfstring{\larger\boldmath\MakeLowercase{$t,n$}}{t,n}}
\subsection{How to Set Parameters {\texorpdfstring{\larger\boldmath\MakeLowercase{$t$}}{t}} and \texorpdfstring{\larger\boldmath\MakeLowercase{$n$}}{n}}\label{subsec:parameterize-n-t}

In PBS (i.e., PBS-for-large-$d$), we have to make some design decisions that we don't have to in PBS-for-small-$d$.  
One of them is how to set the error-correction capacities of the BCH codes used 
for each of the $g$ group pairs. 
Let $\delta_i$, $i=1,2,...,g$, be the number of distinct elements that group pair $i$ have.  
{\color{red}If we knew the precise values of $\delta_1$, $\delta_2$, 
..., $\delta_g$, we would simply set the BCH error-correction capacity 
% (the maximum number of bit errors a BCH codeword is designed to correct) 
for each group pair $i$, which we denote as $t_i$, to $\delta_i$.} This way, each BCH codeword is the shortest possible for the respective task, which minimizes the communication overhead of transmitting these codewords. 
In reality, we do not know the exact value of any $\delta_i$, since it is a random variable with distribution $Binomial(d, 1/g)$ thanks to the hash-partitioning (of $A$ and $B$ each into $g$ groups);  
we only know that $E[\delta_i] = d/g = \delta$  
but that does not help much.
In theory, we can measure $\delta_i$ using a (set difference) cardinality estimation protocol.  However, as will be shown in~\autoref{subsec:ToW}, to obtain such an estimate using the 
best protocol
would incur hundreds of bytes of communication overhead.  In comparison, the ``savings'' on the communication overhead that such an estimate would bring (for the corresponding group pair) 
is only tens of bytes, as we will elaborate next.

In PBS, we set an identical BCH error-correction capability $t$ for all $g$ group pairs.  It intuitively makes sense since random variables $\delta_1$, $\delta_2$, 
..., and $\delta_g$ are identically distributed.  Now the next question is ``How should we set this $t$?".   This is a tricky question because, 
on one hand, if $t$ is too large (say several times larger than $\delta$), then the total size of the BCH codewords is unnecessarily large, resulting in ``wastes" in communication overhead; 
but on the other hand, if $t$ is too small (say equal to $\delta$), then a large proportion of the BCH codewords cannot decode, resulting in considerable additional efforts and costs (i.e., 
``penalties'')
for reconciling the large proportion of affected group pairs.   In \autoref{sec:tail_bound} and \autoref{sec:parameter_settings}, we propose an analytical framework that can be used to
identify the optimal $t$ value that minimizes ``wastes + penalties''.   The optimal $t$ value can range from $1.5\delta$ to $3.5\delta$  depending on how large this $d$ is.
%or $\hat{d}$ (an estimate of $d$ if we do not know its precise value in advance), is.

Based on a similar rationale, we set another parameter for each group pair $i$ to the same value $n$:  Each group pair $i$ is to be partitioned into $n$ subsets, so that the parity bitmaps 
($A[1..n]$ and $B[1..n]$ in PBS-for-small-$d$) for all groups have the same length of $n$ bits.  This $n$ is also a tunable parameter (for optimal PBS performance), since 
the probability for the ideal case (of all distinct elements between a group pair being hashed to distinct subsets) to happen is a function of $n$ and $\delta = 5$.  
As will be elaborated in \autoref{sec:parameter_settings}, our 
analytical framework can also be used for the optimal tuning of $n$.

\begin{comment}


On one hand, $t$ should be larger than or equal to most of $\delta_i$'s for $i=1,2,...,g$, so that most of the group pairs will not encounter BCH decoding failures, and the rest of group pairs (no more than several) only incur negligible ``penalties'' on BCH decoding failures; on the other hand, $t$ should not be too large to incur huge ``waste'' on communication overhead. To find the optimal $t$ that minimizes ``wastes''+``penalties'', we establish an analytical framework for parameter settings, as will be elaborated in \autoref{sec:tail_bound} and \autoref{sec:parameter_settings}. Typically, the optimal $t$ is $1.5$ to $3.5$ times of $\delta$.

Similarly, This randomness of $\delta_i$ also induces a parameter tuning issue on the number of subset pairs in group pair $i$. For the same reason, we set a universal $n$ as the number of subset pairs in each group pair. The analytical framework that is used for finding the optimal $t$ can also be used to find the optimal $n$, as will be elaborated in \autoref{sec:parameter_settings}. 


{\bf (previous) The error-correction capability $t$, defined as the maximum number of errors that the BCH code used by any group pair can correct, is a critical parameter for PBS to perform well. On one hand, if $t$ is too large (say $t=10\delta$), then the communication overhead on transmitting BCH codeword ($t\log n$ bits per group pair) is unnecessarily large; but on the other hand, {\bf if $t$ is too small (say equal to $\delta$), any group pair $i$ could contain more than $t$ distinct elements with a nontrivial probability (i.e., $Pr[\delta_i>t]$ is nontrivial). If so, in the ideal case, the $\delta_i$ distinct elements incur $\delta_i$ bit errors in the BCH codeword, which exceeds the error-correction capability $t$ and a BCH decoding failure happens (we will describe in \autoref{sec:BCH_exception}). if $t$ is too small (say equal to $\delta$), then close to half of the group pairs fail to decode the BCH codeword due to the insufficient error-correction capability, which can result in hefty penalties on BCH decoding failures (to be described in \autoref{sec:BCH_exception}). }
In PBS, we manage to make $t$ as small as possible (so that the communication overhead on transmitting BCH codewords is kept to a minimum) yet pay negligible penalties of BCH decoding failures. }



We continue to assume that the number of distinct elements $d$ is precisely known. Even so, due to the randomness of hash-partition, the number of distinct elements in group pair $i$, denoted as $\delta_i$, is a random variable with mean $\delta$ for $i=1,2,...,g$. Here $g\triangleq d/\delta$ denotes the number of group pairs. This randomness induces a parameter tuning issue on the error-correction capability. On one hand, if the error-correction capability of group pair $i$, denoted as $t_i$, is larger than $\delta_i$, the corresponding BCH codeword is unnecessarily long, which results in ``wastes'' on communication overhead. On the other hand, if $t_i$ is smaller than $\delta_i$, the BCH decoding would fail with high probability, which results in hefty ``penalties'' on BCH decoding failures, as will be described in \autoref{sec:BCH_exception}. Ideally, if $\delta_i$ is precisely known, we can set $t_i$ equal to $\delta_i$ that results neither ``wastes'' nor ``penalties''. However, to estimate each $\delta_i$ with high accuracy requires much larger additional communication overhead than the savings, as we will explain shortly in this section.

%which is roughly $2.5$ times of that in the perfect scenario (when $t$ is roughly $2.5\delta$). Due to this addition
One alternative solution is to estimate each $\delta_i$ and then set $t_i$ to be slightly larger than the estimate of $\delta_i$. It can save considerate communication overhead on transmitting the BCH code. However, to estimate all the $g$ values of $\{\delta_i\}_{i=1}^g$ in high accuracy requires huge additional communication overhead. For instance, estimating each $\delta_i$ requires $288$ bytes of additional communication overhead using the ToW estimator, as we will describe in \autoref{subsec:ToW}. However, the ``savings'' on the communication overhead is much smaller, which is typically no more than a few dozens of bytes.
%However, the ``savings'' on the communication overhead for group pair $i$ is no more than a few dozens of bytes.

\end{comment}


% We continue to assume that the number of distinct elements $d$ is precisely known. Even so, due to the randomness of hash-partition, the number of distinct elements in the $i$-th group pair, denoted as $\delta_i$, is a random variable with mean of $\delta$ for $i=1,2,...,g$, which are not precisely known. Since $\delta_1, \delta_2, ..., \delta_g$ follows the same distribution, it does not make sense to select different parameters for the $g$ group pairs. Hence, we set two universal parameters, $t$ and $n$, for all group pairs, where $t$ is the error-correction capability of the BCH code used for reconciling each group pair, and $n$ is the number of subset pairs in each group pair.

% We continue to assume that the number of distinct elements $d$ is precisely known. Even so, due to the randomness of hash-partition, denoted as $\delta_i$, the number of distinct elements in the $i$-th group pair, is a Binomial random variable with mean of $\delta$ for $i=1,2,...,g$, which cannot be precisely known without a huge amount of additional communication overhead. Since $\delta_1, \delta_2, ..., \delta_g$ follows the identical Binomial distribution, it does not make sense to select different parameters for the $g$ group pairs. Hence, we set two universal parameters, $t$ and $n$, for all group pairs, where $t$ is the error-correction capability of the BCH code used for reconciling each group pair, and $n$ is the number of subset pairs in each group pair.

%To deal with this randomness, we set two global parameters, denoted as $t$, that corresponds to the error-correction capability of the BCH code used for reconciling every group pair. identical no sense or additonal info

%{\bf (modified based on the next paragraph from intro)} 
%{\bf (previous) The error-correction capability $t$, defined as the maximum number of errors that the BCH code used by any group pair can correct, is a critical parameter for PBS to perform well. On one hand, if $t$ is too large (say $t=10\delta$), then the communication overhead on transmitting BCH codeword ($t\log n$ bits per group pair) is unnecessarily large; but on the other hand, {\bf if $t$ is too small (say equal to $\delta$), any group pair $i$ could contain more than $t$ distinct elements with a nontrivial probability (i.e., $Pr[\delta_i>t]$ is nontrivial). If so, in the ideal case, the $\delta_i$ distinct elements incur $\delta_i$ bit errors in the BCH codeword, which exceeds the error-correction capability $t$ and a BCH decoding failure happens (we will describe in \autoref{sec:BCH_exception}). if $t$ is too small (say equal to $\delta$), then close to half of the group pairs fail to decode the BCH codeword due to the insufficient error-correction capability, which can result in hefty penalties on BCH decoding failures (to be described in \autoref{sec:BCH_exception}). }
%In PBS, we manage to make $t$ as small as possible (so that the communication overhead on transmitting BCH codewords is kept to a minimum) yet pay negligible penalties of BCH decoding failures. }

%{\bf (moved from intro, to be removed)} The number of elements in the set difference between any group pair is in general not a constant.  Rather, it is a random variable that has roughly a Poisson distribution with mean $\delta$.  The potential issue arises from dealing with this randomness in setting a global parameter that corresponds to the error-correction capability of the BCH code used for reconciling every group pair.  This parameter, denoted as $t$ (consistent with other literatures on BCH code), is the maximum number of errors that the BCH code used by any group pair can correct, and the size of each such codeword is roughly $8t$ bits (assuming $n = 255$ as explained above). The issue is that, on one hand, if $t$ is too large (say several times larger than $\delta$), then the total size of the BCH codewords, which is the bulk of the extra communication cost, is unnecessarily large; but on the other hand, if $t$ is too small (say equal to $\delta$), then close to half of the BCH codewords cannot decode or worse decode incorrectly (unknown to Alice and Bob), which can result in hefty penalties in the latter case of incorrect decoding.   In PBS, we manage to make $t$ as small as possible (so that the total size of the BCH codewords is kept to a minimum) yet pay negligible penalties of incorrect BCH decoding.
%We will discuss the case that $d_i>t$ in \autoref{sec:BCH_exception}.


% To ensure the error-correction capability $t$ is sufficient (i.e., $t\geq \delta_i$ for $i=1,2,...,g$) for every group pair with high probability, we set $t$ conservatively and leave a sufficient `safety margin' between $t$ and the average number of distinct elements in each group pair $\delta$. 

% Note that the `safety margin' between $t$ and $\delta$ incurs additional communication overhead on transmitting BCH codeword: In the perfect scenario (i.e., $\{d_i\}_{i=1}^g$ is precisely known), the average communication overhead on transmitting BCH codeword per group pair is $\delta\log n$; On the other hand, when we set $t$ to be the error-correction capability for each group pair, the average communication overhead becomes $t\log n$. If we set the `safety margin' to be too large (say $t=10\delta$), it will incur huge additional communication overhead. Due to this reason, we set a moderate `safety margin' that  $t$ in the range from $1.5\delta$ to $3\delta$. 

% {\bf (moved from intro, to be removed)} The number of elements in the set difference between any group pair is in general not a constant.  Rather, it is a random variable that has roughly a Poisson distribution with mean $\delta$.  The potential issue arises from dealing with this randomness in setting a global parameter that corresponds to the error-correction capability of the BCH code used for reconciling every group pair.  This parameter, denoted as $t$ (consistent with other literatures on BCH code), is the maximum number of errors that the BCH code used by any group pair can correct, and the size of each such codeword is roughly $8t$ bits (assuming $n = 255$ as explained above). The issue is that, on one hand, if $t$ is too large (say several times larger than $\delta$), then the total size of the BCH codewords, which is the bulk of the extra communication cost, is unnecessarily large; but on the other hand, if $t$ is too small (say equal to $\delta$), then close to half of the BCH codewords cannot decode or worse decode incorrectly (unknown to Alice and Bob), which can result in hefty penalties in the latter case of incorrect decoding.   In PBS, we manage to make $t$ as small as possible (so that the total size of the BCH codewords is kept to a minimum) yet pay negligible penalties of incorrect BCH decoding.
%We will discuss the case that $d_i>t$ in \autoref{sec:BCH_exception}.

% Hence, we can no longer set the error-correction capability of the BCH code for each group pair based on the exact number of distinct element in it, as we did in \autoref{sec:scheme}. Instead, we set a conservative error-correction capability $t$ (say $2.5\delta$) for all group pairs, which is sufficient for them (i.e., $t\geq d_i$ for $i=1,2,...,g$) with high probability. We will discuss the case that $d_i>t$ in \autoref{sec:BCH_exception}.


% ===============================
% To differentiate from the PBS described in \autoref{sucsec:our-scheme}, we refer it as PBS-basic in this section. Note that the BCH decoding computational complexity is $O(d^2\log ^2 n)$, which is $\Omega(d^2\log^2 d)$ when $n=\Omega(d^2)$, with the state-of-the-art decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019}. It is too large in PBS-basic for large $d$. To overcome this drawback and generalize PBS-basic for large $d$, we partition sets $A$ and $B$ each into $d/\delta$ subsets (which we call {\it groups} to distinguish from subsets) for some small integer $\delta$ (say $5$) and reconcile the $d/\delta$ group pairs respectively using PBS-basic. After this partition, each group has $\delta$ distinct elements on average. The BCH decoding computational complexity of each group pair can be considered as $O(1)$, since $\delta$ is a small number. As a result, the overall computational complexity of PBS is reduced from $O(d^2\log ^2 n)$ to $O(d)$. 

% % To differentiate from the PBS described in \autoref{sucsec:our-scheme}, we refer it as PBS-basic in this section. PBS-basic is not suitable for large $d$ for two reasons: First, its communication overhead is asymptotically $O(d\log n)\!=\!O(d\log d)$ (since $n=\Omega(d^2)$), which is not asymptotically optimal. Second, the decoding computational complexity is proportional to $d^2$ with the state-of-the-art decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} for BCH codes, which is too high when $d$ is large. To overcome these two drawbacks, we use a simple algorithmic trick to (1) reduce the communication overhead from $O(d\log d)$ to $d\log u \!+\! O(d)$; (2) reduce the decoding computational complexity from $O(d^2)$ to $O(d)$. 

% Now, we describe the generalized PBS in details: In the first step, we hash-partition $A$ and $B$ (by some hash function $h_1(\cdot)$) into $g$ group pairs, just like what we did in \autoref{sucsec:our-scheme}. The objective of this partition is however different: In \autoref{sucsec:our-scheme}, we aim to ensure each subset pair contains at most $1$ distinct element (i.e., the ideal case) with high probability; Here we aim to make each group pair contains roughly $\delta$ distinct elements for some small constant $\delta$ (say $5$) by setting $g=d/\delta$. 
% %To differentiate the $g$ subset pairs here from those in \autoref{sec:hash_partition}, we call them the $g$ {\bf groups} in the sequel. 
% In the second step, we just apply PBS-basic (described in \autoref{sucsec:our-scheme}) to reconcile each group pair and obtain the distinct elements. 
% ================================

% To differentiate from the PBS described in \autoref{sucsec:our-scheme}, we refer it as PBS-basic in this section. When $d$ is large (more than several), we hash-partition set $A$ and $B$ into groups, such that each group pair contains $\delta$ distinct elements on average for small $\delta$ (say $5$), as described in \autoref{sec:larged}. Then each group pair can be reconciled by PBS-basic.

% When describing the PBS-basic in \autoref{sucsec:our-scheme}, we assume that the number of distinct elements is precisely known. We set the error-correction capability of the BCH code (denoted as $t$) just enough to correct $d$ errors (i.e., $t=d$). However, due to the randomness of hash-partition, $d_i$, the number of distinct elements in the $i^{th}$ group pair, is a Binomial random variable $Binomial(d,1/g)$ with expectation of $\delta$ $(=d/g)$ for $i=1,2,...,g$, which cannot be precisely known without a huge amount of additional communication overhead. Hence, we can no longer set the error-correction capability of the BCH code for each group pair based on the exact number of distinct element in it, as we did in \autoref{sucsec:our-scheme}. Instead, we set a universal error-correction capability $t$ (say $2.5\delta$) for all group pairs, which is sufficient for all group pairs (i.e., $t\geq d_i$ for $i=1,2,...,g$) with high probability. We will discuss the case that $d_i>t$ in \autoref{sec:BCH_exception}.

%This assumption in general does not hold: 
% Let $d_i$ denote the number of distinct elements in Group $i$. Due to the property of hash-partition, each $d_i$ is a Binomial random variable $Binomial(d,1/g)$ with expectation of $\delta$ $(=d/g)$. Even if $d$ is precisely known, each $d_i$ is not. To ensure the error-correction capability $t$ is sufficient for each group (i.e., $d_i\leq t$) with high probability, we leave some safety margin for the randomness of $d_i$ and conservatively set $t$ roughly $2.5\delta$ (the factor $2.5$ varies depend on other parameters, which will be discussed in \autoref{sec:parameter_settings}), so that $Pr[d_i>t]$ is tiny. We will discuss the case that $d_i>t$ in \autoref{sec:BCH_exception}.

% Note that the `safety margin' between $t$ and $\delta$ incurs additional communication overhead on transmitting BCH codeword: In the perfect scenario (i.e., $\{d_i\}_{i=1}^g$ is precisely known), the average communication overhead on transmitting BCH codeword per group pair is $\delta\log n$; On the other hand, when we set $t$ to be the error-correction capability for each group pair, the average communication overhead becomes $t\log n$. If we set the `safety margin' to be too large (say $t=10\delta$), it will incur huge additional communication overhead. Due to this reason, we set a moderate `safety margin' that  $t$ in the range from $1.5\delta$ to $3\delta$. 


\smallskip
\noindent
{\bf Communication Overhead Per Group Pair.} 
%\subsection{Communication Cost Per Group Pair}\label{sec:communication_overhead_single_PBS}
%To correct $d$ bit errors, the length of the net-codeword only is no more than $d\log n$ bits. 
Here we analyze the total communication overhead of the first round of PBS.  Since the vast majority of distinct elements are discovered and reconciled in the first round, 
as will be shown in \autoref{sec:piecewise_decodability}, it represents the vast majority (over $95\%$) of that over all rounds.  
For each group pair $i$, the communication overhead (of running PBS-for-small-$d$ on this pair) in the first round contains the following four components: (1) the BCH codeword that is $t\log n$ bits long; (2) the $\delta_i$ ``bit error locations'' whose total length is $\delta_i\log n$ bits; (3) the  $\delta_i$ \code{XOR} sums whose total length is $\delta_i\log |\mathcal{U}|$ bits; and (4) the checksum that is $\log |\mathcal{U}|$ bits long. Hence the average communication overhead of PBS per group pair in the first round is 


%Formula \autoref{eq:communication_overhead} also roughly equals to the average communication overhead of PBS per group pair in all rounds, since the bulk of the communication overhead %happens in the first round, .

%Since each group pair is reconciled by \autoref{alg:single_round_pbs} in the first round, the communication overhead of a group pair $i$ in the first round corresponds to the steps in 
%\autoref{alg:single_round_pbs}, which consists of the following four components: 

\begin{comment}
For each group pair $i$, There are four components 
\begin{itemize}
	\setlength\itemsep{0.1em}
	\item The BCH codeword that is $t\log n$ bits long
	%(\autoref{step:BCH_encode} in \autoref{alg:single_round_pbs});
	\item The subset pair indices (\autoref{step:send_xor} in \autoref{alg:single_round_pbs}) that are $\delta_i\log n$ bits long;
	\item The bitwise \code{XOR} sums (\autoref{step:send_xor} in \autoref{alg:single_round_pbs}) that are $\delta_i\log |\mathcal{U}|$ bits long;
	\item The checksum (\autoref{step:terminate_condition} in \autoref{alg:single_round_pbs}) that is $\log |\mathcal{U}|$ bits long;
\end{itemize}
\end{comment}



\begin{equation}\label{eq:communication_overhead}
t\log n + \delta\log n +\delta \log |\mathcal{U}|+\log |\mathcal{U}|
\end{equation}

% \begin{itemize}
% 	\setlength\itemsep{0.1em}
% 	\item the BCH codeword that is $t\log n$ bits long;
% 	%(\autoref{step:BCH_encode} in \autoref{alg:single_round_pbs});
% 	\item the $\delta_i$ ``bit error locations" whose total length is $\delta_i\log n$ bits;
% 	\item the  $\delta_i$ \code{XOR} sums whose total length is $\delta_i\log |\mathcal{U}|$ bits;
% 	\item the checksum that is $\log |\mathcal{U}|$ bits long.
% \end{itemize}

% %Hence the total communication overhead in the first round over all $g$ groups is  $gt\log n + d\log n + d \log |\mathcal{U}|+ g\log |\mathcal{U}|$.
% %Since $\delta_i$ is a random variable with mean $\delta$ for $i=1,2,...,g$, 
% Hence the average communication overhead of PBS per group pair in the first round is 
% \begin{equation}\label{eq:communication_overhead}
% t\log n + \delta\log n +\delta \log |\mathcal{U}|+\log |\mathcal{U}|
% \end{equation}

%Formula \autoref{eq:communication_overhead} also roughly equals to the average communication overhead of PBS per group pair in all rounds, since the bulk of the communication overhead happens in the first round, as will be explained in \autoref{sec:piecewise_decodability}.

\begin{comment}
{\bf (previous)} the BCH codeword $\xi_A$ in \autoref{step:BCH_encode}; (2) the subset pair indices $i_1,i_2,...,i_d$ in \autoref{step:trivial_reconcile}; (3) the bitwise \code{XOR} sums of sets $B_{i_1}, B_{i_2},...,B_{i_d}$ of $d\log |\mathcal{U}|$ bits in \autoref{step:trivial_reconcile}; and (4) transmit the $32$-bit checksum of $B$ (i.e., $c(B)$) from Bob to Alice for precomputing $c(A\triangle B)$ in \autoref{step:terminate_condition}. These four components contribute roughly (1) $d\log n$ bits (recall that to ``correct'' $d$ bit errors, the length of the BCH codeword is no more than $d\log n$ bits); (2) $d\log n$ bits; (3) $d\log |\mathcal{U}|$ bits; and (4) $32$ bits respectively to the overall communcation overhead of \autoref{alg:single_round_pbs}. 
\noindent {\bf Communication overhead of PBS Per Group Pair in the first round:} Same as PBS-for-small-$d$, the communication overhead of PBS per group pair in the first round also consists of the four components described in \autoref{sec:communication_overhead_single_PBS}. The expectation of the communication overhead of each component equals to the corresponding component of PBS-for-small-$d$ when $d=\delta$, except for the BCH codeword, which is $t\log n$ bits as we described earlier. The communication overhead of PBS per group pair in the first round on average is roughly
\end{comment}

% \begin{equation}\label{eq:communication_overhead}
% t\log n + \delta\log n +\delta \log |\mathcal{U}|+32
% \end{equation}

% {\bf (previous)} Readers may wonder if we can reduce this additional communication overhead by using some technique to estimate $\{d_i\}_{i=1}^g$ (e.g., ToW estimator in \autoref{subsec:ToW}), so that we can set the error-correction capability of each group more wisely and save some waste on the safety margin. However, to achieve that, the estimation on $\{d_i\}_{i=1}^g$ must be in extremely high precision (since $\{d_i\}_{i=1}^g$ are small numbers with mean of $\delta$), which incurs much larger additional communication overhead than the savings. Due to the same reason (i.e., estimate $\{d_i\}_{i=1}^g$ is costly), we set the number of subset pairs for each group pair to be all equal (denoted as $n$). 
%based on $\delta$ ($n=\Omega(\delta^2)$). 

% {\bf (moved from the small d case)} Note that the set reconciliation process of the group pairs are independent with each other, and each group pair runs as many rounds of PBS-for-small-$d$ as needed to reconcile all distinct elements in it. Therefore, different group pairs may need different number of rounds to be successfully reconciled. Intuitively, we want all group pairs to be successfully reconciled in only a few rounds (say $3$) with high probability (say $99\%$). Hence, when tuning parameters (to be discussed in \autoref{sec:parameter_settings}), we set a {\it target success probability} $p_0$ combined with a {\it target number of rounds} $r$ as the {\it paramenter setting requirement}, which aims to ensure that the {\it success probability}, the probability that all distinct elements (of all group pairs) are reconciled, within $r$ rounds to be at least $p_0$. 
% {\bf Normally, to achieve the same target success probability within fewer rounds (smaller $r$), PBS need more resources (e.g., larger $n$, $t$) for the ideal case happening with higher probability (fewer exceptions happen and need to be handled in later rounds), as we will explain in \autoref{sec:vary_r}.}

% {\bf (moved from the small d case)} Although PBS runs as many rounds as needed to reconcile all distinct elements (in each group pair), we want PBS to successfully reconcile all distinct elements in only a few rounds (say $3$) with high probability (say $99\%$). Hence, when tuning parameters (to be discussed in \autoref{sec:parameter_settings}), we set a {\it target success probability} $p_0$ combined with a {\it target number of rounds} $r$ as the {\it paramenter setting requirement}, which aims to ensure that the {\it success probability}, the probability that all distinct elements are reconciled, within $r$ rounds to be larger than $p_0$. 
% {\bf Normally, to achieve the same target success probability within fewer rounds (smaller $r$), PBS need more resources (e.g., larger $n$, $t$) for the ideal case happening with higher probability (fewer exceptions happen and need to be handled in later rounds), as we will explain in \autoref{sec:parameter_settings}.}

%This success probability (within $r$ rounds) is also the expected value of the {\it success rate} of PBS, which is defined as the number of `successful' experiments (all distinct elements are successfully reconciled within $r$ rounds) divided by the total number of experiments. 

%The requirement above should also ensure the majority of the distinct elements are reconciled in the first round. 
% Note that PBS reconciles the distinct elements gradually round by round. The distinct elements that have been reconciled in the first round are no longer needed to be reconciled again in later rounds. This is the ``piecewise decodability'' mentioned in \autoref{sec:intro_oursolution}. The requirement above also ensures the majority of the distinct elements are reconciled in the first round, as we will show in \autoref{sec:piecewise_decodability}. Therefore, the majority of the overall communication overhead happens in the first round. In other words, the overall communication overhead of all rounds is only slightly larger than ($1.01$ to $1.07$ times of) that in the first round. Due to this reason, we use the communication overhead in the first round (described in \autoref{sec:communication_overhead_single_PBS}) to approximate the overall communication overhead of all rounds in parameter settings (to be elaborated in \autoref{sec:parameter_settings}.


% Like what we did in \autoref{sec:multi-rounds}, we set a paramenter setting requirement on the target success probability $p_0$ of $r$ rounds for all group pairs, which ensures the probability that all group pairs are completely reconciled in $r$ rounds to be larger than $p_0$. The detail about how to set $n$, $g$, and $t$ given such a success probability requirement will be elaborated in \autoref{sec:parameter_settings}. 

% we set a {\it target success probability} $p_0$ of $r$ rounds as a paramenter setting requirement, which aims to ensure the probability that all distinct elements are reconciled in $r$ rounds to be larger than $p_0$. This requirement should also ensure the majority of the distinct elements are reconciled in the first round. Use the same example ($d=5, n=255$), on average $4.81$ out of $5$ distinct elements should be reconciled in the first round. So the total communication overhead in all rounds is only slightly larger than ($1.01$ to $1.07$ times of, as we will show in \autoref{fig:per-round-con}) that in the first round. Due to this reason, we use the communication overhead in the first round (described in \autoref{sec:communication_overhead_single_PBS}) to approximate the total communication overhead of all rounds in parameter settings (to be elaborated in \autoref{sec:parameter_settings}.

% Note that this safety margin incurs additional communication overhead on transmitting BCH codeword: In the perfect scenario (i.e., $\{d_i\}_{i=1}^g$ is precisely known), the average communication overhead on transmitting BCH codeword per group is $\delta\log n$; On the other hand, when we set $t$ to be the error-correction capability for each group, then the average overhead becomes $t\log n$, which is roughly $2.5$ times of that in the perfect scenario (when $t$ is roughly $2.5\delta$). Readers may wonder if we can reduce this additional communication overhead by using some technique to estimate $\{d_i\}_{i=1}^g$ (e.g., ToW estimator in \autoref{subsec:ToW}), so that we can set the error-correction capability of each group more wisely and save some waste on the safety margin. However, to achieve that, the estimation on $\{d_i\}_{i=1}^g$ must be in high precision, which requires a much higher communication overhead than the savings.

% Although PBS may need to run many rounds to reconcile all distinct elements, the communication overhead mostly happens in the first round, since the majority of the distinct elements should be reconciled in the first round. Use the same example ($d=5, n=255$), on average $4.81$ out of $5$ distinct elements should be reconciled in the first round. So the total communication overhead in all rounds is only slightly larger than ($1.01$ to $1.07$ times of, to be shown in \autoref{fig:per-round-con}) that in the first round. Due to this reason, we use the communication overhead in the first round (described in \autoref{sec:communication_overhead_single_PBS}) to approximate the total communication overhead (all rounds) in parameter settings (to be elaborated in \autoref{sec:parameter_settings}).

%For the moment, we assume no ``fake'' distinct element in type (\RN{2}) subset pairs fails to be detected, which happens with overwhelming probability as explained in \autoref{subsec:exception_hash_partition}. Then 

% PBS reconciles the distinct elements gradually round by round. This is the ``piecewise decodability'' mentioned in \autoref{sec:intro_oursolution}. We use the following example to describe it in details: 
% Given two sets with $10$ distinct elements, in the first round, PBS tries to reconcile the $10$ distinct elements and say $6$ out of the $10$ distinct elements are successfully reconciled. Then the $6$ reconciled distinct elements are removed and PBS tries to reconcile the remaining $4$ distinct elements in the second round. Say $2$ out of the $4$ remaining distinct elements are successfully reconciled, and that leaves $2$ remaining distinct elements to be reconciled in the third round, so on so force. 
% % Given two sets $A$, $B$ with $10$ distinct elements, in the first round, PBS hashes them into $7$ distinct subset pairs. $6$ distinct elements are hashed into $6$ distinct subset pairs, and the other $4$ distinct elements are hashed into the same subset pair. Then the former $6$ distinct elements are successfully reconciled in the first round and the later $4$ distinct elements remain to be reconciled in the second round, which are hashed into $3$ distinct subset pairs (under a different hash function). $2$ remaining distinct elements are hashed into $2$ distinct subset pairs, and the other $2$ remaining distinct elements are hashed into the same subset pair. Then the former $2$ remaining distinct elements are successfully reconciled in the second round and the later $2$ remaining distinct elements remain to be reconciled in the third round, so on so force. 
% The dynamics of the number of remaining distinct elements (i.e., $10\leadsto 4\leadsto 2\leadsto \cdots$ in the example) is in nature a Markov chain, which will be elaborated and analyzed in \autoref{sec:single_markov} to derive a tight tail bound of the probability that all distinct elements are reconciled in $r$ rounds. 

%, which we will show in \autoref{subsec:mini-partition}.

% The same algorithmic trick can also be implemented in PinSketch~\cite{Dodis_PinSketch_2008} to reduce it computational complexity from $O(d^2)$ to $O(d)$. However, it will encounter the same randomness problem and have to set up a safety margin on the error-correction capability. This safety margin will incur much more communication overhead on PinSketch than on our scheme: Considering the average communication overhead per group, in our scheme, this overhead can be expressed as $t\log n+\delta\log n+\delta \log u+32$, in which $t\log n$ accounts for the BCH codeword, $\delta\log n$ accounts for the index of the subset pairs, $\delta \log u$ accounts for the bitwise \code{XOR} in \autoref{alg:trivial_case}, and $32$ accounts for the $32$-bit CRC in \autoref{proto:multirounds}. In PinSketch, this overhead increases from $O(\delta\log u)$ (optimal) to $O(t\log u)$ (PinSketch does not need to transmit bitwise \code{XOR}) if it uses the same algorithmic trick. Use the same example in \autoref{sec:intro}, when $\delta=5, n=255, u=2^{32}, t=2.5\delta$, the overhead of PinSketch using the trick is $2.5$ times of the optimal, while that of our scheme is $2.075$ times of the optimal (as we introduced in \autoref{sec:intro_oursolution}). That means our scheme has a lower communication overhead than PinSketch if they both use the algorithmic trick. Furthermore, as the signiture size $\log u$ increases, the advantage of our scheme over PinSketch becomes more significantly, which we will show in \autoref{subsec:mini-partition}.

% In PinSketch, each bit encodes only a single element in the universe, so the size of the bitmap is equal to the size of the universe.  
% For example, in the set reconciliation problem we usually assume each element is ``indexed" by a $32$-bit-long (hash) signature, so the universe contains a total of $2^{32}$ elements. In this case, the bitmap encoding for any set in PinSketch is $2^{32}$ bits long, and the Galois field involved in its BCH decoding is the ``$32$-bit-wide" $GF(2^{32})$.  In contrast, as explained earlier, in PBS 
% %since each bit encodes the oddness or evenness of the cardinality of a subset,   
% the size $n$ of a bitmap is dependent only on $d$, and not on the size of the universe or on the cardinality of the set the bitmap encodes.   For example, as shown in the example above, $n = 255$ is large enough for $d = 5$.  In this case, the BCH decoding operates in the much shorter
% ``8-bit-wide" $GF(2^{8})$.  This shorter ``width" alone in theory translates into roughly $16$ times shorter BCH decoding time, which as will be explained in~\ref{} grows quadratically with the ``width" of the underlying Galois field.  This shorter ``width" also implies four times shorter BCH codeword in PBS than in PinSketch, resulting in lower communication complexity as will be shown in~\autoref{}.

% Note that our scheme only takes 1 round trip delay to both identify the $d$ subset pairs and reconcile them: In the first half, Bob computes and sends PBS to Alice. Then Alice locally identifies the $d$ subset pairs and then initiates the reconciliation ({\it i.e.,} \autoref{alg:trivial_case}) for them, {\it i.e.,} computes the bitwise \code{XOR} of the corresponded $d$ subsets. In the second half, Alice sends the bitwise \code{XOR} of the $d$ subsets with their indexes to Bob. Then Bob can compute the set difference $A\triangle B$ locally.


% We can certainly use some communication-efficient technique to estimate $d_i$ (e.g., \autoref{subsec:ToW}). However, to obtain $d_i$ precisely will require a communication cost almost as large as to reconcile Group $i$. So instead of obtaining $d_i$ and set $c_i$ (i.e., the error-correction capability of Group $i$) equal to $d_i$, we leave the randomness of $d_i$ and set $c_i$ neither too conservative, nor too libertive in the following sense: (1) $c_i$ is not too big (conservative, i.e., $10\delta$) to make the total size of PBS unnecessarily large and incur too much extra communication overhead; (2) $c_i$ is not too small (libertive, i.e., $\delta$) to incur a high probability of insufficient decode capability, which can result in hefty penalties in the latter case of incorrect decoding (will be elaborated in \autoref{sec:BCH_exception}). In our scheme, we set $c_i$ to be $2-3$ times of $\delta$, which will be shown in \autoref{sec:tail_bound} that it is just enough to make the probability of decode failure very small. Meanwhile, we set the error-correction capability of each group ($c_1,c_2,...,c_k$) to be all equal and denote it as $c$. 

%Since the decoding capacity $t$ and the number of subset pairs for each group $n$ are both small constants independent of $d$, therefore, the communication overhead per group is $t\cdot\log n \!=\!O(1)$, which implies a total communication overhead of $O(d)$. Similarly, the total decoding computational complexity is also $O(d)$. 

% \subsection{Exception Handling}\label{sec:exceptions}

% \subsubsection{Exception Handling on Hash-Partition}\label{subsec:exception_hash_partition}

% As we have described in \autoref{sec:hash_partition}, the ideal case does not always happen, which means some subset pair may contain more than 1 distinct elements and cannot be successfully reconciled by \autoref{alg:trivial_case}. Due to the parity encoding, we can classify such subset pair into the following two scenarios:

% \begin{itemize}
%     \item Scenario 1: If a subset pair $(A_i, B_i)$ contains even number ($\geq 2$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be the same and our scheme will not reconcile the subset pair. Hence, the distinct elements in the subset pair will not be reconciled;
%     \item Scenario 2: If a subset pair $(A_i, B_i)$ contains odd number ($\geq 3$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be different and our scheme will reconcile the subset pair using \autoref{alg:trivial_case}. However, as we described in \autoref{subsec:protocol0}, when a subset pair contains more than 1 distinct elements, \autoref{alg:trivial_case} will output the bitwise \code{XOR} of them as the `distinct element', which is not a real distinct element with high probability;
% \end{itemize}

% In both scenarios, the distinct elements in the subset pair cannot be reconciled. Even worse, in the second scenario, a false-positive could happen (i.e., the output of \autoref{subsec:protocol0} is not a real distinct element). For example, if subset pair $(A_i, B_i)$ contains $3$ distinct elements $s_1, s_2, s_3$, then the output of \autoref{alg:trivial_case} is $\tilde{s}_4=s_1\oplus s_2\oplus s_3$, which is normally not a distinct element. The good thing is, the probability of the false-positive is extremely small for small $d$. For instance, if $d=5$ and $n=255$, the probability of the false-positive is $7.6\times 10^{-6}$, which is very small. To further reduce the chance of false-positives, we add a verification step at the end of \autoref{subsec:protocol0} to check whether the output of \autoref{subsec:protocol0} $s$ is a real distinct element or not. The verification step works as follows: Given the output $s$ of subset pair $(A_i,B_i)$, if $s\in\mathcal{U}_i$ (i.e., $h(s)=i$), we consider $s$ as a real distinct element; Otherwise, we consider $s$ as an incorrect output and discard it. 

% Note that if $s$ is a real distinct element of $(A_i,B_i)$, $s$ must be in sub-universe $\mathcal{U}_i$. However, if $s$ is the bitwise \code{XOR} of the distinct elements in $(A_i,B_i)$ (i.e., the second scenario happens), $s$ could be in any sub-universe other than $\mathcal{U}_i$. In fact, if we assume the hash-partition described in \autoref{sec:hash_partition} hashes the elements of $\mathcal{U}$ uniformly, independently, and randomly into $n$ sub-universes, the output $s$ in the second scenario will be in a different sub-universe $\mathcal{U}_j (j\neq i)$ with a high probability of $1-\frac{1}{n}$. Hence, this verfication method can further reduce the probability of false-positives by a factor of $\frac{1}{n}$. Use the same example (i.e., $d=5$, $n=255$), the probability is reduced from $7.6\times 10^{-6}$ to $3\times 10^{-8}$ by this verification method. 

% In some super critical cases (i.e., no false-positive is allowed), we can use a more powerful verification method to completely eliminate false-positives. That is, to check if the output $s$ exists in exactly one of the two sets (i.e., $s\in A\setminus B$ or $s\in B\setminus A$). To do so, Bob transmits $s$ along with an identification bit $\mathbb{1}_{\{s\in B\}}$ to Alice, then Alice checks if $s$ . This method verification costs $d(\log u+1)$ bits of additional communication overhead. In most applications, rigorously $0\%$ probability of false-positives is unnecessary and the probability of the former verification method is small enough, so we use the former verfication method in our evaluation. Based on our observation, the false-positive does not happen even once in our evaluation using the former verfication method.

\subsection{Exception Handling on BCH Decoding}\label{sec:BCH_exception}

Recall that in PBS-for-small-$d$ we need to handle two types of exceptions:  type (\RN{1}) and type (\RN{2}). 
In PBS-for-large-$d$, we have another exception to worry about.
% This exception arises when $\delta_i$, the number of distinct elements between group pair $i$, 
% is larger than $t$, the universal BCH error-correction capability (for every group pair).  
{\color{red}This exception arises when the number of bit positions where bitmaps $A$ and $B$ in~\autoref{alg:single_round_pbs} 
differ is larger than $t$, the universal BCH error-correction capability (for every group pair).
%Note that $\delta_i$ (the number of distinct elements between group pair $i$)
%being larger than $t$ (the universal BCH error-correction capability) is only a necessary condition for this 
%exception to happen in reconciling this group pair, 
%since type (\RN{1}) and/or type (\RN{2}) exceptions could result in that the 
%number of different bits between the corresponding two bitmaps is no more than $t$. 
% In this case, 
When this exception happens,} the BCH decoding would fail (when executing \autoref{step:BCH_decode} in \autoref{alg:single_round_pbs}) 
and the decoder would report a failure.
With $t$ appropriately parameterized as explained earlier, this exception should happen with a small probability to any group pair. 
For example, when $d=\num{1000}$, $\delta=5$ (so that $g=d/\delta=200$), and $t$ is set to the 
optimal value of $13$ ($=2.6\delta$), the probability for this exception to happen to any group pair
is only $6.7\times 10^{-4}$. 

To handle this type of exceptions, we further hash-partition each trouble-causing group pair (whose BCH decoding has failed) 
into $3$ sub-group-pairs and reconcile each of them using PBS-for-small-$d$. 
With this three-way split, with an overwhelming probability, each sub-group-pair should contain no more than $t$ distinct elements and its BCH decoding operation should be 
successful in the next round.  For example, when $\delta=5$ and $t=13$ (same as in the example above), 
the conditional (upon the event $\{\delta_i>t\}$, which happens with probability $6.7\times 10^{-4}$ as 
just explained) probability for any sub-group-pair to contain more than $t$ distinct elements is only $9.5\times 10^{-10}$. 
{\color{red} We use a three-way split here because a two-way split would result in a much higher conditional probability for this event:
%splitting a trouble-causing group pair into only $2$ sub-group-pairs cannot achieve such an 
%overwhelming probability to guarantee each sub-group-pair has no more than $t$ distinct elements: 
In the same example above ($\delta=5$ and $t=13$), this conditional probability becomes $0.0012$.} 
All said, if necessary, a trouble-causing sub-group-pair will be further split three-way.

{\color{red}
As explained earlier, the ultimate gatekeeper for ensuring the correctness of set reconciliation is the checksum verification step, which
in this case (of large $d$) is applied to each group pair.  BCH decoding exceptions alone, or in combination with type I or II exceptions, may only 
delay the inevitable eventual correct reconciliation of $A$ and $B$, as long as a  false checksum verification event does not happen.
}

\begin{comment}
{\color{red}
Like type (\RN{1}) and type (\RN{2}) exceptions, this exception will not result in reconciliation error, but more 
rounds. From~\autoref{thm:corrctness}, we have the following corollary concerning the correctness of PBS-for-large-d. 

\begin{corollary}
Assuming that the verification in~\autoref{step:terminate_condition} of~\autoref{alg:single_round_pbs} is always correct. 
If PBS-for-large-d terminates, the result, {\it i.e.,} the union of the set difference obtained for each group pair, 
is equal to $A\triangle B$.
\end{corollary}

\noindent
{\bf Remarks.}
The number of rounds, for PBS to correctly reconcile all distinct elements, is small (with overwhelming probability), 
since, as explained earlier, the probability that an exception happens is quite low.  
For example, as shown in~\autoref{app:completed-rounds}, 
even when $d$ is as large as $10^5$, in all our experimental instances, 
the number of rounds (for PBS-for-large-d, which we will describe in~\autoref{sec:pbs-for-large-d}) is no mare than $3$ and 
in $81.8$\% of those instances, it is only $2$. 
}
\end{comment}

\begin{comment}
There is an additional type of exceptions that arise only from setting the universal error-correction capability $t$. That is, when $\delta_i$, the number of distinct elements in group pair $i$, is larger than $t$, the parity bitmaps $A[1..n]$ and $B[1..n]$ could differ at more than $t$ bit positions (e.g., in the ideal case, $A[1..n]$ and $B[1..n]$ differ at exactly $\delta_i$ bit positions), which exceeds the error-correction capability $t$. If so, the BCH decoding fails in \autoref{step:BCH_decode} in \autoref{alg:single_round_pbs} and the decoder reports a failure. This exception happens with a small probability in each group pair: For example, when $d=1000$, $\delta$ is set to $5$ (so that $g=d/\delta=200$), and $t$ is set to $13$ ($2.6$ times of $\delta$), the probability that this exception happens is only $6.7\times 10^{-4}$. 

Note that $\delta_i$ is a Binomial random variable with mean $\delta$, $t$ is typically $1.5$ to $3.5$ times of $\delta$. Even conditioned upon the event $\{\delta_i>t\}$, $\delta_i$ should be only slightly larger than $t$ with high probability. Hence, after partitioning the $\delta_i$ distinct elements into $3$ sub-group-pairs, each of them should have no more than $t$ distinct elements with overwhelming probability. For example, when $\delta=5$, $t=13$ $(2.6\delta)$, the probability that some sub-group-pair contains more than $t$ distinct elements conditioned upon the event $\{\delta_i>t\}$ is only $9.5\times 10^{-10}$. 
\end{comment}

% The exceptions that happens when the error-correction capability $t$ is sufficient have been discussed and handled in \autoref{subsec:exception_hash_partition} and \autoref{sec:multi-rounds}. In this section, we only discuss the exceptions that are caused by insufficient error-correction capability. That is, when $\delta_i$ (i.e., the number of distinct elements in group pair $i$) is larger than the error-correction capability $t$, the BCH codewords of group pair $i$ differ at $\delta_i$ bit positions in the ideal case, which exceeds the error-correction capability $t$. If so, the BCH decoder cannot decode the bit errors correctly (\autoref{step:BCH_decode} in \autoref{alg:single_round_pbs}) and report a failure. This exception happens with a small probability in each group pair: For example, when $d=1000$, and $\delta$ is set to $5$ (so that $g=d/\delta=200$), and $t$ is set to $13$, the probability that this exception happens is only $6.7\times 10^{-4}$. 


\begin{comment}

{\bf (previous)} To handle this type of exceptions, we further partition each trouble-causing group pair into $3$ sub-group-pairs and reconcile them respectively using PBS-for-small-$d$. 
%Note that $\delta_i$, if is not smaller, should be only slightly larger than $t$ with high probability. Hence, partitioning into $3$ sub-groups is enough to ensure each sub-group has no more than $t$ distinct elements. 
Note that $\delta_i$ is a Binomial random variable with mean $\delta$, $t$ is typically $1.5$ to $3.5$ times of $\delta$. So the probability that some sub-group contains more than $t$ distinct elements conditioned upon $\delta_i>t$ is tiny. 
In the same example above ($d=1000$, $\delta=5$, $t=13$), this conditional probability is $9.5\times 10^{-10}$.%that some sub-group has more than $t$ distinct elements is $9.5\times 10^{-10}$. 
In the next round, each sub-group-pair will hardly encounter this type of expections and can be reconciled by PBS-for-small-$d$ respectively.  More specifically, we add a termination condition of \autoref{alg:3_way_partition} after \autoref{step:BCH_decode} in \autoref{alg:single_round_pbs}.

\begin{algorithm}
\caption{Termination condition when BCH decoding fails}
\label{alg:3_way_partition}

\If{BCH decoding fails\label{step:if1}}
{Hash-partition the group pair into $3$ sub-group-pairs and run PBS-for-small-$d$ for each of them in the next round; Break;}\label{step:term1} 

\end{algorithm}

\end{comment}

% Back to the \autoref{proto:multirounds}, which shows the set reconciliation operations in each round of PBS-basic, this kind of exceptions only affect \autoref{step:reconcile} in \autoref{proto:multirounds}. Now this step needs to check whether BCH decoding is successful or not: If successful, all the operations remain the same; Else, we hash-partition the group ($A$ and $B$) into $3$ sub-groups and reconcile them respectively using \autoref{proto:multirounds}. 
% {\bf I'm not sure if it is necessary to discuss this case, since PinSketch did not mention it, even it may happen in PinSketch}
% Another type of exceptions that happens when $d_i>t$ is, the BCH decoder mistakes the decoding is successful and returns $t$ incorrectly decoded bit errors (i.e., subset pairs). The probability of this type of exceptions is very small. For instance, when $d=1000, \delta=5, t=13$ $(2.5\delta)$, $d_i>t$ happens with probability roughly $6.7\times 10^{-5}$, and the probability that the BCH decoder mistakes the decoding is successful when $d_i>t$ is on the order of $10^{-7}$ \cite{kim1996undetected}. So the probability that this type of exceptions happens in each group is on the order of $10^{-12}$. On the other hand, the impact of this type of exceptions is insignificant. Assume an incorrectly decoded bit error corresponds to a random subset pair, which could contain (1) no distinct element; (2) exactly $1$ distinct element; or (3) more than $1$ distinct elements. Reconcile the subset pair using \autoref{alg:trivial_case} could (1) get nothing and waste $\log |\mathcal{U}|$ bits of communication overhead; (2) get an actual distinct elements; or (3) trigger the exceptions that were discussed and handled in \autoref{subsec:exception_hash_partition}. 

\input{section/multiround_pbs_large_d}



% \subsection{What If PinSketch Also Uses Partitions?}\label{sec:whatifpinsketch}

% {\color{red} Moved to related work section.}

% Arguably, the same algorithmic trick (i.e., hash-partition two sets each into groups) can also be applied to PinSketch~\cite{Dodis_PinSketch_2008} for reducing its BCH decoding computational complexity from $O(d^2)$ to $O(d)$.   Doing so however makes the communication overhead of PinSketch higher than that of PBS for the following reason.
% As just explained, we need to leave a safety margin in setting the BCH error-correction capacity $t$, in the sense that $t$ needs to be ``comfortably'' larger than $\delta$, the average number
% of ``bit errors''.   
% %In other words, the amount of safety margin is $t - \delta$.  
% Hence for each group pair, the average additional communication overhead (incurred for transmitting a longer BCH codeword) of leaving this safety margin
% is $(t-\delta)\log n$ in PBS and is $(t-\delta)\log |\mathcal{U}|$ in PinSketch.
% However, as explained in \autoref{subsec:pbs-vs-pinsketch}, $\log n$ (the Galois field ``width" in PBS) is typically $3$ to $4$ times smaller than $\log |\mathcal{U}|$ 
% (the Galois field ``width" in PinSketch).  Hence PinSketch pays $3$ to $4$ times more for leaving the safety margin, resulting in a higher overall communication overhead.  
% For example, when $\delta=5, n=255, |\mathcal{U}|=2^{32}, t=2.6\delta$ (same as in the example in \autoref{sec:BCH_exception}), the communication overhead of PinSketch using hash-partitioning 
% is $2.6$ times the theoretical minimum, whereas that of PBS is $2.1$ times the theoretical minimum. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%It means PBS could have a lower communication overhead than PinSketch if they both use the algorithmic trick. 
% needs to be ``comfortably" larger than $\delta$

\begin{comment}
This ``safety margin'' will incur much more additional communication overhead on PinSketch than on PBS

However, since the BCH error-correction capability $t$ needs to be ``comfortably" larger than $\delta$, 

it will encounter the same randomness problem and have to set up a ``safety margin'' on the error-correction capability $t$. This ``safety margin'' will incur much more additional communication overhead on PinSketch than on PBS: Considering the average communication overhead per group pair, the additional overhead caused by the ``safety margin'' is $(t-\delta)\log n$ in PBS and $(t-\delta)\log |\mathcal{U}|$ in PinSketch. The latter is roughly $4$ times of the former when $n=255, |\mathcal{U}|=2^{32}$. Recall that the theoretical minimum amount of communication overhead to reconcile $\delta$ distinct elements is $\delta\log |\mathcal{U}|$. Use the same example in \autoref{sec:intro}, when $\delta=5, n=255, |\mathcal{U}|=2^{32}, t=2.5\delta$, the overhead of PinSketch using the algorithmic trick is $2.5$ times of the theoretical minimum, while that of PBS is $2.075$ times of the theoretical minimum. It means PBS could have a lower communication overhead than PinSketch if they both use the algorithmic trick. 
\end{comment}

%{\bf Furthermore, as the signiture length $\log |\mathcal{U}|$ increases, the advantage of PBS over PinSketch will be more significant.}

% We handle this type of exceptions by the same method (i.e., hash-partition into $3$ sub-groups) as above. To detect them, on the other hand, is simple: Note that incorrect decoded bit errors correspond to the subset pairs that do not contain distinct elements. When we reconcile those subset pairs in \autoref{sec:reconcile_by_trivial}, the output (i.e., reconciled elements) will be $\mathbf{0}$, which is abnormal (since $\mathbf{0}\notin A\bigcup B$, as we described in \autoref{subsec:protocol0}). Hence, this type of exceptions happen if and only if one of the reconciled distinct elements is $\mathbf{0}$. 
%Hence, we consider BCH decoding is successful by two criteria: (1) the BCH decoder reports a successful decode; and (2) None of the reconciled elements is $\mathbf{0}$. 
% ========================
% In fact, even if $d_i>t$, PBS-basic is still possible to reconcile group $i$ in some nonideal cases. For example, when $t=10$ and $d_i=11$, if the $11$ distinct elements are distributed in $10$ subset pairs, such that $1$ subset pair contains $2$ distinct elements and $9$ subset pairs contain $1$ distinct element in each, the two parity bitmaps differ at only $9$ bit positions. So BCH decoder is able to decode the later $9$ subset pairs and the corresponding $9$ distinct elements can be reconciled. In the second round, only $2$ distinct elements remain and BCH decoding certainly works. In this case, we do not need to partition the group into sub-groups, and this case does not trigger \autoref{alg:3_way_partition} in PBS. 
% ========================
% Instead, it will either (1) report a failure about exceeding the error-correction capability; or (2) mistake the decoding is successful and return incorrect decoded bit errors. 

% The second case happens with a very small probability (in order of $10^{-7}$ \cite{kim1996undetected}) and is very simple to detect : 

% The first case is easy to handle: We can simply adapt the same algorithmic trick to partition the group into smaller groups and reconcile them respectively. In our scheme, we set the number of smaller groups to be $3$, which is big enough because $d_i$, if not smaller, only slightly larger than $t$ with high probability. The second case on the other hand, although theoretically possible, happens with a very small probability when $d_i>t$ (in order of $10^{-7}$ \cite{kim1996undetected}). Besides, the probability of $d_i>t$ is also very small (e.g., when $t=15$ and $\delta=5$, this probability is about $2.3\times 10^{-4}$), so the overall probability of the second case, which is the multiplication of these two small numbers, is negligible (e.g., in order of $10^{-11}$).

% \subsection{Multi-rounds}

% Even if the ideal case does not happen, most of the distinct elements should be distributed into different subset pairs and therefore can be reconciled. So our scheme, even cannot reconcile all of the distinct elements, can still reconcile the majority of them (piecewise decodability). To reconcile the rest distinct elements, we can just run our scheme for multi-rounds under different hash-partition functions. For each round, our scheme works as follows: 

% \IncMargin{1em}
% \begin{algorithm}
% \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
% \Input{Two sets $A$ and $B$}
% \Input{Size of set difference $d$}
% \Input{The number of subset pairs $n$}
% \Input{BCH error-correction capability $t$}

% Hash-partition $A$ and $B$ into $n$ subset pairs $\{(A_i,B_i)\}_{i=1}^n$;

% \If{BCH decoding fails}
% 	Hash-partition $A$ and $B$ into $3$ subset pairs and reconcile them respectively in the next round\;
% \ElseIf{BCH decoding success}
	
% \Else{}

% $k \leftarrow \lceil \frac{t}{c}\rceil $\;

% Partition elements into $k$ subsets using~\autoref{alg:random-part}\;

% \For{$j = 0$ \KwTo $k-1$}{
%     Reconcile the $j$-th subset pair using the straw-man scheme with the BCH correcting capability $\tau$, number of smaller subsets $m$, and number of rounds $r$\;
% }

% \caption{PBS (per round)} \label{proto:II}
% \end{algorithm}\DecMargin{1em}

% This {\bf multi-rounds} scheme can significantly increase the success probability (i.e., the probability that all distinct elements are reconciled). Readers may wonder in the later rounds, most distinct elements should be reconciled, and the remaining could be reconciled using degraded parameters (i.e., smaller $n$ and $t$). In fact, degrade parameters in later rounds cannot save much communication overhead, since the majority of it is spent in the first round (i.e., $>90\%$). Therefore, we use the same parameters (i.e., $n,t$) among all rounds in our evaluation. 
% %The tradeoff between the number of rounds and the communication overhead per rounds will be elaborated in \autoref{sec:tail_bound}. In our evaluation, $r=2,3$ rounds are enough to achieve an extremely high success probability. 

% Readers may think the cost (i.e., communication overhead and the computational complexity) of this multi-rounds scheme is proportional to the number of rounds (denoted as $r$) and increases linearly with $r$. In fact, the cost of each round is roughly proportional to the number of remaining distinct elements, which decreases exponentially as $r$ increases (i.e., the first round reconciles $99\%$ of distinct elements, the second round reconciles $99\%$ of the remaining $1\%$ distinct elements, etc.). So the cost of this multi-rounds scheme is only slightly larger than that of the single-round scheme. Furthermore, as we explained in \autoref{sec:intro}, {\bf from intro thanks for the piecewise decodability of our solution, in almost all practical application scenarios, this tradeoff does not lead to longer response time because the reconciliation of objects identified by the successfully decodable codewords, which constitute the vast majority of all codewords, can run in parallel with the transmissions and decodings of the rest.  In other words, the piecewise decodability effective masks the slightly larger number of communication rounds as far as the response time is concerned.} 





\begin{comment}
\subsubsection{Random Partition}

\IncMargin{1em}
\begin{algorithm}
% \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
% \Input{Set $S$}
% \Input{The number of subsets $m$ for partition}
% \Output{Subsets $S_1, S_2, ..., S_m$}

% Generate hash function $h(\cdot)$ that maps each element into $\{1,2,...,m\}$;

\ForEach{$s \in S$}{
    $j \leftarrow h(s) \bmod m$\;    
    Insert $s$ into the $j$-th subset $S_j$\;
}

\caption{Partition using hash function $h(\cdot)$.} \label{alg:random-part}
\end{algorithm}\DecMargin{1em}

Like the strawman scheme, our scheme randomly partitions sets $A$ and $B$ into $m$ subsets. This random partition 
can be easily accomplished by using some hash function, $h(\cdot)$, and inserting each element $x$ into the subset 
corresponding to $h(x)$. \autoref{alg:random-part} presents the pseudo-code of this random partition using hash 
function $h(\cdot)$.  

% Unlike the strawman scheme, our scheme only reconciles those subset pairs that need to be reconciled, 
% because 



Like the strawman scheme, our scheme hash-partitions the two sets $A$ and $B$ into $m$ subset pairs $(A_i, B_i)$ for $i=1,2,\cdots,m$. 
We note that, among those $m$ bins (subset pairs), 
at most $t$ ($t\!\ll\!m$ as shown in our analysis in~\autoref{subsec:protocol1}) bins contain balls 
(elements belonging to the set difference), {\it i.e.,} requiring reconciliation.  
Motivated by this observation, we, therefore, propose to first detect those bins that 
contain balls and then only reconcile them. The detection is solved with a simple encoding approach that 
will be detailed in the next section.

\subsubsection{Detection before Reconciliation} 

In fact, identifying those non-empty bins is easy when each bin contains at most one ball. In this section, we assume that 
each bin after the random partition contains at most one ball, we will show later how to handle the cases when some 
bins contain more than one balls later in~\autoref{subsec:exceptions}. 

Given an arbitrary bin (say subset pair $(A_i, B_i)$) that contains one ball ({\it i.e.,} $A_i\triangle B_i$ contains exactly one element), 
the corresponding two subsets $A_i$ and $B_i$ differ exactly one element, which implies that 
$||A_i|\!-\!|B_i||\!=\!1$. Hence, if $|A_i|$ ({\it i.e.,} number of 
elements in $A_i$) is odd (or even), then $|B_i|$ must be even (or odd). In other words, the odevity of $|A_i|$ 
and $|B_i|$ are opposite. %differs if $|A_i\triangle B_i|\!=\!1$. 
Based on this property, we propose the {\it odevity encoding}: 
A subset is encoded as ``1'' if it contains odd number of elements, and as ``0'' otherwise. 
Using this odevity encoding, the $m$ subsets of $A$ can be encoded as a bit string $b_A$ in $\{0,1\}^m$, 
where the $i$-th bit in $b_A$ corresponds to the odevity encoding of $|A_i|$. Similarly, the $m$ subsets of $B$ can also 
be encoded as a bit string $b_B$. Clearly, $b_A$ and $b_B$ differ at $t$ different positions, or in other words, 
the Hamming distance of bit strings $b_A$ and $b_B$ is $t$. A straightforward approach is 
to let Alice send $b_A$ to Bob, and then Bob compares $b_B$ against $b_A$ to obtain those non-empty bins. 

This approach, however, has a communication overhead of $m$ bits, which is still unnecessarily high. As 
analyzed in~\autoref{subsec:protocol0}, $t$ is usually much smaller than $m$. 
That means $b_A$ and $b_B$ differ only at a tiny portion of bits. %have much more in common than differences. 
Therefore, if we view $b_B$ as a corrupted message of $b_A$ with $t$ corrupted bits, the detection of those $t$ bins can be converted to 
the detection of the positions of the $t$ corrupted bits. The latter can be solved using an Error-Correction Code (ECC)~\cite{Lin_ErrorControlCoding_1983} that can correct up to $t$ errors. In this work, we use the BCH code~\cite{Lint_IntroductionCodingTheory_1998}. 
More precisely, this ECC-based approach (with the BCH code) works as follows. 
Alice computes the parity bits for $b_A$ using a $t$-error-correcting BCH code with a block length of 
$(2^{\lceil \log m\rceil} -1)$ and sends the parity bits to Bob. Bob then decodes the positions of the $t$ corrupted bits 
using the BCH decoding algorithm with $b_B$ and those parity bits received from Alice. The communication overhead of 
this approach is roughly $t\lceil \log m\rceil$ ($=O(t\log t)$) bits. In the example above, this communication overhead is 
roughly $\num{17000}$ bits, which is approximately $6$ times lower 
than $m\!=\!\num{108469}$ bits, the communication overhead of the aforementioned straightforward approach. 

At first sight, it seems that the detection of non-empty bins and reconciliation of subsets in those bins require two rounds 
(or at least two round trip delays), {\it i.e.,} one round for detection and the other for reconciliation. In fact, 
it only requires one. After Bob receives the parity bits from Alice and decodes out those non-empty bins, it initiates 
the reconciliation ({\it i.e.,} \autoref{alg:trivial_case}) for each bin (subset pair) immediately, 
{\it i.e.,} sends the \code{XOR} sums of subsets in those bins together the indexes of those bins. 
After receiving those \code{XOR} sums and bin indexes, Alice can compute the set difference. 

% A naive way to combine the detection of non-empty bins and reconciliation of subset pairs in those bins is to first detect 
% those non-empty bins via one round of message exchanges between Alice and Bob and then to reconcile the corresponding 
% subset pairs in those bins with another round of message exchanges. This requires two rounds ({\it i.e.,} taking at least 
% two round trip delays). In fact, after Bob receives the parity bits from Alice and obtains those 

\subsubsection{Multiple Rounds}\label{sec:multiround}

{\bf This section was not clear enough. I need more time to think about and revise it.}


In the above section, we have assumed that each bin contains at most one ball. 
However, even with a sufficient large $m$, some bin might contain more than one balls though with tiny probability. 
We will show in~\autoref{subsec:exceptions}, how such rare events, {\it i.e.,} one bin contains more than one balls, 
can be easily detected.
To ensure our scheme can successfully reconcile all elements even when such rare events happen, 
we propose to use multiple rounds (of communication between Alice and Bob). More precisely, instead of 
selecting a prohibitively large $m$ to ensure that each bin contains at most one ball with a extremely high probability 
(say 0.99999), we select a reasonably large $m$ so that the communication overhead is not very high and very few bins contain 
more than one balls (or in other words, most bins contain at most one ball). Therefore, after running one round of 
our scheme, most elements in the set difference will be reconciled. Only those in the bins that contain more than one balls 
fail to be reconciled. For elements in the subsets corresponding to those bins, we run another round of our scheme. 
If some elements still fail to be reconcile, we can run one more round of our scheme. So on so forth,  
our scheme can keep running for more rounds until all elements are reconciled. 

With the same communication overhead, multiple rounds can significantly increase the success rate, 
{\it i.e.,} the probability that all elements in the set difference will be successfully reconciles, 
which will be elaborated in~\autoref{sec:tail_bound}. 

% % to be emphasized
% % say that too many rounds should be avoided (latency & communication overhead reduction is negligible when r is too large, 2 - 3 is good enough)
% % multiple rounds is not an issue when r is small

% We note that the number of rounds $r$, however, should not be large. On one hand, it results in large latency (at least $r$ round trip delays). 
% On the other hand, when $r$ is large, the reduction of communication overhead by the increase of $r$ gradually diminishes. 

We note that multiple rounds, when $r$ is small, would not really increase the ``latency'', as long as most elements in the 
set difference can be reconciled in the first rounds, since the underlying synchronization of data objects corresponding to 
those elements can start immediately after the first round of our scheme. Therefore, the actual latency is one round trip delay instead of 
$r$. 

As we mentioned, this straw-man protocol works correctly if each subset pair has at most one exclusive element (i.e., \autoref{eq:requirement_strawman} holds). On the other hand, if a subset pair has more than one exclusive elements, some of which will not be successfully reconciled:

\begin{itemize}
\item If a subset pair has even number of exclusive elements, Odevity coding will encode it as 0. Then the straw-man scheme will consider the subset pair having no exclusive element and all exclusive elements in this subset will not be reconciled;

\item If a subset pair has odd number ($\geq 3$) of exclusive elements, Odevity coding will encode it as 1 and consider the subset pair having only 1 exclusive element. Then the straw-man scheme will use \autoref{alg:trivial_case} to decode only one exclusive element and dismiss all others. Even worse, the only decoded element is probably not a real exclusive element, since the element computed by \autoref{alg:trivial_case} is the \code{XOR} sum of all exclusive elements, not one of them. 
\end{itemize}

In summary, if a subset pair has more than one exclusive elements, most of its exclusive elements cannot be reconciled, and the reconciled element is usually incorrect (i.e., false-positive). The false-positive however is easy to check, which will be elaborated in \autoref{subsec:exceptions}. The good thing is, even if not all subset pairs have at most one exclusive element and are successfully decoded, most of them will be w.h.p.. In other words, even if the straw-man protocol cannot reconcile all exclusive elements, it still can reconcile most of them. To reconcile all exclusive elements w.h.p., we can simply extend the single-round straw-man scheme to multi-round. And each round adapts the straw-man scheme to do set reconciliation using independent hashing functions $h(\cdot)$ for partition (i.e., in \autoref{alg:random-part}). This multi-round extension can significantly increase the probability of a successful reconciliation, which will be elaborated in \autoref{sec:tail_bound}. 



\subsection{Our Scheme: The Final Version}\label{subsec:protocol2}

{\bf Under revision~}

The preliminary version of our scheme suffers from two major drawbacks. 
First, its communication overhead is asymptotically 
$O(t\log m)\!=\!O(t\log t)$, which is not asymptotically optimal. 
Second, the decoding computational complexity is proportional to 
$t^2$ with the state-of-the-art decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} for BCH codes, 
which is too high when $t$ is large. 
To overcome these two drawbacks, we use a simple algorithmic trick: divide and conquer. With this algorithmic 
trick, the decoding computational complexity is reduced to $O(t)$, 
and the communication overhead is reduced to $t\cdot\frac{\log u}{8} \!+\! O(t)$ (with a small 
hidden constant roughly varying from 4 to 8) bytes which implies that 
our scheme has an additive communication overhead (compared to the optimal scheme) 
of 4 to 8 bytes per element in the 
set difference and this additive overhead is independent of the key size ({\it i.e.}, $\log u$). 
Recall that the IBF-based schemes usually have a communication overhead of roughly 6 times of the 
optimal scheme, which increases linearly as the key size. Therefore, our scheme is much more 
communication-efficient. 

Now, we describe in detail this algorithmic trick. We let Alice divide elements in $A$ into $\lceil\frac{t}{c}\rceil$ groups (subsets)  
for some small constant $c$ (say $5$) so that each group contains roughly $c$ elements from the set difference on average. We let Bob do the same operations on $B$. To ensure that any common element ({\it i.e.,} any element $x\!\in\! A\bigcup B$) goes into 
the same group ({\it i.e.,} groups at Alice and Bob with the same index), we can use the partition procedure with a hash function shown 
in~\autoref{alg:random-part}. Then, we can apply the preliminary version on each group with a constant $m$ (say $m\!=\!256$) independent of 
$t$. To ensure that each group can be reconciled with a high probability, we need to use BCH codes whose decoding capacity 
larger than $c$ (say $\tau\!=\!2c$), as exact number of elements to be reconciled could be larger than $c$. 
Since this decoding capacity $\tau$ is still a small constant independent of $t$, therefore, the communication 
overhead per group is $\tau\cdot\log m \!=\!O(1)$, which implies a total communication overhead of $O(t)$. 
Similarly, the total decoding computational complexity is also $O(t)$. 

\subsubsection{Parameter Configurations} 

Our scheme now has several parameters: $c$ (average number of elements from the set difference in each group), 
$\tau$ (the correcting capability of the BCH code), $m$ (number of bins for each group), and $r$ (maximum number of rounds). 
We note that the maximum number of rounds $r$ is usually associated with another parameter $p$ the desired success rate: With 
at most $r$ rounds, our scheme should guarantee that the success rate is at least $p$. 
%How to tune these parameters to achieve favorable performance will be detailed later in~\autoref{sec:tail_bound}. 
Here, we provide some guidances for the parameter configurations using our theoretical analysis, which gives the tail bound of 
the success probability of our scheme and will be shown in~\autoref{sec:tail_bound}. 

\noindent
{\bf Parameterizing $c$ and $r$.} The values of $c$ and $r$ are usually provided by users based on the requirements of 
applications. For the value of $c$, a larger $c$ results in a longer decoding time yet lower communication overhead.  
So if the decoding time is a big concern, then a smaller $c$ (say $c=5$) should be used; otherwise, a larger $c$ could be used. 
For the values of $r$, a larger $r$ leads to lower communication overhead and usually lower decoding time (as it allows to use 
a smaller $\tau$), however, the reduction is marginal when $r>3$. Therefore, we suggest users to configure $r$ to be $2$ or $3$. 
% The configuration of $c$ is relatively straightforward, as a larger $c$ will result in 
% a longer decoding time and a slightly lower communication overhead. The former is ..., The latter is slightly tricky. 


\noindent
{\bf Using $c$ and $r$ to parameterize other parameters.} After users specify the values for $c$ and $r$ (associated with a value for 
$p$), we can use our theoretical analysis in~\autoref{sec:tail_bound} to parameterize $\tau$ and $m$. 
Since in a BCH code, the block length is in the form of $2^q-1$, we only need to consider $m=2^q-1$. 

{\bf Liang, please revise the following algorithm!}

\begin{algorithm}
\SetKwProg{Proc}{}{}{end}
\SetKwFunction{algo}{\small Search}

\Proc{Search($c$, $r$, $p$)}{\label{search:entrance}

$\mbox{co}_{best}\leftarrow\infty$\tcc*{\small Best communication overhead}

\For{$\tau \leftarrow c\,\KwTo\, \infty$}{}



}
\end{algorithm}


% , unlike 
% the IBF-based schemes which have an multiplicative overhead of 6 
% The inspiration is from the famous 
% divide and conquer algorithm for the selection problem, in which, given an array with $n$ elements, we want to get the $k$-th largest 
% element. A straightforward idea for this problem is sorting. However, if using insertion-sorting, the complexity would be $O(n^2)$. 
% Then the famous divide and conquer trick comes. It first divides the array into $\lceil n/5\rceil$ groups so that the first 
% $\lfloor n/5\rfloor$ contains $5$ elements and at most one group contains the rest $n \mod 5$ elements, and find the median of each 
% group using the insertion-sorting and th


% This straw-man scheme still has a problem on decoding computational complexity. More specific, the complexity increases dramatically with the total number of corrupted bits $t$. Therefore, when $t$ is moderate or large, the decoding computational complexity could be very high. For instance, the decoding complexity of BCH codes~\cite{Lint_IntroductionCodingTheory_1998} is $O(t^3)$, which could be quite high for a large $t$. To keep the decoding complexity reasonably low, we design the following two-layer protocol: In the first layer, we use a hash function to partition the two sets into $\lceil\frac{t}{c}\rceil$ subsets for some small constant $c$ (say $5$), just like the first step of our straw-man scheme. The objective, which is however different from before, is to make each subset pair contains roughly $c$ exclusive elements on average. In the second layer, we use the straw-man scheme with the same configuration (number of subsets $m$, and error-correction capability $\tau$, number of rounds $r$) to reconcile each subset pair. 

% In fact, the straw-man scheme is a proper solution when $t$ is small. First, the decoding complexity will not be a problem for a small $t$; Second, we do not need an extremely large $m$ to guarantee \autoref{eq:requirement_strawman} w.h.p.. For instance, when $t=5$ and $m=1024$, \autoref{eq:requirement_strawman} holds with probability $\frac{m\,!}{(m-t)\,!m^t}\approx 99\%$. This motivates us to design the following two-layer protocol: In the first layer, we use a hash function to partition the two sets into $\lceil\frac{t}{c}\rceil$ subsets for some small constant $c$ (say $5$), just like the first step of our straw-man scheme. The objective, which is however different from before, is to make each subset pair contains roughly $c$ exclusive elements on average. In the second layer, we use the straw-man scheme with the same configuration (number of subsets $m$, and error-correction capability $\tau$) to reconcile each subset pair. 

\autoref{proto:II} shows the pseudocode of our scheme. It first uses the same hash-function based random partition algorithm as \autoref{alg:random-part} to partition elements into $k\triangleq\lceil \frac{t}{c} \rceil$ subsets. Note that the random partition only guarantees that each such subset 
contains $c$ exclusive elements on average, and the exact number is not known. Hence, our scheme uses a BCH code with a capability of 
correcting up to $\tau$ errors with $\tau > c$ to make sure that the BCH code has a high probability to decode successfully. We will describe how to deal with situation where the size of set difference exceeds $\tau$ later in~\autoref{subsec:exceptions}.

As the decoding of a $\tau$-error-correcting BCH code where $\tau$ is a small constant has a constant-time computational complexity, the decoding complexity of 
our scheme is $O(k)=O(t)$. We now have several parameters, average number of exclusive elements in each subset $c$, the correcting capability $\tau$ of BCH code, the number of smaller subsets $m$ for each subset to be divided to, and the number of rounds $r$. How to tune these parameters to achieve favorable performance will be detailed later in~\autoref{sec:tail_bound}. 

\IncMargin{1em}
\begin{algorithm}
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
\Input{Size of set difference $t$}
\Input{The number of subsets $m$ for each partition}
\Input{Average number of exclusive elements in each partition $c$}
\Input{BCH code capability $\tau$}

$k \leftarrow \lceil \frac{t}{c}\rceil $\;

Partition elements into $k$ subsets using~\autoref{alg:random-part}\;

\For{$j = 0$ \KwTo $k-1$}{
    Reconcile the $j$-th subset pair using the straw-man scheme with the BCH correcting capability $\tau$, number of smaller subsets $m$, and number of rounds $r$\;
}

\caption{Our Scheme} \label{proto:II}
\end{algorithm}\DecMargin{1em}




\subsection{Exceptional Handling}\label{subsec:exceptions}

{\bf To be revised~}

In this section, we will elaborate how to handle the following two types of exceptions that we mentioned in \autoref{sec:multiround} and \autoref{subsec:protocol2}:
\begin{itemize}
    \item Exception 1: A subset pair has odd number ($\geq 3$) of exclusive elements and causes false-positives (i.e., a decoded distinct element is not a real one);
    \item Exception 2: A subset pair contains too many exclusive elements, such that a BCH code with capability of correcting up to $\tau$ errors cannot decode it (i.e., $t>\tau$).
	\item Exception 3: A subset pair has even number ($\geq 2$) of exclusive elements and causes false-negatives(i.e., two or more distinct elements are neglected as the parity bit is 0);
\end{itemize}

To handle Exception 1, we need to check whether a computed exclusive element by \autoref{alg:trivial_case} is a real exclusive element or not. (The group index happens to come in handy if we use it as a fingerprint of the element we computed. If this element is truly an exclusive element, it should be hashed into the same group as before. Notably, We have two group indices available for this check, one is in the initial divide and conquer phase, the other is in the BCH code part) It can be easily done at the end of set reconciliation, during which two hosts exchange their exclusive elements. In fact, as we will elaborate in \autoref{sec:tail_bound}, Exception 1 hardly happens if we set parameters properly. 

On the other hand, when Exception 2 happens, the BCH decoder will report a failure about exceeding the error-correction capability. For such a subset pair, we can use the same approach as in \autoref{subsec:protocol2} to partition it into smaller subsets and use the straw-man scheme to reconcile them respectively. We set the number of small subsets to be 3. It is because, as we will elaborate in \autoref{sec:tail_bound}, the number of exclusive elements for each subset pair $t$ should be, if not smaller, only slightly larger than $\tau$ w.h.p.. Partitioning those exclusive elements into 3 small subsets is enough to guarentee that each of them has less than $\tau$ exclusive elements.

\end{comment}

==> section/pbs_large_d_copy.tex <==
\section{PBS for large \texorpdfstring{\larger\boldmath\MakeLowercase{$d$}}{d}}\label{subsec:protocol2}\label{sec:pbs-for-large-d}

In this section, we continue to assume that the number of distinct elements $d$ is precisely known in advance.
As explained in \autoref{sec:larged}, the PBS-for-small-$d$ scheme described in the previous section is no longer suitable when $d$ is very large, since its BCH decoding computational complexity is 
$O(d^2)$ finite field operations.  Instead, we first hash-partition sets $A$ and $B$ each into $g = d/\delta$ groups, and then apply PBS-for-small-$d$ to each of the $g$ group pairs.  
{\color{red}Here $\delta$ is a small constant, by which we can control the tradeoff between 
the communication and computational overheads of PBS. Generally, the larger $\delta$ is, 
the lower the communication overhead is and the higher the computational overhead. 
We will elaborate how 
$\delta$ controls this tradeoff in~\autoref{app:vs-delta}. 
Nonetheless, we have found that $\delta$=5 is a nice tradeoff point, and hence we fix $\delta$ at $5$ in this paper.}
Since each group pair contains on average $\delta = 5$ distinct elements, the BCH decoding computational complexity per group pair can be considered $O(1)$.  
As a result, the overall BCH decoding computational complexity is $O(d)$ for all $g = d/\delta$ group pairs.  We refer to this PBS-for-large-$d$ scheme as PBS in the sequel except in 
places where this abbreviation would result in ambiguity or confusion.


\begin{comment}
The scheme described above, which we refer to as PBS-for-small-$d$, can also do set reconciliation when $d$ is large. However, the BCH decoding computational complexity in it is $O(d^2)$ of finite field operations, 
%even using the state-of-the-art decoding algorithm~\cite{Dodis_SyndromeEncodingDecoding_2006}, 
which is too expensive for large $d$. To overcome this drawback, we first consistently partition sets $A$ and $B$ each into $d/\delta$ smaller subsets (which we call {\it groups} to distinguish from subsets) for some small integer $\delta$ (say $5$). In this way, each group pair contains roughly $\delta$ distinct elements. Then we apply PBS-for-small-$d$ to reconcile each group pair respectively. The BCH decoding computational complexity of each group pair is roughly $O(\delta^2)$, which can be considered as $O(1)$, since $\delta$ is a small number. As a result, the overall BCH decoding computational complexity is reduced from $O(d^2)$ to $O(d)$. 
\end{comment}

% To overcome this drawback, we use the same technique in \autoref{sec:hash_partition} to hash-partition sets $A$ and $B$ each into $d/\delta$ subsets (which we call {\it groups} to distinguish from subsets) for some small integer $\delta$ (say $5$), so that each of the group pairs contains roughly $\delta$ distinct elements and can be reconciled by PBS-for-small-$d$ respectively. The BCH decoding computational complexity of each group pair is roughly $O(\delta^2)$, which can be considered as $O(1)$, since $\delta$ is a small number. As a result, the overall computational complexity is reduced from $O(d^2)$ to $O(d)$. 
%{\bf In PBS, we set $\delta = 5$. }

%Note that the BCH decoding computational complexity is $O(d^2)$ of finite field operations (in GF($2^{8}$) when $n=255$) using the state-of-the-art decoding algorithm~\cite{Dodis_SyndromeEncodingDecoding_2006}, which is too expensive for large $d$. To overcome this drawback, we first hash-partition sets $A$ and $B$ each into $d/\delta$ subsets (which we call {\it groups} to distinguish from subsets), just like what we did in \autoref{sec:hash_partition}, for some small integer $\delta$ (say $5$), then reconcile each of the group pairs by the PBS we described in \autoref{sec:scheme}. After the partition, each group pair has $\delta$ distinct elements on average. So the BCH decoding computational complexity of each group pair is roughly $O(\delta^2)$, which can be considered as a constant, since $\delta$ is a small number. As a result, the overall computational complexity of PBS is reduced from $O(d^2)$ to $O(d)$. 

%To differentiate from the PBS described in \autoref{sec:scheme}, we refer to it as PBS-basic in this section. 

% \subsection{How to Set Parameters \texorpdfstring{\larger\boldmath\MakeLowercase{$t,n$}}{t,n}}
\subsection{How to Set Parameters {\texorpdfstring{\larger\boldmath\MakeLowercase{$t$}}{t}} and \texorpdfstring{\larger\boldmath\MakeLowercase{$n$}}{n}}\label{subsec:parameterize-n-t}

In PBS (i.e., PBS-for-large-$d$), we have to make some design decisions that we don't have to in PBS-for-small-$d$.  
One of them is how to set the error-correction capacities of the BCH codes used 
for each of the $g$ group pairs. 
Let $\delta_i$, $i=1,2,...,g$, be the number of distinct elements that group pair $i$ have.  
{\color{red}If we knew the precise values of $\delta_1$, $\delta_2$, 
..., $\delta_g$, we would simply set the BCH error-correction capacity 
% (the maximum number of bit errors a BCH codeword is designed to correct) 
for each group pair $i$, which we denote as $t_i$, to $\delta_i$.} This way, each BCH codeword is the shortest possible for the respective task, which minimizes the communication overhead of transmitting these codewords. 
In reality, we do not know the exact value of any $\delta_i$, since it is a random variable with distribution $Binomial(d, 1/g)$ thanks to the hash-partitioning (of $A$ and $B$ each into $g$ groups);  
we only know that $E[\delta_i] = d/g = \delta$  
but that does not help much.
In theory, we can measure $\delta_i$ using a (set difference) cardinality estimation protocol.  However, as will be shown in~\autoref{subsec:ToW}, to obtain such an estimate using the 
best protocol
would incur hundreds of bytes of communication overhead.  In comparison, the ``savings'' on the communication overhead that such an estimate would bring (for the corresponding group pair) 
is only tens of bytes, as we will elaborate next.

In PBS, we set an identical BCH error-correction capability $t$ for all $g$ group pairs.  It intuitively makes sense since random variables $\delta_1$, $\delta_2$, 
..., and $\delta_g$ are identically distributed.  Now the next question is ``How should we set this $t$?".   This is a tricky question because, 
on one hand, if $t$ is too large (say several times larger than $\delta$), then the total size of the BCH codewords is unnecessarily large, resulting in ``wastes" in communication overhead; 
but on the other hand, if $t$ is too small (say equal to $\delta$), then a large proportion of the BCH codewords cannot decode, resulting in considerable additional efforts and costs (i.e., 
``penalties'')
for reconciling the large proportion of affected group pairs.   In \autoref{sec:tail_bound} and \autoref{sec:parameter_settings}, we propose an analytical framework that can be used to
identify the optimal $t$ value that minimizes ``wastes + penalties''.   The optimal $t$ value can range from $1.5\delta$ to $3.5\delta$  depending on how large this $d$ is.
%or $\hat{d}$ (an estimate of $d$ if we do not know its precise value in advance), is.

Based on a similar rationale, we set another parameter for each group pair $i$ to the same value $n$:  Each group pair $i$ is to be partitioned into $n$ subsets, so that the parity bitmaps 
($A[1..n]$ and $B[1..n]$ in PBS-for-small-$d$) for all groups have the same length of $n$ bits.  This $n$ is also a tunable parameter (for optimal PBS performance), since 
the probability for the ideal case (of all distinct elements between a group pair being hashed to distinct subsets) to happen is a function of $n$ and $\delta = 5$.  
As will be elaborated in \autoref{sec:parameter_settings}, our 
analytical framework can also be used for the optimal tuning of $n$.

\begin{comment}


On one hand, $t$ should be larger than or equal to most of $\delta_i$'s for $i=1,2,...,g$, so that most of the group pairs will not encounter BCH decoding failures, and the rest of group pairs (no more than several) only incur negligible ``penalties'' on BCH decoding failures; on the other hand, $t$ should not be too large to incur huge ``waste'' on communication overhead. To find the optimal $t$ that minimizes ``wastes''+``penalties'', we establish an analytical framework for parameter settings, as will be elaborated in \autoref{sec:tail_bound} and \autoref{sec:parameter_settings}. Typically, the optimal $t$ is $1.5$ to $3.5$ times of $\delta$.

Similarly, This randomness of $\delta_i$ also induces a parameter tuning issue on the number of subset pairs in group pair $i$. For the same reason, we set a universal $n$ as the number of subset pairs in each group pair. The analytical framework that is used for finding the optimal $t$ can also be used to find the optimal $n$, as will be elaborated in \autoref{sec:parameter_settings}. 


{\bf (previous) The error-correction capability $t$, defined as the maximum number of errors that the BCH code used by any group pair can correct, is a critical parameter for PBS to perform well. On one hand, if $t$ is too large (say $t=10\delta$), then the communication overhead on transmitting BCH codeword ($t\log n$ bits per group pair) is unnecessarily large; but on the other hand, {\bf if $t$ is too small (say equal to $\delta$), any group pair $i$ could contain more than $t$ distinct elements with a nontrivial probability (i.e., $Pr[\delta_i>t]$ is nontrivial). If so, in the ideal case, the $\delta_i$ distinct elements incur $\delta_i$ bit errors in the BCH codeword, which exceeds the error-correction capability $t$ and a BCH decoding failure happens (we will describe in \autoref{sec:BCH_exception}). if $t$ is too small (say equal to $\delta$), then close to half of the group pairs fail to decode the BCH codeword due to the insufficient error-correction capability, which can result in hefty penalties on BCH decoding failures (to be described in \autoref{sec:BCH_exception}). }
In PBS, we manage to make $t$ as small as possible (so that the communication overhead on transmitting BCH codewords is kept to a minimum) yet pay negligible penalties of BCH decoding failures. }



We continue to assume that the number of distinct elements $d$ is precisely known. Even so, due to the randomness of hash-partition, the number of distinct elements in group pair $i$, denoted as $\delta_i$, is a random variable with mean $\delta$ for $i=1,2,...,g$. Here $g\triangleq d/\delta$ denotes the number of group pairs. This randomness induces a parameter tuning issue on the error-correction capability. On one hand, if the error-correction capability of group pair $i$, denoted as $t_i$, is larger than $\delta_i$, the corresponding BCH codeword is unnecessarily long, which results in ``wastes'' on communication overhead. On the other hand, if $t_i$ is smaller than $\delta_i$, the BCH decoding would fail with high probability, which results in hefty ``penalties'' on BCH decoding failures, as will be described in \autoref{sec:BCH_exception}. Ideally, if $\delta_i$ is precisely known, we can set $t_i$ equal to $\delta_i$ that results neither ``wastes'' nor ``penalties''. However, to estimate each $\delta_i$ with high accuracy requires much larger additional communication overhead than the savings, as we will explain shortly in this section.

%which is roughly $2.5$ times of that in the perfect scenario (when $t$ is roughly $2.5\delta$). Due to this addition
One alternative solution is to estimate each $\delta_i$ and then set $t_i$ to be slightly larger than the estimate of $\delta_i$. It can save considerate communication overhead on transmitting the BCH code. However, to estimate all the $g$ values of $\{\delta_i\}_{i=1}^g$ in high accuracy requires huge additional communication overhead. For instance, estimating each $\delta_i$ requires $288$ bytes of additional communication overhead using the ToW estimator, as we will describe in \autoref{subsec:ToW}. However, the ``savings'' on the communication overhead is much smaller, which is typically no more than a few dozens of bytes.
%However, the ``savings'' on the communication overhead for group pair $i$ is no more than a few dozens of bytes.

\end{comment}


% We continue to assume that the number of distinct elements $d$ is precisely known. Even so, due to the randomness of hash-partition, the number of distinct elements in the $i$-th group pair, denoted as $\delta_i$, is a random variable with mean of $\delta$ for $i=1,2,...,g$, which are not precisely known. Since $\delta_1, \delta_2, ..., \delta_g$ follows the same distribution, it does not make sense to select different parameters for the $g$ group pairs. Hence, we set two universal parameters, $t$ and $n$, for all group pairs, where $t$ is the error-correction capability of the BCH code used for reconciling each group pair, and $n$ is the number of subset pairs in each group pair.

% We continue to assume that the number of distinct elements $d$ is precisely known. Even so, due to the randomness of hash-partition, denoted as $\delta_i$, the number of distinct elements in the $i$-th group pair, is a Binomial random variable with mean of $\delta$ for $i=1,2,...,g$, which cannot be precisely known without a huge amount of additional communication overhead. Since $\delta_1, \delta_2, ..., \delta_g$ follows the identical Binomial distribution, it does not make sense to select different parameters for the $g$ group pairs. Hence, we set two universal parameters, $t$ and $n$, for all group pairs, where $t$ is the error-correction capability of the BCH code used for reconciling each group pair, and $n$ is the number of subset pairs in each group pair.

%To deal with this randomness, we set two global parameters, denoted as $t$, that corresponds to the error-correction capability of the BCH code used for reconciling every group pair. identical no sense or additonal info

%{\bf (modified based on the next paragraph from intro)} 
%{\bf (previous) The error-correction capability $t$, defined as the maximum number of errors that the BCH code used by any group pair can correct, is a critical parameter for PBS to perform well. On one hand, if $t$ is too large (say $t=10\delta$), then the communication overhead on transmitting BCH codeword ($t\log n$ bits per group pair) is unnecessarily large; but on the other hand, {\bf if $t$ is too small (say equal to $\delta$), any group pair $i$ could contain more than $t$ distinct elements with a nontrivial probability (i.e., $Pr[\delta_i>t]$ is nontrivial). If so, in the ideal case, the $\delta_i$ distinct elements incur $\delta_i$ bit errors in the BCH codeword, which exceeds the error-correction capability $t$ and a BCH decoding failure happens (we will describe in \autoref{sec:BCH_exception}). if $t$ is too small (say equal to $\delta$), then close to half of the group pairs fail to decode the BCH codeword due to the insufficient error-correction capability, which can result in hefty penalties on BCH decoding failures (to be described in \autoref{sec:BCH_exception}). }
%In PBS, we manage to make $t$ as small as possible (so that the communication overhead on transmitting BCH codewords is kept to a minimum) yet pay negligible penalties of BCH decoding failures. }

%{\bf (moved from intro, to be removed)} The number of elements in the set difference between any group pair is in general not a constant.  Rather, it is a random variable that has roughly a Poisson distribution with mean $\delta$.  The potential issue arises from dealing with this randomness in setting a global parameter that corresponds to the error-correction capability of the BCH code used for reconciling every group pair.  This parameter, denoted as $t$ (consistent with other literatures on BCH code), is the maximum number of errors that the BCH code used by any group pair can correct, and the size of each such codeword is roughly $8t$ bits (assuming $n = 255$ as explained above). The issue is that, on one hand, if $t$ is too large (say several times larger than $\delta$), then the total size of the BCH codewords, which is the bulk of the extra communication cost, is unnecessarily large; but on the other hand, if $t$ is too small (say equal to $\delta$), then close to half of the BCH codewords cannot decode or worse decode incorrectly (unknown to Alice and Bob), which can result in hefty penalties in the latter case of incorrect decoding.   In PBS, we manage to make $t$ as small as possible (so that the total size of the BCH codewords is kept to a minimum) yet pay negligible penalties of incorrect BCH decoding.
%We will discuss the case that $d_i>t$ in \autoref{sec:BCH_exception}.


% To ensure the error-correction capability $t$ is sufficient (i.e., $t\geq \delta_i$ for $i=1,2,...,g$) for every group pair with high probability, we set $t$ conservatively and leave a sufficient `safety margin' between $t$ and the average number of distinct elements in each group pair $\delta$. 

% Note that the `safety margin' between $t$ and $\delta$ incurs additional communication overhead on transmitting BCH codeword: In the perfect scenario (i.e., $\{d_i\}_{i=1}^g$ is precisely known), the average communication overhead on transmitting BCH codeword per group pair is $\delta\log n$; On the other hand, when we set $t$ to be the error-correction capability for each group pair, the average communication overhead becomes $t\log n$. If we set the `safety margin' to be too large (say $t=10\delta$), it will incur huge additional communication overhead. Due to this reason, we set a moderate `safety margin' that  $t$ in the range from $1.5\delta$ to $3\delta$. 

% {\bf (moved from intro, to be removed)} The number of elements in the set difference between any group pair is in general not a constant.  Rather, it is a random variable that has roughly a Poisson distribution with mean $\delta$.  The potential issue arises from dealing with this randomness in setting a global parameter that corresponds to the error-correction capability of the BCH code used for reconciling every group pair.  This parameter, denoted as $t$ (consistent with other literatures on BCH code), is the maximum number of errors that the BCH code used by any group pair can correct, and the size of each such codeword is roughly $8t$ bits (assuming $n = 255$ as explained above). The issue is that, on one hand, if $t$ is too large (say several times larger than $\delta$), then the total size of the BCH codewords, which is the bulk of the extra communication cost, is unnecessarily large; but on the other hand, if $t$ is too small (say equal to $\delta$), then close to half of the BCH codewords cannot decode or worse decode incorrectly (unknown to Alice and Bob), which can result in hefty penalties in the latter case of incorrect decoding.   In PBS, we manage to make $t$ as small as possible (so that the total size of the BCH codewords is kept to a minimum) yet pay negligible penalties of incorrect BCH decoding.
%We will discuss the case that $d_i>t$ in \autoref{sec:BCH_exception}.

% Hence, we can no longer set the error-correction capability of the BCH code for each group pair based on the exact number of distinct element in it, as we did in \autoref{sec:scheme}. Instead, we set a conservative error-correction capability $t$ (say $2.5\delta$) for all group pairs, which is sufficient for them (i.e., $t\geq d_i$ for $i=1,2,...,g$) with high probability. We will discuss the case that $d_i>t$ in \autoref{sec:BCH_exception}.


% ===============================
% To differentiate from the PBS described in \autoref{sucsec:our-scheme}, we refer it as PBS-basic in this section. Note that the BCH decoding computational complexity is $O(d^2\log ^2 n)$, which is $\Omega(d^2\log^2 d)$ when $n=\Omega(d^2)$, with the state-of-the-art decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019}. It is too large in PBS-basic for large $d$. To overcome this drawback and generalize PBS-basic for large $d$, we partition sets $A$ and $B$ each into $d/\delta$ subsets (which we call {\it groups} to distinguish from subsets) for some small integer $\delta$ (say $5$) and reconcile the $d/\delta$ group pairs respectively using PBS-basic. After this partition, each group has $\delta$ distinct elements on average. The BCH decoding computational complexity of each group pair can be considered as $O(1)$, since $\delta$ is a small number. As a result, the overall computational complexity of PBS is reduced from $O(d^2\log ^2 n)$ to $O(d)$. 

% % To differentiate from the PBS described in \autoref{sucsec:our-scheme}, we refer it as PBS-basic in this section. PBS-basic is not suitable for large $d$ for two reasons: First, its communication overhead is asymptotically $O(d\log n)\!=\!O(d\log d)$ (since $n=\Omega(d^2)$), which is not asymptotically optimal. Second, the decoding computational complexity is proportional to $d^2$ with the state-of-the-art decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} for BCH codes, which is too high when $d$ is large. To overcome these two drawbacks, we use a simple algorithmic trick to (1) reduce the communication overhead from $O(d\log d)$ to $d\log u \!+\! O(d)$; (2) reduce the decoding computational complexity from $O(d^2)$ to $O(d)$. 

% Now, we describe the generalized PBS in details: In the first step, we hash-partition $A$ and $B$ (by some hash function $h_1(\cdot)$) into $g$ group pairs, just like what we did in \autoref{sucsec:our-scheme}. The objective of this partition is however different: In \autoref{sucsec:our-scheme}, we aim to ensure each subset pair contains at most $1$ distinct element (i.e., the ideal case) with high probability; Here we aim to make each group pair contains roughly $\delta$ distinct elements for some small constant $\delta$ (say $5$) by setting $g=d/\delta$. 
% %To differentiate the $g$ subset pairs here from those in \autoref{sec:hash_partition}, we call them the $g$ {\bf groups} in the sequel. 
% In the second step, we just apply PBS-basic (described in \autoref{sucsec:our-scheme}) to reconcile each group pair and obtain the distinct elements. 
% ================================

% To differentiate from the PBS described in \autoref{sucsec:our-scheme}, we refer it as PBS-basic in this section. When $d$ is large (more than several), we hash-partition set $A$ and $B$ into groups, such that each group pair contains $\delta$ distinct elements on average for small $\delta$ (say $5$), as described in \autoref{sec:larged}. Then each group pair can be reconciled by PBS-basic.

% When describing the PBS-basic in \autoref{sucsec:our-scheme}, we assume that the number of distinct elements is precisely known. We set the error-correction capability of the BCH code (denoted as $t$) just enough to correct $d$ errors (i.e., $t=d$). However, due to the randomness of hash-partition, $d_i$, the number of distinct elements in the $i^{th}$ group pair, is a Binomial random variable $Binomial(d,1/g)$ with expectation of $\delta$ $(=d/g)$ for $i=1,2,...,g$, which cannot be precisely known without a huge amount of additional communication overhead. Hence, we can no longer set the error-correction capability of the BCH code for each group pair based on the exact number of distinct element in it, as we did in \autoref{sucsec:our-scheme}. Instead, we set a universal error-correction capability $t$ (say $2.5\delta$) for all group pairs, which is sufficient for all group pairs (i.e., $t\geq d_i$ for $i=1,2,...,g$) with high probability. We will discuss the case that $d_i>t$ in \autoref{sec:BCH_exception}.

%This assumption in general does not hold: 
% Let $d_i$ denote the number of distinct elements in Group $i$. Due to the property of hash-partition, each $d_i$ is a Binomial random variable $Binomial(d,1/g)$ with expectation of $\delta$ $(=d/g)$. Even if $d$ is precisely known, each $d_i$ is not. To ensure the error-correction capability $t$ is sufficient for each group (i.e., $d_i\leq t$) with high probability, we leave some safety margin for the randomness of $d_i$ and conservatively set $t$ roughly $2.5\delta$ (the factor $2.5$ varies depend on other parameters, which will be discussed in \autoref{sec:parameter_settings}), so that $Pr[d_i>t]$ is tiny. We will discuss the case that $d_i>t$ in \autoref{sec:BCH_exception}.

% Note that the `safety margin' between $t$ and $\delta$ incurs additional communication overhead on transmitting BCH codeword: In the perfect scenario (i.e., $\{d_i\}_{i=1}^g$ is precisely known), the average communication overhead on transmitting BCH codeword per group pair is $\delta\log n$; On the other hand, when we set $t$ to be the error-correction capability for each group pair, the average communication overhead becomes $t\log n$. If we set the `safety margin' to be too large (say $t=10\delta$), it will incur huge additional communication overhead. Due to this reason, we set a moderate `safety margin' that  $t$ in the range from $1.5\delta$ to $3\delta$. 


\smallskip
\noindent
{\bf Communication Overhead Per Group Pair.} 
%\subsection{Communication Cost Per Group Pair}\label{sec:communication_overhead_single_PBS}
%To correct $d$ bit errors, the length of the net-codeword only is no more than $d\log n$ bits. 
Here we analyze the total communication overhead of the first round of PBS.  Since the vast majority of distinct elements are discovered and reconciled in the first round, 
as will be shown in \autoref{sec:piecewise_decodability}, it represents the vast majority (over $95\%$) of that over all rounds.  
For each group pair $i$, the communication overhead (of running PBS-for-small-$d$ on this pair) in the first round contains the following four components: (1) the BCH codeword that is $t\log n$ bits long; (2) the $\delta_i$ ``bit error locations'' whose total length is $\delta_i\log n$ bits; (3) the  $\delta_i$ \code{XOR} sums whose total length is $\delta_i\log |\mathcal{U}|$ bits; and (4) the checksum that is $\log |\mathcal{U}|$ bits long. Hence the average communication overhead of PBS per group pair in the first round is 


%Formula \autoref{eq:communication_overhead} also roughly equals to the average communication overhead of PBS per group pair in all rounds, since the bulk of the communication overhead %happens in the first round, .

%Since each group pair is reconciled by \autoref{alg:single_round_pbs} in the first round, the communication overhead of a group pair $i$ in the first round corresponds to the steps in 
%\autoref{alg:single_round_pbs}, which consists of the following four components: 

\begin{comment}
For each group pair $i$, There are four components 
\begin{itemize}
	\setlength\itemsep{0.1em}
	\item The BCH codeword that is $t\log n$ bits long
	%(\autoref{step:BCH_encode} in \autoref{alg:single_round_pbs});
	\item The subset pair indices (\autoref{step:send_xor} in \autoref{alg:single_round_pbs}) that are $\delta_i\log n$ bits long;
	\item The bitwise \code{XOR} sums (\autoref{step:send_xor} in \autoref{alg:single_round_pbs}) that are $\delta_i\log |\mathcal{U}|$ bits long;
	\item The checksum (\autoref{step:terminate_condition} in \autoref{alg:single_round_pbs}) that is $\log |\mathcal{U}|$ bits long;
\end{itemize}
\end{comment}



\begin{equation}\label{eq:communication_overhead}
t\log n + \delta\log n +\delta \log |\mathcal{U}|+\log |\mathcal{U}|
\end{equation}

% \begin{itemize}
% 	\setlength\itemsep{0.1em}
% 	\item the BCH codeword that is $t\log n$ bits long;
% 	%(\autoref{step:BCH_encode} in \autoref{alg:single_round_pbs});
% 	\item the $\delta_i$ ``bit error locations" whose total length is $\delta_i\log n$ bits;
% 	\item the  $\delta_i$ \code{XOR} sums whose total length is $\delta_i\log |\mathcal{U}|$ bits;
% 	\item the checksum that is $\log |\mathcal{U}|$ bits long.
% \end{itemize}

% %Hence the total communication overhead in the first round over all $g$ groups is  $gt\log n + d\log n + d \log |\mathcal{U}|+ g\log |\mathcal{U}|$.
% %Since $\delta_i$ is a random variable with mean $\delta$ for $i=1,2,...,g$, 
% Hence the average communication overhead of PBS per group pair in the first round is 
% \begin{equation}\label{eq:communication_overhead}
% t\log n + \delta\log n +\delta \log |\mathcal{U}|+\log |\mathcal{U}|
% \end{equation}

%Formula \autoref{eq:communication_overhead} also roughly equals to the average communication overhead of PBS per group pair in all rounds, since the bulk of the communication overhead happens in the first round, as will be explained in \autoref{sec:piecewise_decodability}.

\begin{comment}
{\bf (previous)} the BCH codeword $\xi_A$ in \autoref{step:BCH_encode}; (2) the subset pair indices $i_1,i_2,...,i_d$ in \autoref{step:trivial_reconcile}; (3) the bitwise \code{XOR} sums of sets $B_{i_1}, B_{i_2},...,B_{i_d}$ of $d\log |\mathcal{U}|$ bits in \autoref{step:trivial_reconcile}; and (4) transmit the $32$-bit checksum of $B$ (i.e., $c(B)$) from Bob to Alice for precomputing $c(A\triangle B)$ in \autoref{step:terminate_condition}. These four components contribute roughly (1) $d\log n$ bits (recall that to ``correct'' $d$ bit errors, the length of the BCH codeword is no more than $d\log n$ bits); (2) $d\log n$ bits; (3) $d\log |\mathcal{U}|$ bits; and (4) $32$ bits respectively to the overall communcation overhead of \autoref{alg:single_round_pbs}. 
\noindent {\bf Communication overhead of PBS Per Group Pair in the first round:} Same as PBS-for-small-$d$, the communication overhead of PBS per group pair in the first round also consists of the four components described in \autoref{sec:communication_overhead_single_PBS}. The expectation of the communication overhead of each component equals to the corresponding component of PBS-for-small-$d$ when $d=\delta$, except for the BCH codeword, which is $t\log n$ bits as we described earlier. The communication overhead of PBS per group pair in the first round on average is roughly
\end{comment}

% \begin{equation}\label{eq:communication_overhead}
% t\log n + \delta\log n +\delta \log |\mathcal{U}|+32
% \end{equation}

% {\bf (previous)} Readers may wonder if we can reduce this additional communication overhead by using some technique to estimate $\{d_i\}_{i=1}^g$ (e.g., ToW estimator in \autoref{subsec:ToW}), so that we can set the error-correction capability of each group more wisely and save some waste on the safety margin. However, to achieve that, the estimation on $\{d_i\}_{i=1}^g$ must be in extremely high precision (since $\{d_i\}_{i=1}^g$ are small numbers with mean of $\delta$), which incurs much larger additional communication overhead than the savings. Due to the same reason (i.e., estimate $\{d_i\}_{i=1}^g$ is costly), we set the number of subset pairs for each group pair to be all equal (denoted as $n$). 
%based on $\delta$ ($n=\Omega(\delta^2)$). 

% {\bf (moved from the small d case)} Note that the set reconciliation process of the group pairs are independent with each other, and each group pair runs as many rounds of PBS-for-small-$d$ as needed to reconcile all distinct elements in it. Therefore, different group pairs may need different number of rounds to be successfully reconciled. Intuitively, we want all group pairs to be successfully reconciled in only a few rounds (say $3$) with high probability (say $99\%$). Hence, when tuning parameters (to be discussed in \autoref{sec:parameter_settings}), we set a {\it target success probability} $p_0$ combined with a {\it target number of rounds} $r$ as the {\it paramenter setting requirement}, which aims to ensure that the {\it success probability}, the probability that all distinct elements (of all group pairs) are reconciled, within $r$ rounds to be at least $p_0$. 
% {\bf Normally, to achieve the same target success probability within fewer rounds (smaller $r$), PBS need more resources (e.g., larger $n$, $t$) for the ideal case happening with higher probability (fewer exceptions happen and need to be handled in later rounds), as we will explain in \autoref{sec:vary_r}.}

% {\bf (moved from the small d case)} Although PBS runs as many rounds as needed to reconcile all distinct elements (in each group pair), we want PBS to successfully reconcile all distinct elements in only a few rounds (say $3$) with high probability (say $99\%$). Hence, when tuning parameters (to be discussed in \autoref{sec:parameter_settings}), we set a {\it target success probability} $p_0$ combined with a {\it target number of rounds} $r$ as the {\it paramenter setting requirement}, which aims to ensure that the {\it success probability}, the probability that all distinct elements are reconciled, within $r$ rounds to be larger than $p_0$. 
% {\bf Normally, to achieve the same target success probability within fewer rounds (smaller $r$), PBS need more resources (e.g., larger $n$, $t$) for the ideal case happening with higher probability (fewer exceptions happen and need to be handled in later rounds), as we will explain in \autoref{sec:parameter_settings}.}

%This success probability (within $r$ rounds) is also the expected value of the {\it success rate} of PBS, which is defined as the number of `successful' experiments (all distinct elements are successfully reconciled within $r$ rounds) divided by the total number of experiments. 

%The requirement above should also ensure the majority of the distinct elements are reconciled in the first round. 
% Note that PBS reconciles the distinct elements gradually round by round. The distinct elements that have been reconciled in the first round are no longer needed to be reconciled again in later rounds. This is the ``piecewise decodability'' mentioned in \autoref{sec:intro_oursolution}. The requirement above also ensures the majority of the distinct elements are reconciled in the first round, as we will show in \autoref{sec:piecewise_decodability}. Therefore, the majority of the overall communication overhead happens in the first round. In other words, the overall communication overhead of all rounds is only slightly larger than ($1.01$ to $1.07$ times of) that in the first round. Due to this reason, we use the communication overhead in the first round (described in \autoref{sec:communication_overhead_single_PBS}) to approximate the overall communication overhead of all rounds in parameter settings (to be elaborated in \autoref{sec:parameter_settings}.


% Like what we did in \autoref{sec:multi-rounds}, we set a paramenter setting requirement on the target success probability $p_0$ of $r$ rounds for all group pairs, which ensures the probability that all group pairs are completely reconciled in $r$ rounds to be larger than $p_0$. The detail about how to set $n$, $g$, and $t$ given such a success probability requirement will be elaborated in \autoref{sec:parameter_settings}. 

% we set a {\it target success probability} $p_0$ of $r$ rounds as a paramenter setting requirement, which aims to ensure the probability that all distinct elements are reconciled in $r$ rounds to be larger than $p_0$. This requirement should also ensure the majority of the distinct elements are reconciled in the first round. Use the same example ($d=5, n=255$), on average $4.81$ out of $5$ distinct elements should be reconciled in the first round. So the total communication overhead in all rounds is only slightly larger than ($1.01$ to $1.07$ times of, as we will show in \autoref{fig:per-round-con}) that in the first round. Due to this reason, we use the communication overhead in the first round (described in \autoref{sec:communication_overhead_single_PBS}) to approximate the total communication overhead of all rounds in parameter settings (to be elaborated in \autoref{sec:parameter_settings}.

% Note that this safety margin incurs additional communication overhead on transmitting BCH codeword: In the perfect scenario (i.e., $\{d_i\}_{i=1}^g$ is precisely known), the average communication overhead on transmitting BCH codeword per group is $\delta\log n$; On the other hand, when we set $t$ to be the error-correction capability for each group, then the average overhead becomes $t\log n$, which is roughly $2.5$ times of that in the perfect scenario (when $t$ is roughly $2.5\delta$). Readers may wonder if we can reduce this additional communication overhead by using some technique to estimate $\{d_i\}_{i=1}^g$ (e.g., ToW estimator in \autoref{subsec:ToW}), so that we can set the error-correction capability of each group more wisely and save some waste on the safety margin. However, to achieve that, the estimation on $\{d_i\}_{i=1}^g$ must be in high precision, which requires a much higher communication overhead than the savings.

% Although PBS may need to run many rounds to reconcile all distinct elements, the communication overhead mostly happens in the first round, since the majority of the distinct elements should be reconciled in the first round. Use the same example ($d=5, n=255$), on average $4.81$ out of $5$ distinct elements should be reconciled in the first round. So the total communication overhead in all rounds is only slightly larger than ($1.01$ to $1.07$ times of, to be shown in \autoref{fig:per-round-con}) that in the first round. Due to this reason, we use the communication overhead in the first round (described in \autoref{sec:communication_overhead_single_PBS}) to approximate the total communication overhead (all rounds) in parameter settings (to be elaborated in \autoref{sec:parameter_settings}).

%For the moment, we assume no ``fake'' distinct element in type (\RN{2}) subset pairs fails to be detected, which happens with overwhelming probability as explained in \autoref{subsec:exception_hash_partition}. Then 

% PBS reconciles the distinct elements gradually round by round. This is the ``piecewise decodability'' mentioned in \autoref{sec:intro_oursolution}. We use the following example to describe it in details: 
% Given two sets with $10$ distinct elements, in the first round, PBS tries to reconcile the $10$ distinct elements and say $6$ out of the $10$ distinct elements are successfully reconciled. Then the $6$ reconciled distinct elements are removed and PBS tries to reconcile the remaining $4$ distinct elements in the second round. Say $2$ out of the $4$ remaining distinct elements are successfully reconciled, and that leaves $2$ remaining distinct elements to be reconciled in the third round, so on so force. 
% % Given two sets $A$, $B$ with $10$ distinct elements, in the first round, PBS hashes them into $7$ distinct subset pairs. $6$ distinct elements are hashed into $6$ distinct subset pairs, and the other $4$ distinct elements are hashed into the same subset pair. Then the former $6$ distinct elements are successfully reconciled in the first round and the later $4$ distinct elements remain to be reconciled in the second round, which are hashed into $3$ distinct subset pairs (under a different hash function). $2$ remaining distinct elements are hashed into $2$ distinct subset pairs, and the other $2$ remaining distinct elements are hashed into the same subset pair. Then the former $2$ remaining distinct elements are successfully reconciled in the second round and the later $2$ remaining distinct elements remain to be reconciled in the third round, so on so force. 
% The dynamics of the number of remaining distinct elements (i.e., $10\leadsto 4\leadsto 2\leadsto \cdots$ in the example) is in nature a Markov chain, which will be elaborated and analyzed in \autoref{sec:single_markov} to derive a tight tail bound of the probability that all distinct elements are reconciled in $r$ rounds. 

%, which we will show in \autoref{subsec:mini-partition}.

% The same algorithmic trick can also be implemented in PinSketch~\cite{Dodis_PinSketch_2008} to reduce it computational complexity from $O(d^2)$ to $O(d)$. However, it will encounter the same randomness problem and have to set up a safety margin on the error-correction capability. This safety margin will incur much more communication overhead on PinSketch than on our scheme: Considering the average communication overhead per group, in our scheme, this overhead can be expressed as $t\log n+\delta\log n+\delta \log u+32$, in which $t\log n$ accounts for the BCH codeword, $\delta\log n$ accounts for the index of the subset pairs, $\delta \log u$ accounts for the bitwise \code{XOR} in \autoref{alg:trivial_case}, and $32$ accounts for the $32$-bit CRC in \autoref{proto:multirounds}. In PinSketch, this overhead increases from $O(\delta\log u)$ (optimal) to $O(t\log u)$ (PinSketch does not need to transmit bitwise \code{XOR}) if it uses the same algorithmic trick. Use the same example in \autoref{sec:intro}, when $\delta=5, n=255, u=2^{32}, t=2.5\delta$, the overhead of PinSketch using the trick is $2.5$ times of the optimal, while that of our scheme is $2.075$ times of the optimal (as we introduced in \autoref{sec:intro_oursolution}). That means our scheme has a lower communication overhead than PinSketch if they both use the algorithmic trick. Furthermore, as the signiture size $\log u$ increases, the advantage of our scheme over PinSketch becomes more significantly, which we will show in \autoref{subsec:mini-partition}.

% In PinSketch, each bit encodes only a single element in the universe, so the size of the bitmap is equal to the size of the universe.  
% For example, in the set reconciliation problem we usually assume each element is ``indexed" by a $32$-bit-long (hash) signature, so the universe contains a total of $2^{32}$ elements. In this case, the bitmap encoding for any set in PinSketch is $2^{32}$ bits long, and the Galois field involved in its BCH decoding is the ``$32$-bit-wide" $GF(2^{32})$.  In contrast, as explained earlier, in PBS 
% %since each bit encodes the oddness or evenness of the cardinality of a subset,   
% the size $n$ of a bitmap is dependent only on $d$, and not on the size of the universe or on the cardinality of the set the bitmap encodes.   For example, as shown in the example above, $n = 255$ is large enough for $d = 5$.  In this case, the BCH decoding operates in the much shorter
% ``8-bit-wide" $GF(2^{8})$.  This shorter ``width" alone in theory translates into roughly $16$ times shorter BCH decoding time, which as will be explained in~\ref{} grows quadratically with the ``width" of the underlying Galois field.  This shorter ``width" also implies four times shorter BCH codeword in PBS than in PinSketch, resulting in lower communication complexity as will be shown in~\autoref{}.

% Note that our scheme only takes 1 round trip delay to both identify the $d$ subset pairs and reconcile them: In the first half, Bob computes and sends PBS to Alice. Then Alice locally identifies the $d$ subset pairs and then initiates the reconciliation ({\it i.e.,} \autoref{alg:trivial_case}) for them, {\it i.e.,} computes the bitwise \code{XOR} of the corresponded $d$ subsets. In the second half, Alice sends the bitwise \code{XOR} of the $d$ subsets with their indexes to Bob. Then Bob can compute the set difference $A\triangle B$ locally.


% We can certainly use some communication-efficient technique to estimate $d_i$ (e.g., \autoref{subsec:ToW}). However, to obtain $d_i$ precisely will require a communication cost almost as large as to reconcile Group $i$. So instead of obtaining $d_i$ and set $c_i$ (i.e., the error-correction capability of Group $i$) equal to $d_i$, we leave the randomness of $d_i$ and set $c_i$ neither too conservative, nor too libertive in the following sense: (1) $c_i$ is not too big (conservative, i.e., $10\delta$) to make the total size of PBS unnecessarily large and incur too much extra communication overhead; (2) $c_i$ is not too small (libertive, i.e., $\delta$) to incur a high probability of insufficient decode capability, which can result in hefty penalties in the latter case of incorrect decoding (will be elaborated in \autoref{sec:BCH_exception}). In our scheme, we set $c_i$ to be $2-3$ times of $\delta$, which will be shown in \autoref{sec:tail_bound} that it is just enough to make the probability of decode failure very small. Meanwhile, we set the error-correction capability of each group ($c_1,c_2,...,c_k$) to be all equal and denote it as $c$. 

%Since the decoding capacity $t$ and the number of subset pairs for each group $n$ are both small constants independent of $d$, therefore, the communication overhead per group is $t\cdot\log n \!=\!O(1)$, which implies a total communication overhead of $O(d)$. Similarly, the total decoding computational complexity is also $O(d)$. 

% \subsection{Exception Handling}\label{sec:exceptions}

% \subsubsection{Exception Handling on Hash-Partition}\label{subsec:exception_hash_partition}

% As we have described in \autoref{sec:hash_partition}, the ideal case does not always happen, which means some subset pair may contain more than 1 distinct elements and cannot be successfully reconciled by \autoref{alg:trivial_case}. Due to the parity encoding, we can classify such subset pair into the following two scenarios:

% \begin{itemize}
%     \item Scenario 1: If a subset pair $(A_i, B_i)$ contains even number ($\geq 2$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be the same and our scheme will not reconcile the subset pair. Hence, the distinct elements in the subset pair will not be reconciled;
%     \item Scenario 2: If a subset pair $(A_i, B_i)$ contains odd number ($\geq 3$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be different and our scheme will reconcile the subset pair using \autoref{alg:trivial_case}. However, as we described in \autoref{subsec:protocol0}, when a subset pair contains more than 1 distinct elements, \autoref{alg:trivial_case} will output the bitwise \code{XOR} of them as the `distinct element', which is not a real distinct element with high probability;
% \end{itemize}

% In both scenarios, the distinct elements in the subset pair cannot be reconciled. Even worse, in the second scenario, a false-positive could happen (i.e., the output of \autoref{subsec:protocol0} is not a real distinct element). For example, if subset pair $(A_i, B_i)$ contains $3$ distinct elements $s_1, s_2, s_3$, then the output of \autoref{alg:trivial_case} is $\tilde{s}_4=s_1\oplus s_2\oplus s_3$, which is normally not a distinct element. The good thing is, the probability of the false-positive is extremely small for small $d$. For instance, if $d=5$ and $n=255$, the probability of the false-positive is $7.6\times 10^{-6}$, which is very small. To further reduce the chance of false-positives, we add a verification step at the end of \autoref{subsec:protocol0} to check whether the output of \autoref{subsec:protocol0} $s$ is a real distinct element or not. The verification step works as follows: Given the output $s$ of subset pair $(A_i,B_i)$, if $s\in\mathcal{U}_i$ (i.e., $h(s)=i$), we consider $s$ as a real distinct element; Otherwise, we consider $s$ as an incorrect output and discard it. 

% Note that if $s$ is a real distinct element of $(A_i,B_i)$, $s$ must be in sub-universe $\mathcal{U}_i$. However, if $s$ is the bitwise \code{XOR} of the distinct elements in $(A_i,B_i)$ (i.e., the second scenario happens), $s$ could be in any sub-universe other than $\mathcal{U}_i$. In fact, if we assume the hash-partition described in \autoref{sec:hash_partition} hashes the elements of $\mathcal{U}$ uniformly, independently, and randomly into $n$ sub-universes, the output $s$ in the second scenario will be in a different sub-universe $\mathcal{U}_j (j\neq i)$ with a high probability of $1-\frac{1}{n}$. Hence, this verfication method can further reduce the probability of false-positives by a factor of $\frac{1}{n}$. Use the same example (i.e., $d=5$, $n=255$), the probability is reduced from $7.6\times 10^{-6}$ to $3\times 10^{-8}$ by this verification method. 

% In some super critical cases (i.e., no false-positive is allowed), we can use a more powerful verification method to completely eliminate false-positives. That is, to check if the output $s$ exists in exactly one of the two sets (i.e., $s\in A\setminus B$ or $s\in B\setminus A$). To do so, Bob transmits $s$ along with an identification bit $\mathbb{1}_{\{s\in B\}}$ to Alice, then Alice checks if $s$ . This method verification costs $d(\log u+1)$ bits of additional communication overhead. In most applications, rigorously $0\%$ probability of false-positives is unnecessary and the probability of the former verification method is small enough, so we use the former verfication method in our evaluation. Based on our observation, the false-positive does not happen even once in our evaluation using the former verfication method.

\subsection{Exception Handling on BCH Decoding}\label{sec:BCH_exception}

Recall that in PBS-for-small-$d$ we need to handle two exceptions:  type (\RN{1}) and type (\RN{2}). 
In PBS-for-large-$d$, we have another exception to worry about.
% This exception arises when $\delta_i$, the number of distinct elements between group pair $i$, 
% is larger than $t$, the universal BCH error-correction capability (for every group pair).  
{\color{red}This exception arises when the number of bit positions where bitmaps $A$ and $B$ in~\autoref{alg:single_round_pbs} 
differ is larger than $t$, the universal BCH error-correction capability (for every group pair).
Note that $\delta_i$, the number of distinct elements between group pair $i$, 
is larger than $t$, the universal BCH error-correction capability is only a necessary condition for this 
exception to happen in reconciling this group pair, 
since type (\RN{1}) and/or type (\RN{2}) exceptions could result in that the 
number of different bits between the corresponding two bitmaps is no more than $t$. 
% In this case, 
When this exception happens,} the BCH decoding would fail (when executing \autoref{step:BCH_decode} in \autoref{alg:single_round_pbs}) 
and the decoder would report a failure.
With $t$ appropriately parameterized as explained earlier, this exception should happen with a small probability to any group pair. 
For example, when $d=\num{1000}$, $\delta=5$ (so that $g=d/\delta=200$), and $t$ is set to the 
optimal value of $13$ ($=2.6\delta$), the probability for this exception to happen to any group pair
is only $6.7\times 10^{-4}$. 

To handle this type of exceptions, we further hash-partition each trouble-causing group pair (whose BCH decoding has failed) 
into $3$ sub-group-pairs and reconcile each of them using PBS-for-small-$d$. 
With this three-way-split, with an overwhelming probability, each sub-group-pair should contain no more than $t$ distinct elements and its BCH decoding operation should be 
successful in the next round.  For example, when $\delta=5$ and $t=13$ (same as in the example above), 
the conditional (upon the event $\{\delta_i>t\}$, which happens with probability $6.7\times 10^{-4}$ as 
just explained) probability for any sub-group-pair to contain more than $t$ distinct elements is only $9.5\times 10^{-10}$. 
{\color{red} Note that splitting a trouble-causing group pair into less than $3$ sub-group-pair cannot achieve such an 
overwhelming probability to guarantee each sub-group-pair has no more than $t$ distinct elements: 
Use the same example ($\delta=5$ and $t=13$), the above conditional probability becomes $0.0012$.} 
All said, if necessary, a trouble-causing sub-group-pair will be further split three-way.


{\color{red}
Like type (\RN{1}) and type (\RN{2}) exceptions, this exception will not result in reconciliation error, but more 
rounds. From~\autoref{thm:corrctness}, we have the following corollary concerning the correctness of PBS-for-large-d. 

\begin{corollary}
Assuming that the verification in~\autoref{step:terminate_condition} of~\autoref{alg:single_round_pbs} is always correct. 
If PBS-for-large-d terminates, the result, {\it i.e.,} the union of the set difference obtained for each group pair, 
is equal to $A\triangle B$.
\end{corollary}

\noindent
{\bf Remarks.}
The number of rounds, for PBS to correctly reconcile all distinct elements, is small (with overwhelming probability), 
since, as explained earlier, the probability that an exception happens is quite low.  
For example, as shown in~\autoref{app:completed-rounds}, 
even when $d$ is as large as $10^5$, in all our experimental instances, 
the number of rounds (for PBS-for-large-d, which we will describe in~\autoref{sec:pbs-for-large-d}) is no mare than $3$ and 
in $81.8$\% of those instances, it is only $2$. 
}


\begin{comment}
There is an additional type of exceptions that arise only from setting the universal error-correction capability $t$. That is, when $\delta_i$, the number of distinct elements in group pair $i$, is larger than $t$, the parity bitmaps $A[1..n]$ and $B[1..n]$ could differ at more than $t$ bit positions (e.g., in the ideal case, $A[1..n]$ and $B[1..n]$ differ at exactly $\delta_i$ bit positions), which exceeds the error-correction capability $t$. If so, the BCH decoding fails in \autoref{step:BCH_decode} in \autoref{alg:single_round_pbs} and the decoder reports a failure. This exception happens with a small probability in each group pair: For example, when $d=1000$, $\delta$ is set to $5$ (so that $g=d/\delta=200$), and $t$ is set to $13$ ($2.6$ times of $\delta$), the probability that this exception happens is only $6.7\times 10^{-4}$. 

Note that $\delta_i$ is a Binomial random variable with mean $\delta$, $t$ is typically $1.5$ to $3.5$ times of $\delta$. Even conditioned upon the event $\{\delta_i>t\}$, $\delta_i$ should be only slightly larger than $t$ with high probability. Hence, after partitioning the $\delta_i$ distinct elements into $3$ sub-group-pairs, each of them should have no more than $t$ distinct elements with overwhelming probability. For example, when $\delta=5$, $t=13$ $(2.6\delta)$, the probability that some sub-group-pair contains more than $t$ distinct elements conditioned upon the event $\{\delta_i>t\}$ is only $9.5\times 10^{-10}$. 
\end{comment}

% The exceptions that happens when the error-correction capability $t$ is sufficient have been discussed and handled in \autoref{subsec:exception_hash_partition} and \autoref{sec:multi-rounds}. In this section, we only discuss the exceptions that are caused by insufficient error-correction capability. That is, when $\delta_i$ (i.e., the number of distinct elements in group pair $i$) is larger than the error-correction capability $t$, the BCH codewords of group pair $i$ differ at $\delta_i$ bit positions in the ideal case, which exceeds the error-correction capability $t$. If so, the BCH decoder cannot decode the bit errors correctly (\autoref{step:BCH_decode} in \autoref{alg:single_round_pbs}) and report a failure. This exception happens with a small probability in each group pair: For example, when $d=1000$, and $\delta$ is set to $5$ (so that $g=d/\delta=200$), and $t$ is set to $13$, the probability that this exception happens is only $6.7\times 10^{-4}$. 


\begin{comment}

{\bf (previous)} To handle this type of exceptions, we further partition each trouble-causing group pair into $3$ sub-group-pairs and reconcile them respectively using PBS-for-small-$d$. 
%Note that $\delta_i$, if is not smaller, should be only slightly larger than $t$ with high probability. Hence, partitioning into $3$ sub-groups is enough to ensure each sub-group has no more than $t$ distinct elements. 
Note that $\delta_i$ is a Binomial random variable with mean $\delta$, $t$ is typically $1.5$ to $3.5$ times of $\delta$. So the probability that some sub-group contains more than $t$ distinct elements conditioned upon $\delta_i>t$ is tiny. 
In the same example above ($d=1000$, $\delta=5$, $t=13$), this conditional probability is $9.5\times 10^{-10}$.%that some sub-group has more than $t$ distinct elements is $9.5\times 10^{-10}$. 
In the next round, each sub-group-pair will hardly encounter this type of expections and can be reconciled by PBS-for-small-$d$ respectively.  More specifically, we add a termination condition of \autoref{alg:3_way_partition} after \autoref{step:BCH_decode} in \autoref{alg:single_round_pbs}.

\begin{algorithm}
\caption{Termination condition when BCH decoding fails}
\label{alg:3_way_partition}

\If{BCH decoding fails\label{step:if1}}
{Hash-partition the group pair into $3$ sub-group-pairs and run PBS-for-small-$d$ for each of them in the next round; Break;}\label{step:term1} 

\end{algorithm}

\end{comment}

% Back to the \autoref{proto:multirounds}, which shows the set reconciliation operations in each round of PBS-basic, this kind of exceptions only affect \autoref{step:reconcile} in \autoref{proto:multirounds}. Now this step needs to check whether BCH decoding is successful or not: If successful, all the operations remain the same; Else, we hash-partition the group ($A$ and $B$) into $3$ sub-groups and reconcile them respectively using \autoref{proto:multirounds}. 
% {\bf I'm not sure if it is necessary to discuss this case, since PinSketch did not mention it, even it may happen in PinSketch}
% Another type of exceptions that happens when $d_i>t$ is, the BCH decoder mistakes the decoding is successful and returns $t$ incorrectly decoded bit errors (i.e., subset pairs). The probability of this type of exceptions is very small. For instance, when $d=1000, \delta=5, t=13$ $(2.5\delta)$, $d_i>t$ happens with probability roughly $6.7\times 10^{-5}$, and the probability that the BCH decoder mistakes the decoding is successful when $d_i>t$ is on the order of $10^{-7}$ \cite{kim1996undetected}. So the probability that this type of exceptions happens in each group is on the order of $10^{-12}$. On the other hand, the impact of this type of exceptions is insignificant. Assume an incorrectly decoded bit error corresponds to a random subset pair, which could contain (1) no distinct element; (2) exactly $1$ distinct element; or (3) more than $1$ distinct elements. Reconcile the subset pair using \autoref{alg:trivial_case} could (1) get nothing and waste $\log |\mathcal{U}|$ bits of communication overhead; (2) get an actual distinct elements; or (3) trigger the exceptions that were discussed and handled in \autoref{subsec:exception_hash_partition}. 

\input{section/multiround_pbs_large_d}



% \subsection{What If PinSketch Also Uses Partitions?}\label{sec:whatifpinsketch}

% {\color{red} Moved to related work section.}

% Arguably, the same algorithmic trick (i.e., hash-partition two sets each into groups) can also be applied to PinSketch~\cite{Dodis_PinSketch_2008} for reducing its BCH decoding computational complexity from $O(d^2)$ to $O(d)$.   Doing so however makes the communication overhead of PinSketch higher than that of PBS for the following reason.
% As just explained, we need to leave a safety margin in setting the BCH error-correction capacity $t$, in the sense that $t$ needs to be ``comfortably'' larger than $\delta$, the average number
% of ``bit errors''.   
% %In other words, the amount of safety margin is $t - \delta$.  
% Hence for each group pair, the average additional communication overhead (incurred for transmitting a longer BCH codeword) of leaving this safety margin
% is $(t-\delta)\log n$ in PBS and is $(t-\delta)\log |\mathcal{U}|$ in PinSketch.
% However, as explained in \autoref{subsec:pbs-vs-pinsketch}, $\log n$ (the Galois field ``width" in PBS) is typically $3$ to $4$ times smaller than $\log |\mathcal{U}|$ 
% (the Galois field ``width" in PinSketch).  Hence PinSketch pays $3$ to $4$ times more for leaving the safety margin, resulting in a higher overall communication overhead.  
% For example, when $\delta=5, n=255, |\mathcal{U}|=2^{32}, t=2.6\delta$ (same as in the example in \autoref{sec:BCH_exception}), the communication overhead of PinSketch using hash-partitioning 
% is $2.6$ times the theoretical minimum, whereas that of PBS is $2.1$ times the theoretical minimum. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%It means PBS could have a lower communication overhead than PinSketch if they both use the algorithmic trick. 
% needs to be ``comfortably" larger than $\delta$

\begin{comment}
This ``safety margin'' will incur much more additional communication overhead on PinSketch than on PBS

However, since the BCH error-correction capability $t$ needs to be ``comfortably" larger than $\delta$, 

it will encounter the same randomness problem and have to set up a ``safety margin'' on the error-correction capability $t$. This ``safety margin'' will incur much more additional communication overhead on PinSketch than on PBS: Considering the average communication overhead per group pair, the additional overhead caused by the ``safety margin'' is $(t-\delta)\log n$ in PBS and $(t-\delta)\log |\mathcal{U}|$ in PinSketch. The latter is roughly $4$ times of the former when $n=255, |\mathcal{U}|=2^{32}$. Recall that the theoretical minimum amount of communication overhead to reconcile $\delta$ distinct elements is $\delta\log |\mathcal{U}|$. Use the same example in \autoref{sec:intro}, when $\delta=5, n=255, |\mathcal{U}|=2^{32}, t=2.5\delta$, the overhead of PinSketch using the algorithmic trick is $2.5$ times of the theoretical minimum, while that of PBS is $2.075$ times of the theoretical minimum. It means PBS could have a lower communication overhead than PinSketch if they both use the algorithmic trick. 
\end{comment}

%{\bf Furthermore, as the signiture length $\log |\mathcal{U}|$ increases, the advantage of PBS over PinSketch will be more significant.}

% We handle this type of exceptions by the same method (i.e., hash-partition into $3$ sub-groups) as above. To detect them, on the other hand, is simple: Note that incorrect decoded bit errors correspond to the subset pairs that do not contain distinct elements. When we reconcile those subset pairs in \autoref{sec:reconcile_by_trivial}, the output (i.e., reconciled elements) will be $\mathbf{0}$, which is abnormal (since $\mathbf{0}\notin A\bigcup B$, as we described in \autoref{subsec:protocol0}). Hence, this type of exceptions happen if and only if one of the reconciled distinct elements is $\mathbf{0}$. 
%Hence, we consider BCH decoding is successful by two criteria: (1) the BCH decoder reports a successful decode; and (2) None of the reconciled elements is $\mathbf{0}$. 
% ========================
% In fact, even if $d_i>t$, PBS-basic is still possible to reconcile group $i$ in some nonideal cases. For example, when $t=10$ and $d_i=11$, if the $11$ distinct elements are distributed in $10$ subset pairs, such that $1$ subset pair contains $2$ distinct elements and $9$ subset pairs contain $1$ distinct element in each, the two parity bitmaps differ at only $9$ bit positions. So BCH decoder is able to decode the later $9$ subset pairs and the corresponding $9$ distinct elements can be reconciled. In the second round, only $2$ distinct elements remain and BCH decoding certainly works. In this case, we do not need to partition the group into sub-groups, and this case does not trigger \autoref{alg:3_way_partition} in PBS. 
% ========================
% Instead, it will either (1) report a failure about exceeding the error-correction capability; or (2) mistake the decoding is successful and return incorrect decoded bit errors. 

% The second case happens with a very small probability (in order of $10^{-7}$ \cite{kim1996undetected}) and is very simple to detect : 

% The first case is easy to handle: We can simply adapt the same algorithmic trick to partition the group into smaller groups and reconcile them respectively. In our scheme, we set the number of smaller groups to be $3$, which is big enough because $d_i$, if not smaller, only slightly larger than $t$ with high probability. The second case on the other hand, although theoretically possible, happens with a very small probability when $d_i>t$ (in order of $10^{-7}$ \cite{kim1996undetected}). Besides, the probability of $d_i>t$ is also very small (e.g., when $t=15$ and $\delta=5$, this probability is about $2.3\times 10^{-4}$), so the overall probability of the second case, which is the multiplication of these two small numbers, is negligible (e.g., in order of $10^{-11}$).

% \subsection{Multi-rounds}

% Even if the ideal case does not happen, most of the distinct elements should be distributed into different subset pairs and therefore can be reconciled. So our scheme, even cannot reconcile all of the distinct elements, can still reconcile the majority of them (piecewise decodability). To reconcile the rest distinct elements, we can just run our scheme for multi-rounds under different hash-partition functions. For each round, our scheme works as follows: 

% \IncMargin{1em}
% \begin{algorithm}
% \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
% \Input{Two sets $A$ and $B$}
% \Input{Size of set difference $d$}
% \Input{The number of subset pairs $n$}
% \Input{BCH error-correction capability $t$}

% Hash-partition $A$ and $B$ into $n$ subset pairs $\{(A_i,B_i)\}_{i=1}^n$;

% \If{BCH decoding fails}
% 	Hash-partition $A$ and $B$ into $3$ subset pairs and reconcile them respectively in the next round\;
% \ElseIf{BCH decoding success}
	
% \Else{}

% $k \leftarrow \lceil \frac{t}{c}\rceil $\;

% Partition elements into $k$ subsets using~\autoref{alg:random-part}\;

% \For{$j = 0$ \KwTo $k-1$}{
%     Reconcile the $j$-th subset pair using the straw-man scheme with the BCH correcting capability $\tau$, number of smaller subsets $m$, and number of rounds $r$\;
% }

% \caption{PBS (per round)} \label{proto:II}
% \end{algorithm}\DecMargin{1em}

% This {\bf multi-rounds} scheme can significantly increase the success probability (i.e., the probability that all distinct elements are reconciled). Readers may wonder in the later rounds, most distinct elements should be reconciled, and the remaining could be reconciled using degraded parameters (i.e., smaller $n$ and $t$). In fact, degrade parameters in later rounds cannot save much communication overhead, since the majority of it is spent in the first round (i.e., $>90\%$). Therefore, we use the same parameters (i.e., $n,t$) among all rounds in our evaluation. 
% %The tradeoff between the number of rounds and the communication overhead per rounds will be elaborated in \autoref{sec:tail_bound}. In our evaluation, $r=2,3$ rounds are enough to achieve an extremely high success probability. 

% Readers may think the cost (i.e., communication overhead and the computational complexity) of this multi-rounds scheme is proportional to the number of rounds (denoted as $r$) and increases linearly with $r$. In fact, the cost of each round is roughly proportional to the number of remaining distinct elements, which decreases exponentially as $r$ increases (i.e., the first round reconciles $99\%$ of distinct elements, the second round reconciles $99\%$ of the remaining $1\%$ distinct elements, etc.). So the cost of this multi-rounds scheme is only slightly larger than that of the single-round scheme. Furthermore, as we explained in \autoref{sec:intro}, {\bf from intro thanks for the piecewise decodability of our solution, in almost all practical application scenarios, this tradeoff does not lead to longer response time because the reconciliation of objects identified by the successfully decodable codewords, which constitute the vast majority of all codewords, can run in parallel with the transmissions and decodings of the rest.  In other words, the piecewise decodability effective masks the slightly larger number of communication rounds as far as the response time is concerned.} 





\begin{comment}
\subsubsection{Random Partition}

\IncMargin{1em}
\begin{algorithm}
% \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
% \Input{Set $S$}
% \Input{The number of subsets $m$ for partition}
% \Output{Subsets $S_1, S_2, ..., S_m$}

% Generate hash function $h(\cdot)$ that maps each element into $\{1,2,...,m\}$;

\ForEach{$s \in S$}{
    $j \leftarrow h(s) \bmod m$\;    
    Insert $s$ into the $j$-th subset $S_j$\;
}

\caption{Partition using hash function $h(\cdot)$.} \label{alg:random-part}
\end{algorithm}\DecMargin{1em}

Like the strawman scheme, our scheme randomly partitions sets $A$ and $B$ into $m$ subsets. This random partition 
can be easily accomplished by using some hash function, $h(\cdot)$, and inserting each element $x$ into the subset 
corresponding to $h(x)$. \autoref{alg:random-part} presents the pseudo-code of this random partition using hash 
function $h(\cdot)$.  

% Unlike the strawman scheme, our scheme only reconciles those subset pairs that need to be reconciled, 
% because 



Like the strawman scheme, our scheme hash-partitions the two sets $A$ and $B$ into $m$ subset pairs $(A_i, B_i)$ for $i=1,2,\cdots,m$. 
We note that, among those $m$ bins (subset pairs), 
at most $t$ ($t\!\ll\!m$ as shown in our analysis in~\autoref{subsec:protocol1}) bins contain balls 
(elements belonging to the set difference), {\it i.e.,} requiring reconciliation.  
Motivated by this observation, we, therefore, propose to first detect those bins that 
contain balls and then only reconcile them. The detection is solved with a simple encoding approach that 
will be detailed in the next section.

\subsubsection{Detection before Reconciliation} 

In fact, identifying those non-empty bins is easy when each bin contains at most one ball. In this section, we assume that 
each bin after the random partition contains at most one ball, we will show later how to handle the cases when some 
bins contain more than one balls later in~\autoref{subsec:exceptions}. 

Given an arbitrary bin (say subset pair $(A_i, B_i)$) that contains one ball ({\it i.e.,} $A_i\triangle B_i$ contains exactly one element), 
the corresponding two subsets $A_i$ and $B_i$ differ exactly one element, which implies that 
$||A_i|\!-\!|B_i||\!=\!1$. Hence, if $|A_i|$ ({\it i.e.,} number of 
elements in $A_i$) is odd (or even), then $|B_i|$ must be even (or odd). In other words, the odevity of $|A_i|$ 
and $|B_i|$ are opposite. %differs if $|A_i\triangle B_i|\!=\!1$. 
Based on this property, we propose the {\it odevity encoding}: 
A subset is encoded as ``1'' if it contains odd number of elements, and as ``0'' otherwise. 
Using this odevity encoding, the $m$ subsets of $A$ can be encoded as a bit string $b_A$ in $\{0,1\}^m$, 
where the $i$-th bit in $b_A$ corresponds to the odevity encoding of $|A_i|$. Similarly, the $m$ subsets of $B$ can also 
be encoded as a bit string $b_B$. Clearly, $b_A$ and $b_B$ differ at $t$ different positions, or in other words, 
the Hamming distance of bit strings $b_A$ and $b_B$ is $t$. A straightforward approach is 
to let Alice send $b_A$ to Bob, and then Bob compares $b_B$ against $b_A$ to obtain those non-empty bins. 

This approach, however, has a communication overhead of $m$ bits, which is still unnecessarily high. As 
analyzed in~\autoref{subsec:protocol0}, $t$ is usually much smaller than $m$. 
That means $b_A$ and $b_B$ differ only at a tiny portion of bits. %have much more in common than differences. 
Therefore, if we view $b_B$ as a corrupted message of $b_A$ with $t$ corrupted bits, the detection of those $t$ bins can be converted to 
the detection of the positions of the $t$ corrupted bits. The latter can be solved using an Error-Correction Code (ECC)~\cite{Lin_ErrorControlCoding_1983} that can correct up to $t$ errors. In this work, we use the BCH code~\cite{Lint_IntroductionCodingTheory_1998}. 
More precisely, this ECC-based approach (with the BCH code) works as follows. 
Alice computes the parity bits for $b_A$ using a $t$-error-correcting BCH code with a block length of 
$(2^{\lceil \log m\rceil} -1)$ and sends the parity bits to Bob. Bob then decodes the positions of the $t$ corrupted bits 
using the BCH decoding algorithm with $b_B$ and those parity bits received from Alice. The communication overhead of 
this approach is roughly $t\lceil \log m\rceil$ ($=O(t\log t)$) bits. In the example above, this communication overhead is 
roughly $\num{17000}$ bits, which is approximately $6$ times lower 
than $m\!=\!\num{108469}$ bits, the communication overhead of the aforementioned straightforward approach. 

At first sight, it seems that the detection of non-empty bins and reconciliation of subsets in those bins require two rounds 
(or at least two round trip delays), {\it i.e.,} one round for detection and the other for reconciliation. In fact, 
it only requires one. After Bob receives the parity bits from Alice and decodes out those non-empty bins, it initiates 
the reconciliation ({\it i.e.,} \autoref{alg:trivial_case}) for each bin (subset pair) immediately, 
{\it i.e.,} sends the \code{XOR} sums of subsets in those bins together the indexes of those bins. 
After receiving those \code{XOR} sums and bin indexes, Alice can compute the set difference. 

% A naive way to combine the detection of non-empty bins and reconciliation of subset pairs in those bins is to first detect 
% those non-empty bins via one round of message exchanges between Alice and Bob and then to reconcile the corresponding 
% subset pairs in those bins with another round of message exchanges. This requires two rounds ({\it i.e.,} taking at least 
% two round trip delays). In fact, after Bob receives the parity bits from Alice and obtains those 

\subsubsection{Multiple Rounds}\label{sec:multiround}

{\bf This section was not clear enough. I need more time to think about and revise it.}


In the above section, we have assumed that each bin contains at most one ball. 
However, even with a sufficient large $m$, some bin might contain more than one balls though with tiny probability. 
We will show in~\autoref{subsec:exceptions}, how such rare events, {\it i.e.,} one bin contains more than one balls, 
can be easily detected.
To ensure our scheme can successfully reconcile all elements even when such rare events happen, 
we propose to use multiple rounds (of communication between Alice and Bob). More precisely, instead of 
selecting a prohibitively large $m$ to ensure that each bin contains at most one ball with a extremely high probability 
(say 0.99999), we select a reasonably large $m$ so that the communication overhead is not very high and very few bins contain 
more than one balls (or in other words, most bins contain at most one ball). Therefore, after running one round of 
our scheme, most elements in the set difference will be reconciled. Only those in the bins that contain more than one balls 
fail to be reconciled. For elements in the subsets corresponding to those bins, we run another round of our scheme. 
If some elements still fail to be reconcile, we can run one more round of our scheme. So on so forth,  
our scheme can keep running for more rounds until all elements are reconciled. 

With the same communication overhead, multiple rounds can significantly increase the success rate, 
{\it i.e.,} the probability that all elements in the set difference will be successfully reconciles, 
which will be elaborated in~\autoref{sec:tail_bound}. 

% % to be emphasized
% % say that too many rounds should be avoided (latency & communication overhead reduction is negligible when r is too large, 2 - 3 is good enough)
% % multiple rounds is not an issue when r is small

% We note that the number of rounds $r$, however, should not be large. On one hand, it results in large latency (at least $r$ round trip delays). 
% On the other hand, when $r$ is large, the reduction of communication overhead by the increase of $r$ gradually diminishes. 

We note that multiple rounds, when $r$ is small, would not really increase the ``latency'', as long as most elements in the 
set difference can be reconciled in the first rounds, since the underlying synchronization of data objects corresponding to 
those elements can start immediately after the first round of our scheme. Therefore, the actual latency is one round trip delay instead of 
$r$. 

As we mentioned, this straw-man protocol works correctly if each subset pair has at most one exclusive element (i.e., \autoref{eq:requirement_strawman} holds). On the other hand, if a subset pair has more than one exclusive elements, some of which will not be successfully reconciled:

\begin{itemize}
\item If a subset pair has even number of exclusive elements, Odevity coding will encode it as 0. Then the straw-man scheme will consider the subset pair having no exclusive element and all exclusive elements in this subset will not be reconciled;

\item If a subset pair has odd number ($\geq 3$) of exclusive elements, Odevity coding will encode it as 1 and consider the subset pair having only 1 exclusive element. Then the straw-man scheme will use \autoref{alg:trivial_case} to decode only one exclusive element and dismiss all others. Even worse, the only decoded element is probably not a real exclusive element, since the element computed by \autoref{alg:trivial_case} is the \code{XOR} sum of all exclusive elements, not one of them. 
\end{itemize}

In summary, if a subset pair has more than one exclusive elements, most of its exclusive elements cannot be reconciled, and the reconciled element is usually incorrect (i.e., false-positive). The false-positive however is easy to check, which will be elaborated in \autoref{subsec:exceptions}. The good thing is, even if not all subset pairs have at most one exclusive element and are successfully decoded, most of them will be w.h.p.. In other words, even if the straw-man protocol cannot reconcile all exclusive elements, it still can reconcile most of them. To reconcile all exclusive elements w.h.p., we can simply extend the single-round straw-man scheme to multi-round. And each round adapts the straw-man scheme to do set reconciliation using independent hashing functions $h(\cdot)$ for partition (i.e., in \autoref{alg:random-part}). This multi-round extension can significantly increase the probability of a successful reconciliation, which will be elaborated in \autoref{sec:tail_bound}. 



\subsection{Our Scheme: The Final Version}\label{subsec:protocol2}

{\bf Under revision~}

The preliminary version of our scheme suffers from two major drawbacks. 
First, its communication overhead is asymptotically 
$O(t\log m)\!=\!O(t\log t)$, which is not asymptotically optimal. 
Second, the decoding computational complexity is proportional to 
$t^2$ with the state-of-the-art decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} for BCH codes, 
which is too high when $t$ is large. 
To overcome these two drawbacks, we use a simple algorithmic trick: divide and conquer. With this algorithmic 
trick, the decoding computational complexity is reduced to $O(t)$, 
and the communication overhead is reduced to $t\cdot\frac{\log u}{8} \!+\! O(t)$ (with a small 
hidden constant roughly varying from 4 to 8) bytes which implies that 
our scheme has an additive communication overhead (compared to the optimal scheme) 
of 4 to 8 bytes per element in the 
set difference and this additive overhead is independent of the key size ({\it i.e.}, $\log u$). 
Recall that the IBF-based schemes usually have a communication overhead of roughly 6 times of the 
optimal scheme, which increases linearly as the key size. Therefore, our scheme is much more 
communication-efficient. 

Now, we describe in detail this algorithmic trick. We let Alice divide elements in $A$ into $\lceil\frac{t}{c}\rceil$ groups (subsets)  
for some small constant $c$ (say $5$) so that each group contains roughly $c$ elements from the set difference on average. We let Bob do the same operations on $B$. To ensure that any common element ({\it i.e.,} any element $x\!\in\! A\bigcup B$) goes into 
the same group ({\it i.e.,} groups at Alice and Bob with the same index), we can use the partition procedure with a hash function shown 
in~\autoref{alg:random-part}. Then, we can apply the preliminary version on each group with a constant $m$ (say $m\!=\!256$) independent of 
$t$. To ensure that each group can be reconciled with a high probability, we need to use BCH codes whose decoding capacity 
larger than $c$ (say $\tau\!=\!2c$), as exact number of elements to be reconciled could be larger than $c$. 
Since this decoding capacity $\tau$ is still a small constant independent of $t$, therefore, the communication 
overhead per group is $\tau\cdot\log m \!=\!O(1)$, which implies a total communication overhead of $O(t)$. 
Similarly, the total decoding computational complexity is also $O(t)$. 

\subsubsection{Parameter Configurations} 

Our scheme now has several parameters: $c$ (average number of elements from the set difference in each group), 
$\tau$ (the correcting capability of the BCH code), $m$ (number of bins for each group), and $r$ (maximum number of rounds). 
We note that the maximum number of rounds $r$ is usually associated with another parameter $p$ the desired success rate: With 
at most $r$ rounds, our scheme should guarantee that the success rate is at least $p$. 
%How to tune these parameters to achieve favorable performance will be detailed later in~\autoref{sec:tail_bound}. 
Here, we provide some guidances for the parameter configurations using our theoretical analysis, which gives the tail bound of 
the success probability of our scheme and will be shown in~\autoref{sec:tail_bound}. 

\noindent
{\bf Parameterizing $c$ and $r$.} The values of $c$ and $r$ are usually provided by users based on the requirements of 
applications. For the value of $c$, a larger $c$ results in a longer decoding time yet lower communication overhead.  
So if the decoding time is a big concern, then a smaller $c$ (say $c=5$) should be used; otherwise, a larger $c$ could be used. 
For the values of $r$, a larger $r$ leads to lower communication overhead and usually lower decoding time (as it allows to use 
a smaller $\tau$), however, the reduction is marginal when $r>3$. Therefore, we suggest users to configure $r$ to be $2$ or $3$. 
% The configuration of $c$ is relatively straightforward, as a larger $c$ will result in 
% a longer decoding time and a slightly lower communication overhead. The former is ..., The latter is slightly tricky. 


\noindent
{\bf Using $c$ and $r$ to parameterize other parameters.} After users specify the values for $c$ and $r$ (associated with a value for 
$p$), we can use our theoretical analysis in~\autoref{sec:tail_bound} to parameterize $\tau$ and $m$. 
Since in a BCH code, the block length is in the form of $2^q-1$, we only need to consider $m=2^q-1$. 

{\bf Liang, please revise the following algorithm!}

\begin{algorithm}
\SetKwProg{Proc}{}{}{end}
\SetKwFunction{algo}{\small Search}

\Proc{Search($c$, $r$, $p$)}{\label{search:entrance}

$\mbox{co}_{best}\leftarrow\infty$\tcc*{\small Best communication overhead}

\For{$\tau \leftarrow c\,\KwTo\, \infty$}{}



}
\end{algorithm}


% , unlike 
% the IBF-based schemes which have an multiplicative overhead of 6 
% The inspiration is from the famous 
% divide and conquer algorithm for the selection problem, in which, given an array with $n$ elements, we want to get the $k$-th largest 
% element. A straightforward idea for this problem is sorting. However, if using insertion-sorting, the complexity would be $O(n^2)$. 
% Then the famous divide and conquer trick comes. It first divides the array into $\lceil n/5\rceil$ groups so that the first 
% $\lfloor n/5\rfloor$ contains $5$ elements and at most one group contains the rest $n \mod 5$ elements, and find the median of each 
% group using the insertion-sorting and th


% This straw-man scheme still has a problem on decoding computational complexity. More specific, the complexity increases dramatically with the total number of corrupted bits $t$. Therefore, when $t$ is moderate or large, the decoding computational complexity could be very high. For instance, the decoding complexity of BCH codes~\cite{Lint_IntroductionCodingTheory_1998} is $O(t^3)$, which could be quite high for a large $t$. To keep the decoding complexity reasonably low, we design the following two-layer protocol: In the first layer, we use a hash function to partition the two sets into $\lceil\frac{t}{c}\rceil$ subsets for some small constant $c$ (say $5$), just like the first step of our straw-man scheme. The objective, which is however different from before, is to make each subset pair contains roughly $c$ exclusive elements on average. In the second layer, we use the straw-man scheme with the same configuration (number of subsets $m$, and error-correction capability $\tau$, number of rounds $r$) to reconcile each subset pair. 

% In fact, the straw-man scheme is a proper solution when $t$ is small. First, the decoding complexity will not be a problem for a small $t$; Second, we do not need an extremely large $m$ to guarantee \autoref{eq:requirement_strawman} w.h.p.. For instance, when $t=5$ and $m=1024$, \autoref{eq:requirement_strawman} holds with probability $\frac{m\,!}{(m-t)\,!m^t}\approx 99\%$. This motivates us to design the following two-layer protocol: In the first layer, we use a hash function to partition the two sets into $\lceil\frac{t}{c}\rceil$ subsets for some small constant $c$ (say $5$), just like the first step of our straw-man scheme. The objective, which is however different from before, is to make each subset pair contains roughly $c$ exclusive elements on average. In the second layer, we use the straw-man scheme with the same configuration (number of subsets $m$, and error-correction capability $\tau$) to reconcile each subset pair. 

\autoref{proto:II} shows the pseudocode of our scheme. It first uses the same hash-function based random partition algorithm as \autoref{alg:random-part} to partition elements into $k\triangleq\lceil \frac{t}{c} \rceil$ subsets. Note that the random partition only guarantees that each such subset 
contains $c$ exclusive elements on average, and the exact number is not known. Hence, our scheme uses a BCH code with a capability of 
correcting up to $\tau$ errors with $\tau > c$ to make sure that the BCH code has a high probability to decode successfully. We will describe how to deal with situation where the size of set difference exceeds $\tau$ later in~\autoref{subsec:exceptions}.

As the decoding of a $\tau$-error-correcting BCH code where $\tau$ is a small constant has a constant-time computational complexity, the decoding complexity of 
our scheme is $O(k)=O(t)$. We now have several parameters, average number of exclusive elements in each subset $c$, the correcting capability $\tau$ of BCH code, the number of smaller subsets $m$ for each subset to be divided to, and the number of rounds $r$. How to tune these parameters to achieve favorable performance will be detailed later in~\autoref{sec:tail_bound}. 

\IncMargin{1em}
\begin{algorithm}
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
\Input{Size of set difference $t$}
\Input{The number of subsets $m$ for each partition}
\Input{Average number of exclusive elements in each partition $c$}
\Input{BCH code capability $\tau$}

$k \leftarrow \lceil \frac{t}{c}\rceil $\;

Partition elements into $k$ subsets using~\autoref{alg:random-part}\;

\For{$j = 0$ \KwTo $k-1$}{
    Reconcile the $j$-th subset pair using the straw-man scheme with the BCH correcting capability $\tau$, number of smaller subsets $m$, and number of rounds $r$\;
}

\caption{Our Scheme} \label{proto:II}
\end{algorithm}\DecMargin{1em}




\subsection{Exceptional Handling}\label{subsec:exceptions}

{\bf To be revised~}

In this section, we will elaborate how to handle the following two types of exceptions that we mentioned in \autoref{sec:multiround} and \autoref{subsec:protocol2}:
\begin{itemize}
    \item Exception 1: A subset pair has odd number ($\geq 3$) of exclusive elements and causes false-positives (i.e., a decoded distinct element is not a real one);
    \item Exception 2: A subset pair contains too many exclusive elements, such that a BCH code with capability of correcting up to $\tau$ errors cannot decode it (i.e., $t>\tau$).
	\item Exception 3: A subset pair has even number ($\geq 2$) of exclusive elements and causes false-negatives(i.e., two or more distinct elements are neglected as the parity bit is 0);
\end{itemize}

To handle Exception 1, we need to check whether a computed exclusive element by \autoref{alg:trivial_case} is a real exclusive element or not. (The group index happens to come in handy if we use it as a fingerprint of the element we computed. If this element is truly an exclusive element, it should be hashed into the same group as before. Notably, We have two group indices available for this check, one is in the initial divide and conquer phase, the other is in the BCH code part) It can be easily done at the end of set reconciliation, during which two hosts exchange their exclusive elements. In fact, as we will elaborate in \autoref{sec:tail_bound}, Exception 1 hardly happens if we set parameters properly. 

On the other hand, when Exception 2 happens, the BCH decoder will report a failure about exceeding the error-correction capability. For such a subset pair, we can use the same approach as in \autoref{subsec:protocol2} to partition it into smaller subsets and use the straw-man scheme to reconcile them respectively. We set the number of small subsets to be 3. It is because, as we will elaborate in \autoref{sec:tail_bound}, the number of exclusive elements for each subset pair $t$ should be, if not smaller, only slightly larger than $\tau$ w.h.p.. Partitioning those exclusive elements into 3 small subsets is enough to guarentee that each of them has less than $\tau$ exclusive elements.

\end{comment}

==> section/pbs_small_d.bk.0719.tex <==
%\section{PBS for small \texorpdfstring{$d$}{d}}\label{sec:scheme}
\section[PBS for small \texorpdfstring{$d$}{d}]{PBS for small \texorpdfstring{\larger\boldmath\MakeLowercase{$d$}}{d}}\label{sec:scheme} 

In this section, we describe how the PBS scheme allows Alice and Bob to reconcile their respective sets $A$ and $B$, where $d\!=\!|A\triangle B|$ is assumed to be small and precisely known. 
%Throughout this paper, we call each element in $A\triangle B$ a \textit{distinct element}, and each element in $A\bigcap B$ a \textit{common element}. 
We start with the trivial case where $d\!\leq\! 1$ in \autoref{subsec:protocol0} and then generalize the scheme for the case where $d$ is a small number in \autoref{sec:pbs_smalld}. 
{\color{red}As will be explained later in~\autoref{sec:BCH_code}, the latter will use the former as a building block.}
% We build up our scheme gradually by starting with the trivial case where $d\leq 1$ in \autoref{subsec:protocol0}. Then we generalize our scheme to the case where $d$ is a small number in \autoref{sec:pbs_smalld}. 

\begin{comment}
\subsection{Problem Statement}\label{sec:model}

In this work, we adopt the commonly used model for the set reconciliation problem. 
Two remote sets $A$ and $B$ are stored at hosts Alice and Bob respectively. 
Each element in $A$ and $B$ is a hash signiture in the key space (universe) $\mathcal{U}$, which is the set of all $(\log |\mathcal{U}|)$-bit binary strings. 
%Each element in $A$ and $B$ is a hash signiture with signiture width $w$ in the key space (universe) $\mathcal{U}$, which is the set of all $w$-bit binary strings (i.e., $|\mathcal{U}|=2^w$). 
%We use $\mathcal{U}$ to denote the set of all $w$-bit binary strings and name it the universe of signitures. 
The set reconciliation problem is to compute the symmetric set difference between $A$ and $B$, 
{\it i.e.,} $A\triangle B\triangleq (A\!\setminus\! B) \bigcup (B\!\setminus\! A)$. 
Let $d\!=\!|A\triangle B|$ be the cardinality of this difference.
%We denote $d\!=\!|A\triangle B|$. 
Throughout this paper, we call each element in $A\triangle B$ a \textit{distinct element}, and each element in $A\bigcap B$ a \textit{common element}.
{\bf Like in all existing solutions, we describe only {\it unidirectional} set reconciliation, in which Alice or Bob learns the set difference $A\triangle B$. Since the performance of our scheme does not depend on who learns the set difference, we assume Bob learns the set difference $A\triangle B$ in the rest of the paper, as mentioned in \autoref{sec:psea}.}
% As mentioned in \autoref{sec:psea}, we describe {\it unidirectional} set reconciliation that Bob learns the set difference $A\triangle B$. 
%In \autoref{sec:evaluation}, we use the same semantic to measure the communication cost of our scheme and other compared set reconciliation schemes. 
\end{comment}

\subsection{The Trivial Case of \texorpdfstring{\larger\boldmath $d\leqslant 1$}{d<2}}\label{subsec:protocol0}

%We start with the trivial case, in which $A$ and $B$ have at most one distinct element ({\it i.e.,} $d\leq 1$), we have a simple set reconciliation scheme showed in \autoref{alg:trivial_case}:
\begin{algorithm}
\caption{Set reconciliation when $d\le 1$}
\label{alg:trivial_case}

{\it Bob}: $s_B\leftarrow\underset{b\in B}{\oplus} b$; Send $s_B$ to Alice\; \label{alg1:sender}

{\it Alice}: $s_A\leftarrow\underset{a\in A}{\oplus} a$; $s\leftarrow s_A \oplus s_B$\; \label{alg1:receiver}
\end{algorithm}

\autoref{alg:trivial_case} shows the set reconciliation scheme for the trivial case, in which $A$ and $B$ differ by at most one (distinct) element. 
It consists of two steps. First, Bob calculates the \code{XOR} sum $s_B$, the bitwise-\code{XOR} of all elements in $B$, and sends it to Alice. 
Second, Alice calculates $s_A$, the \code{XOR} sum of all elements in $A$.  Upon receiving $s_B$ from Bob, Alice computes $s\!\triangleq\! s_A \!\oplus\! s_B$. 
The value of $s$ tells Alice which of the following two cases happens.
%Depending on whether $A$ and $B$ have a distinct element, there are  two possibilities:

\begin{sitemize}
	\item Case (\RN{1}): If $s=\mathbf{0}$, which implies $s_A=s_B$, Alice concludes that $A$ and $B$ have no distinct element or $A=B$. 
	Here $\mathbf{0}$ denotes the $\log |\mathcal{U}|$-bit-long all-$0$ string;
	\item Case (\RN{2}): If $s\not=\mathbf{0}$, which implies $s_A\not=s_B$, Alice concludes that $A$ and $B$ have exactly one distinct element which is $s$, i.e., 
	$A\triangle B=\{s\}$.  This is because \code{XOR}ing $s_A$ and $s_B$ (to obtain $s$) cancels out all (common) elements in $A\bigcap B$.   
%	Here {\it common elements} are defined as the 
%	Here an element that is contained in both sets is called a common element  
	%And $s$ is the missing element of $A$ (i.e., $s\in B\!\setminus\! A$) if $s\in B$, or the missing element of $B$ (i.e., $s\in A\!\setminus\! B$) otherwise;
	% \item If $A$ and $B$ has more than one distinct elements (i.e., $d>1$), the bitwise \code{XOR} of $s_A$ and $s_B$ will still cancel out all common elements and remain the \code{XOR} of the distinct elements, i.e., $s$ is the \code{XOR} of all distinct elements;
\end{sitemize}

Like in most of the literature on set reconciliation, we assume that the all-$0$ element 
$\mathbf{0}$ is excluded from the universe  $\mathcal{U}$, since otherwise \autoref{alg:trivial_case} does not work 
%when $\mathbf{0}\!\in\! A\bigcup B$ %$\mathbf{0}\in A\bigcap B$ 
for the following reason.  When the computed $s$ is $\mathbf{0}$, Alice cannot tell whether $A$ and $B$ are identical, or they have $\mathbf{0}$ as their distinct element. 
%However, we can extend our scheme to support $\mathbf{0}$. For example, we let Alice send to Bob a single bit to indicate whether Alice has element $\mathbf{0}$, so Bob will know whether $\mathbf{0}\in A\triangle B$ or not. 

\autoref{alg:trivial_case} also does not work when there are more than one distinct elements in $A\triangle B$ (i.e., $d>1$), since the computed $s$ in this case 
is the \code{XOR} sum of all these distinct elements.

% Note that \autoref{alg:trivial_case} works if and only if $|A\triangle B|\!\leq\! 1$ and $0\!\notin\! (A\!\cup\! B)$ (which we have explained in~\autoref{sec:model}). 

%\subsection{PBS: When $d$ is small}\label{sucsec:our-scheme}

%In this section, we generalize PBS to the case when $d$ is a small number, as we described in \autoref{sec:smalld}. 
%First, we describe each step of single-round PBS from \autoref{sec:hash_partition} to \autoref{sec:reconcile_by_trivial} and summarize it in \autoref{sec:single_round_pbs}. Second, we discuss the exceptions in single-round PBS in \autoref{subsec:exception_hash_partition}. Third, we propose multi-round PBS to handle the exceptions.

\subsection{The General Case}\label{sec:pbs_smalld}
%\subsection{PBS for small \texorpdfstring{\larger\boldmath $d$}{d}}\label{sec:pbs_smalld}

In this section, we describe the scheme for the more general case where $d$ is 
%no longer limited to be no more than $1$, but 
a small number that is no more than several, but is not necessarily $0$ or $1$.
%In this section, we substantiate the scheme described in \autoref{sec:smalld} for small $d$.

\subsubsection{Hash-partitioning and parity bitmap encoding}\label{sec:hash_partition}
% \medskip
% \noindent{\bf Hash Partition} 

Here we formalize the aforementioned process of partitioning $A$ into $\{A_i\}_{i=1}^n$, $B$ into $\{B_i\}_{i=1}^n$, and $A\triangle B$ into $\{A_i\triangle B_i\}_{i=1}^n$ 
using a hash function $h$. % $h(\cdot)$ changed by Long @0229-2020 for consistency
%as described in \autoref{sec:smalld} by introducing the concept of {\it sub-universes}. Given a hash function $h(\cdot): \mathcal{U}\rightarrow \{1,2,\cdots,n\}$, we 
Define {\it sub-universe} $\mathcal{U}_i$ as the set of elements in the universe $\mathcal{U}$ that are hashed into value $i$. More precisely, $\mathcal{U}_i\triangleq\{s\!\mid\! s\in \mathcal{U} \mbox{ and } h(s)=i\}$ for $i=1,2,...,n$. Then defining $A_i\triangleq A\bigcap\mathcal{U}_i$ and $B_i\triangleq B\bigcap\mathcal{U}_i$ for $i=1,2,...,n$ induces the partitioning of $A$, $B$, and $A\triangle B$.
%, as mentioned in \autoref{sec:smalld}. 

%{\bf (merged from the later two paragraphs)} 
How the $d$ distinct elements (balls) in $A\triangle B$ are ``scattered" into the $n$ subset-pair-differences (bins) $\{A_i\triangle B_i\}_{i=1}^n$ can be precisely modeled as throwing $d$ balls each uniformly and randomly into one of the $n$ bins. 
For the moment, we assume the following {\it ideal case} happens: Every subset-pair-difference $A_i\triangle B_i$ contains at most one distinct element.  
This ideal case corresponds to the $d$ balls ending up in $d$ distinct bins. It happens with probability $\prod_{k=1}^{d - 1}(1 - \frac{k}{n})$, which is on the order of $1-O(d^2/n)$ when $n\!\gg\!d$.
%approximately $e^{-\frac{d(d-1)}{2n}}$ when $d\!\ll\!n$. 
Hence, $n$ must be $\Omega(d^2)$ to ensure the ideal case happens with a nontrivial probability, as mentioned earlier in \autoref{sec:smalld}. 
%The nonideal case of a subset pair difference containing more than $1$ distinct elements will be discussed in \autoref{subsec:exception_hash_partition}.

% {\bf (Previous)} For the moment, we assume the following {\it ideal case} happens: Every subset-pair-difference $A_i\triangle B_i$ contains at most one distinct element. The nonideal case of a subset pair difference containing more than $1$ distinct elements will be discussed in \autoref{subsec:exception_hash_partition}. 

%In this section, we give a detailed description on how to partition $A$ and $B$ (as introduced in \autoref{sec:smalld}) by introducing {\it sub-universes}, which is defined as follows: Given a hash function $h(\cdot): \mathcal{U}\rightarrow \{1,2,\cdots,n\}$, we define {\it sub-universes} $\{\mathcal{U}_i\}_{i=1}^n$, a partition of the universe $\mathcal{U}$, as $\mathcal{U}_i=\{s\!\mid\! s\in \mathcal{U} \mbox{ and } h(s)=i\}$ for $i=1,2,...,n$. Based on $\{\mathcal{U}_i\}_{i=1}^n$, we define $\{A_i\}_{i=1}^n$, the partition of $A$ introduced in \autoref{sec:smalld}, as $A_i\! \triangleq\! A\bigcap \mathcal{U}_i$ for $i=1,2,...,n$. $\{B_i\}_{i=1}^n$ is similarly defined. By this definition, the set difference $A\triangle B$ is partitioned into $n$ set differences of the partitioned subset pairs (i.e., $\{(A_i, B_i)\}_{i=1}^n$). From \autoref{sec:hash_partition} to \autoref{sec:reconcile_by_trivial}, we assume the following {\bf ideal case} happens: Each subset pair $(A_i, B_i)$ contains at most one distinct element ({\it i.e.,} $|A_i\triangle B_i|\!\leq\!1$). The nonideal case of a subset pair contains more than $1$ distinct elements will be discussed in \autoref{subsec:exception_hash_partition}. 

% Here we describe the hash-partition step introduced in \autoref{sec:smalld} in details. First, we use a hash function $h(\cdot): \mathcal{U}\rightarrow \{1,2,\cdots,n\}$ to partition the universe $\mathcal{U}$ into $n$ sub-universes: $\mathcal{U}_i=\{s\!\mid\! s\in \mathcal{U} \mbox{ and } h(s)=i\}$ for $\forall i=1,2,\cdots,n$. The hash function $h(\cdot)$ can be predetermined between Alice and Bob and does not require additional communication cost. Define $A_i\! \triangleq\! A\bigcap \mathcal{U}_i$ and $B_i\! \triangleq\! B\bigcap \mathcal{U}_i$ for $i=1,2,\cdots,n$. Then $\{A_i\}_{i=1}^n$ and $\{B_i\}_{i=1}^n$ are partitions of $A$ and $B$ respectively. Furthermore, $\{A_i\triangle B_i\}_{i=1}^n$ is a partition of $A\triangle B$. From \autoref{sec:hash_partition} to \autoref{sec:reconcile_by_trivial}, we assume the following {\bf ideal case} happens: Each subset pair $(A_i, B_i)$ contains at most one distinct element ({\it i.e.,} $|A_i\triangle B_i|\!\leq\!1$). The nonideal case of a subset pair contains more than $1$ distinct elements will be discussed in \autoref{subsec:exception_hash_partition}. 

% {\bf (Previous)} How the $d$ distinct elements (balls) in $A\triangle B$ are distributed into the $n$ subset pair differences $\{A_i\triangle B_i\}_{i=1}^n$ (bins) 
% can be viewed as throwing $d$ balls each uniformly and randomly into one of the $n$ bins. 

%follows the familiar {\it balls-into-bins} probability model. 
%The distinct elements are viewed as balls and the subset pairs are viewed as bins. 
%Each of the $d$ balls is uniformly and randomly thrown by the hash function $h(\cdot)$ into one of the $n$ bins. 
% The aforementioned ideal case that corresponds to the $d$ balls ending up in $d$ distinct bins happens with probability $\prod_{k=1}^{d - 1}(1 - \frac{k}{n})$, which is on the order of $1-O(d^2/n)$ when $d\!\ll\!n$.
% %approximately $e^{-\frac{d(d-1)}{2n}}$ when $d\!\ll\!n$. 
% Hence, $n$ must be $\Omega(d^2)$ to ensure the ideal case happens with a nontrivial probability, as mentioned in \autoref{sec:smalld}.


%in which the distinct elements are viewed as balls and the subset pairs are viewed as bins. The hash-parition basically throws (hashes) $d$ balls (distinct elements) uniformly and randomly into $n$ bins (subset pairs). The aforementioned ideal case in this context becomes, after throwing $d$ balls uniformly and randomly into $n$ bins, each bin receives at most $1$ ball (i.e., $d$ nonempty bins have $1$ ball in each and the rest $n-d$ bins are empty). The number of balls in each bin is a Binomial random variable $Binomial(d,1/n)$.
%{\bf It may remind readers about the Birthday problem. And the ideal case can be analogous to the case that no people share the same birthday.} 
% The ideal case happens with a probability of $p\!=\!\prod_{k=1}^{d - 1}(1 - \frac{k}{n})\!\approx\! e^{-\frac{d(d-1)}{2n}}$ when $d\!\ll\!n$. In other words, $n$ must be at least $O(d^2)$ to ensure the ideal case happens with a nontrivial probability, as described in \autoref{sec:smalld}.  

% Note that the ideal case does not always happen. However, we can ensure that the ideal case happens with high probability by properly setting $n$ based on $d$ (i.e., $n=\Omega(d^2)$). Furthermore, as we will describe in \autoref{subsec:nonideal}, even if the ideal case does not happen (i.e., some distinct elements are hashed into the same subset pair), most of the distinct elements should be distributed into different subset pairs and therefore can be reconciled. So the scheme, even cannot reconcile all of the distinct elements, can still reconcile the majority of them (i.e., piecewise decodability in \autoref{sec:intro_oursolution}). Based on this property, we will extend our scheme from single-round to multi-rounds in \autoref{subsec:nonideal} to further increase the probability of reconciling all distinct elements. 

% \medskip
% \noindent{\bf Parity Bitmap Encoding} 

% to let Alice obtain $A\triangle B$.

% {\bf (Modified)} Recall that the partition $\{A_i\}_{i=1}^n$ and $\{B_i\}_{i=1}^n$ can be encoded as $A[1..n]$ and $B[1..n]$ respectively, in which $A[i]$, the $i$-th bit of the parity bitmap $A[1..n]$, is equal to the oddness / evenness (parity) of the cardinality of $A_i$ (i.e., $A[i]=1$ if $|A_i|$ is odd; otherwise $A[i]=0$). $B[i]$, the $i$-th bit of the parity bitmap $B[1..n]$, is similarly defined. In the ideal case, $A[1..n]$ and $B[1..n]$ differ in exactly $d$ distinct bit positions $i_1,i_2,...,i_d$, and each subset-pair-difference $(A_{i_1},B_{i_1}), (A_{i_2},B_{i_2}),...,(A_{i_d},B_{i_d})$ contains exactly $1$ distinct element. If Bob knows $i_1,i_2,...,i_d$, he can start to reconcile the $d$ subset pairs respectively using \autoref{alg:trivial_case}, then Alice will obtain $A\triangle B$.

% {\bf (Modified)} The partition $\{A_i\}_{i=1}^n$ is encoded into an $n$-bit-long parity bitmap $A[1..n]$, in which $A[i]$, the $i$-th bit of the parity bitmap, is equal to the oddness / evenness (parity) of the cardinality of $A_i$ (i.e., $A[i]=1$ if $|A_i|$ is odd; otherwise $A[i]=0$). $B[1..n]$, the parity bitmap of $\{B_i\}_{i=1}^n$, is similarly defined. In the ideal case, $A[1..n]$ and $B[1..n]$ differ in exactly $d$ distinct bit positions $i_1,i_2,...,i_d$, and each subset-pair-difference $(A_{i_1},B_{i_1}), (A_{i_2},B_{i_2}),...,(A_{i_d},B_{i_d})$ contains exactly $1$ distinct element. If Bob knows $i_1,i_2,...,i_d$, he can start to reconcile the $d$ subset pairs respectively using \autoref{alg:trivial_case}, then Alice will obtain $A\triangle B$.

% {\bf (Previous)} We encode $\{A_i\}_{i=1}^n$ into an $n$-bit-long parity bitmap $A[1..n]$, in which $A[i]$, the $i^{th}$ bit of the parity bitmap, is equal to the oddness / evenness (parity) of the cardinality of $A_i$ (i.e., $A[i]=1$ if $|A_i|$ is odd; otherwise $A[i]=0$). In the ideal case, the two bitmaps $A[1..n]$, $B[1..n]$ differ in exactly $d$ bit positions $i_1,i_2,...,i_d$, each of which corresponds to a subset pair that contains $1$ distinct element. The next step is to let Alice and Bob know these bit positions.

%Once the $d$ bit positions are known, Alice and Bob can start to reconcile $(A_{i_1},B_{i_1}), (A_{i_2},B_{i_2}),...,(A_{i_d},B_{i_d})$ using \autoref{alg:trivial_case} and obtain the $d$ distinct elements (i.e., $A\triangle B$). 

% \subsubsection{Parity Bitmap Encoding}\label{sec:parity_bitmap_encoding}

% %After hash-partitioning $A$ and $B$ into partitions $\{A_i\}_{i=1}^n$ and $\{B_i\}_{i=1}^n$, 
% As introduced in \autoref{sec:smalld}, we encode each partition into an $n$-bit-long parity bitmap and denote them as $A[1..n]$ and $B[1..n]$ respectively, as introduced in \autoref{sec:smalld}. For $i=1,2,...,n$, $A[i]$ (the $i^{th}$ bit of the parity bitmap $A[i]$) is equal to $1$ if $A_i$ contains an odd number of elements, and is equal to $0$ otherwise.
% % More specifically, for $i=1,2,...,n$, $A[i]$ (the $i^{th}$ bit of the parity bitmap $A[i]$) is defined as follows: $A[i]=1$ if $A_i$ contains an odd number of elements, and $A[i]=0$ otherwise. In this way, each bit $A[i]$ encodes the oddness / evenness (parity) of the cardinality of $A_i$. The $n$-bit-long parity bitmap $B[1..n]$ and $B[i]$ (the $i^{th}$ bit of $B[1..n]$) are similarly defined. 
% In the ideal case, 
% %$A[i]$ and $B[i]$ differ if and only if $A_i$ and $B_i$ have exactly $1$ distinct element, and $A[i]$ and $B[i]$ are the same if and only if $A_i=B_i$. Meanwhile, the $d$ distinct elements are hashed into $d$ different subset pairs. So 
% the two bitmaps $A[1..n]$, $B[1..n]$ differ in exactly $d$ bit positions, each of which corresponds to a subset pair that contains $1$ distinct element. Once the $d$ bit positions are known, Alice starts to reconcile each of the $d$ corresponding subset pairs by \autoref{alg:trivial_case} and gets the $d$ distinct elements (i.e., $A\triangle B$). 
% %If knowing the $d$ bit positions (i.e., the $d$ corresponding subset pairs), we can use \autoref{alg:trivial_case} to reconcile the $d$ subset pairs respectively to obtain all the $d$ distinct elements (i.e., $A\triangle B$). 
% In \autoref{sec:BCH_code}, we will describe how to find the $d$ bit positions using BCH code~\cite{Lint_IntroductionCodingTheory_1998}. 

% \medskip
% \noindent{\bf Find the $d$ Bit Positions Using ECC} 

%\subsubsection{Find the $d$ Bit Positions Using ECC}\label{sec:BCH_code}
\subsubsection{Find and reconcile the \texorpdfstring{$d$}{d} subset pairs}\label{sec:BCH_code}


\begin{algorithm}
\caption{PBS-for-small-$d$ (first round)}
\label{alg:single_round_pbs}

%Hash-partition $A$, $B$ into $\{A_i\}_{i=1}^n$, $\{B_i\}_{i=1}^n$\; \label{step:hash_partition}

%Parity encode $\{A_i\}_{i=1}^n$, $\{B_i\}_{i=1}^n$ into $A[1..n]$, $B[1..n]$\; \label{step:parity_encode}
{\it Alice}: Send $\xi_A$, the BCH codeword of $A[1..n]$, to Bob\; \label{step:BCH_encode}

{\it Bob}: Decode $(B[1..n], \xi_A)$ to obtain $i_1, i_2, ..., i_d$\; \label{step:BCH_decode}

{\it Bob}: Send \code{XOR} sums of sets $B_{i_1}, B_{i_2},...,B_{i_d}$ (\autoref{alg1:sender} in \autoref{alg:trivial_case}), indices $i_1, i_2, ..., i_d$,
and checksum $c(B)$ to Alice\; \label{step:send_xor}

{\it Alice}: Obtain $A_{i_1}\triangle B_{i_1}, A_{i_2}\triangle B_{i_2},...,$ and $A_{i_d}\triangle B_{i_d}$ (\autoref{alg1:receiver} in \autoref{alg:trivial_case}); $\hat{D}\leftarrow \bigcup_{k=1}^d (A_{i_k}\triangle B_{i_k})$\; \label{step:trivial_reconcile}

{\it Alice}: Check whether $c(A\triangle\hat{D})\stackrel{?}{=}c(B)$\; \label{step:terminate_condition}

\end{algorithm}

The remaining steps of the PBS scheme are summarized in \autoref{alg:single_round_pbs}.
Recall that the partitions $\{A_i\}_{i=1}^n$ and $\{B_i\}_{i=1}^n$ can be encoded as parity bitmaps $A[1..n]$ and $B[1..n]$ respectively, in which each $A[i]$ or $B[i]$
%, the $i$-th bit of the parity bitmap $A[1..n]$ or $B[1..n]$, 
corresponds to the parity (oddness or evenness) of the cardinality of the subset $A_i$ or $B_i$.  In the ideal case, $A[1..n]$ and $B[1..n]$ differ in exactly $d$ distinct bit positions. 
Suppose these $d$ bit positions are $i_1, i_2, ..., i_d$.  
Then subset pairs $(A_{i_1}, B_{i_1}), (A_{i_2}, B_{i_2}),...,(A_{i_d}, B_{i_d})$ each differs by exactly $1$ (distinct) element
and hence can be reconciled using \autoref{alg:trivial_case}.

For this to happen, however, both Alice and Bob need to first know the values of $i_1, i_2, ..., i_d$, or the bit
positions where
$A[1..n]$ and $B[1..n]$ differ.
%;  their ``starting position" is that Alice knows only $A[1..n]$ 
%and Bob knows only $B[1..n]$.  
To this end, a naive solution is for Alice to send $A[1..n]$ to Bob and for Bob to compare 
it with $B[1..n]$.    
% he can initiate the process of reconciling these $d$ subset pairs each using \autoref{alg:trivial_case}.
However, as mentioned earlier in \autoref{sec:smalld}, Alice can achieve the same goal by sending 
an ECC codeword $\xi_A$ that is much shorter than $A[1..n]$.  
The idea is that since $B[1..n]$ (which Bob already knows) 
can be viewed as a ``corrupted" 
(with $d$ bit errors in the positions $i_1, i_2, ..., i_d$) copy of 
$A[1..n]$, as long as the codeword $\xi_A$ is parameterized to correct at least $d$ bit errors, 
Bob can decode $B[1..n]\|\|\xi_A$ (the ``corrupted" message concatenated with the ECC codeword
of the ``uncorrupted" message)
to find out the $d$ bit error positions.  

Although several ECC schemes are suitable for this purpose, we choose the BCH scheme for 
PBS because it results in near-optimal codeword length 
in the following sense: In the context of PBS, to ``correct up to $t$ bit errors", 
$\xi_A$ only needs to be $t \lceil\log_2 (n + 1)\rceil$ bits long; 
even if Alice knew these $t$ bit positions precisely, specifying each bit position (to Bob) 
would require $\lceil\log_2 n\rceil$ bits. 
BCH is also the choice of PinSkech~\cite{Dodis_PinSketch_2008} for the same reason.



%chosen as the ECC scheme in both pinskech and PBS due to its near-optimal 
%coding efficiency, as will be explained in ???

%Alice only needs to send a BCH encoding of $A[1..n]$, denoted as $\xi_A$, that can pinpoint (to Bob) these $d$ bit %locations in Bob's local bitmap $B[1..n]$ (\autoref{step:BCH_encode} in \autoref{alg:single_round_pbs}).  

%{\bf We will provide some details of this BCH encoding and decoding
%in Section ???[the last subsection of Section 2].}
%Then Bob can decode and recover $A[1..n]$ (original message) and obtain $i_1,i_2,...,i_d$.

%{\bf (Previous)} In the ideal case, for Bob to obtain $i_1,i_2,...,i_d$, Alice only needs to send $\xi_A$, the BCH code of $A[1..n]$, that can ``correct'' these $d$ bit errors in $B[1..n]$. Then Bob can decode and recover $A[1..n]$ (original message) and obtain $i_1,i_2,...,i_d$.

% {\bf (Previous)} We view $A[1..n]$ as a corrupted message of $B[1..n]$ sent ({\bf not actually being sent}) from Bob to Alice through an {\it unreliable} commnunication channel that flips $d$ bits. To locate these $d$ bit positions, we let Bob also send an {\it error-correction code} that encodes $B[1..n]$ to Alice, such that Alice can recover $B[1..n]$ (original message) and obtain the $d$ bit positions $i_1,i_2,...,i_d$. In PBS, we use BCH code~\cite{bch1} to encode $B[1..n]$ and get the error-correction code.


%To correct $d$ bit errors, the length of the net-codeword only is no more than $d\log n$ bits. 
% Without causing any ambiguity, we use the term `codeword' to refer to the net-codeword in the rest of this paper.
%The computational complexity of the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} is $O(d^2\log^2 n)$.

% There are two different BCH encoding techniques: {\it systematic} and {\it unsystematic}. The difference is that, the message appears as the prefix of the codeword (i.e., codeword = [message net-codeword]) in systematic BCH encoding, whereas it does not appear as a substring of the codeword in unsystematic BCH encoding. In PBS, we choose systematic BCH encoding because we are sending not the ``message'', but the net-codeword. 
% %To correct $d$ bit errors, the length of the net-codeword only is no more than $d\log n$ bits. 
% Without causing any ambiguity, we use the term `codeword' to refer to the net-codeword in the rest of this paper.
% %The computational complexity of the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} is $O(d^2\log^2 n)$.

%The systematic BCH encoding is also used in other ECC-based set reconciliation works, such as PinSketch \cite{Wuille_Minisketchoptimizedlibrary_2019}, while PinSketch encodes a much longer message (e.g., $2^{32}$ bits) than in ours (hundreds of bits).  

%\subsubsection{Find the $d$ Bit Positions Using ECC}\label{sec:BCH_code}

% A straightforward approach to find the $d$ bit positions is to let Bob send the complete parity bitmap $B[1..n]$ to Alice, then Alice compares $A[1..n]$ with $B[1..n]$ locally. This approach has a communication overhead of $n$ bits, which is quite wasteful. As we discussed in~\autoref{sec:hash_partition}, $d$ is usually much smaller than $n$. It means $A[1..n]$ and $B[1..n]$ differ only at a tiny portion of bits. Therefore, we can view $A[1..n]$ as a corrupted message of $B[1..n]$ with $d$ bit errors, and the bit positions of the $d$ bit errors basically correspond to the $d$ subset pairs that contain distinct elements. The detection of bit errors, on the other hand, can be solved by Error-Correction Code (ECC)~\cite{Lin_ErrorControlCoding_1983}. 

% Since $A[1..n]$ and $B[1..n]$ differ at $d$ bit positions, we can view $A[1..n]$ as a corrupted message of $B[1..n]$ from Bob to Alice through an {\it unreliable} commnunication channel with $d$ corrupted bits, which are located on the $d$ bit positions. Therefore, to find the $d$ bit position, we only need to correct the $d$ corrupted bits in $A[1..n]$, which is done by transmitting a ``code'' that can correct upto $d$ bit errors from Bob to Alice through a {\it reliable} communication channel. 

% In PBS, we use {\it systematic} BCH code to generate the ``code'' by encoding the message $B[1..n]$. The codeword of the systematic BCH code is in the form of [message, net-codeword], since the message appears as the prefix of the codeword in systematic BCH code. The ``code'' is simply the net-codeword in the BCH codeword. We choose {\it systematic} BCH code because the (corrupted) message is already transmitted and we only need to pay a small communication overhead on transmitting ``code'' (i.e., net-codeword). To correct upto $d$ bit errors, the length of the net-codeword is no more than $d\log n$ bits, which is much smaller than the message when $d\!\ll\! n$. The computational complexity of the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} is $O(d^2\log^2 n)$. This type of BCH code is also used in other ECC-based set reconciliation works, such as PinSketch \cite{Wuille_Minisketchoptimizedlibrary_2019}. 

% Different from {\it unsystematic} BCH code
% The ``code'' is generated by {\it systematic} BCH code, which encodes the message $B[1..n]$ into a BCH codeword in the form of [message, net-codeword]. The ``code'' transmitted on the reliable channel is the net-codeword of the BCH codeword. In {\it systematic} BCH code, the message appears as the prefix of the codeword. 

% More specifically, PBS uses {\it systematic} BCH code~\cite{Lint_IntroductionCodingTheory_1998} that can correct upto $d$ bit errors to encode the parity bitmaps. In the {\it systematic} BCH code \footnote{In unsystematic BCH code, message does not appear to be the prefix of the codeword}, the message (i.e., the parity bitmap) appears as the prefix of the raw codeword, which in the form of [message, net codeword]. Normally, to correct upto $d$ errors, the length of the net codeword is $2n\log d$, where $n$ is the length of the message (i.e., parity bitmap). However, our case is special in the sense that the net codeword is error-free (all $d$ bit errors are in the message), so the length of the net codeword can be reduced to $n\log d$. This type of BCH code is also used in other ECC-based set reconciliation works, such as PinSketch \cite{Wuille_Minisketchoptimizedlibrary_2019}. 

% Now we can formally describe how to find the $d$ bit positions: First, Bob uses a $d$-error-correcting systematic BCH code to encode $B[1..n]$ and sends the net codeword ($d\log n$ bits) to Alice. Upon receiving the net codeword and combining it with the corrupted message $A[1..n]$, Alice uses the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} to decode the $d$ bit errors in $A[1..n]$. The communication overhead of transmitting the net codeword is $d\log n$ bits. The computational complexity of the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} is $O(d^2\log^2 n)$. Both the communication overhead and the computational complexity here are relatively small when $d$ is small.

% \medskip
% \noindent{\bf Reconcile the $d$ subset pairs using \autoref{alg:trivial_case}} 

%Once the $d$ bit positions are known, Alice can start to reconcile $(A_{i_1},B_{i_1}), (A_{i_2},B_{i_2}),...,(A_{i_d},B_{i_d})$ using \autoref{alg:trivial_case} and obtain the $d$ distinct elements (i.e., $A\triangle B$). 
Once Bob decodes $\xi_A$ (\autoref{step:BCH_decode} in \autoref{alg:single_round_pbs}) to obtain $i_1,i_2,...,i_d$, 
%the corresponding subset pairs $(A_{i_1},B_{i_1})$, $(A_{i_2},B_{i_2})$, $...$, 
%$(A_{i_d},B_{i_d})$ each can be reconciled using \autoref{alg:trivial_case}.  To do so, 
Bob sends the \code{XOR} sums of the corresponding 
subsets $B_{i_1}$, $B_{i_2}$,$...$,$B_{i_d}$ to Alice (\autoref{alg1:sender} in \autoref{alg:trivial_case}).  Bob also needs to send the decoded ``bit error positions'' $i_1, i_2, ..., i_d$ to Alice (\autoref{step:send_xor} in \autoref{alg:single_round_pbs}), 
{\color{red} since Alice cannot obtain this information
by herself without knowing anything about $B[1..n]$.} 
%{\color{red} since Alice cannot obtain this information (in the same way as Bob did in \autoref{step:BCH_decode} of \autoref{alg:single_round_pbs}) by herself without knowing $B[1..n]$.} 
% {\color{red} since Alice cannot decode $\xi_A$ herself without knowing $B[1..n]$.}
In addition, for Alice to verify whether the set reconciliation is successfully completed (to be described next), Bob sends $c(B)$, a checksum of its set $B$, to Alice.  
%Alice, without knowing $B[1..n]$ otherwise would not know the ``bit error positions'' . 
%As each ``bit error position'' can be encoded into $\log n$ bits, the resulting additional communication overhead is $d\log n$ bits. 
% When reconciling $(A_{i_1},B_{i_1}), (A_{i_2},B_{i_2}),...,(A_{i_d},B_{i_d})$ using \autoref{alg:trivial_case}, Alice needs to send not only the bitwise \code{XOR} of $A_{i_1}, A_{i_2},..., A_{i_d}$, but also the indices of the subset pairs ($i_1,i_2,...,i_d$), since Bob does not know which of the $d$ subset pairs are being reconciled. Each index is an integer between $1$ and $n$ and can be encoded into $\log n$ bits, So the additional communication overhead on transmitting the indices is $d\log n$ bits. 

% \subsubsection{Reconcile the $d$ subset pairs using \autoref{alg:trivial_case}}\label{sec:reconcile_by_trivial}

% After decoding the $d$ bit errors that corresponds to the $d$ subset pairs, Alice starts to reconcile them using \autoref{alg:trivial_case}. For each of the $d$ subset pairs, Alice needs to send not only the bitwise \code{XOR} of the subset pair, but also the index of the subset pair (since Bob does not know the $d$ subset pairs to reconcile). So the communication overhead on \autoref{alg:trivial_case} is $d\log |\mathcal{U}|+d\log n$ bits. 
%Plus the communication overhead on transmitting the net codeword of parity bitmap ($d\log n$, as we explained in \autoref{sec:BCH_code}), the overall communication overhead of single-round PBS is $d\log u+2d\log n$ bits.

% \medskip
% \noindent{\bf Check if set reconciliation is complete} 

%{\bf We need a subsubsection on verification}\
\subsubsection{Verify the estimated set difference}\label{sec:checksum_verification}

Once Alice receives the ``bit error positions" and the corresponding \code{XOR} sums, 
she can recover the distinct elements each using \autoref{alg:trivial_case} to arrive at the estimated set difference
(\autoref{step:trivial_reconcile} in \autoref{alg:single_round_pbs}), which we denote as 
$\hat{D}$.   {\color{red}It is not hard to verify that in the ideal case this estimated set difference $\hat{D}$ is necessarily the same as the
actual set difference $A\triangle B$, so the unidirectional set reconciliation process is successfully completed.

However, the nonideal case can happen and when that happens $\hat{D}$ is in general not the same as $A\triangle B$.
Hence, Alice in general needs to verify whether $\hat{D}\stackrel{?}{=}A\triangle B$ after a round of set reconciliation process.}
%because only in the ideal case is this estimated set difference $\hat{D}$ the same as the
%actual set difference $A\triangle B$, as we will explain in the next section.   
Alice does so by checking an equivalent condition $A\triangle\hat{D}\stackrel{?}{=}B$ 
as follows.  She applies a
checksum function $c(\cdot)$ to $A\triangle\hat{D}$ and comparing (\autoref{step:terminate_condition} in \autoref{alg:single_round_pbs}) 
the resulting checksum $c(A\triangle\hat{D})$ with $c(B)$ that Alice received earlier from Bob. 
%While many different checksum function $c(\cdot)$ can be used here, 
{\color{red}
We use as $c(\cdot)$ here the plain-vanilla summation function, with which the checksum of a set $S$ is the sum
of all elements (viewed as integers) modulo $|\mathcal{U}|$.   The length of such a checksum is $(\log |\mathcal{U}|)$ bits, the same as that of an element.
We use this checksum function for two reasons.  First, because it uses the `+' operation whereas the set reconciliation process (\autoref{alg:trivial_case}) involves a very different
operation (XOR), a 
false verification event is intuitively almost statistically uncorrelated\footnote{If we absolutely have to ensure any two such events to be provably strictly statistically uncorrelated, we can apply a one-way hash function to 
each element first and adding their hash values (viewed as integers) up instead, at a bit extra computation cost.} with any reconciliation error (called an exception and to be described shortly) event, which makes the verification
step meaningful and effective to the maximum extent.  
%In~\ref{} we will present an exception event that will lead to incorrect set
%reconciliation if the false verification event also happens, and show through Monte-Carlo simulations that these two events 
%are indeed almost statistically uncorrelated. 
Second, this checksum function can be incrementally computed. 
}   


%While $c(\cdot)$ can be any checksum function, for performance considerations, a linear checksum function is preferred here.  
%We call $c(\cdot)$ linear if $c(S_1\triangle S_2)=c(S_1)\oplus c(S_2)$ for any two sets $S_1$ and $S_2$.
%With a linear $c(\cdot)$, the total time complexity of computing 
%both $c(A\triangle\hat{D})$ and $c(B)$ is only $O(d)$, because when a large set (say $B$) changes slightly (from one time to another),  

\begin{comment}
because it allows for incremental updates, 
This checking can be achieved using a checksum function $c(\cdot)$ that maps any subset of the universe $\mathcal{U}$ to a checksum by checking whether $c(\hat{D})\stackrel{?}{=}c(A\triangle B)$. With incremental updates, $c(\hat{D})$ can be computed in $O(d)$ time. However, computing $c(A\triangle B)$ is tricky, since $A$ and $B$ are {\it remote} sets and stored at hosts Alice and Bob respectively. 

To ease the computation of $c(A\triangle B)$, we choose a ``linear'' checksum function, so that $c(A\triangle B)=c(A)\oplus c(B)$ can be precomputed. Here we call a checksum function ``linear'' if $c(S_1\triangle S_2)=c(S_1)\oplus c(S_2)$ for any two subsets $S_1$ and $S_2$ of the universe $\mathcal{U}$. More specifically, to obtain $c(A\triangle B)$, Bob precomputes $c(B)$ and sends it to Alice. Alice also precomputes $c(A)$, and upon receiving $c(B)$, Alice can compute $c(A\triangle B)=c(A)\oplus c(B)$. In PBS, we select {\it longitudinal parity check}, the bitwise \code{XOR} of all elements (recall each element is a $(\log |\mathcal{U}|)$-bit-long binary string) in the set, as the ``linear'' checksum function. The precomputation of $c(A\triangle B)$ incurs additional communication overhead on transmitting $c(B)$ that is $\log |\mathcal{U}|$ bits.

{\bf (previous)} This can be achieved using a ``linear'' checksum function $c(\cdot)$ that maps any subset of the universe $\mathcal{U}$ to a $32$-bit checksum by checking whether $c(\hat{D})\stackrel{?}{=}c(A\triangle B)$. Here we call a checksum function ``linear'' if $c(S_1\triangle S_2)=c(S_1)\oplus c(S_2)$ for any two subsets $S_1$ and $S_2$ of the universe $\mathcal{U}$. We choose a checksum function that is ``linear'', so that $c(A\triangle B)=c(A)\oplus c(B)$ can be precomputed. This precomputation incurs $32$ bits of communication overhead on transmitting $c(B)$ from Bob to Alice. With incremental updates, $c(\hat{D})$ can be computed in $O(d)$ time. In PBS, we select {\it longitudinal parity check}, the bitwise \code{XOR} of all elements (assuming each element is a $32$-bit-long binary string) in the set, as the ``linear'' checksum function. 
%It is not hard to verify it is linear.  

\end{comment}

%In the nonideal case, however, $\hat{D}$ will deviate from $A\triangle B$. 
%Hence, Alice needs to verify whether $\hat{D}\stackrel{?}{=}A\triangle B$.  This can be accomplished using a checksum function 




% Once Alice receives the \code{XOR} sums and the indices, she can compute the distinct elements, as described in \autoref{subsec:protocol0}, to obtain the set difference (denoted as $\hat{D}$). However, this reconciled set difference could be incorrect if the ideal case does not happen. Therefore, Alice needs to check if set reconciliation is successfully completed (or whether $\hat{D}=A\triangle B$). To do so, we introduce some ``linear'' checksum function $c(\cdot)$ that maps any subset of the universe $\mathcal{U}$ (such as $A$ and $B$) to a $32$-bit checksum (e.g., bitwise \code{XOR}). Here the ``linearity'' of a chechsum function refers to the fact that $c(S_1\triangle S_2)=c(S_1)\oplus c(S_2)$ for any two subsets $S_1$ and $S_2$ of the universe $\mathcal{U}$. We use this checksum function to check if $\hat{D}=A\triangle B$ by comparing $c(\hat{D})$ to $c(A\triangle B)$. Note that $c(\hat{D})$ can be computed in $O(d)$ time and $c(A\triangle B)=c(A)\oplus c(B)$ can be precomputed {\bf during the encoding period, which costs $32$ bits of communication overhead on transmitting $c(B)$ from Bob to Alice. In PBS, we select {\it longitudinal parity check}, the bitwise \code{XOR} of all elements (recall each element is a $32$-bit-long binary string) in the set, as the checksum function. It is not hard to verify it is linear.}  

% {\bf (Previous)} After reconciling the subset pairs and obtaining the reconciled set difference (denoted as $\hat{D}$), PBS needs to check if set reconciliation is complete (or whether $\hat{D}=A\triangle B$), since the reconciled set difference $\hat{D}$ is not the actual set difference $A\triangle B$ in the nonideal case (to be discussed in \autoref{subsec:exception_hash_partition}). Hence, we add a verfication step after obtaining $\hat{D}$ to check if $\hat{D}=A\triangle B$. In PBS, we check an equivalent condition, $A=B\triangle\hat{D}$, instead of $\hat{D}=A\triangle B$, since $B$ and $\hat{D}$ are both known by Bob and their set difference $B\triangle\hat{D}$ can be locally computed. More specifically, to check if the remote sets $A$ and $B\triangle\hat{D}$ are equal, we let Alice compute a $32$-bit checksum of $A$ and send it to Bob. {\bf Then Bob computes the $32$-bit checksum of $B\triangle\hat{D}$ using the same checksum algorithm and compare the two checksums. In PBS, we select {\it longitudinal parity check} (i.e., bitwise \code{XOR} of all elements in the set) as the checksum algorithm, so that the checksum $B\triangle\hat{D}$ can be efficiently computed as the bitwise \code{XOR} between the checksum of $B$ (can be pre-computed) and that of $\hat{D}$. Other checksum algorithms that are {\it linear} to the set difference operator (i.e., $\triangle$) also work for PBS. }
% Then Bob checks if $B\triangle\hat{D}$ satisfies the receiving checksum. 

Using a 32-bit-long checksum (assuming $\log |\mathcal{U}| = 32$), the probability for Alice to mistakenly believe $A\triangle\hat{D}\!=\!B$ when the opposite 
(i.e., $\{A\triangle\hat{D}\!\neq\! B\}$) is true 
%the condition {\bf ????} can be correctly verified with an overwhelming probability of 
is only $O(10^{-12})$ for the following reason. 
The false verification event $\{A\triangle\hat{D}\! \neq\! B\}$ can happen only in the nonideal case, which happens with a probability of $O(10^{-2})$ (as we will show in \autoref{subsec:exception_hash_partition}).
Then, conditioned upon the event $\{A\triangle\hat{D}\! \neq\! B\}$ happening, 
the probability for their 32-bit-long checksums happen to be equal (i.e., $c(A\triangle\hat{D})\! =\! c(B)$) is only $2^{-32}\!\approx\! 2.3\!\times\! 10^{-10}$.
%a 32-bit-long checksum to fail to detect $\hat{D}\neq A\triangle B$ .
This $O(10^{-12})$ probability of incorrect verification should be acceptable in most applications.  
% In applications that allow no incorrect verification ({\it e.g.,} Bitcoin), additional
% verification techniques such as a Merkle tree~\cite{merkle87} can be used in conjunction.  

{\color{red}In applications in which correct verification absolutely has to be guaranteed ({\it e.g.,} blockchain), 
additional built-in verification mechanisms, such as Merkle tree, are usually used, which can
reduce the probability of false verification to practically zero at no extra cost (to PBS).
% to guarantee the correctness of the verification. 
For example, blockchain platforms Ethereum~\cite{Wood_Ethereumsecuredecentralised_2014} 
and Bitcoin~\cite{Nakamoto_Bitcoinpeerpeer_2019} both have Merkle tree~\cite{merkle87} based mechanisms for verifing the 
integrity and the consistency of transactions. 
A Merkle tree is a binary tree in which a parent node digitally certifies (verifies) its two children.  
In the cases of Ethereum and Bitcoin, each transaction corresponds to a leaf node of the Merkle tree that records 
the cryptographic hash value of the transaction, and 
each non-leaf node records the cryptographic hash value of its two children.  This way, the
root node digitally certifies the integrity and the consistency of all transactions.  
For mission-critical applications that do not have such an additional built-in verification mechanism, we can add one at a small cost. 
%there are many techniques we can 
%use to achieve correct verification. 
For example, we can compute and check $H(A\triangle\hat{D})\!\stackrel{?}{=}\!H(B)$, where $H$ is a 
one-way multiset hash function such as MSet-XOR-Hash~\cite{Clarke_IncrementalMultisetHash_2003}, 
%$H$, to 
%both $A\triangle\hat{D}$ and $B$ and verify $H(A\triangle\hat{D})\!\stackrel{?}{=}\!H(B)$ 
at the additional cost of $O(\max\{|A|+d, |B|\})$ computation overhead and constant communication overhead. 
}

\begin{comment}
%Therefore, in such applications, we can rely on 
%the built-in technique to do the verification with no cost. 
For mission-critical applications itself does not have built-in verification component, there are many techniques we can 
use to achieve correct verification. 
For example, we can apply an one-way multiset hash function, 
{\it e.g.}, MSet-XOR-Hash~\cite{Clarke_IncrementalMultisetHash_2003}, $H$, to 
both $A\triangle\hat{D}$ and $B$ and verify $H(A\triangle\hat{D})\!\stackrel{?}{=}\!H(B)$ 
with an additional computational overhead of $O(\max\{|A|+d,|B|\})$ and constant communication overhead. 
We do not count the overhead of this ``correctness-guaranteed'' verification in the calculation of 
the communication overhead in the sequel, since all schemes described in 
this paper requires it when the application allows no incorrect verification. 
\end{comment}

{\color{red}
In this case of PBS-for-small-$d$, the set reconciliation process will run as many rounds as it takes (to be explained in \autoref{sec:multi-rounds}) 
for the checksums of two sets being reconciled to eventually 
match each other;   
in the case of PBS-for-large-$d$, the same as can be said about the set reconciliation process for each group pair (to be explained in~\autoref{sec:pbs-for-large-d}).
Hence, barring the false verification event, which as just explained happens with $O(10^{-12})$ probability when using only a 32-bit checksum or with practically zero probability when
using additional cryptographic verification techniques, the set conciliation process (for both large and small $d$) 
guarantees to correctly reconcile $A$ and $B$ (and the respective referenced objects) when it halts.
With this understanding, for ease of presentation, we assume in the sequel that the checksum verification step will never produce a false verification.  

In~\Cref{subsec:exception_hash_partition,sec:BCH_exception}, we describe three types of exceptions may result in a $\hat{D}$ that is incorrect (not the same as $A\triangle B$).  
When that happens, the checksum verification step will not accept $\hat{D}$ as is, as just explained.  Hence, these exceptions will never result in 
an incorrect set reconciliation.  They can only delay the inevitable (eventual correct reconciliation of $A$ and $B$)  by triggering additional rounds of set reconciliation process.
%executed to ``make it right".  
}

\begin{comment}
stop when the checksum of 
Note that the existence of the above two types of exceptions 
will not result in reconciliation error, since 
whenever such an exception happens, the checksum verification in~\autoref{step:terminate_condition} of~\autoref{alg:single_round_pbs}
would fail (as now $\hat{D}\neq (A\triangle B)$, thus $c(A\triangle \hat{D})\neq c(B)$), triggering one or more rounds of 
further reconciliation attempts (to be described next), by which PBS will correctly reconcile all 
distinct elements. We also note that PBS does not need to know in which bins those exceptions happened 
to continue the subsequent reconciliation attempts. 
\end{comment}


%To simplify our presentation, we 
%assume that the $c(A\triangle\hat{D})\!\stackrel{?}{=}\!c(B)$ verification is always correct in the sequel. 

% Using a 32-bit-long checksum (assuming $(\log |\mathcal{U}|) = 32$), the probability for Alice to mistakenly believe {\bf ????} when the opposite is true 
% %the condition {\bf ????} can be correctly verified with an overwhelming probability of 
% is only $O(10^{-12})$ for the following reason. 
% The event {\bf ????} can happen only in the nonideal case, which happens with a probability $O(10^{-2})$ (as we will show in \autoref{subsec:exception_hash_partition}).
% Then, conditioned upon the nonideal case happening, the probability for a 32-bit-long checksum to fail to detect {\bf ????} is only $2^{-32}\approx 2.3\times 10^{-10}$.
% This tiny probability of incorrect verification should be acceptable in most applications.  In applications that allow no incorrect verification ({\it e.g.,} Bitcoin), additional
% verification techniques such as a Merkle tree~\cite{merkle87} can be used in conjunction.  To simplify our presentation, we ignore this $O(10^{-12})$ 
% probability event and assume that the {\bf ???? WITH c on both sides} verification is always correct in the sequel. 

% {\bf although it could mistakenly believes two different sets as identical ones.} This event happens with probability $2^{-32}\approx 2.3\times 10^{-10}$ when the ideal case does not happen, {\bf which has a probability on the order of $10^{-2}$.} Although this event could cause PBS mistakenly believes the set reconciliation is completed, it happens with an extremely small probability (on the order of $10^{-12}$) and should be acceptable in most applications. In few applications which allow no room for error ({\it e.g.,} Bitcoin), additional techniques such as Merkle tree~\cite{merkle87} based validation will be used to verify the correctness of the results anyway. 
% %If such techniques find out that the set reconciliation is not completed, we could simply start it over and use PBS to reconcile the two sets again under a different hash function $h$. In this case, the checksum will be different If so, the  (note that PBS is a `randomized' algorithm when assuming the hash functions for hash-partition are random hash functions). 
% To simplify our description, we ignore this small probability event and assume the checksum always correctly verify $\hat{D}\stackrel{?}{=}A\triangle B$ in the sequal. 

% The condition $\hat{D}=A\triangle B$ can be almost surely verified by the checksum, 
% {\bf although it could mistakenly believes two different sets as identical ones.} This event happens with probability $2^{-32}\approx 2.3\times 10^{-10}$ when the ideal case does not happen, {\bf which has a probability on the order of $10^{-2}$.} Although this event could cause PBS mistakenly believes the set reconciliation is completed, it happens with an extremely small probability (on the order of $10^{-12}$) and should be acceptable in most applications. In few applications which allow no room for error ({\it e.g.,} Bitcoin), additional techniques such as Merkle tree~\cite{merkle87} based validation will be used to verify the correctness of the results anyway. 
% %If such techniques find out that the set reconciliation is not completed, we could simply start it over and use PBS to reconcile the two sets again under a different hash function $h$. In this case, the checksum will be different If so, the  (note that PBS is a `randomized' algorithm when assuming the hash functions for hash-partition are random hash functions). 
% To simplify our description, we ignore this small probability event and assume the checksum works perfectly in this rest of this paper. 

% We summarize all the above steps of PBS (in the first round) in \autoref{alg:single_round_pbs}.
% %{\bf not a good position to mention `for super critical applications, use a checksum for all groups', since we are describing single-group scenario. }

% \begin{algorithm}
% \caption{Single-round PBS}
% \label{alg:single_round_pbs}

% %Hash-partition $A$, $B$ into $\{A_i\}_{i=1}^n$, $\{B_i\}_{i=1}^n$\; \label{step:hash_partition}

% %Parity encode $\{A_i\}_{i=1}^n$, $\{B_i\}_{i=1}^n$ into $A[1..n]$, $B[1..n]$\; \label{step:parity_encode}
% {\it Alice}: Send $\xi_A$, the BCH codeword of $A[1..n]$, to Bob\; \label{step:BCH_encode}

% {\it Bob}: Decode $(B[1..n], \xi_A)$ to obtain $i_1,i_2,...,i_d$\; \label{step:BCH_decode}

% {\it Bob}: Send the \code{XOR} sums of sets $B_{i_1}, B_{i_2},...,B_{i_d}$ (\autoref{alg1:sender} in \autoref{alg:trivial_case}) and $i_1,i_2,...,i_d$ to Alice\; \label{step:BCH_decode}

% {\it Alice}: Obtain $A_{i_1}\triangle B_{i_1}, A_{i_2}\triangle B_{i_2},...,$ and $A_{i_d}\triangle B_{i_d}$ (\autoref{alg1:receiver} in \autoref{alg:trivial_case}); $\hat{D}\leftarrow \bigcup_{k=1}^d (A_{i_k}\triangle B_{i_k})$\; \label{step:trivial_reconcile}

% {\it Alice}: Check if $c(\hat{D})=c(A\triangle B)$\; \label{step:terminate_condition}

% \end{algorithm}
% {\color{blue}This probability is low enough for most applications. In few applications which allow no room for error ({\it e.g.,} Bitcoin), additional techniques such as Merkle tree~\cite{merkle87} based validation will be used to verify the correctness of the results anyway.}

% {\bf (Previous)} The condition $A=B\triangle\hat{D}$ can be almost surely verified by a $32$-bit checksum, although it could mistakenly believe two different sets as identical ones with probability $2^{-32}\approx 2.3\times 10^{-10}$ {\bf on top of the probability that the nonideal case happens (on the order of $10^{-2}$).} Although this event could cause an ``early'' termination and leave some distinct elements unreconciled, it happens with an extremely small probability (on the order of $10^{-12}$) and should be acceptable in most applications. {\bf To simplify our description, we ignore this small probability event and assume the checksum works perfectly in this rest of this paper. }
%and such an event (i.e., mistaken $A$ and $B\triangle\hat{D}$ are identical when they are different) never happens in our evaluation. For some super critical applications, we can certainly use a $64$-bit checksum to reduce this probability to $5.4\times 10^{-20}$ if needed.

% When the ideal case does not happen, set reconciliation cannot accomplish in one round, as we will explain in \autoref{subsec:exception_hash_partition}. Hence, we add a verfication step to check if set reconciliation is complete. Let $\hat{D}$ denote the set of reconciled elements. The idea of this verification is basically to compare $A$ with $B\triangle \hat{D}$: If $A=B\triangle \hat{D}$ (i.e., $\hat{D}=A\triangle B$), we know the set reconciliation is complete; Otherwise, the set reconciliation is incomplete.  using a $32$-bit checksum. 

% \subsubsection{Communication overhead of PBS (First Round)}\label{sec:communication_overhead_single_PBS}

% %To correct $d$ bit errors, the length of the net-codeword only is no more than $d\log n$ bits. 

% The communication overhead of \autoref{alg:single_round_pbs} consists of four components: (1) the BCH codeword $\xi_A$ in \autoref{step:BCH_encode}; (2) the subset pair indices $i_1,i_2,...,i_d$ in \autoref{step:trivial_reconcile}; (3) the bitwise \code{XOR} sums of sets $B_{i_1}, B_{i_2},...,B_{i_d}$ of $d\log |\mathcal{U}|$ bits in \autoref{step:trivial_reconcile}; and (4) transmit the $32$-bit checksum of $B$ (i.e., $c(B)$) from Bob to Alice for precomputing $c(A\triangle B)$ in \autoref{step:terminate_condition}. These four components contribute roughly (1) $d\log n$ bits (recall that to ``correct'' $d$ bit errors, the length of the BCH codeword is no more than $d\log n$ bits); (2) $d\log n$ bits; (3) $d\log |\mathcal{U}|$ bits; and (4) $32$ bits respectively to the overall communcation overhead of \autoref{alg:single_round_pbs}. 

% All the steps of PBS in the first round are summarized in \autoref{alg:single_round_pbs}. The overall communication overhead consists of three components: (1) the BCH codeword of $d\log n$ bits in \autoref{step:BCH_encode}; (2) the subset pair indices $i_1,i_2,...,i_d$ and the corresponding bitwise \code{XOR}s of $d\log n+d\log |\mathcal{U}|$ bits in \autoref{step:trivial_reconcile}; and (3) the $32$-bit checksum of $A$ in \autoref{step:terminate_condition}. 


% {\it Bob}: BCH-Encodeing $B[1..n]$ and send the codeword to Alice\; \label{step:BCH_encode}

% {\it Alice}: Upon receiving the codeword, decode the bit errors between $A[1..n]$ and $B[1..n]$\; \label{step:BCH_decode}

% {\it Alice}: For each bit error, start reconciling the corresponding subset pair by \autoref{alg:trivial_case}\; \label{step:trivial_reconcile}

% {\it Bob}: Upon receiving the reconciled set difference $\hat{D}$, check if $A=B\triangle \hat{D}$ via checksum\; \label{step:terminate_condition}


% \subsubsection{Single-round PBS}\label{sec:single_round_pbs}

% Here we summarize all the steps of single-round PBS and represent it by pseudocode in \autoref{alg:single_round_pbs}. \autoref{step:hash_partition} and \autoref{step:parity_encode} operates at both hosts (i.e., Alice and Bob). \autoref{step:hash_partition} to \autoref{step:trivial_reconcile} have been elaborated from \autoref{sec:hash_partition} to \autoref{sec:reconcile_by_trivial}. The last step in \autoref{step:terminate_condition} aims to check whether reconciliation is complete (i.e., $\mathcal{D}=A\triangle B$). More specifically, Alice calculates the checksum (e.g., CRC-$32$) of $A$ and send it to Bob. Then Bob calculates the checksum of $B\triangle \mathcal{D}$ and compares it to the receiving checksum of $A$. If the two checksums are the same, we believe $A=B\triangle \mathcal{D}$ and therefore $\mathcal{D}=A\triangle B$ (i.e., reconciliation is complete); Else, we know some elements are reconciled incorrectly. We classify those elements (i.e., the ones in the set difference between $A\triangle B$ and $\mathcal{D}$) into two subsets $A\triangle B\!\setminus\!\mathcal{D}$ and $\mathcal{D}\!\setminus\!(A\triangle B)$ and refer the elements in the former as {\it false-negatives}, and refer the elements in the later as {\it false-positives}. 

% In the ideal case, neither false-positives nor false-negatives will happen and the two checksums always equal. However, in real life, the ideal case does not always happen. We will discuss the nonideal case in \autoref{subsec:exception_hash_partition}. In our evaluation, we use a $32$-bit checksum for comparing $A$ to $B\triangle \mathcal{D}$ that has {\bf an error probability} roughly $10^{-9}$. This error (i.e., mistake $A=B\triangle \mathcal{D}$) incurs false-negatives. All set reconciliation schemes have the same problem on their termination conditions (i.e., check whether $\mathcal{D}=A\triangle B$). For some super critical applications, we can certainly decrease the error probability by using more powerful checksums (i.e., $64-$bit). Using a $32$-bit checksum, this kind of false-negatives never happen in the evaluation. 
% %For simplification, we assume no error happens when checking $\mathcal{D}=A\triangle B$ in the rest of the paper.

% \begin{algorithm}
% \caption{Single-round PBS}
% \label{alg:single_round_pbs}

% Hash-partition $A$, $B$ into $\{A_i\}_{i=1}^n$, $\{B_i\}_{i=1}^n$\; \label{step:hash_partition}

% Parity encode $\{A_i\}_{i=1}^n$, $\{B_i\}_{i=1}^n$ into $A[1..n]$, $B[1..n]$\; \label{step:parity_encode}

% {\it Bob}: Encode $B[1..n]$ by BCH code, then send the codeword to Alice\; \label{step:BCH_encode}

% {\it Alice}: Upon receiving the codeword, decode the bit errors between $A[1..n]$ and $B[1..n]$\; \label{step:BCH_decode}

% {\it Alice}: For each bit error, reconcile the corresponding subset pair by \autoref{alg:trivial_case}\; \label{step:trivial_reconcile}

% {\it Bob}: Upon the reconciled distinct elements $\mathcal{D}$, check whether $A=B\triangle \mathcal{D}$ via checksum\; \label{step:terminate_condition}
% \end{algorithm}



\subsection{Exception Handling}\label{subsec:exception_hash_partition}

When the ideal case does not happen, some subset pairs may contain more than one distinct elements and cannot be successfully reconciled by \autoref{alg:trivial_case}. 
In this case, the checksum verification step will detect this event and trigger another round of PBS to reconcile the ``remaining'' distinct elements, as will be elaborated in \autoref{sec:multi-rounds}.  There are two types of exceptions that can possibly happen in such a subset pair, say $(A_i, B_i)$.

\smallskip
\noindent {\bf Type (\RN{1}) exception}:  $A_i\triangle B_i$ contains a nonzero even number of distinct elements.  In this case $A[i]=B[i]$
since the cardinalities of $A_i$ and $B_i$ are either both even or both odd.  The BCH codeword $\xi_A$ cannot detect this exception.
% and PBS will not reconcile the subset pair yet in this round. 
This exception happens with a small but nontrivial probability.  For example, when $d=5$ and $n=255$ (i.e., throwing $5$ balls each uniformly and randomly into $255$ bins), the probability that some bin has a nonzero even number of (in this case either $2$ or $4$) balls is roughly $0.04$. 
%Note that when a type (\RN{1}) event happens, the checksum (\autoref{step:terminate_condition} in \autoref{alg:single_round_pbs}) can detect that the set reconciliation has not been completed. Then PBS will start another round to reconcile the ``hidden'' distinct elements (the ones that have not been reconciled in this round), 
%so on so force, until all distinct elements are successfully reconciled and the checksum is verified to be correct, 
%as we will describe in \autoref{sec:multi-rounds}. 

% Note that when a Type (\RN{1}) subset pair exists, the $32$-bit checksum (\autoref{step:terminate_condition} in \autoref{alg:single_round_pbs}) can almost surely detect that the set reconciliation is incomplete. If this is the case (i.e., the checksum is verified to be incorrect), PBS will start another round of set reconciliation to reconcile the remaining distinct elements (e.g., the ``hidden'' distinct elements in Type (\RN{1}) subset pairs), so on so force, until all distinct elements are reconciled and the checksum is verified to be correct, as we will describe in \autoref{sec:multi-rounds}. 

\smallskip
\noindent {\bf Type (\RN{2}) exception}: $A_i\triangle B_i$ contains an odd number (at least $3$) of distinct elements.  In this case, $A[i]\neq B[i]$. 
Bob will mistakenly believe that $(A_i, B_i)$ contains exactly one distinct element and try to recover it using \autoref{alg:trivial_case}. The ``recovered'' element $s$ is however the \code{XOR} sum of all distinct elements in $A_i\triangle B_i$ as explained at the end of \autoref{subsec:protocol0}.
We call this $s$ a fake distinct element.
%, which will be mistakenly believed as the distinct element of $(A_i, B_i)$. 
This event happens with a tiny probability.  In the same example above ($d=5$ and $n=255$), 
the probability that some bin has an odd number of balls 
(in this case either $3$ or $5$) is only $1.52\times 10^{-4}$.  
This probability can be further reduced, thanks to the consistent nature of hash-partitioning, which provides us with a no-cost mechanism that can detect fake distinct elements 
{\color{red}(so that they will not be included in $\hat{D}$)} with high probability. 



%%%% Comment out druing revision:
%%%% Although we have describe how to use hash partition to detect type (II) exception, however, we actually
%%%% does not make any use of it (Since anyhow we have to use further reconciliation attempts). 
%%%% For example, we do not describe what should we do when an element s passed 
%%%% or failed this detection. The information here is that the probability that we a fake element passing
%%%% this detection is so low. However, from the feedback of reviewers, this paragraph seems make them confused.
%%%% So I suggest to comment out this paragraph to simplify that information we want to delivery: we can handle 
%%%% the two exceptions so that they will not result in reconciliation errors. 
\begin{algorithm}
\caption{Check whether $s\in \mathcal{U}_i$}
\label{alg:verification}
\If{$h(s)\neq i$} {Discard the ``recovered'' element $s$;}
\end{algorithm}

As shown in \autoref{alg:verification}, the detection mechanism is simply to check whether $s\in \mathcal{U}_i$ (i.e., whether $h(s)\! =\! i$), 
a necessary condition 
for $s$ to be an element in $A_i\triangle B_i$.  
The conditional (upon a type (\RN{2}) exception happening) probability for a fake distinct element, which belongs to any of the $n$ sub-universes with equal probability $1/n$
since it is the \code{XOR} sum of multiple distinct elements in $A_i\triangle B_i$, to pass this check is only $1/n$.  In the same example above ($d\!=\!5$, $n\!=\!255$), 
this conditional probability
is roughly $3.9\!\times\! 10^{-3}$, and hence the probability for both a type (\RN{2}) exception to happen and the resulting fake distinct element to pass this check is 
$1.52 \times 10^{-4} \times 3.9 \times 10^{-3} \approx$ $6\times 10^{-7}$.
%The probability for both events to happen in the same example above ($d=5$ and $n=255$) is $6\times 10^{-7}$, which is the multiplication between the probability for the %type (\RN{2}) exception to happen ($1.52\times 10^{-4}$) and the conditional probability ($3.9\times 10^{-3}$). 
% overhead
This mechanism only requires Alice to locally verify the ``recovered'' elements of \autoref{alg:trivial_case} and 
hence incurs no additional communication overhead. 
%{\color{red}Note that whenever such an element $s$ failed to pass this 
%sub-universe verification check, \autoref{alg:single_round_pbs} excludes it from $\hat{D}$.}
%  Alice can perform the check locally by computing $h(s)$.
% This mechanism only needs to locally verify the ``recovered'' elements of \autoref{alg:trivial_case}.  
% It clearly incurs no additional communication overhead:  Alice can perform the check locally by computing $h(s)$.
%does not incur any additional communication overhead.
%However, fake distinct element belongs to any of the $n$ sub-universes with equal probability $1/n$
%since it is the \code{XOR} sum of multiple distinct elements $A_i\triangle B_i$
% \end{comment}

%Although a distinct element of $(A_i, B_i)$ must be in sub-universe $\mathcal{U}_i$ (i.e., the hash value of the element under $h$ equals to $i$), 


%could be in any sub-universe with probability $1/n$, since it is the bitwise \code{XOR} of multiple distinct elements of $(A_i, B_i)$. Therefore, even when a type (\RN{2}) %exception happens to $(A_i, B_i)$, \autoref{alg:verification} only fails to identify a fake distinct element with a conditional probability of $1/n$, 

\begin{comment}
%% comment out by Long during revision
This said, a fake distinct element $s$ could pass this check and go undetected by \autoref{alg:verification}, albeit with a tiny probability as just shown.  
Even in this case, however, such an $s$ will not be mistakenly ``reconciled into" $A\triangle B$ for the following reason.
%and become a ``trouble-causing'' element.  
In this case, even when all actual distinct elements are successfully reconciled (so that $A\triangle\hat{D}=B\triangle \{s\}$), the checksum verification $c(A\triangle\hat{D})\stackrel{?}{=}c(B)$ would fail, triggering one or more rounds of 
further reconciliation attempts (to be described next) during which the fakeness of this ``trouble-causing'' element $s$ will be detected by Alice.  

Note that the existence of the above two types of exceptions 
will not result in reconciliation error, since 
whenever such an exception happens, the checksum verification in~\autoref{step:terminate_condition} of~\autoref{alg:single_round_pbs}
would fail (as now $\hat{D}\neq (A\triangle B)$, thus $c(A\triangle \hat{D})\neq c(B)$), triggering one or more rounds of 
further reconciliation attempts (to be described next), by which PBS will correctly reconcile all 
distinct elements. We also note that PBS does not need to know in which bins those exceptions happened 
to continue the subsequent reconciliation attempts. 

\end{comment}
%if a fake distinct element $s$ is contained in $\hat{D}$, it is not hard to verify that  is not equal to $B$. Hence the checksums of these two sets will not match and the checksum verification will mistakenly believe that some of the distinct elements in $(A_i, B_i)$ have not %been reconciled yet. This is not a problem for PBS, because the ``trouble-causing'' elements can be detected in the latter rounds of the set reconciliation process, as we will explain in \autoref{sec:multi-rounds}. 

%(i.e., $\hat{D}=(A\triangle B)\cup\{s\}$) will induce that the two sets $A\triangle\hat{D}$ and $B$  of $A\triangle\hat{D}$ and the checksum of $B$ to be different.  and another round of PBS will be triggered. This is not a problem for PBS, because the ``trouble-causing'' elements can be detected in the set reconciliation process of PBS, as we will explain in \autoref{sec:multi-rounds}. 

%Note that a fake distinct element could accidentally happen to be an actual distinct element with vanishing probability. Such a fac element that is not detected by \autoref{alg:verification} 

% Note that a fake distinct element could accidentally happen to be an actual distinct element with vanishing probability. For example, when $(A_i, B_i)$ contains $5$ distinct elements $s_1,s_2,...,s_5$ and $s_1$ happens to be equal to $s_1\oplus s_2\oplus\cdots\oplus s_5$, the fake element (i.e., $s_1\oplus s_2\oplus\cdots\oplus s_5$) happens to be an actual distinct element (i.e., $s_1$), which will be contained in $\hat{D}$. This is not a problem, since in the next round $s_2,s_3,s_4,s_5$ will be hash-partitioned into different subset pairs In this case, the ``fake ''element does not cause any trouble in Each fake distinct element that is not detected by \autoref{alg:verification}, if does not happen to an actual distinct element, is a ``trouble-causing'' element that will be detected in the latter rounds, as we will explain in \autoref{sec:multi-rounds}. Note that a fake distinct element could accidentally happen to be an actual distinct element with vanishing probability. Such a fac element that is not detected by \autoref{alg:verification} 


% \subsection{Running PBS for Multiple Rounds}\label{sec:multi-rounds}

% %{\bf (merged from the following two paragraphs)} 
% To deal with the ``remaining'' distinct elements, we remove (and save) all the distinct elements that has been reconciled in the first round (i.e., $\hat{D}$) and run another round of PBS. More precisely, in the second round, we try to reconcile $A\triangle \hat{D}$ and $B$ by running the same procedure except for using a different and independent hash function (than $h$) to do hash-partition. 
% %instead of reconciling $A$ and $B$ for both (1) removing all the distinct elements that have been reconciled; and (2) keeping all the distinct elements that have not been reconciled, which we will explain shortly. 
% Here we use a different and independent hash function to avoid the same type (\RN{1}), (\RN{2}) exceptions happen again. 
% % We use a different hash function for hash-partition in the second round to avoid the same exceptions (i.e., type (\RN{1}), (\RN{2}) events) that happened in the first round happen again. 
% PBS keeps running until the set reconciliation is successfully completed as verified by the checksum (\autoref{alg:single_round_pbs} of \autoref{step:terminate_condition}). The use of independent hash functions in different rounds naturally enables the Markov chain modeling of the reconciliation process, which will be elaborated in \autoref{sec:single_markov}. 

% {\bf (new content)} Note that a fake distinct element $s$, if is not detected by \autoref{alg:verification}, will be mistakenly believed as a distinct element (between $A$ and $B$) and contained in $\hat{D}$. This is not an issue because in this case, $s$ is an actual distinct element between $A\triangle \hat{D}$ and $B$. Starting with the second round, PBS will try to reconcile $s$ and eventually ``correct'' this fake distinct element. 

% We emphasize that the fake distinct elements (incurred by type (\RN{2}) exception) that are not detected by \autoref{alg:verification} in the first round can also be reconciled in the second round. also keeps all the distinct elements that need to be reconciled. Note that the ``remaining'' distinct elements can be classified into two catagories: (1) the ``hidden'' distinct elements that have not been reconciled yet (i.e., $D\!\setminus\!\hat{D}$), which are incurred by either a type (\RN{1}) event or a type (\RN{2}) event; and (2) the ``fake'' distinct elements incurred by both a type (\RN{2}) event and the corresponding verification failure in \autoref{alg:verification} (i.e., $\hat{D}\!\setminus\!D$). It is not hard to verify that this classification of the ``rest'' distinct elements (i.e., $D\!\setminus\!\hat{D}$ and $\hat{D}\!\setminus\!D$) is a partition of the set difference between $A\triangle \hat{D}$ and $B$, which confirms our emphasis. 

% {\bf (new content)} We emphasize that reconciling $A\triangle \hat{D}$ and $B$ not only removes all the distinct elements that have been reconciled, but also keeps all the distinct elements that need to be reconciled. Note that the ``rest'' distinct elements can be classified into two catagories: (1) the ``hidden'' distinct elements that have not been reconciled yet (i.e., $D\!\setminus\!\hat{D}$), which are incurred by either a type (\RN{1}) event or a type (\RN{2}) event; and (2) the ``fake'' distinct elements incurred by both a type (\RN{2}) event and the corresponding verification failure in \autoref{alg:verification} (i.e., $\hat{D}\!\setminus\!D$). It is not hard to verify that this classification of the ``rest'' distinct elements (i.e., $D\!\setminus\!\hat{D}$ and $\hat{D}\!\setminus\!D$) is a partition of the set difference between $A\triangle \hat{D}$ and $B$, which confirms our emphasis. 

% To deal with the ``remaining'' distinct elements, we remove (and save) all the distinct elements that has been reconciled in the first round (i.e., $\hat{D}$) and run another round of PBS. In the second round, we reconcile $A\triangle \hat{D}$ and $B$ instead of reconciling $A$ and $B$ to remove all the reconciled distinct elements. We use a different hash function for hash-partition in the second round to avoid the same exceptions (i.e., type (\RN{1}), (\RN{2}) events) that happened in the first round happen again. This procedure replicates until If until all distinct elements are successfully reconciled and the checksum is verified to be correct. 

% {\bf (to be removed)} When the ideal case does not happen (i.e., type (\RN{1}) or type (\RN{2}) event happens), PBS will know the set reconciliation has not been completed via the $32$-bit checksum (\autoref{step:terminate_condition} in \autoref{alg:single_round_pbs}). To reconcile those distinct elements that have not been reconciled yet in the first round, we rule out all successfully reconciled elements and run another round of PBS. This procedure replicates until all distinct elements are successfully reconciled and the checksum is verified to be correct.

% {\bf (to be removed)} More specifically, in the second round, we run PBS to reconcile $A$ and $B\triangle \hat{D}$ instead of $A$ and $B$ to rule out all elements that have been reconciled, where $\hat{D}$ is the set of reconciled distinct elements in the first round. We use a different hash function for hash-partition in the second round to avoid the same exceptions (i.e., type (\RN{1}), (\RN{2}) events) that happened in the first round happen again. The later rounds are similarly operated. 

%{\bf Normally, we want PBS to successfully reconcile all distinct elements in only a few rounds (say $3$) with high probability (say $99\%$). Hence, when tuning parameters (to be discussed in \autoref{sec:parameter_settings}), we set a {\it target success probability} $p_0$ of $r$ rounds as a paramenter setting requirement, which aims to ensure the probability that all distinct elements are reconciled in $r$ rounds to be larger than $p_0$. This requirement should also ensure the majority of the distinct elements are reconciled in the first round. Use the same example ($d=5, n=255$), on average $4.81$ out of $5$ distinct elements should be reconciled in the first round. So the total communication overhead in all rounds is only slightly larger than ($1.01$ to $1.07$ times of, as we will show in \autoref{fig:per-round-con}) that in the first round. Due to this reason, we use the communication overhead in the first round (described in \autoref{sec:communication_overhead_single_PBS}) to approximate the total communication overhead of all rounds in parameter settings (to be elaborated in \autoref{sec:parameter_settings}.}

% Although PBS may need to run many rounds to reconcile all distinct elements, the communication overhead mostly happens in the first round, since the majority of the distinct elements should be reconciled in the first round. Use the same example ($d=5, n=255$), on average $4.81$ out of $5$ distinct elements should be reconciled in the first round. So the total communication overhead in all rounds is only slightly larger than ($1.01$ to $1.07$ times of, to be shown in \autoref{fig:per-round-con}) that in the first round. Due to this reason, we use the communication overhead in the first round (described in \autoref{sec:communication_overhead_single_PBS}) to approximate the total communication overhead (all rounds) in parameter settings (to be elaborated in \autoref{sec:parameter_settings}).

%For the moment, we assume no ``fake'' distinct element in type (\RN{2}) subset pairs fails to be detected, which happens with overwhelming probability as explained in \autoref{subsec:exception_hash_partition}. Then 
%PBS reconciles the distinct elements gradually round by round. This is the ``piecewise decodability'' mentioned in \autoref{sec:intro_oursolution}. We use the following example to describe it in details: 
%Given two sets with $10$ distinct elements, in the first round, PBS tries to reconcile the $10$ distinct elements and say $6$ out of the $10$ distinct elements are successfully reconciled. Then the $6$ reconciled distinct elements are removed and PBS tries to reconcile the remaining $4$ distinct elements in the second round. Say $2$ out of the $4$ remaining distinct elements are successfully reconciled, and that leaves $2$ remaining distinct elements to be reconciled in the third round, so on so force. 
% Given two sets $A$, $B$ with $10$ distinct elements, in the first round, PBS hashes them into $7$ distinct subset pairs. $6$ distinct elements are hashed into $6$ distinct subset pairs, and the other $4$ distinct elements are hashed into the same subset pair. Then the former $6$ distinct elements are successfully reconciled in the first round and the later $4$ distinct elements remain to be reconciled in the second round, which are hashed into $3$ distinct subset pairs (under a different hash function). $2$ remaining distinct elements are hashed into $2$ distinct subset pairs, and the other $2$ remaining distinct elements are hashed into the same subset pair. Then the former $2$ remaining distinct elements are successfully reconciled in the second round and the later $2$ remaining distinct elements remain to be reconciled in the third round, so on so force. 
%The dynamics of the number of remaining distinct elements (i.e., $10\leadsto 4\leadsto 2\leadsto \cdots$ in the example) is in nature a Markov chain, which will be elaborated and analyzed in \autoref{sec:single_markov} to derive a tight tail bound of the probability that all distinct elements are reconciled in $r$ rounds.

% Even if the ideal case does not happen, most of the distinct elements should be distributed into different subset pairs, one distinct element in each, and therefore can be successfully reconciled. So in the first round, even if PBS cannot reconcile all distinct elements, it can reconcile the majority of them.
% % (piecewise decodability mentioned in \autoref{sec:intro_oursolution})
% Based on this intuition, we generalize PBS to multi-round, so that the distinct elements that are not reconciled yet in the first round can be reconciled in later rounds.  

% Without loss of generality, we only describe the second round of multi-round PBS, the reconciliation in the later rounds are similar. Let $\hat{D}_1$ denote the set of reconciled elements in the first round. If set reconciliation is not complete in the first round (i.e., the checksum infers $A\neq B\triangle \hat{D}_1$), then multi-round PBS saves $\hat{D}_1$, which includes correctly and incorrectly reconciled elements as described in \autoref{subsec:exception_hash_partition}, and starts the second round to find (1) the remaining distinct elements; (2) the incorrectly reconciled distinct elements in the first round. In the second round, multi-round PBS reconciles $A$ and $B\triangle \hat{D}_1$ instead of $A$ and $B$ (i.e., $B\leftarrow B\triangle\hat{D}_1$) to rule out all elements that have been reconciled. {\bf It uses a hash function that is different from the one used in the first round for hash-partition, otherwise every remaining distinct element will be hashed into the same subset pair and cause the same exception (described in \autoref{subsec:exception_hash_partition}) that happened in the first round.}

% If set reconciliation is complete in the second round, the set of reconciled elements in the second round (denoted as $\hat{D}_2$) should be the union of (1) all distinct elements that have not been reconciled in the first round (i.e., $(A\triangle B)\!\setminus\!\hat{D}_1$); and (2) all incorrectly reconciled elements in the first round (i.e., $\hat{D}_1\!\setminus\!(A\triangle B)$), which is by definition the set difference between $A\triangle B$ and $\hat{D}_1$. Therefore, the overall set difference $A\triangle B$ equals to the set difference between $\hat{D}_1$ and $\hat{D}_2$; Else, multiround PBS saves $\hat{D}_2$ and starts the third round, so on so force. 

% {\bf May need this algorithm to show the dynamics, if so, the earlier algorithm needs to change accordingly.}
% \IncMargin{1em}
% \begin{algorithm}
% \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
% \Input{$A$ and $B$}
% \Input{Maximum number of rounds $r$}
% \Output{$D$}

% $\hat{D},\mbox{ complete} \leftarrow PBS(A,B)$\;

% $D \leftarrow \hat{D}$\;

% \While{!complete and $r>0$}{
	
% 	$B \leftarrow B\triangle\hat{D}$\;

% 	$\hat{D},\mbox{ complete} \leftarrow PBS(A,B)$\;

% 	$D \leftarrow D\triangle\hat{D}$\;

% 	$r \leftarrow r-1$\;
% }

% \caption{Multi-round PBS} \label{proto:multirounds}
% \end{algorithm}\DecMargin{1em}

% The idea of multi-round PBS is quite simple: In each round, we discard the reconciled distinct elements in the previous rounds and aim to find the rest distinct elements from the remaining elements. More specifically, the first round of multi-round PBS is just the same as single-round PBS in \autoref{alg:single_round_pbs}. The second round has the same procedures as the first round. One difference is, we update $B$ by $B\leftarrow B\triangle\mathcal{D}$ in the second round, so that (1) Reconciled distinct elements in $\mathcal{D}$ that were contained in $A\triangle B$ are not longer contained in $A\triangle (B\triangle\mathcal{D})$; and (2) The other distinct elements remain in $A\triangle (B\triangle\mathcal{D})$ and can be reconciled later. The other difference is, we use a different hash function for partition (\autoref{step:hash_partition}) in the second round. Later rounds update $B$ in the same way and also use different hash functions. Multi-round terminates if the check in \autoref{step:termination} is correct. The overall set difference $A\triangle B$ is simply the union of reconciled distinct elements in all rounds. 

% A straightforward approach to discard reconciled distinct elements is to remove them from both $A$ and $B$. This approach however incurs additional communication overhead to update $A$, since only Bob learns the partial set difference in \autoref{step:reconcile}. Therefore, we use the approach in \autoref{step:updateb} that only updates $B$. It has another benefit in \autoref{step:termination}, which only needs to transmit the CRC of $A$ from Alice to Bob in the first round. In the later rounds, \autoref{step:termination} can be checked locally by Bob and does not require any additional communication overhead;

% Note that the communication overhead in the first round accounts for a large percentage of the total communication overhead in multi-round PBS, since most of the distinct elements (over $95\%$ as we will show in {\bf point to the figure}) should be reconciled in the first round. Therefore, we use the same parameter $n$ in later rounds because otherwise we have to compute a new parameter that can only save tiny communication overhead, even though the number of remaining distinct elements is small and can be reconciled using smaller $n$ with high probability. {\bf Due to the same reason, we can the same expression of the communication overhead in single-round PBS to approximate the communication overhead in multi-round PBS.}

% The natural termination condition of multi-round PBS is that all distinct elements are reconciled, which could require a large number of rounds and incur large additional communication overhead (each additional round incurs $d\log n$ bits of additional communication overhead on transmitting BCH codeword). To control the amount of additional communication overhead, we set another termination condition that multi-round PBS runs for at most $r$ rounds (typically $2$ or $3$). This termination condition could cause an `early' termination when some distinct elements have not been reconciled. However, under proper parameter settings (to be discussed in \autoref{sec:parameter_settings}), we can prove that the probability of an `early' termination (i.e., set reconciliation is incomplete in $r$ round) is very small
% %, and even if an `early' termination happens, an overwhelming percentage of distinct elements should have been reconciled, which is sufficient for most applications
% . For example, when $d=5, n=255, r=2$, an `early' termination happens with probability $4.8\times 10^{-4}$ (how to compute this probability will be elaborated in \autoref{sec:tail_bound}).

% For the moment, we assume no incorrectly reconciled distinct elements appears in multi-round PBS, which happens with overwhelming probability as explained in \autoref{subsec:exception_hash_partition}. Then multi-round PBS reconciles the distinct elements gradually round by round. This is the ``piecewise decodability'' mentioned in \autoref{sec:intro_oursolution}. We use the following example to describe it in details: Given two sets $A$, $B$ with $10$ distinct elements (i.e., $d=10$), in the first round, multi-round PBS hashes them into $7$ distinct subset pairs. $6$ distinct elements are hashed into $6$ distinct subset pairs, and the other $4$ distinct elements are hashed into the same subset pair. Then the former $6$ distinct elements are successfully reconciled in the first round and the later $4$ distinct elements remain to be reconciled in the second round, which are hashed into $3$ distinct subset pairs (under a different hash function). $2$ remaining distinct elements are hashed into $2$ distinct subset pairs, and the other $2$ remaining distinct elements are hashed into the same subset pair. Then the former $2$ remaining distinct elements are successfully reconciled in the second round and the later $2$ remaining distinct elements remain to be reconciled in the third round, so on so force. The dynamics of the number of remaining distinct elements (i.e., $10\leadsto 4\leadsto 2\leadsto \cdots$ in the example) is in nature a Markov chain, which will be elaborated and analyzed in \autoref{sec:tail_bound_per_group} to derive a tail bound of success probability (i.e., all distinct elements are reconciled in $r$ rounds) for paramenter settings. 

% In most applications, a high percentage of reconciliation (e.g., $>99\%$ distinct elements are reconciled) is good enough. Therefore, we add another termination condition on the maximum number of rounds (denoted as $r$). The larger $r$ is, the higher percentage of distinct elements will be reconciled. How to set parameters based on $r$ will be elaborated in \autoref{sec:parameter_settings};

% Readers may think the communication overhead of multi-round PBS is proportional to the number of rounds. In fact, the majority of the communication overhead is spent in the first round, since most of the distinct elements (over $95\%$ as we will show in {\bf point to the figure}) are reconciled in the first round. Each additional round only incurs a small amount of additional communication overhead. For example, when $d=10, n=255, |\mathcal{U}|=2^{32}$, assume $8$ distinct elements are reconciled in the first round and the rest $2$ distinct elements are reconciled in the second round. Then the communication overhead in the first round is $432$ bits. That number of the second round is only $160$


%the communication overhead of single-round PBS of $272$ ($2d\log n+d\log |\mathcal{U}|+32$) bits, and each additional round incurs $40$ ($d\log n$) bits of additional communication overhead. 

%among the three components of the communication overhead mentioned in \autoref{sec:communication_overhead_single_PBS}, only the first component (i.e., the BCH codeword) is proportional to the number of rounds. The other two components does not depend on the number of rounds.

% The second component only depends on the total number reconciled elements, which is roughly equal to $d$. The third component, the checksum of $A$, only needs to be sent once in the first round.
%Therefore, the communication overhead of multi-round PBS is only slightly larger than that of single-round PBS when the number of rounds is small (say $3$). For example, when $d=5, n=255, |\mathcal{U}|=2^{32}$, the communication overhead of multi-round PBS of $3$ rounds is $352$ bits, which is roughly $1.3$ times of the communication overhead of single-round PBS ($272$ bits).

% Therefore, each additional round of multi-round PBS only incurs a small amount of additional communication overhead. For example, when $d=5, n=255, |\mathcal{U}|=2^{32}$, the communication overhead of single-round PBS of $272$ ($2d\log n+d\log |\mathcal{U}|+32$) bits, and each additional round incurs $40$ ($d\log n$) bits of additional communication overhead. 

% As we explained in \autoref{sec:reconcile_by_trivial}, the communication overhead in each round is proportional to the number of (remaining) distinct elements, which decreases exponentially as the number of round increase (i.e., the first round reconciles $90\%$ of distinct elements, the second round reconciles $90\%$ of the remaining $10\%$ distinct elements, etc.). So the majority of the communication overhead (i.e., $\approx 90\%$) is in the first round. Therefore, we do not bother to optimize parameters (i.e., smaller $n$) in later rounds to save tiny communication overhead, even though remaining distinct elements become fewer and can be reconciled using smaller $n$;

% The termination condition of multi-round PBS is that all distinct elements are reconciled, which may require many rounds. In most applications, a high percentage of reconciliation (e.g., $>99\%$ distinct elements are reconciled) is good enough. Therefore, we add another termination condition on the maximum number of rounds (denoted as $r$). The larger $r$ is, the higher percentage of distinct elements will be reconciled. How to set parameters based on $r$ will be elaborated in \autoref{sec:parameter_settings};

% Multi-round means multiple round-trip delays. {\bf Thanks for the piecewise decodability of PBS, in almost all practical application scenarios, this tradeoff does not lead to longer response time because the reconciliation of objects identified by the successfully decodable codewords, which constitute the vast majority of all codewords, can run in parallel with the transmissions and decodings of the rest.  In other words, the piecewise decodability effective masks the slightly larger number of communication rounds as far as the response time is concerned.}

\begin{comment}
==============================

The pseudocode of set reconciliation operations in each round is shown as follows:

\IncMargin{1em}
\begin{algorithm}
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
\Input{$A$ and $B^{(in)}$}
\Input{Set of reconciled distinct elements $D^{(in)}$}
\Output{$B^{(out)}$}
\Output{Set of reconciled distinct elements $D^{(out)}$}

% Hash-partition $A^{(in)}$, $B^{(in)}$ into $\{A^{(in)}_i\}_{i=1}^n$, $\{B^{(in)}_i\}_{i=1}^n$ (\autoref{sec:hash_partition})\label{step:hash_partition}\;

% Encode $\{A^{(in)}_i\}_{i=1}^n$, $\{B^{(in)}_i\}_{i=1}^n$ into parity bitmaps (\autoref{sec:parity_bitmap_encoding})\;


% Find those subset pairs (denoted them as $(A^{(in)}_{i_1}, B^{(in)}_{i_1}), ...,(A^{(in)}_{i_k}, B^{(in)}_{i_k})$) that parity bits differ (\autoref{sec:BCH_code})\;

Run single-round PBS on $A$ and $B^{(in)}$ to obtain the (partial) set difference $\mathcal{D}$\label{step:reconcile} \;

$D^{(out)} \leftarrow D^{(in)}\bigcup \mathcal{D}$\label{step:updated}\;

$B^{(out)} \leftarrow B^{(in)}\triangle\mathcal{D}$\label{step:updateb}\;

Check whether the set reconciliation is complete by comparing $A$ to $B^{(out)}$ (via CRC)\label{step:termination}\;

\caption{Set reconciliation operations of PBS in each round} \label{proto:multirounds}
\end{algorithm}\DecMargin{1em}

In \autoref{proto:multirounds}, the output $B^{(out)}$ in the $r^{th}$ round is the input $B^{(in)}$ in the $(r+1)^{th}$ round. $D^{(in)}$ and $D^{(out)}$ have the same relationship, and they denote the set of reconciled distinct elements before and after a round. $B^{(in)}$ and $D^{(in)}$ are initialized as $B$ and $\emptyset$ respectively. We omit the currect number of round $r$ in \autoref{proto:multirounds}, since the operations in different rounds are exactly the same. Due to the same reason, we only elaborate the operations in the first round: First, Alice and Bob reconcile $A$ and $B^{(in)}$ $(=B)$ using single-round PBS and Bob obtains the (partial) set difference $\mathcal{D}$ (\autoref{step:reconcile}); Second, Bob updates the set of reconciled distinct elements by merging it with $\mathcal{D}$ (\autoref{step:updated}); Third, Bob updates $B^{(in)}$ $(=B)$ to $B^{(out)}$ as \autoref{step:updateb} shows, such that (1) The reconciled distinct elements in $\mathcal{D}$ that are contained in $A\triangle B^{(in)}$ are not longer contained in $A\triangle B^{(out)}$; and (2) The distinct elements that are not successfully reconciled remain in $A\triangle B^{(out)}$ and can be reconciled in later rounds; Finally, we check whether all distinct elements are reconciled. Note that if it is true, $B^{(out)}$ should be the same as $A$ and multi-round PBS should terminate. We use a $32$-bit CRC (Cyclic Reduncancy Check) to check if $B^{(out)}=A$ in our evaluation. {\bf To achieve higher confidence, we can certainly use longer CRC (e.g., 64-bit). }

{\bf Remarks:}

(1) In each round, hash-partition in \autoref{sec:hash_partition} uses different hash functions, so that the remaining distinct elements from the last round will be hashed into different subset pairs with high probability;

(2) A straightforward approach to discard reconciled distinct elements is to remove them from both $A$ and $B$. This approach however incurs additional communication overhead to update $A$, since only Bob learns the partial set difference in \autoref{step:reconcile}. Therefore, we use the approach in \autoref{step:updateb} that only updates $B$. It has another benefit in \autoref{step:termination}, which only needs to transmit the CRC of $A$ from Alice to Bob in the first round. In the later rounds, \autoref{step:termination} can be checked locally by Bob and does not require any additional communication overhead;

(3) As we explained in \autoref{sec:reconcile_by_trivial}, the communication overhead in each round is proportional to the number of remaining distinct elements, which decreases exponentially as the number of round increase (i.e., the first round reconciles $90\%$ of distinct elements, the second round reconciles $90\%$ of the remaining $10\%$ distinct elements, etc.). So the majority of the communication overhead (i.e., $\approx 90\%$) is in the first round. Therefore, we do not bother to optimize parameters (i.e., smaller $n$) in later rounds to save tiny communication overhead, even though remaining distinct elements become fewer and can be reconciled using smaller $n$;

(4) One termination condition of Multi-round PBS is $B^{(out)}=A$, which refers that all distinct elements are reconciled. In most applications, a high percentage of reconciliation (e.g., $>99\%$ distinct elements are reconciled) is good enough. Therefore, we add another termination condition of the maximum number of rounds (denoted as $r$). The larger $r$ is, the higher percentage distinct elements will be reconciled, and the smaller $n$ is required. How to set parameters (e.g., $n$) based on $r$ will be elaborated in \autoref{sec:parameter_settings};

(5) Multi-round means multiple round-trip delays. {\bf Thanks for the piecewise decodability of PBS, in almost all practical application scenarios, this tradeoff does not lead to longer response time because the reconciliation of objects identified by the successfully decodable codewords, which constitute the vast majority of all codewords, can run in parallel with the transmissions and decodings of the rest.  In other words, the piecewise decodability effective masks the slightly larger number of communication rounds as far as the response time is concerned.}

==============================

\end{comment}

% (3) Readers may wonder in the later rounds, most distinct elements should be reconciled, and the rest distinct elements could be reconciled using degraded parameters (i.e., smaller $n$ and $t$). In fact, degrade parameters in later rounds cannot save much communication overhead, since the majority of it is spent in the first round (i.e., $>90\%$). Therefore, we use the same parameters (i.e., $n,t$) among all rounds in multi-rounds PBS;

% (4) The number of remaining distinct elements decreases exponentially as the number of round increase (i.e., the first round reconciles $90\%$ of distinct elements, the second round reconciles $90\%$ of the remaining $10\%$ distinct elements, etc.). 
% (4) The termination condition of Multi-rounds PBS is $B^{(out)}=A$ to reconcile all distinct elements. In some applications,  


% The output $B^{(out)}$ in the $r^{th}$ round is the input $B^{(in)}$ in the $(r+1)^{th}$ round. $D^{(in)}$ and $D^{(out)}$ are similarly defined. $B^{(in)}$ and $D^{(in)}$ are initialized as $B$ and $\emptyset$ respectively. Since and $D$ are updated in each round, so we use $B^{(in)}$ to denote the input and $B^{(out)}$ to denote the output respectively.  Specifically, in the first round, we initialize $B^{(in)}$ and $D^{(in)}$ as $B$ and $\emptyset$ respectively. we first use the single-round scheme 

% Then we run our (single-round) scheme on the updated two sets (i.e., after removing reconciled distinct elements) using a different (independent) hash-partition function from previous rounds, so that the rest distinct elements are hashed into different subset pairs (i.e., the ideal case) with high probability. At the end of each round, we check whether the set reconciliation is complete (i.e., all distinct elements are found) by computing the bitwise \code{XOR} of the remaining elements in $A$ and $B$ 
 

% This {\bf multi-rounds} scheme can significantly increase the success probability (i.e., the probability that all distinct elements are reconciled). Readers may wonder in the later rounds, most distinct elements should be reconciled, and the rest distinct elements could be reconciled using degraded parameters (i.e., smaller $n$ and $t$). In fact, degrade parameters in later rounds cannot save much communication overhead, since the majority of it is spent in the first round (i.e., $>90\%$). Therefore, we use the same parameters (i.e., $n,t$) among all rounds in our evaluation. 
% %The tradeoff between the number of rounds and the communication overhead per rounds will be elaborated in \autoref{sec:tail_bound}. In our evaluation, $r=2,3$ rounds are enough to achieve an extremely high success probability. 

% Readers may think the cost (i.e., communication overhead and the computational complexity) of this multi-rounds scheme is proportional to the number of rounds (denoted as $r$) and increases linearly with $r$. In fact, the cost of each round is roughly proportional to the number of remaining distinct elements, which decreases exponentially as $r$ increases (i.e., the first round reconciles $99\%$ of distinct elements, the second round reconciles $99\%$ of the remaining $1\%$ distinct elements, etc.). So the cost of this multi-rounds scheme is only slightly larger than that of the single-round scheme. Furthermore, as we explained in \autoref{sec:intro}, {\bf from intro thanks for the piecewise decodability of our solution, in almost all practical application scenarios, this tradeoff does not lead to longer response time because the reconciliation of objects identified by the successfully decodable codewords, which constitute the vast majority of all codewords, can run in parallel with the transmissions and decodings of the rest.  In other words, the piecewise decodability effective masks the slightly larger number of communication rounds as far as the response time is concerned.} 

\begin{comment}

\subsection{Baseline Scheme}\label{subsec:protocol1} 

Note that the set difference $A\triangle B$ can contain more than 1 elements (i.e., $d>1$), and \autoref{alg:trivial_case} cannot reconcile $A$ and $B$ directly in this case. Therefore, we propose a baseline scheme building upon~\autoref{alg:trivial_case} that also works when $d>1$: First, we partition the element universe $\mathcal{U}$ into $n$ sub-universes $\mathcal{U}_1, \mathcal{U}_2, \cdots, \mathcal{U}_n$. Denote $A_i \triangleq A\bigcap \mathcal{U}_i$ and $B_i \triangleq B\bigcap \mathcal{U}_i$ for $i=1,2,\cdots,n$. Then $\{A_i\}_{i=1}^n$ and $\{B_i\}_{i=1}^n$ are partitions of $A$ and $B$ respectively. Furthermore, $\Phi\triangleq\{A_i\triangle B_i\}_{i=1}^n$ is a partition of $A\triangle B$. 

Assume the {\bf ideal case} happens, in which each subset pair $(A_i, B_i)$ contains at most one distinct element ({\it i.e.,} $|A_i\triangle B_i|\!\leq\!1$), we use \autoref{alg:trivial_case} to reconcile each subset pair and obtain $A_i\triangle B_i$ for $i=1,2,\cdots,n$. The overall set difference $A\triangle B$ is simply their union $\bigcup_{i=1}^n \big{(}A_i\triangle B_i\big{)}$. 

In the first step of the baseline scheme, we can use a hash function $h(\cdot): \mathcal{U}\rightarrow \{1,2,\cdots,n\}$ to partition the universe $\mathcal{U}$ into $n$ sub-universes: $\mathcal{U}_i=\{s\mid s\in \mathcal{U} \mbox{ and } h(s)=i\}$ for $\forall i=1,2,\cdots,n$. And the hash function $h(\cdot)$ can be predetermined between Alice and Bob and does not require additional communication cost.

This hash-partition can be modeled as a {\it balls-into-bins problem}, in which the distinct elements are viewed as balls and the subset pairs are viewed as bins. The hash-parition basically throws (hashes) $d$ balls (distinct elements) uniformly and randomly into $n$ bins (subset pairs). The aforementioned ideal case in this context becomes, after throwing $d$ balls uniformly and randomly into $n$ bins, each bin receives at most 1 ball (i.e., $d$ nonempty bins have 1 ball in each and the rest $n-d$ bins are empty). {\bf It may remind readers about the Birthday problem. And the ideal case can be analogous to the case that no people share the same birthday.} The ideal case happens with a probability of $p=\frac{n\,!}{(n-d)\,!n^d}\!=\!\prod_{k=1}^{d - 1}(1 - \frac{k}{n})\!\approx\! e^{-\frac{d(d-1)}{2n}}$ when $d\!\ll\!n$. In other words, $n$ must be $\Omega(d^2)$ to ensure the ideal case happens with a nontrivial probability.  Note that the communication overhead of the baseline scheme is proportional to $n$, as each subset pair requires communication of a bitwise \code{XOR} in \autoref{alg:trivial_case}. So this communication overhead increases at least quadratically as $d$ increases. 

In fact, this communication overhead can be significantly reduced: In the ideal case, $n-d$ out of $n$ subset pairs are identical ones, and only $d (\ll n)$ out of $n$ subset pairs contain distinct elements (one distinct element in each of the $d$ subset pairs) and need to be reconciled. If we can identify these $d$ subset pairs (with a tiny additional communication overhead) and only reconcile them, the overall communication overhead will be significantly reduced from $\Omega(d^2)$ to $O(d)$. Based on this intuition, we propose our scheme in \autoref{sucsec:our-scheme}, which uses Parity Bitmap Sketch (PBS) and Error Correction Coding (ECC) to identify those subset pairs with a tiny additional communication overhead. 

Note that the ideal case does not always happen. However, we can ensure that the ideal case happens with high probability by properly selecting $n$ based on $d$ (i.e., $n=\Omega(d^2)$). Furthermore, as we will describe in \autoref{subsec:nonideal}, even if the ideal case does not happen (i.e., some distinct elements are hashed into the same subset pair), most of the distinct elements should be distributed into different subset pairs and therefore can be reconciled. So the baseline scheme, even cannot reconcile all of the distinct elements, can still reconcile the majority of them. Based on this property, we will extend our scheme from single-round to multi-rounds in \autoref{subsec:nonideal} to further increase the probability of reconciling all distinct elements. 

For general cases ({\it i.e.,} $t=|A\triangle B|$ is an arbitrary number), we have a straightforward strawman scheme building upon~\autoref{alg:trivial_case}, which works as follows: First, Alice and Bob choose some hash function $h(s): \mathcal{U} \rightarrow \{0,1,\cdots,2^{32}-1\}$ to partition $A$ and $B$ into $m$ subsets $A_1,A_2,\cdots,A_m$ and $B_1,B_2,\cdots,B_m$ respectively:

\begin{align}
s\in A_i & \mbox{ iff } s\in A \mbox{ and } h(s)=i\!\mod m, \nonu{}mber\\
s\in B_i & \mbox{ iff } s\in B \mbox{ and } h(s)=i\!\mod m. \nonumber
\end{align} 

{\bf call a subset pair -> partition?} Since Alice and Bob use the same hash function for partition, common elements (i.e., elements in $A\cap B$) are always hashed into the same subset pair $(A_i, B_i)$. And the set difference of each subset pair only contains distinct elements (i.e., elements in $A\triangle B$): $A_i\triangle B_i \subset A\triangle B$. In the ideal case, with a sufficient large $m$, each subset pair $(A_i, B_i)$ contains at most one distinct element ({\it i.e.,} $|A_i\triangle B_i|\!\leq\!1$). Then \autoref{alg:trivial_case} can reconcile each subset pair and obtain $A_i\triangle B_i$ for $i=1,2,\cdots,m$. The overall set difference $A\triangle B$ is simply their union $\bigcup_{i=1}^m \big{(}A_i\triangle B_i\big{)}$. The selection of hash function $h(s)$ can be predetermined between Alice and Bob and it does not require additional communication cost.

%To make sure Alice and Bob use the same hash function for partition, we let them pre-agree on some universal hash family (e.g., \code{xxHash}~\cite{Collet_xxHashExtremelyfast_}) and a common selection order, and each time they choose a hash function from the family in the same order. Note that we can also let Alice generates a hash function and send it to Bob. The hash function that Alice and Bob choose for partition can be either generated by 

This hash-partition is in nature a {\it balls-into-bins model}. We can view the distinct elements as balls and the subset pairs as bins. The hash-parition basically throws (hashes) $t$ balls (distinct elements) uniformly and randomly into $m$ bins (subset pairs). The aforementioned ideal case in this context is, with a sufficient large number of bins, each bin receives at most 1 ball. The strawman scheme works correctly if and only if the ideal case happens, which has a probability of $\frac{m\,!}{(m-t)\,!m^t}\!=\!\prod_{k=1}^{t - 1}(1 - \frac{k}{m})\!\approx\! e^{-\frac{t(t-1)}{2m}}$. In other words, to ensure the strawman scheme works correctly with a probability of $p$, it roughly requires $m \!=\!\lceil \frac{t(t-1)}{-2\ln p}\rceil$ subset pairs. 

Note that the communication overhead of this strawman scheme is proportional to the number of subset pairs $m$, as each subset pair requires communication of an \code{XOR} sum in \autoref{alg:trivial_case} during the reconciliation. When $t$ is small, a small communication cost can guarantee that the strawman scheme works correctly with high probability. For instance, when $t=5$, $m=95$ subset pairs are sufficient for the strawman scheme to work correctly with a probability of $90\%$. However, when $t$ is relatively large, it requires a huge communication cost to ensure the strawman scheme works correctly. For instance, when $t=1,000$, it requires $m=4,740,865$ subset pairs to guarantee a success probability of $90\%$. 

In fact, the majority of subset pairs are identical ones and do not need to reconcile. And only a small portion of them contain distinct elements. If we can identify those subset pairs that contain distinct elements and only reconcile them, the communication cost could be significantly reduced. Our scheme is based on this intuition and uses parity bitmap sketch and BCH code to identify the subset pairs, which we will elaborate in \autoref{sucsec:our-scheme}. 

%To distribute balls as uniformly as possible and maximize the probability of the ideal case, we choose a uniform hashing function $h$ that throws balls uniformly and randomly into bins: $$\mathbb{P}[h(s)=i]=\frac{1}{m} \mbox{ for } \forall i=1,2,\cdots,m, \forall s\in U$$.

%Note that the probability of the ideal case is $\frac{m\,!}{(m-t)\,!m^t}\!=\!\prod_{k=1}^{t - 1}(1 - \frac{k}{m})\!\approx\! e^{-\frac{t(t-1)}{2m}}$. Hence, at least $\lceil \frac{t(t-1)}{-2\ln p}\rceil$ bins are required to ensure that this probability is at least $p$. In other words, to ensure that the ideal case happens with a probability of $p$, the strawman scheme roughly requires $m \!=\!\lceil \frac{t(t-1)}{-2\ln p}\rceil$. For example, suppose $t\!=\!$\num{1000}, %and $p\!=\!0.01$, this strawman scheme roughly requires $m\!=\!$\num{720626} bins (partitions) to ensure that $|A_i\triangle B_i|\!\leq\!1$ (for any $i=1,2,\cdots,m$) holds with probability $50\%$.  

% A straightforward strawman scheme building upon~\autoref{alg:trivial_case} 
% to reconcile two sets $A$ and $B$ in general 
% ({\it i.e.,} $|A\triangle B|$ is an arbitrary number) is the following: 
% Uniformly randomly partition $A$ and $B$ into $m$ subsets ($A_1,A_2,\cdots,A_m$ 
% and $B_1,B_2,\cdots,B_m$) so that the set difference 
% $A_i\triangle B_i$ of each subset pair $(A_i, B_i)$ contains at most one element 
% ({\it i.e.,} $|A_i\triangle B_i|\!\leq\!1$) {\it w.h.p.} ({\it i.e.,} with high probability), 
% and then reconcile each subset pair with~\autoref{alg:trivial_case}. 

% Now let us analyze this strawman scheme using the {\it balls-into-bins model}. 
% Assume that sets $A$ and $B$ have $t$ elements in their set difference, {\it i.e.,} $|A\triangle B|\!=\!t$. 
% These $t$ elements can be viewed as $t$ balls and the $m$ partitions (subset pairs) can be viewed as 
% $m$ bins. The random partition process in this strawman scheme can be modeled as throwing 
% $t$ balls into $m$ bins in the following manner: Each ball goes into a 
% uniformly random bin and independently of other balls. %so that each bin contains at most one ball, {\it w.h.p.}  
% The probability that each bin contains at most one ball is  
% $\frac{m\,!}{(m-t)\,!m^t}\!=\!\prod_{k=1}^{t - 1}(1 - \frac{k}{m})\!\approx\! e^{-\frac{t(t-1)}{2m}}$. 
% Hence, at least $\lceil \frac{t(t-1)}{-2\ln p}\rceil$ bins are required 
% to ensure that this probability is at least $p$. In other words, to ensure 
% that each bin contains at most one ball with a probability of $p$, 
% the strawman scheme roughly requires $m \!=\!\lceil \frac{t(t-1)}{-2\ln p}\rceil$. 
% For example, suppose $t\!=\!$\num{1000}, %and $p\!=\!0.01$, 
% this scheme roughly requires $m\!=\!$\num{108469} bins (partitions) to 
% ensure that $|A_i\triangle B_i|\!\leq\!1$ (for any $i=1,2,\cdots,m$) holds with probability $0.01$.  

% We note that the communication overhead of this strawman scheme is proportional to 
% $m$ ($\!\gg\! t$), as each partition (subset pair) requires communication of an \code{XOR} sum during the reconciliation. 
% This communication overhead is much higher than that of the optimal scheme, which only requires 
% to exchange the elements in the set difference (assuming an oracle tells it which elements belong to 
% the set difference), {\it i.e.,} proportional to $t$. In the example above, assuming each element takes 4 bytes, 
% the communication overhead of the strawman scheme is $4m$ bytes ($\!\approx\! \num{423.71}\,$KB) to ensure 
% a success rate of only 0.01 ({\it i.e.,} with a probability of $0.0.1$, all elements in 
% the set difference are successfully reconciled), 
% which is approximately 2 orders of magnitude higher than $4t$ bytes ($\!=\!\num{3.90}\,$KB), the communication 
% overhead of the optimal scheme. 

\subsection{Our Scheme: The Preliminary Version}\label{sucsec:our-scheme}

Like the baseline scheme, our scheme also hash-partitions the two sets $A$ and $B$ into $n$ subset pairs. The difference is, instead of reconciling all subset pairs using \autoref{alg:trivial_case}, our scheme identifies the subset pairs that contains distinct elements and only reconciles them. Since the hash-partition and set reconciliation on each subset pair using \autoref{alg:trivial_case} have been described in \autoref{subsec:protocol1}, we only elaborate how to identify the subset pairs that contain distinct elements in this section. 

The general idea of identification is very simple: First, we {\bf encode} each subset into $1$ bit, such that in the ideal case, for $\forall i=1,2,\cdots,n$:

\begin{itemize}
	\item The codewords (bits) of $A_i$ and $B_i$ are different if and only if subset pair $(A_i, B_i)$ contains $1$ distinct element;
	\item The codewords (bits) of $A_i$ and $B_i$ are the same if and only if subset pair $(A_i, B_i)$ contains no distinct element;
\end{itemize}

Second, we {\bf compare} the codewords of each subset pair. And the subset pairs that contain distinct elements are the ones with different codewords (bits). We will describe the two steps in details in \autoref{sec:parity_bitmap_encoding} and \autoref{sec:BCH_code} respectively.

\subsubsection{Parity Bitmap Encoding}\label{sec:parity_bitmap_encoding}

In our scheme, we use {\it parity encoding} to encode each subset into a parity bit. More specific, it encodes a subset as ``1'' if it contains odd number of elements, and as ``0'' otherwise. And it satisfies the aforementioned requirements in the ideal case:

\begin{itemize}
	\item If subset pair $(A_i, B_i)$ contains $1$ distinct element, the corresponding two subsets $A_i$ and $B_i$ differ exactly one element, which implies that $||A_i|\!-\!|B_i||\!=\!1$. Hence, if $|A_i|$ ({\it i.e.,} number of elements in $A_i$) is odd (or even), then $|B_i|$ must be even (or odd). And the parity bits of $A_i$ and $B_i$ will be different;
	\item If subset pair $(A_i, B_i)$ contains no distinct element, the corresponding two subsets $A_i$ and $B_i$ should be the same and therefore contain the same number of elements. Hence, if $|A_i|$ is odd (or even), then $|B_i|$ must be odd (or even). And the parity bits of $A_i$ and $B_i$ will be the same;
\end{itemize}

Using parity encoding, the $n$ subsets of $A$ are encoded as a bit string $A[1..n]$ in $\{0,1\}^n$, 
where the $i$-th bit $A[i]$ in $A[1..n]$ corresponds to the parity encoding bit of $A_i$. Similarly, the $n$ subsets of $B$ are similarly 
encoded as a bit string $B[1..n]$. We call $A[1..n]$ ($B[1..n]$) the {\it parity bitmap} of $\{A_i\}_{i=1}^n$ ($\{B_i\}_{i=1}^n$). In the ideal case, $A[1..n]$ and $B[1..n]$ differ at $d$ different bit-positions, which corresponds to the $d$ subset pairs that contain distinct elements. And our scheme only reconciles those subset pairs that the parity bits are different. We will describe the nonideal case (i.e., some subset pair contains more than 1 distinct elements) in \autoref{subsec:nonideal}.

\subsubsection{Parity Bitmap Comparison Using BCH Code}\label{sec:BCH_code}

A straightforward approach to compare the parity bitmaps is to let Bob send the complete parity bitmap $B[1..n]$ to Alice, then Alice compares $A[1..n]$ with $B[1..n]$ locally. This approach has a communication overhead of $n$ bits, which is unnecessarily high. As we discussed in~\autoref{subsec:protocol0}, $d$ is usually much smaller than $n$. It means $A[1..n]$ and $B[1..n]$ differ only at a tiny portion of bits. Therefore, we can view $A[1..n]$ as a corrupted message of $B[1..n]$ with $d$ corrupted bits, and the bit-positions of the $d$ corrupted bits basically correspond to the $d$ subset pairs that contain distinct elements. The detection of corrupted bits, on the other hand, can be solved by Error-Correction Code (ECC)~\cite{Lin_ErrorControlCoding_1983}. And our scheme uses BCH code~\cite{Lint_IntroductionCodingTheory_1998} to encode the parity bitmap and detect the $d$ corrupted bits.

More specific, after the parity bitmap encoding, Bob uses a $d$-error-correcting systematic BCH code to encode $B[1..n]$ into an $n+d\log n$ codeword, in which the first $n$ bits are $B[1..n]$ (property of systematic BCH code). Then Bob sends the rest $d\log n$ bits, which we denote as {\it parity bitmap sketch (PBS)}, to Alice. Upon the received PBS and $A[1..n]$ (corrupted message), Alice uses the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} to detect the $d$ corrupted bits in $A[1..n]$. The communication overhead of this approach is $d\log n$ bits (i.e., length of PBS), which is much smaller than that of the straightforward approach ($n$ bits, when $d\!\ll\!n$). On the other hand, the computational complexity of the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} is $O(d^2\log^2 n)$. 

\subsubsection{Exceptional Handling and Multi-rounds}\label{subsec:nonideal}

As we described in \autoref{subsec:protocol1}, the ideal case does not always happen, which means some subset pair may contain more than 1 distinct elements and cannot be successfully reconciled by \autoref{alg:trivial_case}. Due to the parity encoding, we can classify such subset pair into the following two scenarios:

\begin{itemize}
    \item Scenario 1: If a subset pair $(A_i, B_i)$ contains even number ($\geq 2$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be the same and our scheme will not reconcile the subset pair. Hence, the distinct elements in the subset pair will not be reconciled;
    \item Scenario 2: If a subset pair $(A_i, B_i)$ contains odd number ($\geq 3$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be different and our scheme will reconcile the subset pair using \autoref{alg:trivial_case}. However, as we described in \autoref{subsec:protocol0}, when a subset pair contains more than 1 distinct elements, \autoref{alg:trivial_case} will output the bitwise \code{XOR} of them as the `distinct element', which is not a real distinct element with high probability;
\end{itemize}

In both scenarios, the distinct elements in the subset pair cannot be reconciled. Even worse, in the second scenario, a false-positive could happen (i.e., the output of \autoref{subsec:protocol0} is not a real distinct element). However, as we will analyze in \autoref{sec:tail_bound} and show in {\bf the evaluation section}, the second scenario barely happens both theoretically and empirically. To further reduce the chance of false-positives, we add a verification step at the end of \autoref{subsec:protocol0} to check whether the output of \autoref{subsec:protocol0} $s$ is a real distinct element or not. The verification step works as follows: Given the output $s$ of subset pair $(A_i,B_i)$, if $s\in\mathcal{U}_i$ (i.e., $h(s)=i$), we consider $s$ as a real distinct element; Otherwise, we consider $s$ as an incorrect output and discard it. 

Note that if $s$ is a real distinct element of $(A_i,B_i)$, $s$ must be in sub-universe $\mathcal{U}_i$. However, if $s$ is the bitwise \code{XOR} of the distinct elements in $(A_i,B_i)$ (i.e., the second scenario happens), $s$ could be in any sub-universe other than $\mathcal{U}_i$. In fact, if we assume the hash-partition described in \autoref{subsec:protocol1} hashes the elements of $\mathcal{U}$ uniformly, independently, and randomly into $n$ sub-universes, the output $s$ in the second scenario will be in a different sub-universe $\mathcal{U}_j (j\neq i)$ with a high probability of $1-\frac{1}{n}$. Hence, this verfication step can reduce the chance of false-positives by a factor of $\frac{1}{n}$. 

Even if the ideal case does not happen, most of the distinct elements should be distributed into different subset pairs and therefore can be reconciled. So our scheme, even cannot reconcile all of the distinct elements, can still reconcile the majority of them (piecewise decodability). To reconcile the rest distinct elements, we can just run our scheme for another round under a different hash-partition function, so on so force. This {\bf multi-rounds} scheme can significantly increase the success probability (i.e., the probability that all distinct elements are reconciled). Readers may wonder in the later rounds, most distinct elements should be reconciled, and the remaining could be reconciled using degraded parameters (i.e., smaller $n$ and $t$). In fact, degrade parameters in later rounds cannot save much communication overhead, since the majority of it is spent in the first round (i.e., $>90\%$). Therefore, we use the same parameters (i.e., $n,t$) among all rounds in our evaluation.
%The tradeoff between the number of rounds and the communication overhead per rounds will be elaborated in \autoref{sec:tail_bound}. In our evaluation, $r=2,3$ rounds are enough to achieve an extremely high success probability. 

Readers may think the cost (i.e., communication overhead and the computational complexity) of this multi-rounds scheme is proportional to the number of rounds (denoted as $r$) and increases linearly with $r$. In fact, the cost of each round is roughly proportional to the number of remaining distinct elements, which decreases exponentially as $r$ increases (i.e., the first round reconciles $99\%$ of distinct elements, the second round reconciles $99\%$ of the remaining $1\%$ distinct elements, etc.). So the cost of this multi-rounds scheme is only slightly larger than that of the single-round scheme. Furthermore, as we explained in \autoref{sec:intro}, {\bf from intro thanks for the piecewise decodability of our solution, in almost all practical application scenarios, this tradeoff does not lead to longer response time because the reconciliation of objects identified by the successfully decodable codewords, which constitute the vast majority of all codewords, can run in parallel with the transmissions and decodings of the rest.  In other words, the piecewise decodability effective masks the slightly larger number of communication rounds as far as the response time is concerned.} 

\end{comment}

\input{section/multiround}

\subsection{BCH Encoding and Decoding}\label{sec:ecc-trick-bch}

\begin{comment}
{\color{red}
%%%%%%%%% by Long %%%%%%
%% Reason: I think that the following description of BCH can not 
%%         fully address BCH related comments.
%%%%%%%%%%%%%%%%
%% suggested to change to Error-Correction Coding Trick  and move to somewhere earlier
% Since PBS uses the error-correction coding (ECC) trick, we first give some background on 
% ECC. Then, we explain this trick and why we choose BCH codes in trick. 
%As explained earlier and 
%As shown in {\bf Procedure 2!!!}, 
In this section, we explain the error-correction coding trick and why we choose BCH codes in this trick. 
Before that, we first give some background on ECC for this paper to be self-contained. 
Given a message $u\in\{0,1\}^k$, an ECC encodes $u$ into $v\in\{0,1\}^{k'}$ with $k'>k$, where 
$v$ is referred to as the {\it codeword} of the message $u$. 
% Note that the the original message $u$ 
% may or may not appear in its codeword; codes that embed the original message in the codeword are 
% systematic and that do not are non-systematic. 
In this work, we only use the systematic codes, in which the original message is part of its codeword. 
For ease of presentation, we assume that the first $k$ bits in the codeword $v$ are from the original message.  
Thus the codeword can be written as $v=[u,\xi_u]$, where $\xi_u$ is referred to as the parity-check 
digits. 
When the codeword $v$ is transmitted over a noisy channel, the output of the channel or the received 
vector $v'$ may be different from $v$. For example, an error pattern of $l$ errors will cause 
$l$ different bits between $v'$ and $v$. Upon receiving $v'$, this ECC needs to decode $v'$ (to learn the original message): 
Locating the bit errors in $v'$ (of course, without knowing $v$ or the error pattern), 
{\it i.e.,} identifying the bit positions where $v'$ differs from $v$. 
Properly designed, an ECC can guarantee correcting 
all error patterns of no more than $t$ errors, where $t$ is called the error-correcting capacity of this code. 
%
% An ECC has an error-correcting capacity. This capacity is defined as the maximum 
% number of bit errors this code is designed to correct. 
Clearly,  
the larger the error-correcting capacity $t$ is, the longer the parity-check digits should be.

Now, we can explain the ECC trick used in PBS. Recall that, in PBS we view the bitmap $A[1..n]$ as the original message. 
The codeword $[A,\xi_A]$ of $A$, after transmitting over an imaginary noisy channel, becomes $[B,\xi_A]$. 
Properly parameterized,  
$\xi_A$ (together with $B$) can pinpoint to Bob all bit positions where $B[1..n]$ and $A[1..n]$ differ.  
% ({\it i.e.}, ``correct all bit errors in $B[1..n]$"). 
While many error-correction codes can be used in this ECC trick, we choose BCH codes in PBS because 
they are close to optimal in the following sense: In the context of PBS, to ``correct up to $t$ bit errors", 
$\xi_A$ only needs to be $t \lceil\log_2 (n + 1)\rceil$ bits long; 
even if Alice knew these $t$ bit positions precisely, specifying each bit position would require $\lceil\log_2 n\rceil$ bits. 
Note that, $n$ is almost always set to $2^m-1$ for some positive integer $m$ in BCH codes 
for achieving the maximum coding efficiency. We also assume this throughout this paper. 

We note that the BCH encoding in PBS differs slightly from the standard BCH encoding, 
since errors only happen in the message part of the codeword in the imaginary noisy channel in PBS, whereas 
they could happen anywhere in the codeword in general. How they differ from each other will be elaborated in~\autoref{app:bch}
}
% \begin{comment}

Recall that in~\autoref{step:BCH_encode} of~\autoref{alg:single_round_pbs}, Alice sends, instead of the ``message'' $A[1..n]$ itself, its much shorter BCH codeword $\xi_A$ to Bob.  Properly parameterized,  
$\xi_A$ can pinpoint to Bob all bit positions where $B[1..n]$ and $A[1..n]$ differ ({\it i.e.}, ``correct all bit errors in $B[1..n]$").  
In the context of PBS, to ``correct up to $t$ bit errors", $\xi_A$ needs to be $t \lceil\log_2 (n + 1)\rceil$ bits long.  This length is intuitively close to the optimal:  
Even if Alice knew these $t$ bit positions precisely, specifying each bit position would require $\log_2 n$ bits.  
%Since, in PBS, $n$ is always set to $2^m - 1$ for some 
%integer $m$, we drop the ``floor" and ``ceiling" and simply write the length of $\xi_A$ as $t \log_2 n$ in the sequel.
\end{comment}

%%%%%
{\color{red}
In this section, we describe the specific BCH encoding and decoding in PBS;  how this encoding differs from 
%that are closely related to the PBS design and parameterization;
%explain the differences between this encoding and the BCH encoding 
that for its usual application of communication over a noisy channel will be explained in~\autoref{app:bch}. 
Recall that in~\autoref{step:BCH_encode} of~\autoref{alg:single_round_pbs}, Alice sends, instead of the ``message'' $A[1..n]$ itself, its much shorter BCH codeword $\xi_A$ to Bob.  
We define the {\it error-correction capacity} of an ECC codeword as the maximum number of bit errors it can correct.
In the case of PBS-for-small-$d$, where $d$ is assumed to be known 
precisely beforehand,   
the error-correction capacity of $\xi_A$ is set to $d$
so the BCH decoding is always successful.  
However, as will be explained in~\autoref{subsec:parameterize-n-t}, when $d$ is large and the sets $A$ and $B$ each has to be partitioned into groups,
the number of ``bit errors" that occur to a group pair can exceed the error-correction capacity 
of the corresponding BCH codeword.  
In this case, a BCH decoding failure will happen and how to deal with its fallout will be explained in~\autoref{sec:BCH_exception}.

We now briefly explain what is involved for Bob to decode the BCH codeword $\xi_A$ against its local bitmap $B[1..n]$.
Here the only task is to figure out the ``bit error positions" (in which $A[1..n]$ and $B[1..n]$ differ).  To do so, Bob needs to 
invert a $t \times t$ matrix in which each matrix entry is an element of the finite field $GF(2^m)$ where $m = \lceil\log_2 (n + 1)\rceil$.
In PBS, $n$ is always set to $2^m-1$ for some positive integer $m$ in BCH codes 
for achieving the maximum coding efficiency.  Hence, 
we drop ``floor" and ``ceiling" and consider $m = \log_2 n$ in the sequel.
Normally such a matrix inversion would take $O(t^3)$ finite field operations over $GF(2^m)$.   However, since this matrix takes a special form called Toeplitz, 
it can be inverted in $O(t^2)$ operations over $GF(2^m)$ using the Levinson algorithm~\cite{levinson1946wiener}.  
}

% \end{comment}


\begin{comment}
There are two different BCH encoding techniques: {\it systematic} and {\it unsystematic}. The difference is that, in systematic encoding, the message appears as the prefix of 
the codeword (i.e., 
codeword = [message, net-codeword]), whereas in unsystematic BCH encoding, the message does not.  Only systematic BCH encoding is suitable for PBS, 
since Alice sends not the ``message'' $A[1..n]$ itself, but the net-codeword $\xi_A$. With this understanding, in the sequel we drop the prefix ``net-" and simply 
call $\xi_A$ a BCH {\it codeword}. 
\end{comment}

\begin{comment}


=== move to appendix in the arxiv version === begin


%In general, BCH decoding consists of two steps:  locating bit errors 

In this section, we describe the standard BCH encoding 
for its usual application of communication over a noisy channel and explain how it differs from the BCH encoding in BPS.   
In the standard BCH encoding, a coded message, which is the uncoded message concatenated with the codeword, is $n = 2^m - 1$ bits long 
in total.  For the codeword to correct up to $t$ bit errors, that may occur to both the uncoded message part and the codeword part 
during the transmission of the coded message over the noisy channel, it needs to be $tm$ bits long, resulting in a ``leftover" of 
at most $n - tm$ bits for the uncoded message.
%To summarize, in the standard BCH encoding, a codeword roughly of length $2tm$ bits is needed to correct 
%up to $t$ bit errors that may occur to either the uncoded message roughly of length $n - 2tm$ bits or the codeword.  

In PBS, the codeword $\xi_A$ is also $tm$ bits long, but the uncoded message $A[1..n]$ (which is not transmitted at all) can be $n$ bits 
(instead of $n - mt$ bits) long.  The uncoded message is allowed to be longer here because, unlike in the usual application 
of communication over a noisy channel where bit errors can happen also to the codeword, 
in PBS no bit error will happen to the codeword $\xi_A$ during its transmission.  


=== end ===
\end{comment}
%%% Moved from related work
%\input{section/pinsketch} 

==> section/pbs_small_d_copy.tex <==
%\section{PBS for small \texorpdfstring{$d$}{d}}\label{sec:scheme}
\section[PBS for small \texorpdfstring{$d$}{d}]{PBS for small \texorpdfstring{\larger\boldmath\MakeLowercase{$d$}}{d}}\label{sec:scheme} 

In this section, we describe how the PBS scheme allows Alice and Bob to reconcile their respective sets $A$ and $B$, where $d\!=\!|A\triangle B|$ is assumed to be small and precisely known. 
%Throughout this paper, we call each element in $A\triangle B$ a \textit{distinct element}, and each element in $A\bigcap B$ a \textit{common element}. 
We start with the trivial case where $d\!\leq\! 1$ in \autoref{subsec:protocol0} and then generalize the scheme for the case where $d$ is a small number in \autoref{sec:pbs_smalld}. 
{\color{red}As will be explained later in~\autoref{sec:BCH_code}, the latter will use the former as a building block.}
% We build up our scheme gradually by starting with the trivial case where $d\leq 1$ in \autoref{subsec:protocol0}. Then we generalize our scheme to the case where $d$ is a small number in \autoref{sec:pbs_smalld}. 

\begin{comment}
\subsection{Problem Statement}\label{sec:model}

In this work, we adopt the commonly used model for the set reconciliation problem. 
Two remote sets $A$ and $B$ are stored at hosts Alice and Bob respectively. 
Each element in $A$ and $B$ is a hash signiture in the key space (universe) $\mathcal{U}$, which is the set of all $(\log |\mathcal{U}|)$-bit binary strings. 
%Each element in $A$ and $B$ is a hash signiture with signiture width $w$ in the key space (universe) $\mathcal{U}$, which is the set of all $w$-bit binary strings (i.e., $|\mathcal{U}|=2^w$). 
%We use $\mathcal{U}$ to denote the set of all $w$-bit binary strings and name it the universe of signitures. 
The set reconciliation problem is to compute the symmetric set difference between $A$ and $B$, 
{\it i.e.,} $A\triangle B\triangleq (A\!\setminus\! B) \bigcup (B\!\setminus\! A)$. 
Let $d\!=\!|A\triangle B|$ be the cardinality of this difference.
%We denote $d\!=\!|A\triangle B|$. 
Throughout this paper, we call each element in $A\triangle B$ a \textit{distinct element}, and each element in $A\bigcap B$ a \textit{common element}.
{\bf Like in all existing solutions, we describe only {\it unidirectional} set reconciliation, in which Alice or Bob learns the set difference $A\triangle B$. Since the performance of our scheme does not depend on who learns the set difference, we assume Bob learns the set difference $A\triangle B$ in the rest of the paper, as mentioned in \autoref{sec:psea}.}
% As mentioned in \autoref{sec:psea}, we describe {\it unidirectional} set reconciliation that Bob learns the set difference $A\triangle B$. 
%In \autoref{sec:evaluation}, we use the same semantic to measure the communication cost of our scheme and other compared set reconciliation schemes. 
\end{comment}

\subsection{The Trivial Case of \texorpdfstring{\larger\boldmath $d\leqslant 1$}{d<2}}\label{subsec:protocol0}

%We start with the trivial case, in which $A$ and $B$ have at most one distinct element ({\it i.e.,} $d\leq 1$), we have a simple set reconciliation scheme showed in \autoref{alg:trivial_case}:
\begin{algorithm}
\caption{Set reconciliation when $d\le 1$}
\label{alg:trivial_case}

{\it Bob}: $s_B\leftarrow\underset{b\in B}{\oplus} b$; Send $s_B$ to Alice\; \label{alg1:sender}

{\it Alice}: $s_A\leftarrow\underset{a\in A}{\oplus} a$; $s\leftarrow s_A \oplus s_B$\; \label{alg1:receiver}
\end{algorithm}

\autoref{alg:trivial_case} shows the set reconciliation scheme for the trivial case, in which $A$ and $B$ differ by at most one (distinct) element. 
It consists of two steps. First, Bob calculates the \code{XOR} sum $s_B$, the bitwise-\code{XOR} of all elements in $B$, and sends it to Alice. 
Second, Alice calculates $s_A$, the \code{XOR} sum of all elements in $A$.  Upon receiving $s_B$ from Bob, Alice computes $s\!\triangleq\! s_A \!\oplus\! s_B$. 
The value of $s$ tells Alice which of the following two cases happens.
%Depending on whether $A$ and $B$ have a distinct element, there are  two possibilities:

\begin{sitemize}
	\item Case (\RN{1}): If $s=\mathbf{0}$, which implies $s_A=s_B$, Alice concludes that $A$ and $B$ have no distinct element or $A=B$. 
	Here $\mathbf{0}$ denotes the $\log |\mathcal{U}|$-bit-long all-$0$ string;
	\item Case (\RN{2}): If $s\not=\mathbf{0}$, which implies $s_A\not=s_B$, Alice concludes that $A$ and $B$ have exactly one distinct element which is $s$, i.e., 
	$A\triangle B=\{s\}$.  This is because \code{XOR}ing $s_A$ and $s_B$ (to obtain $s$) cancels out all (common) elements in $A\bigcap B$.   
%	Here {\it common elements} are defined as the 
%	Here an element that is contained in both sets is called a common element  
	%And $s$ is the missing element of $A$ (i.e., $s\in B\!\setminus\! A$) if $s\in B$, or the missing element of $B$ (i.e., $s\in A\!\setminus\! B$) otherwise;
	% \item If $A$ and $B$ has more than one distinct elements (i.e., $d>1$), the bitwise \code{XOR} of $s_A$ and $s_B$ will still cancel out all common elements and remain the \code{XOR} of the distinct elements, i.e., $s$ is the \code{XOR} of all distinct elements;
\end{sitemize}

Like in most of the literature on set reconciliation, we assume that the all-$0$ element 
$\mathbf{0}$ is excluded from the universe  $\mathcal{U}$, since otherwise \autoref{alg:trivial_case} does not work 
%when $\mathbf{0}\!\in\! A\bigcup B$ %$\mathbf{0}\in A\bigcap B$ 
for the following reason.  When the computed $s$ is $\mathbf{0}$, Alice cannot tell whether $A$ and $B$ are identical, or they have $\mathbf{0}$ as their distinct element. 
%However, we can extend our scheme to support $\mathbf{0}$. For example, we let Alice send to Bob a single bit to indicate whether Alice has element $\mathbf{0}$, so Bob will know whether $\mathbf{0}\in A\triangle B$ or not. 

\autoref{alg:trivial_case} also does not work when there are more than one distinct elements in $A\triangle B$ (i.e., $d>1$), since the computed $s$ in this case 
is the \code{XOR} sum of all these distinct elements.

% Note that \autoref{alg:trivial_case} works if and only if $|A\triangle B|\!\leq\! 1$ and $0\!\notin\! (A\!\cup\! B)$ (which we have explained in~\autoref{sec:model}). 

%\subsection{PBS: When $d$ is small}\label{sucsec:our-scheme}

%In this section, we generalize PBS to the case when $d$ is a small number, as we described in \autoref{sec:smalld}. 
%First, we describe each step of single-round PBS from \autoref{sec:hash_partition} to \autoref{sec:reconcile_by_trivial} and summarize it in \autoref{sec:single_round_pbs}. Second, we discuss the exceptions in single-round PBS in \autoref{subsec:exception_hash_partition}. Third, we propose multi-round PBS to handle the exceptions.

\subsection{The General Case}\label{sec:pbs_smalld}
%\subsection{PBS for small \texorpdfstring{\larger\boldmath $d$}{d}}\label{sec:pbs_smalld}

In this section, we describe the scheme for the more general case where $d$ is 
%no longer limited to be no more than $1$, but 
a small number that is no more than several, but is not necessarily $0$ or $1$.
%In this section, we substantiate the scheme described in \autoref{sec:smalld} for small $d$.

\subsubsection{Hash-partitioning and parity bitmap encoding}\label{sec:hash_partition}
% \medskip
% \noindent{\bf Hash Partition} 

Here we formalize the aforementioned process of partitioning $A$ into $\{A_i\}_{i=1}^n$, $B$ into $\{B_i\}_{i=1}^n$, and $A\triangle B$ into $\{A_i\triangle B_i\}_{i=1}^n$ 
using a hash function $h$. % $h(\cdot)$ changed by Long @0229-2020 for consistency
%as described in \autoref{sec:smalld} by introducing the concept of {\it sub-universes}. Given a hash function $h(\cdot): \mathcal{U}\rightarrow \{1,2,\cdots,n\}$, we 
Define {\it sub-universe} $\mathcal{U}_i$ as the set of elements in the universe $\mathcal{U}$ that are hashed into value $i$. More precisely, $\mathcal{U}_i\triangleq\{s\!\mid\! s\in \mathcal{U} \mbox{ and } h(s)=i\}$ for $i=1,2,...,n$. Then defining $A_i\triangleq A\bigcap\mathcal{U}_i$ and $B_i\triangleq B\bigcap\mathcal{U}_i$ for $i=1,2,...,n$ induces the partitioning of $A$, $B$, and $A\triangle B$.
%, as mentioned in \autoref{sec:smalld}. 

%{\bf (merged from the later two paragraphs)} 
How the $d$ distinct elements (balls) in $A\triangle B$ are ``scattered" into the $n$ subset-pair-differences (bins) $\{A_i\triangle B_i\}_{i=1}^n$ can be precisely modeled as throwing $d$ balls each uniformly and randomly into one of the $n$ bins. 
For the moment, we assume the following {\it ideal case} happens: Every subset-pair-difference $A_i\triangle B_i$ contains at most one distinct element.  
This ideal case corresponds to the $d$ balls ending up in $d$ distinct bins. It happens with probability $\prod_{k=1}^{d - 1}(1 - \frac{k}{n})$, which is on the order of $1-O(d^2/n)$ when $n\!\gg\!d$.
%approximately $e^{-\frac{d(d-1)}{2n}}$ when $d\!\ll\!n$. 
Hence, $n$ must be $\Omega(d^2)$ to ensure the ideal case happens with a nontrivial probability, as mentioned earlier in \autoref{sec:smalld}. 
%The nonideal case of a subset pair difference containing more than $1$ distinct elements will be discussed in \autoref{subsec:exception_hash_partition}.

% {\bf (Previous)} For the moment, we assume the following {\it ideal case} happens: Every subset-pair-difference $A_i\triangle B_i$ contains at most one distinct element. The nonideal case of a subset pair difference containing more than $1$ distinct elements will be discussed in \autoref{subsec:exception_hash_partition}. 

%In this section, we give a detailed description on how to partition $A$ and $B$ (as introduced in \autoref{sec:smalld}) by introducing {\it sub-universes}, which is defined as follows: Given a hash function $h(\cdot): \mathcal{U}\rightarrow \{1,2,\cdots,n\}$, we define {\it sub-universes} $\{\mathcal{U}_i\}_{i=1}^n$, a partition of the universe $\mathcal{U}$, as $\mathcal{U}_i=\{s\!\mid\! s\in \mathcal{U} \mbox{ and } h(s)=i\}$ for $i=1,2,...,n$. Based on $\{\mathcal{U}_i\}_{i=1}^n$, we define $\{A_i\}_{i=1}^n$, the partition of $A$ introduced in \autoref{sec:smalld}, as $A_i\! \triangleq\! A\bigcap \mathcal{U}_i$ for $i=1,2,...,n$. $\{B_i\}_{i=1}^n$ is similarly defined. By this definition, the set difference $A\triangle B$ is partitioned into $n$ set differences of the partitioned subset pairs (i.e., $\{(A_i, B_i)\}_{i=1}^n$). From \autoref{sec:hash_partition} to \autoref{sec:reconcile_by_trivial}, we assume the following {\bf ideal case} happens: Each subset pair $(A_i, B_i)$ contains at most one distinct element ({\it i.e.,} $|A_i\triangle B_i|\!\leq\!1$). The nonideal case of a subset pair contains more than $1$ distinct elements will be discussed in \autoref{subsec:exception_hash_partition}. 

% Here we describe the hash-partition step introduced in \autoref{sec:smalld} in details. First, we use a hash function $h(\cdot): \mathcal{U}\rightarrow \{1,2,\cdots,n\}$ to partition the universe $\mathcal{U}$ into $n$ sub-universes: $\mathcal{U}_i=\{s\!\mid\! s\in \mathcal{U} \mbox{ and } h(s)=i\}$ for $\forall i=1,2,\cdots,n$. The hash function $h(\cdot)$ can be predetermined between Alice and Bob and does not require additional communication cost. Define $A_i\! \triangleq\! A\bigcap \mathcal{U}_i$ and $B_i\! \triangleq\! B\bigcap \mathcal{U}_i$ for $i=1,2,\cdots,n$. Then $\{A_i\}_{i=1}^n$ and $\{B_i\}_{i=1}^n$ are partitions of $A$ and $B$ respectively. Furthermore, $\{A_i\triangle B_i\}_{i=1}^n$ is a partition of $A\triangle B$. From \autoref{sec:hash_partition} to \autoref{sec:reconcile_by_trivial}, we assume the following {\bf ideal case} happens: Each subset pair $(A_i, B_i)$ contains at most one distinct element ({\it i.e.,} $|A_i\triangle B_i|\!\leq\!1$). The nonideal case of a subset pair contains more than $1$ distinct elements will be discussed in \autoref{subsec:exception_hash_partition}. 

% {\bf (Previous)} How the $d$ distinct elements (balls) in $A\triangle B$ are distributed into the $n$ subset pair differences $\{A_i\triangle B_i\}_{i=1}^n$ (bins) 
% can be viewed as throwing $d$ balls each uniformly and randomly into one of the $n$ bins. 

%follows the familiar {\it balls-into-bins} probability model. 
%The distinct elements are viewed as balls and the subset pairs are viewed as bins. 
%Each of the $d$ balls is uniformly and randomly thrown by the hash function $h(\cdot)$ into one of the $n$ bins. 
% The aforementioned ideal case that corresponds to the $d$ balls ending up in $d$ distinct bins happens with probability $\prod_{k=1}^{d - 1}(1 - \frac{k}{n})$, which is on the order of $1-O(d^2/n)$ when $d\!\ll\!n$.
% %approximately $e^{-\frac{d(d-1)}{2n}}$ when $d\!\ll\!n$. 
% Hence, $n$ must be $\Omega(d^2)$ to ensure the ideal case happens with a nontrivial probability, as mentioned in \autoref{sec:smalld}.


%in which the distinct elements are viewed as balls and the subset pairs are viewed as bins. The hash-parition basically throws (hashes) $d$ balls (distinct elements) uniformly and randomly into $n$ bins (subset pairs). The aforementioned ideal case in this context becomes, after throwing $d$ balls uniformly and randomly into $n$ bins, each bin receives at most $1$ ball (i.e., $d$ nonempty bins have $1$ ball in each and the rest $n-d$ bins are empty). The number of balls in each bin is a Binomial random variable $Binomial(d,1/n)$.
%{\bf It may remind readers about the Birthday problem. And the ideal case can be analogous to the case that no people share the same birthday.} 
% The ideal case happens with a probability of $p\!=\!\prod_{k=1}^{d - 1}(1 - \frac{k}{n})\!\approx\! e^{-\frac{d(d-1)}{2n}}$ when $d\!\ll\!n$. In other words, $n$ must be at least $O(d^2)$ to ensure the ideal case happens with a nontrivial probability, as described in \autoref{sec:smalld}.  

% Note that the ideal case does not always happen. However, we can ensure that the ideal case happens with high probability by properly setting $n$ based on $d$ (i.e., $n=\Omega(d^2)$). Furthermore, as we will describe in \autoref{subsec:nonideal}, even if the ideal case does not happen (i.e., some distinct elements are hashed into the same subset pair), most of the distinct elements should be distributed into different subset pairs and therefore can be reconciled. So the scheme, even cannot reconcile all of the distinct elements, can still reconcile the majority of them (i.e., piecewise decodability in \autoref{sec:intro_oursolution}). Based on this property, we will extend our scheme from single-round to multi-rounds in \autoref{subsec:nonideal} to further increase the probability of reconciling all distinct elements. 

% \medskip
% \noindent{\bf Parity Bitmap Encoding} 

% to let Alice obtain $A\triangle B$.

% {\bf (Modified)} Recall that the partition $\{A_i\}_{i=1}^n$ and $\{B_i\}_{i=1}^n$ can be encoded as $A[1..n]$ and $B[1..n]$ respectively, in which $A[i]$, the $i$-th bit of the parity bitmap $A[1..n]$, is equal to the oddness / evenness (parity) of the cardinality of $A_i$ (i.e., $A[i]=1$ if $|A_i|$ is odd; otherwise $A[i]=0$). $B[i]$, the $i$-th bit of the parity bitmap $B[1..n]$, is similarly defined. In the ideal case, $A[1..n]$ and $B[1..n]$ differ in exactly $d$ distinct bit positions $i_1,i_2,...,i_d$, and each subset-pair-difference $(A_{i_1},B_{i_1}), (A_{i_2},B_{i_2}),...,(A_{i_d},B_{i_d})$ contains exactly $1$ distinct element. If Bob knows $i_1,i_2,...,i_d$, he can start to reconcile the $d$ subset pairs respectively using \autoref{alg:trivial_case}, then Alice will obtain $A\triangle B$.

% {\bf (Modified)} The partition $\{A_i\}_{i=1}^n$ is encoded into an $n$-bit-long parity bitmap $A[1..n]$, in which $A[i]$, the $i$-th bit of the parity bitmap, is equal to the oddness / evenness (parity) of the cardinality of $A_i$ (i.e., $A[i]=1$ if $|A_i|$ is odd; otherwise $A[i]=0$). $B[1..n]$, the parity bitmap of $\{B_i\}_{i=1}^n$, is similarly defined. In the ideal case, $A[1..n]$ and $B[1..n]$ differ in exactly $d$ distinct bit positions $i_1,i_2,...,i_d$, and each subset-pair-difference $(A_{i_1},B_{i_1}), (A_{i_2},B_{i_2}),...,(A_{i_d},B_{i_d})$ contains exactly $1$ distinct element. If Bob knows $i_1,i_2,...,i_d$, he can start to reconcile the $d$ subset pairs respectively using \autoref{alg:trivial_case}, then Alice will obtain $A\triangle B$.

% {\bf (Previous)} We encode $\{A_i\}_{i=1}^n$ into an $n$-bit-long parity bitmap $A[1..n]$, in which $A[i]$, the $i^{th}$ bit of the parity bitmap, is equal to the oddness / evenness (parity) of the cardinality of $A_i$ (i.e., $A[i]=1$ if $|A_i|$ is odd; otherwise $A[i]=0$). In the ideal case, the two bitmaps $A[1..n]$, $B[1..n]$ differ in exactly $d$ bit positions $i_1,i_2,...,i_d$, each of which corresponds to a subset pair that contains $1$ distinct element. The next step is to let Alice and Bob know these bit positions.

%Once the $d$ bit positions are known, Alice and Bob can start to reconcile $(A_{i_1},B_{i_1}), (A_{i_2},B_{i_2}),...,(A_{i_d},B_{i_d})$ using \autoref{alg:trivial_case} and obtain the $d$ distinct elements (i.e., $A\triangle B$). 

% \subsubsection{Parity Bitmap Encoding}\label{sec:parity_bitmap_encoding}

% %After hash-partitioning $A$ and $B$ into partitions $\{A_i\}_{i=1}^n$ and $\{B_i\}_{i=1}^n$, 
% As introduced in \autoref{sec:smalld}, we encode each partition into an $n$-bit-long parity bitmap and denote them as $A[1..n]$ and $B[1..n]$ respectively, as introduced in \autoref{sec:smalld}. For $i=1,2,...,n$, $A[i]$ (the $i^{th}$ bit of the parity bitmap $A[i]$) is equal to $1$ if $A_i$ contains an odd number of elements, and is equal to $0$ otherwise.
% % More specifically, for $i=1,2,...,n$, $A[i]$ (the $i^{th}$ bit of the parity bitmap $A[i]$) is defined as follows: $A[i]=1$ if $A_i$ contains an odd number of elements, and $A[i]=0$ otherwise. In this way, each bit $A[i]$ encodes the oddness / evenness (parity) of the cardinality of $A_i$. The $n$-bit-long parity bitmap $B[1..n]$ and $B[i]$ (the $i^{th}$ bit of $B[1..n]$) are similarly defined. 
% In the ideal case, 
% %$A[i]$ and $B[i]$ differ if and only if $A_i$ and $B_i$ have exactly $1$ distinct element, and $A[i]$ and $B[i]$ are the same if and only if $A_i=B_i$. Meanwhile, the $d$ distinct elements are hashed into $d$ different subset pairs. So 
% the two bitmaps $A[1..n]$, $B[1..n]$ differ in exactly $d$ bit positions, each of which corresponds to a subset pair that contains $1$ distinct element. Once the $d$ bit positions are known, Alice starts to reconcile each of the $d$ corresponding subset pairs by \autoref{alg:trivial_case} and gets the $d$ distinct elements (i.e., $A\triangle B$). 
% %If knowing the $d$ bit positions (i.e., the $d$ corresponding subset pairs), we can use \autoref{alg:trivial_case} to reconcile the $d$ subset pairs respectively to obtain all the $d$ distinct elements (i.e., $A\triangle B$). 
% In \autoref{sec:BCH_code}, we will describe how to find the $d$ bit positions using BCH code~\cite{Lint_IntroductionCodingTheory_1998}. 

% \medskip
% \noindent{\bf Find the $d$ Bit Positions Using ECC} 

%\subsubsection{Find the $d$ Bit Positions Using ECC}\label{sec:BCH_code}
\subsubsection{Find and reconcile the \texorpdfstring{$d$}{d} subset pairs}\label{sec:BCH_code}


\begin{algorithm}
\caption{PBS-for-small-$d$ (first round)}
\label{alg:single_round_pbs}

%Hash-partition $A$, $B$ into $\{A_i\}_{i=1}^n$, $\{B_i\}_{i=1}^n$\; \label{step:hash_partition}

%Parity encode $\{A_i\}_{i=1}^n$, $\{B_i\}_{i=1}^n$ into $A[1..n]$, $B[1..n]$\; \label{step:parity_encode}
{\it Alice}: Send $\xi_A$, the BCH codeword of $A[1..n]$, to Bob\; \label{step:BCH_encode}

{\it Bob}: Decode $(B[1..n], \xi_A)$ to obtain $i_1, i_2, ..., i_d$\; \label{step:BCH_decode}

{\it Bob}: Send \code{XOR} sums of sets $B_{i_1}, B_{i_2},...,B_{i_d}$ (\autoref{alg1:sender} in \autoref{alg:trivial_case}), indices $i_1, i_2, ..., i_d$,
and checksum $c(B)$ to Alice\; \label{step:send_xor}

{\it Alice}: Obtain $A_{i_1}\triangle B_{i_1}, A_{i_2}\triangle B_{i_2},...,$ and $A_{i_d}\triangle B_{i_d}$ (\autoref{alg1:receiver} in \autoref{alg:trivial_case}); $\hat{D}\leftarrow \bigcup_{k=1}^d (A_{i_k}\triangle B_{i_k})$\; \label{step:trivial_reconcile}

{\it Alice}: Check whether $c(A\triangle\hat{D})\stackrel{?}{=}c(B)$\; \label{step:terminate_condition}

\end{algorithm}

The remaining steps of the PBS scheme are summarized in \autoref{alg:single_round_pbs}.
Recall that the partitions $\{A_i\}_{i=1}^n$ and $\{B_i\}_{i=1}^n$ can be encoded as parity bitmaps $A[1..n]$ and $B[1..n]$ respectively, in which each $A[i]$ or $B[i]$
%, the $i$-th bit of the parity bitmap $A[1..n]$ or $B[1..n]$, 
corresponds to the parity (oddness or evenness) of the cardinality of the subset $A_i$ or $B_i$.  In the ideal case, $A[1..n]$ and $B[1..n]$ differ in exactly $d$ distinct bit positions. 
Suppose these $d$ bit positions are $i_1, i_2, ..., i_d$.  Then subset pairs $(A_{i_1}, B_{i_1}), (A_{i_2}, B_{i_2}),...,(A_{i_d}, B_{i_d})$ each differs by exactly $1$ (distinct) element
and hence can be reconciled using \autoref{alg:trivial_case}.
For this to happen, however, Bob needs to first know the values of $i_1, i_2, ..., i_d$.
% he can initiate the process of reconciling these $d$ subset pairs each using \autoref{alg:trivial_case}.
As mentioned earlier in \autoref{sec:smalld}, to this end, Alice only needs to send a BCH encoding of $A[1..n]$, denoted as $\xi_A$, that can pinpoint (to Bob) these $d$ bit locations in Bob's local bitmap $B[1..n]$ (\autoref{step:BCH_encode} in \autoref{alg:single_round_pbs}).  {\bf We will provide some details of this BCH encoding and decoding
in Section ???[the last subsection of Section 2].}
%Then Bob can decode and recover $A[1..n]$ (original message) and obtain $i_1,i_2,...,i_d$.

%{\bf (Previous)} In the ideal case, for Bob to obtain $i_1,i_2,...,i_d$, Alice only needs to send $\xi_A$, the BCH code of $A[1..n]$, that can ``correct'' these $d$ bit errors in $B[1..n]$. Then Bob can decode and recover $A[1..n]$ (original message) and obtain $i_1,i_2,...,i_d$.

% {\bf (Previous)} We view $A[1..n]$ as a corrupted message of $B[1..n]$ sent ({\bf not actually being sent}) from Bob to Alice through an {\it unreliable} commnunication channel that flips $d$ bits. To locate these $d$ bit positions, we let Bob also send an {\it error-correction code} that encodes $B[1..n]$ to Alice, such that Alice can recover $B[1..n]$ (original message) and obtain the $d$ bit positions $i_1,i_2,...,i_d$. In PBS, we use BCH code~\cite{bch1} to encode $B[1..n]$ and get the error-correction code.


%To correct $d$ bit errors, the length of the net-codeword only is no more than $d\log n$ bits. 
% Without causing any ambiguity, we use the term `codeword' to refer to the net-codeword in the rest of this paper.
%The computational complexity of the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} is $O(d^2\log^2 n)$.

% There are two different BCH encoding techniques: {\it systematic} and {\it unsystematic}. The difference is that, the message appears as the prefix of the codeword (i.e., codeword = [message net-codeword]) in systematic BCH encoding, whereas it does not appear as a substring of the codeword in unsystematic BCH encoding. In PBS, we choose systematic BCH encoding because we are sending not the ``message'', but the net-codeword. 
% %To correct $d$ bit errors, the length of the net-codeword only is no more than $d\log n$ bits. 
% Without causing any ambiguity, we use the term `codeword' to refer to the net-codeword in the rest of this paper.
% %The computational complexity of the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} is $O(d^2\log^2 n)$.

%The systematic BCH encoding is also used in other ECC-based set reconciliation works, such as PinSketch \cite{Wuille_Minisketchoptimizedlibrary_2019}, while PinSketch encodes a much longer message (e.g., $2^{32}$ bits) than in ours (hundreds of bits).  

%\subsubsection{Find the $d$ Bit Positions Using ECC}\label{sec:BCH_code}

% A straightforward approach to find the $d$ bit positions is to let Bob send the complete parity bitmap $B[1..n]$ to Alice, then Alice compares $A[1..n]$ with $B[1..n]$ locally. This approach has a communication overhead of $n$ bits, which is quite wasteful. As we discussed in~\autoref{sec:hash_partition}, $d$ is usually much smaller than $n$. It means $A[1..n]$ and $B[1..n]$ differ only at a tiny portion of bits. Therefore, we can view $A[1..n]$ as a corrupted message of $B[1..n]$ with $d$ bit errors, and the bit positions of the $d$ bit errors basically correspond to the $d$ subset pairs that contain distinct elements. The detection of bit errors, on the other hand, can be solved by Error-Correction Code (ECC)~\cite{Lin_ErrorControlCoding_1983}. 

% Since $A[1..n]$ and $B[1..n]$ differ at $d$ bit positions, we can view $A[1..n]$ as a corrupted message of $B[1..n]$ from Bob to Alice through an {\it unreliable} commnunication channel with $d$ corrupted bits, which are located on the $d$ bit positions. Therefore, to find the $d$ bit position, we only need to correct the $d$ corrupted bits in $A[1..n]$, which is done by transmitting a ``code'' that can correct upto $d$ bit errors from Bob to Alice through a {\it reliable} communication channel. 

% In PBS, we use {\it systematic} BCH code to generate the ``code'' by encoding the message $B[1..n]$. The codeword of the systematic BCH code is in the form of [message, net-codeword], since the message appears as the prefix of the codeword in systematic BCH code. The ``code'' is simply the net-codeword in the BCH codeword. We choose {\it systematic} BCH code because the (corrupted) message is already transmitted and we only need to pay a small communication overhead on transmitting ``code'' (i.e., net-codeword). To correct upto $d$ bit errors, the length of the net-codeword is no more than $d\log n$ bits, which is much smaller than the message when $d\!\ll\! n$. The computational complexity of the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} is $O(d^2\log^2 n)$. This type of BCH code is also used in other ECC-based set reconciliation works, such as PinSketch \cite{Wuille_Minisketchoptimizedlibrary_2019}. 

% Different from {\it unsystematic} BCH code
% The ``code'' is generated by {\it systematic} BCH code, which encodes the message $B[1..n]$ into a BCH codeword in the form of [message, net-codeword]. The ``code'' transmitted on the reliable channel is the net-codeword of the BCH codeword. In {\it systematic} BCH code, the message appears as the prefix of the codeword. 

% More specifically, PBS uses {\it systematic} BCH code~\cite{Lint_IntroductionCodingTheory_1998} that can correct upto $d$ bit errors to encode the parity bitmaps. In the {\it systematic} BCH code \footnote{In unsystematic BCH code, message does not appear to be the prefix of the codeword}, the message (i.e., the parity bitmap) appears as the prefix of the raw codeword, which in the form of [message, net codeword]. Normally, to correct upto $d$ errors, the length of the net codeword is $2n\log d$, where $n$ is the length of the message (i.e., parity bitmap). However, our case is special in the sense that the net codeword is error-free (all $d$ bit errors are in the message), so the length of the net codeword can be reduced to $n\log d$. This type of BCH code is also used in other ECC-based set reconciliation works, such as PinSketch \cite{Wuille_Minisketchoptimizedlibrary_2019}. 

% Now we can formally describe how to find the $d$ bit positions: First, Bob uses a $d$-error-correcting systematic BCH code to encode $B[1..n]$ and sends the net codeword ($d\log n$ bits) to Alice. Upon receiving the net codeword and combining it with the corrupted message $A[1..n]$, Alice uses the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} to decode the $d$ bit errors in $A[1..n]$. The communication overhead of transmitting the net codeword is $d\log n$ bits. The computational complexity of the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} is $O(d^2\log^2 n)$. Both the communication overhead and the computational complexity here are relatively small when $d$ is small.

% \medskip
% \noindent{\bf Reconcile the $d$ subset pairs using \autoref{alg:trivial_case}} 

%Once the $d$ bit positions are known, Alice can start to reconcile $(A_{i_1},B_{i_1}), (A_{i_2},B_{i_2}),...,(A_{i_d},B_{i_d})$ using \autoref{alg:trivial_case} and obtain the $d$ distinct elements (i.e., $A\triangle B$). 
Once Bob decodes $\xi_A$ (\autoref{step:BCH_decode} in \autoref{alg:single_round_pbs}) to obtain $i_1,i_2,...,i_d$, 
%the corresponding subset pairs $(A_{i_1},B_{i_1})$, $(A_{i_2},B_{i_2})$, $...$, 
%$(A_{i_d},B_{i_d})$ each can be reconciled using \autoref{alg:trivial_case}.  To do so, 
Bob sends the \code{XOR} sums of the corresponding 
subsets $B_{i_1}$, $B_{i_2}$,$...$,$B_{i_d}$ to Alice (\autoref{alg1:sender} in \autoref{alg:trivial_case}).  Bob also needs to send the decoded ``bit error positions'' $i_1, i_2, ..., i_d$ to Alice (\autoref{step:send_xor} in \autoref{alg:single_round_pbs}), {\color{red} since Alice cannot obtain this information (in the same way as Bob did in \autoref{step:BCH_decode} of \autoref{alg:single_round_pbs}) by herself without knowing $B[1..n]$.} 
% {\color{red} since Alice cannot decode $\xi_A$ herself without knowing $B[1..n]$.}
In addition, for Alice to verify whether the set reconciliation is successfully completed (to be described next), Bob sends $c(B)$, a checksum of its set $B$, to Alice.  
%Alice, without knowing $B[1..n]$ otherwise would not know the ``bit error positions'' . 
%As each ``bit error position'' can be encoded into $\log n$ bits, the resulting additional communication overhead is $d\log n$ bits. 
% When reconciling $(A_{i_1},B_{i_1}), (A_{i_2},B_{i_2}),...,(A_{i_d},B_{i_d})$ using \autoref{alg:trivial_case}, Alice needs to send not only the bitwise \code{XOR} of $A_{i_1}, A_{i_2},..., A_{i_d}$, but also the indices of the subset pairs ($i_1,i_2,...,i_d$), since Bob does not know which of the $d$ subset pairs are being reconciled. Each index is an integer between $1$ and $n$ and can be encoded into $\log n$ bits, So the additional communication overhead on transmitting the indices is $d\log n$ bits. 

% \subsubsection{Reconcile the $d$ subset pairs using \autoref{alg:trivial_case}}\label{sec:reconcile_by_trivial}

% After decoding the $d$ bit errors that corresponds to the $d$ subset pairs, Alice starts to reconcile them using \autoref{alg:trivial_case}. For each of the $d$ subset pairs, Alice needs to send not only the bitwise \code{XOR} of the subset pair, but also the index of the subset pair (since Bob does not know the $d$ subset pairs to reconcile). So the communication overhead on \autoref{alg:trivial_case} is $d\log |\mathcal{U}|+d\log n$ bits. 
%Plus the communication overhead on transmitting the net codeword of parity bitmap ($d\log n$, as we explained in \autoref{sec:BCH_code}), the overall communication overhead of single-round PBS is $d\log u+2d\log n$ bits.

% \medskip
% \noindent{\bf Check if set reconciliation is complete} 

%{\bf We need a subsubsection on verification}\
\subsubsection{Verify the estimated set difference}\label{sec:checksum_verification}

Once Alice receives the ``bit error positions" and the corresponding \code{XOR} sums, 
she can recover the distinct elements each using \autoref{alg:trivial_case} to arrive at the estimated set difference
(\autoref{step:trivial_reconcile} in \autoref{alg:single_round_pbs}), which we denote as 
$\hat{D}$.   Alice needs to verify whether $\hat{D}\stackrel{?}{=}A\triangle B$ because only in the ideal case is this estimated set difference $\hat{D}$ the same as the
actual set difference $A\triangle B$, as we will explain in the next section.   Alice does so by checking an equivalent condition $A\triangle\hat{D}\stackrel{?}{=}B$ 
as follows.  She applies a
checksum function $c(\cdot)$ to $A\triangle\hat{D}$ and comparing (\autoref{step:terminate_condition} in \autoref{alg:single_round_pbs}) 
the resulting checksum $c(A\triangle\hat{D})$ with $c(B)$ that Alice received earlier from Bob. 
While any checksum function $c(\cdot)$ can be used here, we use {\it longitudinal parity check} function, with which the checksum of a set $S$ is the bitwise-\code{XOR} 
of all elements in $S$.   The length of such a checksum is $(\log |\mathcal{U}|)$ bits, the same as that of an element.   


%While $c(\cdot)$ can be any checksum function, for performance considerations, a linear checksum function is preferred here.  
%We call $c(\cdot)$ linear if $c(S_1\triangle S_2)=c(S_1)\oplus c(S_2)$ for any two sets $S_1$ and $S_2$.
%With a linear $c(\cdot)$, the total time complexity of computing 
%both $c(A\triangle\hat{D})$ and $c(B)$ is only $O(d)$, because when a large set (say $B$) changes slightly (from one time to another),  

\begin{comment}
because it allows for incremental updates, 
This checking can be achieved using a checksum function $c(\cdot)$ that maps any subset of the universe $\mathcal{U}$ to a checksum by checking whether $c(\hat{D})\stackrel{?}{=}c(A\triangle B)$. With incremental updates, $c(\hat{D})$ can be computed in $O(d)$ time. However, computing $c(A\triangle B)$ is tricky, since $A$ and $B$ are {\it remote} sets and stored at hosts Alice and Bob respectively. 

To ease the computation of $c(A\triangle B)$, we choose a ``linear'' checksum function, so that $c(A\triangle B)=c(A)\oplus c(B)$ can be precomputed. Here we call a checksum function ``linear'' if $c(S_1\triangle S_2)=c(S_1)\oplus c(S_2)$ for any two subsets $S_1$ and $S_2$ of the universe $\mathcal{U}$. More specifically, to obtain $c(A\triangle B)$, Bob precomputes $c(B)$ and sends it to Alice. Alice also precomputes $c(A)$, and upon receiving $c(B)$, Alice can compute $c(A\triangle B)=c(A)\oplus c(B)$. In PBS, we select {\it longitudinal parity check}, the bitwise \code{XOR} of all elements (recall each element is a $(\log |\mathcal{U}|)$-bit-long binary string) in the set, as the ``linear'' checksum function. The precomputation of $c(A\triangle B)$ incurs additional communication overhead on transmitting $c(B)$ that is $\log |\mathcal{U}|$ bits.

{\bf (previous)} This can be achieved using a ``linear'' checksum function $c(\cdot)$ that maps any subset of the universe $\mathcal{U}$ to a $32$-bit checksum by checking whether $c(\hat{D})\stackrel{?}{=}c(A\triangle B)$. Here we call a checksum function ``linear'' if $c(S_1\triangle S_2)=c(S_1)\oplus c(S_2)$ for any two subsets $S_1$ and $S_2$ of the universe $\mathcal{U}$. We choose a checksum function that is ``linear'', so that $c(A\triangle B)=c(A)\oplus c(B)$ can be precomputed. This precomputation incurs $32$ bits of communication overhead on transmitting $c(B)$ from Bob to Alice. With incremental updates, $c(\hat{D})$ can be computed in $O(d)$ time. In PBS, we select {\it longitudinal parity check}, the bitwise \code{XOR} of all elements (assuming each element is a $32$-bit-long binary string) in the set, as the ``linear'' checksum function. 
%It is not hard to verify it is linear.  

\end{comment}

%In the nonideal case, however, $\hat{D}$ will deviate from $A\triangle B$. 
%Hence, Alice needs to verify whether $\hat{D}\stackrel{?}{=}A\triangle B$.  This can be accomplished using a checksum function 




% Once Alice receives the \code{XOR} sums and the indices, she can compute the distinct elements, as described in \autoref{subsec:protocol0}, to obtain the set difference (denoted as $\hat{D}$). However, this reconciled set difference could be incorrect if the ideal case does not happen. Therefore, Alice needs to check if set reconciliation is successfully completed (or whether $\hat{D}=A\triangle B$). To do so, we introduce some ``linear'' checksum function $c(\cdot)$ that maps any subset of the universe $\mathcal{U}$ (such as $A$ and $B$) to a $32$-bit checksum (e.g., bitwise \code{XOR}). Here the ``linearity'' of a chechsum function refers to the fact that $c(S_1\triangle S_2)=c(S_1)\oplus c(S_2)$ for any two subsets $S_1$ and $S_2$ of the universe $\mathcal{U}$. We use this checksum function to check if $\hat{D}=A\triangle B$ by comparing $c(\hat{D})$ to $c(A\triangle B)$. Note that $c(\hat{D})$ can be computed in $O(d)$ time and $c(A\triangle B)=c(A)\oplus c(B)$ can be precomputed {\bf during the encoding period, which costs $32$ bits of communication overhead on transmitting $c(B)$ from Bob to Alice. In PBS, we select {\it longitudinal parity check}, the bitwise \code{XOR} of all elements (recall each element is a $32$-bit-long binary string) in the set, as the checksum function. It is not hard to verify it is linear.}  

% {\bf (Previous)} After reconciling the subset pairs and obtaining the reconciled set difference (denoted as $\hat{D}$), PBS needs to check if set reconciliation is complete (or whether $\hat{D}=A\triangle B$), since the reconciled set difference $\hat{D}$ is not the actual set difference $A\triangle B$ in the nonideal case (to be discussed in \autoref{subsec:exception_hash_partition}). Hence, we add a verfication step after obtaining $\hat{D}$ to check if $\hat{D}=A\triangle B$. In PBS, we check an equivalent condition, $A=B\triangle\hat{D}$, instead of $\hat{D}=A\triangle B$, since $B$ and $\hat{D}$ are both known by Bob and their set difference $B\triangle\hat{D}$ can be locally computed. More specifically, to check if the remote sets $A$ and $B\triangle\hat{D}$ are equal, we let Alice compute a $32$-bit checksum of $A$ and send it to Bob. {\bf Then Bob computes the $32$-bit checksum of $B\triangle\hat{D}$ using the same checksum algorithm and compare the two checksums. In PBS, we select {\it longitudinal parity check} (i.e., bitwise \code{XOR} of all elements in the set) as the checksum algorithm, so that the checksum $B\triangle\hat{D}$ can be efficiently computed as the bitwise \code{XOR} between the checksum of $B$ (can be pre-computed) and that of $\hat{D}$. Other checksum algorithms that are {\it linear} to the set difference operator (i.e., $\triangle$) also work for PBS. }
% Then Bob checks if $B\triangle\hat{D}$ satisfies the receiving checksum. 

Using a 32-bit-long checksum (assuming $\log |\mathcal{U}| = 32$), the probability for Alice to mistakenly believe $A\triangle\hat{D}\!=\!B$ when the opposite 
(i.e., $\{A\triangle\hat{D}\!\neq\! B\}$) is true 
%the condition {\bf ????} can be correctly verified with an overwhelming probability of 
is only $O(10^{-12})$ for the following reason. 
The event $\{A\triangle\hat{D}\! \neq\! B\}$ can happen only in the nonideal case, which happens with a probability of $O(10^{-2})$ (as we will show in \autoref{subsec:exception_hash_partition}).
Then, conditioned upon the event $\{A\triangle\hat{D}\! \neq\! B\}$ happening, 
the probability for their 32-bit-long checksums happen to be equal (i.e., $c(A\triangle\hat{D})\! =\! c(B)$) is only $2^{-32}\!\approx\! 2.3\!\times\! 10^{-10}$.
%a 32-bit-long checksum to fail to detect $\hat{D}\neq A\triangle B$ .
This $O(10^{-12})$ probability of incorrect verification should be acceptable in most applications.  
% In applications that allow no incorrect verification ({\it e.g.,} Bitcoin), additional
% verification techniques such as a Merkle tree~\cite{merkle87} can be used in conjunction.  
{\color{red}In applications that allow no incorrect verification ({\it e.g.,} blockchain), 
they usually has some built-in technique to guarantee the correctness of the verification. 
For example, blockchain platforms Ethereum~\cite{Wood_Ethereumsecuredecentralised_2014} 
and Bitcoin~\cite{Nakamoto_Bitcoinpeerpeer_2019} both have built-in component to verify the 
integrity and consistency of transactions based the Merkle tree~\cite{merkle87}. 
A Merkle tree is a binary tree. In Ethereum and Bitcoin, each leaf node of the Merkle tree 
is a cryptographic hash value of a transaction, and 
each non-leaf node is the hash of its two children, and its 
root validates the consistency of all transactions. Therefore, in such applications, we can rely on 
the built-in technique to do the verification with no cost. 
Even if the application itself does not have built-in verification component, there are many techniques we can 
use to achieve correct verification. 
For example, we can apply an one-way multiset hash function, 
{\it e.g.}, MSet-XOR-Hash~\cite{Clarke_IncrementalMultisetHash_2003}, $H$, to 
both $A\triangle\hat{D}$ and $B$ and verify $H(A\triangle\hat{D})\!\stackrel{?}{=}\!H(B)$ 
with an additional computational overhead of $O(\max\{|A|+d,|B|\})$ and constant communication overhead. 
We do not count the overhead of this ``correctness-guaranteed'' verification in the calculation of 
the communication overhead in the sequel, since all schemes described in 
this paper requires it when the application allows no incorrect verification. 
To simplify our presentation, we 
% ignore this $O(10^{-12})$ 
% probability event and 
assume that the $c(A\triangle\hat{D})\!\stackrel{?}{=}\!c(B)$ verification is always correct in the sequel. }

% Using a 32-bit-long checksum (assuming $(\log |\mathcal{U}|) = 32$), the probability for Alice to mistakenly believe {\bf ????} when the opposite is true 
% %the condition {\bf ????} can be correctly verified with an overwhelming probability of 
% is only $O(10^{-12})$ for the following reason. 
% The event {\bf ????} can happen only in the nonideal case, which happens with a probability $O(10^{-2})$ (as we will show in \autoref{subsec:exception_hash_partition}).
% Then, conditioned upon the nonideal case happening, the probability for a 32-bit-long checksum to fail to detect {\bf ????} is only $2^{-32}\approx 2.3\times 10^{-10}$.
% This tiny probability of incorrect verification should be acceptable in most applications.  In applications that allow no incorrect verification ({\it e.g.,} Bitcoin), additional
% verification techniques such as a Merkle tree~\cite{merkle87} can be used in conjunction.  To simplify our presentation, we ignore this $O(10^{-12})$ 
% probability event and assume that the {\bf ???? WITH c on both sides} verification is always correct in the sequel. 

% {\bf although it could mistakenly believes two different sets as identical ones.} This event happens with probability $2^{-32}\approx 2.3\times 10^{-10}$ when the ideal case does not happen, {\bf which has a probability on the order of $10^{-2}$.} Although this event could cause PBS mistakenly believes the set reconciliation is completed, it happens with an extremely small probability (on the order of $10^{-12}$) and should be acceptable in most applications. In few applications which allow no room for error ({\it e.g.,} Bitcoin), additional techniques such as Merkle tree~\cite{merkle87} based validation will be used to verify the correctness of the results anyway. 
% %If such techniques find out that the set reconciliation is not completed, we could simply start it over and use PBS to reconcile the two sets again under a different hash function $h$. In this case, the checksum will be different If so, the  (note that PBS is a `randomized' algorithm when assuming the hash functions for hash-partition are random hash functions). 
% To simplify our description, we ignore this small probability event and assume the checksum always correctly verify $\hat{D}\stackrel{?}{=}A\triangle B$ in the sequal. 

% The condition $\hat{D}=A\triangle B$ can be almost surely verified by the checksum, 
% {\bf although it could mistakenly believes two different sets as identical ones.} This event happens with probability $2^{-32}\approx 2.3\times 10^{-10}$ when the ideal case does not happen, {\bf which has a probability on the order of $10^{-2}$.} Although this event could cause PBS mistakenly believes the set reconciliation is completed, it happens with an extremely small probability (on the order of $10^{-12}$) and should be acceptable in most applications. In few applications which allow no room for error ({\it e.g.,} Bitcoin), additional techniques such as Merkle tree~\cite{merkle87} based validation will be used to verify the correctness of the results anyway. 
% %If such techniques find out that the set reconciliation is not completed, we could simply start it over and use PBS to reconcile the two sets again under a different hash function $h$. In this case, the checksum will be different If so, the  (note that PBS is a `randomized' algorithm when assuming the hash functions for hash-partition are random hash functions). 
% To simplify our description, we ignore this small probability event and assume the checksum works perfectly in this rest of this paper. 

% We summarize all the above steps of PBS (in the first round) in \autoref{alg:single_round_pbs}.
% %{\bf not a good position to mention `for super critical applications, use a checksum for all groups', since we are describing single-group scenario. }

% \begin{algorithm}
% \caption{Single-round PBS}
% \label{alg:single_round_pbs}

% %Hash-partition $A$, $B$ into $\{A_i\}_{i=1}^n$, $\{B_i\}_{i=1}^n$\; \label{step:hash_partition}

% %Parity encode $\{A_i\}_{i=1}^n$, $\{B_i\}_{i=1}^n$ into $A[1..n]$, $B[1..n]$\; \label{step:parity_encode}
% {\it Alice}: Send $\xi_A$, the BCH codeword of $A[1..n]$, to Bob\; \label{step:BCH_encode}

% {\it Bob}: Decode $(B[1..n], \xi_A)$ to obtain $i_1,i_2,...,i_d$\; \label{step:BCH_decode}

% {\it Bob}: Send the \code{XOR} sums of sets $B_{i_1}, B_{i_2},...,B_{i_d}$ (\autoref{alg1:sender} in \autoref{alg:trivial_case}) and $i_1,i_2,...,i_d$ to Alice\; \label{step:BCH_decode}

% {\it Alice}: Obtain $A_{i_1}\triangle B_{i_1}, A_{i_2}\triangle B_{i_2},...,$ and $A_{i_d}\triangle B_{i_d}$ (\autoref{alg1:receiver} in \autoref{alg:trivial_case}); $\hat{D}\leftarrow \bigcup_{k=1}^d (A_{i_k}\triangle B_{i_k})$\; \label{step:trivial_reconcile}

% {\it Alice}: Check if $c(\hat{D})=c(A\triangle B)$\; \label{step:terminate_condition}

% \end{algorithm}
% {\color{blue}This probability is low enough for most applications. In few applications which allow no room for error ({\it e.g.,} Bitcoin), additional techniques such as Merkle tree~\cite{merkle87} based validation will be used to verify the correctness of the results anyway.}

% {\bf (Previous)} The condition $A=B\triangle\hat{D}$ can be almost surely verified by a $32$-bit checksum, although it could mistakenly believe two different sets as identical ones with probability $2^{-32}\approx 2.3\times 10^{-10}$ {\bf on top of the probability that the nonideal case happens (on the order of $10^{-2}$).} Although this event could cause an ``early'' termination and leave some distinct elements unreconciled, it happens with an extremely small probability (on the order of $10^{-12}$) and should be acceptable in most applications. {\bf To simplify our description, we ignore this small probability event and assume the checksum works perfectly in this rest of this paper. }
%and such an event (i.e., mistaken $A$ and $B\triangle\hat{D}$ are identical when they are different) never happens in our evaluation. For some super critical applications, we can certainly use a $64$-bit checksum to reduce this probability to $5.4\times 10^{-20}$ if needed.

% When the ideal case does not happen, set reconciliation cannot accomplish in one round, as we will explain in \autoref{subsec:exception_hash_partition}. Hence, we add a verfication step to check if set reconciliation is complete. Let $\hat{D}$ denote the set of reconciled elements. The idea of this verification is basically to compare $A$ with $B\triangle \hat{D}$: If $A=B\triangle \hat{D}$ (i.e., $\hat{D}=A\triangle B$), we know the set reconciliation is complete; Otherwise, the set reconciliation is incomplete.  using a $32$-bit checksum. 

% \subsubsection{Communication overhead of PBS (First Round)}\label{sec:communication_overhead_single_PBS}

% %To correct $d$ bit errors, the length of the net-codeword only is no more than $d\log n$ bits. 

% The communication overhead of \autoref{alg:single_round_pbs} consists of four components: (1) the BCH codeword $\xi_A$ in \autoref{step:BCH_encode}; (2) the subset pair indices $i_1,i_2,...,i_d$ in \autoref{step:trivial_reconcile}; (3) the bitwise \code{XOR} sums of sets $B_{i_1}, B_{i_2},...,B_{i_d}$ of $d\log |\mathcal{U}|$ bits in \autoref{step:trivial_reconcile}; and (4) transmit the $32$-bit checksum of $B$ (i.e., $c(B)$) from Bob to Alice for precomputing $c(A\triangle B)$ in \autoref{step:terminate_condition}. These four components contribute roughly (1) $d\log n$ bits (recall that to ``correct'' $d$ bit errors, the length of the BCH codeword is no more than $d\log n$ bits); (2) $d\log n$ bits; (3) $d\log |\mathcal{U}|$ bits; and (4) $32$ bits respectively to the overall communcation overhead of \autoref{alg:single_round_pbs}. 

% All the steps of PBS in the first round are summarized in \autoref{alg:single_round_pbs}. The overall communication overhead consists of three components: (1) the BCH codeword of $d\log n$ bits in \autoref{step:BCH_encode}; (2) the subset pair indices $i_1,i_2,...,i_d$ and the corresponding bitwise \code{XOR}s of $d\log n+d\log |\mathcal{U}|$ bits in \autoref{step:trivial_reconcile}; and (3) the $32$-bit checksum of $A$ in \autoref{step:terminate_condition}. 


% {\it Bob}: BCH-Encodeing $B[1..n]$ and send the codeword to Alice\; \label{step:BCH_encode}

% {\it Alice}: Upon receiving the codeword, decode the bit errors between $A[1..n]$ and $B[1..n]$\; \label{step:BCH_decode}

% {\it Alice}: For each bit error, start reconciling the corresponding subset pair by \autoref{alg:trivial_case}\; \label{step:trivial_reconcile}

% {\it Bob}: Upon receiving the reconciled set difference $\hat{D}$, check if $A=B\triangle \hat{D}$ via checksum\; \label{step:terminate_condition}


% \subsubsection{Single-round PBS}\label{sec:single_round_pbs}

% Here we summarize all the steps of single-round PBS and represent it by pseudocode in \autoref{alg:single_round_pbs}. \autoref{step:hash_partition} and \autoref{step:parity_encode} operates at both hosts (i.e., Alice and Bob). \autoref{step:hash_partition} to \autoref{step:trivial_reconcile} have been elaborated from \autoref{sec:hash_partition} to \autoref{sec:reconcile_by_trivial}. The last step in \autoref{step:terminate_condition} aims to check whether reconciliation is complete (i.e., $\mathcal{D}=A\triangle B$). More specifically, Alice calculates the checksum (e.g., CRC-$32$) of $A$ and send it to Bob. Then Bob calculates the checksum of $B\triangle \mathcal{D}$ and compares it to the receiving checksum of $A$. If the two checksums are the same, we believe $A=B\triangle \mathcal{D}$ and therefore $\mathcal{D}=A\triangle B$ (i.e., reconciliation is complete); Else, we know some elements are reconciled incorrectly. We classify those elements (i.e., the ones in the set difference between $A\triangle B$ and $\mathcal{D}$) into two subsets $A\triangle B\!\setminus\!\mathcal{D}$ and $\mathcal{D}\!\setminus\!(A\triangle B)$ and refer the elements in the former as {\it false-negatives}, and refer the elements in the later as {\it false-positives}. 

% In the ideal case, neither false-positives nor false-negatives will happen and the two checksums always equal. However, in real life, the ideal case does not always happen. We will discuss the nonideal case in \autoref{subsec:exception_hash_partition}. In our evaluation, we use a $32$-bit checksum for comparing $A$ to $B\triangle \mathcal{D}$ that has {\bf an error probability} roughly $10^{-9}$. This error (i.e., mistake $A=B\triangle \mathcal{D}$) incurs false-negatives. All set reconciliation schemes have the same problem on their termination conditions (i.e., check whether $\mathcal{D}=A\triangle B$). For some super critical applications, we can certainly decrease the error probability by using more powerful checksums (i.e., $64-$bit). Using a $32$-bit checksum, this kind of false-negatives never happen in the evaluation. 
% %For simplification, we assume no error happens when checking $\mathcal{D}=A\triangle B$ in the rest of the paper.

% \begin{algorithm}
% \caption{Single-round PBS}
% \label{alg:single_round_pbs}

% Hash-partition $A$, $B$ into $\{A_i\}_{i=1}^n$, $\{B_i\}_{i=1}^n$\; \label{step:hash_partition}

% Parity encode $\{A_i\}_{i=1}^n$, $\{B_i\}_{i=1}^n$ into $A[1..n]$, $B[1..n]$\; \label{step:parity_encode}

% {\it Bob}: Encode $B[1..n]$ by BCH code, then send the codeword to Alice\; \label{step:BCH_encode}

% {\it Alice}: Upon receiving the codeword, decode the bit errors between $A[1..n]$ and $B[1..n]$\; \label{step:BCH_decode}

% {\it Alice}: For each bit error, reconcile the corresponding subset pair by \autoref{alg:trivial_case}\; \label{step:trivial_reconcile}

% {\it Bob}: Upon the reconciled distinct elements $\mathcal{D}$, check whether $A=B\triangle \mathcal{D}$ via checksum\; \label{step:terminate_condition}
% \end{algorithm}



\subsection{Exception Handling}\label{subsec:exception_hash_partition}

When the ideal case does not happen, some subset pairs may contain more than one distinct elements and cannot be successfully reconciled by \autoref{alg:trivial_case}. 
In this case, the checksum will detect this event and trigger another round of PBS to reconcile the ``remaining'' distinct elements, as will be elaborated in \autoref{sec:multi-rounds}. There are two types of exceptions that can possibly happen in such a subset pair, say $(A_i, B_i)$.

\smallskip
\noindent {\bf Type (\RN{1}) exception}:  $A_i\triangle B_i$ contains a nonzero even number of distinct elements.  In this case $A[i]=B[i]$
since the cardinalities of $A_i$ and $B_i$ are either both even or both odd.  The BCH codeword $\xi_A$ cannot detect this exception.
% and PBS will not reconcile the subset pair yet in this round. 
This exception happens with a small but nontrivial probability.  For example, when $d=5$ and $n=255$ (i.e., throwing $5$ balls each uniformly and randomly into $255$ bins), the probability that some bin has a nonzero even number of (in this case either $2$ or $4$) balls is roughly $0.04$. 
%Note that when a type (\RN{1}) event happens, the checksum (\autoref{step:terminate_condition} in \autoref{alg:single_round_pbs}) can detect that the set reconciliation has not been completed. Then PBS will start another round to reconcile the ``hidden'' distinct elements (the ones that have not been reconciled in this round), 
%so on so force, until all distinct elements are successfully reconciled and the checksum is verified to be correct, 
%as we will describe in \autoref{sec:multi-rounds}. 

% Note that when a Type (\RN{1}) subset pair exists, the $32$-bit checksum (\autoref{step:terminate_condition} in \autoref{alg:single_round_pbs}) can almost surely detect that the set reconciliation is incomplete. If this is the case (i.e., the checksum is verified to be incorrect), PBS will start another round of set reconciliation to reconcile the remaining distinct elements (e.g., the ``hidden'' distinct elements in Type (\RN{1}) subset pairs), so on so force, until all distinct elements are reconciled and the checksum is verified to be correct, as we will describe in \autoref{sec:multi-rounds}. 

\smallskip
\noindent {\bf Type (\RN{2}) exception}: $A_i\triangle B_i$ contains an odd number (at least $3$) of distinct elements.  In this case, $A[i]\neq B[i]$. 
Bob will mistakenly believe that $(A_i, B_i)$ contains exactly one distinct element and try to recover it using \autoref{alg:trivial_case}. The ``recovered'' element $s$ is however the \code{XOR} sum of all distinct elements in $A_i\triangle B_i$ as explained at the end of \autoref{subsec:protocol0}.
We call this $s$ a fake distinct element.
%, which will be mistakenly believed as the distinct element of $(A_i, B_i)$. 
This event happens with a tiny probability.  In the same example above ($d=5$ and $n=255$), 
the probability that some bin has an odd number of balls 
(in this case either $3$ or $5$) is only $1.52\times 10^{-4}$.  
This probability can be further reduced, thanks to the consistent nature of hash-partitioning, which provides us with a no-cost mechanism that can detect fake distinct elements with high probability. 



%%%% Comment out druing revision:
%%%% Although we have describe how to use hash partition to detect type (II) exception, however, we actually
%%%% does not make any use of it (Since anyhow we have to use further reconciliation attempts). 
%%%% For example, we do not describe what should we do when an element s passed 
%%%% or failed this detection. The information here is that the probability that we a fake element passing
%%%% this detection is so low. However, from the feedback of reviewers, this paragraph seems make them confused.
%%%% So I suggest to comment out this paragraph to simplify that information we want to delivery: we can handle 
%%%% the two exceptions so that they will not result in reconciliation errors. 
\begin{algorithm}
\caption{Check whether $s\in \mathcal{U}_i$}
\label{alg:verification}
\If{$h(s)\neq i$} {Discard the ``recovered'' element $s$;}
\end{algorithm}

As shown in \autoref{alg:verification}, the detection mechanism is simply to check whether $s\in \mathcal{U}_i$ (i.e., whether $h(s)\! =\! i$), 
a necessary condition 
for $s$ to be an element in $A_i\triangle B_i$.  
The conditional (upon a type (\RN{2}) exception happening) probability for a fake distinct element, which belongs to any of the $n$ sub-universes with equal probability $1/n$
since it is the \code{XOR} sum of multiple distinct elements in $A_i\triangle B_i$, to pass this check is only $1/n$.  In the same example above ($d\!=\!5$, $n\!=\!255$), 
this conditional probability
is roughly $3.9\!\times\! 10^{-3}$, and hence the probability for both a type (\RN{2}) exception to happen and the resulting fake distinct element to pass this check is 
$1.52 \times 10^{-4} \times 3.9 \times 10^{-3} \approx$ $6\times 10^{-7}$.
%The probability for both events to happen in the same example above ($d=5$ and $n=255$) is $6\times 10^{-7}$, which is the multiplication between the probability for the %type (\RN{2}) exception to happen ($1.52\times 10^{-4}$) and the conditional probability ($3.9\times 10^{-3}$). 
% overhead
This mechanism only requires Alice to locally verify the ``recovered'' elements of \autoref{alg:trivial_case} and 
hence incurs no additional communication overhead. {\color{red}Note that whenever such an element $s$ failed to pass this 
sub-universe verification check, \autoref{alg:single_round_pbs} excludes it from $\hat{D}$.}
%  Alice can perform the check locally by computing $h(s)$.
% This mechanism only needs to locally verify the ``recovered'' elements of \autoref{alg:trivial_case}.  
% It clearly incurs no additional communication overhead:  Alice can perform the check locally by computing $h(s)$.
%does not incur any additional communication overhead.
%However, fake distinct element belongs to any of the $n$ sub-universes with equal probability $1/n$
%since it is the \code{XOR} sum of multiple distinct elements $A_i\triangle B_i$
% \end{comment}

%Although a distinct element of $(A_i, B_i)$ must be in sub-universe $\mathcal{U}_i$ (i.e., the hash value of the element under $h$ equals to $i$), 


%could be in any sub-universe with probability $1/n$, since it is the bitwise \code{XOR} of multiple distinct elements of $(A_i, B_i)$. Therefore, even when a type (\RN{2}) %exception happens to $(A_i, B_i)$, \autoref{alg:verification} only fails to identify a fake distinct element with a conditional probability of $1/n$, 

\begin{comment}
%% comment out by Long during revision
This said, a fake distinct element $s$ could pass this check and go undetected by \autoref{alg:verification}, albeit with a tiny probability as just shown.  
Even in this case, however, such an $s$ will not be mistakenly ``reconciled into" $A\triangle B$ for the following reason.
%and become a ``trouble-causing'' element.  
In this case, even when all actual distinct elements are successfully reconciled (so that $A\triangle\hat{D}=B\triangle \{s\}$), the checksum verification $c(A\triangle\hat{D})\stackrel{?}{=}c(B)$ would fail, triggering one or more rounds of 
further reconciliation attempts (to be described next) during which the fakeness of this ``trouble-causing'' element $s$ will be detected by Alice.  
\end{comment}

{\color{red}
Note that the existence of the above two types of exceptions 
will not result in reconciliation error, since 
whenever such an exception happens, the checksum verification in~\autoref{step:terminate_condition} of~\autoref{alg:single_round_pbs}
would fail (as now $\hat{D}\neq (A\triangle B)$, thus $c(A\triangle \hat{D})\neq c(B)$), triggering one or more rounds of 
further reconciliation attempts (to be described next), by which PBS will correctly reconcile all 
distinct elements. We also note that PBS does not need to know in which bins those exceptions happened 
to continue the subsequent reconciliation attempts. 
}

%if a fake distinct element $s$ is contained in $\hat{D}$, it is not hard to verify that  is not equal to $B$. Hence the checksums of these two sets will not match and the checksum verification will mistakenly believe that some of the distinct elements in $(A_i, B_i)$ have not %been reconciled yet. This is not a problem for PBS, because the ``trouble-causing'' elements can be detected in the latter rounds of the set reconciliation process, as we will explain in \autoref{sec:multi-rounds}. 

%(i.e., $\hat{D}=(A\triangle B)\cup\{s\}$) will induce that the two sets $A\triangle\hat{D}$ and $B$  of $A\triangle\hat{D}$ and the checksum of $B$ to be different.  and another round of PBS will be triggered. This is not a problem for PBS, because the ``trouble-causing'' elements can be detected in the set reconciliation process of PBS, as we will explain in \autoref{sec:multi-rounds}. 

%Note that a fake distinct element could accidentally happen to be an actual distinct element with vanishing probability. Such a fac element that is not detected by \autoref{alg:verification} 

% Note that a fake distinct element could accidentally happen to be an actual distinct element with vanishing probability. For example, when $(A_i, B_i)$ contains $5$ distinct elements $s_1,s_2,...,s_5$ and $s_1$ happens to be equal to $s_1\oplus s_2\oplus\cdots\oplus s_5$, the fake element (i.e., $s_1\oplus s_2\oplus\cdots\oplus s_5$) happens to be an actual distinct element (i.e., $s_1$), which will be contained in $\hat{D}$. This is not a problem, since in the next round $s_2,s_3,s_4,s_5$ will be hash-partitioned into different subset pairs In this case, the ``fake ''element does not cause any trouble in Each fake distinct element that is not detected by \autoref{alg:verification}, if does not happen to an actual distinct element, is a ``trouble-causing'' element that will be detected in the latter rounds, as we will explain in \autoref{sec:multi-rounds}. Note that a fake distinct element could accidentally happen to be an actual distinct element with vanishing probability. Such a fac element that is not detected by \autoref{alg:verification} 


% \subsection{Running PBS for Multiple Rounds}\label{sec:multi-rounds}

% %{\bf (merged from the following two paragraphs)} 
% To deal with the ``remaining'' distinct elements, we remove (and save) all the distinct elements that has been reconciled in the first round (i.e., $\hat{D}$) and run another round of PBS. More precisely, in the second round, we try to reconcile $A\triangle \hat{D}$ and $B$ by running the same procedure except for using a different and independent hash function (than $h$) to do hash-partition. 
% %instead of reconciling $A$ and $B$ for both (1) removing all the distinct elements that have been reconciled; and (2) keeping all the distinct elements that have not been reconciled, which we will explain shortly. 
% Here we use a different and independent hash function to avoid the same type (\RN{1}), (\RN{2}) exceptions happen again. 
% % We use a different hash function for hash-partition in the second round to avoid the same exceptions (i.e., type (\RN{1}), (\RN{2}) events) that happened in the first round happen again. 
% PBS keeps running until the set reconciliation is successfully completed as verified by the checksum (\autoref{alg:single_round_pbs} of \autoref{step:terminate_condition}). The use of independent hash functions in different rounds naturally enables the Markov chain modeling of the reconciliation process, which will be elaborated in \autoref{sec:single_markov}. 

% {\bf (new content)} Note that a fake distinct element $s$, if is not detected by \autoref{alg:verification}, will be mistakenly believed as a distinct element (between $A$ and $B$) and contained in $\hat{D}$. This is not an issue because in this case, $s$ is an actual distinct element between $A\triangle \hat{D}$ and $B$. Starting with the second round, PBS will try to reconcile $s$ and eventually ``correct'' this fake distinct element. 

% We emphasize that the fake distinct elements (incurred by type (\RN{2}) exception) that are not detected by \autoref{alg:verification} in the first round can also be reconciled in the second round. also keeps all the distinct elements that need to be reconciled. Note that the ``remaining'' distinct elements can be classified into two catagories: (1) the ``hidden'' distinct elements that have not been reconciled yet (i.e., $D\!\setminus\!\hat{D}$), which are incurred by either a type (\RN{1}) event or a type (\RN{2}) event; and (2) the ``fake'' distinct elements incurred by both a type (\RN{2}) event and the corresponding verification failure in \autoref{alg:verification} (i.e., $\hat{D}\!\setminus\!D$). It is not hard to verify that this classification of the ``rest'' distinct elements (i.e., $D\!\setminus\!\hat{D}$ and $\hat{D}\!\setminus\!D$) is a partition of the set difference between $A\triangle \hat{D}$ and $B$, which confirms our emphasis. 

% {\bf (new content)} We emphasize that reconciling $A\triangle \hat{D}$ and $B$ not only removes all the distinct elements that have been reconciled, but also keeps all the distinct elements that need to be reconciled. Note that the ``rest'' distinct elements can be classified into two catagories: (1) the ``hidden'' distinct elements that have not been reconciled yet (i.e., $D\!\setminus\!\hat{D}$), which are incurred by either a type (\RN{1}) event or a type (\RN{2}) event; and (2) the ``fake'' distinct elements incurred by both a type (\RN{2}) event and the corresponding verification failure in \autoref{alg:verification} (i.e., $\hat{D}\!\setminus\!D$). It is not hard to verify that this classification of the ``rest'' distinct elements (i.e., $D\!\setminus\!\hat{D}$ and $\hat{D}\!\setminus\!D$) is a partition of the set difference between $A\triangle \hat{D}$ and $B$, which confirms our emphasis. 

% To deal with the ``remaining'' distinct elements, we remove (and save) all the distinct elements that has been reconciled in the first round (i.e., $\hat{D}$) and run another round of PBS. In the second round, we reconcile $A\triangle \hat{D}$ and $B$ instead of reconciling $A$ and $B$ to remove all the reconciled distinct elements. We use a different hash function for hash-partition in the second round to avoid the same exceptions (i.e., type (\RN{1}), (\RN{2}) events) that happened in the first round happen again. This procedure replicates until If until all distinct elements are successfully reconciled and the checksum is verified to be correct. 

% {\bf (to be removed)} When the ideal case does not happen (i.e., type (\RN{1}) or type (\RN{2}) event happens), PBS will know the set reconciliation has not been completed via the $32$-bit checksum (\autoref{step:terminate_condition} in \autoref{alg:single_round_pbs}). To reconcile those distinct elements that have not been reconciled yet in the first round, we rule out all successfully reconciled elements and run another round of PBS. This procedure replicates until all distinct elements are successfully reconciled and the checksum is verified to be correct.

% {\bf (to be removed)} More specifically, in the second round, we run PBS to reconcile $A$ and $B\triangle \hat{D}$ instead of $A$ and $B$ to rule out all elements that have been reconciled, where $\hat{D}$ is the set of reconciled distinct elements in the first round. We use a different hash function for hash-partition in the second round to avoid the same exceptions (i.e., type (\RN{1}), (\RN{2}) events) that happened in the first round happen again. The later rounds are similarly operated. 

%{\bf Normally, we want PBS to successfully reconcile all distinct elements in only a few rounds (say $3$) with high probability (say $99\%$). Hence, when tuning parameters (to be discussed in \autoref{sec:parameter_settings}), we set a {\it target success probability} $p_0$ of $r$ rounds as a paramenter setting requirement, which aims to ensure the probability that all distinct elements are reconciled in $r$ rounds to be larger than $p_0$. This requirement should also ensure the majority of the distinct elements are reconciled in the first round. Use the same example ($d=5, n=255$), on average $4.81$ out of $5$ distinct elements should be reconciled in the first round. So the total communication overhead in all rounds is only slightly larger than ($1.01$ to $1.07$ times of, as we will show in \autoref{fig:per-round-con}) that in the first round. Due to this reason, we use the communication overhead in the first round (described in \autoref{sec:communication_overhead_single_PBS}) to approximate the total communication overhead of all rounds in parameter settings (to be elaborated in \autoref{sec:parameter_settings}.}

% Although PBS may need to run many rounds to reconcile all distinct elements, the communication overhead mostly happens in the first round, since the majority of the distinct elements should be reconciled in the first round. Use the same example ($d=5, n=255$), on average $4.81$ out of $5$ distinct elements should be reconciled in the first round. So the total communication overhead in all rounds is only slightly larger than ($1.01$ to $1.07$ times of, to be shown in \autoref{fig:per-round-con}) that in the first round. Due to this reason, we use the communication overhead in the first round (described in \autoref{sec:communication_overhead_single_PBS}) to approximate the total communication overhead (all rounds) in parameter settings (to be elaborated in \autoref{sec:parameter_settings}).

%For the moment, we assume no ``fake'' distinct element in type (\RN{2}) subset pairs fails to be detected, which happens with overwhelming probability as explained in \autoref{subsec:exception_hash_partition}. Then 
%PBS reconciles the distinct elements gradually round by round. This is the ``piecewise decodability'' mentioned in \autoref{sec:intro_oursolution}. We use the following example to describe it in details: 
%Given two sets with $10$ distinct elements, in the first round, PBS tries to reconcile the $10$ distinct elements and say $6$ out of the $10$ distinct elements are successfully reconciled. Then the $6$ reconciled distinct elements are removed and PBS tries to reconcile the remaining $4$ distinct elements in the second round. Say $2$ out of the $4$ remaining distinct elements are successfully reconciled, and that leaves $2$ remaining distinct elements to be reconciled in the third round, so on so force. 
% Given two sets $A$, $B$ with $10$ distinct elements, in the first round, PBS hashes them into $7$ distinct subset pairs. $6$ distinct elements are hashed into $6$ distinct subset pairs, and the other $4$ distinct elements are hashed into the same subset pair. Then the former $6$ distinct elements are successfully reconciled in the first round and the later $4$ distinct elements remain to be reconciled in the second round, which are hashed into $3$ distinct subset pairs (under a different hash function). $2$ remaining distinct elements are hashed into $2$ distinct subset pairs, and the other $2$ remaining distinct elements are hashed into the same subset pair. Then the former $2$ remaining distinct elements are successfully reconciled in the second round and the later $2$ remaining distinct elements remain to be reconciled in the third round, so on so force. 
%The dynamics of the number of remaining distinct elements (i.e., $10\leadsto 4\leadsto 2\leadsto \cdots$ in the example) is in nature a Markov chain, which will be elaborated and analyzed in \autoref{sec:single_markov} to derive a tight tail bound of the probability that all distinct elements are reconciled in $r$ rounds.

% Even if the ideal case does not happen, most of the distinct elements should be distributed into different subset pairs, one distinct element in each, and therefore can be successfully reconciled. So in the first round, even if PBS cannot reconcile all distinct elements, it can reconcile the majority of them.
% % (piecewise decodability mentioned in \autoref{sec:intro_oursolution})
% Based on this intuition, we generalize PBS to multi-round, so that the distinct elements that are not reconciled yet in the first round can be reconciled in later rounds.  

% Without loss of generality, we only describe the second round of multi-round PBS, the reconciliation in the later rounds are similar. Let $\hat{D}_1$ denote the set of reconciled elements in the first round. If set reconciliation is not complete in the first round (i.e., the checksum infers $A\neq B\triangle \hat{D}_1$), then multi-round PBS saves $\hat{D}_1$, which includes correctly and incorrectly reconciled elements as described in \autoref{subsec:exception_hash_partition}, and starts the second round to find (1) the remaining distinct elements; (2) the incorrectly reconciled distinct elements in the first round. In the second round, multi-round PBS reconciles $A$ and $B\triangle \hat{D}_1$ instead of $A$ and $B$ (i.e., $B\leftarrow B\triangle\hat{D}_1$) to rule out all elements that have been reconciled. {\bf It uses a hash function that is different from the one used in the first round for hash-partition, otherwise every remaining distinct element will be hashed into the same subset pair and cause the same exception (described in \autoref{subsec:exception_hash_partition}) that happened in the first round.}

% If set reconciliation is complete in the second round, the set of reconciled elements in the second round (denoted as $\hat{D}_2$) should be the union of (1) all distinct elements that have not been reconciled in the first round (i.e., $(A\triangle B)\!\setminus\!\hat{D}_1$); and (2) all incorrectly reconciled elements in the first round (i.e., $\hat{D}_1\!\setminus\!(A\triangle B)$), which is by definition the set difference between $A\triangle B$ and $\hat{D}_1$. Therefore, the overall set difference $A\triangle B$ equals to the set difference between $\hat{D}_1$ and $\hat{D}_2$; Else, multiround PBS saves $\hat{D}_2$ and starts the third round, so on so force. 

% {\bf May need this algorithm to show the dynamics, if so, the earlier algorithm needs to change accordingly.}
% \IncMargin{1em}
% \begin{algorithm}
% \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
% \Input{$A$ and $B$}
% \Input{Maximum number of rounds $r$}
% \Output{$D$}

% $\hat{D},\mbox{ complete} \leftarrow PBS(A,B)$\;

% $D \leftarrow \hat{D}$\;

% \While{!complete and $r>0$}{
	
% 	$B \leftarrow B\triangle\hat{D}$\;

% 	$\hat{D},\mbox{ complete} \leftarrow PBS(A,B)$\;

% 	$D \leftarrow D\triangle\hat{D}$\;

% 	$r \leftarrow r-1$\;
% }

% \caption{Multi-round PBS} \label{proto:multirounds}
% \end{algorithm}\DecMargin{1em}

% The idea of multi-round PBS is quite simple: In each round, we discard the reconciled distinct elements in the previous rounds and aim to find the rest distinct elements from the remaining elements. More specifically, the first round of multi-round PBS is just the same as single-round PBS in \autoref{alg:single_round_pbs}. The second round has the same procedures as the first round. One difference is, we update $B$ by $B\leftarrow B\triangle\mathcal{D}$ in the second round, so that (1) Reconciled distinct elements in $\mathcal{D}$ that were contained in $A\triangle B$ are not longer contained in $A\triangle (B\triangle\mathcal{D})$; and (2) The other distinct elements remain in $A\triangle (B\triangle\mathcal{D})$ and can be reconciled later. The other difference is, we use a different hash function for partition (\autoref{step:hash_partition}) in the second round. Later rounds update $B$ in the same way and also use different hash functions. Multi-round terminates if the check in \autoref{step:termination} is correct. The overall set difference $A\triangle B$ is simply the union of reconciled distinct elements in all rounds. 

% A straightforward approach to discard reconciled distinct elements is to remove them from both $A$ and $B$. This approach however incurs additional communication overhead to update $A$, since only Bob learns the partial set difference in \autoref{step:reconcile}. Therefore, we use the approach in \autoref{step:updateb} that only updates $B$. It has another benefit in \autoref{step:termination}, which only needs to transmit the CRC of $A$ from Alice to Bob in the first round. In the later rounds, \autoref{step:termination} can be checked locally by Bob and does not require any additional communication overhead;

% Note that the communication overhead in the first round accounts for a large percentage of the total communication overhead in multi-round PBS, since most of the distinct elements (over $95\%$ as we will show in {\bf point to the figure}) should be reconciled in the first round. Therefore, we use the same parameter $n$ in later rounds because otherwise we have to compute a new parameter that can only save tiny communication overhead, even though the number of remaining distinct elements is small and can be reconciled using smaller $n$ with high probability. {\bf Due to the same reason, we can the same expression of the communication overhead in single-round PBS to approximate the communication overhead in multi-round PBS.}

% The natural termination condition of multi-round PBS is that all distinct elements are reconciled, which could require a large number of rounds and incur large additional communication overhead (each additional round incurs $d\log n$ bits of additional communication overhead on transmitting BCH codeword). To control the amount of additional communication overhead, we set another termination condition that multi-round PBS runs for at most $r$ rounds (typically $2$ or $3$). This termination condition could cause an `early' termination when some distinct elements have not been reconciled. However, under proper parameter settings (to be discussed in \autoref{sec:parameter_settings}), we can prove that the probability of an `early' termination (i.e., set reconciliation is incomplete in $r$ round) is very small
% %, and even if an `early' termination happens, an overwhelming percentage of distinct elements should have been reconciled, which is sufficient for most applications
% . For example, when $d=5, n=255, r=2$, an `early' termination happens with probability $4.8\times 10^{-4}$ (how to compute this probability will be elaborated in \autoref{sec:tail_bound}).

% For the moment, we assume no incorrectly reconciled distinct elements appears in multi-round PBS, which happens with overwhelming probability as explained in \autoref{subsec:exception_hash_partition}. Then multi-round PBS reconciles the distinct elements gradually round by round. This is the ``piecewise decodability'' mentioned in \autoref{sec:intro_oursolution}. We use the following example to describe it in details: Given two sets $A$, $B$ with $10$ distinct elements (i.e., $d=10$), in the first round, multi-round PBS hashes them into $7$ distinct subset pairs. $6$ distinct elements are hashed into $6$ distinct subset pairs, and the other $4$ distinct elements are hashed into the same subset pair. Then the former $6$ distinct elements are successfully reconciled in the first round and the later $4$ distinct elements remain to be reconciled in the second round, which are hashed into $3$ distinct subset pairs (under a different hash function). $2$ remaining distinct elements are hashed into $2$ distinct subset pairs, and the other $2$ remaining distinct elements are hashed into the same subset pair. Then the former $2$ remaining distinct elements are successfully reconciled in the second round and the later $2$ remaining distinct elements remain to be reconciled in the third round, so on so force. The dynamics of the number of remaining distinct elements (i.e., $10\leadsto 4\leadsto 2\leadsto \cdots$ in the example) is in nature a Markov chain, which will be elaborated and analyzed in \autoref{sec:tail_bound_per_group} to derive a tail bound of success probability (i.e., all distinct elements are reconciled in $r$ rounds) for paramenter settings. 

% In most applications, a high percentage of reconciliation (e.g., $>99\%$ distinct elements are reconciled) is good enough. Therefore, we add another termination condition on the maximum number of rounds (denoted as $r$). The larger $r$ is, the higher percentage of distinct elements will be reconciled. How to set parameters based on $r$ will be elaborated in \autoref{sec:parameter_settings};

% Readers may think the communication overhead of multi-round PBS is proportional to the number of rounds. In fact, the majority of the communication overhead is spent in the first round, since most of the distinct elements (over $95\%$ as we will show in {\bf point to the figure}) are reconciled in the first round. Each additional round only incurs a small amount of additional communication overhead. For example, when $d=10, n=255, |\mathcal{U}|=2^{32}$, assume $8$ distinct elements are reconciled in the first round and the rest $2$ distinct elements are reconciled in the second round. Then the communication overhead in the first round is $432$ bits. That number of the second round is only $160$


%the communication overhead of single-round PBS of $272$ ($2d\log n+d\log |\mathcal{U}|+32$) bits, and each additional round incurs $40$ ($d\log n$) bits of additional communication overhead. 

%among the three components of the communication overhead mentioned in \autoref{sec:communication_overhead_single_PBS}, only the first component (i.e., the BCH codeword) is proportional to the number of rounds. The other two components does not depend on the number of rounds.

% The second component only depends on the total number reconciled elements, which is roughly equal to $d$. The third component, the checksum of $A$, only needs to be sent once in the first round.
%Therefore, the communication overhead of multi-round PBS is only slightly larger than that of single-round PBS when the number of rounds is small (say $3$). For example, when $d=5, n=255, |\mathcal{U}|=2^{32}$, the communication overhead of multi-round PBS of $3$ rounds is $352$ bits, which is roughly $1.3$ times of the communication overhead of single-round PBS ($272$ bits).

% Therefore, each additional round of multi-round PBS only incurs a small amount of additional communication overhead. For example, when $d=5, n=255, |\mathcal{U}|=2^{32}$, the communication overhead of single-round PBS of $272$ ($2d\log n+d\log |\mathcal{U}|+32$) bits, and each additional round incurs $40$ ($d\log n$) bits of additional communication overhead. 

% As we explained in \autoref{sec:reconcile_by_trivial}, the communication overhead in each round is proportional to the number of (remaining) distinct elements, which decreases exponentially as the number of round increase (i.e., the first round reconciles $90\%$ of distinct elements, the second round reconciles $90\%$ of the remaining $10\%$ distinct elements, etc.). So the majority of the communication overhead (i.e., $\approx 90\%$) is in the first round. Therefore, we do not bother to optimize parameters (i.e., smaller $n$) in later rounds to save tiny communication overhead, even though remaining distinct elements become fewer and can be reconciled using smaller $n$;

% The termination condition of multi-round PBS is that all distinct elements are reconciled, which may require many rounds. In most applications, a high percentage of reconciliation (e.g., $>99\%$ distinct elements are reconciled) is good enough. Therefore, we add another termination condition on the maximum number of rounds (denoted as $r$). The larger $r$ is, the higher percentage of distinct elements will be reconciled. How to set parameters based on $r$ will be elaborated in \autoref{sec:parameter_settings};

% Multi-round means multiple round-trip delays. {\bf Thanks for the piecewise decodability of PBS, in almost all practical application scenarios, this tradeoff does not lead to longer response time because the reconciliation of objects identified by the successfully decodable codewords, which constitute the vast majority of all codewords, can run in parallel with the transmissions and decodings of the rest.  In other words, the piecewise decodability effective masks the slightly larger number of communication rounds as far as the response time is concerned.}

\begin{comment}
==============================

The pseudocode of set reconciliation operations in each round is shown as follows:

\IncMargin{1em}
\begin{algorithm}
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
\Input{$A$ and $B^{(in)}$}
\Input{Set of reconciled distinct elements $D^{(in)}$}
\Output{$B^{(out)}$}
\Output{Set of reconciled distinct elements $D^{(out)}$}

% Hash-partition $A^{(in)}$, $B^{(in)}$ into $\{A^{(in)}_i\}_{i=1}^n$, $\{B^{(in)}_i\}_{i=1}^n$ (\autoref{sec:hash_partition})\label{step:hash_partition}\;

% Encode $\{A^{(in)}_i\}_{i=1}^n$, $\{B^{(in)}_i\}_{i=1}^n$ into parity bitmaps (\autoref{sec:parity_bitmap_encoding})\;


% Find those subset pairs (denoted them as $(A^{(in)}_{i_1}, B^{(in)}_{i_1}), ...,(A^{(in)}_{i_k}, B^{(in)}_{i_k})$) that parity bits differ (\autoref{sec:BCH_code})\;

Run single-round PBS on $A$ and $B^{(in)}$ to obtain the (partial) set difference $\mathcal{D}$\label{step:reconcile} \;

$D^{(out)} \leftarrow D^{(in)}\bigcup \mathcal{D}$\label{step:updated}\;

$B^{(out)} \leftarrow B^{(in)}\triangle\mathcal{D}$\label{step:updateb}\;

Check whether the set reconciliation is complete by comparing $A$ to $B^{(out)}$ (via CRC)\label{step:termination}\;

\caption{Set reconciliation operations of PBS in each round} \label{proto:multirounds}
\end{algorithm}\DecMargin{1em}

In \autoref{proto:multirounds}, the output $B^{(out)}$ in the $r^{th}$ round is the input $B^{(in)}$ in the $(r+1)^{th}$ round. $D^{(in)}$ and $D^{(out)}$ have the same relationship, and they denote the set of reconciled distinct elements before and after a round. $B^{(in)}$ and $D^{(in)}$ are initialized as $B$ and $\emptyset$ respectively. We omit the currect number of round $r$ in \autoref{proto:multirounds}, since the operations in different rounds are exactly the same. Due to the same reason, we only elaborate the operations in the first round: First, Alice and Bob reconcile $A$ and $B^{(in)}$ $(=B)$ using single-round PBS and Bob obtains the (partial) set difference $\mathcal{D}$ (\autoref{step:reconcile}); Second, Bob updates the set of reconciled distinct elements by merging it with $\mathcal{D}$ (\autoref{step:updated}); Third, Bob updates $B^{(in)}$ $(=B)$ to $B^{(out)}$ as \autoref{step:updateb} shows, such that (1) The reconciled distinct elements in $\mathcal{D}$ that are contained in $A\triangle B^{(in)}$ are not longer contained in $A\triangle B^{(out)}$; and (2) The distinct elements that are not successfully reconciled remain in $A\triangle B^{(out)}$ and can be reconciled in later rounds; Finally, we check whether all distinct elements are reconciled. Note that if it is true, $B^{(out)}$ should be the same as $A$ and multi-round PBS should terminate. We use a $32$-bit CRC (Cyclic Reduncancy Check) to check if $B^{(out)}=A$ in our evaluation. {\bf To achieve higher confidence, we can certainly use longer CRC (e.g., 64-bit). }

{\bf Remarks:}

(1) In each round, hash-partition in \autoref{sec:hash_partition} uses different hash functions, so that the remaining distinct elements from the last round will be hashed into different subset pairs with high probability;

(2) A straightforward approach to discard reconciled distinct elements is to remove them from both $A$ and $B$. This approach however incurs additional communication overhead to update $A$, since only Bob learns the partial set difference in \autoref{step:reconcile}. Therefore, we use the approach in \autoref{step:updateb} that only updates $B$. It has another benefit in \autoref{step:termination}, which only needs to transmit the CRC of $A$ from Alice to Bob in the first round. In the later rounds, \autoref{step:termination} can be checked locally by Bob and does not require any additional communication overhead;

(3) As we explained in \autoref{sec:reconcile_by_trivial}, the communication overhead in each round is proportional to the number of remaining distinct elements, which decreases exponentially as the number of round increase (i.e., the first round reconciles $90\%$ of distinct elements, the second round reconciles $90\%$ of the remaining $10\%$ distinct elements, etc.). So the majority of the communication overhead (i.e., $\approx 90\%$) is in the first round. Therefore, we do not bother to optimize parameters (i.e., smaller $n$) in later rounds to save tiny communication overhead, even though remaining distinct elements become fewer and can be reconciled using smaller $n$;

(4) One termination condition of Multi-round PBS is $B^{(out)}=A$, which refers that all distinct elements are reconciled. In most applications, a high percentage of reconciliation (e.g., $>99\%$ distinct elements are reconciled) is good enough. Therefore, we add another termination condition of the maximum number of rounds (denoted as $r$). The larger $r$ is, the higher percentage distinct elements will be reconciled, and the smaller $n$ is required. How to set parameters (e.g., $n$) based on $r$ will be elaborated in \autoref{sec:parameter_settings};

(5) Multi-round means multiple round-trip delays. {\bf Thanks for the piecewise decodability of PBS, in almost all practical application scenarios, this tradeoff does not lead to longer response time because the reconciliation of objects identified by the successfully decodable codewords, which constitute the vast majority of all codewords, can run in parallel with the transmissions and decodings of the rest.  In other words, the piecewise decodability effective masks the slightly larger number of communication rounds as far as the response time is concerned.}

==============================

\end{comment}

% (3) Readers may wonder in the later rounds, most distinct elements should be reconciled, and the rest distinct elements could be reconciled using degraded parameters (i.e., smaller $n$ and $t$). In fact, degrade parameters in later rounds cannot save much communication overhead, since the majority of it is spent in the first round (i.e., $>90\%$). Therefore, we use the same parameters (i.e., $n,t$) among all rounds in multi-rounds PBS;

% (4) The number of remaining distinct elements decreases exponentially as the number of round increase (i.e., the first round reconciles $90\%$ of distinct elements, the second round reconciles $90\%$ of the remaining $10\%$ distinct elements, etc.). 
% (4) The termination condition of Multi-rounds PBS is $B^{(out)}=A$ to reconcile all distinct elements. In some applications,  


% The output $B^{(out)}$ in the $r^{th}$ round is the input $B^{(in)}$ in the $(r+1)^{th}$ round. $D^{(in)}$ and $D^{(out)}$ are similarly defined. $B^{(in)}$ and $D^{(in)}$ are initialized as $B$ and $\emptyset$ respectively. Since and $D$ are updated in each round, so we use $B^{(in)}$ to denote the input and $B^{(out)}$ to denote the output respectively.  Specifically, in the first round, we initialize $B^{(in)}$ and $D^{(in)}$ as $B$ and $\emptyset$ respectively. we first use the single-round scheme 

% Then we run our (single-round) scheme on the updated two sets (i.e., after removing reconciled distinct elements) using a different (independent) hash-partition function from previous rounds, so that the rest distinct elements are hashed into different subset pairs (i.e., the ideal case) with high probability. At the end of each round, we check whether the set reconciliation is complete (i.e., all distinct elements are found) by computing the bitwise \code{XOR} of the remaining elements in $A$ and $B$ 
 

% This {\bf multi-rounds} scheme can significantly increase the success probability (i.e., the probability that all distinct elements are reconciled). Readers may wonder in the later rounds, most distinct elements should be reconciled, and the rest distinct elements could be reconciled using degraded parameters (i.e., smaller $n$ and $t$). In fact, degrade parameters in later rounds cannot save much communication overhead, since the majority of it is spent in the first round (i.e., $>90\%$). Therefore, we use the same parameters (i.e., $n,t$) among all rounds in our evaluation. 
% %The tradeoff between the number of rounds and the communication overhead per rounds will be elaborated in \autoref{sec:tail_bound}. In our evaluation, $r=2,3$ rounds are enough to achieve an extremely high success probability. 

% Readers may think the cost (i.e., communication overhead and the computational complexity) of this multi-rounds scheme is proportional to the number of rounds (denoted as $r$) and increases linearly with $r$. In fact, the cost of each round is roughly proportional to the number of remaining distinct elements, which decreases exponentially as $r$ increases (i.e., the first round reconciles $99\%$ of distinct elements, the second round reconciles $99\%$ of the remaining $1\%$ distinct elements, etc.). So the cost of this multi-rounds scheme is only slightly larger than that of the single-round scheme. Furthermore, as we explained in \autoref{sec:intro}, {\bf from intro thanks for the piecewise decodability of our solution, in almost all practical application scenarios, this tradeoff does not lead to longer response time because the reconciliation of objects identified by the successfully decodable codewords, which constitute the vast majority of all codewords, can run in parallel with the transmissions and decodings of the rest.  In other words, the piecewise decodability effective masks the slightly larger number of communication rounds as far as the response time is concerned.} 

\begin{comment}

\subsection{Baseline Scheme}\label{subsec:protocol1} 

Note that the set difference $A\triangle B$ can contain more than 1 elements (i.e., $d>1$), and \autoref{alg:trivial_case} cannot reconcile $A$ and $B$ directly in this case. Therefore, we propose a baseline scheme building upon~\autoref{alg:trivial_case} that also works when $d>1$: First, we partition the element universe $\mathcal{U}$ into $n$ sub-universes $\mathcal{U}_1, \mathcal{U}_2, \cdots, \mathcal{U}_n$. Denote $A_i \triangleq A\bigcap \mathcal{U}_i$ and $B_i \triangleq B\bigcap \mathcal{U}_i$ for $i=1,2,\cdots,n$. Then $\{A_i\}_{i=1}^n$ and $\{B_i\}_{i=1}^n$ are partitions of $A$ and $B$ respectively. Furthermore, $\Phi\triangleq\{A_i\triangle B_i\}_{i=1}^n$ is a partition of $A\triangle B$. 

Assume the {\bf ideal case} happens, in which each subset pair $(A_i, B_i)$ contains at most one distinct element ({\it i.e.,} $|A_i\triangle B_i|\!\leq\!1$), we use \autoref{alg:trivial_case} to reconcile each subset pair and obtain $A_i\triangle B_i$ for $i=1,2,\cdots,n$. The overall set difference $A\triangle B$ is simply their union $\bigcup_{i=1}^n \big{(}A_i\triangle B_i\big{)}$. 

In the first step of the baseline scheme, we can use a hash function $h(\cdot): \mathcal{U}\rightarrow \{1,2,\cdots,n\}$ to partition the universe $\mathcal{U}$ into $n$ sub-universes: $\mathcal{U}_i=\{s\mid s\in \mathcal{U} \mbox{ and } h(s)=i\}$ for $\forall i=1,2,\cdots,n$. And the hash function $h(\cdot)$ can be predetermined between Alice and Bob and does not require additional communication cost.

This hash-partition can be modeled as a {\it balls-into-bins problem}, in which the distinct elements are viewed as balls and the subset pairs are viewed as bins. The hash-parition basically throws (hashes) $d$ balls (distinct elements) uniformly and randomly into $n$ bins (subset pairs). The aforementioned ideal case in this context becomes, after throwing $d$ balls uniformly and randomly into $n$ bins, each bin receives at most 1 ball (i.e., $d$ nonempty bins have 1 ball in each and the rest $n-d$ bins are empty). {\bf It may remind readers about the Birthday problem. And the ideal case can be analogous to the case that no people share the same birthday.} The ideal case happens with a probability of $p=\frac{n\,!}{(n-d)\,!n^d}\!=\!\prod_{k=1}^{d - 1}(1 - \frac{k}{n})\!\approx\! e^{-\frac{d(d-1)}{2n}}$ when $d\!\ll\!n$. In other words, $n$ must be $\Omega(d^2)$ to ensure the ideal case happens with a nontrivial probability.  Note that the communication overhead of the baseline scheme is proportional to $n$, as each subset pair requires communication of a bitwise \code{XOR} in \autoref{alg:trivial_case}. So this communication overhead increases at least quadratically as $d$ increases. 

In fact, this communication overhead can be significantly reduced: In the ideal case, $n-d$ out of $n$ subset pairs are identical ones, and only $d (\ll n)$ out of $n$ subset pairs contain distinct elements (one distinct element in each of the $d$ subset pairs) and need to be reconciled. If we can identify these $d$ subset pairs (with a tiny additional communication overhead) and only reconcile them, the overall communication overhead will be significantly reduced from $\Omega(d^2)$ to $O(d)$. Based on this intuition, we propose our scheme in \autoref{sucsec:our-scheme}, which uses Parity Bitmap Sketch (PBS) and Error Correction Coding (ECC) to identify those subset pairs with a tiny additional communication overhead. 

Note that the ideal case does not always happen. However, we can ensure that the ideal case happens with high probability by properly selecting $n$ based on $d$ (i.e., $n=\Omega(d^2)$). Furthermore, as we will describe in \autoref{subsec:nonideal}, even if the ideal case does not happen (i.e., some distinct elements are hashed into the same subset pair), most of the distinct elements should be distributed into different subset pairs and therefore can be reconciled. So the baseline scheme, even cannot reconcile all of the distinct elements, can still reconcile the majority of them. Based on this property, we will extend our scheme from single-round to multi-rounds in \autoref{subsec:nonideal} to further increase the probability of reconciling all distinct elements. 

For general cases ({\it i.e.,} $t=|A\triangle B|$ is an arbitrary number), we have a straightforward strawman scheme building upon~\autoref{alg:trivial_case}, which works as follows: First, Alice and Bob choose some hash function $h(s): \mathcal{U} \rightarrow \{0,1,\cdots,2^{32}-1\}$ to partition $A$ and $B$ into $m$ subsets $A_1,A_2,\cdots,A_m$ and $B_1,B_2,\cdots,B_m$ respectively:

\begin{align}
s\in A_i & \mbox{ iff } s\in A \mbox{ and } h(s)=i\!\mod m, \nonu{}mber\\
s\in B_i & \mbox{ iff } s\in B \mbox{ and } h(s)=i\!\mod m. \nonumber
\end{align} 

{\bf call a subset pair -> partition?} Since Alice and Bob use the same hash function for partition, common elements (i.e., elements in $A\cap B$) are always hashed into the same subset pair $(A_i, B_i)$. And the set difference of each subset pair only contains distinct elements (i.e., elements in $A\triangle B$): $A_i\triangle B_i \subset A\triangle B$. In the ideal case, with a sufficient large $m$, each subset pair $(A_i, B_i)$ contains at most one distinct element ({\it i.e.,} $|A_i\triangle B_i|\!\leq\!1$). Then \autoref{alg:trivial_case} can reconcile each subset pair and obtain $A_i\triangle B_i$ for $i=1,2,\cdots,m$. The overall set difference $A\triangle B$ is simply their union $\bigcup_{i=1}^m \big{(}A_i\triangle B_i\big{)}$. The selection of hash function $h(s)$ can be predetermined between Alice and Bob and it does not require additional communication cost.

%To make sure Alice and Bob use the same hash function for partition, we let them pre-agree on some universal hash family (e.g., \code{xxHash}~\cite{Collet_xxHashExtremelyfast_}) and a common selection order, and each time they choose a hash function from the family in the same order. Note that we can also let Alice generates a hash function and send it to Bob. The hash function that Alice and Bob choose for partition can be either generated by 

This hash-partition is in nature a {\it balls-into-bins model}. We can view the distinct elements as balls and the subset pairs as bins. The hash-parition basically throws (hashes) $t$ balls (distinct elements) uniformly and randomly into $m$ bins (subset pairs). The aforementioned ideal case in this context is, with a sufficient large number of bins, each bin receives at most 1 ball. The strawman scheme works correctly if and only if the ideal case happens, which has a probability of $\frac{m\,!}{(m-t)\,!m^t}\!=\!\prod_{k=1}^{t - 1}(1 - \frac{k}{m})\!\approx\! e^{-\frac{t(t-1)}{2m}}$. In other words, to ensure the strawman scheme works correctly with a probability of $p$, it roughly requires $m \!=\!\lceil \frac{t(t-1)}{-2\ln p}\rceil$ subset pairs. 

Note that the communication overhead of this strawman scheme is proportional to the number of subset pairs $m$, as each subset pair requires communication of an \code{XOR} sum in \autoref{alg:trivial_case} during the reconciliation. When $t$ is small, a small communication cost can guarantee that the strawman scheme works correctly with high probability. For instance, when $t=5$, $m=95$ subset pairs are sufficient for the strawman scheme to work correctly with a probability of $90\%$. However, when $t$ is relatively large, it requires a huge communication cost to ensure the strawman scheme works correctly. For instance, when $t=1,000$, it requires $m=4,740,865$ subset pairs to guarantee a success probability of $90\%$. 

In fact, the majority of subset pairs are identical ones and do not need to reconcile. And only a small portion of them contain distinct elements. If we can identify those subset pairs that contain distinct elements and only reconcile them, the communication cost could be significantly reduced. Our scheme is based on this intuition and uses parity bitmap sketch and BCH code to identify the subset pairs, which we will elaborate in \autoref{sucsec:our-scheme}. 

%To distribute balls as uniformly as possible and maximize the probability of the ideal case, we choose a uniform hashing function $h$ that throws balls uniformly and randomly into bins: $$\mathbb{P}[h(s)=i]=\frac{1}{m} \mbox{ for } \forall i=1,2,\cdots,m, \forall s\in U$$.

%Note that the probability of the ideal case is $\frac{m\,!}{(m-t)\,!m^t}\!=\!\prod_{k=1}^{t - 1}(1 - \frac{k}{m})\!\approx\! e^{-\frac{t(t-1)}{2m}}$. Hence, at least $\lceil \frac{t(t-1)}{-2\ln p}\rceil$ bins are required to ensure that this probability is at least $p$. In other words, to ensure that the ideal case happens with a probability of $p$, the strawman scheme roughly requires $m \!=\!\lceil \frac{t(t-1)}{-2\ln p}\rceil$. For example, suppose $t\!=\!$\num{1000}, %and $p\!=\!0.01$, this strawman scheme roughly requires $m\!=\!$\num{720626} bins (partitions) to ensure that $|A_i\triangle B_i|\!\leq\!1$ (for any $i=1,2,\cdots,m$) holds with probability $50\%$.  

% A straightforward strawman scheme building upon~\autoref{alg:trivial_case} 
% to reconcile two sets $A$ and $B$ in general 
% ({\it i.e.,} $|A\triangle B|$ is an arbitrary number) is the following: 
% Uniformly randomly partition $A$ and $B$ into $m$ subsets ($A_1,A_2,\cdots,A_m$ 
% and $B_1,B_2,\cdots,B_m$) so that the set difference 
% $A_i\triangle B_i$ of each subset pair $(A_i, B_i)$ contains at most one element 
% ({\it i.e.,} $|A_i\triangle B_i|\!\leq\!1$) {\it w.h.p.} ({\it i.e.,} with high probability), 
% and then reconcile each subset pair with~\autoref{alg:trivial_case}. 

% Now let us analyze this strawman scheme using the {\it balls-into-bins model}. 
% Assume that sets $A$ and $B$ have $t$ elements in their set difference, {\it i.e.,} $|A\triangle B|\!=\!t$. 
% These $t$ elements can be viewed as $t$ balls and the $m$ partitions (subset pairs) can be viewed as 
% $m$ bins. The random partition process in this strawman scheme can be modeled as throwing 
% $t$ balls into $m$ bins in the following manner: Each ball goes into a 
% uniformly random bin and independently of other balls. %so that each bin contains at most one ball, {\it w.h.p.}  
% The probability that each bin contains at most one ball is  
% $\frac{m\,!}{(m-t)\,!m^t}\!=\!\prod_{k=1}^{t - 1}(1 - \frac{k}{m})\!\approx\! e^{-\frac{t(t-1)}{2m}}$. 
% Hence, at least $\lceil \frac{t(t-1)}{-2\ln p}\rceil$ bins are required 
% to ensure that this probability is at least $p$. In other words, to ensure 
% that each bin contains at most one ball with a probability of $p$, 
% the strawman scheme roughly requires $m \!=\!\lceil \frac{t(t-1)}{-2\ln p}\rceil$. 
% For example, suppose $t\!=\!$\num{1000}, %and $p\!=\!0.01$, 
% this scheme roughly requires $m\!=\!$\num{108469} bins (partitions) to 
% ensure that $|A_i\triangle B_i|\!\leq\!1$ (for any $i=1,2,\cdots,m$) holds with probability $0.01$.  

% We note that the communication overhead of this strawman scheme is proportional to 
% $m$ ($\!\gg\! t$), as each partition (subset pair) requires communication of an \code{XOR} sum during the reconciliation. 
% This communication overhead is much higher than that of the optimal scheme, which only requires 
% to exchange the elements in the set difference (assuming an oracle tells it which elements belong to 
% the set difference), {\it i.e.,} proportional to $t$. In the example above, assuming each element takes 4 bytes, 
% the communication overhead of the strawman scheme is $4m$ bytes ($\!\approx\! \num{423.71}\,$KB) to ensure 
% a success rate of only 0.01 ({\it i.e.,} with a probability of $0.0.1$, all elements in 
% the set difference are successfully reconciled), 
% which is approximately 2 orders of magnitude higher than $4t$ bytes ($\!=\!\num{3.90}\,$KB), the communication 
% overhead of the optimal scheme. 

\subsection{Our Scheme: The Preliminary Version}\label{sucsec:our-scheme}

Like the baseline scheme, our scheme also hash-partitions the two sets $A$ and $B$ into $n$ subset pairs. The difference is, instead of reconciling all subset pairs using \autoref{alg:trivial_case}, our scheme identifies the subset pairs that contains distinct elements and only reconciles them. Since the hash-partition and set reconciliation on each subset pair using \autoref{alg:trivial_case} have been described in \autoref{subsec:protocol1}, we only elaborate how to identify the subset pairs that contain distinct elements in this section. 

The general idea of identification is very simple: First, we {\bf encode} each subset into $1$ bit, such that in the ideal case, for $\forall i=1,2,\cdots,n$:

\begin{itemize}
	\item The codewords (bits) of $A_i$ and $B_i$ are different if and only if subset pair $(A_i, B_i)$ contains $1$ distinct element;
	\item The codewords (bits) of $A_i$ and $B_i$ are the same if and only if subset pair $(A_i, B_i)$ contains no distinct element;
\end{itemize}

Second, we {\bf compare} the codewords of each subset pair. And the subset pairs that contain distinct elements are the ones with different codewords (bits). We will describe the two steps in details in \autoref{sec:parity_bitmap_encoding} and \autoref{sec:BCH_code} respectively.

\subsubsection{Parity Bitmap Encoding}\label{sec:parity_bitmap_encoding}

In our scheme, we use {\it parity encoding} to encode each subset into a parity bit. More specific, it encodes a subset as ``1'' if it contains odd number of elements, and as ``0'' otherwise. And it satisfies the aforementioned requirements in the ideal case:

\begin{itemize}
	\item If subset pair $(A_i, B_i)$ contains $1$ distinct element, the corresponding two subsets $A_i$ and $B_i$ differ exactly one element, which implies that $||A_i|\!-\!|B_i||\!=\!1$. Hence, if $|A_i|$ ({\it i.e.,} number of elements in $A_i$) is odd (or even), then $|B_i|$ must be even (or odd). And the parity bits of $A_i$ and $B_i$ will be different;
	\item If subset pair $(A_i, B_i)$ contains no distinct element, the corresponding two subsets $A_i$ and $B_i$ should be the same and therefore contain the same number of elements. Hence, if $|A_i|$ is odd (or even), then $|B_i|$ must be odd (or even). And the parity bits of $A_i$ and $B_i$ will be the same;
\end{itemize}

Using parity encoding, the $n$ subsets of $A$ are encoded as a bit string $A[1..n]$ in $\{0,1\}^n$, 
where the $i$-th bit $A[i]$ in $A[1..n]$ corresponds to the parity encoding bit of $A_i$. Similarly, the $n$ subsets of $B$ are similarly 
encoded as a bit string $B[1..n]$. We call $A[1..n]$ ($B[1..n]$) the {\it parity bitmap} of $\{A_i\}_{i=1}^n$ ($\{B_i\}_{i=1}^n$). In the ideal case, $A[1..n]$ and $B[1..n]$ differ at $d$ different bit-positions, which corresponds to the $d$ subset pairs that contain distinct elements. And our scheme only reconciles those subset pairs that the parity bits are different. We will describe the nonideal case (i.e., some subset pair contains more than 1 distinct elements) in \autoref{subsec:nonideal}.

\subsubsection{Parity Bitmap Comparison Using BCH Code}\label{sec:BCH_code}

A straightforward approach to compare the parity bitmaps is to let Bob send the complete parity bitmap $B[1..n]$ to Alice, then Alice compares $A[1..n]$ with $B[1..n]$ locally. This approach has a communication overhead of $n$ bits, which is unnecessarily high. As we discussed in~\autoref{subsec:protocol0}, $d$ is usually much smaller than $n$. It means $A[1..n]$ and $B[1..n]$ differ only at a tiny portion of bits. Therefore, we can view $A[1..n]$ as a corrupted message of $B[1..n]$ with $d$ corrupted bits, and the bit-positions of the $d$ corrupted bits basically correspond to the $d$ subset pairs that contain distinct elements. The detection of corrupted bits, on the other hand, can be solved by Error-Correction Code (ECC)~\cite{Lin_ErrorControlCoding_1983}. And our scheme uses BCH code~\cite{Lint_IntroductionCodingTheory_1998} to encode the parity bitmap and detect the $d$ corrupted bits.

More specific, after the parity bitmap encoding, Bob uses a $d$-error-correcting systematic BCH code to encode $B[1..n]$ into an $n+d\log n$ codeword, in which the first $n$ bits are $B[1..n]$ (property of systematic BCH code). Then Bob sends the rest $d\log n$ bits, which we denote as {\it parity bitmap sketch (PBS)}, to Alice. Upon the received PBS and $A[1..n]$ (corrupted message), Alice uses the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} to detect the $d$ corrupted bits in $A[1..n]$. The communication overhead of this approach is $d\log n$ bits (i.e., length of PBS), which is much smaller than that of the straightforward approach ($n$ bits, when $d\!\ll\!n$). On the other hand, the computational complexity of the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} is $O(d^2\log^2 n)$. 

\subsubsection{Exceptional Handling and Multi-rounds}\label{subsec:nonideal}

As we described in \autoref{subsec:protocol1}, the ideal case does not always happen, which means some subset pair may contain more than 1 distinct elements and cannot be successfully reconciled by \autoref{alg:trivial_case}. Due to the parity encoding, we can classify such subset pair into the following two scenarios:

\begin{itemize}
    \item Scenario 1: If a subset pair $(A_i, B_i)$ contains even number ($\geq 2$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be the same and our scheme will not reconcile the subset pair. Hence, the distinct elements in the subset pair will not be reconciled;
    \item Scenario 2: If a subset pair $(A_i, B_i)$ contains odd number ($\geq 3$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be different and our scheme will reconcile the subset pair using \autoref{alg:trivial_case}. However, as we described in \autoref{subsec:protocol0}, when a subset pair contains more than 1 distinct elements, \autoref{alg:trivial_case} will output the bitwise \code{XOR} of them as the `distinct element', which is not a real distinct element with high probability;
\end{itemize}

In both scenarios, the distinct elements in the subset pair cannot be reconciled. Even worse, in the second scenario, a false-positive could happen (i.e., the output of \autoref{subsec:protocol0} is not a real distinct element). However, as we will analyze in \autoref{sec:tail_bound} and show in {\bf the evaluation section}, the second scenario barely happens both theoretically and empirically. To further reduce the chance of false-positives, we add a verification step at the end of \autoref{subsec:protocol0} to check whether the output of \autoref{subsec:protocol0} $s$ is a real distinct element or not. The verification step works as follows: Given the output $s$ of subset pair $(A_i,B_i)$, if $s\in\mathcal{U}_i$ (i.e., $h(s)=i$), we consider $s$ as a real distinct element; Otherwise, we consider $s$ as an incorrect output and discard it. 

Note that if $s$ is a real distinct element of $(A_i,B_i)$, $s$ must be in sub-universe $\mathcal{U}_i$. However, if $s$ is the bitwise \code{XOR} of the distinct elements in $(A_i,B_i)$ (i.e., the second scenario happens), $s$ could be in any sub-universe other than $\mathcal{U}_i$. In fact, if we assume the hash-partition described in \autoref{subsec:protocol1} hashes the elements of $\mathcal{U}$ uniformly, independently, and randomly into $n$ sub-universes, the output $s$ in the second scenario will be in a different sub-universe $\mathcal{U}_j (j\neq i)$ with a high probability of $1-\frac{1}{n}$. Hence, this verfication step can reduce the chance of false-positives by a factor of $\frac{1}{n}$. 

Even if the ideal case does not happen, most of the distinct elements should be distributed into different subset pairs and therefore can be reconciled. So our scheme, even cannot reconcile all of the distinct elements, can still reconcile the majority of them (piecewise decodability). To reconcile the rest distinct elements, we can just run our scheme for another round under a different hash-partition function, so on so force. This {\bf multi-rounds} scheme can significantly increase the success probability (i.e., the probability that all distinct elements are reconciled). Readers may wonder in the later rounds, most distinct elements should be reconciled, and the remaining could be reconciled using degraded parameters (i.e., smaller $n$ and $t$). In fact, degrade parameters in later rounds cannot save much communication overhead, since the majority of it is spent in the first round (i.e., $>90\%$). Therefore, we use the same parameters (i.e., $n,t$) among all rounds in our evaluation.
%The tradeoff between the number of rounds and the communication overhead per rounds will be elaborated in \autoref{sec:tail_bound}. In our evaluation, $r=2,3$ rounds are enough to achieve an extremely high success probability. 

Readers may think the cost (i.e., communication overhead and the computational complexity) of this multi-rounds scheme is proportional to the number of rounds (denoted as $r$) and increases linearly with $r$. In fact, the cost of each round is roughly proportional to the number of remaining distinct elements, which decreases exponentially as $r$ increases (i.e., the first round reconciles $99\%$ of distinct elements, the second round reconciles $99\%$ of the remaining $1\%$ distinct elements, etc.). So the cost of this multi-rounds scheme is only slightly larger than that of the single-round scheme. Furthermore, as we explained in \autoref{sec:intro}, {\bf from intro thanks for the piecewise decodability of our solution, in almost all practical application scenarios, this tradeoff does not lead to longer response time because the reconciliation of objects identified by the successfully decodable codewords, which constitute the vast majority of all codewords, can run in parallel with the transmissions and decodings of the rest.  In other words, the piecewise decodability effective masks the slightly larger number of communication rounds as far as the response time is concerned.} 

\end{comment}

\input{section/multiround}

\subsection{BCH Encoding and Decoding}\label{sec:ecc-trick-bch}

{\color{red}
%%%%%%%%% by Long %%%%%%
%% Reason: I think that the following description of BCH can not 
%%         fully address BCH related comments.
%%%%%%%%%%%%%%%%
%% suggested to change to Error-Correction Coding Trick  and move to somewhere earlier
% Since PBS uses the error-correction coding (ECC) trick, we first give some background on 
% ECC. Then, we explain this trick and why we choose BCH codes in trick. 
In this section, we explain the error-correction coding trick and why we choose BCH codes in this trick. 
Before that, we first give some background on ECC for this paper to be self-contained. 
Given a message $u\in\{0,1\}^k$, an ECC encodes $u$ into $v\in\{0,1\}^{k'}$ with $k'>k$, where 
$v$ is referred to as the {\it codeword} of the message $u$. 
% Note that the the original message $u$ 
% may or may not appear in its codeword; codes that embed the original message in the codeword are 
% systematic and that do not are non-systematic. 
In this work, we only use the systematic codes, in which the original message is part of its codeword. 
For ease of presentation, we assume that the first $k$ bits in the codeword $v$ are from the original message.  
Thus the codeword can be written as $v=[u,\xi_u]$, where $\xi_u$ is referred to as the parity-check 
digits. 
When the codeword $v$ is transmitted over a noisy channel, the output of the channel or the received 
vector $v'$ may be different from $v$. For example, an error pattern of $l$ errors will cause 
$l$ different bits between $v'$ and $v$. Upon receiving $v'$, this ECC needs to decode $v'$ (to learn the original message): 
Locating the bit errors in $v'$ (of course, without knowing $v$ or the error pattern), 
{\it i.e.,} identifying the bit positions where $v'$ differs from $v$. 
Properly designed, an ECC can guarantee correcting 
all error patterns of no more than $t$ errors, where $t$ is called the error-correcting capacity of this code. 
%
% An ECC has an error-correcting capacity. This capacity is defined as the maximum 
% number of bit errors this code is designed to correct. 
Clearly,  
the larger the error-correcting capacity $t$ is, the longer the parity-check digits should be.

Now, we can explain the ECC trick used in PBS. Recall that, in PBS we view the bitmap $A[1..n]$ as the original message. 
The codeword $[A,\xi_A]$ of $A$, after transmitting over an imaginary noisy channel, becomes $[B,\xi_A]$. 
Properly parameterized,  
$\xi_A$ (together with $B$) can pinpoint to Bob all bit positions where $B[1..n]$ and $A[1..n]$ differ.  
% ({\it i.e.}, ``correct all bit errors in $B[1..n]$"). 
While many error-correction codes can be used in this ECC trick, we choose BCH codes in PBS because 
they are close to optimal in the following sense: In the context of PBS, to ``correct up to $t$ bit errors", 
$\xi_A$ only needs to be $t \lceil\log_2 (n + 1)\rceil$ bits long; 
even if Alice knew these $t$ bit positions precisely, specifying each bit position would require $\lceil\log_2 n\rceil$ bits. 
Note that, $n$ is almost always set to $2^m-1$ for some positive integer $m$ in BCH codes 
for achieving the maximum coding efficiency. We also assume this throughout this paper. 

We note that the BCH encoding in PBS differs slightly from the standard BCH encoding, 
since errors only happen in the message part of the codeword in the imaginary noisy channel in PBS, whereas 
they could happen anywhere in the codeword in general. How they differ from each other will be elaborated in~\autoref{app:bch}
}
% \begin{comment}


---
%%%%%
{\color{red}
In this section, we describe the specific BCH encoding and decoding in PBS;  how this encoding differs from 
%that are closely related to the PBS design and parameterization;
%explain the differences between this encoding and the BCH encoding 
that for its usual application of communication over a noisy channel will be explained in~\autoref{app:bch}. 
Recall that in~\autoref{step:BCH_encode} of~\autoref{alg:single_round_pbs}, Alice sends, instead of the ``message'' $A[1..n]$ itself, its much shorter BCH codeword $\xi_A$ to Bob.  Properly parameterized,  
$\xi_A$ can pinpoint to Bob all bit positions where $B[1..n]$ and $A[1..n]$ differ ({\it i.e.}, ``correct all bit errors in $B[1..n]$").  
In the context of PBS, to ``correct up to $t$ bit errors", $\xi_A$ needs to be $t \lceil\log_2 (n + 1)\rceil$ bits long.  This length is intuitively close to the optimal:  
Even if Alice knew these $t$ bit positions precisely, specifying each bit position would require $\log_2 n$ bits.  
%Since, in PBS, $n$ is always set to $2^m - 1$ for some 
%integer $m$, we drop the ``floor" and ``ceiling" and simply write the length of $\xi_A$ as $t \log_2 n$ in the sequel.

In the case of PBS-for-small-$d$, the number of ``bit errors" is $d$, which is assumed to be known beforehand.  
In this case, $\xi_A$ is parameterized to 
correct exactly $d$ ``bit errors" so the BCH decoding is always successful.  
However, as will be explained in~\autoref{subsec:parameterize-n-t}, when $d$ is large and the sets $A$ and $B$ each has to be partitioned into groups,
the number of ``bit errors" that occur to a group pair can exceed that the corresponding BCH codeword is parameterized to correct.  
In this case, a BCH decoding failure will happen and how to deal with its fallout will be explained in~\autoref{sec:BCH_exception}.

We now briefly explain what is involved for Bob to decode the BCH codeword $\xi_A$ against its local bitmap $B[1..n]$.
Here the only task is to figure out the ``bit error positions" (in which $A[1..n]$ and $B[1..n]$ differ).  To do so, Bob needs to 
invert a $t \times t$ matrix in which each matrix entry is an element of the finite field $GF(2^m)$ where $m = \lceil\log_2 (n + 1)\rceil$;  
since $n$ is always set to $2^m - 1$ for some integer $m$ in PBS, we drop the ``floor" and ``ceiling" and consider $m = \log_2 n$ in the sequel.
Normally such a matrix inversion would take $O(t^3)$ finite field operations over $GF(2^m)$.   However, since this matrix takes a special form called Toeplitz, 
it can be inverted in $O(t^2)$ operations over $GF(2^m)$ using the Levinson algorithm~\cite{levinson1946wiener}.  
}

% \end{comment}


\begin{comment}
There are two different BCH encoding techniques: {\it systematic} and {\it unsystematic}. The difference is that, in systematic encoding, the message appears as the prefix of 
the codeword (i.e., 
codeword = [message, net-codeword]), whereas in unsystematic BCH encoding, the message does not.  Only systematic BCH encoding is suitable for PBS, 
since Alice sends not the ``message'' $A[1..n]$ itself, but the net-codeword $\xi_A$. With this understanding, in the sequel we drop the prefix ``net-" and simply 
call $\xi_A$ a BCH {\it codeword}. 
\end{comment}

\begin{comment}


=== move to appendix in the arxiv version === begin


%In general, BCH decoding consists of two steps:  locating bit errors 

In this section, we describe the standard BCH encoding 
for its usual application of communication over a noisy channel and explain how it differs from the BCH encoding in BPS.   
In the standard BCH encoding, a coded message, which is the uncoded message concatenated with the codeword, is $n = 2^m - 1$ bits long 
in total.  For the codeword to correct up to $t$ bit errors, that may occur to both the uncoded message part and the codeword part 
during the transmission of the coded message over the noisy channel, it needs to be $tm$ bits long, resulting in a ``leftover" of 
at most $n - tm$ bits for the uncoded message.
%To summarize, in the standard BCH encoding, a codeword roughly of length $2tm$ bits is needed to correct 
%up to $t$ bit errors that may occur to either the uncoded message roughly of length $n - 2tm$ bits or the codeword.  

In PBS, the codeword $\xi_A$ is also $tm$ bits long, but the uncoded message $A[1..n]$ (which is not transmitted at all) can be $n$ bits 
(instead of $n - mt$ bits) long.  The uncoded message is allowed to be longer here because, unlike in the usual application 
of communication over a noisy channel where bit errors can happen also to the codeword, 
in PBS no bit error will happen to the codeword $\xi_A$ during its transmission.  


=== end ===
\end{comment}
%%% Moved from related work
%\input{section/pinsketch} 

==> section/pbs_vs_pinsketchwp.bk.0719.tex <==
\subsection{PBS vs. PinSketch with Partition}\label{subsec:vs-pinsketchwp}

% \begin{figure*}[!htbp]
% \centering
% \begin{subfigure}[t]{0.25\textwidth}
% \centering
% \includegraphics[width=0.99\textwidth]{figures/for-revision/success_rate_vs_PinSketchWP}
% % \caption{PBS vs. D.Digest and PinSketch (targeted success rate: 0.99).}
% % \caption{Target success rate: 0.99.}
% \caption{Success rate}
% \label{fig:success-rate-99-pswp}
% \end{subfigure}%
% \begin{subfigure}[t]{0.25\textwidth}
% \centering
% \includegraphics[width=0.99\textwidth]{figures/for-revision/communication_costs_vs_PinSketchWP}
% % \caption{PBS vs. D.Digest and PinSketch (targeted success rate: 0.99).}
% % \caption{Target success rate: 0.99.}
% \caption{Communication overhead}
% \label{fig:co-99-pswp}
% \end{subfigure}%
% \begin{subfigure}[t]{0.25\textwidth}
% \centering
% \includegraphics[width=0.99\textwidth]{figures/for-revision/encoding_time_vs_PinSketchWP}
% \caption{Encoding time}
% \label{fig:et-99-psbwp}
% \end{subfigure}%
% \begin{subfigure}[t]{0.25\textwidth}
% \centering
% \includegraphics[width=0.99\textwidth]{figures/for-revision/decoding_time_vs_PinSketchWP}
% \caption{Decoding time}
% \label{fig:dt-99-pbswp}
% \end{subfigure}%
% \caption{Comparisons against PinSketch/WP, with a target success rate of 0.99.}\label{fig:comp99-pswp}
% \end{figure*}

{\color{red}
Arguably, the same algorithmic trick ({\it i.e.}, hash-partition $A$ and $B$ each into groups) can 
also be applied also to PinSketch~\cite{Dodis_PinSketch_2008} 
for reducing its BCH decoding time from $O(d^2)$ to $O(d)$.  
Doing so however makes the communication overhead of PinSketch higher than that of PBS for the following reason.
As explained in~\autoref{subsec:parameterize-n-t}, 
we need to leave a safety margin in setting the BCH error-correction capacity $t$, in the sense that $t$ needs to be ``comfortably'' larger than $\delta$, the average number
of ``bit errors'' per group.   
%In other words, the amount of safety margin is $t - \delta$.  
Hence for each group pair, the average additional communication overhead (incurred for transmitting a longer BCH codeword) of leaving this safety margin
is $(t-\delta)\log n$ in PBS and is $(t-\delta)\log |\mathcal{U}|$ in PinSketch.
However, as explained in \autoref{sec:related}, 
$\log n$ is typically $3$ to $4$ times smaller than $\log |\mathcal{U}|$.  
Hence PinSketch pays $3$ to $4$ times more for leaving the safety margin, resulting in a higher overall communication overhead, as we elaborate next.  

Now we compare the performance of PBS against that of PinSketch with hash partition, which we refer to as PinSKetch/WP. 
For PinSketch/WP, we use the 
%same default parameter 
%setting as we use for PBS 
%({\it i.e.,} the default parameter setting), 
 %That is, PinSketch/WP uses the 
same parameter values ($\delta = 5$ and $t = 13$) as in PBS (there is no parameter $n$ in PinSketch/WP since it does not use a parity bitmap), 
with a target success probability of $p_0$=0.99 within $r$=3 rounds, in each experiment instance. 
The experimental results are reported in~\autoref{fig:comp99-pswp}.  It clearly shows that 
PBS outperforms PinSketch/WP in both communication 
overhead and computational overhead (the sum of the encoding and the decoding time).  
Note this outperformance will increase significantly when the hash signature length $\log|\mathcal{U}|$ increases ($\log|\mathcal{U}| = 32$ bits in~\autoref{fig:comp99-pswp}).
Hence, PBS would outperform significantly in real-world blockchain applications where $\log|\mathcal{U}|$ is much larger (e.g., $\log|\mathcal{U}| = 256$ bits in Bitcoin~\cite{Nakamoto_Bitcoinpeerpeer_2019}).
%in \autoref{fig:comp99-pswp} the hash signature length $\log|\mathcal{U}|$ is $32$.  
%an increasing margin
%he performance gains of PBS over 
%PinSketch/WP increase 
%as the hash signature length $\log|\mathcal{U}|$ increases.  This suggests that  and the 
% key size (length of each element in the universe) 
%hash signature length is much higher than 
%32 bits in many application. For example, the transaction ID (``hash signature'') in Bitcoin~\cite{Nakamoto_Bitcoinpeerpeer_2019} is 
%\SI{256}{bits}. 
}

==> section/pinsketch.tex <==
\subsection{PBS vs. PinSketch}\label{subsec:pbs-vs-pinsketch}

As we have mentioned earlier, PinSketch~\cite{Dodis_PinSketch_2008} also uses BCH coding to ``locate the $d$ bit errors", 
but in a different manner. 
% PinSketch~\cite{Dodis_PinSketch_2008} is an error-correction code (ECC) based set reconciliation algorithm.  
Given a universe $\mathcal{U}$ % of binary strings, %with $|\mathcal{U}|=u$, 
in which each element is assigned an index between $1$ and $|\mathcal{U}|$, 
% 
PinSketch 
% (and other ECC-based set reconciliation algorithms) represents 
encodes each set $S\!\subset \!\mathcal{U}$ as a %is viewed 
% as a characteristic vector (binary string) $s$ in $\{0,1\}^n$.  
$|\mathcal{U}|$-bit-long bitmap $S[1..|\mathcal{U}|]$: $S[i]$ (the $i^{th}$ bit of $S[1..|\mathcal{U}|]$) 
is equal to $1$ 
if the element, whose index is $i$, is contained in $S$; otherwise, $S[i]=0$. 
For example, when $|\mathcal{U}| \!=\! 2^{32}$ as assumed in most existing works, 
the bitmap encoding for any set in PinSketch is $2^{32}$ bits long.
In contrast, in PBS 
%since each bit encodes the oddness or evenness of the cardinality of a subset,   
the size $n$ of a bitmap is dependent only on $d$ (when $d$ is small) or $t$ (when $d$ is large), 
and not on the size of the universe or the cardinality of the set the bitmap encodes, and is hence much shorter.   
For example, as shown in the example in~\autoref{subsec:exception_hash_partition}, $n \!=\! 255$ is large enough for $d \!=\! 5$.  
As explained in~\ref{The BCH coding section}, the length of each BCH sub-codeword for ``locating each bit error" is the logarithm of the bitmap size.
This length is typically 3 to 4 times larger ($\log_2 |\mathcal{U}|$ = 32 bits in the example above) 
in PinSketch than in PBS ($\log_2 n = 8$ bits in the example above), a fact we will use in~\ref{evaluation subsection on partitions}.



[move the following paragraph to the evaluation section]

Arguably, the same algorithmic trick (i.e., hash-partition two sets each into groups) can also be applied to PinSketch~\cite{Dodis_PinSketch_2008} 
for reducing its BCH decoding time from $O(d^2)$ to $O(d)$.   Doing so however makes the communication overhead of PinSketch higher than that of PBS for the following reason.
As explained in~\ref{}, 
we need to leave a safety margin in setting the BCH error-correction capacity $t$, in the sense that $t$ needs to be ``comfortably'' larger than $\delta$, the average number
of ``bit errors'' per group.   
%In other words, the amount of safety margin is $t - \delta$.  
Hence for each group pair, the average additional communication overhead (incurred for transmitting a longer BCH codeword) of leaving this safety margin
is $(t-\delta)\log n$ in PBS and is $(t-\delta)\log |\mathcal{U}|$ in PinSketch.
However, as explained in \autoref{subsec:pbs-vs-pinsketch}, 
$\log n$ is typically $3$ to $4$ times smaller than $\log |\mathcal{U}|$.  
Hence PinSketch pays $3$ to $4$ times more for leaving the safety margin, resulting in a higher overall communication overhead, as we will elaborate next.  
%For example, when $\delta=5, n=255, |\mathcal{U}|=2^{32}, t=2.6\delta$ (same as in the example in \autoref{sec:BCH_exception}), the communication overhead of PinSketch using hash-partitioning 
%is $2.6$ times the theoretical minimum, whereas that of PBS is $2.1$ times the theoretical minimum. 



\begin{comment}

%With this encoding, the two bitmaps $A[1..|U|]$ and $B[1..|U]|$ for sets $A$ and $B$ differ 
%in $d$ bit positions (``errors") that correspond to the $d$ distinct elements in $A\triangle B$. 

Since the bitmap size is much smaller in PBS,  

Hence, this length is $\log_2 |\mathcal{U}|$ ($=32$ in the PinSketch example above) in the case of PinSketch and $\log_2 n$ 
($=8$ in the PBS example above) in the case of PBS.  In general, the former is 3 to 4 times shorter than the latter, 
making it 
more costly
for PinSketch to also use partitions (for reducing the BCH-decoding time from $O(d^2)$ to $O(d)$) for the following reason.


 in PinSketch than in PBS. 
, and a BCH codeword of length $32t$ bits 
is needed for ``correcting $t$ bit errors".
In this case, 
the BCH decoding operates in the much shorter
``8-bit-wide" GF($2^{8}$).  


the Galois field involved in its BCH encoding is the ``$32$-bit-wide" GF($2^{32}$).  

This shorter ``width" also implies $4$ times shorter BCH codeword in PBS than in PinSketch, 
We will elaborate on this point  
in \autoref{sec:whatifpinsketch}.  

%\subsection{What If PinSketch Also Uses Partitions?}\label{sec:whatifpinsketch}



This shorter ``width" alone in theory translates into roughly $16$ times shorter BCH decoding time, 
which grows quadratically with the ``width" of the underlying Galois field using the state-of-the-art BCH decoding algorithm~\cite{Dodis_SyndromeEncodingDecoding_2006}.  

%in the set reconciliation problem we usually assume each element is ``indexed" by a $32$-bit-long (hash) signature, so the universe contains a total of $2^{32}$ elements. In this case, 

We emphasize that BCH coding is used in PBS in a very different and much more efficient manner than that in PinSketch~\cite{Dodis_PinSketch_2008}.  
As explained above, in PinSketch, each bit encodes only a single element in the universe $\mathcal{U}$, 
so the 
length % size 
of the bitmap is equal to the cardinality %size 
of the universe $\mathcal{U}$.  


\end{comment}

%We call $m$ the ``width" of $GF(2^m)$ since the binary representation of each field element is $m$ bits long.  
%The time complexity of each operation over $GF(2^m)$ is $O(m^2)$, an important fact we will use in the sequel.  


%Like in PBS, the systematic BCH code is used to pinpoint these $d$ bit positions.

% if $i\in S$; 
%
% For example, $s_x=1$ for $x\in \mathcal{U}$ if 
% $x\in S$; otherwise $s_x=0$. 
% Using such a representation, 
% With such encoding, 
% set reconciliation problems can be converted into 
% error-correcting problems in Hamming space. More precisely, 
% With this encoding, reconciling two 
% sets $A$ and $B$ whose difference $A\triangle B$ has $d$ elements is equivalent to recovering 
% from $B[1..|\mathcal{U}|]$ (viewed as a corrupted version of $A[1..|\mathcal{U}|]$ with $d$ corrupted bit positions) 
% to $A[1..|\mathcal{U}|]$. 
% from a corrupted binary string in $\{0,1\}^{|\mathcal{U}|}$ where the number of errors is at most $d$. 
% With a suitable error-correcting code, ECC-based set reconciliation algorithms can achieve the 
% optimal communication overhead $t\log n$ (assuming $t$ is known a prior). 
% Unfortunately, as mentioned in~\autoref{sec:intro}, their 
% decoding computational complexity can be as high as $O(t^3)$. % where $t$ is the set-difference size. 
% PinSketch uses BCH codes~\cite{Lin_ErrorControlCoding_1983} with a decoding capacity $t=d$ (assuming $d$ is known a prior) 
% to solve this error-correcting problem. 
% However, the decoding algorithm of BCH codes has a computational complexity of 
% $O(d^2)$ finite field operations with the recent optimized implementation~\cite{Wuille_Minisketchoptimizedlibrary_2019}, 
% $O(d^3)$ finite field operations 
% in general 
% (can be reduced to $O(d^2)$ by exploiting the algebraic structures of certain 
% codes~\cite{Dodis_SyndromeEncodingDecoding_2006,Wuille_Minisketchoptimizedlibrary_2019}). 
% % as it requires to solve 
% % systems of linear equations in the form of $Mx=y$ where $M$ is a $d\times d$ matrix with Gaussian elimination. 
% % has a communication complexity of $t \log n$ and a 
% % (decoding) computational complexity of $O(d^3)$ using the implementation 
% % of the standard BCH decoding algorithm proposed in~\cite{Dodis_SyndromeEncodingDecoding_2006}. 
% Recently, 
% an optimized implementation of the PinSketch algorithm, 
% called Minisketch~\cite{Wuille_Minisketchoptimizedlibrary_2019}, was designed and open-sourced by the authors 
% of~\cite{naumenko2019bandwidth}. %Minisketch 
% This implementation has a computational complexity of $O(d^2)$ (instead of $O(d^3)$), 
% which, however, is too high when $d$ is large. For example, we will show in~\autoref{subsec:recon-perf}, 
% on a workstation with an Intel Core i7-9800X processor, PinSketch needs around 20\,\si{\second} 
% when $d\!=\!$\num{10000}, whereas 
% PBS only requires around $10^{-2}$\,\si{\second} (three orders of magnitude lower). 
% In the sequel, we still use ``PinSketch'' (not Minisketch) with the understanding that 
% the optimized implementation is used. 
% To avoid any confusions, only Minisketch (not PinSketch) will be used in the sequel.
%
%
% +++++++
% {\bf New Version (Copied from intro); I do not think it is proper to move the following paragraph here. 
% It is more proper to move it to somewhere in the scheme section. 
% So that we just remove the description on PinSketch in the related work section. } 
%
% {\bf PinSketch.} 
% As mentioned in~\autoref{sec:intro}, like PBS, PinSketch also uses BCH coding, yet in a very different manner. 






% which as will be explained in \autoref{sec:BCH_code} 
% which, as have be explained in \autoref{sec:BCH_code},  

==> section/related_work.bk.0719.tex <==
\section{Related Work}\label{sec:related}

In this section, we provide a brief survey of existing set reconciliation algorithms. 
% , focusing on 
% those that are not based on Error-Correction Codes (EECs), because the basic ideas of 
% EEC-based algorithms~\cite{Minsky2003,Dodis_PinSketch_2008,naumenko2019bandwidth,Karpovsky_eccreconciliation_2003} 
% are similar to that of PinSketch~\cite{Dodis_PinSketch_2008}, which we have described in detail in~\autoref{}. 
% Recall from~\autoref{sec:intro} that prior set reconciliation algorithms are mainly based on 
% either Bloom Filters (BF) or Error-Correction Codes (EEC). The basic ideas of 
% EEC-based algorithms~\cite{Minsky2003,Dodis_PinSketch_2008,naumenko2019bandwidth,Karpovsky_eccreconciliation_2003} 
% are similar to that of PinSketch~\cite{Dodis_PinSketch_2008}, which we have described in detail in~\autoref{}. 
% Hence, we only describe those are based on BFs in this section. 
As mentioned in~\autoref{sec:intro_prob_formulation}, in describing and comparing them with PBS, 
we only consider the unidirectional set reconciliation in which 
Alice learns $A\triangle B$. %in this work. 

\begin{comment}
Approximate set difference can be learned by Alice through exchanging BFs for 
sets $A$ and $B$ between Alice and Bob. Upon receiving the BF (for $B$) from Bob, 
Alice can infer ``common elements'' 
$\widehat{A\cap B}$ by querying this BF, 
from which Alice can infer $\widehat{A\setminus B}\!=\!A\setminus \widehat{A\cap B}$. Note that 
$\widehat{A\cap B}\!\supseteq\! (A\cap B)$ because of the false positive errors in BFs, and thus
$\widehat{A\setminus B}\!\subseteq\!A\setminus B$. Similarly, Bob 
can infer $\widehat{B\setminus A}$ ($\!\subseteq\!B\setminus A$) and Bob sends it to Alice, from which Alice can infer  
$\widehat{A\triangle B}\!=\!\widehat{A\setminus B}\bigcup\widehat{B\setminus A}$ ($\!\subseteq\!A\triangle B$). 
This scheme was extended by using more advanced data structures, such as Approximate Reconciliation Trees (ART) in~\cite{Byers_Informedcontentdelivery_2004}, Counting Bloom Filters (CBF) in~\cite{Guo_SetReconciliationvia_2013}, and 
Cuckoo Filters (CF)~\cite{Fan_CuckooFilterPractically_2014} in~\cite{Luo_SetReconciliationCuckoo_2019}. 
These schemes, however, have a flaw: Alice may only learn the approximate set difference, more precisely 
a subset of the set difference $A\triangle B$ 
(instead of the exact $A\triangle B$). This flaw is undesirable in most applications. 
\end{comment}

Bloom filters (BF)~\cite{Bloom_Space/TimeTradeoffs_1970} can be used to construct a crude set reconciliation scheme as follows.  
% Approximate 
% Set difference can be learned by Alice via exchanging BFs for 
% sets $A$ and $B$ between Alice and Bob. 
First, Alice and Bob exchange BFs for sets $A$ and $B$.  Upon receiving the BF (for $B$) from Bob, 
Alice can obtain an estimate, denoted as $\widehat{A\!\setminus\! B}$, of the set $A\!\setminus\! B$ 
by checking each element in $A$ against this BF. 
Note that $\widehat{A\!\setminus\! B}$ is in general an underestimate:
$\widehat{A\!\setminus\! B}$ may not contain all elements in $A\!\setminus\!B$, because this BF may produce false positives  
%% this sentence was "copied" from "Network Applications of Bloom Filters: A Survey"
that each suggests an element is in $B$ when it is not. 
Similarly, Bob can obtain $\widehat{B\!\setminus\! A}$ and sends it to Alice, from which Alice can infer an underestimate (of $A\triangle B$)
$\widehat{A\triangle B}\!=\!\widehat{A\!\setminus\! B}\bigcup\widehat{B\!\setminus\! A}$. 
% This scheme, however, has a flaw: 
%In this approach, Alice may only learn an approximate set difference, 
%more precisely a subset of the set difference $A\triangle B$ 
%(not the exact $A\triangle B$). 
Set reconciliation solutions that build on and extend this BF-based technique, including~\cite{Byers_Informedcontentdelivery_2004,Guo_SetReconciliationvia_2013,Luo_SetReconciliationCuckoo_2019},
all suffer from this underestimation problem, and hence 
% can only be used 
{\color{red}are only suitable} 
for few applications that do not require perfect data
synchronization.  


% Several 
As mentioned earlier, most exact set reconciliation algorithms
% , which focus on discovering the exact set difference, have been proposed. 
% Recall from~\autoref{sec:intro} that these algorithms are mainly 
are based on either invertible Bloom filters (IBF)~\cite{Goodrich_InvertibleBloomLookup_2011} or error-correction codes (ECC). 

\smallskip
\noindent
{\bf IBF-Based Algorithms.}
% In the following, we focus on IBF-based algorithms, since we have already described PinSketch~\cite{Dodis_PinSketch_2008} in detail
% and other ECC-based algorithms~\cite{Minsky2003,naumenko2019bandwidth,Karpovsky_eccreconciliation_2003} have similar core ideas.
%The basic ideas of 
%ECC-based algorithms~\cite{Minsky2003,Dodis_PinSketch_2008,naumenko2019bandwidth,Karpovsky_eccreconciliation_2003} 
%are similar to that of PinSketch~\cite{Dodis_PinSketch_2008}, which we have described in detail in~\autoref{subsec:pbs-vs-pinsketch}, 
%hence we will only describe the IBF-based algorithms~\cite{Eppstein_WhatsDifference?Efficient_2011,Ozisik2019} in the rest of this section. 
% Difference Digest (D.Digest)~\cite{Eppstein_WhatsDifference?Efficient_2011} is one such algorithm that based purely on IBFs. 
In an IBF, each element (from a set) is inserted into $k$ cells indexed by $k$ independent hash functions. Whereas each cell is a single 
bit in a BF, it has three fields in an IBF, each of which requires a single word of length $\log |\mathcal{U}|$. Therefore, IBFs are much more powerful than BFs: The set difference $A\triangle B$ of sets $A$ and $B$ can be recovered from the ``difference'' of their IBFs using a ``peeling process'' 
% which  
% is 
similar to that used in the decoding algorithms for some erasure-correcting codes, such as Tornado codes~\cite{luby1998tornado}.  
% However, %as shown in~\cite{Eppstein_WhatsDifference?Efficient_2011}, 
For this decoding process to succeed with a high enough probability, 
IBF-based solutions, such as 
Difference Digest (D.Digest)~\cite{Eppstein_WhatsDifference?Efficient_2011}, have to use roughly $2d$ cells.
%the number of cells need to be roughly at least $2d$. % to roughly ensure a success rate of $0.99$. 
This translates into a communication overhead of roughly $6d\log|\mathcal{U}|$, or
6 times the theoretical minimum. %of $d\log|\mathcal{U}|$. 
%In comparison, 
%PBS is much more space-efficient, whose communication overhead is roughly twice the theoretical minimum. 

%An approach of combing BFs with IBFs, called Graphene, was proposed in 

A recent solution called Graphene~\cite{Ozisik2019} reduces the high communication overhead of IBF-based solutions by augmenting it with  BFs.
% Recently, an approach, c that combines BFs and IBFs was proposed inGraphene~\cite{Ozisik2019} is another such algorithm that combines BFs and IBFs. 
Here, we only describe its simplest version (Protocol I in~\cite{Ozisik2019}) %, % of Graphene, 
% which only 
that works only for the special case of $B\!\subset\! A$. %, and which we will compare PBS with in~\autoref{sec:evaluation}. 
%
Its basic idea is for Alice to first obtain $\widehat{A\!\setminus\! B}$, an underestimate of of $A\!\setminus\! B$, by querying the BF for the set $B$ as described above, and then
recover only the ``missing" part $(A\!\setminus\! B) \!\setminus\! (\widehat{A\!\setminus\! B})$ using an IBF.   When the BF is configured to have a reasonably low false 
positive rate say $\epsilon$, 
the IBF needs only to ``encode" the roughly $\epsilon d$ ``missing" distinct elements rather than all the $d$ elements in $A\!\setminus\! B$, resulting in savings of 
``$O((1-\epsilon)d)$" in the size of IBF.    
%As a result, in this case the
%IBF in Graphene has a much smaller size than that in other IBF-based solutions.   
In general, for this $\epsilon$ to be reasonably low (say meaningfully away from $1$), 
the size of the BF has to be $O(|B|)$ with a nontrivial constant factor~\cite{Bloom_Space/TimeTradeoffs_1970}. % {\bf cite the original BF paper}.  
However, when $|B| \!\gg\! d$, which as explained earlier is often the case in most applications, 
the savings of ``$O((1\!-\!\epsilon)d)$" in the IBF size is no longer worth the $O(|B|)$ cost of the BF;
in this case Graphene drops the BF and degenerates to an IBF-only solution.    
For this reason, Graphene is more communication-efficient than other IBF-based solutions only when
$d$ is sufficiently large with respect to $|B|$.  Furthermore, this efficiency grows with $d$, as we will show 
in~\autoref{subsec:vs-graphene}.

{\color{red}
\smallskip
\noindent
{\bf ECC-Based Algorithms.}
% \input{section/pinsketch}
% [moved from Section 2.5 in the original submission]
% We will describe PinSketch~\cite{Dodis_PinSketch_2008} in detail
% and other ECC-based algorithms~\cite{Minsky2003,naumenko2019bandwidth,Karpovsky_eccreconciliation_2003} have similar core ideas.
The basic ideas of 
ECC-based algorithms~\cite{Minsky2003,Dodis_PinSketch_2008,Naumenko_ErlayEfficientTransaction_2019,Karpovsky_eccreconciliation_2003} 
are similar to that of PinSketch~\cite{Dodis_PinSketch_2008}, which we describe in detail next. 
% As we have mentioned earlier, PinSketch~\cite{Dodis_PinSketch_2008} also uses BCH coding to ``locate the $d$ bit errors", 
% but in a different manner. 
% PinSketch~\cite{Dodis_PinSketch_2008} is an error-correction code (ECC) based set reconciliation algorithm.  
Given a universe $\mathcal{U}$ % of binary strings, %with $|\mathcal{U}|=u$, 
in which each element is assigned an index between $1$ and $|\mathcal{U}|$, 
% 
PinSketch 
% (and other ECC-based set reconciliation algorithms) represents 
encodes each set $S\!\subset \!\mathcal{U}$ as a %is viewed 
% as a characteristic vector (binary string) $s$ in $\{0,1\}^n$.  
$|\mathcal{U}|$-bit-long bitmap $S[1..|\mathcal{U}|]$: $S[i]$ (the $i^{th}$ bit of $S[1..|\mathcal{U}|]$) 
is equal to $1$ 
if the element, whose index is $i$, is contained in $S$; otherwise, $S[i]=0$. 
For example, when $|\mathcal{U}| \!=\! 2^{32}$ as assumed in most existing works, 
the bitmap encoding for any set in PinSketch is $2^{32}$ bits long.
In contrast, in PBS 
%since each bit encodes the oddness or evenness of the cardinality of a subset,   
the size $n$ of a bitmap is dependent only on $d$ (when $d$ is small) or $t$ (when $d$ is large), 
and not on the size of the universe or the cardinality of the set the bitmap encodes, and is hence much shorter.  
Using BCH coding to ``locate the $d$ bit errors" in the bitmaps for sets $A$ and $B$, PinSketch learns 
the $d$ distinct elements in $A\triangle B$.

As mentioned earlier, ECC-based algorithms suffer from a much higher decoding 
computational complexity of at least $O(d^2)$. 
In~\cite{Minsky_Practicalsetreconciliation_2002}, a partition-based solution was proposed 
%the authors proposed a scheme that also uses the  
to reduce this computational complexity to $O(d)$, but in a different manner than the partitioning in PBS. 
This solution contains an ECC-based algorithm,  
called {\it BASIC-RECON}, that can 
reconcile a small number of distinct elements, just like what PBS-for-small-$d$ does.      

and recursively partition sets $A$ and $B$ until each partition can 
be successfully reconciled by {\it BASIC-RECON}. However, this partition scheme requires $O(\log d)$ rounds of message 
exchanges on average, which is generally much larger than that of PBS. 
}

\begin{comment}
For example, as shown in the example in~\autoref{subsec:exception_hash_partition}, $n \!=\! 255$ is large enough for $d \!=\! 5$.  
As explained in~\ref{The BCH coding section}, the length of each BCH sub-codeword for ``locating each bit error" is the logarithm of the bitmap size.
This length is typically 3 to 4 times larger ($\log_2 |\mathcal{U}|$ = 32 bits in the example above) 
in PinSketch than in PBS ($\log_2 n = 8$ bits in the example above), a fact we will use in~\ref{evaluation subsection on partitions}. 
\end{comment}


%The basic ideas of 
%ECC-based algorithms~\cite{Minsky2003,Dodis_PinSketch_2008,naumenko2019bandwidth,Karpovsky_eccreconciliation_2003} 
%are similar to that of PinSketch~\cite{Dodis_PinSketch_2008}
\begin{comment}
{\bf\color{cyan}
% Alice sends the cardinality $|A|$ of set A to Bob, which is required by Bob during the parameterization of the BF and IBF. 
% Upon receiving $|A|$, Bob creates a BF and an IBF for set $B$ parameterized to minimize the communication overhead
Bob sends to Alice a BF for the set $B$ and an IBF for 
% , parameterized to minimize the communication overhead, to Alice. %~\footnote{The parameters for the BF and IBFs }
With this BF, 
Alice can infer $\widehat{A\setminus B}$, which, as explained earlier, 
% may not contain all elements in $A\setminus B\!=\!A\triangle B$ because 
may be missing some elements in $A\setminus B\!=\!A\triangle B$ (since $B\subset A$) due to the false positives, which  
%To discover the exact set difference $A\triangle B$, 
Alice %corrects these false positives, {\it i.e.,} 
recovers 
%these elements 
% that are not in $B$ but suggested by the BF as in $B$, 
% that are
% (elements in $A\setminus B$ but suggested by the BF as in $B$), 
% in $(A\setminus B)\setminus\widehat{A\setminus B}$,  
from the IBF received from Bob. 
The number of such elements is on average $\epsilon|A\!\setminus\!B|\!=\!\epsilon d$ when the false positive rate (FPR) is $\epsilon$, since 
each element in $A\!\setminus\!B$ will be mistakenly determined by the BF as in $B$ with probability $\epsilon$. 
Therefore, when $\epsilon\!<\!1$, the number of IBF cells in Graphene is 
less than that required by IBF-only solutions ({\it e.g.,} D.Digest). 
The space saving compared to IBF-only solutions, is however not enough for compensating for the overhead of the BF when $d\!\ll\! |B|$, since
the space overhead of BF is proportional to $|B|$. 
For this reason, Graphene uses only an IBF 
when $d\!\ll\! |B|$. 
}

%, or in other words, $|A\triangle B|\!\ll\! |A\cap B|$ (since $B\subset A$) that is usual in most applications. 
% Graphene uses the optimal FPR, including the FPR of $1$ that corresponds to using the IBF only, to minimize its communication overhead. 
% % Note that an FPR of $1$ in Graphene corresponds to using the IBF only. 
% Therefore, Graphene is at least as space-efficient as IBF-based solutions. %solutions that use IBFs only. 
% However, as we will elaborate next, Graphene is generally less computationally-efficient that IBF-based solutions.    
% We note that when $d\ll |B|$  ({\it i.e.,} $|A\triangle B|\!\ll\! |A\cap B|$) that is common in most application scenarios, 
% the optimal FPR is generally $1$.



{\bf\color{cyan}
The communication overhead of PBS is between 2.21 to 2.75 times the theoretical minimum, which is higher than that in~\autoref{fig:co-99} 
as the target success rate here is higher. 
Unlike in other algorithms, in Graphene, the average amount of 
communication per distinct element 
% varies significantly as $d$ changes and %as shown in~\autoref{fig:co-9958}, 
% it 
decreases as $d$ increases. %which we have explained in~\autoref{sec:related}. 
Our explanation for this phenomenon is as follows.  
On one hand, as shown in~\cite{Ozisik2019}, given a success rate the size (space) of an IBF is roughly proportional to the number of 
distinct elements that need to be recovered from the IBF, which is $d$ when the BF is not used by Graphene.  
With a slight abuse of notation, we call this size ``$O(d)$".   
As explained in~\autoref{sec:related}, when $d$ is large enough, the BF starts to be used, 
producing a low FPR, say $\epsilon$.   In this case, only $\epsilon\cdot d$ elements needs to be recovered from
the IBF, so the size of the IBF becomes ``$O(\epsilon d)$", resulting in a savings of ``$O(1 - \epsilon)$" per distinct element.
On the other hand, the overhead of the BF is proportional to $|B|$, which is roughly a fixed cost, so the BF cost per distinct element 
decreases when $d$ increases.  
Therefore, the overall 
per-distinct-element overhead, including those of both the IBF and the BF, decreases as $d$ gets larger. 
}


{\bf\color{cyan}
We note that Graphene requires one more round to transmit an additional BF and a second IBF between Alice and Bob in the cases where $B\not\subset A$. 
{\bf OLD) } The number of such elements $d'$ (a random number) is on average $f|A\setminus B|\!=\!fd$, 
where $f$ is the false positive rate of the BF received from Bob. 
The total communication overhead of Graphene, therefore, is roughly 
$T(f)\!\triangleq\!-|B|\log_2(f)/\ln2\!+\!\tau fd\cdot 3\log|\mathcal{U}|$, 
where $\tau$ is the ``safety margin'' to account for both the randomness of $d'$ and the IBF decoding. 
The first term is the space for the BF and the second is that for the IBF.   
The value of $f$ that minimizes the communication overhead $T(f)$ is used in Graphene. 
% {\bf Here, I want to say that the results (for Graphene) we will show in the evaluation are just visualization of the minimum 
% $T(f)$ ({\it w.r.t.} $d$ and $\log|\mathcal{U}|$).} 
It is not hard to check 
the optimal value of $f$ is $f^*\!=\!\min\{1,|B|/(dC)\}$, where $C\!=\!3(\ln2)^2\tau\log|\mathcal{U}|$. 
We note that Graphene reduces to a pure IBF-based solution when $f^*\!=\!1$ and thus it  
has roughly the same communication overhead as D.Digest.  
When $f^*\!=\!|B|/(dC)\!<\!1$ ($d$ is relatively large), Graphene is more space-efficient 
than D.Digest as now $T(f^*)<T(1)$. %, which roughly corresponds to the communication overhead of D.Digest. 
In addition, It is easy to verify that, when $|A|$ is fixed, the overhead per distinct element $T(f^*)/(d\log|\mathcal{U}|)$, 
viewing as a function of $d$, is a decreasing function in this scenario ($f^*<1$). 
However, when $d\ll |B|$  ({\it i.e.,} $|A\triangle B|\!\ll\! |A\cap B|$) that is common in most application scenarios, 
we have $|B|/(dC)\!>\!1$, thus $f^*=1$ (Graphene reduces to a pure IBF-based solution).  
Therefore, Graphene is much less space-efficient as PBS when $|A\triangle B|\!\ll\! |A\cap B|$.
}

\end{comment}

% It was shown in~\cite{Gabrys2019} that Graphene is generally more space-efficient than D.Digest.
% schemes based purely on BFs or IBFs.  
% However,
% Graphene minimizes this communication overhead by optimally adjusting the space allocated to the BF and the IBF. 
% Roughly speaking, 
% 1000	1400	2000	4000	8000	10000
% 6	5.81711186092606	5.20341025080952	3.66281764169970	2.30540290045341	1.94771937332281
% 1	0.763478353895658	0.531182708694140	0.260171122625701	0.124665329591482	0.0975641709846379
% When $d/|B|$ is relatively large, the BF can have relatively low false positive rate and 
% thus it can help reduce number of cells in the IBF significantly. 
% For example, when $|B|\!=\!\num{90000}$, $d\!=\!\num{10000}$, and $|\mathcal{U}|\!=\!2^{32}$ (another experiment scenario in our evaluation), 
% if $f=0.1$, the number of cells in the IBF is only $\tau fd\!=\!0.2d$ (here, we assume $\tau=2$), much smaller than $2d$ that required in D.Digest. In such a configuration, 
% the communication overhead of Graphene is roughly $6.23\times 10^5$=$1.95\times d\log|\mathcal{U}|$ bits , which is even lower than that of PBS. 
% However, when $d/|B|\ll 1$ ({\it i.e.,} $|A\triangle B|\!\ll\! |A\cap B|$) that is common in most application scenarios, 
% they have similar space-efficiency, 
% because now Graphene has to use a BF that has a false positive rate close to 1 (otherwise, the 
% BF alone could incur a higher communication overhead than D.Digest). 
% For example, when $|B|\!=\!\num{99900}$, $d\!=\!100$, and $|\mathcal{U}|\!=\!2^{32}$ (one experiment scenario in our evaluation), 
% even a BF with a false 
% positive rate of $0.9$ requires $-|B|\log_2(f)/\ln2\!=\!\num{21907}$ bits, which is higher than the communication overhead of D.Digest, $6d\log|\mathcal{U}|\!=\!\num{19200}$ bits. 
% As $d$ gets larger, Graphene becomes more space-efficient, as now a BF with low false positive rate is affordable and 
% thus it can help reduce number of cells in the IBF significantly. 
% For example, when $|B|\!=\!\num{90000}$, $d\!=\!\num{10000}$, and $|\mathcal{U}|\!=\!2^{32}$ (another experiment scenario in our evaluation), 
% if $f=0.1$, the number of cells in the IBF is only $\tau fd\!=\!0.2d$ (here, we assume $\tau=2$), much smaller than $2d$ that required in D.Digest. In such a configuration, 
% the communication overhead of Graphene is roughly $6.23\times 10^5$=$1.95\times d\log|\mathcal{U}|$ bits , which is even lower than that of PBS.  
%
% Therefore, Graphene is more suitable to be used in the application scenarios where $d$ is relatively large when compared with $|A\cap B|$, 
%
% Therefore, Graphene is also not as space-efficient as PBS in such scenarios. 
% As observed in our experiments in~\autoref{sec:evaluation}, the false positive rates  
% are very close to 1 in such scenarios. Therefore, Graphene is also not as space-efficient as PBS in such scenarios. 

% +++{\bf We can only beat Graphene when $|A\triangle B|\ll |A\cup B|$}

% \begin{table}
% \centering
% \caption{Summary of set reconciliation algorithms.}\label{tab:sum-recon}
% \setlength{\tabcolsep}{2pt}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{@{}|l|c|c|@{}}  
% \hline
% Algorithms & \shortstack{Decoding computational complexity} & \# of rounds \\ 
% \hline %\hline
% PinSketch & $O(d^2)$ GF($2^{32}$) ops & 1 \\ \hline
% D.Digest & O(d) & 1\\ \hline
% Graphene & $O(|A|\!+\!|B|)$ & 1 or 2 \\ \hline 
% PBS & $O(d)$ GF($2^{6}$)$\text{-to-}$GF($2^{10}$) ops & 3\\
% \hline
% \end{tabular}
% }
% \end{table}

% \autoref{tab:sum-recon} summarizes the set reconciliation algorithms that we will compare PBS with in~\autoref{sec:evaluation} 
% together with PBS. 
% The ``GF($2^{32}$) ops'' 
% stands for finite field operations in GF($2^{32}$). As explained in~\autoref{subsec:pbs-vs-pinsketch}, the ``32-bit-wide'' GF($2^{32}$) is the Galois field 
% involved in the BCH decoding in PinSketch, which is much shorter in PBS, more precisely, between ``6-bit-wide'' to ``10-bit-wide'' (GF($2^{6}$)$\text{-to-}$GF($2^{10}$)). 

% Note that \autoref{tab:sum-recon} only shows one component of the computational complexity, {\it i.e.,} decoding computational complexity. 
% Another component is encoding computational complexity, which is $O(|A|\!+\!|B|)$
% in D.Digest, Graphene and PBS, and 
% $O\big{(}d(|A|\!+\!|B|)\big{)}$ in PinSketch. 

==> section/related_work_OLD.tex <==
\section{Related Work}\label{sec:related-work}

\section{Set Reconciliation}\label{subsec:rw-set-reconciliation}



\subsubsection{Error-Correcting Codes (ECC) Based}

One family of set reconciliation algorithms~\cite{Dodis_PinSketch_2008,Minsky2003,Juels_FuzzyVaultScheme_2006,Gabrys2019} 
is based on Error-Correcting Codes (ECC)~\cite{Lin_ErrorControlCoding_1983}. 
In this family, a set $S \subseteq \mathcal{U}$ is viewed 
as a characteristic vector (binary string) $s$ in $\{0,1\}^n$, for example, $s_x=1$ for $x\in \mathcal{U}$ if 
$x\in S$; otherwise $s_x=0$. Such a representation of sets translates the set reconciliation problems into 
Error-Correcting problems in Hamming space. More precisely, under this representation, reconciling two 
sets $A$ and $B$ whose symmetric difference $D=A\Delta B$ has at most $t$ elements is equivalent to recovering 
from a corrupted binary string in $\{0,1\}^n$ where the number of errors is at most $t$. With a suitable error-correcting 
code, this family can achieve the optimal communication overhead 
$t\log (n+1)$ ({\it e.g.,}~\cite{Dodis_PinSketch_2008}). However, the encoding/decoding computational complexity 
could be polynomial in $n$, which is prohibitively high for large universe $\mathcal{U}$. Though several algorithms 
in this family mitigate this downside by proposing clever construction of the error-correcting codes that reduce the 
encoding/decoding computational complexity to the order of polynomial in $\log n$. 
For example, PinSketch~\cite{Dodis_PinSketch_2008} achieves an encoding/decoding computational complexity polynomial 
in $|S|\log n$ using a non-standard BCH codes~\cite{Dodis_SyndromeEncodingDecoding_2006} and 
the reconciliation algorithm in~\cite{Minsky2003} pushes the 
encoding/decoding computational complexity to $O(t^3)$. 
%Clearly, these schemes are still far from practical when the sizes of sets themselves and their symmetric difference are large.

\subsubsection{Bloom-Filter (BF) Based}

Another family of set reconciliation is based on Bloom filters~\cite{Bloom_Space/TimeTradeoffs_1970}. 
A Bloom filter is a space-efficient probabilistic data structure for set membership query. 
[Description of BF may not be necessary]
Given a set $S$ with $n$ elements, a Bloom filter encodes it as an bit array $B$ with $m$ cells as follows. 
For any $x \in S$, the Bloom filter uses $k$ independent hash functions to 
hash $x$ into $k$ different cells and 
set those cells to $1$. For testing the membership of a new element $y$, the Bloom filter 
uses the same $k$ hash functions to hash $y$ to $k$ distinct cells and returns ``YES'' if all those 
cells are set to $1$; otherwise, returns ``NO''. However, false positive answers are possible. 
To guarantee a false positive rate of $p$, a Bloom filer only requires $m=-\frac{n \ln p}{\ln 2}$ cells with $k=\frac{m}{n}\ln 2$. 
[ --- ]
A straightforward idea of using Bloom filter for set reconciliation is to represent set $A$ as a 
Bloom filter at host A, and then send it to host B. By querying the membership of each element in 
$B$ at host B, host B can tell which element belongs $B\setminus A$. Similarly, host 
A can tell which element belongs to $A\setminus B$. However, there are two main disadvantages. First, 
some elements belonging to $A\Delta B$ might not be found because of the false positive issue of 
Bloom filters. Second, this scheme has a communication overhead of $O(n)$, which is too high when the 
set size if large. 

To overcome the above drawbacks of Bloom filters, several extensions were made. A data structure called 
approximate reconciliation trees (ARTs) were proposed in~\cite{Byers_Informedcontentdelivery_2004} 
to extend the Bloom filter approach, which has communication cost of $O(|B|)$ and a computational 
complexity of $t\log |B|$ for recovering $A\setminus B$. A few extended Bloom filters, such as 
inevitable Bloom Filters~\cite{Goodrich_InvertibleBloomLookup_2011} and counting Bloom filters~\cite{Eppstein_StragglerIdentificationRound_2011}, 
were designed. 
In~\cite{Eppstein_WhatsDifference?Efficient_2011}, an invertiable Bloom filer (IBF) was designed for 
set reconciliation. Like Bloom filers, elements are inserted in to 
a table of $m$ cells using $k$ independent hash functions. Unlike the standard Bloom filters, the IBF has 
three fields in each cell (instead of a single bit): A {\it count} field records the number of elements 
hashed in this cell; A {\it idSum} field records the \code{XOR} sum of all the elements hashed into 
this cell; And a {\it hashSum} field records the \code{XOR} sum of the hash value of all the elements 
hashed into this cell. Besides, a subtract operation is added to support removal a whole set so that 
the symmetric difference of sets $A$ and $B$ can be recover from the \code{IBF}$_D\triangleq$\code{IBF}$_A-$
\code{IBF}$_B$ where \code{IBF}$_X$ is the IBF for set $X$. An iterative peeling decoding algorithm was 
proposed in~\cite{Eppstein_WhatsDifference?Efficient_2011} to recover elements within the set difference, by 
attractively finding pure cells, {\it i.e.,} cells whose \code{count} field is $\pm 1$ and \code{hashSum} equals 
to the hash value of its \code{idSum}, and removing them from the IBF. The iterative peeling succeeds if eventually 
all cells are empty; otherwise, it fails. It was shown in~\cite{Eppstein_WhatsDifference?Efficient_2011} roughly 
$1.5t$ cells were required to make sure that the iterative peeling algorithm succeed with a high enough probability, 
which results in a communication cost more than $3$ times of the optimal one. Note that besides the IBF, many 
other variants of Bloom filters can also be used for set reconciliation, such as counting Bloom filters~\cite{counting}, and 
Invertible Bloom Lookup Table (IBLT)~\cite{Goodrich_InvertibleBloomLookup_2011}. However, the communication cost 
is similar or even higher than that of IBFs based set reconciliation. Recently, a set reconciliation scheme,  
which uses a combination of a Bloom filter and an IBLT, was proposed in~\cite{Ozisik2019}. ...


\section{Set-Difference Size Estimation}\label{subsec:rw-set-diff-size-est}

Min-wise sketches~\cite{minwise} are commonly used to estimate set similarity, {\it i.e.,} the Jaccard similarity 
$J(A,B)\triangleq \frac{|A\cap B|}{|A \cup B |}$, which can use adapted to estimate the size of set difference $A\Delta B$. 
Min-wise sketches use the property of min-wise independent permutation: Given a min-wise 
independent permutation family $\mathcal{H}$ on the universe $\mathcal{U}$, and a permutation $\pi$ uniformly randomly selected 
from $\mathcal{H}$, then $\mathbb{P}[\min\{\pi(A)\} = \min\{\pi(B)\}]=J(A,B)$. More precisely, Min-wise sketches use $k$ random permutations 
$\pi_1,\pi_2,\cdots,\pi_k$ from a 
min-wise independent permutation family on the universe $\mathcal{U}$. Define $h_i(S)=\min\{\pi_i(S)\}$ where $S\subseteq \mathcal{U}$, then 
min-wise sketches use $\hat{r}=\frac{|\{i \in \{1,2,\cdots, k\}|h_i(A)=h_i(B)\}|}{k}$ to estimate $J(A,B)$. It is not hard to check that $\hat{t}=\frac{1-\hat{r}}{1 + \hat{r}}(|A| + |B|)$ estimates the set difference size. Besides the standard min-wise sketches described above, many more efficient variants of min-wise sketches~\cite{} are 
proposed to estimate the Jaccard similarity or the extended Jaccard similarity. However, to guarantee a high enough accuracy, the min-wise sketches and its variants 
have to use a prohibitively large $k$, which results in too high communication cost. 

Another approach based on random projection to estimate set difference is proposed in~\cite{l1}, which is designed for 
more generally L1 difference. Similar to our ToW based algorithm, it also achieves near-optimal communication 
overhead. However, it is much more complicated than our ToW based algorithm. 

By using the idea of Flajolet and Martin (FM) sketch ~\cite{}, which is an elegant way to estimate set sizes using only 
$\log |\mathcal{U}|$ bits, an invertiable Bloom filter (IBF) based strata estimator is proposed in~\cite{Eppstein_WhatsDifference?Efficient_2011}. 
The strata estimator uses $L=\log |\mathcal{U}| $ IBFs, and inserts element $s$ into the $i$-th Bloom filter if $s$ has $i$ trailing zeros. 
The strata estimator maintains a counter $c$ that is the number of all elements in the successfully decoded IBFs, 
while traversing the IBFs from the $L$-th to the first one until encountering an IBF that cannot be 
decoded successfully. If the $i$-th IBF fails to decode, the strata estimates with $c2^{i+1}$, otherwise if 
all IBFs decode successfully, it estimates with $c$. As we have shown in~\autoref{eva}, our ToW scheme has much lower communication cost when achieving 
the same accuracy. 



==> section/related_work_copy.tex <==
\section{Related Work}\label{sec:related}

In this section, we provide a brief survey of existing set reconciliation algorithms. 
% , focusing on 
% those that are not based on Error-Correction Codes (EECs), because the basic ideas of 
% EEC-based algorithms~\cite{Minsky2003,Dodis_PinSketch_2008,naumenko2019bandwidth,Karpovsky_eccreconciliation_2003} 
% are similar to that of PinSketch~\cite{Dodis_PinSketch_2008}, which we have described in detail in~\autoref{}. 
% Recall from~\autoref{sec:intro} that prior set reconciliation algorithms are mainly based on 
% either Bloom Filters (BF) or Error-Correction Codes (EEC). The basic ideas of 
% EEC-based algorithms~\cite{Minsky2003,Dodis_PinSketch_2008,naumenko2019bandwidth,Karpovsky_eccreconciliation_2003} 
% are similar to that of PinSketch~\cite{Dodis_PinSketch_2008}, which we have described in detail in~\autoref{}. 
% Hence, we only describe those are based on BFs in this section. 
As mentioned in~\autoref{sec:intro_prob_formulation}, in describing and comparing them with PBS, 
we only consider the unidirectional set reconciliation in which 
Alice learns $A\triangle B$. %in this work. 

\begin{comment}
Approximate set difference can be learned by Alice through exchanging BFs for 
sets $A$ and $B$ between Alice and Bob. Upon receiving the BF (for $B$) from Bob, 
Alice can infer ``common elements'' 
$\widehat{A\cap B}$ by querying this BF, 
from which Alice can infer $\widehat{A\setminus B}\!=\!A\setminus \widehat{A\cap B}$. Note that 
$\widehat{A\cap B}\!\supseteq\! (A\cap B)$ because of the false positive errors in BFs, and thus
$\widehat{A\setminus B}\!\subseteq\!A\setminus B$. Similarly, Bob 
can infer $\widehat{B\setminus A}$ ($\!\subseteq\!B\setminus A$) and Bob sends it to Alice, from which Alice can infer  
$\widehat{A\triangle B}\!=\!\widehat{A\setminus B}\bigcup\widehat{B\setminus A}$ ($\!\subseteq\!A\triangle B$). 
This scheme was extended by using more advanced data structures, such as Approximate Reconciliation Trees (ART) in~\cite{Byers_Informedcontentdelivery_2004}, Counting Bloom Filters (CBF) in~\cite{Guo_SetReconciliationvia_2013}, and 
Cuckoo Filters (CF)~\cite{Fan_CuckooFilterPractically_2014} in~\cite{Luo_SetReconciliationCuckoo_2019}. 
These schemes, however, have a flaw: Alice may only learn the approximate set difference, more precisely 
a subset of the set difference $A\triangle B$ 
(instead of the exact $A\triangle B$). This flaw is undesirable in most applications. 
\end{comment}

Bloom filters (BF)~\cite{Bloom_Space/TimeTradeoffs_1970} can be used to construct a crude set reconciliation scheme as follows.  
% Approximate 
% Set difference can be learned by Alice via exchanging BFs for 
% sets $A$ and $B$ between Alice and Bob. 
First, Alice and Bob exchange BFs for sets $A$ and $B$.  Upon receiving the BF (for $B$) from Bob, 
Alice can obtain an estimate, denoted as $\widehat{A\!\setminus\! B}$, of the set $A\!\setminus\! B$ 
by checking each element in $A$ against this BF. 
Note that $\widehat{A\!\setminus\! B}$ is in general an underestimate:
$\widehat{A\!\setminus\! B}$ may not contain all elements in $A\!\setminus\!B$, because this BF may produce false positives  
%% this sentence was "copied" from "Network Applications of Bloom Filters: A Survey"
that each suggests an element is in $B$ when it is not. 
Similarly, Bob can obtain $\widehat{B\!\setminus\! A}$ and sends it to Alice, from which Alice can infer an underestimate (of $A\triangle B$)
$\widehat{A\triangle B}\!=\!\widehat{A\!\setminus\! B}\bigcup\widehat{B\!\setminus\! A}$. 
% This scheme, however, has a flaw: 
%In this approach, Alice may only learn an approximate set difference, 
%more precisely a subset of the set difference $A\triangle B$ 
%(not the exact $A\triangle B$). 
Set reconciliation solutions that build on and extend this BF-based technique, including~\cite{Byers_Informedcontentdelivery_2004,Guo_SetReconciliationvia_2013,Luo_SetReconciliationCuckoo_2019},
all suffer from this underestimation problem, and hence 
% can only be used 
{\color{red}are only suitable} 
for few applications that do not require perfect data
synchronization.  


% Several 
As mentioned earlier, most exact set reconciliation algorithms
% , which focus on discovering the exact set difference, have been proposed. 
% Recall from~\autoref{sec:intro} that these algorithms are mainly 
are based on either invertible Bloom filters (IBF)~\cite{Goodrich_InvertibleBloomLookup_2011} or error-correction codes (ECC). 

\smallskip
\noindent
{\bf IBF-Based Algorithms.}
% In the following, we focus on IBF-based algorithms, since we have already described PinSketch~\cite{Dodis_PinSketch_2008} in detail
% and other ECC-based algorithms~\cite{Minsky2003,naumenko2019bandwidth,Karpovsky_eccreconciliation_2003} have similar core ideas.
%The basic ideas of 
%ECC-based algorithms~\cite{Minsky2003,Dodis_PinSketch_2008,naumenko2019bandwidth,Karpovsky_eccreconciliation_2003} 
%are similar to that of PinSketch~\cite{Dodis_PinSketch_2008}, which we have described in detail in~\autoref{subsec:pbs-vs-pinsketch}, 
%hence we will only describe the IBF-based algorithms~\cite{Eppstein_WhatsDifference?Efficient_2011,Ozisik2019} in the rest of this section. 
% Difference Digest (D.Digest)~\cite{Eppstein_WhatsDifference?Efficient_2011} is one such algorithm that based purely on IBFs. 
In an IBF, each element (from a set) is inserted into $k$ cells indexed by $k$ independent hash functions. Whereas each cell is a single 
bit in a BF, it has three fields in an IBF, each of which requires a single word of length $\log |\mathcal{U}|$. Therefore, IBFs are much more powerful than BFs: The set difference $A\triangle B$ of sets $A$ and $B$ can be recovered from the ``difference'' of their IBFs using a ``peeling process'' 
% which  
% is 
similar to that used in the decoding algorithms for some erasure-correcting codes, such as Tornado codes~\cite{luby1998tornado}.  
% However, %as shown in~\cite{Eppstein_WhatsDifference?Efficient_2011}, 
For this decoding process to succeed with a high enough probability, 
IBF-based solutions, such as 
Difference Digest (D.Digest)~\cite{Eppstein_WhatsDifference?Efficient_2011}, have to use roughly $2d$ cells.
%the number of cells need to be roughly at least $2d$. % to roughly ensure a success rate of $0.99$. 
This translates into a communication overhead of roughly $6d\log|\mathcal{U}|$, or
6 times the theoretical minimum. %of $d\log|\mathcal{U}|$. 
%In comparison, 
%PBS is much more space-efficient, whose communication overhead is roughly twice the theoretical minimum. 

%An approach of combing BFs with IBFs, called Graphene, was proposed in 

A recent solution called Graphene~\cite{Ozisik2019} reduces the high communication overhead of IBF-based solutions by augmenting it with  BFs.
% Recently, an approach, c that combines BFs and IBFs was proposed inGraphene~\cite{Ozisik2019} is another such algorithm that combines BFs and IBFs. 
Here, we only describe its simplest version (Protocol I in~\cite{Ozisik2019}) %, % of Graphene, 
% which only 
that works only for the special case of $B\!\subset\! A$. %, and which we will compare PBS with in~\autoref{sec:evaluation}. 
%
Its basic idea is for Alice to first obtain $\widehat{A\!\setminus\! B}$, an underestimate of of $A\!\setminus\! B$, by querying the BF for the set $B$ as described above, and then
recover only the ``missing" part $(A\!\setminus\! B) \!\setminus\! (\widehat{A\!\setminus\! B})$ using an IBF.   When the BF is configured to have a reasonably low false 
positive rate say $\epsilon$, 
the IBF needs only to ``encode" the roughly $\epsilon d$ ``missing" distinct elements rather than all the $d$ elements in $A\!\setminus\! B$, resulting in savings of 
``$O((1-\epsilon)d)$" in the size of IBF.    
%As a result, in this case the
%IBF in Graphene has a much smaller size than that in other IBF-based solutions.   
In general, for this $\epsilon$ to be reasonably low (say meaningfully away from $1$), 
the size of the BF has to be $O(|B|)$ with a nontrivial constant factor~\cite{Bloom_Space/TimeTradeoffs_1970}. % {\bf cite the original BF paper}.  
However, when $|B| \!\gg\! d$, which as explained earlier is often the case in most applications, 
the savings of ``$O((1\!-\!\epsilon)d)$" in the IBF size is no longer worth the $O(|B|)$ cost of the BF;
in this case Graphene drops the BF and degenerates to an IBF-only solution.    
For this reason, Graphene is more communication-efficient than other IBF-based solutions only when
$d$ is sufficiently large with respect to $|B|$.  Furthermore, this efficiency grows with $d$, as we will show 
in~\autoref{subsec:vs-graphene}.

{\color{red}
\smallskip
\noindent
{\bf ECC-Based Algorithms.}
% \input{section/pinsketch}
% [moved from Section 2.5 in the original submission]
% We will describe PinSketch~\cite{Dodis_PinSketch_2008} in detail
% and other ECC-based algorithms~\cite{Minsky2003,naumenko2019bandwidth,Karpovsky_eccreconciliation_2003} have similar core ideas.
The basic ideas of 
ECC-based algorithms~\cite{Minsky2003,Dodis_PinSketch_2008,Naumenko_ErlayEfficientTransaction_2019,Karpovsky_eccreconciliation_2003} 
are similar to that of PinSketch~\cite{Dodis_PinSketch_2008}, which we will describe in detail next. 
% As we have mentioned earlier, PinSketch~\cite{Dodis_PinSketch_2008} also uses BCH coding to ``locate the $d$ bit errors", 
% but in a different manner. 
% PinSketch~\cite{Dodis_PinSketch_2008} is an error-correction code (ECC) based set reconciliation algorithm.  
Given a universe $\mathcal{U}$ % of binary strings, %with $|\mathcal{U}|=u$, 
in which each element is assigned an index between $1$ and $|\mathcal{U}|$, 
% 
PinSketch 
% (and other ECC-based set reconciliation algorithms) represents 
encodes each set $S\!\subset \!\mathcal{U}$ as a %is viewed 
% as a characteristic vector (binary string) $s$ in $\{0,1\}^n$.  
$|\mathcal{U}|$-bit-long bitmap $S[1..|\mathcal{U}|]$: $S[i]$ (the $i^{th}$ bit of $S[1..|\mathcal{U}|]$) 
is equal to $1$ 
if the element, whose index is $i$, is contained in $S$; otherwise, $S[i]=0$. 
For example, when $|\mathcal{U}| \!=\! 2^{32}$ as assumed in most existing works, 
the bitmap encoding for any set in PinSketch is $2^{32}$ bits long.
In contrast, in PBS 
%since each bit encodes the oddness or evenness of the cardinality of a subset,   
the size $n$ of a bitmap is dependent only on $d$ (when $d$ is small) or $t$ (when $d$ is large), 
and not on the size of the universe or the cardinality of the set the bitmap encodes, and is hence much shorter.  
Using BCH coding to ``locate the $d$ bit errors" in the bitmaps for sets $A$ and $B$, PinSketch learns 
the $d$ distinct elements in $A\triangle B$.

As mentioned earlier, ECC-based algorithms suffer from a much higher decoding 
computational complexity of at least $O(d^2)$. 
Although, in~\cite{Minsky_Practicalsetreconciliation_2002}, the authors proposed a scheme that also uses the partition-based idea 
to reduce this computational complexity to $O(d)$, but in a different manner. They use an ECC-based algorithm,  
referred to as {\it BASIC-RECON}, which can 
reconcile a small constant number of distinct elements, and recursively partition sets $A$ and $B$ until each partition can 
be successfully reconciled by {\it BASIC-RECON}. However, this partition scheme requires $O(\log d)$ rounds of message 
exchanges on average, which is generally much larger than that of PBS. 
}

\begin{comment}
For example, as shown in the example in~\autoref{subsec:exception_hash_partition}, $n \!=\! 255$ is large enough for $d \!=\! 5$.  
As explained in~\ref{The BCH coding section}, the length of each BCH sub-codeword for ``locating each bit error" is the logarithm of the bitmap size.
This length is typically 3 to 4 times larger ($\log_2 |\mathcal{U}|$ = 32 bits in the example above) 
in PinSketch than in PBS ($\log_2 n = 8$ bits in the example above), a fact we will use in~\ref{evaluation subsection on partitions}. 
\end{comment}


%The basic ideas of 
%ECC-based algorithms~\cite{Minsky2003,Dodis_PinSketch_2008,naumenko2019bandwidth,Karpovsky_eccreconciliation_2003} 
%are similar to that of PinSketch~\cite{Dodis_PinSketch_2008}
\begin{comment}
{\bf\color{cyan}
% Alice sends the cardinality $|A|$ of set A to Bob, which is required by Bob during the parameterization of the BF and IBF. 
% Upon receiving $|A|$, Bob creates a BF and an IBF for set $B$ parameterized to minimize the communication overhead
Bob sends to Alice a BF for the set $B$ and an IBF for 
% , parameterized to minimize the communication overhead, to Alice. %~\footnote{The parameters for the BF and IBFs }
With this BF, 
Alice can infer $\widehat{A\setminus B}$, which, as explained earlier, 
% may not contain all elements in $A\setminus B\!=\!A\triangle B$ because 
may be missing some elements in $A\setminus B\!=\!A\triangle B$ (since $B\subset A$) due to the false positives, which  
%To discover the exact set difference $A\triangle B$, 
Alice %corrects these false positives, {\it i.e.,} 
recovers 
%these elements 
% that are not in $B$ but suggested by the BF as in $B$, 
% that are
% (elements in $A\setminus B$ but suggested by the BF as in $B$), 
% in $(A\setminus B)\setminus\widehat{A\setminus B}$,  
from the IBF received from Bob. 
The number of such elements is on average $\epsilon|A\!\setminus\!B|\!=\!\epsilon d$ when the false positive rate (FPR) is $\epsilon$, since 
each element in $A\!\setminus\!B$ will be mistakenly determined by the BF as in $B$ with probability $\epsilon$. 
Therefore, when $\epsilon\!<\!1$, the number of IBF cells in Graphene is 
less than that required by IBF-only solutions ({\it e.g.,} D.Digest). 
The space saving compared to IBF-only solutions, is however not enough for compensating for the overhead of the BF when $d\!\ll\! |B|$, since
the space overhead of BF is proportional to $|B|$. 
For this reason, Graphene uses only an IBF 
when $d\!\ll\! |B|$. 
}

%, or in other words, $|A\triangle B|\!\ll\! |A\cap B|$ (since $B\subset A$) that is usual in most applications. 
% Graphene uses the optimal FPR, including the FPR of $1$ that corresponds to using the IBF only, to minimize its communication overhead. 
% % Note that an FPR of $1$ in Graphene corresponds to using the IBF only. 
% Therefore, Graphene is at least as space-efficient as IBF-based solutions. %solutions that use IBFs only. 
% However, as we will elaborate next, Graphene is generally less computationally-efficient that IBF-based solutions.    
% We note that when $d\ll |B|$  ({\it i.e.,} $|A\triangle B|\!\ll\! |A\cap B|$) that is common in most application scenarios, 
% the optimal FPR is generally $1$.



{\bf\color{cyan}
The communication overhead of PBS is between 2.21 to 2.75 times the theoretical minimum, which is higher than that in~\autoref{fig:co-99} 
as the target success rate here is higher. 
Unlike in other algorithms, in Graphene, the average amount of 
communication per distinct element 
% varies significantly as $d$ changes and %as shown in~\autoref{fig:co-9958}, 
% it 
decreases as $d$ increases. %which we have explained in~\autoref{sec:related}. 
Our explanation for this phenomenon is as follows.  
On one hand, as shown in~\cite{Ozisik2019}, given a success rate the size (space) of an IBF is roughly proportional to the number of 
distinct elements that need to be recovered from the IBF, which is $d$ when the BF is not used by Graphene.  
With a slight abuse of notation, we call this size ``$O(d)$".   
As explained in~\autoref{sec:related}, when $d$ is large enough, the BF starts to be used, 
producing a low FPR, say $\epsilon$.   In this case, only $\epsilon\cdot d$ elements needs to be recovered from
the IBF, so the size of the IBF becomes ``$O(\epsilon d)$", resulting in a savings of ``$O(1 - \epsilon)$" per distinct element.
On the other hand, the overhead of the BF is proportional to $|B|$, which is roughly a fixed cost, so the BF cost per distinct element 
decreases when $d$ increases.  
Therefore, the overall 
per-distinct-element overhead, including those of both the IBF and the BF, decreases as $d$ gets larger. 
}


{\bf\color{cyan}
We note that Graphene requires one more round to transmit an additional BF and a second IBF between Alice and Bob in the cases where $B\not\subset A$. 
{\bf OLD) } The number of such elements $d'$ (a random number) is on average $f|A\setminus B|\!=\!fd$, 
where $f$ is the false positive rate of the BF received from Bob. 
The total communication overhead of Graphene, therefore, is roughly 
$T(f)\!\triangleq\!-|B|\log_2(f)/\ln2\!+\!\tau fd\cdot 3\log|\mathcal{U}|$, 
where $\tau$ is the ``safety margin'' to account for both the randomness of $d'$ and the IBF decoding. 
The first term is the space for the BF and the second is that for the IBF.   
The value of $f$ that minimizes the communication overhead $T(f)$ is used in Graphene. 
% {\bf Here, I want to say that the results (for Graphene) we will show in the evaluation are just visualization of the minimum 
% $T(f)$ ({\it w.r.t.} $d$ and $\log|\mathcal{U}|$).} 
It is not hard to check 
the optimal value of $f$ is $f^*\!=\!\min\{1,|B|/(dC)\}$, where $C\!=\!3(\ln2)^2\tau\log|\mathcal{U}|$. 
We note that Graphene reduces to a pure IBF-based solution when $f^*\!=\!1$ and thus it  
has roughly the same communication overhead as D.Digest.  
When $f^*\!=\!|B|/(dC)\!<\!1$ ($d$ is relatively large), Graphene is more space-efficient 
than D.Digest as now $T(f^*)<T(1)$. %, which roughly corresponds to the communication overhead of D.Digest. 
In addition, It is easy to verify that, when $|A|$ is fixed, the overhead per distinct element $T(f^*)/(d\log|\mathcal{U}|)$, 
viewing as a function of $d$, is a decreasing function in this scenario ($f^*<1$). 
However, when $d\ll |B|$  ({\it i.e.,} $|A\triangle B|\!\ll\! |A\cap B|$) that is common in most application scenarios, 
we have $|B|/(dC)\!>\!1$, thus $f^*=1$ (Graphene reduces to a pure IBF-based solution).  
Therefore, Graphene is much less space-efficient as PBS when $|A\triangle B|\!\ll\! |A\cap B|$.
}

\end{comment}

% It was shown in~\cite{Gabrys2019} that Graphene is generally more space-efficient than D.Digest.
% schemes based purely on BFs or IBFs.  
% However,
% Graphene minimizes this communication overhead by optimally adjusting the space allocated to the BF and the IBF. 
% Roughly speaking, 
% 1000	1400	2000	4000	8000	10000
% 6	5.81711186092606	5.20341025080952	3.66281764169970	2.30540290045341	1.94771937332281
% 1	0.763478353895658	0.531182708694140	0.260171122625701	0.124665329591482	0.0975641709846379
% When $d/|B|$ is relatively large, the BF can have relatively low false positive rate and 
% thus it can help reduce number of cells in the IBF significantly. 
% For example, when $|B|\!=\!\num{90000}$, $d\!=\!\num{10000}$, and $|\mathcal{U}|\!=\!2^{32}$ (another experiment scenario in our evaluation), 
% if $f=0.1$, the number of cells in the IBF is only $\tau fd\!=\!0.2d$ (here, we assume $\tau=2$), much smaller than $2d$ that required in D.Digest. In such a configuration, 
% the communication overhead of Graphene is roughly $6.23\times 10^5$=$1.95\times d\log|\mathcal{U}|$ bits , which is even lower than that of PBS. 
% However, when $d/|B|\ll 1$ ({\it i.e.,} $|A\triangle B|\!\ll\! |A\cap B|$) that is common in most application scenarios, 
% they have similar space-efficiency, 
% because now Graphene has to use a BF that has a false positive rate close to 1 (otherwise, the 
% BF alone could incur a higher communication overhead than D.Digest). 
% For example, when $|B|\!=\!\num{99900}$, $d\!=\!100$, and $|\mathcal{U}|\!=\!2^{32}$ (one experiment scenario in our evaluation), 
% even a BF with a false 
% positive rate of $0.9$ requires $-|B|\log_2(f)/\ln2\!=\!\num{21907}$ bits, which is higher than the communication overhead of D.Digest, $6d\log|\mathcal{U}|\!=\!\num{19200}$ bits. 
% As $d$ gets larger, Graphene becomes more space-efficient, as now a BF with low false positive rate is affordable and 
% thus it can help reduce number of cells in the IBF significantly. 
% For example, when $|B|\!=\!\num{90000}$, $d\!=\!\num{10000}$, and $|\mathcal{U}|\!=\!2^{32}$ (another experiment scenario in our evaluation), 
% if $f=0.1$, the number of cells in the IBF is only $\tau fd\!=\!0.2d$ (here, we assume $\tau=2$), much smaller than $2d$ that required in D.Digest. In such a configuration, 
% the communication overhead of Graphene is roughly $6.23\times 10^5$=$1.95\times d\log|\mathcal{U}|$ bits , which is even lower than that of PBS.  
%
% Therefore, Graphene is more suitable to be used in the application scenarios where $d$ is relatively large when compared with $|A\cap B|$, 
%
% Therefore, Graphene is also not as space-efficient as PBS in such scenarios. 
% As observed in our experiments in~\autoref{sec:evaluation}, the false positive rates  
% are very close to 1 in such scenarios. Therefore, Graphene is also not as space-efficient as PBS in such scenarios. 

% +++{\bf We can only beat Graphene when $|A\triangle B|\ll |A\cup B|$}

% \begin{table}
% \centering
% \caption{Summary of set reconciliation algorithms.}\label{tab:sum-recon}
% \setlength{\tabcolsep}{2pt}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{@{}|l|c|c|@{}}  
% \hline
% Algorithms & \shortstack{Decoding computational complexity} & \# of rounds \\ 
% \hline %\hline
% PinSketch & $O(d^2)$ GF($2^{32}$) ops & 1 \\ \hline
% D.Digest & O(d) & 1\\ \hline
% Graphene & $O(|A|\!+\!|B|)$ & 1 or 2 \\ \hline 
% PBS & $O(d)$ GF($2^{6}$)$\text{-to-}$GF($2^{10}$) ops & 3\\
% \hline
% \end{tabular}
% }
% \end{table}

% \autoref{tab:sum-recon} summarizes the set reconciliation algorithms that we will compare PBS with in~\autoref{sec:evaluation} 
% together with PBS. 
% The ``GF($2^{32}$) ops'' 
% stands for finite field operations in GF($2^{32}$). As explained in~\autoref{subsec:pbs-vs-pinsketch}, the ``32-bit-wide'' GF($2^{32}$) is the Galois field 
% involved in the BCH decoding in PinSketch, which is much shorter in PBS, more precisely, between ``6-bit-wide'' to ``10-bit-wide'' (GF($2^{6}$)$\text{-to-}$GF($2^{10}$)). 

% Note that \autoref{tab:sum-recon} only shows one component of the computational complexity, {\it i.e.,} decoding computational complexity. 
% Another component is encoding computational complexity, which is $O(|A|\!+\!|B|)$
% in D.Digest, Graphene and PBS, and 
% $O\big{(}d(|A|\!+\!|B|)\big{)}$ in PinSketch. 

==> section/schemes.tex <==
\section{Set Reconciliation}\label{sec:scheme}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%     Writing Guideline for This Section     %%%%%%%%%%
% “balls – elements in the symmetric difference of the two sets” 

% Protocol 0 (reconcile two sets whose set difference has at most one ball)

% Protocol I.I (partition elements into a sufficiently large number of subsets such that each subset has at most one ball with high probability and use Protocol 0 to reconcile each of them) 

% Protocol I.II (a two-step refinement of Protocol I.I: first use BCH to identify good bins, i.e., bins/subsets have exactly one ball, and then use Protocol 0 to reconcile each good bin) 

% Protocol II (a two-layer refinement of Protocol I.II: in the first layer, we partition elements into t/c subsets, where t is the size of set difference and c is a small constant, then each subset has c balls on average. In the second layer, we further partition each subset into large enough number of bins/subsets such that with high probability each bin has at most one ball, then use Protocol I.II to reconcile them one by one) 

% Protocol III/IV (mainly fix certain exceptions in Protocol II，e.g., how to address bad bins, how to handle the cases where BCH fails to decode and etc)

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this section, we will describe our set reconciliation scheme in detail. In \autoref{subsec:protocol0}, we introduce a basic scheme for the trivial case, in which the two sets $A$ and $B$ has at most one distinct element. In \autoref{subsec:protocol1}, we build upon the basic scheme and propose a strawman scheme for general cases (i.e., any arbitrary number of distinct elements). In \autoref{subsec:protocol2}, we propose our scheme, which is based on the strawman scheme. And \autoref{subsec:exceptions} describes the exception handling in our scheme.

We assume the total number of distinct elements is known in advance throughout this section except in \autoref{subsec:ToW}, in which we will describe how to handle the cases that the set difference size is not known as a priori. 

\subsection{The Trivial Case: $|A\Delta B|\leq 1$}\label{subsec:protocol0}

\begin{comment}
Start with the trivial case, in which Set $A$ and Set $B$ have at most one exclusive element (i.e., $|A\Delta B|\leq 1$), we have a simple set reconciliation scheme showed in \autoref{alg:trivial_case}:

\begin{algorithm}
\caption{Set reconciliation when $|A\Delta B|\le 1$}
\label{alg:trivial_case}

{\it Host A}: Calculate $s_A\triangleq\oplus_{a\in A} a$, then send $s_A$ to Host B\; \label{alg1:sender}

{\it Host B}: Calculate $s_B\triangleq\oplus_{b\in B} b$ and $d\triangleq s_A \oplus s_B$\; \label{alg1:receiver}
\end{algorithm}

Firstly, Host $A$ calculates the \code{XOR} sum $s_A$ of Set $A$ and send it to Host $B$. Then Host $B$ also calculates the \code{XOR} sum $s_B$ of Set $B$ and then computes $d\triangleq s_A \oplus s_B$. The set difference $A\Delta B$ is simply:

\begin{equation}\label{eq:xor_setiff}
    A\Delta B = \begin{cases} \quad\{d\} & \mbox{ if } d\neq 0,\\
    \hspace{1.5em}\emptyset & \mbox{ otherwise }\\
    \end{cases}
\end{equation}

Note that \autoref{eq:xor_setiff} holds if and only if $|A\Delta B|\leq 1$. Hence \autoref{alg:trivial_case} cannot be directly used to reconcile two general sets (e.g., $|A\Delta B|>1$).
\end{comment}

Start with the trivial case, in which $A$ and $B$ has at most one distinct element ({\it i.e.,} $|A\Delta B|\leq 1$), 
we have a simple set reconciliation scheme showed in \autoref{alg:trivial_case}:

\begin{algorithm}
\caption{Set reconciliation when $|A\Delta B|\le 1$}
\label{alg:trivial_case}

{\it Alice}: Calculate $s_A\triangleq\oplus_{a\in A} a$, then send $s_A$ to Bob\; \label{alg1:sender}

{\it Bob}: Calculate $s_B\triangleq\oplus_{b\in B} b$ and $s\triangleq s_A \oplus s_B$\; \label{alg1:receiver}
\end{algorithm}

First, Alice calculates the \code{XOR} sum $s_A$ of $A$ and send it to Bob. 
Bob also calculates the \code{XOR} sum $s_B$ of $B$ and 
upon receiving $s_A$ Bob computes $s\!\triangleq\! s_A \!\oplus\! s_B$. 
The set difference $A\Delta B\!=\!\{s\}$ if $s\neq 0$; Otherwise $A\Delta B=\emptyset$.

% \begin{equation}\label{eq:xor_setiff}
%     A\Delta B = \begin{cases}\{d\} & \mbox{ if } d\neq 0,\\
%     \quad\emptyset & \mbox{ otherwise. }\\
%     \end{cases}
% \end{equation}

Note that %\autoref{eq:xor_setiff} holds 
\autoref{alg:trivial_case} works 
if and only if $|A\Delta B|\!\leq\! 1$ and 
$0\!\notin\! (A\!\cup\! B)$ (which we have explained in~\autoref{sec:model}). 
% Hence \autoref{alg:trivial_case} cannot be directly used to reconcile two general sets (e.g., $|A\Delta B|>1$).

\subsection{Strawman Scheme}\label{subsec:protocol1} 

\begin{comment}
To reconcile two sets $A$ and $B$ in general ({\it i.e.}, $|A\Delta B|> 1$), we have a naive set reconciliation approach based on \autoref{alg:trivial_case} that works as follows: Firstly, We use a hash-function based random partition algorithm, whose pseudocode is shown in \autoref{alg:random-part}, to coordinately partition $A$ and $B$ into $m$ subsets (say $A_1,A_2,...,A_m$ and $B_1,B_2,...,B_m$ for some $m$) and ``hopefully'' the each subset pair $(A_i, B_i)$ has at most one exclusive element:

\begin{equation}\label{eq:requirement_strawman}
    |A_i\Delta B_i|\leq 1 \mbox{ for } \forall i=1,2,...,m
\end{equation}
\end{comment}

For general cases ({\it i.e.,} $|A\Delta B|$ is an arbitrary number), we have a straightforward reconciliation approach building upon~\autoref{alg:trivial_case}, which works as follows: First, we coordinately partition $A$ and $B$ into $m$ subsets ($A_1,A_2,\cdots,A_m$ and $B_1,B_2,\cdots,B_m$) and ``hopefully'' each subset pair $(A_i, B_i)$ contains at most one distinct element ({\it i.e.,} $|A_i\Delta B_i|\!\leq\!1$). Then we reconcile each subset pair and obtain $A_i\Delta B_i$ for $i=1,2,\cdots,m$ using~\autoref{alg:trivial_case}. The overall set difference $A\Delta B$ is simply their union ({\it i.e.,} $\bigcup A_i\Delta B_i$).

we construct a hash function $h: A\cup B \rightarrow \{1,2,\cdots,m\}$ 
The hash-partition in the first step can be done by hashing the elements in $A\cup B$ into $\{1,2,\cdots,m\}$. 


A straightforward strawman scheme building upon~\autoref{alg:trivial_case} 
to reconcile two sets $A$ and $B$ in general 
({\it i.e.,} $|A\Delta B|$ is an arbitrary number) is as follows: 
Uniformly randomly partition $A$ and $B$ into $m$ subsets ($A_1,A_2,\cdots,A_m$ 
and $B_1,B_2,\cdots,B_m$) so that the set difference 
$A_i\Delta B_i$ of each subset pair $(A_i, B_i)$ contains at most one element 
({\it i.e.,} $|A_i\Delta B_i|\!\leq\!1$) {\it w.h.p.} ({\it i.e.,} with high probability), 
and then reconcile each subset pair by~\autoref{alg:trivial_case}. 

Now let us analyze this strawman scheme using the {\it balls-into-bins model}. 
Assume that sets $A$ and $B$ have $t$ elements in their set difference, {\it i.e.,} $|A\Delta B|\!=\!t$. 
These $t$ elements can be viewed as $t$ balls and the $m$ partitions (subset pairs) can be viewed as 
$m$ bins. The random partition process in this strawman scheme can be modeled as throwing 
$t$ balls into $m$ bins in the following manner: Each ball goes into a 
uniformly random bin and independently of other balls. %so that each bin contains at most one ball, {\it w.h.p.}  
The probability that each bin contains at most one ball is  
$\frac{m\,!}{(m-t)\,!m^t}\!=\!\prod_{k=1}^{t - 1}(1 - \frac{k}{m})\!\approx\! e^{-\frac{t(t-1)}{2m}}$. 
Hence, at least $\lceil \frac{t(t-1)}{-2\ln p}\rceil$ bins are required 
to ensure that this probability is at least $p$. In other words, to ensure 
that each bin contains at most one ball with a probability of $p$, 
the strawman scheme roughly requires $m \!=\!\lceil \frac{t(t-1)}{-2\ln p}\rceil$. 
For example, suppose $t\!=\!$\num{1000}, %and $p\!=\!0.01$, 
this scheme roughly requires $m\!=\!$\num{108469} bins (partitions) to 
ensure that $|A_i\Delta B_i|\!\leq\!1$ (for any $i=1,2,\cdots,m$) holds with probability $0.01$.  

We note that the communication overhead of this strawman scheme is proportional to 
$m$ ($\!\gg\! t$), as each partition (subset pair) requires communication of an \code{XOR} sum during the reconciliation. 
This communication overhead is much higher than that of the optimal scheme, which only requires 
to exchange the elements in the set difference (assuming an oracle tells it which elements belong to 
the set difference), {\it i.e.,} proportional to $t$. In the example above, assuming each element takes 4 bytes, 
the communication overhead of the strawman scheme is $4m$ bytes ($\!\approx\! \num{423.71}\,$KB) to ensure 
a success rate of only 0.01 ({\it i.e.,} with a probability of $0.0.1$, all elements in 
the set difference are successfully reconciled), 
which is approximately 2 orders of magnitude higher than $4t$ bytes ($\!=\!\num{3.90}\,$KB), the communication 
overhead of the optimal scheme. 

% Such a scheme, however, has two major drawbacks. On one hand, to ensure {\it w.h.p.} $|A_i\Delta B_i|\!\leq\!1$ 
% for $i=1,2,\cdots,m$, it requires $m$ to be extremely large: 
% Given two sets $A$, $B$ with $t$ elements in their set difference 
% $A\Delta B$ ({\it i.e.,} $|A\Delta B|\!=\!t$), assuming each element is uniformly and randomly assigned into $m$ subsets, the probability that every subset pair has at most one element in its set difference is $\frac{m\,!}{(m-t)\,!m^t}\!=\!\prod_{k=1}^{t - 1}(1 - \frac{k}{m})\!\approx\! e^{-\frac{t(t-1)}{2m}}$. It is not hard to check at least $\lceil \frac{t(t-1)}{-2\ln p}\rceil$ subsets are required to make sure that this probability is at least $p$. For example, suppose $t=$1,000 (size of set difference), $p=0.01$ (probability of success), we require at least $m=$108,469 subsets to ensure that \autoref{eq:requirement_strawman} holds with $1\%$ probability. 


% First, Alice partitions $A$ into 
% $m$ subsets in a random manner: Each element $x\in A$ goes into a uniformly random subset, independent 
% of other elements, which implies that the probability that an element belongs to the set difference $A\Delta B$ goes into 
% any subset is $1/m$. 

\IncMargin{1em}
\begin{algorithm}
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
\Input{Set $S$}
\Input{The number of subsets $m$ for partition}
\Output{Subsets $S_1, S_2, ..., S_m$}

Generate hash function $h(\cdot)$ that maps each element into $\{1,2,...,m\}$;

\ForEach{$s \in S$}{
    $j\leftarrow h(s) \bmod m$\;    
    Insert $s$ into the $j$-th subset $S_j$\;
}

\caption{Random partition using hash function} \label{alg:random-part}
\end{algorithm}\DecMargin{1em}

% \IncMargin{1em}
% \begin{algorithm}
% \SetKwProg{Proc}{Procedure}{}{}
% \Proc{RandomPartition(S, m)}{
%     \ForEach{$s \in S$}{
%     $j\leftarrow h(s) \bmod m$\;
    
%     Insert $s$ into the $j$-th subset/partition $S_j$\;
%     }
    
%     \Return All partitions $S_1,S_2,...,S_m$\;
% }

% \caption{Random partition using hash function $h$}\label{alg:random-part}
% \end{algorithm}\DecMargin{1em}

Secondly, we reconcile each subset pair to get $A_i\Delta B_i$ for $\forall i=1,2,...,m$ using \autoref{alg:trivial_case}; Thirdly, we obtain the set difference $A\Delta B$ as the union of the set differences between each subset pair:

\begin{equation}
    A\Delta B=\bigcup_{i=1}^m \big{(}A_i\Delta B_i\big{)}
\end{equation}

Partitioning elements into subsets in \autoref{alg:random-part} can be viewed as a Balls-into-Bins problem, in which elements are balls and subsets are bins. Each element is uniformly and randomly inserted into one of the subsets. We consider the exclusive elements are ``bad'' balls and other elements are ``good'' balls. The requirement in \autoref{eq:requirement_strawman} means each bin contains at most 1 ``bad'' ball. We will use the ball-into-bins model to analyze performance theoretically in \autoref{sec:tail_bound}

Note that this naive approach works correctly if and only if each subset pair has at most one exclusive element (i.e., \autoref{eq:requirement_strawman} holds). However, this requirement in general is difficult to meet unless the number of subset $m$ is extremely large: Given two sets $A$, $B$ with $t\triangleq |A\Delta B|$ exclusive elements, assuming each element is uniformly and randomly assigned into $m$ subsets, the probability that every subset pair has at most one element in its set difference is $\frac{m\,!}{(m-t)\,!m^t}\!=\!\prod_{k=1}^{t - 1}(1 - \frac{k}{m})\!\approx\! e^{-\frac{t(t-1)}{2m}}$. It is not hard to check at least $\lceil \frac{t(t-1)}{-2\ln p}\rceil$ subsets are required to make sure that this probability is at least $p$. For example, suppose $t=$1,000 (size of set difference), $p=0.01$ (probability of success), we require at least $m=$108,469 subsets to ensure that \autoref{eq:requirement_strawman} holds with $1\%$ probability.

Even if $m$ is sufficiently large and then ``luckily'' ensures \autoref{eq:requirement_strawman}. This straw-man scheme still suffers a high communication overhead: Note that each subset needs to be reconciled by \autoref{alg:trivial_case}, which requires a communication overhead of an \code{XOR} sum. So the overall communication overhead is proportional to $m$ and could be huge if $m$ is. Use the same example above, suppose each \code{XOR} sum is $256$ bits, then the total communication overhead is $256\times$108,469 bits$\approx 3.47$MB. Note that in this example, among the total 108,469 subset pairs, only 1,000 subset pairs have set differences (one element between each subset pair) and need to reconcile, while the rest 107,469 subset pairs are not. If we can identify these 1,000 ``target'' subset pairs and only reconcile them by \autoref{alg:trivial_case}, the total communication overhead will be significantly reduced to $256\times$1,000 bit=32KB, which is approximately 2 orders of magnitude smaller than before.

\subsubsection{Detect ``target'' subsets by Odevity Coding}

In fact, identifying the ``target'' subset pairs is simple when \autoref{eq:requirement_strawman} holds. In this case, a subset pair needs to reconcile if and only if the two subsets differ exactly one element. Based on this property, we encode each subset into 1 bit, which indicates the odevity of its size: a subset is encoded as 1 if the size of subset is odd, and as 0 otherwise. Using this {\bf odevity coding}, the code words (bits) of a subset pair will be different if its set difference has 1 element and needs to reconcile.

More specific, let $b_A$ and $b_B$ denote the odevity bitstrings (i.e., the concatenation of the odevity code words (bits) of the $m$ subsets) of Set $A$ and $B$. As we discussed, $b_A$ and $b_B$ are two bitstrings with length $m$, and they differ at $s$ bits (i.e., Hamming distance is $t$), which correspond to the $t$ ``target'' subsets. A straightforward approach to find ``target'' subsets is to let Host $A$ send $b_A$ to Host $B$, then Host $B$ compares $b_A$ to $b_B$ to get the subsets.

This straightforward approach has much space to improve, since its communication overhead is unnecessarily large. As we discussed before, $t$ is usually much smaller than $m$ to make \autoref{eq:requirement_strawman} happen. That means $b_A$ and $b_B$ have much more in common than differences. Therefore, we can view $b_B$ as a corrupted message of $b_A$ from Host $A$ to Host $B$ with $t$ corrupted bits. To detect the corrupted bits, we can use Error-Correction Codes (ECC)~\cite{Lin_ErrorControlCoding_1983} to encode $b_A$ and send the code word instead of the original bitstring. Note that the ECC code word is usually much shorter than the original bitstring: Using the same example ($m=108,469$ and $t=1,000$), if we use BCH codes~\cite{Lint_IntroductionCodingTheory_1998} as the ECC method, the code word will be $t\log m\approx 11,000$ bits, which is approximately 10 times shorter than the original bitstring.

\subsubsection{Extension from single-round to multi-round}\label{sec:multiround}

As we mentioned, this straw-man protocol works correctly if each subset pair has at most one exclusive element (i.e., \autoref{eq:requirement_strawman} holds). On the other hand, if a subset pair has more than one exclusive elements, some of which will not be successfully reconciled:

\begin{itemize}
\item If a subset pair has even number of exclusive elements, Odevity coding will encode it as 0. Then the straw-man scheme will consider the subset pair having no exclusive element and all exclusive elements in this subset will not be reconciled;

\item If a subset pair has odd number ($\geq 3$) of exclusive elements, Odevity coding will encode it as 1 and consider the subset pair having only 1 exclusive element. Then the straw-man scheme will use \autoref{alg:trivial_case} to decode only one exclusive element and dismiss all others. Even worse, the only decoded element is probably not a real exclusive element, since the element computed by \autoref{alg:trivial_case} is the \code{XOR} sum of all exclusive elements, not one of them. 
\end{itemize}

In summary, if a subset pair has more than one exclusive elements, most of its exclusive elements cannot be reconciled, and the reconciled element is usually incorrect (i.e., false-positive). The false-positive however is easy to check, which will be elaborated in \autoref{subsec:exceptions}. The good thing is, even if not all subset pairs have at most one exclusive element and are successfully decoded, most of them will be w.h.p.. In other words, even if the straw-man protocol cannot reconcile all exclusive elements, it still can reconcile most of them. To reconcile all exclusive elements w.h.p., we can simply extend the single-round straw-man scheme to multi-round. And each round adapts the straw-man scheme to do set reconciliation using independent hashing functions $h(\cdot)$ for partition (i.e., in \autoref{alg:random-part}). This multi-round extension can significantly increase the probability of a successful reconciliation, which will be elaborated in \autoref{sec:tail_bound}. 

\subsection{Our Scheme}\label{subsec:protocol2}

This straw-man scheme still has a problem on decoding computational complexity. More specific, the complexity increases dramatically with the total number of corrupted bits $t$. Therefore, when $t$ is moderate or large, the decoding computational complexity could be very high. For instance, the decoding complexity of BCH codes~\cite{Lint_IntroductionCodingTheory_1998} is $O(t^3)$, which could be quite high for a large $t$. To keep the decoding complexity reasonably low, we design the following two-layer protocol: In the first layer, we use a hash function to partition the two sets into $\lceil\frac{t}{c}\rceil$ subsets for some small constant $c$ (say $5$), just like the first step of our straw-man scheme. The objective, which is however different from before, is to make each subset pair contains roughly $c$ exclusive elements on average. In the second layer, we use the straw-man scheme with the same configuration (number of subsets $m$, and error-correction capability $\tau$, number of rounds $r$) to reconcile each subset pair. 

% In fact, the straw-man scheme is a proper solution when $t$ is small. First, the decoding complexity will not be a problem for a small $t$; Second, we do not need an extremely large $m$ to guarantee \autoref{eq:requirement_strawman} w.h.p.. For instance, when $t=5$ and $m=1024$, \autoref{eq:requirement_strawman} holds with probability $\frac{m\,!}{(m-t)\,!m^t}\approx 99\%$. This motivates us to design the following two-layer protocol: In the first layer, we use a hash function to partition the two sets into $\lceil\frac{t}{c}\rceil$ subsets for some small constant $c$ (say $5$), just like the first step of our straw-man scheme. The objective, which is however different from before, is to make each subset pair contains roughly $c$ exclusive elements on average. In the second layer, we use the straw-man scheme with the same configuration (number of subsets $m$, and error-correction capability $\tau$) to reconcile each subset pair. 

\autoref{proto:II} shows the pseudocode of our scheme. It first uses the same hash-function based random partition algorithm as \autoref{alg:random-part} to partition elements into $k\triangleq\lceil \frac{t}{c} \rceil$ subsets. Note that the random partition only guarantees that each such subset 
contains $c$ exclusive elements on average, and the exact number is not known. Hence, our scheme uses a BCH code with a capability of 
correcting up to $\tau$ errors with $\tau > c$ to make sure that the BCH code has a high probability to decode successfully. We will describe how to deal with situation where the size of set difference exceeds $\tau$ later in~\autoref{subsec:exceptions}.

As the decoding of a $\tau$-error-correcting BCH code where $\tau$ is a small constant has a constant-time computational complexity, the decoding complexity of 
our scheme is $O(k)=O(t)$. We now have several parameters, average number of exclusive elements in each subset $c$, the correcting capability $\tau$ of BCH code, the number of smaller subsets $m$ for each subset to be divided to, and the number of rounds $r$. How to tune these parameters to achieve favorable performance will be detailed later in~\autoref{sec:tail_bound}. 

\IncMargin{1em}
\begin{algorithm}
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
\Input{Size of set difference $t$}
\Input{The number of subsets $m$ for each partition}
\Input{Average number of exclusive elements in each partition $c$}
\Input{BCH code capability $\tau$}

$k \leftarrow \lceil \frac{t}{c}\rceil $\;

Partition elements into $k$ subsets using~\autoref{alg:random-part}\;

\For{$j = 0$ \KwTo $k-1$}{
    Reconcile the $j$-th subset pair using the straw-man scheme with the BCH correcting capability $\tau$, number of smaller subsets $m$, and number of rounds $r$\;
}

\caption{Our Scheme} \label{proto:II}
\end{algorithm}\DecMargin{1em}


\subsection{Exceptional Handling}\label{subsec:exceptions}

In this section, we will elaborate how to handle the following two types of exceptions that we mentioned in \autoref{sec:multiround} and \autoref{subsec:protocol2}:
\begin{itemize}
    \item Exception 1: A subset pair has odd number ($\geq 3$) of exclusive elements and causes false-positives (i.e., a decoded exclusive element is not a real exclus);
    \item Exception 2: A subset pair contains too many exclusive elements, such that a BCH code with capability of correcting up to $\tau$ errors cannot decode it (i.e., $t>\tau$).
\end{itemize}

To handle Exception 1, we need to check whether a computed exclusive element by \autoref{alg:trivial_case} is a real exclusive element or not. It can be easily done at the end of set reconciliation, during which two hosts exchange their exclusive elements. In fact, as we will elaborate in \autoref{sec:tail_bound}, Exception 1 hardly happens if we set parameters properly. 

On the other hand, when Exception 2 happens, the BCH decoder will report a failure about exceeding the error-correction capability. For such a subset pair, we can use the same approach as in \autoref{subsec:protocol2} to partition it into smaller subsets and use the straw-man scheme to reconcile them respectively. We set the number of small subsets to be 3. It is because, as we will elaborate in \autoref{sec:tail_bound}, the number of exclusive elements for each subset pair $t$ should be, if not smaller, only slightly larger than $\tau$ w.h.p.. Partitioning those exclusive elements into 3 small subsets is enough to guarentee that each of them has less than $\tau$ exclusive elements.












%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% old version

\begin{comment}

In this section, we assume that the size of the symmetric difference is known in advance. We 
will construct an accurate estimator later in \autoref{} and describe how we can use this estimator to handle the cases where the set difference size is not known as a priori.


The core design guideline of our scheme is the following fact: {\it Reconciling two sets whose set 
difference has at most one element is trivial}.  
\autoref{alg:algorithm-0} shows a simple algorithm for set reconciliation in such a scenario, 
i.e., sets $A$ and $B$ have a set difference of $D\triangleq A\Delta B$ such that $|D|\le 1$. 
Host A calculates the \code{XOR} sum $s_A$ of all elements in $A$ and send $s$ to Host 
B (\autoref{alg1:sender}). Host B also calculates the \code{XOR} sum $s_B$, and 
then computes $d=s_A\oplus s_B$. It is easy to check that $D=\{d\}$ if 
$d\neq 0$; otherwise $D=\emptyset$.

\begin{algorithm}
\caption{Set reconciliation with $|A\Delta B|\le 1$}
\label{alg:algorithm-0}

{\it Host A}: Calculate the ``exclusive-or sum'' $s_A=\oplus_{a\in A} a$ and set $s_A$\; \label{alg1:sender}

{\it Host B}: Calculate $s_B=\oplus_{b\in B} b$ and $d=s_A \oplus s_B$\; \label{alg1:receiver}
     
\end{algorithm}

% better naming approaches are required
\subsection{Protocol I}\label{subsec:protocol-i} 

A naive approach is to decompose the two sets into a sufficient large number 
of subsets so that each corresponding pair of subsets 
of $A$ and $B$ respectively has a set difference with at most one element. Then, each such subset pair 
can use~\autoref{alg:algorithm-0} to obtain the element belonging to the set difference (if there is one). 
Given a set difference size of $t$, assuming that there are $m$ subsets and each element is
uniformly randomly mapped to each subset, the probability that each subset pair contains at most one element from the set difference $A\Delta B$ 
is $\frac{m\,!}{(m-t)\,!m^t}\!=\!\prod_{k=1}^{t - 1}(1 - \frac{k}{m})\!\approx\! e^{-\frac{t(t-1)}{2m}}$. It is not hard to check 
at least $\lceil \frac{t(t-1)}{-2\ln p}\rceil$ subsets are required to make sure that this probability is at least $p$. 
That is, the naive approach has a communication cost of $O(t^2 \log n)$ to guarantee the set reconciliation success with a constant probability (say $0.95$), 
which is much higher than the optimal one that is $O(t \log n)$. 

\IncMargin{1em}
\begin{algorithm}
\SetKwProg{Proc}{Procedure}{}{}

\Proc{OdevityEncode($S$, m)}{
    \tcp*[h]{$m$ is \# of subsets}\
    
    $b_S \leftarrow $\code{zeros}($m$, 1)\;
    \ForEach{$s\in S$}{
        $j \leftarrow h(s) \bmod m $\;
        $b_S[j] \leftarrow \neg b_S[j]$\;
    }
    \Return{$b_S$}
}    

\caption{Odevity encode using hash function $h$.} \label{alg:odevity-encoding}
\end{algorithm}\DecMargin{1em}

Protocol I uses a two-step approach to reduce the communication cost. The first step is to identify all the subset pairs whose set differences have exact one 
element using Error-Correcting Codes (ECC)~\cite{Lin_ErrorControlCoding_1983} with a small amount of communication overhead. Then, in the second-step, 
it uses~\autoref{alg:algorithm-0} 
to reconcile those subsets. Note that Protocol I uses ECC in a very different way than all the existing ECC-based set reconciliation schemes, 
which will be detailed later in~\autoref{sec:related-work}. The key 
novelty of Protocol I is that it uses the odevity for the size of each subset to encode those subsets as a bitstring. The pseudocode of 
this odevity encoding is shown in~\autoref{alg:odevity-encoding}. As shown in~\autoref{alg:odevity-encoding}, Protocol I encodes 
each subset $S\subset A$ as a ``1'' if $|S|$ is odd; otherwise, encodes $S$ as a ``0''. Denote as $b_A$ and $b_B$ the bitstrings encoded from all subsets of $A$ 
and $B$ respectively, and as $b$ the bitwise \code{XOR} of $b_A$ and $b_B$. Then identifying subset pairs whose set differences have a size of one is 
equivalent to locating all 1's in $b$. More precisely, viewing $b_A$ as a message in Hamming space transmitted from Host A to 
Host B getting corrupted to $b_B$ with $t$ corrupted bits, then we can use suitable error-correcting codes in Hamming space 
that can correct $t$ bits of errors to identify all the 1's in $b$. BCH codes are a good choice for Protocol I. 
Note that in the context of Protocol I, only the parity bits (instead of a whole codeword) 
need to be sent. For example, if using BCH codes~\cite{Lint_IntroductionCodingTheory_1998}, 
Protocol I only requires $O(t\log m)$ bits and $O(t \log n)$ bits in the first and second step respectively. 
The total communication cost is much lighter than that of the naive approach.
 
Protocol I has the following (?) drawbacks. First, the decoding computational cost is quite high when $t$ is moderate or large, as the decoding complexity of BCH codes is $O(t^3)$ 
(with some clever algorithmic trick, the decoding complexity can be reduced to $O(t^2)$ as shown in~\cite{minisketch}). Second, Protocol I fails to identify subset pairs that contain more than $1$ elements from the set difference $A\Delta B$. 
For example, when a subset pair contains $2$ elements from the set difference $A\Delta B$, Protocol I will falsely identify this subset pair containing no such 
elements. We will 
resolve the first drawback in~\autoref{subsec:protocol-ii} and add several patches to deal with the second one in~\autoref{subsec:protocol-iii}.

%In the sequel, for ease of description, we call those subset pairs whose symmetric difference has exact one element as the desired subset pairs.
% However, to guarantee this with a high enough 
% probability (say $0.95$), a prohibitively large number of 
% subsets would be required, which results in too high communication cost. 

% To resolve the high-communication issue, we propose a two-layer module. In the first layer, we 
% decompose the two sets into subsets so that the symmetric difference of each subset pair has 
% a small number of elements (say $5$) on average. In the second layer, we further decompose each 
% subset into sufficient large number (say $1023$) of smaller subsets so that most such subset 
% pairs have a symmetric difference with at most one element. 
\IncMargin{1em}
\begin{algorithm}
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
\Input{Number of subsets $m$}

{\it Host A}: Encode set $A$ as $s_A=$ \code{OdevityEncode}($A, m$), calculate parity bits $p_A$ for $s_A$, and send $p_A$\;

{\it Host B}: Encode set $B$ as $s_B=$ \code{OdevityEncode}($B, m$), and decode all corrupted locations with $s_B$ and $p_A$\;

Use~\autoref{alg:algorithm-0} to reconcile all subsets at those corrupted locations\;


\caption{Protocol I: identify then reconcile} \label{proto:I}
\end{algorithm}\DecMargin{1em}

\subsection{Protocol II}\label{subsec:protocol-ii}

In this section, we design a two-layer protocol (Protocol II) to reduce the decoding computational complexity. In the first layer, Protocol II partitions 
elements into $\lceil \frac{t}{c} \rceil $ when $c$ is a small constant (say $5$) in a uniformly random manner. [explain a little bit more on ``uniform random'', 
some writing tricks can be learned from the paper titled as ``what's difference''] Then, each such subset pair 
contains roughly $c$ elements from the set difference on average. In the second layer, Protocol II uses Protocol I with the same configurations(number of subsets $m$, and error-correction capability $\tau$) to reconcile each subset pair. 

\autoref{proto:II} shows the pseudocode of Protocol II. It first uses a hash-function based random partition algorithm, whose pseudocode is shown 
~\autoref{alg:random-part}, to partition elements into $k=\lceil \frac{t}{c} \rceil$ subsets. Note that the random partition only guarantees that each such subset 
contains $c$ elements from  the set difference on average, and the exact number is not known. Hence, Protocol II uses a BCH code with a capability of 
correcting up to $\tau$ errors with $\tau > c$ to make sure that the BCH code has a high enough probability to decode successfully. We will describe how to deal with situation where the size of set difference exceeds $\tau$ later in~\autoref{subsec:protocol-iii}.

As the decoding of a $\tau$-error-correcting BCH code where $\tau$ is a small constant has a constant-time computational complexity, the decoding complexity of 
Protocol II is $O(k)=O(t)$.
Note that we now have several parameters, average number of exclusive elements in each subset $c$, the correcting capability $\tau$ of BCH code, and number of smaller subsets $m$ for each subset to be divided to.
How to tune these parameters to achieve favorable performance will be detailed later in~\autoref{}. 



\IncMargin{1em}
\begin{algorithm}
\SetKwProg{Proc}{Procedure}{}{}
\Proc{RandomPartition(S, k)}{
    \ForEach{$s \in S$}{
    $j\leftarrow h(s) \bmod k$\;
    
    Insert $s$ into the $j$-th subset/partition $P_j$\;
    }
    
    \Return All partitions $P$\;
}

%\caption{Random partition using hash function $h$}\label{alg:random-part}
\end{algorithm}\DecMargin{1em}

\IncMargin{1em}
\begin{algorithm}
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
\Input{Size of set difference $t$}
\Input{A required successful probability $p$}
\Input{Small constants $c$ and $\alpha$}

$k \leftarrow \lceil \frac{t}{c}\rceil $\;

Calculate the number of subsets $m$ for each partition with $p$, $k$, and $\alpha$\;

Partition elements into $k$ number of subsets using~\autoref{alg:random-part}\;

\For{$j \leftarrow 0$ \KwTo $k-1$}{
    Reconcile the $j$-th subset pair using Protocol I with size of set difference as $\alpha c$ ($\alpha > 1$) and number of subsets as $m$\;
}


%\caption{Protocol II} \label{proto:II}
\end{algorithm}\DecMargin{1em}

% \subsection{Strawman Scheme I}\label{subsec:strawman-one}

% In this section, We assume that the symmetric difference of each subset pair in the second 
% layer has {\bf at most one} element. We will show later how we can address subset pairs whose 
% symmetric difference has more than one elements. 

% First, we assume that we have an oracle which, given those subset pairs, returns all the desired 
% subset pairs. We will describe the construction of such an oracle later in~\autoref{subsec:desired-subset-pair-detector}. This scheme 
% consists of two phases, namely, an encoding phase and a decoding phase.

% \medskip
% \noindent
% {\bf Encoding phase.} In this phase, host $A$ \code{XOR} all the elements in each subset, 
% which belongs to the desired subset pairs at the side of host $A$, and send to host $B$. 
% \autoref{alg:strawman-one-encoding} shows the pseudocode of the encoding phase. Here we only describe 
% the encoding process for an arbitrary such subset at host $A$; that for any other such subsets 
% is identical. Denote $\tilde{S}^{A}$ as this subset, then the encoding process works as follows. 
% \code{enc}($\tilde{S}^{A}$)=\code{XOR}$_{e \in \tilde{S}^{A}}$. 

% %{\color{red}{\bf @ZiHeng Could you please add the two simple pseudo-codes.}}

% \begin{algorithm}
% \caption{Encoding process of $\tilde{S}^{A}$ on Host $A$}
% \label{alg:strawman-one-encoding}
% \SetKwProg{Proc}{Procedure}{}{}
% \Proc{enc($\tilde{S}^{A}$)}{
%     $sum \longleftarrow 0$\;
%     \ForEach{e in $\tilde{S}^{A}$}{
%         $sum \longleftarrow sum$ $\code{XOR}$ $e$\;
%     }
%     \Return{$sum$}
% }       
% \end{algorithm}

% \medskip
% \noindent
% {\bf Decoding phase.} The decoding phase is almost the same as the encoding. The pseudocode of 
% the decoding phase is shown in~\autoref{alg:strawman-one-decoding}. After receiving those encoding 
% values from host $A$, host $B$ simply \code{XOR} all the elements in the corresponding subset with 
% each such value it receives, the result of which is the element belonging to the symmetric difference. 

% \begin{algorithm}
% \caption{Decoding process of $sum$ and $\tilde{S}^{B}$ on Host $B$}
% \label{alg:strawman-one-decoding}
% \SetKwProg{Proc}{Procedure}{}{}
% \Proc{dec($sum$, $\tilde{S}^{B}$)}{
%     \ForEach{e in $\tilde{S}^{B}$}{
%         $sum \longleftarrow sum$ $\code{XOR}$ $e$\;
%     }
%     \Return{$sum$}
% }       
% \end{algorithm}

% \subsection{Desired Subset Pair Detector}\label{subsec:desired-subset-pair-detector}

% In this section, we propose a scheme to identify those desired subset pairs efficiently. This 
% scheme leverages the properties of error-correction codes (ECC). Note that using ECC to do 
% set reconciliation is not new, many existing research have proposed different schemes to use 
% ECC to reconcile remote sets. However, in this scheme, we use ECC in a totally different way in 
% that almost all existing ECC-based schemes only work for sets whose universe is small whereas 
% our scheme does not have such limitation. 

% As mentioned earlier, we assume that the symmetric difference of each subset pair in the second 
% layer has at most one element. Unlike the existing ECC schemes which ..., this scheme maps 
% each subset to $0$ if it contains even number of elements, otherwise mapping it as $1$. 
% \autoref{} shows the encoding strategy for the first subset in the first layer; that for any other 
% subsets is identical. Let $S^{A}_1,S^{A}_2,\cdots,S^{A}_n$ denote all the smaller subsets 
% (in the second layer) of the first subset in the first layer. The mapped binary string is 
% $\mathbf{v}^{A}=(v^{A}_1,v^{A}_2,\cdots,v^{A}_n)$ where $v^{A}_i=0$ if $|S^{A}_i|$ is even otherwise $v^{A}_i=1$. 
% Similarly, host $B$ calculates $\mathbf{v}^{B}$. Since for any $i$, $|S^{A}_i\Delta S^{B}_i|\leq 1$, $v^{A}_i$ \code{XOR} $v^{B}_i=1$ if $|S^{A}_i\Delta S^{B}_i|=1$; otherwise $v^{A}_i$ \code{XOR} $v^{B}_i=0$. 
% More precisely, the difference between the two subsets in the first layer correspond to the Hamming distance between 
% the two mapped binary strings. Therefore, we can use an ECC that is capable of correcting $t$ errors if the 
% size of difference between the two subsets is bounded by $t$ to identify those ``error bits'', {\it i.e.,} 
% to which subsets (in the second layer) the elements from the symmetric difference $S^{A}\Delta S^{B}$ belong. 
% In this scheme, we choose binary BCH codes. With $(n,t)$ BCH codes, we 
% only need to transmit the check bits, which is less than $t\cdot \log{n}$ bits, to correct all bit errors in the $n$-bit-long binary string if there are no more than $t$ errors. . 
% {\color{red}(TODO: borrowing some sentences from ECC-based papers)} 




--------------------------------

% To avoid wasting communications 
% for those pairs whose symmetric differences are empty or have more than one elements, we propose 
% a novel error-correct-code (ECC) based scheme to identify those desired subset pairs. In this 
% scheme, we encode 


%The core concept of our algorithm is the Balls and Bins model. We scatter all elements in the two sets using the same mapping so that identical elements will be distributed into the same bin. When we use XOR sum, elements that are in both sets will be cancelled out and only the elements in symmetric difference are left in the bins. So the number of bins we need is determined by the size of set difference $d$.
%\[\bigoplus_{x \in A} {x}  \oplus  \bigoplus_{x \in B} {x} = \bigoplus_{x \in A \triangle B} {x} \] trouble with this formula
%When there is only one exclusive element in a bin, we can obtain it directly. To thoroughly scatter all the elements, we need a large number of bins which will lead to much communication overhead. Furthermore, we need to detect which bins contain only one element. So we develop a two-layer balls and bins model which significantly reduce communication overhead.

%On the first layer, we first estimate the set difference $\hat{d}$. Then we throw all elements into $\delta \hat{d}$ bins. The number of elements in a bin is approximately a Poisson distribution with expectation of $\frac{d}{\delta \hat{d}}$. 

%On the second layer, we scatter the elements in each bin into smaller bins. But this time, we use a large number of small bins, trying to make all bins only contain one or no element. To save communication cost, We utilize BCH codes to detect which bins contain exactly one element.

%Details about the estimator and how we leverage BCH codes will be discussed below.
\subsection{Protocol III}\label{subsec:protocol-iii}
In Protocol I, though we partition the set into a large number of subsets, it is still possible that more than one exclusive elements fall into a same subset. 

When even number of exclusive elements are in one subset, the first step of Protocol I will ignore this subset. To deal with this situation, we will compute a checksum of all elements in subsets that are encoded as "0" ("0-subsets")on both host. Then we will send A's checksum along with all the XOR sums to B. B will compare the two checksums. If the two checksums are the same, we will consider all "0-subsets" contain no exclusive elements. Otherwise, we will need to use Protocol I to reconcile the union of all "0-subsets" in the next round using a different hash function. 

When odd number($\geq 3$) of exclusive elements are in one subset, Protocol I will reconcile the XOR sum of all exclusive elements. To identify whether the XOR sum we get in the second step is an exclusive element, we can apply the hash function we used to partition the set to the XOR sum. If it truly is an exclusive element, it will be hashed into the exact subset we are now decoding. Otherwise, it only has a small possibility to be hashed into that subset. 

A new issue results from the uncertainty of how many elements from set difference a subset pair contains is that the true number of elements from set difference may exceeds the error-correction capability $\tau$. We will simply partition this subset into $s$ smaller subsets after BCH decoder reports that it fails to decode.
Then we use the same approach to deal with each smaller subsets in the next round.
We can use the technique in~\cite{naumenko2019bandwidth} to leverage the parity bits sent in the first round. We only need to compute the odevity vector and parity bits of $s-1$ smaller subsets. By XORing the $s-1$ parity bits and the parity bits of the original subset, we can get the parity bits of the left-behind smaller subset.
With extremely low possibility, BCH code may decode the corrupted bit string to irrelevant codeword when error-correction capacity is exceeded.
Thankfully, the two patches above can deal with this situation smoothly.

By adding these three patches above to protocol II, we design a more robust protocol III that can reconcile all elements with high probability.
\end{comment}

\input{section/estimator}

==> section/schemes_new0214.tex <==
%\section{PBS for small \texorpdfstring{$d$}{d}}\label{sec:scheme}
\section[PBS for small \texorpdfstring{$d$}{d}]{PBS for small \texorpdfstring{\larger\boldmath\MakeLowercase{$d$}}{d}}\label{sec:scheme}
%\section{Set Reconciliation}\label{sec:scheme}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%     Writing Guideline for This Section     %%%%%%%%%%
% “balls – elements in the symmetric difference of the two sets” 

% Protocol 0 (reconcile two sets whose set difference has at most one ball)

% Protocol I.I (partition elements into a sufficiently large number of subsets such that each subset has at most one ball with high probability and use Protocol 0 to reconcile each of them) 

% Protocol I.II (a two-step refinement of Protocol I.I: first use BCH to identify good bins, i.e., bins/subsets have exactly one ball, and then use Protocol 0 to reconcile each good bin) 

% Protocol II (a two-layer refinement of Protocol I.II: in the first layer, we partition elements into t/c subsets, where t is the size of set difference and c is a small constant, then each subset has c balls on average. In the second layer, we further partition each subset into large enough number of bins/subsets such that with high probability each bin has at most one ball, then use Protocol I.II to reconcile them one by one) 

% Protocol III/IV (mainly fix certain exceptions in Protocol II，e.g., how to address bad bins, how to handle the cases where BCH fails to decode and etc)

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% In this section, we describe our set reconciliation scheme in details. First, we give a formal problem statement in \autoref{sec:model}. In \autoref{subsec:protocol0}, we introduce a basic scheme for the trivial case, in which the two sets $A$ and $B$ has at most one distinct element. Building upon the basic scheme, we propose the preliminary version of scheme in \autoref{sucsec:our-scheme} that targets to the cases where the total number of distinct elements $d$ is small. Then we extend the preliminary version and propose the final version of our scheme in \autoref{subsec:protocol2} for general cases (i.e., any arbitrary $d$). We assume $d$ is precisely known throughout this section except in \autoref{subsec:ToW}, where we will describe how to estimate $d$ using a Tug-of-War Estimator. 

\subsection{Problem Statement}\label{sec:model}

In this work, we adopt the commonly used model for the set reconciliation problem. 
Two remote sets $A$ and $B$ are stored at hosts Alice and Bob respectively. 
Each element in $A$ and $B$ is a hash signiture in the key space (universe) $\mathcal{U}$, which is the set of all $(\log |\mathcal{U}|)$-bit binary strings. 
%Each element in $A$ and $B$ is a hash signiture with signiture width $w$ in the key space (universe) $\mathcal{U}$, which is the set of all $w$-bit binary strings (i.e., $|\mathcal{U}|=2^w$). 
%We use $\mathcal{U}$ to denote the set of all $w$-bit binary strings and name it the universe of signitures. 
The set reconciliation problem is to compute the symmetric set difference between $A$ and $B$, 
{\it i.e.,} $A\Delta B\triangleq (A\!\setminus\! B) \bigcup (B\!\setminus\! A)$. 
Let $d\!=\!|A\Delta B|$ be the cardinality of this difference.
%We denote $d\!=\!|A\Delta B|$. 
Throughout this paper, we call each element in $A\Delta B$ a \textit{distinct element}, and each element in $A\bigcap B$ a \textit{common element}.
{\bf Like in all existing solutions, we describe only {\it unidirectional} set reconciliation, in which Alice or Bob learns the set difference $A\Delta B$. Since the performance of our scheme does not depend on who learns the set difference, we assume Bob learns the set difference $A\Delta B$ in the rest of the paper, as mentioned in \autoref{sec:psea}.}
% As mentioned in \autoref{sec:psea}, we describe {\it unidirectional} set reconciliation that Bob learns the set difference $A\Delta B$. 
%In \autoref{sec:evaluation}, we use the same semantic to measure the communication cost of our scheme and other compared set reconciliation schemes. 

In the rest of this section, we build up our scheme gradually as follows: We start with the trivial case where $d\leq 1$ in \autoref{subsec:protocol0}. Then we generalize our scheme to the case where $d$ is a small number in \autoref{sec:pbs_smalld}. 
%After that, we further generalize our scheme to the case that $d$ is a large number in \autoref{subsec:protocol2}. 
Throughout this section, we assume $d$ is precisely known.
%except in \autoref{subsec:ToW}, where we will describe how to estimate $d$ using a Tug-of-War Estimator. 

%The rest of this section is organized as follows: In \autoref{subsec:protocol0}, we introduce a basic scheme for the trivial case, in which the two sets $A$ and $B$ has at most one distinct element. In \autoref{sucsec:our-scheme} and \autoref{subsec:protocol2}, we elaborate the two versions of our solution that are introduced in \autoref{sec:smalld} and \autoref{sec:larged} respectively. Throughout this section, we assume $d$ is precisely known except in \autoref{subsec:ToW}, where we will describe how to estimate $d$ using a Tug-of-War Estimator. 

\subsection{The Trivial Case of \texorpdfstring{\larger\boldmath $d\leq 1$}{d<2}}\label{subsec:protocol0}

%We start with the trivial case, in which $A$ and $B$ have at most one distinct element ({\it i.e.,} $d\leq 1$), we have a simple set reconciliation scheme showed in \autoref{alg:trivial_case}:

\autoref{alg:trivial_case} shows the reconciliation scheme for the trivial case, in which $A$ and $B$ differ by at most one distinct element:

\begin{algorithm}
\caption{Set reconciliation when $d\le 1$}
\label{alg:trivial_case}

{\it Alice}: $s_A\leftarrow\underset{a\in A}{\oplus} a$; Send $s_A$ to Bob\; \label{alg1:sender}

{\it Bob}: $s_B\leftarrow\underset{b\in B}{\oplus} b$; $s\leftarrow s_A \oplus s_B$\; \label{alg1:receiver}
\end{algorithm}

First, Alice calculates $s_A$, the bitwise \code{XOR} of all elements in $A$, and send it to Bob. 
Second, Bob also calculates $s_B$, the bitwise \code{XOR} of all elements of $B$. Upon receiving $s_A$, Bob computes $s\!\triangleq\! s_A \!\oplus\! s_B$, and we have

\begin{sitemize}
	\item If $A$ and $B$ are identical sets (i.e., $d=0$), we have $s_A=s_B$ and $s=\mathbf{0}$;
	\item If $A$ and $B$ has one distinct element (i.e., $d=1$), the computed $s$, the bitwise \code{XOR} of $s_A$ and $s_B$, will cancel out all common elements and remain the distinct element. In other words, we have $A\Delta B=\{s\}$. 
	%And $s$ is the missing element of $A$ (i.e., $s\in B\!\setminus\! A$) if $s\in B$, or the missing element of $B$ (i.e., $s\in A\!\setminus\! B$) otherwise;
	% \item If $A$ and $B$ has more than one distinct elements (i.e., $d>1$), the bitwise \code{XOR} of $s_A$ and $s_B$ will still cancel out all common elements and remain the \code{XOR} of the distinct elements, i.e., $s$ is the \code{XOR} of all distinct elements;
\end{sitemize}

Like most works on set reconciliation, we assume $\mathbf{0}$ is excluded from $\mathcal{U}$, as \autoref{alg:trivial_case} does not work when $\mathbf{0}\in A\bigcap B$ for the following reason: When $s=\mathbf{0}$, \autoref{alg:trivial_case} cannot tell whether $A$ and $B$ are identical, or they have a distinct element of value $\mathbf{0}$. 
%However, we can extend our scheme to support $\mathbf{0}$. For example, we let Alice send to Bob a single bit to indicate whether Alice has element $\mathbf{0}$, so Bob will know whether $\mathbf{0}\in A\Delta B$ or not. 
\autoref{alg:trivial_case} also does not work when there are more than one distinct elements in $A\Delta B$ (i.e., $d>1$), since the computed $s$ is the \code{XOR} of all these distinct elements.

% Note that \autoref{alg:trivial_case} works if and only if $|A\Delta B|\!\leq\! 1$ and $0\!\notin\! (A\!\cup\! B)$ (which we have explained in~\autoref{sec:model}). 

%\subsection{PBS: When $d$ is small}\label{sucsec:our-scheme}

%In this section, we generalize PBS to the case when $d$ is a small number, as we described in \autoref{sec:smalld}. 
%First, we describe each step of single-round PBS from \autoref{sec:hash_partition} to \autoref{sec:reconcile_by_trivial} and summarize it in \autoref{sec:single_round_pbs}. Second, we discuss the exceptions in single-round PBS in \autoref{subsec:exception_hash_partition}. Third, we propose multi-round PBS to handle the exceptions.

\subsection{PBS for small \texorpdfstring{\larger\boldmath $d$}{d}}\label{sec:pbs_smalld}

In this section, we substantiate the scheme described in \autoref{sec:smalld} for small $d$.

\subsubsection{Hash Partition and Parity Bitmap Encoding}\label{sec:hash_partition}
% \medskip
% \noindent{\bf Hash Partition} 

Here we formalize the process of partitioning $A$ into $\{A_i\}_{i=1}^n$, $B$ into $\{B_i\}_{i=1}^n$, and $A\Delta B$ into $\{A_i\Delta B_i\}_{i=1}^n$ as described in \autoref{sec:smalld} by introducing the concept of {\it sub-universes}. Given a hash function $h(\cdot): \mathcal{U}\rightarrow \{1,2,\cdots,n\}$, we define {\it sub-universe} $\mathcal{U}_i$ as the set of elements in $\mathcal{U}$ that are hashed into value $i$. More precisely, $\mathcal{U}_i\triangleq\{s\!\mid\! s\in \mathcal{U} \mbox{ and } h(s)=i\}$ for $i=1,2,...,n$. Then defining $A_i\triangleq A\bigcap\mathcal{U}_i$ and $B_i\triangleq B\bigcap\mathcal{U}_i$ for $i=1,2,...,n$ induces the partitioning of $A$, $B$, and $A\Delta B$, as mentioned in \autoref{sec:smalld}. 

For the moment, we assume the following {\bf ideal case} happens: Every subset pair difference $A_i\Delta B_i$ contains at most one distinct element. The nonideal case of a subset pair difference containing more than $1$ distinct elements will be discussed in \autoref{subsec:exception_hash_partition}. 

%In this section, we give a detailed description on how to partition $A$ and $B$ (as introduced in \autoref{sec:smalld}) by introducing {\it sub-universes}, which is defined as follows: Given a hash function $h(\cdot): \mathcal{U}\rightarrow \{1,2,\cdots,n\}$, we define {\it sub-universes} $\{\mathcal{U}_i\}_{i=1}^n$, a partition of the universe $\mathcal{U}$, as $\mathcal{U}_i=\{s\!\mid\! s\in \mathcal{U} \mbox{ and } h(s)=i\}$ for $i=1,2,...,n$. Based on $\{\mathcal{U}_i\}_{i=1}^n$, we define $\{A_i\}_{i=1}^n$, the partition of $A$ introduced in \autoref{sec:smalld}, as $A_i\! \triangleq\! A\bigcap \mathcal{U}_i$ for $i=1,2,...,n$. $\{B_i\}_{i=1}^n$ is similarly defined. By this definition, the set difference $A\Delta B$ is partitioned into $n$ set differences of the partitioned subset pairs (i.e., $\{(A_i, B_i)\}_{i=1}^n$). From \autoref{sec:hash_partition} to \autoref{sec:reconcile_by_trivial}, we assume the following {\bf ideal case} happens: Each subset pair $(A_i, B_i)$ contains at most one distinct element ({\it i.e.,} $|A_i\Delta B_i|\!\leq\!1$). The nonideal case of a subset pair contains more than $1$ distinct elements will be discussed in \autoref{subsec:exception_hash_partition}. 

% Here we describe the hash-partition step introduced in \autoref{sec:smalld} in details. First, we use a hash function $h(\cdot): \mathcal{U}\rightarrow \{1,2,\cdots,n\}$ to partition the universe $\mathcal{U}$ into $n$ sub-universes: $\mathcal{U}_i=\{s\!\mid\! s\in \mathcal{U} \mbox{ and } h(s)=i\}$ for $\forall i=1,2,\cdots,n$. The hash function $h(\cdot)$ can be predetermined between Alice and Bob and does not require additional communication cost. Define $A_i\! \triangleq\! A\bigcap \mathcal{U}_i$ and $B_i\! \triangleq\! B\bigcap \mathcal{U}_i$ for $i=1,2,\cdots,n$. Then $\{A_i\}_{i=1}^n$ and $\{B_i\}_{i=1}^n$ are partitions of $A$ and $B$ respectively. Furthermore, $\{A_i\Delta B_i\}_{i=1}^n$ is a partition of $A\Delta B$. From \autoref{sec:hash_partition} to \autoref{sec:reconcile_by_trivial}, we assume the following {\bf ideal case} happens: Each subset pair $(A_i, B_i)$ contains at most one distinct element ({\it i.e.,} $|A_i\Delta B_i|\!\leq\!1$). The nonideal case of a subset pair contains more than $1$ distinct elements will be discussed in \autoref{subsec:exception_hash_partition}. 

How the $d$ distinct elements (balls) in $A\Delta B$ are distributed into the $n$ subset pair differences $\{A_i\Delta B_i\}_{i=1}^n$ (bins) 
can be viewed as throwing $d$ balls each uniformly and randomly into one of the $n$ bins. 
%follows the familiar {\it balls-into-bins} probability model. 
%The distinct elements are viewed as balls and the subset pairs are viewed as bins. 
%Each of the $d$ balls is uniformly and randomly thrown by the hash function $h(\cdot)$ into one of the $n$ bins. 
The aforementioned ideal case that corresponds to the $d$ balls ending up in $d$ distinct bins happens with probability $\prod_{k=1}^{d - 1}(1 - \frac{k}{n})$, which is on the order of $1-O(d^2/n)$ when $d\!\ll\!n$.
%approximately $e^{-\frac{d(d-1)}{2n}}$ when $d\!\ll\!n$. 
Hence, $n$ must be $\Omega(d^2)$ to ensure the ideal case happens with a nontrivial probability, as mentioned in \autoref{sec:smalld}.


%in which the distinct elements are viewed as balls and the subset pairs are viewed as bins. The hash-parition basically throws (hashes) $d$ balls (distinct elements) uniformly and randomly into $n$ bins (subset pairs). The aforementioned ideal case in this context becomes, after throwing $d$ balls uniformly and randomly into $n$ bins, each bin receives at most $1$ ball (i.e., $d$ nonempty bins have $1$ ball in each and the rest $n-d$ bins are empty). The number of balls in each bin is a Binomial random variable $Binomial(d,1/n)$.
%{\bf It may remind readers about the Birthday problem. And the ideal case can be analogous to the case that no people share the same birthday.} 
% The ideal case happens with a probability of $p\!=\!\prod_{k=1}^{d - 1}(1 - \frac{k}{n})\!\approx\! e^{-\frac{d(d-1)}{2n}}$ when $d\!\ll\!n$. In other words, $n$ must be at least $O(d^2)$ to ensure the ideal case happens with a nontrivial probability, as described in \autoref{sec:smalld}.  

% Note that the ideal case does not always happen. However, we can ensure that the ideal case happens with high probability by properly setting $n$ based on $d$ (i.e., $n=\Omega(d^2)$). Furthermore, as we will describe in \autoref{subsec:nonideal}, even if the ideal case does not happen (i.e., some distinct elements are hashed into the same subset pair), most of the distinct elements should be distributed into different subset pairs and therefore can be reconciled. So the scheme, even cannot reconcile all of the distinct elements, can still reconcile the majority of them (i.e., piecewise decodability in \autoref{sec:intro_oursolution}). Based on this property, we will extend our scheme from single-round to multi-rounds in \autoref{subsec:nonideal} to further increase the probability of reconciling all distinct elements. 

% \medskip
% \noindent{\bf Parity Bitmap Encoding} 

We encode $\{A_i\}_{i=1}^n$ into an $n$-bit-long parity bitmap $A[1..n]$, in which $A[i]$, the $i^{th}$ bit of the parity bitmap, is equal to the oddness / evenness (parity) of the cardinality of $A_i$ (i.e., $A[i]=1$ if $|A_i|$ is odd; otherwise $A[i]=0$). In the ideal case, the two bitmaps $A[1..n]$, $B[1..n]$ differ in exactly $d$ bit positions $i_1,i_2,...,i_d$, each of which corresponds to a subset pair that contains $1$ distinct element. The next step is to let Alice and Bob know these bit positions.
%Once the $d$ bit positions are known, Alice and Bob can start to reconcile $(A_{i_1},B_{i_1}), (A_{i_2},B_{i_2}),...,(A_{i_d},B_{i_d})$ using \autoref{alg:trivial_case} and obtain the $d$ distinct elements (i.e., $A\Delta B$). 

% \subsubsection{Parity Bitmap Encoding}\label{sec:parity_bitmap_encoding}

% %After hash-partitioning $A$ and $B$ into partitions $\{A_i\}_{i=1}^n$ and $\{B_i\}_{i=1}^n$, 
% As introduced in \autoref{sec:smalld}, we encode each partition into an $n$-bit-long parity bitmap and denote them as $A[1..n]$ and $B[1..n]$ respectively, as introduced in \autoref{sec:smalld}. For $i=1,2,...,n$, $A[i]$ (the $i^{th}$ bit of the parity bitmap $A[i]$) is equal to $1$ if $A_i$ contains an odd number of elements, and is equal to $0$ otherwise.
% % More specifically, for $i=1,2,...,n$, $A[i]$ (the $i^{th}$ bit of the parity bitmap $A[i]$) is defined as follows: $A[i]=1$ if $A_i$ contains an odd number of elements, and $A[i]=0$ otherwise. In this way, each bit $A[i]$ encodes the oddness / evenness (parity) of the cardinality of $A_i$. The $n$-bit-long parity bitmap $B[1..n]$ and $B[i]$ (the $i^{th}$ bit of $B[1..n]$) are similarly defined. 
% In the ideal case, 
% %$A[i]$ and $B[i]$ differ if and only if $A_i$ and $B_i$ have exactly $1$ distinct element, and $A[i]$ and $B[i]$ are the same if and only if $A_i=B_i$. Meanwhile, the $d$ distinct elements are hashed into $d$ different subset pairs. So 
% the two bitmaps $A[1..n]$, $B[1..n]$ differ in exactly $d$ bit positions, each of which corresponds to a subset pair that contains $1$ distinct element. Once the $d$ bit positions are known, Alice starts to reconcile each of the $d$ corresponding subset pairs by \autoref{alg:trivial_case} and gets the $d$ distinct elements (i.e., $A\Delta B$). 
% %If knowing the $d$ bit positions (i.e., the $d$ corresponding subset pairs), we can use \autoref{alg:trivial_case} to reconcile the $d$ subset pairs respectively to obtain all the $d$ distinct elements (i.e., $A\Delta B$). 
% In \autoref{sec:BCH_code}, we will describe how to find the $d$ bit positions using BCH code~\cite{Lint_IntroductionCodingTheory_1998}. 

% \medskip
% \noindent{\bf Find the $d$ Bit Positions Using ECC} 

%\subsubsection{Find the $d$ Bit Positions Using ECC}\label{sec:BCH_code}
\subsubsection{Find and Reconcile the \texorpdfstring{$d$}{d} subset pairs}\label{sec:BCH_code}

We view $A[1..n]$ as a corrupted message of $B[1..n]$ sent ({\bf not actually being sent}) from Bob to Alice through an {\it unreliable} commnunication channel that flips $d$ bits. To locate these $d$ bit positions, we let Bob also send an {\it error-correction code} that encodes $B[1..n]$ to Alice, such that Alice can recover $B[1..n]$ (original message) and obtain the $d$ bit positions $i_1,i_2,...,i_d$. In PBS, we use BCH code~\cite{bch1} to encode $B[1..n]$ and get the error-correction code.

There are two different BCH encoding techniques: {\it systematic} and {\it unsystematic}. The difference is, the message appears as the prefix of the codeword (i.e., codeword = [message net-codeword]) in systematic BCH encoding, whereas it does not appear as a substring of the codeword in unsystematic BCH encoding. In PBS, we choose systematic BCH encoding because we are not actually sending the ``message'', and only the net-codeword is transmitted from Bob to Alice. 

To correct $d$ bit errors, the length of the net-codeword only is no more than $d\log n$ bits. We use the term `codeword' to refer to the net-codeword in the rest of this paper.
%The computational complexity of the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} is $O(d^2\log^2 n)$.
The systematic BCH encoding is also used in other ECC-based set reconciliation works, such as PinSketch \cite{Wuille_Minisketchoptimizedlibrary_2019}, while PinSketch encodes a much longer message (e.g., $2^{32}$ bits) than in ours (hundreds of bits).  

%\subsubsection{Find the $d$ Bit Positions Using ECC}\label{sec:BCH_code}

% A straightforward approach to find the $d$ bit positions is to let Bob send the complete parity bitmap $B[1..n]$ to Alice, then Alice compares $A[1..n]$ with $B[1..n]$ locally. This approach has a communication overhead of $n$ bits, which is quite wasteful. As we discussed in~\autoref{sec:hash_partition}, $d$ is usually much smaller than $n$. It means $A[1..n]$ and $B[1..n]$ differ only at a tiny portion of bits. Therefore, we can view $A[1..n]$ as a corrupted message of $B[1..n]$ with $d$ bit errors, and the bit positions of the $d$ bit errors basically correspond to the $d$ subset pairs that contain distinct elements. The detection of bit errors, on the other hand, can be solved by Error-Correction Code (ECC)~\cite{Lin_ErrorControlCoding_1983}. 

% Since $A[1..n]$ and $B[1..n]$ differ at $d$ bit positions, we can view $A[1..n]$ as a corrupted message of $B[1..n]$ from Bob to Alice through an {\it unreliable} commnunication channel with $d$ corrupted bits, which are located on the $d$ bit positions. Therefore, to find the $d$ bit position, we only need to correct the $d$ corrupted bits in $A[1..n]$, which is done by transmitting a ``code'' that can correct upto $d$ bit errors from Bob to Alice through a {\it reliable} communication channel. 

% In PBS, we use {\it systematic} BCH code to generate the ``code'' by encoding the message $B[1..n]$. The codeword of the systematic BCH code is in the form of [message, net-codeword], since the message appears as the prefix of the codeword in systematic BCH code. The ``code'' is simply the net-codeword in the BCH codeword. We choose {\it systematic} BCH code because the (corrupted) message is already transmitted and we only need to pay a small communication overhead on transmitting ``code'' (i.e., net-codeword). To correct upto $d$ bit errors, the length of the net-codeword is no more than $d\log n$ bits, which is much smaller than the message when $d\!\ll\! n$. The computational complexity of the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} is $O(d^2\log^2 n)$. This type of BCH code is also used in other ECC-based set reconciliation works, such as PinSketch \cite{Wuille_Minisketchoptimizedlibrary_2019}. 

% Different from {\it unsystematic} BCH code
% The ``code'' is generated by {\it systematic} BCH code, which encodes the message $B[1..n]$ into a BCH codeword in the form of [message, net-codeword]. The ``code'' transmitted on the reliable channel is the net-codeword of the BCH codeword. In {\it systematic} BCH code, the message appears as the prefix of the codeword. 

% More specifically, PBS uses {\it systematic} BCH code~\cite{Lint_IntroductionCodingTheory_1998} that can correct upto $d$ bit errors to encode the parity bitmaps. In the {\it systematic} BCH code \footnote{In unsystematic BCH code, message does not appear to be the prefix of the codeword}, the message (i.e., the parity bitmap) appears as the prefix of the raw codeword, which in the form of [message, net codeword]. Normally, to correct upto $d$ errors, the length of the net codeword is $2n\log d$, where $n$ is the length of the message (i.e., parity bitmap). However, our case is special in the sense that the net codeword is error-free (all $d$ bit errors are in the message), so the length of the net codeword can be reduced to $n\log d$. This type of BCH code is also used in other ECC-based set reconciliation works, such as PinSketch \cite{Wuille_Minisketchoptimizedlibrary_2019}. 

% Now we can formally describe how to find the $d$ bit positions: First, Bob uses a $d$-error-correcting systematic BCH code to encode $B[1..n]$ and sends the net codeword ($d\log n$ bits) to Alice. Upon receiving the net codeword and combining it with the corrupted message $A[1..n]$, Alice uses the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} to decode the $d$ bit errors in $A[1..n]$. The communication overhead of transmitting the net codeword is $d\log n$ bits. The computational complexity of the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} is $O(d^2\log^2 n)$. Both the communication overhead and the computational complexity here are relatively small when $d$ is small.

% \medskip
% \noindent{\bf Reconcile the $d$ subset pairs using \autoref{alg:trivial_case}} 

%Once the $d$ bit positions are known, Alice can start to reconcile $(A_{i_1},B_{i_1}), (A_{i_2},B_{i_2}),...,(A_{i_d},B_{i_d})$ using \autoref{alg:trivial_case} and obtain the $d$ distinct elements (i.e., $A\Delta B$). 
Once Alice decodes $i_1,i_2,...,i_d$, the corresponding subset pairs $(A_{i_1},B_{i_1}), (A_{i_2},B_{i_2}),...,(A_{i_d},B_{i_d})$ each can be reconciled using \autoref{alg:trivial_case}. To do so, Alice needs to send not only the corresponding \code{XOR} sums $S_{A_{i_1}}$, $S_{A_{i_2}}$, ...,$S_{A_{i_d}}$, but also the subset pair indices $i_1,i_2,...,i_d$, to Bob, since Bob does not know which of the $d$ subset pairs are being reconciled. Each index needs to be encoded into $\log n$ bits, so the additional communication overhead on transmitting the indices is $d\log n$ bits. 
% When reconciling $(A_{i_1},B_{i_1}), (A_{i_2},B_{i_2}),...,(A_{i_d},B_{i_d})$ using \autoref{alg:trivial_case}, Alice needs to send not only the bitwise \code{XOR} of $A_{i_1}, A_{i_2},..., A_{i_d}$, but also the indices of the subset pairs ($i_1,i_2,...,i_d$), since Bob does not know which of the $d$ subset pairs are being reconciled. Each index is an integer between $1$ and $n$ and can be encoded into $\log n$ bits, So the additional communication overhead on transmitting the indices is $d\log n$ bits. 



% \subsubsection{Reconcile the $d$ subset pairs using \autoref{alg:trivial_case}}\label{sec:reconcile_by_trivial}

% After decoding the $d$ bit errors that corresponds to the $d$ subset pairs, Alice starts to reconcile them using \autoref{alg:trivial_case}. For each of the $d$ subset pairs, Alice needs to send not only the bitwise \code{XOR} of the subset pair, but also the index of the subset pair (since Bob does not know the $d$ subset pairs to reconcile). So the communication overhead on \autoref{alg:trivial_case} is $d\log |\mathcal{U}|+d\log n$ bits. 
%Plus the communication overhead on transmitting the net codeword of parity bitmap ($d\log n$, as we explained in \autoref{sec:BCH_code}), the overall communication overhead of single-round PBS is $d\log u+2d\log n$ bits.

% \medskip
% \noindent{\bf Check if set reconciliation is complete} 

After reconciling the subset pairs and obtaining the reconciled set difference (denoted as $\hat{D}$), PBS needs to check if set reconciliation is complete (or whether $\hat{D}=A\Delta B$), since the reconciled set difference $\hat{D}$ is not the actual set difference $A\Delta B$ in the nonideal case (to be discussed in \autoref{subsec:exception_hash_partition}). Hence, we add a verfication step after obtaining $\hat{D}$ to check if $\hat{D}=A\Delta B$. In PBS, we check an equivalent condition, $A=B\Delta\hat{D}$, instead of $\hat{D}=A\Delta B$, since $B$ and $\hat{D}$ are both known by Bob and their set difference $B\Delta\hat{D}$ can be locally computed. More specifically, to check if the remote sets $A$ and $B\Delta\hat{D}$ are equal, we let Alice compute a $32$-bit checksum of $A$ and send it to Bob. {\bf Then Bob computes the $32$-bit checksum of $B\Delta\hat{D}$ using the same checksum algorithm and compare the two checksums. In PBS, we select {\it longitudinal parity check} (i.e., bitwise \code{XOR} of all elements in the set) as the checksum algorithm, so that the checksum $B\Delta\hat{D}$ can be efficiently computed as the bitwise \code{XOR} between the checksum of $B$ (can be pre-computed) and that of $\hat{D}$. Other checksum algorithms that are {\it linear} to the set difference operator (i.e., $\Delta$) also work for PBS. }
% Then Bob checks if $B\Delta\hat{D}$ satisfies the receiving checksum. 

The condition $A=B\Delta\hat{D}$ can be almost surely verified by a $32$-bit checksum, albeit it could mistakenly believe two different sets as identical ones with probability $2^{-32}\approx 2.3\times 10^{-10}$ {\bf on top of the probability that the nonideal case happens (on the order of $10^{-2}$).} This tiny probability of such an event should be acceptable in most applications. {\bf To simplify our description, we ignore this small probability event and assume the checksum works perfectly in this rest of this paper. (Is it OK to say that? or we say this small probability event only in tail bound analysis?)}
%and such an event (i.e., mistaken $A$ and $B\Delta\hat{D}$ are identical when they are different) never happens in our evaluation. For some super critical applications, we can certainly use a $64$-bit checksum to reduce this probability to $5.4\times 10^{-20}$ if needed.

% When the ideal case does not happen, set reconciliation cannot accomplish in one round, as we will explain in \autoref{subsec:exception_hash_partition}. Hence, we add a verfication step to check if set reconciliation is complete. Let $\hat{D}$ denote the set of reconciled elements. The idea of this verification is basically to compare $A$ with $B\Delta \hat{D}$: If $A=B\Delta \hat{D}$ (i.e., $\hat{D}=A\Delta B$), we know the set reconciliation is complete; Otherwise, the set reconciliation is incomplete.  using a $32$-bit checksum. 

\subsubsection{Communication overhead of PBS (First Round)}\label{sec:communication_overhead_single_PBS}

All the steps of PBS in the first round are summarized in \autoref{alg:single_round_pbs}. The overall communication overhead consists of three components: (1) the BCH codeword of $d\log n$ bits in \autoref{step:BCH_encode}; (2) the subset pair indices $i_1,i_2,...,i_d$ and the corresponding bitwise \code{XOR}s of $d\log n+d\log |\mathcal{U}|$ bits in \autoref{step:trivial_reconcile}; and (3) the $32$-bit checksum of $A$ in \autoref{step:terminate_condition}. 

\begin{algorithm}
\caption{Single-round PBS}
\label{alg:single_round_pbs}

%Hash-partition $A$, $B$ into $\{A_i\}_{i=1}^n$, $\{B_i\}_{i=1}^n$\; \label{step:hash_partition}

%Parity encode $\{A_i\}_{i=1}^n$, $\{B_i\}_{i=1}^n$ into $A[1..n]$, $B[1..n]$\; \label{step:parity_encode}

{\it Bob}: BCH-Encodeing $B[1..n]$ and send the codeword to Alice\; \label{step:BCH_encode}

{\it Alice}: Upon receiving the codeword, decode the bit errors between $A[1..n]$ and $B[1..n]$\; \label{step:BCH_decode}

{\it Alice}: For each bit error, start reconciling the corresponding subset pair by \autoref{alg:trivial_case}\; \label{step:trivial_reconcile}

{\it Bob}: Upon receiving the reconciled set difference $\hat{D}$, check whether $A=B\Delta \hat{D}$ via checksum\; \label{step:terminate_condition}
\end{algorithm}


% \subsubsection{Single-round PBS}\label{sec:single_round_pbs}

% Here we summarize all the steps of single-round PBS and represent it by pseudocode in \autoref{alg:single_round_pbs}. \autoref{step:hash_partition} and \autoref{step:parity_encode} operates at both hosts (i.e., Alice and Bob). \autoref{step:hash_partition} to \autoref{step:trivial_reconcile} have been elaborated from \autoref{sec:hash_partition} to \autoref{sec:reconcile_by_trivial}. The last step in \autoref{step:terminate_condition} aims to check whether reconciliation is complete (i.e., $\mathcal{D}=A\Delta B$). More specifically, Alice calculates the checksum (e.g., CRC-$32$) of $A$ and send it to Bob. Then Bob calculates the checksum of $B\Delta \mathcal{D}$ and compares it to the receiving checksum of $A$. If the two checksums are the same, we believe $A=B\Delta \mathcal{D}$ and therefore $\mathcal{D}=A\Delta B$ (i.e., reconciliation is complete); Else, we know some elements are reconciled incorrectly. We classify those elements (i.e., the ones in the set difference between $A\Delta B$ and $\mathcal{D}$) into two subsets $A\Delta B\!\setminus\!\mathcal{D}$ and $\mathcal{D}\!\setminus\!(A\Delta B)$ and refer the elements in the former as {\it false-negatives}, and refer the elements in the later as {\it false-positives}. 

% In the ideal case, neither false-positives nor false-negatives will happen and the two checksums always equal. However, in real life, the ideal case does not always happen. We will discuss the nonideal case in \autoref{subsec:exception_hash_partition}. In our evaluation, we use a $32$-bit checksum for comparing $A$ to $B\Delta \mathcal{D}$ that has {\bf an error probability} roughly $10^{-9}$. This error (i.e., mistake $A=B\Delta \mathcal{D}$) incurs false-negatives. All set reconciliation schemes have the same problem on their termination conditions (i.e., check whether $\mathcal{D}=A\Delta B$). For some super critical applications, we can certainly decrease the error probability by using more powerful checksums (i.e., $64-$bit). Using a $32$-bit checksum, this kind of false-negatives never happen in the evaluation. 
% %For simplification, we assume no error happens when checking $\mathcal{D}=A\Delta B$ in the rest of the paper.

% \begin{algorithm}
% \caption{Single-round PBS}
% \label{alg:single_round_pbs}

% Hash-partition $A$, $B$ into $\{A_i\}_{i=1}^n$, $\{B_i\}_{i=1}^n$\; \label{step:hash_partition}

% Parity encode $\{A_i\}_{i=1}^n$, $\{B_i\}_{i=1}^n$ into $A[1..n]$, $B[1..n]$\; \label{step:parity_encode}

% {\it Bob}: Encode $B[1..n]$ by BCH code, then send the codeword to Alice\; \label{step:BCH_encode}

% {\it Alice}: Upon receiving the codeword, decode the bit errors between $A[1..n]$ and $B[1..n]$\; \label{step:BCH_decode}

% {\it Alice}: For each bit error, reconcile the corresponding subset pair by \autoref{alg:trivial_case}\; \label{step:trivial_reconcile}

% {\it Bob}: Upon the reconciled distinct elements $\mathcal{D}$, check whether $A=B\Delta \mathcal{D}$ via checksum\; \label{step:terminate_condition}
% \end{algorithm}

\subsubsection{Exception Handling}\label{subsec:exception_hash_partition}

When the ideal case does not happen, some subset pair may contain more than $1$ distinct elements and cannot be successfully reconciled by \autoref{alg:trivial_case}. Due to the parity encoding, we can classify the exceptions that happens in such a subset pair into the following two types of events: 

\noindent {\bf Type (\RN{1})}: Subset pair $(A_i, B_i)$ contains even number ($\geq 2$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be the same and PBS will not reconcile the subset pair yet in this round. This event happens with a small but nontrivial probability: For example, $d=5$ and $n=255$ (i.e., throwing $5$ balls uniformly and randomly into $255$ bins), the probability that some bin has $2$ or $4$ balls is roughly $0.04$. 
Note that when a type (\RN{1}) event happens, the $32$-bit checksum (\autoref{step:terminate_condition} in \autoref{alg:single_round_pbs}) can detect that the set reconciliation has not been completed. Then PBS will start another round of set reconciliation to reconcile the ``hidden'' distinct elements (the ones that have not been reconciled in the first round), 
%so on so force, until all distinct elements are successfully reconciled and the checksum is verified to be correct, 
as we will describe in \autoref{sec:multi-rounds}. 

% Note that when a Type (\RN{1}) subset pair exists, the $32$-bit checksum (\autoref{step:terminate_condition} in \autoref{alg:single_round_pbs}) can almost surely detect that the set reconciliation is incomplete. If this is the case (i.e., the checksum is verified to be incorrect), PBS will start another round of set reconciliation to reconcile the remaining distinct elements (e.g., the ``hidden'' distinct elements in Type (\RN{1}) subset pairs), so on so force, until all distinct elements are reconciled and the checksum is verified to be correct, as we will describe in \autoref{sec:multi-rounds}. 

\noindent {\bf Type (\RN{2})}: Subset pair $(A_i, B_i)$ contains odd number ($\geq 3$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be different and PBS will reconcile the subset pair using \autoref{alg:trivial_case}. The reconciled element (i.e., $s$ in \autoref{alg:trivial_case}) is however a ``fake'' distinct element, which is actually the bitwise \code{XOR} of all distinct elements in $(A_i, B_i)$ (explained in \autoref{subsec:protocol0}).
%, which will be mistakenly believed as the distinct element of $(A_i, B_i)$. 
This event happens with a tiny probability: Use the same example ($d=5$ and $n=255$), the probability that some bin has $3$ or $5$ balls is roughly $1.52\times 10^{-4}$. Similarly, the $32$-bit checksum can also detect that the set reconciliation has not been completed when a type (\RN{2}) event happens. Both the ``hidden'' and the ``fake'' distinct elements can also be reconciled in later rounds. 

Note that those ``fake'' distinct elements will become new distinct elements in the next round and therefore incur additional communication overhead to reconcile. To reduce this additional communication overhead, we add a verification on each reconciled distinct element of \autoref{alg:trivial_case} that can detect ``fake'' distinct elements with high probability. \autoref{alg:verification} shows how this verification works, and it does not incur additional communication overhead.

\begin{algorithm}
\caption{Verify reconciled element $s$ of $(A_i, B_i)$}
\label{alg:verification}
\If{$h(s)\neq i$} {Discard the reconciled element $s$;}
\end{algorithm}

Although a distinct element of $(A_i, B_i)$ must be in sub-universe $\mathcal{U}_i$ (i.e., the hash value of the element under $h$ equals to $i$), a ``fake'' distinct element could be in any sub-universe with probability $1/n$, since it is the bitwise \code{XOR} of all distinct elements of $(A_i, B_i)$. Therefore, \autoref{alg:verification} only fails to identify a ``fake'' distinct element with probability $1/n$, which is roughly $3.9\times 10^{-3}$ when $n=255$. On top of the probability of type (\RN{2}) events, a ``fake'' distinct element that cannot be detect by \autoref{alg:verification} appears with probability $6\times 10^{-7}$. {\bf To simplify our description, we also ignore this small probability event and assume all ``fake'' distinct elements are successfully detected by \autoref{alg:verification} in this rest of this paper. (I feel that defining $\tilde{a}_4=a_1\oplus a_2\oplus a_3$ does not help much.)}

{\bf Readers may wonder encoding the exact subset cardinalities (i.e., $|A_i|, |B_i|$) instead of their oddness / evenness (parity) (described in \autoref{sec:hash_partition}) could help to detect and solve Type (\RN{1}), (\RN{2}) events. However, encoding the exact subset cardinalities not only incurs much more additional communication overhead comparing to encoding their parities, but also barely helps on detecting Type (\RN{1}), (\RN{2}) events, since we cannot precisely derive $|A_i\Delta B_i|$, the total number of distinct elements in $(A_i, B_i)$, even knowing $|A_i|, |B_i|$: For instance, when $|A_i|\!=\!|B_i|\!=\!50$, $|A_i\Delta B_i|$ could be any even number ($\leq 100$) if the distinct elements are evenly splitted and placed between $A_i$ and $B_i$. }

% As we have described in \autoref{sec:hash_partition}, the ideal case does not always happen, which means some subset pair may contain more than $1$ distinct elements and cannot be successfully reconciled by \autoref{alg:trivial_case}. Due to the parity encoding, we can classify such subset pair into the following two scenarios:

% \begin{itemize}
%     \item Scenario 1: If a subset pair $(A_i, B_i)$ contains even number ($\geq 2$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be the same and PBS will not reconcile the subset pair yet in this round;
%     \item Scenario 2: If a subset pair $(A_i, B_i)$ contains odd number ($\geq 3$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be different and PBS will reconcile the subset pair using \autoref{alg:trivial_case}. The reconciled element (i.e., $s$ in \autoref{alg:trivial_case}) is however the bitwise \code{XOR} of all distinct elements in $(A_i, B_i)$ (explained in \autoref{subsec:protocol0}), which will be mistakenly believed as the distinct element of $(A_i, B_i)$. 
%     %However, as described in \autoref{subsec:protocol0}, when a subset pair contains more than $1$ distinct elements, \autoref{alg:trivial_case} will output the bitwise \code{XOR} of them as the `distinct element', which is not an actual distinct element with high probability;
% \end{itemize}

% In both scenarios, the distinct elements in the subset pair will not be reconciled in this round. As we will describe in \autoref{sec:multi-rounds}, we generalize PBS into multi-round, so that the distinct elements that have not been reconciled in the first round will be reconciled in later rounds. On the other hand, the second scenario could result in incorrectly reconciled distinct elements, which will become new distinct elements in the next round in multi-round PBS. 

% % In both scenarios, the distinct elements in the subset pair cannot be successfully reconciled in this round and will remain in the set difference (i.e., $(A\Delta B)\!\setminus\!\hat{D}$). On the other hand, the incorrectly reconciled distinct element in the second scenario will appear as a new distinct element (i.e., $\hat{D}\!\setminus\!(A\Delta B)$) in the next round if we generalize PBS into multi-round (to be elaborated in \autoref{sec:multi-rounds}). Both scenarios can be almost surely detected by the 32-bit checksum (\autoref{step:terminate_condition} in \autoref{alg:single_round_pbs}). The set difference after the reconciliation in this round, $D\Delta\hat{D}$, can be reconciled in later rounds, as we will describe in \autoref{sec:multi-rounds}. 

% Naturally, we do not want to generate new distinct elements in the process of set reconciliation, even though it happens with a tiny probability when $n=\Omega(d^2)$: For instance, when $d=5$ and $n=255$ (i.e., throwing $5$ balls uniformly and randomly into $255$ bins), the probability (i.e., some bin has $3$ or $5$ balls) is only $7.6\times 10^{-6}$. Therefore, we add a verification with no additional communication cost on each reconciled element of \autoref{alg:trivial_case}, such that each incorrect dinstinct element can be identified with high probability. The verfication is shown in \autoref{alg:verification}. 

% \begin{algorithm}
% \caption{Verify reconciled element $s$ of $(A_i, B_i)$}
% \label{alg:verification}
% \If{$h(s)\neq i$} {Discard the reconciled element $s$;}
% \end{algorithm}

% Although any distinct element of $(A_i, B_i)$ must be in sub-universe $\mathcal{U}_i$ (i.e., the hash value of the element under $h$ equals to $i$), the bitwise \code{XOR} of multiple distinct elements of $(A_i, B_i)$ could be in any sub-universe with probability $1/n$. Therefore, \autoref{alg:verification} fails to identify an incorrectly reconciled distinct element in the second scenario with probability $1/n$ that is roughly $3.9\times 10^{-3}$ when $n=255$. In other words, an incorrectly reconciled distinct element that cannot be identified by \autoref{alg:verification} appears with probability $3\times 10^{-8}$. {\bf I feel that defining $\tilde{a}_4=a_1\oplus a_2\oplus a_3$ does not help much.}

% In both scenarios, the distinct elements in the subset pair cannot be successfully reconciled in this round. These distinct elements can be reconciled in later rounds if needed, as we will describe in \autoref{sec:multi-rounds}. In this section, we only discuss how to identify the {\it incorrect} distinct element in the second scenario. Let us use an example to elaborate the second scenario: Assume $(A_i, B_i)$ contains $3$ distinct elements $a_1, a_2, a_3$, then Bob computes $\tilde{s}=a_1\oplus a_2\oplus a_3$ using \autoref{alg:trivial_case} and mistakes it as the distinct element in $(A_i, B_i)$. 

% In both scenarios, the distinct elements in the subset pair cannot be successfully reconciled (i.e., false-negatives defined in \autoref{sec:single_round_pbs}. The distinct elements that are not successfully reconciled in this round, if needed, can be reconciled in later rounds as we will describe in \autoref{sec:multi-rounds}. In this section, we only discuss how to identify the {\it incorrect} distinct elements in the second scenario. Let us use an example to elaborate the second scenario: Assume $(A_i, B_i)$ contains $3$ distinct elements $a_1, a_2, a_3$, then Bob computes $\tilde{s}=a_1\oplus a_2\oplus a_3$ using \autoref{alg:trivial_case} and mistakes it as the distinct element in $(A_i, B_i)$. 

\begin{comment}
============================================

We add a no-communication-cost verification step to check whether a reconciled element is an actual distinct element or not. Note that an actual distinct element of $(A_i, B_i)$ must be in sub-universe $\mathcal{U}_i$. On the other hand, an incorrectly reconciled element (e.g., $\tilde{s}$) can be in any sub-universe with probability $1/n$. So at the end \autoref{subsec:protocol0}, we check whether the reconciled element is in $\mathcal{U}_i$ by the hash function $h$ in hash-partition:

This verfication cannot completely eliminate false-positives, since an incorrectly reconciled element (e.g., $\tilde{s}$) can coincidentally end up in $\mathcal{U}_i$ with probability $1/n$. The chance of false-positives is extremely small using the verification. For instance, if $d=5$ and $n=255$, the probability of the second scenario is only $7.6\times 10^{-6}$. The probability of false-positives using the verfication is $1/n$ times this small probability, which is roughly $3\times 10^{-8}$. {\bf Note that a small probability of false-positives only costs a little waste on set reconciliation when synchronizing objectives (e.g., files), which is acceptable for most applications.}

Even worse, in the second scenario, the false-positives defined in \autoref{sec:single_round_pbs} could happen. For example, if subset pair $(A_i, B_i)$ contains $3$ distinct elements $s_1, s_2, s_3$, then \autoref{alg:trivial_case} computes $\tilde{s}=s_1\oplus s_2\oplus s_3$ and Bob mistakes $\tilde{s}$ as an actual distinct element. The good thing is, the probability of this kind of false-positives is extremely small for small $d$. For instance, if $d=5$ and $n=255$, the probability of the false-positives is only $7.6\times 10^{-6}$. To further reduce the chance of false-positives, we add a no-communication-cost verification step at the end of \autoref{subsec:protocol0} to check whether $\tilde{s}$ is an actual distinct element or not. The verification step works as follows: Given the output $s$ of subset pair $(A_i,B_i)$, if $s\in\mathcal{U}_i$ (i.e., $h(s)=i$), we consider $s$ as an actual distinct element; Otherwise, we consider $s$ as an incorrect output and discard it. 

Note that if $\tilde{s}\in A_i\Delta B_i$, $\tilde{s}$ must be in sub-universe $\mathcal{U}_i$. However, if $\tilde{s}$ is the bitwise \code{XOR} of the distinct elements in $(A_i,B_i)$ (i.e., the second scenario happens), it ends up in $\mathcal{U}_i$ with probablity of only $1/n$. 
%In fact, if we assume the hash-partition described in \autoref{sec:hash_partition} hashes the elements of $\mathcal{U}$ uniformly, independently, and randomly into $n$ sub-universes, the output $s$ in the second scenario will be in a different sub-universe $\mathcal{U}_j (j\neq i)$ with a high probability of $1-\frac{1}{n}$. Hence, this verfication method can further reduce the probability of false-positives by a factor of $\frac{1}{n}$. 
Use the same example (i.e., $d=5$, $n=255$), the probability of this kind of false-positives is reduced from $7.6\times 10^{-6}$ to $3\times 10^{-8}$ by this verification method. 
%{\bf This probability can be further reduced in \autoref{subsec:protocol2}, where PBS does two tiers of hash-partitions. So we can do verification on both of the two hash functions.}

%In some super critical cases (i.e., no false-positive is allowed), we can use a more powerful verification method to completely eliminate false-positives. That is, to check if the output $s$ exists in exactly one of the two sets (i.e., $s\in A\!\setminus\! B$ or $s\in B\!\setminus\! A$). To do so, Bob transmits $s$ along with an identification bit $\mathbbm{1}_{\{s\in B\}}$ to Alice, then Alice checks if $s\in (A\!\setminus\! B)\bigcup (B\!\setminus\! A)$ . This method verification costs additional $d(\log u+1)$ bits of communication overhead. In most applications, this rigorous $0\%$ probability guarantee of false-positives is unnecessary and the probability of the former verification method is small enough, so we use the former in the evaluation. Based on our observation, this kind of false-positives do not happen even once in the evaluation using the former verfication method. In the rest of this paper, we assume Scenario 2 is always correctly verified. 

============================================
\end{comment}

\subsection{Running PBS for Multiple Rounds}\label{sec:multi-rounds}

When the ideal case does not happen (i.e., type (\RN{1}) or type (\RN{2}) event happens), PBS will know the set reconciliation has not be completed by the $32$-bit checksum (\autoref{step:terminate_condition} in \autoref{alg:single_round_pbs}). To reconcile those distinct elements that have not been reconciled yet in the first round, we rule out all successfully reconciled elements and run another round of PBS. This procedure replicates until all distinct elements are successfully reconciled the checksum is verified to be correct.

More specifically, in the second round, we run PBS to reconcile $A$ and $B\Delta \hat{D}$ instead of $A$ and $B$ to rule out all elements that have been reconciled, where $\hat{D}$ is the set of reconciled distinct elements in the first round. We use a different hash function for hash-partition in the second round to avoid the same exceptions (i.e., type (\RN{1}) or type (\RN{2}) event) that happened in the first round happen again. The later rounds are similarly operated. 

{\bf Normally, we want PBS to successfully reconcile all distinct elements in only a few rounds (say $3$) with high probability (say $99\%$). Hence, when tuning parameters (to be discussed in \autoref{sec:parameter_settings}), we set a {\it target success probability} $p_0$ of $r$ rounds as a paramenter setting requirement, which aims to ensure the probability that all distinct elements are reconciled in $r$ rounds to be larger than $p_0$. This requirement should also ensure the majority of the distinct elements are reconciled in the first round. Use the same example ($d=5, n=255$), on average $4.81$ out of $5$ distinct elements should be reconciled in the first round. So the total communication overhead in all rounds is only slightly larger than ($1.01$ to $1.07$ times of, as we will show in \autoref{fig:per-round-con}) that in the first round. Due to this reason, we use the communication overhead in the first round (described in \autoref{sec:communication_overhead_single_PBS}) to approximate the total communication overhead of all rounds in parameter settings (to be elaborated in \autoref{sec:parameter_settings}.}

% Although PBS may need to run many rounds to reconcile all distinct elements, the communication overhead mostly happens in the first round, since the majority of the distinct elements should be reconciled in the first round. Use the same example ($d=5, n=255$), on average $4.81$ out of $5$ distinct elements should be reconciled in the first round. So the total communication overhead in all rounds is only slightly larger than ($1.01$ to $1.07$ times of, to be shown in \autoref{fig:per-round-con}) that in the first round. Due to this reason, we use the communication overhead in the first round (described in \autoref{sec:communication_overhead_single_PBS}) to approximate the total communication overhead (all rounds) in parameter settings (to be elaborated in \autoref{sec:parameter_settings}).

%For the moment, we assume no ``fake'' distinct element in type (\RN{2}) subset pairs fails to be detected, which happens with overwhelming probability as explained in \autoref{subsec:exception_hash_partition}. Then 
PBS reconciles the distinct elements gradually round by round. This is the ``piecewise decodability'' mentioned in \autoref{sec:intro_oursolution}. We use the following example to describe it in details: 
Given two sets with $10$ distinct elements, in the first round, PBS tries to reconcile the $10$ distinct elements and say $6$ out of the $10$ distinct elements are successfully reconciled. Then the $6$ reconciled distinct elements are removed and PBS tries to reconcile the remaining $4$ distinct elements in the second round. Say $2$ out of the $4$ remaining distinct elements are successfully reconciled, and that leaves $2$ remaining distinct elements to be reconciled in the third round, so on so force. 
% Given two sets $A$, $B$ with $10$ distinct elements, in the first round, PBS hashes them into $7$ distinct subset pairs. $6$ distinct elements are hashed into $6$ distinct subset pairs, and the other $4$ distinct elements are hashed into the same subset pair. Then the former $6$ distinct elements are successfully reconciled in the first round and the later $4$ distinct elements remain to be reconciled in the second round, which are hashed into $3$ distinct subset pairs (under a different hash function). $2$ remaining distinct elements are hashed into $2$ distinct subset pairs, and the other $2$ remaining distinct elements are hashed into the same subset pair. Then the former $2$ remaining distinct elements are successfully reconciled in the second round and the later $2$ remaining distinct elements remain to be reconciled in the third round, so on so force. 
The dynamics of the number of remaining distinct elements (i.e., $10\leadsto 4\leadsto 2\leadsto \cdots$ in the example) is in nature a Markov chain, which will be elaborated and analyzed in \autoref{sec:single_markov} to derive a tight tail bound of the probability that all distinct elements are reconciled in $r$ rounds.

% Even if the ideal case does not happen, most of the distinct elements should be distributed into different subset pairs, one distinct element in each, and therefore can be successfully reconciled. So in the first round, even if PBS cannot reconcile all distinct elements, it can reconcile the majority of them.
% % (piecewise decodability mentioned in \autoref{sec:intro_oursolution})
% Based on this intuition, we generalize PBS to multi-round, so that the distinct elements that are not reconciled yet in the first round can be reconciled in later rounds.  

% Without loss of generality, we only describe the second round of multi-round PBS, the reconciliation in the later rounds are similar. Let $\hat{D}_1$ denote the set of reconciled elements in the first round. If set reconciliation is not complete in the first round (i.e., the checksum infers $A\neq B\Delta \hat{D}_1$), then multi-round PBS saves $\hat{D}_1$, which includes correctly and incorrectly reconciled elements as described in \autoref{subsec:exception_hash_partition}, and starts the second round to find (1) the remaining distinct elements; (2) the incorrectly reconciled distinct elements in the first round. In the second round, multi-round PBS reconciles $A$ and $B\Delta \hat{D}_1$ instead of $A$ and $B$ (i.e., $B\leftarrow B\Delta\hat{D}_1$) to rule out all elements that have been reconciled. {\bf It uses a hash function that is different from the one used in the first round for hash-partition, otherwise every remaining distinct element will be hashed into the same subset pair and cause the same exception (described in \autoref{subsec:exception_hash_partition}) that happened in the first round.}

% If set reconciliation is complete in the second round, the set of reconciled elements in the second round (denoted as $\hat{D}_2$) should be the union of (1) all distinct elements that have not been reconciled in the first round (i.e., $(A\Delta B)\!\setminus\!\hat{D}_1$); and (2) all incorrectly reconciled elements in the first round (i.e., $\hat{D}_1\!\setminus\!(A\Delta B)$), which is by definition the set difference between $A\Delta B$ and $\hat{D}_1$. Therefore, the overall set difference $A\Delta B$ equals to the set difference between $\hat{D}_1$ and $\hat{D}_2$; Else, multiround PBS saves $\hat{D}_2$ and starts the third round, so on so force. 

% {\bf May need this algorithm to show the dynamics, if so, the earlier algorithm needs to change accordingly.}
% \IncMargin{1em}
% \begin{algorithm}
% \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
% \Input{$A$ and $B$}
% \Input{Maximum number of rounds $r$}
% \Output{$D$}

% $\hat{D},\mbox{ complete} \leftarrow PBS(A,B)$\;

% $D \leftarrow \hat{D}$\;

% \While{!complete and $r>0$}{
	
% 	$B \leftarrow B\Delta\hat{D}$\;

% 	$\hat{D},\mbox{ complete} \leftarrow PBS(A,B)$\;

% 	$D \leftarrow D\Delta\hat{D}$\;

% 	$r \leftarrow r-1$\;
% }

% \caption{Multi-round PBS} \label{proto:multirounds}
% \end{algorithm}\DecMargin{1em}

% The idea of multi-round PBS is quite simple: In each round, we discard the reconciled distinct elements in the previous rounds and aim to find the rest distinct elements from the remaining elements. More specifically, the first round of multi-round PBS is just the same as single-round PBS in \autoref{alg:single_round_pbs}. The second round has the same procedures as the first round. One difference is, we update $B$ by $B\leftarrow B\Delta\mathcal{D}$ in the second round, so that (1) Reconciled distinct elements in $\mathcal{D}$ that were contained in $A\Delta B$ are not longer contained in $A\Delta (B\Delta\mathcal{D})$; and (2) The other distinct elements remain in $A\Delta (B\Delta\mathcal{D})$ and can be reconciled later. The other difference is, we use a different hash function for partition (\autoref{step:hash_partition}) in the second round. Later rounds update $B$ in the same way and also use different hash functions. Multi-round terminates if the check in \autoref{step:termination} is correct. The overall set difference $A\Delta B$ is simply the union of reconciled distinct elements in all rounds. 

% A straightforward approach to discard reconciled distinct elements is to remove them from both $A$ and $B$. This approach however incurs additional communication overhead to update $A$, since only Bob learns the partial set difference in \autoref{step:reconcile}. Therefore, we use the approach in \autoref{step:updateb} that only updates $B$. It has another benefit in \autoref{step:termination}, which only needs to transmit the CRC of $A$ from Alice to Bob in the first round. In the later rounds, \autoref{step:termination} can be checked locally by Bob and does not require any additional communication overhead;

% Note that the communication overhead in the first round accounts for a large percentage of the total communication overhead in multi-round PBS, since most of the distinct elements (over $95\%$ as we will show in {\bf point to the figure}) should be reconciled in the first round. Therefore, we use the same parameter $n$ in later rounds because otherwise we have to compute a new parameter that can only save tiny communication overhead, even though the number of remaining distinct elements is small and can be reconciled using smaller $n$ with high probability. {\bf Due to the same reason, we can the same expression of the communication overhead in single-round PBS to approximate the communication overhead in multi-round PBS.}

% The natural termination condition of multi-round PBS is that all distinct elements are reconciled, which could require a large number of rounds and incur large additional communication overhead (each additional round incurs $d\log n$ bits of additional communication overhead on transmitting BCH codeword). To control the amount of additional communication overhead, we set another termination condition that multi-round PBS runs for at most $r$ rounds (typically $2$ or $3$). This termination condition could cause an `early' termination when some distinct elements have not been reconciled. However, under proper parameter settings (to be discussed in \autoref{sec:parameter_settings}), we can prove that the probability of an `early' termination (i.e., set reconciliation is incomplete in $r$ round) is very small
% %, and even if an `early' termination happens, an overwhelming percentage of distinct elements should have been reconciled, which is sufficient for most applications
% . For example, when $d=5, n=255, r=2$, an `early' termination happens with probability $4.8\times 10^{-4}$ (how to compute this probability will be elaborated in \autoref{sec:tail_bound}).

% For the moment, we assume no incorrectly reconciled distinct elements appears in multi-round PBS, which happens with overwhelming probability as explained in \autoref{subsec:exception_hash_partition}. Then multi-round PBS reconciles the distinct elements gradually round by round. This is the ``piecewise decodability'' mentioned in \autoref{sec:intro_oursolution}. We use the following example to describe it in details: Given two sets $A$, $B$ with $10$ distinct elements (i.e., $d=10$), in the first round, multi-round PBS hashes them into $7$ distinct subset pairs. $6$ distinct elements are hashed into $6$ distinct subset pairs, and the other $4$ distinct elements are hashed into the same subset pair. Then the former $6$ distinct elements are successfully reconciled in the first round and the later $4$ distinct elements remain to be reconciled in the second round, which are hashed into $3$ distinct subset pairs (under a different hash function). $2$ remaining distinct elements are hashed into $2$ distinct subset pairs, and the other $2$ remaining distinct elements are hashed into the same subset pair. Then the former $2$ remaining distinct elements are successfully reconciled in the second round and the later $2$ remaining distinct elements remain to be reconciled in the third round, so on so force. The dynamics of the number of remaining distinct elements (i.e., $10\leadsto 4\leadsto 2\leadsto \cdots$ in the example) is in nature a Markov chain, which will be elaborated and analyzed in \autoref{sec:tail_bound_per_group} to derive a tail bound of success probability (i.e., all distinct elements are reconciled in $r$ rounds) for paramenter settings. 

% In most applications, a high percentage of reconciliation (e.g., $>99\%$ distinct elements are reconciled) is good enough. Therefore, we add another termination condition on the maximum number of rounds (denoted as $r$). The larger $r$ is, the higher percentage of distinct elements will be reconciled. How to set parameters based on $r$ will be elaborated in \autoref{sec:parameter_settings};

% Readers may think the communication overhead of multi-round PBS is proportional to the number of rounds. In fact, the majority of the communication overhead is spent in the first round, since most of the distinct elements (over $95\%$ as we will show in {\bf point to the figure}) are reconciled in the first round. Each additional round only incurs a small amount of additional communication overhead. For example, when $d=10, n=255, |\mathcal{U}|=2^{32}$, assume $8$ distinct elements are reconciled in the first round and the rest $2$ distinct elements are reconciled in the second round. Then the communication overhead in the first round is $432$ bits. That number of the second round is only $160$


%the communication overhead of single-round PBS of $272$ ($2d\log n+d\log |\mathcal{U}|+32$) bits, and each additional round incurs $40$ ($d\log n$) bits of additional communication overhead. 

%among the three components of the communication overhead mentioned in \autoref{sec:communication_overhead_single_PBS}, only the first component (i.e., the BCH codeword) is proportional to the number of rounds. The other two components does not depend on the number of rounds.

% The second component only depends on the total number reconciled elements, which is roughly equal to $d$. The third component, the checksum of $A$, only needs to be sent once in the first round.
%Therefore, the communication overhead of multi-round PBS is only slightly larger than that of single-round PBS when the number of rounds is small (say $3$). For example, when $d=5, n=255, |\mathcal{U}|=2^{32}$, the communication overhead of multi-round PBS of $3$ rounds is $352$ bits, which is roughly $1.3$ times of the communication overhead of single-round PBS ($272$ bits).

% Therefore, each additional round of multi-round PBS only incurs a small amount of additional communication overhead. For example, when $d=5, n=255, |\mathcal{U}|=2^{32}$, the communication overhead of single-round PBS of $272$ ($2d\log n+d\log |\mathcal{U}|+32$) bits, and each additional round incurs $40$ ($d\log n$) bits of additional communication overhead. 

% As we explained in \autoref{sec:reconcile_by_trivial}, the communication overhead in each round is proportional to the number of (remaining) distinct elements, which decreases exponentially as the number of round increase (i.e., the first round reconciles $90\%$ of distinct elements, the second round reconciles $90\%$ of the remaining $10\%$ distinct elements, etc.). So the majority of the communication overhead (i.e., $\approx 90\%$) is in the first round. Therefore, we do not bother to optimize parameters (i.e., smaller $n$) in later rounds to save tiny communication overhead, even though remaining distinct elements become fewer and can be reconciled using smaller $n$;

% The termination condition of multi-round PBS is that all distinct elements are reconciled, which may require many rounds. In most applications, a high percentage of reconciliation (e.g., $>99\%$ distinct elements are reconciled) is good enough. Therefore, we add another termination condition on the maximum number of rounds (denoted as $r$). The larger $r$ is, the higher percentage of distinct elements will be reconciled. How to set parameters based on $r$ will be elaborated in \autoref{sec:parameter_settings};

% Multi-round means multiple round-trip delays. {\bf Thanks for the piecewise decodability of PBS, in almost all practical application scenarios, this tradeoff does not lead to longer response time because the reconciliation of objects identified by the successfully decodable codewords, which constitute the vast majority of all codewords, can run in parallel with the transmissions and decodings of the rest.  In other words, the piecewise decodability effective masks the slightly larger number of communication rounds as far as the response time is concerned.}

\begin{comment}
==============================

The pseudocode of set reconciliation operations in each round is shown as follows:

\IncMargin{1em}
\begin{algorithm}
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
\Input{$A$ and $B^{(in)}$}
\Input{Set of reconciled distinct elements $D^{(in)}$}
\Output{$B^{(out)}$}
\Output{Set of reconciled distinct elements $D^{(out)}$}

% Hash-partition $A^{(in)}$, $B^{(in)}$ into $\{A^{(in)}_i\}_{i=1}^n$, $\{B^{(in)}_i\}_{i=1}^n$ (\autoref{sec:hash_partition})\label{step:hash_partition}\;

% Encode $\{A^{(in)}_i\}_{i=1}^n$, $\{B^{(in)}_i\}_{i=1}^n$ into parity bitmaps (\autoref{sec:parity_bitmap_encoding})\;


% Find those subset pairs (denoted them as $(A^{(in)}_{i_1}, B^{(in)}_{i_1}), ...,(A^{(in)}_{i_k}, B^{(in)}_{i_k})$) that parity bits differ (\autoref{sec:BCH_code})\;

Run single-round PBS on $A$ and $B^{(in)}$ to obtain the (partial) set difference $\mathcal{D}$\label{step:reconcile} \;

$D^{(out)} \leftarrow D^{(in)}\bigcup \mathcal{D}$\label{step:updated}\;

$B^{(out)} \leftarrow B^{(in)}\Delta\mathcal{D}$\label{step:updateb}\;

Check whether the set reconciliation is complete by comparing $A$ to $B^{(out)}$ (via CRC)\label{step:termination}\;

\caption{Set reconciliation operations of PBS in each round} \label{proto:multirounds}
\end{algorithm}\DecMargin{1em}

In \autoref{proto:multirounds}, the output $B^{(out)}$ in the $r^{th}$ round is the input $B^{(in)}$ in the $(r+1)^{th}$ round. $D^{(in)}$ and $D^{(out)}$ have the same relationship, and they denote the set of reconciled distinct elements before and after a round. $B^{(in)}$ and $D^{(in)}$ are initialized as $B$ and $\emptyset$ respectively. We omit the currect number of round $r$ in \autoref{proto:multirounds}, since the operations in different rounds are exactly the same. Due to the same reason, we only elaborate the operations in the first round: First, Alice and Bob reconcile $A$ and $B^{(in)}$ $(=B)$ using single-round PBS and Bob obtains the (partial) set difference $\mathcal{D}$ (\autoref{step:reconcile}); Second, Bob updates the set of reconciled distinct elements by merging it with $\mathcal{D}$ (\autoref{step:updated}); Third, Bob updates $B^{(in)}$ $(=B)$ to $B^{(out)}$ as \autoref{step:updateb} shows, such that (1) The reconciled distinct elements in $\mathcal{D}$ that are contained in $A\Delta B^{(in)}$ are not longer contained in $A\Delta B^{(out)}$; and (2) The distinct elements that are not successfully reconciled remain in $A\Delta B^{(out)}$ and can be reconciled in later rounds; Finally, we check whether all distinct elements are reconciled. Note that if it is true, $B^{(out)}$ should be the same as $A$ and multi-round PBS should terminate. We use a $32$-bit CRC (Cyclic Reduncancy Check) to check if $B^{(out)}=A$ in our evaluation. {\bf To achieve higher confidence, we can certainly use longer CRC (e.g., 64-bit). }

{\bf Remarks:}

(1) In each round, hash-partition in \autoref{sec:hash_partition} uses different hash functions, so that the remaining distinct elements from the last round will be hashed into different subset pairs with high probability;

(2) A straightforward approach to discard reconciled distinct elements is to remove them from both $A$ and $B$. This approach however incurs additional communication overhead to update $A$, since only Bob learns the partial set difference in \autoref{step:reconcile}. Therefore, we use the approach in \autoref{step:updateb} that only updates $B$. It has another benefit in \autoref{step:termination}, which only needs to transmit the CRC of $A$ from Alice to Bob in the first round. In the later rounds, \autoref{step:termination} can be checked locally by Bob and does not require any additional communication overhead;

(3) As we explained in \autoref{sec:reconcile_by_trivial}, the communication overhead in each round is proportional to the number of remaining distinct elements, which decreases exponentially as the number of round increase (i.e., the first round reconciles $90\%$ of distinct elements, the second round reconciles $90\%$ of the remaining $10\%$ distinct elements, etc.). So the majority of the communication overhead (i.e., $\approx 90\%$) is in the first round. Therefore, we do not bother to optimize parameters (i.e., smaller $n$) in later rounds to save tiny communication overhead, even though remaining distinct elements become fewer and can be reconciled using smaller $n$;

(4) One termination condition of Multi-round PBS is $B^{(out)}=A$, which refers that all distinct elements are reconciled. In most applications, a high percentage of reconciliation (e.g., $>99\%$ distinct elements are reconciled) is good enough. Therefore, we add another termination condition of the maximum number of rounds (denoted as $r$). The larger $r$ is, the higher percentage distinct elements will be reconciled, and the smaller $n$ is required. How to set parameters (e.g., $n$) based on $r$ will be elaborated in \autoref{sec:parameter_settings};

(5) Multi-round means multiple round-trip delays. {\bf Thanks for the piecewise decodability of PBS, in almost all practical application scenarios, this tradeoff does not lead to longer response time because the reconciliation of objects identified by the successfully decodable codewords, which constitute the vast majority of all codewords, can run in parallel with the transmissions and decodings of the rest.  In other words, the piecewise decodability effective masks the slightly larger number of communication rounds as far as the response time is concerned.}

==============================

\end{comment}

% (3) Readers may wonder in the later rounds, most distinct elements should be reconciled, and the rest distinct elements could be reconciled using degraded parameters (i.e., smaller $n$ and $t$). In fact, degrade parameters in later rounds cannot save much communication overhead, since the majority of it is spent in the first round (i.e., $>90\%$). Therefore, we use the same parameters (i.e., $n,t$) among all rounds in multi-rounds PBS;

% (4) The number of remaining distinct elements decreases exponentially as the number of round increase (i.e., the first round reconciles $90\%$ of distinct elements, the second round reconciles $90\%$ of the remaining $10\%$ distinct elements, etc.). 
% (4) The termination condition of Multi-rounds PBS is $B^{(out)}=A$ to reconcile all distinct elements. In some applications,  


% The output $B^{(out)}$ in the $r^{th}$ round is the input $B^{(in)}$ in the $(r+1)^{th}$ round. $D^{(in)}$ and $D^{(out)}$ are similarly defined. $B^{(in)}$ and $D^{(in)}$ are initialized as $B$ and $\emptyset$ respectively. Since and $D$ are updated in each round, so we use $B^{(in)}$ to denote the input and $B^{(out)}$ to denote the output respectively.  Specifically, in the first round, we initialize $B^{(in)}$ and $D^{(in)}$ as $B$ and $\emptyset$ respectively. we first use the single-round scheme 

% Then we run our (single-round) scheme on the updated two sets (i.e., after removing reconciled distinct elements) using a different (independent) hash-partition function from previous rounds, so that the rest distinct elements are hashed into different subset pairs (i.e., the ideal case) with high probability. At the end of each round, we check whether the set reconciliation is complete (i.e., all distinct elements are found) by computing the bitwise \code{XOR} of the remaining elements in $A$ and $B$ 
 

% This {\bf multi-rounds} scheme can significantly increase the success probability (i.e., the probability that all distinct elements are reconciled). Readers may wonder in the later rounds, most distinct elements should be reconciled, and the rest distinct elements could be reconciled using degraded parameters (i.e., smaller $n$ and $t$). In fact, degrade parameters in later rounds cannot save much communication overhead, since the majority of it is spent in the first round (i.e., $>90\%$). Therefore, we use the same parameters (i.e., $n,t$) among all rounds in our evaluation. 
% %The tradeoff between the number of rounds and the communication overhead per rounds will be elaborated in \autoref{sec:tail_bound}. In our evaluation, $r=2,3$ rounds are enough to achieve an extremely high success probability. 

% Readers may think the cost (i.e., communication overhead and the computational complexity) of this multi-rounds scheme is proportional to the number of rounds (denoted as $r$) and increases linearly with $r$. In fact, the cost of each round is roughly proportional to the number of remaining distinct elements, which decreases exponentially as $r$ increases (i.e., the first round reconciles $99\%$ of distinct elements, the second round reconciles $99\%$ of the remaining $1\%$ distinct elements, etc.). So the cost of this multi-rounds scheme is only slightly larger than that of the single-round scheme. Furthermore, as we explained in \autoref{sec:intro}, {\bf from intro thanks for the piecewise decodability of our solution, in almost all practical application scenarios, this tradeoff does not lead to longer response time because the reconciliation of objects identified by the successfully decodable codewords, which constitute the vast majority of all codewords, can run in parallel with the transmissions and decodings of the rest.  In other words, the piecewise decodability effective masks the slightly larger number of communication rounds as far as the response time is concerned.} 

\begin{comment}

\subsection{Baseline Scheme}\label{subsec:protocol1} 

Note that the set difference $A\Delta B$ can contain more than 1 elements (i.e., $d>1$), and \autoref{alg:trivial_case} cannot reconcile $A$ and $B$ directly in this case. Therefore, we propose a baseline scheme building upon~\autoref{alg:trivial_case} that also works when $d>1$: First, we partition the element universe $\mathcal{U}$ into $n$ sub-universes $\mathcal{U}_1, \mathcal{U}_2, \cdots, \mathcal{U}_n$. Denote $A_i \triangleq A\bigcap \mathcal{U}_i$ and $B_i \triangleq B\bigcap \mathcal{U}_i$ for $i=1,2,\cdots,n$. Then $\{A_i\}_{i=1}^n$ and $\{B_i\}_{i=1}^n$ are partitions of $A$ and $B$ respectively. Furthermore, $\Phi\triangleq\{A_i\Delta B_i\}_{i=1}^n$ is a partition of $A\Delta B$. 

Assume the {\bf ideal case} happens, in which each subset pair $(A_i, B_i)$ contains at most one distinct element ({\it i.e.,} $|A_i\Delta B_i|\!\leq\!1$), we use \autoref{alg:trivial_case} to reconcile each subset pair and obtain $A_i\Delta B_i$ for $i=1,2,\cdots,n$. The overall set difference $A\Delta B$ is simply their union $\bigcup_{i=1}^n \big{(}A_i\Delta B_i\big{)}$. 

In the first step of the baseline scheme, we can use a hash function $h(\cdot): \mathcal{U}\rightarrow \{1,2,\cdots,n\}$ to partition the universe $\mathcal{U}$ into $n$ sub-universes: $\mathcal{U}_i=\{s\mid s\in \mathcal{U} \mbox{ and } h(s)=i\}$ for $\forall i=1,2,\cdots,n$. And the hash function $h(\cdot)$ can be predetermined between Alice and Bob and does not require additional communication cost.

This hash-partition can be modeled as a {\it balls-into-bins problem}, in which the distinct elements are viewed as balls and the subset pairs are viewed as bins. The hash-parition basically throws (hashes) $d$ balls (distinct elements) uniformly and randomly into $n$ bins (subset pairs). The aforementioned ideal case in this context becomes, after throwing $d$ balls uniformly and randomly into $n$ bins, each bin receives at most 1 ball (i.e., $d$ nonempty bins have 1 ball in each and the rest $n-d$ bins are empty). {\bf It may remind readers about the Birthday problem. And the ideal case can be analogous to the case that no people share the same birthday.} The ideal case happens with a probability of $p=\frac{n\,!}{(n-d)\,!n^d}\!=\!\prod_{k=1}^{d - 1}(1 - \frac{k}{n})\!\approx\! e^{-\frac{d(d-1)}{2n}}$ when $d\!\ll\!n$. In other words, $n$ must be $\Omega(d^2)$ to ensure the ideal case happens with a nontrivial probability.  Note that the communication overhead of the baseline scheme is proportional to $n$, as each subset pair requires communication of a bitwise \code{XOR} in \autoref{alg:trivial_case}. So this communication overhead increases at least quadratically as $d$ increases. 

In fact, this communication overhead can be significantly reduced: In the ideal case, $n-d$ out of $n$ subset pairs are identical ones, and only $d (\ll n)$ out of $n$ subset pairs contain distinct elements (one distinct element in each of the $d$ subset pairs) and need to be reconciled. If we can identify these $d$ subset pairs (with a tiny additional communication overhead) and only reconcile them, the overall communication overhead will be significantly reduced from $\Omega(d^2)$ to $O(d)$. Based on this intuition, we propose our scheme in \autoref{sucsec:our-scheme}, which uses Parity Bitmap Sketch (PBS) and Error Correction Coding (ECC) to identify those subset pairs with a tiny additional communication overhead. 

Note that the ideal case does not always happen. However, we can ensure that the ideal case happens with high probability by properly selecting $n$ based on $d$ (i.e., $n=\Omega(d^2)$). Furthermore, as we will describe in \autoref{subsec:nonideal}, even if the ideal case does not happen (i.e., some distinct elements are hashed into the same subset pair), most of the distinct elements should be distributed into different subset pairs and therefore can be reconciled. So the baseline scheme, even cannot reconcile all of the distinct elements, can still reconcile the majority of them. Based on this property, we will extend our scheme from single-round to multi-rounds in \autoref{subsec:nonideal} to further increase the probability of reconciling all distinct elements. 

For general cases ({\it i.e.,} $t=|A\Delta B|$ is an arbitrary number), we have a straightforward strawman scheme building upon~\autoref{alg:trivial_case}, which works as follows: First, Alice and Bob choose some hash function $h(s): \mathcal{U} \rightarrow \{0,1,\cdots,2^{32}-1\}$ to partition $A$ and $B$ into $m$ subsets $A_1,A_2,\cdots,A_m$ and $B_1,B_2,\cdots,B_m$ respectively:

\begin{align}
s\in A_i & \mbox{ iff } s\in A \mbox{ and } h(s)=i\!\mod m, \nonu{}mber\\
s\in B_i & \mbox{ iff } s\in B \mbox{ and } h(s)=i\!\mod m. \nonumber
\end{align} 

{\bf call a subset pair -> partition?} Since Alice and Bob use the same hash function for partition, common elements (i.e., elements in $A\cap B$) are always hashed into the same subset pair $(A_i, B_i)$. And the set difference of each subset pair only contains distinct elements (i.e., elements in $A\Delta B$): $A_i\Delta B_i \subset A\Delta B$. In the ideal case, with a sufficient large $m$, each subset pair $(A_i, B_i)$ contains at most one distinct element ({\it i.e.,} $|A_i\Delta B_i|\!\leq\!1$). Then \autoref{alg:trivial_case} can reconcile each subset pair and obtain $A_i\Delta B_i$ for $i=1,2,\cdots,m$. The overall set difference $A\Delta B$ is simply their union $\bigcup_{i=1}^m \big{(}A_i\Delta B_i\big{)}$. The selection of hash function $h(s)$ can be predetermined between Alice and Bob and it does not require additional communication cost.

%To make sure Alice and Bob use the same hash function for partition, we let them pre-agree on some universal hash family (e.g., \code{xxHash}~\cite{Collet_xxHashExtremelyfast_}) and a common selection order, and each time they choose a hash function from the family in the same order. Note that we can also let Alice generates a hash function and send it to Bob. The hash function that Alice and Bob choose for partition can be either generated by 

This hash-partition is in nature a {\it balls-into-bins model}. We can view the distinct elements as balls and the subset pairs as bins. The hash-parition basically throws (hashes) $t$ balls (distinct elements) uniformly and randomly into $m$ bins (subset pairs). The aforementioned ideal case in this context is, with a sufficient large number of bins, each bin receives at most 1 ball. The strawman scheme works correctly if and only if the ideal case happens, which has a probability of $\frac{m\,!}{(m-t)\,!m^t}\!=\!\prod_{k=1}^{t - 1}(1 - \frac{k}{m})\!\approx\! e^{-\frac{t(t-1)}{2m}}$. In other words, to ensure the strawman scheme works correctly with a probability of $p$, it roughly requires $m \!=\!\lceil \frac{t(t-1)}{-2\ln p}\rceil$ subset pairs. 

Note that the communication overhead of this strawman scheme is proportional to the number of subset pairs $m$, as each subset pair requires communication of an \code{XOR} sum in \autoref{alg:trivial_case} during the reconciliation. When $t$ is small, a small communication cost can guarantee that the strawman scheme works correctly with high probability. For instance, when $t=5$, $m=95$ subset pairs are sufficient for the strawman scheme to work correctly with a probability of $90\%$. However, when $t$ is relatively large, it requires a huge communication cost to ensure the strawman scheme works correctly. For instance, when $t=1,000$, it requires $m=4,740,865$ subset pairs to guarantee a success probability of $90\%$. 

In fact, the majority of subset pairs are identical ones and do not need to reconcile. And only a small portion of them contain distinct elements. If we can identify those subset pairs that contain distinct elements and only reconcile them, the communication cost could be significantly reduced. Our scheme is based on this intuition and uses parity bitmap sketch and BCH code to identify the subset pairs, which we will elaborate in \autoref{sucsec:our-scheme}. 

%To distribute balls as uniformly as possible and maximize the probability of the ideal case, we choose a uniform hashing function $h$ that throws balls uniformly and randomly into bins: $$\mathbb{P}[h(s)=i]=\frac{1}{m} \mbox{ for } \forall i=1,2,\cdots,m, \forall s\in U$$.

%Note that the probability of the ideal case is $\frac{m\,!}{(m-t)\,!m^t}\!=\!\prod_{k=1}^{t - 1}(1 - \frac{k}{m})\!\approx\! e^{-\frac{t(t-1)}{2m}}$. Hence, at least $\lceil \frac{t(t-1)}{-2\ln p}\rceil$ bins are required to ensure that this probability is at least $p$. In other words, to ensure that the ideal case happens with a probability of $p$, the strawman scheme roughly requires $m \!=\!\lceil \frac{t(t-1)}{-2\ln p}\rceil$. For example, suppose $t\!=\!$\num{1000}, %and $p\!=\!0.01$, this strawman scheme roughly requires $m\!=\!$\num{720626} bins (partitions) to ensure that $|A_i\Delta B_i|\!\leq\!1$ (for any $i=1,2,\cdots,m$) holds with probability $50\%$.  

% A straightforward strawman scheme building upon~\autoref{alg:trivial_case} 
% to reconcile two sets $A$ and $B$ in general 
% ({\it i.e.,} $|A\Delta B|$ is an arbitrary number) is the following: 
% Uniformly randomly partition $A$ and $B$ into $m$ subsets ($A_1,A_2,\cdots,A_m$ 
% and $B_1,B_2,\cdots,B_m$) so that the set difference 
% $A_i\Delta B_i$ of each subset pair $(A_i, B_i)$ contains at most one element 
% ({\it i.e.,} $|A_i\Delta B_i|\!\leq\!1$) {\it w.h.p.} ({\it i.e.,} with high probability), 
% and then reconcile each subset pair with~\autoref{alg:trivial_case}. 

% Now let us analyze this strawman scheme using the {\it balls-into-bins model}. 
% Assume that sets $A$ and $B$ have $t$ elements in their set difference, {\it i.e.,} $|A\Delta B|\!=\!t$. 
% These $t$ elements can be viewed as $t$ balls and the $m$ partitions (subset pairs) can be viewed as 
% $m$ bins. The random partition process in this strawman scheme can be modeled as throwing 
% $t$ balls into $m$ bins in the following manner: Each ball goes into a 
% uniformly random bin and independently of other balls. %so that each bin contains at most one ball, {\it w.h.p.}  
% The probability that each bin contains at most one ball is  
% $\frac{m\,!}{(m-t)\,!m^t}\!=\!\prod_{k=1}^{t - 1}(1 - \frac{k}{m})\!\approx\! e^{-\frac{t(t-1)}{2m}}$. 
% Hence, at least $\lceil \frac{t(t-1)}{-2\ln p}\rceil$ bins are required 
% to ensure that this probability is at least $p$. In other words, to ensure 
% that each bin contains at most one ball with a probability of $p$, 
% the strawman scheme roughly requires $m \!=\!\lceil \frac{t(t-1)}{-2\ln p}\rceil$. 
% For example, suppose $t\!=\!$\num{1000}, %and $p\!=\!0.01$, 
% this scheme roughly requires $m\!=\!$\num{108469} bins (partitions) to 
% ensure that $|A_i\Delta B_i|\!\leq\!1$ (for any $i=1,2,\cdots,m$) holds with probability $0.01$.  

% We note that the communication overhead of this strawman scheme is proportional to 
% $m$ ($\!\gg\! t$), as each partition (subset pair) requires communication of an \code{XOR} sum during the reconciliation. 
% This communication overhead is much higher than that of the optimal scheme, which only requires 
% to exchange the elements in the set difference (assuming an oracle tells it which elements belong to 
% the set difference), {\it i.e.,} proportional to $t$. In the example above, assuming each element takes 4 bytes, 
% the communication overhead of the strawman scheme is $4m$ bytes ($\!\approx\! \num{423.71}\,$KB) to ensure 
% a success rate of only 0.01 ({\it i.e.,} with a probability of $0.0.1$, all elements in 
% the set difference are successfully reconciled), 
% which is approximately 2 orders of magnitude higher than $4t$ bytes ($\!=\!\num{3.90}\,$KB), the communication 
% overhead of the optimal scheme. 

\subsection{Our Scheme: The Preliminary Version}\label{sucsec:our-scheme}

Like the baseline scheme, our scheme also hash-partitions the two sets $A$ and $B$ into $n$ subset pairs. The difference is, instead of reconciling all subset pairs using \autoref{alg:trivial_case}, our scheme identifies the subset pairs that contains distinct elements and only reconciles them. Since the hash-partition and set reconciliation on each subset pair using \autoref{alg:trivial_case} have been described in \autoref{subsec:protocol1}, we only elaborate how to identify the subset pairs that contain distinct elements in this section. 

The general idea of identification is very simple: First, we {\bf encode} each subset into $1$ bit, such that in the ideal case, for $\forall i=1,2,\cdots,n$:

\begin{itemize}
	\item The codewords (bits) of $A_i$ and $B_i$ are different if and only if subset pair $(A_i, B_i)$ contains $1$ distinct element;
	\item The codewords (bits) of $A_i$ and $B_i$ are the same if and only if subset pair $(A_i, B_i)$ contains no distinct element;
\end{itemize}

Second, we {\bf compare} the codewords of each subset pair. And the subset pairs that contain distinct elements are the ones with different codewords (bits). We will describe the two steps in details in \autoref{sec:parity_bitmap_encoding} and \autoref{sec:BCH_code} respectively.

\subsubsection{Parity Bitmap Encoding}\label{sec:parity_bitmap_encoding}

In our scheme, we use {\it parity encoding} to encode each subset into a parity bit. More specific, it encodes a subset as ``1'' if it contains odd number of elements, and as ``0'' otherwise. And it satisfies the aforementioned requirements in the ideal case:

\begin{itemize}
	\item If subset pair $(A_i, B_i)$ contains $1$ distinct element, the corresponding two subsets $A_i$ and $B_i$ differ exactly one element, which implies that $||A_i|\!-\!|B_i||\!=\!1$. Hence, if $|A_i|$ ({\it i.e.,} number of elements in $A_i$) is odd (or even), then $|B_i|$ must be even (or odd). And the parity bits of $A_i$ and $B_i$ will be different;
	\item If subset pair $(A_i, B_i)$ contains no distinct element, the corresponding two subsets $A_i$ and $B_i$ should be the same and therefore contain the same number of elements. Hence, if $|A_i|$ is odd (or even), then $|B_i|$ must be odd (or even). And the parity bits of $A_i$ and $B_i$ will be the same;
\end{itemize}

Using parity encoding, the $n$ subsets of $A$ are encoded as a bit string $A[1..n]$ in $\{0,1\}^n$, 
where the $i$-th bit $A[i]$ in $A[1..n]$ corresponds to the parity encoding bit of $A_i$. Similarly, the $n$ subsets of $B$ are similarly 
encoded as a bit string $B[1..n]$. We call $A[1..n]$ ($B[1..n]$) the {\it parity bitmap} of $\{A_i\}_{i=1}^n$ ($\{B_i\}_{i=1}^n$). In the ideal case, $A[1..n]$ and $B[1..n]$ differ at $d$ different bit-positions, which corresponds to the $d$ subset pairs that contain distinct elements. And our scheme only reconciles those subset pairs that the parity bits are different. We will describe the nonideal case (i.e., some subset pair contains more than 1 distinct elements) in \autoref{subsec:nonideal}.

\subsubsection{Parity Bitmap Comparison Using BCH Code}\label{sec:BCH_code}

A straightforward approach to compare the parity bitmaps is to let Bob send the complete parity bitmap $B[1..n]$ to Alice, then Alice compares $A[1..n]$ with $B[1..n]$ locally. This approach has a communication overhead of $n$ bits, which is unnecessarily high. As we discussed in~\autoref{subsec:protocol0}, $d$ is usually much smaller than $n$. It means $A[1..n]$ and $B[1..n]$ differ only at a tiny portion of bits. Therefore, we can view $A[1..n]$ as a corrupted message of $B[1..n]$ with $d$ corrupted bits, and the bit-positions of the $d$ corrupted bits basically correspond to the $d$ subset pairs that contain distinct elements. The detection of corrupted bits, on the other hand, can be solved by Error-Correction Code (ECC)~\cite{Lin_ErrorControlCoding_1983}. And our scheme uses BCH code~\cite{Lint_IntroductionCodingTheory_1998} to encode the parity bitmap and detect the $d$ corrupted bits.

More specific, after the parity bitmap encoding, Bob uses a $d$-error-correcting systematic BCH code to encode $B[1..n]$ into an $n+d\log n$ codeword, in which the first $n$ bits are $B[1..n]$ (property of systematic BCH code). Then Bob sends the rest $d\log n$ bits, which we denote as {\it parity bitmap sketch (PBS)}, to Alice. Upon the received PBS and $A[1..n]$ (corrupted message), Alice uses the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} to detect the $d$ corrupted bits in $A[1..n]$. The communication overhead of this approach is $d\log n$ bits (i.e., length of PBS), which is much smaller than that of the straightforward approach ($n$ bits, when $d\!\ll\!n$). On the other hand, the computational complexity of the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} is $O(d^2\log^2 n)$. 

\subsubsection{Exceptional Handling and Multi-rounds}\label{subsec:nonideal}

As we described in \autoref{subsec:protocol1}, the ideal case does not always happen, which means some subset pair may contain more than 1 distinct elements and cannot be successfully reconciled by \autoref{alg:trivial_case}. Due to the parity encoding, we can classify such subset pair into the following two scenarios:

\begin{itemize}
    \item Scenario 1: If a subset pair $(A_i, B_i)$ contains even number ($\geq 2$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be the same and our scheme will not reconcile the subset pair. Hence, the distinct elements in the subset pair will not be reconciled;
    \item Scenario 2: If a subset pair $(A_i, B_i)$ contains odd number ($\geq 3$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be different and our scheme will reconcile the subset pair using \autoref{alg:trivial_case}. However, as we described in \autoref{subsec:protocol0}, when a subset pair contains more than 1 distinct elements, \autoref{alg:trivial_case} will output the bitwise \code{XOR} of them as the `distinct element', which is not a real distinct element with high probability;
\end{itemize}

In both scenarios, the distinct elements in the subset pair cannot be reconciled. Even worse, in the second scenario, a false-positive could happen (i.e., the output of \autoref{subsec:protocol0} is not a real distinct element). However, as we will analyze in \autoref{sec:tail_bound} and show in {\bf the evaluation section}, the second scenario barely happens both theoretically and empirically. To further reduce the chance of false-positives, we add a verification step at the end of \autoref{subsec:protocol0} to check whether the output of \autoref{subsec:protocol0} $s$ is a real distinct element or not. The verification step works as follows: Given the output $s$ of subset pair $(A_i,B_i)$, if $s\in\mathcal{U}_i$ (i.e., $h(s)=i$), we consider $s$ as a real distinct element; Otherwise, we consider $s$ as an incorrect output and discard it. 

Note that if $s$ is a real distinct element of $(A_i,B_i)$, $s$ must be in sub-universe $\mathcal{U}_i$. However, if $s$ is the bitwise \code{XOR} of the distinct elements in $(A_i,B_i)$ (i.e., the second scenario happens), $s$ could be in any sub-universe other than $\mathcal{U}_i$. In fact, if we assume the hash-partition described in \autoref{subsec:protocol1} hashes the elements of $\mathcal{U}$ uniformly, independently, and randomly into $n$ sub-universes, the output $s$ in the second scenario will be in a different sub-universe $\mathcal{U}_j (j\neq i)$ with a high probability of $1-\frac{1}{n}$. Hence, this verfication step can reduce the chance of false-positives by a factor of $\frac{1}{n}$. 

Even if the ideal case does not happen, most of the distinct elements should be distributed into different subset pairs and therefore can be reconciled. So our scheme, even cannot reconcile all of the distinct elements, can still reconcile the majority of them (piecewise decodability). To reconcile the rest distinct elements, we can just run our scheme for another round under a different hash-partition function, so on so force. This {\bf multi-rounds} scheme can significantly increase the success probability (i.e., the probability that all distinct elements are reconciled). Readers may wonder in the later rounds, most distinct elements should be reconciled, and the remaining could be reconciled using degraded parameters (i.e., smaller $n$ and $t$). In fact, degrade parameters in later rounds cannot save much communication overhead, since the majority of it is spent in the first round (i.e., $>90\%$). Therefore, we use the same parameters (i.e., $n,t$) among all rounds in our evaluation.
%The tradeoff between the number of rounds and the communication overhead per rounds will be elaborated in \autoref{sec:tail_bound}. In our evaluation, $r=2,3$ rounds are enough to achieve an extremely high success probability. 

Readers may think the cost (i.e., communication overhead and the computational complexity) of this multi-rounds scheme is proportional to the number of rounds (denoted as $r$) and increases linearly with $r$. In fact, the cost of each round is roughly proportional to the number of remaining distinct elements, which decreases exponentially as $r$ increases (i.e., the first round reconciles $99\%$ of distinct elements, the second round reconciles $99\%$ of the remaining $1\%$ distinct elements, etc.). So the cost of this multi-rounds scheme is only slightly larger than that of the single-round scheme. Furthermore, as we explained in \autoref{sec:intro}, {\bf from intro thanks for the piecewise decodability of our solution, in almost all practical application scenarios, this tradeoff does not lead to longer response time because the reconciliation of objects identified by the successfully decodable codewords, which constitute the vast majority of all codewords, can run in parallel with the transmissions and decodings of the rest.  In other words, the piecewise decodability effective masks the slightly larger number of communication rounds as far as the response time is concerned.} 

\end{comment}

\section{PBS for large \texorpdfstring{\larger\boldmath\MakeLowercase{$d$}}{d}}\label{subsec:protocol2}

Note that the BCH decoding computational complexity is $O(d^2)$ of finite field operations in GF($2^{8}$) using the state-of-the-art decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019}, which is too expensive for large $d$. To overcome this drawback, we first hash-partition sets $A$ and $B$ each into $d/\delta$ subsets (which we call {\it groups} to distinguish from subsets), just like what we did in \autoref{sec:hash_partition}, for some small integer $\delta$ (say $5$), then reconcile each of the group pairs by the PBS we described in \autoref{sec:scheme}. After the partition, each group has $\delta$ distinct elements on average. So the BCH decoding computational complexity of each group pair can be considered as $O(1)$, since $\delta$ is a small number. As a result, the overall computational complexity of PBS is reduced from $O(d^2)$ to $O(d)$. 

To differentiate from the PBS described in \autoref{sec:scheme}, we refer to it as PBS-basic in this section. We continue to assume that the number of distinct elements $d$ is precisely known. Even so, due to the randomness of hash-partition, $d_i$, the number of distinct elements in the $i^{th}$ group pair, is a Binomial random variable with mean of $\delta$ $(=d/g)$ for $i=1,2,...,g$, which cannot be precisely known without a huge amount of additional communication overhead. Hence, we can no longer set the error-correction capability of the BCH code for each group pair based on the exact number of distinct element in it, as we did in \autoref{sec:scheme}. Instead, we set a conservative error-correction capability $t$ (say $2.5\delta$) for all group pairs, which is sufficient for all group pairs (i.e., $t\geq d_i$ for $i=1,2,...,g$) with high probability. We will discuss the case that $d_i>t$ in \autoref{sec:BCH_exception}.



% ===============================
% To differentiate from the PBS described in \autoref{sucsec:our-scheme}, we refer it as PBS-basic in this section. Note that the BCH decoding computational complexity is $O(d^2\log ^2 n)$, which is $\Omega(d^2\log^2 d)$ when $n=\Omega(d^2)$, with the state-of-the-art decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019}. It is too large in PBS-basic for large $d$. To overcome this drawback and generalize PBS-basic for large $d$, we partition sets $A$ and $B$ each into $d/\delta$ subsets (which we call {\it groups} to distinguish from subsets) for some small integer $\delta$ (say $5$) and reconcile the $d/\delta$ group pairs respectively using PBS-basic. After this partition, each group has $\delta$ distinct elements on average. The BCH decoding computational complexity of each group pair can be considered as $O(1)$, since $\delta$ is a small number. As a result, the overall computational complexity of PBS is reduced from $O(d^2\log ^2 n)$ to $O(d)$. 

% % To differentiate from the PBS described in \autoref{sucsec:our-scheme}, we refer it as PBS-basic in this section. PBS-basic is not suitable for large $d$ for two reasons: First, its communication overhead is asymptotically $O(d\log n)\!=\!O(d\log d)$ (since $n=\Omega(d^2)$), which is not asymptotically optimal. Second, the decoding computational complexity is proportional to $d^2$ with the state-of-the-art decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} for BCH codes, which is too high when $d$ is large. To overcome these two drawbacks, we use a simple algorithmic trick to (1) reduce the communication overhead from $O(d\log d)$ to $d\log u \!+\! O(d)$; (2) reduce the decoding computational complexity from $O(d^2)$ to $O(d)$. 

% Now, we describe the generalized PBS in details: In the first step, we hash-partition $A$ and $B$ (by some hash function $h_1(\cdot)$) into $g$ group pairs, just like what we did in \autoref{sucsec:our-scheme}. The objective of this partition is however different: In \autoref{sucsec:our-scheme}, we aim to ensure each subset pair contains at most $1$ distinct element (i.e., the ideal case) with high probability; Here we aim to make each group pair contains roughly $\delta$ distinct elements for some small constant $\delta$ (say $5$) by setting $g=d/\delta$. 
% %To differentiate the $g$ subset pairs here from those in \autoref{sec:hash_partition}, we call them the $g$ {\bf groups} in the sequel. 
% In the second step, we just apply PBS-basic (described in \autoref{sucsec:our-scheme}) to reconcile each group pair and obtain the distinct elements. 
% ================================

% To differentiate from the PBS described in \autoref{sucsec:our-scheme}, we refer it as PBS-basic in this section. When $d$ is large (more than several), we hash-partition set $A$ and $B$ into groups, such that each group pair contains $\delta$ distinct elements on average for small $\delta$ (say $5$), as described in \autoref{sec:larged}. Then each group pair can be reconciled by PBS-basic.

% When describing the PBS-basic in \autoref{sucsec:our-scheme}, we assume that the number of distinct elements is precisely known. We set the error-correction capability of the BCH code (denoted as $t$) just enough to correct $d$ errors (i.e., $t=d$). However, due to the randomness of hash-partition, $d_i$, the number of distinct elements in the $i^{th}$ group pair, is a Binomial random variable $Binomial(d,1/g)$ with expectation of $\delta$ $(=d/g)$ for $i=1,2,...,g$, which cannot be precisely known without a huge amount of additional communication overhead. Hence, we can no longer set the error-correction capability of the BCH code for each group pair based on the exact number of distinct element in it, as we did in \autoref{sucsec:our-scheme}. Instead, we set a universal error-correction capability $t$ (say $2.5\delta$) for all group pairs, which is sufficient for all group pairs (i.e., $t\geq d_i$ for $i=1,2,...,g$) with high probability. We will discuss the case that $d_i>t$ in \autoref{sec:BCH_exception}.

%This assumption in general does not hold: 
% Let $d_i$ denote the number of distinct elements in Group $i$. Due to the property of hash-partition, each $d_i$ is a Binomial random variable $Binomial(d,1/g)$ with expectation of $\delta$ $(=d/g)$. Even if $d$ is precisely known, each $d_i$ is not. To ensure the error-correction capability $t$ is sufficient for each group (i.e., $d_i\leq t$) with high probability, we leave some safety margin for the randomness of $d_i$ and conservatively set $t$ roughly $2.5\delta$ (the factor $2.5$ varies depend on other parameters, which will be discussed in \autoref{sec:parameter_settings}), so that $Pr[d_i>t]$ is tiny. We will discuss the case that $d_i>t$ in \autoref{sec:BCH_exception}.

Note that the `safety margin' between $t$ and $\delta$ (i.e., the average number of distinct elements in a group pair) incurs additional communication overhead on transmitting BCH codeword: In the perfect scenario (i.e., $\{d_i\}_{i=1}^g$ is precisely known), the average communication overhead on transmitting BCH codeword per group pair is $\delta\log n$; On the other hand, when we set $t$ to be the error-correction capability for each group pair, the average communication overhead becomes $t\log n$, which is $t/\delta$ times of that in the perfect scenario (e.g., $2.5$ times when $t=2.5\delta$). If we set $t$ too conservatively (say $10\delta$), the `safety margin' will incur huge additional communication overhead. Due to this reason, we suggest to set a neither too conservative nor too libertive $t$ in the range from $1.5\delta$ to $3\delta$. 
%which is roughly $2.5$ times of that in the perfect scenario (when $t$ is roughly $2.5\delta$). Due to this addition

Readers may wonder if we can reduce this additional communication overhead by using some technique to estimate $\{d_i\}_{i=1}^g$ (e.g., ToW estimator in \autoref{subsec:ToW}), so that we can set the error-correction capability of each group more wisely and save some waste on the safety margin. However, to achieve that, the estimation on $\{d_i\}_{i=1}^g$ must be in extremely high precision (since $\{d_i\}_{i=1}^g$ are small numbers with mean of $\delta$), which requires a much higher communication overhead than the savings. Due to the same reason (i.e., estimate $\{d_i\}_{i=1}^g$ is costly), we set the number of subset pairs for each group pair to be all equal (denoted as $n$) based on $\delta$. 

Like what we did in \autoref{sec:multi-rounds}, we set a paramenter setting requirement on success probability for all group pairs: the probability that all group pairs are completely reconciled in $r$ rounds must be larger than $p_0$. The detail about how to set $n$ and $t$ given such a requirement will be elaborated in \autoref{sec:parameter_settings}. 

% we set a {\it target success probability} $p_0$ of $r$ rounds as a paramenter setting requirement, which aims to ensure the probability that all distinct elements are reconciled in $r$ rounds to be larger than $p_0$. This requirement should also ensure the majority of the distinct elements are reconciled in the first round. Use the same example ($d=5, n=255$), on average $4.81$ out of $5$ distinct elements should be reconciled in the first round. So the total communication overhead in all rounds is only slightly larger than ($1.01$ to $1.07$ times of, as we will show in \autoref{fig:per-round-con}) that in the first round. Due to this reason, we use the communication overhead in the first round (described in \autoref{sec:communication_overhead_single_PBS}) to approximate the total communication overhead of all rounds in parameter settings (to be elaborated in \autoref{sec:parameter_settings}.

% Note that this safety margin incurs additional communication overhead on transmitting BCH codeword: In the perfect scenario (i.e., $\{d_i\}_{i=1}^g$ is precisely known), the average communication overhead on transmitting BCH codeword per group is $\delta\log n$; On the other hand, when we set $t$ to be the error-correction capability for each group, then the average overhead becomes $t\log n$, which is roughly $2.5$ times of that in the perfect scenario (when $t$ is roughly $2.5\delta$). Readers may wonder if we can reduce this additional communication overhead by using some technique to estimate $\{d_i\}_{i=1}^g$ (e.g., ToW estimator in \autoref{subsec:ToW}), so that we can set the error-correction capability of each group more wisely and save some waste on the safety margin. However, to achieve that, the estimation on $\{d_i\}_{i=1}^g$ must be in high precision, which requires a much higher communication overhead than the savings. 

\subsection{What if PinSketch also uses partitions?}

The same algorithmic trick (i.e., hash-partition two sets each into groups) can also be implemented in PinSketch~\cite{Dodis_PinSketch_2008} to reduce it computational complexity from $O(d^2)$ (of finite field operations in GF($2^{32}$)) to $O(d)$. However, it will encounter the same randomness problem and have to set up a safety margin on the error-correction capability. This safety margin will incur much more additional communication overhead on PinSketch than on our scheme: Considering the average communication overhead per group pair, the additional overhead caused by the safety margin is $(t-\delta)\log n$ in PBS and $(t-\delta)\log |\mathcal{U}|$ in PinSketch. The later is roughly $4$ times of the former under the default setting ($n=255, |\mathcal{U}|=2^{32}$). Note that the optimal communication overhead to reconcile $d$ distinct elements is $\delta\log |\mathcal{U}|$. Use the same example in \autoref{sec:intro}, when $\delta=5, n=255, |\mathcal{U}|=2^{32}, t=2.5\delta$, the overhead of PinSketch using the algorithmic trick is $2.5$ times of the optimal (i.e., $d\log |\mathcal{U}|$), while that of PBS is $2.075$ times of the optimal. It means PBS could have a lower communication overhead than PinSketch if they both use the algorithmic trick. Furthermore, as the signiture width $\log |\mathcal{U}|$ increases, the advantage of PBS over PinSketch becomes more significant, which we will show in \autoref{subsec:mini-partition}.

% The same algorithmic trick can also be implemented in PinSketch~\cite{Dodis_PinSketch_2008} to reduce it computational complexity from $O(d^2)$ to $O(d)$. However, it will encounter the same randomness problem and have to set up a safety margin on the error-correction capability. This safety margin will incur much more communication overhead on PinSketch than on our scheme: Considering the average communication overhead per group, in our scheme, this overhead can be expressed as $t\log n+\delta\log n+\delta \log u+32$, in which $t\log n$ accounts for the BCH codeword, $\delta\log n$ accounts for the index of the subset pairs, $\delta \log u$ accounts for the bitwise \code{XOR} in \autoref{alg:trivial_case}, and $32$ accounts for the $32$-bit CRC in \autoref{proto:multirounds}. In PinSketch, this overhead increases from $O(\delta\log u)$ (optimal) to $O(t\log u)$ (PinSketch does not need to transmit bitwise \code{XOR}) if it uses the same algorithmic trick. Use the same example in \autoref{sec:intro}, when $\delta=5, n=255, u=2^{32}, t=2.5\delta$, the overhead of PinSketch using the trick is $2.5$ times of the optimal, while that of our scheme is $2.075$ times of the optimal (as we introduced in \autoref{sec:intro_oursolution}). That means our scheme has a lower communication overhead than PinSketch if they both use the algorithmic trick. Furthermore, as the signiture size $\log u$ increases, the advantage of our scheme over PinSketch becomes more significantly, which we will show in \autoref{subsec:mini-partition}.

% In PinSketch, each bit encodes only a single element in the universe, so the size of the bitmap is equal to the size of the universe.  
% For example, in the set reconciliation problem we usually assume each element is ``indexed" by a $32$-bit-long (hash) signature, so the universe contains a total of $2^{32}$ elements. In this case, the bitmap encoding for any set in PinSketch is $2^{32}$ bits long, and the Galois field involved in its BCH decoding is the ``$32$-bit-wide" $GF(2^{32})$.  In contrast, as explained earlier, in PBS 
% %since each bit encodes the oddness or evenness of the cardinality of a subset,   
% the size $n$ of a bitmap is dependent only on $d$, and not on the size of the universe or on the cardinality of the set the bitmap encodes.   For example, as shown in the example above, $n = 255$ is large enough for $d = 5$.  In this case, the BCH decoding operates in the much shorter
% ``8-bit-wide" $GF(2^{8})$.  This shorter ``width" alone in theory translates into roughly $16$ times shorter BCH decoding time, which as will be explained in~\ref{} grows quadratically with the ``width" of the underlying Galois field.  This shorter ``width" also implies four times shorter BCH codeword in PBS than in PinSketch, resulting in lower communication complexity as will be shown in~\autoref{}.

% Note that our scheme only takes 1 round trip delay to both identify the $d$ subset pairs and reconcile them: In the first half, Bob computes and sends PBS to Alice. Then Alice locally identifies the $d$ subset pairs and then initiates the reconciliation ({\it i.e.,} \autoref{alg:trivial_case}) for them, {\it i.e.,} computes the bitwise \code{XOR} of the corresponded $d$ subsets. In the second half, Alice sends the bitwise \code{XOR} of the $d$ subsets with their indexes to Bob. Then Bob can compute the set difference $A\Delta B$ locally.


% We can certainly use some communication-efficient technique to estimate $d_i$ (e.g., \autoref{subsec:ToW}). However, to obtain $d_i$ precisely will require a communication cost almost as large as to reconcile Group $i$. So instead of obtaining $d_i$ and set $c_i$ (i.e., the error-correction capability of Group $i$) equal to $d_i$, we leave the randomness of $d_i$ and set $c_i$ neither too conservative, nor too libertive in the following sense: (1) $c_i$ is not too big (conservative, i.e., $10\delta$) to make the total size of PBS unnecessarily large and incur too much extra communication overhead; (2) $c_i$ is not too small (libertive, i.e., $\delta$) to incur a high probability of insufficient decode capability, which can result in hefty penalties in the latter case of incorrect decoding (will be elaborated in \autoref{sec:BCH_exception}). In our scheme, we set $c_i$ to be $2-3$ times of $\delta$, which will be shown in \autoref{sec:tail_bound} that it is just enough to make the probability of decode failure very small. Meanwhile, we set the error-correction capability of each group ($c_1,c_2,...,c_k$) to be all equal and denote it as $c$. 

%Since the decoding capacity $t$ and the number of subset pairs for each group $n$ are both small constants independent of $d$, therefore, the communication overhead per group is $t\cdot\log n \!=\!O(1)$, which implies a total communication overhead of $O(d)$. Similarly, the total decoding computational complexity is also $O(d)$. 

% \subsection{Exception Handling}\label{sec:exceptions}

% \subsubsection{Exception Handling on Hash-Partition}\label{subsec:exception_hash_partition}

% As we have described in \autoref{sec:hash_partition}, the ideal case does not always happen, which means some subset pair may contain more than 1 distinct elements and cannot be successfully reconciled by \autoref{alg:trivial_case}. Due to the parity encoding, we can classify such subset pair into the following two scenarios:

% \begin{itemize}
%     \item Scenario 1: If a subset pair $(A_i, B_i)$ contains even number ($\geq 2$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be the same and our scheme will not reconcile the subset pair. Hence, the distinct elements in the subset pair will not be reconciled;
%     \item Scenario 2: If a subset pair $(A_i, B_i)$ contains odd number ($\geq 3$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be different and our scheme will reconcile the subset pair using \autoref{alg:trivial_case}. However, as we described in \autoref{subsec:protocol0}, when a subset pair contains more than 1 distinct elements, \autoref{alg:trivial_case} will output the bitwise \code{XOR} of them as the `distinct element', which is not a real distinct element with high probability;
% \end{itemize}

% In both scenarios, the distinct elements in the subset pair cannot be reconciled. Even worse, in the second scenario, a false-positive could happen (i.e., the output of \autoref{subsec:protocol0} is not a real distinct element). For example, if subset pair $(A_i, B_i)$ contains $3$ distinct elements $s_1, s_2, s_3$, then the output of \autoref{alg:trivial_case} is $\tilde{s}_4=s_1\oplus s_2\oplus s_3$, which is normally not a distinct element. The good thing is, the probability of the false-positive is extremely small for small $d$. For instance, if $d=5$ and $n=255$, the probability of the false-positive is $7.6\times 10^{-6}$, which is very small. To further reduce the chance of false-positives, we add a verification step at the end of \autoref{subsec:protocol0} to check whether the output of \autoref{subsec:protocol0} $s$ is a real distinct element or not. The verification step works as follows: Given the output $s$ of subset pair $(A_i,B_i)$, if $s\in\mathcal{U}_i$ (i.e., $h(s)=i$), we consider $s$ as a real distinct element; Otherwise, we consider $s$ as an incorrect output and discard it. 

% Note that if $s$ is a real distinct element of $(A_i,B_i)$, $s$ must be in sub-universe $\mathcal{U}_i$. However, if $s$ is the bitwise \code{XOR} of the distinct elements in $(A_i,B_i)$ (i.e., the second scenario happens), $s$ could be in any sub-universe other than $\mathcal{U}_i$. In fact, if we assume the hash-partition described in \autoref{sec:hash_partition} hashes the elements of $\mathcal{U}$ uniformly, independently, and randomly into $n$ sub-universes, the output $s$ in the second scenario will be in a different sub-universe $\mathcal{U}_j (j\neq i)$ with a high probability of $1-\frac{1}{n}$. Hence, this verfication method can further reduce the probability of false-positives by a factor of $\frac{1}{n}$. Use the same example (i.e., $d=5$, $n=255$), the probability is reduced from $7.6\times 10^{-6}$ to $3\times 10^{-8}$ by this verification method. 

% In some super critical cases (i.e., no false-positive is allowed), we can use a more powerful verification method to completely eliminate false-positives. That is, to check if the output $s$ exists in exactly one of the two sets (i.e., $s\in A\setminus B$ or $s\in B\setminus A$). To do so, Bob transmits $s$ along with an identification bit $\mathbb{1}_{\{s\in B\}}$ to Alice, then Alice checks if $s$ . This method verification costs $d(\log u+1)$ bits of additional communication overhead. In most applications, rigorously $0\%$ probability of false-positives is unnecessary and the probability of the former verification method is small enough, so we use the former verfication method in our evaluation. Based on our observation, the false-positive does not happen even once in our evaluation using the former verfication method.

\subsubsection{Exception Handling on BCH Decoding}\label{sec:BCH_exception}

The exceptions that happens within PBS-basic have been discussed and handled in \autoref{subsec:exception_hash_partition} and \autoref{sec:multi-rounds}. In this section, we only discuss the exceptions that the error-correction capability $t$ is insufficient for some group $i$. More specifically, when $d_i$ (i.e., the number of distinct elements in group $i$) is larger than the error-correction capability $t$, the BCH codewords of group $i$ differ at $d_i$ bit positions in the ideal case, which exceeds the error-correction capability $t$. If so, the BCH decoder cannot decode the bit errors correctly (\autoref{step:BCH_decode} in \autoref{alg:single_round_pbs}) and report a failure. This exception happens with a small probability in each group pair: For example, when $d=1000, g=200$ $(\delta=5), t=13$, the probability that this exception happens is only $6.7\times 10^{-4}$. 

To handle this type of exceptions, we use the same algorithm trick in \autoref{subsec:protocol2} to further partition each problematic group into $3$ sub-groups and reconcile them respectively using PBS-basic. Note that $d_i$, if is not smaller, should be only slightly larger than $t$ with high probability. Hence, partitioning into $3$ sub-groups is enough to ensure each sub-group has no more than $t$ distinct elements. Then in the next round, each sub-group does not encounter this type of expections and can be reconciled by PBS-basic respectively. Use the same example ($d=1000, g=200$ $(\delta=5), t=13$), the probability that some sub-group has more than $t$ distinct elements is $9.5\times 10^{-10}$. More specifically, we add a termination condition of \autoref{alg:3_way_partition} after \autoref{step:BCH_decode} in \autoref{alg:single_round_pbs}.

\begin{algorithm}
\caption{Termination condition when BCH decoding fails}
\label{alg:3_way_partition}

\If{BCH decoding fails\label{step:if1}}
{Hash-partition the group into $3$ sub-groups and do PBS for each of them in the next round; Break;}\label{step:term1} 

\end{algorithm}

% Back to the \autoref{proto:multirounds}, which shows the set reconciliation operations in each round of PBS-basic, this kind of exceptions only affect \autoref{step:reconcile} in \autoref{proto:multirounds}. Now this step needs to check whether BCH decoding is successful or not: If successful, all the operations remain the same; Else, we hash-partition the group ($A$ and $B$) into $3$ sub-groups and reconcile them respectively using \autoref{proto:multirounds}. 
{\bf I'm not sure if it is necessary to discuss this case, since PinSketch did not mention it, even it may happen in PinSketch}
Another type of exceptions that happens when $d_i>t$ is, the BCH decoder mistakes the decoding is successful and returns $t$ incorrectly decoded bit errors (i.e., subset pairs). The probability of this type of exceptions is very small. For instance, when $d=1000, \delta=5, t=13$ $(2.5\delta)$, $d_i>t$ happens with probability roughly $6.7\times 10^{-5}$, and the probability that the BCH decoder mistakes the decoding is successful when $d_i>t$ is on the order of $10^{-7}$ \cite{kim1996undetected}. So the probability that this type of exceptions happens in each group is on the order of $10^{-12}$. On the other hand, the impact of this type of exceptions is insignificant. Assume an incorrectly decoded bit error corresponds to a random subset pair, which could contain (1) no distinct element; (2) exactly $1$ distinct element; or (3) more than $1$ distinct elements. Reconcile the subset pair using \autoref{alg:trivial_case} could (1) get nothing and waste $\log |\mathcal{U}|$ bits of communication overhead; (2) get an actual distinct elements; or (3) trigger the exceptions that were discussed and handled in \autoref{subsec:exception_hash_partition}. 

% We handle this type of exceptions by the same method (i.e., hash-partition into $3$ sub-groups) as above. To detect them, on the other hand, is simple: Note that incorrect decoded bit errors correspond to the subset pairs that do not contain distinct elements. When we reconcile those subset pairs in \autoref{sec:reconcile_by_trivial}, the output (i.e., reconciled elements) will be $\mathbf{0}$, which is abnormal (since $\mathbf{0}\notin A\bigcup B$, as we described in \autoref{subsec:protocol0}). Hence, this type of exceptions happen if and only if one of the reconciled distinct elements is $\mathbf{0}$. 
%Hence, we consider BCH decoding is successful by two criteria: (1) the BCH decoder reports a successful decode; and (2) None of the reconciled elements is $\mathbf{0}$. 
% ========================
% In fact, even if $d_i>t$, PBS-basic is still possible to reconcile group $i$ in some nonideal cases. For example, when $t=10$ and $d_i=11$, if the $11$ distinct elements are distributed in $10$ subset pairs, such that $1$ subset pair contains $2$ distinct elements and $9$ subset pairs contain $1$ distinct element in each, the two parity bitmaps differ at only $9$ bit positions. So BCH decoder is able to decode the later $9$ subset pairs and the corresponding $9$ distinct elements can be reconciled. In the second round, only $2$ distinct elements remain and BCH decoding certainly works. In this case, we do not need to partition the group into sub-groups, and this case does not trigger \autoref{alg:3_way_partition} in PBS. 
% ========================
% Instead, it will either (1) report a failure about exceeding the error-correction capability; or (2) mistake the decoding is successful and return incorrect decoded bit errors. 

% The second case happens with a very small probability (in order of $10^{-7}$ \cite{kim1996undetected}) and is very simple to detect : 

% The first case is easy to handle: We can simply adapt the same algorithmic trick to partition the group into smaller groups and reconcile them respectively. In our scheme, we set the number of smaller groups to be $3$, which is big enough because $d_i$, if not smaller, only slightly larger than $t$ with high probability. The second case on the other hand, although theoretically possible, happens with a very small probability when $d_i>t$ (in order of $10^{-7}$ \cite{kim1996undetected}). Besides, the probability of $d_i>t$ is also very small (e.g., when $t=15$ and $\delta=5$, this probability is about $2.3\times 10^{-4}$), so the overall probability of the second case, which is the multiplication of these two small numbers, is negligible (e.g., in order of $10^{-11}$).

% \subsection{Multi-rounds}

% Even if the ideal case does not happen, most of the distinct elements should be distributed into different subset pairs and therefore can be reconciled. So our scheme, even cannot reconcile all of the distinct elements, can still reconcile the majority of them (piecewise decodability). To reconcile the rest distinct elements, we can just run our scheme for multi-rounds under different hash-partition functions. For each round, our scheme works as follows: 

% \IncMargin{1em}
% \begin{algorithm}
% \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
% \Input{Two sets $A$ and $B$}
% \Input{Size of set difference $d$}
% \Input{The number of subset pairs $n$}
% \Input{BCH error-correction capability $t$}

% Hash-partition $A$ and $B$ into $n$ subset pairs $\{(A_i,B_i)\}_{i=1}^n$;

% \If{BCH decoding fails}
% 	Hash-partition $A$ and $B$ into $3$ subset pairs and reconcile them respectively in the next round\;
% \ElseIf{BCH decoding success}
	
% \Else{}

% $k \leftarrow \lceil \frac{t}{c}\rceil $\;

% Partition elements into $k$ subsets using~\autoref{alg:random-part}\;

% \For{$j = 0$ \KwTo $k-1$}{
%     Reconcile the $j$-th subset pair using the straw-man scheme with the BCH correcting capability $\tau$, number of smaller subsets $m$, and number of rounds $r$\;
% }

% \caption{PBS (per round)} \label{proto:II}
% \end{algorithm}\DecMargin{1em}

% This {\bf multi-rounds} scheme can significantly increase the success probability (i.e., the probability that all distinct elements are reconciled). Readers may wonder in the later rounds, most distinct elements should be reconciled, and the remaining could be reconciled using degraded parameters (i.e., smaller $n$ and $t$). In fact, degrade parameters in later rounds cannot save much communication overhead, since the majority of it is spent in the first round (i.e., $>90\%$). Therefore, we use the same parameters (i.e., $n,t$) among all rounds in our evaluation. 
% %The tradeoff between the number of rounds and the communication overhead per rounds will be elaborated in \autoref{sec:tail_bound}. In our evaluation, $r=2,3$ rounds are enough to achieve an extremely high success probability. 

% Readers may think the cost (i.e., communication overhead and the computational complexity) of this multi-rounds scheme is proportional to the number of rounds (denoted as $r$) and increases linearly with $r$. In fact, the cost of each round is roughly proportional to the number of remaining distinct elements, which decreases exponentially as $r$ increases (i.e., the first round reconciles $99\%$ of distinct elements, the second round reconciles $99\%$ of the remaining $1\%$ distinct elements, etc.). So the cost of this multi-rounds scheme is only slightly larger than that of the single-round scheme. Furthermore, as we explained in \autoref{sec:intro}, {\bf from intro thanks for the piecewise decodability of our solution, in almost all practical application scenarios, this tradeoff does not lead to longer response time because the reconciliation of objects identified by the successfully decodable codewords, which constitute the vast majority of all codewords, can run in parallel with the transmissions and decodings of the rest.  In other words, the piecewise decodability effective masks the slightly larger number of communication rounds as far as the response time is concerned.} 





\begin{comment}
\subsubsection{Random Partition}

\IncMargin{1em}
\begin{algorithm}
% \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
% \Input{Set $S$}
% \Input{The number of subsets $m$ for partition}
% \Output{Subsets $S_1, S_2, ..., S_m$}

% Generate hash function $h(\cdot)$ that maps each element into $\{1,2,...,m\}$;

\ForEach{$s \in S$}{
    $j \leftarrow h(s) \bmod m$\;    
    Insert $s$ into the $j$-th subset $S_j$\;
}

\caption{Partition using hash function $h(\cdot)$.} \label{alg:random-part}
\end{algorithm}\DecMargin{1em}

Like the strawman scheme, our scheme randomly partitions sets $A$ and $B$ into $m$ subsets. This random partition 
can be easily accomplished by using some hash function, $h(\cdot)$, and inserting each element $x$ into the subset 
corresponding to $h(x)$. \autoref{alg:random-part} presents the pseudo-code of this random partition using hash 
function $h(\cdot)$.  

% Unlike the strawman scheme, our scheme only reconciles those subset pairs that need to be reconciled, 
% because 



Like the strawman scheme, our scheme hash-partitions the two sets $A$ and $B$ into $m$ subset pairs $(A_i, B_i)$ for $i=1,2,\cdots,m$. 
We note that, among those $m$ bins (subset pairs), 
at most $t$ ($t\!\ll\!m$ as shown in our analysis in~\autoref{subsec:protocol1}) bins contain balls 
(elements belonging to the set difference), {\it i.e.,} requiring reconciliation.  
Motivated by this observation, we, therefore, propose to first detect those bins that 
contain balls and then only reconcile them. The detection is solved with a simple encoding approach that 
will be detailed in the next section.

\subsubsection{Detection before Reconciliation} 

In fact, identifying those non-empty bins is easy when each bin contains at most one ball. In this section, we assume that 
each bin after the random partition contains at most one ball, we will show later how to handle the cases when some 
bins contain more than one balls later in~\autoref{subsec:exceptions}. 

Given an arbitrary bin (say subset pair $(A_i, B_i)$) that contains one ball ({\it i.e.,} $A_i\Delta B_i$ contains exactly one element), 
the corresponding two subsets $A_i$ and $B_i$ differ exactly one element, which implies that 
$||A_i|\!-\!|B_i||\!=\!1$. Hence, if $|A_i|$ ({\it i.e.,} number of 
elements in $A_i$) is odd (or even), then $|B_i|$ must be even (or odd). In other words, the odevity of $|A_i|$ 
and $|B_i|$ are opposite. %differs if $|A_i\Delta B_i|\!=\!1$. 
Based on this property, we propose the {\it odevity encoding}: 
A subset is encoded as ``1'' if it contains odd number of elements, and as ``0'' otherwise. 
Using this odevity encoding, the $m$ subsets of $A$ can be encoded as a bit string $b_A$ in $\{0,1\}^m$, 
where the $i$-th bit in $b_A$ corresponds to the odevity encoding of $|A_i|$. Similarly, the $m$ subsets of $B$ can also 
be encoded as a bit string $b_B$. Clearly, $b_A$ and $b_B$ differ at $t$ different positions, or in other words, 
the Hamming distance of bit strings $b_A$ and $b_B$ is $t$. A straightforward approach is 
to let Alice send $b_A$ to Bob, and then Bob compares $b_B$ against $b_A$ to obtain those non-empty bins. 

This approach, however, has a communication overhead of $m$ bits, which is still unnecessarily high. As 
analyzed in~\autoref{subsec:protocol0}, $t$ is usually much smaller than $m$. 
That means $b_A$ and $b_B$ differ only at a tiny portion of bits. %have much more in common than differences. 
Therefore, if we view $b_B$ as a corrupted message of $b_A$ with $t$ corrupted bits, the detection of those $t$ bins can be converted to 
the detection of the positions of the $t$ corrupted bits. The latter can be solved using an Error-Correction Code (ECC)~\cite{Lin_ErrorControlCoding_1983} that can correct up to $t$ errors. In this work, we use the BCH code~\cite{Lint_IntroductionCodingTheory_1998}. 
More precisely, this ECC-based approach (with the BCH code) works as follows. 
Alice computes the parity bits for $b_A$ using a $t$-error-correcting BCH code with a block length of 
$(2^{\lceil \log m\rceil} -1)$ and sends the parity bits to Bob. Bob then decodes the positions of the $t$ corrupted bits 
using the BCH decoding algorithm with $b_B$ and those parity bits received from Alice. The communication overhead of 
this approach is roughly $t\lceil \log m\rceil$ ($=O(t\log t)$) bits. In the example above, this communication overhead is 
roughly $\num{17000}$ bits, which is approximately $6$ times lower 
than $m\!=\!\num{108469}$ bits, the communication overhead of the aforementioned straightforward approach. 

At first sight, it seems that the detection of non-empty bins and reconciliation of subsets in those bins require two rounds 
(or at least two round trip delays), {\it i.e.,} one round for detection and the other for reconciliation. In fact, 
it only requires one. After Bob receives the parity bits from Alice and decodes out those non-empty bins, it initiates 
the reconciliation ({\it i.e.,} \autoref{alg:trivial_case}) for each bin (subset pair) immediately, 
{\it i.e.,} sends the \code{XOR} sums of subsets in those bins together the indexes of those bins. 
After receiving those \code{XOR} sums and bin indexes, Alice can compute the set difference. 

% A naive way to combine the detection of non-empty bins and reconciliation of subset pairs in those bins is to first detect 
% those non-empty bins via one round of message exchanges between Alice and Bob and then to reconcile the corresponding 
% subset pairs in those bins with another round of message exchanges. This requires two rounds ({\it i.e.,} taking at least 
% two round trip delays). In fact, after Bob receives the parity bits from Alice and obtains those 

\subsubsection{Multiple Rounds}\label{sec:multiround}

{\bf This section was not clear enough. I need more time to think about and revise it.}


In the above section, we have assumed that each bin contains at most one ball. 
However, even with a sufficient large $m$, some bin might contain more than one balls though with tiny probability. 
We will show in~\autoref{subsec:exceptions}, how such rare events, {\it i.e.,} one bin contains more than one balls, 
can be easily detected.
To ensure our scheme can successfully reconcile all elements even when such rare events happen, 
we propose to use multiple rounds (of communication between Alice and Bob). More precisely, instead of 
selecting a prohibitively large $m$ to ensure that each bin contains at most one ball with a extremely high probability 
(say 0.99999), we select a reasonably large $m$ so that the communication overhead is not very high and very few bins contain 
more than one balls (or in other words, most bins contain at most one ball). Therefore, after running one round of 
our scheme, most elements in the set difference will be reconciled. Only those in the bins that contain more than one balls 
fail to be reconciled. For elements in the subsets corresponding to those bins, we run another round of our scheme. 
If some elements still fail to be reconcile, we can run one more round of our scheme. So on so forth,  
our scheme can keep running for more rounds until all elements are reconciled. 

With the same communication overhead, multiple rounds can significantly increase the success rate, 
{\it i.e.,} the probability that all elements in the set difference will be successfully reconciles, 
which will be elaborated in~\autoref{sec:tail_bound}. 

% % to be emphasized
% % say that too many rounds should be avoided (latency & communication overhead reduction is negligible when r is too large, 2 - 3 is good enough)
% % multiple rounds is not an issue when r is small

% We note that the number of rounds $r$, however, should not be large. On one hand, it results in large latency (at least $r$ round trip delays). 
% On the other hand, when $r$ is large, the reduction of communication overhead by the increase of $r$ gradually diminishes. 

We note that multiple rounds, when $r$ is small, would not really increase the ``latency'', as long as most elements in the 
set difference can be reconciled in the first rounds, since the underlying synchronization of data objects corresponding to 
those elements can start immediately after the first round of our scheme. Therefore, the actual latency is one round trip delay instead of 
$r$. 

As we mentioned, this straw-man protocol works correctly if each subset pair has at most one exclusive element (i.e., \autoref{eq:requirement_strawman} holds). On the other hand, if a subset pair has more than one exclusive elements, some of which will not be successfully reconciled:

\begin{itemize}
\item If a subset pair has even number of exclusive elements, Odevity coding will encode it as 0. Then the straw-man scheme will consider the subset pair having no exclusive element and all exclusive elements in this subset will not be reconciled;

\item If a subset pair has odd number ($\geq 3$) of exclusive elements, Odevity coding will encode it as 1 and consider the subset pair having only 1 exclusive element. Then the straw-man scheme will use \autoref{alg:trivial_case} to decode only one exclusive element and dismiss all others. Even worse, the only decoded element is probably not a real exclusive element, since the element computed by \autoref{alg:trivial_case} is the \code{XOR} sum of all exclusive elements, not one of them. 
\end{itemize}

In summary, if a subset pair has more than one exclusive elements, most of its exclusive elements cannot be reconciled, and the reconciled element is usually incorrect (i.e., false-positive). The false-positive however is easy to check, which will be elaborated in \autoref{subsec:exceptions}. The good thing is, even if not all subset pairs have at most one exclusive element and are successfully decoded, most of them will be w.h.p.. In other words, even if the straw-man protocol cannot reconcile all exclusive elements, it still can reconcile most of them. To reconcile all exclusive elements w.h.p., we can simply extend the single-round straw-man scheme to multi-round. And each round adapts the straw-man scheme to do set reconciliation using independent hashing functions $h(\cdot)$ for partition (i.e., in \autoref{alg:random-part}). This multi-round extension can significantly increase the probability of a successful reconciliation, which will be elaborated in \autoref{sec:tail_bound}. 



\subsection{Our Scheme: The Final Version}\label{subsec:protocol2}

{\bf Under revision~}

The preliminary version of our scheme suffers from two major drawbacks. 
First, its communication overhead is asymptotically 
$O(t\log m)\!=\!O(t\log t)$, which is not asymptotically optimal. 
Second, the decoding computational complexity is proportional to 
$t^2$ with the state-of-the-art decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} for BCH codes, 
which is too high when $t$ is large. 
To overcome these two drawbacks, we use a simple algorithmic trick: divide and conquer. With this algorithmic 
trick, the decoding computational complexity is reduced to $O(t)$, 
and the communication overhead is reduced to $t\cdot\frac{\log u}{8} \!+\! O(t)$ (with a small 
hidden constant roughly varying from 4 to 8) bytes which implies that 
our scheme has an additive communication overhead (compared to the optimal scheme) 
of 4 to 8 bytes per element in the 
set difference and this additive overhead is independent of the key size ({\it i.e.}, $\log u$). 
Recall that the IBF-based schemes usually have a communication overhead of roughly 6 times of the 
optimal scheme, which increases linearly as the key size. Therefore, our scheme is much more 
communication-efficient. 

Now, we describe in detail this algorithmic trick. We let Alice divide elements in $A$ into $\lceil\frac{t}{c}\rceil$ groups (subsets)  
for some small constant $c$ (say $5$) so that each group contains roughly $c$ elements from the set difference on average. We let Bob do the same operations on $B$. To ensure that any common element ({\it i.e.,} any element $x\!\in\! A\bigcup B$) goes into 
the same group ({\it i.e.,} groups at Alice and Bob with the same index), we can use the partition procedure with a hash function shown 
in~\autoref{alg:random-part}. Then, we can apply the preliminary version on each group with a constant $m$ (say $m\!=\!256$) independent of 
$t$. To ensure that each group can be reconciled with a high probability, we need to use BCH codes whose decoding capacity 
larger than $c$ (say $\tau\!=\!2c$), as exact number of elements to be reconciled could be larger than $c$. 
Since this decoding capacity $\tau$ is still a small constant independent of $t$, therefore, the communication 
overhead per group is $\tau\cdot\log m \!=\!O(1)$, which implies a total communication overhead of $O(t)$. 
Similarly, the total decoding computational complexity is also $O(t)$. 

\subsubsection{Parameter Configurations} 

Our scheme now has several parameters: $c$ (average number of elements from the set difference in each group), 
$\tau$ (the correcting capability of the BCH code), $m$ (number of bins for each group), and $r$ (maximum number of rounds). 
We note that the maximum number of rounds $r$ is usually associated with another parameter $p$ the desired success rate: With 
at most $r$ rounds, our scheme should guarantee that the success rate is at least $p$. 
%How to tune these parameters to achieve favorable performance will be detailed later in~\autoref{sec:tail_bound}. 
Here, we provide some guidances for the parameter configurations using our theoretical analysis, which gives the tail bound of 
the success probability of our scheme and will be shown in~\autoref{sec:tail_bound}. 

\noindent
{\bf Parameterizing $c$ and $r$.} The values of $c$ and $r$ are usually provided by users based on the requirements of 
applications. For the value of $c$, a larger $c$ results in a longer decoding time yet lower communication overhead.  
So if the decoding time is a big concern, then a smaller $c$ (say $c=5$) should be used; otherwise, a larger $c$ could be used. 
For the values of $r$, a larger $r$ leads to lower communication overhead and usually lower decoding time (as it allows to use 
a smaller $\tau$), however, the reduction is marginal when $r>3$. Therefore, we suggest users to configure $r$ to be $2$ or $3$. 
% The configuration of $c$ is relatively straightforward, as a larger $c$ will result in 
% a longer decoding time and a slightly lower communication overhead. The former is ..., The latter is slightly tricky. 


\noindent
{\bf Using $c$ and $r$ to parameterize other parameters.} After users specify the values for $c$ and $r$ (associated with a value for 
$p$), we can use our theoretical analysis in~\autoref{sec:tail_bound} to parameterize $\tau$ and $m$. 
Since in a BCH code, the block length is in the form of $2^q-1$, we only need to consider $m=2^q-1$. 

{\bf Liang, please revise the following algorithm!}

\begin{algorithm}
\SetKwProg{Proc}{}{}{end}
\SetKwFunction{algo}{\small Search}

\Proc{Search($c$, $r$, $p$)}{\label{search:entrance}

$\mbox{co}_{best}\leftarrow\infty$\tcc*{\small Best communication overhead}

\For{$\tau \leftarrow c\,\KwTo\, \infty$}{}



}
\end{algorithm}


% , unlike 
% the IBF-based schemes which have an multiplicative overhead of 6 
% The inspiration is from the famous 
% divide and conquer algorithm for the selection problem, in which, given an array with $n$ elements, we want to get the $k$-th largest 
% element. A straightforward idea for this problem is sorting. However, if using insertion-sorting, the complexity would be $O(n^2)$. 
% Then the famous divide and conquer trick comes. It first divides the array into $\lceil n/5\rceil$ groups so that the first 
% $\lfloor n/5\rfloor$ contains $5$ elements and at most one group contains the rest $n \mod 5$ elements, and find the median of each 
% group using the insertion-sorting and th


% This straw-man scheme still has a problem on decoding computational complexity. More specific, the complexity increases dramatically with the total number of corrupted bits $t$. Therefore, when $t$ is moderate or large, the decoding computational complexity could be very high. For instance, the decoding complexity of BCH codes~\cite{Lint_IntroductionCodingTheory_1998} is $O(t^3)$, which could be quite high for a large $t$. To keep the decoding complexity reasonably low, we design the following two-layer protocol: In the first layer, we use a hash function to partition the two sets into $\lceil\frac{t}{c}\rceil$ subsets for some small constant $c$ (say $5$), just like the first step of our straw-man scheme. The objective, which is however different from before, is to make each subset pair contains roughly $c$ exclusive elements on average. In the second layer, we use the straw-man scheme with the same configuration (number of subsets $m$, and error-correction capability $\tau$, number of rounds $r$) to reconcile each subset pair. 

% In fact, the straw-man scheme is a proper solution when $t$ is small. First, the decoding complexity will not be a problem for a small $t$; Second, we do not need an extremely large $m$ to guarantee \autoref{eq:requirement_strawman} w.h.p.. For instance, when $t=5$ and $m=1024$, \autoref{eq:requirement_strawman} holds with probability $\frac{m\,!}{(m-t)\,!m^t}\approx 99\%$. This motivates us to design the following two-layer protocol: In the first layer, we use a hash function to partition the two sets into $\lceil\frac{t}{c}\rceil$ subsets for some small constant $c$ (say $5$), just like the first step of our straw-man scheme. The objective, which is however different from before, is to make each subset pair contains roughly $c$ exclusive elements on average. In the second layer, we use the straw-man scheme with the same configuration (number of subsets $m$, and error-correction capability $\tau$) to reconcile each subset pair. 

\autoref{proto:II} shows the pseudocode of our scheme. It first uses the same hash-function based random partition algorithm as \autoref{alg:random-part} to partition elements into $k\triangleq\lceil \frac{t}{c} \rceil$ subsets. Note that the random partition only guarantees that each such subset 
contains $c$ exclusive elements on average, and the exact number is not known. Hence, our scheme uses a BCH code with a capability of 
correcting up to $\tau$ errors with $\tau > c$ to make sure that the BCH code has a high probability to decode successfully. We will describe how to deal with situation where the size of set difference exceeds $\tau$ later in~\autoref{subsec:exceptions}.

As the decoding of a $\tau$-error-correcting BCH code where $\tau$ is a small constant has a constant-time computational complexity, the decoding complexity of 
our scheme is $O(k)=O(t)$. We now have several parameters, average number of exclusive elements in each subset $c$, the correcting capability $\tau$ of BCH code, the number of smaller subsets $m$ for each subset to be divided to, and the number of rounds $r$. How to tune these parameters to achieve favorable performance will be detailed later in~\autoref{sec:tail_bound}. 

\IncMargin{1em}
\begin{algorithm}
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
\Input{Size of set difference $t$}
\Input{The number of subsets $m$ for each partition}
\Input{Average number of exclusive elements in each partition $c$}
\Input{BCH code capability $\tau$}

$k \leftarrow \lceil \frac{t}{c}\rceil $\;

Partition elements into $k$ subsets using~\autoref{alg:random-part}\;

\For{$j = 0$ \KwTo $k-1$}{
    Reconcile the $j$-th subset pair using the straw-man scheme with the BCH correcting capability $\tau$, number of smaller subsets $m$, and number of rounds $r$\;
}

\caption{Our Scheme} \label{proto:II}
\end{algorithm}\DecMargin{1em}




\subsection{Exceptional Handling}\label{subsec:exceptions}

{\bf To be revised~}

In this section, we will elaborate how to handle the following two types of exceptions that we mentioned in \autoref{sec:multiround} and \autoref{subsec:protocol2}:
\begin{itemize}
    \item Exception 1: A subset pair has odd number ($\geq 3$) of exclusive elements and causes false-positives (i.e., a decoded distinct element is not a real one);
    \item Exception 2: A subset pair contains too many exclusive elements, such that a BCH code with capability of correcting up to $\tau$ errors cannot decode it (i.e., $t>\tau$).
	\item Exception 3: A subset pair has even number ($\geq 2$) of exclusive elements and causes false-negatives(i.e., two or more distinct elements are neglected as the parity bit is 0);
\end{itemize}

To handle Exception 1, we need to check whether a computed exclusive element by \autoref{alg:trivial_case} is a real exclusive element or not. (The group index happens to come in handy if we use it as a fingerprint of the element we computed. If this element is truly an exclusive element, it should be hashed into the same group as before. Notably, We have two group indices available for this check, one is in the initial divide and conquer phase, the other is in the BCH code part) It can be easily done at the end of set reconciliation, during which two hosts exchange their exclusive elements. In fact, as we will elaborate in \autoref{sec:tail_bound}, Exception 1 hardly happens if we set parameters properly. 

On the other hand, when Exception 2 happens, the BCH decoder will report a failure about exceeding the error-correction capability. For such a subset pair, we can use the same approach as in \autoref{subsec:protocol2} to partition it into smaller subsets and use the straw-man scheme to reconcile them respectively. We set the number of small subsets to be 3. It is because, as we will elaborate in \autoref{sec:tail_bound}, the number of exclusive elements for each subset pair $t$ should be, if not smaller, only slightly larger than $\tau$ w.h.p.. Partitioning those exclusive elements into 3 small subsets is enough to guarentee that each of them has less than $\tau$ exclusive elements.

\end{comment}

==> section/schemes_new0222.tex <==
%\section{PBS for small \texorpdfstring{$d$}{d}}\label{sec:scheme}
\section[PBS for small \texorpdfstring{$d$}{d}]{PBS for small \texorpdfstring{\larger\boldmath\MakeLowercase{$d$}}{d}}\label{sec:scheme}
%\section{Set Reconciliation}\label{sec:scheme}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%     Writing Guideline for This Section     %%%%%%%%%%
% “balls – elements in the symmetric difference of the two sets” 

% Protocol 0 (reconcile two sets whose set difference has at most one ball)

% Protocol I.I (partition elements into a sufficiently large number of subsets such that each subset has at most one ball with high probability and use Protocol 0 to reconcile each of them) 

% Protocol I.II (a two-step refinement of Protocol I.I: first use BCH to identify good bins, i.e., bins/subsets have exactly one ball, and then use Protocol 0 to reconcile each good bin) 

% Protocol II (a two-layer refinement of Protocol I.II: in the first layer, we partition elements into t/c subsets, where t is the size of set difference and c is a small constant, then each subset has c balls on average. In the second layer, we further partition each subset into large enough number of bins/subsets such that with high probability each bin has at most one ball, then use Protocol I.II to reconcile them one by one) 

% Protocol III/IV (mainly fix certain exceptions in Protocol II，e.g., how to address bad bins, how to handle the cases where BCH fails to decode and etc)

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% In this section, we describe our set reconciliation scheme in details. First, we give a formal problem statement in \autoref{sec:model}. In \autoref{subsec:protocol0}, we introduce a basic scheme for the trivial case, in which the two sets $A$ and $B$ has at most one distinct element. Building upon the basic scheme, we propose the preliminary version of scheme in \autoref{sucsec:our-scheme} that targets to the cases where the total number of distinct elements $d$ is small. Then we extend the preliminary version and propose the final version of our scheme in \autoref{subsec:protocol2} for general cases (i.e., any arbitrary $d$). We assume $d$ is precisely known throughout this section except in \autoref{subsec:ToW}, where we will describe how to estimate $d$ using a Tug-of-War Estimator. 


In this section, we describe our PBS scheme for Alice and Bob to reconcile their respective sets $A$ and $B$, where $d=|A\Delta B|$ is small and precisely known. Throughout this paper, we call each element in $A\Delta B$ a \textit{distinct element}, and each element in $A\bigcap B$ a \textit{common element}. We build up our scheme gradually by starting with the trivial case where $d\leq 1$ in \autoref{subsec:protocol0}. Then we generalize our scheme to the case where $d$ is a small number in \autoref{sec:pbs_smalld}. 

\begin{comment}
\subsection{Problem Statement}\label{sec:model}

In this work, we adopt the commonly used model for the set reconciliation problem. 
Two remote sets $A$ and $B$ are stored at hosts Alice and Bob respectively. 
Each element in $A$ and $B$ is a hash signiture in the key space (universe) $\mathcal{U}$, which is the set of all $(\log |\mathcal{U}|)$-bit binary strings. 
%Each element in $A$ and $B$ is a hash signiture with signiture width $w$ in the key space (universe) $\mathcal{U}$, which is the set of all $w$-bit binary strings (i.e., $|\mathcal{U}|=2^w$). 
%We use $\mathcal{U}$ to denote the set of all $w$-bit binary strings and name it the universe of signitures. 
The set reconciliation problem is to compute the symmetric set difference between $A$ and $B$, 
{\it i.e.,} $A\Delta B\triangleq (A\!\setminus\! B) \bigcup (B\!\setminus\! A)$. 
Let $d\!=\!|A\Delta B|$ be the cardinality of this difference.
%We denote $d\!=\!|A\Delta B|$. 
Throughout this paper, we call each element in $A\Delta B$ a \textit{distinct element}, and each element in $A\bigcap B$ a \textit{common element}.
{\bf Like in all existing solutions, we describe only {\it unidirectional} set reconciliation, in which Alice or Bob learns the set difference $A\Delta B$. Since the performance of our scheme does not depend on who learns the set difference, we assume Bob learns the set difference $A\Delta B$ in the rest of the paper, as mentioned in \autoref{sec:psea}.}
% As mentioned in \autoref{sec:psea}, we describe {\it unidirectional} set reconciliation that Bob learns the set difference $A\Delta B$. 
%In \autoref{sec:evaluation}, we use the same semantic to measure the communication cost of our scheme and other compared set reconciliation schemes. 
\end{comment}

% In the rest of this section, we build up our scheme gradually as follows: We start with the trivial case where $d\leq 1$ in \autoref{subsec:protocol0}. Then we generalize our scheme to the case where $d$ is a small number in \autoref{sec:pbs_smalld}. 

%After that, we further generalize our scheme to the case that $d$ is a large number in \autoref{subsec:protocol2}. 
%Throughout this section, we assume $d$ is precisely known.
%except in \autoref{subsec:ToW}, where we will describe how to estimate $d$ using a Tug-of-War Estimator. 

%The rest of this section is organized as follows: In \autoref{subsec:protocol0}, we introduce a basic scheme for the trivial case, in which the two sets $A$ and $B$ has at most one distinct element. In \autoref{sucsec:our-scheme} and \autoref{subsec:protocol2}, we elaborate the two versions of our solution that are introduced in \autoref{sec:smalld} and \autoref{sec:larged} respectively. Throughout this section, we assume $d$ is precisely known except in \autoref{subsec:ToW}, where we will describe how to estimate $d$ using a Tug-of-War Estimator. 

\subsection{The Trivial Case of \texorpdfstring{\larger\boldmath $d\leqslant 1$}{d<2}}\label{subsec:protocol0}

%We start with the trivial case, in which $A$ and $B$ have at most one distinct element ({\it i.e.,} $d\leq 1$), we have a simple set reconciliation scheme showed in \autoref{alg:trivial_case}:

\autoref{alg:trivial_case} shows the reconciliation scheme for the trivial case, in which $A$ and $B$ differ by at most one distinct element:

\begin{algorithm}
\caption{Set reconciliation when $d\le 1$}
\label{alg:trivial_case}

{\it Bob}: $s_B\leftarrow\underset{b\in B}{\oplus} b$; Send $s_B$ to Alice\; \label{alg1:sender}

{\it Alice}: $s_A\leftarrow\underset{a\in A}{\oplus} a$; $s\leftarrow s_A \oplus s_B$\; \label{alg1:receiver}
\end{algorithm}

First, Bob calculates $s_B$, the bitwise \code{XOR} of all elements in $B$, and send it to Alice. 
Second, Alice also calculates $s_A$, the bitwise \code{XOR} of all elements of $A$. Upon receiving $s_B$, Alice computes $s\!\triangleq\! s_A \!\oplus\! s_B$, and we have

\begin{sitemize}
	\item If $A$ and $B$ are identical sets (i.e., $d=0$), we have $s_A=s_B$ and $s=\mathbf{0}$;
	\item If $A$ and $B$ has one distinct element (i.e., $d=1$), the computed $s$, the bitwise \code{XOR} of $s_A$ and $s_B$, will cancel out all common elements and remain the distinct element. In other words, we have $A\Delta B=\{s\}$. 
	%And $s$ is the missing element of $A$ (i.e., $s\in B\!\setminus\! A$) if $s\in B$, or the missing element of $B$ (i.e., $s\in A\!\setminus\! B$) otherwise;
	% \item If $A$ and $B$ has more than one distinct elements (i.e., $d>1$), the bitwise \code{XOR} of $s_A$ and $s_B$ will still cancel out all common elements and remain the \code{XOR} of the distinct elements, i.e., $s$ is the \code{XOR} of all distinct elements;
\end{sitemize}

Like most works on set reconciliation, we assume $\mathbf{0}$ is excluded from $\mathcal{U}$, as \autoref{alg:trivial_case} does not work when $\mathbf{0}\in A\bigcap B$ for the following reason: When $s=\mathbf{0}$, \autoref{alg:trivial_case} cannot tell whether $A$ and $B$ are identical, or they have a distinct element of value $\mathbf{0}$. 
%However, we can extend our scheme to support $\mathbf{0}$. For example, we let Alice send to Bob a single bit to indicate whether Alice has element $\mathbf{0}$, so Bob will know whether $\mathbf{0}\in A\Delta B$ or not. 
\autoref{alg:trivial_case} also does not work when there are more than one distinct elements in $A\Delta B$ (i.e., $d>1$), since the computed $s$ is the \code{XOR} of all these distinct elements.

% Note that \autoref{alg:trivial_case} works if and only if $|A\Delta B|\!\leq\! 1$ and $0\!\notin\! (A\!\cup\! B)$ (which we have explained in~\autoref{sec:model}). 

%\subsection{PBS: When $d$ is small}\label{sucsec:our-scheme}

%In this section, we generalize PBS to the case when $d$ is a small number, as we described in \autoref{sec:smalld}. 
%First, we describe each step of single-round PBS from \autoref{sec:hash_partition} to \autoref{sec:reconcile_by_trivial} and summarize it in \autoref{sec:single_round_pbs}. Second, we discuss the exceptions in single-round PBS in \autoref{subsec:exception_hash_partition}. Third, we propose multi-round PBS to handle the exceptions.

\subsection{PBS for small \texorpdfstring{\larger\boldmath $d$}{d}}\label{sec:pbs_smalld}

In this section, we substantiate the scheme described in \autoref{sec:smalld} for small $d$.

\subsubsection{Hash Partition and Parity Bitmap Encoding}\label{sec:hash_partition}
% \medskip
% \noindent{\bf Hash Partition} 

Here we formalize the aforementioned process of partitioning $A$ into $\{A_i\}_{i=1}^n$, $B$ into $\{B_i\}_{i=1}^n$, and $A\Delta B$ into $\{A_i\Delta B_i\}_{i=1}^n$ 
using a hash function $h(\cdot)$.
%as described in \autoref{sec:smalld} by introducing the concept of {\it sub-universes}. Given a hash function $h(\cdot): \mathcal{U}\rightarrow \{1,2,\cdots,n\}$, we 
Define {\it sub-universe} $\mathcal{U}_i$ as the set of elements in the universe $\mathcal{U}$ that are hashed into value $i$. More precisely, $\mathcal{U}_i\triangleq\{s\!\mid\! s\in \mathcal{U} \mbox{ and } h(s)=i\}$ for $i=1,2,...,n$. Then defining $A_i\triangleq A\bigcap\mathcal{U}_i$ and $B_i\triangleq B\bigcap\mathcal{U}_i$ for $i=1,2,...,n$ induces the partitioning of $A$, $B$, and $A\Delta B$.
%, as mentioned in \autoref{sec:smalld}. 

{\bf (merged from the later two paragraphs)} How the $d$ distinct elements (balls) in $A\Delta B$ are distributed into the $n$ subset-pair-differences $\{A_i\Delta B_i\}_{i=1}^n$ (bins) can be viewed as throwing $d$ balls each uniformly and randomly into one of the $n$ bins. 
For the moment, we assume the following {\it ideal case} happens: Every subset-pair-difference $A_i\Delta B_i$ contains at most one distinct element.  
The ideal case corresponds to the $d$ balls ending up in $d$ distinct bins. It happens with probability $\prod_{k=1}^{d - 1}(1 - \frac{k}{n})$, which is on the order of $1-O(d^2/n)$ when $n\!\gg\!d$.
%approximately $e^{-\frac{d(d-1)}{2n}}$ when $d\!\ll\!n$. 
Hence, $n$ must be $\Omega(d^2)$ to ensure the ideal case happens with a nontrivial probability, as mentioned in \autoref{sec:smalld}. 
%The nonideal case of a subset pair difference containing more than $1$ distinct elements will be discussed in \autoref{subsec:exception_hash_partition}.

{\bf (Previous)} For the moment, we assume the following {\it ideal case} happens: Every subset-pair-difference $A_i\Delta B_i$ contains at most one distinct element. The nonideal case of a subset pair difference containing more than $1$ distinct elements will be discussed in \autoref{subsec:exception_hash_partition}. 

%In this section, we give a detailed description on how to partition $A$ and $B$ (as introduced in \autoref{sec:smalld}) by introducing {\it sub-universes}, which is defined as follows: Given a hash function $h(\cdot): \mathcal{U}\rightarrow \{1,2,\cdots,n\}$, we define {\it sub-universes} $\{\mathcal{U}_i\}_{i=1}^n$, a partition of the universe $\mathcal{U}$, as $\mathcal{U}_i=\{s\!\mid\! s\in \mathcal{U} \mbox{ and } h(s)=i\}$ for $i=1,2,...,n$. Based on $\{\mathcal{U}_i\}_{i=1}^n$, we define $\{A_i\}_{i=1}^n$, the partition of $A$ introduced in \autoref{sec:smalld}, as $A_i\! \triangleq\! A\bigcap \mathcal{U}_i$ for $i=1,2,...,n$. $\{B_i\}_{i=1}^n$ is similarly defined. By this definition, the set difference $A\Delta B$ is partitioned into $n$ set differences of the partitioned subset pairs (i.e., $\{(A_i, B_i)\}_{i=1}^n$). From \autoref{sec:hash_partition} to \autoref{sec:reconcile_by_trivial}, we assume the following {\bf ideal case} happens: Each subset pair $(A_i, B_i)$ contains at most one distinct element ({\it i.e.,} $|A_i\Delta B_i|\!\leq\!1$). The nonideal case of a subset pair contains more than $1$ distinct elements will be discussed in \autoref{subsec:exception_hash_partition}. 

% Here we describe the hash-partition step introduced in \autoref{sec:smalld} in details. First, we use a hash function $h(\cdot): \mathcal{U}\rightarrow \{1,2,\cdots,n\}$ to partition the universe $\mathcal{U}$ into $n$ sub-universes: $\mathcal{U}_i=\{s\!\mid\! s\in \mathcal{U} \mbox{ and } h(s)=i\}$ for $\forall i=1,2,\cdots,n$. The hash function $h(\cdot)$ can be predetermined between Alice and Bob and does not require additional communication cost. Define $A_i\! \triangleq\! A\bigcap \mathcal{U}_i$ and $B_i\! \triangleq\! B\bigcap \mathcal{U}_i$ for $i=1,2,\cdots,n$. Then $\{A_i\}_{i=1}^n$ and $\{B_i\}_{i=1}^n$ are partitions of $A$ and $B$ respectively. Furthermore, $\{A_i\Delta B_i\}_{i=1}^n$ is a partition of $A\Delta B$. From \autoref{sec:hash_partition} to \autoref{sec:reconcile_by_trivial}, we assume the following {\bf ideal case} happens: Each subset pair $(A_i, B_i)$ contains at most one distinct element ({\it i.e.,} $|A_i\Delta B_i|\!\leq\!1$). The nonideal case of a subset pair contains more than $1$ distinct elements will be discussed in \autoref{subsec:exception_hash_partition}. 

{\bf (Previous)} How the $d$ distinct elements (balls) in $A\Delta B$ are distributed into the $n$ subset pair differences $\{A_i\Delta B_i\}_{i=1}^n$ (bins) 
can be viewed as throwing $d$ balls each uniformly and randomly into one of the $n$ bins. 
%follows the familiar {\it balls-into-bins} probability model. 
%The distinct elements are viewed as balls and the subset pairs are viewed as bins. 
%Each of the $d$ balls is uniformly and randomly thrown by the hash function $h(\cdot)$ into one of the $n$ bins. 
The aforementioned ideal case that corresponds to the $d$ balls ending up in $d$ distinct bins happens with probability $\prod_{k=1}^{d - 1}(1 - \frac{k}{n})$, which is on the order of $1-O(d^2/n)$ when $d\!\ll\!n$.
%approximately $e^{-\frac{d(d-1)}{2n}}$ when $d\!\ll\!n$. 
Hence, $n$ must be $\Omega(d^2)$ to ensure the ideal case happens with a nontrivial probability, as mentioned in \autoref{sec:smalld}.


%in which the distinct elements are viewed as balls and the subset pairs are viewed as bins. The hash-parition basically throws (hashes) $d$ balls (distinct elements) uniformly and randomly into $n$ bins (subset pairs). The aforementioned ideal case in this context becomes, after throwing $d$ balls uniformly and randomly into $n$ bins, each bin receives at most $1$ ball (i.e., $d$ nonempty bins have $1$ ball in each and the rest $n-d$ bins are empty). The number of balls in each bin is a Binomial random variable $Binomial(d,1/n)$.
%{\bf It may remind readers about the Birthday problem. And the ideal case can be analogous to the case that no people share the same birthday.} 
% The ideal case happens with a probability of $p\!=\!\prod_{k=1}^{d - 1}(1 - \frac{k}{n})\!\approx\! e^{-\frac{d(d-1)}{2n}}$ when $d\!\ll\!n$. In other words, $n$ must be at least $O(d^2)$ to ensure the ideal case happens with a nontrivial probability, as described in \autoref{sec:smalld}.  

% Note that the ideal case does not always happen. However, we can ensure that the ideal case happens with high probability by properly setting $n$ based on $d$ (i.e., $n=\Omega(d^2)$). Furthermore, as we will describe in \autoref{subsec:nonideal}, even if the ideal case does not happen (i.e., some distinct elements are hashed into the same subset pair), most of the distinct elements should be distributed into different subset pairs and therefore can be reconciled. So the scheme, even cannot reconcile all of the distinct elements, can still reconcile the majority of them (i.e., piecewise decodability in \autoref{sec:intro_oursolution}). Based on this property, we will extend our scheme from single-round to multi-rounds in \autoref{subsec:nonideal} to further increase the probability of reconciling all distinct elements. 

% \medskip
% \noindent{\bf Parity Bitmap Encoding} 

{\bf (Modified)} The partition $\{A_i\}_{i=1}^n$ is encoded into an $n$-bit-long parity bitmap $A[1..n]$, in which $A[i]$, the $i$-th bit of the parity bitmap, is equal to the oddness / evenness (parity) of the cardinality of $A_i$ (i.e., $A[i]=1$ if $|A_i|$ is odd; otherwise $A[i]=0$). $B[1..n]$, the parity bitmap of $\{B_i\}_{i=1}^n$, is similarly defined. In the ideal case, $A[1..n]$ and $B[1..n]$ differ in exactly $d$ distinct bit positions $i_1,i_2,...,i_d$, and each subset-pair-difference $(A_{i_1},B_{i_1}), (A_{i_2},B_{i_2}),...,(A_{i_d},B_{i_d})$ contains exactly $1$ distinct element. If Bob knows $i_1,i_2,...,i_d$, he can start to reconcile the $d$ subset pairs respectively using \autoref{alg:trivial_case}, then Alice will obtain $A\Delta B$.

{\bf (Previous)} We encode $\{A_i\}_{i=1}^n$ into an $n$-bit-long parity bitmap $A[1..n]$, in which $A[i]$, the $i^{th}$ bit of the parity bitmap, is equal to the oddness / evenness (parity) of the cardinality of $A_i$ (i.e., $A[i]=1$ if $|A_i|$ is odd; otherwise $A[i]=0$). In the ideal case, the two bitmaps $A[1..n]$, $B[1..n]$ differ in exactly $d$ bit positions $i_1,i_2,...,i_d$, each of which corresponds to a subset pair that contains $1$ distinct element. The next step is to let Alice and Bob know these bit positions.
%Once the $d$ bit positions are known, Alice and Bob can start to reconcile $(A_{i_1},B_{i_1}), (A_{i_2},B_{i_2}),...,(A_{i_d},B_{i_d})$ using \autoref{alg:trivial_case} and obtain the $d$ distinct elements (i.e., $A\Delta B$). 

% \subsubsection{Parity Bitmap Encoding}\label{sec:parity_bitmap_encoding}

% %After hash-partitioning $A$ and $B$ into partitions $\{A_i\}_{i=1}^n$ and $\{B_i\}_{i=1}^n$, 
% As introduced in \autoref{sec:smalld}, we encode each partition into an $n$-bit-long parity bitmap and denote them as $A[1..n]$ and $B[1..n]$ respectively, as introduced in \autoref{sec:smalld}. For $i=1,2,...,n$, $A[i]$ (the $i^{th}$ bit of the parity bitmap $A[i]$) is equal to $1$ if $A_i$ contains an odd number of elements, and is equal to $0$ otherwise.
% % More specifically, for $i=1,2,...,n$, $A[i]$ (the $i^{th}$ bit of the parity bitmap $A[i]$) is defined as follows: $A[i]=1$ if $A_i$ contains an odd number of elements, and $A[i]=0$ otherwise. In this way, each bit $A[i]$ encodes the oddness / evenness (parity) of the cardinality of $A_i$. The $n$-bit-long parity bitmap $B[1..n]$ and $B[i]$ (the $i^{th}$ bit of $B[1..n]$) are similarly defined. 
% In the ideal case, 
% %$A[i]$ and $B[i]$ differ if and only if $A_i$ and $B_i$ have exactly $1$ distinct element, and $A[i]$ and $B[i]$ are the same if and only if $A_i=B_i$. Meanwhile, the $d$ distinct elements are hashed into $d$ different subset pairs. So 
% the two bitmaps $A[1..n]$, $B[1..n]$ differ in exactly $d$ bit positions, each of which corresponds to a subset pair that contains $1$ distinct element. Once the $d$ bit positions are known, Alice starts to reconcile each of the $d$ corresponding subset pairs by \autoref{alg:trivial_case} and gets the $d$ distinct elements (i.e., $A\Delta B$). 
% %If knowing the $d$ bit positions (i.e., the $d$ corresponding subset pairs), we can use \autoref{alg:trivial_case} to reconcile the $d$ subset pairs respectively to obtain all the $d$ distinct elements (i.e., $A\Delta B$). 
% In \autoref{sec:BCH_code}, we will describe how to find the $d$ bit positions using BCH code~\cite{Lint_IntroductionCodingTheory_1998}. 

% \medskip
% \noindent{\bf Find the $d$ Bit Positions Using ECC} 

%\subsubsection{Find the $d$ Bit Positions Using ECC}\label{sec:BCH_code}
\subsubsection{Find and Reconcile the \texorpdfstring{$d$}{d} subset pairs}\label{sec:BCH_code}

{\bf (Modified)} To let Bob obtain $i_1,i_2,...,i_d$, Alice only needs to send a BCH code of $A[1..n]$ that can correct $d$ bit errors. Then Bob can decode and recover $A[1..n]$ (original message) and obtain $i_1,i_2,...,i_d$.

{\bf (Previous)} We view $A[1..n]$ as a corrupted message of $B[1..n]$ sent ({\bf not actually being sent}) from Bob to Alice through an {\it unreliable} commnunication channel that flips $d$ bits. To locate these $d$ bit positions, we let Bob also send an {\it error-correction code} that encodes $B[1..n]$ to Alice, such that Alice can recover $B[1..n]$ (original message) and obtain the $d$ bit positions $i_1,i_2,...,i_d$. In PBS, we use BCH code~\cite{bch1} to encode $B[1..n]$ and get the error-correction code.

There are two different BCH encoding techniques: {\it systematic} and {\it unsystematic}. The difference is, the message appears as the prefix of the codeword (i.e., codeword = [message net-codeword]) in systematic BCH encoding, whereas it does not appear as a substring of the codeword in unsystematic BCH encoding. In PBS, we choose systematic BCH encoding because we are not actually sending the ``message'', and only the net-codeword is transmitted from Alice to Bob. 
To correct $d$ bit errors, the length of the net-codeword only is no more than $d\log n$ bits. We use the term `codeword' to refer to the net-codeword in the rest of this paper.
%The computational complexity of the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} is $O(d^2\log^2 n)$.

%The systematic BCH encoding is also used in other ECC-based set reconciliation works, such as PinSketch \cite{Wuille_Minisketchoptimizedlibrary_2019}, while PinSketch encodes a much longer message (e.g., $2^{32}$ bits) than in ours (hundreds of bits).  

%\subsubsection{Find the $d$ Bit Positions Using ECC}\label{sec:BCH_code}

% A straightforward approach to find the $d$ bit positions is to let Bob send the complete parity bitmap $B[1..n]$ to Alice, then Alice compares $A[1..n]$ with $B[1..n]$ locally. This approach has a communication overhead of $n$ bits, which is quite wasteful. As we discussed in~\autoref{sec:hash_partition}, $d$ is usually much smaller than $n$. It means $A[1..n]$ and $B[1..n]$ differ only at a tiny portion of bits. Therefore, we can view $A[1..n]$ as a corrupted message of $B[1..n]$ with $d$ bit errors, and the bit positions of the $d$ bit errors basically correspond to the $d$ subset pairs that contain distinct elements. The detection of bit errors, on the other hand, can be solved by Error-Correction Code (ECC)~\cite{Lin_ErrorControlCoding_1983}. 

% Since $A[1..n]$ and $B[1..n]$ differ at $d$ bit positions, we can view $A[1..n]$ as a corrupted message of $B[1..n]$ from Bob to Alice through an {\it unreliable} commnunication channel with $d$ corrupted bits, which are located on the $d$ bit positions. Therefore, to find the $d$ bit position, we only need to correct the $d$ corrupted bits in $A[1..n]$, which is done by transmitting a ``code'' that can correct upto $d$ bit errors from Bob to Alice through a {\it reliable} communication channel. 

% In PBS, we use {\it systematic} BCH code to generate the ``code'' by encoding the message $B[1..n]$. The codeword of the systematic BCH code is in the form of [message, net-codeword], since the message appears as the prefix of the codeword in systematic BCH code. The ``code'' is simply the net-codeword in the BCH codeword. We choose {\it systematic} BCH code because the (corrupted) message is already transmitted and we only need to pay a small communication overhead on transmitting ``code'' (i.e., net-codeword). To correct upto $d$ bit errors, the length of the net-codeword is no more than $d\log n$ bits, which is much smaller than the message when $d\!\ll\! n$. The computational complexity of the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} is $O(d^2\log^2 n)$. This type of BCH code is also used in other ECC-based set reconciliation works, such as PinSketch \cite{Wuille_Minisketchoptimizedlibrary_2019}. 

% Different from {\it unsystematic} BCH code
% The ``code'' is generated by {\it systematic} BCH code, which encodes the message $B[1..n]$ into a BCH codeword in the form of [message, net-codeword]. The ``code'' transmitted on the reliable channel is the net-codeword of the BCH codeword. In {\it systematic} BCH code, the message appears as the prefix of the codeword. 

% More specifically, PBS uses {\it systematic} BCH code~\cite{Lint_IntroductionCodingTheory_1998} that can correct upto $d$ bit errors to encode the parity bitmaps. In the {\it systematic} BCH code \footnote{In unsystematic BCH code, message does not appear to be the prefix of the codeword}, the message (i.e., the parity bitmap) appears as the prefix of the raw codeword, which in the form of [message, net codeword]. Normally, to correct upto $d$ errors, the length of the net codeword is $2n\log d$, where $n$ is the length of the message (i.e., parity bitmap). However, our case is special in the sense that the net codeword is error-free (all $d$ bit errors are in the message), so the length of the net codeword can be reduced to $n\log d$. This type of BCH code is also used in other ECC-based set reconciliation works, such as PinSketch \cite{Wuille_Minisketchoptimizedlibrary_2019}. 

% Now we can formally describe how to find the $d$ bit positions: First, Bob uses a $d$-error-correcting systematic BCH code to encode $B[1..n]$ and sends the net codeword ($d\log n$ bits) to Alice. Upon receiving the net codeword and combining it with the corrupted message $A[1..n]$, Alice uses the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} to decode the $d$ bit errors in $A[1..n]$. The communication overhead of transmitting the net codeword is $d\log n$ bits. The computational complexity of the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} is $O(d^2\log^2 n)$. Both the communication overhead and the computational complexity here are relatively small when $d$ is small.

% \medskip
% \noindent{\bf Reconcile the $d$ subset pairs using \autoref{alg:trivial_case}} 

%Once the $d$ bit positions are known, Alice can start to reconcile $(A_{i_1},B_{i_1}), (A_{i_2},B_{i_2}),...,(A_{i_d},B_{i_d})$ using \autoref{alg:trivial_case} and obtain the $d$ distinct elements (i.e., $A\Delta B$). 
Once Bob decodes the codeword to obtain $i_1,i_2,...,i_d$, the corresponding subset pairs $(A_{i_1},B_{i_1})$, $(A_{i_2},B_{i_2})$, $...$, $(A_{i_d},B_{i_d})$ each can be reconciled using \autoref{alg:trivial_case}. To do so, Bob needs to send the respective \code{XOR} sums of the subsets $B_{i_1}$, $B_{i_2}$,$...$,$B_{i_d}$ to Alice (\autoref{alg1:sender} in \autoref{alg:trivial_case}). In addition, Bob needs to send $i_1,i_2,...,i_d$ to Alice, since Alice does not know the indices. Each index needs to be encoded into $\log n$ bits, so the additional communication overhead on transmitting the indices is $d\log n$ bits. 
% When reconciling $(A_{i_1},B_{i_1}), (A_{i_2},B_{i_2}),...,(A_{i_d},B_{i_d})$ using \autoref{alg:trivial_case}, Alice needs to send not only the bitwise \code{XOR} of $A_{i_1}, A_{i_2},..., A_{i_d}$, but also the indices of the subset pairs ($i_1,i_2,...,i_d$), since Bob does not know which of the $d$ subset pairs are being reconciled. Each index is an integer between $1$ and $n$ and can be encoded into $\log n$ bits, So the additional communication overhead on transmitting the indices is $d\log n$ bits. 



% \subsubsection{Reconcile the $d$ subset pairs using \autoref{alg:trivial_case}}\label{sec:reconcile_by_trivial}

% After decoding the $d$ bit errors that corresponds to the $d$ subset pairs, Alice starts to reconcile them using \autoref{alg:trivial_case}. For each of the $d$ subset pairs, Alice needs to send not only the bitwise \code{XOR} of the subset pair, but also the index of the subset pair (since Bob does not know the $d$ subset pairs to reconcile). So the communication overhead on \autoref{alg:trivial_case} is $d\log |\mathcal{U}|+d\log n$ bits. 
%Plus the communication overhead on transmitting the net codeword of parity bitmap ($d\log n$, as we explained in \autoref{sec:BCH_code}), the overall communication overhead of single-round PBS is $d\log u+2d\log n$ bits.

% \medskip
% \noindent{\bf Check if set reconciliation is complete} 

{\bf (Modified)} Once Alice receives the \code{XOR} sums and the indices, she can compute the distinct elements (described in \autoref{subsec:protocol0}) to obtain the set difference (denoted as $\hat{D}$). However, this reconciled set difference could be incorrect if the ideal case does not happen. Therefore, Alice needs to check if set reconciliation is successful (or whether $\hat{D}=A\Delta B$). To do so, we introduce some ``linear'' checksum function $c(\cdot)$ that maps any subset of the universe $\mathcal{U}$ (such as $A$ and $B$) to a $32$-bit checksum (e.g., bitwise \code{XOR}). Here the ``linearity'' of a chechsum function refers to the fact that $c(S_1\Delta S_2)=c(S_1)\oplus c(S_2)$ for any two subsets $S_1$ and $S_2$ of the universe $\mathcal{U}$. We use this checksum function to check if $\hat{D}=A\Delta B$ by comparing $c(\hat{D})$ to $c(A\Delta B)$. Note that $c(\hat{D})$ can be computed in $O(d)$ time and $c(A\Delta B)=c(A)\oplus c(B)$ can be precomputed {\bf during the encoding period, which costs $32$ bits of communication overhead on transmitting $c(B)$ from Bob to Alice. In PBS, we select {\it longitudinal parity check}, the bitwise \code{XOR} of all elements (recall each element is a $32$-bit-long binary string) in the set, as the ``linear'' checksum function.}  

{\bf (Previous)} After reconciling the subset pairs and obtaining the reconciled set difference (denoted as $\hat{D}$), PBS needs to check if set reconciliation is complete (or whether $\hat{D}=A\Delta B$), since the reconciled set difference $\hat{D}$ is not the actual set difference $A\Delta B$ in the nonideal case (to be discussed in \autoref{subsec:exception_hash_partition}). Hence, we add a verfication step after obtaining $\hat{D}$ to check if $\hat{D}=A\Delta B$. In PBS, we check an equivalent condition, $A=B\Delta\hat{D}$, instead of $\hat{D}=A\Delta B$, since $B$ and $\hat{D}$ are both known by Bob and their set difference $B\Delta\hat{D}$ can be locally computed. More specifically, to check if the remote sets $A$ and $B\Delta\hat{D}$ are equal, we let Alice compute a $32$-bit checksum of $A$ and send it to Bob. {\bf Then Bob computes the $32$-bit checksum of $B\Delta\hat{D}$ using the same checksum algorithm and compare the two checksums. In PBS, we select {\it longitudinal parity check} (i.e., bitwise \code{XOR} of all elements in the set) as the checksum algorithm, so that the checksum $B\Delta\hat{D}$ can be efficiently computed as the bitwise \code{XOR} between the checksum of $B$ (can be pre-computed) and that of $\hat{D}$. Other checksum algorithms that are {\it linear} to the set difference operator (i.e., $\Delta$) also work for PBS. }
% Then Bob checks if $B\Delta\hat{D}$ satisfies the receiving checksum. 

{\bf (Modified)} The condition $\hat{D}=A\Delta B$ can be almost surely verified by the checksum, 
{\bf although it could mistakenly believes two different sets as identical ones.} This event happens with probability $2^{-32}\approx 2.3\times 10^{-10}$ when the ideal case does not happen, {\bf which has a probability on the order of $10^{-2}$.} Although this event could cause PBS mistakenly believes the set reconciliation is completed, it happens with an extremely small probability (on the order of $10^{-12}$) and should be acceptable in most applications. In few applications which allow no room for error ({\it e.g.,} Bitcoin), additional techniques such as Merkle tree~\cite{merkle87} based validation will be used to verify the correctness of the results anyway. If such techniques find out that the set reconciliation is not completed, we could simply start it over and use PBS to reconcile the two sets again under different hash function $h$ (note that PBS is a `randomized' algorithm when assuming the hash functions for hash-partition are random hash functions). To simplify our description, we ignore this small probability event and assume the checksum works perfectly in this rest of this paper. {\bf not a good position to mention `for super critical applications, use a checksum for all groups', since we are describing single-group scenario. }

{\color{blue}This probability is low enough for most applications. In few applications which allow no room for error ({\it e.g.,} Bitcoin), additional techniques such as Merkle tree~\cite{merkle87} based validation will be used to verify the correctness of the results anyway.}

{\bf (Previous)} The condition $A=B\Delta\hat{D}$ can be almost surely verified by a $32$-bit checksum, although it could mistakenly believe two different sets as identical ones with probability $2^{-32}\approx 2.3\times 10^{-10}$ {\bf on top of the probability that the nonideal case happens (on the order of $10^{-2}$).} Although this event could cause an ``early'' termination and leave some distinct elements unreconciled, it happens with an extremely small probability (on the order of $10^{-12}$) and should be acceptable in most applications. {\bf To simplify our description, we ignore this small probability event and assume the checksum works perfectly in this rest of this paper. }
%and such an event (i.e., mistaken $A$ and $B\Delta\hat{D}$ are identical when they are different) never happens in our evaluation. For some super critical applications, we can certainly use a $64$-bit checksum to reduce this probability to $5.4\times 10^{-20}$ if needed.

% When the ideal case does not happen, set reconciliation cannot accomplish in one round, as we will explain in \autoref{subsec:exception_hash_partition}. Hence, we add a verfication step to check if set reconciliation is complete. Let $\hat{D}$ denote the set of reconciled elements. The idea of this verification is basically to compare $A$ with $B\Delta \hat{D}$: If $A=B\Delta \hat{D}$ (i.e., $\hat{D}=A\Delta B$), we know the set reconciliation is complete; Otherwise, the set reconciliation is incomplete.  using a $32$-bit checksum. 

\subsubsection{Communication overhead of PBS (First Round)}\label{sec:communication_overhead_single_PBS}

In this section, we summarize all the above steps of PBS (in the first round) in \autoref{alg:single_round_pbs}. The overall communication overhead consists of four components: (1) the BCH codeword of $d\log n$ bits in \autoref{step:BCH_encode}; (2) the subset pair indices $i_1,i_2,...,i_d$ in \autoref{step:trivial_reconcile}; (3) the bitwise \code{XOR} sums of sets $B_{i_1}, B_{i_2},...,B_{i_d}$ of $d\log |\mathcal{U}|$ bits in \autoref{step:trivial_reconcile}; and (4) transmit the $32$-bit checksum of $B$ (i.e., $c(B)$) from Bob to Alice for precomputing $c(A\Delta B)$ in \autoref{step:terminate_condition}. 

% All the steps of PBS in the first round are summarized in \autoref{alg:single_round_pbs}. The overall communication overhead consists of three components: (1) the BCH codeword of $d\log n$ bits in \autoref{step:BCH_encode}; (2) the subset pair indices $i_1,i_2,...,i_d$ and the corresponding bitwise \code{XOR}s of $d\log n+d\log |\mathcal{U}|$ bits in \autoref{step:trivial_reconcile}; and (3) the $32$-bit checksum of $A$ in \autoref{step:terminate_condition}. 

\begin{algorithm}
\caption{Single-round PBS}
\label{alg:single_round_pbs}

%Hash-partition $A$, $B$ into $\{A_i\}_{i=1}^n$, $\{B_i\}_{i=1}^n$\; \label{step:hash_partition}

%Parity encode $\{A_i\}_{i=1}^n$, $\{B_i\}_{i=1}^n$ into $A[1..n]$, $B[1..n]$\; \label{step:parity_encode}
{\it Alice}: Send BCH codeword of $A[1..n]$ to Bob\; \label{step:BCH_encode}

{\it Bob}: Decode the codeword to obtain $i_1,i_2,...,i_d$\; \label{step:BCH_decode}

{\it Bob}: Send $i_1,i_2,...,i_d$ and the \code{XOR} sums of sets $B_{i_1}, B_{i_2},...,B_{i_d}$ to Alice (\autoref{alg1:sender} in \autoref{alg:trivial_case})\; \label{step:BCH_decode}

{\it Alice}: Obtain $A_{i_1}\Delta B_{i_1}, A_{i_2}\Delta B_{i_2},...,A_{i_d}\Delta B_{i_d}$ (\autoref{alg1:receiver} in \autoref{alg:trivial_case}), $\hat{D}\leftarrow \bigcup_{k=1}^d (A_{i_k}\Delta B_{i_k})$\; \label{step:trivial_reconcile}

{\it Alice}: Check if $c(\hat{D})=c(A\Delta B)$\; \label{step:terminate_condition}

% {\it Bob}: BCH-Encodeing $B[1..n]$ and send the codeword to Alice\; \label{step:BCH_encode}

% {\it Alice}: Upon receiving the codeword, decode the bit errors between $A[1..n]$ and $B[1..n]$\; \label{step:BCH_decode}

% {\it Alice}: For each bit error, start reconciling the corresponding subset pair by \autoref{alg:trivial_case}\; \label{step:trivial_reconcile}

% {\it Bob}: Upon receiving the reconciled set difference $\hat{D}$, check if $A=B\Delta \hat{D}$ via checksum\; \label{step:terminate_condition}
\end{algorithm}


% \subsubsection{Single-round PBS}\label{sec:single_round_pbs}

% Here we summarize all the steps of single-round PBS and represent it by pseudocode in \autoref{alg:single_round_pbs}. \autoref{step:hash_partition} and \autoref{step:parity_encode} operates at both hosts (i.e., Alice and Bob). \autoref{step:hash_partition} to \autoref{step:trivial_reconcile} have been elaborated from \autoref{sec:hash_partition} to \autoref{sec:reconcile_by_trivial}. The last step in \autoref{step:terminate_condition} aims to check whether reconciliation is complete (i.e., $\mathcal{D}=A\Delta B$). More specifically, Alice calculates the checksum (e.g., CRC-$32$) of $A$ and send it to Bob. Then Bob calculates the checksum of $B\Delta \mathcal{D}$ and compares it to the receiving checksum of $A$. If the two checksums are the same, we believe $A=B\Delta \mathcal{D}$ and therefore $\mathcal{D}=A\Delta B$ (i.e., reconciliation is complete); Else, we know some elements are reconciled incorrectly. We classify those elements (i.e., the ones in the set difference between $A\Delta B$ and $\mathcal{D}$) into two subsets $A\Delta B\!\setminus\!\mathcal{D}$ and $\mathcal{D}\!\setminus\!(A\Delta B)$ and refer the elements in the former as {\it false-negatives}, and refer the elements in the later as {\it false-positives}. 

% In the ideal case, neither false-positives nor false-negatives will happen and the two checksums always equal. However, in real life, the ideal case does not always happen. We will discuss the nonideal case in \autoref{subsec:exception_hash_partition}. In our evaluation, we use a $32$-bit checksum for comparing $A$ to $B\Delta \mathcal{D}$ that has {\bf an error probability} roughly $10^{-9}$. This error (i.e., mistake $A=B\Delta \mathcal{D}$) incurs false-negatives. All set reconciliation schemes have the same problem on their termination conditions (i.e., check whether $\mathcal{D}=A\Delta B$). For some super critical applications, we can certainly decrease the error probability by using more powerful checksums (i.e., $64-$bit). Using a $32$-bit checksum, this kind of false-negatives never happen in the evaluation. 
% %For simplification, we assume no error happens when checking $\mathcal{D}=A\Delta B$ in the rest of the paper.

% \begin{algorithm}
% \caption{Single-round PBS}
% \label{alg:single_round_pbs}

% Hash-partition $A$, $B$ into $\{A_i\}_{i=1}^n$, $\{B_i\}_{i=1}^n$\; \label{step:hash_partition}

% Parity encode $\{A_i\}_{i=1}^n$, $\{B_i\}_{i=1}^n$ into $A[1..n]$, $B[1..n]$\; \label{step:parity_encode}

% {\it Bob}: Encode $B[1..n]$ by BCH code, then send the codeword to Alice\; \label{step:BCH_encode}

% {\it Alice}: Upon receiving the codeword, decode the bit errors between $A[1..n]$ and $B[1..n]$\; \label{step:BCH_decode}

% {\it Alice}: For each bit error, reconcile the corresponding subset pair by \autoref{alg:trivial_case}\; \label{step:trivial_reconcile}

% {\it Bob}: Upon the reconciled distinct elements $\mathcal{D}$, check whether $A=B\Delta \mathcal{D}$ via checksum\; \label{step:terminate_condition}
% \end{algorithm}

\subsubsection{Exception Handling}\label{subsec:exception_hash_partition}

When the ideal case does not happen, some subset pair may contain more than $1$ distinct elements and cannot be successfully reconciled by \autoref{alg:trivial_case}. We can classify the possible exceptions that happen in such a subset pair into the following two types of events: 

\noindent {\bf Type (\RN{1})}: Subset pair $(A_i, B_i)$ contains even number ($\geq 2$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be the same and PBS will not reconcile the subset pair yet in this round. This event happens with a small but nontrivial probability: For example, $d=5$ and $n=255$ (i.e., throwing $5$ balls uniformly and randomly into $255$ bins), the probability that some bin has an even number of (in this case either $2$ or $4$) balls is roughly $0.04$. 
%Note that when a type (\RN{1}) event happens, the checksum (\autoref{step:terminate_condition} in \autoref{alg:single_round_pbs}) can detect that the set reconciliation has not been completed. Then PBS will start another round to reconcile the ``hidden'' distinct elements (the ones that have not been reconciled in this round), 
%so on so force, until all distinct elements are successfully reconciled and the checksum is verified to be correct, 
%as we will describe in \autoref{sec:multi-rounds}. 

% Note that when a Type (\RN{1}) subset pair exists, the $32$-bit checksum (\autoref{step:terminate_condition} in \autoref{alg:single_round_pbs}) can almost surely detect that the set reconciliation is incomplete. If this is the case (i.e., the checksum is verified to be incorrect), PBS will start another round of set reconciliation to reconcile the remaining distinct elements (e.g., the ``hidden'' distinct elements in Type (\RN{1}) subset pairs), so on so force, until all distinct elements are reconciled and the checksum is verified to be correct, as we will describe in \autoref{sec:multi-rounds}. 

\noindent {\bf Type (\RN{2})}: Subset pair $(A_i, B_i)$ contains odd number ($\geq 3$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be different and PBS will reconcile the subset pair using \autoref{alg:trivial_case}. The reconciled element (i.e., $s$ in \autoref{alg:trivial_case}) is however a ``fake'' distinct element, which is actually the bitwise \code{XOR} of all distinct elements in $(A_i, B_i)$ (explained in \autoref{subsec:protocol0}).
%, which will be mistakenly believed as the distinct element of $(A_i, B_i)$. 
This event happens with a tiny probability: Use the same example above ($d=5$ and $n=255$), the probability that some bin has $3$ or $5$ balls is only $1.52\times 10^{-4}$. 
%Similarly, the $32$-bit checksum can also detect that the set reconciliation has not been completed when a type (\RN{2}) event happens. Both the ``hidden'' and the ``fake'' distinct elements can also be reconciled in later rounds. 

%Note that those ``fake'' distinct elements will become new distinct elements in the next round and therefore incur additional communication overhead to reconcile. 
Note that those ``fake'' distinct elements will incur additional communication overhead if we want to reconcile them ``later''. Therefore, we add a verification on each reconciled distinct element of \autoref{alg:trivial_case} that can detect ``fake'' distinct elements with high probability. \autoref{alg:verification} shows how this verification works, and it does not incur additional communication overhead.

\begin{algorithm}
\caption{Verify reconciled element $s$ of $(A_i, B_i)$}
\label{alg:verification}
\If{$h(s)\neq i$} {Discard the reconciled element $s$;}
\end{algorithm}

Although a distinct element of $(A_i, B_i)$ must be in sub-universe $\mathcal{U}_i$ (i.e., the hash value of the element under $h$ equals to $i$), a ``fake'' distinct element could be in any sub-universe with probability $1/n$, since it is the bitwise \code{XOR} of multiple distinct elements of $(A_i, B_i)$. Therefore, \autoref{alg:verification} only fails to identify a ``fake'' distinct element with probability $1/n$, which is roughly $3.9\times 10^{-3}$ when $n=255$. On top of the probability of the type (\RN{2}) event, a ``fake'' distinct element that fails to be detected by \autoref{alg:verification} happens with a tiny probability of $6\times 10^{-7}$. {\bf (removed to the beginning of theoretical analysis) To simplify our description, we also ignore this small probability event and assume all ``fake'' distinct elements will be successfully detected by \autoref{alg:verification} in this rest of this paper. }

{\bf Note that either a type (\RN{1}) event or a type (\RN{2}) event will cause PBS fails to reconcile all distinct elements, which can be detected by the checksum (\autoref{step:terminate_condition} in \autoref{alg:single_round_pbs}). In this case, PBS will continue to reconcile the ``remaining'' distinct element by starting another round, as we will describe in \autoref{sec:multi-rounds}. The ``remaining'' distinct elements here consist of (1) the ``hidden'' distinct elements that have not been reconciled in this round and (2) the ``fake'' distinct elements that are not verified by \autoref{alg:verification}. }

{\bf (to be removed) Readers may wonder encoding the exact subset cardinalities (i.e., $|A_i|, |B_i|$) instead of their oddness / evenness (parity) (described in \autoref{sec:hash_partition}) could help to detect and solve Type (\RN{1}), (\RN{2}) events. However, encoding the exact subset cardinalities not only incurs much more additional communication overhead comparing to encoding their parities, but also barely helps on detecting Type (\RN{1}), (\RN{2}) events, since we cannot precisely derive $|A_i\Delta B_i|$, the total number of distinct elements in $(A_i, B_i)$, even knowing $|A_i|, |B_i|$: For instance, when $|A_i|\!=\!|B_i|\!=\!50$, $|A_i\Delta B_i|$ could be any even number ($\leq 100$) if the distinct elements are evenly splitted and placed between $A_i$ and $B_i$. }

% As we have described in \autoref{sec:hash_partition}, the ideal case does not always happen, which means some subset pair may contain more than $1$ distinct elements and cannot be successfully reconciled by \autoref{alg:trivial_case}. Due to the parity encoding, we can classify such subset pair into the following two scenarios:

% \begin{itemize}
%     \item Scenario 1: If a subset pair $(A_i, B_i)$ contains even number ($\geq 2$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be the same and PBS will not reconcile the subset pair yet in this round;
%     \item Scenario 2: If a subset pair $(A_i, B_i)$ contains odd number ($\geq 3$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be different and PBS will reconcile the subset pair using \autoref{alg:trivial_case}. The reconciled element (i.e., $s$ in \autoref{alg:trivial_case}) is however the bitwise \code{XOR} of all distinct elements in $(A_i, B_i)$ (explained in \autoref{subsec:protocol0}), which will be mistakenly believed as the distinct element of $(A_i, B_i)$. 
%     %However, as described in \autoref{subsec:protocol0}, when a subset pair contains more than $1$ distinct elements, \autoref{alg:trivial_case} will output the bitwise \code{XOR} of them as the `distinct element', which is not an actual distinct element with high probability;
% \end{itemize}

% In both scenarios, the distinct elements in the subset pair will not be reconciled in this round. As we will describe in \autoref{sec:multi-rounds}, we generalize PBS into multi-round, so that the distinct elements that have not been reconciled in the first round will be reconciled in later rounds. On the other hand, the second scenario could result in incorrectly reconciled distinct elements, which will become new distinct elements in the next round in multi-round PBS. 

% % In both scenarios, the distinct elements in the subset pair cannot be successfully reconciled in this round and will remain in the set difference (i.e., $(A\Delta B)\!\setminus\!\hat{D}$). On the other hand, the incorrectly reconciled distinct element in the second scenario will appear as a new distinct element (i.e., $\hat{D}\!\setminus\!(A\Delta B)$) in the next round if we generalize PBS into multi-round (to be elaborated in \autoref{sec:multi-rounds}). Both scenarios can be almost surely detected by the 32-bit checksum (\autoref{step:terminate_condition} in \autoref{alg:single_round_pbs}). The set difference after the reconciliation in this round, $D\Delta\hat{D}$, can be reconciled in later rounds, as we will describe in \autoref{sec:multi-rounds}. 

% Naturally, we do not want to generate new distinct elements in the process of set reconciliation, even though it happens with a tiny probability when $n=\Omega(d^2)$: For instance, when $d=5$ and $n=255$ (i.e., throwing $5$ balls uniformly and randomly into $255$ bins), the probability (i.e., some bin has $3$ or $5$ balls) is only $7.6\times 10^{-6}$. Therefore, we add a verification with no additional communication cost on each reconciled element of \autoref{alg:trivial_case}, such that each incorrect dinstinct element can be identified with high probability. The verfication is shown in \autoref{alg:verification}. 

% \begin{algorithm}
% \caption{Verify reconciled element $s$ of $(A_i, B_i)$}
% \label{alg:verification}
% \If{$h(s)\neq i$} {Discard the reconciled element $s$;}
% \end{algorithm}

% Although any distinct element of $(A_i, B_i)$ must be in sub-universe $\mathcal{U}_i$ (i.e., the hash value of the element under $h$ equals to $i$), the bitwise \code{XOR} of multiple distinct elements of $(A_i, B_i)$ could be in any sub-universe with probability $1/n$. Therefore, \autoref{alg:verification} fails to identify an incorrectly reconciled distinct element in the second scenario with probability $1/n$ that is roughly $3.9\times 10^{-3}$ when $n=255$. In other words, an incorrectly reconciled distinct element that cannot be identified by \autoref{alg:verification} appears with probability $3\times 10^{-8}$. {\bf I feel that defining $\tilde{a}_4=a_1\oplus a_2\oplus a_3$ does not help much.}

% In both scenarios, the distinct elements in the subset pair cannot be successfully reconciled in this round. These distinct elements can be reconciled in later rounds if needed, as we will describe in \autoref{sec:multi-rounds}. In this section, we only discuss how to identify the {\it incorrect} distinct element in the second scenario. Let us use an example to elaborate the second scenario: Assume $(A_i, B_i)$ contains $3$ distinct elements $a_1, a_2, a_3$, then Bob computes $\tilde{s}=a_1\oplus a_2\oplus a_3$ using \autoref{alg:trivial_case} and mistakes it as the distinct element in $(A_i, B_i)$. 

% In both scenarios, the distinct elements in the subset pair cannot be successfully reconciled (i.e., false-negatives defined in \autoref{sec:single_round_pbs}. The distinct elements that are not successfully reconciled in this round, if needed, can be reconciled in later rounds as we will describe in \autoref{sec:multi-rounds}. In this section, we only discuss how to identify the {\it incorrect} distinct elements in the second scenario. Let us use an example to elaborate the second scenario: Assume $(A_i, B_i)$ contains $3$ distinct elements $a_1, a_2, a_3$, then Bob computes $\tilde{s}=a_1\oplus a_2\oplus a_3$ using \autoref{alg:trivial_case} and mistakes it as the distinct element in $(A_i, B_i)$. 

\begin{comment}
============================================

We add a no-communication-cost verification step to check whether a reconciled element is an actual distinct element or not. Note that an actual distinct element of $(A_i, B_i)$ must be in sub-universe $\mathcal{U}_i$. On the other hand, an incorrectly reconciled element (e.g., $\tilde{s}$) can be in any sub-universe with probability $1/n$. So at the end \autoref{subsec:protocol0}, we check whether the reconciled element is in $\mathcal{U}_i$ by the hash function $h$ in hash-partition:

This verfication cannot completely eliminate false-positives, since an incorrectly reconciled element (e.g., $\tilde{s}$) can coincidentally end up in $\mathcal{U}_i$ with probability $1/n$. The chance of false-positives is extremely small using the verification. For instance, if $d=5$ and $n=255$, the probability of the second scenario is only $7.6\times 10^{-6}$. The probability of false-positives using the verfication is $1/n$ times this small probability, which is roughly $3\times 10^{-8}$. {\bf Note that a small probability of false-positives only costs a little waste on set reconciliation when synchronizing objectives (e.g., files), which is acceptable for most applications.}

Even worse, in the second scenario, the false-positives defined in \autoref{sec:single_round_pbs} could happen. For example, if subset pair $(A_i, B_i)$ contains $3$ distinct elements $s_1, s_2, s_3$, then \autoref{alg:trivial_case} computes $\tilde{s}=s_1\oplus s_2\oplus s_3$ and Bob mistakes $\tilde{s}$ as an actual distinct element. The good thing is, the probability of this kind of false-positives is extremely small for small $d$. For instance, if $d=5$ and $n=255$, the probability of the false-positives is only $7.6\times 10^{-6}$. To further reduce the chance of false-positives, we add a no-communication-cost verification step at the end of \autoref{subsec:protocol0} to check whether $\tilde{s}$ is an actual distinct element or not. The verification step works as follows: Given the output $s$ of subset pair $(A_i,B_i)$, if $s\in\mathcal{U}_i$ (i.e., $h(s)=i$), we consider $s$ as an actual distinct element; Otherwise, we consider $s$ as an incorrect output and discard it. 

Note that if $\tilde{s}\in A_i\Delta B_i$, $\tilde{s}$ must be in sub-universe $\mathcal{U}_i$. However, if $\tilde{s}$ is the bitwise \code{XOR} of the distinct elements in $(A_i,B_i)$ (i.e., the second scenario happens), it ends up in $\mathcal{U}_i$ with probablity of only $1/n$. 
%In fact, if we assume the hash-partition described in \autoref{sec:hash_partition} hashes the elements of $\mathcal{U}$ uniformly, independently, and randomly into $n$ sub-universes, the output $s$ in the second scenario will be in a different sub-universe $\mathcal{U}_j (j\neq i)$ with a high probability of $1-\frac{1}{n}$. Hence, this verfication method can further reduce the probability of false-positives by a factor of $\frac{1}{n}$. 
Use the same example (i.e., $d=5$, $n=255$), the probability of this kind of false-positives is reduced from $7.6\times 10^{-6}$ to $3\times 10^{-8}$ by this verification method. 
%{\bf This probability can be further reduced in \autoref{subsec:protocol2}, where PBS does two tiers of hash-partitions. So we can do verification on both of the two hash functions.}

%In some super critical cases (i.e., no false-positive is allowed), we can use a more powerful verification method to completely eliminate false-positives. That is, to check if the output $s$ exists in exactly one of the two sets (i.e., $s\in A\!\setminus\! B$ or $s\in B\!\setminus\! A$). To do so, Bob transmits $s$ along with an identification bit $\mathbbm{1}_{\{s\in B\}}$ to Alice, then Alice checks if $s\in (A\!\setminus\! B)\bigcup (B\!\setminus\! A)$ . This method verification costs additional $d(\log u+1)$ bits of communication overhead. In most applications, this rigorous $0\%$ probability guarantee of false-positives is unnecessary and the probability of the former verification method is small enough, so we use the former in the evaluation. Based on our observation, this kind of false-positives do not happen even once in the evaluation using the former verfication method. In the rest of this paper, we assume Scenario 2 is always correctly verified. 

============================================
\end{comment}

\subsection{Running PBS for Multiple Rounds}\label{sec:multi-rounds}

{\bf (merged from the following two paragraphs)} To deal with the ``remaining'' distinct elements, we remove (and save) all the distinct elements that has been reconciled in the first round (i.e., $\hat{D}$) and run another round of PBS. In the second round, we reconcile $A\Delta \hat{D}$ and $B$ instead of reconciling $A$ and $B$ to remove all the reconciled distinct elements. We use a different hash function for hash-partition in the second round to avoid the same exceptions (i.e., type (\RN{1}), (\RN{2}) events) that happened in the first round happen again. This procedure replicates until If until all distinct elements are successfully reconciled and the checksum is verified to be correct. 

{\bf (to be removed)} When the ideal case does not happen (i.e., type (\RN{1}) or type (\RN{2}) event happens), PBS will know the set reconciliation has not been completed via the $32$-bit checksum (\autoref{step:terminate_condition} in \autoref{alg:single_round_pbs}). To reconcile those distinct elements that have not been reconciled yet in the first round, we rule out all successfully reconciled elements and run another round of PBS. This procedure replicates until all distinct elements are successfully reconciled and the checksum is verified to be correct.

{\bf (to be removed)} More specifically, in the second round, we run PBS to reconcile $A$ and $B\Delta \hat{D}$ instead of $A$ and $B$ to rule out all elements that have been reconciled, where $\hat{D}$ is the set of reconciled distinct elements in the first round. We use a different hash function for hash-partition in the second round to avoid the same exceptions (i.e., type (\RN{1}), (\RN{2}) events) that happened in the first round happen again. The later rounds are similarly operated. 

%{\bf Normally, we want PBS to successfully reconcile all distinct elements in only a few rounds (say $3$) with high probability (say $99\%$). Hence, when tuning parameters (to be discussed in \autoref{sec:parameter_settings}), we set a {\it target success probability} $p_0$ of $r$ rounds as a paramenter setting requirement, which aims to ensure the probability that all distinct elements are reconciled in $r$ rounds to be larger than $p_0$. This requirement should also ensure the majority of the distinct elements are reconciled in the first round. Use the same example ($d=5, n=255$), on average $4.81$ out of $5$ distinct elements should be reconciled in the first round. So the total communication overhead in all rounds is only slightly larger than ($1.01$ to $1.07$ times of, as we will show in \autoref{fig:per-round-con}) that in the first round. Due to this reason, we use the communication overhead in the first round (described in \autoref{sec:communication_overhead_single_PBS}) to approximate the total communication overhead of all rounds in parameter settings (to be elaborated in \autoref{sec:parameter_settings}.}

% Although PBS may need to run many rounds to reconcile all distinct elements, the communication overhead mostly happens in the first round, since the majority of the distinct elements should be reconciled in the first round. Use the same example ($d=5, n=255$), on average $4.81$ out of $5$ distinct elements should be reconciled in the first round. So the total communication overhead in all rounds is only slightly larger than ($1.01$ to $1.07$ times of, to be shown in \autoref{fig:per-round-con}) that in the first round. Due to this reason, we use the communication overhead in the first round (described in \autoref{sec:communication_overhead_single_PBS}) to approximate the total communication overhead (all rounds) in parameter settings (to be elaborated in \autoref{sec:parameter_settings}).

%For the moment, we assume no ``fake'' distinct element in type (\RN{2}) subset pairs fails to be detected, which happens with overwhelming probability as explained in \autoref{subsec:exception_hash_partition}. Then 
%PBS reconciles the distinct elements gradually round by round. This is the ``piecewise decodability'' mentioned in \autoref{sec:intro_oursolution}. We use the following example to describe it in details: 
%Given two sets with $10$ distinct elements, in the first round, PBS tries to reconcile the $10$ distinct elements and say $6$ out of the $10$ distinct elements are successfully reconciled. Then the $6$ reconciled distinct elements are removed and PBS tries to reconcile the remaining $4$ distinct elements in the second round. Say $2$ out of the $4$ remaining distinct elements are successfully reconciled, and that leaves $2$ remaining distinct elements to be reconciled in the third round, so on so force. 
% Given two sets $A$, $B$ with $10$ distinct elements, in the first round, PBS hashes them into $7$ distinct subset pairs. $6$ distinct elements are hashed into $6$ distinct subset pairs, and the other $4$ distinct elements are hashed into the same subset pair. Then the former $6$ distinct elements are successfully reconciled in the first round and the later $4$ distinct elements remain to be reconciled in the second round, which are hashed into $3$ distinct subset pairs (under a different hash function). $2$ remaining distinct elements are hashed into $2$ distinct subset pairs, and the other $2$ remaining distinct elements are hashed into the same subset pair. Then the former $2$ remaining distinct elements are successfully reconciled in the second round and the later $2$ remaining distinct elements remain to be reconciled in the third round, so on so force. 
%The dynamics of the number of remaining distinct elements (i.e., $10\leadsto 4\leadsto 2\leadsto \cdots$ in the example) is in nature a Markov chain, which will be elaborated and analyzed in \autoref{sec:single_markov} to derive a tight tail bound of the probability that all distinct elements are reconciled in $r$ rounds.

% Even if the ideal case does not happen, most of the distinct elements should be distributed into different subset pairs, one distinct element in each, and therefore can be successfully reconciled. So in the first round, even if PBS cannot reconcile all distinct elements, it can reconcile the majority of them.
% % (piecewise decodability mentioned in \autoref{sec:intro_oursolution})
% Based on this intuition, we generalize PBS to multi-round, so that the distinct elements that are not reconciled yet in the first round can be reconciled in later rounds.  

% Without loss of generality, we only describe the second round of multi-round PBS, the reconciliation in the later rounds are similar. Let $\hat{D}_1$ denote the set of reconciled elements in the first round. If set reconciliation is not complete in the first round (i.e., the checksum infers $A\neq B\Delta \hat{D}_1$), then multi-round PBS saves $\hat{D}_1$, which includes correctly and incorrectly reconciled elements as described in \autoref{subsec:exception_hash_partition}, and starts the second round to find (1) the remaining distinct elements; (2) the incorrectly reconciled distinct elements in the first round. In the second round, multi-round PBS reconciles $A$ and $B\Delta \hat{D}_1$ instead of $A$ and $B$ (i.e., $B\leftarrow B\Delta\hat{D}_1$) to rule out all elements that have been reconciled. {\bf It uses a hash function that is different from the one used in the first round for hash-partition, otherwise every remaining distinct element will be hashed into the same subset pair and cause the same exception (described in \autoref{subsec:exception_hash_partition}) that happened in the first round.}

% If set reconciliation is complete in the second round, the set of reconciled elements in the second round (denoted as $\hat{D}_2$) should be the union of (1) all distinct elements that have not been reconciled in the first round (i.e., $(A\Delta B)\!\setminus\!\hat{D}_1$); and (2) all incorrectly reconciled elements in the first round (i.e., $\hat{D}_1\!\setminus\!(A\Delta B)$), which is by definition the set difference between $A\Delta B$ and $\hat{D}_1$. Therefore, the overall set difference $A\Delta B$ equals to the set difference between $\hat{D}_1$ and $\hat{D}_2$; Else, multiround PBS saves $\hat{D}_2$ and starts the third round, so on so force. 

% {\bf May need this algorithm to show the dynamics, if so, the earlier algorithm needs to change accordingly.}
% \IncMargin{1em}
% \begin{algorithm}
% \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
% \Input{$A$ and $B$}
% \Input{Maximum number of rounds $r$}
% \Output{$D$}

% $\hat{D},\mbox{ complete} \leftarrow PBS(A,B)$\;

% $D \leftarrow \hat{D}$\;

% \While{!complete and $r>0$}{
	
% 	$B \leftarrow B\Delta\hat{D}$\;

% 	$\hat{D},\mbox{ complete} \leftarrow PBS(A,B)$\;

% 	$D \leftarrow D\Delta\hat{D}$\;

% 	$r \leftarrow r-1$\;
% }

% \caption{Multi-round PBS} \label{proto:multirounds}
% \end{algorithm}\DecMargin{1em}

% The idea of multi-round PBS is quite simple: In each round, we discard the reconciled distinct elements in the previous rounds and aim to find the rest distinct elements from the remaining elements. More specifically, the first round of multi-round PBS is just the same as single-round PBS in \autoref{alg:single_round_pbs}. The second round has the same procedures as the first round. One difference is, we update $B$ by $B\leftarrow B\Delta\mathcal{D}$ in the second round, so that (1) Reconciled distinct elements in $\mathcal{D}$ that were contained in $A\Delta B$ are not longer contained in $A\Delta (B\Delta\mathcal{D})$; and (2) The other distinct elements remain in $A\Delta (B\Delta\mathcal{D})$ and can be reconciled later. The other difference is, we use a different hash function for partition (\autoref{step:hash_partition}) in the second round. Later rounds update $B$ in the same way and also use different hash functions. Multi-round terminates if the check in \autoref{step:termination} is correct. The overall set difference $A\Delta B$ is simply the union of reconciled distinct elements in all rounds. 

% A straightforward approach to discard reconciled distinct elements is to remove them from both $A$ and $B$. This approach however incurs additional communication overhead to update $A$, since only Bob learns the partial set difference in \autoref{step:reconcile}. Therefore, we use the approach in \autoref{step:updateb} that only updates $B$. It has another benefit in \autoref{step:termination}, which only needs to transmit the CRC of $A$ from Alice to Bob in the first round. In the later rounds, \autoref{step:termination} can be checked locally by Bob and does not require any additional communication overhead;

% Note that the communication overhead in the first round accounts for a large percentage of the total communication overhead in multi-round PBS, since most of the distinct elements (over $95\%$ as we will show in {\bf point to the figure}) should be reconciled in the first round. Therefore, we use the same parameter $n$ in later rounds because otherwise we have to compute a new parameter that can only save tiny communication overhead, even though the number of remaining distinct elements is small and can be reconciled using smaller $n$ with high probability. {\bf Due to the same reason, we can the same expression of the communication overhead in single-round PBS to approximate the communication overhead in multi-round PBS.}

% The natural termination condition of multi-round PBS is that all distinct elements are reconciled, which could require a large number of rounds and incur large additional communication overhead (each additional round incurs $d\log n$ bits of additional communication overhead on transmitting BCH codeword). To control the amount of additional communication overhead, we set another termination condition that multi-round PBS runs for at most $r$ rounds (typically $2$ or $3$). This termination condition could cause an `early' termination when some distinct elements have not been reconciled. However, under proper parameter settings (to be discussed in \autoref{sec:parameter_settings}), we can prove that the probability of an `early' termination (i.e., set reconciliation is incomplete in $r$ round) is very small
% %, and even if an `early' termination happens, an overwhelming percentage of distinct elements should have been reconciled, which is sufficient for most applications
% . For example, when $d=5, n=255, r=2$, an `early' termination happens with probability $4.8\times 10^{-4}$ (how to compute this probability will be elaborated in \autoref{sec:tail_bound}).

% For the moment, we assume no incorrectly reconciled distinct elements appears in multi-round PBS, which happens with overwhelming probability as explained in \autoref{subsec:exception_hash_partition}. Then multi-round PBS reconciles the distinct elements gradually round by round. This is the ``piecewise decodability'' mentioned in \autoref{sec:intro_oursolution}. We use the following example to describe it in details: Given two sets $A$, $B$ with $10$ distinct elements (i.e., $d=10$), in the first round, multi-round PBS hashes them into $7$ distinct subset pairs. $6$ distinct elements are hashed into $6$ distinct subset pairs, and the other $4$ distinct elements are hashed into the same subset pair. Then the former $6$ distinct elements are successfully reconciled in the first round and the later $4$ distinct elements remain to be reconciled in the second round, which are hashed into $3$ distinct subset pairs (under a different hash function). $2$ remaining distinct elements are hashed into $2$ distinct subset pairs, and the other $2$ remaining distinct elements are hashed into the same subset pair. Then the former $2$ remaining distinct elements are successfully reconciled in the second round and the later $2$ remaining distinct elements remain to be reconciled in the third round, so on so force. The dynamics of the number of remaining distinct elements (i.e., $10\leadsto 4\leadsto 2\leadsto \cdots$ in the example) is in nature a Markov chain, which will be elaborated and analyzed in \autoref{sec:tail_bound_per_group} to derive a tail bound of success probability (i.e., all distinct elements are reconciled in $r$ rounds) for paramenter settings. 

% In most applications, a high percentage of reconciliation (e.g., $>99\%$ distinct elements are reconciled) is good enough. Therefore, we add another termination condition on the maximum number of rounds (denoted as $r$). The larger $r$ is, the higher percentage of distinct elements will be reconciled. How to set parameters based on $r$ will be elaborated in \autoref{sec:parameter_settings};

% Readers may think the communication overhead of multi-round PBS is proportional to the number of rounds. In fact, the majority of the communication overhead is spent in the first round, since most of the distinct elements (over $95\%$ as we will show in {\bf point to the figure}) are reconciled in the first round. Each additional round only incurs a small amount of additional communication overhead. For example, when $d=10, n=255, |\mathcal{U}|=2^{32}$, assume $8$ distinct elements are reconciled in the first round and the rest $2$ distinct elements are reconciled in the second round. Then the communication overhead in the first round is $432$ bits. That number of the second round is only $160$


%the communication overhead of single-round PBS of $272$ ($2d\log n+d\log |\mathcal{U}|+32$) bits, and each additional round incurs $40$ ($d\log n$) bits of additional communication overhead. 

%among the three components of the communication overhead mentioned in \autoref{sec:communication_overhead_single_PBS}, only the first component (i.e., the BCH codeword) is proportional to the number of rounds. The other two components does not depend on the number of rounds.

% The second component only depends on the total number reconciled elements, which is roughly equal to $d$. The third component, the checksum of $A$, only needs to be sent once in the first round.
%Therefore, the communication overhead of multi-round PBS is only slightly larger than that of single-round PBS when the number of rounds is small (say $3$). For example, when $d=5, n=255, |\mathcal{U}|=2^{32}$, the communication overhead of multi-round PBS of $3$ rounds is $352$ bits, which is roughly $1.3$ times of the communication overhead of single-round PBS ($272$ bits).

% Therefore, each additional round of multi-round PBS only incurs a small amount of additional communication overhead. For example, when $d=5, n=255, |\mathcal{U}|=2^{32}$, the communication overhead of single-round PBS of $272$ ($2d\log n+d\log |\mathcal{U}|+32$) bits, and each additional round incurs $40$ ($d\log n$) bits of additional communication overhead. 

% As we explained in \autoref{sec:reconcile_by_trivial}, the communication overhead in each round is proportional to the number of (remaining) distinct elements, which decreases exponentially as the number of round increase (i.e., the first round reconciles $90\%$ of distinct elements, the second round reconciles $90\%$ of the remaining $10\%$ distinct elements, etc.). So the majority of the communication overhead (i.e., $\approx 90\%$) is in the first round. Therefore, we do not bother to optimize parameters (i.e., smaller $n$) in later rounds to save tiny communication overhead, even though remaining distinct elements become fewer and can be reconciled using smaller $n$;

% The termination condition of multi-round PBS is that all distinct elements are reconciled, which may require many rounds. In most applications, a high percentage of reconciliation (e.g., $>99\%$ distinct elements are reconciled) is good enough. Therefore, we add another termination condition on the maximum number of rounds (denoted as $r$). The larger $r$ is, the higher percentage of distinct elements will be reconciled. How to set parameters based on $r$ will be elaborated in \autoref{sec:parameter_settings};

% Multi-round means multiple round-trip delays. {\bf Thanks for the piecewise decodability of PBS, in almost all practical application scenarios, this tradeoff does not lead to longer response time because the reconciliation of objects identified by the successfully decodable codewords, which constitute the vast majority of all codewords, can run in parallel with the transmissions and decodings of the rest.  In other words, the piecewise decodability effective masks the slightly larger number of communication rounds as far as the response time is concerned.}

\begin{comment}
==============================

The pseudocode of set reconciliation operations in each round is shown as follows:

\IncMargin{1em}
\begin{algorithm}
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
\Input{$A$ and $B^{(in)}$}
\Input{Set of reconciled distinct elements $D^{(in)}$}
\Output{$B^{(out)}$}
\Output{Set of reconciled distinct elements $D^{(out)}$}

% Hash-partition $A^{(in)}$, $B^{(in)}$ into $\{A^{(in)}_i\}_{i=1}^n$, $\{B^{(in)}_i\}_{i=1}^n$ (\autoref{sec:hash_partition})\label{step:hash_partition}\;

% Encode $\{A^{(in)}_i\}_{i=1}^n$, $\{B^{(in)}_i\}_{i=1}^n$ into parity bitmaps (\autoref{sec:parity_bitmap_encoding})\;


% Find those subset pairs (denoted them as $(A^{(in)}_{i_1}, B^{(in)}_{i_1}), ...,(A^{(in)}_{i_k}, B^{(in)}_{i_k})$) that parity bits differ (\autoref{sec:BCH_code})\;

Run single-round PBS on $A$ and $B^{(in)}$ to obtain the (partial) set difference $\mathcal{D}$\label{step:reconcile} \;

$D^{(out)} \leftarrow D^{(in)}\bigcup \mathcal{D}$\label{step:updated}\;

$B^{(out)} \leftarrow B^{(in)}\Delta\mathcal{D}$\label{step:updateb}\;

Check whether the set reconciliation is complete by comparing $A$ to $B^{(out)}$ (via CRC)\label{step:termination}\;

\caption{Set reconciliation operations of PBS in each round} \label{proto:multirounds}
\end{algorithm}\DecMargin{1em}

In \autoref{proto:multirounds}, the output $B^{(out)}$ in the $r^{th}$ round is the input $B^{(in)}$ in the $(r+1)^{th}$ round. $D^{(in)}$ and $D^{(out)}$ have the same relationship, and they denote the set of reconciled distinct elements before and after a round. $B^{(in)}$ and $D^{(in)}$ are initialized as $B$ and $\emptyset$ respectively. We omit the currect number of round $r$ in \autoref{proto:multirounds}, since the operations in different rounds are exactly the same. Due to the same reason, we only elaborate the operations in the first round: First, Alice and Bob reconcile $A$ and $B^{(in)}$ $(=B)$ using single-round PBS and Bob obtains the (partial) set difference $\mathcal{D}$ (\autoref{step:reconcile}); Second, Bob updates the set of reconciled distinct elements by merging it with $\mathcal{D}$ (\autoref{step:updated}); Third, Bob updates $B^{(in)}$ $(=B)$ to $B^{(out)}$ as \autoref{step:updateb} shows, such that (1) The reconciled distinct elements in $\mathcal{D}$ that are contained in $A\Delta B^{(in)}$ are not longer contained in $A\Delta B^{(out)}$; and (2) The distinct elements that are not successfully reconciled remain in $A\Delta B^{(out)}$ and can be reconciled in later rounds; Finally, we check whether all distinct elements are reconciled. Note that if it is true, $B^{(out)}$ should be the same as $A$ and multi-round PBS should terminate. We use a $32$-bit CRC (Cyclic Reduncancy Check) to check if $B^{(out)}=A$ in our evaluation. {\bf To achieve higher confidence, we can certainly use longer CRC (e.g., 64-bit). }

{\bf Remarks:}

(1) In each round, hash-partition in \autoref{sec:hash_partition} uses different hash functions, so that the remaining distinct elements from the last round will be hashed into different subset pairs with high probability;

(2) A straightforward approach to discard reconciled distinct elements is to remove them from both $A$ and $B$. This approach however incurs additional communication overhead to update $A$, since only Bob learns the partial set difference in \autoref{step:reconcile}. Therefore, we use the approach in \autoref{step:updateb} that only updates $B$. It has another benefit in \autoref{step:termination}, which only needs to transmit the CRC of $A$ from Alice to Bob in the first round. In the later rounds, \autoref{step:termination} can be checked locally by Bob and does not require any additional communication overhead;

(3) As we explained in \autoref{sec:reconcile_by_trivial}, the communication overhead in each round is proportional to the number of remaining distinct elements, which decreases exponentially as the number of round increase (i.e., the first round reconciles $90\%$ of distinct elements, the second round reconciles $90\%$ of the remaining $10\%$ distinct elements, etc.). So the majority of the communication overhead (i.e., $\approx 90\%$) is in the first round. Therefore, we do not bother to optimize parameters (i.e., smaller $n$) in later rounds to save tiny communication overhead, even though remaining distinct elements become fewer and can be reconciled using smaller $n$;

(4) One termination condition of Multi-round PBS is $B^{(out)}=A$, which refers that all distinct elements are reconciled. In most applications, a high percentage of reconciliation (e.g., $>99\%$ distinct elements are reconciled) is good enough. Therefore, we add another termination condition of the maximum number of rounds (denoted as $r$). The larger $r$ is, the higher percentage distinct elements will be reconciled, and the smaller $n$ is required. How to set parameters (e.g., $n$) based on $r$ will be elaborated in \autoref{sec:parameter_settings};

(5) Multi-round means multiple round-trip delays. {\bf Thanks for the piecewise decodability of PBS, in almost all practical application scenarios, this tradeoff does not lead to longer response time because the reconciliation of objects identified by the successfully decodable codewords, which constitute the vast majority of all codewords, can run in parallel with the transmissions and decodings of the rest.  In other words, the piecewise decodability effective masks the slightly larger number of communication rounds as far as the response time is concerned.}

==============================

\end{comment}

% (3) Readers may wonder in the later rounds, most distinct elements should be reconciled, and the rest distinct elements could be reconciled using degraded parameters (i.e., smaller $n$ and $t$). In fact, degrade parameters in later rounds cannot save much communication overhead, since the majority of it is spent in the first round (i.e., $>90\%$). Therefore, we use the same parameters (i.e., $n,t$) among all rounds in multi-rounds PBS;

% (4) The number of remaining distinct elements decreases exponentially as the number of round increase (i.e., the first round reconciles $90\%$ of distinct elements, the second round reconciles $90\%$ of the remaining $10\%$ distinct elements, etc.). 
% (4) The termination condition of Multi-rounds PBS is $B^{(out)}=A$ to reconcile all distinct elements. In some applications,  


% The output $B^{(out)}$ in the $r^{th}$ round is the input $B^{(in)}$ in the $(r+1)^{th}$ round. $D^{(in)}$ and $D^{(out)}$ are similarly defined. $B^{(in)}$ and $D^{(in)}$ are initialized as $B$ and $\emptyset$ respectively. Since and $D$ are updated in each round, so we use $B^{(in)}$ to denote the input and $B^{(out)}$ to denote the output respectively.  Specifically, in the first round, we initialize $B^{(in)}$ and $D^{(in)}$ as $B$ and $\emptyset$ respectively. we first use the single-round scheme 

% Then we run our (single-round) scheme on the updated two sets (i.e., after removing reconciled distinct elements) using a different (independent) hash-partition function from previous rounds, so that the rest distinct elements are hashed into different subset pairs (i.e., the ideal case) with high probability. At the end of each round, we check whether the set reconciliation is complete (i.e., all distinct elements are found) by computing the bitwise \code{XOR} of the remaining elements in $A$ and $B$ 
 

% This {\bf multi-rounds} scheme can significantly increase the success probability (i.e., the probability that all distinct elements are reconciled). Readers may wonder in the later rounds, most distinct elements should be reconciled, and the rest distinct elements could be reconciled using degraded parameters (i.e., smaller $n$ and $t$). In fact, degrade parameters in later rounds cannot save much communication overhead, since the majority of it is spent in the first round (i.e., $>90\%$). Therefore, we use the same parameters (i.e., $n,t$) among all rounds in our evaluation. 
% %The tradeoff between the number of rounds and the communication overhead per rounds will be elaborated in \autoref{sec:tail_bound}. In our evaluation, $r=2,3$ rounds are enough to achieve an extremely high success probability. 

% Readers may think the cost (i.e., communication overhead and the computational complexity) of this multi-rounds scheme is proportional to the number of rounds (denoted as $r$) and increases linearly with $r$. In fact, the cost of each round is roughly proportional to the number of remaining distinct elements, which decreases exponentially as $r$ increases (i.e., the first round reconciles $99\%$ of distinct elements, the second round reconciles $99\%$ of the remaining $1\%$ distinct elements, etc.). So the cost of this multi-rounds scheme is only slightly larger than that of the single-round scheme. Furthermore, as we explained in \autoref{sec:intro}, {\bf from intro thanks for the piecewise decodability of our solution, in almost all practical application scenarios, this tradeoff does not lead to longer response time because the reconciliation of objects identified by the successfully decodable codewords, which constitute the vast majority of all codewords, can run in parallel with the transmissions and decodings of the rest.  In other words, the piecewise decodability effective masks the slightly larger number of communication rounds as far as the response time is concerned.} 

\begin{comment}

\subsection{Baseline Scheme}\label{subsec:protocol1} 

Note that the set difference $A\Delta B$ can contain more than 1 elements (i.e., $d>1$), and \autoref{alg:trivial_case} cannot reconcile $A$ and $B$ directly in this case. Therefore, we propose a baseline scheme building upon~\autoref{alg:trivial_case} that also works when $d>1$: First, we partition the element universe $\mathcal{U}$ into $n$ sub-universes $\mathcal{U}_1, \mathcal{U}_2, \cdots, \mathcal{U}_n$. Denote $A_i \triangleq A\bigcap \mathcal{U}_i$ and $B_i \triangleq B\bigcap \mathcal{U}_i$ for $i=1,2,\cdots,n$. Then $\{A_i\}_{i=1}^n$ and $\{B_i\}_{i=1}^n$ are partitions of $A$ and $B$ respectively. Furthermore, $\Phi\triangleq\{A_i\Delta B_i\}_{i=1}^n$ is a partition of $A\Delta B$. 

Assume the {\bf ideal case} happens, in which each subset pair $(A_i, B_i)$ contains at most one distinct element ({\it i.e.,} $|A_i\Delta B_i|\!\leq\!1$), we use \autoref{alg:trivial_case} to reconcile each subset pair and obtain $A_i\Delta B_i$ for $i=1,2,\cdots,n$. The overall set difference $A\Delta B$ is simply their union $\bigcup_{i=1}^n \big{(}A_i\Delta B_i\big{)}$. 

In the first step of the baseline scheme, we can use a hash function $h(\cdot): \mathcal{U}\rightarrow \{1,2,\cdots,n\}$ to partition the universe $\mathcal{U}$ into $n$ sub-universes: $\mathcal{U}_i=\{s\mid s\in \mathcal{U} \mbox{ and } h(s)=i\}$ for $\forall i=1,2,\cdots,n$. And the hash function $h(\cdot)$ can be predetermined between Alice and Bob and does not require additional communication cost.

This hash-partition can be modeled as a {\it balls-into-bins problem}, in which the distinct elements are viewed as balls and the subset pairs are viewed as bins. The hash-parition basically throws (hashes) $d$ balls (distinct elements) uniformly and randomly into $n$ bins (subset pairs). The aforementioned ideal case in this context becomes, after throwing $d$ balls uniformly and randomly into $n$ bins, each bin receives at most 1 ball (i.e., $d$ nonempty bins have 1 ball in each and the rest $n-d$ bins are empty). {\bf It may remind readers about the Birthday problem. And the ideal case can be analogous to the case that no people share the same birthday.} The ideal case happens with a probability of $p=\frac{n\,!}{(n-d)\,!n^d}\!=\!\prod_{k=1}^{d - 1}(1 - \frac{k}{n})\!\approx\! e^{-\frac{d(d-1)}{2n}}$ when $d\!\ll\!n$. In other words, $n$ must be $\Omega(d^2)$ to ensure the ideal case happens with a nontrivial probability.  Note that the communication overhead of the baseline scheme is proportional to $n$, as each subset pair requires communication of a bitwise \code{XOR} in \autoref{alg:trivial_case}. So this communication overhead increases at least quadratically as $d$ increases. 

In fact, this communication overhead can be significantly reduced: In the ideal case, $n-d$ out of $n$ subset pairs are identical ones, and only $d (\ll n)$ out of $n$ subset pairs contain distinct elements (one distinct element in each of the $d$ subset pairs) and need to be reconciled. If we can identify these $d$ subset pairs (with a tiny additional communication overhead) and only reconcile them, the overall communication overhead will be significantly reduced from $\Omega(d^2)$ to $O(d)$. Based on this intuition, we propose our scheme in \autoref{sucsec:our-scheme}, which uses Parity Bitmap Sketch (PBS) and Error Correction Coding (ECC) to identify those subset pairs with a tiny additional communication overhead. 

Note that the ideal case does not always happen. However, we can ensure that the ideal case happens with high probability by properly selecting $n$ based on $d$ (i.e., $n=\Omega(d^2)$). Furthermore, as we will describe in \autoref{subsec:nonideal}, even if the ideal case does not happen (i.e., some distinct elements are hashed into the same subset pair), most of the distinct elements should be distributed into different subset pairs and therefore can be reconciled. So the baseline scheme, even cannot reconcile all of the distinct elements, can still reconcile the majority of them. Based on this property, we will extend our scheme from single-round to multi-rounds in \autoref{subsec:nonideal} to further increase the probability of reconciling all distinct elements. 

For general cases ({\it i.e.,} $t=|A\Delta B|$ is an arbitrary number), we have a straightforward strawman scheme building upon~\autoref{alg:trivial_case}, which works as follows: First, Alice and Bob choose some hash function $h(s): \mathcal{U} \rightarrow \{0,1,\cdots,2^{32}-1\}$ to partition $A$ and $B$ into $m$ subsets $A_1,A_2,\cdots,A_m$ and $B_1,B_2,\cdots,B_m$ respectively:

\begin{align}
s\in A_i & \mbox{ iff } s\in A \mbox{ and } h(s)=i\!\mod m, \nonu{}mber\\
s\in B_i & \mbox{ iff } s\in B \mbox{ and } h(s)=i\!\mod m. \nonumber
\end{align} 

{\bf call a subset pair -> partition?} Since Alice and Bob use the same hash function for partition, common elements (i.e., elements in $A\cap B$) are always hashed into the same subset pair $(A_i, B_i)$. And the set difference of each subset pair only contains distinct elements (i.e., elements in $A\Delta B$): $A_i\Delta B_i \subset A\Delta B$. In the ideal case, with a sufficient large $m$, each subset pair $(A_i, B_i)$ contains at most one distinct element ({\it i.e.,} $|A_i\Delta B_i|\!\leq\!1$). Then \autoref{alg:trivial_case} can reconcile each subset pair and obtain $A_i\Delta B_i$ for $i=1,2,\cdots,m$. The overall set difference $A\Delta B$ is simply their union $\bigcup_{i=1}^m \big{(}A_i\Delta B_i\big{)}$. The selection of hash function $h(s)$ can be predetermined between Alice and Bob and it does not require additional communication cost.

%To make sure Alice and Bob use the same hash function for partition, we let them pre-agree on some universal hash family (e.g., \code{xxHash}~\cite{Collet_xxHashExtremelyfast_}) and a common selection order, and each time they choose a hash function from the family in the same order. Note that we can also let Alice generates a hash function and send it to Bob. The hash function that Alice and Bob choose for partition can be either generated by 

This hash-partition is in nature a {\it balls-into-bins model}. We can view the distinct elements as balls and the subset pairs as bins. The hash-parition basically throws (hashes) $t$ balls (distinct elements) uniformly and randomly into $m$ bins (subset pairs). The aforementioned ideal case in this context is, with a sufficient large number of bins, each bin receives at most 1 ball. The strawman scheme works correctly if and only if the ideal case happens, which has a probability of $\frac{m\,!}{(m-t)\,!m^t}\!=\!\prod_{k=1}^{t - 1}(1 - \frac{k}{m})\!\approx\! e^{-\frac{t(t-1)}{2m}}$. In other words, to ensure the strawman scheme works correctly with a probability of $p$, it roughly requires $m \!=\!\lceil \frac{t(t-1)}{-2\ln p}\rceil$ subset pairs. 

Note that the communication overhead of this strawman scheme is proportional to the number of subset pairs $m$, as each subset pair requires communication of an \code{XOR} sum in \autoref{alg:trivial_case} during the reconciliation. When $t$ is small, a small communication cost can guarantee that the strawman scheme works correctly with high probability. For instance, when $t=5$, $m=95$ subset pairs are sufficient for the strawman scheme to work correctly with a probability of $90\%$. However, when $t$ is relatively large, it requires a huge communication cost to ensure the strawman scheme works correctly. For instance, when $t=1,000$, it requires $m=4,740,865$ subset pairs to guarantee a success probability of $90\%$. 

In fact, the majority of subset pairs are identical ones and do not need to reconcile. And only a small portion of them contain distinct elements. If we can identify those subset pairs that contain distinct elements and only reconcile them, the communication cost could be significantly reduced. Our scheme is based on this intuition and uses parity bitmap sketch and BCH code to identify the subset pairs, which we will elaborate in \autoref{sucsec:our-scheme}. 

%To distribute balls as uniformly as possible and maximize the probability of the ideal case, we choose a uniform hashing function $h$ that throws balls uniformly and randomly into bins: $$\mathbb{P}[h(s)=i]=\frac{1}{m} \mbox{ for } \forall i=1,2,\cdots,m, \forall s\in U$$.

%Note that the probability of the ideal case is $\frac{m\,!}{(m-t)\,!m^t}\!=\!\prod_{k=1}^{t - 1}(1 - \frac{k}{m})\!\approx\! e^{-\frac{t(t-1)}{2m}}$. Hence, at least $\lceil \frac{t(t-1)}{-2\ln p}\rceil$ bins are required to ensure that this probability is at least $p$. In other words, to ensure that the ideal case happens with a probability of $p$, the strawman scheme roughly requires $m \!=\!\lceil \frac{t(t-1)}{-2\ln p}\rceil$. For example, suppose $t\!=\!$\num{1000}, %and $p\!=\!0.01$, this strawman scheme roughly requires $m\!=\!$\num{720626} bins (partitions) to ensure that $|A_i\Delta B_i|\!\leq\!1$ (for any $i=1,2,\cdots,m$) holds with probability $50\%$.  

% A straightforward strawman scheme building upon~\autoref{alg:trivial_case} 
% to reconcile two sets $A$ and $B$ in general 
% ({\it i.e.,} $|A\Delta B|$ is an arbitrary number) is the following: 
% Uniformly randomly partition $A$ and $B$ into $m$ subsets ($A_1,A_2,\cdots,A_m$ 
% and $B_1,B_2,\cdots,B_m$) so that the set difference 
% $A_i\Delta B_i$ of each subset pair $(A_i, B_i)$ contains at most one element 
% ({\it i.e.,} $|A_i\Delta B_i|\!\leq\!1$) {\it w.h.p.} ({\it i.e.,} with high probability), 
% and then reconcile each subset pair with~\autoref{alg:trivial_case}. 

% Now let us analyze this strawman scheme using the {\it balls-into-bins model}. 
% Assume that sets $A$ and $B$ have $t$ elements in their set difference, {\it i.e.,} $|A\Delta B|\!=\!t$. 
% These $t$ elements can be viewed as $t$ balls and the $m$ partitions (subset pairs) can be viewed as 
% $m$ bins. The random partition process in this strawman scheme can be modeled as throwing 
% $t$ balls into $m$ bins in the following manner: Each ball goes into a 
% uniformly random bin and independently of other balls. %so that each bin contains at most one ball, {\it w.h.p.}  
% The probability that each bin contains at most one ball is  
% $\frac{m\,!}{(m-t)\,!m^t}\!=\!\prod_{k=1}^{t - 1}(1 - \frac{k}{m})\!\approx\! e^{-\frac{t(t-1)}{2m}}$. 
% Hence, at least $\lceil \frac{t(t-1)}{-2\ln p}\rceil$ bins are required 
% to ensure that this probability is at least $p$. In other words, to ensure 
% that each bin contains at most one ball with a probability of $p$, 
% the strawman scheme roughly requires $m \!=\!\lceil \frac{t(t-1)}{-2\ln p}\rceil$. 
% For example, suppose $t\!=\!$\num{1000}, %and $p\!=\!0.01$, 
% this scheme roughly requires $m\!=\!$\num{108469} bins (partitions) to 
% ensure that $|A_i\Delta B_i|\!\leq\!1$ (for any $i=1,2,\cdots,m$) holds with probability $0.01$.  

% We note that the communication overhead of this strawman scheme is proportional to 
% $m$ ($\!\gg\! t$), as each partition (subset pair) requires communication of an \code{XOR} sum during the reconciliation. 
% This communication overhead is much higher than that of the optimal scheme, which only requires 
% to exchange the elements in the set difference (assuming an oracle tells it which elements belong to 
% the set difference), {\it i.e.,} proportional to $t$. In the example above, assuming each element takes 4 bytes, 
% the communication overhead of the strawman scheme is $4m$ bytes ($\!\approx\! \num{423.71}\,$KB) to ensure 
% a success rate of only 0.01 ({\it i.e.,} with a probability of $0.0.1$, all elements in 
% the set difference are successfully reconciled), 
% which is approximately 2 orders of magnitude higher than $4t$ bytes ($\!=\!\num{3.90}\,$KB), the communication 
% overhead of the optimal scheme. 

\subsection{Our Scheme: The Preliminary Version}\label{sucsec:our-scheme}

Like the baseline scheme, our scheme also hash-partitions the two sets $A$ and $B$ into $n$ subset pairs. The difference is, instead of reconciling all subset pairs using \autoref{alg:trivial_case}, our scheme identifies the subset pairs that contains distinct elements and only reconciles them. Since the hash-partition and set reconciliation on each subset pair using \autoref{alg:trivial_case} have been described in \autoref{subsec:protocol1}, we only elaborate how to identify the subset pairs that contain distinct elements in this section. 

The general idea of identification is very simple: First, we {\bf encode} each subset into $1$ bit, such that in the ideal case, for $\forall i=1,2,\cdots,n$:

\begin{itemize}
	\item The codewords (bits) of $A_i$ and $B_i$ are different if and only if subset pair $(A_i, B_i)$ contains $1$ distinct element;
	\item The codewords (bits) of $A_i$ and $B_i$ are the same if and only if subset pair $(A_i, B_i)$ contains no distinct element;
\end{itemize}

Second, we {\bf compare} the codewords of each subset pair. And the subset pairs that contain distinct elements are the ones with different codewords (bits). We will describe the two steps in details in \autoref{sec:parity_bitmap_encoding} and \autoref{sec:BCH_code} respectively.

\subsubsection{Parity Bitmap Encoding}\label{sec:parity_bitmap_encoding}

In our scheme, we use {\it parity encoding} to encode each subset into a parity bit. More specific, it encodes a subset as ``1'' if it contains odd number of elements, and as ``0'' otherwise. And it satisfies the aforementioned requirements in the ideal case:

\begin{itemize}
	\item If subset pair $(A_i, B_i)$ contains $1$ distinct element, the corresponding two subsets $A_i$ and $B_i$ differ exactly one element, which implies that $||A_i|\!-\!|B_i||\!=\!1$. Hence, if $|A_i|$ ({\it i.e.,} number of elements in $A_i$) is odd (or even), then $|B_i|$ must be even (or odd). And the parity bits of $A_i$ and $B_i$ will be different;
	\item If subset pair $(A_i, B_i)$ contains no distinct element, the corresponding two subsets $A_i$ and $B_i$ should be the same and therefore contain the same number of elements. Hence, if $|A_i|$ is odd (or even), then $|B_i|$ must be odd (or even). And the parity bits of $A_i$ and $B_i$ will be the same;
\end{itemize}

Using parity encoding, the $n$ subsets of $A$ are encoded as a bit string $A[1..n]$ in $\{0,1\}^n$, 
where the $i$-th bit $A[i]$ in $A[1..n]$ corresponds to the parity encoding bit of $A_i$. Similarly, the $n$ subsets of $B$ are similarly 
encoded as a bit string $B[1..n]$. We call $A[1..n]$ ($B[1..n]$) the {\it parity bitmap} of $\{A_i\}_{i=1}^n$ ($\{B_i\}_{i=1}^n$). In the ideal case, $A[1..n]$ and $B[1..n]$ differ at $d$ different bit-positions, which corresponds to the $d$ subset pairs that contain distinct elements. And our scheme only reconciles those subset pairs that the parity bits are different. We will describe the nonideal case (i.e., some subset pair contains more than 1 distinct elements) in \autoref{subsec:nonideal}.

\subsubsection{Parity Bitmap Comparison Using BCH Code}\label{sec:BCH_code}

A straightforward approach to compare the parity bitmaps is to let Bob send the complete parity bitmap $B[1..n]$ to Alice, then Alice compares $A[1..n]$ with $B[1..n]$ locally. This approach has a communication overhead of $n$ bits, which is unnecessarily high. As we discussed in~\autoref{subsec:protocol0}, $d$ is usually much smaller than $n$. It means $A[1..n]$ and $B[1..n]$ differ only at a tiny portion of bits. Therefore, we can view $A[1..n]$ as a corrupted message of $B[1..n]$ with $d$ corrupted bits, and the bit-positions of the $d$ corrupted bits basically correspond to the $d$ subset pairs that contain distinct elements. The detection of corrupted bits, on the other hand, can be solved by Error-Correction Code (ECC)~\cite{Lin_ErrorControlCoding_1983}. And our scheme uses BCH code~\cite{Lint_IntroductionCodingTheory_1998} to encode the parity bitmap and detect the $d$ corrupted bits.

More specific, after the parity bitmap encoding, Bob uses a $d$-error-correcting systematic BCH code to encode $B[1..n]$ into an $n+d\log n$ codeword, in which the first $n$ bits are $B[1..n]$ (property of systematic BCH code). Then Bob sends the rest $d\log n$ bits, which we denote as {\it parity bitmap sketch (PBS)}, to Alice. Upon the received PBS and $A[1..n]$ (corrupted message), Alice uses the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} to detect the $d$ corrupted bits in $A[1..n]$. The communication overhead of this approach is $d\log n$ bits (i.e., length of PBS), which is much smaller than that of the straightforward approach ($n$ bits, when $d\!\ll\!n$). On the other hand, the computational complexity of the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} is $O(d^2\log^2 n)$. 

\subsubsection{Exceptional Handling and Multi-rounds}\label{subsec:nonideal}

As we described in \autoref{subsec:protocol1}, the ideal case does not always happen, which means some subset pair may contain more than 1 distinct elements and cannot be successfully reconciled by \autoref{alg:trivial_case}. Due to the parity encoding, we can classify such subset pair into the following two scenarios:

\begin{itemize}
    \item Scenario 1: If a subset pair $(A_i, B_i)$ contains even number ($\geq 2$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be the same and our scheme will not reconcile the subset pair. Hence, the distinct elements in the subset pair will not be reconciled;
    \item Scenario 2: If a subset pair $(A_i, B_i)$ contains odd number ($\geq 3$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be different and our scheme will reconcile the subset pair using \autoref{alg:trivial_case}. However, as we described in \autoref{subsec:protocol0}, when a subset pair contains more than 1 distinct elements, \autoref{alg:trivial_case} will output the bitwise \code{XOR} of them as the `distinct element', which is not a real distinct element with high probability;
\end{itemize}

In both scenarios, the distinct elements in the subset pair cannot be reconciled. Even worse, in the second scenario, a false-positive could happen (i.e., the output of \autoref{subsec:protocol0} is not a real distinct element). However, as we will analyze in \autoref{sec:tail_bound} and show in {\bf the evaluation section}, the second scenario barely happens both theoretically and empirically. To further reduce the chance of false-positives, we add a verification step at the end of \autoref{subsec:protocol0} to check whether the output of \autoref{subsec:protocol0} $s$ is a real distinct element or not. The verification step works as follows: Given the output $s$ of subset pair $(A_i,B_i)$, if $s\in\mathcal{U}_i$ (i.e., $h(s)=i$), we consider $s$ as a real distinct element; Otherwise, we consider $s$ as an incorrect output and discard it. 

Note that if $s$ is a real distinct element of $(A_i,B_i)$, $s$ must be in sub-universe $\mathcal{U}_i$. However, if $s$ is the bitwise \code{XOR} of the distinct elements in $(A_i,B_i)$ (i.e., the second scenario happens), $s$ could be in any sub-universe other than $\mathcal{U}_i$. In fact, if we assume the hash-partition described in \autoref{subsec:protocol1} hashes the elements of $\mathcal{U}$ uniformly, independently, and randomly into $n$ sub-universes, the output $s$ in the second scenario will be in a different sub-universe $\mathcal{U}_j (j\neq i)$ with a high probability of $1-\frac{1}{n}$. Hence, this verfication step can reduce the chance of false-positives by a factor of $\frac{1}{n}$. 

Even if the ideal case does not happen, most of the distinct elements should be distributed into different subset pairs and therefore can be reconciled. So our scheme, even cannot reconcile all of the distinct elements, can still reconcile the majority of them (piecewise decodability). To reconcile the rest distinct elements, we can just run our scheme for another round under a different hash-partition function, so on so force. This {\bf multi-rounds} scheme can significantly increase the success probability (i.e., the probability that all distinct elements are reconciled). Readers may wonder in the later rounds, most distinct elements should be reconciled, and the remaining could be reconciled using degraded parameters (i.e., smaller $n$ and $t$). In fact, degrade parameters in later rounds cannot save much communication overhead, since the majority of it is spent in the first round (i.e., $>90\%$). Therefore, we use the same parameters (i.e., $n,t$) among all rounds in our evaluation.
%The tradeoff between the number of rounds and the communication overhead per rounds will be elaborated in \autoref{sec:tail_bound}. In our evaluation, $r=2,3$ rounds are enough to achieve an extremely high success probability. 

Readers may think the cost (i.e., communication overhead and the computational complexity) of this multi-rounds scheme is proportional to the number of rounds (denoted as $r$) and increases linearly with $r$. In fact, the cost of each round is roughly proportional to the number of remaining distinct elements, which decreases exponentially as $r$ increases (i.e., the first round reconciles $99\%$ of distinct elements, the second round reconciles $99\%$ of the remaining $1\%$ distinct elements, etc.). So the cost of this multi-rounds scheme is only slightly larger than that of the single-round scheme. Furthermore, as we explained in \autoref{sec:intro}, {\bf from intro thanks for the piecewise decodability of our solution, in almost all practical application scenarios, this tradeoff does not lead to longer response time because the reconciliation of objects identified by the successfully decodable codewords, which constitute the vast majority of all codewords, can run in parallel with the transmissions and decodings of the rest.  In other words, the piecewise decodability effective masks the slightly larger number of communication rounds as far as the response time is concerned.} 

\end{comment}


%%% Moved from related work
\input{section/pinsketch}

\section{PBS for large \texorpdfstring{\larger\boldmath\MakeLowercase{$d$}}{d}}\label{subsec:protocol2}

Note that the BCH decoding computational complexity is $O(d^2)$ of finite field operations (in GF($2^{8}$) when $n=255$) using the state-of-the-art decoding algorithm~\cite{Dodis_SyndromeEncodingDecoding_2006}, which is too expensive for large $d$. To overcome this drawback, we first hash-partition sets $A$ and $B$ each into $d/\delta$ subsets (which we call {\it groups} to distinguish from subsets), just like what we did in \autoref{sec:hash_partition}, for some small integer $\delta$ (say $5$), then reconcile each of the group pairs by the PBS we described in \autoref{sec:scheme}. After the partition, each group pair has $\delta$ distinct elements on average. So the BCH decoding computational complexity of each group pair is roughly $O(\delta^2)$, which can be considered as a constant, since $\delta$ is a small number. As a result, the overall computational complexity of PBS is reduced from $O(d^2)$ to $O(d)$. 

%To differentiate from the PBS described in \autoref{sec:scheme}, we refer to it as PBS-basic in this section. 
We continue to assume that the number of distinct elements $d$ is precisely known. Even so, due to the randomness of hash-partition, $\delta_i$, the number of distinct elements in the $i$-th group pair, is a Binomial random variable with mean of $\delta$ for $i=1,2,...,g$, which cannot be precisely known without a huge amount of additional communication overhead. Since $\delta_1, \delta_2, ..., \delta_g$ follows the identical Binomial distribution, there is no sense to set different parameters among the $g$ group pairs. Hence, we set two universal parameters, $t$ and $n$, for all group pairs, where $t$ is the error-correction capability of the BCH code used for reconciling each group pair, and $n$ is the number of subset pairs in each group pair.

%To deal with this randomness, we set two global parameters, denoted as $t$, that corresponds to the error-correction capability of the BCH code used for reconciling every group pair. identical no sense or additonal info

{\bf (modified based on the next paragraph from intro)} Setting $t$ properly is critical for PBS to perform well. On one hand, if $t$ is too large (say $t=10\delta$), then the communication overhead on transmitting BCH codeword for each group pair ($t\log n$ bits) is unnecessarily large; but on the other hand, if $t$ is too small (say equal to $\delta$), then close to half of the group pairs fail to decode the BCH codeword due to the insufficient error-correction capability, which can result in hefty penalties on BCH decoding failures (to be described in \autoref{sec:BCH_exception}). In PBS, we manage to make $t$ as small as possible (so that the communication overhead on transmitting BCH codewords is kept to a minimum) yet pay negligible penalties of BCH decoding failures. 

% To ensure the error-correction capability $t$ is sufficient (i.e., $t\geq \delta_i$ for $i=1,2,...,g$) for every group pair with high probability, we set $t$ conservatively and leave a sufficient `safety margin' between $t$ and the average number of distinct elements in each group pair $\delta$. 

% Note that the `safety margin' between $t$ and $\delta$ incurs additional communication overhead on transmitting BCH codeword: In the perfect scenario (i.e., $\{d_i\}_{i=1}^g$ is precisely known), the average communication overhead on transmitting BCH codeword per group pair is $\delta\log n$; On the other hand, when we set $t$ to be the error-correction capability for each group pair, the average communication overhead becomes $t\log n$. If we set the `safety margin' to be too large (say $t=10\delta$), it will incur huge additional communication overhead. Due to this reason, we set a moderate `safety margin' that  $t$ in the range from $1.5\delta$ to $3\delta$. 

{\bf (moved from intro, to be removed)} The number of elements in the set difference between any group pair is in general not a constant.  Rather, it is a random variable that has roughly a Poisson distribution with mean $\delta$.  The potential issue arises from dealing with this randomness in setting a global parameter that corresponds to the error-correction capability of the BCH code used for reconciling every group pair.  This parameter, denoted as $t$ (consistent with other literatures on BCH code), is the maximum number of errors that the BCH code used by any group pair can correct, and the size of each such codeword is roughly $8t$ bits (assuming $n = 255$ as explained above). The issue is that, on one hand, if $t$ is too large (say several times larger than $\delta$), then the total size of the BCH codewords, which is the bulk of the extra communication cost, is unnecessarily large; but on the other hand, if $t$ is too small (say equal to $\delta$), then close to half of the BCH codewords cannot decode or worse decode incorrectly (unknown to Alice and Bob), which can result in hefty penalties in the latter case of incorrect decoding.   In PBS, we manage to make $t$ as small as possible (so that the total size of the BCH codewords is kept to a minimum) yet pay negligible penalties of incorrect BCH decoding.
%We will discuss the case that $d_i>t$ in \autoref{sec:BCH_exception}.

% Hence, we can no longer set the error-correction capability of the BCH code for each group pair based on the exact number of distinct element in it, as we did in \autoref{sec:scheme}. Instead, we set a conservative error-correction capability $t$ (say $2.5\delta$) for all group pairs, which is sufficient for them (i.e., $t\geq d_i$ for $i=1,2,...,g$) with high probability. We will discuss the case that $d_i>t$ in \autoref{sec:BCH_exception}.


% ===============================
% To differentiate from the PBS described in \autoref{sucsec:our-scheme}, we refer it as PBS-basic in this section. Note that the BCH decoding computational complexity is $O(d^2\log ^2 n)$, which is $\Omega(d^2\log^2 d)$ when $n=\Omega(d^2)$, with the state-of-the-art decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019}. It is too large in PBS-basic for large $d$. To overcome this drawback and generalize PBS-basic for large $d$, we partition sets $A$ and $B$ each into $d/\delta$ subsets (which we call {\it groups} to distinguish from subsets) for some small integer $\delta$ (say $5$) and reconcile the $d/\delta$ group pairs respectively using PBS-basic. After this partition, each group has $\delta$ distinct elements on average. The BCH decoding computational complexity of each group pair can be considered as $O(1)$, since $\delta$ is a small number. As a result, the overall computational complexity of PBS is reduced from $O(d^2\log ^2 n)$ to $O(d)$. 

% % To differentiate from the PBS described in \autoref{sucsec:our-scheme}, we refer it as PBS-basic in this section. PBS-basic is not suitable for large $d$ for two reasons: First, its communication overhead is asymptotically $O(d\log n)\!=\!O(d\log d)$ (since $n=\Omega(d^2)$), which is not asymptotically optimal. Second, the decoding computational complexity is proportional to $d^2$ with the state-of-the-art decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} for BCH codes, which is too high when $d$ is large. To overcome these two drawbacks, we use a simple algorithmic trick to (1) reduce the communication overhead from $O(d\log d)$ to $d\log u \!+\! O(d)$; (2) reduce the decoding computational complexity from $O(d^2)$ to $O(d)$. 

% Now, we describe the generalized PBS in details: In the first step, we hash-partition $A$ and $B$ (by some hash function $h_1(\cdot)$) into $g$ group pairs, just like what we did in \autoref{sucsec:our-scheme}. The objective of this partition is however different: In \autoref{sucsec:our-scheme}, we aim to ensure each subset pair contains at most $1$ distinct element (i.e., the ideal case) with high probability; Here we aim to make each group pair contains roughly $\delta$ distinct elements for some small constant $\delta$ (say $5$) by setting $g=d/\delta$. 
% %To differentiate the $g$ subset pairs here from those in \autoref{sec:hash_partition}, we call them the $g$ {\bf groups} in the sequel. 
% In the second step, we just apply PBS-basic (described in \autoref{sucsec:our-scheme}) to reconcile each group pair and obtain the distinct elements. 
% ================================

% To differentiate from the PBS described in \autoref{sucsec:our-scheme}, we refer it as PBS-basic in this section. When $d$ is large (more than several), we hash-partition set $A$ and $B$ into groups, such that each group pair contains $\delta$ distinct elements on average for small $\delta$ (say $5$), as described in \autoref{sec:larged}. Then each group pair can be reconciled by PBS-basic.

% When describing the PBS-basic in \autoref{sucsec:our-scheme}, we assume that the number of distinct elements is precisely known. We set the error-correction capability of the BCH code (denoted as $t$) just enough to correct $d$ errors (i.e., $t=d$). However, due to the randomness of hash-partition, $d_i$, the number of distinct elements in the $i^{th}$ group pair, is a Binomial random variable $Binomial(d,1/g)$ with expectation of $\delta$ $(=d/g)$ for $i=1,2,...,g$, which cannot be precisely known without a huge amount of additional communication overhead. Hence, we can no longer set the error-correction capability of the BCH code for each group pair based on the exact number of distinct element in it, as we did in \autoref{sucsec:our-scheme}. Instead, we set a universal error-correction capability $t$ (say $2.5\delta$) for all group pairs, which is sufficient for all group pairs (i.e., $t\geq d_i$ for $i=1,2,...,g$) with high probability. We will discuss the case that $d_i>t$ in \autoref{sec:BCH_exception}.

%This assumption in general does not hold: 
% Let $d_i$ denote the number of distinct elements in Group $i$. Due to the property of hash-partition, each $d_i$ is a Binomial random variable $Binomial(d,1/g)$ with expectation of $\delta$ $(=d/g)$. Even if $d$ is precisely known, each $d_i$ is not. To ensure the error-correction capability $t$ is sufficient for each group (i.e., $d_i\leq t$) with high probability, we leave some safety margin for the randomness of $d_i$ and conservatively set $t$ roughly $2.5\delta$ (the factor $2.5$ varies depend on other parameters, which will be discussed in \autoref{sec:parameter_settings}), so that $Pr[d_i>t]$ is tiny. We will discuss the case that $d_i>t$ in \autoref{sec:BCH_exception}.

% Note that the `safety margin' between $t$ and $\delta$ incurs additional communication overhead on transmitting BCH codeword: In the perfect scenario (i.e., $\{d_i\}_{i=1}^g$ is precisely known), the average communication overhead on transmitting BCH codeword per group pair is $\delta\log n$; On the other hand, when we set $t$ to be the error-correction capability for each group pair, the average communication overhead becomes $t\log n$. If we set the `safety margin' to be too large (say $t=10\delta$), it will incur huge additional communication overhead. Due to this reason, we set a moderate `safety margin' that  $t$ in the range from $1.5\delta$ to $3\delta$. 

%which is roughly $2.5$ times of that in the perfect scenario (when $t$ is roughly $2.5\delta$). Due to this addition
{\bf (modified)} If we have an accurate estimation of $\{\delta_i\}_{i=1}^g$, we can set $\{t_i\}_{i=1}^g$, the error-correction capabilities of the $g$ group pairs, to be very close to (slightly larger) those estimations. It can save considerate communication overhead on transmitting the BCH code. However, to estimate all the $g$ values of $\{\delta_i\}_{i=1}^g$ in high accuracy requires much larger additional communication overhead than the savings. 

{\bf (previous)} Readers may wonder if we can reduce this additional communication overhead by using some technique to estimate $\{d_i\}_{i=1}^g$ (e.g., ToW estimator in \autoref{subsec:ToW}), so that we can set the error-correction capability of each group more wisely and save some waste on the safety margin. However, to achieve that, the estimation on $\{d_i\}_{i=1}^g$ must be in extremely high precision (since $\{d_i\}_{i=1}^g$ are small numbers with mean of $\delta$), which incurs much larger additional communication overhead than the savings. Due to the same reason (i.e., estimate $\{d_i\}_{i=1}^g$ is costly), we set the number of subset pairs for each group pair to be all equal (denoted as $n$). 
%based on $\delta$ ($n=\Omega(\delta^2)$). 

{\bf (moved from the small d case)} Although PBS runs as many rounds as to reconcile all distinct elements (in each group pair), we want PBS to successfully reconcile all distinct elements in only a few rounds (say $3$) with high probability (say $99\%$). Hence, when tuning parameters (to be discussed in \autoref{sec:parameter_settings}), we set a {\it target success probability} $p_0$ combined with a {\it target number of rounds} $r$ as the {\it paramenter setting requirement}, which aims to ensure that the {\it success probability}, the probability that all distinct elements are reconciled, within $r$ rounds to be larger than $p_0$. 
{\bf Normally, to achieve the same target success probability within fewer rounds (smaller $r$), PBS need more resources (e.g., larger $n$, $t$) for the ideal case happening with higher probability (fewer exceptions happen and need to be handled in later rounds), as we will explain in \autoref{sec:parameter_settings}.}
This success probability (within $r$ rounds) is also the expected value of the {\it success rate} of PBS, which is defined as the number of `successful' experiments (all distinct elements are successfully reconciled within $r$ rounds) divided by the total number of experiments. 

%The requirement above should also ensure the majority of the distinct elements are reconciled in the first round. 
% Note that PBS reconciles the distinct elements gradually round by round. The distinct elements that have been reconciled in the first round are no longer needed to be reconciled again in later rounds. This is the ``piecewise decodability'' mentioned in \autoref{sec:intro_oursolution}. The requirement above also ensures the majority of the distinct elements are reconciled in the first round, as we will show in \autoref{sec:piecewise_decodability}. Therefore, the majority of the overall communication overhead happens in the first round. In other words, the overall communication overhead of all rounds is only slightly larger than ($1.01$ to $1.07$ times of) that in the first round. Due to this reason, we use the communication overhead in the first round (described in \autoref{sec:communication_overhead_single_PBS}) to approximate the overall communication overhead of all rounds in parameter settings (to be elaborated in \autoref{sec:parameter_settings}.


% Like what we did in \autoref{sec:multi-rounds}, we set a paramenter setting requirement on the target success probability $p_0$ of $r$ rounds for all group pairs, which ensures the probability that all group pairs are completely reconciled in $r$ rounds to be larger than $p_0$. The detail about how to set $n$, $g$, and $t$ given such a success probability requirement will be elaborated in \autoref{sec:parameter_settings}. 

% we set a {\it target success probability} $p_0$ of $r$ rounds as a paramenter setting requirement, which aims to ensure the probability that all distinct elements are reconciled in $r$ rounds to be larger than $p_0$. This requirement should also ensure the majority of the distinct elements are reconciled in the first round. Use the same example ($d=5, n=255$), on average $4.81$ out of $5$ distinct elements should be reconciled in the first round. So the total communication overhead in all rounds is only slightly larger than ($1.01$ to $1.07$ times of, as we will show in \autoref{fig:per-round-con}) that in the first round. Due to this reason, we use the communication overhead in the first round (described in \autoref{sec:communication_overhead_single_PBS}) to approximate the total communication overhead of all rounds in parameter settings (to be elaborated in \autoref{sec:parameter_settings}.

% Note that this safety margin incurs additional communication overhead on transmitting BCH codeword: In the perfect scenario (i.e., $\{d_i\}_{i=1}^g$ is precisely known), the average communication overhead on transmitting BCH codeword per group is $\delta\log n$; On the other hand, when we set $t$ to be the error-correction capability for each group, then the average overhead becomes $t\log n$, which is roughly $2.5$ times of that in the perfect scenario (when $t$ is roughly $2.5\delta$). Readers may wonder if we can reduce this additional communication overhead by using some technique to estimate $\{d_i\}_{i=1}^g$ (e.g., ToW estimator in \autoref{subsec:ToW}), so that we can set the error-correction capability of each group more wisely and save some waste on the safety margin. However, to achieve that, the estimation on $\{d_i\}_{i=1}^g$ must be in high precision, which requires a much higher communication overhead than the savings.

% Although PBS may need to run many rounds to reconcile all distinct elements, the communication overhead mostly happens in the first round, since the majority of the distinct elements should be reconciled in the first round. Use the same example ($d=5, n=255$), on average $4.81$ out of $5$ distinct elements should be reconciled in the first round. So the total communication overhead in all rounds is only slightly larger than ($1.01$ to $1.07$ times of, to be shown in \autoref{fig:per-round-con}) that in the first round. Due to this reason, we use the communication overhead in the first round (described in \autoref{sec:communication_overhead_single_PBS}) to approximate the total communication overhead (all rounds) in parameter settings (to be elaborated in \autoref{sec:parameter_settings}).

%For the moment, we assume no ``fake'' distinct element in type (\RN{2}) subset pairs fails to be detected, which happens with overwhelming probability as explained in \autoref{subsec:exception_hash_partition}. Then 

% PBS reconciles the distinct elements gradually round by round. This is the ``piecewise decodability'' mentioned in \autoref{sec:intro_oursolution}. We use the following example to describe it in details: 
% Given two sets with $10$ distinct elements, in the first round, PBS tries to reconcile the $10$ distinct elements and say $6$ out of the $10$ distinct elements are successfully reconciled. Then the $6$ reconciled distinct elements are removed and PBS tries to reconcile the remaining $4$ distinct elements in the second round. Say $2$ out of the $4$ remaining distinct elements are successfully reconciled, and that leaves $2$ remaining distinct elements to be reconciled in the third round, so on so force. 
% % Given two sets $A$, $B$ with $10$ distinct elements, in the first round, PBS hashes them into $7$ distinct subset pairs. $6$ distinct elements are hashed into $6$ distinct subset pairs, and the other $4$ distinct elements are hashed into the same subset pair. Then the former $6$ distinct elements are successfully reconciled in the first round and the later $4$ distinct elements remain to be reconciled in the second round, which are hashed into $3$ distinct subset pairs (under a different hash function). $2$ remaining distinct elements are hashed into $2$ distinct subset pairs, and the other $2$ remaining distinct elements are hashed into the same subset pair. Then the former $2$ remaining distinct elements are successfully reconciled in the second round and the later $2$ remaining distinct elements remain to be reconciled in the third round, so on so force. 
% The dynamics of the number of remaining distinct elements (i.e., $10\leadsto 4\leadsto 2\leadsto \cdots$ in the example) is in nature a Markov chain, which will be elaborated and analyzed in \autoref{sec:single_markov} to derive a tight tail bound of the probability that all distinct elements are reconciled in $r$ rounds. 

%, which we will show in \autoref{subsec:mini-partition}.

% The same algorithmic trick can also be implemented in PinSketch~\cite{Dodis_PinSketch_2008} to reduce it computational complexity from $O(d^2)$ to $O(d)$. However, it will encounter the same randomness problem and have to set up a safety margin on the error-correction capability. This safety margin will incur much more communication overhead on PinSketch than on our scheme: Considering the average communication overhead per group, in our scheme, this overhead can be expressed as $t\log n+\delta\log n+\delta \log u+32$, in which $t\log n$ accounts for the BCH codeword, $\delta\log n$ accounts for the index of the subset pairs, $\delta \log u$ accounts for the bitwise \code{XOR} in \autoref{alg:trivial_case}, and $32$ accounts for the $32$-bit CRC in \autoref{proto:multirounds}. In PinSketch, this overhead increases from $O(\delta\log u)$ (optimal) to $O(t\log u)$ (PinSketch does not need to transmit bitwise \code{XOR}) if it uses the same algorithmic trick. Use the same example in \autoref{sec:intro}, when $\delta=5, n=255, u=2^{32}, t=2.5\delta$, the overhead of PinSketch using the trick is $2.5$ times of the optimal, while that of our scheme is $2.075$ times of the optimal (as we introduced in \autoref{sec:intro_oursolution}). That means our scheme has a lower communication overhead than PinSketch if they both use the algorithmic trick. Furthermore, as the signiture size $\log u$ increases, the advantage of our scheme over PinSketch becomes more significantly, which we will show in \autoref{subsec:mini-partition}.

% In PinSketch, each bit encodes only a single element in the universe, so the size of the bitmap is equal to the size of the universe.  
% For example, in the set reconciliation problem we usually assume each element is ``indexed" by a $32$-bit-long (hash) signature, so the universe contains a total of $2^{32}$ elements. In this case, the bitmap encoding for any set in PinSketch is $2^{32}$ bits long, and the Galois field involved in its BCH decoding is the ``$32$-bit-wide" $GF(2^{32})$.  In contrast, as explained earlier, in PBS 
% %since each bit encodes the oddness or evenness of the cardinality of a subset,   
% the size $n$ of a bitmap is dependent only on $d$, and not on the size of the universe or on the cardinality of the set the bitmap encodes.   For example, as shown in the example above, $n = 255$ is large enough for $d = 5$.  In this case, the BCH decoding operates in the much shorter
% ``8-bit-wide" $GF(2^{8})$.  This shorter ``width" alone in theory translates into roughly $16$ times shorter BCH decoding time, which as will be explained in~\ref{} grows quadratically with the ``width" of the underlying Galois field.  This shorter ``width" also implies four times shorter BCH codeword in PBS than in PinSketch, resulting in lower communication complexity as will be shown in~\autoref{}.

% Note that our scheme only takes 1 round trip delay to both identify the $d$ subset pairs and reconcile them: In the first half, Bob computes and sends PBS to Alice. Then Alice locally identifies the $d$ subset pairs and then initiates the reconciliation ({\it i.e.,} \autoref{alg:trivial_case}) for them, {\it i.e.,} computes the bitwise \code{XOR} of the corresponded $d$ subsets. In the second half, Alice sends the bitwise \code{XOR} of the $d$ subsets with their indexes to Bob. Then Bob can compute the set difference $A\Delta B$ locally.


% We can certainly use some communication-efficient technique to estimate $d_i$ (e.g., \autoref{subsec:ToW}). However, to obtain $d_i$ precisely will require a communication cost almost as large as to reconcile Group $i$. So instead of obtaining $d_i$ and set $c_i$ (i.e., the error-correction capability of Group $i$) equal to $d_i$, we leave the randomness of $d_i$ and set $c_i$ neither too conservative, nor too libertive in the following sense: (1) $c_i$ is not too big (conservative, i.e., $10\delta$) to make the total size of PBS unnecessarily large and incur too much extra communication overhead; (2) $c_i$ is not too small (libertive, i.e., $\delta$) to incur a high probability of insufficient decode capability, which can result in hefty penalties in the latter case of incorrect decoding (will be elaborated in \autoref{sec:BCH_exception}). In our scheme, we set $c_i$ to be $2-3$ times of $\delta$, which will be shown in \autoref{sec:tail_bound} that it is just enough to make the probability of decode failure very small. Meanwhile, we set the error-correction capability of each group ($c_1,c_2,...,c_k$) to be all equal and denote it as $c$. 

%Since the decoding capacity $t$ and the number of subset pairs for each group $n$ are both small constants independent of $d$, therefore, the communication overhead per group is $t\cdot\log n \!=\!O(1)$, which implies a total communication overhead of $O(d)$. Similarly, the total decoding computational complexity is also $O(d)$. 

% \subsection{Exception Handling}\label{sec:exceptions}

% \subsubsection{Exception Handling on Hash-Partition}\label{subsec:exception_hash_partition}

% As we have described in \autoref{sec:hash_partition}, the ideal case does not always happen, which means some subset pair may contain more than 1 distinct elements and cannot be successfully reconciled by \autoref{alg:trivial_case}. Due to the parity encoding, we can classify such subset pair into the following two scenarios:

% \begin{itemize}
%     \item Scenario 1: If a subset pair $(A_i, B_i)$ contains even number ($\geq 2$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be the same and our scheme will not reconcile the subset pair. Hence, the distinct elements in the subset pair will not be reconciled;
%     \item Scenario 2: If a subset pair $(A_i, B_i)$ contains odd number ($\geq 3$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be different and our scheme will reconcile the subset pair using \autoref{alg:trivial_case}. However, as we described in \autoref{subsec:protocol0}, when a subset pair contains more than 1 distinct elements, \autoref{alg:trivial_case} will output the bitwise \code{XOR} of them as the `distinct element', which is not a real distinct element with high probability;
% \end{itemize}

% In both scenarios, the distinct elements in the subset pair cannot be reconciled. Even worse, in the second scenario, a false-positive could happen (i.e., the output of \autoref{subsec:protocol0} is not a real distinct element). For example, if subset pair $(A_i, B_i)$ contains $3$ distinct elements $s_1, s_2, s_3$, then the output of \autoref{alg:trivial_case} is $\tilde{s}_4=s_1\oplus s_2\oplus s_3$, which is normally not a distinct element. The good thing is, the probability of the false-positive is extremely small for small $d$. For instance, if $d=5$ and $n=255$, the probability of the false-positive is $7.6\times 10^{-6}$, which is very small. To further reduce the chance of false-positives, we add a verification step at the end of \autoref{subsec:protocol0} to check whether the output of \autoref{subsec:protocol0} $s$ is a real distinct element or not. The verification step works as follows: Given the output $s$ of subset pair $(A_i,B_i)$, if $s\in\mathcal{U}_i$ (i.e., $h(s)=i$), we consider $s$ as a real distinct element; Otherwise, we consider $s$ as an incorrect output and discard it. 

% Note that if $s$ is a real distinct element of $(A_i,B_i)$, $s$ must be in sub-universe $\mathcal{U}_i$. However, if $s$ is the bitwise \code{XOR} of the distinct elements in $(A_i,B_i)$ (i.e., the second scenario happens), $s$ could be in any sub-universe other than $\mathcal{U}_i$. In fact, if we assume the hash-partition described in \autoref{sec:hash_partition} hashes the elements of $\mathcal{U}$ uniformly, independently, and randomly into $n$ sub-universes, the output $s$ in the second scenario will be in a different sub-universe $\mathcal{U}_j (j\neq i)$ with a high probability of $1-\frac{1}{n}$. Hence, this verfication method can further reduce the probability of false-positives by a factor of $\frac{1}{n}$. Use the same example (i.e., $d=5$, $n=255$), the probability is reduced from $7.6\times 10^{-6}$ to $3\times 10^{-8}$ by this verification method. 

% In some super critical cases (i.e., no false-positive is allowed), we can use a more powerful verification method to completely eliminate false-positives. That is, to check if the output $s$ exists in exactly one of the two sets (i.e., $s\in A\setminus B$ or $s\in B\setminus A$). To do so, Bob transmits $s$ along with an identification bit $\mathbb{1}_{\{s\in B\}}$ to Alice, then Alice checks if $s$ . This method verification costs $d(\log u+1)$ bits of additional communication overhead. In most applications, rigorously $0\%$ probability of false-positives is unnecessary and the probability of the former verification method is small enough, so we use the former verfication method in our evaluation. Based on our observation, the false-positive does not happen even once in our evaluation using the former verfication method.

\subsection{Exception Handling on BCH Decoding}\label{sec:BCH_exception}

The exceptions that happens when the error-correction capability $t$ is sufficient have been discussed and handled in \autoref{subsec:exception_hash_partition} and \autoref{sec:multi-rounds}. In this section, we only discuss the exceptions that are caused by insufficient error-correction capability. That is, when $\delta_i$ (i.e., the number of distinct elements in group pair $i$) is larger than the error-correction capability $t$, the BCH codewords of group pair $i$ differ at $\delta_i$ bit positions in the ideal case, which exceeds the error-correction capability $t$. If so, the BCH decoder cannot decode the bit errors correctly (\autoref{step:BCH_decode} in \autoref{alg:single_round_pbs}) and report a failure. This exception happens with a small probability in each group pair: For example, when $d=1000$, and $\delta$ is set to $5$ (so that $g=d/\delta=200$), and $t$ is set to $13$, the probability that this exception happens is only $6.7\times 10^{-4}$. 

To handle this type of exceptions, we use the same algorithm trick in \autoref{subsec:protocol2} to further partition each problematic group into $3$ sub-groups and reconcile them respectively using the PBS we described in \autoref{sec:scheme}. Note that $\delta_i$, if is not smaller, should be only slightly larger than $t$ with high probability. Hence, partitioning into $3$ sub-groups is enough to ensure each sub-group has no more than $t$ distinct elements. Then in the next round, each sub-group does not encounter this type of expections and can be reconciled by the PBS we described in \autoref{sec:scheme} respectively. Use the same example above ($d=1000$, $\delta=5$, $t=13$), the probability that some sub-group has more than $t$ distinct elements is $9.5\times 10^{-10}$. More specifically, we add a termination condition of \autoref{alg:3_way_partition} after \autoref{step:BCH_decode} in \autoref{alg:single_round_pbs}.

\begin{algorithm}
\caption{Termination condition when BCH decoding fails}
\label{alg:3_way_partition}

\If{BCH decoding fails\label{step:if1}}
{Hash-partition the group into $3$ sub-groups and do PBS for each of them in the next round; Break;}\label{step:term1} 

\end{algorithm}

% Back to the \autoref{proto:multirounds}, which shows the set reconciliation operations in each round of PBS-basic, this kind of exceptions only affect \autoref{step:reconcile} in \autoref{proto:multirounds}. Now this step needs to check whether BCH decoding is successful or not: If successful, all the operations remain the same; Else, we hash-partition the group ($A$ and $B$) into $3$ sub-groups and reconcile them respectively using \autoref{proto:multirounds}. 
{\bf I'm not sure if it is necessary to discuss this case, since PinSketch did not mention it, even it may happen in PinSketch}
Another type of exceptions that happens when $d_i>t$ is, the BCH decoder mistakes the decoding is successful and returns $t$ incorrectly decoded bit errors (i.e., subset pairs). The probability of this type of exceptions is very small. For instance, when $d=1000, \delta=5, t=13$ $(2.5\delta)$, $d_i>t$ happens with probability roughly $6.7\times 10^{-5}$, and the probability that the BCH decoder mistakes the decoding is successful when $d_i>t$ is on the order of $10^{-7}$ \cite{kim1996undetected}. So the probability that this type of exceptions happens in each group is on the order of $10^{-12}$. On the other hand, the impact of this type of exceptions is insignificant. Assume an incorrectly decoded bit error corresponds to a random subset pair, which could contain (1) no distinct element; (2) exactly $1$ distinct element; or (3) more than $1$ distinct elements. Reconcile the subset pair using \autoref{alg:trivial_case} could (1) get nothing and waste $\log |\mathcal{U}|$ bits of communication overhead; (2) get an actual distinct elements; or (3) trigger the exceptions that were discussed and handled in \autoref{subsec:exception_hash_partition}. 

\subsection{What if PinSketch also uses partitions?}

The same algorithmic trick (i.e., hash-partition two sets each into groups) can also be implemented in PinSketch~\cite{Dodis_PinSketch_2008} to reduce it computational complexity from $O(d^2)$ (of finite field operations in GF($2^{32}$)) to $O(d)$. However, it will encounter the same randomness problem and have to set up a ``safety margin'' on the error-correction capability $t$. This ``safety margin'' will incur much more additional communication overhead on PinSketch than on our scheme: Considering the average communication overhead per group pair, the additional overhead caused by the ``safety margin'' is $(t-\delta)\log n$ in PBS and $(t-\delta)\log |\mathcal{U}|$ in PinSketch. The later is roughly $4$ times of the former under the default setting ($n=255, |\mathcal{U}|=2^{32}$). Note that the optimal communication overhead to reconcile $d$ distinct elements is $\delta\log |\mathcal{U}|$. Use the same example in \autoref{sec:intro}, when $\delta=5, n=255, |\mathcal{U}|=2^{32}, t=2.5\delta$, the overhead of PinSketch using the algorithmic trick is $2.5$ times of the optimal (i.e., $d\log |\mathcal{U}|$), while that of PBS is $2.075$ times of the optimal. It means PBS could have a lower communication overhead than PinSketch if they both use the algorithmic trick. Furthermore, as the signiture length $\log |\mathcal{U}|$ increases, the advantage of PBS over PinSketch will be more significant.

% We handle this type of exceptions by the same method (i.e., hash-partition into $3$ sub-groups) as above. To detect them, on the other hand, is simple: Note that incorrect decoded bit errors correspond to the subset pairs that do not contain distinct elements. When we reconcile those subset pairs in \autoref{sec:reconcile_by_trivial}, the output (i.e., reconciled elements) will be $\mathbf{0}$, which is abnormal (since $\mathbf{0}\notin A\bigcup B$, as we described in \autoref{subsec:protocol0}). Hence, this type of exceptions happen if and only if one of the reconciled distinct elements is $\mathbf{0}$. 
%Hence, we consider BCH decoding is successful by two criteria: (1) the BCH decoder reports a successful decode; and (2) None of the reconciled elements is $\mathbf{0}$. 
% ========================
% In fact, even if $d_i>t$, PBS-basic is still possible to reconcile group $i$ in some nonideal cases. For example, when $t=10$ and $d_i=11$, if the $11$ distinct elements are distributed in $10$ subset pairs, such that $1$ subset pair contains $2$ distinct elements and $9$ subset pairs contain $1$ distinct element in each, the two parity bitmaps differ at only $9$ bit positions. So BCH decoder is able to decode the later $9$ subset pairs and the corresponding $9$ distinct elements can be reconciled. In the second round, only $2$ distinct elements remain and BCH decoding certainly works. In this case, we do not need to partition the group into sub-groups, and this case does not trigger \autoref{alg:3_way_partition} in PBS. 
% ========================
% Instead, it will either (1) report a failure about exceeding the error-correction capability; or (2) mistake the decoding is successful and return incorrect decoded bit errors. 

% The second case happens with a very small probability (in order of $10^{-7}$ \cite{kim1996undetected}) and is very simple to detect : 

% The first case is easy to handle: We can simply adapt the same algorithmic trick to partition the group into smaller groups and reconcile them respectively. In our scheme, we set the number of smaller groups to be $3$, which is big enough because $d_i$, if not smaller, only slightly larger than $t$ with high probability. The second case on the other hand, although theoretically possible, happens with a very small probability when $d_i>t$ (in order of $10^{-7}$ \cite{kim1996undetected}). Besides, the probability of $d_i>t$ is also very small (e.g., when $t=15$ and $\delta=5$, this probability is about $2.3\times 10^{-4}$), so the overall probability of the second case, which is the multiplication of these two small numbers, is negligible (e.g., in order of $10^{-11}$).

% \subsection{Multi-rounds}

% Even if the ideal case does not happen, most of the distinct elements should be distributed into different subset pairs and therefore can be reconciled. So our scheme, even cannot reconcile all of the distinct elements, can still reconcile the majority of them (piecewise decodability). To reconcile the rest distinct elements, we can just run our scheme for multi-rounds under different hash-partition functions. For each round, our scheme works as follows: 

% \IncMargin{1em}
% \begin{algorithm}
% \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
% \Input{Two sets $A$ and $B$}
% \Input{Size of set difference $d$}
% \Input{The number of subset pairs $n$}
% \Input{BCH error-correction capability $t$}

% Hash-partition $A$ and $B$ into $n$ subset pairs $\{(A_i,B_i)\}_{i=1}^n$;

% \If{BCH decoding fails}
% 	Hash-partition $A$ and $B$ into $3$ subset pairs and reconcile them respectively in the next round\;
% \ElseIf{BCH decoding success}
	
% \Else{}

% $k \leftarrow \lceil \frac{t}{c}\rceil $\;

% Partition elements into $k$ subsets using~\autoref{alg:random-part}\;

% \For{$j = 0$ \KwTo $k-1$}{
%     Reconcile the $j$-th subset pair using the straw-man scheme with the BCH correcting capability $\tau$, number of smaller subsets $m$, and number of rounds $r$\;
% }

% \caption{PBS (per round)} \label{proto:II}
% \end{algorithm}\DecMargin{1em}

% This {\bf multi-rounds} scheme can significantly increase the success probability (i.e., the probability that all distinct elements are reconciled). Readers may wonder in the later rounds, most distinct elements should be reconciled, and the remaining could be reconciled using degraded parameters (i.e., smaller $n$ and $t$). In fact, degrade parameters in later rounds cannot save much communication overhead, since the majority of it is spent in the first round (i.e., $>90\%$). Therefore, we use the same parameters (i.e., $n,t$) among all rounds in our evaluation. 
% %The tradeoff between the number of rounds and the communication overhead per rounds will be elaborated in \autoref{sec:tail_bound}. In our evaluation, $r=2,3$ rounds are enough to achieve an extremely high success probability. 

% Readers may think the cost (i.e., communication overhead and the computational complexity) of this multi-rounds scheme is proportional to the number of rounds (denoted as $r$) and increases linearly with $r$. In fact, the cost of each round is roughly proportional to the number of remaining distinct elements, which decreases exponentially as $r$ increases (i.e., the first round reconciles $99\%$ of distinct elements, the second round reconciles $99\%$ of the remaining $1\%$ distinct elements, etc.). So the cost of this multi-rounds scheme is only slightly larger than that of the single-round scheme. Furthermore, as we explained in \autoref{sec:intro}, {\bf from intro thanks for the piecewise decodability of our solution, in almost all practical application scenarios, this tradeoff does not lead to longer response time because the reconciliation of objects identified by the successfully decodable codewords, which constitute the vast majority of all codewords, can run in parallel with the transmissions and decodings of the rest.  In other words, the piecewise decodability effective masks the slightly larger number of communication rounds as far as the response time is concerned.} 





\begin{comment}
\subsubsection{Random Partition}

\IncMargin{1em}
\begin{algorithm}
% \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
% \Input{Set $S$}
% \Input{The number of subsets $m$ for partition}
% \Output{Subsets $S_1, S_2, ..., S_m$}

% Generate hash function $h(\cdot)$ that maps each element into $\{1,2,...,m\}$;

\ForEach{$s \in S$}{
    $j \leftarrow h(s) \bmod m$\;    
    Insert $s$ into the $j$-th subset $S_j$\;
}

\caption{Partition using hash function $h(\cdot)$.} \label{alg:random-part}
\end{algorithm}\DecMargin{1em}

Like the strawman scheme, our scheme randomly partitions sets $A$ and $B$ into $m$ subsets. This random partition 
can be easily accomplished by using some hash function, $h(\cdot)$, and inserting each element $x$ into the subset 
corresponding to $h(x)$. \autoref{alg:random-part} presents the pseudo-code of this random partition using hash 
function $h(\cdot)$.  

% Unlike the strawman scheme, our scheme only reconciles those subset pairs that need to be reconciled, 
% because 



Like the strawman scheme, our scheme hash-partitions the two sets $A$ and $B$ into $m$ subset pairs $(A_i, B_i)$ for $i=1,2,\cdots,m$. 
We note that, among those $m$ bins (subset pairs), 
at most $t$ ($t\!\ll\!m$ as shown in our analysis in~\autoref{subsec:protocol1}) bins contain balls 
(elements belonging to the set difference), {\it i.e.,} requiring reconciliation.  
Motivated by this observation, we, therefore, propose to first detect those bins that 
contain balls and then only reconcile them. The detection is solved with a simple encoding approach that 
will be detailed in the next section.

\subsubsection{Detection before Reconciliation} 

In fact, identifying those non-empty bins is easy when each bin contains at most one ball. In this section, we assume that 
each bin after the random partition contains at most one ball, we will show later how to handle the cases when some 
bins contain more than one balls later in~\autoref{subsec:exceptions}. 

Given an arbitrary bin (say subset pair $(A_i, B_i)$) that contains one ball ({\it i.e.,} $A_i\Delta B_i$ contains exactly one element), 
the corresponding two subsets $A_i$ and $B_i$ differ exactly one element, which implies that 
$||A_i|\!-\!|B_i||\!=\!1$. Hence, if $|A_i|$ ({\it i.e.,} number of 
elements in $A_i$) is odd (or even), then $|B_i|$ must be even (or odd). In other words, the odevity of $|A_i|$ 
and $|B_i|$ are opposite. %differs if $|A_i\Delta B_i|\!=\!1$. 
Based on this property, we propose the {\it odevity encoding}: 
A subset is encoded as ``1'' if it contains odd number of elements, and as ``0'' otherwise. 
Using this odevity encoding, the $m$ subsets of $A$ can be encoded as a bit string $b_A$ in $\{0,1\}^m$, 
where the $i$-th bit in $b_A$ corresponds to the odevity encoding of $|A_i|$. Similarly, the $m$ subsets of $B$ can also 
be encoded as a bit string $b_B$. Clearly, $b_A$ and $b_B$ differ at $t$ different positions, or in other words, 
the Hamming distance of bit strings $b_A$ and $b_B$ is $t$. A straightforward approach is 
to let Alice send $b_A$ to Bob, and then Bob compares $b_B$ against $b_A$ to obtain those non-empty bins. 

This approach, however, has a communication overhead of $m$ bits, which is still unnecessarily high. As 
analyzed in~\autoref{subsec:protocol0}, $t$ is usually much smaller than $m$. 
That means $b_A$ and $b_B$ differ only at a tiny portion of bits. %have much more in common than differences. 
Therefore, if we view $b_B$ as a corrupted message of $b_A$ with $t$ corrupted bits, the detection of those $t$ bins can be converted to 
the detection of the positions of the $t$ corrupted bits. The latter can be solved using an Error-Correction Code (ECC)~\cite{Lin_ErrorControlCoding_1983} that can correct up to $t$ errors. In this work, we use the BCH code~\cite{Lint_IntroductionCodingTheory_1998}. 
More precisely, this ECC-based approach (with the BCH code) works as follows. 
Alice computes the parity bits for $b_A$ using a $t$-error-correcting BCH code with a block length of 
$(2^{\lceil \log m\rceil} -1)$ and sends the parity bits to Bob. Bob then decodes the positions of the $t$ corrupted bits 
using the BCH decoding algorithm with $b_B$ and those parity bits received from Alice. The communication overhead of 
this approach is roughly $t\lceil \log m\rceil$ ($=O(t\log t)$) bits. In the example above, this communication overhead is 
roughly $\num{17000}$ bits, which is approximately $6$ times lower 
than $m\!=\!\num{108469}$ bits, the communication overhead of the aforementioned straightforward approach. 

At first sight, it seems that the detection of non-empty bins and reconciliation of subsets in those bins require two rounds 
(or at least two round trip delays), {\it i.e.,} one round for detection and the other for reconciliation. In fact, 
it only requires one. After Bob receives the parity bits from Alice and decodes out those non-empty bins, it initiates 
the reconciliation ({\it i.e.,} \autoref{alg:trivial_case}) for each bin (subset pair) immediately, 
{\it i.e.,} sends the \code{XOR} sums of subsets in those bins together the indexes of those bins. 
After receiving those \code{XOR} sums and bin indexes, Alice can compute the set difference. 

% A naive way to combine the detection of non-empty bins and reconciliation of subset pairs in those bins is to first detect 
% those non-empty bins via one round of message exchanges between Alice and Bob and then to reconcile the corresponding 
% subset pairs in those bins with another round of message exchanges. This requires two rounds ({\it i.e.,} taking at least 
% two round trip delays). In fact, after Bob receives the parity bits from Alice and obtains those 

\subsubsection{Multiple Rounds}\label{sec:multiround}

{\bf This section was not clear enough. I need more time to think about and revise it.}


In the above section, we have assumed that each bin contains at most one ball. 
However, even with a sufficient large $m$, some bin might contain more than one balls though with tiny probability. 
We will show in~\autoref{subsec:exceptions}, how such rare events, {\it i.e.,} one bin contains more than one balls, 
can be easily detected.
To ensure our scheme can successfully reconcile all elements even when such rare events happen, 
we propose to use multiple rounds (of communication between Alice and Bob). More precisely, instead of 
selecting a prohibitively large $m$ to ensure that each bin contains at most one ball with a extremely high probability 
(say 0.99999), we select a reasonably large $m$ so that the communication overhead is not very high and very few bins contain 
more than one balls (or in other words, most bins contain at most one ball). Therefore, after running one round of 
our scheme, most elements in the set difference will be reconciled. Only those in the bins that contain more than one balls 
fail to be reconciled. For elements in the subsets corresponding to those bins, we run another round of our scheme. 
If some elements still fail to be reconcile, we can run one more round of our scheme. So on so forth,  
our scheme can keep running for more rounds until all elements are reconciled. 

With the same communication overhead, multiple rounds can significantly increase the success rate, 
{\it i.e.,} the probability that all elements in the set difference will be successfully reconciles, 
which will be elaborated in~\autoref{sec:tail_bound}. 

% % to be emphasized
% % say that too many rounds should be avoided (latency & communication overhead reduction is negligible when r is too large, 2 - 3 is good enough)
% % multiple rounds is not an issue when r is small

% We note that the number of rounds $r$, however, should not be large. On one hand, it results in large latency (at least $r$ round trip delays). 
% On the other hand, when $r$ is large, the reduction of communication overhead by the increase of $r$ gradually diminishes. 

We note that multiple rounds, when $r$ is small, would not really increase the ``latency'', as long as most elements in the 
set difference can be reconciled in the first rounds, since the underlying synchronization of data objects corresponding to 
those elements can start immediately after the first round of our scheme. Therefore, the actual latency is one round trip delay instead of 
$r$. 

As we mentioned, this straw-man protocol works correctly if each subset pair has at most one exclusive element (i.e., \autoref{eq:requirement_strawman} holds). On the other hand, if a subset pair has more than one exclusive elements, some of which will not be successfully reconciled:

\begin{itemize}
\item If a subset pair has even number of exclusive elements, Odevity coding will encode it as 0. Then the straw-man scheme will consider the subset pair having no exclusive element and all exclusive elements in this subset will not be reconciled;

\item If a subset pair has odd number ($\geq 3$) of exclusive elements, Odevity coding will encode it as 1 and consider the subset pair having only 1 exclusive element. Then the straw-man scheme will use \autoref{alg:trivial_case} to decode only one exclusive element and dismiss all others. Even worse, the only decoded element is probably not a real exclusive element, since the element computed by \autoref{alg:trivial_case} is the \code{XOR} sum of all exclusive elements, not one of them. 
\end{itemize}

In summary, if a subset pair has more than one exclusive elements, most of its exclusive elements cannot be reconciled, and the reconciled element is usually incorrect (i.e., false-positive). The false-positive however is easy to check, which will be elaborated in \autoref{subsec:exceptions}. The good thing is, even if not all subset pairs have at most one exclusive element and are successfully decoded, most of them will be w.h.p.. In other words, even if the straw-man protocol cannot reconcile all exclusive elements, it still can reconcile most of them. To reconcile all exclusive elements w.h.p., we can simply extend the single-round straw-man scheme to multi-round. And each round adapts the straw-man scheme to do set reconciliation using independent hashing functions $h(\cdot)$ for partition (i.e., in \autoref{alg:random-part}). This multi-round extension can significantly increase the probability of a successful reconciliation, which will be elaborated in \autoref{sec:tail_bound}. 



\subsection{Our Scheme: The Final Version}\label{subsec:protocol2}

{\bf Under revision~}

The preliminary version of our scheme suffers from two major drawbacks. 
First, its communication overhead is asymptotically 
$O(t\log m)\!=\!O(t\log t)$, which is not asymptotically optimal. 
Second, the decoding computational complexity is proportional to 
$t^2$ with the state-of-the-art decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} for BCH codes, 
which is too high when $t$ is large. 
To overcome these two drawbacks, we use a simple algorithmic trick: divide and conquer. With this algorithmic 
trick, the decoding computational complexity is reduced to $O(t)$, 
and the communication overhead is reduced to $t\cdot\frac{\log u}{8} \!+\! O(t)$ (with a small 
hidden constant roughly varying from 4 to 8) bytes which implies that 
our scheme has an additive communication overhead (compared to the optimal scheme) 
of 4 to 8 bytes per element in the 
set difference and this additive overhead is independent of the key size ({\it i.e.}, $\log u$). 
Recall that the IBF-based schemes usually have a communication overhead of roughly 6 times of the 
optimal scheme, which increases linearly as the key size. Therefore, our scheme is much more 
communication-efficient. 

Now, we describe in detail this algorithmic trick. We let Alice divide elements in $A$ into $\lceil\frac{t}{c}\rceil$ groups (subsets)  
for some small constant $c$ (say $5$) so that each group contains roughly $c$ elements from the set difference on average. We let Bob do the same operations on $B$. To ensure that any common element ({\it i.e.,} any element $x\!\in\! A\bigcup B$) goes into 
the same group ({\it i.e.,} groups at Alice and Bob with the same index), we can use the partition procedure with a hash function shown 
in~\autoref{alg:random-part}. Then, we can apply the preliminary version on each group with a constant $m$ (say $m\!=\!256$) independent of 
$t$. To ensure that each group can be reconciled with a high probability, we need to use BCH codes whose decoding capacity 
larger than $c$ (say $\tau\!=\!2c$), as exact number of elements to be reconciled could be larger than $c$. 
Since this decoding capacity $\tau$ is still a small constant independent of $t$, therefore, the communication 
overhead per group is $\tau\cdot\log m \!=\!O(1)$, which implies a total communication overhead of $O(t)$. 
Similarly, the total decoding computational complexity is also $O(t)$. 

\subsubsection{Parameter Configurations} 

Our scheme now has several parameters: $c$ (average number of elements from the set difference in each group), 
$\tau$ (the correcting capability of the BCH code), $m$ (number of bins for each group), and $r$ (maximum number of rounds). 
We note that the maximum number of rounds $r$ is usually associated with another parameter $p$ the desired success rate: With 
at most $r$ rounds, our scheme should guarantee that the success rate is at least $p$. 
%How to tune these parameters to achieve favorable performance will be detailed later in~\autoref{sec:tail_bound}. 
Here, we provide some guidances for the parameter configurations using our theoretical analysis, which gives the tail bound of 
the success probability of our scheme and will be shown in~\autoref{sec:tail_bound}. 

\noindent
{\bf Parameterizing $c$ and $r$.} The values of $c$ and $r$ are usually provided by users based on the requirements of 
applications. For the value of $c$, a larger $c$ results in a longer decoding time yet lower communication overhead.  
So if the decoding time is a big concern, then a smaller $c$ (say $c=5$) should be used; otherwise, a larger $c$ could be used. 
For the values of $r$, a larger $r$ leads to lower communication overhead and usually lower decoding time (as it allows to use 
a smaller $\tau$), however, the reduction is marginal when $r>3$. Therefore, we suggest users to configure $r$ to be $2$ or $3$. 
% The configuration of $c$ is relatively straightforward, as a larger $c$ will result in 
% a longer decoding time and a slightly lower communication overhead. The former is ..., The latter is slightly tricky. 


\noindent
{\bf Using $c$ and $r$ to parameterize other parameters.} After users specify the values for $c$ and $r$ (associated with a value for 
$p$), we can use our theoretical analysis in~\autoref{sec:tail_bound} to parameterize $\tau$ and $m$. 
Since in a BCH code, the block length is in the form of $2^q-1$, we only need to consider $m=2^q-1$. 

{\bf Liang, please revise the following algorithm!}

\begin{algorithm}
\SetKwProg{Proc}{}{}{end}
\SetKwFunction{algo}{\small Search}

\Proc{Search($c$, $r$, $p$)}{\label{search:entrance}

$\mbox{co}_{best}\leftarrow\infty$\tcc*{\small Best communication overhead}

\For{$\tau \leftarrow c\,\KwTo\, \infty$}{}



}
\end{algorithm}


% , unlike 
% the IBF-based schemes which have an multiplicative overhead of 6 
% The inspiration is from the famous 
% divide and conquer algorithm for the selection problem, in which, given an array with $n$ elements, we want to get the $k$-th largest 
% element. A straightforward idea for this problem is sorting. However, if using insertion-sorting, the complexity would be $O(n^2)$. 
% Then the famous divide and conquer trick comes. It first divides the array into $\lceil n/5\rceil$ groups so that the first 
% $\lfloor n/5\rfloor$ contains $5$ elements and at most one group contains the rest $n \mod 5$ elements, and find the median of each 
% group using the insertion-sorting and th


% This straw-man scheme still has a problem on decoding computational complexity. More specific, the complexity increases dramatically with the total number of corrupted bits $t$. Therefore, when $t$ is moderate or large, the decoding computational complexity could be very high. For instance, the decoding complexity of BCH codes~\cite{Lint_IntroductionCodingTheory_1998} is $O(t^3)$, which could be quite high for a large $t$. To keep the decoding complexity reasonably low, we design the following two-layer protocol: In the first layer, we use a hash function to partition the two sets into $\lceil\frac{t}{c}\rceil$ subsets for some small constant $c$ (say $5$), just like the first step of our straw-man scheme. The objective, which is however different from before, is to make each subset pair contains roughly $c$ exclusive elements on average. In the second layer, we use the straw-man scheme with the same configuration (number of subsets $m$, and error-correction capability $\tau$, number of rounds $r$) to reconcile each subset pair. 

% In fact, the straw-man scheme is a proper solution when $t$ is small. First, the decoding complexity will not be a problem for a small $t$; Second, we do not need an extremely large $m$ to guarantee \autoref{eq:requirement_strawman} w.h.p.. For instance, when $t=5$ and $m=1024$, \autoref{eq:requirement_strawman} holds with probability $\frac{m\,!}{(m-t)\,!m^t}\approx 99\%$. This motivates us to design the following two-layer protocol: In the first layer, we use a hash function to partition the two sets into $\lceil\frac{t}{c}\rceil$ subsets for some small constant $c$ (say $5$), just like the first step of our straw-man scheme. The objective, which is however different from before, is to make each subset pair contains roughly $c$ exclusive elements on average. In the second layer, we use the straw-man scheme with the same configuration (number of subsets $m$, and error-correction capability $\tau$) to reconcile each subset pair. 

\autoref{proto:II} shows the pseudocode of our scheme. It first uses the same hash-function based random partition algorithm as \autoref{alg:random-part} to partition elements into $k\triangleq\lceil \frac{t}{c} \rceil$ subsets. Note that the random partition only guarantees that each such subset 
contains $c$ exclusive elements on average, and the exact number is not known. Hence, our scheme uses a BCH code with a capability of 
correcting up to $\tau$ errors with $\tau > c$ to make sure that the BCH code has a high probability to decode successfully. We will describe how to deal with situation where the size of set difference exceeds $\tau$ later in~\autoref{subsec:exceptions}.

As the decoding of a $\tau$-error-correcting BCH code where $\tau$ is a small constant has a constant-time computational complexity, the decoding complexity of 
our scheme is $O(k)=O(t)$. We now have several parameters, average number of exclusive elements in each subset $c$, the correcting capability $\tau$ of BCH code, the number of smaller subsets $m$ for each subset to be divided to, and the number of rounds $r$. How to tune these parameters to achieve favorable performance will be detailed later in~\autoref{sec:tail_bound}. 

\IncMargin{1em}
\begin{algorithm}
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
\Input{Size of set difference $t$}
\Input{The number of subsets $m$ for each partition}
\Input{Average number of exclusive elements in each partition $c$}
\Input{BCH code capability $\tau$}

$k \leftarrow \lceil \frac{t}{c}\rceil $\;

Partition elements into $k$ subsets using~\autoref{alg:random-part}\;

\For{$j = 0$ \KwTo $k-1$}{
    Reconcile the $j$-th subset pair using the straw-man scheme with the BCH correcting capability $\tau$, number of smaller subsets $m$, and number of rounds $r$\;
}

\caption{Our Scheme} \label{proto:II}
\end{algorithm}\DecMargin{1em}




\subsection{Exceptional Handling}\label{subsec:exceptions}

{\bf To be revised~}

In this section, we will elaborate how to handle the following two types of exceptions that we mentioned in \autoref{sec:multiround} and \autoref{subsec:protocol2}:
\begin{itemize}
    \item Exception 1: A subset pair has odd number ($\geq 3$) of exclusive elements and causes false-positives (i.e., a decoded distinct element is not a real one);
    \item Exception 2: A subset pair contains too many exclusive elements, such that a BCH code with capability of correcting up to $\tau$ errors cannot decode it (i.e., $t>\tau$).
	\item Exception 3: A subset pair has even number ($\geq 2$) of exclusive elements and causes false-negatives(i.e., two or more distinct elements are neglected as the parity bit is 0);
\end{itemize}

To handle Exception 1, we need to check whether a computed exclusive element by \autoref{alg:trivial_case} is a real exclusive element or not. (The group index happens to come in handy if we use it as a fingerprint of the element we computed. If this element is truly an exclusive element, it should be hashed into the same group as before. Notably, We have two group indices available for this check, one is in the initial divide and conquer phase, the other is in the BCH code part) It can be easily done at the end of set reconciliation, during which two hosts exchange their exclusive elements. In fact, as we will elaborate in \autoref{sec:tail_bound}, Exception 1 hardly happens if we set parameters properly. 

On the other hand, when Exception 2 happens, the BCH decoder will report a failure about exceeding the error-correction capability. For such a subset pair, we can use the same approach as in \autoref{subsec:protocol2} to partition it into smaller subsets and use the straw-man scheme to reconcile them respectively. We set the number of small subsets to be 3. It is because, as we will elaborate in \autoref{sec:tail_bound}, the number of exclusive elements for each subset pair $t$ should be, if not smaller, only slightly larger than $\tau$ w.h.p.. Partitioning those exclusive elements into 3 small subsets is enough to guarentee that each of them has less than $\tau$ exclusive elements.

\end{comment}

==> section/schemes_new0224.tex <==
%\section{PBS for small \texorpdfstring{$d$}{d}}\label{sec:scheme}
\section[PBS for small \texorpdfstring{$d$}{d}]{PBS for small \texorpdfstring{\larger\boldmath\MakeLowercase{$d$}}{d}}\label{sec:scheme}
%\section{Set Reconciliation}\label{sec:scheme}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%     Writing Guideline for This Section     %%%%%%%%%%
% “balls – elements in the symmetric difference of the two sets” 

% Protocol 0 (reconcile two sets whose set difference has at most one ball)

% Protocol I.I (partition elements into a sufficiently large number of subsets such that each subset has at most one ball with high probability and use Protocol 0 to reconcile each of them) 

% Protocol I.II (a two-step refinement of Protocol I.I: first use BCH to identify good bins, i.e., bins/subsets have exactly one ball, and then use Protocol 0 to reconcile each good bin) 

% Protocol II (a two-layer refinement of Protocol I.II: in the first layer, we partition elements into t/c subsets, where t is the size of set difference and c is a small constant, then each subset has c balls on average. In the second layer, we further partition each subset into large enough number of bins/subsets such that with high probability each bin has at most one ball, then use Protocol I.II to reconcile them one by one) 

% Protocol III/IV (mainly fix certain exceptions in Protocol II，e.g., how to address bad bins, how to handle the cases where BCH fails to decode and etc)

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% In this section, we describe our set reconciliation scheme in details. First, we give a formal problem statement in \autoref{sec:model}. In \autoref{subsec:protocol0}, we introduce a basic scheme for the trivial case, in which the two sets $A$ and $B$ has at most one distinct element. Building upon the basic scheme, we propose the preliminary version of scheme in \autoref{sucsec:our-scheme} that targets to the cases where the total number of distinct elements $d$ is small. Then we extend the preliminary version and propose the final version of our scheme in \autoref{subsec:protocol2} for general cases (i.e., any arbitrary $d$). We assume $d$ is precisely known throughout this section except in \autoref{subsec:ToW}, where we will describe how to estimate $d$ using a Tug-of-War Estimator. 


In this section, we describe how PBS scheme allows Alice and Bob to reconcile their respective sets $A$ and $B$, where $d=|A\Delta B|$ is small and precisely known. 
%Throughout this paper, we call each element in $A\Delta B$ a \textit{distinct element}, and each element in $A\bigcap B$ a \textit{common element}. 
We start with the trivial case where $d\leq 1$ in \autoref{subsec:protocol0}. Then we generalize our scheme to a more general case where $d$ is a small number in \autoref{sec:pbs_smalld}. 
% We build up our scheme gradually by starting with the trivial case where $d\leq 1$ in \autoref{subsec:protocol0}. Then we generalize our scheme to the case where $d$ is a small number in \autoref{sec:pbs_smalld}. 

\begin{comment}
\subsection{Problem Statement}\label{sec:model}

In this work, we adopt the commonly used model for the set reconciliation problem. 
Two remote sets $A$ and $B$ are stored at hosts Alice and Bob respectively. 
Each element in $A$ and $B$ is a hash signiture in the key space (universe) $\mathcal{U}$, which is the set of all $(\log |\mathcal{U}|)$-bit binary strings. 
%Each element in $A$ and $B$ is a hash signiture with signiture width $w$ in the key space (universe) $\mathcal{U}$, which is the set of all $w$-bit binary strings (i.e., $|\mathcal{U}|=2^w$). 
%We use $\mathcal{U}$ to denote the set of all $w$-bit binary strings and name it the universe of signitures. 
The set reconciliation problem is to compute the symmetric set difference between $A$ and $B$, 
{\it i.e.,} $A\Delta B\triangleq (A\!\setminus\! B) \bigcup (B\!\setminus\! A)$. 
Let $d\!=\!|A\Delta B|$ be the cardinality of this difference.
%We denote $d\!=\!|A\Delta B|$. 
Throughout this paper, we call each element in $A\Delta B$ a \textit{distinct element}, and each element in $A\bigcap B$ a \textit{common element}.
{\bf Like in all existing solutions, we describe only {\it unidirectional} set reconciliation, in which Alice or Bob learns the set difference $A\Delta B$. Since the performance of our scheme does not depend on who learns the set difference, we assume Bob learns the set difference $A\Delta B$ in the rest of the paper, as mentioned in \autoref{sec:psea}.}
% As mentioned in \autoref{sec:psea}, we describe {\it unidirectional} set reconciliation that Bob learns the set difference $A\Delta B$. 
%In \autoref{sec:evaluation}, we use the same semantic to measure the communication cost of our scheme and other compared set reconciliation schemes. 
\end{comment}

% In the rest of this section, we build up our scheme gradually as follows: We start with the trivial case where $d\leq 1$ in \autoref{subsec:protocol0}. Then we generalize our scheme to the case where $d$ is a small number in \autoref{sec:pbs_smalld}. 

%After that, we further generalize our scheme to the case that $d$ is a large number in \autoref{subsec:protocol2}. 
%Throughout this section, we assume $d$ is precisely known.
%except in \autoref{subsec:ToW}, where we will describe how to estimate $d$ using a Tug-of-War Estimator. 

%The rest of this section is organized as follows: In \autoref{subsec:protocol0}, we introduce a basic scheme for the trivial case, in which the two sets $A$ and $B$ has at most one distinct element. In \autoref{sucsec:our-scheme} and \autoref{subsec:protocol2}, we elaborate the two versions of our solution that are introduced in \autoref{sec:smalld} and \autoref{sec:larged} respectively. Throughout this section, we assume $d$ is precisely known except in \autoref{subsec:ToW}, where we will describe how to estimate $d$ using a Tug-of-War Estimator. 

\subsection{The Trivial Case of \texorpdfstring{\larger\boldmath $d\leqslant 1$}{d<2}}\label{subsec:protocol0}

%We start with the trivial case, in which $A$ and $B$ have at most one distinct element ({\it i.e.,} $d\leq 1$), we have a simple set reconciliation scheme showed in \autoref{alg:trivial_case}:
\begin{algorithm}
\caption{Set reconciliation when $d\le 1$}
\label{alg:trivial_case}

{\it Bob}: $s_B\leftarrow\underset{b\in B}{\oplus} b$; Send $s_B$ to Alice\; \label{alg1:sender}

{\it Alice}: $s_A\leftarrow\underset{a\in A}{\oplus} a$; $s\leftarrow s_A \oplus s_B$\; \label{alg1:receiver}
\end{algorithm}

\autoref{alg:trivial_case} shows the reconciliation scheme for the trivial case, in which $A$ and $B$ differ by at most one distinct element. It consists of two steps. First, Bob calculates $s_B$, the bitwise \code{XOR} of all elements in $B$, and send it to Alice. 
Second, Alice also calculates $s_A$, the bitwise \code{XOR} of all elements of $A$. Upon receiving $s_B$, Alice computes $s\!\triangleq\! s_A \!\oplus\! s_B$. According to whether $A$ and $B$ have a distinct element, there are the following two cases:

\begin{sitemize}
	\item Case \RN{1}: When $A$ and $B$ have no distinct element, we have $s_A=s_B$ and $s=\mathbf{0}$\footnote{$\mathbf{0}$ denotes the $\log |\mathcal{U}|$-bit-long all-0 string.};
	\item Case \RN{2}: When $A$ and $B$ have exactly one distinct element, the computed $s$, the bitwise \code{XOR} of $s_A$ and $s_B$, will cancel out all the {\it common elements}, defined as the elements that are contained by both sets, and only the distinct element remains. In other words, we have $A\Delta B=\{s\}$. 
	%And $s$ is the missing element of $A$ (i.e., $s\in B\!\setminus\! A$) if $s\in B$, or the missing element of $B$ (i.e., $s\in A\!\setminus\! B$) otherwise;
	% \item If $A$ and $B$ has more than one distinct elements (i.e., $d>1$), the bitwise \code{XOR} of $s_A$ and $s_B$ will still cancel out all common elements and remain the \code{XOR} of the distinct elements, i.e., $s$ is the \code{XOR} of all distinct elements;
\end{sitemize}

Like most works on set reconciliation, we assume $\mathbf{0}$ is excluded from $\mathcal{U}$, as \autoref{alg:trivial_case} does not work when $\mathbf{0}\in A\bigcap B$ for the following reason: When $s_A=s_B$ (i.e., $s=\mathbf{0}$), \autoref{alg:trivial_case} cannot tell whether $A$ and $B$ are identical, or they have a distinct element of value $\mathbf{0}$. 
%However, we can extend our scheme to support $\mathbf{0}$. For example, we let Alice send to Bob a single bit to indicate whether Alice has element $\mathbf{0}$, so Bob will know whether $\mathbf{0}\in A\Delta B$ or not. 
\autoref{alg:trivial_case} also does not work when there are more than one distinct elements in $A\Delta B$ (i.e., $d>1$), since the computed $s$ is the \code{XOR} of all these distinct elements.

% Note that \autoref{alg:trivial_case} works if and only if $|A\Delta B|\!\leq\! 1$ and $0\!\notin\! (A\!\cup\! B)$ (which we have explained in~\autoref{sec:model}). 

%\subsection{PBS: When $d$ is small}\label{sucsec:our-scheme}

%In this section, we generalize PBS to the case when $d$ is a small number, as we described in \autoref{sec:smalld}. 
%First, we describe each step of single-round PBS from \autoref{sec:hash_partition} to \autoref{sec:reconcile_by_trivial} and summarize it in \autoref{sec:single_round_pbs}. Second, we discuss the exceptions in single-round PBS in \autoref{subsec:exception_hash_partition}. Third, we propose multi-round PBS to handle the exceptions.

\subsection{PBS for small \texorpdfstring{\larger\boldmath $d$}{d}}\label{sec:pbs_smalld}

In this section, we describe the scheme for a more general case, where $d$ is no longer limited to be no more than $1$, but a small number that is no more than several.
%In this section, we substantiate the scheme described in \autoref{sec:smalld} for small $d$.

\subsubsection{Hash Partition and Parity Bitmap Encoding}\label{sec:hash_partition}
% \medskip
% \noindent{\bf Hash Partition} 

Here we formalize the aforementioned process of partitioning $A$ into $\{A_i\}_{i=1}^n$, $B$ into $\{B_i\}_{i=1}^n$, and $A\Delta B$ into $\{A_i\Delta B_i\}_{i=1}^n$ 
using a hash function $h(\cdot)$.
%as described in \autoref{sec:smalld} by introducing the concept of {\it sub-universes}. Given a hash function $h(\cdot): \mathcal{U}\rightarrow \{1,2,\cdots,n\}$, we 
Define {\it sub-universe} $\mathcal{U}_i$ as the set of elements in the universe $\mathcal{U}$ that are hashed into value $i$. More precisely, $\mathcal{U}_i\triangleq\{s\!\mid\! s\in \mathcal{U} \mbox{ and } h(s)=i\}$ for $i=1,2,...,n$. Then defining $A_i\triangleq A\bigcap\mathcal{U}_i$ and $B_i\triangleq B\bigcap\mathcal{U}_i$ for $i=1,2,...,n$ induces the partitioning of $A$, $B$, and $A\Delta B$.
%, as mentioned in \autoref{sec:smalld}. 

%{\bf (merged from the later two paragraphs)} 
How the $d$ distinct elements (balls) in $A\Delta B$ are distributed into the $n$ subset-pair-differences $\{A_i\Delta B_i\}_{i=1}^n$ (bins) can be viewed as throwing $d$ balls each uniformly and randomly into one of the $n$ bins. 
For the moment, we assume the following {\it ideal case} happens: Every subset-pair-difference $A_i\Delta B_i$ contains at most one distinct element.  
The ideal case corresponds to the $d$ balls ending up in $d$ distinct bins. It happens with probability $\prod_{k=1}^{d - 1}(1 - \frac{k}{n})$, which is on the order of $1-O(d^2/n)$ when $n\!\gg\!d$.
%approximately $e^{-\frac{d(d-1)}{2n}}$ when $d\!\ll\!n$. 
Hence, $n$ must be $\Omega(d^2)$ to ensure the ideal case happens with a nontrivial probability, as mentioned in \autoref{sec:smalld}. 
%The nonideal case of a subset pair difference containing more than $1$ distinct elements will be discussed in \autoref{subsec:exception_hash_partition}.

% {\bf (Previous)} For the moment, we assume the following {\it ideal case} happens: Every subset-pair-difference $A_i\Delta B_i$ contains at most one distinct element. The nonideal case of a subset pair difference containing more than $1$ distinct elements will be discussed in \autoref{subsec:exception_hash_partition}. 

%In this section, we give a detailed description on how to partition $A$ and $B$ (as introduced in \autoref{sec:smalld}) by introducing {\it sub-universes}, which is defined as follows: Given a hash function $h(\cdot): \mathcal{U}\rightarrow \{1,2,\cdots,n\}$, we define {\it sub-universes} $\{\mathcal{U}_i\}_{i=1}^n$, a partition of the universe $\mathcal{U}$, as $\mathcal{U}_i=\{s\!\mid\! s\in \mathcal{U} \mbox{ and } h(s)=i\}$ for $i=1,2,...,n$. Based on $\{\mathcal{U}_i\}_{i=1}^n$, we define $\{A_i\}_{i=1}^n$, the partition of $A$ introduced in \autoref{sec:smalld}, as $A_i\! \triangleq\! A\bigcap \mathcal{U}_i$ for $i=1,2,...,n$. $\{B_i\}_{i=1}^n$ is similarly defined. By this definition, the set difference $A\Delta B$ is partitioned into $n$ set differences of the partitioned subset pairs (i.e., $\{(A_i, B_i)\}_{i=1}^n$). From \autoref{sec:hash_partition} to \autoref{sec:reconcile_by_trivial}, we assume the following {\bf ideal case} happens: Each subset pair $(A_i, B_i)$ contains at most one distinct element ({\it i.e.,} $|A_i\Delta B_i|\!\leq\!1$). The nonideal case of a subset pair contains more than $1$ distinct elements will be discussed in \autoref{subsec:exception_hash_partition}. 

% Here we describe the hash-partition step introduced in \autoref{sec:smalld} in details. First, we use a hash function $h(\cdot): \mathcal{U}\rightarrow \{1,2,\cdots,n\}$ to partition the universe $\mathcal{U}$ into $n$ sub-universes: $\mathcal{U}_i=\{s\!\mid\! s\in \mathcal{U} \mbox{ and } h(s)=i\}$ for $\forall i=1,2,\cdots,n$. The hash function $h(\cdot)$ can be predetermined between Alice and Bob and does not require additional communication cost. Define $A_i\! \triangleq\! A\bigcap \mathcal{U}_i$ and $B_i\! \triangleq\! B\bigcap \mathcal{U}_i$ for $i=1,2,\cdots,n$. Then $\{A_i\}_{i=1}^n$ and $\{B_i\}_{i=1}^n$ are partitions of $A$ and $B$ respectively. Furthermore, $\{A_i\Delta B_i\}_{i=1}^n$ is a partition of $A\Delta B$. From \autoref{sec:hash_partition} to \autoref{sec:reconcile_by_trivial}, we assume the following {\bf ideal case} happens: Each subset pair $(A_i, B_i)$ contains at most one distinct element ({\it i.e.,} $|A_i\Delta B_i|\!\leq\!1$). The nonideal case of a subset pair contains more than $1$ distinct elements will be discussed in \autoref{subsec:exception_hash_partition}. 

% {\bf (Previous)} How the $d$ distinct elements (balls) in $A\Delta B$ are distributed into the $n$ subset pair differences $\{A_i\Delta B_i\}_{i=1}^n$ (bins) 
% can be viewed as throwing $d$ balls each uniformly and randomly into one of the $n$ bins. 

%follows the familiar {\it balls-into-bins} probability model. 
%The distinct elements are viewed as balls and the subset pairs are viewed as bins. 
%Each of the $d$ balls is uniformly and randomly thrown by the hash function $h(\cdot)$ into one of the $n$ bins. 
% The aforementioned ideal case that corresponds to the $d$ balls ending up in $d$ distinct bins happens with probability $\prod_{k=1}^{d - 1}(1 - \frac{k}{n})$, which is on the order of $1-O(d^2/n)$ when $d\!\ll\!n$.
% %approximately $e^{-\frac{d(d-1)}{2n}}$ when $d\!\ll\!n$. 
% Hence, $n$ must be $\Omega(d^2)$ to ensure the ideal case happens with a nontrivial probability, as mentioned in \autoref{sec:smalld}.


%in which the distinct elements are viewed as balls and the subset pairs are viewed as bins. The hash-parition basically throws (hashes) $d$ balls (distinct elements) uniformly and randomly into $n$ bins (subset pairs). The aforementioned ideal case in this context becomes, after throwing $d$ balls uniformly and randomly into $n$ bins, each bin receives at most $1$ ball (i.e., $d$ nonempty bins have $1$ ball in each and the rest $n-d$ bins are empty). The number of balls in each bin is a Binomial random variable $Binomial(d,1/n)$.
%{\bf It may remind readers about the Birthday problem. And the ideal case can be analogous to the case that no people share the same birthday.} 
% The ideal case happens with a probability of $p\!=\!\prod_{k=1}^{d - 1}(1 - \frac{k}{n})\!\approx\! e^{-\frac{d(d-1)}{2n}}$ when $d\!\ll\!n$. In other words, $n$ must be at least $O(d^2)$ to ensure the ideal case happens with a nontrivial probability, as described in \autoref{sec:smalld}.  

% Note that the ideal case does not always happen. However, we can ensure that the ideal case happens with high probability by properly setting $n$ based on $d$ (i.e., $n=\Omega(d^2)$). Furthermore, as we will describe in \autoref{subsec:nonideal}, even if the ideal case does not happen (i.e., some distinct elements are hashed into the same subset pair), most of the distinct elements should be distributed into different subset pairs and therefore can be reconciled. So the scheme, even cannot reconcile all of the distinct elements, can still reconcile the majority of them (i.e., piecewise decodability in \autoref{sec:intro_oursolution}). Based on this property, we will extend our scheme from single-round to multi-rounds in \autoref{subsec:nonideal} to further increase the probability of reconciling all distinct elements. 

% \medskip
% \noindent{\bf Parity Bitmap Encoding} 

{\bf (Modified)} Recall that the partition $\{A_i\}_{i=1}^n$ and $\{B_i\}_{i=1}^n$ can be encoded as $A[1..n]$ and $B[1..n]$ respectively, in which $A[i]$, the $i$-th bit of the parity bitmap $A[1..n]$, is equal to the oddness / evenness (parity) of the cardinality of $A_i$ (i.e., $A[i]=1$ if $|A_i|$ is odd; otherwise $A[i]=0$). $B[i]$, the $i$-th bit of the parity bitmap $B[1..n]$, is similarly defined. In the ideal case, $A[1..n]$ and $B[1..n]$ differ in exactly $d$ distinct bit positions $i_1,i_2,...,i_d$, and each subset-pair-difference $(A_{i_1},B_{i_1}), (A_{i_2},B_{i_2}),...,(A_{i_d},B_{i_d})$ contains exactly $1$ distinct element. If Bob knows $i_1,i_2,...,i_d$, he can start to reconcile the $d$ subset pairs respectively using \autoref{alg:trivial_case}, then Alice will obtain $A\Delta B$.

% {\bf (Modified)} The partition $\{A_i\}_{i=1}^n$ is encoded into an $n$-bit-long parity bitmap $A[1..n]$, in which $A[i]$, the $i$-th bit of the parity bitmap, is equal to the oddness / evenness (parity) of the cardinality of $A_i$ (i.e., $A[i]=1$ if $|A_i|$ is odd; otherwise $A[i]=0$). $B[1..n]$, the parity bitmap of $\{B_i\}_{i=1}^n$, is similarly defined. In the ideal case, $A[1..n]$ and $B[1..n]$ differ in exactly $d$ distinct bit positions $i_1,i_2,...,i_d$, and each subset-pair-difference $(A_{i_1},B_{i_1}), (A_{i_2},B_{i_2}),...,(A_{i_d},B_{i_d})$ contains exactly $1$ distinct element. If Bob knows $i_1,i_2,...,i_d$, he can start to reconcile the $d$ subset pairs respectively using \autoref{alg:trivial_case}, then Alice will obtain $A\Delta B$.

{\bf (Previous)} We encode $\{A_i\}_{i=1}^n$ into an $n$-bit-long parity bitmap $A[1..n]$, in which $A[i]$, the $i^{th}$ bit of the parity bitmap, is equal to the oddness / evenness (parity) of the cardinality of $A_i$ (i.e., $A[i]=1$ if $|A_i|$ is odd; otherwise $A[i]=0$). In the ideal case, the two bitmaps $A[1..n]$, $B[1..n]$ differ in exactly $d$ bit positions $i_1,i_2,...,i_d$, each of which corresponds to a subset pair that contains $1$ distinct element. The next step is to let Alice and Bob know these bit positions.
%Once the $d$ bit positions are known, Alice and Bob can start to reconcile $(A_{i_1},B_{i_1}), (A_{i_2},B_{i_2}),...,(A_{i_d},B_{i_d})$ using \autoref{alg:trivial_case} and obtain the $d$ distinct elements (i.e., $A\Delta B$). 

% \subsubsection{Parity Bitmap Encoding}\label{sec:parity_bitmap_encoding}

% %After hash-partitioning $A$ and $B$ into partitions $\{A_i\}_{i=1}^n$ and $\{B_i\}_{i=1}^n$, 
% As introduced in \autoref{sec:smalld}, we encode each partition into an $n$-bit-long parity bitmap and denote them as $A[1..n]$ and $B[1..n]$ respectively, as introduced in \autoref{sec:smalld}. For $i=1,2,...,n$, $A[i]$ (the $i^{th}$ bit of the parity bitmap $A[i]$) is equal to $1$ if $A_i$ contains an odd number of elements, and is equal to $0$ otherwise.
% % More specifically, for $i=1,2,...,n$, $A[i]$ (the $i^{th}$ bit of the parity bitmap $A[i]$) is defined as follows: $A[i]=1$ if $A_i$ contains an odd number of elements, and $A[i]=0$ otherwise. In this way, each bit $A[i]$ encodes the oddness / evenness (parity) of the cardinality of $A_i$. The $n$-bit-long parity bitmap $B[1..n]$ and $B[i]$ (the $i^{th}$ bit of $B[1..n]$) are similarly defined. 
% In the ideal case, 
% %$A[i]$ and $B[i]$ differ if and only if $A_i$ and $B_i$ have exactly $1$ distinct element, and $A[i]$ and $B[i]$ are the same if and only if $A_i=B_i$. Meanwhile, the $d$ distinct elements are hashed into $d$ different subset pairs. So 
% the two bitmaps $A[1..n]$, $B[1..n]$ differ in exactly $d$ bit positions, each of which corresponds to a subset pair that contains $1$ distinct element. Once the $d$ bit positions are known, Alice starts to reconcile each of the $d$ corresponding subset pairs by \autoref{alg:trivial_case} and gets the $d$ distinct elements (i.e., $A\Delta B$). 
% %If knowing the $d$ bit positions (i.e., the $d$ corresponding subset pairs), we can use \autoref{alg:trivial_case} to reconcile the $d$ subset pairs respectively to obtain all the $d$ distinct elements (i.e., $A\Delta B$). 
% In \autoref{sec:BCH_code}, we will describe how to find the $d$ bit positions using BCH code~\cite{Lint_IntroductionCodingTheory_1998}. 

% \medskip
% \noindent{\bf Find the $d$ Bit Positions Using ECC} 

%\subsubsection{Find the $d$ Bit Positions Using ECC}\label{sec:BCH_code}
\subsubsection{Find and Reconcile the \texorpdfstring{$d$}{d} subset pairs}\label{sec:BCH_code}

{\bf (Modified)} In the ideal case, for Bob to obtain $i_1,i_2,...,i_d$, Alice only needs to send $\xi_A$, the BCH code of $A[1..n]$, that can ``correct'' these $d$ bit errors in $B[1..n]$. Then Bob can decode and recover $A[1..n]$ (original message) and obtain $i_1,i_2,...,i_d$.

{\bf (Previous)} We view $A[1..n]$ as a corrupted message of $B[1..n]$ sent ({\bf not actually being sent}) from Bob to Alice through an {\it unreliable} commnunication channel that flips $d$ bits. To locate these $d$ bit positions, we let Bob also send an {\it error-correction code} that encodes $B[1..n]$ to Alice, such that Alice can recover $B[1..n]$ (original message) and obtain the $d$ bit positions $i_1,i_2,...,i_d$. In PBS, we use BCH code~\cite{bch1} to encode $B[1..n]$ and get the error-correction code.

There are two different BCH encoding techniques: {\it systematic} and {\it unsystematic}. The difference is that, the message appears as the prefix of the codeword (i.e., codeword = [message net-codeword]) in systematic BCH encoding, whereas it does not appear as a substring of the codeword in unsystematic BCH encoding. In PBS, we choose systematic BCH encoding because we are sending not the ``message'', but the net-codeword. 
%To correct $d$ bit errors, the length of the net-codeword only is no more than $d\log n$ bits. 
Without causing any ambiguity, we use the term `codeword' to refer to the net-codeword in the rest of this paper.
%The computational complexity of the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} is $O(d^2\log^2 n)$.

%The systematic BCH encoding is also used in other ECC-based set reconciliation works, such as PinSketch \cite{Wuille_Minisketchoptimizedlibrary_2019}, while PinSketch encodes a much longer message (e.g., $2^{32}$ bits) than in ours (hundreds of bits).  

%\subsubsection{Find the $d$ Bit Positions Using ECC}\label{sec:BCH_code}

% A straightforward approach to find the $d$ bit positions is to let Bob send the complete parity bitmap $B[1..n]$ to Alice, then Alice compares $A[1..n]$ with $B[1..n]$ locally. This approach has a communication overhead of $n$ bits, which is quite wasteful. As we discussed in~\autoref{sec:hash_partition}, $d$ is usually much smaller than $n$. It means $A[1..n]$ and $B[1..n]$ differ only at a tiny portion of bits. Therefore, we can view $A[1..n]$ as a corrupted message of $B[1..n]$ with $d$ bit errors, and the bit positions of the $d$ bit errors basically correspond to the $d$ subset pairs that contain distinct elements. The detection of bit errors, on the other hand, can be solved by Error-Correction Code (ECC)~\cite{Lin_ErrorControlCoding_1983}. 

% Since $A[1..n]$ and $B[1..n]$ differ at $d$ bit positions, we can view $A[1..n]$ as a corrupted message of $B[1..n]$ from Bob to Alice through an {\it unreliable} commnunication channel with $d$ corrupted bits, which are located on the $d$ bit positions. Therefore, to find the $d$ bit position, we only need to correct the $d$ corrupted bits in $A[1..n]$, which is done by transmitting a ``code'' that can correct upto $d$ bit errors from Bob to Alice through a {\it reliable} communication channel. 

% In PBS, we use {\it systematic} BCH code to generate the ``code'' by encoding the message $B[1..n]$. The codeword of the systematic BCH code is in the form of [message, net-codeword], since the message appears as the prefix of the codeword in systematic BCH code. The ``code'' is simply the net-codeword in the BCH codeword. We choose {\it systematic} BCH code because the (corrupted) message is already transmitted and we only need to pay a small communication overhead on transmitting ``code'' (i.e., net-codeword). To correct upto $d$ bit errors, the length of the net-codeword is no more than $d\log n$ bits, which is much smaller than the message when $d\!\ll\! n$. The computational complexity of the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} is $O(d^2\log^2 n)$. This type of BCH code is also used in other ECC-based set reconciliation works, such as PinSketch \cite{Wuille_Minisketchoptimizedlibrary_2019}. 

% Different from {\it unsystematic} BCH code
% The ``code'' is generated by {\it systematic} BCH code, which encodes the message $B[1..n]$ into a BCH codeword in the form of [message, net-codeword]. The ``code'' transmitted on the reliable channel is the net-codeword of the BCH codeword. In {\it systematic} BCH code, the message appears as the prefix of the codeword. 

% More specifically, PBS uses {\it systematic} BCH code~\cite{Lint_IntroductionCodingTheory_1998} that can correct upto $d$ bit errors to encode the parity bitmaps. In the {\it systematic} BCH code \footnote{In unsystematic BCH code, message does not appear to be the prefix of the codeword}, the message (i.e., the parity bitmap) appears as the prefix of the raw codeword, which in the form of [message, net codeword]. Normally, to correct upto $d$ errors, the length of the net codeword is $2n\log d$, where $n$ is the length of the message (i.e., parity bitmap). However, our case is special in the sense that the net codeword is error-free (all $d$ bit errors are in the message), so the length of the net codeword can be reduced to $n\log d$. This type of BCH code is also used in other ECC-based set reconciliation works, such as PinSketch \cite{Wuille_Minisketchoptimizedlibrary_2019}. 

% Now we can formally describe how to find the $d$ bit positions: First, Bob uses a $d$-error-correcting systematic BCH code to encode $B[1..n]$ and sends the net codeword ($d\log n$ bits) to Alice. Upon receiving the net codeword and combining it with the corrupted message $A[1..n]$, Alice uses the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} to decode the $d$ bit errors in $A[1..n]$. The communication overhead of transmitting the net codeword is $d\log n$ bits. The computational complexity of the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} is $O(d^2\log^2 n)$. Both the communication overhead and the computational complexity here are relatively small when $d$ is small.

% \medskip
% \noindent{\bf Reconcile the $d$ subset pairs using \autoref{alg:trivial_case}} 

%Once the $d$ bit positions are known, Alice can start to reconcile $(A_{i_1},B_{i_1}), (A_{i_2},B_{i_2}),...,(A_{i_d},B_{i_d})$ using \autoref{alg:trivial_case} and obtain the $d$ distinct elements (i.e., $A\Delta B$). 
Once Bob decodes the codeword to obtain $i_1,i_2,...,i_d$, the corresponding subset pairs $(A_{i_1},B_{i_1})$, $(A_{i_2},B_{i_2})$, $...$, $(A_{i_d},B_{i_d})$ each can be reconciled using \autoref{alg:trivial_case}. To do so, Bob needs to send the respective \code{XOR} sums of the subsets $B_{i_1}$, $B_{i_2}$,$...$,$B_{i_d}$ to Alice (\autoref{alg1:sender} in \autoref{alg:trivial_case}). In addition, Bob needs to send $i_1,i_2,...,i_d$ to Alice, since Alice does not know the ``bit error positions'' yet. Each ``bit error position'' corresponds to the index of the corresponding subset pair, which needs to be encoded into $\log n$ bits, so the additional communication overhead on transmitting these indices is $d\log n$ bits. 
% When reconciling $(A_{i_1},B_{i_1}), (A_{i_2},B_{i_2}),...,(A_{i_d},B_{i_d})$ using \autoref{alg:trivial_case}, Alice needs to send not only the bitwise \code{XOR} of $A_{i_1}, A_{i_2},..., A_{i_d}$, but also the indices of the subset pairs ($i_1,i_2,...,i_d$), since Bob does not know which of the $d$ subset pairs are being reconciled. Each index is an integer between $1$ and $n$ and can be encoded into $\log n$ bits, So the additional communication overhead on transmitting the indices is $d\log n$ bits. 



% \subsubsection{Reconcile the $d$ subset pairs using \autoref{alg:trivial_case}}\label{sec:reconcile_by_trivial}

% After decoding the $d$ bit errors that corresponds to the $d$ subset pairs, Alice starts to reconcile them using \autoref{alg:trivial_case}. For each of the $d$ subset pairs, Alice needs to send not only the bitwise \code{XOR} of the subset pair, but also the index of the subset pair (since Bob does not know the $d$ subset pairs to reconcile). So the communication overhead on \autoref{alg:trivial_case} is $d\log |\mathcal{U}|+d\log n$ bits. 
%Plus the communication overhead on transmitting the net codeword of parity bitmap ($d\log n$, as we explained in \autoref{sec:BCH_code}), the overall communication overhead of single-round PBS is $d\log u+2d\log n$ bits.

% \medskip
% \noindent{\bf Check if set reconciliation is complete} 

Once Alice receives the \code{XOR} sums and the indices, she can compute the distinct elements, as described in \autoref{subsec:protocol0}, to obtain the set difference (denoted as $\hat{D}$). However, this reconciled set difference could be incorrect if the ideal case does not happen. Therefore, Alice needs to check if set reconciliation is successfully completed (or whether $\hat{D}=A\Delta B$). To do so, we introduce some ``linear'' checksum function $c(\cdot)$ that maps any subset of the universe $\mathcal{U}$ (such as $A$ and $B$) to a $32$-bit checksum (e.g., bitwise \code{XOR}). Here the ``linearity'' of a chechsum function refers to the fact that $c(S_1\Delta S_2)=c(S_1)\oplus c(S_2)$ for any two subsets $S_1$ and $S_2$ of the universe $\mathcal{U}$. We use this checksum function to check if $\hat{D}=A\Delta B$ by comparing $c(\hat{D})$ to $c(A\Delta B)$. Note that $c(\hat{D})$ can be computed in $O(d)$ time and $c(A\Delta B)=c(A)\oplus c(B)$ can be precomputed {\bf during the encoding period, which costs $32$ bits of communication overhead on transmitting $c(B)$ from Bob to Alice. In PBS, we select {\it longitudinal parity check}, the bitwise \code{XOR} of all elements (recall each element is a $32$-bit-long binary string) in the set, as the checksum function. It is not hard to verify it is linear.}  

% {\bf (Previous)} After reconciling the subset pairs and obtaining the reconciled set difference (denoted as $\hat{D}$), PBS needs to check if set reconciliation is complete (or whether $\hat{D}=A\Delta B$), since the reconciled set difference $\hat{D}$ is not the actual set difference $A\Delta B$ in the nonideal case (to be discussed in \autoref{subsec:exception_hash_partition}). Hence, we add a verfication step after obtaining $\hat{D}$ to check if $\hat{D}=A\Delta B$. In PBS, we check an equivalent condition, $A=B\Delta\hat{D}$, instead of $\hat{D}=A\Delta B$, since $B$ and $\hat{D}$ are both known by Bob and their set difference $B\Delta\hat{D}$ can be locally computed. More specifically, to check if the remote sets $A$ and $B\Delta\hat{D}$ are equal, we let Alice compute a $32$-bit checksum of $A$ and send it to Bob. {\bf Then Bob computes the $32$-bit checksum of $B\Delta\hat{D}$ using the same checksum algorithm and compare the two checksums. In PBS, we select {\it longitudinal parity check} (i.e., bitwise \code{XOR} of all elements in the set) as the checksum algorithm, so that the checksum $B\Delta\hat{D}$ can be efficiently computed as the bitwise \code{XOR} between the checksum of $B$ (can be pre-computed) and that of $\hat{D}$. Other checksum algorithms that are {\it linear} to the set difference operator (i.e., $\Delta$) also work for PBS. }
% Then Bob checks if $B\Delta\hat{D}$ satisfies the receiving checksum. 

The condition $\hat{D}=A\Delta B$ can be almost surely verified by the checksum, 
{\bf although it could mistakenly believes two different sets as identical ones.} This event happens with probability $2^{-32}\approx 2.3\times 10^{-10}$ when the ideal case does not happen, {\bf which has a probability on the order of $10^{-2}$.} Although this event could cause PBS mistakenly believes the set reconciliation is completed, it happens with an extremely small probability (on the order of $10^{-12}$) and should be acceptable in most applications. In few applications which allow no room for error ({\it e.g.,} Bitcoin), additional techniques such as Merkle tree~\cite{merkle87} based validation will be used to verify the correctness of the results anyway. 
%If such techniques find out that the set reconciliation is not completed, we could simply start it over and use PBS to reconcile the two sets again under a different hash function $h$. In this case, the checksum will be different If so, the  (note that PBS is a `randomized' algorithm when assuming the hash functions for hash-partition are random hash functions). 
To simplify our description, we ignore this small probability event and assume the checksum works perfectly in this rest of this paper. We summarize all the above steps of PBS (in the first round) in \autoref{alg:single_round_pbs}.
%{\bf not a good position to mention `for super critical applications, use a checksum for all groups', since we are describing single-group scenario. }

\begin{algorithm}
\caption{Single-round PBS}
\label{alg:single_round_pbs}

%Hash-partition $A$, $B$ into $\{A_i\}_{i=1}^n$, $\{B_i\}_{i=1}^n$\; \label{step:hash_partition}

%Parity encode $\{A_i\}_{i=1}^n$, $\{B_i\}_{i=1}^n$ into $A[1..n]$, $B[1..n]$\; \label{step:parity_encode}
{\it Alice}: Send $\xi_A$, the BCH codeword of $A[1..n]$, to Bob\; \label{step:BCH_encode}

{\it Bob}: Decode $(B[1..n], \xi_A)$ to obtain $i_1,i_2,...,i_d$\; \label{step:BCH_decode}

{\it Bob}: Send the \code{XOR} sums of sets $B_{i_1}, B_{i_2},...,B_{i_d}$ (\autoref{alg1:sender} in \autoref{alg:trivial_case}) and $i_1,i_2,...,i_d$ to Alice\; \label{step:BCH_decode}

{\it Alice}: Obtain $A_{i_1}\Delta B_{i_1}, A_{i_2}\Delta B_{i_2},...,$ and $A_{i_d}\Delta B_{i_d}$ (\autoref{alg1:receiver} in \autoref{alg:trivial_case}); $\hat{D}\leftarrow \bigcup_{k=1}^d (A_{i_k}\Delta B_{i_k})$\; \label{step:trivial_reconcile}

{\it Alice}: Check if $c(\hat{D})=c(A\Delta B)$\; \label{step:terminate_condition}

\end{algorithm}
% {\color{blue}This probability is low enough for most applications. In few applications which allow no room for error ({\it e.g.,} Bitcoin), additional techniques such as Merkle tree~\cite{merkle87} based validation will be used to verify the correctness of the results anyway.}

% {\bf (Previous)} The condition $A=B\Delta\hat{D}$ can be almost surely verified by a $32$-bit checksum, although it could mistakenly believe two different sets as identical ones with probability $2^{-32}\approx 2.3\times 10^{-10}$ {\bf on top of the probability that the nonideal case happens (on the order of $10^{-2}$).} Although this event could cause an ``early'' termination and leave some distinct elements unreconciled, it happens with an extremely small probability (on the order of $10^{-12}$) and should be acceptable in most applications. {\bf To simplify our description, we ignore this small probability event and assume the checksum works perfectly in this rest of this paper. }
%and such an event (i.e., mistaken $A$ and $B\Delta\hat{D}$ are identical when they are different) never happens in our evaluation. For some super critical applications, we can certainly use a $64$-bit checksum to reduce this probability to $5.4\times 10^{-20}$ if needed.

% When the ideal case does not happen, set reconciliation cannot accomplish in one round, as we will explain in \autoref{subsec:exception_hash_partition}. Hence, we add a verfication step to check if set reconciliation is complete. Let $\hat{D}$ denote the set of reconciled elements. The idea of this verification is basically to compare $A$ with $B\Delta \hat{D}$: If $A=B\Delta \hat{D}$ (i.e., $\hat{D}=A\Delta B$), we know the set reconciliation is complete; Otherwise, the set reconciliation is incomplete.  using a $32$-bit checksum. 

\subsubsection{Communication overhead of PBS (First Round)}\label{sec:communication_overhead_single_PBS}

%To correct $d$ bit errors, the length of the net-codeword only is no more than $d\log n$ bits. 

The communication overhead of \autoref{alg:single_round_pbs} consists of four components: (1) the BCH codeword $\xi_A$ in \autoref{step:BCH_encode}; (2) the subset pair indices $i_1,i_2,...,i_d$ in \autoref{step:trivial_reconcile}; (3) the bitwise \code{XOR} sums of sets $B_{i_1}, B_{i_2},...,B_{i_d}$ of $d\log |\mathcal{U}|$ bits in \autoref{step:trivial_reconcile}; and (4) transmit the $32$-bit checksum of $B$ (i.e., $c(B)$) from Bob to Alice for precomputing $c(A\Delta B)$ in \autoref{step:terminate_condition}. These four components contribute (1) $d\log n$ bits (recall that to ``correct'' $d$ bit errors, the length of the BCH codeword is no more than $d\log n$ bits); (2) $d\log n$ bits; (3) $d\log |\mathcal{U}|$ bits; and (4) $32$ bits respectively to the overall communcation overhead of \autoref{alg:single_round_pbs}.

% All the steps of PBS in the first round are summarized in \autoref{alg:single_round_pbs}. The overall communication overhead consists of three components: (1) the BCH codeword of $d\log n$ bits in \autoref{step:BCH_encode}; (2) the subset pair indices $i_1,i_2,...,i_d$ and the corresponding bitwise \code{XOR}s of $d\log n+d\log |\mathcal{U}|$ bits in \autoref{step:trivial_reconcile}; and (3) the $32$-bit checksum of $A$ in \autoref{step:terminate_condition}. 


% {\it Bob}: BCH-Encodeing $B[1..n]$ and send the codeword to Alice\; \label{step:BCH_encode}

% {\it Alice}: Upon receiving the codeword, decode the bit errors between $A[1..n]$ and $B[1..n]$\; \label{step:BCH_decode}

% {\it Alice}: For each bit error, start reconciling the corresponding subset pair by \autoref{alg:trivial_case}\; \label{step:trivial_reconcile}

% {\it Bob}: Upon receiving the reconciled set difference $\hat{D}$, check if $A=B\Delta \hat{D}$ via checksum\; \label{step:terminate_condition}


% \subsubsection{Single-round PBS}\label{sec:single_round_pbs}

% Here we summarize all the steps of single-round PBS and represent it by pseudocode in \autoref{alg:single_round_pbs}. \autoref{step:hash_partition} and \autoref{step:parity_encode} operates at both hosts (i.e., Alice and Bob). \autoref{step:hash_partition} to \autoref{step:trivial_reconcile} have been elaborated from \autoref{sec:hash_partition} to \autoref{sec:reconcile_by_trivial}. The last step in \autoref{step:terminate_condition} aims to check whether reconciliation is complete (i.e., $\mathcal{D}=A\Delta B$). More specifically, Alice calculates the checksum (e.g., CRC-$32$) of $A$ and send it to Bob. Then Bob calculates the checksum of $B\Delta \mathcal{D}$ and compares it to the receiving checksum of $A$. If the two checksums are the same, we believe $A=B\Delta \mathcal{D}$ and therefore $\mathcal{D}=A\Delta B$ (i.e., reconciliation is complete); Else, we know some elements are reconciled incorrectly. We classify those elements (i.e., the ones in the set difference between $A\Delta B$ and $\mathcal{D}$) into two subsets $A\Delta B\!\setminus\!\mathcal{D}$ and $\mathcal{D}\!\setminus\!(A\Delta B)$ and refer the elements in the former as {\it false-negatives}, and refer the elements in the later as {\it false-positives}. 

% In the ideal case, neither false-positives nor false-negatives will happen and the two checksums always equal. However, in real life, the ideal case does not always happen. We will discuss the nonideal case in \autoref{subsec:exception_hash_partition}. In our evaluation, we use a $32$-bit checksum for comparing $A$ to $B\Delta \mathcal{D}$ that has {\bf an error probability} roughly $10^{-9}$. This error (i.e., mistake $A=B\Delta \mathcal{D}$) incurs false-negatives. All set reconciliation schemes have the same problem on their termination conditions (i.e., check whether $\mathcal{D}=A\Delta B$). For some super critical applications, we can certainly decrease the error probability by using more powerful checksums (i.e., $64-$bit). Using a $32$-bit checksum, this kind of false-negatives never happen in the evaluation. 
% %For simplification, we assume no error happens when checking $\mathcal{D}=A\Delta B$ in the rest of the paper.

% \begin{algorithm}
% \caption{Single-round PBS}
% \label{alg:single_round_pbs}

% Hash-partition $A$, $B$ into $\{A_i\}_{i=1}^n$, $\{B_i\}_{i=1}^n$\; \label{step:hash_partition}

% Parity encode $\{A_i\}_{i=1}^n$, $\{B_i\}_{i=1}^n$ into $A[1..n]$, $B[1..n]$\; \label{step:parity_encode}

% {\it Bob}: Encode $B[1..n]$ by BCH code, then send the codeword to Alice\; \label{step:BCH_encode}

% {\it Alice}: Upon receiving the codeword, decode the bit errors between $A[1..n]$ and $B[1..n]$\; \label{step:BCH_decode}

% {\it Alice}: For each bit error, reconcile the corresponding subset pair by \autoref{alg:trivial_case}\; \label{step:trivial_reconcile}

% {\it Bob}: Upon the reconciled distinct elements $\mathcal{D}$, check whether $A=B\Delta \mathcal{D}$ via checksum\; \label{step:terminate_condition}
% \end{algorithm}

\subsubsection{Exception Handling}\label{subsec:exception_hash_partition}

When the ideal case does not happen, some subset pair may contain more than $1$ distinct elements and cannot be successfully reconciled by \autoref{alg:trivial_case}. We can classify the possible exceptions that happen in such a subset pair into the following two types of events: 

\noindent {\bf Type (\RN{1}) event}: Subset pair $(A_i, B_i)$ contains a nonzero even number of distinct elements, the parity bits of $A_i$ and $B_i$ are the same. So the BCH code $\xi_A$ cannot detect it and PBS will not reconcile the subset pair yet in this round. This event happens with a small but nontrivial probability: For example, when $d=5$ and $n=255$ (i.e., throwing $5$ balls each uniformly and randomly into $255$ bins), the probability that some bin has a nonzero even number of (in this case either $2$ or $4$) balls is roughly $0.04$. 
%Note that when a type (\RN{1}) event happens, the checksum (\autoref{step:terminate_condition} in \autoref{alg:single_round_pbs}) can detect that the set reconciliation has not been completed. Then PBS will start another round to reconcile the ``hidden'' distinct elements (the ones that have not been reconciled in this round), 
%so on so force, until all distinct elements are successfully reconciled and the checksum is verified to be correct, 
%as we will describe in \autoref{sec:multi-rounds}. 

% Note that when a Type (\RN{1}) subset pair exists, the $32$-bit checksum (\autoref{step:terminate_condition} in \autoref{alg:single_round_pbs}) can almost surely detect that the set reconciliation is incomplete. If this is the case (i.e., the checksum is verified to be incorrect), PBS will start another round of set reconciliation to reconcile the remaining distinct elements (e.g., the ``hidden'' distinct elements in Type (\RN{1}) subset pairs), so on so force, until all distinct elements are reconciled and the checksum is verified to be correct, as we will describe in \autoref{sec:multi-rounds}. 

\noindent {\bf Type (\RN{2}) event}: Subset pair $(A_i, B_i)$ contains distinct elements whose quantity is an odd number no less than $3$, the parity bits of $A_i$ and $B_i$ will be different and PBS will reconcile the subset pair using \autoref{alg:trivial_case}. The reconciled element $s$ is however the bitwise \code{XOR} of all distinct elements in $(A_i, B_i)$ (explained in \autoref{subsec:protocol0}), which is a ``fake'' distinct element.
%, which will be mistakenly believed as the distinct element of $(A_i, B_i)$. 
This event happens with a tiny probability: In the same example above ($d=5$ and $n=255$), the probability that some bin has an odd number of balls that is no less than $3$ (in this case $3$ or $5$) is only $1.52\times 10^{-4}$. 
%Similarly, the $32$-bit checksum can also detect that the set reconciliation has not been completed when a type (\RN{2}) event happens. Both the ``hidden'' and the ``fake'' distinct elements can also be reconciled in later rounds. 

%Note that those ``fake'' distinct elements will become new distinct elements in the next round and therefore incur additional communication overhead to reconcile. 
%Note that those ``fake'' distinct elements will incur additional communication overhead if we want to reconcile them ``later''. Therefore, we add a verification on each reconciled distinct element of \autoref{alg:trivial_case} that can detect ``fake'' distinct elements with high probability. \autoref{alg:verification} shows how this verification works, and it does not incur additional communication overhead.

Note that the nature of hash-partition provides us an approach that can detect ``fake'' distinct elements with high probability. This approach only needs to locally verify the reconciled elements of \autoref{alg:trivial_case} and does not incur any additional overhead. \autoref{alg:verification} shows how this verification works.

\begin{algorithm}
\caption{Verify reconciled element $s$ of $(A_i, B_i)$}
\label{alg:verification}
\If{$h(s)\neq i$} {Discard the reconciled element $s$;}
\end{algorithm}

Although a distinct element of $(A_i, B_i)$ must be in sub-universe $\mathcal{U}_i$ (i.e., the hash value of the element under $h$ equals to $i$), a ``fake'' distinct element could be in any sub-universe with probability $1/n$, since it is the bitwise \code{XOR} of multiple distinct elements of $(A_i, B_i)$. Therefore, \autoref{alg:verification} only fails to identify a ``fake'' distinct element with probability $1/n$, which is roughly $3.9\times 10^{-3}$ when $n=255$, under the condition that the type (\RN{2}) event happens, which also has a tiny probability as we explained earlier. In the same example above ($d=5$ and $n=255$), a ``fake'' distinct element that fails to be detected by \autoref{alg:verification} happens with a tiny probability of $6\times 10^{-7}$, which is the multiplication of the probability of the type (\RN{2}) event ($1.52\times 10^{-4}$) and the probability of \autoref{alg:verification} fails ($3.9\times 10^{-3}$). 
%{\bf (removed to the beginning of theoretical analysis) To simplify our description, we also ignore this small probability event and assume all ``fake'' distinct elements will be successfully detected by \autoref{alg:verification} in this rest of this paper. }

Note that either a type (\RN{1}) event or a type (\RN{2}) event will cause PBS fails to reconcile all distinct elements, which can be detected by the checksum (\autoref{step:terminate_condition} in \autoref{alg:single_round_pbs}). In this case, PBS will continue to reconcile the ``rest'' of distinct elements using additional rounds. 
%In this case, PBS will continue to reconcile the ``remaining'' distinct element by starting another round, as we will describe in \autoref{sec:multi-rounds}. The ``remaining'' distinct elements here consist of (1) the ``hidden'' distinct elements that have not been reconciled in this round and (2) the ``fake'' distinct elements that are not verified by \autoref{alg:verification}.

% {\bf (to be removed) Readers may wonder encoding the exact subset cardinalities (i.e., $|A_i|, |B_i|$) instead of their oddness / evenness (parity) (described in \autoref{sec:hash_partition}) could help to detect and solve Type (\RN{1}), (\RN{2}) events. However, encoding the exact subset cardinalities not only incurs much more additional communication overhead comparing to encoding their parities, but also barely helps on detecting Type (\RN{1}), (\RN{2}) events, since we cannot precisely derive $|A_i\Delta B_i|$, the total number of distinct elements in $(A_i, B_i)$, even knowing $|A_i|, |B_i|$: For instance, when $|A_i|\!=\!|B_i|\!=\!50$, $|A_i\Delta B_i|$ could be any even number ($\leq 100$) if the distinct elements are evenly splitted and placed between $A_i$ and $B_i$. }

% As we have described in \autoref{sec:hash_partition}, the ideal case does not always happen, which means some subset pair may contain more than $1$ distinct elements and cannot be successfully reconciled by \autoref{alg:trivial_case}. Due to the parity encoding, we can classify such subset pair into the following two scenarios:

% \begin{itemize}
%     \item Scenario 1: If a subset pair $(A_i, B_i)$ contains even number ($\geq 2$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be the same and PBS will not reconcile the subset pair yet in this round;
%     \item Scenario 2: If a subset pair $(A_i, B_i)$ contains odd number ($\geq 3$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be different and PBS will reconcile the subset pair using \autoref{alg:trivial_case}. The reconciled element (i.e., $s$ in \autoref{alg:trivial_case}) is however the bitwise \code{XOR} of all distinct elements in $(A_i, B_i)$ (explained in \autoref{subsec:protocol0}), which will be mistakenly believed as the distinct element of $(A_i, B_i)$. 
%     %However, as described in \autoref{subsec:protocol0}, when a subset pair contains more than $1$ distinct elements, \autoref{alg:trivial_case} will output the bitwise \code{XOR} of them as the `distinct element', which is not an actual distinct element with high probability;
% \end{itemize}

% In both scenarios, the distinct elements in the subset pair will not be reconciled in this round. As we will describe in \autoref{sec:multi-rounds}, we generalize PBS into multi-round, so that the distinct elements that have not been reconciled in the first round will be reconciled in later rounds. On the other hand, the second scenario could result in incorrectly reconciled distinct elements, which will become new distinct elements in the next round in multi-round PBS. 

% % In both scenarios, the distinct elements in the subset pair cannot be successfully reconciled in this round and will remain in the set difference (i.e., $(A\Delta B)\!\setminus\!\hat{D}$). On the other hand, the incorrectly reconciled distinct element in the second scenario will appear as a new distinct element (i.e., $\hat{D}\!\setminus\!(A\Delta B)$) in the next round if we generalize PBS into multi-round (to be elaborated in \autoref{sec:multi-rounds}). Both scenarios can be almost surely detected by the 32-bit checksum (\autoref{step:terminate_condition} in \autoref{alg:single_round_pbs}). The set difference after the reconciliation in this round, $D\Delta\hat{D}$, can be reconciled in later rounds, as we will describe in \autoref{sec:multi-rounds}. 

% Naturally, we do not want to generate new distinct elements in the process of set reconciliation, even though it happens with a tiny probability when $n=\Omega(d^2)$: For instance, when $d=5$ and $n=255$ (i.e., throwing $5$ balls uniformly and randomly into $255$ bins), the probability (i.e., some bin has $3$ or $5$ balls) is only $7.6\times 10^{-6}$. Therefore, we add a verification with no additional communication cost on each reconciled element of \autoref{alg:trivial_case}, such that each incorrect dinstinct element can be identified with high probability. The verfication is shown in \autoref{alg:verification}. 

% \begin{algorithm}
% \caption{Verify reconciled element $s$ of $(A_i, B_i)$}
% \label{alg:verification}
% \If{$h(s)\neq i$} {Discard the reconciled element $s$;}
% \end{algorithm}

% Although any distinct element of $(A_i, B_i)$ must be in sub-universe $\mathcal{U}_i$ (i.e., the hash value of the element under $h$ equals to $i$), the bitwise \code{XOR} of multiple distinct elements of $(A_i, B_i)$ could be in any sub-universe with probability $1/n$. Therefore, \autoref{alg:verification} fails to identify an incorrectly reconciled distinct element in the second scenario with probability $1/n$ that is roughly $3.9\times 10^{-3}$ when $n=255$. In other words, an incorrectly reconciled distinct element that cannot be identified by \autoref{alg:verification} appears with probability $3\times 10^{-8}$. {\bf I feel that defining $\tilde{a}_4=a_1\oplus a_2\oplus a_3$ does not help much.}

% In both scenarios, the distinct elements in the subset pair cannot be successfully reconciled in this round. These distinct elements can be reconciled in later rounds if needed, as we will describe in \autoref{sec:multi-rounds}. In this section, we only discuss how to identify the {\it incorrect} distinct element in the second scenario. Let us use an example to elaborate the second scenario: Assume $(A_i, B_i)$ contains $3$ distinct elements $a_1, a_2, a_3$, then Bob computes $\tilde{s}=a_1\oplus a_2\oplus a_3$ using \autoref{alg:trivial_case} and mistakes it as the distinct element in $(A_i, B_i)$. 

% In both scenarios, the distinct elements in the subset pair cannot be successfully reconciled (i.e., false-negatives defined in \autoref{sec:single_round_pbs}. The distinct elements that are not successfully reconciled in this round, if needed, can be reconciled in later rounds as we will describe in \autoref{sec:multi-rounds}. In this section, we only discuss how to identify the {\it incorrect} distinct elements in the second scenario. Let us use an example to elaborate the second scenario: Assume $(A_i, B_i)$ contains $3$ distinct elements $a_1, a_2, a_3$, then Bob computes $\tilde{s}=a_1\oplus a_2\oplus a_3$ using \autoref{alg:trivial_case} and mistakes it as the distinct element in $(A_i, B_i)$. 

\begin{comment}
============================================

We add a no-communication-cost verification step to check whether a reconciled element is an actual distinct element or not. Note that an actual distinct element of $(A_i, B_i)$ must be in sub-universe $\mathcal{U}_i$. On the other hand, an incorrectly reconciled element (e.g., $\tilde{s}$) can be in any sub-universe with probability $1/n$. So at the end \autoref{subsec:protocol0}, we check whether the reconciled element is in $\mathcal{U}_i$ by the hash function $h$ in hash-partition:

This verfication cannot completely eliminate false-positives, since an incorrectly reconciled element (e.g., $\tilde{s}$) can coincidentally end up in $\mathcal{U}_i$ with probability $1/n$. The chance of false-positives is extremely small using the verification. For instance, if $d=5$ and $n=255$, the probability of the second scenario is only $7.6\times 10^{-6}$. The probability of false-positives using the verfication is $1/n$ times this small probability, which is roughly $3\times 10^{-8}$. {\bf Note that a small probability of false-positives only costs a little waste on set reconciliation when synchronizing objectives (e.g., files), which is acceptable for most applications.}

Even worse, in the second scenario, the false-positives defined in \autoref{sec:single_round_pbs} could happen. For example, if subset pair $(A_i, B_i)$ contains $3$ distinct elements $s_1, s_2, s_3$, then \autoref{alg:trivial_case} computes $\tilde{s}=s_1\oplus s_2\oplus s_3$ and Bob mistakes $\tilde{s}$ as an actual distinct element. The good thing is, the probability of this kind of false-positives is extremely small for small $d$. For instance, if $d=5$ and $n=255$, the probability of the false-positives is only $7.6\times 10^{-6}$. To further reduce the chance of false-positives, we add a no-communication-cost verification step at the end of \autoref{subsec:protocol0} to check whether $\tilde{s}$ is an actual distinct element or not. The verification step works as follows: Given the output $s$ of subset pair $(A_i,B_i)$, if $s\in\mathcal{U}_i$ (i.e., $h(s)=i$), we consider $s$ as an actual distinct element; Otherwise, we consider $s$ as an incorrect output and discard it. 

Note that if $\tilde{s}\in A_i\Delta B_i$, $\tilde{s}$ must be in sub-universe $\mathcal{U}_i$. However, if $\tilde{s}$ is the bitwise \code{XOR} of the distinct elements in $(A_i,B_i)$ (i.e., the second scenario happens), it ends up in $\mathcal{U}_i$ with probablity of only $1/n$. 
%In fact, if we assume the hash-partition described in \autoref{sec:hash_partition} hashes the elements of $\mathcal{U}$ uniformly, independently, and randomly into $n$ sub-universes, the output $s$ in the second scenario will be in a different sub-universe $\mathcal{U}_j (j\neq i)$ with a high probability of $1-\frac{1}{n}$. Hence, this verfication method can further reduce the probability of false-positives by a factor of $\frac{1}{n}$. 
Use the same example (i.e., $d=5$, $n=255$), the probability of this kind of false-positives is reduced from $7.6\times 10^{-6}$ to $3\times 10^{-8}$ by this verification method. 
%{\bf This probability can be further reduced in \autoref{subsec:protocol2}, where PBS does two tiers of hash-partitions. So we can do verification on both of the two hash functions.}

%In some super critical cases (i.e., no false-positive is allowed), we can use a more powerful verification method to completely eliminate false-positives. That is, to check if the output $s$ exists in exactly one of the two sets (i.e., $s\in A\!\setminus\! B$ or $s\in B\!\setminus\! A$). To do so, Bob transmits $s$ along with an identification bit $\mathbbm{1}_{\{s\in B\}}$ to Alice, then Alice checks if $s\in (A\!\setminus\! B)\bigcup (B\!\setminus\! A)$ . This method verification costs additional $d(\log u+1)$ bits of communication overhead. In most applications, this rigorous $0\%$ probability guarantee of false-positives is unnecessary and the probability of the former verification method is small enough, so we use the former in the evaluation. Based on our observation, this kind of false-positives do not happen even once in the evaluation using the former verfication method. In the rest of this paper, we assume Scenario 2 is always correctly verified. 

============================================
\end{comment}

\subsection{Running PBS for Multiple Rounds}\label{sec:multi-rounds}

%{\bf (merged from the following two paragraphs)} 
To deal with the ``rest'' of distinct elements, we remove (and save) all the distinct elements that has been reconciled in the first round (i.e., $\hat{D}$) and run another round of PBS. In the second round, we reconcile $A\Delta \hat{D}$ and $B$ instead of reconciling $A$ and $B$ for both (1) removing all the distinct elements that have been reconciled; and (2) keeping all the distinct elements that have not been reconciled, which we will explain shortly. We use a different hash function for hash-partition in the second round to avoid the same exceptions (i.e., type (\RN{1}), (\RN{2}) events) that happened in the first round happen again. PBS keeps running until the set reconciliation is successfully completed, which is verified by the checksum (\autoref{alg:single_round_pbs} of \autoref{step:terminate_condition}). The use of independent hash functions in different rounds naturally enables the Markov chain modeling of the reconciliation process, which we will elaborate in \autoref{sec:single_markov}. 

{\bf (new content)} We emphasize that reconciling $A\Delta \hat{D}$ and $B$ not only removes all the distinct elements that have been reconciled, but also keeps all the distinct elements that need to be reconciled. Note that the ``rest'' distinct elements can be classified into two catagories: (1) the ``hidden'' distinct elements that have not been reconciled yet (i.e., $D\!\setminus\!\hat{D}$), which are incurred by either a type (\RN{1}) event or a type (\RN{2}) event; and (2) the ``fake'' distinct elements incurred by both a type (\RN{2}) event and the corresponding verification failure in \autoref{alg:verification} (i.e., $\hat{D}\!\setminus\!D$). It is not hard to verify that this classification of the ``rest'' distinct elements (i.e., $D\!\setminus\!\hat{D}$ and $\hat{D}\!\setminus\!D$) is a partition of the set difference between $A\Delta \hat{D}$ and $B$, which confirms our emphasis. 

% To deal with the ``remaining'' distinct elements, we remove (and save) all the distinct elements that has been reconciled in the first round (i.e., $\hat{D}$) and run another round of PBS. In the second round, we reconcile $A\Delta \hat{D}$ and $B$ instead of reconciling $A$ and $B$ to remove all the reconciled distinct elements. We use a different hash function for hash-partition in the second round to avoid the same exceptions (i.e., type (\RN{1}), (\RN{2}) events) that happened in the first round happen again. This procedure replicates until If until all distinct elements are successfully reconciled and the checksum is verified to be correct. 

% {\bf (to be removed)} When the ideal case does not happen (i.e., type (\RN{1}) or type (\RN{2}) event happens), PBS will know the set reconciliation has not been completed via the $32$-bit checksum (\autoref{step:terminate_condition} in \autoref{alg:single_round_pbs}). To reconcile those distinct elements that have not been reconciled yet in the first round, we rule out all successfully reconciled elements and run another round of PBS. This procedure replicates until all distinct elements are successfully reconciled and the checksum is verified to be correct.

% {\bf (to be removed)} More specifically, in the second round, we run PBS to reconcile $A$ and $B\Delta \hat{D}$ instead of $A$ and $B$ to rule out all elements that have been reconciled, where $\hat{D}$ is the set of reconciled distinct elements in the first round. We use a different hash function for hash-partition in the second round to avoid the same exceptions (i.e., type (\RN{1}), (\RN{2}) events) that happened in the first round happen again. The later rounds are similarly operated. 

%{\bf Normally, we want PBS to successfully reconcile all distinct elements in only a few rounds (say $3$) with high probability (say $99\%$). Hence, when tuning parameters (to be discussed in \autoref{sec:parameter_settings}), we set a {\it target success probability} $p_0$ of $r$ rounds as a paramenter setting requirement, which aims to ensure the probability that all distinct elements are reconciled in $r$ rounds to be larger than $p_0$. This requirement should also ensure the majority of the distinct elements are reconciled in the first round. Use the same example ($d=5, n=255$), on average $4.81$ out of $5$ distinct elements should be reconciled in the first round. So the total communication overhead in all rounds is only slightly larger than ($1.01$ to $1.07$ times of, as we will show in \autoref{fig:per-round-con}) that in the first round. Due to this reason, we use the communication overhead in the first round (described in \autoref{sec:communication_overhead_single_PBS}) to approximate the total communication overhead of all rounds in parameter settings (to be elaborated in \autoref{sec:parameter_settings}.}

% Although PBS may need to run many rounds to reconcile all distinct elements, the communication overhead mostly happens in the first round, since the majority of the distinct elements should be reconciled in the first round. Use the same example ($d=5, n=255$), on average $4.81$ out of $5$ distinct elements should be reconciled in the first round. So the total communication overhead in all rounds is only slightly larger than ($1.01$ to $1.07$ times of, to be shown in \autoref{fig:per-round-con}) that in the first round. Due to this reason, we use the communication overhead in the first round (described in \autoref{sec:communication_overhead_single_PBS}) to approximate the total communication overhead (all rounds) in parameter settings (to be elaborated in \autoref{sec:parameter_settings}).

%For the moment, we assume no ``fake'' distinct element in type (\RN{2}) subset pairs fails to be detected, which happens with overwhelming probability as explained in \autoref{subsec:exception_hash_partition}. Then 
%PBS reconciles the distinct elements gradually round by round. This is the ``piecewise decodability'' mentioned in \autoref{sec:intro_oursolution}. We use the following example to describe it in details: 
%Given two sets with $10$ distinct elements, in the first round, PBS tries to reconcile the $10$ distinct elements and say $6$ out of the $10$ distinct elements are successfully reconciled. Then the $6$ reconciled distinct elements are removed and PBS tries to reconcile the remaining $4$ distinct elements in the second round. Say $2$ out of the $4$ remaining distinct elements are successfully reconciled, and that leaves $2$ remaining distinct elements to be reconciled in the third round, so on so force. 
% Given two sets $A$, $B$ with $10$ distinct elements, in the first round, PBS hashes them into $7$ distinct subset pairs. $6$ distinct elements are hashed into $6$ distinct subset pairs, and the other $4$ distinct elements are hashed into the same subset pair. Then the former $6$ distinct elements are successfully reconciled in the first round and the later $4$ distinct elements remain to be reconciled in the second round, which are hashed into $3$ distinct subset pairs (under a different hash function). $2$ remaining distinct elements are hashed into $2$ distinct subset pairs, and the other $2$ remaining distinct elements are hashed into the same subset pair. Then the former $2$ remaining distinct elements are successfully reconciled in the second round and the later $2$ remaining distinct elements remain to be reconciled in the third round, so on so force. 
%The dynamics of the number of remaining distinct elements (i.e., $10\leadsto 4\leadsto 2\leadsto \cdots$ in the example) is in nature a Markov chain, which will be elaborated and analyzed in \autoref{sec:single_markov} to derive a tight tail bound of the probability that all distinct elements are reconciled in $r$ rounds.

% Even if the ideal case does not happen, most of the distinct elements should be distributed into different subset pairs, one distinct element in each, and therefore can be successfully reconciled. So in the first round, even if PBS cannot reconcile all distinct elements, it can reconcile the majority of them.
% % (piecewise decodability mentioned in \autoref{sec:intro_oursolution})
% Based on this intuition, we generalize PBS to multi-round, so that the distinct elements that are not reconciled yet in the first round can be reconciled in later rounds.  

% Without loss of generality, we only describe the second round of multi-round PBS, the reconciliation in the later rounds are similar. Let $\hat{D}_1$ denote the set of reconciled elements in the first round. If set reconciliation is not complete in the first round (i.e., the checksum infers $A\neq B\Delta \hat{D}_1$), then multi-round PBS saves $\hat{D}_1$, which includes correctly and incorrectly reconciled elements as described in \autoref{subsec:exception_hash_partition}, and starts the second round to find (1) the remaining distinct elements; (2) the incorrectly reconciled distinct elements in the first round. In the second round, multi-round PBS reconciles $A$ and $B\Delta \hat{D}_1$ instead of $A$ and $B$ (i.e., $B\leftarrow B\Delta\hat{D}_1$) to rule out all elements that have been reconciled. {\bf It uses a hash function that is different from the one used in the first round for hash-partition, otherwise every remaining distinct element will be hashed into the same subset pair and cause the same exception (described in \autoref{subsec:exception_hash_partition}) that happened in the first round.}

% If set reconciliation is complete in the second round, the set of reconciled elements in the second round (denoted as $\hat{D}_2$) should be the union of (1) all distinct elements that have not been reconciled in the first round (i.e., $(A\Delta B)\!\setminus\!\hat{D}_1$); and (2) all incorrectly reconciled elements in the first round (i.e., $\hat{D}_1\!\setminus\!(A\Delta B)$), which is by definition the set difference between $A\Delta B$ and $\hat{D}_1$. Therefore, the overall set difference $A\Delta B$ equals to the set difference between $\hat{D}_1$ and $\hat{D}_2$; Else, multiround PBS saves $\hat{D}_2$ and starts the third round, so on so force. 

% {\bf May need this algorithm to show the dynamics, if so, the earlier algorithm needs to change accordingly.}
% \IncMargin{1em}
% \begin{algorithm}
% \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
% \Input{$A$ and $B$}
% \Input{Maximum number of rounds $r$}
% \Output{$D$}

% $\hat{D},\mbox{ complete} \leftarrow PBS(A,B)$\;

% $D \leftarrow \hat{D}$\;

% \While{!complete and $r>0$}{
	
% 	$B \leftarrow B\Delta\hat{D}$\;

% 	$\hat{D},\mbox{ complete} \leftarrow PBS(A,B)$\;

% 	$D \leftarrow D\Delta\hat{D}$\;

% 	$r \leftarrow r-1$\;
% }

% \caption{Multi-round PBS} \label{proto:multirounds}
% \end{algorithm}\DecMargin{1em}

% The idea of multi-round PBS is quite simple: In each round, we discard the reconciled distinct elements in the previous rounds and aim to find the rest distinct elements from the remaining elements. More specifically, the first round of multi-round PBS is just the same as single-round PBS in \autoref{alg:single_round_pbs}. The second round has the same procedures as the first round. One difference is, we update $B$ by $B\leftarrow B\Delta\mathcal{D}$ in the second round, so that (1) Reconciled distinct elements in $\mathcal{D}$ that were contained in $A\Delta B$ are not longer contained in $A\Delta (B\Delta\mathcal{D})$; and (2) The other distinct elements remain in $A\Delta (B\Delta\mathcal{D})$ and can be reconciled later. The other difference is, we use a different hash function for partition (\autoref{step:hash_partition}) in the second round. Later rounds update $B$ in the same way and also use different hash functions. Multi-round terminates if the check in \autoref{step:termination} is correct. The overall set difference $A\Delta B$ is simply the union of reconciled distinct elements in all rounds. 

% A straightforward approach to discard reconciled distinct elements is to remove them from both $A$ and $B$. This approach however incurs additional communication overhead to update $A$, since only Bob learns the partial set difference in \autoref{step:reconcile}. Therefore, we use the approach in \autoref{step:updateb} that only updates $B$. It has another benefit in \autoref{step:termination}, which only needs to transmit the CRC of $A$ from Alice to Bob in the first round. In the later rounds, \autoref{step:termination} can be checked locally by Bob and does not require any additional communication overhead;

% Note that the communication overhead in the first round accounts for a large percentage of the total communication overhead in multi-round PBS, since most of the distinct elements (over $95\%$ as we will show in {\bf point to the figure}) should be reconciled in the first round. Therefore, we use the same parameter $n$ in later rounds because otherwise we have to compute a new parameter that can only save tiny communication overhead, even though the number of remaining distinct elements is small and can be reconciled using smaller $n$ with high probability. {\bf Due to the same reason, we can the same expression of the communication overhead in single-round PBS to approximate the communication overhead in multi-round PBS.}

% The natural termination condition of multi-round PBS is that all distinct elements are reconciled, which could require a large number of rounds and incur large additional communication overhead (each additional round incurs $d\log n$ bits of additional communication overhead on transmitting BCH codeword). To control the amount of additional communication overhead, we set another termination condition that multi-round PBS runs for at most $r$ rounds (typically $2$ or $3$). This termination condition could cause an `early' termination when some distinct elements have not been reconciled. However, under proper parameter settings (to be discussed in \autoref{sec:parameter_settings}), we can prove that the probability of an `early' termination (i.e., set reconciliation is incomplete in $r$ round) is very small
% %, and even if an `early' termination happens, an overwhelming percentage of distinct elements should have been reconciled, which is sufficient for most applications
% . For example, when $d=5, n=255, r=2$, an `early' termination happens with probability $4.8\times 10^{-4}$ (how to compute this probability will be elaborated in \autoref{sec:tail_bound}).

% For the moment, we assume no incorrectly reconciled distinct elements appears in multi-round PBS, which happens with overwhelming probability as explained in \autoref{subsec:exception_hash_partition}. Then multi-round PBS reconciles the distinct elements gradually round by round. This is the ``piecewise decodability'' mentioned in \autoref{sec:intro_oursolution}. We use the following example to describe it in details: Given two sets $A$, $B$ with $10$ distinct elements (i.e., $d=10$), in the first round, multi-round PBS hashes them into $7$ distinct subset pairs. $6$ distinct elements are hashed into $6$ distinct subset pairs, and the other $4$ distinct elements are hashed into the same subset pair. Then the former $6$ distinct elements are successfully reconciled in the first round and the later $4$ distinct elements remain to be reconciled in the second round, which are hashed into $3$ distinct subset pairs (under a different hash function). $2$ remaining distinct elements are hashed into $2$ distinct subset pairs, and the other $2$ remaining distinct elements are hashed into the same subset pair. Then the former $2$ remaining distinct elements are successfully reconciled in the second round and the later $2$ remaining distinct elements remain to be reconciled in the third round, so on so force. The dynamics of the number of remaining distinct elements (i.e., $10\leadsto 4\leadsto 2\leadsto \cdots$ in the example) is in nature a Markov chain, which will be elaborated and analyzed in \autoref{sec:tail_bound_per_group} to derive a tail bound of success probability (i.e., all distinct elements are reconciled in $r$ rounds) for paramenter settings. 

% In most applications, a high percentage of reconciliation (e.g., $>99\%$ distinct elements are reconciled) is good enough. Therefore, we add another termination condition on the maximum number of rounds (denoted as $r$). The larger $r$ is, the higher percentage of distinct elements will be reconciled. How to set parameters based on $r$ will be elaborated in \autoref{sec:parameter_settings};

% Readers may think the communication overhead of multi-round PBS is proportional to the number of rounds. In fact, the majority of the communication overhead is spent in the first round, since most of the distinct elements (over $95\%$ as we will show in {\bf point to the figure}) are reconciled in the first round. Each additional round only incurs a small amount of additional communication overhead. For example, when $d=10, n=255, |\mathcal{U}|=2^{32}$, assume $8$ distinct elements are reconciled in the first round and the rest $2$ distinct elements are reconciled in the second round. Then the communication overhead in the first round is $432$ bits. That number of the second round is only $160$


%the communication overhead of single-round PBS of $272$ ($2d\log n+d\log |\mathcal{U}|+32$) bits, and each additional round incurs $40$ ($d\log n$) bits of additional communication overhead. 

%among the three components of the communication overhead mentioned in \autoref{sec:communication_overhead_single_PBS}, only the first component (i.e., the BCH codeword) is proportional to the number of rounds. The other two components does not depend on the number of rounds.

% The second component only depends on the total number reconciled elements, which is roughly equal to $d$. The third component, the checksum of $A$, only needs to be sent once in the first round.
%Therefore, the communication overhead of multi-round PBS is only slightly larger than that of single-round PBS when the number of rounds is small (say $3$). For example, when $d=5, n=255, |\mathcal{U}|=2^{32}$, the communication overhead of multi-round PBS of $3$ rounds is $352$ bits, which is roughly $1.3$ times of the communication overhead of single-round PBS ($272$ bits).

% Therefore, each additional round of multi-round PBS only incurs a small amount of additional communication overhead. For example, when $d=5, n=255, |\mathcal{U}|=2^{32}$, the communication overhead of single-round PBS of $272$ ($2d\log n+d\log |\mathcal{U}|+32$) bits, and each additional round incurs $40$ ($d\log n$) bits of additional communication overhead. 

% As we explained in \autoref{sec:reconcile_by_trivial}, the communication overhead in each round is proportional to the number of (remaining) distinct elements, which decreases exponentially as the number of round increase (i.e., the first round reconciles $90\%$ of distinct elements, the second round reconciles $90\%$ of the remaining $10\%$ distinct elements, etc.). So the majority of the communication overhead (i.e., $\approx 90\%$) is in the first round. Therefore, we do not bother to optimize parameters (i.e., smaller $n$) in later rounds to save tiny communication overhead, even though remaining distinct elements become fewer and can be reconciled using smaller $n$;

% The termination condition of multi-round PBS is that all distinct elements are reconciled, which may require many rounds. In most applications, a high percentage of reconciliation (e.g., $>99\%$ distinct elements are reconciled) is good enough. Therefore, we add another termination condition on the maximum number of rounds (denoted as $r$). The larger $r$ is, the higher percentage of distinct elements will be reconciled. How to set parameters based on $r$ will be elaborated in \autoref{sec:parameter_settings};

% Multi-round means multiple round-trip delays. {\bf Thanks for the piecewise decodability of PBS, in almost all practical application scenarios, this tradeoff does not lead to longer response time because the reconciliation of objects identified by the successfully decodable codewords, which constitute the vast majority of all codewords, can run in parallel with the transmissions and decodings of the rest.  In other words, the piecewise decodability effective masks the slightly larger number of communication rounds as far as the response time is concerned.}

\begin{comment}
==============================

The pseudocode of set reconciliation operations in each round is shown as follows:

\IncMargin{1em}
\begin{algorithm}
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
\Input{$A$ and $B^{(in)}$}
\Input{Set of reconciled distinct elements $D^{(in)}$}
\Output{$B^{(out)}$}
\Output{Set of reconciled distinct elements $D^{(out)}$}

% Hash-partition $A^{(in)}$, $B^{(in)}$ into $\{A^{(in)}_i\}_{i=1}^n$, $\{B^{(in)}_i\}_{i=1}^n$ (\autoref{sec:hash_partition})\label{step:hash_partition}\;

% Encode $\{A^{(in)}_i\}_{i=1}^n$, $\{B^{(in)}_i\}_{i=1}^n$ into parity bitmaps (\autoref{sec:parity_bitmap_encoding})\;


% Find those subset pairs (denoted them as $(A^{(in)}_{i_1}, B^{(in)}_{i_1}), ...,(A^{(in)}_{i_k}, B^{(in)}_{i_k})$) that parity bits differ (\autoref{sec:BCH_code})\;

Run single-round PBS on $A$ and $B^{(in)}$ to obtain the (partial) set difference $\mathcal{D}$\label{step:reconcile} \;

$D^{(out)} \leftarrow D^{(in)}\bigcup \mathcal{D}$\label{step:updated}\;

$B^{(out)} \leftarrow B^{(in)}\Delta\mathcal{D}$\label{step:updateb}\;

Check whether the set reconciliation is complete by comparing $A$ to $B^{(out)}$ (via CRC)\label{step:termination}\;

\caption{Set reconciliation operations of PBS in each round} \label{proto:multirounds}
\end{algorithm}\DecMargin{1em}

In \autoref{proto:multirounds}, the output $B^{(out)}$ in the $r^{th}$ round is the input $B^{(in)}$ in the $(r+1)^{th}$ round. $D^{(in)}$ and $D^{(out)}$ have the same relationship, and they denote the set of reconciled distinct elements before and after a round. $B^{(in)}$ and $D^{(in)}$ are initialized as $B$ and $\emptyset$ respectively. We omit the currect number of round $r$ in \autoref{proto:multirounds}, since the operations in different rounds are exactly the same. Due to the same reason, we only elaborate the operations in the first round: First, Alice and Bob reconcile $A$ and $B^{(in)}$ $(=B)$ using single-round PBS and Bob obtains the (partial) set difference $\mathcal{D}$ (\autoref{step:reconcile}); Second, Bob updates the set of reconciled distinct elements by merging it with $\mathcal{D}$ (\autoref{step:updated}); Third, Bob updates $B^{(in)}$ $(=B)$ to $B^{(out)}$ as \autoref{step:updateb} shows, such that (1) The reconciled distinct elements in $\mathcal{D}$ that are contained in $A\Delta B^{(in)}$ are not longer contained in $A\Delta B^{(out)}$; and (2) The distinct elements that are not successfully reconciled remain in $A\Delta B^{(out)}$ and can be reconciled in later rounds; Finally, we check whether all distinct elements are reconciled. Note that if it is true, $B^{(out)}$ should be the same as $A$ and multi-round PBS should terminate. We use a $32$-bit CRC (Cyclic Reduncancy Check) to check if $B^{(out)}=A$ in our evaluation. {\bf To achieve higher confidence, we can certainly use longer CRC (e.g., 64-bit). }

{\bf Remarks:}

(1) In each round, hash-partition in \autoref{sec:hash_partition} uses different hash functions, so that the remaining distinct elements from the last round will be hashed into different subset pairs with high probability;

(2) A straightforward approach to discard reconciled distinct elements is to remove them from both $A$ and $B$. This approach however incurs additional communication overhead to update $A$, since only Bob learns the partial set difference in \autoref{step:reconcile}. Therefore, we use the approach in \autoref{step:updateb} that only updates $B$. It has another benefit in \autoref{step:termination}, which only needs to transmit the CRC of $A$ from Alice to Bob in the first round. In the later rounds, \autoref{step:termination} can be checked locally by Bob and does not require any additional communication overhead;

(3) As we explained in \autoref{sec:reconcile_by_trivial}, the communication overhead in each round is proportional to the number of remaining distinct elements, which decreases exponentially as the number of round increase (i.e., the first round reconciles $90\%$ of distinct elements, the second round reconciles $90\%$ of the remaining $10\%$ distinct elements, etc.). So the majority of the communication overhead (i.e., $\approx 90\%$) is in the first round. Therefore, we do not bother to optimize parameters (i.e., smaller $n$) in later rounds to save tiny communication overhead, even though remaining distinct elements become fewer and can be reconciled using smaller $n$;

(4) One termination condition of Multi-round PBS is $B^{(out)}=A$, which refers that all distinct elements are reconciled. In most applications, a high percentage of reconciliation (e.g., $>99\%$ distinct elements are reconciled) is good enough. Therefore, we add another termination condition of the maximum number of rounds (denoted as $r$). The larger $r$ is, the higher percentage distinct elements will be reconciled, and the smaller $n$ is required. How to set parameters (e.g., $n$) based on $r$ will be elaborated in \autoref{sec:parameter_settings};

(5) Multi-round means multiple round-trip delays. {\bf Thanks for the piecewise decodability of PBS, in almost all practical application scenarios, this tradeoff does not lead to longer response time because the reconciliation of objects identified by the successfully decodable codewords, which constitute the vast majority of all codewords, can run in parallel with the transmissions and decodings of the rest.  In other words, the piecewise decodability effective masks the slightly larger number of communication rounds as far as the response time is concerned.}

==============================

\end{comment}

% (3) Readers may wonder in the later rounds, most distinct elements should be reconciled, and the rest distinct elements could be reconciled using degraded parameters (i.e., smaller $n$ and $t$). In fact, degrade parameters in later rounds cannot save much communication overhead, since the majority of it is spent in the first round (i.e., $>90\%$). Therefore, we use the same parameters (i.e., $n,t$) among all rounds in multi-rounds PBS;

% (4) The number of remaining distinct elements decreases exponentially as the number of round increase (i.e., the first round reconciles $90\%$ of distinct elements, the second round reconciles $90\%$ of the remaining $10\%$ distinct elements, etc.). 
% (4) The termination condition of Multi-rounds PBS is $B^{(out)}=A$ to reconcile all distinct elements. In some applications,  


% The output $B^{(out)}$ in the $r^{th}$ round is the input $B^{(in)}$ in the $(r+1)^{th}$ round. $D^{(in)}$ and $D^{(out)}$ are similarly defined. $B^{(in)}$ and $D^{(in)}$ are initialized as $B$ and $\emptyset$ respectively. Since and $D$ are updated in each round, so we use $B^{(in)}$ to denote the input and $B^{(out)}$ to denote the output respectively.  Specifically, in the first round, we initialize $B^{(in)}$ and $D^{(in)}$ as $B$ and $\emptyset$ respectively. we first use the single-round scheme 

% Then we run our (single-round) scheme on the updated two sets (i.e., after removing reconciled distinct elements) using a different (independent) hash-partition function from previous rounds, so that the rest distinct elements are hashed into different subset pairs (i.e., the ideal case) with high probability. At the end of each round, we check whether the set reconciliation is complete (i.e., all distinct elements are found) by computing the bitwise \code{XOR} of the remaining elements in $A$ and $B$ 
 

% This {\bf multi-rounds} scheme can significantly increase the success probability (i.e., the probability that all distinct elements are reconciled). Readers may wonder in the later rounds, most distinct elements should be reconciled, and the rest distinct elements could be reconciled using degraded parameters (i.e., smaller $n$ and $t$). In fact, degrade parameters in later rounds cannot save much communication overhead, since the majority of it is spent in the first round (i.e., $>90\%$). Therefore, we use the same parameters (i.e., $n,t$) among all rounds in our evaluation. 
% %The tradeoff between the number of rounds and the communication overhead per rounds will be elaborated in \autoref{sec:tail_bound}. In our evaluation, $r=2,3$ rounds are enough to achieve an extremely high success probability. 

% Readers may think the cost (i.e., communication overhead and the computational complexity) of this multi-rounds scheme is proportional to the number of rounds (denoted as $r$) and increases linearly with $r$. In fact, the cost of each round is roughly proportional to the number of remaining distinct elements, which decreases exponentially as $r$ increases (i.e., the first round reconciles $99\%$ of distinct elements, the second round reconciles $99\%$ of the remaining $1\%$ distinct elements, etc.). So the cost of this multi-rounds scheme is only slightly larger than that of the single-round scheme. Furthermore, as we explained in \autoref{sec:intro}, {\bf from intro thanks for the piecewise decodability of our solution, in almost all practical application scenarios, this tradeoff does not lead to longer response time because the reconciliation of objects identified by the successfully decodable codewords, which constitute the vast majority of all codewords, can run in parallel with the transmissions and decodings of the rest.  In other words, the piecewise decodability effective masks the slightly larger number of communication rounds as far as the response time is concerned.} 

\begin{comment}

\subsection{Baseline Scheme}\label{subsec:protocol1} 

Note that the set difference $A\Delta B$ can contain more than 1 elements (i.e., $d>1$), and \autoref{alg:trivial_case} cannot reconcile $A$ and $B$ directly in this case. Therefore, we propose a baseline scheme building upon~\autoref{alg:trivial_case} that also works when $d>1$: First, we partition the element universe $\mathcal{U}$ into $n$ sub-universes $\mathcal{U}_1, \mathcal{U}_2, \cdots, \mathcal{U}_n$. Denote $A_i \triangleq A\bigcap \mathcal{U}_i$ and $B_i \triangleq B\bigcap \mathcal{U}_i$ for $i=1,2,\cdots,n$. Then $\{A_i\}_{i=1}^n$ and $\{B_i\}_{i=1}^n$ are partitions of $A$ and $B$ respectively. Furthermore, $\Phi\triangleq\{A_i\Delta B_i\}_{i=1}^n$ is a partition of $A\Delta B$. 

Assume the {\bf ideal case} happens, in which each subset pair $(A_i, B_i)$ contains at most one distinct element ({\it i.e.,} $|A_i\Delta B_i|\!\leq\!1$), we use \autoref{alg:trivial_case} to reconcile each subset pair and obtain $A_i\Delta B_i$ for $i=1,2,\cdots,n$. The overall set difference $A\Delta B$ is simply their union $\bigcup_{i=1}^n \big{(}A_i\Delta B_i\big{)}$. 

In the first step of the baseline scheme, we can use a hash function $h(\cdot): \mathcal{U}\rightarrow \{1,2,\cdots,n\}$ to partition the universe $\mathcal{U}$ into $n$ sub-universes: $\mathcal{U}_i=\{s\mid s\in \mathcal{U} \mbox{ and } h(s)=i\}$ for $\forall i=1,2,\cdots,n$. And the hash function $h(\cdot)$ can be predetermined between Alice and Bob and does not require additional communication cost.

This hash-partition can be modeled as a {\it balls-into-bins problem}, in which the distinct elements are viewed as balls and the subset pairs are viewed as bins. The hash-parition basically throws (hashes) $d$ balls (distinct elements) uniformly and randomly into $n$ bins (subset pairs). The aforementioned ideal case in this context becomes, after throwing $d$ balls uniformly and randomly into $n$ bins, each bin receives at most 1 ball (i.e., $d$ nonempty bins have 1 ball in each and the rest $n-d$ bins are empty). {\bf It may remind readers about the Birthday problem. And the ideal case can be analogous to the case that no people share the same birthday.} The ideal case happens with a probability of $p=\frac{n\,!}{(n-d)\,!n^d}\!=\!\prod_{k=1}^{d - 1}(1 - \frac{k}{n})\!\approx\! e^{-\frac{d(d-1)}{2n}}$ when $d\!\ll\!n$. In other words, $n$ must be $\Omega(d^2)$ to ensure the ideal case happens with a nontrivial probability.  Note that the communication overhead of the baseline scheme is proportional to $n$, as each subset pair requires communication of a bitwise \code{XOR} in \autoref{alg:trivial_case}. So this communication overhead increases at least quadratically as $d$ increases. 

In fact, this communication overhead can be significantly reduced: In the ideal case, $n-d$ out of $n$ subset pairs are identical ones, and only $d (\ll n)$ out of $n$ subset pairs contain distinct elements (one distinct element in each of the $d$ subset pairs) and need to be reconciled. If we can identify these $d$ subset pairs (with a tiny additional communication overhead) and only reconcile them, the overall communication overhead will be significantly reduced from $\Omega(d^2)$ to $O(d)$. Based on this intuition, we propose our scheme in \autoref{sucsec:our-scheme}, which uses Parity Bitmap Sketch (PBS) and Error Correction Coding (ECC) to identify those subset pairs with a tiny additional communication overhead. 

Note that the ideal case does not always happen. However, we can ensure that the ideal case happens with high probability by properly selecting $n$ based on $d$ (i.e., $n=\Omega(d^2)$). Furthermore, as we will describe in \autoref{subsec:nonideal}, even if the ideal case does not happen (i.e., some distinct elements are hashed into the same subset pair), most of the distinct elements should be distributed into different subset pairs and therefore can be reconciled. So the baseline scheme, even cannot reconcile all of the distinct elements, can still reconcile the majority of them. Based on this property, we will extend our scheme from single-round to multi-rounds in \autoref{subsec:nonideal} to further increase the probability of reconciling all distinct elements. 

For general cases ({\it i.e.,} $t=|A\Delta B|$ is an arbitrary number), we have a straightforward strawman scheme building upon~\autoref{alg:trivial_case}, which works as follows: First, Alice and Bob choose some hash function $h(s): \mathcal{U} \rightarrow \{0,1,\cdots,2^{32}-1\}$ to partition $A$ and $B$ into $m$ subsets $A_1,A_2,\cdots,A_m$ and $B_1,B_2,\cdots,B_m$ respectively:

\begin{align}
s\in A_i & \mbox{ iff } s\in A \mbox{ and } h(s)=i\!\mod m, \nonu{}mber\\
s\in B_i & \mbox{ iff } s\in B \mbox{ and } h(s)=i\!\mod m. \nonumber
\end{align} 

{\bf call a subset pair -> partition?} Since Alice and Bob use the same hash function for partition, common elements (i.e., elements in $A\cap B$) are always hashed into the same subset pair $(A_i, B_i)$. And the set difference of each subset pair only contains distinct elements (i.e., elements in $A\Delta B$): $A_i\Delta B_i \subset A\Delta B$. In the ideal case, with a sufficient large $m$, each subset pair $(A_i, B_i)$ contains at most one distinct element ({\it i.e.,} $|A_i\Delta B_i|\!\leq\!1$). Then \autoref{alg:trivial_case} can reconcile each subset pair and obtain $A_i\Delta B_i$ for $i=1,2,\cdots,m$. The overall set difference $A\Delta B$ is simply their union $\bigcup_{i=1}^m \big{(}A_i\Delta B_i\big{)}$. The selection of hash function $h(s)$ can be predetermined between Alice and Bob and it does not require additional communication cost.

%To make sure Alice and Bob use the same hash function for partition, we let them pre-agree on some universal hash family (e.g., \code{xxHash}~\cite{Collet_xxHashExtremelyfast_}) and a common selection order, and each time they choose a hash function from the family in the same order. Note that we can also let Alice generates a hash function and send it to Bob. The hash function that Alice and Bob choose for partition can be either generated by 

This hash-partition is in nature a {\it balls-into-bins model}. We can view the distinct elements as balls and the subset pairs as bins. The hash-parition basically throws (hashes) $t$ balls (distinct elements) uniformly and randomly into $m$ bins (subset pairs). The aforementioned ideal case in this context is, with a sufficient large number of bins, each bin receives at most 1 ball. The strawman scheme works correctly if and only if the ideal case happens, which has a probability of $\frac{m\,!}{(m-t)\,!m^t}\!=\!\prod_{k=1}^{t - 1}(1 - \frac{k}{m})\!\approx\! e^{-\frac{t(t-1)}{2m}}$. In other words, to ensure the strawman scheme works correctly with a probability of $p$, it roughly requires $m \!=\!\lceil \frac{t(t-1)}{-2\ln p}\rceil$ subset pairs. 

Note that the communication overhead of this strawman scheme is proportional to the number of subset pairs $m$, as each subset pair requires communication of an \code{XOR} sum in \autoref{alg:trivial_case} during the reconciliation. When $t$ is small, a small communication cost can guarantee that the strawman scheme works correctly with high probability. For instance, when $t=5$, $m=95$ subset pairs are sufficient for the strawman scheme to work correctly with a probability of $90\%$. However, when $t$ is relatively large, it requires a huge communication cost to ensure the strawman scheme works correctly. For instance, when $t=1,000$, it requires $m=4,740,865$ subset pairs to guarantee a success probability of $90\%$. 

In fact, the majority of subset pairs are identical ones and do not need to reconcile. And only a small portion of them contain distinct elements. If we can identify those subset pairs that contain distinct elements and only reconcile them, the communication cost could be significantly reduced. Our scheme is based on this intuition and uses parity bitmap sketch and BCH code to identify the subset pairs, which we will elaborate in \autoref{sucsec:our-scheme}. 

%To distribute balls as uniformly as possible and maximize the probability of the ideal case, we choose a uniform hashing function $h$ that throws balls uniformly and randomly into bins: $$\mathbb{P}[h(s)=i]=\frac{1}{m} \mbox{ for } \forall i=1,2,\cdots,m, \forall s\in U$$.

%Note that the probability of the ideal case is $\frac{m\,!}{(m-t)\,!m^t}\!=\!\prod_{k=1}^{t - 1}(1 - \frac{k}{m})\!\approx\! e^{-\frac{t(t-1)}{2m}}$. Hence, at least $\lceil \frac{t(t-1)}{-2\ln p}\rceil$ bins are required to ensure that this probability is at least $p$. In other words, to ensure that the ideal case happens with a probability of $p$, the strawman scheme roughly requires $m \!=\!\lceil \frac{t(t-1)}{-2\ln p}\rceil$. For example, suppose $t\!=\!$\num{1000}, %and $p\!=\!0.01$, this strawman scheme roughly requires $m\!=\!$\num{720626} bins (partitions) to ensure that $|A_i\Delta B_i|\!\leq\!1$ (for any $i=1,2,\cdots,m$) holds with probability $50\%$.  

% A straightforward strawman scheme building upon~\autoref{alg:trivial_case} 
% to reconcile two sets $A$ and $B$ in general 
% ({\it i.e.,} $|A\Delta B|$ is an arbitrary number) is the following: 
% Uniformly randomly partition $A$ and $B$ into $m$ subsets ($A_1,A_2,\cdots,A_m$ 
% and $B_1,B_2,\cdots,B_m$) so that the set difference 
% $A_i\Delta B_i$ of each subset pair $(A_i, B_i)$ contains at most one element 
% ({\it i.e.,} $|A_i\Delta B_i|\!\leq\!1$) {\it w.h.p.} ({\it i.e.,} with high probability), 
% and then reconcile each subset pair with~\autoref{alg:trivial_case}. 

% Now let us analyze this strawman scheme using the {\it balls-into-bins model}. 
% Assume that sets $A$ and $B$ have $t$ elements in their set difference, {\it i.e.,} $|A\Delta B|\!=\!t$. 
% These $t$ elements can be viewed as $t$ balls and the $m$ partitions (subset pairs) can be viewed as 
% $m$ bins. The random partition process in this strawman scheme can be modeled as throwing 
% $t$ balls into $m$ bins in the following manner: Each ball goes into a 
% uniformly random bin and independently of other balls. %so that each bin contains at most one ball, {\it w.h.p.}  
% The probability that each bin contains at most one ball is  
% $\frac{m\,!}{(m-t)\,!m^t}\!=\!\prod_{k=1}^{t - 1}(1 - \frac{k}{m})\!\approx\! e^{-\frac{t(t-1)}{2m}}$. 
% Hence, at least $\lceil \frac{t(t-1)}{-2\ln p}\rceil$ bins are required 
% to ensure that this probability is at least $p$. In other words, to ensure 
% that each bin contains at most one ball with a probability of $p$, 
% the strawman scheme roughly requires $m \!=\!\lceil \frac{t(t-1)}{-2\ln p}\rceil$. 
% For example, suppose $t\!=\!$\num{1000}, %and $p\!=\!0.01$, 
% this scheme roughly requires $m\!=\!$\num{108469} bins (partitions) to 
% ensure that $|A_i\Delta B_i|\!\leq\!1$ (for any $i=1,2,\cdots,m$) holds with probability $0.01$.  

% We note that the communication overhead of this strawman scheme is proportional to 
% $m$ ($\!\gg\! t$), as each partition (subset pair) requires communication of an \code{XOR} sum during the reconciliation. 
% This communication overhead is much higher than that of the optimal scheme, which only requires 
% to exchange the elements in the set difference (assuming an oracle tells it which elements belong to 
% the set difference), {\it i.e.,} proportional to $t$. In the example above, assuming each element takes 4 bytes, 
% the communication overhead of the strawman scheme is $4m$ bytes ($\!\approx\! \num{423.71}\,$KB) to ensure 
% a success rate of only 0.01 ({\it i.e.,} with a probability of $0.0.1$, all elements in 
% the set difference are successfully reconciled), 
% which is approximately 2 orders of magnitude higher than $4t$ bytes ($\!=\!\num{3.90}\,$KB), the communication 
% overhead of the optimal scheme. 

\subsection{Our Scheme: The Preliminary Version}\label{sucsec:our-scheme}

Like the baseline scheme, our scheme also hash-partitions the two sets $A$ and $B$ into $n$ subset pairs. The difference is, instead of reconciling all subset pairs using \autoref{alg:trivial_case}, our scheme identifies the subset pairs that contains distinct elements and only reconciles them. Since the hash-partition and set reconciliation on each subset pair using \autoref{alg:trivial_case} have been described in \autoref{subsec:protocol1}, we only elaborate how to identify the subset pairs that contain distinct elements in this section. 

The general idea of identification is very simple: First, we {\bf encode} each subset into $1$ bit, such that in the ideal case, for $\forall i=1,2,\cdots,n$:

\begin{itemize}
	\item The codewords (bits) of $A_i$ and $B_i$ are different if and only if subset pair $(A_i, B_i)$ contains $1$ distinct element;
	\item The codewords (bits) of $A_i$ and $B_i$ are the same if and only if subset pair $(A_i, B_i)$ contains no distinct element;
\end{itemize}

Second, we {\bf compare} the codewords of each subset pair. And the subset pairs that contain distinct elements are the ones with different codewords (bits). We will describe the two steps in details in \autoref{sec:parity_bitmap_encoding} and \autoref{sec:BCH_code} respectively.

\subsubsection{Parity Bitmap Encoding}\label{sec:parity_bitmap_encoding}

In our scheme, we use {\it parity encoding} to encode each subset into a parity bit. More specific, it encodes a subset as ``1'' if it contains odd number of elements, and as ``0'' otherwise. And it satisfies the aforementioned requirements in the ideal case:

\begin{itemize}
	\item If subset pair $(A_i, B_i)$ contains $1$ distinct element, the corresponding two subsets $A_i$ and $B_i$ differ exactly one element, which implies that $||A_i|\!-\!|B_i||\!=\!1$. Hence, if $|A_i|$ ({\it i.e.,} number of elements in $A_i$) is odd (or even), then $|B_i|$ must be even (or odd). And the parity bits of $A_i$ and $B_i$ will be different;
	\item If subset pair $(A_i, B_i)$ contains no distinct element, the corresponding two subsets $A_i$ and $B_i$ should be the same and therefore contain the same number of elements. Hence, if $|A_i|$ is odd (or even), then $|B_i|$ must be odd (or even). And the parity bits of $A_i$ and $B_i$ will be the same;
\end{itemize}

Using parity encoding, the $n$ subsets of $A$ are encoded as a bit string $A[1..n]$ in $\{0,1\}^n$, 
where the $i$-th bit $A[i]$ in $A[1..n]$ corresponds to the parity encoding bit of $A_i$. Similarly, the $n$ subsets of $B$ are similarly 
encoded as a bit string $B[1..n]$. We call $A[1..n]$ ($B[1..n]$) the {\it parity bitmap} of $\{A_i\}_{i=1}^n$ ($\{B_i\}_{i=1}^n$). In the ideal case, $A[1..n]$ and $B[1..n]$ differ at $d$ different bit-positions, which corresponds to the $d$ subset pairs that contain distinct elements. And our scheme only reconciles those subset pairs that the parity bits are different. We will describe the nonideal case (i.e., some subset pair contains more than 1 distinct elements) in \autoref{subsec:nonideal}.

\subsubsection{Parity Bitmap Comparison Using BCH Code}\label{sec:BCH_code}

A straightforward approach to compare the parity bitmaps is to let Bob send the complete parity bitmap $B[1..n]$ to Alice, then Alice compares $A[1..n]$ with $B[1..n]$ locally. This approach has a communication overhead of $n$ bits, which is unnecessarily high. As we discussed in~\autoref{subsec:protocol0}, $d$ is usually much smaller than $n$. It means $A[1..n]$ and $B[1..n]$ differ only at a tiny portion of bits. Therefore, we can view $A[1..n]$ as a corrupted message of $B[1..n]$ with $d$ corrupted bits, and the bit-positions of the $d$ corrupted bits basically correspond to the $d$ subset pairs that contain distinct elements. The detection of corrupted bits, on the other hand, can be solved by Error-Correction Code (ECC)~\cite{Lin_ErrorControlCoding_1983}. And our scheme uses BCH code~\cite{Lint_IntroductionCodingTheory_1998} to encode the parity bitmap and detect the $d$ corrupted bits.

More specific, after the parity bitmap encoding, Bob uses a $d$-error-correcting systematic BCH code to encode $B[1..n]$ into an $n+d\log n$ codeword, in which the first $n$ bits are $B[1..n]$ (property of systematic BCH code). Then Bob sends the rest $d\log n$ bits, which we denote as {\it parity bitmap sketch (PBS)}, to Alice. Upon the received PBS and $A[1..n]$ (corrupted message), Alice uses the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} to detect the $d$ corrupted bits in $A[1..n]$. The communication overhead of this approach is $d\log n$ bits (i.e., length of PBS), which is much smaller than that of the straightforward approach ($n$ bits, when $d\!\ll\!n$). On the other hand, the computational complexity of the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} is $O(d^2\log^2 n)$. 

\subsubsection{Exceptional Handling and Multi-rounds}\label{subsec:nonideal}

As we described in \autoref{subsec:protocol1}, the ideal case does not always happen, which means some subset pair may contain more than 1 distinct elements and cannot be successfully reconciled by \autoref{alg:trivial_case}. Due to the parity encoding, we can classify such subset pair into the following two scenarios:

\begin{itemize}
    \item Scenario 1: If a subset pair $(A_i, B_i)$ contains even number ($\geq 2$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be the same and our scheme will not reconcile the subset pair. Hence, the distinct elements in the subset pair will not be reconciled;
    \item Scenario 2: If a subset pair $(A_i, B_i)$ contains odd number ($\geq 3$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be different and our scheme will reconcile the subset pair using \autoref{alg:trivial_case}. However, as we described in \autoref{subsec:protocol0}, when a subset pair contains more than 1 distinct elements, \autoref{alg:trivial_case} will output the bitwise \code{XOR} of them as the `distinct element', which is not a real distinct element with high probability;
\end{itemize}

In both scenarios, the distinct elements in the subset pair cannot be reconciled. Even worse, in the second scenario, a false-positive could happen (i.e., the output of \autoref{subsec:protocol0} is not a real distinct element). However, as we will analyze in \autoref{sec:tail_bound} and show in {\bf the evaluation section}, the second scenario barely happens both theoretically and empirically. To further reduce the chance of false-positives, we add a verification step at the end of \autoref{subsec:protocol0} to check whether the output of \autoref{subsec:protocol0} $s$ is a real distinct element or not. The verification step works as follows: Given the output $s$ of subset pair $(A_i,B_i)$, if $s\in\mathcal{U}_i$ (i.e., $h(s)=i$), we consider $s$ as a real distinct element; Otherwise, we consider $s$ as an incorrect output and discard it. 

Note that if $s$ is a real distinct element of $(A_i,B_i)$, $s$ must be in sub-universe $\mathcal{U}_i$. However, if $s$ is the bitwise \code{XOR} of the distinct elements in $(A_i,B_i)$ (i.e., the second scenario happens), $s$ could be in any sub-universe other than $\mathcal{U}_i$. In fact, if we assume the hash-partition described in \autoref{subsec:protocol1} hashes the elements of $\mathcal{U}$ uniformly, independently, and randomly into $n$ sub-universes, the output $s$ in the second scenario will be in a different sub-universe $\mathcal{U}_j (j\neq i)$ with a high probability of $1-\frac{1}{n}$. Hence, this verfication step can reduce the chance of false-positives by a factor of $\frac{1}{n}$. 

Even if the ideal case does not happen, most of the distinct elements should be distributed into different subset pairs and therefore can be reconciled. So our scheme, even cannot reconcile all of the distinct elements, can still reconcile the majority of them (piecewise decodability). To reconcile the rest distinct elements, we can just run our scheme for another round under a different hash-partition function, so on so force. This {\bf multi-rounds} scheme can significantly increase the success probability (i.e., the probability that all distinct elements are reconciled). Readers may wonder in the later rounds, most distinct elements should be reconciled, and the remaining could be reconciled using degraded parameters (i.e., smaller $n$ and $t$). In fact, degrade parameters in later rounds cannot save much communication overhead, since the majority of it is spent in the first round (i.e., $>90\%$). Therefore, we use the same parameters (i.e., $n,t$) among all rounds in our evaluation.
%The tradeoff between the number of rounds and the communication overhead per rounds will be elaborated in \autoref{sec:tail_bound}. In our evaluation, $r=2,3$ rounds are enough to achieve an extremely high success probability. 

Readers may think the cost (i.e., communication overhead and the computational complexity) of this multi-rounds scheme is proportional to the number of rounds (denoted as $r$) and increases linearly with $r$. In fact, the cost of each round is roughly proportional to the number of remaining distinct elements, which decreases exponentially as $r$ increases (i.e., the first round reconciles $99\%$ of distinct elements, the second round reconciles $99\%$ of the remaining $1\%$ distinct elements, etc.). So the cost of this multi-rounds scheme is only slightly larger than that of the single-round scheme. Furthermore, as we explained in \autoref{sec:intro}, {\bf from intro thanks for the piecewise decodability of our solution, in almost all practical application scenarios, this tradeoff does not lead to longer response time because the reconciliation of objects identified by the successfully decodable codewords, which constitute the vast majority of all codewords, can run in parallel with the transmissions and decodings of the rest.  In other words, the piecewise decodability effective masks the slightly larger number of communication rounds as far as the response time is concerned.} 

\end{comment}


%%% Moved from related work
\input{section/pinsketch}

\section{PBS for large \texorpdfstring{\larger\boldmath\MakeLowercase{$d$}}{d}}\label{subsec:protocol2}
 
The scheme above, which we refer as PBS-for-small-$d$, can also do set reconciliation when $d$ is large. However, the BCH decoding computational complexity in it is $O(d^2)$ of finite field operations (in GF($2^{8}$) when $n=255$) using the state-of-the-art decoding algorithm~\cite{Dodis_SyndromeEncodingDecoding_2006}, which is too expensive for large $d$. To overcome this drawback, we use the same technique in \autoref{sec:hash_partition} to hash-partition sets $A$ and $B$ each into $d/\delta$ subsets (which we call {\it groups} to distinguish from subsets) for some small integer $\delta$ (say $5$), so that each of the group pairs contains roughly $\delta$ distinct elements and can be reconciled by PBS-for-small-$d$ respectively. The BCH decoding computational complexity of each group pair is roughly $O(\delta^2)$, which can be considered as $O(1)$, since $\delta$ is a small number. As a result, the overall computational complexity is reduced from $O(d^2)$ to $O(d)$. 

%Note that the BCH decoding computational complexity is $O(d^2)$ of finite field operations (in GF($2^{8}$) when $n=255$) using the state-of-the-art decoding algorithm~\cite{Dodis_SyndromeEncodingDecoding_2006}, which is too expensive for large $d$. To overcome this drawback, we first hash-partition sets $A$ and $B$ each into $d/\delta$ subsets (which we call {\it groups} to distinguish from subsets), just like what we did in \autoref{sec:hash_partition}, for some small integer $\delta$ (say $5$), then reconcile each of the group pairs by the PBS we described in \autoref{sec:scheme}. After the partition, each group pair has $\delta$ distinct elements on average. So the BCH decoding computational complexity of each group pair is roughly $O(\delta^2)$, which can be considered as a constant, since $\delta$ is a small number. As a result, the overall computational complexity of PBS is reduced from $O(d^2)$ to $O(d)$. 

%To differentiate from the PBS described in \autoref{sec:scheme}, we refer to it as PBS-basic in this section. 
We continue to assume that the number of distinct elements $d$ is precisely known. Even so, due to the randomness of hash-partition, denoted as $\delta_i$, the number of distinct elements in the $i$-th group pair, is a variable with mean of $\delta$ for $i=1,2,...,g$, which are not precisely known. Since $\delta_1, \delta_2, ..., \delta_g$ follows the same distribution, it does not make sense to select different parameters for the $g$ group pairs. Hence, we set two universal parameters, $t$ and $n$, for all group pairs, where $t$ is the error-correction capability of the BCH code used for reconciling each group pair, and $n$ is the number of subset pairs in each group pair.

% We continue to assume that the number of distinct elements $d$ is precisely known. Even so, due to the randomness of hash-partition, denoted as $\delta_i$, the number of distinct elements in the $i$-th group pair, is a Binomial random variable with mean of $\delta$ for $i=1,2,...,g$, which cannot be precisely known without a huge amount of additional communication overhead. Since $\delta_1, \delta_2, ..., \delta_g$ follows the identical Binomial distribution, it does not make sense to select different parameters for the $g$ group pairs. Hence, we set two universal parameters, $t$ and $n$, for all group pairs, where $t$ is the error-correction capability of the BCH code used for reconciling each group pair, and $n$ is the number of subset pairs in each group pair.

%To deal with this randomness, we set two global parameters, denoted as $t$, that corresponds to the error-correction capability of the BCH code used for reconciling every group pair. identical no sense or additonal info

%{\bf (modified based on the next paragraph from intro)} 
The error-correction capability $t$, defined as the maximum number of errors that the BCH code used by any group pair can correct, is a critical parameter for PBS to perform well. On one hand, if $t$ is too large (say $t=10\delta$), then the communication overhead on transmitting BCH codeword for each group pair ($t\log n$ bits) is unnecessarily large; but on the other hand, if $t$ is too small (say equal to $\delta$), then close to half of the group pairs fail to decode the BCH codeword due to the insufficient error-correction capability, which can result in hefty penalties on BCH decoding failures (to be described in \autoref{sec:BCH_exception}). In PBS, we manage to make $t$ as small as possible (so that the communication overhead on transmitting BCH codewords is kept to a minimum) yet pay negligible penalties of BCH decoding failures. 

% To ensure the error-correction capability $t$ is sufficient (i.e., $t\geq \delta_i$ for $i=1,2,...,g$) for every group pair with high probability, we set $t$ conservatively and leave a sufficient `safety margin' between $t$ and the average number of distinct elements in each group pair $\delta$. 

% Note that the `safety margin' between $t$ and $\delta$ incurs additional communication overhead on transmitting BCH codeword: In the perfect scenario (i.e., $\{d_i\}_{i=1}^g$ is precisely known), the average communication overhead on transmitting BCH codeword per group pair is $\delta\log n$; On the other hand, when we set $t$ to be the error-correction capability for each group pair, the average communication overhead becomes $t\log n$. If we set the `safety margin' to be too large (say $t=10\delta$), it will incur huge additional communication overhead. Due to this reason, we set a moderate `safety margin' that  $t$ in the range from $1.5\delta$ to $3\delta$. 

% {\bf (moved from intro, to be removed)} The number of elements in the set difference between any group pair is in general not a constant.  Rather, it is a random variable that has roughly a Poisson distribution with mean $\delta$.  The potential issue arises from dealing with this randomness in setting a global parameter that corresponds to the error-correction capability of the BCH code used for reconciling every group pair.  This parameter, denoted as $t$ (consistent with other literatures on BCH code), is the maximum number of errors that the BCH code used by any group pair can correct, and the size of each such codeword is roughly $8t$ bits (assuming $n = 255$ as explained above). The issue is that, on one hand, if $t$ is too large (say several times larger than $\delta$), then the total size of the BCH codewords, which is the bulk of the extra communication cost, is unnecessarily large; but on the other hand, if $t$ is too small (say equal to $\delta$), then close to half of the BCH codewords cannot decode or worse decode incorrectly (unknown to Alice and Bob), which can result in hefty penalties in the latter case of incorrect decoding.   In PBS, we manage to make $t$ as small as possible (so that the total size of the BCH codewords is kept to a minimum) yet pay negligible penalties of incorrect BCH decoding.
%We will discuss the case that $d_i>t$ in \autoref{sec:BCH_exception}.

% Hence, we can no longer set the error-correction capability of the BCH code for each group pair based on the exact number of distinct element in it, as we did in \autoref{sec:scheme}. Instead, we set a conservative error-correction capability $t$ (say $2.5\delta$) for all group pairs, which is sufficient for them (i.e., $t\geq d_i$ for $i=1,2,...,g$) with high probability. We will discuss the case that $d_i>t$ in \autoref{sec:BCH_exception}.


% ===============================
% To differentiate from the PBS described in \autoref{sucsec:our-scheme}, we refer it as PBS-basic in this section. Note that the BCH decoding computational complexity is $O(d^2\log ^2 n)$, which is $\Omega(d^2\log^2 d)$ when $n=\Omega(d^2)$, with the state-of-the-art decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019}. It is too large in PBS-basic for large $d$. To overcome this drawback and generalize PBS-basic for large $d$, we partition sets $A$ and $B$ each into $d/\delta$ subsets (which we call {\it groups} to distinguish from subsets) for some small integer $\delta$ (say $5$) and reconcile the $d/\delta$ group pairs respectively using PBS-basic. After this partition, each group has $\delta$ distinct elements on average. The BCH decoding computational complexity of each group pair can be considered as $O(1)$, since $\delta$ is a small number. As a result, the overall computational complexity of PBS is reduced from $O(d^2\log ^2 n)$ to $O(d)$. 

% % To differentiate from the PBS described in \autoref{sucsec:our-scheme}, we refer it as PBS-basic in this section. PBS-basic is not suitable for large $d$ for two reasons: First, its communication overhead is asymptotically $O(d\log n)\!=\!O(d\log d)$ (since $n=\Omega(d^2)$), which is not asymptotically optimal. Second, the decoding computational complexity is proportional to $d^2$ with the state-of-the-art decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} for BCH codes, which is too high when $d$ is large. To overcome these two drawbacks, we use a simple algorithmic trick to (1) reduce the communication overhead from $O(d\log d)$ to $d\log u \!+\! O(d)$; (2) reduce the decoding computational complexity from $O(d^2)$ to $O(d)$. 

% Now, we describe the generalized PBS in details: In the first step, we hash-partition $A$ and $B$ (by some hash function $h_1(\cdot)$) into $g$ group pairs, just like what we did in \autoref{sucsec:our-scheme}. The objective of this partition is however different: In \autoref{sucsec:our-scheme}, we aim to ensure each subset pair contains at most $1$ distinct element (i.e., the ideal case) with high probability; Here we aim to make each group pair contains roughly $\delta$ distinct elements for some small constant $\delta$ (say $5$) by setting $g=d/\delta$. 
% %To differentiate the $g$ subset pairs here from those in \autoref{sec:hash_partition}, we call them the $g$ {\bf groups} in the sequel. 
% In the second step, we just apply PBS-basic (described in \autoref{sucsec:our-scheme}) to reconcile each group pair and obtain the distinct elements. 
% ================================

% To differentiate from the PBS described in \autoref{sucsec:our-scheme}, we refer it as PBS-basic in this section. When $d$ is large (more than several), we hash-partition set $A$ and $B$ into groups, such that each group pair contains $\delta$ distinct elements on average for small $\delta$ (say $5$), as described in \autoref{sec:larged}. Then each group pair can be reconciled by PBS-basic.

% When describing the PBS-basic in \autoref{sucsec:our-scheme}, we assume that the number of distinct elements is precisely known. We set the error-correction capability of the BCH code (denoted as $t$) just enough to correct $d$ errors (i.e., $t=d$). However, due to the randomness of hash-partition, $d_i$, the number of distinct elements in the $i^{th}$ group pair, is a Binomial random variable $Binomial(d,1/g)$ with expectation of $\delta$ $(=d/g)$ for $i=1,2,...,g$, which cannot be precisely known without a huge amount of additional communication overhead. Hence, we can no longer set the error-correction capability of the BCH code for each group pair based on the exact number of distinct element in it, as we did in \autoref{sucsec:our-scheme}. Instead, we set a universal error-correction capability $t$ (say $2.5\delta$) for all group pairs, which is sufficient for all group pairs (i.e., $t\geq d_i$ for $i=1,2,...,g$) with high probability. We will discuss the case that $d_i>t$ in \autoref{sec:BCH_exception}.

%This assumption in general does not hold: 
% Let $d_i$ denote the number of distinct elements in Group $i$. Due to the property of hash-partition, each $d_i$ is a Binomial random variable $Binomial(d,1/g)$ with expectation of $\delta$ $(=d/g)$. Even if $d$ is precisely known, each $d_i$ is not. To ensure the error-correction capability $t$ is sufficient for each group (i.e., $d_i\leq t$) with high probability, we leave some safety margin for the randomness of $d_i$ and conservatively set $t$ roughly $2.5\delta$ (the factor $2.5$ varies depend on other parameters, which will be discussed in \autoref{sec:parameter_settings}), so that $Pr[d_i>t]$ is tiny. We will discuss the case that $d_i>t$ in \autoref{sec:BCH_exception}.

% Note that the `safety margin' between $t$ and $\delta$ incurs additional communication overhead on transmitting BCH codeword: In the perfect scenario (i.e., $\{d_i\}_{i=1}^g$ is precisely known), the average communication overhead on transmitting BCH codeword per group pair is $\delta\log n$; On the other hand, when we set $t$ to be the error-correction capability for each group pair, the average communication overhead becomes $t\log n$. If we set the `safety margin' to be too large (say $t=10\delta$), it will incur huge additional communication overhead. Due to this reason, we set a moderate `safety margin' that  $t$ in the range from $1.5\delta$ to $3\delta$. 

%which is roughly $2.5$ times of that in the perfect scenario (when $t$ is roughly $2.5\delta$). Due to this addition
{\bf (modified)} One alternative is to estimate each $\delta_i$ and then set $t_i$, defined as the error-correction capabilities of the $i$-th group pairs, to be very close to (slightly larger) the estimation of $\delta_i$. It can save considerate communication overhead on transmitting the BCH code. However, to estimate all the $g$ values of $\{\delta_i\}_{i=1}^g$ in high accuracy requires much larger additional communication overhead than the savings. For example, estimating each $\delta_i$ requires $288$ bytes of additional communication overhead using the ToW estimator, as we will describe in \autoref{subsec:ToW}. However, the ``savings'' on the communication overhead for group pair $i$ is at most $t\log n-\delta_i\log n$, which is only $10$ bytes when $\delta_i=5, t=15, n=255$.

% {\bf (previous)} Readers may wonder if we can reduce this additional communication overhead by using some technique to estimate $\{d_i\}_{i=1}^g$ (e.g., ToW estimator in \autoref{subsec:ToW}), so that we can set the error-correction capability of each group more wisely and save some waste on the safety margin. However, to achieve that, the estimation on $\{d_i\}_{i=1}^g$ must be in extremely high precision (since $\{d_i\}_{i=1}^g$ are small numbers with mean of $\delta$), which incurs much larger additional communication overhead than the savings. Due to the same reason (i.e., estimate $\{d_i\}_{i=1}^g$ is costly), we set the number of subset pairs for each group pair to be all equal (denoted as $n$). 
%based on $\delta$ ($n=\Omega(\delta^2)$). 

{\bf (moved from the small d case)} Note that the set reconciliation process of the group pairs are independent with each other, and each group pair runs as many rounds of PBS-for-small-$d$ as needed to reconcile all distinct elements in it. Therefore, different group pairs may need different number of rounds to be successfully reconciled. Intuitively, we want all group pairs to be successfully reconciled in only a few rounds (say $3$) with high probability (say $99\%$). Hence, when tuning parameters (to be discussed in \autoref{sec:parameter_settings}), we set a {\it target success probability} $p_0$ combined with a {\it target number of rounds} $r$ as the {\it paramenter setting requirement}, which aims to ensure that the {\it success probability}, the probability that all distinct elements (of all group pairs) are reconciled, within $r$ rounds to be at least $p_0$. 
{\bf Normally, to achieve the same target success probability within fewer rounds (smaller $r$), PBS need more resources (e.g., larger $n$, $t$) for the ideal case happening with higher probability (fewer exceptions happen and need to be handled in later rounds), as we will explain in \autoref{sec:vary_r}.}

% {\bf (moved from the small d case)} Although PBS runs as many rounds as needed to reconcile all distinct elements (in each group pair), we want PBS to successfully reconcile all distinct elements in only a few rounds (say $3$) with high probability (say $99\%$). Hence, when tuning parameters (to be discussed in \autoref{sec:parameter_settings}), we set a {\it target success probability} $p_0$ combined with a {\it target number of rounds} $r$ as the {\it paramenter setting requirement}, which aims to ensure that the {\it success probability}, the probability that all distinct elements are reconciled, within $r$ rounds to be larger than $p_0$. 
% {\bf Normally, to achieve the same target success probability within fewer rounds (smaller $r$), PBS need more resources (e.g., larger $n$, $t$) for the ideal case happening with higher probability (fewer exceptions happen and need to be handled in later rounds), as we will explain in \autoref{sec:parameter_settings}.}

%This success probability (within $r$ rounds) is also the expected value of the {\it success rate} of PBS, which is defined as the number of `successful' experiments (all distinct elements are successfully reconciled within $r$ rounds) divided by the total number of experiments. 

%The requirement above should also ensure the majority of the distinct elements are reconciled in the first round. 
% Note that PBS reconciles the distinct elements gradually round by round. The distinct elements that have been reconciled in the first round are no longer needed to be reconciled again in later rounds. This is the ``piecewise decodability'' mentioned in \autoref{sec:intro_oursolution}. The requirement above also ensures the majority of the distinct elements are reconciled in the first round, as we will show in \autoref{sec:piecewise_decodability}. Therefore, the majority of the overall communication overhead happens in the first round. In other words, the overall communication overhead of all rounds is only slightly larger than ($1.01$ to $1.07$ times of) that in the first round. Due to this reason, we use the communication overhead in the first round (described in \autoref{sec:communication_overhead_single_PBS}) to approximate the overall communication overhead of all rounds in parameter settings (to be elaborated in \autoref{sec:parameter_settings}.


% Like what we did in \autoref{sec:multi-rounds}, we set a paramenter setting requirement on the target success probability $p_0$ of $r$ rounds for all group pairs, which ensures the probability that all group pairs are completely reconciled in $r$ rounds to be larger than $p_0$. The detail about how to set $n$, $g$, and $t$ given such a success probability requirement will be elaborated in \autoref{sec:parameter_settings}. 

% we set a {\it target success probability} $p_0$ of $r$ rounds as a paramenter setting requirement, which aims to ensure the probability that all distinct elements are reconciled in $r$ rounds to be larger than $p_0$. This requirement should also ensure the majority of the distinct elements are reconciled in the first round. Use the same example ($d=5, n=255$), on average $4.81$ out of $5$ distinct elements should be reconciled in the first round. So the total communication overhead in all rounds is only slightly larger than ($1.01$ to $1.07$ times of, as we will show in \autoref{fig:per-round-con}) that in the first round. Due to this reason, we use the communication overhead in the first round (described in \autoref{sec:communication_overhead_single_PBS}) to approximate the total communication overhead of all rounds in parameter settings (to be elaborated in \autoref{sec:parameter_settings}.

% Note that this safety margin incurs additional communication overhead on transmitting BCH codeword: In the perfect scenario (i.e., $\{d_i\}_{i=1}^g$ is precisely known), the average communication overhead on transmitting BCH codeword per group is $\delta\log n$; On the other hand, when we set $t$ to be the error-correction capability for each group, then the average overhead becomes $t\log n$, which is roughly $2.5$ times of that in the perfect scenario (when $t$ is roughly $2.5\delta$). Readers may wonder if we can reduce this additional communication overhead by using some technique to estimate $\{d_i\}_{i=1}^g$ (e.g., ToW estimator in \autoref{subsec:ToW}), so that we can set the error-correction capability of each group more wisely and save some waste on the safety margin. However, to achieve that, the estimation on $\{d_i\}_{i=1}^g$ must be in high precision, which requires a much higher communication overhead than the savings.

% Although PBS may need to run many rounds to reconcile all distinct elements, the communication overhead mostly happens in the first round, since the majority of the distinct elements should be reconciled in the first round. Use the same example ($d=5, n=255$), on average $4.81$ out of $5$ distinct elements should be reconciled in the first round. So the total communication overhead in all rounds is only slightly larger than ($1.01$ to $1.07$ times of, to be shown in \autoref{fig:per-round-con}) that in the first round. Due to this reason, we use the communication overhead in the first round (described in \autoref{sec:communication_overhead_single_PBS}) to approximate the total communication overhead (all rounds) in parameter settings (to be elaborated in \autoref{sec:parameter_settings}).

%For the moment, we assume no ``fake'' distinct element in type (\RN{2}) subset pairs fails to be detected, which happens with overwhelming probability as explained in \autoref{subsec:exception_hash_partition}. Then 

% PBS reconciles the distinct elements gradually round by round. This is the ``piecewise decodability'' mentioned in \autoref{sec:intro_oursolution}. We use the following example to describe it in details: 
% Given two sets with $10$ distinct elements, in the first round, PBS tries to reconcile the $10$ distinct elements and say $6$ out of the $10$ distinct elements are successfully reconciled. Then the $6$ reconciled distinct elements are removed and PBS tries to reconcile the remaining $4$ distinct elements in the second round. Say $2$ out of the $4$ remaining distinct elements are successfully reconciled, and that leaves $2$ remaining distinct elements to be reconciled in the third round, so on so force. 
% % Given two sets $A$, $B$ with $10$ distinct elements, in the first round, PBS hashes them into $7$ distinct subset pairs. $6$ distinct elements are hashed into $6$ distinct subset pairs, and the other $4$ distinct elements are hashed into the same subset pair. Then the former $6$ distinct elements are successfully reconciled in the first round and the later $4$ distinct elements remain to be reconciled in the second round, which are hashed into $3$ distinct subset pairs (under a different hash function). $2$ remaining distinct elements are hashed into $2$ distinct subset pairs, and the other $2$ remaining distinct elements are hashed into the same subset pair. Then the former $2$ remaining distinct elements are successfully reconciled in the second round and the later $2$ remaining distinct elements remain to be reconciled in the third round, so on so force. 
% The dynamics of the number of remaining distinct elements (i.e., $10\leadsto 4\leadsto 2\leadsto \cdots$ in the example) is in nature a Markov chain, which will be elaborated and analyzed in \autoref{sec:single_markov} to derive a tight tail bound of the probability that all distinct elements are reconciled in $r$ rounds. 

%, which we will show in \autoref{subsec:mini-partition}.

% The same algorithmic trick can also be implemented in PinSketch~\cite{Dodis_PinSketch_2008} to reduce it computational complexity from $O(d^2)$ to $O(d)$. However, it will encounter the same randomness problem and have to set up a safety margin on the error-correction capability. This safety margin will incur much more communication overhead on PinSketch than on our scheme: Considering the average communication overhead per group, in our scheme, this overhead can be expressed as $t\log n+\delta\log n+\delta \log u+32$, in which $t\log n$ accounts for the BCH codeword, $\delta\log n$ accounts for the index of the subset pairs, $\delta \log u$ accounts for the bitwise \code{XOR} in \autoref{alg:trivial_case}, and $32$ accounts for the $32$-bit CRC in \autoref{proto:multirounds}. In PinSketch, this overhead increases from $O(\delta\log u)$ (optimal) to $O(t\log u)$ (PinSketch does not need to transmit bitwise \code{XOR}) if it uses the same algorithmic trick. Use the same example in \autoref{sec:intro}, when $\delta=5, n=255, u=2^{32}, t=2.5\delta$, the overhead of PinSketch using the trick is $2.5$ times of the optimal, while that of our scheme is $2.075$ times of the optimal (as we introduced in \autoref{sec:intro_oursolution}). That means our scheme has a lower communication overhead than PinSketch if they both use the algorithmic trick. Furthermore, as the signiture size $\log u$ increases, the advantage of our scheme over PinSketch becomes more significantly, which we will show in \autoref{subsec:mini-partition}.

% In PinSketch, each bit encodes only a single element in the universe, so the size of the bitmap is equal to the size of the universe.  
% For example, in the set reconciliation problem we usually assume each element is ``indexed" by a $32$-bit-long (hash) signature, so the universe contains a total of $2^{32}$ elements. In this case, the bitmap encoding for any set in PinSketch is $2^{32}$ bits long, and the Galois field involved in its BCH decoding is the ``$32$-bit-wide" $GF(2^{32})$.  In contrast, as explained earlier, in PBS 
% %since each bit encodes the oddness or evenness of the cardinality of a subset,   
% the size $n$ of a bitmap is dependent only on $d$, and not on the size of the universe or on the cardinality of the set the bitmap encodes.   For example, as shown in the example above, $n = 255$ is large enough for $d = 5$.  In this case, the BCH decoding operates in the much shorter
% ``8-bit-wide" $GF(2^{8})$.  This shorter ``width" alone in theory translates into roughly $16$ times shorter BCH decoding time, which as will be explained in~\ref{} grows quadratically with the ``width" of the underlying Galois field.  This shorter ``width" also implies four times shorter BCH codeword in PBS than in PinSketch, resulting in lower communication complexity as will be shown in~\autoref{}.

% Note that our scheme only takes 1 round trip delay to both identify the $d$ subset pairs and reconcile them: In the first half, Bob computes and sends PBS to Alice. Then Alice locally identifies the $d$ subset pairs and then initiates the reconciliation ({\it i.e.,} \autoref{alg:trivial_case}) for them, {\it i.e.,} computes the bitwise \code{XOR} of the corresponded $d$ subsets. In the second half, Alice sends the bitwise \code{XOR} of the $d$ subsets with their indexes to Bob. Then Bob can compute the set difference $A\Delta B$ locally.


% We can certainly use some communication-efficient technique to estimate $d_i$ (e.g., \autoref{subsec:ToW}). However, to obtain $d_i$ precisely will require a communication cost almost as large as to reconcile Group $i$. So instead of obtaining $d_i$ and set $c_i$ (i.e., the error-correction capability of Group $i$) equal to $d_i$, we leave the randomness of $d_i$ and set $c_i$ neither too conservative, nor too libertive in the following sense: (1) $c_i$ is not too big (conservative, i.e., $10\delta$) to make the total size of PBS unnecessarily large and incur too much extra communication overhead; (2) $c_i$ is not too small (libertive, i.e., $\delta$) to incur a high probability of insufficient decode capability, which can result in hefty penalties in the latter case of incorrect decoding (will be elaborated in \autoref{sec:BCH_exception}). In our scheme, we set $c_i$ to be $2-3$ times of $\delta$, which will be shown in \autoref{sec:tail_bound} that it is just enough to make the probability of decode failure very small. Meanwhile, we set the error-correction capability of each group ($c_1,c_2,...,c_k$) to be all equal and denote it as $c$. 

%Since the decoding capacity $t$ and the number of subset pairs for each group $n$ are both small constants independent of $d$, therefore, the communication overhead per group is $t\cdot\log n \!=\!O(1)$, which implies a total communication overhead of $O(d)$. Similarly, the total decoding computational complexity is also $O(d)$. 

% \subsection{Exception Handling}\label{sec:exceptions}

% \subsubsection{Exception Handling on Hash-Partition}\label{subsec:exception_hash_partition}

% As we have described in \autoref{sec:hash_partition}, the ideal case does not always happen, which means some subset pair may contain more than 1 distinct elements and cannot be successfully reconciled by \autoref{alg:trivial_case}. Due to the parity encoding, we can classify such subset pair into the following two scenarios:

% \begin{itemize}
%     \item Scenario 1: If a subset pair $(A_i, B_i)$ contains even number ($\geq 2$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be the same and our scheme will not reconcile the subset pair. Hence, the distinct elements in the subset pair will not be reconciled;
%     \item Scenario 2: If a subset pair $(A_i, B_i)$ contains odd number ($\geq 3$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be different and our scheme will reconcile the subset pair using \autoref{alg:trivial_case}. However, as we described in \autoref{subsec:protocol0}, when a subset pair contains more than 1 distinct elements, \autoref{alg:trivial_case} will output the bitwise \code{XOR} of them as the `distinct element', which is not a real distinct element with high probability;
% \end{itemize}

% In both scenarios, the distinct elements in the subset pair cannot be reconciled. Even worse, in the second scenario, a false-positive could happen (i.e., the output of \autoref{subsec:protocol0} is not a real distinct element). For example, if subset pair $(A_i, B_i)$ contains $3$ distinct elements $s_1, s_2, s_3$, then the output of \autoref{alg:trivial_case} is $\tilde{s}_4=s_1\oplus s_2\oplus s_3$, which is normally not a distinct element. The good thing is, the probability of the false-positive is extremely small for small $d$. For instance, if $d=5$ and $n=255$, the probability of the false-positive is $7.6\times 10^{-6}$, which is very small. To further reduce the chance of false-positives, we add a verification step at the end of \autoref{subsec:protocol0} to check whether the output of \autoref{subsec:protocol0} $s$ is a real distinct element or not. The verification step works as follows: Given the output $s$ of subset pair $(A_i,B_i)$, if $s\in\mathcal{U}_i$ (i.e., $h(s)=i$), we consider $s$ as a real distinct element; Otherwise, we consider $s$ as an incorrect output and discard it. 

% Note that if $s$ is a real distinct element of $(A_i,B_i)$, $s$ must be in sub-universe $\mathcal{U}_i$. However, if $s$ is the bitwise \code{XOR} of the distinct elements in $(A_i,B_i)$ (i.e., the second scenario happens), $s$ could be in any sub-universe other than $\mathcal{U}_i$. In fact, if we assume the hash-partition described in \autoref{sec:hash_partition} hashes the elements of $\mathcal{U}$ uniformly, independently, and randomly into $n$ sub-universes, the output $s$ in the second scenario will be in a different sub-universe $\mathcal{U}_j (j\neq i)$ with a high probability of $1-\frac{1}{n}$. Hence, this verfication method can further reduce the probability of false-positives by a factor of $\frac{1}{n}$. Use the same example (i.e., $d=5$, $n=255$), the probability is reduced from $7.6\times 10^{-6}$ to $3\times 10^{-8}$ by this verification method. 

% In some super critical cases (i.e., no false-positive is allowed), we can use a more powerful verification method to completely eliminate false-positives. That is, to check if the output $s$ exists in exactly one of the two sets (i.e., $s\in A\setminus B$ or $s\in B\setminus A$). To do so, Bob transmits $s$ along with an identification bit $\mathbb{1}_{\{s\in B\}}$ to Alice, then Alice checks if $s$ . This method verification costs $d(\log u+1)$ bits of additional communication overhead. In most applications, rigorously $0\%$ probability of false-positives is unnecessary and the probability of the former verification method is small enough, so we use the former verfication method in our evaluation. Based on our observation, the false-positive does not happen even once in our evaluation using the former verfication method.

\subsection{Exception Handling on BCH Decoding}\label{sec:BCH_exception}

There is an additional type of exceptions that arises only from setting the universal error-correction capability $t$. That is, when $\delta_i$ (i.e., the number of distinct elements in group pair $i$) is larger than the error-correction capability $t$, the BCH codewords of group pair $i$ could differ at more than $t$ bit positions (e.g., in the ideal case, the BCH codewords differ at exactly $\delta_i$ bit positions), which exceeds the error-correction capability $t$. If so, the BCH decoder cannot decode the bit errors correctly (\autoref{step:BCH_decode} in \autoref{alg:single_round_pbs}) and report a failure. This exception happens with a small probability in each group pair: For example, when $d=1000$, and $\delta$ is set to $5$ (so that $g=d/\delta=200$), and $t$ is set to $13$ ($2.6$ times of $\delta$), the probability that this exception happens is only $6.7\times 10^{-4}$. 

% The exceptions that happens when the error-correction capability $t$ is sufficient have been discussed and handled in \autoref{subsec:exception_hash_partition} and \autoref{sec:multi-rounds}. In this section, we only discuss the exceptions that are caused by insufficient error-correction capability. That is, when $\delta_i$ (i.e., the number of distinct elements in group pair $i$) is larger than the error-correction capability $t$, the BCH codewords of group pair $i$ differ at $\delta_i$ bit positions in the ideal case, which exceeds the error-correction capability $t$. If so, the BCH decoder cannot decode the bit errors correctly (\autoref{step:BCH_decode} in \autoref{alg:single_round_pbs}) and report a failure. This exception happens with a small probability in each group pair: For example, when $d=1000$, and $\delta$ is set to $5$ (so that $g=d/\delta=200$), and $t$ is set to $13$, the probability that this exception happens is only $6.7\times 10^{-4}$. 

To handle this type of exceptions, we use the same algorithmic trick in \autoref{subsec:protocol2} to further partition each trouble-causing group into $3$ sub-groups and reconcile them respectively using PBS-for-small-$d$. 
%Note that $\delta_i$, if is not smaller, should be only slightly larger than $t$ with high probability. Hence, partitioning into $3$ sub-groups is enough to ensure each sub-group has no more than $t$ distinct elements. 
Note that $\delta_i$ is a Binomial random variable with mean of $\delta$, $t$ is $2$ to $3$ times of $\delta$. So the probability that some sub-group contains more than $t$ distinct elements conditioned upon $\delta_i>t$ is tiny. 
In the same example above ($d=1000$, $\delta=5$, $t=13$), this conditional probability is $9.5\times 10^{-10}$.%that some sub-group has more than $t$ distinct elements is $9.5\times 10^{-10}$. 
So in the next round, each sub-group will hardly encounter this type of expections and can be reconciled by PBS-for-small-$d$ respectively.  More specifically, we add a termination condition of \autoref{alg:3_way_partition} after \autoref{step:BCH_decode} in \autoref{alg:single_round_pbs}.

\begin{algorithm}
\caption{Termination condition when BCH decoding fails}
\label{alg:3_way_partition}

\If{BCH decoding fails\label{step:if1}}
{Hash-partition the group into $3$ sub-groups and run PBS-for-small-$d$ for each of them in the next round; Break;}\label{step:term1} 

\end{algorithm}

% Back to the \autoref{proto:multirounds}, which shows the set reconciliation operations in each round of PBS-basic, this kind of exceptions only affect \autoref{step:reconcile} in \autoref{proto:multirounds}. Now this step needs to check whether BCH decoding is successful or not: If successful, all the operations remain the same; Else, we hash-partition the group ($A$ and $B$) into $3$ sub-groups and reconcile them respectively using \autoref{proto:multirounds}. 
% {\bf I'm not sure if it is necessary to discuss this case, since PinSketch did not mention it, even it may happen in PinSketch}
% Another type of exceptions that happens when $d_i>t$ is, the BCH decoder mistakes the decoding is successful and returns $t$ incorrectly decoded bit errors (i.e., subset pairs). The probability of this type of exceptions is very small. For instance, when $d=1000, \delta=5, t=13$ $(2.5\delta)$, $d_i>t$ happens with probability roughly $6.7\times 10^{-5}$, and the probability that the BCH decoder mistakes the decoding is successful when $d_i>t$ is on the order of $10^{-7}$ \cite{kim1996undetected}. So the probability that this type of exceptions happens in each group is on the order of $10^{-12}$. On the other hand, the impact of this type of exceptions is insignificant. Assume an incorrectly decoded bit error corresponds to a random subset pair, which could contain (1) no distinct element; (2) exactly $1$ distinct element; or (3) more than $1$ distinct elements. Reconcile the subset pair using \autoref{alg:trivial_case} could (1) get nothing and waste $\log |\mathcal{U}|$ bits of communication overhead; (2) get an actual distinct elements; or (3) trigger the exceptions that were discussed and handled in \autoref{subsec:exception_hash_partition}. 

\subsection{What if PinSketch also uses partitions?}

Arguably, the same algorithmic trick (i.e., hash-partition two sets each into groups) can also be implemented in PinSketch~\cite{Dodis_PinSketch_2008} to reduce it computational complexity from $O(d^2)$ (of finite field operations in GF($2^{32}$)) to $O(d)$. However, it will encounter the same randomness problem and have to set up a ``safety margin'' on the error-correction capability $t$. This ``safety margin'' will incur much more additional communication overhead on PinSketch than on our scheme: Considering the average communication overhead per group pair, the additional overhead caused by the ``safety margin'' is $(t-\delta)\log n$ in PBS and $(t-\delta)\log |\mathcal{U}|$ in PinSketch. The later is roughly $4$ times of the former under the default setting ($n=255, |\mathcal{U}|=2^{32}$). Recall that the theoretical minimum amount of communication overhead to reconcile $d$ distinct elements is $\delta\log |\mathcal{U}|$. Use the same example in \autoref{sec:intro}, when $\delta=5, n=255, |\mathcal{U}|=2^{32}, t=2.5\delta$, the overhead of PinSketch using the algorithmic trick is $2.5$ times of the theoretical minimum, while that of PBS is $2.075$ times of the theoretical minimum. It means PBS could have a lower communication overhead than PinSketch if they both use the algorithmic trick. Furthermore, as the signiture length $\log |\mathcal{U}|$ increases, the advantage of PBS over PinSketch will be more significant.

% We handle this type of exceptions by the same method (i.e., hash-partition into $3$ sub-groups) as above. To detect them, on the other hand, is simple: Note that incorrect decoded bit errors correspond to the subset pairs that do not contain distinct elements. When we reconcile those subset pairs in \autoref{sec:reconcile_by_trivial}, the output (i.e., reconciled elements) will be $\mathbf{0}$, which is abnormal (since $\mathbf{0}\notin A\bigcup B$, as we described in \autoref{subsec:protocol0}). Hence, this type of exceptions happen if and only if one of the reconciled distinct elements is $\mathbf{0}$. 
%Hence, we consider BCH decoding is successful by two criteria: (1) the BCH decoder reports a successful decode; and (2) None of the reconciled elements is $\mathbf{0}$. 
% ========================
% In fact, even if $d_i>t$, PBS-basic is still possible to reconcile group $i$ in some nonideal cases. For example, when $t=10$ and $d_i=11$, if the $11$ distinct elements are distributed in $10$ subset pairs, such that $1$ subset pair contains $2$ distinct elements and $9$ subset pairs contain $1$ distinct element in each, the two parity bitmaps differ at only $9$ bit positions. So BCH decoder is able to decode the later $9$ subset pairs and the corresponding $9$ distinct elements can be reconciled. In the second round, only $2$ distinct elements remain and BCH decoding certainly works. In this case, we do not need to partition the group into sub-groups, and this case does not trigger \autoref{alg:3_way_partition} in PBS. 
% ========================
% Instead, it will either (1) report a failure about exceeding the error-correction capability; or (2) mistake the decoding is successful and return incorrect decoded bit errors. 

% The second case happens with a very small probability (in order of $10^{-7}$ \cite{kim1996undetected}) and is very simple to detect : 

% The first case is easy to handle: We can simply adapt the same algorithmic trick to partition the group into smaller groups and reconcile them respectively. In our scheme, we set the number of smaller groups to be $3$, which is big enough because $d_i$, if not smaller, only slightly larger than $t$ with high probability. The second case on the other hand, although theoretically possible, happens with a very small probability when $d_i>t$ (in order of $10^{-7}$ \cite{kim1996undetected}). Besides, the probability of $d_i>t$ is also very small (e.g., when $t=15$ and $\delta=5$, this probability is about $2.3\times 10^{-4}$), so the overall probability of the second case, which is the multiplication of these two small numbers, is negligible (e.g., in order of $10^{-11}$).

% \subsection{Multi-rounds}

% Even if the ideal case does not happen, most of the distinct elements should be distributed into different subset pairs and therefore can be reconciled. So our scheme, even cannot reconcile all of the distinct elements, can still reconcile the majority of them (piecewise decodability). To reconcile the rest distinct elements, we can just run our scheme for multi-rounds under different hash-partition functions. For each round, our scheme works as follows: 

% \IncMargin{1em}
% \begin{algorithm}
% \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
% \Input{Two sets $A$ and $B$}
% \Input{Size of set difference $d$}
% \Input{The number of subset pairs $n$}
% \Input{BCH error-correction capability $t$}

% Hash-partition $A$ and $B$ into $n$ subset pairs $\{(A_i,B_i)\}_{i=1}^n$;

% \If{BCH decoding fails}
% 	Hash-partition $A$ and $B$ into $3$ subset pairs and reconcile them respectively in the next round\;
% \ElseIf{BCH decoding success}
	
% \Else{}

% $k \leftarrow \lceil \frac{t}{c}\rceil $\;

% Partition elements into $k$ subsets using~\autoref{alg:random-part}\;

% \For{$j = 0$ \KwTo $k-1$}{
%     Reconcile the $j$-th subset pair using the straw-man scheme with the BCH correcting capability $\tau$, number of smaller subsets $m$, and number of rounds $r$\;
% }

% \caption{PBS (per round)} \label{proto:II}
% \end{algorithm}\DecMargin{1em}

% This {\bf multi-rounds} scheme can significantly increase the success probability (i.e., the probability that all distinct elements are reconciled). Readers may wonder in the later rounds, most distinct elements should be reconciled, and the remaining could be reconciled using degraded parameters (i.e., smaller $n$ and $t$). In fact, degrade parameters in later rounds cannot save much communication overhead, since the majority of it is spent in the first round (i.e., $>90\%$). Therefore, we use the same parameters (i.e., $n,t$) among all rounds in our evaluation. 
% %The tradeoff between the number of rounds and the communication overhead per rounds will be elaborated in \autoref{sec:tail_bound}. In our evaluation, $r=2,3$ rounds are enough to achieve an extremely high success probability. 

% Readers may think the cost (i.e., communication overhead and the computational complexity) of this multi-rounds scheme is proportional to the number of rounds (denoted as $r$) and increases linearly with $r$. In fact, the cost of each round is roughly proportional to the number of remaining distinct elements, which decreases exponentially as $r$ increases (i.e., the first round reconciles $99\%$ of distinct elements, the second round reconciles $99\%$ of the remaining $1\%$ distinct elements, etc.). So the cost of this multi-rounds scheme is only slightly larger than that of the single-round scheme. Furthermore, as we explained in \autoref{sec:intro}, {\bf from intro thanks for the piecewise decodability of our solution, in almost all practical application scenarios, this tradeoff does not lead to longer response time because the reconciliation of objects identified by the successfully decodable codewords, which constitute the vast majority of all codewords, can run in parallel with the transmissions and decodings of the rest.  In other words, the piecewise decodability effective masks the slightly larger number of communication rounds as far as the response time is concerned.} 





\begin{comment}
\subsubsection{Random Partition}

\IncMargin{1em}
\begin{algorithm}
% \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
% \Input{Set $S$}
% \Input{The number of subsets $m$ for partition}
% \Output{Subsets $S_1, S_2, ..., S_m$}

% Generate hash function $h(\cdot)$ that maps each element into $\{1,2,...,m\}$;

\ForEach{$s \in S$}{
    $j \leftarrow h(s) \bmod m$\;    
    Insert $s$ into the $j$-th subset $S_j$\;
}

\caption{Partition using hash function $h(\cdot)$.} \label{alg:random-part}
\end{algorithm}\DecMargin{1em}

Like the strawman scheme, our scheme randomly partitions sets $A$ and $B$ into $m$ subsets. This random partition 
can be easily accomplished by using some hash function, $h(\cdot)$, and inserting each element $x$ into the subset 
corresponding to $h(x)$. \autoref{alg:random-part} presents the pseudo-code of this random partition using hash 
function $h(\cdot)$.  

% Unlike the strawman scheme, our scheme only reconciles those subset pairs that need to be reconciled, 
% because 



Like the strawman scheme, our scheme hash-partitions the two sets $A$ and $B$ into $m$ subset pairs $(A_i, B_i)$ for $i=1,2,\cdots,m$. 
We note that, among those $m$ bins (subset pairs), 
at most $t$ ($t\!\ll\!m$ as shown in our analysis in~\autoref{subsec:protocol1}) bins contain balls 
(elements belonging to the set difference), {\it i.e.,} requiring reconciliation.  
Motivated by this observation, we, therefore, propose to first detect those bins that 
contain balls and then only reconcile them. The detection is solved with a simple encoding approach that 
will be detailed in the next section.

\subsubsection{Detection before Reconciliation} 

In fact, identifying those non-empty bins is easy when each bin contains at most one ball. In this section, we assume that 
each bin after the random partition contains at most one ball, we will show later how to handle the cases when some 
bins contain more than one balls later in~\autoref{subsec:exceptions}. 

Given an arbitrary bin (say subset pair $(A_i, B_i)$) that contains one ball ({\it i.e.,} $A_i\Delta B_i$ contains exactly one element), 
the corresponding two subsets $A_i$ and $B_i$ differ exactly one element, which implies that 
$||A_i|\!-\!|B_i||\!=\!1$. Hence, if $|A_i|$ ({\it i.e.,} number of 
elements in $A_i$) is odd (or even), then $|B_i|$ must be even (or odd). In other words, the odevity of $|A_i|$ 
and $|B_i|$ are opposite. %differs if $|A_i\Delta B_i|\!=\!1$. 
Based on this property, we propose the {\it odevity encoding}: 
A subset is encoded as ``1'' if it contains odd number of elements, and as ``0'' otherwise. 
Using this odevity encoding, the $m$ subsets of $A$ can be encoded as a bit string $b_A$ in $\{0,1\}^m$, 
where the $i$-th bit in $b_A$ corresponds to the odevity encoding of $|A_i|$. Similarly, the $m$ subsets of $B$ can also 
be encoded as a bit string $b_B$. Clearly, $b_A$ and $b_B$ differ at $t$ different positions, or in other words, 
the Hamming distance of bit strings $b_A$ and $b_B$ is $t$. A straightforward approach is 
to let Alice send $b_A$ to Bob, and then Bob compares $b_B$ against $b_A$ to obtain those non-empty bins. 

This approach, however, has a communication overhead of $m$ bits, which is still unnecessarily high. As 
analyzed in~\autoref{subsec:protocol0}, $t$ is usually much smaller than $m$. 
That means $b_A$ and $b_B$ differ only at a tiny portion of bits. %have much more in common than differences. 
Therefore, if we view $b_B$ as a corrupted message of $b_A$ with $t$ corrupted bits, the detection of those $t$ bins can be converted to 
the detection of the positions of the $t$ corrupted bits. The latter can be solved using an Error-Correction Code (ECC)~\cite{Lin_ErrorControlCoding_1983} that can correct up to $t$ errors. In this work, we use the BCH code~\cite{Lint_IntroductionCodingTheory_1998}. 
More precisely, this ECC-based approach (with the BCH code) works as follows. 
Alice computes the parity bits for $b_A$ using a $t$-error-correcting BCH code with a block length of 
$(2^{\lceil \log m\rceil} -1)$ and sends the parity bits to Bob. Bob then decodes the positions of the $t$ corrupted bits 
using the BCH decoding algorithm with $b_B$ and those parity bits received from Alice. The communication overhead of 
this approach is roughly $t\lceil \log m\rceil$ ($=O(t\log t)$) bits. In the example above, this communication overhead is 
roughly $\num{17000}$ bits, which is approximately $6$ times lower 
than $m\!=\!\num{108469}$ bits, the communication overhead of the aforementioned straightforward approach. 

At first sight, it seems that the detection of non-empty bins and reconciliation of subsets in those bins require two rounds 
(or at least two round trip delays), {\it i.e.,} one round for detection and the other for reconciliation. In fact, 
it only requires one. After Bob receives the parity bits from Alice and decodes out those non-empty bins, it initiates 
the reconciliation ({\it i.e.,} \autoref{alg:trivial_case}) for each bin (subset pair) immediately, 
{\it i.e.,} sends the \code{XOR} sums of subsets in those bins together the indexes of those bins. 
After receiving those \code{XOR} sums and bin indexes, Alice can compute the set difference. 

% A naive way to combine the detection of non-empty bins and reconciliation of subset pairs in those bins is to first detect 
% those non-empty bins via one round of message exchanges between Alice and Bob and then to reconcile the corresponding 
% subset pairs in those bins with another round of message exchanges. This requires two rounds ({\it i.e.,} taking at least 
% two round trip delays). In fact, after Bob receives the parity bits from Alice and obtains those 

\subsubsection{Multiple Rounds}\label{sec:multiround}

{\bf This section was not clear enough. I need more time to think about and revise it.}


In the above section, we have assumed that each bin contains at most one ball. 
However, even with a sufficient large $m$, some bin might contain more than one balls though with tiny probability. 
We will show in~\autoref{subsec:exceptions}, how such rare events, {\it i.e.,} one bin contains more than one balls, 
can be easily detected.
To ensure our scheme can successfully reconcile all elements even when such rare events happen, 
we propose to use multiple rounds (of communication between Alice and Bob). More precisely, instead of 
selecting a prohibitively large $m$ to ensure that each bin contains at most one ball with a extremely high probability 
(say 0.99999), we select a reasonably large $m$ so that the communication overhead is not very high and very few bins contain 
more than one balls (or in other words, most bins contain at most one ball). Therefore, after running one round of 
our scheme, most elements in the set difference will be reconciled. Only those in the bins that contain more than one balls 
fail to be reconciled. For elements in the subsets corresponding to those bins, we run another round of our scheme. 
If some elements still fail to be reconcile, we can run one more round of our scheme. So on so forth,  
our scheme can keep running for more rounds until all elements are reconciled. 

With the same communication overhead, multiple rounds can significantly increase the success rate, 
{\it i.e.,} the probability that all elements in the set difference will be successfully reconciles, 
which will be elaborated in~\autoref{sec:tail_bound}. 

% % to be emphasized
% % say that too many rounds should be avoided (latency & communication overhead reduction is negligible when r is too large, 2 - 3 is good enough)
% % multiple rounds is not an issue when r is small

% We note that the number of rounds $r$, however, should not be large. On one hand, it results in large latency (at least $r$ round trip delays). 
% On the other hand, when $r$ is large, the reduction of communication overhead by the increase of $r$ gradually diminishes. 

We note that multiple rounds, when $r$ is small, would not really increase the ``latency'', as long as most elements in the 
set difference can be reconciled in the first rounds, since the underlying synchronization of data objects corresponding to 
those elements can start immediately after the first round of our scheme. Therefore, the actual latency is one round trip delay instead of 
$r$. 

As we mentioned, this straw-man protocol works correctly if each subset pair has at most one exclusive element (i.e., \autoref{eq:requirement_strawman} holds). On the other hand, if a subset pair has more than one exclusive elements, some of which will not be successfully reconciled:

\begin{itemize}
\item If a subset pair has even number of exclusive elements, Odevity coding will encode it as 0. Then the straw-man scheme will consider the subset pair having no exclusive element and all exclusive elements in this subset will not be reconciled;

\item If a subset pair has odd number ($\geq 3$) of exclusive elements, Odevity coding will encode it as 1 and consider the subset pair having only 1 exclusive element. Then the straw-man scheme will use \autoref{alg:trivial_case} to decode only one exclusive element and dismiss all others. Even worse, the only decoded element is probably not a real exclusive element, since the element computed by \autoref{alg:trivial_case} is the \code{XOR} sum of all exclusive elements, not one of them. 
\end{itemize}

In summary, if a subset pair has more than one exclusive elements, most of its exclusive elements cannot be reconciled, and the reconciled element is usually incorrect (i.e., false-positive). The false-positive however is easy to check, which will be elaborated in \autoref{subsec:exceptions}. The good thing is, even if not all subset pairs have at most one exclusive element and are successfully decoded, most of them will be w.h.p.. In other words, even if the straw-man protocol cannot reconcile all exclusive elements, it still can reconcile most of them. To reconcile all exclusive elements w.h.p., we can simply extend the single-round straw-man scheme to multi-round. And each round adapts the straw-man scheme to do set reconciliation using independent hashing functions $h(\cdot)$ for partition (i.e., in \autoref{alg:random-part}). This multi-round extension can significantly increase the probability of a successful reconciliation, which will be elaborated in \autoref{sec:tail_bound}. 



\subsection{Our Scheme: The Final Version}\label{subsec:protocol2}

{\bf Under revision~}

The preliminary version of our scheme suffers from two major drawbacks. 
First, its communication overhead is asymptotically 
$O(t\log m)\!=\!O(t\log t)$, which is not asymptotically optimal. 
Second, the decoding computational complexity is proportional to 
$t^2$ with the state-of-the-art decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} for BCH codes, 
which is too high when $t$ is large. 
To overcome these two drawbacks, we use a simple algorithmic trick: divide and conquer. With this algorithmic 
trick, the decoding computational complexity is reduced to $O(t)$, 
and the communication overhead is reduced to $t\cdot\frac{\log u}{8} \!+\! O(t)$ (with a small 
hidden constant roughly varying from 4 to 8) bytes which implies that 
our scheme has an additive communication overhead (compared to the optimal scheme) 
of 4 to 8 bytes per element in the 
set difference and this additive overhead is independent of the key size ({\it i.e.}, $\log u$). 
Recall that the IBF-based schemes usually have a communication overhead of roughly 6 times of the 
optimal scheme, which increases linearly as the key size. Therefore, our scheme is much more 
communication-efficient. 

Now, we describe in detail this algorithmic trick. We let Alice divide elements in $A$ into $\lceil\frac{t}{c}\rceil$ groups (subsets)  
for some small constant $c$ (say $5$) so that each group contains roughly $c$ elements from the set difference on average. We let Bob do the same operations on $B$. To ensure that any common element ({\it i.e.,} any element $x\!\in\! A\bigcup B$) goes into 
the same group ({\it i.e.,} groups at Alice and Bob with the same index), we can use the partition procedure with a hash function shown 
in~\autoref{alg:random-part}. Then, we can apply the preliminary version on each group with a constant $m$ (say $m\!=\!256$) independent of 
$t$. To ensure that each group can be reconciled with a high probability, we need to use BCH codes whose decoding capacity 
larger than $c$ (say $\tau\!=\!2c$), as exact number of elements to be reconciled could be larger than $c$. 
Since this decoding capacity $\tau$ is still a small constant independent of $t$, therefore, the communication 
overhead per group is $\tau\cdot\log m \!=\!O(1)$, which implies a total communication overhead of $O(t)$. 
Similarly, the total decoding computational complexity is also $O(t)$. 

\subsubsection{Parameter Configurations} 

Our scheme now has several parameters: $c$ (average number of elements from the set difference in each group), 
$\tau$ (the correcting capability of the BCH code), $m$ (number of bins for each group), and $r$ (maximum number of rounds). 
We note that the maximum number of rounds $r$ is usually associated with another parameter $p$ the desired success rate: With 
at most $r$ rounds, our scheme should guarantee that the success rate is at least $p$. 
%How to tune these parameters to achieve favorable performance will be detailed later in~\autoref{sec:tail_bound}. 
Here, we provide some guidances for the parameter configurations using our theoretical analysis, which gives the tail bound of 
the success probability of our scheme and will be shown in~\autoref{sec:tail_bound}. 

\noindent
{\bf Parameterizing $c$ and $r$.} The values of $c$ and $r$ are usually provided by users based on the requirements of 
applications. For the value of $c$, a larger $c$ results in a longer decoding time yet lower communication overhead.  
So if the decoding time is a big concern, then a smaller $c$ (say $c=5$) should be used; otherwise, a larger $c$ could be used. 
For the values of $r$, a larger $r$ leads to lower communication overhead and usually lower decoding time (as it allows to use 
a smaller $\tau$), however, the reduction is marginal when $r>3$. Therefore, we suggest users to configure $r$ to be $2$ or $3$. 
% The configuration of $c$ is relatively straightforward, as a larger $c$ will result in 
% a longer decoding time and a slightly lower communication overhead. The former is ..., The latter is slightly tricky. 


\noindent
{\bf Using $c$ and $r$ to parameterize other parameters.} After users specify the values for $c$ and $r$ (associated with a value for 
$p$), we can use our theoretical analysis in~\autoref{sec:tail_bound} to parameterize $\tau$ and $m$. 
Since in a BCH code, the block length is in the form of $2^q-1$, we only need to consider $m=2^q-1$. 

{\bf Liang, please revise the following algorithm!}

\begin{algorithm}
\SetKwProg{Proc}{}{}{end}
\SetKwFunction{algo}{\small Search}

\Proc{Search($c$, $r$, $p$)}{\label{search:entrance}

$\mbox{co}_{best}\leftarrow\infty$\tcc*{\small Best communication overhead}

\For{$\tau \leftarrow c\,\KwTo\, \infty$}{}



}
\end{algorithm}


% , unlike 
% the IBF-based schemes which have an multiplicative overhead of 6 
% The inspiration is from the famous 
% divide and conquer algorithm for the selection problem, in which, given an array with $n$ elements, we want to get the $k$-th largest 
% element. A straightforward idea for this problem is sorting. However, if using insertion-sorting, the complexity would be $O(n^2)$. 
% Then the famous divide and conquer trick comes. It first divides the array into $\lceil n/5\rceil$ groups so that the first 
% $\lfloor n/5\rfloor$ contains $5$ elements and at most one group contains the rest $n \mod 5$ elements, and find the median of each 
% group using the insertion-sorting and th


% This straw-man scheme still has a problem on decoding computational complexity. More specific, the complexity increases dramatically with the total number of corrupted bits $t$. Therefore, when $t$ is moderate or large, the decoding computational complexity could be very high. For instance, the decoding complexity of BCH codes~\cite{Lint_IntroductionCodingTheory_1998} is $O(t^3)$, which could be quite high for a large $t$. To keep the decoding complexity reasonably low, we design the following two-layer protocol: In the first layer, we use a hash function to partition the two sets into $\lceil\frac{t}{c}\rceil$ subsets for some small constant $c$ (say $5$), just like the first step of our straw-man scheme. The objective, which is however different from before, is to make each subset pair contains roughly $c$ exclusive elements on average. In the second layer, we use the straw-man scheme with the same configuration (number of subsets $m$, and error-correction capability $\tau$, number of rounds $r$) to reconcile each subset pair. 

% In fact, the straw-man scheme is a proper solution when $t$ is small. First, the decoding complexity will not be a problem for a small $t$; Second, we do not need an extremely large $m$ to guarantee \autoref{eq:requirement_strawman} w.h.p.. For instance, when $t=5$ and $m=1024$, \autoref{eq:requirement_strawman} holds with probability $\frac{m\,!}{(m-t)\,!m^t}\approx 99\%$. This motivates us to design the following two-layer protocol: In the first layer, we use a hash function to partition the two sets into $\lceil\frac{t}{c}\rceil$ subsets for some small constant $c$ (say $5$), just like the first step of our straw-man scheme. The objective, which is however different from before, is to make each subset pair contains roughly $c$ exclusive elements on average. In the second layer, we use the straw-man scheme with the same configuration (number of subsets $m$, and error-correction capability $\tau$) to reconcile each subset pair. 

\autoref{proto:II} shows the pseudocode of our scheme. It first uses the same hash-function based random partition algorithm as \autoref{alg:random-part} to partition elements into $k\triangleq\lceil \frac{t}{c} \rceil$ subsets. Note that the random partition only guarantees that each such subset 
contains $c$ exclusive elements on average, and the exact number is not known. Hence, our scheme uses a BCH code with a capability of 
correcting up to $\tau$ errors with $\tau > c$ to make sure that the BCH code has a high probability to decode successfully. We will describe how to deal with situation where the size of set difference exceeds $\tau$ later in~\autoref{subsec:exceptions}.

As the decoding of a $\tau$-error-correcting BCH code where $\tau$ is a small constant has a constant-time computational complexity, the decoding complexity of 
our scheme is $O(k)=O(t)$. We now have several parameters, average number of exclusive elements in each subset $c$, the correcting capability $\tau$ of BCH code, the number of smaller subsets $m$ for each subset to be divided to, and the number of rounds $r$. How to tune these parameters to achieve favorable performance will be detailed later in~\autoref{sec:tail_bound}. 

\IncMargin{1em}
\begin{algorithm}
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
\Input{Size of set difference $t$}
\Input{The number of subsets $m$ for each partition}
\Input{Average number of exclusive elements in each partition $c$}
\Input{BCH code capability $\tau$}

$k \leftarrow \lceil \frac{t}{c}\rceil $\;

Partition elements into $k$ subsets using~\autoref{alg:random-part}\;

\For{$j = 0$ \KwTo $k-1$}{
    Reconcile the $j$-th subset pair using the straw-man scheme with the BCH correcting capability $\tau$, number of smaller subsets $m$, and number of rounds $r$\;
}

\caption{Our Scheme} \label{proto:II}
\end{algorithm}\DecMargin{1em}




\subsection{Exceptional Handling}\label{subsec:exceptions}

{\bf To be revised~}

In this section, we will elaborate how to handle the following two types of exceptions that we mentioned in \autoref{sec:multiround} and \autoref{subsec:protocol2}:
\begin{itemize}
    \item Exception 1: A subset pair has odd number ($\geq 3$) of exclusive elements and causes false-positives (i.e., a decoded distinct element is not a real one);
    \item Exception 2: A subset pair contains too many exclusive elements, such that a BCH code with capability of correcting up to $\tau$ errors cannot decode it (i.e., $t>\tau$).
	\item Exception 3: A subset pair has even number ($\geq 2$) of exclusive elements and causes false-negatives(i.e., two or more distinct elements are neglected as the parity bit is 0);
\end{itemize}

To handle Exception 1, we need to check whether a computed exclusive element by \autoref{alg:trivial_case} is a real exclusive element or not. (The group index happens to come in handy if we use it as a fingerprint of the element we computed. If this element is truly an exclusive element, it should be hashed into the same group as before. Notably, We have two group indices available for this check, one is in the initial divide and conquer phase, the other is in the BCH code part) It can be easily done at the end of set reconciliation, during which two hosts exchange their exclusive elements. In fact, as we will elaborate in \autoref{sec:tail_bound}, Exception 1 hardly happens if we set parameters properly. 

On the other hand, when Exception 2 happens, the BCH decoder will report a failure about exceeding the error-correction capability. For such a subset pair, we can use the same approach as in \autoref{subsec:protocol2} to partition it into smaller subsets and use the straw-man scheme to reconcile them respectively. We set the number of small subsets to be 3. It is because, as we will elaborate in \autoref{sec:tail_bound}, the number of exclusive elements for each subset pair $t$ should be, if not smaller, only slightly larger than $\tau$ w.h.p.. Partitioning those exclusive elements into 3 small subsets is enough to guarentee that each of them has less than $\tau$ exclusive elements.

\end{comment}

==> section/schemes_new0226.tex <==
%\section{PBS for small \texorpdfstring{$d$}{d}}\label{sec:scheme}
\section[PBS for small \texorpdfstring{$d$}{d}]{PBS for small \texorpdfstring{\larger\boldmath\MakeLowercase{$d$}}{d}}\label{sec:scheme}
%\section{Set Reconciliation}\label{sec:scheme}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%     Writing Guideline for This Section     %%%%%%%%%%
% “balls – elements in the symmetric difference of the two sets” 

% Protocol 0 (reconcile two sets whose set difference has at most one ball)

% Protocol I.I (partition elements into a sufficiently large number of subsets such that each subset has at most one ball with high probability and use Protocol 0 to reconcile each of them) 

% Protocol I.II (a two-step refinement of Protocol I.I: first use BCH to identify good bins, i.e., bins/subsets have exactly one ball, and then use Protocol 0 to reconcile each good bin) 

% Protocol II (a two-layer refinement of Protocol I.II: in the first layer, we partition elements into t/c subsets, where t is the size of set difference and c is a small constant, then each subset has c balls on average. In the second layer, we further partition each subset into large enough number of bins/subsets such that with high probability each bin has at most one ball, then use Protocol I.II to reconcile them one by one) 

% Protocol III/IV (mainly fix certain exceptions in Protocol II，e.g., how to address bad bins, how to handle the cases where BCH fails to decode and etc)

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% In this section, we describe our set reconciliation scheme in details. First, we give a formal problem statement in \autoref{sec:model}. In \autoref{subsec:protocol0}, we introduce a basic scheme for the trivial case, in which the two sets $A$ and $B$ has at most one distinct element. Building upon the basic scheme, we propose the preliminary version of scheme in \autoref{sucsec:our-scheme} that targets to the cases where the total number of distinct elements $d$ is small. Then we extend the preliminary version and propose the final version of our scheme in \autoref{subsec:protocol2} for general cases (i.e., any arbitrary $d$). We assume $d$ is precisely known throughout this section except in \autoref{subsec:ToW}, where we will describe how to estimate $d$ using a Tug-of-War Estimator. 


In this section, we describe how PBS scheme allows Alice and Bob to reconcile their respective sets $A$ and $B$, where $d=|A\Delta B|$ is small and precisely known. 
%Throughout this paper, we call each element in $A\Delta B$ a \textit{distinct element}, and each element in $A\bigcap B$ a \textit{common element}. 
We start with the trivial case where $d\leq 1$ in \autoref{subsec:protocol0}. Then we generalize our scheme to a more general case where $d$ is a small number in \autoref{sec:pbs_smalld}. 
% We build up our scheme gradually by starting with the trivial case where $d\leq 1$ in \autoref{subsec:protocol0}. Then we generalize our scheme to the case where $d$ is a small number in \autoref{sec:pbs_smalld}. 

\begin{comment}
\subsection{Problem Statement}\label{sec:model}

In this work, we adopt the commonly used model for the set reconciliation problem. 
Two remote sets $A$ and $B$ are stored at hosts Alice and Bob respectively. 
Each element in $A$ and $B$ is a hash signiture in the key space (universe) $\mathcal{U}$, which is the set of all $(\log |\mathcal{U}|)$-bit binary strings. 
%Each element in $A$ and $B$ is a hash signiture with signiture width $w$ in the key space (universe) $\mathcal{U}$, which is the set of all $w$-bit binary strings (i.e., $|\mathcal{U}|=2^w$). 
%We use $\mathcal{U}$ to denote the set of all $w$-bit binary strings and name it the universe of signitures. 
The set reconciliation problem is to compute the symmetric set difference between $A$ and $B$, 
{\it i.e.,} $A\Delta B\triangleq (A\!\setminus\! B) \bigcup (B\!\setminus\! A)$. 
Let $d\!=\!|A\Delta B|$ be the cardinality of this difference.
%We denote $d\!=\!|A\Delta B|$. 
Throughout this paper, we call each element in $A\Delta B$ a \textit{distinct element}, and each element in $A\bigcap B$ a \textit{common element}.
{\bf Like in all existing solutions, we describe only {\it unidirectional} set reconciliation, in which Alice or Bob learns the set difference $A\Delta B$. Since the performance of our scheme does not depend on who learns the set difference, we assume Bob learns the set difference $A\Delta B$ in the rest of the paper, as mentioned in \autoref{sec:psea}.}
% As mentioned in \autoref{sec:psea}, we describe {\it unidirectional} set reconciliation that Bob learns the set difference $A\Delta B$. 
%In \autoref{sec:evaluation}, we use the same semantic to measure the communication cost of our scheme and other compared set reconciliation schemes. 
\end{comment}

% In the rest of this section, we build up our scheme gradually as follows: We start with the trivial case where $d\leq 1$ in \autoref{subsec:protocol0}. Then we generalize our scheme to the case where $d$ is a small number in \autoref{sec:pbs_smalld}. 

%After that, we further generalize our scheme to the case that $d$ is a large number in \autoref{subsec:protocol2}. 
%Throughout this section, we assume $d$ is precisely known.
%except in \autoref{subsec:ToW}, where we will describe how to estimate $d$ using a Tug-of-War Estimator. 

%The rest of this section is organized as follows: In \autoref{subsec:protocol0}, we introduce a basic scheme for the trivial case, in which the two sets $A$ and $B$ has at most one distinct element. In \autoref{sucsec:our-scheme} and \autoref{subsec:protocol2}, we elaborate the two versions of our solution that are introduced in \autoref{sec:smalld} and \autoref{sec:larged} respectively. Throughout this section, we assume $d$ is precisely known except in \autoref{subsec:ToW}, where we will describe how to estimate $d$ using a Tug-of-War Estimator. 

\subsection{The Trivial Case of \texorpdfstring{\larger\boldmath $d\leqslant 1$}{d<2}}\label{subsec:protocol0}

%We start with the trivial case, in which $A$ and $B$ have at most one distinct element ({\it i.e.,} $d\leq 1$), we have a simple set reconciliation scheme showed in \autoref{alg:trivial_case}:
\begin{algorithm}
\caption{Set reconciliation when $d\le 1$}
\label{alg:trivial_case}

{\it Bob}: $s_B\leftarrow\underset{b\in B}{\oplus} b$; Send $s_B$ to Alice\; \label{alg1:sender}

{\it Alice}: $s_A\leftarrow\underset{a\in A}{\oplus} a$; $s\leftarrow s_A \oplus s_B$\; \label{alg1:receiver}
\end{algorithm}

\autoref{alg:trivial_case} shows the reconciliation scheme for the trivial case, in which $A$ and $B$ differ by at most one distinct element. It consists of two steps. First, Bob calculates $s_B$, the bitwise \code{XOR} of all elements in $B$, and send it to Alice. 
Second, Alice also calculates $s_A$, the bitwise \code{XOR} of all elements of $A$. Upon receiving $s_B$, Alice computes $s\!\triangleq\! s_A \!\oplus\! s_B$. According to whether $A$ and $B$ have a distinct element, there are the following two cases:

\begin{sitemize}
	\item Case \RN{1}: When $A$ and $B$ have no distinct element, we have $s_A=s_B$ and $s=\mathbf{0}$\footnote{$\mathbf{0}$ denotes the $\log |\mathcal{U}|$-bit-long all-0 string.};
	\item Case \RN{2}: When $A$ and $B$ have exactly one distinct element, the computed $s$, the bitwise \code{XOR} of $s_A$ and $s_B$, will cancel out all the {\it common elements}, defined as the elements that are contained by both sets, and only the distinct element remains. In other words, we have $A\Delta B=\{s\}$. 
	%And $s$ is the missing element of $A$ (i.e., $s\in B\!\setminus\! A$) if $s\in B$, or the missing element of $B$ (i.e., $s\in A\!\setminus\! B$) otherwise;
	% \item If $A$ and $B$ has more than one distinct elements (i.e., $d>1$), the bitwise \code{XOR} of $s_A$ and $s_B$ will still cancel out all common elements and remain the \code{XOR} of the distinct elements, i.e., $s$ is the \code{XOR} of all distinct elements;
\end{sitemize}

Like most works on set reconciliation, we assume $\mathbf{0}$ is excluded from $\mathcal{U}$, as \autoref{alg:trivial_case} does not work when $\mathbf{0}\!\in\! A\bigcup B$ %$\mathbf{0}\in A\bigcap B$ 
for the following reason: When $s_A=s_B$ (i.e., $s=\mathbf{0}$), \autoref{alg:trivial_case} cannot tell whether $A$ and $B$ are identical, or they have a distinct element of value $\mathbf{0}$. 
%However, we can extend our scheme to support $\mathbf{0}$. For example, we let Alice send to Bob a single bit to indicate whether Alice has element $\mathbf{0}$, so Bob will know whether $\mathbf{0}\in A\Delta B$ or not. 
\autoref{alg:trivial_case} also does not work when there are more than one distinct elements in $A\Delta B$ (i.e., $d>1$), since the computed $s$ is the \code{XOR} of all these distinct elements.

% Note that \autoref{alg:trivial_case} works if and only if $|A\Delta B|\!\leq\! 1$ and $0\!\notin\! (A\!\cup\! B)$ (which we have explained in~\autoref{sec:model}). 

%\subsection{PBS: When $d$ is small}\label{sucsec:our-scheme}

%In this section, we generalize PBS to the case when $d$ is a small number, as we described in \autoref{sec:smalld}. 
%First, we describe each step of single-round PBS from \autoref{sec:hash_partition} to \autoref{sec:reconcile_by_trivial} and summarize it in \autoref{sec:single_round_pbs}. Second, we discuss the exceptions in single-round PBS in \autoref{subsec:exception_hash_partition}. Third, we propose multi-round PBS to handle the exceptions.

\subsection{PBS for small \texorpdfstring{\larger\boldmath $d$}{d}}\label{sec:pbs_smalld}

In this section, we describe the scheme for a more general case, where $d$ is no longer limited to be no more than $1$, but a small number that is no more than several.
%In this section, we substantiate the scheme described in \autoref{sec:smalld} for small $d$.

\subsubsection{Hash Partition and Parity Bitmap Encoding}\label{sec:hash_partition}
% \medskip
% \noindent{\bf Hash Partition} 

Here we formalize the aforementioned process of partitioning $A$ into $\{A_i\}_{i=1}^n$, $B$ into $\{B_i\}_{i=1}^n$, and $A\Delta B$ into $\{A_i\Delta B_i\}_{i=1}^n$ 
using a hash function $h(\cdot)$.
%as described in \autoref{sec:smalld} by introducing the concept of {\it sub-universes}. Given a hash function $h(\cdot): \mathcal{U}\rightarrow \{1,2,\cdots,n\}$, we 
Define {\it sub-universe} $\mathcal{U}_i$ as the set of elements in the universe $\mathcal{U}$ that are hashed into value $i$. More precisely, $\mathcal{U}_i\triangleq\{s\!\mid\! s\in \mathcal{U} \mbox{ and } h(s)=i\}$ for $i=1,2,...,n$. Then defining $A_i\triangleq A\bigcap\mathcal{U}_i$ and $B_i\triangleq B\bigcap\mathcal{U}_i$ for $i=1,2,...,n$ induces the partitioning of $A$, $B$, and $A\Delta B$.
%, as mentioned in \autoref{sec:smalld}. 

%{\bf (merged from the later two paragraphs)} 
How the $d$ distinct elements (balls) in $A\Delta B$ are distributed into the $n$ subset-pair-differences $\{A_i\Delta B_i\}_{i=1}^n$ (bins) can be viewed as throwing $d$ balls each uniformly and randomly into one of the $n$ bins. 
For the moment, we assume the following {\it ideal case} happens: Every subset-pair-difference $A_i\Delta B_i$ contains at most one distinct element.  
The ideal case corresponds to the $d$ balls ending up in $d$ distinct bins. It happens with probability $\prod_{k=1}^{d - 1}(1 - \frac{k}{n})$, which is on the order of $1-O(d^2/n)$ when $n\!\gg\!d$.
%approximately $e^{-\frac{d(d-1)}{2n}}$ when $d\!\ll\!n$. 
Hence, $n$ must be $\Omega(d^2)$ to ensure the ideal case happens with a nontrivial probability, as mentioned in \autoref{sec:smalld}. 
%The nonideal case of a subset pair difference containing more than $1$ distinct elements will be discussed in \autoref{subsec:exception_hash_partition}.

% {\bf (Previous)} For the moment, we assume the following {\it ideal case} happens: Every subset-pair-difference $A_i\Delta B_i$ contains at most one distinct element. The nonideal case of a subset pair difference containing more than $1$ distinct elements will be discussed in \autoref{subsec:exception_hash_partition}. 

%In this section, we give a detailed description on how to partition $A$ and $B$ (as introduced in \autoref{sec:smalld}) by introducing {\it sub-universes}, which is defined as follows: Given a hash function $h(\cdot): \mathcal{U}\rightarrow \{1,2,\cdots,n\}$, we define {\it sub-universes} $\{\mathcal{U}_i\}_{i=1}^n$, a partition of the universe $\mathcal{U}$, as $\mathcal{U}_i=\{s\!\mid\! s\in \mathcal{U} \mbox{ and } h(s)=i\}$ for $i=1,2,...,n$. Based on $\{\mathcal{U}_i\}_{i=1}^n$, we define $\{A_i\}_{i=1}^n$, the partition of $A$ introduced in \autoref{sec:smalld}, as $A_i\! \triangleq\! A\bigcap \mathcal{U}_i$ for $i=1,2,...,n$. $\{B_i\}_{i=1}^n$ is similarly defined. By this definition, the set difference $A\Delta B$ is partitioned into $n$ set differences of the partitioned subset pairs (i.e., $\{(A_i, B_i)\}_{i=1}^n$). From \autoref{sec:hash_partition} to \autoref{sec:reconcile_by_trivial}, we assume the following {\bf ideal case} happens: Each subset pair $(A_i, B_i)$ contains at most one distinct element ({\it i.e.,} $|A_i\Delta B_i|\!\leq\!1$). The nonideal case of a subset pair contains more than $1$ distinct elements will be discussed in \autoref{subsec:exception_hash_partition}. 

% Here we describe the hash-partition step introduced in \autoref{sec:smalld} in details. First, we use a hash function $h(\cdot): \mathcal{U}\rightarrow \{1,2,\cdots,n\}$ to partition the universe $\mathcal{U}$ into $n$ sub-universes: $\mathcal{U}_i=\{s\!\mid\! s\in \mathcal{U} \mbox{ and } h(s)=i\}$ for $\forall i=1,2,\cdots,n$. The hash function $h(\cdot)$ can be predetermined between Alice and Bob and does not require additional communication cost. Define $A_i\! \triangleq\! A\bigcap \mathcal{U}_i$ and $B_i\! \triangleq\! B\bigcap \mathcal{U}_i$ for $i=1,2,\cdots,n$. Then $\{A_i\}_{i=1}^n$ and $\{B_i\}_{i=1}^n$ are partitions of $A$ and $B$ respectively. Furthermore, $\{A_i\Delta B_i\}_{i=1}^n$ is a partition of $A\Delta B$. From \autoref{sec:hash_partition} to \autoref{sec:reconcile_by_trivial}, we assume the following {\bf ideal case} happens: Each subset pair $(A_i, B_i)$ contains at most one distinct element ({\it i.e.,} $|A_i\Delta B_i|\!\leq\!1$). The nonideal case of a subset pair contains more than $1$ distinct elements will be discussed in \autoref{subsec:exception_hash_partition}. 

% {\bf (Previous)} How the $d$ distinct elements (balls) in $A\Delta B$ are distributed into the $n$ subset pair differences $\{A_i\Delta B_i\}_{i=1}^n$ (bins) 
% can be viewed as throwing $d$ balls each uniformly and randomly into one of the $n$ bins. 

%follows the familiar {\it balls-into-bins} probability model. 
%The distinct elements are viewed as balls and the subset pairs are viewed as bins. 
%Each of the $d$ balls is uniformly and randomly thrown by the hash function $h(\cdot)$ into one of the $n$ bins. 
% The aforementioned ideal case that corresponds to the $d$ balls ending up in $d$ distinct bins happens with probability $\prod_{k=1}^{d - 1}(1 - \frac{k}{n})$, which is on the order of $1-O(d^2/n)$ when $d\!\ll\!n$.
% %approximately $e^{-\frac{d(d-1)}{2n}}$ when $d\!\ll\!n$. 
% Hence, $n$ must be $\Omega(d^2)$ to ensure the ideal case happens with a nontrivial probability, as mentioned in \autoref{sec:smalld}.


%in which the distinct elements are viewed as balls and the subset pairs are viewed as bins. The hash-parition basically throws (hashes) $d$ balls (distinct elements) uniformly and randomly into $n$ bins (subset pairs). The aforementioned ideal case in this context becomes, after throwing $d$ balls uniformly and randomly into $n$ bins, each bin receives at most $1$ ball (i.e., $d$ nonempty bins have $1$ ball in each and the rest $n-d$ bins are empty). The number of balls in each bin is a Binomial random variable $Binomial(d,1/n)$.
%{\bf It may remind readers about the Birthday problem. And the ideal case can be analogous to the case that no people share the same birthday.} 
% The ideal case happens with a probability of $p\!=\!\prod_{k=1}^{d - 1}(1 - \frac{k}{n})\!\approx\! e^{-\frac{d(d-1)}{2n}}$ when $d\!\ll\!n$. In other words, $n$ must be at least $O(d^2)$ to ensure the ideal case happens with a nontrivial probability, as described in \autoref{sec:smalld}.  

% Note that the ideal case does not always happen. However, we can ensure that the ideal case happens with high probability by properly setting $n$ based on $d$ (i.e., $n=\Omega(d^2)$). Furthermore, as we will describe in \autoref{subsec:nonideal}, even if the ideal case does not happen (i.e., some distinct elements are hashed into the same subset pair), most of the distinct elements should be distributed into different subset pairs and therefore can be reconciled. So the scheme, even cannot reconcile all of the distinct elements, can still reconcile the majority of them (i.e., piecewise decodability in \autoref{sec:intro_oursolution}). Based on this property, we will extend our scheme from single-round to multi-rounds in \autoref{subsec:nonideal} to further increase the probability of reconciling all distinct elements. 

% \medskip
% \noindent{\bf Parity Bitmap Encoding} 

{\bf (Modified)} Recall that the partition $\{A_i\}_{i=1}^n$ and $\{B_i\}_{i=1}^n$ can be encoded as $A[1..n]$ and $B[1..n]$ respectively, in which $A[i]$, the $i$-th bit of the parity bitmap $A[1..n]$, is equal to the oddness / evenness (parity) of the cardinality of $A_i$ (i.e., $A[i]=1$ if $|A_i|$ is odd; otherwise $A[i]=0$). $B[i]$, the $i$-th bit of the parity bitmap $B[1..n]$, is similarly defined. In the ideal case, $A[1..n]$ and $B[1..n]$ differ in exactly $d$ distinct bit positions $i_1,i_2,...,i_d$, and each subset-pair-difference $(A_{i_1},B_{i_1}), (A_{i_2},B_{i_2}),...,(A_{i_d},B_{i_d})$ contains exactly $1$ distinct element. If Bob knows $i_1,i_2,...,i_d$, he can start to reconcile the $d$ subset pairs respectively using \autoref{alg:trivial_case}, then Alice will obtain $A\Delta B$.

% {\bf (Modified)} The partition $\{A_i\}_{i=1}^n$ is encoded into an $n$-bit-long parity bitmap $A[1..n]$, in which $A[i]$, the $i$-th bit of the parity bitmap, is equal to the oddness / evenness (parity) of the cardinality of $A_i$ (i.e., $A[i]=1$ if $|A_i|$ is odd; otherwise $A[i]=0$). $B[1..n]$, the parity bitmap of $\{B_i\}_{i=1}^n$, is similarly defined. In the ideal case, $A[1..n]$ and $B[1..n]$ differ in exactly $d$ distinct bit positions $i_1,i_2,...,i_d$, and each subset-pair-difference $(A_{i_1},B_{i_1}), (A_{i_2},B_{i_2}),...,(A_{i_d},B_{i_d})$ contains exactly $1$ distinct element. If Bob knows $i_1,i_2,...,i_d$, he can start to reconcile the $d$ subset pairs respectively using \autoref{alg:trivial_case}, then Alice will obtain $A\Delta B$.

{\bf (Previous)} We encode $\{A_i\}_{i=1}^n$ into an $n$-bit-long parity bitmap $A[1..n]$, in which $A[i]$, the $i^{th}$ bit of the parity bitmap, is equal to the oddness / evenness (parity) of the cardinality of $A_i$ (i.e., $A[i]=1$ if $|A_i|$ is odd; otherwise $A[i]=0$). In the ideal case, the two bitmaps $A[1..n]$, $B[1..n]$ differ in exactly $d$ bit positions $i_1,i_2,...,i_d$, each of which corresponds to a subset pair that contains $1$ distinct element. The next step is to let Alice and Bob know these bit positions.
%Once the $d$ bit positions are known, Alice and Bob can start to reconcile $(A_{i_1},B_{i_1}), (A_{i_2},B_{i_2}),...,(A_{i_d},B_{i_d})$ using \autoref{alg:trivial_case} and obtain the $d$ distinct elements (i.e., $A\Delta B$). 

% \subsubsection{Parity Bitmap Encoding}\label{sec:parity_bitmap_encoding}

% %After hash-partitioning $A$ and $B$ into partitions $\{A_i\}_{i=1}^n$ and $\{B_i\}_{i=1}^n$, 
% As introduced in \autoref{sec:smalld}, we encode each partition into an $n$-bit-long parity bitmap and denote them as $A[1..n]$ and $B[1..n]$ respectively, as introduced in \autoref{sec:smalld}. For $i=1,2,...,n$, $A[i]$ (the $i^{th}$ bit of the parity bitmap $A[i]$) is equal to $1$ if $A_i$ contains an odd number of elements, and is equal to $0$ otherwise.
% % More specifically, for $i=1,2,...,n$, $A[i]$ (the $i^{th}$ bit of the parity bitmap $A[i]$) is defined as follows: $A[i]=1$ if $A_i$ contains an odd number of elements, and $A[i]=0$ otherwise. In this way, each bit $A[i]$ encodes the oddness / evenness (parity) of the cardinality of $A_i$. The $n$-bit-long parity bitmap $B[1..n]$ and $B[i]$ (the $i^{th}$ bit of $B[1..n]$) are similarly defined. 
% In the ideal case, 
% %$A[i]$ and $B[i]$ differ if and only if $A_i$ and $B_i$ have exactly $1$ distinct element, and $A[i]$ and $B[i]$ are the same if and only if $A_i=B_i$. Meanwhile, the $d$ distinct elements are hashed into $d$ different subset pairs. So 
% the two bitmaps $A[1..n]$, $B[1..n]$ differ in exactly $d$ bit positions, each of which corresponds to a subset pair that contains $1$ distinct element. Once the $d$ bit positions are known, Alice starts to reconcile each of the $d$ corresponding subset pairs by \autoref{alg:trivial_case} and gets the $d$ distinct elements (i.e., $A\Delta B$). 
% %If knowing the $d$ bit positions (i.e., the $d$ corresponding subset pairs), we can use \autoref{alg:trivial_case} to reconcile the $d$ subset pairs respectively to obtain all the $d$ distinct elements (i.e., $A\Delta B$). 
% In \autoref{sec:BCH_code}, we will describe how to find the $d$ bit positions using BCH code~\cite{Lint_IntroductionCodingTheory_1998}. 

% \medskip
% \noindent{\bf Find the $d$ Bit Positions Using ECC} 

%\subsubsection{Find the $d$ Bit Positions Using ECC}\label{sec:BCH_code}
\subsubsection{Find and Reconcile the \texorpdfstring{$d$}{d} subset pairs}\label{sec:BCH_code}

{\bf (Modified)} In the ideal case, for Bob to obtain $i_1,i_2,...,i_d$, Alice only needs to send $\xi_A$, the BCH code of $A[1..n]$, that can ``correct'' these $d$ bit errors in $B[1..n]$. Then Bob can decode and recover $A[1..n]$ (original message) and obtain $i_1,i_2,...,i_d$.

{\bf (Previous)} We view $A[1..n]$ as a corrupted message of $B[1..n]$ sent ({\bf not actually being sent}) from Bob to Alice through an {\it unreliable} commnunication channel that flips $d$ bits. To locate these $d$ bit positions, we let Bob also send an {\it error-correction code} that encodes $B[1..n]$ to Alice, such that Alice can recover $B[1..n]$ (original message) and obtain the $d$ bit positions $i_1,i_2,...,i_d$. In PBS, we use BCH code~\cite{bch1} to encode $B[1..n]$ and get the error-correction code.

There are two different BCH encoding techniques: {\it systematic} and {\it unsystematic}. The difference is that, the message appears as the prefix of the codeword (i.e., codeword = [message net-codeword]) in systematic BCH encoding, whereas it does not appear as a substring of the codeword in unsystematic BCH encoding. In PBS, we choose systematic BCH encoding because we are sending not the ``message'', but the net-codeword. 
%To correct $d$ bit errors, the length of the net-codeword only is no more than $d\log n$ bits. 
Without causing any ambiguity, we use the term `codeword' to refer to the net-codeword in the rest of this paper.
%The computational complexity of the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} is $O(d^2\log^2 n)$.

%The systematic BCH encoding is also used in other ECC-based set reconciliation works, such as PinSketch \cite{Wuille_Minisketchoptimizedlibrary_2019}, while PinSketch encodes a much longer message (e.g., $2^{32}$ bits) than in ours (hundreds of bits).  

%\subsubsection{Find the $d$ Bit Positions Using ECC}\label{sec:BCH_code}

% A straightforward approach to find the $d$ bit positions is to let Bob send the complete parity bitmap $B[1..n]$ to Alice, then Alice compares $A[1..n]$ with $B[1..n]$ locally. This approach has a communication overhead of $n$ bits, which is quite wasteful. As we discussed in~\autoref{sec:hash_partition}, $d$ is usually much smaller than $n$. It means $A[1..n]$ and $B[1..n]$ differ only at a tiny portion of bits. Therefore, we can view $A[1..n]$ as a corrupted message of $B[1..n]$ with $d$ bit errors, and the bit positions of the $d$ bit errors basically correspond to the $d$ subset pairs that contain distinct elements. The detection of bit errors, on the other hand, can be solved by Error-Correction Code (ECC)~\cite{Lin_ErrorControlCoding_1983}. 

% Since $A[1..n]$ and $B[1..n]$ differ at $d$ bit positions, we can view $A[1..n]$ as a corrupted message of $B[1..n]$ from Bob to Alice through an {\it unreliable} commnunication channel with $d$ corrupted bits, which are located on the $d$ bit positions. Therefore, to find the $d$ bit position, we only need to correct the $d$ corrupted bits in $A[1..n]$, which is done by transmitting a ``code'' that can correct upto $d$ bit errors from Bob to Alice through a {\it reliable} communication channel. 

% In PBS, we use {\it systematic} BCH code to generate the ``code'' by encoding the message $B[1..n]$. The codeword of the systematic BCH code is in the form of [message, net-codeword], since the message appears as the prefix of the codeword in systematic BCH code. The ``code'' is simply the net-codeword in the BCH codeword. We choose {\it systematic} BCH code because the (corrupted) message is already transmitted and we only need to pay a small communication overhead on transmitting ``code'' (i.e., net-codeword). To correct upto $d$ bit errors, the length of the net-codeword is no more than $d\log n$ bits, which is much smaller than the message when $d\!\ll\! n$. The computational complexity of the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} is $O(d^2\log^2 n)$. This type of BCH code is also used in other ECC-based set reconciliation works, such as PinSketch \cite{Wuille_Minisketchoptimizedlibrary_2019}. 

% Different from {\it unsystematic} BCH code
% The ``code'' is generated by {\it systematic} BCH code, which encodes the message $B[1..n]$ into a BCH codeword in the form of [message, net-codeword]. The ``code'' transmitted on the reliable channel is the net-codeword of the BCH codeword. In {\it systematic} BCH code, the message appears as the prefix of the codeword. 

% More specifically, PBS uses {\it systematic} BCH code~\cite{Lint_IntroductionCodingTheory_1998} that can correct upto $d$ bit errors to encode the parity bitmaps. In the {\it systematic} BCH code \footnote{In unsystematic BCH code, message does not appear to be the prefix of the codeword}, the message (i.e., the parity bitmap) appears as the prefix of the raw codeword, which in the form of [message, net codeword]. Normally, to correct upto $d$ errors, the length of the net codeword is $2n\log d$, where $n$ is the length of the message (i.e., parity bitmap). However, our case is special in the sense that the net codeword is error-free (all $d$ bit errors are in the message), so the length of the net codeword can be reduced to $n\log d$. This type of BCH code is also used in other ECC-based set reconciliation works, such as PinSketch \cite{Wuille_Minisketchoptimizedlibrary_2019}. 

% Now we can formally describe how to find the $d$ bit positions: First, Bob uses a $d$-error-correcting systematic BCH code to encode $B[1..n]$ and sends the net codeword ($d\log n$ bits) to Alice. Upon receiving the net codeword and combining it with the corrupted message $A[1..n]$, Alice uses the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} to decode the $d$ bit errors in $A[1..n]$. The communication overhead of transmitting the net codeword is $d\log n$ bits. The computational complexity of the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} is $O(d^2\log^2 n)$. Both the communication overhead and the computational complexity here are relatively small when $d$ is small.

% \medskip
% \noindent{\bf Reconcile the $d$ subset pairs using \autoref{alg:trivial_case}} 

%Once the $d$ bit positions are known, Alice can start to reconcile $(A_{i_1},B_{i_1}), (A_{i_2},B_{i_2}),...,(A_{i_d},B_{i_d})$ using \autoref{alg:trivial_case} and obtain the $d$ distinct elements (i.e., $A\Delta B$). 
Once Bob decodes the codeword to obtain $i_1,i_2,...,i_d$, the corresponding subset pairs $(A_{i_1},B_{i_1})$, $(A_{i_2},B_{i_2})$, $...$, $(A_{i_d},B_{i_d})$ each can be reconciled using \autoref{alg:trivial_case}. To do so, Bob needs to send the respective \code{XOR} sums of the subsets $B_{i_1}$, $B_{i_2}$,$...$,$B_{i_d}$ to Alice (\autoref{alg1:sender} in \autoref{alg:trivial_case}). In addition, Bob needs to send $i_1,i_2,...,i_d$ to Alice, since Alice does not know the ``bit error positions'' yet. Each ``bit error position'' corresponds to the index of the corresponding subset pair, which needs to be encoded into $\log n$ bits, so the additional communication overhead on transmitting these indices is $d\log n$ bits. 
% When reconciling $(A_{i_1},B_{i_1}), (A_{i_2},B_{i_2}),...,(A_{i_d},B_{i_d})$ using \autoref{alg:trivial_case}, Alice needs to send not only the bitwise \code{XOR} of $A_{i_1}, A_{i_2},..., A_{i_d}$, but also the indices of the subset pairs ($i_1,i_2,...,i_d$), since Bob does not know which of the $d$ subset pairs are being reconciled. Each index is an integer between $1$ and $n$ and can be encoded into $\log n$ bits, So the additional communication overhead on transmitting the indices is $d\log n$ bits. 



% \subsubsection{Reconcile the $d$ subset pairs using \autoref{alg:trivial_case}}\label{sec:reconcile_by_trivial}

% After decoding the $d$ bit errors that corresponds to the $d$ subset pairs, Alice starts to reconcile them using \autoref{alg:trivial_case}. For each of the $d$ subset pairs, Alice needs to send not only the bitwise \code{XOR} of the subset pair, but also the index of the subset pair (since Bob does not know the $d$ subset pairs to reconcile). So the communication overhead on \autoref{alg:trivial_case} is $d\log |\mathcal{U}|+d\log n$ bits. 
%Plus the communication overhead on transmitting the net codeword of parity bitmap ($d\log n$, as we explained in \autoref{sec:BCH_code}), the overall communication overhead of single-round PBS is $d\log u+2d\log n$ bits.

% \medskip
% \noindent{\bf Check if set reconciliation is complete} 

Once Alice receives the \code{XOR} sums and the indices, she can compute the distinct elements, as described in \autoref{subsec:protocol0}, to obtain the set difference (denoted as $\hat{D}$). However, this reconciled set difference could be incorrect if the ideal case does not happen. Therefore, Alice needs to check if set reconciliation is successfully completed (or whether $\hat{D}=A\Delta B$). To do so, we introduce some ``linear'' checksum function $c(\cdot)$ that maps any subset of the universe $\mathcal{U}$ (such as $A$ and $B$) to a $32$-bit checksum (e.g., bitwise \code{XOR}). Here the ``linearity'' of a chechsum function refers to the fact that $c(S_1\Delta S_2)=c(S_1)\oplus c(S_2)$ for any two subsets $S_1$ and $S_2$ of the universe $\mathcal{U}$. We use this checksum function to check if $\hat{D}=A\Delta B$ by comparing $c(\hat{D})$ to $c(A\Delta B)$. Note that $c(\hat{D})$ can be computed in $O(d)$ time and $c(A\Delta B)=c(A)\oplus c(B)$ can be precomputed {\bf during the encoding period, which costs $32$ bits of communication overhead on transmitting $c(B)$ from Bob to Alice. In PBS, we select {\it longitudinal parity check}, the bitwise \code{XOR} of all elements (recall each element is a $32$-bit-long binary string) in the set, as the checksum function. It is not hard to verify it is linear.}  

% {\bf (Previous)} After reconciling the subset pairs and obtaining the reconciled set difference (denoted as $\hat{D}$), PBS needs to check if set reconciliation is complete (or whether $\hat{D}=A\Delta B$), since the reconciled set difference $\hat{D}$ is not the actual set difference $A\Delta B$ in the nonideal case (to be discussed in \autoref{subsec:exception_hash_partition}). Hence, we add a verfication step after obtaining $\hat{D}$ to check if $\hat{D}=A\Delta B$. In PBS, we check an equivalent condition, $A=B\Delta\hat{D}$, instead of $\hat{D}=A\Delta B$, since $B$ and $\hat{D}$ are both known by Bob and their set difference $B\Delta\hat{D}$ can be locally computed. More specifically, to check if the remote sets $A$ and $B\Delta\hat{D}$ are equal, we let Alice compute a $32$-bit checksum of $A$ and send it to Bob. {\bf Then Bob computes the $32$-bit checksum of $B\Delta\hat{D}$ using the same checksum algorithm and compare the two checksums. In PBS, we select {\it longitudinal parity check} (i.e., bitwise \code{XOR} of all elements in the set) as the checksum algorithm, so that the checksum $B\Delta\hat{D}$ can be efficiently computed as the bitwise \code{XOR} between the checksum of $B$ (can be pre-computed) and that of $\hat{D}$. Other checksum algorithms that are {\it linear} to the set difference operator (i.e., $\Delta$) also work for PBS. }
% Then Bob checks if $B\Delta\hat{D}$ satisfies the receiving checksum. 

The condition $\hat{D}=A\Delta B$ can be almost surely verified by the checksum, 
{\bf although it could mistakenly believes two different sets as identical ones.} This event happens with probability $2^{-32}\approx 2.3\times 10^{-10}$ when the ideal case does not happen, {\bf which has a probability on the order of $10^{-2}$.} Although this event could cause PBS mistakenly believes the set reconciliation is completed, it happens with an extremely small probability (on the order of $10^{-12}$) and should be acceptable in most applications. In few applications which allow no room for error ({\it e.g.,} Bitcoin), additional techniques such as Merkle tree~\cite{merkle87} based validation will be used to verify the correctness of the results anyway. 
%If such techniques find out that the set reconciliation is not completed, we could simply start it over and use PBS to reconcile the two sets again under a different hash function $h$. In this case, the checksum will be different If so, the  (note that PBS is a `randomized' algorithm when assuming the hash functions for hash-partition are random hash functions). 
To simplify our description, we ignore this small probability event and assume the checksum works perfectly in this rest of this paper. We summarize all the above steps of PBS (in the first round) in \autoref{alg:single_round_pbs}.
%{\bf not a good position to mention `for super critical applications, use a checksum for all groups', since we are describing single-group scenario. }

\begin{algorithm}
\caption{Single-round PBS}
\label{alg:single_round_pbs}

%Hash-partition $A$, $B$ into $\{A_i\}_{i=1}^n$, $\{B_i\}_{i=1}^n$\; \label{step:hash_partition}

%Parity encode $\{A_i\}_{i=1}^n$, $\{B_i\}_{i=1}^n$ into $A[1..n]$, $B[1..n]$\; \label{step:parity_encode}
{\it Alice}: Send $\xi_A$, the BCH codeword of $A[1..n]$, to Bob\; \label{step:BCH_encode}

{\it Bob}: Decode $(B[1..n], \xi_A)$ to obtain $i_1,i_2,...,i_d$\; \label{step:BCH_decode}

{\it Bob}: Send the \code{XOR} sums of sets $B_{i_1}, B_{i_2},...,B_{i_d}$ (\autoref{alg1:sender} in \autoref{alg:trivial_case}) and $i_1,i_2,...,i_d$ to Alice\; \label{step:BCH_decode}

{\it Alice}: Obtain $A_{i_1}\Delta B_{i_1}, A_{i_2}\Delta B_{i_2},...,$ and $A_{i_d}\Delta B_{i_d}$ (\autoref{alg1:receiver} in \autoref{alg:trivial_case}); $\hat{D}\leftarrow \bigcup_{k=1}^d (A_{i_k}\Delta B_{i_k})$\; \label{step:trivial_reconcile}

{\it Alice}: Check if $c(\hat{D})=c(A\Delta B)$\; \label{step:terminate_condition}

\end{algorithm}
% {\color{blue}This probability is low enough for most applications. In few applications which allow no room for error ({\it e.g.,} Bitcoin), additional techniques such as Merkle tree~\cite{merkle87} based validation will be used to verify the correctness of the results anyway.}

% {\bf (Previous)} The condition $A=B\Delta\hat{D}$ can be almost surely verified by a $32$-bit checksum, although it could mistakenly believe two different sets as identical ones with probability $2^{-32}\approx 2.3\times 10^{-10}$ {\bf on top of the probability that the nonideal case happens (on the order of $10^{-2}$).} Although this event could cause an ``early'' termination and leave some distinct elements unreconciled, it happens with an extremely small probability (on the order of $10^{-12}$) and should be acceptable in most applications. {\bf To simplify our description, we ignore this small probability event and assume the checksum works perfectly in this rest of this paper. }
%and such an event (i.e., mistaken $A$ and $B\Delta\hat{D}$ are identical when they are different) never happens in our evaluation. For some super critical applications, we can certainly use a $64$-bit checksum to reduce this probability to $5.4\times 10^{-20}$ if needed.

% When the ideal case does not happen, set reconciliation cannot accomplish in one round, as we will explain in \autoref{subsec:exception_hash_partition}. Hence, we add a verfication step to check if set reconciliation is complete. Let $\hat{D}$ denote the set of reconciled elements. The idea of this verification is basically to compare $A$ with $B\Delta \hat{D}$: If $A=B\Delta \hat{D}$ (i.e., $\hat{D}=A\Delta B$), we know the set reconciliation is complete; Otherwise, the set reconciliation is incomplete.  using a $32$-bit checksum. 

\subsubsection{Communication overhead of PBS (First Round)}\label{sec:communication_overhead_single_PBS}

%To correct $d$ bit errors, the length of the net-codeword only is no more than $d\log n$ bits. 

The communication overhead of \autoref{alg:single_round_pbs} consists of four components: (1) the BCH codeword $\xi_A$ in \autoref{step:BCH_encode}; (2) the subset pair indices $i_1,i_2,...,i_d$ in \autoref{step:trivial_reconcile}; (3) the bitwise \code{XOR} sums of sets $B_{i_1}, B_{i_2},...,B_{i_d}$ of $d\log |\mathcal{U}|$ bits in \autoref{step:trivial_reconcile}; and (4) transmit the $32$-bit checksum of $B$ (i.e., $c(B)$) from Bob to Alice for precomputing $c(A\Delta B)$ in \autoref{step:terminate_condition}. These four components contribute roughly (1) $d\log n$ bits (recall that to ``correct'' $d$ bit errors, the length of the BCH codeword is no more than $d\log n$ bits); (2) $d\log n$ bits; (3) $d\log |\mathcal{U}|$ bits; and (4) $32$ bits respectively to the overall communcation overhead of \autoref{alg:single_round_pbs}. 

% All the steps of PBS in the first round are summarized in \autoref{alg:single_round_pbs}. The overall communication overhead consists of three components: (1) the BCH codeword of $d\log n$ bits in \autoref{step:BCH_encode}; (2) the subset pair indices $i_1,i_2,...,i_d$ and the corresponding bitwise \code{XOR}s of $d\log n+d\log |\mathcal{U}|$ bits in \autoref{step:trivial_reconcile}; and (3) the $32$-bit checksum of $A$ in \autoref{step:terminate_condition}. 


% {\it Bob}: BCH-Encodeing $B[1..n]$ and send the codeword to Alice\; \label{step:BCH_encode}

% {\it Alice}: Upon receiving the codeword, decode the bit errors between $A[1..n]$ and $B[1..n]$\; \label{step:BCH_decode}

% {\it Alice}: For each bit error, start reconciling the corresponding subset pair by \autoref{alg:trivial_case}\; \label{step:trivial_reconcile}

% {\it Bob}: Upon receiving the reconciled set difference $\hat{D}$, check if $A=B\Delta \hat{D}$ via checksum\; \label{step:terminate_condition}


% \subsubsection{Single-round PBS}\label{sec:single_round_pbs}

% Here we summarize all the steps of single-round PBS and represent it by pseudocode in \autoref{alg:single_round_pbs}. \autoref{step:hash_partition} and \autoref{step:parity_encode} operates at both hosts (i.e., Alice and Bob). \autoref{step:hash_partition} to \autoref{step:trivial_reconcile} have been elaborated from \autoref{sec:hash_partition} to \autoref{sec:reconcile_by_trivial}. The last step in \autoref{step:terminate_condition} aims to check whether reconciliation is complete (i.e., $\mathcal{D}=A\Delta B$). More specifically, Alice calculates the checksum (e.g., CRC-$32$) of $A$ and send it to Bob. Then Bob calculates the checksum of $B\Delta \mathcal{D}$ and compares it to the receiving checksum of $A$. If the two checksums are the same, we believe $A=B\Delta \mathcal{D}$ and therefore $\mathcal{D}=A\Delta B$ (i.e., reconciliation is complete); Else, we know some elements are reconciled incorrectly. We classify those elements (i.e., the ones in the set difference between $A\Delta B$ and $\mathcal{D}$) into two subsets $A\Delta B\!\setminus\!\mathcal{D}$ and $\mathcal{D}\!\setminus\!(A\Delta B)$ and refer the elements in the former as {\it false-negatives}, and refer the elements in the later as {\it false-positives}. 

% In the ideal case, neither false-positives nor false-negatives will happen and the two checksums always equal. However, in real life, the ideal case does not always happen. We will discuss the nonideal case in \autoref{subsec:exception_hash_partition}. In our evaluation, we use a $32$-bit checksum for comparing $A$ to $B\Delta \mathcal{D}$ that has {\bf an error probability} roughly $10^{-9}$. This error (i.e., mistake $A=B\Delta \mathcal{D}$) incurs false-negatives. All set reconciliation schemes have the same problem on their termination conditions (i.e., check whether $\mathcal{D}=A\Delta B$). For some super critical applications, we can certainly decrease the error probability by using more powerful checksums (i.e., $64-$bit). Using a $32$-bit checksum, this kind of false-negatives never happen in the evaluation. 
% %For simplification, we assume no error happens when checking $\mathcal{D}=A\Delta B$ in the rest of the paper.

% \begin{algorithm}
% \caption{Single-round PBS}
% \label{alg:single_round_pbs}

% Hash-partition $A$, $B$ into $\{A_i\}_{i=1}^n$, $\{B_i\}_{i=1}^n$\; \label{step:hash_partition}

% Parity encode $\{A_i\}_{i=1}^n$, $\{B_i\}_{i=1}^n$ into $A[1..n]$, $B[1..n]$\; \label{step:parity_encode}

% {\it Bob}: Encode $B[1..n]$ by BCH code, then send the codeword to Alice\; \label{step:BCH_encode}

% {\it Alice}: Upon receiving the codeword, decode the bit errors between $A[1..n]$ and $B[1..n]$\; \label{step:BCH_decode}

% {\it Alice}: For each bit error, reconcile the corresponding subset pair by \autoref{alg:trivial_case}\; \label{step:trivial_reconcile}

% {\it Bob}: Upon the reconciled distinct elements $\mathcal{D}$, check whether $A=B\Delta \mathcal{D}$ via checksum\; \label{step:terminate_condition}
% \end{algorithm}

\subsubsection{Exception Handling}\label{subsec:exception_hash_partition}

When the ideal case does not happen, some subset pair may contain more than $1$ distinct elements and cannot be successfully reconciled by \autoref{alg:trivial_case}. We can classify the possible exceptions that happen in such a subset pair into the following two types of events: 

\noindent {\bf Type (\RN{1}) event}: Subset pair $(A_i, B_i)$ contains a nonzero even number of distinct elements, the parity bits of $A_i$ and $B_i$ are the same. So the BCH code $\xi_A$ cannot detect it and PBS will not reconcile the subset pair yet in this round. This event happens with a small but nontrivial probability: For example, when $d=5$ and $n=255$ (i.e., throwing $5$ balls each uniformly and randomly into $255$ bins), the probability that some bin has a nonzero even number of (in this case either $2$ or $4$) balls is roughly $0.04$. 
%Note that when a type (\RN{1}) event happens, the checksum (\autoref{step:terminate_condition} in \autoref{alg:single_round_pbs}) can detect that the set reconciliation has not been completed. Then PBS will start another round to reconcile the ``hidden'' distinct elements (the ones that have not been reconciled in this round), 
%so on so force, until all distinct elements are successfully reconciled and the checksum is verified to be correct, 
%as we will describe in \autoref{sec:multi-rounds}. 

% Note that when a Type (\RN{1}) subset pair exists, the $32$-bit checksum (\autoref{step:terminate_condition} in \autoref{alg:single_round_pbs}) can almost surely detect that the set reconciliation is incomplete. If this is the case (i.e., the checksum is verified to be incorrect), PBS will start another round of set reconciliation to reconcile the remaining distinct elements (e.g., the ``hidden'' distinct elements in Type (\RN{1}) subset pairs), so on so force, until all distinct elements are reconciled and the checksum is verified to be correct, as we will describe in \autoref{sec:multi-rounds}. 

\noindent {\bf Type (\RN{2}) event}: Subset pair $(A_i, B_i)$ contains distinct elements whose quantity is an odd number no less than $3$, the parity bits of $A_i$ and $B_i$ will be different and PBS will reconcile the subset pair using \autoref{alg:trivial_case}. The reconciled element $s$ is however the bitwise \code{XOR} of all distinct elements in $(A_i, B_i)$ (explained in \autoref{subsec:protocol0}), which is a ``fake'' distinct element.
%, which will be mistakenly believed as the distinct element of $(A_i, B_i)$. 
This event happens with a tiny probability: In the same example above ($d=5$ and $n=255$), the probability that some bin has an odd number of balls that is no less than $3$ (in this case $3$ or $5$) is only $1.52\times 10^{-4}$. 
%Similarly, the $32$-bit checksum can also detect that the set reconciliation has not been completed when a type (\RN{2}) event happens. Both the ``hidden'' and the ``fake'' distinct elements can also be reconciled in later rounds. 

%Note that those ``fake'' distinct elements will become new distinct elements in the next round and therefore incur additional communication overhead to reconcile. 
%Note that those ``fake'' distinct elements will incur additional communication overhead if we want to reconcile them ``later''. Therefore, we add a verification on each reconciled distinct element of \autoref{alg:trivial_case} that can detect ``fake'' distinct elements with high probability. \autoref{alg:verification} shows how this verification works, and it does not incur additional communication overhead.

Note that the nature of hash-partition provides us an approach that can detect ``fake'' distinct elements with high probability. This approach only needs to locally verify the reconciled elements of \autoref{alg:trivial_case} and does not incur any additional overhead. \autoref{alg:verification} shows how this verification works.

\begin{algorithm}
\caption{Verify reconciled element $s$ of $(A_i, B_i)$}
\label{alg:verification}
\If{$h(s)\neq i$} {Discard the reconciled element $s$;}
\end{algorithm}

Although a distinct element of $(A_i, B_i)$ must be in sub-universe $\mathcal{U}_i$ (i.e., the hash value of the element under $h$ equals to $i$), a ``fake'' distinct element could be in any sub-universe with probability $1/n$, since it is the bitwise \code{XOR} of multiple distinct elements of $(A_i, B_i)$. Therefore, \autoref{alg:verification} only fails to identify a ``fake'' distinct element with probability $1/n$, which is roughly $3.9\times 10^{-3}$ when $n=255$, under the condition that the type (\RN{2}) event happens, which also has a tiny probability as we explained earlier. In the same example above ($d=5$ and $n=255$), a ``fake'' distinct element that fails to be detected by \autoref{alg:verification} happens with a tiny probability of $6\times 10^{-7}$, which is the multiplication of the probability of the type (\RN{2}) event ($1.52\times 10^{-4}$) and the probability of \autoref{alg:verification} fails ($3.9\times 10^{-3}$). 
%{\bf (removed to the beginning of theoretical analysis) To simplify our description, we also ignore this small probability event and assume all ``fake'' distinct elements will be successfully detected by \autoref{alg:verification} in this rest of this paper. }

Note that either a type (\RN{1}) event or a type (\RN{2}) event will cause PBS fails to reconcile all distinct elements, which can be detected by the checksum (\autoref{step:terminate_condition} in \autoref{alg:single_round_pbs}). In this case, PBS will continue to reconcile the ``rest'' of distinct elements using additional rounds. 
%In this case, PBS will continue to reconcile the ``remaining'' distinct element by starting another round, as we will describe in \autoref{sec:multi-rounds}. The ``remaining'' distinct elements here consist of (1) the ``hidden'' distinct elements that have not been reconciled in this round and (2) the ``fake'' distinct elements that are not verified by \autoref{alg:verification}.

% {\bf (to be removed) Readers may wonder encoding the exact subset cardinalities (i.e., $|A_i|, |B_i|$) instead of their oddness / evenness (parity) (described in \autoref{sec:hash_partition}) could help to detect and solve Type (\RN{1}), (\RN{2}) events. However, encoding the exact subset cardinalities not only incurs much more additional communication overhead comparing to encoding their parities, but also barely helps on detecting Type (\RN{1}), (\RN{2}) events, since we cannot precisely derive $|A_i\Delta B_i|$, the total number of distinct elements in $(A_i, B_i)$, even knowing $|A_i|, |B_i|$: For instance, when $|A_i|\!=\!|B_i|\!=\!50$, $|A_i\Delta B_i|$ could be any even number ($\leq 100$) if the distinct elements are evenly splitted and placed between $A_i$ and $B_i$. }

% As we have described in \autoref{sec:hash_partition}, the ideal case does not always happen, which means some subset pair may contain more than $1$ distinct elements and cannot be successfully reconciled by \autoref{alg:trivial_case}. Due to the parity encoding, we can classify such subset pair into the following two scenarios:

% \begin{itemize}
%     \item Scenario 1: If a subset pair $(A_i, B_i)$ contains even number ($\geq 2$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be the same and PBS will not reconcile the subset pair yet in this round;
%     \item Scenario 2: If a subset pair $(A_i, B_i)$ contains odd number ($\geq 3$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be different and PBS will reconcile the subset pair using \autoref{alg:trivial_case}. The reconciled element (i.e., $s$ in \autoref{alg:trivial_case}) is however the bitwise \code{XOR} of all distinct elements in $(A_i, B_i)$ (explained in \autoref{subsec:protocol0}), which will be mistakenly believed as the distinct element of $(A_i, B_i)$. 
%     %However, as described in \autoref{subsec:protocol0}, when a subset pair contains more than $1$ distinct elements, \autoref{alg:trivial_case} will output the bitwise \code{XOR} of them as the `distinct element', which is not an actual distinct element with high probability;
% \end{itemize}

% In both scenarios, the distinct elements in the subset pair will not be reconciled in this round. As we will describe in \autoref{sec:multi-rounds}, we generalize PBS into multi-round, so that the distinct elements that have not been reconciled in the first round will be reconciled in later rounds. On the other hand, the second scenario could result in incorrectly reconciled distinct elements, which will become new distinct elements in the next round in multi-round PBS. 

% % In both scenarios, the distinct elements in the subset pair cannot be successfully reconciled in this round and will remain in the set difference (i.e., $(A\Delta B)\!\setminus\!\hat{D}$). On the other hand, the incorrectly reconciled distinct element in the second scenario will appear as a new distinct element (i.e., $\hat{D}\!\setminus\!(A\Delta B)$) in the next round if we generalize PBS into multi-round (to be elaborated in \autoref{sec:multi-rounds}). Both scenarios can be almost surely detected by the 32-bit checksum (\autoref{step:terminate_condition} in \autoref{alg:single_round_pbs}). The set difference after the reconciliation in this round, $D\Delta\hat{D}$, can be reconciled in later rounds, as we will describe in \autoref{sec:multi-rounds}. 

% Naturally, we do not want to generate new distinct elements in the process of set reconciliation, even though it happens with a tiny probability when $n=\Omega(d^2)$: For instance, when $d=5$ and $n=255$ (i.e., throwing $5$ balls uniformly and randomly into $255$ bins), the probability (i.e., some bin has $3$ or $5$ balls) is only $7.6\times 10^{-6}$. Therefore, we add a verification with no additional communication cost on each reconciled element of \autoref{alg:trivial_case}, such that each incorrect dinstinct element can be identified with high probability. The verfication is shown in \autoref{alg:verification}. 

% \begin{algorithm}
% \caption{Verify reconciled element $s$ of $(A_i, B_i)$}
% \label{alg:verification}
% \If{$h(s)\neq i$} {Discard the reconciled element $s$;}
% \end{algorithm}

% Although any distinct element of $(A_i, B_i)$ must be in sub-universe $\mathcal{U}_i$ (i.e., the hash value of the element under $h$ equals to $i$), the bitwise \code{XOR} of multiple distinct elements of $(A_i, B_i)$ could be in any sub-universe with probability $1/n$. Therefore, \autoref{alg:verification} fails to identify an incorrectly reconciled distinct element in the second scenario with probability $1/n$ that is roughly $3.9\times 10^{-3}$ when $n=255$. In other words, an incorrectly reconciled distinct element that cannot be identified by \autoref{alg:verification} appears with probability $3\times 10^{-8}$. {\bf I feel that defining $\tilde{a}_4=a_1\oplus a_2\oplus a_3$ does not help much.}

% In both scenarios, the distinct elements in the subset pair cannot be successfully reconciled in this round. These distinct elements can be reconciled in later rounds if needed, as we will describe in \autoref{sec:multi-rounds}. In this section, we only discuss how to identify the {\it incorrect} distinct element in the second scenario. Let us use an example to elaborate the second scenario: Assume $(A_i, B_i)$ contains $3$ distinct elements $a_1, a_2, a_3$, then Bob computes $\tilde{s}=a_1\oplus a_2\oplus a_3$ using \autoref{alg:trivial_case} and mistakes it as the distinct element in $(A_i, B_i)$. 

% In both scenarios, the distinct elements in the subset pair cannot be successfully reconciled (i.e., false-negatives defined in \autoref{sec:single_round_pbs}. The distinct elements that are not successfully reconciled in this round, if needed, can be reconciled in later rounds as we will describe in \autoref{sec:multi-rounds}. In this section, we only discuss how to identify the {\it incorrect} distinct elements in the second scenario. Let us use an example to elaborate the second scenario: Assume $(A_i, B_i)$ contains $3$ distinct elements $a_1, a_2, a_3$, then Bob computes $\tilde{s}=a_1\oplus a_2\oplus a_3$ using \autoref{alg:trivial_case} and mistakes it as the distinct element in $(A_i, B_i)$. 

\begin{comment}
============================================

We add a no-communication-cost verification step to check whether a reconciled element is an actual distinct element or not. Note that an actual distinct element of $(A_i, B_i)$ must be in sub-universe $\mathcal{U}_i$. On the other hand, an incorrectly reconciled element (e.g., $\tilde{s}$) can be in any sub-universe with probability $1/n$. So at the end \autoref{subsec:protocol0}, we check whether the reconciled element is in $\mathcal{U}_i$ by the hash function $h$ in hash-partition:

This verfication cannot completely eliminate false-positives, since an incorrectly reconciled element (e.g., $\tilde{s}$) can coincidentally end up in $\mathcal{U}_i$ with probability $1/n$. The chance of false-positives is extremely small using the verification. For instance, if $d=5$ and $n=255$, the probability of the second scenario is only $7.6\times 10^{-6}$. The probability of false-positives using the verfication is $1/n$ times this small probability, which is roughly $3\times 10^{-8}$. {\bf Note that a small probability of false-positives only costs a little waste on set reconciliation when synchronizing objectives (e.g., files), which is acceptable for most applications.}

Even worse, in the second scenario, the false-positives defined in \autoref{sec:single_round_pbs} could happen. For example, if subset pair $(A_i, B_i)$ contains $3$ distinct elements $s_1, s_2, s_3$, then \autoref{alg:trivial_case} computes $\tilde{s}=s_1\oplus s_2\oplus s_3$ and Bob mistakes $\tilde{s}$ as an actual distinct element. The good thing is, the probability of this kind of false-positives is extremely small for small $d$. For instance, if $d=5$ and $n=255$, the probability of the false-positives is only $7.6\times 10^{-6}$. To further reduce the chance of false-positives, we add a no-communication-cost verification step at the end of \autoref{subsec:protocol0} to check whether $\tilde{s}$ is an actual distinct element or not. The verification step works as follows: Given the output $s$ of subset pair $(A_i,B_i)$, if $s\in\mathcal{U}_i$ (i.e., $h(s)=i$), we consider $s$ as an actual distinct element; Otherwise, we consider $s$ as an incorrect output and discard it. 

Note that if $\tilde{s}\in A_i\Delta B_i$, $\tilde{s}$ must be in sub-universe $\mathcal{U}_i$. However, if $\tilde{s}$ is the bitwise \code{XOR} of the distinct elements in $(A_i,B_i)$ (i.e., the second scenario happens), it ends up in $\mathcal{U}_i$ with probablity of only $1/n$. 
%In fact, if we assume the hash-partition described in \autoref{sec:hash_partition} hashes the elements of $\mathcal{U}$ uniformly, independently, and randomly into $n$ sub-universes, the output $s$ in the second scenario will be in a different sub-universe $\mathcal{U}_j (j\neq i)$ with a high probability of $1-\frac{1}{n}$. Hence, this verfication method can further reduce the probability of false-positives by a factor of $\frac{1}{n}$. 
Use the same example (i.e., $d=5$, $n=255$), the probability of this kind of false-positives is reduced from $7.6\times 10^{-6}$ to $3\times 10^{-8}$ by this verification method. 
%{\bf This probability can be further reduced in \autoref{subsec:protocol2}, where PBS does two tiers of hash-partitions. So we can do verification on both of the two hash functions.}

%In some super critical cases (i.e., no false-positive is allowed), we can use a more powerful verification method to completely eliminate false-positives. That is, to check if the output $s$ exists in exactly one of the two sets (i.e., $s\in A\!\setminus\! B$ or $s\in B\!\setminus\! A$). To do so, Bob transmits $s$ along with an identification bit $\mathbbm{1}_{\{s\in B\}}$ to Alice, then Alice checks if $s\in (A\!\setminus\! B)\bigcup (B\!\setminus\! A)$ . This method verification costs additional $d(\log u+1)$ bits of communication overhead. In most applications, this rigorous $0\%$ probability guarantee of false-positives is unnecessary and the probability of the former verification method is small enough, so we use the former in the evaluation. Based on our observation, this kind of false-positives do not happen even once in the evaluation using the former verfication method. In the rest of this paper, we assume Scenario 2 is always correctly verified. 

============================================
\end{comment}

\subsection{Running PBS for Multiple Rounds}\label{sec:multi-rounds}

%{\bf (merged from the following two paragraphs)} 
To deal with the ``rest'' of distinct elements, we remove (and save) all the distinct elements that has been reconciled in the first round (i.e., $\hat{D}$) and run another round of PBS. In the second round, we reconcile $A\Delta \hat{D}$ and $B$ instead of reconciling $A$ and $B$ for both (1) removing all the distinct elements that have been reconciled; and (2) keeping all the distinct elements that have not been reconciled, which we will explain shortly. We use a different hash function for hash-partition in the second round to avoid the same exceptions (i.e., type (\RN{1}), (\RN{2}) events) that happened in the first round happen again. PBS keeps running until the set reconciliation is successfully completed, which is verified by the checksum (\autoref{alg:single_round_pbs} of \autoref{step:terminate_condition}). The use of independent hash functions in different rounds naturally enables the Markov chain modeling of the reconciliation process, which we will elaborate in \autoref{sec:single_markov}. 

{\bf (new content)} We emphasize that reconciling $A\Delta \hat{D}$ and $B$ not only removes all the distinct elements that have been reconciled, but also keeps all the distinct elements that need to be reconciled. Note that the ``rest'' distinct elements can be classified into two catagories: (1) the ``hidden'' distinct elements that have not been reconciled yet (i.e., $D\!\setminus\!\hat{D}$), which are incurred by either a type (\RN{1}) event or a type (\RN{2}) event; and (2) the ``fake'' distinct elements incurred by both a type (\RN{2}) event and the corresponding verification failure in \autoref{alg:verification} (i.e., $\hat{D}\!\setminus\!D$). It is not hard to verify that this classification of the ``rest'' distinct elements (i.e., $D\!\setminus\!\hat{D}$ and $\hat{D}\!\setminus\!D$) is a partition of the set difference between $A\Delta \hat{D}$ and $B$, which confirms our emphasis. 

% To deal with the ``remaining'' distinct elements, we remove (and save) all the distinct elements that has been reconciled in the first round (i.e., $\hat{D}$) and run another round of PBS. In the second round, we reconcile $A\Delta \hat{D}$ and $B$ instead of reconciling $A$ and $B$ to remove all the reconciled distinct elements. We use a different hash function for hash-partition in the second round to avoid the same exceptions (i.e., type (\RN{1}), (\RN{2}) events) that happened in the first round happen again. This procedure replicates until If until all distinct elements are successfully reconciled and the checksum is verified to be correct. 

% {\bf (to be removed)} When the ideal case does not happen (i.e., type (\RN{1}) or type (\RN{2}) event happens), PBS will know the set reconciliation has not been completed via the $32$-bit checksum (\autoref{step:terminate_condition} in \autoref{alg:single_round_pbs}). To reconcile those distinct elements that have not been reconciled yet in the first round, we rule out all successfully reconciled elements and run another round of PBS. This procedure replicates until all distinct elements are successfully reconciled and the checksum is verified to be correct.

% {\bf (to be removed)} More specifically, in the second round, we run PBS to reconcile $A$ and $B\Delta \hat{D}$ instead of $A$ and $B$ to rule out all elements that have been reconciled, where $\hat{D}$ is the set of reconciled distinct elements in the first round. We use a different hash function for hash-partition in the second round to avoid the same exceptions (i.e., type (\RN{1}), (\RN{2}) events) that happened in the first round happen again. The later rounds are similarly operated. 

%{\bf Normally, we want PBS to successfully reconcile all distinct elements in only a few rounds (say $3$) with high probability (say $99\%$). Hence, when tuning parameters (to be discussed in \autoref{sec:parameter_settings}), we set a {\it target success probability} $p_0$ of $r$ rounds as a paramenter setting requirement, which aims to ensure the probability that all distinct elements are reconciled in $r$ rounds to be larger than $p_0$. This requirement should also ensure the majority of the distinct elements are reconciled in the first round. Use the same example ($d=5, n=255$), on average $4.81$ out of $5$ distinct elements should be reconciled in the first round. So the total communication overhead in all rounds is only slightly larger than ($1.01$ to $1.07$ times of, as we will show in \autoref{fig:per-round-con}) that in the first round. Due to this reason, we use the communication overhead in the first round (described in \autoref{sec:communication_overhead_single_PBS}) to approximate the total communication overhead of all rounds in parameter settings (to be elaborated in \autoref{sec:parameter_settings}.}

% Although PBS may need to run many rounds to reconcile all distinct elements, the communication overhead mostly happens in the first round, since the majority of the distinct elements should be reconciled in the first round. Use the same example ($d=5, n=255$), on average $4.81$ out of $5$ distinct elements should be reconciled in the first round. So the total communication overhead in all rounds is only slightly larger than ($1.01$ to $1.07$ times of, to be shown in \autoref{fig:per-round-con}) that in the first round. Due to this reason, we use the communication overhead in the first round (described in \autoref{sec:communication_overhead_single_PBS}) to approximate the total communication overhead (all rounds) in parameter settings (to be elaborated in \autoref{sec:parameter_settings}).

%For the moment, we assume no ``fake'' distinct element in type (\RN{2}) subset pairs fails to be detected, which happens with overwhelming probability as explained in \autoref{subsec:exception_hash_partition}. Then 
%PBS reconciles the distinct elements gradually round by round. This is the ``piecewise decodability'' mentioned in \autoref{sec:intro_oursolution}. We use the following example to describe it in details: 
%Given two sets with $10$ distinct elements, in the first round, PBS tries to reconcile the $10$ distinct elements and say $6$ out of the $10$ distinct elements are successfully reconciled. Then the $6$ reconciled distinct elements are removed and PBS tries to reconcile the remaining $4$ distinct elements in the second round. Say $2$ out of the $4$ remaining distinct elements are successfully reconciled, and that leaves $2$ remaining distinct elements to be reconciled in the third round, so on so force. 
% Given two sets $A$, $B$ with $10$ distinct elements, in the first round, PBS hashes them into $7$ distinct subset pairs. $6$ distinct elements are hashed into $6$ distinct subset pairs, and the other $4$ distinct elements are hashed into the same subset pair. Then the former $6$ distinct elements are successfully reconciled in the first round and the later $4$ distinct elements remain to be reconciled in the second round, which are hashed into $3$ distinct subset pairs (under a different hash function). $2$ remaining distinct elements are hashed into $2$ distinct subset pairs, and the other $2$ remaining distinct elements are hashed into the same subset pair. Then the former $2$ remaining distinct elements are successfully reconciled in the second round and the later $2$ remaining distinct elements remain to be reconciled in the third round, so on so force. 
%The dynamics of the number of remaining distinct elements (i.e., $10\leadsto 4\leadsto 2\leadsto \cdots$ in the example) is in nature a Markov chain, which will be elaborated and analyzed in \autoref{sec:single_markov} to derive a tight tail bound of the probability that all distinct elements are reconciled in $r$ rounds.

% Even if the ideal case does not happen, most of the distinct elements should be distributed into different subset pairs, one distinct element in each, and therefore can be successfully reconciled. So in the first round, even if PBS cannot reconcile all distinct elements, it can reconcile the majority of them.
% % (piecewise decodability mentioned in \autoref{sec:intro_oursolution})
% Based on this intuition, we generalize PBS to multi-round, so that the distinct elements that are not reconciled yet in the first round can be reconciled in later rounds.  

% Without loss of generality, we only describe the second round of multi-round PBS, the reconciliation in the later rounds are similar. Let $\hat{D}_1$ denote the set of reconciled elements in the first round. If set reconciliation is not complete in the first round (i.e., the checksum infers $A\neq B\Delta \hat{D}_1$), then multi-round PBS saves $\hat{D}_1$, which includes correctly and incorrectly reconciled elements as described in \autoref{subsec:exception_hash_partition}, and starts the second round to find (1) the remaining distinct elements; (2) the incorrectly reconciled distinct elements in the first round. In the second round, multi-round PBS reconciles $A$ and $B\Delta \hat{D}_1$ instead of $A$ and $B$ (i.e., $B\leftarrow B\Delta\hat{D}_1$) to rule out all elements that have been reconciled. {\bf It uses a hash function that is different from the one used in the first round for hash-partition, otherwise every remaining distinct element will be hashed into the same subset pair and cause the same exception (described in \autoref{subsec:exception_hash_partition}) that happened in the first round.}

% If set reconciliation is complete in the second round, the set of reconciled elements in the second round (denoted as $\hat{D}_2$) should be the union of (1) all distinct elements that have not been reconciled in the first round (i.e., $(A\Delta B)\!\setminus\!\hat{D}_1$); and (2) all incorrectly reconciled elements in the first round (i.e., $\hat{D}_1\!\setminus\!(A\Delta B)$), which is by definition the set difference between $A\Delta B$ and $\hat{D}_1$. Therefore, the overall set difference $A\Delta B$ equals to the set difference between $\hat{D}_1$ and $\hat{D}_2$; Else, multiround PBS saves $\hat{D}_2$ and starts the third round, so on so force. 

% {\bf May need this algorithm to show the dynamics, if so, the earlier algorithm needs to change accordingly.}
% \IncMargin{1em}
% \begin{algorithm}
% \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
% \Input{$A$ and $B$}
% \Input{Maximum number of rounds $r$}
% \Output{$D$}

% $\hat{D},\mbox{ complete} \leftarrow PBS(A,B)$\;

% $D \leftarrow \hat{D}$\;

% \While{!complete and $r>0$}{
	
% 	$B \leftarrow B\Delta\hat{D}$\;

% 	$\hat{D},\mbox{ complete} \leftarrow PBS(A,B)$\;

% 	$D \leftarrow D\Delta\hat{D}$\;

% 	$r \leftarrow r-1$\;
% }

% \caption{Multi-round PBS} \label{proto:multirounds}
% \end{algorithm}\DecMargin{1em}

% The idea of multi-round PBS is quite simple: In each round, we discard the reconciled distinct elements in the previous rounds and aim to find the rest distinct elements from the remaining elements. More specifically, the first round of multi-round PBS is just the same as single-round PBS in \autoref{alg:single_round_pbs}. The second round has the same procedures as the first round. One difference is, we update $B$ by $B\leftarrow B\Delta\mathcal{D}$ in the second round, so that (1) Reconciled distinct elements in $\mathcal{D}$ that were contained in $A\Delta B$ are not longer contained in $A\Delta (B\Delta\mathcal{D})$; and (2) The other distinct elements remain in $A\Delta (B\Delta\mathcal{D})$ and can be reconciled later. The other difference is, we use a different hash function for partition (\autoref{step:hash_partition}) in the second round. Later rounds update $B$ in the same way and also use different hash functions. Multi-round terminates if the check in \autoref{step:termination} is correct. The overall set difference $A\Delta B$ is simply the union of reconciled distinct elements in all rounds. 

% A straightforward approach to discard reconciled distinct elements is to remove them from both $A$ and $B$. This approach however incurs additional communication overhead to update $A$, since only Bob learns the partial set difference in \autoref{step:reconcile}. Therefore, we use the approach in \autoref{step:updateb} that only updates $B$. It has another benefit in \autoref{step:termination}, which only needs to transmit the CRC of $A$ from Alice to Bob in the first round. In the later rounds, \autoref{step:termination} can be checked locally by Bob and does not require any additional communication overhead;

% Note that the communication overhead in the first round accounts for a large percentage of the total communication overhead in multi-round PBS, since most of the distinct elements (over $95\%$ as we will show in {\bf point to the figure}) should be reconciled in the first round. Therefore, we use the same parameter $n$ in later rounds because otherwise we have to compute a new parameter that can only save tiny communication overhead, even though the number of remaining distinct elements is small and can be reconciled using smaller $n$ with high probability. {\bf Due to the same reason, we can the same expression of the communication overhead in single-round PBS to approximate the communication overhead in multi-round PBS.}

% The natural termination condition of multi-round PBS is that all distinct elements are reconciled, which could require a large number of rounds and incur large additional communication overhead (each additional round incurs $d\log n$ bits of additional communication overhead on transmitting BCH codeword). To control the amount of additional communication overhead, we set another termination condition that multi-round PBS runs for at most $r$ rounds (typically $2$ or $3$). This termination condition could cause an `early' termination when some distinct elements have not been reconciled. However, under proper parameter settings (to be discussed in \autoref{sec:parameter_settings}), we can prove that the probability of an `early' termination (i.e., set reconciliation is incomplete in $r$ round) is very small
% %, and even if an `early' termination happens, an overwhelming percentage of distinct elements should have been reconciled, which is sufficient for most applications
% . For example, when $d=5, n=255, r=2$, an `early' termination happens with probability $4.8\times 10^{-4}$ (how to compute this probability will be elaborated in \autoref{sec:tail_bound}).

% For the moment, we assume no incorrectly reconciled distinct elements appears in multi-round PBS, which happens with overwhelming probability as explained in \autoref{subsec:exception_hash_partition}. Then multi-round PBS reconciles the distinct elements gradually round by round. This is the ``piecewise decodability'' mentioned in \autoref{sec:intro_oursolution}. We use the following example to describe it in details: Given two sets $A$, $B$ with $10$ distinct elements (i.e., $d=10$), in the first round, multi-round PBS hashes them into $7$ distinct subset pairs. $6$ distinct elements are hashed into $6$ distinct subset pairs, and the other $4$ distinct elements are hashed into the same subset pair. Then the former $6$ distinct elements are successfully reconciled in the first round and the later $4$ distinct elements remain to be reconciled in the second round, which are hashed into $3$ distinct subset pairs (under a different hash function). $2$ remaining distinct elements are hashed into $2$ distinct subset pairs, and the other $2$ remaining distinct elements are hashed into the same subset pair. Then the former $2$ remaining distinct elements are successfully reconciled in the second round and the later $2$ remaining distinct elements remain to be reconciled in the third round, so on so force. The dynamics of the number of remaining distinct elements (i.e., $10\leadsto 4\leadsto 2\leadsto \cdots$ in the example) is in nature a Markov chain, which will be elaborated and analyzed in \autoref{sec:tail_bound_per_group} to derive a tail bound of success probability (i.e., all distinct elements are reconciled in $r$ rounds) for paramenter settings. 

% In most applications, a high percentage of reconciliation (e.g., $>99\%$ distinct elements are reconciled) is good enough. Therefore, we add another termination condition on the maximum number of rounds (denoted as $r$). The larger $r$ is, the higher percentage of distinct elements will be reconciled. How to set parameters based on $r$ will be elaborated in \autoref{sec:parameter_settings};

% Readers may think the communication overhead of multi-round PBS is proportional to the number of rounds. In fact, the majority of the communication overhead is spent in the first round, since most of the distinct elements (over $95\%$ as we will show in {\bf point to the figure}) are reconciled in the first round. Each additional round only incurs a small amount of additional communication overhead. For example, when $d=10, n=255, |\mathcal{U}|=2^{32}$, assume $8$ distinct elements are reconciled in the first round and the rest $2$ distinct elements are reconciled in the second round. Then the communication overhead in the first round is $432$ bits. That number of the second round is only $160$


%the communication overhead of single-round PBS of $272$ ($2d\log n+d\log |\mathcal{U}|+32$) bits, and each additional round incurs $40$ ($d\log n$) bits of additional communication overhead. 

%among the three components of the communication overhead mentioned in \autoref{sec:communication_overhead_single_PBS}, only the first component (i.e., the BCH codeword) is proportional to the number of rounds. The other two components does not depend on the number of rounds.

% The second component only depends on the total number reconciled elements, which is roughly equal to $d$. The third component, the checksum of $A$, only needs to be sent once in the first round.
%Therefore, the communication overhead of multi-round PBS is only slightly larger than that of single-round PBS when the number of rounds is small (say $3$). For example, when $d=5, n=255, |\mathcal{U}|=2^{32}$, the communication overhead of multi-round PBS of $3$ rounds is $352$ bits, which is roughly $1.3$ times of the communication overhead of single-round PBS ($272$ bits).

% Therefore, each additional round of multi-round PBS only incurs a small amount of additional communication overhead. For example, when $d=5, n=255, |\mathcal{U}|=2^{32}$, the communication overhead of single-round PBS of $272$ ($2d\log n+d\log |\mathcal{U}|+32$) bits, and each additional round incurs $40$ ($d\log n$) bits of additional communication overhead. 

% As we explained in \autoref{sec:reconcile_by_trivial}, the communication overhead in each round is proportional to the number of (remaining) distinct elements, which decreases exponentially as the number of round increase (i.e., the first round reconciles $90\%$ of distinct elements, the second round reconciles $90\%$ of the remaining $10\%$ distinct elements, etc.). So the majority of the communication overhead (i.e., $\approx 90\%$) is in the first round. Therefore, we do not bother to optimize parameters (i.e., smaller $n$) in later rounds to save tiny communication overhead, even though remaining distinct elements become fewer and can be reconciled using smaller $n$;

% The termination condition of multi-round PBS is that all distinct elements are reconciled, which may require many rounds. In most applications, a high percentage of reconciliation (e.g., $>99\%$ distinct elements are reconciled) is good enough. Therefore, we add another termination condition on the maximum number of rounds (denoted as $r$). The larger $r$ is, the higher percentage of distinct elements will be reconciled. How to set parameters based on $r$ will be elaborated in \autoref{sec:parameter_settings};

% Multi-round means multiple round-trip delays. {\bf Thanks for the piecewise decodability of PBS, in almost all practical application scenarios, this tradeoff does not lead to longer response time because the reconciliation of objects identified by the successfully decodable codewords, which constitute the vast majority of all codewords, can run in parallel with the transmissions and decodings of the rest.  In other words, the piecewise decodability effective masks the slightly larger number of communication rounds as far as the response time is concerned.}

\begin{comment}
==============================

The pseudocode of set reconciliation operations in each round is shown as follows:

\IncMargin{1em}
\begin{algorithm}
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
\Input{$A$ and $B^{(in)}$}
\Input{Set of reconciled distinct elements $D^{(in)}$}
\Output{$B^{(out)}$}
\Output{Set of reconciled distinct elements $D^{(out)}$}

% Hash-partition $A^{(in)}$, $B^{(in)}$ into $\{A^{(in)}_i\}_{i=1}^n$, $\{B^{(in)}_i\}_{i=1}^n$ (\autoref{sec:hash_partition})\label{step:hash_partition}\;

% Encode $\{A^{(in)}_i\}_{i=1}^n$, $\{B^{(in)}_i\}_{i=1}^n$ into parity bitmaps (\autoref{sec:parity_bitmap_encoding})\;


% Find those subset pairs (denoted them as $(A^{(in)}_{i_1}, B^{(in)}_{i_1}), ...,(A^{(in)}_{i_k}, B^{(in)}_{i_k})$) that parity bits differ (\autoref{sec:BCH_code})\;

Run single-round PBS on $A$ and $B^{(in)}$ to obtain the (partial) set difference $\mathcal{D}$\label{step:reconcile} \;

$D^{(out)} \leftarrow D^{(in)}\bigcup \mathcal{D}$\label{step:updated}\;

$B^{(out)} \leftarrow B^{(in)}\Delta\mathcal{D}$\label{step:updateb}\;

Check whether the set reconciliation is complete by comparing $A$ to $B^{(out)}$ (via CRC)\label{step:termination}\;

\caption{Set reconciliation operations of PBS in each round} \label{proto:multirounds}
\end{algorithm}\DecMargin{1em}

In \autoref{proto:multirounds}, the output $B^{(out)}$ in the $r^{th}$ round is the input $B^{(in)}$ in the $(r+1)^{th}$ round. $D^{(in)}$ and $D^{(out)}$ have the same relationship, and they denote the set of reconciled distinct elements before and after a round. $B^{(in)}$ and $D^{(in)}$ are initialized as $B$ and $\emptyset$ respectively. We omit the currect number of round $r$ in \autoref{proto:multirounds}, since the operations in different rounds are exactly the same. Due to the same reason, we only elaborate the operations in the first round: First, Alice and Bob reconcile $A$ and $B^{(in)}$ $(=B)$ using single-round PBS and Bob obtains the (partial) set difference $\mathcal{D}$ (\autoref{step:reconcile}); Second, Bob updates the set of reconciled distinct elements by merging it with $\mathcal{D}$ (\autoref{step:updated}); Third, Bob updates $B^{(in)}$ $(=B)$ to $B^{(out)}$ as \autoref{step:updateb} shows, such that (1) The reconciled distinct elements in $\mathcal{D}$ that are contained in $A\Delta B^{(in)}$ are not longer contained in $A\Delta B^{(out)}$; and (2) The distinct elements that are not successfully reconciled remain in $A\Delta B^{(out)}$ and can be reconciled in later rounds; Finally, we check whether all distinct elements are reconciled. Note that if it is true, $B^{(out)}$ should be the same as $A$ and multi-round PBS should terminate. We use a $32$-bit CRC (Cyclic Reduncancy Check) to check if $B^{(out)}=A$ in our evaluation. {\bf To achieve higher confidence, we can certainly use longer CRC (e.g., 64-bit). }

{\bf Remarks:}

(1) In each round, hash-partition in \autoref{sec:hash_partition} uses different hash functions, so that the remaining distinct elements from the last round will be hashed into different subset pairs with high probability;

(2) A straightforward approach to discard reconciled distinct elements is to remove them from both $A$ and $B$. This approach however incurs additional communication overhead to update $A$, since only Bob learns the partial set difference in \autoref{step:reconcile}. Therefore, we use the approach in \autoref{step:updateb} that only updates $B$. It has another benefit in \autoref{step:termination}, which only needs to transmit the CRC of $A$ from Alice to Bob in the first round. In the later rounds, \autoref{step:termination} can be checked locally by Bob and does not require any additional communication overhead;

(3) As we explained in \autoref{sec:reconcile_by_trivial}, the communication overhead in each round is proportional to the number of remaining distinct elements, which decreases exponentially as the number of round increase (i.e., the first round reconciles $90\%$ of distinct elements, the second round reconciles $90\%$ of the remaining $10\%$ distinct elements, etc.). So the majority of the communication overhead (i.e., $\approx 90\%$) is in the first round. Therefore, we do not bother to optimize parameters (i.e., smaller $n$) in later rounds to save tiny communication overhead, even though remaining distinct elements become fewer and can be reconciled using smaller $n$;

(4) One termination condition of Multi-round PBS is $B^{(out)}=A$, which refers that all distinct elements are reconciled. In most applications, a high percentage of reconciliation (e.g., $>99\%$ distinct elements are reconciled) is good enough. Therefore, we add another termination condition of the maximum number of rounds (denoted as $r$). The larger $r$ is, the higher percentage distinct elements will be reconciled, and the smaller $n$ is required. How to set parameters (e.g., $n$) based on $r$ will be elaborated in \autoref{sec:parameter_settings};

(5) Multi-round means multiple round-trip delays. {\bf Thanks for the piecewise decodability of PBS, in almost all practical application scenarios, this tradeoff does not lead to longer response time because the reconciliation of objects identified by the successfully decodable codewords, which constitute the vast majority of all codewords, can run in parallel with the transmissions and decodings of the rest.  In other words, the piecewise decodability effective masks the slightly larger number of communication rounds as far as the response time is concerned.}

==============================

\end{comment}

% (3) Readers may wonder in the later rounds, most distinct elements should be reconciled, and the rest distinct elements could be reconciled using degraded parameters (i.e., smaller $n$ and $t$). In fact, degrade parameters in later rounds cannot save much communication overhead, since the majority of it is spent in the first round (i.e., $>90\%$). Therefore, we use the same parameters (i.e., $n,t$) among all rounds in multi-rounds PBS;

% (4) The number of remaining distinct elements decreases exponentially as the number of round increase (i.e., the first round reconciles $90\%$ of distinct elements, the second round reconciles $90\%$ of the remaining $10\%$ distinct elements, etc.). 
% (4) The termination condition of Multi-rounds PBS is $B^{(out)}=A$ to reconcile all distinct elements. In some applications,  


% The output $B^{(out)}$ in the $r^{th}$ round is the input $B^{(in)}$ in the $(r+1)^{th}$ round. $D^{(in)}$ and $D^{(out)}$ are similarly defined. $B^{(in)}$ and $D^{(in)}$ are initialized as $B$ and $\emptyset$ respectively. Since and $D$ are updated in each round, so we use $B^{(in)}$ to denote the input and $B^{(out)}$ to denote the output respectively.  Specifically, in the first round, we initialize $B^{(in)}$ and $D^{(in)}$ as $B$ and $\emptyset$ respectively. we first use the single-round scheme 

% Then we run our (single-round) scheme on the updated two sets (i.e., after removing reconciled distinct elements) using a different (independent) hash-partition function from previous rounds, so that the rest distinct elements are hashed into different subset pairs (i.e., the ideal case) with high probability. At the end of each round, we check whether the set reconciliation is complete (i.e., all distinct elements are found) by computing the bitwise \code{XOR} of the remaining elements in $A$ and $B$ 
 

% This {\bf multi-rounds} scheme can significantly increase the success probability (i.e., the probability that all distinct elements are reconciled). Readers may wonder in the later rounds, most distinct elements should be reconciled, and the rest distinct elements could be reconciled using degraded parameters (i.e., smaller $n$ and $t$). In fact, degrade parameters in later rounds cannot save much communication overhead, since the majority of it is spent in the first round (i.e., $>90\%$). Therefore, we use the same parameters (i.e., $n,t$) among all rounds in our evaluation. 
% %The tradeoff between the number of rounds and the communication overhead per rounds will be elaborated in \autoref{sec:tail_bound}. In our evaluation, $r=2,3$ rounds are enough to achieve an extremely high success probability. 

% Readers may think the cost (i.e., communication overhead and the computational complexity) of this multi-rounds scheme is proportional to the number of rounds (denoted as $r$) and increases linearly with $r$. In fact, the cost of each round is roughly proportional to the number of remaining distinct elements, which decreases exponentially as $r$ increases (i.e., the first round reconciles $99\%$ of distinct elements, the second round reconciles $99\%$ of the remaining $1\%$ distinct elements, etc.). So the cost of this multi-rounds scheme is only slightly larger than that of the single-round scheme. Furthermore, as we explained in \autoref{sec:intro}, {\bf from intro thanks for the piecewise decodability of our solution, in almost all practical application scenarios, this tradeoff does not lead to longer response time because the reconciliation of objects identified by the successfully decodable codewords, which constitute the vast majority of all codewords, can run in parallel with the transmissions and decodings of the rest.  In other words, the piecewise decodability effective masks the slightly larger number of communication rounds as far as the response time is concerned.} 

\begin{comment}

\subsection{Baseline Scheme}\label{subsec:protocol1} 

Note that the set difference $A\Delta B$ can contain more than 1 elements (i.e., $d>1$), and \autoref{alg:trivial_case} cannot reconcile $A$ and $B$ directly in this case. Therefore, we propose a baseline scheme building upon~\autoref{alg:trivial_case} that also works when $d>1$: First, we partition the element universe $\mathcal{U}$ into $n$ sub-universes $\mathcal{U}_1, \mathcal{U}_2, \cdots, \mathcal{U}_n$. Denote $A_i \triangleq A\bigcap \mathcal{U}_i$ and $B_i \triangleq B\bigcap \mathcal{U}_i$ for $i=1,2,\cdots,n$. Then $\{A_i\}_{i=1}^n$ and $\{B_i\}_{i=1}^n$ are partitions of $A$ and $B$ respectively. Furthermore, $\Phi\triangleq\{A_i\Delta B_i\}_{i=1}^n$ is a partition of $A\Delta B$. 

Assume the {\bf ideal case} happens, in which each subset pair $(A_i, B_i)$ contains at most one distinct element ({\it i.e.,} $|A_i\Delta B_i|\!\leq\!1$), we use \autoref{alg:trivial_case} to reconcile each subset pair and obtain $A_i\Delta B_i$ for $i=1,2,\cdots,n$. The overall set difference $A\Delta B$ is simply their union $\bigcup_{i=1}^n \big{(}A_i\Delta B_i\big{)}$. 

In the first step of the baseline scheme, we can use a hash function $h(\cdot): \mathcal{U}\rightarrow \{1,2,\cdots,n\}$ to partition the universe $\mathcal{U}$ into $n$ sub-universes: $\mathcal{U}_i=\{s\mid s\in \mathcal{U} \mbox{ and } h(s)=i\}$ for $\forall i=1,2,\cdots,n$. And the hash function $h(\cdot)$ can be predetermined between Alice and Bob and does not require additional communication cost.

This hash-partition can be modeled as a {\it balls-into-bins problem}, in which the distinct elements are viewed as balls and the subset pairs are viewed as bins. The hash-parition basically throws (hashes) $d$ balls (distinct elements) uniformly and randomly into $n$ bins (subset pairs). The aforementioned ideal case in this context becomes, after throwing $d$ balls uniformly and randomly into $n$ bins, each bin receives at most 1 ball (i.e., $d$ nonempty bins have 1 ball in each and the rest $n-d$ bins are empty). {\bf It may remind readers about the Birthday problem. And the ideal case can be analogous to the case that no people share the same birthday.} The ideal case happens with a probability of $p=\frac{n\,!}{(n-d)\,!n^d}\!=\!\prod_{k=1}^{d - 1}(1 - \frac{k}{n})\!\approx\! e^{-\frac{d(d-1)}{2n}}$ when $d\!\ll\!n$. In other words, $n$ must be $\Omega(d^2)$ to ensure the ideal case happens with a nontrivial probability.  Note that the communication overhead of the baseline scheme is proportional to $n$, as each subset pair requires communication of a bitwise \code{XOR} in \autoref{alg:trivial_case}. So this communication overhead increases at least quadratically as $d$ increases. 

In fact, this communication overhead can be significantly reduced: In the ideal case, $n-d$ out of $n$ subset pairs are identical ones, and only $d (\ll n)$ out of $n$ subset pairs contain distinct elements (one distinct element in each of the $d$ subset pairs) and need to be reconciled. If we can identify these $d$ subset pairs (with a tiny additional communication overhead) and only reconcile them, the overall communication overhead will be significantly reduced from $\Omega(d^2)$ to $O(d)$. Based on this intuition, we propose our scheme in \autoref{sucsec:our-scheme}, which uses Parity Bitmap Sketch (PBS) and Error Correction Coding (ECC) to identify those subset pairs with a tiny additional communication overhead. 

Note that the ideal case does not always happen. However, we can ensure that the ideal case happens with high probability by properly selecting $n$ based on $d$ (i.e., $n=\Omega(d^2)$). Furthermore, as we will describe in \autoref{subsec:nonideal}, even if the ideal case does not happen (i.e., some distinct elements are hashed into the same subset pair), most of the distinct elements should be distributed into different subset pairs and therefore can be reconciled. So the baseline scheme, even cannot reconcile all of the distinct elements, can still reconcile the majority of them. Based on this property, we will extend our scheme from single-round to multi-rounds in \autoref{subsec:nonideal} to further increase the probability of reconciling all distinct elements. 

For general cases ({\it i.e.,} $t=|A\Delta B|$ is an arbitrary number), we have a straightforward strawman scheme building upon~\autoref{alg:trivial_case}, which works as follows: First, Alice and Bob choose some hash function $h(s): \mathcal{U} \rightarrow \{0,1,\cdots,2^{32}-1\}$ to partition $A$ and $B$ into $m$ subsets $A_1,A_2,\cdots,A_m$ and $B_1,B_2,\cdots,B_m$ respectively:

\begin{align}
s\in A_i & \mbox{ iff } s\in A \mbox{ and } h(s)=i\!\mod m, \nonu{}mber\\
s\in B_i & \mbox{ iff } s\in B \mbox{ and } h(s)=i\!\mod m. \nonumber
\end{align} 

{\bf call a subset pair -> partition?} Since Alice and Bob use the same hash function for partition, common elements (i.e., elements in $A\cap B$) are always hashed into the same subset pair $(A_i, B_i)$. And the set difference of each subset pair only contains distinct elements (i.e., elements in $A\Delta B$): $A_i\Delta B_i \subset A\Delta B$. In the ideal case, with a sufficient large $m$, each subset pair $(A_i, B_i)$ contains at most one distinct element ({\it i.e.,} $|A_i\Delta B_i|\!\leq\!1$). Then \autoref{alg:trivial_case} can reconcile each subset pair and obtain $A_i\Delta B_i$ for $i=1,2,\cdots,m$. The overall set difference $A\Delta B$ is simply their union $\bigcup_{i=1}^m \big{(}A_i\Delta B_i\big{)}$. The selection of hash function $h(s)$ can be predetermined between Alice and Bob and it does not require additional communication cost.

%To make sure Alice and Bob use the same hash function for partition, we let them pre-agree on some universal hash family (e.g., \code{xxHash}~\cite{Collet_xxHashExtremelyfast_}) and a common selection order, and each time they choose a hash function from the family in the same order. Note that we can also let Alice generates a hash function and send it to Bob. The hash function that Alice and Bob choose for partition can be either generated by 

This hash-partition is in nature a {\it balls-into-bins model}. We can view the distinct elements as balls and the subset pairs as bins. The hash-parition basically throws (hashes) $t$ balls (distinct elements) uniformly and randomly into $m$ bins (subset pairs). The aforementioned ideal case in this context is, with a sufficient large number of bins, each bin receives at most 1 ball. The strawman scheme works correctly if and only if the ideal case happens, which has a probability of $\frac{m\,!}{(m-t)\,!m^t}\!=\!\prod_{k=1}^{t - 1}(1 - \frac{k}{m})\!\approx\! e^{-\frac{t(t-1)}{2m}}$. In other words, to ensure the strawman scheme works correctly with a probability of $p$, it roughly requires $m \!=\!\lceil \frac{t(t-1)}{-2\ln p}\rceil$ subset pairs. 

Note that the communication overhead of this strawman scheme is proportional to the number of subset pairs $m$, as each subset pair requires communication of an \code{XOR} sum in \autoref{alg:trivial_case} during the reconciliation. When $t$ is small, a small communication cost can guarantee that the strawman scheme works correctly with high probability. For instance, when $t=5$, $m=95$ subset pairs are sufficient for the strawman scheme to work correctly with a probability of $90\%$. However, when $t$ is relatively large, it requires a huge communication cost to ensure the strawman scheme works correctly. For instance, when $t=1,000$, it requires $m=4,740,865$ subset pairs to guarantee a success probability of $90\%$. 

In fact, the majority of subset pairs are identical ones and do not need to reconcile. And only a small portion of them contain distinct elements. If we can identify those subset pairs that contain distinct elements and only reconcile them, the communication cost could be significantly reduced. Our scheme is based on this intuition and uses parity bitmap sketch and BCH code to identify the subset pairs, which we will elaborate in \autoref{sucsec:our-scheme}. 

%To distribute balls as uniformly as possible and maximize the probability of the ideal case, we choose a uniform hashing function $h$ that throws balls uniformly and randomly into bins: $$\mathbb{P}[h(s)=i]=\frac{1}{m} \mbox{ for } \forall i=1,2,\cdots,m, \forall s\in U$$.

%Note that the probability of the ideal case is $\frac{m\,!}{(m-t)\,!m^t}\!=\!\prod_{k=1}^{t - 1}(1 - \frac{k}{m})\!\approx\! e^{-\frac{t(t-1)}{2m}}$. Hence, at least $\lceil \frac{t(t-1)}{-2\ln p}\rceil$ bins are required to ensure that this probability is at least $p$. In other words, to ensure that the ideal case happens with a probability of $p$, the strawman scheme roughly requires $m \!=\!\lceil \frac{t(t-1)}{-2\ln p}\rceil$. For example, suppose $t\!=\!$\num{1000}, %and $p\!=\!0.01$, this strawman scheme roughly requires $m\!=\!$\num{720626} bins (partitions) to ensure that $|A_i\Delta B_i|\!\leq\!1$ (for any $i=1,2,\cdots,m$) holds with probability $50\%$.  

% A straightforward strawman scheme building upon~\autoref{alg:trivial_case} 
% to reconcile two sets $A$ and $B$ in general 
% ({\it i.e.,} $|A\Delta B|$ is an arbitrary number) is the following: 
% Uniformly randomly partition $A$ and $B$ into $m$ subsets ($A_1,A_2,\cdots,A_m$ 
% and $B_1,B_2,\cdots,B_m$) so that the set difference 
% $A_i\Delta B_i$ of each subset pair $(A_i, B_i)$ contains at most one element 
% ({\it i.e.,} $|A_i\Delta B_i|\!\leq\!1$) {\it w.h.p.} ({\it i.e.,} with high probability), 
% and then reconcile each subset pair with~\autoref{alg:trivial_case}. 

% Now let us analyze this strawman scheme using the {\it balls-into-bins model}. 
% Assume that sets $A$ and $B$ have $t$ elements in their set difference, {\it i.e.,} $|A\Delta B|\!=\!t$. 
% These $t$ elements can be viewed as $t$ balls and the $m$ partitions (subset pairs) can be viewed as 
% $m$ bins. The random partition process in this strawman scheme can be modeled as throwing 
% $t$ balls into $m$ bins in the following manner: Each ball goes into a 
% uniformly random bin and independently of other balls. %so that each bin contains at most one ball, {\it w.h.p.}  
% The probability that each bin contains at most one ball is  
% $\frac{m\,!}{(m-t)\,!m^t}\!=\!\prod_{k=1}^{t - 1}(1 - \frac{k}{m})\!\approx\! e^{-\frac{t(t-1)}{2m}}$. 
% Hence, at least $\lceil \frac{t(t-1)}{-2\ln p}\rceil$ bins are required 
% to ensure that this probability is at least $p$. In other words, to ensure 
% that each bin contains at most one ball with a probability of $p$, 
% the strawman scheme roughly requires $m \!=\!\lceil \frac{t(t-1)}{-2\ln p}\rceil$. 
% For example, suppose $t\!=\!$\num{1000}, %and $p\!=\!0.01$, 
% this scheme roughly requires $m\!=\!$\num{108469} bins (partitions) to 
% ensure that $|A_i\Delta B_i|\!\leq\!1$ (for any $i=1,2,\cdots,m$) holds with probability $0.01$.  

% We note that the communication overhead of this strawman scheme is proportional to 
% $m$ ($\!\gg\! t$), as each partition (subset pair) requires communication of an \code{XOR} sum during the reconciliation. 
% This communication overhead is much higher than that of the optimal scheme, which only requires 
% to exchange the elements in the set difference (assuming an oracle tells it which elements belong to 
% the set difference), {\it i.e.,} proportional to $t$. In the example above, assuming each element takes 4 bytes, 
% the communication overhead of the strawman scheme is $4m$ bytes ($\!\approx\! \num{423.71}\,$KB) to ensure 
% a success rate of only 0.01 ({\it i.e.,} with a probability of $0.0.1$, all elements in 
% the set difference are successfully reconciled), 
% which is approximately 2 orders of magnitude higher than $4t$ bytes ($\!=\!\num{3.90}\,$KB), the communication 
% overhead of the optimal scheme. 

\subsection{Our Scheme: The Preliminary Version}\label{sucsec:our-scheme}

Like the baseline scheme, our scheme also hash-partitions the two sets $A$ and $B$ into $n$ subset pairs. The difference is, instead of reconciling all subset pairs using \autoref{alg:trivial_case}, our scheme identifies the subset pairs that contains distinct elements and only reconciles them. Since the hash-partition and set reconciliation on each subset pair using \autoref{alg:trivial_case} have been described in \autoref{subsec:protocol1}, we only elaborate how to identify the subset pairs that contain distinct elements in this section. 

The general idea of identification is very simple: First, we {\bf encode} each subset into $1$ bit, such that in the ideal case, for $\forall i=1,2,\cdots,n$:

\begin{itemize}
	\item The codewords (bits) of $A_i$ and $B_i$ are different if and only if subset pair $(A_i, B_i)$ contains $1$ distinct element;
	\item The codewords (bits) of $A_i$ and $B_i$ are the same if and only if subset pair $(A_i, B_i)$ contains no distinct element;
\end{itemize}

Second, we {\bf compare} the codewords of each subset pair. And the subset pairs that contain distinct elements are the ones with different codewords (bits). We will describe the two steps in details in \autoref{sec:parity_bitmap_encoding} and \autoref{sec:BCH_code} respectively.

\subsubsection{Parity Bitmap Encoding}\label{sec:parity_bitmap_encoding}

In our scheme, we use {\it parity encoding} to encode each subset into a parity bit. More specific, it encodes a subset as ``1'' if it contains odd number of elements, and as ``0'' otherwise. And it satisfies the aforementioned requirements in the ideal case:

\begin{itemize}
	\item If subset pair $(A_i, B_i)$ contains $1$ distinct element, the corresponding two subsets $A_i$ and $B_i$ differ exactly one element, which implies that $||A_i|\!-\!|B_i||\!=\!1$. Hence, if $|A_i|$ ({\it i.e.,} number of elements in $A_i$) is odd (or even), then $|B_i|$ must be even (or odd). And the parity bits of $A_i$ and $B_i$ will be different;
	\item If subset pair $(A_i, B_i)$ contains no distinct element, the corresponding two subsets $A_i$ and $B_i$ should be the same and therefore contain the same number of elements. Hence, if $|A_i|$ is odd (or even), then $|B_i|$ must be odd (or even). And the parity bits of $A_i$ and $B_i$ will be the same;
\end{itemize}

Using parity encoding, the $n$ subsets of $A$ are encoded as a bit string $A[1..n]$ in $\{0,1\}^n$, 
where the $i$-th bit $A[i]$ in $A[1..n]$ corresponds to the parity encoding bit of $A_i$. Similarly, the $n$ subsets of $B$ are similarly 
encoded as a bit string $B[1..n]$. We call $A[1..n]$ ($B[1..n]$) the {\it parity bitmap} of $\{A_i\}_{i=1}^n$ ($\{B_i\}_{i=1}^n$). In the ideal case, $A[1..n]$ and $B[1..n]$ differ at $d$ different bit-positions, which corresponds to the $d$ subset pairs that contain distinct elements. And our scheme only reconciles those subset pairs that the parity bits are different. We will describe the nonideal case (i.e., some subset pair contains more than 1 distinct elements) in \autoref{subsec:nonideal}.

\subsubsection{Parity Bitmap Comparison Using BCH Code}\label{sec:BCH_code}

A straightforward approach to compare the parity bitmaps is to let Bob send the complete parity bitmap $B[1..n]$ to Alice, then Alice compares $A[1..n]$ with $B[1..n]$ locally. This approach has a communication overhead of $n$ bits, which is unnecessarily high. As we discussed in~\autoref{subsec:protocol0}, $d$ is usually much smaller than $n$. It means $A[1..n]$ and $B[1..n]$ differ only at a tiny portion of bits. Therefore, we can view $A[1..n]$ as a corrupted message of $B[1..n]$ with $d$ corrupted bits, and the bit-positions of the $d$ corrupted bits basically correspond to the $d$ subset pairs that contain distinct elements. The detection of corrupted bits, on the other hand, can be solved by Error-Correction Code (ECC)~\cite{Lin_ErrorControlCoding_1983}. And our scheme uses BCH code~\cite{Lint_IntroductionCodingTheory_1998} to encode the parity bitmap and detect the $d$ corrupted bits.

More specific, after the parity bitmap encoding, Bob uses a $d$-error-correcting systematic BCH code to encode $B[1..n]$ into an $n+d\log n$ codeword, in which the first $n$ bits are $B[1..n]$ (property of systematic BCH code). Then Bob sends the rest $d\log n$ bits, which we denote as {\it parity bitmap sketch (PBS)}, to Alice. Upon the received PBS and $A[1..n]$ (corrupted message), Alice uses the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} to detect the $d$ corrupted bits in $A[1..n]$. The communication overhead of this approach is $d\log n$ bits (i.e., length of PBS), which is much smaller than that of the straightforward approach ($n$ bits, when $d\!\ll\!n$). On the other hand, the computational complexity of the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} is $O(d^2\log^2 n)$. 

\subsubsection{Exceptional Handling and Multi-rounds}\label{subsec:nonideal}

As we described in \autoref{subsec:protocol1}, the ideal case does not always happen, which means some subset pair may contain more than 1 distinct elements and cannot be successfully reconciled by \autoref{alg:trivial_case}. Due to the parity encoding, we can classify such subset pair into the following two scenarios:

\begin{itemize}
    \item Scenario 1: If a subset pair $(A_i, B_i)$ contains even number ($\geq 2$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be the same and our scheme will not reconcile the subset pair. Hence, the distinct elements in the subset pair will not be reconciled;
    \item Scenario 2: If a subset pair $(A_i, B_i)$ contains odd number ($\geq 3$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be different and our scheme will reconcile the subset pair using \autoref{alg:trivial_case}. However, as we described in \autoref{subsec:protocol0}, when a subset pair contains more than 1 distinct elements, \autoref{alg:trivial_case} will output the bitwise \code{XOR} of them as the `distinct element', which is not a real distinct element with high probability;
\end{itemize}

In both scenarios, the distinct elements in the subset pair cannot be reconciled. Even worse, in the second scenario, a false-positive could happen (i.e., the output of \autoref{subsec:protocol0} is not a real distinct element). However, as we will analyze in \autoref{sec:tail_bound} and show in {\bf the evaluation section}, the second scenario barely happens both theoretically and empirically. To further reduce the chance of false-positives, we add a verification step at the end of \autoref{subsec:protocol0} to check whether the output of \autoref{subsec:protocol0} $s$ is a real distinct element or not. The verification step works as follows: Given the output $s$ of subset pair $(A_i,B_i)$, if $s\in\mathcal{U}_i$ (i.e., $h(s)=i$), we consider $s$ as a real distinct element; Otherwise, we consider $s$ as an incorrect output and discard it. 

Note that if $s$ is a real distinct element of $(A_i,B_i)$, $s$ must be in sub-universe $\mathcal{U}_i$. However, if $s$ is the bitwise \code{XOR} of the distinct elements in $(A_i,B_i)$ (i.e., the second scenario happens), $s$ could be in any sub-universe other than $\mathcal{U}_i$. In fact, if we assume the hash-partition described in \autoref{subsec:protocol1} hashes the elements of $\mathcal{U}$ uniformly, independently, and randomly into $n$ sub-universes, the output $s$ in the second scenario will be in a different sub-universe $\mathcal{U}_j (j\neq i)$ with a high probability of $1-\frac{1}{n}$. Hence, this verfication step can reduce the chance of false-positives by a factor of $\frac{1}{n}$. 

Even if the ideal case does not happen, most of the distinct elements should be distributed into different subset pairs and therefore can be reconciled. So our scheme, even cannot reconcile all of the distinct elements, can still reconcile the majority of them (piecewise decodability). To reconcile the rest distinct elements, we can just run our scheme for another round under a different hash-partition function, so on so force. This {\bf multi-rounds} scheme can significantly increase the success probability (i.e., the probability that all distinct elements are reconciled). Readers may wonder in the later rounds, most distinct elements should be reconciled, and the remaining could be reconciled using degraded parameters (i.e., smaller $n$ and $t$). In fact, degrade parameters in later rounds cannot save much communication overhead, since the majority of it is spent in the first round (i.e., $>90\%$). Therefore, we use the same parameters (i.e., $n,t$) among all rounds in our evaluation.
%The tradeoff between the number of rounds and the communication overhead per rounds will be elaborated in \autoref{sec:tail_bound}. In our evaluation, $r=2,3$ rounds are enough to achieve an extremely high success probability. 

Readers may think the cost (i.e., communication overhead and the computational complexity) of this multi-rounds scheme is proportional to the number of rounds (denoted as $r$) and increases linearly with $r$. In fact, the cost of each round is roughly proportional to the number of remaining distinct elements, which decreases exponentially as $r$ increases (i.e., the first round reconciles $99\%$ of distinct elements, the second round reconciles $99\%$ of the remaining $1\%$ distinct elements, etc.). So the cost of this multi-rounds scheme is only slightly larger than that of the single-round scheme. Furthermore, as we explained in \autoref{sec:intro}, {\bf from intro thanks for the piecewise decodability of our solution, in almost all practical application scenarios, this tradeoff does not lead to longer response time because the reconciliation of objects identified by the successfully decodable codewords, which constitute the vast majority of all codewords, can run in parallel with the transmissions and decodings of the rest.  In other words, the piecewise decodability effective masks the slightly larger number of communication rounds as far as the response time is concerned.} 

\end{comment}


%%% Moved from related work
\input{section/pinsketch}

\section{PBS for large \texorpdfstring{\larger\boldmath\MakeLowercase{$d$}}{d}}\label{subsec:protocol2}

The scheme above, which we refer as PBS-for-small-$d$, can also do set reconciliation when $d$ is large. However, the BCH decoding computational complexity in it is $O(d^2)$ of finite field operations (in GF($2^{8}$) when $n=255$) using the state-of-the-art decoding algorithm~\cite{Dodis_SyndromeEncodingDecoding_2006}, which is too expensive for large $d$. To overcome this drawback, we use the same technique in \autoref{sec:hash_partition} to hash-partition sets $A$ and $B$ each into $d/\delta$ subsets (which we call {\it groups} to distinguish from subsets) for some small integer $\delta$ (say $5$), so that each of the group pairs contains roughly $\delta$ distinct elements and can be reconciled by PBS-for-small-$d$ respectively. The BCH decoding computational complexity of each group pair is roughly $O(\delta^2)$, which can be considered as $O(1)$, since $\delta$ is a small number. As a result, the overall computational complexity is reduced from $O(d^2)$ to $O(d)$. 
%{\bf In PBS, we set $\delta = 5$. }

%Note that the BCH decoding computational complexity is $O(d^2)$ of finite field operations (in GF($2^{8}$) when $n=255$) using the state-of-the-art decoding algorithm~\cite{Dodis_SyndromeEncodingDecoding_2006}, which is too expensive for large $d$. To overcome this drawback, we first hash-partition sets $A$ and $B$ each into $d/\delta$ subsets (which we call {\it groups} to distinguish from subsets), just like what we did in \autoref{sec:hash_partition}, for some small integer $\delta$ (say $5$), then reconcile each of the group pairs by the PBS we described in \autoref{sec:scheme}. After the partition, each group pair has $\delta$ distinct elements on average. So the BCH decoding computational complexity of each group pair is roughly $O(\delta^2)$, which can be considered as a constant, since $\delta$ is a small number. As a result, the overall computational complexity of PBS is reduced from $O(d^2)$ to $O(d)$. 

%To differentiate from the PBS described in \autoref{sec:scheme}, we refer to it as PBS-basic in this section. 
We continue to assume that the number of distinct elements $d$ is precisely known. Even so, due to the randomness of hash-partition, denoted as $\delta_i$, the number of distinct elements in the $i$-th group pair, is a variable with mean of $\delta$ for $i=1,2,...,g$, which are not precisely known. Since $\delta_1, \delta_2, ..., \delta_g$ follows the same distribution, it does not make sense to select different parameters for the $g$ group pairs. Hence, we set two universal parameters, $t$ and $n$, for all group pairs, where $t$ is the error-correction capability of the BCH code used for reconciling each group pair, and $n$ is the number of subset pairs in each group pair.

% We continue to assume that the number of distinct elements $d$ is precisely known. Even so, due to the randomness of hash-partition, denoted as $\delta_i$, the number of distinct elements in the $i$-th group pair, is a Binomial random variable with mean of $\delta$ for $i=1,2,...,g$, which cannot be precisely known without a huge amount of additional communication overhead. Since $\delta_1, \delta_2, ..., \delta_g$ follows the identical Binomial distribution, it does not make sense to select different parameters for the $g$ group pairs. Hence, we set two universal parameters, $t$ and $n$, for all group pairs, where $t$ is the error-correction capability of the BCH code used for reconciling each group pair, and $n$ is the number of subset pairs in each group pair.

%To deal with this randomness, we set two global parameters, denoted as $t$, that corresponds to the error-correction capability of the BCH code used for reconciling every group pair. identical no sense or additonal info

%{\bf (modified based on the next paragraph from intro)} 
{\bf The error-correction capability $t$, defined as the maximum number of errors that the BCH code used by any group pair can correct, is a critical parameter for PBS to perform well. On one hand, if $t$ is too large (say $t=10\delta$), then the communication overhead on transmitting BCH codeword ($t\log n$ bits per group pair) is unnecessarily large; but on the other hand, {\bf if $t$ is too small (say equal to $\delta$), any group pair $i$ could contain more than $t$ distinct elements with a nontrivial probability (i.e., $Pr[\delta_i>t]$ is nontrivial). If so, in the ideal case, the $\delta_i$ distinct elements incur $\delta_i$ bit errors in the BCH codeword, which exceeds the error-correction capability $t$ and a BCH decoding failure happens (we will describe in \autoref{sec:BCH_exception}).}
{\color{blue} (previous) if $t$ is too small (say equal to $\delta$), then close to half of the group pairs fail to decode the BCH codeword due to the insufficient error-correction capability, which can result in hefty penalties on BCH decoding failures (to be described in \autoref{sec:BCH_exception}). }
In PBS, we manage to make $t$ as small as possible (so that the communication overhead on transmitting BCH codewords is kept to a minimum) yet pay negligible penalties of BCH decoding failures. }

\noindent {\bf Communication overhead of PBS Per Group Pair in the first round:} Same as PBS-for-small-$d$, the communication overhead of PBS per group pair in the first round also consists of the four components described in \autoref{sec:communication_overhead_single_PBS}. The expectation of the communication overhead of each component equals to the corresponding component of PBS-for-small-$d$ when $d=\delta$, except for the BCH codeword, which is $t\log n$ bits as we described earlier. The communication overhead of PBS per group pair in the first round on average is roughly

\begin{equation}\label{eq:communication_overhead}
t\log n + \delta\log n +\delta \log |\mathcal{U}|+32
\end{equation}

% To ensure the error-correction capability $t$ is sufficient (i.e., $t\geq \delta_i$ for $i=1,2,...,g$) for every group pair with high probability, we set $t$ conservatively and leave a sufficient `safety margin' between $t$ and the average number of distinct elements in each group pair $\delta$. 

% Note that the `safety margin' between $t$ and $\delta$ incurs additional communication overhead on transmitting BCH codeword: In the perfect scenario (i.e., $\{d_i\}_{i=1}^g$ is precisely known), the average communication overhead on transmitting BCH codeword per group pair is $\delta\log n$; On the other hand, when we set $t$ to be the error-correction capability for each group pair, the average communication overhead becomes $t\log n$. If we set the `safety margin' to be too large (say $t=10\delta$), it will incur huge additional communication overhead. Due to this reason, we set a moderate `safety margin' that  $t$ in the range from $1.5\delta$ to $3\delta$. 

% {\bf (moved from intro, to be removed)} The number of elements in the set difference between any group pair is in general not a constant.  Rather, it is a random variable that has roughly a Poisson distribution with mean $\delta$.  The potential issue arises from dealing with this randomness in setting a global parameter that corresponds to the error-correction capability of the BCH code used for reconciling every group pair.  This parameter, denoted as $t$ (consistent with other literatures on BCH code), is the maximum number of errors that the BCH code used by any group pair can correct, and the size of each such codeword is roughly $8t$ bits (assuming $n = 255$ as explained above). The issue is that, on one hand, if $t$ is too large (say several times larger than $\delta$), then the total size of the BCH codewords, which is the bulk of the extra communication cost, is unnecessarily large; but on the other hand, if $t$ is too small (say equal to $\delta$), then close to half of the BCH codewords cannot decode or worse decode incorrectly (unknown to Alice and Bob), which can result in hefty penalties in the latter case of incorrect decoding.   In PBS, we manage to make $t$ as small as possible (so that the total size of the BCH codewords is kept to a minimum) yet pay negligible penalties of incorrect BCH decoding.
%We will discuss the case that $d_i>t$ in \autoref{sec:BCH_exception}.

% Hence, we can no longer set the error-correction capability of the BCH code for each group pair based on the exact number of distinct element in it, as we did in \autoref{sec:scheme}. Instead, we set a conservative error-correction capability $t$ (say $2.5\delta$) for all group pairs, which is sufficient for them (i.e., $t\geq d_i$ for $i=1,2,...,g$) with high probability. We will discuss the case that $d_i>t$ in \autoref{sec:BCH_exception}.


% ===============================
% To differentiate from the PBS described in \autoref{sucsec:our-scheme}, we refer it as PBS-basic in this section. Note that the BCH decoding computational complexity is $O(d^2\log ^2 n)$, which is $\Omega(d^2\log^2 d)$ when $n=\Omega(d^2)$, with the state-of-the-art decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019}. It is too large in PBS-basic for large $d$. To overcome this drawback and generalize PBS-basic for large $d$, we partition sets $A$ and $B$ each into $d/\delta$ subsets (which we call {\it groups} to distinguish from subsets) for some small integer $\delta$ (say $5$) and reconcile the $d/\delta$ group pairs respectively using PBS-basic. After this partition, each group has $\delta$ distinct elements on average. The BCH decoding computational complexity of each group pair can be considered as $O(1)$, since $\delta$ is a small number. As a result, the overall computational complexity of PBS is reduced from $O(d^2\log ^2 n)$ to $O(d)$. 

% % To differentiate from the PBS described in \autoref{sucsec:our-scheme}, we refer it as PBS-basic in this section. PBS-basic is not suitable for large $d$ for two reasons: First, its communication overhead is asymptotically $O(d\log n)\!=\!O(d\log d)$ (since $n=\Omega(d^2)$), which is not asymptotically optimal. Second, the decoding computational complexity is proportional to $d^2$ with the state-of-the-art decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} for BCH codes, which is too high when $d$ is large. To overcome these two drawbacks, we use a simple algorithmic trick to (1) reduce the communication overhead from $O(d\log d)$ to $d\log u \!+\! O(d)$; (2) reduce the decoding computational complexity from $O(d^2)$ to $O(d)$. 

% Now, we describe the generalized PBS in details: In the first step, we hash-partition $A$ and $B$ (by some hash function $h_1(\cdot)$) into $g$ group pairs, just like what we did in \autoref{sucsec:our-scheme}. The objective of this partition is however different: In \autoref{sucsec:our-scheme}, we aim to ensure each subset pair contains at most $1$ distinct element (i.e., the ideal case) with high probability; Here we aim to make each group pair contains roughly $\delta$ distinct elements for some small constant $\delta$ (say $5$) by setting $g=d/\delta$. 
% %To differentiate the $g$ subset pairs here from those in \autoref{sec:hash_partition}, we call them the $g$ {\bf groups} in the sequel. 
% In the second step, we just apply PBS-basic (described in \autoref{sucsec:our-scheme}) to reconcile each group pair and obtain the distinct elements. 
% ================================

% To differentiate from the PBS described in \autoref{sucsec:our-scheme}, we refer it as PBS-basic in this section. When $d$ is large (more than several), we hash-partition set $A$ and $B$ into groups, such that each group pair contains $\delta$ distinct elements on average for small $\delta$ (say $5$), as described in \autoref{sec:larged}. Then each group pair can be reconciled by PBS-basic.

% When describing the PBS-basic in \autoref{sucsec:our-scheme}, we assume that the number of distinct elements is precisely known. We set the error-correction capability of the BCH code (denoted as $t$) just enough to correct $d$ errors (i.e., $t=d$). However, due to the randomness of hash-partition, $d_i$, the number of distinct elements in the $i^{th}$ group pair, is a Binomial random variable $Binomial(d,1/g)$ with expectation of $\delta$ $(=d/g)$ for $i=1,2,...,g$, which cannot be precisely known without a huge amount of additional communication overhead. Hence, we can no longer set the error-correction capability of the BCH code for each group pair based on the exact number of distinct element in it, as we did in \autoref{sucsec:our-scheme}. Instead, we set a universal error-correction capability $t$ (say $2.5\delta$) for all group pairs, which is sufficient for all group pairs (i.e., $t\geq d_i$ for $i=1,2,...,g$) with high probability. We will discuss the case that $d_i>t$ in \autoref{sec:BCH_exception}.

%This assumption in general does not hold: 
% Let $d_i$ denote the number of distinct elements in Group $i$. Due to the property of hash-partition, each $d_i$ is a Binomial random variable $Binomial(d,1/g)$ with expectation of $\delta$ $(=d/g)$. Even if $d$ is precisely known, each $d_i$ is not. To ensure the error-correction capability $t$ is sufficient for each group (i.e., $d_i\leq t$) with high probability, we leave some safety margin for the randomness of $d_i$ and conservatively set $t$ roughly $2.5\delta$ (the factor $2.5$ varies depend on other parameters, which will be discussed in \autoref{sec:parameter_settings}), so that $Pr[d_i>t]$ is tiny. We will discuss the case that $d_i>t$ in \autoref{sec:BCH_exception}.

% Note that the `safety margin' between $t$ and $\delta$ incurs additional communication overhead on transmitting BCH codeword: In the perfect scenario (i.e., $\{d_i\}_{i=1}^g$ is precisely known), the average communication overhead on transmitting BCH codeword per group pair is $\delta\log n$; On the other hand, when we set $t$ to be the error-correction capability for each group pair, the average communication overhead becomes $t\log n$. If we set the `safety margin' to be too large (say $t=10\delta$), it will incur huge additional communication overhead. Due to this reason, we set a moderate `safety margin' that  $t$ in the range from $1.5\delta$ to $3\delta$. 

%which is roughly $2.5$ times of that in the perfect scenario (when $t$ is roughly $2.5\delta$). Due to this addition
{\bf (modified)} One alternative is to estimate each $\delta_i$ and then set $t_i$, defined as the error-correction capabilities of the $i$-th group pairs, to be very close to (slightly larger) the estimation of $\delta_i$. It can save considerate communication overhead on transmitting the BCH code. However, to estimate all the $g$ values of $\{\delta_i\}_{i=1}^g$ in high accuracy requires much larger additional communication overhead than the savings. For example, estimating each $\delta_i$ requires $288$ bytes of additional communication overhead using the ToW estimator, as we will describe in \autoref{subsec:ToW}. However, the ``savings'' on the communication overhead for group pair $i$ is at most $t\log n-\delta_i\log n$, which is only $10$ bytes when $\delta_i=5, t=15, n=255$.


% {\bf (previous)} Readers may wonder if we can reduce this additional communication overhead by using some technique to estimate $\{d_i\}_{i=1}^g$ (e.g., ToW estimator in \autoref{subsec:ToW}), so that we can set the error-correction capability of each group more wisely and save some waste on the safety margin. However, to achieve that, the estimation on $\{d_i\}_{i=1}^g$ must be in extremely high precision (since $\{d_i\}_{i=1}^g$ are small numbers with mean of $\delta$), which incurs much larger additional communication overhead than the savings. Due to the same reason (i.e., estimate $\{d_i\}_{i=1}^g$ is costly), we set the number of subset pairs for each group pair to be all equal (denoted as $n$). 
%based on $\delta$ ($n=\Omega(\delta^2)$). 

% {\bf (moved from the small d case)} Note that the set reconciliation process of the group pairs are independent with each other, and each group pair runs as many rounds of PBS-for-small-$d$ as needed to reconcile all distinct elements in it. Therefore, different group pairs may need different number of rounds to be successfully reconciled. Intuitively, we want all group pairs to be successfully reconciled in only a few rounds (say $3$) with high probability (say $99\%$). Hence, when tuning parameters (to be discussed in \autoref{sec:parameter_settings}), we set a {\it target success probability} $p_0$ combined with a {\it target number of rounds} $r$ as the {\it paramenter setting requirement}, which aims to ensure that the {\it success probability}, the probability that all distinct elements (of all group pairs) are reconciled, within $r$ rounds to be at least $p_0$. 
% {\bf Normally, to achieve the same target success probability within fewer rounds (smaller $r$), PBS need more resources (e.g., larger $n$, $t$) for the ideal case happening with higher probability (fewer exceptions happen and need to be handled in later rounds), as we will explain in \autoref{sec:vary_r}.}

% {\bf (moved from the small d case)} Although PBS runs as many rounds as needed to reconcile all distinct elements (in each group pair), we want PBS to successfully reconcile all distinct elements in only a few rounds (say $3$) with high probability (say $99\%$). Hence, when tuning parameters (to be discussed in \autoref{sec:parameter_settings}), we set a {\it target success probability} $p_0$ combined with a {\it target number of rounds} $r$ as the {\it paramenter setting requirement}, which aims to ensure that the {\it success probability}, the probability that all distinct elements are reconciled, within $r$ rounds to be larger than $p_0$. 
% {\bf Normally, to achieve the same target success probability within fewer rounds (smaller $r$), PBS need more resources (e.g., larger $n$, $t$) for the ideal case happening with higher probability (fewer exceptions happen and need to be handled in later rounds), as we will explain in \autoref{sec:parameter_settings}.}

%This success probability (within $r$ rounds) is also the expected value of the {\it success rate} of PBS, which is defined as the number of `successful' experiments (all distinct elements are successfully reconciled within $r$ rounds) divided by the total number of experiments. 

%The requirement above should also ensure the majority of the distinct elements are reconciled in the first round. 
% Note that PBS reconciles the distinct elements gradually round by round. The distinct elements that have been reconciled in the first round are no longer needed to be reconciled again in later rounds. This is the ``piecewise decodability'' mentioned in \autoref{sec:intro_oursolution}. The requirement above also ensures the majority of the distinct elements are reconciled in the first round, as we will show in \autoref{sec:piecewise_decodability}. Therefore, the majority of the overall communication overhead happens in the first round. In other words, the overall communication overhead of all rounds is only slightly larger than ($1.01$ to $1.07$ times of) that in the first round. Due to this reason, we use the communication overhead in the first round (described in \autoref{sec:communication_overhead_single_PBS}) to approximate the overall communication overhead of all rounds in parameter settings (to be elaborated in \autoref{sec:parameter_settings}.


% Like what we did in \autoref{sec:multi-rounds}, we set a paramenter setting requirement on the target success probability $p_0$ of $r$ rounds for all group pairs, which ensures the probability that all group pairs are completely reconciled in $r$ rounds to be larger than $p_0$. The detail about how to set $n$, $g$, and $t$ given such a success probability requirement will be elaborated in \autoref{sec:parameter_settings}. 

% we set a {\it target success probability} $p_0$ of $r$ rounds as a paramenter setting requirement, which aims to ensure the probability that all distinct elements are reconciled in $r$ rounds to be larger than $p_0$. This requirement should also ensure the majority of the distinct elements are reconciled in the first round. Use the same example ($d=5, n=255$), on average $4.81$ out of $5$ distinct elements should be reconciled in the first round. So the total communication overhead in all rounds is only slightly larger than ($1.01$ to $1.07$ times of, as we will show in \autoref{fig:per-round-con}) that in the first round. Due to this reason, we use the communication overhead in the first round (described in \autoref{sec:communication_overhead_single_PBS}) to approximate the total communication overhead of all rounds in parameter settings (to be elaborated in \autoref{sec:parameter_settings}.

% Note that this safety margin incurs additional communication overhead on transmitting BCH codeword: In the perfect scenario (i.e., $\{d_i\}_{i=1}^g$ is precisely known), the average communication overhead on transmitting BCH codeword per group is $\delta\log n$; On the other hand, when we set $t$ to be the error-correction capability for each group, then the average overhead becomes $t\log n$, which is roughly $2.5$ times of that in the perfect scenario (when $t$ is roughly $2.5\delta$). Readers may wonder if we can reduce this additional communication overhead by using some technique to estimate $\{d_i\}_{i=1}^g$ (e.g., ToW estimator in \autoref{subsec:ToW}), so that we can set the error-correction capability of each group more wisely and save some waste on the safety margin. However, to achieve that, the estimation on $\{d_i\}_{i=1}^g$ must be in high precision, which requires a much higher communication overhead than the savings.

% Although PBS may need to run many rounds to reconcile all distinct elements, the communication overhead mostly happens in the first round, since the majority of the distinct elements should be reconciled in the first round. Use the same example ($d=5, n=255$), on average $4.81$ out of $5$ distinct elements should be reconciled in the first round. So the total communication overhead in all rounds is only slightly larger than ($1.01$ to $1.07$ times of, to be shown in \autoref{fig:per-round-con}) that in the first round. Due to this reason, we use the communication overhead in the first round (described in \autoref{sec:communication_overhead_single_PBS}) to approximate the total communication overhead (all rounds) in parameter settings (to be elaborated in \autoref{sec:parameter_settings}).

%For the moment, we assume no ``fake'' distinct element in type (\RN{2}) subset pairs fails to be detected, which happens with overwhelming probability as explained in \autoref{subsec:exception_hash_partition}. Then 

% PBS reconciles the distinct elements gradually round by round. This is the ``piecewise decodability'' mentioned in \autoref{sec:intro_oursolution}. We use the following example to describe it in details: 
% Given two sets with $10$ distinct elements, in the first round, PBS tries to reconcile the $10$ distinct elements and say $6$ out of the $10$ distinct elements are successfully reconciled. Then the $6$ reconciled distinct elements are removed and PBS tries to reconcile the remaining $4$ distinct elements in the second round. Say $2$ out of the $4$ remaining distinct elements are successfully reconciled, and that leaves $2$ remaining distinct elements to be reconciled in the third round, so on so force. 
% % Given two sets $A$, $B$ with $10$ distinct elements, in the first round, PBS hashes them into $7$ distinct subset pairs. $6$ distinct elements are hashed into $6$ distinct subset pairs, and the other $4$ distinct elements are hashed into the same subset pair. Then the former $6$ distinct elements are successfully reconciled in the first round and the later $4$ distinct elements remain to be reconciled in the second round, which are hashed into $3$ distinct subset pairs (under a different hash function). $2$ remaining distinct elements are hashed into $2$ distinct subset pairs, and the other $2$ remaining distinct elements are hashed into the same subset pair. Then the former $2$ remaining distinct elements are successfully reconciled in the second round and the later $2$ remaining distinct elements remain to be reconciled in the third round, so on so force. 
% The dynamics of the number of remaining distinct elements (i.e., $10\leadsto 4\leadsto 2\leadsto \cdots$ in the example) is in nature a Markov chain, which will be elaborated and analyzed in \autoref{sec:single_markov} to derive a tight tail bound of the probability that all distinct elements are reconciled in $r$ rounds. 

%, which we will show in \autoref{subsec:mini-partition}.

% The same algorithmic trick can also be implemented in PinSketch~\cite{Dodis_PinSketch_2008} to reduce it computational complexity from $O(d^2)$ to $O(d)$. However, it will encounter the same randomness problem and have to set up a safety margin on the error-correction capability. This safety margin will incur much more communication overhead on PinSketch than on our scheme: Considering the average communication overhead per group, in our scheme, this overhead can be expressed as $t\log n+\delta\log n+\delta \log u+32$, in which $t\log n$ accounts for the BCH codeword, $\delta\log n$ accounts for the index of the subset pairs, $\delta \log u$ accounts for the bitwise \code{XOR} in \autoref{alg:trivial_case}, and $32$ accounts for the $32$-bit CRC in \autoref{proto:multirounds}. In PinSketch, this overhead increases from $O(\delta\log u)$ (optimal) to $O(t\log u)$ (PinSketch does not need to transmit bitwise \code{XOR}) if it uses the same algorithmic trick. Use the same example in \autoref{sec:intro}, when $\delta=5, n=255, u=2^{32}, t=2.5\delta$, the overhead of PinSketch using the trick is $2.5$ times of the optimal, while that of our scheme is $2.075$ times of the optimal (as we introduced in \autoref{sec:intro_oursolution}). That means our scheme has a lower communication overhead than PinSketch if they both use the algorithmic trick. Furthermore, as the signiture size $\log u$ increases, the advantage of our scheme over PinSketch becomes more significantly, which we will show in \autoref{subsec:mini-partition}.

% In PinSketch, each bit encodes only a single element in the universe, so the size of the bitmap is equal to the size of the universe.  
% For example, in the set reconciliation problem we usually assume each element is ``indexed" by a $32$-bit-long (hash) signature, so the universe contains a total of $2^{32}$ elements. In this case, the bitmap encoding for any set in PinSketch is $2^{32}$ bits long, and the Galois field involved in its BCH decoding is the ``$32$-bit-wide" $GF(2^{32})$.  In contrast, as explained earlier, in PBS 
% %since each bit encodes the oddness or evenness of the cardinality of a subset,   
% the size $n$ of a bitmap is dependent only on $d$, and not on the size of the universe or on the cardinality of the set the bitmap encodes.   For example, as shown in the example above, $n = 255$ is large enough for $d = 5$.  In this case, the BCH decoding operates in the much shorter
% ``8-bit-wide" $GF(2^{8})$.  This shorter ``width" alone in theory translates into roughly $16$ times shorter BCH decoding time, which as will be explained in~\ref{} grows quadratically with the ``width" of the underlying Galois field.  This shorter ``width" also implies four times shorter BCH codeword in PBS than in PinSketch, resulting in lower communication complexity as will be shown in~\autoref{}.

% Note that our scheme only takes 1 round trip delay to both identify the $d$ subset pairs and reconcile them: In the first half, Bob computes and sends PBS to Alice. Then Alice locally identifies the $d$ subset pairs and then initiates the reconciliation ({\it i.e.,} \autoref{alg:trivial_case}) for them, {\it i.e.,} computes the bitwise \code{XOR} of the corresponded $d$ subsets. In the second half, Alice sends the bitwise \code{XOR} of the $d$ subsets with their indexes to Bob. Then Bob can compute the set difference $A\Delta B$ locally.


% We can certainly use some communication-efficient technique to estimate $d_i$ (e.g., \autoref{subsec:ToW}). However, to obtain $d_i$ precisely will require a communication cost almost as large as to reconcile Group $i$. So instead of obtaining $d_i$ and set $c_i$ (i.e., the error-correction capability of Group $i$) equal to $d_i$, we leave the randomness of $d_i$ and set $c_i$ neither too conservative, nor too libertive in the following sense: (1) $c_i$ is not too big (conservative, i.e., $10\delta$) to make the total size of PBS unnecessarily large and incur too much extra communication overhead; (2) $c_i$ is not too small (libertive, i.e., $\delta$) to incur a high probability of insufficient decode capability, which can result in hefty penalties in the latter case of incorrect decoding (will be elaborated in \autoref{sec:BCH_exception}). In our scheme, we set $c_i$ to be $2-3$ times of $\delta$, which will be shown in \autoref{sec:tail_bound} that it is just enough to make the probability of decode failure very small. Meanwhile, we set the error-correction capability of each group ($c_1,c_2,...,c_k$) to be all equal and denote it as $c$. 

%Since the decoding capacity $t$ and the number of subset pairs for each group $n$ are both small constants independent of $d$, therefore, the communication overhead per group is $t\cdot\log n \!=\!O(1)$, which implies a total communication overhead of $O(d)$. Similarly, the total decoding computational complexity is also $O(d)$. 

% \subsection{Exception Handling}\label{sec:exceptions}

% \subsubsection{Exception Handling on Hash-Partition}\label{subsec:exception_hash_partition}

% As we have described in \autoref{sec:hash_partition}, the ideal case does not always happen, which means some subset pair may contain more than 1 distinct elements and cannot be successfully reconciled by \autoref{alg:trivial_case}. Due to the parity encoding, we can classify such subset pair into the following two scenarios:

% \begin{itemize}
%     \item Scenario 1: If a subset pair $(A_i, B_i)$ contains even number ($\geq 2$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be the same and our scheme will not reconcile the subset pair. Hence, the distinct elements in the subset pair will not be reconciled;
%     \item Scenario 2: If a subset pair $(A_i, B_i)$ contains odd number ($\geq 3$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be different and our scheme will reconcile the subset pair using \autoref{alg:trivial_case}. However, as we described in \autoref{subsec:protocol0}, when a subset pair contains more than 1 distinct elements, \autoref{alg:trivial_case} will output the bitwise \code{XOR} of them as the `distinct element', which is not a real distinct element with high probability;
% \end{itemize}

% In both scenarios, the distinct elements in the subset pair cannot be reconciled. Even worse, in the second scenario, a false-positive could happen (i.e., the output of \autoref{subsec:protocol0} is not a real distinct element). For example, if subset pair $(A_i, B_i)$ contains $3$ distinct elements $s_1, s_2, s_3$, then the output of \autoref{alg:trivial_case} is $\tilde{s}_4=s_1\oplus s_2\oplus s_3$, which is normally not a distinct element. The good thing is, the probability of the false-positive is extremely small for small $d$. For instance, if $d=5$ and $n=255$, the probability of the false-positive is $7.6\times 10^{-6}$, which is very small. To further reduce the chance of false-positives, we add a verification step at the end of \autoref{subsec:protocol0} to check whether the output of \autoref{subsec:protocol0} $s$ is a real distinct element or not. The verification step works as follows: Given the output $s$ of subset pair $(A_i,B_i)$, if $s\in\mathcal{U}_i$ (i.e., $h(s)=i$), we consider $s$ as a real distinct element; Otherwise, we consider $s$ as an incorrect output and discard it. 

% Note that if $s$ is a real distinct element of $(A_i,B_i)$, $s$ must be in sub-universe $\mathcal{U}_i$. However, if $s$ is the bitwise \code{XOR} of the distinct elements in $(A_i,B_i)$ (i.e., the second scenario happens), $s$ could be in any sub-universe other than $\mathcal{U}_i$. In fact, if we assume the hash-partition described in \autoref{sec:hash_partition} hashes the elements of $\mathcal{U}$ uniformly, independently, and randomly into $n$ sub-universes, the output $s$ in the second scenario will be in a different sub-universe $\mathcal{U}_j (j\neq i)$ with a high probability of $1-\frac{1}{n}$. Hence, this verfication method can further reduce the probability of false-positives by a factor of $\frac{1}{n}$. Use the same example (i.e., $d=5$, $n=255$), the probability is reduced from $7.6\times 10^{-6}$ to $3\times 10^{-8}$ by this verification method. 

% In some super critical cases (i.e., no false-positive is allowed), we can use a more powerful verification method to completely eliminate false-positives. That is, to check if the output $s$ exists in exactly one of the two sets (i.e., $s\in A\setminus B$ or $s\in B\setminus A$). To do so, Bob transmits $s$ along with an identification bit $\mathbb{1}_{\{s\in B\}}$ to Alice, then Alice checks if $s$ . This method verification costs $d(\log u+1)$ bits of additional communication overhead. In most applications, rigorously $0\%$ probability of false-positives is unnecessary and the probability of the former verification method is small enough, so we use the former verfication method in our evaluation. Based on our observation, the false-positive does not happen even once in our evaluation using the former verfication method.

\subsection{Exception Handling on BCH Decoding}\label{sec:BCH_exception}

There is an additional type of exceptions that arises only from setting the universal error-correction capability $t$. That is, when $\delta_i$ (i.e., the number of distinct elements in group pair $i$) is larger than the error-correction capability $t$, the BCH codewords of group pair $i$ could differ at more than $t$ bit positions (e.g., in the ideal case, the BCH codewords differ at exactly $\delta_i$ bit positions), which exceeds the error-correction capability $t$. If so, the BCH decoder cannot decode the bit errors correctly (\autoref{step:BCH_decode} in \autoref{alg:single_round_pbs}) and report a failure. This exception happens with a small probability in each group pair: For example, when $d=1000$, and $\delta$ is set to $5$ (so that $g=d/\delta=200$), and $t$ is set to $13$ ($2.6$ times of $\delta$), the probability that this exception happens is only $6.7\times 10^{-4}$. 

% The exceptions that happens when the error-correction capability $t$ is sufficient have been discussed and handled in \autoref{subsec:exception_hash_partition} and \autoref{sec:multi-rounds}. In this section, we only discuss the exceptions that are caused by insufficient error-correction capability. That is, when $\delta_i$ (i.e., the number of distinct elements in group pair $i$) is larger than the error-correction capability $t$, the BCH codewords of group pair $i$ differ at $\delta_i$ bit positions in the ideal case, which exceeds the error-correction capability $t$. If so, the BCH decoder cannot decode the bit errors correctly (\autoref{step:BCH_decode} in \autoref{alg:single_round_pbs}) and report a failure. This exception happens with a small probability in each group pair: For example, when $d=1000$, and $\delta$ is set to $5$ (so that $g=d/\delta=200$), and $t$ is set to $13$, the probability that this exception happens is only $6.7\times 10^{-4}$. 

To handle this type of exceptions, we use the same algorithmic trick in \autoref{subsec:protocol2} to further partition each trouble-causing group pair into $3$ sub-group-pairs and reconcile them respectively using PBS-for-small-$d$. 
%Note that $\delta_i$, if is not smaller, should be only slightly larger than $t$ with high probability. Hence, partitioning into $3$ sub-groups is enough to ensure each sub-group has no more than $t$ distinct elements. 
Note that $\delta_i$ is a Binomial random variable with mean of $\delta$, $t$ is $2$ to $3$ times of $\delta$. So the probability that some sub-group contains more than $t$ distinct elements conditioned upon $\delta_i>t$ is tiny. 
In the same example above ($d=1000$, $\delta=5$, $t=13$), this conditional probability is $9.5\times 10^{-10}$.%that some sub-group has more than $t$ distinct elements is $9.5\times 10^{-10}$. 
In the next round, each sub-group-pair will hardly encounter this type of expections and can be reconciled by PBS-for-small-$d$ respectively.  More specifically, we add a termination condition of \autoref{alg:3_way_partition} after \autoref{step:BCH_decode} in \autoref{alg:single_round_pbs}.

\begin{algorithm}
\caption{Termination condition when BCH decoding fails}
\label{alg:3_way_partition}

\If{BCH decoding fails\label{step:if1}}
{Hash-partition the group pair into $3$ sub-group-pairs and run PBS-for-small-$d$ for each of them in the next round; Break;}\label{step:term1} 

\end{algorithm}

% Back to the \autoref{proto:multirounds}, which shows the set reconciliation operations in each round of PBS-basic, this kind of exceptions only affect \autoref{step:reconcile} in \autoref{proto:multirounds}. Now this step needs to check whether BCH decoding is successful or not: If successful, all the operations remain the same; Else, we hash-partition the group ($A$ and $B$) into $3$ sub-groups and reconcile them respectively using \autoref{proto:multirounds}. 
% {\bf I'm not sure if it is necessary to discuss this case, since PinSketch did not mention it, even it may happen in PinSketch}
% Another type of exceptions that happens when $d_i>t$ is, the BCH decoder mistakes the decoding is successful and returns $t$ incorrectly decoded bit errors (i.e., subset pairs). The probability of this type of exceptions is very small. For instance, when $d=1000, \delta=5, t=13$ $(2.5\delta)$, $d_i>t$ happens with probability roughly $6.7\times 10^{-5}$, and the probability that the BCH decoder mistakes the decoding is successful when $d_i>t$ is on the order of $10^{-7}$ \cite{kim1996undetected}. So the probability that this type of exceptions happens in each group is on the order of $10^{-12}$. On the other hand, the impact of this type of exceptions is insignificant. Assume an incorrectly decoded bit error corresponds to a random subset pair, which could contain (1) no distinct element; (2) exactly $1$ distinct element; or (3) more than $1$ distinct elements. Reconcile the subset pair using \autoref{alg:trivial_case} could (1) get nothing and waste $\log |\mathcal{U}|$ bits of communication overhead; (2) get an actual distinct elements; or (3) trigger the exceptions that were discussed and handled in \autoref{subsec:exception_hash_partition}. 

\subsection{What if PinSketch also uses partitions?}

Arguably, the same algorithmic trick (i.e., hash-partition two sets each into groups) can also be implemented in PinSketch~\cite{Dodis_PinSketch_2008} to reduce it computational complexity from $O(d^2)$ (of finite field operations in GF($2^{32}$)) to $O(d)$. However, it will encounter the same randomness problem and have to set up a ``safety margin'' on the error-correction capability $t$. This ``safety margin'' will incur much more additional communication overhead on PinSketch than on our scheme: Considering the average communication overhead per group pair, the additional overhead caused by the ``safety margin'' is $(t-\delta)\log n$ in PBS and $(t-\delta)\log |\mathcal{U}|$ in PinSketch. The latter is roughly $4$ times of the former under the default setting ($n=255, |\mathcal{U}|=2^{32}$). Recall that the theoretical minimum amount of communication overhead to reconcile $\delta$ distinct elements is $\delta\log |\mathcal{U}|$. Use the same example in \autoref{sec:intro}, when $\delta=5, n=255, |\mathcal{U}|=2^{32}, t=2.5\delta$, the overhead of PinSketch using the algorithmic trick is $2.5$ times of the theoretical minimum, while that of PBS is $2.075$ times of the theoretical minimum. It means PBS could have a lower communication overhead than PinSketch if they both use the algorithmic trick. Furthermore, as the signiture length $\log |\mathcal{U}|$ increases, the advantage of PBS over PinSketch will be more significant.

% We handle this type of exceptions by the same method (i.e., hash-partition into $3$ sub-groups) as above. To detect them, on the other hand, is simple: Note that incorrect decoded bit errors correspond to the subset pairs that do not contain distinct elements. When we reconcile those subset pairs in \autoref{sec:reconcile_by_trivial}, the output (i.e., reconciled elements) will be $\mathbf{0}$, which is abnormal (since $\mathbf{0}\notin A\bigcup B$, as we described in \autoref{subsec:protocol0}). Hence, this type of exceptions happen if and only if one of the reconciled distinct elements is $\mathbf{0}$. 
%Hence, we consider BCH decoding is successful by two criteria: (1) the BCH decoder reports a successful decode; and (2) None of the reconciled elements is $\mathbf{0}$. 
% ========================
% In fact, even if $d_i>t$, PBS-basic is still possible to reconcile group $i$ in some nonideal cases. For example, when $t=10$ and $d_i=11$, if the $11$ distinct elements are distributed in $10$ subset pairs, such that $1$ subset pair contains $2$ distinct elements and $9$ subset pairs contain $1$ distinct element in each, the two parity bitmaps differ at only $9$ bit positions. So BCH decoder is able to decode the later $9$ subset pairs and the corresponding $9$ distinct elements can be reconciled. In the second round, only $2$ distinct elements remain and BCH decoding certainly works. In this case, we do not need to partition the group into sub-groups, and this case does not trigger \autoref{alg:3_way_partition} in PBS. 
% ========================
% Instead, it will either (1) report a failure about exceeding the error-correction capability; or (2) mistake the decoding is successful and return incorrect decoded bit errors. 

% The second case happens with a very small probability (in order of $10^{-7}$ \cite{kim1996undetected}) and is very simple to detect : 

% The first case is easy to handle: We can simply adapt the same algorithmic trick to partition the group into smaller groups and reconcile them respectively. In our scheme, we set the number of smaller groups to be $3$, which is big enough because $d_i$, if not smaller, only slightly larger than $t$ with high probability. The second case on the other hand, although theoretically possible, happens with a very small probability when $d_i>t$ (in order of $10^{-7}$ \cite{kim1996undetected}). Besides, the probability of $d_i>t$ is also very small (e.g., when $t=15$ and $\delta=5$, this probability is about $2.3\times 10^{-4}$), so the overall probability of the second case, which is the multiplication of these two small numbers, is negligible (e.g., in order of $10^{-11}$).

% \subsection{Multi-rounds}

% Even if the ideal case does not happen, most of the distinct elements should be distributed into different subset pairs and therefore can be reconciled. So our scheme, even cannot reconcile all of the distinct elements, can still reconcile the majority of them (piecewise decodability). To reconcile the rest distinct elements, we can just run our scheme for multi-rounds under different hash-partition functions. For each round, our scheme works as follows: 

% \IncMargin{1em}
% \begin{algorithm}
% \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
% \Input{Two sets $A$ and $B$}
% \Input{Size of set difference $d$}
% \Input{The number of subset pairs $n$}
% \Input{BCH error-correction capability $t$}

% Hash-partition $A$ and $B$ into $n$ subset pairs $\{(A_i,B_i)\}_{i=1}^n$;

% \If{BCH decoding fails}
% 	Hash-partition $A$ and $B$ into $3$ subset pairs and reconcile them respectively in the next round\;
% \ElseIf{BCH decoding success}
	
% \Else{}

% $k \leftarrow \lceil \frac{t}{c}\rceil $\;

% Partition elements into $k$ subsets using~\autoref{alg:random-part}\;

% \For{$j = 0$ \KwTo $k-1$}{
%     Reconcile the $j$-th subset pair using the straw-man scheme with the BCH correcting capability $\tau$, number of smaller subsets $m$, and number of rounds $r$\;
% }

% \caption{PBS (per round)} \label{proto:II}
% \end{algorithm}\DecMargin{1em}

% This {\bf multi-rounds} scheme can significantly increase the success probability (i.e., the probability that all distinct elements are reconciled). Readers may wonder in the later rounds, most distinct elements should be reconciled, and the remaining could be reconciled using degraded parameters (i.e., smaller $n$ and $t$). In fact, degrade parameters in later rounds cannot save much communication overhead, since the majority of it is spent in the first round (i.e., $>90\%$). Therefore, we use the same parameters (i.e., $n,t$) among all rounds in our evaluation. 
% %The tradeoff between the number of rounds and the communication overhead per rounds will be elaborated in \autoref{sec:tail_bound}. In our evaluation, $r=2,3$ rounds are enough to achieve an extremely high success probability. 

% Readers may think the cost (i.e., communication overhead and the computational complexity) of this multi-rounds scheme is proportional to the number of rounds (denoted as $r$) and increases linearly with $r$. In fact, the cost of each round is roughly proportional to the number of remaining distinct elements, which decreases exponentially as $r$ increases (i.e., the first round reconciles $99\%$ of distinct elements, the second round reconciles $99\%$ of the remaining $1\%$ distinct elements, etc.). So the cost of this multi-rounds scheme is only slightly larger than that of the single-round scheme. Furthermore, as we explained in \autoref{sec:intro}, {\bf from intro thanks for the piecewise decodability of our solution, in almost all practical application scenarios, this tradeoff does not lead to longer response time because the reconciliation of objects identified by the successfully decodable codewords, which constitute the vast majority of all codewords, can run in parallel with the transmissions and decodings of the rest.  In other words, the piecewise decodability effective masks the slightly larger number of communication rounds as far as the response time is concerned.} 





\begin{comment}
\subsubsection{Random Partition}

\IncMargin{1em}
\begin{algorithm}
% \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
% \Input{Set $S$}
% \Input{The number of subsets $m$ for partition}
% \Output{Subsets $S_1, S_2, ..., S_m$}

% Generate hash function $h(\cdot)$ that maps each element into $\{1,2,...,m\}$;

\ForEach{$s \in S$}{
    $j \leftarrow h(s) \bmod m$\;    
    Insert $s$ into the $j$-th subset $S_j$\;
}

\caption{Partition using hash function $h(\cdot)$.} \label{alg:random-part}
\end{algorithm}\DecMargin{1em}

Like the strawman scheme, our scheme randomly partitions sets $A$ and $B$ into $m$ subsets. This random partition 
can be easily accomplished by using some hash function, $h(\cdot)$, and inserting each element $x$ into the subset 
corresponding to $h(x)$. \autoref{alg:random-part} presents the pseudo-code of this random partition using hash 
function $h(\cdot)$.  

% Unlike the strawman scheme, our scheme only reconciles those subset pairs that need to be reconciled, 
% because 



Like the strawman scheme, our scheme hash-partitions the two sets $A$ and $B$ into $m$ subset pairs $(A_i, B_i)$ for $i=1,2,\cdots,m$. 
We note that, among those $m$ bins (subset pairs), 
at most $t$ ($t\!\ll\!m$ as shown in our analysis in~\autoref{subsec:protocol1}) bins contain balls 
(elements belonging to the set difference), {\it i.e.,} requiring reconciliation.  
Motivated by this observation, we, therefore, propose to first detect those bins that 
contain balls and then only reconcile them. The detection is solved with a simple encoding approach that 
will be detailed in the next section.

\subsubsection{Detection before Reconciliation} 

In fact, identifying those non-empty bins is easy when each bin contains at most one ball. In this section, we assume that 
each bin after the random partition contains at most one ball, we will show later how to handle the cases when some 
bins contain more than one balls later in~\autoref{subsec:exceptions}. 

Given an arbitrary bin (say subset pair $(A_i, B_i)$) that contains one ball ({\it i.e.,} $A_i\Delta B_i$ contains exactly one element), 
the corresponding two subsets $A_i$ and $B_i$ differ exactly one element, which implies that 
$||A_i|\!-\!|B_i||\!=\!1$. Hence, if $|A_i|$ ({\it i.e.,} number of 
elements in $A_i$) is odd (or even), then $|B_i|$ must be even (or odd). In other words, the odevity of $|A_i|$ 
and $|B_i|$ are opposite. %differs if $|A_i\Delta B_i|\!=\!1$. 
Based on this property, we propose the {\it odevity encoding}: 
A subset is encoded as ``1'' if it contains odd number of elements, and as ``0'' otherwise. 
Using this odevity encoding, the $m$ subsets of $A$ can be encoded as a bit string $b_A$ in $\{0,1\}^m$, 
where the $i$-th bit in $b_A$ corresponds to the odevity encoding of $|A_i|$. Similarly, the $m$ subsets of $B$ can also 
be encoded as a bit string $b_B$. Clearly, $b_A$ and $b_B$ differ at $t$ different positions, or in other words, 
the Hamming distance of bit strings $b_A$ and $b_B$ is $t$. A straightforward approach is 
to let Alice send $b_A$ to Bob, and then Bob compares $b_B$ against $b_A$ to obtain those non-empty bins. 

This approach, however, has a communication overhead of $m$ bits, which is still unnecessarily high. As 
analyzed in~\autoref{subsec:protocol0}, $t$ is usually much smaller than $m$. 
That means $b_A$ and $b_B$ differ only at a tiny portion of bits. %have much more in common than differences. 
Therefore, if we view $b_B$ as a corrupted message of $b_A$ with $t$ corrupted bits, the detection of those $t$ bins can be converted to 
the detection of the positions of the $t$ corrupted bits. The latter can be solved using an Error-Correction Code (ECC)~\cite{Lin_ErrorControlCoding_1983} that can correct up to $t$ errors. In this work, we use the BCH code~\cite{Lint_IntroductionCodingTheory_1998}. 
More precisely, this ECC-based approach (with the BCH code) works as follows. 
Alice computes the parity bits for $b_A$ using a $t$-error-correcting BCH code with a block length of 
$(2^{\lceil \log m\rceil} -1)$ and sends the parity bits to Bob. Bob then decodes the positions of the $t$ corrupted bits 
using the BCH decoding algorithm with $b_B$ and those parity bits received from Alice. The communication overhead of 
this approach is roughly $t\lceil \log m\rceil$ ($=O(t\log t)$) bits. In the example above, this communication overhead is 
roughly $\num{17000}$ bits, which is approximately $6$ times lower 
than $m\!=\!\num{108469}$ bits, the communication overhead of the aforementioned straightforward approach. 

At first sight, it seems that the detection of non-empty bins and reconciliation of subsets in those bins require two rounds 
(or at least two round trip delays), {\it i.e.,} one round for detection and the other for reconciliation. In fact, 
it only requires one. After Bob receives the parity bits from Alice and decodes out those non-empty bins, it initiates 
the reconciliation ({\it i.e.,} \autoref{alg:trivial_case}) for each bin (subset pair) immediately, 
{\it i.e.,} sends the \code{XOR} sums of subsets in those bins together the indexes of those bins. 
After receiving those \code{XOR} sums and bin indexes, Alice can compute the set difference. 

% A naive way to combine the detection of non-empty bins and reconciliation of subset pairs in those bins is to first detect 
% those non-empty bins via one round of message exchanges between Alice and Bob and then to reconcile the corresponding 
% subset pairs in those bins with another round of message exchanges. This requires two rounds ({\it i.e.,} taking at least 
% two round trip delays). In fact, after Bob receives the parity bits from Alice and obtains those 

\subsubsection{Multiple Rounds}\label{sec:multiround}

{\bf This section was not clear enough. I need more time to think about and revise it.}


In the above section, we have assumed that each bin contains at most one ball. 
However, even with a sufficient large $m$, some bin might contain more than one balls though with tiny probability. 
We will show in~\autoref{subsec:exceptions}, how such rare events, {\it i.e.,} one bin contains more than one balls, 
can be easily detected.
To ensure our scheme can successfully reconcile all elements even when such rare events happen, 
we propose to use multiple rounds (of communication between Alice and Bob). More precisely, instead of 
selecting a prohibitively large $m$ to ensure that each bin contains at most one ball with a extremely high probability 
(say 0.99999), we select a reasonably large $m$ so that the communication overhead is not very high and very few bins contain 
more than one balls (or in other words, most bins contain at most one ball). Therefore, after running one round of 
our scheme, most elements in the set difference will be reconciled. Only those in the bins that contain more than one balls 
fail to be reconciled. For elements in the subsets corresponding to those bins, we run another round of our scheme. 
If some elements still fail to be reconcile, we can run one more round of our scheme. So on so forth,  
our scheme can keep running for more rounds until all elements are reconciled. 

With the same communication overhead, multiple rounds can significantly increase the success rate, 
{\it i.e.,} the probability that all elements in the set difference will be successfully reconciles, 
which will be elaborated in~\autoref{sec:tail_bound}. 

% % to be emphasized
% % say that too many rounds should be avoided (latency & communication overhead reduction is negligible when r is too large, 2 - 3 is good enough)
% % multiple rounds is not an issue when r is small

% We note that the number of rounds $r$, however, should not be large. On one hand, it results in large latency (at least $r$ round trip delays). 
% On the other hand, when $r$ is large, the reduction of communication overhead by the increase of $r$ gradually diminishes. 

We note that multiple rounds, when $r$ is small, would not really increase the ``latency'', as long as most elements in the 
set difference can be reconciled in the first rounds, since the underlying synchronization of data objects corresponding to 
those elements can start immediately after the first round of our scheme. Therefore, the actual latency is one round trip delay instead of 
$r$. 

As we mentioned, this straw-man protocol works correctly if each subset pair has at most one exclusive element (i.e., \autoref{eq:requirement_strawman} holds). On the other hand, if a subset pair has more than one exclusive elements, some of which will not be successfully reconciled:

\begin{itemize}
\item If a subset pair has even number of exclusive elements, Odevity coding will encode it as 0. Then the straw-man scheme will consider the subset pair having no exclusive element and all exclusive elements in this subset will not be reconciled;

\item If a subset pair has odd number ($\geq 3$) of exclusive elements, Odevity coding will encode it as 1 and consider the subset pair having only 1 exclusive element. Then the straw-man scheme will use \autoref{alg:trivial_case} to decode only one exclusive element and dismiss all others. Even worse, the only decoded element is probably not a real exclusive element, since the element computed by \autoref{alg:trivial_case} is the \code{XOR} sum of all exclusive elements, not one of them. 
\end{itemize}

In summary, if a subset pair has more than one exclusive elements, most of its exclusive elements cannot be reconciled, and the reconciled element is usually incorrect (i.e., false-positive). The false-positive however is easy to check, which will be elaborated in \autoref{subsec:exceptions}. The good thing is, even if not all subset pairs have at most one exclusive element and are successfully decoded, most of them will be w.h.p.. In other words, even if the straw-man protocol cannot reconcile all exclusive elements, it still can reconcile most of them. To reconcile all exclusive elements w.h.p., we can simply extend the single-round straw-man scheme to multi-round. And each round adapts the straw-man scheme to do set reconciliation using independent hashing functions $h(\cdot)$ for partition (i.e., in \autoref{alg:random-part}). This multi-round extension can significantly increase the probability of a successful reconciliation, which will be elaborated in \autoref{sec:tail_bound}. 



\subsection{Our Scheme: The Final Version}\label{subsec:protocol2}

{\bf Under revision~}

The preliminary version of our scheme suffers from two major drawbacks. 
First, its communication overhead is asymptotically 
$O(t\log m)\!=\!O(t\log t)$, which is not asymptotically optimal. 
Second, the decoding computational complexity is proportional to 
$t^2$ with the state-of-the-art decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} for BCH codes, 
which is too high when $t$ is large. 
To overcome these two drawbacks, we use a simple algorithmic trick: divide and conquer. With this algorithmic 
trick, the decoding computational complexity is reduced to $O(t)$, 
and the communication overhead is reduced to $t\cdot\frac{\log u}{8} \!+\! O(t)$ (with a small 
hidden constant roughly varying from 4 to 8) bytes which implies that 
our scheme has an additive communication overhead (compared to the optimal scheme) 
of 4 to 8 bytes per element in the 
set difference and this additive overhead is independent of the key size ({\it i.e.}, $\log u$). 
Recall that the IBF-based schemes usually have a communication overhead of roughly 6 times of the 
optimal scheme, which increases linearly as the key size. Therefore, our scheme is much more 
communication-efficient. 

Now, we describe in detail this algorithmic trick. We let Alice divide elements in $A$ into $\lceil\frac{t}{c}\rceil$ groups (subsets)  
for some small constant $c$ (say $5$) so that each group contains roughly $c$ elements from the set difference on average. We let Bob do the same operations on $B$. To ensure that any common element ({\it i.e.,} any element $x\!\in\! A\bigcup B$) goes into 
the same group ({\it i.e.,} groups at Alice and Bob with the same index), we can use the partition procedure with a hash function shown 
in~\autoref{alg:random-part}. Then, we can apply the preliminary version on each group with a constant $m$ (say $m\!=\!256$) independent of 
$t$. To ensure that each group can be reconciled with a high probability, we need to use BCH codes whose decoding capacity 
larger than $c$ (say $\tau\!=\!2c$), as exact number of elements to be reconciled could be larger than $c$. 
Since this decoding capacity $\tau$ is still a small constant independent of $t$, therefore, the communication 
overhead per group is $\tau\cdot\log m \!=\!O(1)$, which implies a total communication overhead of $O(t)$. 
Similarly, the total decoding computational complexity is also $O(t)$. 

\subsubsection{Parameter Configurations} 

Our scheme now has several parameters: $c$ (average number of elements from the set difference in each group), 
$\tau$ (the correcting capability of the BCH code), $m$ (number of bins for each group), and $r$ (maximum number of rounds). 
We note that the maximum number of rounds $r$ is usually associated with another parameter $p$ the desired success rate: With 
at most $r$ rounds, our scheme should guarantee that the success rate is at least $p$. 
%How to tune these parameters to achieve favorable performance will be detailed later in~\autoref{sec:tail_bound}. 
Here, we provide some guidances for the parameter configurations using our theoretical analysis, which gives the tail bound of 
the success probability of our scheme and will be shown in~\autoref{sec:tail_bound}. 

\noindent
{\bf Parameterizing $c$ and $r$.} The values of $c$ and $r$ are usually provided by users based on the requirements of 
applications. For the value of $c$, a larger $c$ results in a longer decoding time yet lower communication overhead.  
So if the decoding time is a big concern, then a smaller $c$ (say $c=5$) should be used; otherwise, a larger $c$ could be used. 
For the values of $r$, a larger $r$ leads to lower communication overhead and usually lower decoding time (as it allows to use 
a smaller $\tau$), however, the reduction is marginal when $r>3$. Therefore, we suggest users to configure $r$ to be $2$ or $3$. 
% The configuration of $c$ is relatively straightforward, as a larger $c$ will result in 
% a longer decoding time and a slightly lower communication overhead. The former is ..., The latter is slightly tricky. 


\noindent
{\bf Using $c$ and $r$ to parameterize other parameters.} After users specify the values for $c$ and $r$ (associated with a value for 
$p$), we can use our theoretical analysis in~\autoref{sec:tail_bound} to parameterize $\tau$ and $m$. 
Since in a BCH code, the block length is in the form of $2^q-1$, we only need to consider $m=2^q-1$. 

{\bf Liang, please revise the following algorithm!}

\begin{algorithm}
\SetKwProg{Proc}{}{}{end}
\SetKwFunction{algo}{\small Search}

\Proc{Search($c$, $r$, $p$)}{\label{search:entrance}

$\mbox{co}_{best}\leftarrow\infty$\tcc*{\small Best communication overhead}

\For{$\tau \leftarrow c\,\KwTo\, \infty$}{}



}
\end{algorithm}


% , unlike 
% the IBF-based schemes which have an multiplicative overhead of 6 
% The inspiration is from the famous 
% divide and conquer algorithm for the selection problem, in which, given an array with $n$ elements, we want to get the $k$-th largest 
% element. A straightforward idea for this problem is sorting. However, if using insertion-sorting, the complexity would be $O(n^2)$. 
% Then the famous divide and conquer trick comes. It first divides the array into $\lceil n/5\rceil$ groups so that the first 
% $\lfloor n/5\rfloor$ contains $5$ elements and at most one group contains the rest $n \mod 5$ elements, and find the median of each 
% group using the insertion-sorting and th


% This straw-man scheme still has a problem on decoding computational complexity. More specific, the complexity increases dramatically with the total number of corrupted bits $t$. Therefore, when $t$ is moderate or large, the decoding computational complexity could be very high. For instance, the decoding complexity of BCH codes~\cite{Lint_IntroductionCodingTheory_1998} is $O(t^3)$, which could be quite high for a large $t$. To keep the decoding complexity reasonably low, we design the following two-layer protocol: In the first layer, we use a hash function to partition the two sets into $\lceil\frac{t}{c}\rceil$ subsets for some small constant $c$ (say $5$), just like the first step of our straw-man scheme. The objective, which is however different from before, is to make each subset pair contains roughly $c$ exclusive elements on average. In the second layer, we use the straw-man scheme with the same configuration (number of subsets $m$, and error-correction capability $\tau$, number of rounds $r$) to reconcile each subset pair. 

% In fact, the straw-man scheme is a proper solution when $t$ is small. First, the decoding complexity will not be a problem for a small $t$; Second, we do not need an extremely large $m$ to guarantee \autoref{eq:requirement_strawman} w.h.p.. For instance, when $t=5$ and $m=1024$, \autoref{eq:requirement_strawman} holds with probability $\frac{m\,!}{(m-t)\,!m^t}\approx 99\%$. This motivates us to design the following two-layer protocol: In the first layer, we use a hash function to partition the two sets into $\lceil\frac{t}{c}\rceil$ subsets for some small constant $c$ (say $5$), just like the first step of our straw-man scheme. The objective, which is however different from before, is to make each subset pair contains roughly $c$ exclusive elements on average. In the second layer, we use the straw-man scheme with the same configuration (number of subsets $m$, and error-correction capability $\tau$) to reconcile each subset pair. 

\autoref{proto:II} shows the pseudocode of our scheme. It first uses the same hash-function based random partition algorithm as \autoref{alg:random-part} to partition elements into $k\triangleq\lceil \frac{t}{c} \rceil$ subsets. Note that the random partition only guarantees that each such subset 
contains $c$ exclusive elements on average, and the exact number is not known. Hence, our scheme uses a BCH code with a capability of 
correcting up to $\tau$ errors with $\tau > c$ to make sure that the BCH code has a high probability to decode successfully. We will describe how to deal with situation where the size of set difference exceeds $\tau$ later in~\autoref{subsec:exceptions}.

As the decoding of a $\tau$-error-correcting BCH code where $\tau$ is a small constant has a constant-time computational complexity, the decoding complexity of 
our scheme is $O(k)=O(t)$. We now have several parameters, average number of exclusive elements in each subset $c$, the correcting capability $\tau$ of BCH code, the number of smaller subsets $m$ for each subset to be divided to, and the number of rounds $r$. How to tune these parameters to achieve favorable performance will be detailed later in~\autoref{sec:tail_bound}. 

\IncMargin{1em}
\begin{algorithm}
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
\Input{Size of set difference $t$}
\Input{The number of subsets $m$ for each partition}
\Input{Average number of exclusive elements in each partition $c$}
\Input{BCH code capability $\tau$}

$k \leftarrow \lceil \frac{t}{c}\rceil $\;

Partition elements into $k$ subsets using~\autoref{alg:random-part}\;

\For{$j = 0$ \KwTo $k-1$}{
    Reconcile the $j$-th subset pair using the straw-man scheme with the BCH correcting capability $\tau$, number of smaller subsets $m$, and number of rounds $r$\;
}

\caption{Our Scheme} \label{proto:II}
\end{algorithm}\DecMargin{1em}




\subsection{Exceptional Handling}\label{subsec:exceptions}

{\bf To be revised~}

In this section, we will elaborate how to handle the following two types of exceptions that we mentioned in \autoref{sec:multiround} and \autoref{subsec:protocol2}:
\begin{itemize}
    \item Exception 1: A subset pair has odd number ($\geq 3$) of exclusive elements and causes false-positives (i.e., a decoded distinct element is not a real one);
    \item Exception 2: A subset pair contains too many exclusive elements, such that a BCH code with capability of correcting up to $\tau$ errors cannot decode it (i.e., $t>\tau$).
	\item Exception 3: A subset pair has even number ($\geq 2$) of exclusive elements and causes false-negatives(i.e., two or more distinct elements are neglected as the parity bit is 0);
\end{itemize}

To handle Exception 1, we need to check whether a computed exclusive element by \autoref{alg:trivial_case} is a real exclusive element or not. (The group index happens to come in handy if we use it as a fingerprint of the element we computed. If this element is truly an exclusive element, it should be hashed into the same group as before. Notably, We have two group indices available for this check, one is in the initial divide and conquer phase, the other is in the BCH code part) It can be easily done at the end of set reconciliation, during which two hosts exchange their exclusive elements. In fact, as we will elaborate in \autoref{sec:tail_bound}, Exception 1 hardly happens if we set parameters properly. 

On the other hand, when Exception 2 happens, the BCH decoder will report a failure about exceeding the error-correction capability. For such a subset pair, we can use the same approach as in \autoref{subsec:protocol2} to partition it into smaller subsets and use the straw-man scheme to reconcile them respectively. We set the number of small subsets to be 3. It is because, as we will elaborate in \autoref{sec:tail_bound}, the number of exclusive elements for each subset pair $t$ should be, if not smaller, only slightly larger than $\tau$ w.h.p.. Partitioning those exclusive elements into 3 small subsets is enough to guarentee that each of them has less than $\tau$ exclusive elements.

\end{comment}

==> section/schemes_new0227.tex <==
%\section{PBS for small \texorpdfstring{$d$}{d}}\label{sec:scheme}
\section[PBS for small \texorpdfstring{$d$}{d}]{PBS for small \texorpdfstring{\larger\boldmath\MakeLowercase{$d$}}{d}}\label{sec:scheme}
%\section{Set Reconciliation}\label{sec:scheme}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%     Writing Guideline for This Section     %%%%%%%%%%
% “balls – elements in the symmetric difference of the two sets” 

% Protocol 0 (reconcile two sets whose set difference has at most one ball)

% Protocol I.I (partition elements into a sufficiently large number of subsets such that each subset has at most one ball with high probability and use Protocol 0 to reconcile each of them) 

% Protocol I.II (a two-step refinement of Protocol I.I: first use BCH to identify good bins, i.e., bins/subsets have exactly one ball, and then use Protocol 0 to reconcile each good bin) 

% Protocol II (a two-layer refinement of Protocol I.II: in the first layer, we partition elements into t/c subsets, where t is the size of set difference and c is a small constant, then each subset has c balls on average. In the second layer, we further partition each subset into large enough number of bins/subsets such that with high probability each bin has at most one ball, then use Protocol I.II to reconcile them one by one) 

% Protocol III/IV (mainly fix certain exceptions in Protocol II，e.g., how to address bad bins, how to handle the cases where BCH fails to decode and etc)

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% In this section, we describe our set reconciliation scheme in details. First, we give a formal problem statement in \autoref{sec:model}. In \autoref{subsec:protocol0}, we introduce a basic scheme for the trivial case, in which the two sets $A$ and $B$ has at most one distinct element. Building upon the basic scheme, we propose the preliminary version of scheme in \autoref{sucsec:our-scheme} that targets to the cases where the total number of distinct elements $d$ is small. Then we extend the preliminary version and propose the final version of our scheme in \autoref{subsec:protocol2} for general cases (i.e., any arbitrary $d$). We assume $d$ is precisely known throughout this section except in \autoref{subsec:ToW}, where we will describe how to estimate $d$ using a Tug-of-War Estimator. 


In this section, we describe how PBS scheme allows Alice and Bob to reconcile their respective sets $A$ and $B$, where $d=|A\Delta B|$ is assumed to be small and precisely known. 
%Throughout this paper, we call each element in $A\Delta B$ a \textit{distinct element}, and each element in $A\bigcap B$ a \textit{common element}. 
We start with the trivial case where $d\leq 1$ in \autoref{subsec:protocol0} and then generalize the scheme for the case where $d$ is a small number in \autoref{sec:pbs_smalld}. 
% We build up our scheme gradually by starting with the trivial case where $d\leq 1$ in \autoref{subsec:protocol0}. Then we generalize our scheme to the case where $d$ is a small number in \autoref{sec:pbs_smalld}. 

\begin{comment}
\subsection{Problem Statement}\label{sec:model}

In this work, we adopt the commonly used model for the set reconciliation problem. 
Two remote sets $A$ and $B$ are stored at hosts Alice and Bob respectively. 
Each element in $A$ and $B$ is a hash signiture in the key space (universe) $\mathcal{U}$, which is the set of all $(\log |\mathcal{U}|)$-bit binary strings. 
%Each element in $A$ and $B$ is a hash signiture with signiture width $w$ in the key space (universe) $\mathcal{U}$, which is the set of all $w$-bit binary strings (i.e., $|\mathcal{U}|=2^w$). 
%We use $\mathcal{U}$ to denote the set of all $w$-bit binary strings and name it the universe of signitures. 
The set reconciliation problem is to compute the symmetric set difference between $A$ and $B$, 
{\it i.e.,} $A\Delta B\triangleq (A\!\setminus\! B) \bigcup (B\!\setminus\! A)$. 
Let $d\!=\!|A\Delta B|$ be the cardinality of this difference.
%We denote $d\!=\!|A\Delta B|$. 
Throughout this paper, we call each element in $A\Delta B$ a \textit{distinct element}, and each element in $A\bigcap B$ a \textit{common element}.
{\bf Like in all existing solutions, we describe only {\it unidirectional} set reconciliation, in which Alice or Bob learns the set difference $A\Delta B$. Since the performance of our scheme does not depend on who learns the set difference, we assume Bob learns the set difference $A\Delta B$ in the rest of the paper, as mentioned in \autoref{sec:psea}.}
% As mentioned in \autoref{sec:psea}, we describe {\it unidirectional} set reconciliation that Bob learns the set difference $A\Delta B$. 
%In \autoref{sec:evaluation}, we use the same semantic to measure the communication cost of our scheme and other compared set reconciliation schemes. 
\end{comment}

% In the rest of this section, we build up our scheme gradually as follows: We start with the trivial case where $d\leq 1$ in \autoref{subsec:protocol0}. Then we generalize our scheme to the case where $d$ is a small number in \autoref{sec:pbs_smalld}. 

%After that, we further generalize our scheme to the case that $d$ is a large number in \autoref{subsec:protocol2}. 
%Throughout this section, we assume $d$ is precisely known.
%except in \autoref{subsec:ToW}, where we will describe how to estimate $d$ using a Tug-of-War Estimator. 

%The rest of this section is organized as follows: In \autoref{subsec:protocol0}, we introduce a basic scheme for the trivial case, in which the two sets $A$ and $B$ has at most one distinct element. In \autoref{sucsec:our-scheme} and \autoref{subsec:protocol2}, we elaborate the two versions of our solution that are introduced in \autoref{sec:smalld} and \autoref{sec:larged} respectively. Throughout this section, we assume $d$ is precisely known except in \autoref{subsec:ToW}, where we will describe how to estimate $d$ using a Tug-of-War Estimator. 

\subsection{The Trivial Case of \texorpdfstring{\larger\boldmath $d\leqslant 1$}{d<2}}\label{subsec:protocol0}

%We start with the trivial case, in which $A$ and $B$ have at most one distinct element ({\it i.e.,} $d\leq 1$), we have a simple set reconciliation scheme showed in \autoref{alg:trivial_case}:
\begin{algorithm}
\caption{Set reconciliation when $d\le 1$}
\label{alg:trivial_case}

{\it Bob}: $s_B\leftarrow\underset{b\in B}{\oplus} b$; Send $s_B$ to Alice\; \label{alg1:sender}

{\it Alice}: $s_A\leftarrow\underset{a\in A}{\oplus} a$; $s\leftarrow s_A \oplus s_B$\; \label{alg1:receiver}
\end{algorithm}

\autoref{alg:trivial_case} shows our set reconciliation scheme for the trivial case, in which $A$ and $B$ differ by at most one (distinct) element. It consists of two steps. First, Bob calculates $s_B$, the bitwise-\code{XOR} of all elements in $B$, and send it to Alice. 
Second, Alice calculates $s_A$, the bitwise-\code{XOR} of all elements in $A$.  Upon receiving $s_B$ from Bob, Alice computes $s\!\triangleq\! s_A \!\oplus\! s_B$. 
The value of $s$ tells Alice which of the following two cases happens.
%Depending on whether $A$ and $B$ have a distinct element, there are  two possibilities:

\begin{sitemize}
	\item Case (\RN{1}): If $s=\mathbf{0}$, which implies $s_A=s_B$, Alice concludes that that $A$ and $B$ have no distinct element or $A=B$. 
	Here $mathbf{0}$ denotes the $\log |\mathcal{U}|$-bit-long all-$0$ string;
	\item Case (\RN{2}): If $s\not=\mathbf{0}$, which implies $s_A\not=s_B$, Alice concludes that $A$ and $B$ have exactly one distinct element which is $s$, i.e., 
	$A\Delta B=\{s\}$.  This is because bitwise-\code{XOR}ing $s_A$ and $s_B$ (to obtain $s$) cancels out all (common) elements in $A\bigcap B$.   
%	Here {\it common elements} are defined as the 
%	Here an element that is contained in both sets is called a common element  
	%And $s$ is the missing element of $A$ (i.e., $s\in B\!\setminus\! A$) if $s\in B$, or the missing element of $B$ (i.e., $s\in A\!\setminus\! B$) otherwise;
	% \item If $A$ and $B$ has more than one distinct elements (i.e., $d>1$), the bitwise \code{XOR} of $s_A$ and $s_B$ will still cancel out all common elements and remain the \code{XOR} of the distinct elements, i.e., $s$ is the \code{XOR} of all distinct elements;
\end{sitemize}

Like in most of the literature on set reconciliation, we assume that the all-$0$ element 
$\mathbf{0}$ is excluded from the universe  $\mathcal{U}$, since otherwise \autoref{alg:trivial_case} does not work 
%when $\mathbf{0}\!\in\! A\bigcup B$ %$\mathbf{0}\in A\bigcap B$ 
for the following reason:  When $s=\mathbf{0}$, Alice cannot tell whether $A$ and $B$ are identical, or they have $\mathbf{0}$ as their distinct element. 
%However, we can extend our scheme to support $\mathbf{0}$. For example, we let Alice send to Bob a single bit to indicate whether Alice has element $\mathbf{0}$, so Bob will know whether $\mathbf{0}\in A\Delta B$ or not. 

\autoref{alg:trivial_case} also does not work when there are more than one distinct elements in $A\Delta B$ (i.e., $d>1$), since the computed $s$ in this case 
is the \code{XOR} of all these distinct elements.

% Note that \autoref{alg:trivial_case} works if and only if $|A\Delta B|\!\leq\! 1$ and $0\!\notin\! (A\!\cup\! B)$ (which we have explained in~\autoref{sec:model}). 

%\subsection{PBS: When $d$ is small}\label{sucsec:our-scheme}

%In this section, we generalize PBS to the case when $d$ is a small number, as we described in \autoref{sec:smalld}. 
%First, we describe each step of single-round PBS from \autoref{sec:hash_partition} to \autoref{sec:reconcile_by_trivial} and summarize it in \autoref{sec:single_round_pbs}. Second, we discuss the exceptions in single-round PBS in \autoref{subsec:exception_hash_partition}. Third, we propose multi-round PBS to handle the exceptions.

\subsection{The General Case}\label{sec:pbs_smalld}
%\subsection{PBS for small \texorpdfstring{\larger\boldmath $d$}{d}}\label{sec:pbs_smalld}

In this section, we describe the scheme for a more general case, where $d$ is 
%no longer limited to be no more than $1$, but 
a small number that is no more than several, but is not necessarily $0$ or $1$.
%In this section, we substantiate the scheme described in \autoref{sec:smalld} for small $d$.

\subsubsection{Hash Partition and Parity Bitmap Encoding}\label{sec:hash_partition}
% \medskip
% \noindent{\bf Hash Partition} 

Here we formalize the aforementioned process of partitioning $A$ into $\{A_i\}_{i=1}^n$, $B$ into $\{B_i\}_{i=1}^n$, and $A\Delta B$ into $\{A_i\Delta B_i\}_{i=1}^n$ 
using a hash function $h(\cdot)$.
%as described in \autoref{sec:smalld} by introducing the concept of {\it sub-universes}. Given a hash function $h(\cdot): \mathcal{U}\rightarrow \{1,2,\cdots,n\}$, we 
Define {\it sub-universe} $\mathcal{U}_i$ as the set of elements in the universe $\mathcal{U}$ that are hashed into value $i$. More precisely, $\mathcal{U}_i\triangleq\{s\!\mid\! s\in \mathcal{U} \mbox{ and } h(s)=i\}$ for $i=1,2,...,n$. Then defining $A_i\triangleq A\bigcap\mathcal{U}_i$ and $B_i\triangleq B\bigcap\mathcal{U}_i$ for $i=1,2,...,n$ induces the partitioning of $A$, $B$, and $A\Delta B$.
%, as mentioned in \autoref{sec:smalld}. 

%{\bf (merged from the later two paragraphs)} 
How the $d$ distinct elements (balls) in $A\Delta B$ are ``scattered" into the $n$ subset-pair-differences $\{A_i\Delta B_i\}_{i=1}^n$ (bins) can be precisely modeled as throwing $d$ balls each uniformly and randomly into one of the $n$ bins. 
For the moment, we assume the following {\it ideal case} happens: Every subset-pair-difference $A_i\Delta B_i$ contains at most one distinct element.  
This ideal case corresponds to the $d$ balls ending up in $d$ distinct bins. It happens with probability $\prod_{k=1}^{d - 1}(1 - \frac{k}{n})$, which is on the order of $1-O(d^2/n)$ when $n\!\gg\!d$.
%approximately $e^{-\frac{d(d-1)}{2n}}$ when $d\!\ll\!n$. 
Hence, $n$ must be $\Omega(d^2)$ to ensure the ideal case happens with a nontrivial probability, as mentioned in \autoref{sec:smalld}. 
%The nonideal case of a subset pair difference containing more than $1$ distinct elements will be discussed in \autoref{subsec:exception_hash_partition}.

% {\bf (Previous)} For the moment, we assume the following {\it ideal case} happens: Every subset-pair-difference $A_i\Delta B_i$ contains at most one distinct element. The nonideal case of a subset pair difference containing more than $1$ distinct elements will be discussed in \autoref{subsec:exception_hash_partition}. 

%In this section, we give a detailed description on how to partition $A$ and $B$ (as introduced in \autoref{sec:smalld}) by introducing {\it sub-universes}, which is defined as follows: Given a hash function $h(\cdot): \mathcal{U}\rightarrow \{1,2,\cdots,n\}$, we define {\it sub-universes} $\{\mathcal{U}_i\}_{i=1}^n$, a partition of the universe $\mathcal{U}$, as $\mathcal{U}_i=\{s\!\mid\! s\in \mathcal{U} \mbox{ and } h(s)=i\}$ for $i=1,2,...,n$. Based on $\{\mathcal{U}_i\}_{i=1}^n$, we define $\{A_i\}_{i=1}^n$, the partition of $A$ introduced in \autoref{sec:smalld}, as $A_i\! \triangleq\! A\bigcap \mathcal{U}_i$ for $i=1,2,...,n$. $\{B_i\}_{i=1}^n$ is similarly defined. By this definition, the set difference $A\Delta B$ is partitioned into $n$ set differences of the partitioned subset pairs (i.e., $\{(A_i, B_i)\}_{i=1}^n$). From \autoref{sec:hash_partition} to \autoref{sec:reconcile_by_trivial}, we assume the following {\bf ideal case} happens: Each subset pair $(A_i, B_i)$ contains at most one distinct element ({\it i.e.,} $|A_i\Delta B_i|\!\leq\!1$). The nonideal case of a subset pair contains more than $1$ distinct elements will be discussed in \autoref{subsec:exception_hash_partition}. 

% Here we describe the hash-partition step introduced in \autoref{sec:smalld} in details. First, we use a hash function $h(\cdot): \mathcal{U}\rightarrow \{1,2,\cdots,n\}$ to partition the universe $\mathcal{U}$ into $n$ sub-universes: $\mathcal{U}_i=\{s\!\mid\! s\in \mathcal{U} \mbox{ and } h(s)=i\}$ for $\forall i=1,2,\cdots,n$. The hash function $h(\cdot)$ can be predetermined between Alice and Bob and does not require additional communication cost. Define $A_i\! \triangleq\! A\bigcap \mathcal{U}_i$ and $B_i\! \triangleq\! B\bigcap \mathcal{U}_i$ for $i=1,2,\cdots,n$. Then $\{A_i\}_{i=1}^n$ and $\{B_i\}_{i=1}^n$ are partitions of $A$ and $B$ respectively. Furthermore, $\{A_i\Delta B_i\}_{i=1}^n$ is a partition of $A\Delta B$. From \autoref{sec:hash_partition} to \autoref{sec:reconcile_by_trivial}, we assume the following {\bf ideal case} happens: Each subset pair $(A_i, B_i)$ contains at most one distinct element ({\it i.e.,} $|A_i\Delta B_i|\!\leq\!1$). The nonideal case of a subset pair contains more than $1$ distinct elements will be discussed in \autoref{subsec:exception_hash_partition}. 

% {\bf (Previous)} How the $d$ distinct elements (balls) in $A\Delta B$ are distributed into the $n$ subset pair differences $\{A_i\Delta B_i\}_{i=1}^n$ (bins) 
% can be viewed as throwing $d$ balls each uniformly and randomly into one of the $n$ bins. 

%follows the familiar {\it balls-into-bins} probability model. 
%The distinct elements are viewed as balls and the subset pairs are viewed as bins. 
%Each of the $d$ balls is uniformly and randomly thrown by the hash function $h(\cdot)$ into one of the $n$ bins. 
% The aforementioned ideal case that corresponds to the $d$ balls ending up in $d$ distinct bins happens with probability $\prod_{k=1}^{d - 1}(1 - \frac{k}{n})$, which is on the order of $1-O(d^2/n)$ when $d\!\ll\!n$.
% %approximately $e^{-\frac{d(d-1)}{2n}}$ when $d\!\ll\!n$. 
% Hence, $n$ must be $\Omega(d^2)$ to ensure the ideal case happens with a nontrivial probability, as mentioned in \autoref{sec:smalld}.


%in which the distinct elements are viewed as balls and the subset pairs are viewed as bins. The hash-parition basically throws (hashes) $d$ balls (distinct elements) uniformly and randomly into $n$ bins (subset pairs). The aforementioned ideal case in this context becomes, after throwing $d$ balls uniformly and randomly into $n$ bins, each bin receives at most $1$ ball (i.e., $d$ nonempty bins have $1$ ball in each and the rest $n-d$ bins are empty). The number of balls in each bin is a Binomial random variable $Binomial(d,1/n)$.
%{\bf It may remind readers about the Birthday problem. And the ideal case can be analogous to the case that no people share the same birthday.} 
% The ideal case happens with a probability of $p\!=\!\prod_{k=1}^{d - 1}(1 - \frac{k}{n})\!\approx\! e^{-\frac{d(d-1)}{2n}}$ when $d\!\ll\!n$. In other words, $n$ must be at least $O(d^2)$ to ensure the ideal case happens with a nontrivial probability, as described in \autoref{sec:smalld}.  

% Note that the ideal case does not always happen. However, we can ensure that the ideal case happens with high probability by properly setting $n$ based on $d$ (i.e., $n=\Omega(d^2)$). Furthermore, as we will describe in \autoref{subsec:nonideal}, even if the ideal case does not happen (i.e., some distinct elements are hashed into the same subset pair), most of the distinct elements should be distributed into different subset pairs and therefore can be reconciled. So the scheme, even cannot reconcile all of the distinct elements, can still reconcile the majority of them (i.e., piecewise decodability in \autoref{sec:intro_oursolution}). Based on this property, we will extend our scheme from single-round to multi-rounds in \autoref{subsec:nonideal} to further increase the probability of reconciling all distinct elements. 

% \medskip
% \noindent{\bf Parity Bitmap Encoding} 

% to let Alice obtain $A\Delta B$.

% {\bf (Modified)} Recall that the partition $\{A_i\}_{i=1}^n$ and $\{B_i\}_{i=1}^n$ can be encoded as $A[1..n]$ and $B[1..n]$ respectively, in which $A[i]$, the $i$-th bit of the parity bitmap $A[1..n]$, is equal to the oddness / evenness (parity) of the cardinality of $A_i$ (i.e., $A[i]=1$ if $|A_i|$ is odd; otherwise $A[i]=0$). $B[i]$, the $i$-th bit of the parity bitmap $B[1..n]$, is similarly defined. In the ideal case, $A[1..n]$ and $B[1..n]$ differ in exactly $d$ distinct bit positions $i_1,i_2,...,i_d$, and each subset-pair-difference $(A_{i_1},B_{i_1}), (A_{i_2},B_{i_2}),...,(A_{i_d},B_{i_d})$ contains exactly $1$ distinct element. If Bob knows $i_1,i_2,...,i_d$, he can start to reconcile the $d$ subset pairs respectively using \autoref{alg:trivial_case}, then Alice will obtain $A\Delta B$.

% {\bf (Modified)} The partition $\{A_i\}_{i=1}^n$ is encoded into an $n$-bit-long parity bitmap $A[1..n]$, in which $A[i]$, the $i$-th bit of the parity bitmap, is equal to the oddness / evenness (parity) of the cardinality of $A_i$ (i.e., $A[i]=1$ if $|A_i|$ is odd; otherwise $A[i]=0$). $B[1..n]$, the parity bitmap of $\{B_i\}_{i=1}^n$, is similarly defined. In the ideal case, $A[1..n]$ and $B[1..n]$ differ in exactly $d$ distinct bit positions $i_1,i_2,...,i_d$, and each subset-pair-difference $(A_{i_1},B_{i_1}), (A_{i_2},B_{i_2}),...,(A_{i_d},B_{i_d})$ contains exactly $1$ distinct element. If Bob knows $i_1,i_2,...,i_d$, he can start to reconcile the $d$ subset pairs respectively using \autoref{alg:trivial_case}, then Alice will obtain $A\Delta B$.

% {\bf (Previous)} We encode $\{A_i\}_{i=1}^n$ into an $n$-bit-long parity bitmap $A[1..n]$, in which $A[i]$, the $i^{th}$ bit of the parity bitmap, is equal to the oddness / evenness (parity) of the cardinality of $A_i$ (i.e., $A[i]=1$ if $|A_i|$ is odd; otherwise $A[i]=0$). In the ideal case, the two bitmaps $A[1..n]$, $B[1..n]$ differ in exactly $d$ bit positions $i_1,i_2,...,i_d$, each of which corresponds to a subset pair that contains $1$ distinct element. The next step is to let Alice and Bob know these bit positions.

%Once the $d$ bit positions are known, Alice and Bob can start to reconcile $(A_{i_1},B_{i_1}), (A_{i_2},B_{i_2}),...,(A_{i_d},B_{i_d})$ using \autoref{alg:trivial_case} and obtain the $d$ distinct elements (i.e., $A\Delta B$). 

% \subsubsection{Parity Bitmap Encoding}\label{sec:parity_bitmap_encoding}

% %After hash-partitioning $A$ and $B$ into partitions $\{A_i\}_{i=1}^n$ and $\{B_i\}_{i=1}^n$, 
% As introduced in \autoref{sec:smalld}, we encode each partition into an $n$-bit-long parity bitmap and denote them as $A[1..n]$ and $B[1..n]$ respectively, as introduced in \autoref{sec:smalld}. For $i=1,2,...,n$, $A[i]$ (the $i^{th}$ bit of the parity bitmap $A[i]$) is equal to $1$ if $A_i$ contains an odd number of elements, and is equal to $0$ otherwise.
% % More specifically, for $i=1,2,...,n$, $A[i]$ (the $i^{th}$ bit of the parity bitmap $A[i]$) is defined as follows: $A[i]=1$ if $A_i$ contains an odd number of elements, and $A[i]=0$ otherwise. In this way, each bit $A[i]$ encodes the oddness / evenness (parity) of the cardinality of $A_i$. The $n$-bit-long parity bitmap $B[1..n]$ and $B[i]$ (the $i^{th}$ bit of $B[1..n]$) are similarly defined. 
% In the ideal case, 
% %$A[i]$ and $B[i]$ differ if and only if $A_i$ and $B_i$ have exactly $1$ distinct element, and $A[i]$ and $B[i]$ are the same if and only if $A_i=B_i$. Meanwhile, the $d$ distinct elements are hashed into $d$ different subset pairs. So 
% the two bitmaps $A[1..n]$, $B[1..n]$ differ in exactly $d$ bit positions, each of which corresponds to a subset pair that contains $1$ distinct element. Once the $d$ bit positions are known, Alice starts to reconcile each of the $d$ corresponding subset pairs by \autoref{alg:trivial_case} and gets the $d$ distinct elements (i.e., $A\Delta B$). 
% %If knowing the $d$ bit positions (i.e., the $d$ corresponding subset pairs), we can use \autoref{alg:trivial_case} to reconcile the $d$ subset pairs respectively to obtain all the $d$ distinct elements (i.e., $A\Delta B$). 
% In \autoref{sec:BCH_code}, we will describe how to find the $d$ bit positions using BCH code~\cite{Lint_IntroductionCodingTheory_1998}. 

% \medskip
% \noindent{\bf Find the $d$ Bit Positions Using ECC} 

%\subsubsection{Find the $d$ Bit Positions Using ECC}\label{sec:BCH_code}
\subsubsection{Find and Reconcile the \texorpdfstring{$d$}{d} Subset Pairs}\label{sec:BCH_code}


\begin{algorithm}
\caption{PBS-for-small-$d$ (first round)}
\label{alg:single_round_pbs}

%Hash-partition $A$, $B$ into $\{A_i\}_{i=1}^n$, $\{B_i\}_{i=1}^n$\; \label{step:hash_partition}

%Parity encode $\{A_i\}_{i=1}^n$, $\{B_i\}_{i=1}^n$ into $A[1..n]$, $B[1..n]$\; \label{step:parity_encode}
{\it Alice}: Send $\xi_A$, the BCH codeword of $A[1..n]$, to Bob\; \label{step:BCH_encode}

{\it Bob}: Decode $(B[1..n], \xi_A)$ to obtain $i_1,i_2,...,i_d$\; \label{step:BCH_decode}

{\it Bob}: Send the \code{XOR} sums of sets $B_{i_1}, B_{i_2},...,B_{i_d}$ (\autoref{alg1:sender} in \autoref{alg:trivial_case}) and $i_1,i_2,...,i_d$ to Alice\; \label{step:send_xor}

{\it Alice}: Obtain $A_{i_1}\Delta B_{i_1}, A_{i_2}\Delta B_{i_2},...,$ and $A_{i_d}\Delta B_{i_d}$ (\autoref{alg1:receiver} in \autoref{alg:trivial_case}); $\hat{D}\leftarrow \bigcup_{k=1}^d (A_{i_k}\Delta B_{i_k})$\; \label{step:trivial_reconcile}

{\it Alice}: Check $c(\hat{D})\stackrel{?}{=}c(A\Delta B)$\; \label{step:terminate_condition}

\end{algorithm}

The remaining steps of the PBS scheme are summarized in \autoref{alg:single_round_pbs}.
Recall that the partition $\{A_i\}_{i=1}^n$ and $\{B_i\}_{i=1}^n$ can be encoded as parity bitmaps $A[1..n]$ and $B[1..n]$ respectively, in which $A[i]$ or $B[i]$
%, the $i$-th bit of the parity bitmap $A[1..n]$ or $B[1..n]$, 
corresponds to the parity (oddness or evenness) of the cardinality of the subset $A_i$ or $B_i$. In the ideal case, $A[1..n]$ and $B[1..n]$ differ in exactly $d$ distinct bit positions. 
Suppose these $d$ bit positions are $i_1, i_2, ..., i_d$.  Then subset pairs $(A_{i_1}, B_{i_1}), (A_{i_2}, B_{i_2}),...,(A_{i_d}, B_{i_d})$ each differs by exactly $1$ (distinct) element
and hence can be reconciled using \autoref{alg:trivial_case}.
For this to happen, however, Bob needs to first know the values of $i_1, i_2, ..., i_d$.
% he can initiate the process of reconciling these $d$ subset pairs each using \autoref{alg:trivial_case}.
As mentioned earlier in \autoref{sec:smalld}, to this end, Alice only needs to send a BCH encoding of $A[1..n]$, denoted as $\xi_A$, that can pinpoint (to Bob) these $d$ bit locations in Bob's local bitmap $B[1..n]$ (\autoref{step:BCH_encode} in \autoref{alg:single_round_pbs}). 
%Then Bob can decode and recover $A[1..n]$ (original message) and obtain $i_1,i_2,...,i_d$.

%{\bf (Previous)} In the ideal case, for Bob to obtain $i_1,i_2,...,i_d$, Alice only needs to send $\xi_A$, the BCH code of $A[1..n]$, that can ``correct'' these $d$ bit errors in $B[1..n]$. Then Bob can decode and recover $A[1..n]$ (original message) and obtain $i_1,i_2,...,i_d$.

% {\bf (Previous)} We view $A[1..n]$ as a corrupted message of $B[1..n]$ sent ({\bf not actually being sent}) from Bob to Alice through an {\it unreliable} commnunication channel that flips $d$ bits. To locate these $d$ bit positions, we let Bob also send an {\it error-correction code} that encodes $B[1..n]$ to Alice, such that Alice can recover $B[1..n]$ (original message) and obtain the $d$ bit positions $i_1,i_2,...,i_d$. In PBS, we use BCH code~\cite{bch1} to encode $B[1..n]$ and get the error-correction code.

There are two different BCH encoding techniques: {\it systematic} and {\it unsystematic}. The difference is that, in systematic encoding, the message appears as the prefix of the codeword (i.e., 
codeword = [message, net-codeword]), whereas in unsystematic BCH encoding, the message does not.  Only systematic BCH encoding is suitable for PBS, 
since Alice sends not the ``message'' $A[1..n]$ itself, but the net-codeword $\xi_A$. With this understanding, in the sequel we drop the prefix `net-' and call $\xi_A$ a BCH {\it codeword}. 
%To correct $d$ bit errors, the length of the net-codeword only is no more than $d\log n$ bits. 
% Without causing any ambiguity, we use the term `codeword' to refer to the net-codeword in the rest of this paper.
%The computational complexity of the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} is $O(d^2\log^2 n)$.

% There are two different BCH encoding techniques: {\it systematic} and {\it unsystematic}. The difference is that, the message appears as the prefix of the codeword (i.e., codeword = [message net-codeword]) in systematic BCH encoding, whereas it does not appear as a substring of the codeword in unsystematic BCH encoding. In PBS, we choose systematic BCH encoding because we are sending not the ``message'', but the net-codeword. 
% %To correct $d$ bit errors, the length of the net-codeword only is no more than $d\log n$ bits. 
% Without causing any ambiguity, we use the term `codeword' to refer to the net-codeword in the rest of this paper.
% %The computational complexity of the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} is $O(d^2\log^2 n)$.

%The systematic BCH encoding is also used in other ECC-based set reconciliation works, such as PinSketch \cite{Wuille_Minisketchoptimizedlibrary_2019}, while PinSketch encodes a much longer message (e.g., $2^{32}$ bits) than in ours (hundreds of bits).  

%\subsubsection{Find the $d$ Bit Positions Using ECC}\label{sec:BCH_code}

% A straightforward approach to find the $d$ bit positions is to let Bob send the complete parity bitmap $B[1..n]$ to Alice, then Alice compares $A[1..n]$ with $B[1..n]$ locally. This approach has a communication overhead of $n$ bits, which is quite wasteful. As we discussed in~\autoref{sec:hash_partition}, $d$ is usually much smaller than $n$. It means $A[1..n]$ and $B[1..n]$ differ only at a tiny portion of bits. Therefore, we can view $A[1..n]$ as a corrupted message of $B[1..n]$ with $d$ bit errors, and the bit positions of the $d$ bit errors basically correspond to the $d$ subset pairs that contain distinct elements. The detection of bit errors, on the other hand, can be solved by Error-Correction Code (ECC)~\cite{Lin_ErrorControlCoding_1983}. 

% Since $A[1..n]$ and $B[1..n]$ differ at $d$ bit positions, we can view $A[1..n]$ as a corrupted message of $B[1..n]$ from Bob to Alice through an {\it unreliable} commnunication channel with $d$ corrupted bits, which are located on the $d$ bit positions. Therefore, to find the $d$ bit position, we only need to correct the $d$ corrupted bits in $A[1..n]$, which is done by transmitting a ``code'' that can correct upto $d$ bit errors from Bob to Alice through a {\it reliable} communication channel. 

% In PBS, we use {\it systematic} BCH code to generate the ``code'' by encoding the message $B[1..n]$. The codeword of the systematic BCH code is in the form of [message, net-codeword], since the message appears as the prefix of the codeword in systematic BCH code. The ``code'' is simply the net-codeword in the BCH codeword. We choose {\it systematic} BCH code because the (corrupted) message is already transmitted and we only need to pay a small communication overhead on transmitting ``code'' (i.e., net-codeword). To correct upto $d$ bit errors, the length of the net-codeword is no more than $d\log n$ bits, which is much smaller than the message when $d\!\ll\! n$. The computational complexity of the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} is $O(d^2\log^2 n)$. This type of BCH code is also used in other ECC-based set reconciliation works, such as PinSketch \cite{Wuille_Minisketchoptimizedlibrary_2019}. 

% Different from {\it unsystematic} BCH code
% The ``code'' is generated by {\it systematic} BCH code, which encodes the message $B[1..n]$ into a BCH codeword in the form of [message, net-codeword]. The ``code'' transmitted on the reliable channel is the net-codeword of the BCH codeword. In {\it systematic} BCH code, the message appears as the prefix of the codeword. 

% More specifically, PBS uses {\it systematic} BCH code~\cite{Lint_IntroductionCodingTheory_1998} that can correct upto $d$ bit errors to encode the parity bitmaps. In the {\it systematic} BCH code \footnote{In unsystematic BCH code, message does not appear to be the prefix of the codeword}, the message (i.e., the parity bitmap) appears as the prefix of the raw codeword, which in the form of [message, net codeword]. Normally, to correct upto $d$ errors, the length of the net codeword is $2n\log d$, where $n$ is the length of the message (i.e., parity bitmap). However, our case is special in the sense that the net codeword is error-free (all $d$ bit errors are in the message), so the length of the net codeword can be reduced to $n\log d$. This type of BCH code is also used in other ECC-based set reconciliation works, such as PinSketch \cite{Wuille_Minisketchoptimizedlibrary_2019}. 

% Now we can formally describe how to find the $d$ bit positions: First, Bob uses a $d$-error-correcting systematic BCH code to encode $B[1..n]$ and sends the net codeword ($d\log n$ bits) to Alice. Upon receiving the net codeword and combining it with the corrupted message $A[1..n]$, Alice uses the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} to decode the $d$ bit errors in $A[1..n]$. The communication overhead of transmitting the net codeword is $d\log n$ bits. The computational complexity of the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} is $O(d^2\log^2 n)$. Both the communication overhead and the computational complexity here are relatively small when $d$ is small.

% \medskip
% \noindent{\bf Reconcile the $d$ subset pairs using \autoref{alg:trivial_case}} 

%Once the $d$ bit positions are known, Alice can start to reconcile $(A_{i_1},B_{i_1}), (A_{i_2},B_{i_2}),...,(A_{i_d},B_{i_d})$ using \autoref{alg:trivial_case} and obtain the $d$ distinct elements (i.e., $A\Delta B$). 
Once Bob decodes $\xi_A$ (\autoref{step:BCH_decode} in \autoref{alg:single_round_pbs}) to obtain $i_1,i_2,...,i_d$, the corresponding subset pairs $(A_{i_1},B_{i_1})$, $(A_{i_2},B_{i_2})$, $...$, 
$(A_{i_d},B_{i_d})$ each can be reconciled using \autoref{alg:trivial_case}.  To do so, Bob needs to send the respective bitwise-\code{XOR} sums of the subsets $B_{i_1}$, $B_{i_2}$,$...$,$B_{i_d}$ to Alice (\autoref{alg1:sender} in \autoref{alg:trivial_case}).  In addition, Bob needs to also send the decoded ``bit error positions" $i_1, i_2, ..., i_d$ to Alice (\autoref{step:send_xor} in \autoref{alg:single_round_pbs}), who cannot decode $\xi_A$ herself without knowing $B[1..n]$.
%Alice, without knowing $B[1..n]$ otherwise would not know the ``bit error positions'' . 
Each ``bit error position'' can be encoded into $\log n$ bits, so the resulting additional communication overhead is $d\log n$ bits. 
% When reconciling $(A_{i_1},B_{i_1}), (A_{i_2},B_{i_2}),...,(A_{i_d},B_{i_d})$ using \autoref{alg:trivial_case}, Alice needs to send not only the bitwise \code{XOR} of $A_{i_1}, A_{i_2},..., A_{i_d}$, but also the indices of the subset pairs ($i_1,i_2,...,i_d$), since Bob does not know which of the $d$ subset pairs are being reconciled. Each index is an integer between $1$ and $n$ and can be encoded into $\log n$ bits, So the additional communication overhead on transmitting the indices is $d\log n$ bits. 

% \subsubsection{Reconcile the $d$ subset pairs using \autoref{alg:trivial_case}}\label{sec:reconcile_by_trivial}

% After decoding the $d$ bit errors that corresponds to the $d$ subset pairs, Alice starts to reconcile them using \autoref{alg:trivial_case}. For each of the $d$ subset pairs, Alice needs to send not only the bitwise \code{XOR} of the subset pair, but also the index of the subset pair (since Bob does not know the $d$ subset pairs to reconcile). So the communication overhead on \autoref{alg:trivial_case} is $d\log |\mathcal{U}|+d\log n$ bits. 
%Plus the communication overhead on transmitting the net codeword of parity bitmap ($d\log n$, as we explained in \autoref{sec:BCH_code}), the overall communication overhead of single-round PBS is $d\log u+2d\log n$ bits.

% \medskip
% \noindent{\bf Check if set reconciliation is complete} 

%{\bf We need a subsubsection on verification}\
\subsubsection{Verify the estimated set difference}

Once Alice receives the \code{XOR} sums and the ``bit error positions", she can recover the distinct elements each using \autoref{alg:trivial_case} to arrive at the estimated set difference
(\autoref{step:trivial_reconcile} in \autoref{alg:single_round_pbs}), denoted as 
$\hat{D}$.  However, this estimated difference $\hat{D}$ will deviate from the actual difference $A\Delta B$ when the ideal case does not happen. 
Hence, Alice needs to verify whether $\hat{D}\stackrel{?}{=}A\Delta B$ (\autoref{step:terminate_condition} in \autoref{alg:single_round_pbs}). 

{\bf Please state that you need a checksum before stating it is linear}
This can be achieved using a checksum function $c(\cdot)$ that maps any subset of the universe $\mathcal{U}$ to a $32$-bit checksum by checking $c(\hat{D})\stackrel{?}{=}c(A\Delta B)$. With incremental updates, $c(\hat{D})$ can be computed in $O(d)$ time. However, computing $c(A\Delta B)$ can be tricky, since $A$ and $B$ are {\it remote} sets and stored at hosts Alice and Bob respectively. To make the computation of $c(A\Delta B)$ easier, we choose a checksum function that is ``linear'', so that $c(A\Delta B)=c(A)\oplus c(B)$ can be precomputed. More specifically, Bob precomputes $c(B)$ and sends it to Alice. Alice also precomputes $c(A)$, and upon receiving $c(B)$, Alice can compute $c(A\Delta B)$. Here we call a checksum function ``linear'' if $c(S_1\Delta S_2)=c(S_1)\oplus c(S_2)$ for any two subsets $S_1$ and $S_2$ of the universe $\mathcal{U}$. The precomputation of $c(A\Delta B)$ incurs $32$ bits of communication overhead on transmitting $c(B)$ from Bob to Alice. In PBS, we select {\it longitudinal parity check}, the bitwise \code{XOR} of all elements (assuming each element is a $32$-bit-long binary string) in the set, as the ``linear'' checksum function. 

{\bf (previous)} This can be achieved using a ``linear'' checksum function $c(\cdot)$ that maps any subset of the universe $\mathcal{U}$ to a $32$-bit checksum by checking $c(\hat{D})\stackrel{?}{=}c(A\Delta B)$. Here we call a checksum function ``linear'' if $c(S_1\Delta S_2)=c(S_1)\oplus c(S_2)$ for any two subsets $S_1$ and $S_2$ of the universe $\mathcal{U}$. We choose a checksum function that is ``linear'', so that $c(A\Delta B)=c(A)\oplus c(B)$ can be precomputed. This precomputation incurs $32$ bits of communication overhead on transmitting $c(B)$ from Bob to Alice. With incremental updates, $c(\hat{D})$ can be computed in $O(d)$ time. In PBS, we select {\it longitudinal parity check}, the bitwise \code{XOR} of all elements (assuming each element is a $32$-bit-long binary string) in the set, as the ``linear'' checksum function. 
%It is not hard to verify it is linear.  

% Once Alice receives the \code{XOR} sums and the indices, she can compute the distinct elements, as described in \autoref{subsec:protocol0}, to obtain the set difference (denoted as $\hat{D}$). However, this reconciled set difference could be incorrect if the ideal case does not happen. Therefore, Alice needs to check if set reconciliation is successfully completed (or whether $\hat{D}=A\Delta B$). To do so, we introduce some ``linear'' checksum function $c(\cdot)$ that maps any subset of the universe $\mathcal{U}$ (such as $A$ and $B$) to a $32$-bit checksum (e.g., bitwise \code{XOR}). Here the ``linearity'' of a chechsum function refers to the fact that $c(S_1\Delta S_2)=c(S_1)\oplus c(S_2)$ for any two subsets $S_1$ and $S_2$ of the universe $\mathcal{U}$. We use this checksum function to check if $\hat{D}=A\Delta B$ by comparing $c(\hat{D})$ to $c(A\Delta B)$. Note that $c(\hat{D})$ can be computed in $O(d)$ time and $c(A\Delta B)=c(A)\oplus c(B)$ can be precomputed {\bf during the encoding period, which costs $32$ bits of communication overhead on transmitting $c(B)$ from Bob to Alice. In PBS, we select {\it longitudinal parity check}, the bitwise \code{XOR} of all elements (recall each element is a $32$-bit-long binary string) in the set, as the checksum function. It is not hard to verify it is linear.}  

% {\bf (Previous)} After reconciling the subset pairs and obtaining the reconciled set difference (denoted as $\hat{D}$), PBS needs to check if set reconciliation is complete (or whether $\hat{D}=A\Delta B$), since the reconciled set difference $\hat{D}$ is not the actual set difference $A\Delta B$ in the nonideal case (to be discussed in \autoref{subsec:exception_hash_partition}). Hence, we add a verfication step after obtaining $\hat{D}$ to check if $\hat{D}=A\Delta B$. In PBS, we check an equivalent condition, $A=B\Delta\hat{D}$, instead of $\hat{D}=A\Delta B$, since $B$ and $\hat{D}$ are both known by Bob and their set difference $B\Delta\hat{D}$ can be locally computed. More specifically, to check if the remote sets $A$ and $B\Delta\hat{D}$ are equal, we let Alice compute a $32$-bit checksum of $A$ and send it to Bob. {\bf Then Bob computes the $32$-bit checksum of $B\Delta\hat{D}$ using the same checksum algorithm and compare the two checksums. In PBS, we select {\it longitudinal parity check} (i.e., bitwise \code{XOR} of all elements in the set) as the checksum algorithm, so that the checksum $B\Delta\hat{D}$ can be efficiently computed as the bitwise \code{XOR} between the checksum of $B$ (can be pre-computed) and that of $\hat{D}$. Other checksum algorithms that are {\it linear} to the set difference operator (i.e., $\Delta$) also work for PBS. }
% Then Bob checks if $B\Delta\hat{D}$ satisfies the receiving checksum. 

The condition $\hat{D}\stackrel{?}{=}A\Delta B$ can be correctly verified by the checksum with an overwhelming probability of $1-O(10^{-12})$. More specifically, only in the nonideal case that $\hat{D}\neq A\Delta B$, which happens with a probability on the order of $10^{-2}$ (as we will show in \autoref{subsec:exception_hash_partition}), our $32$-bit checksum could possibly fail to detect that and mistakenly believe $\hat{D} = A\Delta B$ with a conditional probability of $2^{-32}\approx 2.3\times 10^{-10}$. This tiny probability of incorrect validations should be acceptable in most applications. In a few applications that allow no incorrect validation ({\it e.g.,} Bitcoin), additional techniques such as Merkle tree~\cite{merkle87} can be used in conjunction. To simplify our description, we ignore this $O(10^{-12})$ probability of incorrect validations and assume the checksum always correctly verify $\hat{D}\stackrel{?}{=}A\Delta B$ in the sequal. 

% {\bf although it could mistakenly believes two different sets as identical ones.} This event happens with probability $2^{-32}\approx 2.3\times 10^{-10}$ when the ideal case does not happen, {\bf which has a probability on the order of $10^{-2}$.} Although this event could cause PBS mistakenly believes the set reconciliation is completed, it happens with an extremely small probability (on the order of $10^{-12}$) and should be acceptable in most applications. In few applications which allow no room for error ({\it e.g.,} Bitcoin), additional techniques such as Merkle tree~\cite{merkle87} based validation will be used to verify the correctness of the results anyway. 
% %If such techniques find out that the set reconciliation is not completed, we could simply start it over and use PBS to reconcile the two sets again under a different hash function $h$. In this case, the checksum will be different If so, the  (note that PBS is a `randomized' algorithm when assuming the hash functions for hash-partition are random hash functions). 
% To simplify our description, we ignore this small probability event and assume the checksum always correctly verify $\hat{D}\stackrel{?}{=}A\Delta B$ in the sequal. 

% The condition $\hat{D}=A\Delta B$ can be almost surely verified by the checksum, 
% {\bf although it could mistakenly believes two different sets as identical ones.} This event happens with probability $2^{-32}\approx 2.3\times 10^{-10}$ when the ideal case does not happen, {\bf which has a probability on the order of $10^{-2}$.} Although this event could cause PBS mistakenly believes the set reconciliation is completed, it happens with an extremely small probability (on the order of $10^{-12}$) and should be acceptable in most applications. In few applications which allow no room for error ({\it e.g.,} Bitcoin), additional techniques such as Merkle tree~\cite{merkle87} based validation will be used to verify the correctness of the results anyway. 
% %If such techniques find out that the set reconciliation is not completed, we could simply start it over and use PBS to reconcile the two sets again under a different hash function $h$. In this case, the checksum will be different If so, the  (note that PBS is a `randomized' algorithm when assuming the hash functions for hash-partition are random hash functions). 
% To simplify our description, we ignore this small probability event and assume the checksum works perfectly in this rest of this paper. 

% We summarize all the above steps of PBS (in the first round) in \autoref{alg:single_round_pbs}.
% %{\bf not a good position to mention `for super critical applications, use a checksum for all groups', since we are describing single-group scenario. }

% \begin{algorithm}
% \caption{Single-round PBS}
% \label{alg:single_round_pbs}

% %Hash-partition $A$, $B$ into $\{A_i\}_{i=1}^n$, $\{B_i\}_{i=1}^n$\; \label{step:hash_partition}

% %Parity encode $\{A_i\}_{i=1}^n$, $\{B_i\}_{i=1}^n$ into $A[1..n]$, $B[1..n]$\; \label{step:parity_encode}
% {\it Alice}: Send $\xi_A$, the BCH codeword of $A[1..n]$, to Bob\; \label{step:BCH_encode}

% {\it Bob}: Decode $(B[1..n], \xi_A)$ to obtain $i_1,i_2,...,i_d$\; \label{step:BCH_decode}

% {\it Bob}: Send the \code{XOR} sums of sets $B_{i_1}, B_{i_2},...,B_{i_d}$ (\autoref{alg1:sender} in \autoref{alg:trivial_case}) and $i_1,i_2,...,i_d$ to Alice\; \label{step:BCH_decode}

% {\it Alice}: Obtain $A_{i_1}\Delta B_{i_1}, A_{i_2}\Delta B_{i_2},...,$ and $A_{i_d}\Delta B_{i_d}$ (\autoref{alg1:receiver} in \autoref{alg:trivial_case}); $\hat{D}\leftarrow \bigcup_{k=1}^d (A_{i_k}\Delta B_{i_k})$\; \label{step:trivial_reconcile}

% {\it Alice}: Check if $c(\hat{D})=c(A\Delta B)$\; \label{step:terminate_condition}

% \end{algorithm}
% {\color{blue}This probability is low enough for most applications. In few applications which allow no room for error ({\it e.g.,} Bitcoin), additional techniques such as Merkle tree~\cite{merkle87} based validation will be used to verify the correctness of the results anyway.}

% {\bf (Previous)} The condition $A=B\Delta\hat{D}$ can be almost surely verified by a $32$-bit checksum, although it could mistakenly believe two different sets as identical ones with probability $2^{-32}\approx 2.3\times 10^{-10}$ {\bf on top of the probability that the nonideal case happens (on the order of $10^{-2}$).} Although this event could cause an ``early'' termination and leave some distinct elements unreconciled, it happens with an extremely small probability (on the order of $10^{-12}$) and should be acceptable in most applications. {\bf To simplify our description, we ignore this small probability event and assume the checksum works perfectly in this rest of this paper. }
%and such an event (i.e., mistaken $A$ and $B\Delta\hat{D}$ are identical when they are different) never happens in our evaluation. For some super critical applications, we can certainly use a $64$-bit checksum to reduce this probability to $5.4\times 10^{-20}$ if needed.

% When the ideal case does not happen, set reconciliation cannot accomplish in one round, as we will explain in \autoref{subsec:exception_hash_partition}. Hence, we add a verfication step to check if set reconciliation is complete. Let $\hat{D}$ denote the set of reconciled elements. The idea of this verification is basically to compare $A$ with $B\Delta \hat{D}$: If $A=B\Delta \hat{D}$ (i.e., $\hat{D}=A\Delta B$), we know the set reconciliation is complete; Otherwise, the set reconciliation is incomplete.  using a $32$-bit checksum. 

% \subsubsection{Communication overhead of PBS (First Round)}\label{sec:communication_overhead_single_PBS}

% %To correct $d$ bit errors, the length of the net-codeword only is no more than $d\log n$ bits. 

% The communication overhead of \autoref{alg:single_round_pbs} consists of four components: (1) the BCH codeword $\xi_A$ in \autoref{step:BCH_encode}; (2) the subset pair indices $i_1,i_2,...,i_d$ in \autoref{step:trivial_reconcile}; (3) the bitwise \code{XOR} sums of sets $B_{i_1}, B_{i_2},...,B_{i_d}$ of $d\log |\mathcal{U}|$ bits in \autoref{step:trivial_reconcile}; and (4) transmit the $32$-bit checksum of $B$ (i.e., $c(B)$) from Bob to Alice for precomputing $c(A\Delta B)$ in \autoref{step:terminate_condition}. These four components contribute roughly (1) $d\log n$ bits (recall that to ``correct'' $d$ bit errors, the length of the BCH codeword is no more than $d\log n$ bits); (2) $d\log n$ bits; (3) $d\log |\mathcal{U}|$ bits; and (4) $32$ bits respectively to the overall communcation overhead of \autoref{alg:single_round_pbs}. 

% All the steps of PBS in the first round are summarized in \autoref{alg:single_round_pbs}. The overall communication overhead consists of three components: (1) the BCH codeword of $d\log n$ bits in \autoref{step:BCH_encode}; (2) the subset pair indices $i_1,i_2,...,i_d$ and the corresponding bitwise \code{XOR}s of $d\log n+d\log |\mathcal{U}|$ bits in \autoref{step:trivial_reconcile}; and (3) the $32$-bit checksum of $A$ in \autoref{step:terminate_condition}. 


% {\it Bob}: BCH-Encodeing $B[1..n]$ and send the codeword to Alice\; \label{step:BCH_encode}

% {\it Alice}: Upon receiving the codeword, decode the bit errors between $A[1..n]$ and $B[1..n]$\; \label{step:BCH_decode}

% {\it Alice}: For each bit error, start reconciling the corresponding subset pair by \autoref{alg:trivial_case}\; \label{step:trivial_reconcile}

% {\it Bob}: Upon receiving the reconciled set difference $\hat{D}$, check if $A=B\Delta \hat{D}$ via checksum\; \label{step:terminate_condition}


% \subsubsection{Single-round PBS}\label{sec:single_round_pbs}

% Here we summarize all the steps of single-round PBS and represent it by pseudocode in \autoref{alg:single_round_pbs}. \autoref{step:hash_partition} and \autoref{step:parity_encode} operates at both hosts (i.e., Alice and Bob). \autoref{step:hash_partition} to \autoref{step:trivial_reconcile} have been elaborated from \autoref{sec:hash_partition} to \autoref{sec:reconcile_by_trivial}. The last step in \autoref{step:terminate_condition} aims to check whether reconciliation is complete (i.e., $\mathcal{D}=A\Delta B$). More specifically, Alice calculates the checksum (e.g., CRC-$32$) of $A$ and send it to Bob. Then Bob calculates the checksum of $B\Delta \mathcal{D}$ and compares it to the receiving checksum of $A$. If the two checksums are the same, we believe $A=B\Delta \mathcal{D}$ and therefore $\mathcal{D}=A\Delta B$ (i.e., reconciliation is complete); Else, we know some elements are reconciled incorrectly. We classify those elements (i.e., the ones in the set difference between $A\Delta B$ and $\mathcal{D}$) into two subsets $A\Delta B\!\setminus\!\mathcal{D}$ and $\mathcal{D}\!\setminus\!(A\Delta B)$ and refer the elements in the former as {\it false-negatives}, and refer the elements in the later as {\it false-positives}. 

% In the ideal case, neither false-positives nor false-negatives will happen and the two checksums always equal. However, in real life, the ideal case does not always happen. We will discuss the nonideal case in \autoref{subsec:exception_hash_partition}. In our evaluation, we use a $32$-bit checksum for comparing $A$ to $B\Delta \mathcal{D}$ that has {\bf an error probability} roughly $10^{-9}$. This error (i.e., mistake $A=B\Delta \mathcal{D}$) incurs false-negatives. All set reconciliation schemes have the same problem on their termination conditions (i.e., check whether $\mathcal{D}=A\Delta B$). For some super critical applications, we can certainly decrease the error probability by using more powerful checksums (i.e., $64-$bit). Using a $32$-bit checksum, this kind of false-negatives never happen in the evaluation. 
% %For simplification, we assume no error happens when checking $\mathcal{D}=A\Delta B$ in the rest of the paper.

% \begin{algorithm}
% \caption{Single-round PBS}
% \label{alg:single_round_pbs}

% Hash-partition $A$, $B$ into $\{A_i\}_{i=1}^n$, $\{B_i\}_{i=1}^n$\; \label{step:hash_partition}

% Parity encode $\{A_i\}_{i=1}^n$, $\{B_i\}_{i=1}^n$ into $A[1..n]$, $B[1..n]$\; \label{step:parity_encode}

% {\it Bob}: Encode $B[1..n]$ by BCH code, then send the codeword to Alice\; \label{step:BCH_encode}

% {\it Alice}: Upon receiving the codeword, decode the bit errors between $A[1..n]$ and $B[1..n]$\; \label{step:BCH_decode}

% {\it Alice}: For each bit error, reconcile the corresponding subset pair by \autoref{alg:trivial_case}\; \label{step:trivial_reconcile}

% {\it Bob}: Upon the reconciled distinct elements $\mathcal{D}$, check whether $A=B\Delta \mathcal{D}$ via checksum\; \label{step:terminate_condition}
% \end{algorithm}

\subsubsection{Exception Handling}\label{subsec:exception_hash_partition}

When the ideal case does not happen, some subset pair may contain more than $1$ distinct elements and cannot be successfully reconciled by \autoref{alg:trivial_case}. In this case, the checksum will detect this event and run another round of PBS to reconcile the ``remaining'' distinct elements, as will be elaborated in \autoref{sec:multi-rounds}. There are two types of exceptions that possibly happen in such a subset pair: 

\noindent {\bf Type (\RN{1}) exception}: Subset pair $(A_i, B_i)$ contains a nonzero even number of distinct elements. In this case $A[i]=B[i]$. The BCH codeword $\xi_A$ cannot detect this exception and PBS will not reconcile the subset pair yet in this round. This exception happens with a small but nontrivial probability: For example, when $d=5$ and $n=255$ (i.e., throwing $5$ balls each uniformly and randomly into $255$ bins), the probability that some bin has a nonzero even number of (in this case either $2$ or $4$) balls is roughly $0.04$. 
%Note that when a type (\RN{1}) event happens, the checksum (\autoref{step:terminate_condition} in \autoref{alg:single_round_pbs}) can detect that the set reconciliation has not been completed. Then PBS will start another round to reconcile the ``hidden'' distinct elements (the ones that have not been reconciled in this round), 
%so on so force, until all distinct elements are successfully reconciled and the checksum is verified to be correct, 
%as we will describe in \autoref{sec:multi-rounds}. 

% Note that when a Type (\RN{1}) subset pair exists, the $32$-bit checksum (\autoref{step:terminate_condition} in \autoref{alg:single_round_pbs}) can almost surely detect that the set reconciliation is incomplete. If this is the case (i.e., the checksum is verified to be incorrect), PBS will start another round of set reconciliation to reconcile the remaining distinct elements (e.g., the ``hidden'' distinct elements in Type (\RN{1}) subset pairs), so on so force, until all distinct elements are reconciled and the checksum is verified to be correct, as we will describe in \autoref{sec:multi-rounds}. 

\noindent {\bf Type (\RN{2}) exception}: Subset pair $(A_i, B_i)$ contains an odd number of distinct elements. In this case, $A[i]\neq B[i]$. Bob will mistakenly believe that $(A_i, B_i)$ contains exactly one distinct element and try to recover it using \autoref{alg:trivial_case}. The ``recovered'' element $s$ is however the bitwise \code{XOR} of all distinct elements in $(A_i, B_i)$ (explained in \autoref{subsec:protocol0}), which is a fake distinct element.
%, which will be mistakenly believed as the distinct element of $(A_i, B_i)$. 
This event happens with a tiny probability: In the same example above ($d=5$ and $n=255$), the probability that some bin has an odd number of balls (in this case $3$ or $5$) is only $1.52\times 10^{-4}$. 

% \noindent {\bf Type (\RN{2}) exception}: Subset pair $(A_i, B_i)$ contains an odd number of distinct elements whose quantity is an odd number no less than $3$, the parity bits of $A_i$ and $B_i$ will be different and PBS will reconcile the subset pair using \autoref{alg:trivial_case}. The reconciled element $s$ is however the bitwise \code{XOR} of all distinct elements in $(A_i, B_i)$ (explained in \autoref{subsec:protocol0}), which is a ``fake'' distinct element.
% %, which will be mistakenly believed as the distinct element of $(A_i, B_i)$. 
% This event happens with a tiny probability: In the same example above ($d=5$ and $n=255$), the probability that some bin has an odd number of balls that is no less than $3$ (in this case $3$ or $5$) is only $1.52\times 10^{-4}$.

%Similarly, the $32$-bit checksum can also detect that the set reconciliation has not been completed when a type (\RN{2}) event happens. Both the ``hidden'' and the ``fake'' distinct elements can also be reconciled in later rounds. 

%Note that those ``fake'' distinct elements will become new distinct elements in the next round and therefore incur additional communication overhead to reconcile. 
%Note that those ``fake'' distinct elements will incur additional communication overhead if we want to reconcile them ``later''. Therefore, we add a verification on each reconciled distinct element of \autoref{alg:trivial_case} that can detect ``fake'' distinct elements with high probability. \autoref{alg:verification} shows how this verification works, and it does not incur additional communication overhead.

Note that the consistent nature of hash-partition provides us a mechanism that can help detect fake distinct elements with high probability. \autoref{alg:verification} shows how this verification works.

\begin{algorithm}
\caption{Verify the ``recovered'' element $s$ of $(A_i, B_i)$}
\label{alg:verification}
\If{$h(s)\neq i$} {Discard the ``recovered'' element $s$;}
\end{algorithm}

Although a distinct element of $(A_i, B_i)$ must be in sub-universe $\mathcal{U}_i$ (i.e., the hash value of the element under $h$ equals to $i$), a fake distinct element could be in any sub-universe with probability $1/n$, since it is the bitwise \code{XOR} of multiple distinct elements of $(A_i, B_i)$. Therefore, even when a type (\RN{2}) exception happens to $(A_i, B_i)$, \autoref{alg:verification} only fails to identify a ``fake'' distinct element with a conditional probability of $1/n$, which is roughly $3.9\times 10^{-3}$ when $n=255$. The probability for both events to happen in the same example above ($d=5$ and $n=255$) is $6\times 10^{-7}$, which is the multiplication between the probability for the type (\RN{2}) exception to happen ($1.52\times 10^{-4}$) and the conditional probability ($3.9\times 10^{-3}$). This mechanism only needs to locally verify the ``recovered'' elements of \autoref{alg:trivial_case} and does not incur any additional communication overhead.

% Although a distinct element of $(A_i, B_i)$ must be in sub-universe $\mathcal{U}_i$ (i.e., the hash value of the element under $h$ equals to $i$), a fake distinct element could be in any sub-universe with probability $1/n$, since it is the bitwise \code{XOR} of multiple distinct elements of $(A_i, B_i)$. Therefore, even when a type (\RN{2}) exception happens to $(A_i, B_i)$, \autoref{alg:verification} only fails to identify a ``fake'' distinct element with a conditional probability of $1/n$, which is roughly $3.9\times 10^{-3}$ when $n=255$, under the condition that the type (\RN{2}) event happens, which also has a tiny probability as we explained earlier. In the same example above ($d=5$ and $n=255$), a ``fake'' distinct element that fails to be detected by \autoref{alg:verification} happens with a tiny probability of $6\times 10^{-7}$, which is the multiplication of the probability of the type (\RN{2}) event ($1.52\times 10^{-4}$) and the probability of \autoref{alg:verification} fails ($3.9\times 10^{-3}$).  This mechanism only needs to locally verify the reconciled elements of \autoref{alg:trivial_case} and does not incur any additional overhead.
%{\bf (removed to the beginning of theoretical analysis) To simplify our description, we also ignore this small probability event and assume all ``fake'' distinct elements will be successfully detected by \autoref{alg:verification} in this rest of this paper. }

% Note that either a type (\RN{1}) event or a type (\RN{2}) event will cause PBS fails to reconcile all distinct elements, which can be detected by the checksum (\autoref{step:terminate_condition} in \autoref{alg:single_round_pbs}). In this case, PBS will continue to reconcile the ``rest'' of distinct elements using additional rounds. 

%In this case, PBS will continue to reconcile the ``remaining'' distinct element by starting another round, as we will describe in \autoref{sec:multi-rounds}. The ``remaining'' distinct elements here consist of (1) the ``hidden'' distinct elements that have not been reconciled in this round and (2) the ``fake'' distinct elements that are not verified by \autoref{alg:verification}.

% {\bf (to be removed) Readers may wonder encoding the exact subset cardinalities (i.e., $|A_i|, |B_i|$) instead of their oddness / evenness (parity) (described in \autoref{sec:hash_partition}) could help to detect and solve Type (\RN{1}), (\RN{2}) events. However, encoding the exact subset cardinalities not only incurs much more additional communication overhead comparing to encoding their parities, but also barely helps on detecting Type (\RN{1}), (\RN{2}) events, since we cannot precisely derive $|A_i\Delta B_i|$, the total number of distinct elements in $(A_i, B_i)$, even knowing $|A_i|, |B_i|$: For instance, when $|A_i|\!=\!|B_i|\!=\!50$, $|A_i\Delta B_i|$ could be any even number ($\leq 100$) if the distinct elements are evenly splitted and placed between $A_i$ and $B_i$. }

% As we have described in \autoref{sec:hash_partition}, the ideal case does not always happen, which means some subset pair may contain more than $1$ distinct elements and cannot be successfully reconciled by \autoref{alg:trivial_case}. Due to the parity encoding, we can classify such subset pair into the following two scenarios:

% \begin{itemize}
%     \item Scenario 1: If a subset pair $(A_i, B_i)$ contains even number ($\geq 2$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be the same and PBS will not reconcile the subset pair yet in this round;
%     \item Scenario 2: If a subset pair $(A_i, B_i)$ contains odd number ($\geq 3$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be different and PBS will reconcile the subset pair using \autoref{alg:trivial_case}. The reconciled element (i.e., $s$ in \autoref{alg:trivial_case}) is however the bitwise \code{XOR} of all distinct elements in $(A_i, B_i)$ (explained in \autoref{subsec:protocol0}), which will be mistakenly believed as the distinct element of $(A_i, B_i)$. 
%     %However, as described in \autoref{subsec:protocol0}, when a subset pair contains more than $1$ distinct elements, \autoref{alg:trivial_case} will output the bitwise \code{XOR} of them as the `distinct element', which is not an actual distinct element with high probability;
% \end{itemize}

% In both scenarios, the distinct elements in the subset pair will not be reconciled in this round. As we will describe in \autoref{sec:multi-rounds}, we generalize PBS into multi-round, so that the distinct elements that have not been reconciled in the first round will be reconciled in later rounds. On the other hand, the second scenario could result in incorrectly reconciled distinct elements, which will become new distinct elements in the next round in multi-round PBS. 

% % In both scenarios, the distinct elements in the subset pair cannot be successfully reconciled in this round and will remain in the set difference (i.e., $(A\Delta B)\!\setminus\!\hat{D}$). On the other hand, the incorrectly reconciled distinct element in the second scenario will appear as a new distinct element (i.e., $\hat{D}\!\setminus\!(A\Delta B)$) in the next round if we generalize PBS into multi-round (to be elaborated in \autoref{sec:multi-rounds}). Both scenarios can be almost surely detected by the 32-bit checksum (\autoref{step:terminate_condition} in \autoref{alg:single_round_pbs}). The set difference after the reconciliation in this round, $D\Delta\hat{D}$, can be reconciled in later rounds, as we will describe in \autoref{sec:multi-rounds}. 

% Naturally, we do not want to generate new distinct elements in the process of set reconciliation, even though it happens with a tiny probability when $n=\Omega(d^2)$: For instance, when $d=5$ and $n=255$ (i.e., throwing $5$ balls uniformly and randomly into $255$ bins), the probability (i.e., some bin has $3$ or $5$ balls) is only $7.6\times 10^{-6}$. Therefore, we add a verification with no additional communication cost on each reconciled element of \autoref{alg:trivial_case}, such that each incorrect dinstinct element can be identified with high probability. The verfication is shown in \autoref{alg:verification}. 

% \begin{algorithm}
% \caption{Verify reconciled element $s$ of $(A_i, B_i)$}
% \label{alg:verification}
% \If{$h(s)\neq i$} {Discard the reconciled element $s$;}
% \end{algorithm}

% Although any distinct element of $(A_i, B_i)$ must be in sub-universe $\mathcal{U}_i$ (i.e., the hash value of the element under $h$ equals to $i$), the bitwise \code{XOR} of multiple distinct elements of $(A_i, B_i)$ could be in any sub-universe with probability $1/n$. Therefore, \autoref{alg:verification} fails to identify an incorrectly reconciled distinct element in the second scenario with probability $1/n$ that is roughly $3.9\times 10^{-3}$ when $n=255$. In other words, an incorrectly reconciled distinct element that cannot be identified by \autoref{alg:verification} appears with probability $3\times 10^{-8}$. {\bf I feel that defining $\tilde{a}_4=a_1\oplus a_2\oplus a_3$ does not help much.}

% In both scenarios, the distinct elements in the subset pair cannot be successfully reconciled in this round. These distinct elements can be reconciled in later rounds if needed, as we will describe in \autoref{sec:multi-rounds}. In this section, we only discuss how to identify the {\it incorrect} distinct element in the second scenario. Let us use an example to elaborate the second scenario: Assume $(A_i, B_i)$ contains $3$ distinct elements $a_1, a_2, a_3$, then Bob computes $\tilde{s}=a_1\oplus a_2\oplus a_3$ using \autoref{alg:trivial_case} and mistakes it as the distinct element in $(A_i, B_i)$. 

% In both scenarios, the distinct elements in the subset pair cannot be successfully reconciled (i.e., false-negatives defined in \autoref{sec:single_round_pbs}. The distinct elements that are not successfully reconciled in this round, if needed, can be reconciled in later rounds as we will describe in \autoref{sec:multi-rounds}. In this section, we only discuss how to identify the {\it incorrect} distinct elements in the second scenario. Let us use an example to elaborate the second scenario: Assume $(A_i, B_i)$ contains $3$ distinct elements $a_1, a_2, a_3$, then Bob computes $\tilde{s}=a_1\oplus a_2\oplus a_3$ using \autoref{alg:trivial_case} and mistakes it as the distinct element in $(A_i, B_i)$. 

\begin{comment}
============================================

We add a no-communication-cost verification step to check whether a reconciled element is an actual distinct element or not. Note that an actual distinct element of $(A_i, B_i)$ must be in sub-universe $\mathcal{U}_i$. On the other hand, an incorrectly reconciled element (e.g., $\tilde{s}$) can be in any sub-universe with probability $1/n$. So at the end \autoref{subsec:protocol0}, we check whether the reconciled element is in $\mathcal{U}_i$ by the hash function $h$ in hash-partition:

This verfication cannot completely eliminate false-positives, since an incorrectly reconciled element (e.g., $\tilde{s}$) can coincidentally end up in $\mathcal{U}_i$ with probability $1/n$. The chance of false-positives is extremely small using the verification. For instance, if $d=5$ and $n=255$, the probability of the second scenario is only $7.6\times 10^{-6}$. The probability of false-positives using the verfication is $1/n$ times this small probability, which is roughly $3\times 10^{-8}$. {\bf Note that a small probability of false-positives only costs a little waste on set reconciliation when synchronizing objectives (e.g., files), which is acceptable for most applications.}

Even worse, in the second scenario, the false-positives defined in \autoref{sec:single_round_pbs} could happen. For example, if subset pair $(A_i, B_i)$ contains $3$ distinct elements $s_1, s_2, s_3$, then \autoref{alg:trivial_case} computes $\tilde{s}=s_1\oplus s_2\oplus s_3$ and Bob mistakes $\tilde{s}$ as an actual distinct element. The good thing is, the probability of this kind of false-positives is extremely small for small $d$. For instance, if $d=5$ and $n=255$, the probability of the false-positives is only $7.6\times 10^{-6}$. To further reduce the chance of false-positives, we add a no-communication-cost verification step at the end of \autoref{subsec:protocol0} to check whether $\tilde{s}$ is an actual distinct element or not. The verification step works as follows: Given the output $s$ of subset pair $(A_i,B_i)$, if $s\in\mathcal{U}_i$ (i.e., $h(s)=i$), we consider $s$ as an actual distinct element; Otherwise, we consider $s$ as an incorrect output and discard it. 

Note that if $\tilde{s}\in A_i\Delta B_i$, $\tilde{s}$ must be in sub-universe $\mathcal{U}_i$. However, if $\tilde{s}$ is the bitwise \code{XOR} of the distinct elements in $(A_i,B_i)$ (i.e., the second scenario happens), it ends up in $\mathcal{U}_i$ with probablity of only $1/n$. 
%In fact, if we assume the hash-partition described in \autoref{sec:hash_partition} hashes the elements of $\mathcal{U}$ uniformly, independently, and randomly into $n$ sub-universes, the output $s$ in the second scenario will be in a different sub-universe $\mathcal{U}_j (j\neq i)$ with a high probability of $1-\frac{1}{n}$. Hence, this verfication method can further reduce the probability of false-positives by a factor of $\frac{1}{n}$. 
Use the same example (i.e., $d=5$, $n=255$), the probability of this kind of false-positives is reduced from $7.6\times 10^{-6}$ to $3\times 10^{-8}$ by this verification method. 
%{\bf This probability can be further reduced in \autoref{subsec:protocol2}, where PBS does two tiers of hash-partitions. So we can do verification on both of the two hash functions.}

%In some super critical cases (i.e., no false-positive is allowed), we can use a more powerful verification method to completely eliminate false-positives. That is, to check if the output $s$ exists in exactly one of the two sets (i.e., $s\in A\!\setminus\! B$ or $s\in B\!\setminus\! A$). To do so, Bob transmits $s$ along with an identification bit $\mathbbm{1}_{\{s\in B\}}$ to Alice, then Alice checks if $s\in (A\!\setminus\! B)\bigcup (B\!\setminus\! A)$ . This method verification costs additional $d(\log u+1)$ bits of communication overhead. In most applications, this rigorous $0\%$ probability guarantee of false-positives is unnecessary and the probability of the former verification method is small enough, so we use the former in the evaluation. Based on our observation, this kind of false-positives do not happen even once in the evaluation using the former verfication method. In the rest of this paper, we assume Scenario 2 is always correctly verified. 

============================================
\end{comment}

\subsection{Running PBS for Multiple Rounds}\label{sec:multi-rounds}

%{\bf (merged from the following two paragraphs)} 
To deal with the ``remaining'' distinct elements, we remove (and save) all the distinct elements that has been reconciled in the first round (i.e., $\hat{D}$) and run another round of PBS. More precisely, in the second round, we try to reconcile $A\Delta \hat{D}$ and $B$ by running the same procedure except for using a different and independent hash function (than $h$) to do hash-partition. 
%instead of reconciling $A$ and $B$ for both (1) removing all the distinct elements that have been reconciled; and (2) keeping all the distinct elements that have not been reconciled, which we will explain shortly. 
Here we use a different and independent hash function to avoid the same type (\RN{1}), (\RN{2}) exceptions happen again. 
% We use a different hash function for hash-partition in the second round to avoid the same exceptions (i.e., type (\RN{1}), (\RN{2}) events) that happened in the first round happen again. 
PBS keeps running until the set reconciliation is successfully completed as verified by the checksum (\autoref{alg:single_round_pbs} of \autoref{step:terminate_condition}). The use of independent hash functions in different rounds naturally enables the Markov chain modeling of the reconciliation process, which will be elaborated in \autoref{sec:single_markov}. 

{\bf (new content)} Note that a fake distinct element $s$, if is not detected by \autoref{alg:verification}, will be mistakenly believed as a distinct element (between $A$ and $B$) and contained in $\hat{D}$. This is not an issue because in this case, $s$ is an actual distinct element between $A\Delta \hat{D}$ and $B$. Starting with the second round, PBS will try to reconcile $s$ and eventually ``correct'' this fake distinct element. 

% We emphasize that the fake distinct elements (incurred by type (\RN{2}) exception) that are not detected by \autoref{alg:verification} in the first round can also be reconciled in the second round. also keeps all the distinct elements that need to be reconciled. Note that the ``remaining'' distinct elements can be classified into two catagories: (1) the ``hidden'' distinct elements that have not been reconciled yet (i.e., $D\!\setminus\!\hat{D}$), which are incurred by either a type (\RN{1}) event or a type (\RN{2}) event; and (2) the ``fake'' distinct elements incurred by both a type (\RN{2}) event and the corresponding verification failure in \autoref{alg:verification} (i.e., $\hat{D}\!\setminus\!D$). It is not hard to verify that this classification of the ``rest'' distinct elements (i.e., $D\!\setminus\!\hat{D}$ and $\hat{D}\!\setminus\!D$) is a partition of the set difference between $A\Delta \hat{D}$ and $B$, which confirms our emphasis. 

% {\bf (new content)} We emphasize that reconciling $A\Delta \hat{D}$ and $B$ not only removes all the distinct elements that have been reconciled, but also keeps all the distinct elements that need to be reconciled. Note that the ``rest'' distinct elements can be classified into two catagories: (1) the ``hidden'' distinct elements that have not been reconciled yet (i.e., $D\!\setminus\!\hat{D}$), which are incurred by either a type (\RN{1}) event or a type (\RN{2}) event; and (2) the ``fake'' distinct elements incurred by both a type (\RN{2}) event and the corresponding verification failure in \autoref{alg:verification} (i.e., $\hat{D}\!\setminus\!D$). It is not hard to verify that this classification of the ``rest'' distinct elements (i.e., $D\!\setminus\!\hat{D}$ and $\hat{D}\!\setminus\!D$) is a partition of the set difference between $A\Delta \hat{D}$ and $B$, which confirms our emphasis. 

% To deal with the ``remaining'' distinct elements, we remove (and save) all the distinct elements that has been reconciled in the first round (i.e., $\hat{D}$) and run another round of PBS. In the second round, we reconcile $A\Delta \hat{D}$ and $B$ instead of reconciling $A$ and $B$ to remove all the reconciled distinct elements. We use a different hash function for hash-partition in the second round to avoid the same exceptions (i.e., type (\RN{1}), (\RN{2}) events) that happened in the first round happen again. This procedure replicates until If until all distinct elements are successfully reconciled and the checksum is verified to be correct. 

% {\bf (to be removed)} When the ideal case does not happen (i.e., type (\RN{1}) or type (\RN{2}) event happens), PBS will know the set reconciliation has not been completed via the $32$-bit checksum (\autoref{step:terminate_condition} in \autoref{alg:single_round_pbs}). To reconcile those distinct elements that have not been reconciled yet in the first round, we rule out all successfully reconciled elements and run another round of PBS. This procedure replicates until all distinct elements are successfully reconciled and the checksum is verified to be correct.

% {\bf (to be removed)} More specifically, in the second round, we run PBS to reconcile $A$ and $B\Delta \hat{D}$ instead of $A$ and $B$ to rule out all elements that have been reconciled, where $\hat{D}$ is the set of reconciled distinct elements in the first round. We use a different hash function for hash-partition in the second round to avoid the same exceptions (i.e., type (\RN{1}), (\RN{2}) events) that happened in the first round happen again. The later rounds are similarly operated. 

%{\bf Normally, we want PBS to successfully reconcile all distinct elements in only a few rounds (say $3$) with high probability (say $99\%$). Hence, when tuning parameters (to be discussed in \autoref{sec:parameter_settings}), we set a {\it target success probability} $p_0$ of $r$ rounds as a paramenter setting requirement, which aims to ensure the probability that all distinct elements are reconciled in $r$ rounds to be larger than $p_0$. This requirement should also ensure the majority of the distinct elements are reconciled in the first round. Use the same example ($d=5, n=255$), on average $4.81$ out of $5$ distinct elements should be reconciled in the first round. So the total communication overhead in all rounds is only slightly larger than ($1.01$ to $1.07$ times of, as we will show in \autoref{fig:per-round-con}) that in the first round. Due to this reason, we use the communication overhead in the first round (described in \autoref{sec:communication_overhead_single_PBS}) to approximate the total communication overhead of all rounds in parameter settings (to be elaborated in \autoref{sec:parameter_settings}.}

% Although PBS may need to run many rounds to reconcile all distinct elements, the communication overhead mostly happens in the first round, since the majority of the distinct elements should be reconciled in the first round. Use the same example ($d=5, n=255$), on average $4.81$ out of $5$ distinct elements should be reconciled in the first round. So the total communication overhead in all rounds is only slightly larger than ($1.01$ to $1.07$ times of, to be shown in \autoref{fig:per-round-con}) that in the first round. Due to this reason, we use the communication overhead in the first round (described in \autoref{sec:communication_overhead_single_PBS}) to approximate the total communication overhead (all rounds) in parameter settings (to be elaborated in \autoref{sec:parameter_settings}).

%For the moment, we assume no ``fake'' distinct element in type (\RN{2}) subset pairs fails to be detected, which happens with overwhelming probability as explained in \autoref{subsec:exception_hash_partition}. Then 
%PBS reconciles the distinct elements gradually round by round. This is the ``piecewise decodability'' mentioned in \autoref{sec:intro_oursolution}. We use the following example to describe it in details: 
%Given two sets with $10$ distinct elements, in the first round, PBS tries to reconcile the $10$ distinct elements and say $6$ out of the $10$ distinct elements are successfully reconciled. Then the $6$ reconciled distinct elements are removed and PBS tries to reconcile the remaining $4$ distinct elements in the second round. Say $2$ out of the $4$ remaining distinct elements are successfully reconciled, and that leaves $2$ remaining distinct elements to be reconciled in the third round, so on so force. 
% Given two sets $A$, $B$ with $10$ distinct elements, in the first round, PBS hashes them into $7$ distinct subset pairs. $6$ distinct elements are hashed into $6$ distinct subset pairs, and the other $4$ distinct elements are hashed into the same subset pair. Then the former $6$ distinct elements are successfully reconciled in the first round and the later $4$ distinct elements remain to be reconciled in the second round, which are hashed into $3$ distinct subset pairs (under a different hash function). $2$ remaining distinct elements are hashed into $2$ distinct subset pairs, and the other $2$ remaining distinct elements are hashed into the same subset pair. Then the former $2$ remaining distinct elements are successfully reconciled in the second round and the later $2$ remaining distinct elements remain to be reconciled in the third round, so on so force. 
%The dynamics of the number of remaining distinct elements (i.e., $10\leadsto 4\leadsto 2\leadsto \cdots$ in the example) is in nature a Markov chain, which will be elaborated and analyzed in \autoref{sec:single_markov} to derive a tight tail bound of the probability that all distinct elements are reconciled in $r$ rounds.

% Even if the ideal case does not happen, most of the distinct elements should be distributed into different subset pairs, one distinct element in each, and therefore can be successfully reconciled. So in the first round, even if PBS cannot reconcile all distinct elements, it can reconcile the majority of them.
% % (piecewise decodability mentioned in \autoref{sec:intro_oursolution})
% Based on this intuition, we generalize PBS to multi-round, so that the distinct elements that are not reconciled yet in the first round can be reconciled in later rounds.  

% Without loss of generality, we only describe the second round of multi-round PBS, the reconciliation in the later rounds are similar. Let $\hat{D}_1$ denote the set of reconciled elements in the first round. If set reconciliation is not complete in the first round (i.e., the checksum infers $A\neq B\Delta \hat{D}_1$), then multi-round PBS saves $\hat{D}_1$, which includes correctly and incorrectly reconciled elements as described in \autoref{subsec:exception_hash_partition}, and starts the second round to find (1) the remaining distinct elements; (2) the incorrectly reconciled distinct elements in the first round. In the second round, multi-round PBS reconciles $A$ and $B\Delta \hat{D}_1$ instead of $A$ and $B$ (i.e., $B\leftarrow B\Delta\hat{D}_1$) to rule out all elements that have been reconciled. {\bf It uses a hash function that is different from the one used in the first round for hash-partition, otherwise every remaining distinct element will be hashed into the same subset pair and cause the same exception (described in \autoref{subsec:exception_hash_partition}) that happened in the first round.}

% If set reconciliation is complete in the second round, the set of reconciled elements in the second round (denoted as $\hat{D}_2$) should be the union of (1) all distinct elements that have not been reconciled in the first round (i.e., $(A\Delta B)\!\setminus\!\hat{D}_1$); and (2) all incorrectly reconciled elements in the first round (i.e., $\hat{D}_1\!\setminus\!(A\Delta B)$), which is by definition the set difference between $A\Delta B$ and $\hat{D}_1$. Therefore, the overall set difference $A\Delta B$ equals to the set difference between $\hat{D}_1$ and $\hat{D}_2$; Else, multiround PBS saves $\hat{D}_2$ and starts the third round, so on so force. 

% {\bf May need this algorithm to show the dynamics, if so, the earlier algorithm needs to change accordingly.}
% \IncMargin{1em}
% \begin{algorithm}
% \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
% \Input{$A$ and $B$}
% \Input{Maximum number of rounds $r$}
% \Output{$D$}

% $\hat{D},\mbox{ complete} \leftarrow PBS(A,B)$\;

% $D \leftarrow \hat{D}$\;

% \While{!complete and $r>0$}{
	
% 	$B \leftarrow B\Delta\hat{D}$\;

% 	$\hat{D},\mbox{ complete} \leftarrow PBS(A,B)$\;

% 	$D \leftarrow D\Delta\hat{D}$\;

% 	$r \leftarrow r-1$\;
% }

% \caption{Multi-round PBS} \label{proto:multirounds}
% \end{algorithm}\DecMargin{1em}

% The idea of multi-round PBS is quite simple: In each round, we discard the reconciled distinct elements in the previous rounds and aim to find the rest distinct elements from the remaining elements. More specifically, the first round of multi-round PBS is just the same as single-round PBS in \autoref{alg:single_round_pbs}. The second round has the same procedures as the first round. One difference is, we update $B$ by $B\leftarrow B\Delta\mathcal{D}$ in the second round, so that (1) Reconciled distinct elements in $\mathcal{D}$ that were contained in $A\Delta B$ are not longer contained in $A\Delta (B\Delta\mathcal{D})$; and (2) The other distinct elements remain in $A\Delta (B\Delta\mathcal{D})$ and can be reconciled later. The other difference is, we use a different hash function for partition (\autoref{step:hash_partition}) in the second round. Later rounds update $B$ in the same way and also use different hash functions. Multi-round terminates if the check in \autoref{step:termination} is correct. The overall set difference $A\Delta B$ is simply the union of reconciled distinct elements in all rounds. 

% A straightforward approach to discard reconciled distinct elements is to remove them from both $A$ and $B$. This approach however incurs additional communication overhead to update $A$, since only Bob learns the partial set difference in \autoref{step:reconcile}. Therefore, we use the approach in \autoref{step:updateb} that only updates $B$. It has another benefit in \autoref{step:termination}, which only needs to transmit the CRC of $A$ from Alice to Bob in the first round. In the later rounds, \autoref{step:termination} can be checked locally by Bob and does not require any additional communication overhead;

% Note that the communication overhead in the first round accounts for a large percentage of the total communication overhead in multi-round PBS, since most of the distinct elements (over $95\%$ as we will show in {\bf point to the figure}) should be reconciled in the first round. Therefore, we use the same parameter $n$ in later rounds because otherwise we have to compute a new parameter that can only save tiny communication overhead, even though the number of remaining distinct elements is small and can be reconciled using smaller $n$ with high probability. {\bf Due to the same reason, we can the same expression of the communication overhead in single-round PBS to approximate the communication overhead in multi-round PBS.}

% The natural termination condition of multi-round PBS is that all distinct elements are reconciled, which could require a large number of rounds and incur large additional communication overhead (each additional round incurs $d\log n$ bits of additional communication overhead on transmitting BCH codeword). To control the amount of additional communication overhead, we set another termination condition that multi-round PBS runs for at most $r$ rounds (typically $2$ or $3$). This termination condition could cause an `early' termination when some distinct elements have not been reconciled. However, under proper parameter settings (to be discussed in \autoref{sec:parameter_settings}), we can prove that the probability of an `early' termination (i.e., set reconciliation is incomplete in $r$ round) is very small
% %, and even if an `early' termination happens, an overwhelming percentage of distinct elements should have been reconciled, which is sufficient for most applications
% . For example, when $d=5, n=255, r=2$, an `early' termination happens with probability $4.8\times 10^{-4}$ (how to compute this probability will be elaborated in \autoref{sec:tail_bound}).

% For the moment, we assume no incorrectly reconciled distinct elements appears in multi-round PBS, which happens with overwhelming probability as explained in \autoref{subsec:exception_hash_partition}. Then multi-round PBS reconciles the distinct elements gradually round by round. This is the ``piecewise decodability'' mentioned in \autoref{sec:intro_oursolution}. We use the following example to describe it in details: Given two sets $A$, $B$ with $10$ distinct elements (i.e., $d=10$), in the first round, multi-round PBS hashes them into $7$ distinct subset pairs. $6$ distinct elements are hashed into $6$ distinct subset pairs, and the other $4$ distinct elements are hashed into the same subset pair. Then the former $6$ distinct elements are successfully reconciled in the first round and the later $4$ distinct elements remain to be reconciled in the second round, which are hashed into $3$ distinct subset pairs (under a different hash function). $2$ remaining distinct elements are hashed into $2$ distinct subset pairs, and the other $2$ remaining distinct elements are hashed into the same subset pair. Then the former $2$ remaining distinct elements are successfully reconciled in the second round and the later $2$ remaining distinct elements remain to be reconciled in the third round, so on so force. The dynamics of the number of remaining distinct elements (i.e., $10\leadsto 4\leadsto 2\leadsto \cdots$ in the example) is in nature a Markov chain, which will be elaborated and analyzed in \autoref{sec:tail_bound_per_group} to derive a tail bound of success probability (i.e., all distinct elements are reconciled in $r$ rounds) for paramenter settings. 

% In most applications, a high percentage of reconciliation (e.g., $>99\%$ distinct elements are reconciled) is good enough. Therefore, we add another termination condition on the maximum number of rounds (denoted as $r$). The larger $r$ is, the higher percentage of distinct elements will be reconciled. How to set parameters based on $r$ will be elaborated in \autoref{sec:parameter_settings};

% Readers may think the communication overhead of multi-round PBS is proportional to the number of rounds. In fact, the majority of the communication overhead is spent in the first round, since most of the distinct elements (over $95\%$ as we will show in {\bf point to the figure}) are reconciled in the first round. Each additional round only incurs a small amount of additional communication overhead. For example, when $d=10, n=255, |\mathcal{U}|=2^{32}$, assume $8$ distinct elements are reconciled in the first round and the rest $2$ distinct elements are reconciled in the second round. Then the communication overhead in the first round is $432$ bits. That number of the second round is only $160$


%the communication overhead of single-round PBS of $272$ ($2d\log n+d\log |\mathcal{U}|+32$) bits, and each additional round incurs $40$ ($d\log n$) bits of additional communication overhead. 

%among the three components of the communication overhead mentioned in \autoref{sec:communication_overhead_single_PBS}, only the first component (i.e., the BCH codeword) is proportional to the number of rounds. The other two components does not depend on the number of rounds.

% The second component only depends on the total number reconciled elements, which is roughly equal to $d$. The third component, the checksum of $A$, only needs to be sent once in the first round.
%Therefore, the communication overhead of multi-round PBS is only slightly larger than that of single-round PBS when the number of rounds is small (say $3$). For example, when $d=5, n=255, |\mathcal{U}|=2^{32}$, the communication overhead of multi-round PBS of $3$ rounds is $352$ bits, which is roughly $1.3$ times of the communication overhead of single-round PBS ($272$ bits).

% Therefore, each additional round of multi-round PBS only incurs a small amount of additional communication overhead. For example, when $d=5, n=255, |\mathcal{U}|=2^{32}$, the communication overhead of single-round PBS of $272$ ($2d\log n+d\log |\mathcal{U}|+32$) bits, and each additional round incurs $40$ ($d\log n$) bits of additional communication overhead. 

% As we explained in \autoref{sec:reconcile_by_trivial}, the communication overhead in each round is proportional to the number of (remaining) distinct elements, which decreases exponentially as the number of round increase (i.e., the first round reconciles $90\%$ of distinct elements, the second round reconciles $90\%$ of the remaining $10\%$ distinct elements, etc.). So the majority of the communication overhead (i.e., $\approx 90\%$) is in the first round. Therefore, we do not bother to optimize parameters (i.e., smaller $n$) in later rounds to save tiny communication overhead, even though remaining distinct elements become fewer and can be reconciled using smaller $n$;

% The termination condition of multi-round PBS is that all distinct elements are reconciled, which may require many rounds. In most applications, a high percentage of reconciliation (e.g., $>99\%$ distinct elements are reconciled) is good enough. Therefore, we add another termination condition on the maximum number of rounds (denoted as $r$). The larger $r$ is, the higher percentage of distinct elements will be reconciled. How to set parameters based on $r$ will be elaborated in \autoref{sec:parameter_settings};

% Multi-round means multiple round-trip delays. {\bf Thanks for the piecewise decodability of PBS, in almost all practical application scenarios, this tradeoff does not lead to longer response time because the reconciliation of objects identified by the successfully decodable codewords, which constitute the vast majority of all codewords, can run in parallel with the transmissions and decodings of the rest.  In other words, the piecewise decodability effective masks the slightly larger number of communication rounds as far as the response time is concerned.}

\begin{comment}
==============================

The pseudocode of set reconciliation operations in each round is shown as follows:

\IncMargin{1em}
\begin{algorithm}
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
\Input{$A$ and $B^{(in)}$}
\Input{Set of reconciled distinct elements $D^{(in)}$}
\Output{$B^{(out)}$}
\Output{Set of reconciled distinct elements $D^{(out)}$}

% Hash-partition $A^{(in)}$, $B^{(in)}$ into $\{A^{(in)}_i\}_{i=1}^n$, $\{B^{(in)}_i\}_{i=1}^n$ (\autoref{sec:hash_partition})\label{step:hash_partition}\;

% Encode $\{A^{(in)}_i\}_{i=1}^n$, $\{B^{(in)}_i\}_{i=1}^n$ into parity bitmaps (\autoref{sec:parity_bitmap_encoding})\;


% Find those subset pairs (denoted them as $(A^{(in)}_{i_1}, B^{(in)}_{i_1}), ...,(A^{(in)}_{i_k}, B^{(in)}_{i_k})$) that parity bits differ (\autoref{sec:BCH_code})\;

Run single-round PBS on $A$ and $B^{(in)}$ to obtain the (partial) set difference $\mathcal{D}$\label{step:reconcile} \;

$D^{(out)} \leftarrow D^{(in)}\bigcup \mathcal{D}$\label{step:updated}\;

$B^{(out)} \leftarrow B^{(in)}\Delta\mathcal{D}$\label{step:updateb}\;

Check whether the set reconciliation is complete by comparing $A$ to $B^{(out)}$ (via CRC)\label{step:termination}\;

\caption{Set reconciliation operations of PBS in each round} \label{proto:multirounds}
\end{algorithm}\DecMargin{1em}

In \autoref{proto:multirounds}, the output $B^{(out)}$ in the $r^{th}$ round is the input $B^{(in)}$ in the $(r+1)^{th}$ round. $D^{(in)}$ and $D^{(out)}$ have the same relationship, and they denote the set of reconciled distinct elements before and after a round. $B^{(in)}$ and $D^{(in)}$ are initialized as $B$ and $\emptyset$ respectively. We omit the currect number of round $r$ in \autoref{proto:multirounds}, since the operations in different rounds are exactly the same. Due to the same reason, we only elaborate the operations in the first round: First, Alice and Bob reconcile $A$ and $B^{(in)}$ $(=B)$ using single-round PBS and Bob obtains the (partial) set difference $\mathcal{D}$ (\autoref{step:reconcile}); Second, Bob updates the set of reconciled distinct elements by merging it with $\mathcal{D}$ (\autoref{step:updated}); Third, Bob updates $B^{(in)}$ $(=B)$ to $B^{(out)}$ as \autoref{step:updateb} shows, such that (1) The reconciled distinct elements in $\mathcal{D}$ that are contained in $A\Delta B^{(in)}$ are not longer contained in $A\Delta B^{(out)}$; and (2) The distinct elements that are not successfully reconciled remain in $A\Delta B^{(out)}$ and can be reconciled in later rounds; Finally, we check whether all distinct elements are reconciled. Note that if it is true, $B^{(out)}$ should be the same as $A$ and multi-round PBS should terminate. We use a $32$-bit CRC (Cyclic Reduncancy Check) to check if $B^{(out)}=A$ in our evaluation. {\bf To achieve higher confidence, we can certainly use longer CRC (e.g., 64-bit). }

{\bf Remarks:}

(1) In each round, hash-partition in \autoref{sec:hash_partition} uses different hash functions, so that the remaining distinct elements from the last round will be hashed into different subset pairs with high probability;

(2) A straightforward approach to discard reconciled distinct elements is to remove them from both $A$ and $B$. This approach however incurs additional communication overhead to update $A$, since only Bob learns the partial set difference in \autoref{step:reconcile}. Therefore, we use the approach in \autoref{step:updateb} that only updates $B$. It has another benefit in \autoref{step:termination}, which only needs to transmit the CRC of $A$ from Alice to Bob in the first round. In the later rounds, \autoref{step:termination} can be checked locally by Bob and does not require any additional communication overhead;

(3) As we explained in \autoref{sec:reconcile_by_trivial}, the communication overhead in each round is proportional to the number of remaining distinct elements, which decreases exponentially as the number of round increase (i.e., the first round reconciles $90\%$ of distinct elements, the second round reconciles $90\%$ of the remaining $10\%$ distinct elements, etc.). So the majority of the communication overhead (i.e., $\approx 90\%$) is in the first round. Therefore, we do not bother to optimize parameters (i.e., smaller $n$) in later rounds to save tiny communication overhead, even though remaining distinct elements become fewer and can be reconciled using smaller $n$;

(4) One termination condition of Multi-round PBS is $B^{(out)}=A$, which refers that all distinct elements are reconciled. In most applications, a high percentage of reconciliation (e.g., $>99\%$ distinct elements are reconciled) is good enough. Therefore, we add another termination condition of the maximum number of rounds (denoted as $r$). The larger $r$ is, the higher percentage distinct elements will be reconciled, and the smaller $n$ is required. How to set parameters (e.g., $n$) based on $r$ will be elaborated in \autoref{sec:parameter_settings};

(5) Multi-round means multiple round-trip delays. {\bf Thanks for the piecewise decodability of PBS, in almost all practical application scenarios, this tradeoff does not lead to longer response time because the reconciliation of objects identified by the successfully decodable codewords, which constitute the vast majority of all codewords, can run in parallel with the transmissions and decodings of the rest.  In other words, the piecewise decodability effective masks the slightly larger number of communication rounds as far as the response time is concerned.}

==============================

\end{comment}

% (3) Readers may wonder in the later rounds, most distinct elements should be reconciled, and the rest distinct elements could be reconciled using degraded parameters (i.e., smaller $n$ and $t$). In fact, degrade parameters in later rounds cannot save much communication overhead, since the majority of it is spent in the first round (i.e., $>90\%$). Therefore, we use the same parameters (i.e., $n,t$) among all rounds in multi-rounds PBS;

% (4) The number of remaining distinct elements decreases exponentially as the number of round increase (i.e., the first round reconciles $90\%$ of distinct elements, the second round reconciles $90\%$ of the remaining $10\%$ distinct elements, etc.). 
% (4) The termination condition of Multi-rounds PBS is $B^{(out)}=A$ to reconcile all distinct elements. In some applications,  


% The output $B^{(out)}$ in the $r^{th}$ round is the input $B^{(in)}$ in the $(r+1)^{th}$ round. $D^{(in)}$ and $D^{(out)}$ are similarly defined. $B^{(in)}$ and $D^{(in)}$ are initialized as $B$ and $\emptyset$ respectively. Since and $D$ are updated in each round, so we use $B^{(in)}$ to denote the input and $B^{(out)}$ to denote the output respectively.  Specifically, in the first round, we initialize $B^{(in)}$ and $D^{(in)}$ as $B$ and $\emptyset$ respectively. we first use the single-round scheme 

% Then we run our (single-round) scheme on the updated two sets (i.e., after removing reconciled distinct elements) using a different (independent) hash-partition function from previous rounds, so that the rest distinct elements are hashed into different subset pairs (i.e., the ideal case) with high probability. At the end of each round, we check whether the set reconciliation is complete (i.e., all distinct elements are found) by computing the bitwise \code{XOR} of the remaining elements in $A$ and $B$ 
 

% This {\bf multi-rounds} scheme can significantly increase the success probability (i.e., the probability that all distinct elements are reconciled). Readers may wonder in the later rounds, most distinct elements should be reconciled, and the rest distinct elements could be reconciled using degraded parameters (i.e., smaller $n$ and $t$). In fact, degrade parameters in later rounds cannot save much communication overhead, since the majority of it is spent in the first round (i.e., $>90\%$). Therefore, we use the same parameters (i.e., $n,t$) among all rounds in our evaluation. 
% %The tradeoff between the number of rounds and the communication overhead per rounds will be elaborated in \autoref{sec:tail_bound}. In our evaluation, $r=2,3$ rounds are enough to achieve an extremely high success probability. 

% Readers may think the cost (i.e., communication overhead and the computational complexity) of this multi-rounds scheme is proportional to the number of rounds (denoted as $r$) and increases linearly with $r$. In fact, the cost of each round is roughly proportional to the number of remaining distinct elements, which decreases exponentially as $r$ increases (i.e., the first round reconciles $99\%$ of distinct elements, the second round reconciles $99\%$ of the remaining $1\%$ distinct elements, etc.). So the cost of this multi-rounds scheme is only slightly larger than that of the single-round scheme. Furthermore, as we explained in \autoref{sec:intro}, {\bf from intro thanks for the piecewise decodability of our solution, in almost all practical application scenarios, this tradeoff does not lead to longer response time because the reconciliation of objects identified by the successfully decodable codewords, which constitute the vast majority of all codewords, can run in parallel with the transmissions and decodings of the rest.  In other words, the piecewise decodability effective masks the slightly larger number of communication rounds as far as the response time is concerned.} 

\begin{comment}

\subsection{Baseline Scheme}\label{subsec:protocol1} 

Note that the set difference $A\Delta B$ can contain more than 1 elements (i.e., $d>1$), and \autoref{alg:trivial_case} cannot reconcile $A$ and $B$ directly in this case. Therefore, we propose a baseline scheme building upon~\autoref{alg:trivial_case} that also works when $d>1$: First, we partition the element universe $\mathcal{U}$ into $n$ sub-universes $\mathcal{U}_1, \mathcal{U}_2, \cdots, \mathcal{U}_n$. Denote $A_i \triangleq A\bigcap \mathcal{U}_i$ and $B_i \triangleq B\bigcap \mathcal{U}_i$ for $i=1,2,\cdots,n$. Then $\{A_i\}_{i=1}^n$ and $\{B_i\}_{i=1}^n$ are partitions of $A$ and $B$ respectively. Furthermore, $\Phi\triangleq\{A_i\Delta B_i\}_{i=1}^n$ is a partition of $A\Delta B$. 

Assume the {\bf ideal case} happens, in which each subset pair $(A_i, B_i)$ contains at most one distinct element ({\it i.e.,} $|A_i\Delta B_i|\!\leq\!1$), we use \autoref{alg:trivial_case} to reconcile each subset pair and obtain $A_i\Delta B_i$ for $i=1,2,\cdots,n$. The overall set difference $A\Delta B$ is simply their union $\bigcup_{i=1}^n \big{(}A_i\Delta B_i\big{)}$. 

In the first step of the baseline scheme, we can use a hash function $h(\cdot): \mathcal{U}\rightarrow \{1,2,\cdots,n\}$ to partition the universe $\mathcal{U}$ into $n$ sub-universes: $\mathcal{U}_i=\{s\mid s\in \mathcal{U} \mbox{ and } h(s)=i\}$ for $\forall i=1,2,\cdots,n$. And the hash function $h(\cdot)$ can be predetermined between Alice and Bob and does not require additional communication cost.

This hash-partition can be modeled as a {\it balls-into-bins problem}, in which the distinct elements are viewed as balls and the subset pairs are viewed as bins. The hash-parition basically throws (hashes) $d$ balls (distinct elements) uniformly and randomly into $n$ bins (subset pairs). The aforementioned ideal case in this context becomes, after throwing $d$ balls uniformly and randomly into $n$ bins, each bin receives at most 1 ball (i.e., $d$ nonempty bins have 1 ball in each and the rest $n-d$ bins are empty). {\bf It may remind readers about the Birthday problem. And the ideal case can be analogous to the case that no people share the same birthday.} The ideal case happens with a probability of $p=\frac{n\,!}{(n-d)\,!n^d}\!=\!\prod_{k=1}^{d - 1}(1 - \frac{k}{n})\!\approx\! e^{-\frac{d(d-1)}{2n}}$ when $d\!\ll\!n$. In other words, $n$ must be $\Omega(d^2)$ to ensure the ideal case happens with a nontrivial probability.  Note that the communication overhead of the baseline scheme is proportional to $n$, as each subset pair requires communication of a bitwise \code{XOR} in \autoref{alg:trivial_case}. So this communication overhead increases at least quadratically as $d$ increases. 

In fact, this communication overhead can be significantly reduced: In the ideal case, $n-d$ out of $n$ subset pairs are identical ones, and only $d (\ll n)$ out of $n$ subset pairs contain distinct elements (one distinct element in each of the $d$ subset pairs) and need to be reconciled. If we can identify these $d$ subset pairs (with a tiny additional communication overhead) and only reconcile them, the overall communication overhead will be significantly reduced from $\Omega(d^2)$ to $O(d)$. Based on this intuition, we propose our scheme in \autoref{sucsec:our-scheme}, which uses Parity Bitmap Sketch (PBS) and Error Correction Coding (ECC) to identify those subset pairs with a tiny additional communication overhead. 

Note that the ideal case does not always happen. However, we can ensure that the ideal case happens with high probability by properly selecting $n$ based on $d$ (i.e., $n=\Omega(d^2)$). Furthermore, as we will describe in \autoref{subsec:nonideal}, even if the ideal case does not happen (i.e., some distinct elements are hashed into the same subset pair), most of the distinct elements should be distributed into different subset pairs and therefore can be reconciled. So the baseline scheme, even cannot reconcile all of the distinct elements, can still reconcile the majority of them. Based on this property, we will extend our scheme from single-round to multi-rounds in \autoref{subsec:nonideal} to further increase the probability of reconciling all distinct elements. 

For general cases ({\it i.e.,} $t=|A\Delta B|$ is an arbitrary number), we have a straightforward strawman scheme building upon~\autoref{alg:trivial_case}, which works as follows: First, Alice and Bob choose some hash function $h(s): \mathcal{U} \rightarrow \{0,1,\cdots,2^{32}-1\}$ to partition $A$ and $B$ into $m$ subsets $A_1,A_2,\cdots,A_m$ and $B_1,B_2,\cdots,B_m$ respectively:

\begin{align}
s\in A_i & \mbox{ iff } s\in A \mbox{ and } h(s)=i\!\mod m, \nonu{}mber\\
s\in B_i & \mbox{ iff } s\in B \mbox{ and } h(s)=i\!\mod m. \nonumber
\end{align} 

{\bf call a subset pair -> partition?} Since Alice and Bob use the same hash function for partition, common elements (i.e., elements in $A\cap B$) are always hashed into the same subset pair $(A_i, B_i)$. And the set difference of each subset pair only contains distinct elements (i.e., elements in $A\Delta B$): $A_i\Delta B_i \subset A\Delta B$. In the ideal case, with a sufficient large $m$, each subset pair $(A_i, B_i)$ contains at most one distinct element ({\it i.e.,} $|A_i\Delta B_i|\!\leq\!1$). Then \autoref{alg:trivial_case} can reconcile each subset pair and obtain $A_i\Delta B_i$ for $i=1,2,\cdots,m$. The overall set difference $A\Delta B$ is simply their union $\bigcup_{i=1}^m \big{(}A_i\Delta B_i\big{)}$. The selection of hash function $h(s)$ can be predetermined between Alice and Bob and it does not require additional communication cost.

%To make sure Alice and Bob use the same hash function for partition, we let them pre-agree on some universal hash family (e.g., \code{xxHash}~\cite{Collet_xxHashExtremelyfast_}) and a common selection order, and each time they choose a hash function from the family in the same order. Note that we can also let Alice generates a hash function and send it to Bob. The hash function that Alice and Bob choose for partition can be either generated by 

This hash-partition is in nature a {\it balls-into-bins model}. We can view the distinct elements as balls and the subset pairs as bins. The hash-parition basically throws (hashes) $t$ balls (distinct elements) uniformly and randomly into $m$ bins (subset pairs). The aforementioned ideal case in this context is, with a sufficient large number of bins, each bin receives at most 1 ball. The strawman scheme works correctly if and only if the ideal case happens, which has a probability of $\frac{m\,!}{(m-t)\,!m^t}\!=\!\prod_{k=1}^{t - 1}(1 - \frac{k}{m})\!\approx\! e^{-\frac{t(t-1)}{2m}}$. In other words, to ensure the strawman scheme works correctly with a probability of $p$, it roughly requires $m \!=\!\lceil \frac{t(t-1)}{-2\ln p}\rceil$ subset pairs. 

Note that the communication overhead of this strawman scheme is proportional to the number of subset pairs $m$, as each subset pair requires communication of an \code{XOR} sum in \autoref{alg:trivial_case} during the reconciliation. When $t$ is small, a small communication cost can guarantee that the strawman scheme works correctly with high probability. For instance, when $t=5$, $m=95$ subset pairs are sufficient for the strawman scheme to work correctly with a probability of $90\%$. However, when $t$ is relatively large, it requires a huge communication cost to ensure the strawman scheme works correctly. For instance, when $t=1,000$, it requires $m=4,740,865$ subset pairs to guarantee a success probability of $90\%$. 

In fact, the majority of subset pairs are identical ones and do not need to reconcile. And only a small portion of them contain distinct elements. If we can identify those subset pairs that contain distinct elements and only reconcile them, the communication cost could be significantly reduced. Our scheme is based on this intuition and uses parity bitmap sketch and BCH code to identify the subset pairs, which we will elaborate in \autoref{sucsec:our-scheme}. 

%To distribute balls as uniformly as possible and maximize the probability of the ideal case, we choose a uniform hashing function $h$ that throws balls uniformly and randomly into bins: $$\mathbb{P}[h(s)=i]=\frac{1}{m} \mbox{ for } \forall i=1,2,\cdots,m, \forall s\in U$$.

%Note that the probability of the ideal case is $\frac{m\,!}{(m-t)\,!m^t}\!=\!\prod_{k=1}^{t - 1}(1 - \frac{k}{m})\!\approx\! e^{-\frac{t(t-1)}{2m}}$. Hence, at least $\lceil \frac{t(t-1)}{-2\ln p}\rceil$ bins are required to ensure that this probability is at least $p$. In other words, to ensure that the ideal case happens with a probability of $p$, the strawman scheme roughly requires $m \!=\!\lceil \frac{t(t-1)}{-2\ln p}\rceil$. For example, suppose $t\!=\!$\num{1000}, %and $p\!=\!0.01$, this strawman scheme roughly requires $m\!=\!$\num{720626} bins (partitions) to ensure that $|A_i\Delta B_i|\!\leq\!1$ (for any $i=1,2,\cdots,m$) holds with probability $50\%$.  

% A straightforward strawman scheme building upon~\autoref{alg:trivial_case} 
% to reconcile two sets $A$ and $B$ in general 
% ({\it i.e.,} $|A\Delta B|$ is an arbitrary number) is the following: 
% Uniformly randomly partition $A$ and $B$ into $m$ subsets ($A_1,A_2,\cdots,A_m$ 
% and $B_1,B_2,\cdots,B_m$) so that the set difference 
% $A_i\Delta B_i$ of each subset pair $(A_i, B_i)$ contains at most one element 
% ({\it i.e.,} $|A_i\Delta B_i|\!\leq\!1$) {\it w.h.p.} ({\it i.e.,} with high probability), 
% and then reconcile each subset pair with~\autoref{alg:trivial_case}. 

% Now let us analyze this strawman scheme using the {\it balls-into-bins model}. 
% Assume that sets $A$ and $B$ have $t$ elements in their set difference, {\it i.e.,} $|A\Delta B|\!=\!t$. 
% These $t$ elements can be viewed as $t$ balls and the $m$ partitions (subset pairs) can be viewed as 
% $m$ bins. The random partition process in this strawman scheme can be modeled as throwing 
% $t$ balls into $m$ bins in the following manner: Each ball goes into a 
% uniformly random bin and independently of other balls. %so that each bin contains at most one ball, {\it w.h.p.}  
% The probability that each bin contains at most one ball is  
% $\frac{m\,!}{(m-t)\,!m^t}\!=\!\prod_{k=1}^{t - 1}(1 - \frac{k}{m})\!\approx\! e^{-\frac{t(t-1)}{2m}}$. 
% Hence, at least $\lceil \frac{t(t-1)}{-2\ln p}\rceil$ bins are required 
% to ensure that this probability is at least $p$. In other words, to ensure 
% that each bin contains at most one ball with a probability of $p$, 
% the strawman scheme roughly requires $m \!=\!\lceil \frac{t(t-1)}{-2\ln p}\rceil$. 
% For example, suppose $t\!=\!$\num{1000}, %and $p\!=\!0.01$, 
% this scheme roughly requires $m\!=\!$\num{108469} bins (partitions) to 
% ensure that $|A_i\Delta B_i|\!\leq\!1$ (for any $i=1,2,\cdots,m$) holds with probability $0.01$.  

% We note that the communication overhead of this strawman scheme is proportional to 
% $m$ ($\!\gg\! t$), as each partition (subset pair) requires communication of an \code{XOR} sum during the reconciliation. 
% This communication overhead is much higher than that of the optimal scheme, which only requires 
% to exchange the elements in the set difference (assuming an oracle tells it which elements belong to 
% the set difference), {\it i.e.,} proportional to $t$. In the example above, assuming each element takes 4 bytes, 
% the communication overhead of the strawman scheme is $4m$ bytes ($\!\approx\! \num{423.71}\,$KB) to ensure 
% a success rate of only 0.01 ({\it i.e.,} with a probability of $0.0.1$, all elements in 
% the set difference are successfully reconciled), 
% which is approximately 2 orders of magnitude higher than $4t$ bytes ($\!=\!\num{3.90}\,$KB), the communication 
% overhead of the optimal scheme. 

\subsection{Our Scheme: The Preliminary Version}\label{sucsec:our-scheme}

Like the baseline scheme, our scheme also hash-partitions the two sets $A$ and $B$ into $n$ subset pairs. The difference is, instead of reconciling all subset pairs using \autoref{alg:trivial_case}, our scheme identifies the subset pairs that contains distinct elements and only reconciles them. Since the hash-partition and set reconciliation on each subset pair using \autoref{alg:trivial_case} have been described in \autoref{subsec:protocol1}, we only elaborate how to identify the subset pairs that contain distinct elements in this section. 

The general idea of identification is very simple: First, we {\bf encode} each subset into $1$ bit, such that in the ideal case, for $\forall i=1,2,\cdots,n$:

\begin{itemize}
	\item The codewords (bits) of $A_i$ and $B_i$ are different if and only if subset pair $(A_i, B_i)$ contains $1$ distinct element;
	\item The codewords (bits) of $A_i$ and $B_i$ are the same if and only if subset pair $(A_i, B_i)$ contains no distinct element;
\end{itemize}

Second, we {\bf compare} the codewords of each subset pair. And the subset pairs that contain distinct elements are the ones with different codewords (bits). We will describe the two steps in details in \autoref{sec:parity_bitmap_encoding} and \autoref{sec:BCH_code} respectively.

\subsubsection{Parity Bitmap Encoding}\label{sec:parity_bitmap_encoding}

In our scheme, we use {\it parity encoding} to encode each subset into a parity bit. More specific, it encodes a subset as ``1'' if it contains odd number of elements, and as ``0'' otherwise. And it satisfies the aforementioned requirements in the ideal case:

\begin{itemize}
	\item If subset pair $(A_i, B_i)$ contains $1$ distinct element, the corresponding two subsets $A_i$ and $B_i$ differ exactly one element, which implies that $||A_i|\!-\!|B_i||\!=\!1$. Hence, if $|A_i|$ ({\it i.e.,} number of elements in $A_i$) is odd (or even), then $|B_i|$ must be even (or odd). And the parity bits of $A_i$ and $B_i$ will be different;
	\item If subset pair $(A_i, B_i)$ contains no distinct element, the corresponding two subsets $A_i$ and $B_i$ should be the same and therefore contain the same number of elements. Hence, if $|A_i|$ is odd (or even), then $|B_i|$ must be odd (or even). And the parity bits of $A_i$ and $B_i$ will be the same;
\end{itemize}

Using parity encoding, the $n$ subsets of $A$ are encoded as a bit string $A[1..n]$ in $\{0,1\}^n$, 
where the $i$-th bit $A[i]$ in $A[1..n]$ corresponds to the parity encoding bit of $A_i$. Similarly, the $n$ subsets of $B$ are similarly 
encoded as a bit string $B[1..n]$. We call $A[1..n]$ ($B[1..n]$) the {\it parity bitmap} of $\{A_i\}_{i=1}^n$ ($\{B_i\}_{i=1}^n$). In the ideal case, $A[1..n]$ and $B[1..n]$ differ at $d$ different bit-positions, which corresponds to the $d$ subset pairs that contain distinct elements. And our scheme only reconciles those subset pairs that the parity bits are different. We will describe the nonideal case (i.e., some subset pair contains more than 1 distinct elements) in \autoref{subsec:nonideal}.

\subsubsection{Parity Bitmap Comparison Using BCH Code}\label{sec:BCH_code}

A straightforward approach to compare the parity bitmaps is to let Bob send the complete parity bitmap $B[1..n]$ to Alice, then Alice compares $A[1..n]$ with $B[1..n]$ locally. This approach has a communication overhead of $n$ bits, which is unnecessarily high. As we discussed in~\autoref{subsec:protocol0}, $d$ is usually much smaller than $n$. It means $A[1..n]$ and $B[1..n]$ differ only at a tiny portion of bits. Therefore, we can view $A[1..n]$ as a corrupted message of $B[1..n]$ with $d$ corrupted bits, and the bit-positions of the $d$ corrupted bits basically correspond to the $d$ subset pairs that contain distinct elements. The detection of corrupted bits, on the other hand, can be solved by Error-Correction Code (ECC)~\cite{Lin_ErrorControlCoding_1983}. And our scheme uses BCH code~\cite{Lint_IntroductionCodingTheory_1998} to encode the parity bitmap and detect the $d$ corrupted bits.

More specific, after the parity bitmap encoding, Bob uses a $d$-error-correcting systematic BCH code to encode $B[1..n]$ into an $n+d\log n$ codeword, in which the first $n$ bits are $B[1..n]$ (property of systematic BCH code). Then Bob sends the rest $d\log n$ bits, which we denote as {\it parity bitmap sketch (PBS)}, to Alice. Upon the received PBS and $A[1..n]$ (corrupted message), Alice uses the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} to detect the $d$ corrupted bits in $A[1..n]$. The communication overhead of this approach is $d\log n$ bits (i.e., length of PBS), which is much smaller than that of the straightforward approach ($n$ bits, when $d\!\ll\!n$). On the other hand, the computational complexity of the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} is $O(d^2\log^2 n)$. 

\subsubsection{Exceptional Handling and Multi-rounds}\label{subsec:nonideal}

As we described in \autoref{subsec:protocol1}, the ideal case does not always happen, which means some subset pair may contain more than 1 distinct elements and cannot be successfully reconciled by \autoref{alg:trivial_case}. Due to the parity encoding, we can classify such subset pair into the following two scenarios:

\begin{itemize}
    \item Scenario 1: If a subset pair $(A_i, B_i)$ contains even number ($\geq 2$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be the same and our scheme will not reconcile the subset pair. Hence, the distinct elements in the subset pair will not be reconciled;
    \item Scenario 2: If a subset pair $(A_i, B_i)$ contains odd number ($\geq 3$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be different and our scheme will reconcile the subset pair using \autoref{alg:trivial_case}. However, as we described in \autoref{subsec:protocol0}, when a subset pair contains more than 1 distinct elements, \autoref{alg:trivial_case} will output the bitwise \code{XOR} of them as the `distinct element', which is not a real distinct element with high probability;
\end{itemize}

In both scenarios, the distinct elements in the subset pair cannot be reconciled. Even worse, in the second scenario, a false-positive could happen (i.e., the output of \autoref{subsec:protocol0} is not a real distinct element). However, as we will analyze in \autoref{sec:tail_bound} and show in {\bf the evaluation section}, the second scenario barely happens both theoretically and empirically. To further reduce the chance of false-positives, we add a verification step at the end of \autoref{subsec:protocol0} to check whether the output of \autoref{subsec:protocol0} $s$ is a real distinct element or not. The verification step works as follows: Given the output $s$ of subset pair $(A_i,B_i)$, if $s\in\mathcal{U}_i$ (i.e., $h(s)=i$), we consider $s$ as a real distinct element; Otherwise, we consider $s$ as an incorrect output and discard it. 

Note that if $s$ is a real distinct element of $(A_i,B_i)$, $s$ must be in sub-universe $\mathcal{U}_i$. However, if $s$ is the bitwise \code{XOR} of the distinct elements in $(A_i,B_i)$ (i.e., the second scenario happens), $s$ could be in any sub-universe other than $\mathcal{U}_i$. In fact, if we assume the hash-partition described in \autoref{subsec:protocol1} hashes the elements of $\mathcal{U}$ uniformly, independently, and randomly into $n$ sub-universes, the output $s$ in the second scenario will be in a different sub-universe $\mathcal{U}_j (j\neq i)$ with a high probability of $1-\frac{1}{n}$. Hence, this verfication step can reduce the chance of false-positives by a factor of $\frac{1}{n}$. 

Even if the ideal case does not happen, most of the distinct elements should be distributed into different subset pairs and therefore can be reconciled. So our scheme, even cannot reconcile all of the distinct elements, can still reconcile the majority of them (piecewise decodability). To reconcile the rest distinct elements, we can just run our scheme for another round under a different hash-partition function, so on so force. This {\bf multi-rounds} scheme can significantly increase the success probability (i.e., the probability that all distinct elements are reconciled). Readers may wonder in the later rounds, most distinct elements should be reconciled, and the remaining could be reconciled using degraded parameters (i.e., smaller $n$ and $t$). In fact, degrade parameters in later rounds cannot save much communication overhead, since the majority of it is spent in the first round (i.e., $>90\%$). Therefore, we use the same parameters (i.e., $n,t$) among all rounds in our evaluation.
%The tradeoff between the number of rounds and the communication overhead per rounds will be elaborated in \autoref{sec:tail_bound}. In our evaluation, $r=2,3$ rounds are enough to achieve an extremely high success probability. 

Readers may think the cost (i.e., communication overhead and the computational complexity) of this multi-rounds scheme is proportional to the number of rounds (denoted as $r$) and increases linearly with $r$. In fact, the cost of each round is roughly proportional to the number of remaining distinct elements, which decreases exponentially as $r$ increases (i.e., the first round reconciles $99\%$ of distinct elements, the second round reconciles $99\%$ of the remaining $1\%$ distinct elements, etc.). So the cost of this multi-rounds scheme is only slightly larger than that of the single-round scheme. Furthermore, as we explained in \autoref{sec:intro}, {\bf from intro thanks for the piecewise decodability of our solution, in almost all practical application scenarios, this tradeoff does not lead to longer response time because the reconciliation of objects identified by the successfully decodable codewords, which constitute the vast majority of all codewords, can run in parallel with the transmissions and decodings of the rest.  In other words, the piecewise decodability effective masks the slightly larger number of communication rounds as far as the response time is concerned.} 

\end{comment}


%%% Moved from related work
\input{section/pinsketch}

\section{PBS for large \texorpdfstring{\larger\boldmath\MakeLowercase{$d$}}{d}}\label{subsec:protocol2}

The scheme described above, which we refer as PBS-for-small-$d$, can also do set reconciliation when $d$ is large. However, the BCH decoding computational complexity in it is $O(d^2)$ of finite field operations even using the state-of-the-art decoding algorithm~\cite{Dodis_SyndromeEncodingDecoding_2006}, which is too expensive for large $d$. To overcome this drawback, we first consistently partition sets $A$ and $B$ each into $d/\delta$ smaller subsets (which we call {\it groups} to distinguish from subsets) for some small integer $\delta$ (say $5$). In this way, each of the group pairs contains roughly $\delta$ distinct elements. Then we apply PBS-for-small-$d$ to reconcile each group pair respectively. The BCH decoding computational complexity of each group pair is roughly $O(\delta^2)$, which can be considered as $O(1)$, since $\delta$ is a small number. As a result, the overall computational complexity is reduced from $O(d^2)$ to $O(d)$. 

% To overcome this drawback, we use the same technique in \autoref{sec:hash_partition} to hash-partition sets $A$ and $B$ each into $d/\delta$ subsets (which we call {\it groups} to distinguish from subsets) for some small integer $\delta$ (say $5$), so that each of the group pairs contains roughly $\delta$ distinct elements and can be reconciled by PBS-for-small-$d$ respectively. The BCH decoding computational complexity of each group pair is roughly $O(\delta^2)$, which can be considered as $O(1)$, since $\delta$ is a small number. As a result, the overall computational complexity is reduced from $O(d^2)$ to $O(d)$. 
%{\bf In PBS, we set $\delta = 5$. }

%Note that the BCH decoding computational complexity is $O(d^2)$ of finite field operations (in GF($2^{8}$) when $n=255$) using the state-of-the-art decoding algorithm~\cite{Dodis_SyndromeEncodingDecoding_2006}, which is too expensive for large $d$. To overcome this drawback, we first hash-partition sets $A$ and $B$ each into $d/\delta$ subsets (which we call {\it groups} to distinguish from subsets), just like what we did in \autoref{sec:hash_partition}, for some small integer $\delta$ (say $5$), then reconcile each of the group pairs by the PBS we described in \autoref{sec:scheme}. After the partition, each group pair has $\delta$ distinct elements on average. So the BCH decoding computational complexity of each group pair is roughly $O(\delta^2)$, which can be considered as a constant, since $\delta$ is a small number. As a result, the overall computational complexity of PBS is reduced from $O(d^2)$ to $O(d)$. 

%To differentiate from the PBS described in \autoref{sec:scheme}, we refer to it as PBS-basic in this section. 
We continue to assume that the number of distinct elements $d$ is precisely known. Even so, due to the randomness of hash-partition, the number of distinct elements in group pair $i$, denoted as $\delta_i$, is a random variable with mean of $\delta$ for $i=1,2,...,g$. This randomness induces a parameter tuning issue on the error-correction capability. Note that if the error-correction capability of group pair $i$, denoted as $t_i$, is larger than $\delta_i$, the corresponding BCH codeword is unnecessarily long and results in ``wastes'' on communication overhead. On the other hand, if $t_i$ is smaller than $\delta_i$, the BCH decoding would fail with high probability and result in hefty ``penalties'', as will be described in \autoref{sec:BCH_exception}. Ideally, if $\delta_i$ is precisely known, we can set $t_i$ equal to $\delta_i$ that results neither ``wastes'' or ``penalties''. However, to estimate each $\delta_i$ with high accuracy requires much larger additional communication overhead than the savings, as we will explain shortly in this section.

Our solution to this parameter tuning problem is to set a univeral error-correction capability $t$ for all group pairs. Set $t$ is a delicate issue: On one hand, $t$ should be larger than or equal to most of $\delta_i$'s for $i=1,2,...,g$, so that most of the group pairs will not encounter BCH decoding failures, and the rest of group pairs (no more than several) only incur negligible ``penalties'' on BCH decoding failures; on the other hand, $t$ should not be too large to incur huge ``waste'' on communication overhead. To find the optimal $t$ that minimizes ``wastes''+``penalties'', we establish an analytical framework for parameter settings, as will be elaborated in \autoref{sec:tail_bound} and \autoref{sec:parameter_settings}. Typically, the optimal $t$ is $1.5$ to $3.5$ times of $\delta$.

Similarly, This randomness of $\delta_i$ also induces a parameter tuning issue on the number of subset pairs in group pair $i$. For the same reason, we set a universal $n$ as the number of subset pairs in each group pair. The analytical framework that is used for finding the optimal $t$ can also be used to find the optimal $n$, as will be elaborated in \autoref{sec:parameter_settings}. 


% We continue to assume that the number of distinct elements $d$ is precisely known. Even so, due to the randomness of hash-partition, the number of distinct elements in the $i$-th group pair, denoted as $\delta_i$, is a random variable with mean of $\delta$ for $i=1,2,...,g$, which are not precisely known. Since $\delta_1, \delta_2, ..., \delta_g$ follows the same distribution, it does not make sense to select different parameters for the $g$ group pairs. Hence, we set two universal parameters, $t$ and $n$, for all group pairs, where $t$ is the error-correction capability of the BCH code used for reconciling each group pair, and $n$ is the number of subset pairs in each group pair.

% We continue to assume that the number of distinct elements $d$ is precisely known. Even so, due to the randomness of hash-partition, denoted as $\delta_i$, the number of distinct elements in the $i$-th group pair, is a Binomial random variable with mean of $\delta$ for $i=1,2,...,g$, which cannot be precisely known without a huge amount of additional communication overhead. Since $\delta_1, \delta_2, ..., \delta_g$ follows the identical Binomial distribution, it does not make sense to select different parameters for the $g$ group pairs. Hence, we set two universal parameters, $t$ and $n$, for all group pairs, where $t$ is the error-correction capability of the BCH code used for reconciling each group pair, and $n$ is the number of subset pairs in each group pair.

%To deal with this randomness, we set two global parameters, denoted as $t$, that corresponds to the error-correction capability of the BCH code used for reconciling every group pair. identical no sense or additonal info

%{\bf (modified based on the next paragraph from intro)} 
{\bf (previous) The error-correction capability $t$, defined as the maximum number of errors that the BCH code used by any group pair can correct, is a critical parameter for PBS to perform well. On one hand, if $t$ is too large (say $t=10\delta$), then the communication overhead on transmitting BCH codeword ($t\log n$ bits per group pair) is unnecessarily large; but on the other hand, {\bf if $t$ is too small (say equal to $\delta$), any group pair $i$ could contain more than $t$ distinct elements with a nontrivial probability (i.e., $Pr[\delta_i>t]$ is nontrivial). If so, in the ideal case, the $\delta_i$ distinct elements incur $\delta_i$ bit errors in the BCH codeword, which exceeds the error-correction capability $t$ and a BCH decoding failure happens (we will describe in \autoref{sec:BCH_exception}). if $t$ is too small (say equal to $\delta$), then close to half of the group pairs fail to decode the BCH codeword due to the insufficient error-correction capability, which can result in hefty penalties on BCH decoding failures (to be described in \autoref{sec:BCH_exception}). }
In PBS, we manage to make $t$ as small as possible (so that the communication overhead on transmitting BCH codewords is kept to a minimum) yet pay negligible penalties of BCH decoding failures. }


% To ensure the error-correction capability $t$ is sufficient (i.e., $t\geq \delta_i$ for $i=1,2,...,g$) for every group pair with high probability, we set $t$ conservatively and leave a sufficient `safety margin' between $t$ and the average number of distinct elements in each group pair $\delta$. 

% Note that the `safety margin' between $t$ and $\delta$ incurs additional communication overhead on transmitting BCH codeword: In the perfect scenario (i.e., $\{d_i\}_{i=1}^g$ is precisely known), the average communication overhead on transmitting BCH codeword per group pair is $\delta\log n$; On the other hand, when we set $t$ to be the error-correction capability for each group pair, the average communication overhead becomes $t\log n$. If we set the `safety margin' to be too large (say $t=10\delta$), it will incur huge additional communication overhead. Due to this reason, we set a moderate `safety margin' that  $t$ in the range from $1.5\delta$ to $3\delta$. 

% {\bf (moved from intro, to be removed)} The number of elements in the set difference between any group pair is in general not a constant.  Rather, it is a random variable that has roughly a Poisson distribution with mean $\delta$.  The potential issue arises from dealing with this randomness in setting a global parameter that corresponds to the error-correction capability of the BCH code used for reconciling every group pair.  This parameter, denoted as $t$ (consistent with other literatures on BCH code), is the maximum number of errors that the BCH code used by any group pair can correct, and the size of each such codeword is roughly $8t$ bits (assuming $n = 255$ as explained above). The issue is that, on one hand, if $t$ is too large (say several times larger than $\delta$), then the total size of the BCH codewords, which is the bulk of the extra communication cost, is unnecessarily large; but on the other hand, if $t$ is too small (say equal to $\delta$), then close to half of the BCH codewords cannot decode or worse decode incorrectly (unknown to Alice and Bob), which can result in hefty penalties in the latter case of incorrect decoding.   In PBS, we manage to make $t$ as small as possible (so that the total size of the BCH codewords is kept to a minimum) yet pay negligible penalties of incorrect BCH decoding.
%We will discuss the case that $d_i>t$ in \autoref{sec:BCH_exception}.

% Hence, we can no longer set the error-correction capability of the BCH code for each group pair based on the exact number of distinct element in it, as we did in \autoref{sec:scheme}. Instead, we set a conservative error-correction capability $t$ (say $2.5\delta$) for all group pairs, which is sufficient for them (i.e., $t\geq d_i$ for $i=1,2,...,g$) with high probability. We will discuss the case that $d_i>t$ in \autoref{sec:BCH_exception}.


% ===============================
% To differentiate from the PBS described in \autoref{sucsec:our-scheme}, we refer it as PBS-basic in this section. Note that the BCH decoding computational complexity is $O(d^2\log ^2 n)$, which is $\Omega(d^2\log^2 d)$ when $n=\Omega(d^2)$, with the state-of-the-art decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019}. It is too large in PBS-basic for large $d$. To overcome this drawback and generalize PBS-basic for large $d$, we partition sets $A$ and $B$ each into $d/\delta$ subsets (which we call {\it groups} to distinguish from subsets) for some small integer $\delta$ (say $5$) and reconcile the $d/\delta$ group pairs respectively using PBS-basic. After this partition, each group has $\delta$ distinct elements on average. The BCH decoding computational complexity of each group pair can be considered as $O(1)$, since $\delta$ is a small number. As a result, the overall computational complexity of PBS is reduced from $O(d^2\log ^2 n)$ to $O(d)$. 

% % To differentiate from the PBS described in \autoref{sucsec:our-scheme}, we refer it as PBS-basic in this section. PBS-basic is not suitable for large $d$ for two reasons: First, its communication overhead is asymptotically $O(d\log n)\!=\!O(d\log d)$ (since $n=\Omega(d^2)$), which is not asymptotically optimal. Second, the decoding computational complexity is proportional to $d^2$ with the state-of-the-art decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} for BCH codes, which is too high when $d$ is large. To overcome these two drawbacks, we use a simple algorithmic trick to (1) reduce the communication overhead from $O(d\log d)$ to $d\log u \!+\! O(d)$; (2) reduce the decoding computational complexity from $O(d^2)$ to $O(d)$. 

% Now, we describe the generalized PBS in details: In the first step, we hash-partition $A$ and $B$ (by some hash function $h_1(\cdot)$) into $g$ group pairs, just like what we did in \autoref{sucsec:our-scheme}. The objective of this partition is however different: In \autoref{sucsec:our-scheme}, we aim to ensure each subset pair contains at most $1$ distinct element (i.e., the ideal case) with high probability; Here we aim to make each group pair contains roughly $\delta$ distinct elements for some small constant $\delta$ (say $5$) by setting $g=d/\delta$. 
% %To differentiate the $g$ subset pairs here from those in \autoref{sec:hash_partition}, we call them the $g$ {\bf groups} in the sequel. 
% In the second step, we just apply PBS-basic (described in \autoref{sucsec:our-scheme}) to reconcile each group pair and obtain the distinct elements. 
% ================================

% To differentiate from the PBS described in \autoref{sucsec:our-scheme}, we refer it as PBS-basic in this section. When $d$ is large (more than several), we hash-partition set $A$ and $B$ into groups, such that each group pair contains $\delta$ distinct elements on average for small $\delta$ (say $5$), as described in \autoref{sec:larged}. Then each group pair can be reconciled by PBS-basic.

% When describing the PBS-basic in \autoref{sucsec:our-scheme}, we assume that the number of distinct elements is precisely known. We set the error-correction capability of the BCH code (denoted as $t$) just enough to correct $d$ errors (i.e., $t=d$). However, due to the randomness of hash-partition, $d_i$, the number of distinct elements in the $i^{th}$ group pair, is a Binomial random variable $Binomial(d,1/g)$ with expectation of $\delta$ $(=d/g)$ for $i=1,2,...,g$, which cannot be precisely known without a huge amount of additional communication overhead. Hence, we can no longer set the error-correction capability of the BCH code for each group pair based on the exact number of distinct element in it, as we did in \autoref{sucsec:our-scheme}. Instead, we set a universal error-correction capability $t$ (say $2.5\delta$) for all group pairs, which is sufficient for all group pairs (i.e., $t\geq d_i$ for $i=1,2,...,g$) with high probability. We will discuss the case that $d_i>t$ in \autoref{sec:BCH_exception}.

%This assumption in general does not hold: 
% Let $d_i$ denote the number of distinct elements in Group $i$. Due to the property of hash-partition, each $d_i$ is a Binomial random variable $Binomial(d,1/g)$ with expectation of $\delta$ $(=d/g)$. Even if $d$ is precisely known, each $d_i$ is not. To ensure the error-correction capability $t$ is sufficient for each group (i.e., $d_i\leq t$) with high probability, we leave some safety margin for the randomness of $d_i$ and conservatively set $t$ roughly $2.5\delta$ (the factor $2.5$ varies depend on other parameters, which will be discussed in \autoref{sec:parameter_settings}), so that $Pr[d_i>t]$ is tiny. We will discuss the case that $d_i>t$ in \autoref{sec:BCH_exception}.

% Note that the `safety margin' between $t$ and $\delta$ incurs additional communication overhead on transmitting BCH codeword: In the perfect scenario (i.e., $\{d_i\}_{i=1}^g$ is precisely known), the average communication overhead on transmitting BCH codeword per group pair is $\delta\log n$; On the other hand, when we set $t$ to be the error-correction capability for each group pair, the average communication overhead becomes $t\log n$. If we set the `safety margin' to be too large (say $t=10\delta$), it will incur huge additional communication overhead. Due to this reason, we set a moderate `safety margin' that  $t$ in the range from $1.5\delta$ to $3\delta$. 

%which is roughly $2.5$ times of that in the perfect scenario (when $t$ is roughly $2.5\delta$). Due to this addition
One alternative is to estimate each $\delta_i$ and then set $t_i$ to be very close to (slightly larger) the estimation of $\delta_i$. It can save considerate communication overhead on transmitting the BCH code. However, to estimate all the $g$ values of $\{\delta_i\}_{i=1}^g$ in high accuracy requires much larger additional communication overhead than the savings. For instance, estimating each $\delta_i$ requires $288$ bytes of additional communication overhead using the ToW estimator, as we will describe in \autoref{subsec:ToW}. However, the ``savings'' on the communication overhead is typically no more than a few dozens of bytes.
%However, the ``savings'' on the communication overhead for group pair $i$ is no more than a few dozens of bytes.


\subsection{Communication overhead of PBS Per Group Pair}\label{sec:communication_overhead_single_PBS}

%To correct $d$ bit errors, the length of the net-codeword only is no more than $d\log n$ bits. 
Since each group pair is reconciled by PBS-for-small-$d$, the communication overhead of PBS of group pair $i$ in the first round corresponds to the steps in \autoref{alg:single_round_pbs}, which consists of the following four components: 
\begin{itemize}
	\setlength\itemsep{0.1em}
	\item The BCH codeword with error-correction capability $t$ that is $t\log n$ bits (\autoref{step:BCH_encode} in \autoref{alg:single_round_pbs});
	\item The subset pair indices (\autoref{step:send_xor} in \autoref{alg:single_round_pbs}) that are roughly $\delta_i\log n$ bits;
	\item The bitwise \code{XOR} sums (\autoref{step:send_xor} in \autoref{alg:single_round_pbs}) that are roughly $\delta_i\log |\mathcal{U}|$ bits;
	\item The checksum (\autoref{step:terminate_condition} in \autoref{alg:single_round_pbs}) that is $\log |\mathcal{U}|$ bits;
\end{itemize}

Since $\delta_i$ is a random variable with mean of $\delta$ for $i=1,2,...,g$, the average communication overhead of PBS per group pair in the first round is roughly 

\begin{equation}\label{eq:communication_overhead}
t\log n + \delta\log n +\delta \log |\mathcal{U}|+\log |\mathcal{U}|
\end{equation}

Formula \autoref{eq:communication_overhead} also roughly equals to the average communication overhead of PBS per group pair in all rounds, since the bulk of the communication overhead happens in the first round, as will be explained in \autoref{sec:piecewise_decodability}.

{\bf (previous)} the BCH codeword $\xi_A$ in \autoref{step:BCH_encode}; (2) the subset pair indices $i_1,i_2,...,i_d$ in \autoref{step:trivial_reconcile}; (3) the bitwise \code{XOR} sums of sets $B_{i_1}, B_{i_2},...,B_{i_d}$ of $d\log |\mathcal{U}|$ bits in \autoref{step:trivial_reconcile}; and (4) transmit the $32$-bit checksum of $B$ (i.e., $c(B)$) from Bob to Alice for precomputing $c(A\Delta B)$ in \autoref{step:terminate_condition}. These four components contribute roughly (1) $d\log n$ bits (recall that to ``correct'' $d$ bit errors, the length of the BCH codeword is no more than $d\log n$ bits); (2) $d\log n$ bits; (3) $d\log |\mathcal{U}|$ bits; and (4) $32$ bits respectively to the overall communcation overhead of \autoref{alg:single_round_pbs}. 
\noindent {\bf Communication overhead of PBS Per Group Pair in the first round:} Same as PBS-for-small-$d$, the communication overhead of PBS per group pair in the first round also consists of the four components described in \autoref{sec:communication_overhead_single_PBS}. The expectation of the communication overhead of each component equals to the corresponding component of PBS-for-small-$d$ when $d=\delta$, except for the BCH codeword, which is $t\log n$ bits as we described earlier. The communication overhead of PBS per group pair in the first round on average is roughly

% \begin{equation}\label{eq:communication_overhead}
% t\log n + \delta\log n +\delta \log |\mathcal{U}|+32
% \end{equation}

% {\bf (previous)} Readers may wonder if we can reduce this additional communication overhead by using some technique to estimate $\{d_i\}_{i=1}^g$ (e.g., ToW estimator in \autoref{subsec:ToW}), so that we can set the error-correction capability of each group more wisely and save some waste on the safety margin. However, to achieve that, the estimation on $\{d_i\}_{i=1}^g$ must be in extremely high precision (since $\{d_i\}_{i=1}^g$ are small numbers with mean of $\delta$), which incurs much larger additional communication overhead than the savings. Due to the same reason (i.e., estimate $\{d_i\}_{i=1}^g$ is costly), we set the number of subset pairs for each group pair to be all equal (denoted as $n$). 
%based on $\delta$ ($n=\Omega(\delta^2)$). 

% {\bf (moved from the small d case)} Note that the set reconciliation process of the group pairs are independent with each other, and each group pair runs as many rounds of PBS-for-small-$d$ as needed to reconcile all distinct elements in it. Therefore, different group pairs may need different number of rounds to be successfully reconciled. Intuitively, we want all group pairs to be successfully reconciled in only a few rounds (say $3$) with high probability (say $99\%$). Hence, when tuning parameters (to be discussed in \autoref{sec:parameter_settings}), we set a {\it target success probability} $p_0$ combined with a {\it target number of rounds} $r$ as the {\it paramenter setting requirement}, which aims to ensure that the {\it success probability}, the probability that all distinct elements (of all group pairs) are reconciled, within $r$ rounds to be at least $p_0$. 
% {\bf Normally, to achieve the same target success probability within fewer rounds (smaller $r$), PBS need more resources (e.g., larger $n$, $t$) for the ideal case happening with higher probability (fewer exceptions happen and need to be handled in later rounds), as we will explain in \autoref{sec:vary_r}.}

% {\bf (moved from the small d case)} Although PBS runs as many rounds as needed to reconcile all distinct elements (in each group pair), we want PBS to successfully reconcile all distinct elements in only a few rounds (say $3$) with high probability (say $99\%$). Hence, when tuning parameters (to be discussed in \autoref{sec:parameter_settings}), we set a {\it target success probability} $p_0$ combined with a {\it target number of rounds} $r$ as the {\it paramenter setting requirement}, which aims to ensure that the {\it success probability}, the probability that all distinct elements are reconciled, within $r$ rounds to be larger than $p_0$. 
% {\bf Normally, to achieve the same target success probability within fewer rounds (smaller $r$), PBS need more resources (e.g., larger $n$, $t$) for the ideal case happening with higher probability (fewer exceptions happen and need to be handled in later rounds), as we will explain in \autoref{sec:parameter_settings}.}

%This success probability (within $r$ rounds) is also the expected value of the {\it success rate} of PBS, which is defined as the number of `successful' experiments (all distinct elements are successfully reconciled within $r$ rounds) divided by the total number of experiments. 

%The requirement above should also ensure the majority of the distinct elements are reconciled in the first round. 
% Note that PBS reconciles the distinct elements gradually round by round. The distinct elements that have been reconciled in the first round are no longer needed to be reconciled again in later rounds. This is the ``piecewise decodability'' mentioned in \autoref{sec:intro_oursolution}. The requirement above also ensures the majority of the distinct elements are reconciled in the first round, as we will show in \autoref{sec:piecewise_decodability}. Therefore, the majority of the overall communication overhead happens in the first round. In other words, the overall communication overhead of all rounds is only slightly larger than ($1.01$ to $1.07$ times of) that in the first round. Due to this reason, we use the communication overhead in the first round (described in \autoref{sec:communication_overhead_single_PBS}) to approximate the overall communication overhead of all rounds in parameter settings (to be elaborated in \autoref{sec:parameter_settings}.


% Like what we did in \autoref{sec:multi-rounds}, we set a paramenter setting requirement on the target success probability $p_0$ of $r$ rounds for all group pairs, which ensures the probability that all group pairs are completely reconciled in $r$ rounds to be larger than $p_0$. The detail about how to set $n$, $g$, and $t$ given such a success probability requirement will be elaborated in \autoref{sec:parameter_settings}. 

% we set a {\it target success probability} $p_0$ of $r$ rounds as a paramenter setting requirement, which aims to ensure the probability that all distinct elements are reconciled in $r$ rounds to be larger than $p_0$. This requirement should also ensure the majority of the distinct elements are reconciled in the first round. Use the same example ($d=5, n=255$), on average $4.81$ out of $5$ distinct elements should be reconciled in the first round. So the total communication overhead in all rounds is only slightly larger than ($1.01$ to $1.07$ times of, as we will show in \autoref{fig:per-round-con}) that in the first round. Due to this reason, we use the communication overhead in the first round (described in \autoref{sec:communication_overhead_single_PBS}) to approximate the total communication overhead of all rounds in parameter settings (to be elaborated in \autoref{sec:parameter_settings}.

% Note that this safety margin incurs additional communication overhead on transmitting BCH codeword: In the perfect scenario (i.e., $\{d_i\}_{i=1}^g$ is precisely known), the average communication overhead on transmitting BCH codeword per group is $\delta\log n$; On the other hand, when we set $t$ to be the error-correction capability for each group, then the average overhead becomes $t\log n$, which is roughly $2.5$ times of that in the perfect scenario (when $t$ is roughly $2.5\delta$). Readers may wonder if we can reduce this additional communication overhead by using some technique to estimate $\{d_i\}_{i=1}^g$ (e.g., ToW estimator in \autoref{subsec:ToW}), so that we can set the error-correction capability of each group more wisely and save some waste on the safety margin. However, to achieve that, the estimation on $\{d_i\}_{i=1}^g$ must be in high precision, which requires a much higher communication overhead than the savings.

% Although PBS may need to run many rounds to reconcile all distinct elements, the communication overhead mostly happens in the first round, since the majority of the distinct elements should be reconciled in the first round. Use the same example ($d=5, n=255$), on average $4.81$ out of $5$ distinct elements should be reconciled in the first round. So the total communication overhead in all rounds is only slightly larger than ($1.01$ to $1.07$ times of, to be shown in \autoref{fig:per-round-con}) that in the first round. Due to this reason, we use the communication overhead in the first round (described in \autoref{sec:communication_overhead_single_PBS}) to approximate the total communication overhead (all rounds) in parameter settings (to be elaborated in \autoref{sec:parameter_settings}).

%For the moment, we assume no ``fake'' distinct element in type (\RN{2}) subset pairs fails to be detected, which happens with overwhelming probability as explained in \autoref{subsec:exception_hash_partition}. Then 

% PBS reconciles the distinct elements gradually round by round. This is the ``piecewise decodability'' mentioned in \autoref{sec:intro_oursolution}. We use the following example to describe it in details: 
% Given two sets with $10$ distinct elements, in the first round, PBS tries to reconcile the $10$ distinct elements and say $6$ out of the $10$ distinct elements are successfully reconciled. Then the $6$ reconciled distinct elements are removed and PBS tries to reconcile the remaining $4$ distinct elements in the second round. Say $2$ out of the $4$ remaining distinct elements are successfully reconciled, and that leaves $2$ remaining distinct elements to be reconciled in the third round, so on so force. 
% % Given two sets $A$, $B$ with $10$ distinct elements, in the first round, PBS hashes them into $7$ distinct subset pairs. $6$ distinct elements are hashed into $6$ distinct subset pairs, and the other $4$ distinct elements are hashed into the same subset pair. Then the former $6$ distinct elements are successfully reconciled in the first round and the later $4$ distinct elements remain to be reconciled in the second round, which are hashed into $3$ distinct subset pairs (under a different hash function). $2$ remaining distinct elements are hashed into $2$ distinct subset pairs, and the other $2$ remaining distinct elements are hashed into the same subset pair. Then the former $2$ remaining distinct elements are successfully reconciled in the second round and the later $2$ remaining distinct elements remain to be reconciled in the third round, so on so force. 
% The dynamics of the number of remaining distinct elements (i.e., $10\leadsto 4\leadsto 2\leadsto \cdots$ in the example) is in nature a Markov chain, which will be elaborated and analyzed in \autoref{sec:single_markov} to derive a tight tail bound of the probability that all distinct elements are reconciled in $r$ rounds. 

%, which we will show in \autoref{subsec:mini-partition}.

% The same algorithmic trick can also be implemented in PinSketch~\cite{Dodis_PinSketch_2008} to reduce it computational complexity from $O(d^2)$ to $O(d)$. However, it will encounter the same randomness problem and have to set up a safety margin on the error-correction capability. This safety margin will incur much more communication overhead on PinSketch than on our scheme: Considering the average communication overhead per group, in our scheme, this overhead can be expressed as $t\log n+\delta\log n+\delta \log u+32$, in which $t\log n$ accounts for the BCH codeword, $\delta\log n$ accounts for the index of the subset pairs, $\delta \log u$ accounts for the bitwise \code{XOR} in \autoref{alg:trivial_case}, and $32$ accounts for the $32$-bit CRC in \autoref{proto:multirounds}. In PinSketch, this overhead increases from $O(\delta\log u)$ (optimal) to $O(t\log u)$ (PinSketch does not need to transmit bitwise \code{XOR}) if it uses the same algorithmic trick. Use the same example in \autoref{sec:intro}, when $\delta=5, n=255, u=2^{32}, t=2.5\delta$, the overhead of PinSketch using the trick is $2.5$ times of the optimal, while that of our scheme is $2.075$ times of the optimal (as we introduced in \autoref{sec:intro_oursolution}). That means our scheme has a lower communication overhead than PinSketch if they both use the algorithmic trick. Furthermore, as the signiture size $\log u$ increases, the advantage of our scheme over PinSketch becomes more significantly, which we will show in \autoref{subsec:mini-partition}.

% In PinSketch, each bit encodes only a single element in the universe, so the size of the bitmap is equal to the size of the universe.  
% For example, in the set reconciliation problem we usually assume each element is ``indexed" by a $32$-bit-long (hash) signature, so the universe contains a total of $2^{32}$ elements. In this case, the bitmap encoding for any set in PinSketch is $2^{32}$ bits long, and the Galois field involved in its BCH decoding is the ``$32$-bit-wide" $GF(2^{32})$.  In contrast, as explained earlier, in PBS 
% %since each bit encodes the oddness or evenness of the cardinality of a subset,   
% the size $n$ of a bitmap is dependent only on $d$, and not on the size of the universe or on the cardinality of the set the bitmap encodes.   For example, as shown in the example above, $n = 255$ is large enough for $d = 5$.  In this case, the BCH decoding operates in the much shorter
% ``8-bit-wide" $GF(2^{8})$.  This shorter ``width" alone in theory translates into roughly $16$ times shorter BCH decoding time, which as will be explained in~\ref{} grows quadratically with the ``width" of the underlying Galois field.  This shorter ``width" also implies four times shorter BCH codeword in PBS than in PinSketch, resulting in lower communication complexity as will be shown in~\autoref{}.

% Note that our scheme only takes 1 round trip delay to both identify the $d$ subset pairs and reconcile them: In the first half, Bob computes and sends PBS to Alice. Then Alice locally identifies the $d$ subset pairs and then initiates the reconciliation ({\it i.e.,} \autoref{alg:trivial_case}) for them, {\it i.e.,} computes the bitwise \code{XOR} of the corresponded $d$ subsets. In the second half, Alice sends the bitwise \code{XOR} of the $d$ subsets with their indexes to Bob. Then Bob can compute the set difference $A\Delta B$ locally.


% We can certainly use some communication-efficient technique to estimate $d_i$ (e.g., \autoref{subsec:ToW}). However, to obtain $d_i$ precisely will require a communication cost almost as large as to reconcile Group $i$. So instead of obtaining $d_i$ and set $c_i$ (i.e., the error-correction capability of Group $i$) equal to $d_i$, we leave the randomness of $d_i$ and set $c_i$ neither too conservative, nor too libertive in the following sense: (1) $c_i$ is not too big (conservative, i.e., $10\delta$) to make the total size of PBS unnecessarily large and incur too much extra communication overhead; (2) $c_i$ is not too small (libertive, i.e., $\delta$) to incur a high probability of insufficient decode capability, which can result in hefty penalties in the latter case of incorrect decoding (will be elaborated in \autoref{sec:BCH_exception}). In our scheme, we set $c_i$ to be $2-3$ times of $\delta$, which will be shown in \autoref{sec:tail_bound} that it is just enough to make the probability of decode failure very small. Meanwhile, we set the error-correction capability of each group ($c_1,c_2,...,c_k$) to be all equal and denote it as $c$. 

%Since the decoding capacity $t$ and the number of subset pairs for each group $n$ are both small constants independent of $d$, therefore, the communication overhead per group is $t\cdot\log n \!=\!O(1)$, which implies a total communication overhead of $O(d)$. Similarly, the total decoding computational complexity is also $O(d)$. 

% \subsection{Exception Handling}\label{sec:exceptions}

% \subsubsection{Exception Handling on Hash-Partition}\label{subsec:exception_hash_partition}

% As we have described in \autoref{sec:hash_partition}, the ideal case does not always happen, which means some subset pair may contain more than 1 distinct elements and cannot be successfully reconciled by \autoref{alg:trivial_case}. Due to the parity encoding, we can classify such subset pair into the following two scenarios:

% \begin{itemize}
%     \item Scenario 1: If a subset pair $(A_i, B_i)$ contains even number ($\geq 2$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be the same and our scheme will not reconcile the subset pair. Hence, the distinct elements in the subset pair will not be reconciled;
%     \item Scenario 2: If a subset pair $(A_i, B_i)$ contains odd number ($\geq 3$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be different and our scheme will reconcile the subset pair using \autoref{alg:trivial_case}. However, as we described in \autoref{subsec:protocol0}, when a subset pair contains more than 1 distinct elements, \autoref{alg:trivial_case} will output the bitwise \code{XOR} of them as the `distinct element', which is not a real distinct element with high probability;
% \end{itemize}

% In both scenarios, the distinct elements in the subset pair cannot be reconciled. Even worse, in the second scenario, a false-positive could happen (i.e., the output of \autoref{subsec:protocol0} is not a real distinct element). For example, if subset pair $(A_i, B_i)$ contains $3$ distinct elements $s_1, s_2, s_3$, then the output of \autoref{alg:trivial_case} is $\tilde{s}_4=s_1\oplus s_2\oplus s_3$, which is normally not a distinct element. The good thing is, the probability of the false-positive is extremely small for small $d$. For instance, if $d=5$ and $n=255$, the probability of the false-positive is $7.6\times 10^{-6}$, which is very small. To further reduce the chance of false-positives, we add a verification step at the end of \autoref{subsec:protocol0} to check whether the output of \autoref{subsec:protocol0} $s$ is a real distinct element or not. The verification step works as follows: Given the output $s$ of subset pair $(A_i,B_i)$, if $s\in\mathcal{U}_i$ (i.e., $h(s)=i$), we consider $s$ as a real distinct element; Otherwise, we consider $s$ as an incorrect output and discard it. 

% Note that if $s$ is a real distinct element of $(A_i,B_i)$, $s$ must be in sub-universe $\mathcal{U}_i$. However, if $s$ is the bitwise \code{XOR} of the distinct elements in $(A_i,B_i)$ (i.e., the second scenario happens), $s$ could be in any sub-universe other than $\mathcal{U}_i$. In fact, if we assume the hash-partition described in \autoref{sec:hash_partition} hashes the elements of $\mathcal{U}$ uniformly, independently, and randomly into $n$ sub-universes, the output $s$ in the second scenario will be in a different sub-universe $\mathcal{U}_j (j\neq i)$ with a high probability of $1-\frac{1}{n}$. Hence, this verfication method can further reduce the probability of false-positives by a factor of $\frac{1}{n}$. Use the same example (i.e., $d=5$, $n=255$), the probability is reduced from $7.6\times 10^{-6}$ to $3\times 10^{-8}$ by this verification method. 

% In some super critical cases (i.e., no false-positive is allowed), we can use a more powerful verification method to completely eliminate false-positives. That is, to check if the output $s$ exists in exactly one of the two sets (i.e., $s\in A\setminus B$ or $s\in B\setminus A$). To do so, Bob transmits $s$ along with an identification bit $\mathbb{1}_{\{s\in B\}}$ to Alice, then Alice checks if $s$ . This method verification costs $d(\log u+1)$ bits of additional communication overhead. In most applications, rigorously $0\%$ probability of false-positives is unnecessary and the probability of the former verification method is small enough, so we use the former verfication method in our evaluation. Based on our observation, the false-positive does not happen even once in our evaluation using the former verfication method.

\subsection{Exception Handling on BCH Decoding}\label{sec:BCH_exception}

There is an additional type of exceptions that arises only from setting the universal error-correction capability $t$. That is, when $\delta_i$ (i.e., the number of distinct elements in group pair $i$) is larger than the error-correction capability $t$, the BCH codewords of group pair $i$ could differ at more than $t$ bit positions (e.g., in the ideal case, the BCH codewords differ at exactly $\delta_i$ bit positions), which exceeds the error-correction capability $t$. If so, the BCH decoder cannot decode the bit errors correctly (\autoref{step:BCH_decode} in \autoref{alg:single_round_pbs}) and report a failure. This exception happens with a small probability in each group pair: For example, when $d=1000$, and $\delta$ is set to $5$ (so that $g=d/\delta=200$), and $t$ is set to $13$ ($2.6$ times of $\delta$), the probability that this exception happens is only $6.7\times 10^{-4}$. 

% The exceptions that happens when the error-correction capability $t$ is sufficient have been discussed and handled in \autoref{subsec:exception_hash_partition} and \autoref{sec:multi-rounds}. In this section, we only discuss the exceptions that are caused by insufficient error-correction capability. That is, when $\delta_i$ (i.e., the number of distinct elements in group pair $i$) is larger than the error-correction capability $t$, the BCH codewords of group pair $i$ differ at $\delta_i$ bit positions in the ideal case, which exceeds the error-correction capability $t$. If so, the BCH decoder cannot decode the bit errors correctly (\autoref{step:BCH_decode} in \autoref{alg:single_round_pbs}) and report a failure. This exception happens with a small probability in each group pair: For example, when $d=1000$, and $\delta$ is set to $5$ (so that $g=d/\delta=200$), and $t$ is set to $13$, the probability that this exception happens is only $6.7\times 10^{-4}$. 

To handle this type of exceptions, we further partition each trouble-causing group pair (say group pair $i$) into $3$ sub-group-pairs and reconcile them respectively using PBS-for-small-$d$. Note that $\delta_i$ is a Binomial random variable with mean of $\delta$, $t$ is typically $1.5$ to $3.5$ times of $\delta$. Even conditioned upon the event $\{\delta_i>t\}$, $\delta_i$ should be only slightly larger than $t$ with high probability. Hence, after partitioning the $\delta_i$ distinct elements into $3$ sub-group-pairs, each of them should have no more than $t$ distinct elements with overwhelming probability: For example, when $\delta=5$, $t=13$ $(2.6\delta)$, the probability that some sub-group contains more than $t$ distinct elements conditioned upon the event $\{\delta_i>t\}$ is $9.5\times 10^{-10}$.  More specifically, \autoref{alg:3_way_partition} is triggered when BCH decoding fails in \autoref{step:BCH_decode} in \autoref{alg:single_round_pbs}.

{\bf (previous)} To handle this type of exceptions, we further partition each trouble-causing group pair into $3$ sub-group-pairs and reconcile them respectively using PBS-for-small-$d$. 
%Note that $\delta_i$, if is not smaller, should be only slightly larger than $t$ with high probability. Hence, partitioning into $3$ sub-groups is enough to ensure each sub-group has no more than $t$ distinct elements. 
Note that $\delta_i$ is a Binomial random variable with mean of $\delta$, $t$ is typically $1.5$ to $3.5$ times of $\delta$. So the probability that some sub-group contains more than $t$ distinct elements conditioned upon $\delta_i>t$ is tiny. 
In the same example above ($d=1000$, $\delta=5$, $t=13$), this conditional probability is $9.5\times 10^{-10}$.%that some sub-group has more than $t$ distinct elements is $9.5\times 10^{-10}$. 
In the next round, each sub-group-pair will hardly encounter this type of expections and can be reconciled by PBS-for-small-$d$ respectively.  More specifically, we add a termination condition of \autoref{alg:3_way_partition} after \autoref{step:BCH_decode} in \autoref{alg:single_round_pbs}.

\begin{algorithm}
\caption{Termination condition when BCH decoding fails}
\label{alg:3_way_partition}

\If{BCH decoding fails\label{step:if1}}
{Hash-partition the group pair into $3$ sub-group-pairs and run PBS-for-small-$d$ for each of them in the next round; Break;}\label{step:term1} 

\end{algorithm}

% Back to the \autoref{proto:multirounds}, which shows the set reconciliation operations in each round of PBS-basic, this kind of exceptions only affect \autoref{step:reconcile} in \autoref{proto:multirounds}. Now this step needs to check whether BCH decoding is successful or not: If successful, all the operations remain the same; Else, we hash-partition the group ($A$ and $B$) into $3$ sub-groups and reconcile them respectively using \autoref{proto:multirounds}. 
% {\bf I'm not sure if it is necessary to discuss this case, since PinSketch did not mention it, even it may happen in PinSketch}
% Another type of exceptions that happens when $d_i>t$ is, the BCH decoder mistakes the decoding is successful and returns $t$ incorrectly decoded bit errors (i.e., subset pairs). The probability of this type of exceptions is very small. For instance, when $d=1000, \delta=5, t=13$ $(2.5\delta)$, $d_i>t$ happens with probability roughly $6.7\times 10^{-5}$, and the probability that the BCH decoder mistakes the decoding is successful when $d_i>t$ is on the order of $10^{-7}$ \cite{kim1996undetected}. So the probability that this type of exceptions happens in each group is on the order of $10^{-12}$. On the other hand, the impact of this type of exceptions is insignificant. Assume an incorrectly decoded bit error corresponds to a random subset pair, which could contain (1) no distinct element; (2) exactly $1$ distinct element; or (3) more than $1$ distinct elements. Reconcile the subset pair using \autoref{alg:trivial_case} could (1) get nothing and waste $\log |\mathcal{U}|$ bits of communication overhead; (2) get an actual distinct elements; or (3) trigger the exceptions that were discussed and handled in \autoref{subsec:exception_hash_partition}. 

\subsection{What if PinSketch also uses partitions?}

Arguably, the same algorithmic trick (i.e., hash-partition two sets each into groups) can also be implemented in PinSketch~\cite{Dodis_PinSketch_2008} to reduce it computational complexity from $O(d^2)$ (of finite field operations in GF($2^{32}$)) to $O(d)$. However, it will encounter the same randomness problem and have to set up a ``safety margin'' on the error-correction capability $t$. This ``safety margin'' will incur much more additional communication overhead on PinSketch than on our scheme: Considering the average communication overhead per group pair, the additional overhead caused by the ``safety margin'' is $(t-\delta)\log n$ in PBS and $(t-\delta)\log |\mathcal{U}|$ in PinSketch. The latter is roughly $4$ times of the former when $n=255, |\mathcal{U}|=2^{32}$. Recall that the theoretical minimum amount of communication overhead to reconcile $\delta$ distinct elements is $\delta\log |\mathcal{U}|$. Use the same example in \autoref{sec:intro}, when $\delta=5, n=255, |\mathcal{U}|=2^{32}, t=2.5\delta$, the overhead of PinSketch using the algorithmic trick is $2.5$ times of the theoretical minimum, while that of PBS is $2.075$ times of the theoretical minimum. It means PBS could have a lower communication overhead than PinSketch if they both use the algorithmic trick. {\bf Furthermore, as the signiture length $\log |\mathcal{U}|$ increases, the advantage of PBS over PinSketch will be more significant.}

% We handle this type of exceptions by the same method (i.e., hash-partition into $3$ sub-groups) as above. To detect them, on the other hand, is simple: Note that incorrect decoded bit errors correspond to the subset pairs that do not contain distinct elements. When we reconcile those subset pairs in \autoref{sec:reconcile_by_trivial}, the output (i.e., reconciled elements) will be $\mathbf{0}$, which is abnormal (since $\mathbf{0}\notin A\bigcup B$, as we described in \autoref{subsec:protocol0}). Hence, this type of exceptions happen if and only if one of the reconciled distinct elements is $\mathbf{0}$. 
%Hence, we consider BCH decoding is successful by two criteria: (1) the BCH decoder reports a successful decode; and (2) None of the reconciled elements is $\mathbf{0}$. 
% ========================
% In fact, even if $d_i>t$, PBS-basic is still possible to reconcile group $i$ in some nonideal cases. For example, when $t=10$ and $d_i=11$, if the $11$ distinct elements are distributed in $10$ subset pairs, such that $1$ subset pair contains $2$ distinct elements and $9$ subset pairs contain $1$ distinct element in each, the two parity bitmaps differ at only $9$ bit positions. So BCH decoder is able to decode the later $9$ subset pairs and the corresponding $9$ distinct elements can be reconciled. In the second round, only $2$ distinct elements remain and BCH decoding certainly works. In this case, we do not need to partition the group into sub-groups, and this case does not trigger \autoref{alg:3_way_partition} in PBS. 
% ========================
% Instead, it will either (1) report a failure about exceeding the error-correction capability; or (2) mistake the decoding is successful and return incorrect decoded bit errors. 

% The second case happens with a very small probability (in order of $10^{-7}$ \cite{kim1996undetected}) and is very simple to detect : 

% The first case is easy to handle: We can simply adapt the same algorithmic trick to partition the group into smaller groups and reconcile them respectively. In our scheme, we set the number of smaller groups to be $3$, which is big enough because $d_i$, if not smaller, only slightly larger than $t$ with high probability. The second case on the other hand, although theoretically possible, happens with a very small probability when $d_i>t$ (in order of $10^{-7}$ \cite{kim1996undetected}). Besides, the probability of $d_i>t$ is also very small (e.g., when $t=15$ and $\delta=5$, this probability is about $2.3\times 10^{-4}$), so the overall probability of the second case, which is the multiplication of these two small numbers, is negligible (e.g., in order of $10^{-11}$).

% \subsection{Multi-rounds}

% Even if the ideal case does not happen, most of the distinct elements should be distributed into different subset pairs and therefore can be reconciled. So our scheme, even cannot reconcile all of the distinct elements, can still reconcile the majority of them (piecewise decodability). To reconcile the rest distinct elements, we can just run our scheme for multi-rounds under different hash-partition functions. For each round, our scheme works as follows: 

% \IncMargin{1em}
% \begin{algorithm}
% \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
% \Input{Two sets $A$ and $B$}
% \Input{Size of set difference $d$}
% \Input{The number of subset pairs $n$}
% \Input{BCH error-correction capability $t$}

% Hash-partition $A$ and $B$ into $n$ subset pairs $\{(A_i,B_i)\}_{i=1}^n$;

% \If{BCH decoding fails}
% 	Hash-partition $A$ and $B$ into $3$ subset pairs and reconcile them respectively in the next round\;
% \ElseIf{BCH decoding success}
	
% \Else{}

% $k \leftarrow \lceil \frac{t}{c}\rceil $\;

% Partition elements into $k$ subsets using~\autoref{alg:random-part}\;

% \For{$j = 0$ \KwTo $k-1$}{
%     Reconcile the $j$-th subset pair using the straw-man scheme with the BCH correcting capability $\tau$, number of smaller subsets $m$, and number of rounds $r$\;
% }

% \caption{PBS (per round)} \label{proto:II}
% \end{algorithm}\DecMargin{1em}

% This {\bf multi-rounds} scheme can significantly increase the success probability (i.e., the probability that all distinct elements are reconciled). Readers may wonder in the later rounds, most distinct elements should be reconciled, and the remaining could be reconciled using degraded parameters (i.e., smaller $n$ and $t$). In fact, degrade parameters in later rounds cannot save much communication overhead, since the majority of it is spent in the first round (i.e., $>90\%$). Therefore, we use the same parameters (i.e., $n,t$) among all rounds in our evaluation. 
% %The tradeoff between the number of rounds and the communication overhead per rounds will be elaborated in \autoref{sec:tail_bound}. In our evaluation, $r=2,3$ rounds are enough to achieve an extremely high success probability. 

% Readers may think the cost (i.e., communication overhead and the computational complexity) of this multi-rounds scheme is proportional to the number of rounds (denoted as $r$) and increases linearly with $r$. In fact, the cost of each round is roughly proportional to the number of remaining distinct elements, which decreases exponentially as $r$ increases (i.e., the first round reconciles $99\%$ of distinct elements, the second round reconciles $99\%$ of the remaining $1\%$ distinct elements, etc.). So the cost of this multi-rounds scheme is only slightly larger than that of the single-round scheme. Furthermore, as we explained in \autoref{sec:intro}, {\bf from intro thanks for the piecewise decodability of our solution, in almost all practical application scenarios, this tradeoff does not lead to longer response time because the reconciliation of objects identified by the successfully decodable codewords, which constitute the vast majority of all codewords, can run in parallel with the transmissions and decodings of the rest.  In other words, the piecewise decodability effective masks the slightly larger number of communication rounds as far as the response time is concerned.} 





\begin{comment}
\subsubsection{Random Partition}

\IncMargin{1em}
\begin{algorithm}
% \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
% \Input{Set $S$}
% \Input{The number of subsets $m$ for partition}
% \Output{Subsets $S_1, S_2, ..., S_m$}

% Generate hash function $h(\cdot)$ that maps each element into $\{1,2,...,m\}$;

\ForEach{$s \in S$}{
    $j \leftarrow h(s) \bmod m$\;    
    Insert $s$ into the $j$-th subset $S_j$\;
}

\caption{Partition using hash function $h(\cdot)$.} \label{alg:random-part}
\end{algorithm}\DecMargin{1em}

Like the strawman scheme, our scheme randomly partitions sets $A$ and $B$ into $m$ subsets. This random partition 
can be easily accomplished by using some hash function, $h(\cdot)$, and inserting each element $x$ into the subset 
corresponding to $h(x)$. \autoref{alg:random-part} presents the pseudo-code of this random partition using hash 
function $h(\cdot)$.  

% Unlike the strawman scheme, our scheme only reconciles those subset pairs that need to be reconciled, 
% because 



Like the strawman scheme, our scheme hash-partitions the two sets $A$ and $B$ into $m$ subset pairs $(A_i, B_i)$ for $i=1,2,\cdots,m$. 
We note that, among those $m$ bins (subset pairs), 
at most $t$ ($t\!\ll\!m$ as shown in our analysis in~\autoref{subsec:protocol1}) bins contain balls 
(elements belonging to the set difference), {\it i.e.,} requiring reconciliation.  
Motivated by this observation, we, therefore, propose to first detect those bins that 
contain balls and then only reconcile them. The detection is solved with a simple encoding approach that 
will be detailed in the next section.

\subsubsection{Detection before Reconciliation} 

In fact, identifying those non-empty bins is easy when each bin contains at most one ball. In this section, we assume that 
each bin after the random partition contains at most one ball, we will show later how to handle the cases when some 
bins contain more than one balls later in~\autoref{subsec:exceptions}. 

Given an arbitrary bin (say subset pair $(A_i, B_i)$) that contains one ball ({\it i.e.,} $A_i\Delta B_i$ contains exactly one element), 
the corresponding two subsets $A_i$ and $B_i$ differ exactly one element, which implies that 
$||A_i|\!-\!|B_i||\!=\!1$. Hence, if $|A_i|$ ({\it i.e.,} number of 
elements in $A_i$) is odd (or even), then $|B_i|$ must be even (or odd). In other words, the odevity of $|A_i|$ 
and $|B_i|$ are opposite. %differs if $|A_i\Delta B_i|\!=\!1$. 
Based on this property, we propose the {\it odevity encoding}: 
A subset is encoded as ``1'' if it contains odd number of elements, and as ``0'' otherwise. 
Using this odevity encoding, the $m$ subsets of $A$ can be encoded as a bit string $b_A$ in $\{0,1\}^m$, 
where the $i$-th bit in $b_A$ corresponds to the odevity encoding of $|A_i|$. Similarly, the $m$ subsets of $B$ can also 
be encoded as a bit string $b_B$. Clearly, $b_A$ and $b_B$ differ at $t$ different positions, or in other words, 
the Hamming distance of bit strings $b_A$ and $b_B$ is $t$. A straightforward approach is 
to let Alice send $b_A$ to Bob, and then Bob compares $b_B$ against $b_A$ to obtain those non-empty bins. 

This approach, however, has a communication overhead of $m$ bits, which is still unnecessarily high. As 
analyzed in~\autoref{subsec:protocol0}, $t$ is usually much smaller than $m$. 
That means $b_A$ and $b_B$ differ only at a tiny portion of bits. %have much more in common than differences. 
Therefore, if we view $b_B$ as a corrupted message of $b_A$ with $t$ corrupted bits, the detection of those $t$ bins can be converted to 
the detection of the positions of the $t$ corrupted bits. The latter can be solved using an Error-Correction Code (ECC)~\cite{Lin_ErrorControlCoding_1983} that can correct up to $t$ errors. In this work, we use the BCH code~\cite{Lint_IntroductionCodingTheory_1998}. 
More precisely, this ECC-based approach (with the BCH code) works as follows. 
Alice computes the parity bits for $b_A$ using a $t$-error-correcting BCH code with a block length of 
$(2^{\lceil \log m\rceil} -1)$ and sends the parity bits to Bob. Bob then decodes the positions of the $t$ corrupted bits 
using the BCH decoding algorithm with $b_B$ and those parity bits received from Alice. The communication overhead of 
this approach is roughly $t\lceil \log m\rceil$ ($=O(t\log t)$) bits. In the example above, this communication overhead is 
roughly $\num{17000}$ bits, which is approximately $6$ times lower 
than $m\!=\!\num{108469}$ bits, the communication overhead of the aforementioned straightforward approach. 

At first sight, it seems that the detection of non-empty bins and reconciliation of subsets in those bins require two rounds 
(or at least two round trip delays), {\it i.e.,} one round for detection and the other for reconciliation. In fact, 
it only requires one. After Bob receives the parity bits from Alice and decodes out those non-empty bins, it initiates 
the reconciliation ({\it i.e.,} \autoref{alg:trivial_case}) for each bin (subset pair) immediately, 
{\it i.e.,} sends the \code{XOR} sums of subsets in those bins together the indexes of those bins. 
After receiving those \code{XOR} sums and bin indexes, Alice can compute the set difference. 

% A naive way to combine the detection of non-empty bins and reconciliation of subset pairs in those bins is to first detect 
% those non-empty bins via one round of message exchanges between Alice and Bob and then to reconcile the corresponding 
% subset pairs in those bins with another round of message exchanges. This requires two rounds ({\it i.e.,} taking at least 
% two round trip delays). In fact, after Bob receives the parity bits from Alice and obtains those 

\subsubsection{Multiple Rounds}\label{sec:multiround}

{\bf This section was not clear enough. I need more time to think about and revise it.}


In the above section, we have assumed that each bin contains at most one ball. 
However, even with a sufficient large $m$, some bin might contain more than one balls though with tiny probability. 
We will show in~\autoref{subsec:exceptions}, how such rare events, {\it i.e.,} one bin contains more than one balls, 
can be easily detected.
To ensure our scheme can successfully reconcile all elements even when such rare events happen, 
we propose to use multiple rounds (of communication between Alice and Bob). More precisely, instead of 
selecting a prohibitively large $m$ to ensure that each bin contains at most one ball with a extremely high probability 
(say 0.99999), we select a reasonably large $m$ so that the communication overhead is not very high and very few bins contain 
more than one balls (or in other words, most bins contain at most one ball). Therefore, after running one round of 
our scheme, most elements in the set difference will be reconciled. Only those in the bins that contain more than one balls 
fail to be reconciled. For elements in the subsets corresponding to those bins, we run another round of our scheme. 
If some elements still fail to be reconcile, we can run one more round of our scheme. So on so forth,  
our scheme can keep running for more rounds until all elements are reconciled. 

With the same communication overhead, multiple rounds can significantly increase the success rate, 
{\it i.e.,} the probability that all elements in the set difference will be successfully reconciles, 
which will be elaborated in~\autoref{sec:tail_bound}. 

% % to be emphasized
% % say that too many rounds should be avoided (latency & communication overhead reduction is negligible when r is too large, 2 - 3 is good enough)
% % multiple rounds is not an issue when r is small

% We note that the number of rounds $r$, however, should not be large. On one hand, it results in large latency (at least $r$ round trip delays). 
% On the other hand, when $r$ is large, the reduction of communication overhead by the increase of $r$ gradually diminishes. 

We note that multiple rounds, when $r$ is small, would not really increase the ``latency'', as long as most elements in the 
set difference can be reconciled in the first rounds, since the underlying synchronization of data objects corresponding to 
those elements can start immediately after the first round of our scheme. Therefore, the actual latency is one round trip delay instead of 
$r$. 

As we mentioned, this straw-man protocol works correctly if each subset pair has at most one exclusive element (i.e., \autoref{eq:requirement_strawman} holds). On the other hand, if a subset pair has more than one exclusive elements, some of which will not be successfully reconciled:

\begin{itemize}
\item If a subset pair has even number of exclusive elements, Odevity coding will encode it as 0. Then the straw-man scheme will consider the subset pair having no exclusive element and all exclusive elements in this subset will not be reconciled;

\item If a subset pair has odd number ($\geq 3$) of exclusive elements, Odevity coding will encode it as 1 and consider the subset pair having only 1 exclusive element. Then the straw-man scheme will use \autoref{alg:trivial_case} to decode only one exclusive element and dismiss all others. Even worse, the only decoded element is probably not a real exclusive element, since the element computed by \autoref{alg:trivial_case} is the \code{XOR} sum of all exclusive elements, not one of them. 
\end{itemize}

In summary, if a subset pair has more than one exclusive elements, most of its exclusive elements cannot be reconciled, and the reconciled element is usually incorrect (i.e., false-positive). The false-positive however is easy to check, which will be elaborated in \autoref{subsec:exceptions}. The good thing is, even if not all subset pairs have at most one exclusive element and are successfully decoded, most of them will be w.h.p.. In other words, even if the straw-man protocol cannot reconcile all exclusive elements, it still can reconcile most of them. To reconcile all exclusive elements w.h.p., we can simply extend the single-round straw-man scheme to multi-round. And each round adapts the straw-man scheme to do set reconciliation using independent hashing functions $h(\cdot)$ for partition (i.e., in \autoref{alg:random-part}). This multi-round extension can significantly increase the probability of a successful reconciliation, which will be elaborated in \autoref{sec:tail_bound}. 



\subsection{Our Scheme: The Final Version}\label{subsec:protocol2}

{\bf Under revision~}

The preliminary version of our scheme suffers from two major drawbacks. 
First, its communication overhead is asymptotically 
$O(t\log m)\!=\!O(t\log t)$, which is not asymptotically optimal. 
Second, the decoding computational complexity is proportional to 
$t^2$ with the state-of-the-art decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} for BCH codes, 
which is too high when $t$ is large. 
To overcome these two drawbacks, we use a simple algorithmic trick: divide and conquer. With this algorithmic 
trick, the decoding computational complexity is reduced to $O(t)$, 
and the communication overhead is reduced to $t\cdot\frac{\log u}{8} \!+\! O(t)$ (with a small 
hidden constant roughly varying from 4 to 8) bytes which implies that 
our scheme has an additive communication overhead (compared to the optimal scheme) 
of 4 to 8 bytes per element in the 
set difference and this additive overhead is independent of the key size ({\it i.e.}, $\log u$). 
Recall that the IBF-based schemes usually have a communication overhead of roughly 6 times of the 
optimal scheme, which increases linearly as the key size. Therefore, our scheme is much more 
communication-efficient. 

Now, we describe in detail this algorithmic trick. We let Alice divide elements in $A$ into $\lceil\frac{t}{c}\rceil$ groups (subsets)  
for some small constant $c$ (say $5$) so that each group contains roughly $c$ elements from the set difference on average. We let Bob do the same operations on $B$. To ensure that any common element ({\it i.e.,} any element $x\!\in\! A\bigcup B$) goes into 
the same group ({\it i.e.,} groups at Alice and Bob with the same index), we can use the partition procedure with a hash function shown 
in~\autoref{alg:random-part}. Then, we can apply the preliminary version on each group with a constant $m$ (say $m\!=\!256$) independent of 
$t$. To ensure that each group can be reconciled with a high probability, we need to use BCH codes whose decoding capacity 
larger than $c$ (say $\tau\!=\!2c$), as exact number of elements to be reconciled could be larger than $c$. 
Since this decoding capacity $\tau$ is still a small constant independent of $t$, therefore, the communication 
overhead per group is $\tau\cdot\log m \!=\!O(1)$, which implies a total communication overhead of $O(t)$. 
Similarly, the total decoding computational complexity is also $O(t)$. 

\subsubsection{Parameter Configurations} 

Our scheme now has several parameters: $c$ (average number of elements from the set difference in each group), 
$\tau$ (the correcting capability of the BCH code), $m$ (number of bins for each group), and $r$ (maximum number of rounds). 
We note that the maximum number of rounds $r$ is usually associated with another parameter $p$ the desired success rate: With 
at most $r$ rounds, our scheme should guarantee that the success rate is at least $p$. 
%How to tune these parameters to achieve favorable performance will be detailed later in~\autoref{sec:tail_bound}. 
Here, we provide some guidances for the parameter configurations using our theoretical analysis, which gives the tail bound of 
the success probability of our scheme and will be shown in~\autoref{sec:tail_bound}. 

\noindent
{\bf Parameterizing $c$ and $r$.} The values of $c$ and $r$ are usually provided by users based on the requirements of 
applications. For the value of $c$, a larger $c$ results in a longer decoding time yet lower communication overhead.  
So if the decoding time is a big concern, then a smaller $c$ (say $c=5$) should be used; otherwise, a larger $c$ could be used. 
For the values of $r$, a larger $r$ leads to lower communication overhead and usually lower decoding time (as it allows to use 
a smaller $\tau$), however, the reduction is marginal when $r>3$. Therefore, we suggest users to configure $r$ to be $2$ or $3$. 
% The configuration of $c$ is relatively straightforward, as a larger $c$ will result in 
% a longer decoding time and a slightly lower communication overhead. The former is ..., The latter is slightly tricky. 


\noindent
{\bf Using $c$ and $r$ to parameterize other parameters.} After users specify the values for $c$ and $r$ (associated with a value for 
$p$), we can use our theoretical analysis in~\autoref{sec:tail_bound} to parameterize $\tau$ and $m$. 
Since in a BCH code, the block length is in the form of $2^q-1$, we only need to consider $m=2^q-1$. 

{\bf Liang, please revise the following algorithm!}

\begin{algorithm}
\SetKwProg{Proc}{}{}{end}
\SetKwFunction{algo}{\small Search}

\Proc{Search($c$, $r$, $p$)}{\label{search:entrance}

$\mbox{co}_{best}\leftarrow\infty$\tcc*{\small Best communication overhead}

\For{$\tau \leftarrow c\,\KwTo\, \infty$}{}



}
\end{algorithm}


% , unlike 
% the IBF-based schemes which have an multiplicative overhead of 6 
% The inspiration is from the famous 
% divide and conquer algorithm for the selection problem, in which, given an array with $n$ elements, we want to get the $k$-th largest 
% element. A straightforward idea for this problem is sorting. However, if using insertion-sorting, the complexity would be $O(n^2)$. 
% Then the famous divide and conquer trick comes. It first divides the array into $\lceil n/5\rceil$ groups so that the first 
% $\lfloor n/5\rfloor$ contains $5$ elements and at most one group contains the rest $n \mod 5$ elements, and find the median of each 
% group using the insertion-sorting and th


% This straw-man scheme still has a problem on decoding computational complexity. More specific, the complexity increases dramatically with the total number of corrupted bits $t$. Therefore, when $t$ is moderate or large, the decoding computational complexity could be very high. For instance, the decoding complexity of BCH codes~\cite{Lint_IntroductionCodingTheory_1998} is $O(t^3)$, which could be quite high for a large $t$. To keep the decoding complexity reasonably low, we design the following two-layer protocol: In the first layer, we use a hash function to partition the two sets into $\lceil\frac{t}{c}\rceil$ subsets for some small constant $c$ (say $5$), just like the first step of our straw-man scheme. The objective, which is however different from before, is to make each subset pair contains roughly $c$ exclusive elements on average. In the second layer, we use the straw-man scheme with the same configuration (number of subsets $m$, and error-correction capability $\tau$, number of rounds $r$) to reconcile each subset pair. 

% In fact, the straw-man scheme is a proper solution when $t$ is small. First, the decoding complexity will not be a problem for a small $t$; Second, we do not need an extremely large $m$ to guarantee \autoref{eq:requirement_strawman} w.h.p.. For instance, when $t=5$ and $m=1024$, \autoref{eq:requirement_strawman} holds with probability $\frac{m\,!}{(m-t)\,!m^t}\approx 99\%$. This motivates us to design the following two-layer protocol: In the first layer, we use a hash function to partition the two sets into $\lceil\frac{t}{c}\rceil$ subsets for some small constant $c$ (say $5$), just like the first step of our straw-man scheme. The objective, which is however different from before, is to make each subset pair contains roughly $c$ exclusive elements on average. In the second layer, we use the straw-man scheme with the same configuration (number of subsets $m$, and error-correction capability $\tau$) to reconcile each subset pair. 

\autoref{proto:II} shows the pseudocode of our scheme. It first uses the same hash-function based random partition algorithm as \autoref{alg:random-part} to partition elements into $k\triangleq\lceil \frac{t}{c} \rceil$ subsets. Note that the random partition only guarantees that each such subset 
contains $c$ exclusive elements on average, and the exact number is not known. Hence, our scheme uses a BCH code with a capability of 
correcting up to $\tau$ errors with $\tau > c$ to make sure that the BCH code has a high probability to decode successfully. We will describe how to deal with situation where the size of set difference exceeds $\tau$ later in~\autoref{subsec:exceptions}.

As the decoding of a $\tau$-error-correcting BCH code where $\tau$ is a small constant has a constant-time computational complexity, the decoding complexity of 
our scheme is $O(k)=O(t)$. We now have several parameters, average number of exclusive elements in each subset $c$, the correcting capability $\tau$ of BCH code, the number of smaller subsets $m$ for each subset to be divided to, and the number of rounds $r$. How to tune these parameters to achieve favorable performance will be detailed later in~\autoref{sec:tail_bound}. 

\IncMargin{1em}
\begin{algorithm}
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
\Input{Size of set difference $t$}
\Input{The number of subsets $m$ for each partition}
\Input{Average number of exclusive elements in each partition $c$}
\Input{BCH code capability $\tau$}

$k \leftarrow \lceil \frac{t}{c}\rceil $\;

Partition elements into $k$ subsets using~\autoref{alg:random-part}\;

\For{$j = 0$ \KwTo $k-1$}{
    Reconcile the $j$-th subset pair using the straw-man scheme with the BCH correcting capability $\tau$, number of smaller subsets $m$, and number of rounds $r$\;
}

\caption{Our Scheme} \label{proto:II}
\end{algorithm}\DecMargin{1em}




\subsection{Exceptional Handling}\label{subsec:exceptions}

{\bf To be revised~}

In this section, we will elaborate how to handle the following two types of exceptions that we mentioned in \autoref{sec:multiround} and \autoref{subsec:protocol2}:
\begin{itemize}
    \item Exception 1: A subset pair has odd number ($\geq 3$) of exclusive elements and causes false-positives (i.e., a decoded distinct element is not a real one);
    \item Exception 2: A subset pair contains too many exclusive elements, such that a BCH code with capability of correcting up to $\tau$ errors cannot decode it (i.e., $t>\tau$).
	\item Exception 3: A subset pair has even number ($\geq 2$) of exclusive elements and causes false-negatives(i.e., two or more distinct elements are neglected as the parity bit is 0);
\end{itemize}

To handle Exception 1, we need to check whether a computed exclusive element by \autoref{alg:trivial_case} is a real exclusive element or not. (The group index happens to come in handy if we use it as a fingerprint of the element we computed. If this element is truly an exclusive element, it should be hashed into the same group as before. Notably, We have two group indices available for this check, one is in the initial divide and conquer phase, the other is in the BCH code part) It can be easily done at the end of set reconciliation, during which two hosts exchange their exclusive elements. In fact, as we will elaborate in \autoref{sec:tail_bound}, Exception 1 hardly happens if we set parameters properly. 

On the other hand, when Exception 2 happens, the BCH decoder will report a failure about exceeding the error-correction capability. For such a subset pair, we can use the same approach as in \autoref{subsec:protocol2} to partition it into smaller subsets and use the straw-man scheme to reconcile them respectively. We set the number of small subsets to be 3. It is because, as we will elaborate in \autoref{sec:tail_bound}, the number of exclusive elements for each subset pair $t$ should be, if not smaller, only slightly larger than $\tau$ w.h.p.. Partitioning those exclusive elements into 3 small subsets is enough to guarentee that each of them has less than $\tau$ exclusive elements.

\end{comment}

==> section/schemes_new_0210.tex <==
\section{Set Reconciliation}\label{sec:scheme}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%     Writing Guideline for This Section     %%%%%%%%%%
% “balls – elements in the symmetric difference of the two sets” 

% Protocol 0 (reconcile two sets whose set difference has at most one ball)

% Protocol I.I (partition elements into a sufficiently large number of subsets such that each subset has at most one ball with high probability and use Protocol 0 to reconcile each of them) 

% Protocol I.II (a two-step refinement of Protocol I.I: first use BCH to identify good bins, i.e., bins/subsets have exactly one ball, and then use Protocol 0 to reconcile each good bin) 

% Protocol II (a two-layer refinement of Protocol I.II: in the first layer, we partition elements into t/c subsets, where t is the size of set difference and c is a small constant, then each subset has c balls on average. In the second layer, we further partition each subset into large enough number of bins/subsets such that with high probability each bin has at most one ball, then use Protocol I.II to reconcile them one by one) 

% Protocol III/IV (mainly fix certain exceptions in Protocol II，e.g., how to address bad bins, how to handle the cases where BCH fails to decode and etc)

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% In this section, we describe our set reconciliation scheme in details. First, we give a formal problem statement in \autoref{sec:model}. In \autoref{subsec:protocol0}, we introduce a basic scheme for the trivial case, in which the two sets $A$ and $B$ has at most one distinct element. Building upon the basic scheme, we propose the preliminary version of scheme in \autoref{sucsec:our-scheme} that targets to the cases where the total number of distinct elements $d$ is small. Then we extend the preliminary version and propose the final version of our scheme in \autoref{subsec:protocol2} for general cases (i.e., any arbitrary $d$). We assume $d$ is precisely known throughout this section except in \autoref{subsec:ToW}, where we will describe how to estimate $d$ using a Tug-of-War Estimator. 

\subsection{Problem Statement}\label{sec:model}

In this work, we adopt the commonly used model for the set reconciliation problem. 
Two remote sets $A$ and $B$ are stored at hosts Alice and Bob respectively. Each element in $A$ and $B$ is a hash signiture with signiture width $w$ in the key space (universe) $\mathcal{U}$, which is the set of all $w$-bit binary strings (i.e., $|\mathcal{U}|=2^w$). 
%We use $\mathcal{U}$ to denote the set of all $w$-bit binary strings and name it the universe of signitures. 
The set reconciliation problem is to compute the symmetric set difference between $A$ and $B$, 
{\it i.e.,} $A\Delta B\triangleq (A\!\setminus\! B) \bigcup (B\!\setminus\! A)$. We denote $d\!=\!|A\Delta B|$. Throught this paper, we call each element in $A\Delta B$ a \textit{distinct element}.
%, and we call each element in $A\bigcap B$ a \textit{common element}.
{\bf Like in all existing solutions, we describe only {\it unidirectional} set reconciliation that Alice or Bob learns the set difference $A\Delta B$. Since the performance of our scheme does not depend on who learns the set difference, we assume Bob learns the set difference $A\Delta B$ in the rest of the paper, as mentioned in \autoref{sec:psea}.}
% As mentioned in \autoref{sec:psea}, we describe {\it unidirectional} set reconciliation that Bob learns the set difference $A\Delta B$. 
%In \autoref{sec:evaluation}, we use the same semantic to measure the communication cost of our scheme and other compared set reconciliation schemes. 

In the rest of this section, we build up our scheme incrementally as follows: We start with the trivial case when $d\leq 1$ in \autoref{subsec:protocol0}. Then we generalize our scheme to the case that $d$ is a small number in \autoref{sucsec:our-scheme}. After that, we further generalize our scheme to the case that $d$ is a large number in \autoref{subsec:protocol2}. Throughout this section, we assume $d$ is precisely known except in \autoref{subsec:ToW}, where we will describe how to estimate $d$ using a Tug-of-War Estimator. 

%The rest of this section is organized as follows: In \autoref{subsec:protocol0}, we introduce a basic scheme for the trivial case, in which the two sets $A$ and $B$ has at most one distinct element. In \autoref{sucsec:our-scheme} and \autoref{subsec:protocol2}, we elaborate the two versions of our solution that are introduced in \autoref{sec:smalld} and \autoref{sec:larged} respectively. Throughout this section, we assume $d$ is precisely known except in \autoref{subsec:ToW}, where we will describe how to estimate $d$ using a Tug-of-War Estimator. 

\subsection{The Trivial Case: $d\leq 1$}\label{subsec:protocol0}

%We start with the trivial case, in which $A$ and $B$ have at most one distinct element ({\it i.e.,} $d\leq 1$), we have a simple set reconciliation scheme showed in \autoref{alg:trivial_case}:

\autoref{alg:trivial_case} shows the reconciliation scheme for the trivial case as follows:

\begin{algorithm}
\caption{Set reconciliation when $d\le 1$}
\label{alg:trivial_case}

{\it Alice}: $s_A\leftarrow\underset{a\in A}{\oplus} a$; Send $s_A$ to Bob\; \label{alg1:sender}

{\it Bob}: $s_B\leftarrow\underset{b\in B}{\oplus} b$; $s\leftarrow s_A \oplus s_B$\; \label{alg1:receiver}
\end{algorithm}

First, Alice calculates $s_A$, the bitwise \code{XOR} of all elements in $A$, and send it to Bob. 
Second, Bob also calculates $s_B$, the bitwise \code{XOR} of all elements of $B$. Upon receiving $s_A$, Bob computes $s\!\triangleq\! s_A \!\oplus\! s_B$, and we have

\begin{itemize}
	\item If $A$ and $B$ are identical sets (i.e., $d=0$), we have $s_A=s_B$ and $s=0$;
	\item If $A$ and $B$ has one distinct element (i.e., $d=1$), the computed $s$, the bitwise \code{XOR} of $s_A$ and $s_B$, will cancel out all common elements and remain the distinct element: $A\Delta B=\{s\}$. 
	%And $s$ is the missing element of $A$ (i.e., $s\in B\!\setminus\! A$) if $s\in B$, or the missing element of $B$ (i.e., $s\in A\!\setminus\! B$) otherwise;
	% \item If $A$ and $B$ has more than one distinct elements (i.e., $d>1$), the bitwise \code{XOR} of $s_A$ and $s_B$ will still cancel out all common elements and remain the \code{XOR} of the distinct elements, i.e., $s$ is the \code{XOR} of all distinct elements;
\end{itemize}

Like most works on set reconciliation, we assume $\mathbf{0}$ is excluded from $\mathcal{U}$, since \autoref{alg:trivial_case} does not work when $\mathbf{0}\in A\bigcap B$: When $s=0$, \autoref{alg:trivial_case} cannot tell whether $A$ and $B$ are identical, or they have a distinct element of value $\mathbf{0}$. 
%However, we can extend our scheme to support $\mathbf{0}$. For example, we let Alice send to Bob a single bit to indicate whether Alice has element $\mathbf{0}$, so Bob will know whether $\mathbf{0}\in A\Delta B$ or not. 
\autoref{alg:trivial_case} also does not work when $d>1$, since the computed $s$, the bitwise \code{XOR} of $s_A$ and $s_B$, is the \code{XOR} of all distinct elements in $A\Delta B$.

% Note that \autoref{alg:trivial_case} works if and only if $|A\Delta B|\!\leq\! 1$ and $0\!\notin\! (A\!\cup\! B)$ (which we have explained in~\autoref{sec:model}). 

\subsection{PBS: When $d$ is small}\label{sucsec:our-scheme}

In this section, we generalize PBS to the case when $d$ is a small number, as we described in \autoref{sec:smalld}. 
%First, we describe each step of single-round PBS from \autoref{sec:hash_partition} to \autoref{sec:reconcile_by_trivial} and summarize it in \autoref{sec:single_round_pbs}. Second, we discuss the exceptions in single-round PBS in \autoref{subsec:exception_hash_partition}. Third, we propose multi-round PBS to handle the exceptions.

%\subsubsection{Hash Partition}\label{sec:hash_partition}
\medskip
\noindent{\bf Hash Partition} 

Here we formalize the process of partitioning $A$ into $\{A_i\}_{i=1}^n$, $B$ into $\{B_i\}_{i=1}^n$, and $A\Delta B$ into $\{A_i\Delta B_i\}_{i=1}^n$ as described in \autoref{sec:smalld} by introducing the concept of {\it sub-universes}. Given a hash function $h(\cdot): \mathcal{U}\rightarrow \{1,2,\cdots,n\}$, we define {\it sub-universe} $\mathcal{U}_i$ as the set of elements in $\mathcal{U}$ that are hashed into value $i$: $\mathcal{U}_i\triangleq\{s\!\mid\! s\in \mathcal{U} \mbox{ and } h(s)=i\}$ for $i=1,2,...,n$. Based on $\{\mathcal{U}_i\}_{i=1}^n$, we define $A_i\triangleq A\bigcap\mathcal{U}_i$ and $B_i\triangleq B\bigcap\mathcal{U}_i$ for $i=1,2,...,n$. For the moment, we assume the following {\bf ideal case} happens: Every subset pair difference $A_i\Delta B_i$ contains at most one distinct element. The nonideal case of a subset pair difference containing more than $1$ distinct elements will be discussed in \autoref{subsec:exception_hash_partition}. 

%In this section, we give a detailed description on how to partition $A$ and $B$ (as introduced in \autoref{sec:smalld}) by introducing {\it sub-universes}, which is defined as follows: Given a hash function $h(\cdot): \mathcal{U}\rightarrow \{1,2,\cdots,n\}$, we define {\it sub-universes} $\{\mathcal{U}_i\}_{i=1}^n$, a partition of the universe $\mathcal{U}$, as $\mathcal{U}_i=\{s\!\mid\! s\in \mathcal{U} \mbox{ and } h(s)=i\}$ for $i=1,2,...,n$. Based on $\{\mathcal{U}_i\}_{i=1}^n$, we define $\{A_i\}_{i=1}^n$, the partition of $A$ introduced in \autoref{sec:smalld}, as $A_i\! \triangleq\! A\bigcap \mathcal{U}_i$ for $i=1,2,...,n$. $\{B_i\}_{i=1}^n$ is similarly defined. By this definition, the set difference $A\Delta B$ is partitioned into $n$ set differences of the partitioned subset pairs (i.e., $\{(A_i, B_i)\}_{i=1}^n$). From \autoref{sec:hash_partition} to \autoref{sec:reconcile_by_trivial}, we assume the following {\bf ideal case} happens: Each subset pair $(A_i, B_i)$ contains at most one distinct element ({\it i.e.,} $|A_i\Delta B_i|\!\leq\!1$). The nonideal case of a subset pair contains more than $1$ distinct elements will be discussed in \autoref{subsec:exception_hash_partition}. 

% Here we describe the hash-partition step introduced in \autoref{sec:smalld} in details. First, we use a hash function $h(\cdot): \mathcal{U}\rightarrow \{1,2,\cdots,n\}$ to partition the universe $\mathcal{U}$ into $n$ sub-universes: $\mathcal{U}_i=\{s\!\mid\! s\in \mathcal{U} \mbox{ and } h(s)=i\}$ for $\forall i=1,2,\cdots,n$. The hash function $h(\cdot)$ can be predetermined between Alice and Bob and does not require additional communication cost. Define $A_i\! \triangleq\! A\bigcap \mathcal{U}_i$ and $B_i\! \triangleq\! B\bigcap \mathcal{U}_i$ for $i=1,2,\cdots,n$. Then $\{A_i\}_{i=1}^n$ and $\{B_i\}_{i=1}^n$ are partitions of $A$ and $B$ respectively. Furthermore, $\{A_i\Delta B_i\}_{i=1}^n$ is a partition of $A\Delta B$. From \autoref{sec:hash_partition} to \autoref{sec:reconcile_by_trivial}, we assume the following {\bf ideal case} happens: Each subset pair $(A_i, B_i)$ contains at most one distinct element ({\it i.e.,} $|A_i\Delta B_i|\!\leq\!1$). The nonideal case of a subset pair contains more than $1$ distinct elements will be discussed in \autoref{subsec:exception_hash_partition}. 

How the $d$ distinct elements (balls) in $A\Delta B$ are distributed into the $n$ subset pair differences $\{A_i\Delta B_i\}_{i=1}^n$ (bins) follows the familiar {\it balls-into-bins} probability model. 
%The distinct elements are viewed as balls and the subset pairs are viewed as bins. 
Each of the $d$ balls is uniformly and randomly thrown by the hash function $h(\cdot)$ into one of the $n$ bins. The aforementioned ideal case that corresponds to the $d$ balls ending up in $d$ distinct bins happens with probability $\prod_{k=1}^{d - 1}(1 - \frac{k}{n})$, which equals to $1-O(d^2/n)$
% when $d\!\ll\!n$ 
%approximately $e^{-\frac{d(d-1)}{2n}}$ when $d\!\ll\!n$. 
.Hence, $n$ must be $\Omega(d^2)$ to ensure the ideal case happens with a high probability, as mentioned in \autoref{sec:smalld}.


%in which the distinct elements are viewed as balls and the subset pairs are viewed as bins. The hash-parition basically throws (hashes) $d$ balls (distinct elements) uniformly and randomly into $n$ bins (subset pairs). The aforementioned ideal case in this context becomes, after throwing $d$ balls uniformly and randomly into $n$ bins, each bin receives at most $1$ ball (i.e., $d$ nonempty bins have $1$ ball in each and the rest $n-d$ bins are empty). The number of balls in each bin is a Binomial random variable $Binomial(d,1/n)$.
%{\bf It may remind readers about the Birthday problem. And the ideal case can be analogous to the case that no people share the same birthday.} 
% The ideal case happens with a probability of $p\!=\!\prod_{k=1}^{d - 1}(1 - \frac{k}{n})\!\approx\! e^{-\frac{d(d-1)}{2n}}$ when $d\!\ll\!n$. In other words, $n$ must be at least $O(d^2)$ to ensure the ideal case happens with a nontrivial probability, as described in \autoref{sec:smalld}.  

% Note that the ideal case does not always happen. However, we can ensure that the ideal case happens with high probability by properly setting $n$ based on $d$ (i.e., $n=\Omega(d^2)$). Furthermore, as we will describe in \autoref{subsec:nonideal}, even if the ideal case does not happen (i.e., some distinct elements are hashed into the same subset pair), most of the distinct elements should be distributed into different subset pairs and therefore can be reconciled. So the scheme, even cannot reconcile all of the distinct elements, can still reconcile the majority of them (i.e., piecewise decodability in \autoref{sec:intro_oursolution}). Based on this property, we will extend our scheme from single-round to multi-rounds in \autoref{subsec:nonideal} to further increase the probability of reconciling all distinct elements. 
\medskip
\noindent{\bf Parity Bitmap Encoding} 

We encode $\{A_i\}_{i=1}^n$ into an $n$-bit-long parity bitmap $A[1..n]$, in which $A[i]$, the $i^{th}$ bit of the parity bitmap, is equal to the oddness / evenness (parity) of the cardinality of $A_i$ (i.e., $A[i]=1$ if $|A_i|$ is odd; otherwise $A[i]=0$). In the ideal case, the two bitmaps $A[1..n]$, $B[1..n]$ differ in exactly $d$ bit positions $i_1,i_2,...,i_d$, each of which corresponds to a subset pair that contains $1$ distinct element. Once the $d$ bit positions are known, Alice and Bob can start to reconcile $(A_{i_1},B_{i_1}), (A_{i_2},B_{i_2}),...,(A_{i_d},B_{i_d})$ using \autoref{alg:trivial_case} and obtain the $d$ distinct elements (i.e., $A\Delta B$). 

% \subsubsection{Parity Bitmap Encoding}\label{sec:parity_bitmap_encoding}

% %After hash-partitioning $A$ and $B$ into partitions $\{A_i\}_{i=1}^n$ and $\{B_i\}_{i=1}^n$, 
% As introduced in \autoref{sec:smalld}, we encode each partition into an $n$-bit-long parity bitmap and denote them as $A[1..n]$ and $B[1..n]$ respectively, as introduced in \autoref{sec:smalld}. For $i=1,2,...,n$, $A[i]$ (the $i^{th}$ bit of the parity bitmap $A[i]$) is equal to $1$ if $A_i$ contains an odd number of elements, and is equal to $0$ otherwise.
% % More specifically, for $i=1,2,...,n$, $A[i]$ (the $i^{th}$ bit of the parity bitmap $A[i]$) is defined as follows: $A[i]=1$ if $A_i$ contains an odd number of elements, and $A[i]=0$ otherwise. In this way, each bit $A[i]$ encodes the oddness / evenness (parity) of the cardinality of $A_i$. The $n$-bit-long parity bitmap $B[1..n]$ and $B[i]$ (the $i^{th}$ bit of $B[1..n]$) are similarly defined. 
% In the ideal case, 
% %$A[i]$ and $B[i]$ differ if and only if $A_i$ and $B_i$ have exactly $1$ distinct element, and $A[i]$ and $B[i]$ are the same if and only if $A_i=B_i$. Meanwhile, the $d$ distinct elements are hashed into $d$ different subset pairs. So 
% the two bitmaps $A[1..n]$, $B[1..n]$ differ in exactly $d$ bit positions, each of which corresponds to a subset pair that contains $1$ distinct element. Once the $d$ bit positions are known, Alice starts to reconcile each of the $d$ corresponding subset pairs by \autoref{alg:trivial_case} and gets the $d$ distinct elements (i.e., $A\Delta B$). 
% %If knowing the $d$ bit positions (i.e., the $d$ corresponding subset pairs), we can use \autoref{alg:trivial_case} to reconcile the $d$ subset pairs respectively to obtain all the $d$ distinct elements (i.e., $A\Delta B$). 
% In \autoref{sec:BCH_code}, we will describe how to find the $d$ bit positions using BCH code~\cite{Lint_IntroductionCodingTheory_1998}. 
\medskip
\noindent{\bf Find the $d$ Bit Positions Using ECC} 

We view $A[1..n]$ as a corrupted message of $B[1..n]$ sent ({\bf virtually}) from Bob to Alice through an {\it unreliable} commnunication channel that flips $d$ bits. To locate the $d$ bit positions, we let Bob also send an error-correction code that encodes $B[1..n]$ to Alice, such that Alice can recover $B[1..n]$ (original message) and obtain the $d$ bit positions $i_1,i_2,...,i_d$. In PBS, we choose BCH code~\cite{bch1} as the error-correction code.

There are two different BCH encoding methods: {\it systematic} and {\it unsystematic}. The difference is, the message appears as the prefix of the codeword (i.e., codeword = [message net-codeword]) in systematic BCH encoding, while it does not appear as a substring of the codeword in unsystematic BCH encoding. In PBS, we choose systematic BCH encoding because we are not actually sending the message, and only the net-codeword is transmitted from Bob to Alice. 

To correct $d$ bit errors, the length of the net-codeword is no more than $d\log n$ bits. We use the term `codeword' to refer the net-codeword in the rest of this paper.
%The computational complexity of the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} is $O(d^2\log^2 n)$.
The systematic BCH encoding is also used in other ECC-based set reconciliation works, such as PinSketch \cite{Wuille_Minisketchoptimizedlibrary_2019}, albeit PinSketch encodes a much longer message (e.g., $2^{32}$ bits) than ours (hundreds of bits).  

%\subsubsection{Find the $d$ Bit Positions Using ECC}\label{sec:BCH_code}

% A straightforward approach to find the $d$ bit positions is to let Bob send the complete parity bitmap $B[1..n]$ to Alice, then Alice compares $A[1..n]$ with $B[1..n]$ locally. This approach has a communication overhead of $n$ bits, which is quite wasteful. As we discussed in~\autoref{sec:hash_partition}, $d$ is usually much smaller than $n$. It means $A[1..n]$ and $B[1..n]$ differ only at a tiny portion of bits. Therefore, we can view $A[1..n]$ as a corrupted message of $B[1..n]$ with $d$ bit errors, and the bit positions of the $d$ bit errors basically correspond to the $d$ subset pairs that contain distinct elements. The detection of bit errors, on the other hand, can be solved by Error-Correction Code (ECC)~\cite{Lin_ErrorControlCoding_1983}. 

% Since $A[1..n]$ and $B[1..n]$ differ at $d$ bit positions, we can view $A[1..n]$ as a corrupted message of $B[1..n]$ from Bob to Alice through an {\it unreliable} commnunication channel with $d$ corrupted bits, which are located on the $d$ bit positions. Therefore, to find the $d$ bit position, we only need to correct the $d$ corrupted bits in $A[1..n]$, which is done by transmitting a ``code'' that can correct upto $d$ bit errors from Bob to Alice through a {\it reliable} communication channel. 

% In PBS, we use {\it systematic} BCH code to generate the ``code'' by encoding the message $B[1..n]$. The codeword of the systematic BCH code is in the form of [message, net-codeword], since the message appears as the prefix of the codeword in systematic BCH code. The ``code'' is simply the net-codeword in the BCH codeword. We choose {\it systematic} BCH code because the (corrupted) message is already transmitted and we only need to pay a small communication overhead on transmitting ``code'' (i.e., net-codeword). To correct upto $d$ bit errors, the length of the net-codeword is no more than $d\log n$ bits, which is much smaller than the message when $d\!\ll\! n$. The computational complexity of the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} is $O(d^2\log^2 n)$. This type of BCH code is also used in other ECC-based set reconciliation works, such as PinSketch \cite{Wuille_Minisketchoptimizedlibrary_2019}. 

% Different from {\it unsystematic} BCH code
% The ``code'' is generated by {\it systematic} BCH code, which encodes the message $B[1..n]$ into a BCH codeword in the form of [message, net-codeword]. The ``code'' transmitted on the reliable channel is the net-codeword of the BCH codeword. In {\it systematic} BCH code, the message appears as the prefix of the codeword. 

% More specifically, PBS uses {\it systematic} BCH code~\cite{Lint_IntroductionCodingTheory_1998} that can correct upto $d$ bit errors to encode the parity bitmaps. In the {\it systematic} BCH code \footnote{In unsystematic BCH code, message does not appear to be the prefix of the codeword}, the message (i.e., the parity bitmap) appears as the prefix of the raw codeword, which in the form of [message, net codeword]. Normally, to correct upto $d$ errors, the length of the net codeword is $2n\log d$, where $n$ is the length of the message (i.e., parity bitmap). However, our case is special in the sense that the net codeword is error-free (all $d$ bit errors are in the message), so the length of the net codeword can be reduced to $n\log d$. This type of BCH code is also used in other ECC-based set reconciliation works, such as PinSketch \cite{Wuille_Minisketchoptimizedlibrary_2019}. 

% Now we can formally describe how to find the $d$ bit positions: First, Bob uses a $d$-error-correcting systematic BCH code to encode $B[1..n]$ and sends the net codeword ($d\log n$ bits) to Alice. Upon receiving the net codeword and combining it with the corrupted message $A[1..n]$, Alice uses the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} to decode the $d$ bit errors in $A[1..n]$. The communication overhead of transmitting the net codeword is $d\log n$ bits. The computational complexity of the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} is $O(d^2\log^2 n)$. Both the communication overhead and the computational complexity here are relatively small when $d$ is small.
\medskip
\noindent{\bf Reconcile the $d$ subset pairs using \autoref{alg:trivial_case}} 

When reconciling $(A_{i_1},B_{i_1}), (A_{i_2},B_{i_2}),...,(A_{i_d},B_{i_d})$ using \autoref{alg:trivial_case}, Alice needs to send not only the bitwise \code{XOR} of $A_{i_1}, A_{i_2},..., A_{i_d}$, but also the indices of the subset pairs (i.e., $i_1,i_2,...,i_d$), since Bob does not know which of the $d$ subset pairs are being reconciled. Each index is an integer between $1$ and $n$ and can be encoded into $\log n$ bits, So the additional communication overhead on transmitting the indices is $d\log n$ bits. 



% \subsubsection{Reconcile the $d$ subset pairs using \autoref{alg:trivial_case}}\label{sec:reconcile_by_trivial}

% After decoding the $d$ bit errors that corresponds to the $d$ subset pairs, Alice starts to reconcile them using \autoref{alg:trivial_case}. For each of the $d$ subset pairs, Alice needs to send not only the bitwise \code{XOR} of the subset pair, but also the index of the subset pair (since Bob does not know the $d$ subset pairs to reconcile). So the communication overhead on \autoref{alg:trivial_case} is $d\log |\mathcal{U}|+d\log n$ bits. 
%Plus the communication overhead on transmitting the net codeword of parity bitmap ($d\log n$, as we explained in \autoref{sec:BCH_code}), the overall communication overhead of single-round PBS is $d\log u+2d\log n$ bits.

\medskip
\noindent{\bf Check if set reconciliation is complete} 

After reconciling the subset pairs and obtaining the reconciled set difference (denoted as $\hat{D}$), PBS needs to check if set reconciliation is complete (i.e., $\hat{D}=A\Delta B$), since the reconciled set difference $\hat{D}$ is not the actual set difference $A\Delta B$ in the nonideal case (to be discussed in \autoref{subsec:exception_hash_partition}). Hence, we add a verfication step after obtaining $\hat{D}$ to check if $\hat{D}=A\Delta B$. In PBS, we check an equivalent condition, $A=B\Delta\hat{D}$, instead of $\hat{D}=A\Delta B$, since $B$ and $\hat{D}$ are both known by Bob and their set difference $B\Delta\hat{D}$ can be locally computed. More specifically, to check if the remote sets $A$ and $B\Delta\hat{D}$ are equal, we let Alice compute a $32$-bit checksum of $A$ and send it to Bob. Then Bob checks if $B\Delta\hat{D}$ satisfies the receiving checksum. 

The condition $A=B\Delta\hat{D}$ can be almost surely verified by a $32$-bit checksum, albeit it could mistakenly believe two different sets as identical ones with probability $2^{-32}\approx 2.3\times 10^{-10}$. This probability should be small enough for most applications and such an event (i.e., mistaken $A$ and $B\Delta\hat{D}$ are identical when they are different) never happens in our evaluation. For some super critical applications, we can certainly use a $64$-bit checksum to reduce this probability to $5.4\times 10^{-20}$ if needed.
% When the ideal case does not happen, set reconciliation cannot accomplish in one round, as we will explain in \autoref{subsec:exception_hash_partition}. Hence, we add a verfication step to check if set reconciliation is complete. Let $\hat{D}$ denote the set of reconciled elements. The idea of this verification is basically to compare $A$ with $B\Delta \hat{D}$: If $A=B\Delta \hat{D}$ (i.e., $\hat{D}=A\Delta B$), we know the set reconciliation is complete; Otherwise, the set reconciliation is incomplete.  using a $32$-bit checksum. 

\subsubsection{Communication overhead of single-round PBS}\label{sec:communication_overhead_single_PBS}

All the steps of PBS in the first round are summarized in \autoref{alg:single_round_pbs}. The overall communication overhead consists of three components: (1) the BCH codeword of $d\log n$ bits in \autoref{step:BCH_encode}; (2) the subset pair indices $i_1,i_2,...,i_d$ and the corresponding bitwise \code{XOR}s of $d\log n+d\log |\mathcal{U}|$ bits in \autoref{step:trivial_reconcile}; and (3) the $32$-bit checksum of $A$ in \autoref{step:terminate_condition}. 

\begin{algorithm}
\caption{Single-round PBS}
\label{alg:single_round_pbs}

Hash-partition $A$, $B$ into $\{A_i\}_{i=1}^n$, $\{B_i\}_{i=1}^n$\; \label{step:hash_partition}
{}
Parity encode $\{A_i\}_{i=1}^n$, $\{B_i\}_{i=1}^n$ into $A[1..n]$, $B[1..n]$\; \label{step:parity_encode}

{\it Bob}: BCH-Encodeing $B[1..n]$ and send the codeword to Alice\; \label{step:BCH_encode}

{\it Alice}: Upon receiving the codeword, decode the bit errors between $A[1..n]$ and $B[1..n]$\; \label{step:BCH_decode}

{\it Alice}: For each bit error, start reconciling the corresponding subset pair by \autoref{alg:trivial_case}\; \label{step:trivial_reconcile}

{\it Bob}: Upon the reconciled set difference $\hat{D}$, check whether $A=B\Delta \hat{D}$ via checksum\; \label{step:terminate_condition}
\end{algorithm}


% \subsubsection{Single-round PBS}\label{sec:single_round_pbs}

% Here we summarize all the steps of single-round PBS and represent it by pseudocode in \autoref{alg:single_round_pbs}. \autoref{step:hash_partition} and \autoref{step:parity_encode} operates at both hosts (i.e., Alice and Bob). \autoref{step:hash_partition} to \autoref{step:trivial_reconcile} have been elaborated from \autoref{sec:hash_partition} to \autoref{sec:reconcile_by_trivial}. The last step in \autoref{step:terminate_condition} aims to check whether reconciliation is complete (i.e., $\mathcal{D}=A\Delta B$). More specifically, Alice calculates the checksum (e.g., CRC-$32$) of $A$ and send it to Bob. Then Bob calculates the checksum of $B\Delta \mathcal{D}$ and compares it to the receiving checksum of $A$. If the two checksums are the same, we believe $A=B\Delta \mathcal{D}$ and therefore $\mathcal{D}=A\Delta B$ (i.e., reconciliation is complete); Else, we know some elements are reconciled incorrectly. We classify those elements (i.e., the ones in the set difference between $A\Delta B$ and $\mathcal{D}$) into two subsets $A\Delta B\!\setminus\!\mathcal{D}$ and $\mathcal{D}\!\setminus\!(A\Delta B)$ and refer the elements in the former as {\it false-negatives}, and refer the elements in the later as {\it false-positives}. 

% In the ideal case, neither false-positives nor false-negatives will happen and the two checksums always equal. However, in real life, the ideal case does not always happen. We will discuss the nonideal case in \autoref{subsec:exception_hash_partition}. In our evaluation, we use a $32$-bit checksum for comparing $A$ to $B\Delta \mathcal{D}$ that has {\bf an error probability} roughly $10^{-9}$. This error (i.e., mistake $A=B\Delta \mathcal{D}$) incurs false-negatives. All set reconciliation schemes have the same problem on their termination conditions (i.e., check whether $\mathcal{D}=A\Delta B$). For some super critical applications, we can certainly decrease the error probability by using more powerful checksums (i.e., $64-$bit). Using a $32$-bit checksum, this kind of false-negatives never happen in the evaluation. 
% %For simplification, we assume no error happens when checking $\mathcal{D}=A\Delta B$ in the rest of the paper.

% \begin{algorithm}
% \caption{Single-round PBS}
% \label{alg:single_round_pbs}

% Hash-partition $A$, $B$ into $\{A_i\}_{i=1}^n$, $\{B_i\}_{i=1}^n$\; \label{step:hash_partition}

% Parity encode $\{A_i\}_{i=1}^n$, $\{B_i\}_{i=1}^n$ into $A[1..n]$, $B[1..n]$\; \label{step:parity_encode}

% {\it Bob}: Encode $B[1..n]$ by BCH code, then send the codeword to Alice\; \label{step:BCH_encode}

% {\it Alice}: Upon receiving the codeword, decode the bit errors between $A[1..n]$ and $B[1..n]$\; \label{step:BCH_decode}

% {\it Alice}: For each bit error, reconcile the corresponding subset pair by \autoref{alg:trivial_case}\; \label{step:trivial_reconcile}

% {\it Bob}: Upon the reconciled distinct elements $\mathcal{D}$, check whether $A=B\Delta \mathcal{D}$ via checksum\; \label{step:terminate_condition}
% \end{algorithm}

\subsubsection{Exception Handling on Hash-Partition}\label{subsec:exception_hash_partition}

When the ideal case does not happen, some subset pair may contain more than $1$ distinct elements and cannot be successfully reconciled by \autoref{alg:trivial_case}. Due to the parity encoding, we can classify such a subset pair into the following two scenarios:

% As we have described in \autoref{sec:hash_partition}, the ideal case does not always happen, which means some subset pair may contain more than $1$ distinct elements and cannot be successfully reconciled by \autoref{alg:trivial_case}. Due to the parity encoding, we can classify such subset pair into the following two scenarios:

\begin{itemize}
    \item Scenario 1: If a subset pair $(A_i, B_i)$ contains even number ($\geq 2$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be the same and PBS will not reconcile the subset pair yet in this round;
    \item Scenario 2: If a subset pair $(A_i, B_i)$ contains odd number ($\geq 3$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be different and PBS will reconcile the subset pair using \autoref{alg:trivial_case}. The reconciled element (i.e., $s$ in \autoref{alg:trivial_case}) is however the bitwise \code{XOR} of all distinct elements in $(A_i, B_i)$ (explained in \autoref{subsec:protocol0}), which will be mistakenly believed as the distinct element of $(A_i, B_i)$. 
    %However, as described in \autoref{subsec:protocol0}, when a subset pair contains more than $1$ distinct elements, \autoref{alg:trivial_case} will output the bitwise \code{XOR} of them as the `distinct element', which is not an actual distinct element with high probability;
\end{itemize}

In both scenarios, the distinct elements in the subset pair will not be reconciled in this round. As we will describe in \autoref{sec:multi-rounds}, we generalize PBS into multi-round, so that the distinct elements that have not been reconciled in the first round will be reconciled in later rounds. On the other hand, the second scenario could result in incorrectly reconciled distinct elements, which will become new distinct elements in the next round in multi-round PBS. 

% In both scenarios, the distinct elements in the subset pair cannot be successfully reconciled in this round and will remain in the set difference (i.e., $(A\Delta B)\!\setminus\!\hat{D}$). On the other hand, the incorrectly reconciled distinct element in the second scenario will appear as a new distinct element (i.e., $\hat{D}\!\setminus\!(A\Delta B)$) in the next round if we generalize PBS into multi-round (to be elaborated in \autoref{sec:multi-rounds}). Both scenarios can be almost surely detected by the 32-bit checksum (\autoref{step:terminate_condition} in \autoref{alg:single_round_pbs}). The set difference after the reconciliation in this round, $D\Delta\hat{D}$, can be reconciled in later rounds, as we will describe in \autoref{sec:multi-rounds}. 

Naturally, we do not want to generate new distinct elements in the process of set reconciliation, even though it happens with a tiny probability when $n=\Omega(d^2)$: For instance, when $d=5$ and $n=255$ (i.e., throwing $5$ balls uniformly and randomly into $255$ bins), the probability (i.e., some bin has $3$ or $5$ balls) is only $7.6\times 10^{-6}$. Therefore, we add a verification with no additional communication cost on each reconciled element of \autoref{alg:trivial_case}, such that each incorrect dinstinct element can be identified with high probability. The verfication is shown in \autoref{alg:verification}. 

\begin{algorithm}
\caption{Verify reconciled element $s$ of $(A_i, B_i)$}
\label{alg:verification}
\If{$h(s)\neq i$} {Discard the reconciled element $s$;}
\end{algorithm}

Although any distinct element of $(A_i, B_i)$ must be in sub-universe $\mathcal{U}_i$ (i.e., the hash value of the element under $h$ equals to $i$), the bitwise \code{XOR} of multiple distinct elements of $(A_i, B_i)$ could be in any sub-universe with probability $1/n$. Therefore, \autoref{alg:verification} can identify an incorrectly reconciled distinct element in the second scenario with probability $1-1/n$ that is roughly $99.6\%$ when $n=255$. In other words, an incorrectly reconciled distinct element that cannot be identified by \autoref{alg:verification} appears with probability $3\times 10^{-8}$. {\bf I feel that defining $\tilde{a}_4=a_1\oplus a_2\oplus a_3$ does not help much.}
% In both scenarios, the distinct elements in the subset pair cannot be successfully reconciled in this round. These distinct elements can be reconciled in later rounds if needed, as we will describe in \autoref{sec:multi-rounds}. In this section, we only discuss how to identify the {\it incorrect} distinct element in the second scenario. Let us use an example to elaborate the second scenario: Assume $(A_i, B_i)$ contains $3$ distinct elements $a_1, a_2, a_3$, then Bob computes $\tilde{s}=a_1\oplus a_2\oplus a_3$ using \autoref{alg:trivial_case} and mistakes it as the distinct element in $(A_i, B_i)$. 

% In both scenarios, the distinct elements in the subset pair cannot be successfully reconciled (i.e., false-negatives defined in \autoref{sec:single_round_pbs}. The distinct elements that are not successfully reconciled in this round, if needed, can be reconciled in later rounds as we will describe in \autoref{sec:multi-rounds}. In this section, we only discuss how to identify the {\it incorrect} distinct elements in the second scenario. Let us use an example to elaborate the second scenario: Assume $(A_i, B_i)$ contains $3$ distinct elements $a_1, a_2, a_3$, then Bob computes $\tilde{s}=a_1\oplus a_2\oplus a_3$ using \autoref{alg:trivial_case} and mistakes it as the distinct element in $(A_i, B_i)$. 

\begin{comment}
============================================

We add a no-communication-cost verification step to check whether a reconciled element is an actual distinct element or not. Note that an actual distinct element of $(A_i, B_i)$ must be in sub-universe $\mathcal{U}_i$. On the other hand, an incorrectly reconciled element (e.g., $\tilde{s}$) can be in any sub-universe with probability $1/n$. So at the end \autoref{subsec:protocol0}, we check whether the reconciled element is in $\mathcal{U}_i$ by the hash function $h$ in hash-partition:

This verfication cannot completely eliminate false-positives, since an incorrectly reconciled element (e.g., $\tilde{s}$) can coincidentally end up in $\mathcal{U}_i$ with probability $1/n$. The chance of false-positives is extremely small using the verification. For instance, if $d=5$ and $n=255$, the probability of the second scenario is only $7.6\times 10^{-6}$. The probability of false-positives using the verfication is $1/n$ times this small probability, which is roughly $3\times 10^{-8}$. {\bf Note that a small probability of false-positives only costs a little waste on set reconciliation when synchronizing objectives (e.g., files), which is acceptable for most applications.}

Even worse, in the second scenario, the false-positives defined in \autoref{sec:single_round_pbs} could happen. For example, if subset pair $(A_i, B_i)$ contains $3$ distinct elements $s_1, s_2, s_3$, then \autoref{alg:trivial_case} computes $\tilde{s}=s_1\oplus s_2\oplus s_3$ and Bob mistakes $\tilde{s}$ as an actual distinct element. The good thing is, the probability of this kind of false-positives is extremely small for small $d$. For instance, if $d=5$ and $n=255$, the probability of the false-positives is only $7.6\times 10^{-6}$. To further reduce the chance of false-positives, we add a no-communication-cost verification step at the end of \autoref{subsec:protocol0} to check whether $\tilde{s}$ is an actual distinct element or not. The verification step works as follows: Given the output $s$ of subset pair $(A_i,B_i)$, if $s\in\mathcal{U}_i$ (i.e., $h(s)=i$), we consider $s$ as an actual distinct element; Otherwise, we consider $s$ as an incorrect output and discard it. 

Note that if $\tilde{s}\in A_i\Delta B_i$, $\tilde{s}$ must be in sub-universe $\mathcal{U}_i$. However, if $\tilde{s}$ is the bitwise \code{XOR} of the distinct elements in $(A_i,B_i)$ (i.e., the second scenario happens), it ends up in $\mathcal{U}_i$ with probablity of only $1/n$. 
%In fact, if we assume the hash-partition described in \autoref{sec:hash_partition} hashes the elements of $\mathcal{U}$ uniformly, independently, and randomly into $n$ sub-universes, the output $s$ in the second scenario will be in a different sub-universe $\mathcal{U}_j (j\neq i)$ with a high probability of $1-\frac{1}{n}$. Hence, this verfication method can further reduce the probability of false-positives by a factor of $\frac{1}{n}$. 
Use the same example (i.e., $d=5$, $n=255$), the probability of this kind of false-positives is reduced from $7.6\times 10^{-6}$ to $3\times 10^{-8}$ by this verification method. 
%{\bf This probability can be further reduced in \autoref{subsec:protocol2}, where PBS does two tiers of hash-partitions. So we can do verification on both of the two hash functions.}

%In some super critical cases (i.e., no false-positive is allowed), we can use a more powerful verification method to completely eliminate false-positives. That is, to check if the output $s$ exists in exactly one of the two sets (i.e., $s\in A\!\setminus\! B$ or $s\in B\!\setminus\! A$). To do so, Bob transmits $s$ along with an identification bit $\mathbbm{1}_{\{s\in B\}}$ to Alice, then Alice checks if $s\in (A\!\setminus\! B)\bigcup (B\!\setminus\! A)$ . This method verification costs additional $d(\log u+1)$ bits of communication overhead. In most applications, this rigorous $0\%$ probability guarantee of false-positives is unnecessary and the probability of the former verification method is small enough, so we use the former in the evaluation. Based on our observation, this kind of false-positives do not happen even once in the evaluation using the former verfication method. In the rest of this paper, we assume Scenario 2 is always correctly verified. 

============================================
\end{comment}

\subsubsection{Multi-round PBS}\label{sec:multi-rounds}

Even if the ideal case does not happen, most of the distinct elements should be distributed into different subset pairs, one distinct element in each, and therefore can be successfully reconciled. So in the first round, even if PBS cannot reconcile all distinct elements, it can reconcile the majority of them.
% (piecewise decodability mentioned in \autoref{sec:intro_oursolution})
Based on this intuition, we generalize PBS to multi-round, so that the distinct elements that are not reconciled yet in the first round can be reconciled in later rounds.  

Without loss of generality, we only describe the second round of multi-round PBS, the reconciliation in the later rounds are similar. Let $\hat{D}_1$ denote the set of reconciled elements in the first round. If set reconciliation is not complete in the first round (i.e., the checksum infers $A\neq B\Delta \hat{D}_1$), then multi-round PBS saves $\hat{D}_1$, which includes correctly and incorrectly reconciled elements as described in \autoref{subsec:exception_hash_partition}, and starts the second round to find (1) the remaining distinct elements; (2) the incorrectly reconciled distinct elements in the first round. In the second round, multi-round PBS reconciles $A$ and $B\Delta \hat{D}_1$ instead of $A$ and $B$ (i.e., $B\leftarrow B\Delta\hat{D}_1$) to rule out all elements that have been reconciled. {\bf It uses a hash function that is different from the one used in the first round for hash-partition, otherwise every remaining distinct element will be hashed into the same subset pair and cause the same exception (described in \autoref{subsec:exception_hash_partition}) that happened in the first round.}

If set reconciliation is complete in the second round, the set of reconciled elements in the second round (denoted as $\hat{D}_2$) should be the union of (1) all distinct elements that have not been reconciled in the first round (i.e., $(A\Delta B)\!\setminus\!\hat{D}_1$); and (2) all incorrectly reconciled elements in the first round (i.e., $\hat{D}_1\!\setminus\!(A\Delta B)$), which is by definition the set difference between $A\Delta B$ and $\hat{D}_1$. Therefore, the overall set difference $A\Delta B$ equals to the set difference between $\hat{D}_1$ and $\hat{D}_2$; Else, multiround PBS saves $\hat{D}_2$ and starts the third round, so on so force. 

{\bf May need this algorithm to show the dynamics, if so, the earlier algorithm needs to change accordingly.}
\IncMargin{1em}
\begin{algorithm}
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
\Input{$A$ and $B$}
\Input{Maximum number of rounds $r$}
\Output{$D$}

$\hat{D},\mbox{ complete} \leftarrow PBS(A,B)$\;

$D \leftarrow \hat{D}$\;

\While{!complete and $r>0$}{
	
	$B \leftarrow B\Delta\hat{D}$\;

	$\hat{D},\mbox{ complete} \leftarrow PBS(A,B)$\;

	$D \leftarrow D\Delta\hat{D}$\;

	$r \leftarrow r-1$\;
}

\caption{Multi-round PBS} \label{proto:multirounds}
\end{algorithm}\DecMargin{1em}

% The idea of multi-round PBS is quite simple: In each round, we discard the reconciled distinct elements in the previous rounds and aim to find the rest distinct elements from the remaining elements. More specifically, the first round of multi-round PBS is just the same as single-round PBS in \autoref{alg:single_round_pbs}. The second round has the same procedures as the first round. One difference is, we update $B$ by $B\leftarrow B\Delta\mathcal{D}$ in the second round, so that (1) Reconciled distinct elements in $\mathcal{D}$ that were contained in $A\Delta B$ are not longer contained in $A\Delta (B\Delta\mathcal{D})$; and (2) The other distinct elements remain in $A\Delta (B\Delta\mathcal{D})$ and can be reconciled later. The other difference is, we use a different hash function for partition (\autoref{step:hash_partition}) in the second round. Later rounds update $B$ in the same way and also use different hash functions. Multi-round terminates if the check in \autoref{step:termination} is correct. The overall set difference $A\Delta B$ is simply the union of reconciled distinct elements in all rounds. 

% A straightforward approach to discard reconciled distinct elements is to remove them from both $A$ and $B$. This approach however incurs additional communication overhead to update $A$, since only Bob learns the partial set difference in \autoref{step:reconcile}. Therefore, we use the approach in \autoref{step:updateb} that only updates $B$. It has another benefit in \autoref{step:termination}, which only needs to transmit the CRC of $A$ from Alice to Bob in the first round. In the later rounds, \autoref{step:termination} can be checked locally by Bob and does not require any additional communication overhead;

Note that the communication overhead in the first round accounts for a large percentage of the total communication overhead in multi-round PBS, since most of the distinct elements (over $95\%$ as we will show in {\bf point to the figure}) should be reconciled in the first round. Therefore, we use the same parameter $n$ in later rounds because otherwise we have to compute a new parameter that can only save tiny communication overhead, even though the number of remaining distinct elements is small and can be reconciled using smaller $n$ with high probability. {\bf Due to the same reason, we can the same expression of the communication overhead in single-round PBS to approximate the communication overhead in multi-round PBS.}

The natural termination condition of multi-round PBS is that all distinct elements are reconciled, which could require a large number of rounds and incur large additional communication overhead (each additional round incurs $d\log n$ bits of additional communication overhead on transmitting BCH codeword). To control the amount of additional communication overhead, we set another termination condition that multi-round PBS runs for at most $r$ rounds (typically $2$ or $3$). This termination condition could cause an `early' termination when some distinct elements have not been reconciled. However, under proper parameter settings (to be discussed in \autoref{sec:parameter_settings}), we can prove that the probability of an `early' termination (i.e., set reconciliation is incomplete in $r$ round) is very small
%, and even if an `early' termination happens, an overwhelming percentage of distinct elements should have been reconciled, which is sufficient for most applications
. For example, when $d=5, n=255, r=2$, an `early' termination happens with probability $4.8\times 10^{-4}$ (how to compute this probability will be elaborated in \autoref{sec:tail_bound}).

For the moment, we assume no incorrectly reconciled distinct elements appears in multi-round PBS, which happens with overwhelming probability as explained in \autoref{subsec:exception_hash_partition}. Then multi-round PBS reconciles the distinct elements gradually round by round. This is the ``piecewise decodability'' mentioned in \autoref{sec:intro_oursolution}. We use the following example to describe it in details: Given two sets $A$, $B$ with $10$ distinct elements (i.e., $d=10$), in the first round, multi-round PBS hashes them into $7$ distinct subset pairs. $6$ distinct elements are hashed into $6$ distinct subset pairs, and the other $4$ distinct elements are hashed into the same subset pair. Then the former $6$ distinct elements are successfully reconciled in the first round and the later $4$ distinct elements remain to be reconciled in the second round, which are hashed into $3$ distinct subset pairs (under a different hash function). $2$ remaining distinct elements are hashed into $2$ distinct subset pairs, and the other $2$ remaining distinct elements are hashed into the same subset pair. Then the former $2$ remaining distinct elements are successfully reconciled in the second round and the later $2$ remaining distinct elements remain to be reconciled in the third round, so on so force. The dynamics of the number of remaining distinct elements (i.e., $10\leadsto 4\leadsto 2\leadsto \cdots$ in the example) is in nature a Markov chain, which will be elaborated and analyzed in \autoref{sec:tail_bound_per_group} to derive a tail bound of success probability (i.e., all distinct elements are reconciled in $r$ rounds) for paramenter settings. 

% In most applications, a high percentage of reconciliation (e.g., $>99\%$ distinct elements are reconciled) is good enough. Therefore, we add another termination condition on the maximum number of rounds (denoted as $r$). The larger $r$ is, the higher percentage of distinct elements will be reconciled. How to set parameters based on $r$ will be elaborated in \autoref{sec:parameter_settings};

% Readers may think the communication overhead of multi-round PBS is proportional to the number of rounds. In fact, the majority of the communication overhead is spent in the first round, since most of the distinct elements (over $95\%$ as we will show in {\bf point to the figure}) are reconciled in the first round. Each additional round only incurs a small amount of additional communication overhead. For example, when $d=10, n=255, |\mathcal{U}|=2^{32}$, assume $8$ distinct elements are reconciled in the first round and the rest $2$ distinct elements are reconciled in the second round. Then the communication overhead in the first round is $432$ bits. That number of the second round is only $160$


%the communication overhead of single-round PBS of $272$ ($2d\log n+d\log |\mathcal{U}|+32$) bits, and each additional round incurs $40$ ($d\log n$) bits of additional communication overhead. 

%among the three components of the communication overhead mentioned in \autoref{sec:communication_overhead_single_PBS}, only the first component (i.e., the BCH codeword) is proportional to the number of rounds. The other two components does not depend on the number of rounds.

% The second component only depends on the total number reconciled elements, which is roughly equal to $d$. The third component, the checksum of $A$, only needs to be sent once in the first round.
%Therefore, the communication overhead of multi-round PBS is only slightly larger than that of single-round PBS when the number of rounds is small (say $3$). For example, when $d=5, n=255, |\mathcal{U}|=2^{32}$, the communication overhead of multi-round PBS of $3$ rounds is $352$ bits, which is roughly $1.3$ times of the communication overhead of single-round PBS ($272$ bits).

% Therefore, each additional round of multi-round PBS only incurs a small amount of additional communication overhead. For example, when $d=5, n=255, |\mathcal{U}|=2^{32}$, the communication overhead of single-round PBS of $272$ ($2d\log n+d\log |\mathcal{U}|+32$) bits, and each additional round incurs $40$ ($d\log n$) bits of additional communication overhead. 

% As we explained in \autoref{sec:reconcile_by_trivial}, the communication overhead in each round is proportional to the number of (remaining) distinct elements, which decreases exponentially as the number of round increase (i.e., the first round reconciles $90\%$ of distinct elements, the second round reconciles $90\%$ of the remaining $10\%$ distinct elements, etc.). So the majority of the communication overhead (i.e., $\approx 90\%$) is in the first round. Therefore, we do not bother to optimize parameters (i.e., smaller $n$) in later rounds to save tiny communication overhead, even though remaining distinct elements become fewer and can be reconciled using smaller $n$;

% The termination condition of multi-round PBS is that all distinct elements are reconciled, which may require many rounds. In most applications, a high percentage of reconciliation (e.g., $>99\%$ distinct elements are reconciled) is good enough. Therefore, we add another termination condition on the maximum number of rounds (denoted as $r$). The larger $r$ is, the higher percentage of distinct elements will be reconciled. How to set parameters based on $r$ will be elaborated in \autoref{sec:parameter_settings};

% Multi-round means multiple round-trip delays. {\bf Thanks for the piecewise decodability of PBS, in almost all practical application scenarios, this tradeoff does not lead to longer response time because the reconciliation of objects identified by the successfully decodable codewords, which constitute the vast majority of all codewords, can run in parallel with the transmissions and decodings of the rest.  In other words, the piecewise decodability effective masks the slightly larger number of communication rounds as far as the response time is concerned.}

\begin{comment}
==============================

The pseudocode of set reconciliation operations in each round is shown as follows:

\IncMargin{1em}
\begin{algorithm}
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
\Input{$A$ and $B^{(in)}$}
\Input{Set of reconciled distinct elements $D^{(in)}$}
\Output{$B^{(out)}$}
\Output{Set of reconciled distinct elements $D^{(out)}$}

% Hash-partition $A^{(in)}$, $B^{(in)}$ into $\{A^{(in)}_i\}_{i=1}^n$, $\{B^{(in)}_i\}_{i=1}^n$ (\autoref{sec:hash_partition})\label{step:hash_partition}\;

% Encode $\{A^{(in)}_i\}_{i=1}^n$, $\{B^{(in)}_i\}_{i=1}^n$ into parity bitmaps (\autoref{sec:parity_bitmap_encoding})\;


% Find those subset pairs (denoted them as $(A^{(in)}_{i_1}, B^{(in)}_{i_1}), ...,(A^{(in)}_{i_k}, B^{(in)}_{i_k})$) that parity bits differ (\autoref{sec:BCH_code})\;

Run single-round PBS on $A$ and $B^{(in)}$ to obtain the (partial) set difference $\mathcal{D}$\label{step:reconcile} \;

$D^{(out)} \leftarrow D^{(in)}\bigcup \mathcal{D}$\label{step:updated}\;

$B^{(out)} \leftarrow B^{(in)}\Delta\mathcal{D}$\label{step:updateb}\;

Check whether the set reconciliation is complete by comparing $A$ to $B^{(out)}$ (via CRC)\label{step:termination}\;

\caption{Set reconciliation operations of PBS in each round} \label{proto:multirounds}
\end{algorithm}\DecMargin{1em}

In \autoref{proto:multirounds}, the output $B^{(out)}$ in the $r^{th}$ round is the input $B^{(in)}$ in the $(r+1)^{th}$ round. $D^{(in)}$ and $D^{(out)}$ have the same relationship, and they denote the set of reconciled distinct elements before and after a round. $B^{(in)}$ and $D^{(in)}$ are initialized as $B$ and $\emptyset$ respectively. We omit the currect number of round $r$ in \autoref{proto:multirounds}, since the operations in different rounds are exactly the same. Due to the same reason, we only elaborate the operations in the first round: First, Alice and Bob reconcile $A$ and $B^{(in)}$ $(=B)$ using single-round PBS and Bob obtains the (partial) set difference $\mathcal{D}$ (\autoref{step:reconcile}); Second, Bob updates the set of reconciled distinct elements by merging it with $\mathcal{D}$ (\autoref{step:updated}); Third, Bob updates $B^{(in)}$ $(=B)$ to $B^{(out)}$ as \autoref{step:updateb} shows, such that (1) The reconciled distinct elements in $\mathcal{D}$ that are contained in $A\Delta B^{(in)}$ are not longer contained in $A\Delta B^{(out)}$; and (2) The distinct elements that are not successfully reconciled remain in $A\Delta B^{(out)}$ and can be reconciled in later rounds; Finally, we check whether all distinct elements are reconciled. Note that if it is true, $B^{(out)}$ should be the same as $A$ and multi-round PBS should terminate. We use a $32$-bit CRC (Cyclic Reduncancy Check) to check if $B^{(out)}=A$ in our evaluation. {\bf To achieve higher confidence, we can certainly use longer CRC (e.g., 64-bit). }

{\bf Remarks:}

(1) In each round, hash-partition in \autoref{sec:hash_partition} uses different hash functions, so that the remaining distinct elements from the last round will be hashed into different subset pairs with high probability;

(2) A straightforward approach to discard reconciled distinct elements is to remove them from both $A$ and $B$. This approach however incurs additional communication overhead to update $A$, since only Bob learns the partial set difference in \autoref{step:reconcile}. Therefore, we use the approach in \autoref{step:updateb} that only updates $B$. It has another benefit in \autoref{step:termination}, which only needs to transmit the CRC of $A$ from Alice to Bob in the first round. In the later rounds, \autoref{step:termination} can be checked locally by Bob and does not require any additional communication overhead;

(3) As we explained in \autoref{sec:reconcile_by_trivial}, the communication overhead in each round is proportional to the number of remaining distinct elements, which decreases exponentially as the number of round increase (i.e., the first round reconciles $90\%$ of distinct elements, the second round reconciles $90\%$ of the remaining $10\%$ distinct elements, etc.). So the majority of the communication overhead (i.e., $\approx 90\%$) is in the first round. Therefore, we do not bother to optimize parameters (i.e., smaller $n$) in later rounds to save tiny communication overhead, even though remaining distinct elements become fewer and can be reconciled using smaller $n$;

(4) One termination condition of Multi-round PBS is $B^{(out)}=A$, which refers that all distinct elements are reconciled. In most applications, a high percentage of reconciliation (e.g., $>99\%$ distinct elements are reconciled) is good enough. Therefore, we add another termination condition of the maximum number of rounds (denoted as $r$). The larger $r$ is, the higher percentage distinct elements will be reconciled, and the smaller $n$ is required. How to set parameters (e.g., $n$) based on $r$ will be elaborated in \autoref{sec:parameter_settings};

(5) Multi-round means multiple round-trip delays. {\bf Thanks for the piecewise decodability of PBS, in almost all practical application scenarios, this tradeoff does not lead to longer response time because the reconciliation of objects identified by the successfully decodable codewords, which constitute the vast majority of all codewords, can run in parallel with the transmissions and decodings of the rest.  In other words, the piecewise decodability effective masks the slightly larger number of communication rounds as far as the response time is concerned.}

==============================

\end{comment}

% (3) Readers may wonder in the later rounds, most distinct elements should be reconciled, and the rest distinct elements could be reconciled using degraded parameters (i.e., smaller $n$ and $t$). In fact, degrade parameters in later rounds cannot save much communication overhead, since the majority of it is spent in the first round (i.e., $>90\%$). Therefore, we use the same parameters (i.e., $n,t$) among all rounds in multi-rounds PBS;

% (4) The number of remaining distinct elements decreases exponentially as the number of round increase (i.e., the first round reconciles $90\%$ of distinct elements, the second round reconciles $90\%$ of the remaining $10\%$ distinct elements, etc.). 
% (4) The termination condition of Multi-rounds PBS is $B^{(out)}=A$ to reconcile all distinct elements. In some applications,  


% The output $B^{(out)}$ in the $r^{th}$ round is the input $B^{(in)}$ in the $(r+1)^{th}$ round. $D^{(in)}$ and $D^{(out)}$ are similarly defined. $B^{(in)}$ and $D^{(in)}$ are initialized as $B$ and $\emptyset$ respectively. Since and $D$ are updated in each round, so we use $B^{(in)}$ to denote the input and $B^{(out)}$ to denote the output respectively.  Specifically, in the first round, we initialize $B^{(in)}$ and $D^{(in)}$ as $B$ and $\emptyset$ respectively. we first use the single-round scheme 

% Then we run our (single-round) scheme on the updated two sets (i.e., after removing reconciled distinct elements) using a different (independent) hash-partition function from previous rounds, so that the rest distinct elements are hashed into different subset pairs (i.e., the ideal case) with high probability. At the end of each round, we check whether the set reconciliation is complete (i.e., all distinct elements are found) by computing the bitwise \code{XOR} of the remaining elements in $A$ and $B$ 
 

% This {\bf multi-rounds} scheme can significantly increase the success probability (i.e., the probability that all distinct elements are reconciled). Readers may wonder in the later rounds, most distinct elements should be reconciled, and the rest distinct elements could be reconciled using degraded parameters (i.e., smaller $n$ and $t$). In fact, degrade parameters in later rounds cannot save much communication overhead, since the majority of it is spent in the first round (i.e., $>90\%$). Therefore, we use the same parameters (i.e., $n,t$) among all rounds in our evaluation. 
% %The tradeoff between the number of rounds and the communication overhead per rounds will be elaborated in \autoref{sec:tail_bound}. In our evaluation, $r=2,3$ rounds are enough to achieve an extremely high success probability. 

% Readers may think the cost (i.e., communication overhead and the computational complexity) of this multi-rounds scheme is proportional to the number of rounds (denoted as $r$) and increases linearly with $r$. In fact, the cost of each round is roughly proportional to the number of remaining distinct elements, which decreases exponentially as $r$ increases (i.e., the first round reconciles $99\%$ of distinct elements, the second round reconciles $99\%$ of the remaining $1\%$ distinct elements, etc.). So the cost of this multi-rounds scheme is only slightly larger than that of the single-round scheme. Furthermore, as we explained in \autoref{sec:intro}, {\bf from intro thanks for the piecewise decodability of our solution, in almost all practical application scenarios, this tradeoff does not lead to longer response time because the reconciliation of objects identified by the successfully decodable codewords, which constitute the vast majority of all codewords, can run in parallel with the transmissions and decodings of the rest.  In other words, the piecewise decodability effective masks the slightly larger number of communication rounds as far as the response time is concerned.} 

\begin{comment}

\subsection{Baseline Scheme}\label{subsec:protocol1} 

Note that the set difference $A\Delta B$ can contain more than 1 elements (i.e., $d>1$), and \autoref{alg:trivial_case} cannot reconcile $A$ and $B$ directly in this case. Therefore, we propose a baseline scheme building upon~\autoref{alg:trivial_case} that also works when $d>1$: First, we partition the element universe $\mathcal{U}$ into $n$ sub-universes $\mathcal{U}_1, \mathcal{U}_2, \cdots, \mathcal{U}_n$. Denote $A_i \triangleq A\bigcap \mathcal{U}_i$ and $B_i \triangleq B\bigcap \mathcal{U}_i$ for $i=1,2,\cdots,n$. Then $\{A_i\}_{i=1}^n$ and $\{B_i\}_{i=1}^n$ are partitions of $A$ and $B$ respectively. Furthermore, $\Phi\triangleq\{A_i\Delta B_i\}_{i=1}^n$ is a partition of $A\Delta B$. 

Assume the {\bf ideal case} happens, in which each subset pair $(A_i, B_i)$ contains at most one distinct element ({\it i.e.,} $|A_i\Delta B_i|\!\leq\!1$), we use \autoref{alg:trivial_case} to reconcile each subset pair and obtain $A_i\Delta B_i$ for $i=1,2,\cdots,n$. The overall set difference $A\Delta B$ is simply their union $\bigcup_{i=1}^n \big{(}A_i\Delta B_i\big{)}$. 

In the first step of the baseline scheme, we can use a hash function $h(\cdot): \mathcal{U}\rightarrow \{1,2,\cdots,n\}$ to partition the universe $\mathcal{U}$ into $n$ sub-universes: $\mathcal{U}_i=\{s\mid s\in \mathcal{U} \mbox{ and } h(s)=i\}$ for $\forall i=1,2,\cdots,n$. And the hash function $h(\cdot)$ can be predetermined between Alice and Bob and does not require additional communication cost.

This hash-partition can be modeled as a {\it balls-into-bins problem}, in which the distinct elements are viewed as balls and the subset pairs are viewed as bins. The hash-parition basically throws (hashes) $d$ balls (distinct elements) uniformly and randomly into $n$ bins (subset pairs). The aforementioned ideal case in this context becomes, after throwing $d$ balls uniformly and randomly into $n$ bins, each bin receives at most 1 ball (i.e., $d$ nonempty bins have 1 ball in each and the rest $n-d$ bins are empty). {\bf It may remind readers about the Birthday problem. And the ideal case can be analogous to the case that no people share the same birthday.} The ideal case happens with a probability of $p=\frac{n\,!}{(n-d)\,!n^d}\!=\!\prod_{k=1}^{d - 1}(1 - \frac{k}{n})\!\approx\! e^{-\frac{d(d-1)}{2n}}$ when $d\!\ll\!n$. In other words, $n$ must be $\Omega(d^2)$ to ensure the ideal case happens with a nontrivial probability.  Note that the communication overhead of the baseline scheme is proportional to $n$, as each subset pair requires communication of a bitwise \code{XOR} in \autoref{alg:trivial_case}. So this communication overhead increases at least quadratically as $d$ increases. 

In fact, this communication overhead can be significantly reduced: In the ideal case, $n-d$ out of $n$ subset pairs are identical ones, and only $d (\ll n)$ out of $n$ subset pairs contain distinct elements (one distinct element in each of the $d$ subset pairs) and need to be reconciled. If we can identify these $d$ subset pairs (with a tiny additional communication overhead) and only reconcile them, the overall communication overhead will be significantly reduced from $\Omega(d^2)$ to $O(d)$. Based on this intuition, we propose our scheme in \autoref{sucsec:our-scheme}, which uses Parity Bitmap Sketch (PBS) and Error Correction Coding (ECC) to identify those subset pairs with a tiny additional communication overhead. 

Note that the ideal case does not always happen. However, we can ensure that the ideal case happens with high probability by properly selecting $n$ based on $d$ (i.e., $n=\Omega(d^2)$). Furthermore, as we will describe in \autoref{subsec:nonideal}, even if the ideal case does not happen (i.e., some distinct elements are hashed into the same subset pair), most of the distinct elements should be distributed into different subset pairs and therefore can be reconciled. So the baseline scheme, even cannot reconcile all of the distinct elements, can still reconcile the majority of them. Based on this property, we will extend our scheme from single-round to multi-rounds in \autoref{subsec:nonideal} to further increase the probability of reconciling all distinct elements. 

For general cases ({\it i.e.,} $t=|A\Delta B|$ is an arbitrary number), we have a straightforward strawman scheme building upon~\autoref{alg:trivial_case}, which works as follows: First, Alice and Bob choose some hash function $h(s): \mathcal{U} \rightarrow \{0,1,\cdots,2^{32}-1\}$ to partition $A$ and $B$ into $m$ subsets $A_1,A_2,\cdots,A_m$ and $B_1,B_2,\cdots,B_m$ respectively:

\begin{align}
s\in A_i & \mbox{ iff } s\in A \mbox{ and } h(s)=i\!\mod m, \nonu{}mber\\
s\in B_i & \mbox{ iff } s\in B \mbox{ and } h(s)=i\!\mod m. \nonumber
\end{align} 

{\bf call a subset pair -> partition?} Since Alice and Bob use the same hash function for partition, common elements (i.e., elements in $A\cap B$) are always hashed into the same subset pair $(A_i, B_i)$. And the set difference of each subset pair only contains distinct elements (i.e., elements in $A\Delta B$): $A_i\Delta B_i \subset A\Delta B$. In the ideal case, with a sufficient large $m$, each subset pair $(A_i, B_i)$ contains at most one distinct element ({\it i.e.,} $|A_i\Delta B_i|\!\leq\!1$). Then \autoref{alg:trivial_case} can reconcile each subset pair and obtain $A_i\Delta B_i$ for $i=1,2,\cdots,m$. The overall set difference $A\Delta B$ is simply their union $\bigcup_{i=1}^m \big{(}A_i\Delta B_i\big{)}$. The selection of hash function $h(s)$ can be predetermined between Alice and Bob and it does not require additional communication cost.

%To make sure Alice and Bob use the same hash function for partition, we let them pre-agree on some universal hash family (e.g., \code{xxHash}~\cite{Collet_xxHashExtremelyfast_}) and a common selection order, and each time they choose a hash function from the family in the same order. Note that we can also let Alice generates a hash function and send it to Bob. The hash function that Alice and Bob choose for partition can be either generated by 

This hash-partition is in nature a {\it balls-into-bins model}. We can view the distinct elements as balls and the subset pairs as bins. The hash-parition basically throws (hashes) $t$ balls (distinct elements) uniformly and randomly into $m$ bins (subset pairs). The aforementioned ideal case in this context is, with a sufficient large number of bins, each bin receives at most 1 ball. The strawman scheme works correctly if and only if the ideal case happens, which has a probability of $\frac{m\,!}{(m-t)\,!m^t}\!=\!\prod_{k=1}^{t - 1}(1 - \frac{k}{m})\!\approx\! e^{-\frac{t(t-1)}{2m}}$. In other words, to ensure the strawman scheme works correctly with a probability of $p$, it roughly requires $m \!=\!\lceil \frac{t(t-1)}{-2\ln p}\rceil$ subset pairs. 

Note that the communication overhead of this strawman scheme is proportional to the number of subset pairs $m$, as each subset pair requires communication of an \code{XOR} sum in \autoref{alg:trivial_case} during the reconciliation. When $t$ is small, a small communication cost can guarantee that the strawman scheme works correctly with high probability. For instance, when $t=5$, $m=95$ subset pairs are sufficient for the strawman scheme to work correctly with a probability of $90\%$. However, when $t$ is relatively large, it requires a huge communication cost to ensure the strawman scheme works correctly. For instance, when $t=1,000$, it requires $m=4,740,865$ subset pairs to guarantee a success probability of $90\%$. 

In fact, the majority of subset pairs are identical ones and do not need to reconcile. And only a small portion of them contain distinct elements. If we can identify those subset pairs that contain distinct elements and only reconcile them, the communication cost could be significantly reduced. Our scheme is based on this intuition and uses parity bitmap sketch and BCH code to identify the subset pairs, which we will elaborate in \autoref{sucsec:our-scheme}. 

%To distribute balls as uniformly as possible and maximize the probability of the ideal case, we choose a uniform hashing function $h$ that throws balls uniformly and randomly into bins: $$\mathbb{P}[h(s)=i]=\frac{1}{m} \mbox{ for } \forall i=1,2,\cdots,m, \forall s\in U$$.

%Note that the probability of the ideal case is $\frac{m\,!}{(m-t)\,!m^t}\!=\!\prod_{k=1}^{t - 1}(1 - \frac{k}{m})\!\approx\! e^{-\frac{t(t-1)}{2m}}$. Hence, at least $\lceil \frac{t(t-1)}{-2\ln p}\rceil$ bins are required to ensure that this probability is at least $p$. In other words, to ensure that the ideal case happens with a probability of $p$, the strawman scheme roughly requires $m \!=\!\lceil \frac{t(t-1)}{-2\ln p}\rceil$. For example, suppose $t\!=\!$\num{1000}, %and $p\!=\!0.01$, this strawman scheme roughly requires $m\!=\!$\num{720626} bins (partitions) to ensure that $|A_i\Delta B_i|\!\leq\!1$ (for any $i=1,2,\cdots,m$) holds with probability $50\%$.  

% A straightforward strawman scheme building upon~\autoref{alg:trivial_case} 
% to reconcile two sets $A$ and $B$ in general 
% ({\it i.e.,} $|A\Delta B|$ is an arbitrary number) is the following: 
% Uniformly randomly partition $A$ and $B$ into $m$ subsets ($A_1,A_2,\cdots,A_m$ 
% and $B_1,B_2,\cdots,B_m$) so that the set difference 
% $A_i\Delta B_i$ of each subset pair $(A_i, B_i)$ contains at most one element 
% ({\it i.e.,} $|A_i\Delta B_i|\!\leq\!1$) {\it w.h.p.} ({\it i.e.,} with high probability), 
% and then reconcile each subset pair with~\autoref{alg:trivial_case}. 

% Now let us analyze this strawman scheme using the {\it balls-into-bins model}. 
% Assume that sets $A$ and $B$ have $t$ elements in their set difference, {\it i.e.,} $|A\Delta B|\!=\!t$. 
% These $t$ elements can be viewed as $t$ balls and the $m$ partitions (subset pairs) can be viewed as 
% $m$ bins. The random partition process in this strawman scheme can be modeled as throwing 
% $t$ balls into $m$ bins in the following manner: Each ball goes into a 
% uniformly random bin and independently of other balls. %so that each bin contains at most one ball, {\it w.h.p.}  
% The probability that each bin contains at most one ball is  
% $\frac{m\,!}{(m-t)\,!m^t}\!=\!\prod_{k=1}^{t - 1}(1 - \frac{k}{m})\!\approx\! e^{-\frac{t(t-1)}{2m}}$. 
% Hence, at least $\lceil \frac{t(t-1)}{-2\ln p}\rceil$ bins are required 
% to ensure that this probability is at least $p$. In other words, to ensure 
% that each bin contains at most one ball with a probability of $p$, 
% the strawman scheme roughly requires $m \!=\!\lceil \frac{t(t-1)}{-2\ln p}\rceil$. 
% For example, suppose $t\!=\!$\num{1000}, %and $p\!=\!0.01$, 
% this scheme roughly requires $m\!=\!$\num{108469} bins (partitions) to 
% ensure that $|A_i\Delta B_i|\!\leq\!1$ (for any $i=1,2,\cdots,m$) holds with probability $0.01$.  

% We note that the communication overhead of this strawman scheme is proportional to 
% $m$ ($\!\gg\! t$), as each partition (subset pair) requires communication of an \code{XOR} sum during the reconciliation. 
% This communication overhead is much higher than that of the optimal scheme, which only requires 
% to exchange the elements in the set difference (assuming an oracle tells it which elements belong to 
% the set difference), {\it i.e.,} proportional to $t$. In the example above, assuming each element takes 4 bytes, 
% the communication overhead of the strawman scheme is $4m$ bytes ($\!\approx\! \num{423.71}\,$KB) to ensure 
% a success rate of only 0.01 ({\it i.e.,} with a probability of $0.0.1$, all elements in 
% the set difference are successfully reconciled), 
% which is approximately 2 orders of magnitude higher than $4t$ bytes ($\!=\!\num{3.90}\,$KB), the communication 
% overhead of the optimal scheme. 

\subsection{Our Scheme: The Preliminary Version}\label{sucsec:our-scheme}

Like the baseline scheme, our scheme also hash-partitions the two sets $A$ and $B$ into $n$ subset pairs. The difference is, instead of reconciling all subset pairs using \autoref{alg:trivial_case}, our scheme identifies the subset pairs that contains distinct elements and only reconciles them. Since the hash-partition and set reconciliation on each subset pair using \autoref{alg:trivial_case} have been described in \autoref{subsec:protocol1}, we only elaborate how to identify the subset pairs that contain distinct elements in this section. 

The general idea of identification is very simple: First, we {\bf encode} each subset into $1$ bit, such that in the ideal case, for $\forall i=1,2,\cdots,n$:

\begin{itemize}
	\item The codewords (bits) of $A_i$ and $B_i$ are different if and only if subset pair $(A_i, B_i)$ contains $1$ distinct element;
	\item The codewords (bits) of $A_i$ and $B_i$ are the same if and only if subset pair $(A_i, B_i)$ contains no distinct element;
\end{itemize}

Second, we {\bf compare} the codewords of each subset pair. And the subset pairs that contain distinct elements are the ones with different codewords (bits). We will describe the two steps in details in \autoref{sec:parity_bitmap_encoding} and \autoref{sec:BCH_code} respectively.

\subsubsection{Parity Bitmap Encoding}\label{sec:parity_bitmap_encoding}

In our scheme, we use {\it parity encoding} to encode each subset into a parity bit. More specific, it encodes a subset as ``1'' if it contains odd number of elements, and as ``0'' otherwise. And it satisfies the aforementioned requirements in the ideal case:

\begin{itemize}
	\item If subset pair $(A_i, B_i)$ contains $1$ distinct element, the corresponding two subsets $A_i$ and $B_i$ differ exactly one element, which implies that $||A_i|\!-\!|B_i||\!=\!1$. Hence, if $|A_i|$ ({\it i.e.,} number of elements in $A_i$) is odd (or even), then $|B_i|$ must be even (or odd). And the parity bits of $A_i$ and $B_i$ will be different;
	\item If subset pair $(A_i, B_i)$ contains no distinct element, the corresponding two subsets $A_i$ and $B_i$ should be the same and therefore contain the same number of elements. Hence, if $|A_i|$ is odd (or even), then $|B_i|$ must be odd (or even). And the parity bits of $A_i$ and $B_i$ will be the same;
\end{itemize}

Using parity encoding, the $n$ subsets of $A$ are encoded as a bit string $A[1..n]$ in $\{0,1\}^n$, 
where the $i$-th bit $A[i]$ in $A[1..n]$ corresponds to the parity encoding bit of $A_i$. Similarly, the $n$ subsets of $B$ are similarly 
encoded as a bit string $B[1..n]$. We call $A[1..n]$ ($B[1..n]$) the {\it parity bitmap} of $\{A_i\}_{i=1}^n$ ($\{B_i\}_{i=1}^n$). In the ideal case, $A[1..n]$ and $B[1..n]$ differ at $d$ different bit-positions, which corresponds to the $d$ subset pairs that contain distinct elements. And our scheme only reconciles those subset pairs that the parity bits are different. We will describe the nonideal case (i.e., some subset pair contains more than 1 distinct elements) in \autoref{subsec:nonideal}.

\subsubsection{Parity Bitmap Comparison Using BCH Code}\label{sec:BCH_code}

A straightforward approach to compare the parity bitmaps is to let Bob send the complete parity bitmap $B[1..n]$ to Alice, then Alice compares $A[1..n]$ with $B[1..n]$ locally. This approach has a communication overhead of $n$ bits, which is unnecessarily high. As we discussed in~\autoref{subsec:protocol0}, $d$ is usually much smaller than $n$. It means $A[1..n]$ and $B[1..n]$ differ only at a tiny portion of bits. Therefore, we can view $A[1..n]$ as a corrupted message of $B[1..n]$ with $d$ corrupted bits, and the bit-positions of the $d$ corrupted bits basically correspond to the $d$ subset pairs that contain distinct elements. The detection of corrupted bits, on the other hand, can be solved by Error-Correction Code (ECC)~\cite{Lin_ErrorControlCoding_1983}. And our scheme uses BCH code~\cite{Lint_IntroductionCodingTheory_1998} to encode the parity bitmap and detect the $d$ corrupted bits.

More specific, after the parity bitmap encoding, Bob uses a $d$-error-correcting systematic BCH code to encode $B[1..n]$ into an $n+d\log n$ codeword, in which the first $n$ bits are $B[1..n]$ (property of systematic BCH code). Then Bob sends the rest $d\log n$ bits, which we denote as {\it parity bitmap sketch (PBS)}, to Alice. Upon the received PBS and $A[1..n]$ (corrupted message), Alice uses the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} to detect the $d$ corrupted bits in $A[1..n]$. The communication overhead of this approach is $d\log n$ bits (i.e., length of PBS), which is much smaller than that of the straightforward approach ($n$ bits, when $d\!\ll\!n$). On the other hand, the computational complexity of the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} is $O(d^2\log^2 n)$. 

\subsubsection{Exceptional Handling and Multi-rounds}\label{subsec:nonideal}

As we described in \autoref{subsec:protocol1}, the ideal case does not always happen, which means some subset pair may contain more than 1 distinct elements and cannot be successfully reconciled by \autoref{alg:trivial_case}. Due to the parity encoding, we can classify such subset pair into the following two scenarios:

\begin{itemize}
    \item Scenario 1: If a subset pair $(A_i, B_i)$ contains even number ($\geq 2$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be the same and our scheme will not reconcile the subset pair. Hence, the distinct elements in the subset pair will not be reconciled;
    \item Scenario 2: If a subset pair $(A_i, B_i)$ contains odd number ($\geq 3$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be different and our scheme will reconcile the subset pair using \autoref{alg:trivial_case}. However, as we described in \autoref{subsec:protocol0}, when a subset pair contains more than 1 distinct elements, \autoref{alg:trivial_case} will output the bitwise \code{XOR} of them as the `distinct element', which is not a real distinct element with high probability;
\end{itemize}

In both scenarios, the distinct elements in the subset pair cannot be reconciled. Even worse, in the second scenario, a false-positive could happen (i.e., the output of \autoref{subsec:protocol0} is not a real distinct element). However, as we will analyze in \autoref{sec:tail_bound} and show in {\bf the evaluation section}, the second scenario barely happens both theoretically and empirically. To further reduce the chance of false-positives, we add a verification step at the end of \autoref{subsec:protocol0} to check whether the output of \autoref{subsec:protocol0} $s$ is a real distinct element or not. The verification step works as follows: Given the output $s$ of subset pair $(A_i,B_i)$, if $s\in\mathcal{U}_i$ (i.e., $h(s)=i$), we consider $s$ as a real distinct element; Otherwise, we consider $s$ as an incorrect output and discard it. 

Note that if $s$ is a real distinct element of $(A_i,B_i)$, $s$ must be in sub-universe $\mathcal{U}_i$. However, if $s$ is the bitwise \code{XOR} of the distinct elements in $(A_i,B_i)$ (i.e., the second scenario happens), $s$ could be in any sub-universe other than $\mathcal{U}_i$. In fact, if we assume the hash-partition described in \autoref{subsec:protocol1} hashes the elements of $\mathcal{U}$ uniformly, independently, and randomly into $n$ sub-universes, the output $s$ in the second scenario will be in a different sub-universe $\mathcal{U}_j (j\neq i)$ with a high probability of $1-\frac{1}{n}$. Hence, this verfication step can reduce the chance of false-positives by a factor of $\frac{1}{n}$. 

Even if the ideal case does not happen, most of the distinct elements should be distributed into different subset pairs and therefore can be reconciled. So our scheme, even cannot reconcile all of the distinct elements, can still reconcile the majority of them (piecewise decodability). To reconcile the rest distinct elements, we can just run our scheme for another round under a different hash-partition function, so on so force. This {\bf multi-rounds} scheme can significantly increase the success probability (i.e., the probability that all distinct elements are reconciled). Readers may wonder in the later rounds, most distinct elements should be reconciled, and the remaining could be reconciled using degraded parameters (i.e., smaller $n$ and $t$). In fact, degrade parameters in later rounds cannot save much communication overhead, since the majority of it is spent in the first round (i.e., $>90\%$). Therefore, we use the same parameters (i.e., $n,t$) among all rounds in our evaluation.
%The tradeoff between the number of rounds and the communication overhead per rounds will be elaborated in \autoref{sec:tail_bound}. In our evaluation, $r=2,3$ rounds are enough to achieve an extremely high success probability. 

Readers may think the cost (i.e., communication overhead and the computational complexity) of this multi-rounds scheme is proportional to the number of rounds (denoted as $r$) and increases linearly with $r$. In fact, the cost of each round is roughly proportional to the number of remaining distinct elements, which decreases exponentially as $r$ increases (i.e., the first round reconciles $99\%$ of distinct elements, the second round reconciles $99\%$ of the remaining $1\%$ distinct elements, etc.). So the cost of this multi-rounds scheme is only slightly larger than that of the single-round scheme. Furthermore, as we explained in \autoref{sec:intro}, {\bf from intro thanks for the piecewise decodability of our solution, in almost all practical application scenarios, this tradeoff does not lead to longer response time because the reconciliation of objects identified by the successfully decodable codewords, which constitute the vast majority of all codewords, can run in parallel with the transmissions and decodings of the rest.  In other words, the piecewise decodability effective masks the slightly larger number of communication rounds as far as the response time is concerned.} 

\end{comment}

\subsection{PBS: When $d$ is large}\label{subsec:protocol2}

===============================
To differentiate from the PBS described in \autoref{sucsec:our-scheme}, we refer it as PBS-basic in this section. Note that the BCH decoding computational complexity is $O(d^2\log ^2 n)$, which is $\Omega(d^2\log^2 d)$ when $n=\Omega(d^2)$, with the state-of-the-art decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019}. It is too large in PBS-basic for large $d$. To overcome this drawback and generalize PBS-basic for large $d$, we partition sets $A$ and $B$ each into $d/\delta$ subsets (which we call {\it groups} to distinguish from subsets) for some small integer $\delta$ (say $5$) and reconcile the $d/\delta$ group pairs respectively using PBS-basic. After this partition, each group has $\delta$ distinct elements on average. The BCH decoding computational complexity of each group pair can be considered as $O(1)$, since $\delta$ is a small number. As a result, the overall computational complexity of PBS is reduced from $O(d^2\log ^2 n)$ to $O(d)$. 

% To differentiate from the PBS described in \autoref{sucsec:our-scheme}, we refer it as PBS-basic in this section. PBS-basic is not suitable for large $d$ for two reasons: First, its communication overhead is asymptotically $O(d\log n)\!=\!O(d\log d)$ (since $n=\Omega(d^2)$), which is not asymptotically optimal. Second, the decoding computational complexity is proportional to $d^2$ with the state-of-the-art decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} for BCH codes, which is too high when $d$ is large. To overcome these two drawbacks, we use a simple algorithmic trick to (1) reduce the communication overhead from $O(d\log d)$ to $d\log u \!+\! O(d)$; (2) reduce the decoding computational complexity from $O(d^2)$ to $O(d)$. 

Now, we describe the generalized PBS in details: In the first step, we hash-partition $A$ and $B$ (by some hash function $h_1(\cdot)$) into $g$ group pairs, just like what we did in \autoref{sucsec:our-scheme}. The objective of this partition is however different: In \autoref{sucsec:our-scheme}, we aim to ensure each subset pair contains at most $1$ distinct element (i.e., the ideal case) with high probability; Here we aim to make each group pair contains roughly $\delta$ distinct elements for some small constant $\delta$ (say $5$) by setting $g=d/\delta$. 
%To differentiate the $g$ subset pairs here from those in \autoref{sec:hash_partition}, we call them the $g$ {\bf groups} in the sequel. 
In the second step, we just apply PBS-basic (described in \autoref{sucsec:our-scheme}) to reconcile each group pair and obtain the distinct elements. 
================================

To differentiate from the PBS described in \autoref{sucsec:our-scheme}, we refer it as PBS-basic in this section. When $d$ is large (more than several), we hash-partition set $A$ and $B$ into groups, such that each group pair contains $\delta$ distinct elements on average for small $\delta$ (say $5$), as described in \autoref{sec:larged}. Then each group pair can be reconciled by PBS-basic.

When describing the PBS-basic in \autoref{sucsec:our-scheme}, we assume that the number of distinct elements is precisely known. We set the error-correction capability of the BCH code (denoted as $t$) just enough to correct $d$ errors (i.e., $t=d$). However, due to the randomness of hash-partition, $d_i$, the number of distinct elements in the $i^{th}$ group pair, is a Binomial random variable $Binomial(d,1/g)$ with expectation of $\delta$ $(=d/g)$ for $i=1,2,...,g$, which cannot be precisely known without a huge amount of additional communication overhead. Hence, we can no longer set the error-correction capability of the BCH code for each group pair based on the exact number of distinct element in it, as we did in \autoref{sucsec:our-scheme}. Instead, we set a universal error-correction capability $t$ (say $2.5\delta$) for all group pairs, which is sufficient for all group pairs (i.e., $t\geq d_i$ for $i=1,2,...,g$) with high probability. We will discuss the case that $d_i>t$ in \autoref{sec:BCH_exception}.

%This assumption in general does not hold: 
% Let $d_i$ denote the number of distinct elements in Group $i$. Due to the property of hash-partition, each $d_i$ is a Binomial random variable $Binomial(d,1/g)$ with expectation of $\delta$ $(=d/g)$. Even if $d$ is precisely known, each $d_i$ is not. To ensure the error-correction capability $t$ is sufficient for each group (i.e., $d_i\leq t$) with high probability, we leave some safety margin for the randomness of $d_i$ and conservatively set $t$ roughly $2.5\delta$ (the factor $2.5$ varies depend on other parameters, which will be discussed in \autoref{sec:parameter_settings}), so that $Pr[d_i>t]$ is tiny. We will discuss the case that $d_i>t$ in \autoref{sec:BCH_exception}.

Note that the `safety margin' between $t$ and $\delta$ (i.e., the average number of distinct elements in a group pair) incurs additional communication overhead on transmitting BCH codeword: In the perfect scenario (i.e., $\{d_i\}_{i=1}^g$ is precisely known), the average communication overhead on transmitting BCH codeword per group pair is $\delta\log n$; On the other hand, when we set $t$ to be the error-correction capability for each group pair, then the average overhead becomes $t\log n$, which is roughly $2.5$ times of that in the perfect scenario (when $t$ is roughly $2.5\delta$). Readers may wonder if we can reduce this additional communication overhead by using some technique to estimate $\{d_i\}_{i=1}^g$ (e.g., ToW estimator in \autoref{subsec:ToW}), so that we can set the error-correction capability of each group more wisely and save some waste on the safety margin. However, to achieve that, the estimation on $\{d_i\}_{i=1}^g$ must be in high precision, which requires a much higher communication overhead than the savings. 

% Note that this safety margin incurs additional communication overhead on transmitting BCH codeword: In the perfect scenario (i.e., $\{d_i\}_{i=1}^g$ is precisely known), the average communication overhead on transmitting BCH codeword per group is $\delta\log n$; On the other hand, when we set $t$ to be the error-correction capability for each group, then the average overhead becomes $t\log n$, which is roughly $2.5$ times of that in the perfect scenario (when $t$ is roughly $2.5\delta$). Readers may wonder if we can reduce this additional communication overhead by using some technique to estimate $\{d_i\}_{i=1}^g$ (e.g., ToW estimator in \autoref{subsec:ToW}), so that we can set the error-correction capability of each group more wisely and save some waste on the safety margin. However, to achieve that, the estimation on $\{d_i\}_{i=1}^g$ must be in high precision, which requires a much higher communication overhead than the savings. 

The same algorithmic trick (i.e., hash-partition two sets each into groups) can also be implemented in PinSketch~\cite{Dodis_PinSketch_2008} to reduce it computational complexity from $O(d^2\log^2 |\mathcal{U}|)$ to $O(d)$. However, it will encounter the same randomness problem and have to set up a safety margin on the error-correction capability. This safety margin will incur much more additional communication overhead on PinSketch than on our scheme: Considering the average communication overhead per group pair, the additional overhead caused by the safety margin is $(t-\delta)\log n$ in PBS and $(t-\delta)\log |\mathcal{U}|$ in PinSketch. The later is roughly $4$ times of the former under the default setting ($n=255, |\mathcal{U}|=2^{32}$). Note that the optimal communication overhead to reconcile $d$ distinct elements is $\delta\log |\mathcal{U}|$. Use the same example in \autoref{sec:intro}, when $\delta=5, n=255, u=2^{32}, t=2.5\delta$, the overhead of PinSketch using the algorithmic trick is $2.5$ times of the optimal, while that of PBS is $2.075$ times of the optimal (as we mentioned in \autoref{sec:intro_oursolution}). It means PBS could have a lower communication overhead than PinSketch if they both use the algorithmic trick. Furthermore, as the signiture width $\log |\mathcal{U}|$ increases, the advantage of PBS over PinSketch becomes more significant, which we will show in \autoref{subsec:mini-partition}.

% The same algorithmic trick can also be implemented in PinSketch~\cite{Dodis_PinSketch_2008} to reduce it computational complexity from $O(d^2)$ to $O(d)$. However, it will encounter the same randomness problem and have to set up a safety margin on the error-correction capability. This safety margin will incur much more communication overhead on PinSketch than on our scheme: Considering the average communication overhead per group, in our scheme, this overhead can be expressed as $t\log n+\delta\log n+\delta \log u+32$, in which $t\log n$ accounts for the BCH codeword, $\delta\log n$ accounts for the index of the subset pairs, $\delta \log u$ accounts for the bitwise \code{XOR} in \autoref{alg:trivial_case}, and $32$ accounts for the $32$-bit CRC in \autoref{proto:multirounds}. In PinSketch, this overhead increases from $O(\delta\log u)$ (optimal) to $O(t\log u)$ (PinSketch does not need to transmit bitwise \code{XOR}) if it uses the same algorithmic trick. Use the same example in \autoref{sec:intro}, when $\delta=5, n=255, u=2^{32}, t=2.5\delta$, the overhead of PinSketch using the trick is $2.5$ times of the optimal, while that of our scheme is $2.075$ times of the optimal (as we introduced in \autoref{sec:intro_oursolution}). That means our scheme has a lower communication overhead than PinSketch if they both use the algorithmic trick. Furthermore, as the signiture size $\log u$ increases, the advantage of our scheme over PinSketch becomes more significantly, which we will show in \autoref{subsec:mini-partition}.

% In PinSketch, each bit encodes only a single element in the universe, so the size of the bitmap is equal to the size of the universe.  
% For example, in the set reconciliation problem we usually assume each element is ``indexed" by a $32$-bit-long (hash) signature, so the universe contains a total of $2^{32}$ elements. In this case, the bitmap encoding for any set in PinSketch is $2^{32}$ bits long, and the Galois field involved in its BCH decoding is the ``$32$-bit-wide" $GF(2^{32})$.  In contrast, as explained earlier, in PBS 
% %since each bit encodes the oddness or evenness of the cardinality of a subset,   
% the size $n$ of a bitmap is dependent only on $d$, and not on the size of the universe or on the cardinality of the set the bitmap encodes.   For example, as shown in the example above, $n = 255$ is large enough for $d = 5$.  In this case, the BCH decoding operates in the much shorter
% ``8-bit-wide" $GF(2^{8})$.  This shorter ``width" alone in theory translates into roughly $16$ times shorter BCH decoding time, which as will be explained in~\ref{} grows quadratically with the ``width" of the underlying Galois field.  This shorter ``width" also implies four times shorter BCH codeword in PBS than in PinSketch, resulting in lower communication complexity as will be shown in~\autoref{}.

% Note that our scheme only takes 1 round trip delay to both identify the $d$ subset pairs and reconcile them: In the first half, Bob computes and sends PBS to Alice. Then Alice locally identifies the $d$ subset pairs and then initiates the reconciliation ({\it i.e.,} \autoref{alg:trivial_case}) for them, {\it i.e.,} computes the bitwise \code{XOR} of the corresponded $d$ subsets. In the second half, Alice sends the bitwise \code{XOR} of the $d$ subsets with their indexes to Bob. Then Bob can compute the set difference $A\Delta B$ locally.


% We can certainly use some communication-efficient technique to estimate $d_i$ (e.g., \autoref{subsec:ToW}). However, to obtain $d_i$ precisely will require a communication cost almost as large as to reconcile Group $i$. So instead of obtaining $d_i$ and set $c_i$ (i.e., the error-correction capability of Group $i$) equal to $d_i$, we leave the randomness of $d_i$ and set $c_i$ neither too conservative, nor too libertive in the following sense: (1) $c_i$ is not too big (conservative, i.e., $10\delta$) to make the total size of PBS unnecessarily large and incur too much extra communication overhead; (2) $c_i$ is not too small (libertive, i.e., $\delta$) to incur a high probability of insufficient decode capability, which can result in hefty penalties in the latter case of incorrect decoding (will be elaborated in \autoref{sec:BCH_exception}). In our scheme, we set $c_i$ to be $2-3$ times of $\delta$, which will be shown in \autoref{sec:tail_bound} that it is just enough to make the probability of decode failure very small. Meanwhile, we set the error-correction capability of each group ($c_1,c_2,...,c_k$) to be all equal and denote it as $c$. 

Due to the same reason (i.e., estimate $\{d_i\}_{i=1}^g$ is costly), we set the number of subset pairs for each group pair to be all equal (denoted as $n$) based on $\delta$. The detail about how to set $n$ and $t$ will be elaborated in \autoref{sec:parameter_settings}. 
%Since the decoding capacity $t$ and the number of subset pairs for each group $n$ are both small constants independent of $d$, therefore, the communication overhead per group is $t\cdot\log n \!=\!O(1)$, which implies a total communication overhead of $O(d)$. Similarly, the total decoding computational complexity is also $O(d)$. 

% \subsection{Exception Handling}\label{sec:exceptions}

% \subsubsection{Exception Handling on Hash-Partition}\label{subsec:exception_hash_partition}

% As we have described in \autoref{sec:hash_partition}, the ideal case does not always happen, which means some subset pair may contain more than 1 distinct elements and cannot be successfully reconciled by \autoref{alg:trivial_case}. Due to the parity encoding, we can classify such subset pair into the following two scenarios:

% \begin{itemize}
%     \item Scenario 1: If a subset pair $(A_i, B_i)$ contains even number ($\geq 2$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be the same and our scheme will not reconcile the subset pair. Hence, the distinct elements in the subset pair will not be reconciled;
%     \item Scenario 2: If a subset pair $(A_i, B_i)$ contains odd number ($\geq 3$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be different and our scheme will reconcile the subset pair using \autoref{alg:trivial_case}. However, as we described in \autoref{subsec:protocol0}, when a subset pair contains more than 1 distinct elements, \autoref{alg:trivial_case} will output the bitwise \code{XOR} of them as the `distinct element', which is not a real distinct element with high probability;
% \end{itemize}

% In both scenarios, the distinct elements in the subset pair cannot be reconciled. Even worse, in the second scenario, a false-positive could happen (i.e., the output of \autoref{subsec:protocol0} is not a real distinct element). For example, if subset pair $(A_i, B_i)$ contains $3$ distinct elements $s_1, s_2, s_3$, then the output of \autoref{alg:trivial_case} is $\tilde{s}_4=s_1\oplus s_2\oplus s_3$, which is normally not a distinct element. The good thing is, the probability of the false-positive is extremely small for small $d$. For instance, if $d=5$ and $n=255$, the probability of the false-positive is $7.6\times 10^{-6}$, which is very small. To further reduce the chance of false-positives, we add a verification step at the end of \autoref{subsec:protocol0} to check whether the output of \autoref{subsec:protocol0} $s$ is a real distinct element or not. The verification step works as follows: Given the output $s$ of subset pair $(A_i,B_i)$, if $s\in\mathcal{U}_i$ (i.e., $h(s)=i$), we consider $s$ as a real distinct element; Otherwise, we consider $s$ as an incorrect output and discard it. 

% Note that if $s$ is a real distinct element of $(A_i,B_i)$, $s$ must be in sub-universe $\mathcal{U}_i$. However, if $s$ is the bitwise \code{XOR} of the distinct elements in $(A_i,B_i)$ (i.e., the second scenario happens), $s$ could be in any sub-universe other than $\mathcal{U}_i$. In fact, if we assume the hash-partition described in \autoref{sec:hash_partition} hashes the elements of $\mathcal{U}$ uniformly, independently, and randomly into $n$ sub-universes, the output $s$ in the second scenario will be in a different sub-universe $\mathcal{U}_j (j\neq i)$ with a high probability of $1-\frac{1}{n}$. Hence, this verfication method can further reduce the probability of false-positives by a factor of $\frac{1}{n}$. Use the same example (i.e., $d=5$, $n=255$), the probability is reduced from $7.6\times 10^{-6}$ to $3\times 10^{-8}$ by this verification method. 

% In some super critical cases (i.e., no false-positive is allowed), we can use a more powerful verification method to completely eliminate false-positives. That is, to check if the output $s$ exists in exactly one of the two sets (i.e., $s\in A\setminus B$ or $s\in B\setminus A$). To do so, Bob transmits $s$ along with an identification bit $\mathbb{1}_{\{s\in B\}}$ to Alice, then Alice checks if $s$ . This method verification costs $d(\log u+1)$ bits of additional communication overhead. In most applications, rigorously $0\%$ probability of false-positives is unnecessary and the probability of the former verification method is small enough, so we use the former verfication method in our evaluation. Based on our observation, the false-positive does not happen even once in our evaluation using the former verfication method.

\subsubsection{Exception Handling on BCH Decoding}\label{sec:BCH_exception}

The exceptions that happens within PBS-basic have been discussed and handled in \autoref{subsec:exception_hash_partition} and \autoref{sec:multi-rounds}. In this section, we only discuss the exceptions (out of PBS-basic) that are caused by the algorithm trick in \autoref{subsec:protocol2} (i.e., $d_i>t$), which is, the error-correction capability $t$ is insufficient for some group $i$. More specifically, when $d_i$ (i.e., the number of distinct elements in group $i$) is larger than the error-correction capability $t$, the BCH codewords of group $i$ differ at $d_i$ bit positions in the ideal case, which exceeds the error-correction capability $t$. If so, the BCH decoder cannot decode the bit errors correctly (\autoref{step:BCH_decode} in \autoref{alg:single_round_pbs}) and report a failure. 

To handle this type of exceptions, we use the same algorithm trick in \autoref{subsec:protocol2} to partition each problematic group into $3$ sub-groups and reconcile them respectively using PBS-basic. Note that $d_i$, if is not smaller, should be only slightly larger than $t$ with high probability. Hence, partitioning into $3$ sub-groups is enough to make sure each sub-group has no more than $t$ distinct elements. Then in the next round, each subgroup does not encounter this type of expections and can be reconciled by PBS-basic respectively. More specifically, we add a termination condition of \autoref{alg:3_way_partition} after \autoref{step:BCH_decode} in \autoref{alg:single_round_pbs}:

\begin{algorithm}
\caption{Termination condition when BCH decoding fails}
\label{alg:3_way_partition}

\If{BCH decoding fails\label{step:if1}}
{Hash-partition the group into $3$ sub-groups and do PBS for each of them in the next round; Break;}\label{step:term1} 

\end{algorithm}

% Back to the \autoref{proto:multirounds}, which shows the set reconciliation operations in each round of PBS-basic, this kind of exceptions only affect \autoref{step:reconcile} in \autoref{proto:multirounds}. Now this step needs to check whether BCH decoding is successful or not: If successful, all the operations remain the same; Else, we hash-partition the group ($A$ and $B$) into $3$ sub-groups and reconcile them respectively using \autoref{proto:multirounds}. 

Another type of exceptions that happens when $d_i>t$ is, the BCH decoder mistakes the decoding is successful and returns $t$ incorrectly decoded bit errors (i.e., subset pairs). The probability of this type of exceptions is very small. For instance, when $d=1000, \delta=5, t=13$ $(2.5\delta)$, $d_i>t$ happens with probability roughly $6.7\times 10^{-5}$, and the probability that the BCH decoder mistakes the decoding is successful when $d_i>t$ is in order of $10^{-7}$ \cite{kim1996undetected}. So the probability that this type of exceptions happens in each group is in order of $10^{-12}$. On the other hand, the impact of this type of exceptions is insignificant. Assume an incorrectly decoded bit error corresponds to a random subset pair, which could contain (1) no distinct element; (2) exactly $1$ distinct element; or (3) more than $1$ distinct elements. Reconcile the subset pair using \autoref{alg:trivial_case} could (1) get nothing and waste $\log |\mathcal{U}|$ bits of communication overhead; (2) get an actual distinct elements; or (3) trigger the exceptions that were discussed and handled in \autoref{subsec:exception_hash_partition}. 

% We handle this type of exceptions by the same method (i.e., hash-partition into $3$ sub-groups) as above. To detect them, on the other hand, is simple: Note that incorrect decoded bit errors correspond to the subset pairs that do not contain distinct elements. When we reconcile those subset pairs in \autoref{sec:reconcile_by_trivial}, the output (i.e., reconciled elements) will be $\mathbf{0}$, which is abnormal (since $\mathbf{0}\notin A\bigcup B$, as we described in \autoref{subsec:protocol0}). Hence, this type of exceptions happen if and only if one of the reconciled distinct elements is $\mathbf{0}$. 
%Hence, we consider BCH decoding is successful by two criteria: (1) the BCH decoder reports a successful decode; and (2) None of the reconciled elements is $\mathbf{0}$. 
========================
In fact, even if $d_i>t$, PBS-basic is still possible to reconcile group $i$ in some nonideal cases. For example, when $t=10$ and $d_i=11$, if the $11$ distinct elements are distributed in $10$ subset pairs, such that $1$ subset pair contains $2$ distinct elements and $9$ subset pairs contain $1$ distinct element in each, the two parity bitmaps differ at only $9$ bit positions. So BCH decoder is able to decode the later $9$ subset pairs and the corresponding $9$ distinct elements can be reconciled. In the second round, only $2$ distinct elements remain and BCH decoding certainly works. In this case, we do not need to partition the group into sub-groups, and this case does not trigger \autoref{alg:3_way_partition} in PBS. 
========================
% Instead, it will either (1) report a failure about exceeding the error-correction capability; or (2) mistake the decoding is successful and return incorrect decoded bit errors. 

% The second case happens with a very small probability (in order of $10^{-7}$ \cite{kim1996undetected}) and is very simple to detect : 

% The first case is easy to handle: We can simply adapt the same algorithmic trick to partition the group into smaller groups and reconcile them respectively. In our scheme, we set the number of smaller groups to be $3$, which is big enough because $d_i$, if not smaller, only slightly larger than $t$ with high probability. The second case on the other hand, although theoretically possible, happens with a very small probability when $d_i>t$ (in order of $10^{-7}$ \cite{kim1996undetected}). Besides, the probability of $d_i>t$ is also very small (e.g., when $t=15$ and $\delta=5$, this probability is about $2.3\times 10^{-4}$), so the overall probability of the second case, which is the multiplication of these two small numbers, is negligible (e.g., in order of $10^{-11}$).

% \subsection{Multi-rounds}

% Even if the ideal case does not happen, most of the distinct elements should be distributed into different subset pairs and therefore can be reconciled. So our scheme, even cannot reconcile all of the distinct elements, can still reconcile the majority of them (piecewise decodability). To reconcile the rest distinct elements, we can just run our scheme for multi-rounds under different hash-partition functions. For each round, our scheme works as follows: 

% \IncMargin{1em}
% \begin{algorithm}
% \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
% \Input{Two sets $A$ and $B$}
% \Input{Size of set difference $d$}
% \Input{The number of subset pairs $n$}
% \Input{BCH error-correction capability $t$}

% Hash-partition $A$ and $B$ into $n$ subset pairs $\{(A_i,B_i)\}_{i=1}^n$;

% \If{BCH decoding fails}
% 	Hash-partition $A$ and $B$ into $3$ subset pairs and reconcile them respectively in the next round\;
% \ElseIf{BCH decoding success}
	
% \Else{}

% $k \leftarrow \lceil \frac{t}{c}\rceil $\;

% Partition elements into $k$ subsets using~\autoref{alg:random-part}\;

% \For{$j = 0$ \KwTo $k-1$}{
%     Reconcile the $j$-th subset pair using the straw-man scheme with the BCH correcting capability $\tau$, number of smaller subsets $m$, and number of rounds $r$\;
% }

% \caption{PBS (per round)} \label{proto:II}
% \end{algorithm}\DecMargin{1em}

% This {\bf multi-rounds} scheme can significantly increase the success probability (i.e., the probability that all distinct elements are reconciled). Readers may wonder in the later rounds, most distinct elements should be reconciled, and the remaining could be reconciled using degraded parameters (i.e., smaller $n$ and $t$). In fact, degrade parameters in later rounds cannot save much communication overhead, since the majority of it is spent in the first round (i.e., $>90\%$). Therefore, we use the same parameters (i.e., $n,t$) among all rounds in our evaluation. 
% %The tradeoff between the number of rounds and the communication overhead per rounds will be elaborated in \autoref{sec:tail_bound}. In our evaluation, $r=2,3$ rounds are enough to achieve an extremely high success probability. 

% Readers may think the cost (i.e., communication overhead and the computational complexity) of this multi-rounds scheme is proportional to the number of rounds (denoted as $r$) and increases linearly with $r$. In fact, the cost of each round is roughly proportional to the number of remaining distinct elements, which decreases exponentially as $r$ increases (i.e., the first round reconciles $99\%$ of distinct elements, the second round reconciles $99\%$ of the remaining $1\%$ distinct elements, etc.). So the cost of this multi-rounds scheme is only slightly larger than that of the single-round scheme. Furthermore, as we explained in \autoref{sec:intro}, {\bf from intro thanks for the piecewise decodability of our solution, in almost all practical application scenarios, this tradeoff does not lead to longer response time because the reconciliation of objects identified by the successfully decodable codewords, which constitute the vast majority of all codewords, can run in parallel with the transmissions and decodings of the rest.  In other words, the piecewise decodability effective masks the slightly larger number of communication rounds as far as the response time is concerned.} 





\begin{comment}
\subsubsection{Random Partition}

\IncMargin{1em}
\begin{algorithm}
% \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
% \Input{Set $S$}
% \Input{The number of subsets $m$ for partition}
% \Output{Subsets $S_1, S_2, ..., S_m$}

% Generate hash function $h(\cdot)$ that maps each element into $\{1,2,...,m\}$;

\ForEach{$s \in S$}{
    $j \leftarrow h(s) \bmod m$\;    
    Insert $s$ into the $j$-th subset $S_j$\;
}

\caption{Partition using hash function $h(\cdot)$.} \label{alg:random-part}
\end{algorithm}\DecMargin{1em}

Like the strawman scheme, our scheme randomly partitions sets $A$ and $B$ into $m$ subsets. This random partition 
can be easily accomplished by using some hash function, $h(\cdot)$, and inserting each element $x$ into the subset 
corresponding to $h(x)$. \autoref{alg:random-part} presents the pseudo-code of this random partition using hash 
function $h(\cdot)$.  

% Unlike the strawman scheme, our scheme only reconciles those subset pairs that need to be reconciled, 
% because 



Like the strawman scheme, our scheme hash-partitions the two sets $A$ and $B$ into $m$ subset pairs $(A_i, B_i)$ for $i=1,2,\cdots,m$. 
We note that, among those $m$ bins (subset pairs), 
at most $t$ ($t\!\ll\!m$ as shown in our analysis in~\autoref{subsec:protocol1}) bins contain balls 
(elements belonging to the set difference), {\it i.e.,} requiring reconciliation.  
Motivated by this observation, we, therefore, propose to first detect those bins that 
contain balls and then only reconcile them. The detection is solved with a simple encoding approach that 
will be detailed in the next section.

\subsubsection{Detection before Reconciliation} 

In fact, identifying those non-empty bins is easy when each bin contains at most one ball. In this section, we assume that 
each bin after the random partition contains at most one ball, we will show later how to handle the cases when some 
bins contain more than one balls later in~\autoref{subsec:exceptions}. 

Given an arbitrary bin (say subset pair $(A_i, B_i)$) that contains one ball ({\it i.e.,} $A_i\Delta B_i$ contains exactly one element), 
the corresponding two subsets $A_i$ and $B_i$ differ exactly one element, which implies that 
$||A_i|\!-\!|B_i||\!=\!1$. Hence, if $|A_i|$ ({\it i.e.,} number of 
elements in $A_i$) is odd (or even), then $|B_i|$ must be even (or odd). In other words, the odevity of $|A_i|$ 
and $|B_i|$ are opposite. %differs if $|A_i\Delta B_i|\!=\!1$. 
Based on this property, we propose the {\it odevity encoding}: 
A subset is encoded as ``1'' if it contains odd number of elements, and as ``0'' otherwise. 
Using this odevity encoding, the $m$ subsets of $A$ can be encoded as a bit string $b_A$ in $\{0,1\}^m$, 
where the $i$-th bit in $b_A$ corresponds to the odevity encoding of $|A_i|$. Similarly, the $m$ subsets of $B$ can also 
be encoded as a bit string $b_B$. Clearly, $b_A$ and $b_B$ differ at $t$ different positions, or in other words, 
the Hamming distance of bit strings $b_A$ and $b_B$ is $t$. A straightforward approach is 
to let Alice send $b_A$ to Bob, and then Bob compares $b_B$ against $b_A$ to obtain those non-empty bins. 

This approach, however, has a communication overhead of $m$ bits, which is still unnecessarily high. As 
analyzed in~\autoref{subsec:protocol0}, $t$ is usually much smaller than $m$. 
That means $b_A$ and $b_B$ differ only at a tiny portion of bits. %have much more in common than differences. 
Therefore, if we view $b_B$ as a corrupted message of $b_A$ with $t$ corrupted bits, the detection of those $t$ bins can be converted to 
the detection of the positions of the $t$ corrupted bits. The latter can be solved using an Error-Correction Code (ECC)~\cite{Lin_ErrorControlCoding_1983} that can correct up to $t$ errors. In this work, we use the BCH code~\cite{Lint_IntroductionCodingTheory_1998}. 
More precisely, this ECC-based approach (with the BCH code) works as follows. 
Alice computes the parity bits for $b_A$ using a $t$-error-correcting BCH code with a block length of 
$(2^{\lceil \log m\rceil} -1)$ and sends the parity bits to Bob. Bob then decodes the positions of the $t$ corrupted bits 
using the BCH decoding algorithm with $b_B$ and those parity bits received from Alice. The communication overhead of 
this approach is roughly $t\lceil \log m\rceil$ ($=O(t\log t)$) bits. In the example above, this communication overhead is 
roughly $\num{17000}$ bits, which is approximately $6$ times lower 
than $m\!=\!\num{108469}$ bits, the communication overhead of the aforementioned straightforward approach. 

At first sight, it seems that the detection of non-empty bins and reconciliation of subsets in those bins require two rounds 
(or at least two round trip delays), {\it i.e.,} one round for detection and the other for reconciliation. In fact, 
it only requires one. After Bob receives the parity bits from Alice and decodes out those non-empty bins, it initiates 
the reconciliation ({\it i.e.,} \autoref{alg:trivial_case}) for each bin (subset pair) immediately, 
{\it i.e.,} sends the \code{XOR} sums of subsets in those bins together the indexes of those bins. 
After receiving those \code{XOR} sums and bin indexes, Alice can compute the set difference. 

% A naive way to combine the detection of non-empty bins and reconciliation of subset pairs in those bins is to first detect 
% those non-empty bins via one round of message exchanges between Alice and Bob and then to reconcile the corresponding 
% subset pairs in those bins with another round of message exchanges. This requires two rounds ({\it i.e.,} taking at least 
% two round trip delays). In fact, after Bob receives the parity bits from Alice and obtains those 

\subsubsection{Multiple Rounds}\label{sec:multiround}

{\bf This section was not clear enough. I need more time to think about and revise it.}


In the above section, we have assumed that each bin contains at most one ball. 
However, even with a sufficient large $m$, some bin might contain more than one balls though with tiny probability. 
We will show in~\autoref{subsec:exceptions}, how such rare events, {\it i.e.,} one bin contains more than one balls, 
can be easily detected.
To ensure our scheme can successfully reconcile all elements even when such rare events happen, 
we propose to use multiple rounds (of communication between Alice and Bob). More precisely, instead of 
selecting a prohibitively large $m$ to ensure that each bin contains at most one ball with a extremely high probability 
(say 0.99999), we select a reasonably large $m$ so that the communication overhead is not very high and very few bins contain 
more than one balls (or in other words, most bins contain at most one ball). Therefore, after running one round of 
our scheme, most elements in the set difference will be reconciled. Only those in the bins that contain more than one balls 
fail to be reconciled. For elements in the subsets corresponding to those bins, we run another round of our scheme. 
If some elements still fail to be reconcile, we can run one more round of our scheme. So on so forth,  
our scheme can keep running for more rounds until all elements are reconciled. 

With the same communication overhead, multiple rounds can significantly increase the success rate, 
{\it i.e.,} the probability that all elements in the set difference will be successfully reconciles, 
which will be elaborated in~\autoref{sec:tail_bound}. 

% % to be emphasized
% % say that too many rounds should be avoided (latency & communication overhead reduction is negligible when r is too large, 2 - 3 is good enough)
% % multiple rounds is not an issue when r is small

% We note that the number of rounds $r$, however, should not be large. On one hand, it results in large latency (at least $r$ round trip delays). 
% On the other hand, when $r$ is large, the reduction of communication overhead by the increase of $r$ gradually diminishes. 

We note that multiple rounds, when $r$ is small, would not really increase the ``latency'', as long as most elements in the 
set difference can be reconciled in the first rounds, since the underlying synchronization of data objects corresponding to 
those elements can start immediately after the first round of our scheme. Therefore, the actual latency is one round trip delay instead of 
$r$. 

As we mentioned, this straw-man protocol works correctly if each subset pair has at most one exclusive element (i.e., \autoref{eq:requirement_strawman} holds). On the other hand, if a subset pair has more than one exclusive elements, some of which will not be successfully reconciled:

\begin{itemize}
\item If a subset pair has even number of exclusive elements, Odevity coding will encode it as 0. Then the straw-man scheme will consider the subset pair having no exclusive element and all exclusive elements in this subset will not be reconciled;

\item If a subset pair has odd number ($\geq 3$) of exclusive elements, Odevity coding will encode it as 1 and consider the subset pair having only 1 exclusive element. Then the straw-man scheme will use \autoref{alg:trivial_case} to decode only one exclusive element and dismiss all others. Even worse, the only decoded element is probably not a real exclusive element, since the element computed by \autoref{alg:trivial_case} is the \code{XOR} sum of all exclusive elements, not one of them. 
\end{itemize}

In summary, if a subset pair has more than one exclusive elements, most of its exclusive elements cannot be reconciled, and the reconciled element is usually incorrect (i.e., false-positive). The false-positive however is easy to check, which will be elaborated in \autoref{subsec:exceptions}. The good thing is, even if not all subset pairs have at most one exclusive element and are successfully decoded, most of them will be w.h.p.. In other words, even if the straw-man protocol cannot reconcile all exclusive elements, it still can reconcile most of them. To reconcile all exclusive elements w.h.p., we can simply extend the single-round straw-man scheme to multi-round. And each round adapts the straw-man scheme to do set reconciliation using independent hashing functions $h(\cdot)$ for partition (i.e., in \autoref{alg:random-part}). This multi-round extension can significantly increase the probability of a successful reconciliation, which will be elaborated in \autoref{sec:tail_bound}. 



\subsection{Our Scheme: The Final Version}\label{subsec:protocol2}

{\bf Under revision~}

The preliminary version of our scheme suffers from two major drawbacks. 
First, its communication overhead is asymptotically 
$O(t\log m)\!=\!O(t\log t)$, which is not asymptotically optimal. 
Second, the decoding computational complexity is proportional to 
$t^2$ with the state-of-the-art decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} for BCH codes, 
which is too high when $t$ is large. 
To overcome these two drawbacks, we use a simple algorithmic trick: divide and conquer. With this algorithmic 
trick, the decoding computational complexity is reduced to $O(t)$, 
and the communication overhead is reduced to $t\cdot\frac{\log u}{8} \!+\! O(t)$ (with a small 
hidden constant roughly varying from 4 to 8) bytes which implies that 
our scheme has an additive communication overhead (compared to the optimal scheme) 
of 4 to 8 bytes per element in the 
set difference and this additive overhead is independent of the key size ({\it i.e.}, $\log u$). 
Recall that the IBF-based schemes usually have a communication overhead of roughly 6 times of the 
optimal scheme, which increases linearly as the key size. Therefore, our scheme is much more 
communication-efficient. 

Now, we describe in detail this algorithmic trick. We let Alice divide elements in $A$ into $\lceil\frac{t}{c}\rceil$ groups (subsets)  
for some small constant $c$ (say $5$) so that each group contains roughly $c$ elements from the set difference on average. We let Bob do the same operations on $B$. To ensure that any common element ({\it i.e.,} any element $x\!\in\! A\bigcup B$) goes into 
the same group ({\it i.e.,} groups at Alice and Bob with the same index), we can use the partition procedure with a hash function shown 
in~\autoref{alg:random-part}. Then, we can apply the preliminary version on each group with a constant $m$ (say $m\!=\!256$) independent of 
$t$. To ensure that each group can be reconciled with a high probability, we need to use BCH codes whose decoding capacity 
larger than $c$ (say $\tau\!=\!2c$), as exact number of elements to be reconciled could be larger than $c$. 
Since this decoding capacity $\tau$ is still a small constant independent of $t$, therefore, the communication 
overhead per group is $\tau\cdot\log m \!=\!O(1)$, which implies a total communication overhead of $O(t)$. 
Similarly, the total decoding computational complexity is also $O(t)$. 

\subsubsection{Parameter Configurations} 

Our scheme now has several parameters: $c$ (average number of elements from the set difference in each group), 
$\tau$ (the correcting capability of the BCH code), $m$ (number of bins for each group), and $r$ (maximum number of rounds). 
We note that the maximum number of rounds $r$ is usually associated with another parameter $p$ the desired success rate: With 
at most $r$ rounds, our scheme should guarantee that the success rate is at least $p$. 
%How to tune these parameters to achieve favorable performance will be detailed later in~\autoref{sec:tail_bound}. 
Here, we provide some guidances for the parameter configurations using our theoretical analysis, which gives the tail bound of 
the success probability of our scheme and will be shown in~\autoref{sec:tail_bound}. 

\noindent
{\bf Parameterizing $c$ and $r$.} The values of $c$ and $r$ are usually provided by users based on the requirements of 
applications. For the value of $c$, a larger $c$ results in a longer decoding time yet lower communication overhead.  
So if the decoding time is a big concern, then a smaller $c$ (say $c=5$) should be used; otherwise, a larger $c$ could be used. 
For the values of $r$, a larger $r$ leads to lower communication overhead and usually lower decoding time (as it allows to use 
a smaller $\tau$), however, the reduction is marginal when $r>3$. Therefore, we suggest users to configure $r$ to be $2$ or $3$. 
% The configuration of $c$ is relatively straightforward, as a larger $c$ will result in 
% a longer decoding time and a slightly lower communication overhead. The former is ..., The latter is slightly tricky. 


\noindent
{\bf Using $c$ and $r$ to parameterize other parameters.} After users specify the values for $c$ and $r$ (associated with a value for 
$p$), we can use our theoretical analysis in~\autoref{sec:tail_bound} to parameterize $\tau$ and $m$. 
Since in a BCH code, the block length is in the form of $2^q-1$, we only need to consider $m=2^q-1$. 

{\bf Liang, please revise the following algorithm!}

\begin{algorithm}
\SetKwProg{Proc}{}{}{end}
\SetKwFunction{algo}{\small Search}

\Proc{Search($c$, $r$, $p$)}{\label{search:entrance}

$\mbox{co}_{best}\leftarrow\infty$\tcc*{\small Best communication overhead}

\For{$\tau \leftarrow c\,\KwTo\, \infty$}{}



}
\end{algorithm}


% , unlike 
% the IBF-based schemes which have an multiplicative overhead of 6 
% The inspiration is from the famous 
% divide and conquer algorithm for the selection problem, in which, given an array with $n$ elements, we want to get the $k$-th largest 
% element. A straightforward idea for this problem is sorting. However, if using insertion-sorting, the complexity would be $O(n^2)$. 
% Then the famous divide and conquer trick comes. It first divides the array into $\lceil n/5\rceil$ groups so that the first 
% $\lfloor n/5\rfloor$ contains $5$ elements and at most one group contains the rest $n \mod 5$ elements, and find the median of each 
% group using the insertion-sorting and th


% This straw-man scheme still has a problem on decoding computational complexity. More specific, the complexity increases dramatically with the total number of corrupted bits $t$. Therefore, when $t$ is moderate or large, the decoding computational complexity could be very high. For instance, the decoding complexity of BCH codes~\cite{Lint_IntroductionCodingTheory_1998} is $O(t^3)$, which could be quite high for a large $t$. To keep the decoding complexity reasonably low, we design the following two-layer protocol: In the first layer, we use a hash function to partition the two sets into $\lceil\frac{t}{c}\rceil$ subsets for some small constant $c$ (say $5$), just like the first step of our straw-man scheme. The objective, which is however different from before, is to make each subset pair contains roughly $c$ exclusive elements on average. In the second layer, we use the straw-man scheme with the same configuration (number of subsets $m$, and error-correction capability $\tau$, number of rounds $r$) to reconcile each subset pair. 

% In fact, the straw-man scheme is a proper solution when $t$ is small. First, the decoding complexity will not be a problem for a small $t$; Second, we do not need an extremely large $m$ to guarantee \autoref{eq:requirement_strawman} w.h.p.. For instance, when $t=5$ and $m=1024$, \autoref{eq:requirement_strawman} holds with probability $\frac{m\,!}{(m-t)\,!m^t}\approx 99\%$. This motivates us to design the following two-layer protocol: In the first layer, we use a hash function to partition the two sets into $\lceil\frac{t}{c}\rceil$ subsets for some small constant $c$ (say $5$), just like the first step of our straw-man scheme. The objective, which is however different from before, is to make each subset pair contains roughly $c$ exclusive elements on average. In the second layer, we use the straw-man scheme with the same configuration (number of subsets $m$, and error-correction capability $\tau$) to reconcile each subset pair. 

\autoref{proto:II} shows the pseudocode of our scheme. It first uses the same hash-function based random partition algorithm as \autoref{alg:random-part} to partition elements into $k\triangleq\lceil \frac{t}{c} \rceil$ subsets. Note that the random partition only guarantees that each such subset 
contains $c$ exclusive elements on average, and the exact number is not known. Hence, our scheme uses a BCH code with a capability of 
correcting up to $\tau$ errors with $\tau > c$ to make sure that the BCH code has a high probability to decode successfully. We will describe how to deal with situation where the size of set difference exceeds $\tau$ later in~\autoref{subsec:exceptions}.

As the decoding of a $\tau$-error-correcting BCH code where $\tau$ is a small constant has a constant-time computational complexity, the decoding complexity of 
our scheme is $O(k)=O(t)$. We now have several parameters, average number of exclusive elements in each subset $c$, the correcting capability $\tau$ of BCH code, the number of smaller subsets $m$ for each subset to be divided to, and the number of rounds $r$. How to tune these parameters to achieve favorable performance will be detailed later in~\autoref{sec:tail_bound}. 

\IncMargin{1em}
\begin{algorithm}
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
\Input{Size of set difference $t$}
\Input{The number of subsets $m$ for each partition}
\Input{Average number of exclusive elements in each partition $c$}
\Input{BCH code capability $\tau$}

$k \leftarrow \lceil \frac{t}{c}\rceil $\;

Partition elements into $k$ subsets using~\autoref{alg:random-part}\;

\For{$j = 0$ \KwTo $k-1$}{
    Reconcile the $j$-th subset pair using the straw-man scheme with the BCH correcting capability $\tau$, number of smaller subsets $m$, and number of rounds $r$\;
}

\caption{Our Scheme} \label{proto:II}
\end{algorithm}\DecMargin{1em}




\subsection{Exceptional Handling}\label{subsec:exceptions}

{\bf To be revised~}

In this section, we will elaborate how to handle the following two types of exceptions that we mentioned in \autoref{sec:multiround} and \autoref{subsec:protocol2}:
\begin{itemize}
    \item Exception 1: A subset pair has odd number ($\geq 3$) of exclusive elements and causes false-positives (i.e., a decoded distinct element is not a real one);
    \item Exception 2: A subset pair contains too many exclusive elements, such that a BCH code with capability of correcting up to $\tau$ errors cannot decode it (i.e., $t>\tau$).
	\item Exception 3: A subset pair has even number ($\geq 2$) of exclusive elements and causes false-negatives(i.e., two or more distinct elements are neglected as the parity bit is 0);
\end{itemize}

To handle Exception 1, we need to check whether a computed exclusive element by \autoref{alg:trivial_case} is a real exclusive element or not. (The group index happens to come in handy if we use it as a fingerprint of the element we computed. If this element is truly an exclusive element, it should be hashed into the same group as before. Notably, We have two group indices available for this check, one is in the initial divide and conquer phase, the other is in the BCH code part) It can be easily done at the end of set reconciliation, during which two hosts exchange their exclusive elements. In fact, as we will elaborate in \autoref{sec:tail_bound}, Exception 1 hardly happens if we set parameters properly. 

On the other hand, when Exception 2 happens, the BCH decoder will report a failure about exceeding the error-correction capability. For such a subset pair, we can use the same approach as in \autoref{subsec:protocol2} to partition it into smaller subsets and use the straw-man scheme to reconcile them respectively. We set the number of small subsets to be 3. It is because, as we will elaborate in \autoref{sec:tail_bound}, the number of exclusive elements for each subset pair $t$ should be, if not smaller, only slightly larger than $\tau$ w.h.p.. Partitioning those exclusive elements into 3 small subsets is enough to guarentee that each of them has less than $\tau$ exclusive elements.

\end{comment}

==> section/schemes_new_bak0126.tex <==
\section{Set Reconciliation}\label{sec:scheme}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%     Writing Guideline for This Section     %%%%%%%%%%
% “balls – elements in the symmetric difference of the two sets” 

% Protocol 0 (reconcile two sets whose set difference has at most one ball)

% Protocol I.I (partition elements into a sufficiently large number of subsets such that each subset has at most one ball with high probability and use Protocol 0 to reconcile each of them) 

% Protocol I.II (a two-step refinement of Protocol I.I: first use BCH to identify good bins, i.e., bins/subsets have exactly one ball, and then use Protocol 0 to reconcile each good bin) 

% Protocol II (a two-layer refinement of Protocol I.II: in the first layer, we partition elements into t/c subsets, where t is the size of set difference and c is a small constant, then each subset has c balls on average. In the second layer, we further partition each subset into large enough number of bins/subsets such that with high probability each bin has at most one ball, then use Protocol I.II to reconcile them one by one) 

% Protocol III/IV (mainly fix certain exceptions in Protocol II，e.g., how to address bad bins, how to handle the cases where BCH fails to decode and etc)

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this section, we describe our set reconciliation scheme in details. In \autoref{subsec:protocol0}, we introduce a basic scheme for the trivial case, in which the two sets $A$ and $B$ has at most one distinct element. In \autoref{subsec:protocol1}, we build upon the basic scheme and propose a baseline scheme for general cases (i.e., any arbitrary number of distinct elements). In \autoref{sucsec:our-scheme}, we propose the preliminary version of our scheme, which is based on the baseline scheme. And we further improve the preliminary version on the communication overhead and computational complexity and propose the final version of our scheme in \autoref{subsec:protocol2}. We assume the total number of distinct elements $d$ is known in advance throughout this section except in \autoref{subsec:ToW}, where we will describe how to estimate $d$ using a Tug-of-War Estimator. 

\subsection{The Trivial Case: $d\leq 1$}\label{subsec:protocol0}

We start with the trivial case, in which $A$ and $B$ have at most one distinct element ({\it i.e.,} $d\leq 1$), 
we have a simple set reconciliation scheme showed in \autoref{alg:trivial_case}:

\begin{algorithm}
\caption{Set reconciliation when $d\le 1$}
\label{alg:trivial_case}

{\it Alice}: Calculate $s_A\triangleq\underset{a\in A}{\oplus} a$, then send $s_A$ to Bob\; \label{alg1:sender}

{\it Bob}: Calculate $s_B\triangleq\underset{a\in B}{\oplus} b$ and $s\triangleq s_A \oplus s_B$\; \label{alg1:receiver}
\end{algorithm}

First, Alice calculates the bitwise \code{XOR} of all elements in $A$ (denote as $s_A$) and send it to Bob. 
Second, Bob also calculates the bitwise \code{XOR} of all elements of $B$ (denote as $s_B$). Upon the received $s_A$, Bob computes $s\!\triangleq\! s_A \!\oplus\! s_B$, and we have

\begin{itemize}
	\item If $A$ and $B$ are identical (i.e., $d=0$), $s_A$ and $s_B$ will be the same and $s=0$;
	\item If $A$ and $B$ has one distinct element (i.e., $d=1$), the bitwise \code{XOR} of $s_A$ and $s_B$ will cancel out all common elements and remain the distinct element, so $s=A\Delta B$. And $s$ is the missing element of $A$ (i.e., $s\in B\!\setminus\! A$) if $s\in B$, or the missing element of $B$ (i.e., $s\in A\!\setminus\! B$) otherwise;
	% \item If $A$ and $B$ has more than one distinct elements (i.e., $d>1$), the bitwise \code{XOR} of $s_A$ and $s_B$ will still cancel out all common elements and remain the \code{XOR} of the distinct elements, i.e., $s$ is the \code{XOR} of all distinct elements;
\end{itemize}

Note that \autoref{alg:trivial_case} does not work when $0\in A\bigcap B$, because when $s=0$, \autoref{alg:trivial_case} cannot tell whether $A$ and $B$ are identical, or they have a distinct element of $0$. However, we can extend our scheme to support $0$. For example, we let Alice send to Bob a single bit to indicate whether Alice has element $0$, so Bob will know whether $0\in A\Delta B$ or not. Like other set reconciliation works, we assume $0$ is excluded from $\mathcal{U}$ in the sequel of this paper. 

Meanwhile, \autoref{alg:trivial_case} does not work when $d>1$. In this case, the bitwise \code{XOR} of $s_A$ and $s_B$ will still cancel out all common elements and remain the \code{XOR} of the distinct elements, i.e., the output of \autoref{alg:trivial_case} $s$ is the \code{XOR} of all distinct elements;

% Note that \autoref{alg:trivial_case} works if and only if $|A\Delta B|\!\leq\! 1$ and $0\!\notin\! (A\!\cup\! B)$ (which we have explained in~\autoref{sec:model}). 

\subsection{Baseline Scheme}\label{subsec:protocol1} 

Note that the set difference $A\Delta B$ can contain more than 1 elements (i.e., $d>1$), and \autoref{alg:trivial_case} cannot reconcile $A$ and $B$ directly in this case. Therefore, we propose a baseline scheme building upon~\autoref{alg:trivial_case} that also works when $d>1$: First, we partition the element universe $\mathcal{U}$ into $n$ sub-universes $\mathcal{U}_1, \mathcal{U}_2, \cdots, \mathcal{U}_n$. Denote $A_i \triangleq A\bigcap \mathcal{U}_i$ and $B_i \triangleq B\bigcap \mathcal{U}_i$ for $i=1,2,\cdots,n$. Then $\{A_i\}_{i=1}^n$ and $\{B_i\}_{i=1}^n$ are partitions of $A$ and $B$ respectively. Furthermore, $\Phi\triangleq\{A_i\Delta B_i\}_{i=1}^n$ is a partition of $A\Delta B$. 

Assume the {\bf ideal case} happens, in which each subset pair $(A_i, B_i)$ contains at most one distinct element ({\it i.e.,} $|A_i\Delta B_i|\!\leq\!1$), we use \autoref{alg:trivial_case} to reconcile each subset pair and obtain $A_i\Delta B_i$ for $i=1,2,\cdots,n$. The overall set difference $A\Delta B$ is simply their union $\bigcup_{i=1}^n \big{(}A_i\Delta B_i\big{)}$. 

In the first step of the baseline scheme, we can use a hash function $h(\cdot): \mathcal{U}\rightarrow \{1,2,\cdots,n\}$ to partition the universe $\mathcal{U}$ into $n$ sub-universes: $\mathcal{U}_i=\{s\mid s\in \mathcal{U} \mbox{ and } h(s)=i\}$ for $\forall i=1,2,\cdots,n$. And the hash function $h(\cdot)$ can be predetermined between Alice and Bob and does not require additional communication cost.

This hash-partition can be modeled as a {\it balls-into-bins problem}, in which the distinct elements are viewed as balls and the subset pairs are viewed as bins. The hash-parition basically throws (hashes) $d$ balls (distinct elements) uniformly and randomly into $n$ bins (subset pairs). The aforementioned ideal case in this context becomes, after throwing $d$ balls uniformly and randomly into $n$ bins, each bin receives at most 1 ball (i.e., $d$ nonempty bins have 1 ball in each and the rest $n-d$ bins are empty). {\bf It may remind readers about the Birthday problem. And the ideal case can be analogous to the case that no people share the same birthday.} The ideal case happens with a probability of $p=\frac{n\,!}{(n-d)\,!n^d}\!=\!\prod_{k=1}^{d - 1}(1 - \frac{k}{n})\!\approx\! e^{-\frac{d(d-1)}{2n}}$ when $d\!\ll\!n$. In other words, $n$ must be $\Omega(d^2)$ to ensure the ideal case happens with a nontrivial probability.  Note that the communication overhead of the baseline scheme is proportional to $n$, as each subset pair requires communication of a bitwise \code{XOR} in \autoref{alg:trivial_case}. So this communication overhead increases at least quadratically as $d$ increases. 

In fact, this communication overhead can be significantly reduced: In the ideal case, $n-d$ out of $n$ subset pairs are identical ones, and only $d (\ll n)$ out of $n$ subset pairs contain distinct elements (one distinct element in each of the $d$ subset pairs) and need to be reconciled. If we can identify these $d$ subset pairs (with a tiny additional communication overhead) and only reconcile them, the overall communication overhead will be significantly reduced from $\Omega(d^2)$ to $O(d)$. Based on this intuition, we propose our scheme in \autoref{sucsec:our-scheme}, which uses Parity Bitmap Sketch (PBS) and Error Correction Coding (ECC) to identify those subset pairs with a tiny additional communication overhead. 

Note that the ideal case does not always happen. However, we can ensure that the ideal case happens with high probability by properly selecting $n$ based on $d$ (i.e., $n=\Omega(d^2)$). Furthermore, as we will describe in \autoref{subsec:nonideal}, even if the ideal case does not happen (i.e., some distinct elements are hashed into the same subset pair), most of the distinct elements should be distributed into different subset pairs and therefore can be reconciled. So the baseline scheme, even cannot reconcile all of the distinct elements, can still reconcile the majority of them. Based on this property, we will extend our scheme from single-round to multi-rounds in \autoref{subsec:nonideal} to further increase the probability of reconciling all distinct elements. 

\begin{comment}
For general cases ({\it i.e.,} $t=|A\Delta B|$ is an arbitrary number), we have a straightforward strawman scheme building upon~\autoref{alg:trivial_case}, which works as follows: First, Alice and Bob choose some hash function $h(s): \mathcal{U} \rightarrow \{0,1,\cdots,2^{32}-1\}$ to partition $A$ and $B$ into $m$ subsets $A_1,A_2,\cdots,A_m$ and $B_1,B_2,\cdots,B_m$ respectively:

\begin{align}
s\in A_i & \mbox{ iff } s\in A \mbox{ and } h(s)=i\!\mod m, \nonu{}mber\\
s\in B_i & \mbox{ iff } s\in B \mbox{ and } h(s)=i\!\mod m. \nonumber
\end{align} 

{\bf call a subset pair -> partition?} Since Alice and Bob use the same hash function for partition, common elements (i.e., elements in $A\cap B$) are always hashed into the same subset pair $(A_i, B_i)$. And the set difference of each subset pair only contains distinct elements (i.e., elements in $A\Delta B$): $A_i\Delta B_i \subset A\Delta B$. In the ideal case, with a sufficient large $m$, each subset pair $(A_i, B_i)$ contains at most one distinct element ({\it i.e.,} $|A_i\Delta B_i|\!\leq\!1$). Then \autoref{alg:trivial_case} can reconcile each subset pair and obtain $A_i\Delta B_i$ for $i=1,2,\cdots,m$. The overall set difference $A\Delta B$ is simply their union $\bigcup_{i=1}^m \big{(}A_i\Delta B_i\big{)}$. The selection of hash function $h(s)$ can be predetermined between Alice and Bob and it does not require additional communication cost.

%To make sure Alice and Bob use the same hash function for partition, we let them pre-agree on some universal hash family (e.g., \code{xxHash}~\cite{Collet_xxHashExtremelyfast_}) and a common selection order, and each time they choose a hash function from the family in the same order. Note that we can also let Alice generates a hash function and send it to Bob. The hash function that Alice and Bob choose for partition can be either generated by 

This hash-partition is in nature a {\it balls-into-bins model}. We can view the distinct elements as balls and the subset pairs as bins. The hash-parition basically throws (hashes) $t$ balls (distinct elements) uniformly and randomly into $m$ bins (subset pairs). The aforementioned ideal case in this context is, with a sufficient large number of bins, each bin receives at most 1 ball. The strawman scheme works correctly if and only if the ideal case happens, which has a probability of $\frac{m\,!}{(m-t)\,!m^t}\!=\!\prod_{k=1}^{t - 1}(1 - \frac{k}{m})\!\approx\! e^{-\frac{t(t-1)}{2m}}$. In other words, to ensure the strawman scheme works correctly with a probability of $p$, it roughly requires $m \!=\!\lceil \frac{t(t-1)}{-2\ln p}\rceil$ subset pairs. 

Note that the communication overhead of this strawman scheme is proportional to the number of subset pairs $m$, as each subset pair requires communication of an \code{XOR} sum in \autoref{alg:trivial_case} during the reconciliation. When $t$ is small, a small communication cost can guarantee that the strawman scheme works correctly with high probability. For instance, when $t=5$, $m=95$ subset pairs are sufficient for the strawman scheme to work correctly with a probability of $90\%$. However, when $t$ is relatively large, it requires a huge communication cost to ensure the strawman scheme works correctly. For instance, when $t=1,000$, it requires $m=4,740,865$ subset pairs to guarantee a success probability of $90\%$. 

In fact, the majority of subset pairs are identical ones and do not need to reconcile. And only a small portion of them contain distinct elements. If we can identify those subset pairs that contain distinct elements and only reconcile them, the communication cost could be significantly reduced. Our scheme is based on this intuition and uses parity bitmap sketch and BCH code to identify the subset pairs, which we will elaborate in \autoref{sucsec:our-scheme}. 

\end{comment}

%To distribute balls as uniformly as possible and maximize the probability of the ideal case, we choose a uniform hashing function $h$ that throws balls uniformly and randomly into bins: $$\mathbb{P}[h(s)=i]=\frac{1}{m} \mbox{ for } \forall i=1,2,\cdots,m, \forall s\in U$$.

%Note that the probability of the ideal case is $\frac{m\,!}{(m-t)\,!m^t}\!=\!\prod_{k=1}^{t - 1}(1 - \frac{k}{m})\!\approx\! e^{-\frac{t(t-1)}{2m}}$. Hence, at least $\lceil \frac{t(t-1)}{-2\ln p}\rceil$ bins are required to ensure that this probability is at least $p$. In other words, to ensure that the ideal case happens with a probability of $p$, the strawman scheme roughly requires $m \!=\!\lceil \frac{t(t-1)}{-2\ln p}\rceil$. For example, suppose $t\!=\!$\num{1000}, %and $p\!=\!0.01$, this strawman scheme roughly requires $m\!=\!$\num{720626} bins (partitions) to ensure that $|A_i\Delta B_i|\!\leq\!1$ (for any $i=1,2,\cdots,m$) holds with probability $50\%$.  

% A straightforward strawman scheme building upon~\autoref{alg:trivial_case} 
% to reconcile two sets $A$ and $B$ in general 
% ({\it i.e.,} $|A\Delta B|$ is an arbitrary number) is the following: 
% Uniformly randomly partition $A$ and $B$ into $m$ subsets ($A_1,A_2,\cdots,A_m$ 
% and $B_1,B_2,\cdots,B_m$) so that the set difference 
% $A_i\Delta B_i$ of each subset pair $(A_i, B_i)$ contains at most one element 
% ({\it i.e.,} $|A_i\Delta B_i|\!\leq\!1$) {\it w.h.p.} ({\it i.e.,} with high probability), 
% and then reconcile each subset pair with~\autoref{alg:trivial_case}. 

% Now let us analyze this strawman scheme using the {\it balls-into-bins model}. 
% Assume that sets $A$ and $B$ have $t$ elements in their set difference, {\it i.e.,} $|A\Delta B|\!=\!t$. 
% These $t$ elements can be viewed as $t$ balls and the $m$ partitions (subset pairs) can be viewed as 
% $m$ bins. The random partition process in this strawman scheme can be modeled as throwing 
% $t$ balls into $m$ bins in the following manner: Each ball goes into a 
% uniformly random bin and independently of other balls. %so that each bin contains at most one ball, {\it w.h.p.}  
% The probability that each bin contains at most one ball is  
% $\frac{m\,!}{(m-t)\,!m^t}\!=\!\prod_{k=1}^{t - 1}(1 - \frac{k}{m})\!\approx\! e^{-\frac{t(t-1)}{2m}}$. 
% Hence, at least $\lceil \frac{t(t-1)}{-2\ln p}\rceil$ bins are required 
% to ensure that this probability is at least $p$. In other words, to ensure 
% that each bin contains at most one ball with a probability of $p$, 
% the strawman scheme roughly requires $m \!=\!\lceil \frac{t(t-1)}{-2\ln p}\rceil$. 
% For example, suppose $t\!=\!$\num{1000}, %and $p\!=\!0.01$, 
% this scheme roughly requires $m\!=\!$\num{108469} bins (partitions) to 
% ensure that $|A_i\Delta B_i|\!\leq\!1$ (for any $i=1,2,\cdots,m$) holds with probability $0.01$.  

% We note that the communication overhead of this strawman scheme is proportional to 
% $m$ ($\!\gg\! t$), as each partition (subset pair) requires communication of an \code{XOR} sum during the reconciliation. 
% This communication overhead is much higher than that of the optimal scheme, which only requires 
% to exchange the elements in the set difference (assuming an oracle tells it which elements belong to 
% the set difference), {\it i.e.,} proportional to $t$. In the example above, assuming each element takes 4 bytes, 
% the communication overhead of the strawman scheme is $4m$ bytes ($\!\approx\! \num{423.71}\,$KB) to ensure 
% a success rate of only 0.01 ({\it i.e.,} with a probability of $0.0.1$, all elements in 
% the set difference are successfully reconciled), 
% which is approximately 2 orders of magnitude higher than $4t$ bytes ($\!=\!\num{3.90}\,$KB), the communication 
% overhead of the optimal scheme. 

\subsection{Our Scheme: The Preliminary Version}\label{sucsec:our-scheme}

Like the baseline scheme, our scheme also hash-partitions the two sets $A$ and $B$ into $n$ subset pairs. The difference is, instead of reconciling all subset pairs using \autoref{alg:trivial_case}, our scheme identifies the subset pairs that contains distinct elements and only reconciles them. Since the hash-partition and set reconciliation on each subset pair using \autoref{alg:trivial_case} have been described in \autoref{subsec:protocol1}, we only elaborate how to identify the subset pairs that contain distinct elements in this section. 

The general idea of identification is very simple: First, we {\bf encode} each subset into $1$ bit, such that in the ideal case, for $\forall i=1,2,\cdots,n$:

\begin{itemize}
	\item The codewords (bits) of $A_i$ and $B_i$ are different if and only if subset pair $(A_i, B_i)$ contains $1$ distinct element;
	\item The codewords (bits) of $A_i$ and $B_i$ are the same if and only if subset pair $(A_i, B_i)$ contains no distinct element;
\end{itemize}

Second, we {\bf compare} the codewords of each subset pair. And the subset pairs that contain distinct elements are the ones with different codewords (bits). We will describe the two steps in details in \autoref{sec:parity_bitmap_encoding} and \autoref{sec:BCH_code} respectively.

\subsubsection{Parity Bitmap Encoding}\label{sec:parity_bitmap_encoding}

In our scheme, we use {\it parity encoding} to encode each subset into a parity bit. More specific, it encodes a subset as ``1'' if it contains odd number of elements, and as ``0'' otherwise. And it satisfies the aforementioned requirements in the ideal case:

\begin{itemize}
	\item If subset pair $(A_i, B_i)$ contains $1$ distinct element, the corresponding two subsets $A_i$ and $B_i$ differ exactly one element, which implies that $||A_i|\!-\!|B_i||\!=\!1$. Hence, if $|A_i|$ ({\it i.e.,} number of elements in $A_i$) is odd (or even), then $|B_i|$ must be even (or odd). And the parity bits of $A_i$ and $B_i$ will be different;
	\item If subset pair $(A_i, B_i)$ contains no distinct element, the corresponding two subsets $A_i$ and $B_i$ should be the same and therefore contain the same number of elements. Hence, if $|A_i|$ is odd (or even), then $|B_i|$ must be odd (or even). And the parity bits of $A_i$ and $B_i$ will be the same;
\end{itemize}

Using parity encoding, the $n$ subsets of $A$ are encoded as a bit string $A[1..n]$ in $\{0,1\}^n$, 
where the $i$-th bit $A[i]$ in $A[1..n]$ corresponds to the parity encoding bit of $A_i$. Similarly, the $n$ subsets of $B$ are similarly 
encoded as a bit string $B[1..n]$. We call $A[1..n]$ ($B[1..n]$) the {\it parity bitmap} of $\{A_i\}_{i=1}^n$ ($\{B_i\}_{i=1}^n$). In the ideal case, $A[1..n]$ and $B[1..n]$ differ at $d$ different bit-positions, which corresponds to the $d$ subset pairs that contain distinct elements. And our scheme only reconciles those subset pairs that the parity bits are different. We will describe the nonideal case (i.e., some subset pair contains more than 1 distinct elements) in \autoref{subsec:nonideal}.

\subsubsection{Parity Bitmap Comparison Using BCH Code}\label{sec:BCH_code}

A straightforward approach to compare the parity bitmaps is to let Bob send the complete parity bitmap $B[1..n]$ to Alice, then Alice compares $A[1..n]$ with $B[1..n]$ locally. This approach has a communication overhead of $n$ bits, which is unnecessarily high. As we discussed in~\autoref{subsec:protocol0}, $d$ is usually much smaller than $n$. It means $A[1..n]$ and $B[1..n]$ differ only at a tiny portion of bits. Therefore, we can view $A[1..n]$ as a corrupted message of $B[1..n]$ with $d$ corrupted bits, and the bit-positions of the $d$ corrupted bits basically correspond to the $d$ subset pairs that contain distinct elements. The detection of corrupted bits, on the other hand, can be solved by Error-Correction Code (ECC)~\cite{Lin_ErrorControlCoding_1983}. And our scheme uses BCH code~\cite{Lint_IntroductionCodingTheory_1998} to encode the parity bitmap and detect the $d$ corrupted bits.

More specific, after the parity bitmap encoding, Bob uses a $d$-error-correcting systematic BCH code to encode $B[1..n]$ into an $n+d\log n$ codeword, in which the first $n$ bits are $B[1..n]$ (property of systematic BCH code). Then Bob sends the rest $d\log n$ bits, which we denote as {\it parity bitmap sketch (PBS)}, to Alice. Upon the received PBS and $A[1..n]$ (corrupted message), Alice uses the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} to detect the $d$ corrupted bits in $A[1..n]$. The communication overhead of this approach is $d\log n$ bits (i.e., length of PBS), which is much smaller than that of the straightforward approach ($n$ bits, when $d\!\ll\!n$). On the other hand, the computational complexity of the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} is $O(d^2\log^2 n)$. 

Fix the length of PBS to be $dm$ for some integer $m$, $n$ ranges  

\subsubsection{Exceptional Handling and Multi-rounds}\label{subsec:nonideal}

As we described in \autoref{subsec:protocol1}, the ideal case does not always happen, which means some subset pair may contain more than 1 distinct elements and cannot be successfully reconciled by \autoref{alg:trivial_case}. Due to the parity encoding, we can classify such subset pair into the following two scenarios:

\begin{itemize}
    \item Scenario 1: If a subset pair $(A_i, B_i)$ contains even number ($\geq 2$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be the same and our scheme will not reconcile the subset pair. Hence, the distinct elements in the subset pair will not be reconciled;
    \item Scenario 2: If a subset pair $(A_i, B_i)$ contains odd number ($\geq 3$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be different and our scheme will reconcile the subset pair using \autoref{alg:trivial_case}. However, as we described in \autoref{subsec:protocol0}, when a subset pair contains more than 1 distinct elements, \autoref{alg:trivial_case} will output the bitwise \code{XOR} of them as the `distinct element', which is not a real distinct element with high probability;
\end{itemize}

In both scenarios, the distinct elements in the subset pair cannot be reconciled. Even worse, in the second scenario, a false-positive could happen (i.e., the output of \autoref{subsec:protocol0} is not a real distinct element). However, as we will analyze in \autoref{sec:tail_bound} and show in {\bf the evaluation section}, the second scenario barely happens both theoretically and empirically. To further reduce the chance of false-positives, we add a verification step at the end of \autoref{subsec:protocol0} to check whether the output of \autoref{subsec:protocol0} $s$ is a real distinct element or not. The verification step works as follows: Given the output $s$ of subset pair $(A_i,B_i)$, if $s\in\mathcal{U}_i$ (i.e., $h(s)=i$), we consider $s$ as a real distinct element; Otherwise, we consider $s$ as an incorrect output and discard it. 

Note that if $s$ is a real distinct element of $(A_i,B_i)$, $s$ must be in sub-universe $\mathcal{U}_i$. However, if $s$ is the bitwise \code{XOR} of the distinct elements in $(A_i,B_i)$ (i.e., the second scenario happens), $s$ could be in any sub-universe other than $\mathcal{U}_i$. In fact, if we assume the hash-partition described in \autoref{subsec:protocol1} hashes the elements of $\mathcal{U}$ uniformly, independently, and randomly into $n$ sub-universes, the output $s$ in the second scenario will be in a different sub-universe $\mathcal{U}_j (j\neq i)$ with a high probability of $1-\frac{1}{n}$. Hence, this verfication step can reduce the chance of false-positives by a factor of $\frac{1}{n}$. 

Even if the ideal case does not happen, most of the distinct elements should be distributed into different subset pairs and therefore can be reconciled. So our scheme, even cannot reconcile all of the distinct elements, can still reconcile the majority of them (piecewise decodability). To reconcile the rest distinct elements, we can just run our scheme for another round under a different hash-partition function, so on so force. This {\bf multi-rounds} scheme can significantly increase the success probability (i.e., the probability that all distinct elements are reconciled). Readers may wonder in the later rounds, most distinct elements should be reconciled, and the remaining could be reconciled using degraded parameters (i.e., smaller $n$ and $t$). In fact, degrade parameters in later rounds cannot save much communication overhead, since the majority of it is spent in the first round (i.e., $>90\%$). Therefore, we use the same parameters (i.e., $n,t$) among all rounds in our evaluation.
%The tradeoff between the number of rounds and the communication overhead per rounds will be elaborated in \autoref{sec:tail_bound}. In our evaluation, $r=2,3$ rounds are enough to achieve an extremely high success probability. 

Readers may think the cost (i.e., communication overhead and the computational complexity) of this multi-rounds scheme is proportional to the number of rounds (denoted as $r$) and increases linearly with $r$. In fact, the cost of each round is roughly proportional to the number of remaining distinct elements, which decreases exponentially as $r$ increases (i.e., the first round reconciles $99\%$ of distinct elements, the second round reconciles $99\%$ of the remaining $1\%$ distinct elements, etc.). So the cost of this multi-rounds scheme is only slightly larger than that of the single-round scheme. Furthermore, as we explained in \autoref{sec:intro}, {\bf from intro thanks for the piecewise decodability of our solution, in almost all practical application scenarios, this tradeoff does not lead to longer response time because the reconciliation of objects identified by the successfully decodable codewords, which constitute the vast majority of all codewords, can run in parallel with the transmissions and decodings of the rest.  In other words, the piecewise decodability effective masks the slightly larger number of communication rounds as far as the response time is concerned.} 



\subsection{Our Scheme: The Final Version}\label{subsec:protocol2}

The preliminary version of our scheme suffers from two major drawbacks. First, its communication overhead is asymptotically 
$O(d\log n)\!=\!O(d\log d)$, which is not asymptotically optimal. Second, the decoding computational complexity is proportional to 
$d^2$ with the state-of-the-art decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} for BCH codes, which is too high when $d$ is large. To overcome these two drawbacks, we use a simple algorithmic trick: divide and conquer. With this algorithmic trick, the decoding computational complexity is reduced to $O(d)$, and the communication overhead is reduced to $d\log u \!+\! O(d)$. 

Now, we describe the idea of this algorithmic trick. In the first step, we hash-partition $A$ and $B$ (by some hash function $h_1(\cdot)$) into $g$ subset pairs, just like what we did in \autoref{subsec:protocol1}. The objective of this partition is however different: In \autoref{subsec:protocol1}, we target to ensure each subset pair contains at most 1 distinct element with high probability; Here we target to make each subset pair contains roughly $\delta$ distinct elements for some small constant $\delta$ (say $5$) by setting $g=d/\delta$. To differentiate the $g$ subset pairs here from those in \autoref{subsec:protocol1}, we call them the $g$ {\bf groups} in the sequel. In the second step, we just apply the preliminary version of our scheme on each group and obtain the distinct elements. 

When describing the preliminary version in \autoref{sucsec:our-scheme}, we assume that the number of distinct elements is known in advance. And we set the error-correction capability of the BCH code $t$ just enough to correct $d$ errors (i.e., $t=d$). However, this assumption does not hold here: Let $d_i$ denote the number of distinct elements in Group $i$. Due to the property of hash-partition, each $d_i$ is a Binomial random variable $\mathcal{B}(d,g)$ with expectation of $\delta$, which is not known precisely. To ensure the error-correction capability $t$ is sufficient for all groups with high probability, we leave some safety margin for the randomness of $d_i$ and conservatively set $t$ roughly $2-3$ times of $\delta$ (so that $Pr[d_i>t]$ is tiny). 

Note that this safety margin incurs additional communication overhead on transmitting PBS: In the perfect scenario (i.e., $\{d_i\}_{i=1}^g$ is known), the overall communication overhead on transmitting PBS is $\sum_{i=1}^g d_i\log n=g\delta\log n$; On the other hand, when we set $t$ to be the error-correction capability for each group, then the overall overhead on transmitting PBS becomes $gt\log n$, which is roughly $2-3$ times of that in the perfect scenario (when $t$ is roughly $2-3$ times of $\delta$). Readers may wonder if we can reduce this additional communication overhead by using some technique to estimate $\{d_i\}_{i=1}^g$ (e.g., ToW estimator in \autoref{subsec:ToW}), so that we can set the error-correction capability for each group more wisely and save some waste on the safety margin. However, to achieve that, the estimation on $\{d_i\}_{i=1}^g$ must be in high precision (smaller range than $[0,3\delta]$), which requires a much higher communication cost than the savings. 

The same algorithmic trick can also be implemented in pinsketch~\cite{Dodis_PinSketch_2008} to reduce it computational complexity. However, it will encounter the same randomness problem and have to set up a safety margin on the error-correction capability. Compare to our scheme, in which the additional communication overhead is $gt\log n-g\delta\log n$, pinsketch will incur a much larger additional communication overhead ($gt\log u-g\delta \log u$) using the same parameter settings (i.e., $g,\delta$). Use the same example in \autoref{sec:intro}, when $\delta=5, n=255, u=2^{64}$, the additional communication overhead of pinsketch is roughly $8$ times larger than that of our scheme. And as the signiture size $\log u$ increases, the communication overhead of pinsketch under the algorithmic trick increases much faster than that of our scheme, which we will show in \autoref{subsec:mini-partition}.

% In pinsketch, each bit encodes only a single element in the universe, so the size of the bitmap is equal to the size of the universe.  
% For example, in the set reconciliation problem we usually assume each element is ``indexed" by a $32$-bit-long (hash) signature, so the universe contains a total of $2^{32}$ elements. In this case, the bitmap encoding for any set in pinsketch is $2^{32}$ bits long, and the Galois field involved in its BCH decoding is the ``$32$-bit-wide" $GF(2^{32})$.  In contrast, as explained earlier, in PBS 
% %since each bit encodes the oddness or evenness of the cardinality of a subset,   
% the size $n$ of a bitmap is dependent only on $d$, and not on the size of the universe or on the cardinality of the set the bitmap encodes.   For example, as shown in the example above, $n = 255$ is large enough for $d = 5$.  In this case, the BCH decoding operates in the much shorter
% ``8-bit-wide" $GF(2^{8})$.  This shorter ``width" alone in theory translates into roughly $16$ times shorter BCH decoding time, which as will be explained in~\ref{} grows quadratically with the ``width" of the underlying Galois field.  This shorter ``width" also implies four times shorter BCH codeword in PBS than in pinsketch, resulting in lower communication complexity as will be shown in~\autoref{}.

% Note that our scheme only takes 1 round trip delay to both identify the $d$ subset pairs and reconcile them: In the first half, Bob computes and sends PBS to Alice. Then Alice locally identifies the $d$ subset pairs and then initiates the reconciliation ({\it i.e.,} \autoref{alg:trivial_case}) for them, {\it i.e.,} computes the bitwise \code{XOR} of the corresponded $d$ subsets. In the second half, Alice sends the bitwise \code{XOR} of the $d$ subsets with their indexes to Bob. Then Bob can compute the set difference $A\Delta B$ locally.


% We can certainly use some communication-efficient technique to estimate $d_i$ (e.g., \autoref{subsec:ToW}). However, to obtain $d_i$ precisely will require a communication cost almost as large as to reconcile Group $i$. So instead of obtaining $d_i$ and set $c_i$ (i.e., the error-correction capability of Group $i$) equal to $d_i$, we leave the randomness of $d_i$ and set $c_i$ neither too conservative, nor too libertive in the following sense: (1) $c_i$ is not too big (conservative, i.e., $10\delta$) to make the total size of PBS unnecessarily large and incur too much extra communication overhead; (2) $c_i$ is not too small (libertive, i.e., $\delta$) to incur a high probability of insufficient decode capability, which can result in hefty penalties in the latter case of incorrect decoding (will be elaborated in \autoref{sec:BCH_exception}). In our scheme, we set $c_i$ to be $2-3$ times of $\delta$, which will be shown in \autoref{sec:tail_bound} that it is just enough to make the probability of decode failure very small. Meanwhile, we set the error-correction capability of each group ($c_1,c_2,...,c_k$) to be all equal and denote it as $c$. 

Similarly, we set the number of subset pairs for each group to be all equal (denoted as $n$), which is also neither too conservative, nor too libertive in the above sense. The detail about how to set $n$ and $t$ will be elaborated in \autoref{sec:parameter_settings}. Since the decoding capacity $t$ and the number of subset pairs for each group $n$ are both small constants independent of $d$, therefore, the communication overhead per group is $t\cdot\log n \!=\!O(1)$, which implies a total communication overhead of $O(d)$. Similarly, the total decoding computational complexity is also $O(d)$. 

\subsubsection{Exceptional Handling when $t<d_i$}\label{sec:BCH_exception}

When $d_i$ (i.e., the number of distinct elements in Group $i$) is unluckily larger than the error-correction capability $t$, the BCH codewords of Group $i$ could differ up to $d_i$ bits (ideal case), which is larger than $t$ with high probability. If so, the BCH decoder cannot decode the bit errors correctly. Instead, it will either (1) report a failure about exceeding the error-correction capability; or (2) mistake the decoding is successful and return incorrect decoded bit errors. The first case is easy to handle: We can simply adapt the same algorithmic trick to partition the group into smaller groups and reconcile them respectively. In our scheme, we set the number of smaller groups to be $3$, which is big enough because, as we will elaborate in \autoref{sec:tail_bound}, $d_i$, if not smaller, only slightly larger than $t$ with high probability. The second case on the other hand, although theoretically possible, happens with a very small probability when $d_i>t$ (in order of $10^{-7}$ \cite{kim1996undetected}). Besides, the probability of $d_i>t$ is also very small (e.g., when $t=15$ and $\delta=5$, this probability is about $2.3\times 10^{-4}$), so the overall probability of the second case, which is the multiplication of these two small numbers, is negligible.

% \begin{table}
% \centering
% \caption{Probability of the second case}\label{tab:second_case}
% \setlength{\tabcolsep}{3pt}
% \begin{tabular}{@{}|l|c|c|c|@{}}  
% \hline
% Number of bit errors & 11 & 12 & 13 \\ 
% \hline
% \mathbb{P} & YES & O(t) & 2\\ \hline
% Graphene & NO  & $O(|A|+|B|)$ & 2 or 3 \\ \hline 
% Minisketch & YES & $O(t^2)$ & 2 \\ \hline
% Our scheme & YES &$O(t)$ & 3 or 4\\
% \hline
% \end{tabular}
% \end{table}


\begin{comment}
\subsubsection{Random Partition}

\IncMargin{1em}
\begin{algorithm}
% \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
% \Input{Set $S$}
% \Input{The number of subsets $m$ for partition}
% \Output{Subsets $S_1, S_2, ..., S_m$}

% Generate hash function $h(\cdot)$ that maps each element into $\{1,2,...,m\}$;

\ForEach{$s \in S$}{
    $j \leftarrow h(s) \bmod m$\;    
    Insert $s$ into the $j$-th subset $S_j$\;
}

\caption{Partition using hash function $h(\cdot)$.} \label{alg:random-part}
\end{algorithm}\DecMargin{1em}

Like the strawman scheme, our scheme randomly partitions sets $A$ and $B$ into $m$ subsets. This random partition 
can be easily accomplished by using some hash function, $h(\cdot)$, and inserting each element $x$ into the subset 
corresponding to $h(x)$. \autoref{alg:random-part} presents the pseudo-code of this random partition using hash 
function $h(\cdot)$.  

% Unlike the strawman scheme, our scheme only reconciles those subset pairs that need to be reconciled, 
% because 



Like the strawman scheme, our scheme hash-partitions the two sets $A$ and $B$ into $m$ subset pairs $(A_i, B_i)$ for $i=1,2,\cdots,m$. 
We note that, among those $m$ bins (subset pairs), 
at most $t$ ($t\!\ll\!m$ as shown in our analysis in~\autoref{subsec:protocol1}) bins contain balls 
(elements belonging to the set difference), {\it i.e.,} requiring reconciliation.  
Motivated by this observation, we, therefore, propose to first detect those bins that 
contain balls and then only reconcile them. The detection is solved with a simple encoding approach that 
will be detailed in the next section.

\subsubsection{Detection before Reconciliation} 

In fact, identifying those non-empty bins is easy when each bin contains at most one ball. In this section, we assume that 
each bin after the random partition contains at most one ball, we will show later how to handle the cases when some 
bins contain more than one balls later in~\autoref{subsec:exceptions}. 

Given an arbitrary bin (say subset pair $(A_i, B_i)$) that contains one ball ({\it i.e.,} $A_i\Delta B_i$ contains exactly one element), 
the corresponding two subsets $A_i$ and $B_i$ differ exactly one element, which implies that 
$||A_i|\!-\!|B_i||\!=\!1$. Hence, if $|A_i|$ ({\it i.e.,} number of 
elements in $A_i$) is odd (or even), then $|B_i|$ must be even (or odd). In other words, the odevity of $|A_i|$ 
and $|B_i|$ are opposite. %differs if $|A_i\Delta B_i|\!=\!1$. 
Based on this property, we propose the {\it odevity encoding}: 
A subset is encoded as ``1'' if it contains odd number of elements, and as ``0'' otherwise. 
Using this odevity encoding, the $m$ subsets of $A$ can be encoded as a bit string $b_A$ in $\{0,1\}^m$, 
where the $i$-th bit in $b_A$ corresponds to the odevity encoding of $|A_i|$. Similarly, the $m$ subsets of $B$ can also 
be encoded as a bit string $b_B$. Clearly, $b_A$ and $b_B$ differ at $t$ different positions, or in other words, 
the Hamming distance of bit strings $b_A$ and $b_B$ is $t$. A straightforward approach is 
to let Alice send $b_A$ to Bob, and then Bob compares $b_B$ against $b_A$ to obtain those non-empty bins. 

This approach, however, has a communication overhead of $m$ bits, which is still unnecessarily high. As 
analyzed in~\autoref{subsec:protocol0}, $t$ is usually much smaller than $m$. 
That means $b_A$ and $b_B$ differ only at a tiny portion of bits. %have much more in common than differences. 
Therefore, if we view $b_B$ as a corrupted message of $b_A$ with $t$ corrupted bits, the detection of those $t$ bins can be converted to 
the detection of the positions of the $t$ corrupted bits. The latter can be solved using an Error-Correction Code (ECC)~\cite{Lin_ErrorControlCoding_1983} that can correct up to $t$ errors. In this work, we use the BCH code~\cite{Lint_IntroductionCodingTheory_1998}. 
More precisely, this ECC-based approach (with the BCH code) works as follows. 
Alice computes the parity bits for $b_A$ using a $t$-error-correcting BCH code with a block length of 
$(2^{\lceil \log m\rceil} -1)$ and sends the parity bits to Bob. Bob then decodes the positions of the $t$ corrupted bits 
using the BCH decoding algorithm with $b_B$ and those parity bits received from Alice. The communication overhead of 
this approach is roughly $t\lceil \log m\rceil$ ($=O(t\log t)$) bits. In the example above, this communication overhead is 
roughly $\num{17000}$ bits, which is approximately $6$ times lower 
than $m\!=\!\num{108469}$ bits, the communication overhead of the aforementioned straightforward approach. 

At first sight, it seems that the detection of non-empty bins and reconciliation of subsets in those bins require two rounds 
(or at least two round trip delays), {\it i.e.,} one round for detection and the other for reconciliation. In fact, 
it only requires one. After Bob receives the parity bits from Alice and decodes out those non-empty bins, it initiates 
the reconciliation ({\it i.e.,} \autoref{alg:trivial_case}) for each bin (subset pair) immediately, 
{\it i.e.,} sends the \code{XOR} sums of subsets in those bins together the indexes of those bins. 
After receiving those \code{XOR} sums and bin indexes, Alice can compute the set difference. 

% A naive way to combine the detection of non-empty bins and reconciliation of subset pairs in those bins is to first detect 
% those non-empty bins via one round of message exchanges between Alice and Bob and then to reconcile the corresponding 
% subset pairs in those bins with another round of message exchanges. This requires two rounds ({\it i.e.,} taking at least 
% two round trip delays). In fact, after Bob receives the parity bits from Alice and obtains those 

\subsubsection{Multiple Rounds}\label{sec:multiround}

{\bf This section was not clear enough. I need more time to think about and revise it.}


In the above section, we have assumed that each bin contains at most one ball. 
However, even with a sufficient large $m$, some bin might contain more than one balls though with tiny probability. 
We will show in~\autoref{subsec:exceptions}, how such rare events, {\it i.e.,} one bin contains more than one balls, 
can be easily detected.
To ensure our scheme can successfully reconcile all elements even when such rare events happen, 
we propose to use multiple rounds (of communication between Alice and Bob). More precisely, instead of 
selecting a prohibitively large $m$ to ensure that each bin contains at most one ball with a extremely high probability 
(say 0.99999), we select a reasonably large $m$ so that the communication overhead is not very high and very few bins contain 
more than one balls (or in other words, most bins contain at most one ball). Therefore, after running one round of 
our scheme, most elements in the set difference will be reconciled. Only those in the bins that contain more than one balls 
fail to be reconciled. For elements in the subsets corresponding to those bins, we run another round of our scheme. 
If some elements still fail to be reconcile, we can run one more round of our scheme. So on so forth,  
our scheme can keep running for more rounds until all elements are reconciled. 

With the same communication overhead, multiple rounds can significantly increase the success rate, 
{\it i.e.,} the probability that all elements in the set difference will be successfully reconciles, 
which will be elaborated in~\autoref{sec:tail_bound}. 

% % to be emphasized
% % say that too many rounds should be avoided (latency & communication overhead reduction is negligible when r is too large, 2 - 3 is good enough)
% % multiple rounds is not an issue when r is small

% We note that the number of rounds $r$, however, should not be large. On one hand, it results in large latency (at least $r$ round trip delays). 
% On the other hand, when $r$ is large, the reduction of communication overhead by the increase of $r$ gradually diminishes. 

We note that multiple rounds, when $r$ is small, would not really increase the ``latency'', as long as most elements in the 
set difference can be reconciled in the first rounds, since the underlying synchronization of data objects corresponding to 
those elements can start immediately after the first round of our scheme. Therefore, the actual latency is one round trip delay instead of 
$r$. 

As we mentioned, this straw-man protocol works correctly if each subset pair has at most one exclusive element (i.e., \autoref{eq:requirement_strawman} holds). On the other hand, if a subset pair has more than one exclusive elements, some of which will not be successfully reconciled:

\begin{itemize}
\item If a subset pair has even number of exclusive elements, Odevity coding will encode it as 0. Then the straw-man scheme will consider the subset pair having no exclusive element and all exclusive elements in this subset will not be reconciled;

\item If a subset pair has odd number ($\geq 3$) of exclusive elements, Odevity coding will encode it as 1 and consider the subset pair having only 1 exclusive element. Then the straw-man scheme will use \autoref{alg:trivial_case} to decode only one exclusive element and dismiss all others. Even worse, the only decoded element is probably not a real exclusive element, since the element computed by \autoref{alg:trivial_case} is the \code{XOR} sum of all exclusive elements, not one of them. 
\end{itemize}

In summary, if a subset pair has more than one exclusive elements, most of its exclusive elements cannot be reconciled, and the reconciled element is usually incorrect (i.e., false-positive). The false-positive however is easy to check, which will be elaborated in \autoref{subsec:exceptions}. The good thing is, even if not all subset pairs have at most one exclusive element and are successfully decoded, most of them will be w.h.p.. In other words, even if the straw-man protocol cannot reconcile all exclusive elements, it still can reconcile most of them. To reconcile all exclusive elements w.h.p., we can simply extend the single-round straw-man scheme to multi-round. And each round adapts the straw-man scheme to do set reconciliation using independent hashing functions $h(\cdot)$ for partition (i.e., in \autoref{alg:random-part}). This multi-round extension can significantly increase the probability of a successful reconciliation, which will be elaborated in \autoref{sec:tail_bound}. 



\subsection{Our Scheme: The Final Version}\label{subsec:protocol2}

{\bf Under revision~}

The preliminary version of our scheme suffers from two major drawbacks. 
First, its communication overhead is asymptotically 
$O(t\log m)\!=\!O(t\log t)$, which is not asymptotically optimal. 
Second, the decoding computational complexity is proportional to 
$t^2$ with the state-of-the-art decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} for BCH codes, 
which is too high when $t$ is large. 
To overcome these two drawbacks, we use a simple algorithmic trick: divide and conquer. With this algorithmic 
trick, the decoding computational complexity is reduced to $O(t)$, 
and the communication overhead is reduced to $t\cdot\frac{\log u}{8} \!+\! O(t)$ (with a small 
hidden constant roughly varying from 4 to 8) bytes which implies that 
our scheme has an additive communication overhead (compared to the optimal scheme) 
of 4 to 8 bytes per element in the 
set difference and this additive overhead is independent of the key size ({\it i.e.}, $\log u$). 
Recall that the IBF-based schemes usually have a communication overhead of roughly 6 times of the 
optimal scheme, which increases linearly as the key size. Therefore, our scheme is much more 
communication-efficient. 

Now, we describe in detail this algorithmic trick. We let Alice divide elements in $A$ into $\lceil\frac{t}{c}\rceil$ groups (subsets)  
for some small constant $c$ (say $5$) so that each group contains roughly $c$ elements from the set difference on average. We let Bob do the same operations on $B$. To ensure that any common element ({\it i.e.,} any element $x\!\in\! A\bigcup B$) goes into 
the same group ({\it i.e.,} groups at Alice and Bob with the same index), we can use the partition procedure with a hash function shown 
in~\autoref{alg:random-part}. Then, we can apply the preliminary version on each group with a constant $m$ (say $m\!=\!256$) independent of 
$t$. To ensure that each group can be reconciled with a high probability, we need to use BCH codes whose decoding capacity 
larger than $c$ (say $\tau\!=\!2c$), as exact number of elements to be reconciled could be larger than $c$. 
Since this decoding capacity $\tau$ is still a small constant independent of $t$, therefore, the communication 
overhead per group is $\tau\cdot\log m \!=\!O(1)$, which implies a total communication overhead of $O(t)$. 
Similarly, the total decoding computational complexity is also $O(t)$. 

\subsubsection{Parameter Configurations} 

Our scheme now has several parameters: $c$ (average number of elements from the set difference in each group), 
$\tau$ (the correcting capability of the BCH code), $m$ (number of bins for each group), and $r$ (maximum number of rounds). 
We note that the maximum number of rounds $r$ is usually associated with another parameter $p$ the desired success rate: With 
at most $r$ rounds, our scheme should guarantee that the success rate is at least $p$. 
%How to tune these parameters to achieve favorable performance will be detailed later in~\autoref{sec:tail_bound}. 
Here, we provide some guidances for the parameter configurations using our theoretical analysis, which gives the tail bound of 
the success probability of our scheme and will be shown in~\autoref{sec:tail_bound}. 

\noindent
{\bf Parameterizing $c$ and $r$.} The values of $c$ and $r$ are usually provided by users based on the requirements of 
applications. For the value of $c$, a larger $c$ results in a longer decoding time yet lower communication overhead.  
So if the decoding time is a big concern, then a smaller $c$ (say $c=5$) should be used; otherwise, a larger $c$ could be used. 
For the values of $r$, a larger $r$ leads to lower communication overhead and usually lower decoding time (as it allows to use 
a smaller $\tau$), however, the reduction is marginal when $r>3$. Therefore, we suggest users to configure $r$ to be $2$ or $3$. 
% The configuration of $c$ is relatively straightforward, as a larger $c$ will result in 
% a longer decoding time and a slightly lower communication overhead. The former is ..., The latter is slightly tricky. 


\noindent
{\bf Using $c$ and $r$ to parameterize other parameters.} After users specify the values for $c$ and $r$ (associated with a value for 
$p$), we can use our theoretical analysis in~\autoref{sec:tail_bound} to parameterize $\tau$ and $m$. 
Since in a BCH code, the block length is in the form of $2^q-1$, we only need to consider $m=2^q-1$. 

{\bf Liang, please revise the following algorithm!}

\begin{algorithm}
\SetKwProg{Proc}{}{}{end}
\SetKwFunction{algo}{\small Search}

\Proc{Search($c$, $r$, $p$)}{\label{search:entrance}

$\mbox{co}_{best}\leftarrow\infty$\tcc*{\small Best communication overhead}

\For{$\tau \leftarrow c\,\KwTo\, \infty$}{}



}
\end{algorithm}


% , unlike 
% the IBF-based schemes which have an multiplicative overhead of 6 
% The inspiration is from the famous 
% divide and conquer algorithm for the selection problem, in which, given an array with $n$ elements, we want to get the $k$-th largest 
% element. A straightforward idea for this problem is sorting. However, if using insertion-sorting, the complexity would be $O(n^2)$. 
% Then the famous divide and conquer trick comes. It first divides the array into $\lceil n/5\rceil$ groups so that the first 
% $\lfloor n/5\rfloor$ contains $5$ elements and at most one group contains the rest $n \mod 5$ elements, and find the median of each 
% group using the insertion-sorting and th


% This straw-man scheme still has a problem on decoding computational complexity. More specific, the complexity increases dramatically with the total number of corrupted bits $t$. Therefore, when $t$ is moderate or large, the decoding computational complexity could be very high. For instance, the decoding complexity of BCH codes~\cite{Lint_IntroductionCodingTheory_1998} is $O(t^3)$, which could be quite high for a large $t$. To keep the decoding complexity reasonably low, we design the following two-layer protocol: In the first layer, we use a hash function to partition the two sets into $\lceil\frac{t}{c}\rceil$ subsets for some small constant $c$ (say $5$), just like the first step of our straw-man scheme. The objective, which is however different from before, is to make each subset pair contains roughly $c$ exclusive elements on average. In the second layer, we use the straw-man scheme with the same configuration (number of subsets $m$, and error-correction capability $\tau$, number of rounds $r$) to reconcile each subset pair. 

% In fact, the straw-man scheme is a proper solution when $t$ is small. First, the decoding complexity will not be a problem for a small $t$; Second, we do not need an extremely large $m$ to guarantee \autoref{eq:requirement_strawman} w.h.p.. For instance, when $t=5$ and $m=1024$, \autoref{eq:requirement_strawman} holds with probability $\frac{m\,!}{(m-t)\,!m^t}\approx 99\%$. This motivates us to design the following two-layer protocol: In the first layer, we use a hash function to partition the two sets into $\lceil\frac{t}{c}\rceil$ subsets for some small constant $c$ (say $5$), just like the first step of our straw-man scheme. The objective, which is however different from before, is to make each subset pair contains roughly $c$ exclusive elements on average. In the second layer, we use the straw-man scheme with the same configuration (number of subsets $m$, and error-correction capability $\tau$) to reconcile each subset pair. 

\autoref{proto:II} shows the pseudocode of our scheme. It first uses the same hash-function based random partition algorithm as \autoref{alg:random-part} to partition elements into $k\triangleq\lceil \frac{t}{c} \rceil$ subsets. Note that the random partition only guarantees that each such subset 
contains $c$ exclusive elements on average, and the exact number is not known. Hence, our scheme uses a BCH code with a capability of 
correcting up to $\tau$ errors with $\tau > c$ to make sure that the BCH code has a high probability to decode successfully. We will describe how to deal with situation where the size of set difference exceeds $\tau$ later in~\autoref{subsec:exceptions}.

As the decoding of a $\tau$-error-correcting BCH code where $\tau$ is a small constant has a constant-time computational complexity, the decoding complexity of 
our scheme is $O(k)=O(t)$. We now have several parameters, average number of exclusive elements in each subset $c$, the correcting capability $\tau$ of BCH code, the number of smaller subsets $m$ for each subset to be divided to, and the number of rounds $r$. How to tune these parameters to achieve favorable performance will be detailed later in~\autoref{sec:tail_bound}. 

\IncMargin{1em}
\begin{algorithm}
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
\Input{Size of set difference $t$}
\Input{The number of subsets $m$ for each partition}
\Input{Average number of exclusive elements in each partition $c$}
\Input{BCH code capability $\tau$}

$k \leftarrow \lceil \frac{t}{c}\rceil $\;

Partition elements into $k$ subsets using~\autoref{alg:random-part}\;

\For{$j = 0$ \KwTo $k-1$}{
    Reconcile the $j$-th subset pair using the straw-man scheme with the BCH correcting capability $\tau$, number of smaller subsets $m$, and number of rounds $r$\;
}

\caption{Our Scheme} \label{proto:II}
\end{algorithm}\DecMargin{1em}




\subsection{Exceptional Handling}\label{subsec:exceptions}

{\bf To be revised~}

In this section, we will elaborate how to handle the following two types of exceptions that we mentioned in \autoref{sec:multiround} and \autoref{subsec:protocol2}:
\begin{itemize}
    \item Exception 1: A subset pair has odd number ($\geq 3$) of exclusive elements and causes false-positives (i.e., a decoded distinct element is not a real one);
    \item Exception 2: A subset pair contains too many exclusive elements, such that a BCH code with capability of correcting up to $\tau$ errors cannot decode it (i.e., $t>\tau$).
	\item Exception 3: A subset pair has even number ($\geq 2$) of exclusive elements and causes false-negatives(i.e., two or more distinct elements are neglected as the parity bit is 0);
\end{itemize}

To handle Exception 1, we need to check whether a computed exclusive element by \autoref{alg:trivial_case} is a real exclusive element or not. (The group index happens to come in handy if we use it as a fingerprint of the element we computed. If this element is truly an exclusive element, it should be hashed into the same group as before. Notably, We have two group indices available for this check, one is in the initial divide and conquer phase, the other is in the BCH code part) It can be easily done at the end of set reconciliation, during which two hosts exchange their exclusive elements. In fact, as we will elaborate in \autoref{sec:tail_bound}, Exception 1 hardly happens if we set parameters properly. 

On the other hand, when Exception 2 happens, the BCH decoder will report a failure about exceeding the error-correction capability. For such a subset pair, we can use the same approach as in \autoref{subsec:protocol2} to partition it into smaller subsets and use the straw-man scheme to reconcile them respectively. We set the number of small subsets to be 3. It is because, as we will elaborate in \autoref{sec:tail_bound}, the number of exclusive elements for each subset pair $t$ should be, if not smaller, only slightly larger than $\tau$ w.h.p.. Partitioning those exclusive elements into 3 small subsets is enough to guarentee that each of them has less than $\tau$ exclusive elements.

\end{comment}

==> section/schemes_new_without_comments.tex <==
%\section{PBS for small \texorpdfstring{$d$}{d}}\label{sec:scheme}
\section[PBS for small \texorpdfstring{$d$}{d}]{PBS for small \texorpdfstring{\larger\boldmath\MakeLowercase{$d$}}{d}}\label{sec:scheme}
%\section{Set Reconciliation}\label{sec:scheme}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%     Writing Guideline for This Section     %%%%%%%%%%
% “balls – elements in the symmetric difference of the two sets” 

% Protocol 0 (reconcile two sets whose set difference has at most one ball)

% Protocol I.I (partition elements into a sufficiently large number of subsets such that each subset has at most one ball with high probability and use Protocol 0 to reconcile each of them) 

% Protocol I.II (a two-step refinement of Protocol I.I: first use BCH to identify good bins, i.e., bins/subsets have exactly one ball, and then use Protocol 0 to reconcile each good bin) 

% Protocol II (a two-layer refinement of Protocol I.II: in the first layer, we partition elements into t/c subsets, where t is the size of set difference and c is a small constant, then each subset has c balls on average. In the second layer, we further partition each subset into large enough number of bins/subsets such that with high probability each bin has at most one ball, then use Protocol I.II to reconcile them one by one) 

% Protocol III/IV (mainly fix certain exceptions in Protocol II，e.g., how to address bad bins, how to handle the cases where BCH fails to decode and etc)

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% In this section, we describe our set reconciliation scheme in details. First, we give a formal problem statement in \autoref{sec:model}. In \autoref{subsec:protocol0}, we introduce a basic scheme for the trivial case, in which the two sets $A$ and $B$ has at most one distinct element. Building upon the basic scheme, we propose the preliminary version of scheme in \autoref{sucsec:our-scheme} that targets to the cases where the total number of distinct elements $d$ is small. Then we extend the preliminary version and propose the final version of our scheme in \autoref{subsec:protocol2} for general cases (i.e., any arbitrary $d$). We assume $d$ is precisely known throughout this section except in \autoref{subsec:ToW}, where we will describe how to estimate $d$ using a Tug-of-War Estimator. 


In this section, we describe our PBS scheme for Alice and Bob to reconcile their respective sets $A$ and $B$, where $d=|A\Delta B|$ is small and precisely known. Throughout this paper, we call each element in $A\Delta B$ a \textit{distinct element}, and each element in $A\bigcap B$ a \textit{common element}. We build up our scheme gradually by starting with the trivial case where $d\leq 1$ in \autoref{subsec:protocol0}. Then we generalize our scheme to the case where $d$ is a small number in \autoref{sec:pbs_smalld}. 

\begin{comment}
\subsection{Problem Statement}\label{sec:model}

In this work, we adopt the commonly used model for the set reconciliation problem. 
Two remote sets $A$ and $B$ are stored at hosts Alice and Bob respectively. 
Each element in $A$ and $B$ is a hash signiture in the key space (universe) $\mathcal{U}$, which is the set of all $(\log |\mathcal{U}|)$-bit binary strings. 
%Each element in $A$ and $B$ is a hash signiture with signiture width $w$ in the key space (universe) $\mathcal{U}$, which is the set of all $w$-bit binary strings (i.e., $|\mathcal{U}|=2^w$). 
%We use $\mathcal{U}$ to denote the set of all $w$-bit binary strings and name it the universe of signitures. 
The set reconciliation problem is to compute the symmetric set difference between $A$ and $B$, 
{\it i.e.,} $A\Delta B\triangleq (A\!\setminus\! B) \bigcup (B\!\setminus\! A)$. 
Let $d\!=\!|A\Delta B|$ be the cardinality of this difference.
%We denote $d\!=\!|A\Delta B|$. 
Throughout this paper, we call each element in $A\Delta B$ a \textit{distinct element}, and each element in $A\bigcap B$ a \textit{common element}.
{\bf Like in all existing solutions, we describe only {\it unidirectional} set reconciliation, in which Alice or Bob learns the set difference $A\Delta B$. Since the performance of our scheme does not depend on who learns the set difference, we assume Bob learns the set difference $A\Delta B$ in the rest of the paper, as mentioned in \autoref{sec:psea}.}
% As mentioned in \autoref{sec:psea}, we describe {\it unidirectional} set reconciliation that Bob learns the set difference $A\Delta B$. 
%In \autoref{sec:evaluation}, we use the same semantic to measure the communication cost of our scheme and other compared set reconciliation schemes. 
\end{comment}

% In the rest of this section, we build up our scheme gradually as follows: We start with the trivial case where $d\leq 1$ in \autoref{subsec:protocol0}. Then we generalize our scheme to the case where $d$ is a small number in \autoref{sec:pbs_smalld}. 

%After that, we further generalize our scheme to the case that $d$ is a large number in \autoref{subsec:protocol2}. 
%Throughout this section, we assume $d$ is precisely known.
%except in \autoref{subsec:ToW}, where we will describe how to estimate $d$ using a Tug-of-War Estimator. 

%The rest of this section is organized as follows: In \autoref{subsec:protocol0}, we introduce a basic scheme for the trivial case, in which the two sets $A$ and $B$ has at most one distinct element. In \autoref{sucsec:our-scheme} and \autoref{subsec:protocol2}, we elaborate the two versions of our solution that are introduced in \autoref{sec:smalld} and \autoref{sec:larged} respectively. Throughout this section, we assume $d$ is precisely known except in \autoref{subsec:ToW}, where we will describe how to estimate $d$ using a Tug-of-War Estimator. 

\subsection{The Trivial Case of \texorpdfstring{\larger\boldmath $d\leqslant 1$}{d<2}}\label{subsec:protocol0}

%We start with the trivial case, in which $A$ and $B$ have at most one distinct element ({\it i.e.,} $d\leq 1$), we have a simple set reconciliation scheme showed in \autoref{alg:trivial_case}:

\autoref{alg:trivial_case} shows the reconciliation scheme for the trivial case, in which $A$ and $B$ differ by at most one distinct element:

\begin{algorithm}
\caption{Set reconciliation when $d\le 1$}
\label{alg:trivial_case}

{\it Bob}: $s_B\leftarrow\underset{b\in B}{\oplus} b$; Send $s_B$ to Alice\; \label{alg1:sender}

{\it Alice}: $s_A\leftarrow\underset{a\in A}{\oplus} a$; $s\leftarrow s_A \oplus s_B$\; \label{alg1:receiver}
\end{algorithm}

First, Bob calculates $s_B$, the bitwise \code{XOR} of all elements in $B$, and send it to Alice. 
Second, Alice also calculates $s_A$, the bitwise \code{XOR} of all elements of $A$. Upon receiving $s_B$, Alice computes $s\!\triangleq\! s_A \!\oplus\! s_B$, and we have

\begin{sitemize}
	\item If $A$ and $B$ are identical sets (i.e., $d=0$), we have $s_A=s_B$ and $s=\mathbf{0}$;
	\item If $A$ and $B$ has one distinct element (i.e., $d=1$), the computed $s$, the bitwise \code{XOR} of $s_A$ and $s_B$, will cancel out all common elements and remain the distinct element. In other words, we have $A\Delta B=\{s\}$. 
	%And $s$ is the missing element of $A$ (i.e., $s\in B\!\setminus\! A$) if $s\in B$, or the missing element of $B$ (i.e., $s\in A\!\setminus\! B$) otherwise;
	% \item If $A$ and $B$ has more than one distinct elements (i.e., $d>1$), the bitwise \code{XOR} of $s_A$ and $s_B$ will still cancel out all common elements and remain the \code{XOR} of the distinct elements, i.e., $s$ is the \code{XOR} of all distinct elements;
\end{sitemize}

Like most works on set reconciliation, we assume $\mathbf{0}$ is excluded from $\mathcal{U}$, as \autoref{alg:trivial_case} does not work when $\mathbf{0}\in A\bigcap B$ for the following reason: When $s=\mathbf{0}$, \autoref{alg:trivial_case} cannot tell whether $A$ and $B$ are identical, or they have a distinct element of value $\mathbf{0}$. 
%However, we can extend our scheme to support $\mathbf{0}$. For example, we let Alice send to Bob a single bit to indicate whether Alice has element $\mathbf{0}$, so Bob will know whether $\mathbf{0}\in A\Delta B$ or not. 
\autoref{alg:trivial_case} also does not work when there are more than one distinct elements in $A\Delta B$ (i.e., $d>1$), since the computed $s$ is the \code{XOR} of all these distinct elements.

% Note that \autoref{alg:trivial_case} works if and only if $|A\Delta B|\!\leq\! 1$ and $0\!\notin\! (A\!\cup\! B)$ (which we have explained in~\autoref{sec:model}). 

%\subsection{PBS: When $d$ is small}\label{sucsec:our-scheme}

%In this section, we generalize PBS to the case when $d$ is a small number, as we described in \autoref{sec:smalld}. 
%First, we describe each step of single-round PBS from \autoref{sec:hash_partition} to \autoref{sec:reconcile_by_trivial} and summarize it in \autoref{sec:single_round_pbs}. Second, we discuss the exceptions in single-round PBS in \autoref{subsec:exception_hash_partition}. Third, we propose multi-round PBS to handle the exceptions.

\subsection{PBS for small \texorpdfstring{\larger\boldmath $d$}{d}}\label{sec:pbs_smalld}

In this section, we substantiate the scheme described in \autoref{sec:smalld} for small $d$.

\subsubsection{Hash Partition and Parity Bitmap Encoding}\label{sec:hash_partition}
% \medskip
% \noindent{\bf Hash Partition} 

Here we formalize the aforementioned process of partitioning $A$ into $\{A_i\}_{i=1}^n$, $B$ into $\{B_i\}_{i=1}^n$, and $A\Delta B$ into $\{A_i\Delta B_i\}_{i=1}^n$ 
using a hash function $h(\cdot)$.
%as described in \autoref{sec:smalld} by introducing the concept of {\it sub-universes}. Given a hash function $h(\cdot): \mathcal{U}\rightarrow \{1,2,\cdots,n\}$, we 
Define {\it sub-universe} $\mathcal{U}_i$ as the set of elements in the universe $\mathcal{U}$ that are hashed into value $i$. More precisely, $\mathcal{U}_i\triangleq\{s\!\mid\! s\in \mathcal{U} \mbox{ and } h(s)=i\}$ for $i=1,2,...,n$. Then defining $A_i\triangleq A\bigcap\mathcal{U}_i$ and $B_i\triangleq B\bigcap\mathcal{U}_i$ for $i=1,2,...,n$ induces the partitioning of $A$, $B$, and $A\Delta B$.
%, as mentioned in \autoref{sec:smalld}. 

{\bf (merged from the later two paragraphs)} How the $d$ distinct elements (balls) in $A\Delta B$ are distributed into the $n$ subset-pair-differences $\{A_i\Delta B_i\}_{i=1}^n$ (bins) can be viewed as throwing $d$ balls each uniformly and randomly into one of the $n$ bins. 
For the moment, we assume the following {\it ideal case} happens: Every subset-pair-difference $A_i\Delta B_i$ contains at most one distinct element.  
The ideal case corresponds to the $d$ balls ending up in $d$ distinct bins. It happens with probability $\prod_{k=1}^{d - 1}(1 - \frac{k}{n})$, which is on the order of $1-O(d^2/n)$ when $n\!\gg\!d$.
%approximately $e^{-\frac{d(d-1)}{2n}}$ when $d\!\ll\!n$. 
Hence, $n$ must be $\Omega(d^2)$ to ensure the ideal case happens with a nontrivial probability, as mentioned in \autoref{sec:smalld}. 
%The nonideal case of a subset pair difference containing more than $1$ distinct elements will be discussed in \autoref{subsec:exception_hash_partition}.

% {\bf (Previous)} For the moment, we assume the following {\it ideal case} happens: Every subset-pair-difference $A_i\Delta B_i$ contains at most one distinct element. The nonideal case of a subset pair difference containing more than $1$ distinct elements will be discussed in \autoref{subsec:exception_hash_partition}. 

%In this section, we give a detailed description on how to partition $A$ and $B$ (as introduced in \autoref{sec:smalld}) by introducing {\it sub-universes}, which is defined as follows: Given a hash function $h(\cdot): \mathcal{U}\rightarrow \{1,2,\cdots,n\}$, we define {\it sub-universes} $\{\mathcal{U}_i\}_{i=1}^n$, a partition of the universe $\mathcal{U}$, as $\mathcal{U}_i=\{s\!\mid\! s\in \mathcal{U} \mbox{ and } h(s)=i\}$ for $i=1,2,...,n$. Based on $\{\mathcal{U}_i\}_{i=1}^n$, we define $\{A_i\}_{i=1}^n$, the partition of $A$ introduced in \autoref{sec:smalld}, as $A_i\! \triangleq\! A\bigcap \mathcal{U}_i$ for $i=1,2,...,n$. $\{B_i\}_{i=1}^n$ is similarly defined. By this definition, the set difference $A\Delta B$ is partitioned into $n$ set differences of the partitioned subset pairs (i.e., $\{(A_i, B_i)\}_{i=1}^n$). From \autoref{sec:hash_partition} to \autoref{sec:reconcile_by_trivial}, we assume the following {\bf ideal case} happens: Each subset pair $(A_i, B_i)$ contains at most one distinct element ({\it i.e.,} $|A_i\Delta B_i|\!\leq\!1$). The nonideal case of a subset pair contains more than $1$ distinct elements will be discussed in \autoref{subsec:exception_hash_partition}. 

% Here we describe the hash-partition step introduced in \autoref{sec:smalld} in details. First, we use a hash function $h(\cdot): \mathcal{U}\rightarrow \{1,2,\cdots,n\}$ to partition the universe $\mathcal{U}$ into $n$ sub-universes: $\mathcal{U}_i=\{s\!\mid\! s\in \mathcal{U} \mbox{ and } h(s)=i\}$ for $\forall i=1,2,\cdots,n$. The hash function $h(\cdot)$ can be predetermined between Alice and Bob and does not require additional communication cost. Define $A_i\! \triangleq\! A\bigcap \mathcal{U}_i$ and $B_i\! \triangleq\! B\bigcap \mathcal{U}_i$ for $i=1,2,\cdots,n$. Then $\{A_i\}_{i=1}^n$ and $\{B_i\}_{i=1}^n$ are partitions of $A$ and $B$ respectively. Furthermore, $\{A_i\Delta B_i\}_{i=1}^n$ is a partition of $A\Delta B$. From \autoref{sec:hash_partition} to \autoref{sec:reconcile_by_trivial}, we assume the following {\bf ideal case} happens: Each subset pair $(A_i, B_i)$ contains at most one distinct element ({\it i.e.,} $|A_i\Delta B_i|\!\leq\!1$). The nonideal case of a subset pair contains more than $1$ distinct elements will be discussed in \autoref{subsec:exception_hash_partition}. 

% {\bf (Previous)} How the $d$ distinct elements (balls) in $A\Delta B$ are distributed into the $n$ subset pair differences $\{A_i\Delta B_i\}_{i=1}^n$ (bins) 
% can be viewed as throwing $d$ balls each uniformly and randomly into one of the $n$ bins. 
% %follows the familiar {\it balls-into-bins} probability model. 
% %The distinct elements are viewed as balls and the subset pairs are viewed as bins. 
% %Each of the $d$ balls is uniformly and randomly thrown by the hash function $h(\cdot)$ into one of the $n$ bins. 
% The aforementioned ideal case that corresponds to the $d$ balls ending up in $d$ distinct bins happens with probability $\prod_{k=1}^{d - 1}(1 - \frac{k}{n})$, which is on the order of $1-O(d^2/n)$ when $d\!\ll\!n$.
% %approximately $e^{-\frac{d(d-1)}{2n}}$ when $d\!\ll\!n$. 
% Hence, $n$ must be $\Omega(d^2)$ to ensure the ideal case happens with a nontrivial probability, as mentioned in \autoref{sec:smalld}.


%in which the distinct elements are viewed as balls and the subset pairs are viewed as bins. The hash-parition basically throws (hashes) $d$ balls (distinct elements) uniformly and randomly into $n$ bins (subset pairs). The aforementioned ideal case in this context becomes, after throwing $d$ balls uniformly and randomly into $n$ bins, each bin receives at most $1$ ball (i.e., $d$ nonempty bins have $1$ ball in each and the rest $n-d$ bins are empty). The number of balls in each bin is a Binomial random variable $Binomial(d,1/n)$.
%{\bf It may remind readers about the Birthday problem. And the ideal case can be analogous to the case that no people share the same birthday.} 
% The ideal case happens with a probability of $p\!=\!\prod_{k=1}^{d - 1}(1 - \frac{k}{n})\!\approx\! e^{-\frac{d(d-1)}{2n}}$ when $d\!\ll\!n$. In other words, $n$ must be at least $O(d^2)$ to ensure the ideal case happens with a nontrivial probability, as described in \autoref{sec:smalld}.  

% Note that the ideal case does not always happen. However, we can ensure that the ideal case happens with high probability by properly setting $n$ based on $d$ (i.e., $n=\Omega(d^2)$). Furthermore, as we will describe in \autoref{subsec:nonideal}, even if the ideal case does not happen (i.e., some distinct elements are hashed into the same subset pair), most of the distinct elements should be distributed into different subset pairs and therefore can be reconciled. So the scheme, even cannot reconcile all of the distinct elements, can still reconcile the majority of them (i.e., piecewise decodability in \autoref{sec:intro_oursolution}). Based on this property, we will extend our scheme from single-round to multi-rounds in \autoref{subsec:nonideal} to further increase the probability of reconciling all distinct elements. 

% \medskip
% \noindent{\bf Parity Bitmap Encoding} 

{\bf (Modified)} The partition $\{A_i\}_{i=1}^n$ is encoded into an $n$-bit-long parity bitmap $A[1..n]$, in which $A[i]$, the $i$-th bit of the parity bitmap, is equal to the oddness / evenness (parity) of the cardinality of $A_i$ (i.e., $A[i]=1$ if $|A_i|$ is odd; otherwise $A[i]=0$). $B[1..n]$, the parity bitmap of $\{B_i\}_{i=1}^n$, is similarly defined. In the ideal case, $A[1..n]$ and $B[1..n]$ differ in exactly $d$ bit positions $i_1,i_2,...,i_d$, and subset-pair-differences $(A_{i_1},B_{i_1}), (A_{i_2},B_{i_2}),...,(A_{i_d},B_{i_d})$ contains exactly $1$ distinct element in each. If Bob knows $i_1,i_2,...,i_d$, he can start to reconcile the $d$ subset pairs respectively using \autoref{alg:trivial_case}, then Alice will obtain $A\Delta B$.

% {\bf (Previous)} We encode $\{A_i\}_{i=1}^n$ into an $n$-bit-long parity bitmap $A[1..n]$, in which $A[i]$, the $i^{th}$ bit of the parity bitmap, is equal to the oddness / evenness (parity) of the cardinality of $A_i$ (i.e., $A[i]=1$ if $|A_i|$ is odd; otherwise $A[i]=0$). In the ideal case, the two bitmaps $A[1..n]$, $B[1..n]$ differ in exactly $d$ bit positions $i_1,i_2,...,i_d$, each of which corresponds to a subset pair that contains $1$ distinct element. The next step is to let Alice and Bob know these bit positions.
%Once the $d$ bit positions are known, Alice and Bob can start to reconcile $(A_{i_1},B_{i_1}), (A_{i_2},B_{i_2}),...,(A_{i_d},B_{i_d})$ using \autoref{alg:trivial_case} and obtain the $d$ distinct elements (i.e., $A\Delta B$). 

% \subsubsection{Parity Bitmap Encoding}\label{sec:parity_bitmap_encoding}

% %After hash-partitioning $A$ and $B$ into partitions $\{A_i\}_{i=1}^n$ and $\{B_i\}_{i=1}^n$, 
% As introduced in \autoref{sec:smalld}, we encode each partition into an $n$-bit-long parity bitmap and denote them as $A[1..n]$ and $B[1..n]$ respectively, as introduced in \autoref{sec:smalld}. For $i=1,2,...,n$, $A[i]$ (the $i^{th}$ bit of the parity bitmap $A[i]$) is equal to $1$ if $A_i$ contains an odd number of elements, and is equal to $0$ otherwise.
% % More specifically, for $i=1,2,...,n$, $A[i]$ (the $i^{th}$ bit of the parity bitmap $A[i]$) is defined as follows: $A[i]=1$ if $A_i$ contains an odd number of elements, and $A[i]=0$ otherwise. In this way, each bit $A[i]$ encodes the oddness / evenness (parity) of the cardinality of $A_i$. The $n$-bit-long parity bitmap $B[1..n]$ and $B[i]$ (the $i^{th}$ bit of $B[1..n]$) are similarly defined. 
% In the ideal case, 
% %$A[i]$ and $B[i]$ differ if and only if $A_i$ and $B_i$ have exactly $1$ distinct element, and $A[i]$ and $B[i]$ are the same if and only if $A_i=B_i$. Meanwhile, the $d$ distinct elements are hashed into $d$ different subset pairs. So 
% the two bitmaps $A[1..n]$, $B[1..n]$ differ in exactly $d$ bit positions, each of which corresponds to a subset pair that contains $1$ distinct element. Once the $d$ bit positions are known, Alice starts to reconcile each of the $d$ corresponding subset pairs by \autoref{alg:trivial_case} and gets the $d$ distinct elements (i.e., $A\Delta B$). 
% %If knowing the $d$ bit positions (i.e., the $d$ corresponding subset pairs), we can use \autoref{alg:trivial_case} to reconcile the $d$ subset pairs respectively to obtain all the $d$ distinct elements (i.e., $A\Delta B$). 
% In \autoref{sec:BCH_code}, we will describe how to find the $d$ bit positions using BCH code~\cite{Lint_IntroductionCodingTheory_1998}. 

% \medskip
% \noindent{\bf Find the $d$ Bit Positions Using ECC} 

%\subsubsection{Find the $d$ Bit Positions Using ECC}\label{sec:BCH_code}
\subsubsection{Find and Reconcile the \texorpdfstring{$d$}{d} subset pairs}\label{sec:BCH_code}

{\bf (Modified)} To let Bob obtain $i_1,i_2,...,i_d$, Alice only needs to send a BCH code of $A[1..n]$ that can correct $d$ bit errors. Then Bob can decode and recover $A[1..n]$ (original message) and obtain $i_1,i_2,...,i_d$.

% {\bf (Previous)} We view $A[1..n]$ as a corrupted message of $B[1..n]$ sent ({\bf not actually being sent}) from Bob to Alice through an {\it unreliable} commnunication channel that flips $d$ bits. To locate these $d$ bit positions, we let Bob also send an {\it error-correction code} that encodes $B[1..n]$ to Alice, such that Alice can recover $B[1..n]$ (original message) and obtain the $d$ bit positions $i_1,i_2,...,i_d$. In PBS, we use BCH code~\cite{bch1} to encode $B[1..n]$ and get the error-correction code.

There are two different BCH encoding techniques: {\it systematic} and {\it unsystematic}. The difference is, the message appears as the prefix of the codeword (i.e., codeword = [message net-codeword]) in systematic BCH encoding, whereas it does not appear as a substring of the codeword in unsystematic BCH encoding. In PBS, we choose systematic BCH encoding because we are not actually sending the ``message'', and only the net-codeword is transmitted from Alice to Bob. 
To correct $d$ bit errors, the length of the net-codeword only is no more than $d\log n$ bits. We use the term `codeword' to refer to the net-codeword in the rest of this paper.
%The computational complexity of the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} is $O(d^2\log^2 n)$.

%The systematic BCH encoding is also used in other ECC-based set reconciliation works, such as PinSketch \cite{Wuille_Minisketchoptimizedlibrary_2019}, while PinSketch encodes a much longer message (e.g., $2^{32}$ bits) than in ours (hundreds of bits).  

%\subsubsection{Find the $d$ Bit Positions Using ECC}\label{sec:BCH_code}

% A straightforward approach to find the $d$ bit positions is to let Bob send the complete parity bitmap $B[1..n]$ to Alice, then Alice compares $A[1..n]$ with $B[1..n]$ locally. This approach has a communication overhead of $n$ bits, which is quite wasteful. As we discussed in~\autoref{sec:hash_partition}, $d$ is usually much smaller than $n$. It means $A[1..n]$ and $B[1..n]$ differ only at a tiny portion of bits. Therefore, we can view $A[1..n]$ as a corrupted message of $B[1..n]$ with $d$ bit errors, and the bit positions of the $d$ bit errors basically correspond to the $d$ subset pairs that contain distinct elements. The detection of bit errors, on the other hand, can be solved by Error-Correction Code (ECC)~\cite{Lin_ErrorControlCoding_1983}. 

% Since $A[1..n]$ and $B[1..n]$ differ at $d$ bit positions, we can view $A[1..n]$ as a corrupted message of $B[1..n]$ from Bob to Alice through an {\it unreliable} commnunication channel with $d$ corrupted bits, which are located on the $d$ bit positions. Therefore, to find the $d$ bit position, we only need to correct the $d$ corrupted bits in $A[1..n]$, which is done by transmitting a ``code'' that can correct upto $d$ bit errors from Bob to Alice through a {\it reliable} communication channel. 

% In PBS, we use {\it systematic} BCH code to generate the ``code'' by encoding the message $B[1..n]$. The codeword of the systematic BCH code is in the form of [message, net-codeword], since the message appears as the prefix of the codeword in systematic BCH code. The ``code'' is simply the net-codeword in the BCH codeword. We choose {\it systematic} BCH code because the (corrupted) message is already transmitted and we only need to pay a small communication overhead on transmitting ``code'' (i.e., net-codeword). To correct upto $d$ bit errors, the length of the net-codeword is no more than $d\log n$ bits, which is much smaller than the message when $d\!\ll\! n$. The computational complexity of the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} is $O(d^2\log^2 n)$. This type of BCH code is also used in other ECC-based set reconciliation works, such as PinSketch \cite{Wuille_Minisketchoptimizedlibrary_2019}. 

% Different from {\it unsystematic} BCH code
% The ``code'' is generated by {\it systematic} BCH code, which encodes the message $B[1..n]$ into a BCH codeword in the form of [message, net-codeword]. The ``code'' transmitted on the reliable channel is the net-codeword of the BCH codeword. In {\it systematic} BCH code, the message appears as the prefix of the codeword. 

% More specifically, PBS uses {\it systematic} BCH code~\cite{Lint_IntroductionCodingTheory_1998} that can correct upto $d$ bit errors to encode the parity bitmaps. In the {\it systematic} BCH code \footnote{In unsystematic BCH code, message does not appear to be the prefix of the codeword}, the message (i.e., the parity bitmap) appears as the prefix of the raw codeword, which in the form of [message, net codeword]. Normally, to correct upto $d$ errors, the length of the net codeword is $2n\log d$, where $n$ is the length of the message (i.e., parity bitmap). However, our case is special in the sense that the net codeword is error-free (all $d$ bit errors are in the message), so the length of the net codeword can be reduced to $n\log d$. This type of BCH code is also used in other ECC-based set reconciliation works, such as PinSketch \cite{Wuille_Minisketchoptimizedlibrary_2019}. 

% Now we can formally describe how to find the $d$ bit positions: First, Bob uses a $d$-error-correcting systematic BCH code to encode $B[1..n]$ and sends the net codeword ($d\log n$ bits) to Alice. Upon receiving the net codeword and combining it with the corrupted message $A[1..n]$, Alice uses the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} to decode the $d$ bit errors in $A[1..n]$. The communication overhead of transmitting the net codeword is $d\log n$ bits. The computational complexity of the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} is $O(d^2\log^2 n)$. Both the communication overhead and the computational complexity here are relatively small when $d$ is small.

% \medskip
% \noindent{\bf Reconcile the $d$ subset pairs using \autoref{alg:trivial_case}} 

%Once the $d$ bit positions are known, Alice can start to reconcile $(A_{i_1},B_{i_1}), (A_{i_2},B_{i_2}),...,(A_{i_d},B_{i_d})$ using \autoref{alg:trivial_case} and obtain the $d$ distinct elements (i.e., $A\Delta B$). 
Once Bob decodes the codeword to obtain $i_1,i_2,...,i_d$, the corresponding subset pairs $(A_{i_1},B_{i_1}), (A_{i_2},B_{i_2}),...,(A_{i_d},B_{i_d})$ each can be reconciled using \autoref{alg:trivial_case}. To do so, Bob needs to send the respective \code{XOR} sums of the subsets $A_{i_1}$, $A_{i_2}$, ...,$A_{i_d}$. In addition, Bob needs to send $i_1,i_2,...,i_d$ to Alice, since Alice does not know the indices. Each index needs to be encoded into $\log n$ bits, so the additional communication overhead on transmitting the indices is $d\log n$ bits. 
% When reconciling $(A_{i_1},B_{i_1}), (A_{i_2},B_{i_2}),...,(A_{i_d},B_{i_d})$ using \autoref{alg:trivial_case}, Alice needs to send not only the bitwise \code{XOR} of $A_{i_1}, A_{i_2},..., A_{i_d}$, but also the indices of the subset pairs ($i_1,i_2,...,i_d$), since Bob does not know which of the $d$ subset pairs are being reconciled. Each index is an integer between $1$ and $n$ and can be encoded into $\log n$ bits, So the additional communication overhead on transmitting the indices is $d\log n$ bits. 



% \subsubsection{Reconcile the $d$ subset pairs using \autoref{alg:trivial_case}}\label{sec:reconcile_by_trivial}

% After decoding the $d$ bit errors that corresponds to the $d$ subset pairs, Alice starts to reconcile them using \autoref{alg:trivial_case}. For each of the $d$ subset pairs, Alice needs to send not only the bitwise \code{XOR} of the subset pair, but also the index of the subset pair (since Bob does not know the $d$ subset pairs to reconcile). So the communication overhead on \autoref{alg:trivial_case} is $d\log |\mathcal{U}|+d\log n$ bits. 
%Plus the communication overhead on transmitting the net codeword of parity bitmap ($d\log n$, as we explained in \autoref{sec:BCH_code}), the overall communication overhead of single-round PBS is $d\log u+2d\log n$ bits.

% \medskip
% \noindent{\bf Check if set reconciliation is complete} 

{\bf (Modified)} Once Alice receives the \code{XOR} sums and the indices, she can compute the distinct elements (described in \autoref{subsec:protocol0}) to obtain the set difference (denoted as $\hat{D}$). However, this reconciled set difference could be incorrect if the ideal case does not happen. Therefore, Alice needs to check if set reconciliation is successful (or whether $\hat{D}=A\Delta B$). To do so, we introduce some ``linear'' checksum function $c(\cdot)$ (e.g., bitwise \code{XOR}) that maps an arbitrary set to a $32$-bit checksum. Here the ``linearity'' of a chechsum function refers to that $c(S_1\Delta S_2)=c(S_1)\oplus c(S_2)$ for any two sets $S_1$ and $S_2$. We use this checksum function to check if $\hat{D}=A\Delta B$ by comparing $c(\hat{D})$ to $c(A\Delta B)$. Note that $c(\hat{D})$ can be computed in $O(d)$ time and $c(A\Delta B)=c(A)\oplus c(B)$ can be precomputed {\bf during the encoding period, which costs $32$-bit communication overhead on transmitting $c(B)$ from Bob to Alice.}  

% {\bf (Previous)} After reconciling the subset pairs and obtaining the reconciled set difference (denoted as $\hat{D}$), PBS needs to check if set reconciliation is complete (or whether $\hat{D}=A\Delta B$), since the reconciled set difference $\hat{D}$ is not the actual set difference $A\Delta B$ in the nonideal case (to be discussed in \autoref{subsec:exception_hash_partition}). Hence, we add a verfication step after obtaining $\hat{D}$ to check if $\hat{D}=A\Delta B$. In PBS, we check an equivalent condition, $A=B\Delta\hat{D}$, instead of $\hat{D}=A\Delta B$, since $B$ and $\hat{D}$ are both known by Bob and their set difference $B\Delta\hat{D}$ can be locally computed. More specifically, to check if the remote sets $A$ and $B\Delta\hat{D}$ are equal, we let Alice compute a $32$-bit checksum of $A$ and send it to Bob. {\bf Then Bob computes the $32$-bit checksum of $B\Delta\hat{D}$ using the same checksum algorithm and compare the two checksums. In PBS, we select {\it longitudinal parity check} (i.e., bitwise \code{XOR} of all elements in the set) as the checksum algorithm, so that the checksum $B\Delta\hat{D}$ can be efficiently computed as the bitwise \code{XOR} between the checksum of $B$ (can be pre-computed) and that of $\hat{D}$. Other checksum algorithms that are {\it linear} to the set difference operator (i.e., $\Delta$) also work for PBS. }
% Then Bob checks if $B\Delta\hat{D}$ satisfies the receiving checksum. 

{\bf (Modified)} The condition $\hat{D}=A\Delta B$ can be almost surely verified by the checksum, although it could mistakenly believes two different sets as identical ones. This event happens with probability $2^{-32}\approx 2.3\times 10^{-10}$ when the ideal case does not happen, which has a probability on the order of $10^{-2}$. Although this event could cause PBS mistakenly believes the set reconciliation is completed, it happens with an extremely small probability (on the order of $10^{-12}$) and should be acceptable in most applications. To simplify our description, we ignore this small probability event and assume the checksum works perfectly in this rest of this paper. {\bf not a good position to mention `for super critical applications, use a checksum for all groups', since we are describing single-group scenario. }

% {\bf (Previous)} The condition $A=B\Delta\hat{D}$ can be almost surely verified by a $32$-bit checksum, although it could mistakenly believe two different sets as identical ones with probability $2^{-32}\approx 2.3\times 10^{-10}$ {\bf on top of the probability that the nonideal case happens (on the order of $10^{-2}$).} Although this event could cause an ``early'' termination and leave some distinct elements unreconciled, it happens with an extremely small probability (on the order of $10^{-12}$) and should be acceptable in most applications. {\bf To simplify our description, we ignore this small probability event and assume the checksum works perfectly in this rest of this paper. }
%and such an event (i.e., mistaken $A$ and $B\Delta\hat{D}$ are identical when they are different) never happens in our evaluation. For some super critical applications, we can certainly use a $64$-bit checksum to reduce this probability to $5.4\times 10^{-20}$ if needed.

% When the ideal case does not happen, set reconciliation cannot accomplish in one round, as we will explain in \autoref{subsec:exception_hash_partition}. Hence, we add a verfication step to check if set reconciliation is complete. Let $\hat{D}$ denote the set of reconciled elements. The idea of this verification is basically to compare $A$ with $B\Delta \hat{D}$: If $A=B\Delta \hat{D}$ (i.e., $\hat{D}=A\Delta B$), we know the set reconciliation is complete; Otherwise, the set reconciliation is incomplete.  using a $32$-bit checksum. 

\subsubsection{Communication overhead of PBS (First Round)}\label{sec:communication_overhead_single_PBS}

In this section, we summarize all the steps of PBS (in the first round) in \autoref{alg:single_round_pbs}. The overall communication overhead consists of four components: (1) the BCH codeword of $d\log n$ bits in \autoref{step:BCH_encode}; (2) the subset pair indices $i_1,i_2,...,i_d$ in \autoref{step:trivial_reconcile}; (3) the bitwise \code{XOR} sums of sets $B_{i_1}, B_{i_2},...,B_{i_d}$ of $d\log |\mathcal{U}|$ bits in \autoref{step:trivial_reconcile}; and (4) the $32$-bit checksum of $B$ in \autoref{step:terminate_condition}. 

% All the steps of PBS in the first round are summarized in \autoref{alg:single_round_pbs}. The overall communication overhead consists of three components: (1) the BCH codeword of $d\log n$ bits in \autoref{step:BCH_encode}; (2) the subset pair indices $i_1,i_2,...,i_d$ and the corresponding bitwise \code{XOR}s of $d\log n+d\log |\mathcal{U}|$ bits in \autoref{step:trivial_reconcile}; and (3) the $32$-bit checksum of $A$ in \autoref{step:terminate_condition}. 

\begin{algorithm}
\caption{Single-round PBS}
\label{alg:single_round_pbs}

%Hash-partition $A$, $B$ into $\{A_i\}_{i=1}^n$, $\{B_i\}_{i=1}^n$\; \label{step:hash_partition}

%Parity encode $\{A_i\}_{i=1}^n$, $\{B_i\}_{i=1}^n$ into $A[1..n]$, $B[1..n]$\; \label{step:parity_encode}
{\it Alice}: Send BCH codeword of $A[1..n]$ to Bob\; \label{step:BCH_encode}

{\it Bob}: Decode the codeword to obtain $i_1,i_2,...,i_d$\; \label{step:BCH_decode}

{\it Bob}: Send $i_1,i_2,...,i_d$ and the \code{XOR} sums of sets $B_{i_1}, B_{i_2},...,B_{i_d}$ to Alice (\autoref{alg1:sender} in \autoref{alg:trivial_case})\; \label{step:BCH_decode}

{\it Alice}: Obtain $A_{i_1}\Delta B_{i_1}, A_{i_2}\Delta B_{i_2},...,A_{i_d}\Delta B_{i_d}$ by \autoref{alg1:receiver} in \autoref{alg:trivial_case} and obtain $\hat{D}$\; \label{step:trivial_reconcile}

{\it Alice}: Check if $c(\hat{D})=c(A\Delta B)$\; \label{step:terminate_condition}

% {\it Bob}: BCH-Encodeing $B[1..n]$ and send the codeword to Alice\; \label{step:BCH_encode}

% {\it Alice}: Upon receiving the codeword, decode the bit errors between $A[1..n]$ and $B[1..n]$\; \label{step:BCH_decode}

% {\it Alice}: For each bit error, start reconciling the corresponding subset pair by \autoref{alg:trivial_case}\; \label{step:trivial_reconcile}

% {\it Bob}: Upon receiving the reconciled set difference $\hat{D}$, check if $A=B\Delta \hat{D}$ via checksum\; \label{step:terminate_condition}
\end{algorithm}


% \subsubsection{Single-round PBS}\label{sec:single_round_pbs}

% Here we summarize all the steps of single-round PBS and represent it by pseudocode in \autoref{alg:single_round_pbs}. \autoref{step:hash_partition} and \autoref{step:parity_encode} operates at both hosts (i.e., Alice and Bob). \autoref{step:hash_partition} to \autoref{step:trivial_reconcile} have been elaborated from \autoref{sec:hash_partition} to \autoref{sec:reconcile_by_trivial}. The last step in \autoref{step:terminate_condition} aims to check whether reconciliation is complete (i.e., $\mathcal{D}=A\Delta B$). More specifically, Alice calculates the checksum (e.g., CRC-$32$) of $A$ and send it to Bob. Then Bob calculates the checksum of $B\Delta \mathcal{D}$ and compares it to the receiving checksum of $A$. If the two checksums are the same, we believe $A=B\Delta \mathcal{D}$ and therefore $\mathcal{D}=A\Delta B$ (i.e., reconciliation is complete); Else, we know some elements are reconciled incorrectly. We classify those elements (i.e., the ones in the set difference between $A\Delta B$ and $\mathcal{D}$) into two subsets $A\Delta B\!\setminus\!\mathcal{D}$ and $\mathcal{D}\!\setminus\!(A\Delta B)$ and refer the elements in the former as {\it false-negatives}, and refer the elements in the later as {\it false-positives}. 

% In the ideal case, neither false-positives nor false-negatives will happen and the two checksums always equal. However, in real life, the ideal case does not always happen. We will discuss the nonideal case in \autoref{subsec:exception_hash_partition}. In our evaluation, we use a $32$-bit checksum for comparing $A$ to $B\Delta \mathcal{D}$ that has {\bf an error probability} roughly $10^{-9}$. This error (i.e., mistake $A=B\Delta \mathcal{D}$) incurs false-negatives. All set reconciliation schemes have the same problem on their termination conditions (i.e., check whether $\mathcal{D}=A\Delta B$). For some super critical applications, we can certainly decrease the error probability by using more powerful checksums (i.e., $64-$bit). Using a $32$-bit checksum, this kind of false-negatives never happen in the evaluation. 
% %For simplification, we assume no error happens when checking $\mathcal{D}=A\Delta B$ in the rest of the paper.

% \begin{algorithm}
% \caption{Single-round PBS}
% \label{alg:single_round_pbs}

% Hash-partition $A$, $B$ into $\{A_i\}_{i=1}^n$, $\{B_i\}_{i=1}^n$\; \label{step:hash_partition}

% Parity encode $\{A_i\}_{i=1}^n$, $\{B_i\}_{i=1}^n$ into $A[1..n]$, $B[1..n]$\; \label{step:parity_encode}

% {\it Bob}: Encode $B[1..n]$ by BCH code, then send the codeword to Alice\; \label{step:BCH_encode}

% {\it Alice}: Upon receiving the codeword, decode the bit errors between $A[1..n]$ and $B[1..n]$\; \label{step:BCH_decode}

% {\it Alice}: For each bit error, reconcile the corresponding subset pair by \autoref{alg:trivial_case}\; \label{step:trivial_reconcile}

% {\it Bob}: Upon the reconciled distinct elements $\mathcal{D}$, check whether $A=B\Delta \mathcal{D}$ via checksum\; \label{step:terminate_condition}
% \end{algorithm}

\subsubsection{Exception Handling}\label{subsec:exception_hash_partition}

When the ideal case does not happen, some subset pair may contain more than $1$ distinct elements and cannot be successfully reconciled by \autoref{alg:trivial_case}. We can classify the possible exceptions that happen in such a subset pair into the following two types of events: 

\noindent {\bf Type (\RN{1})}: Subset pair $(A_i, B_i)$ contains even number ($\geq 2$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be the same and PBS will not reconcile the subset pair yet in this round. This event happens with a small but nontrivial probability: For example, $d=5$ and $n=255$ (i.e., throwing $5$ balls uniformly and randomly into $255$ bins), the probability that some bin has an even number of (in this case either $2$ or $4$) balls is roughly $0.04$. 
%Note that when a type (\RN{1}) event happens, the checksum (\autoref{step:terminate_condition} in \autoref{alg:single_round_pbs}) can detect that the set reconciliation has not been completed. Then PBS will start another round to reconcile the ``hidden'' distinct elements (the ones that have not been reconciled in this round), 
%so on so force, until all distinct elements are successfully reconciled and the checksum is verified to be correct, 
%as we will describe in \autoref{sec:multi-rounds}. 

% Note that when a Type (\RN{1}) subset pair exists, the $32$-bit checksum (\autoref{step:terminate_condition} in \autoref{alg:single_round_pbs}) can almost surely detect that the set reconciliation is incomplete. If this is the case (i.e., the checksum is verified to be incorrect), PBS will start another round of set reconciliation to reconcile the remaining distinct elements (e.g., the ``hidden'' distinct elements in Type (\RN{1}) subset pairs), so on so force, until all distinct elements are reconciled and the checksum is verified to be correct, as we will describe in \autoref{sec:multi-rounds}. 

\noindent {\bf Type (\RN{2})}: Subset pair $(A_i, B_i)$ contains odd number ($\geq 3$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be different and PBS will reconcile the subset pair using \autoref{alg:trivial_case}. The reconciled element (i.e., $s$ in \autoref{alg:trivial_case}) is however a ``fake'' distinct element, which is actually the bitwise \code{XOR} of all distinct elements in $(A_i, B_i)$ (explained in \autoref{subsec:protocol0}).
%, which will be mistakenly believed as the distinct element of $(A_i, B_i)$. 
This event happens with a tiny probability: Use the same example above ($d=5$ and $n=255$), the probability that some bin has $3$ or $5$ balls is only $1.52\times 10^{-4}$. 
%Similarly, the $32$-bit checksum can also detect that the set reconciliation has not been completed when a type (\RN{2}) event happens. Both the ``hidden'' and the ``fake'' distinct elements can also be reconciled in later rounds. 

%Note that those ``fake'' distinct elements will become new distinct elements in the next round and therefore incur additional communication overhead to reconcile. 
Note that those ``fake'' distinct elements will incur additional communication overhead if we want to reconcile them in later rounds. Therefore, we add a verification on each reconciled distinct element of \autoref{alg:trivial_case} that can detect ``fake'' distinct elements with high probability. \autoref{alg:verification} shows how this verification works, and it does not incur additional communication overhead.

\begin{algorithm}
\caption{Verify reconciled element $s$ of $(A_i, B_i)$}
\label{alg:verification}
\If{$h(s)\neq i$} {Discard the reconciled element $s$;}
\end{algorithm}

Although a distinct element of $(A_i, B_i)$ must be in sub-universe $\mathcal{U}_i$ (i.e., the hash value of the element under $h$ equals to $i$), a ``fake'' distinct element could be in any sub-universe with probability $1/n$, since it is the bitwise \code{XOR} of multiple distinct elements of $(A_i, B_i)$. Therefore, \autoref{alg:verification} only fails to identify a ``fake'' distinct element with probability $1/n$, which is roughly $3.9\times 10^{-3}$ when $n=255$. On top of the probability of the type (\RN{2}) event, a ``fake'' distinct element that fails to be detected by \autoref{alg:verification} happens with a tiny probability of $6\times 10^{-7}$. {\bf (removed to the beginning of theoretical analysis) To simplify our description, we also ignore this small probability event and assume all ``fake'' distinct elements will be successfully detected by \autoref{alg:verification} in this rest of this paper. }

{\bf Note that either a type (\RN{1}) event or a type (\RN{2}) event will cause PBS fails to reconcile all distinct elements, which can be detected by the checksum (\autoref{step:terminate_condition} in \autoref{alg:single_round_pbs}). In this case, PBS will continue to reconcile the ``remaining'' distinct element by starting another round, as we will describe in \autoref{sec:multi-rounds}. The ``remaining'' distinct elements here consist of (1) the ``hidden'' distinct elements that have not been reconciled in this round and (2) the ``fake'' distinct elements that are not verified by \autoref{alg:verification}. }

% {\bf (to be removed) Readers may wonder encoding the exact subset cardinalities (i.e., $|A_i|, |B_i|$) instead of their oddness / evenness (parity) (described in \autoref{sec:hash_partition}) could help to detect and solve Type (\RN{1}), (\RN{2}) events. However, encoding the exact subset cardinalities not only incurs much more additional communication overhead comparing to encoding their parities, but also barely helps on detecting Type (\RN{1}), (\RN{2}) events, since we cannot precisely derive $|A_i\Delta B_i|$, the total number of distinct elements in $(A_i, B_i)$, even knowing $|A_i|, |B_i|$: For instance, when $|A_i|\!=\!|B_i|\!=\!50$, $|A_i\Delta B_i|$ could be any even number ($\leq 100$) if the distinct elements are evenly splitted and placed between $A_i$ and $B_i$. }

% As we have described in \autoref{sec:hash_partition}, the ideal case does not always happen, which means some subset pair may contain more than $1$ distinct elements and cannot be successfully reconciled by \autoref{alg:trivial_case}. Due to the parity encoding, we can classify such subset pair into the following two scenarios:

% \begin{itemize}
%     \item Scenario 1: If a subset pair $(A_i, B_i)$ contains even number ($\geq 2$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be the same and PBS will not reconcile the subset pair yet in this round;
%     \item Scenario 2: If a subset pair $(A_i, B_i)$ contains odd number ($\geq 3$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be different and PBS will reconcile the subset pair using \autoref{alg:trivial_case}. The reconciled element (i.e., $s$ in \autoref{alg:trivial_case}) is however the bitwise \code{XOR} of all distinct elements in $(A_i, B_i)$ (explained in \autoref{subsec:protocol0}), which will be mistakenly believed as the distinct element of $(A_i, B_i)$. 
%     %However, as described in \autoref{subsec:protocol0}, when a subset pair contains more than $1$ distinct elements, \autoref{alg:trivial_case} will output the bitwise \code{XOR} of them as the `distinct element', which is not an actual distinct element with high probability;
% \end{itemize}

% In both scenarios, the distinct elements in the subset pair will not be reconciled in this round. As we will describe in \autoref{sec:multi-rounds}, we generalize PBS into multi-round, so that the distinct elements that have not been reconciled in the first round will be reconciled in later rounds. On the other hand, the second scenario could result in incorrectly reconciled distinct elements, which will become new distinct elements in the next round in multi-round PBS. 

% % In both scenarios, the distinct elements in the subset pair cannot be successfully reconciled in this round and will remain in the set difference (i.e., $(A\Delta B)\!\setminus\!\hat{D}$). On the other hand, the incorrectly reconciled distinct element in the second scenario will appear as a new distinct element (i.e., $\hat{D}\!\setminus\!(A\Delta B)$) in the next round if we generalize PBS into multi-round (to be elaborated in \autoref{sec:multi-rounds}). Both scenarios can be almost surely detected by the 32-bit checksum (\autoref{step:terminate_condition} in \autoref{alg:single_round_pbs}). The set difference after the reconciliation in this round, $D\Delta\hat{D}$, can be reconciled in later rounds, as we will describe in \autoref{sec:multi-rounds}. 

% Naturally, we do not want to generate new distinct elements in the process of set reconciliation, even though it happens with a tiny probability when $n=\Omega(d^2)$: For instance, when $d=5$ and $n=255$ (i.e., throwing $5$ balls uniformly and randomly into $255$ bins), the probability (i.e., some bin has $3$ or $5$ balls) is only $7.6\times 10^{-6}$. Therefore, we add a verification with no additional communication cost on each reconciled element of \autoref{alg:trivial_case}, such that each incorrect dinstinct element can be identified with high probability. The verfication is shown in \autoref{alg:verification}. 

% \begin{algorithm}
% \caption{Verify reconciled element $s$ of $(A_i, B_i)$}
% \label{alg:verification}
% \If{$h(s)\neq i$} {Discard the reconciled element $s$;}
% \end{algorithm}

% Although any distinct element of $(A_i, B_i)$ must be in sub-universe $\mathcal{U}_i$ (i.e., the hash value of the element under $h$ equals to $i$), the bitwise \code{XOR} of multiple distinct elements of $(A_i, B_i)$ could be in any sub-universe with probability $1/n$. Therefore, \autoref{alg:verification} fails to identify an incorrectly reconciled distinct element in the second scenario with probability $1/n$ that is roughly $3.9\times 10^{-3}$ when $n=255$. In other words, an incorrectly reconciled distinct element that cannot be identified by \autoref{alg:verification} appears with probability $3\times 10^{-8}$. {\bf I feel that defining $\tilde{a}_4=a_1\oplus a_2\oplus a_3$ does not help much.}

% In both scenarios, the distinct elements in the subset pair cannot be successfully reconciled in this round. These distinct elements can be reconciled in later rounds if needed, as we will describe in \autoref{sec:multi-rounds}. In this section, we only discuss how to identify the {\it incorrect} distinct element in the second scenario. Let us use an example to elaborate the second scenario: Assume $(A_i, B_i)$ contains $3$ distinct elements $a_1, a_2, a_3$, then Bob computes $\tilde{s}=a_1\oplus a_2\oplus a_3$ using \autoref{alg:trivial_case} and mistakes it as the distinct element in $(A_i, B_i)$. 

% In both scenarios, the distinct elements in the subset pair cannot be successfully reconciled (i.e., false-negatives defined in \autoref{sec:single_round_pbs}. The distinct elements that are not successfully reconciled in this round, if needed, can be reconciled in later rounds as we will describe in \autoref{sec:multi-rounds}. In this section, we only discuss how to identify the {\it incorrect} distinct elements in the second scenario. Let us use an example to elaborate the second scenario: Assume $(A_i, B_i)$ contains $3$ distinct elements $a_1, a_2, a_3$, then Bob computes $\tilde{s}=a_1\oplus a_2\oplus a_3$ using \autoref{alg:trivial_case} and mistakes it as the distinct element in $(A_i, B_i)$. 

\begin{comment}
============================================

We add a no-communication-cost verification step to check whether a reconciled element is an actual distinct element or not. Note that an actual distinct element of $(A_i, B_i)$ must be in sub-universe $\mathcal{U}_i$. On the other hand, an incorrectly reconciled element (e.g., $\tilde{s}$) can be in any sub-universe with probability $1/n$. So at the end \autoref{subsec:protocol0}, we check whether the reconciled element is in $\mathcal{U}_i$ by the hash function $h$ in hash-partition:

This verfication cannot completely eliminate false-positives, since an incorrectly reconciled element (e.g., $\tilde{s}$) can coincidentally end up in $\mathcal{U}_i$ with probability $1/n$. The chance of false-positives is extremely small using the verification. For instance, if $d=5$ and $n=255$, the probability of the second scenario is only $7.6\times 10^{-6}$. The probability of false-positives using the verfication is $1/n$ times this small probability, which is roughly $3\times 10^{-8}$. {\bf Note that a small probability of false-positives only costs a little waste on set reconciliation when synchronizing objectives (e.g., files), which is acceptable for most applications.}

Even worse, in the second scenario, the false-positives defined in \autoref{sec:single_round_pbs} could happen. For example, if subset pair $(A_i, B_i)$ contains $3$ distinct elements $s_1, s_2, s_3$, then \autoref{alg:trivial_case} computes $\tilde{s}=s_1\oplus s_2\oplus s_3$ and Bob mistakes $\tilde{s}$ as an actual distinct element. The good thing is, the probability of this kind of false-positives is extremely small for small $d$. For instance, if $d=5$ and $n=255$, the probability of the false-positives is only $7.6\times 10^{-6}$. To further reduce the chance of false-positives, we add a no-communication-cost verification step at the end of \autoref{subsec:protocol0} to check whether $\tilde{s}$ is an actual distinct element or not. The verification step works as follows: Given the output $s$ of subset pair $(A_i,B_i)$, if $s\in\mathcal{U}_i$ (i.e., $h(s)=i$), we consider $s$ as an actual distinct element; Otherwise, we consider $s$ as an incorrect output and discard it. 

Note that if $\tilde{s}\in A_i\Delta B_i$, $\tilde{s}$ must be in sub-universe $\mathcal{U}_i$. However, if $\tilde{s}$ is the bitwise \code{XOR} of the distinct elements in $(A_i,B_i)$ (i.e., the second scenario happens), it ends up in $\mathcal{U}_i$ with probablity of only $1/n$. 
%In fact, if we assume the hash-partition described in \autoref{sec:hash_partition} hashes the elements of $\mathcal{U}$ uniformly, independently, and randomly into $n$ sub-universes, the output $s$ in the second scenario will be in a different sub-universe $\mathcal{U}_j (j\neq i)$ with a high probability of $1-\frac{1}{n}$. Hence, this verfication method can further reduce the probability of false-positives by a factor of $\frac{1}{n}$. 
Use the same example (i.e., $d=5$, $n=255$), the probability of this kind of false-positives is reduced from $7.6\times 10^{-6}$ to $3\times 10^{-8}$ by this verification method. 
%{\bf This probability can be further reduced in \autoref{subsec:protocol2}, where PBS does two tiers of hash-partitions. So we can do verification on both of the two hash functions.}

%In some super critical cases (i.e., no false-positive is allowed), we can use a more powerful verification method to completely eliminate false-positives. That is, to check if the output $s$ exists in exactly one of the two sets (i.e., $s\in A\!\setminus\! B$ or $s\in B\!\setminus\! A$). To do so, Bob transmits $s$ along with an identification bit $\mathbbm{1}_{\{s\in B\}}$ to Alice, then Alice checks if $s\in (A\!\setminus\! B)\bigcup (B\!\setminus\! A)$ . This method verification costs additional $d(\log u+1)$ bits of communication overhead. In most applications, this rigorous $0\%$ probability guarantee of false-positives is unnecessary and the probability of the former verification method is small enough, so we use the former in the evaluation. Based on our observation, this kind of false-positives do not happen even once in the evaluation using the former verfication method. In the rest of this paper, we assume Scenario 2 is always correctly verified. 

============================================
\end{comment}

\subsection{Running PBS for Multiple Rounds}\label{sec:multi-rounds}

{\bf (merged from the following two paragraphs)} To deal with the ``remaining'' distinct elements, we remove (and save) all the distinct elements that has been reconciled in the first round (i.e., $\hat{D}$) and run another round of PBS. In the second round, we reconcile $A\Delta \hat{D}$ and $B$ instead of reconciling $A$ and $B$ to remove all the reconciled distinct elements. We use a different hash function for hash-partition in the second round to avoid the same exceptions (i.e., type (\RN{1}), (\RN{2}) events) that happened in the first round happen again. This procedure replicates until If until all distinct elements are successfully reconciled and the checksum is verified to be correct. 

% When the ideal case does not happen (i.e., type (\RN{1}) or type (\RN{2}) event happens), PBS will know the set reconciliation has not been completed via the $32$-bit checksum (\autoref{step:terminate_condition} in \autoref{alg:single_round_pbs}). To reconcile those distinct elements that have not been reconciled yet in the first round, we rule out all successfully reconciled elements and run another round of PBS. This procedure replicates until all distinct elements are successfully reconciled and the checksum is verified to be correct.

% More specifically, in the second round, we run PBS to reconcile $A$ and $B\Delta \hat{D}$ instead of $A$ and $B$ to rule out all elements that have been reconciled, where $\hat{D}$ is the set of reconciled distinct elements in the first round. We use a different hash function for hash-partition in the second round to avoid the same exceptions (i.e., type (\RN{1}), (\RN{2}) events) that happened in the first round happen again. The later rounds are similarly operated. 

%{\bf Normally, we want PBS to successfully reconcile all distinct elements in only a few rounds (say $3$) with high probability (say $99\%$). Hence, when tuning parameters (to be discussed in \autoref{sec:parameter_settings}), we set a {\it target success probability} $p_0$ of $r$ rounds as a paramenter setting requirement, which aims to ensure the probability that all distinct elements are reconciled in $r$ rounds to be larger than $p_0$. This requirement should also ensure the majority of the distinct elements are reconciled in the first round. Use the same example ($d=5, n=255$), on average $4.81$ out of $5$ distinct elements should be reconciled in the first round. So the total communication overhead in all rounds is only slightly larger than ($1.01$ to $1.07$ times of, as we will show in \autoref{fig:per-round-con}) that in the first round. Due to this reason, we use the communication overhead in the first round (described in \autoref{sec:communication_overhead_single_PBS}) to approximate the total communication overhead of all rounds in parameter settings (to be elaborated in \autoref{sec:parameter_settings}.}

% Although PBS may need to run many rounds to reconcile all distinct elements, the communication overhead mostly happens in the first round, since the majority of the distinct elements should be reconciled in the first round. Use the same example ($d=5, n=255$), on average $4.81$ out of $5$ distinct elements should be reconciled in the first round. So the total communication overhead in all rounds is only slightly larger than ($1.01$ to $1.07$ times of, to be shown in \autoref{fig:per-round-con}) that in the first round. Due to this reason, we use the communication overhead in the first round (described in \autoref{sec:communication_overhead_single_PBS}) to approximate the total communication overhead (all rounds) in parameter settings (to be elaborated in \autoref{sec:parameter_settings}).

%For the moment, we assume no ``fake'' distinct element in type (\RN{2}) subset pairs fails to be detected, which happens with overwhelming probability as explained in \autoref{subsec:exception_hash_partition}. Then 
%PBS reconciles the distinct elements gradually round by round. This is the ``piecewise decodability'' mentioned in \autoref{sec:intro_oursolution}. We use the following example to describe it in details: 
%Given two sets with $10$ distinct elements, in the first round, PBS tries to reconcile the $10$ distinct elements and say $6$ out of the $10$ distinct elements are successfully reconciled. Then the $6$ reconciled distinct elements are removed and PBS tries to reconcile the remaining $4$ distinct elements in the second round. Say $2$ out of the $4$ remaining distinct elements are successfully reconciled, and that leaves $2$ remaining distinct elements to be reconciled in the third round, so on so force. 
% Given two sets $A$, $B$ with $10$ distinct elements, in the first round, PBS hashes them into $7$ distinct subset pairs. $6$ distinct elements are hashed into $6$ distinct subset pairs, and the other $4$ distinct elements are hashed into the same subset pair. Then the former $6$ distinct elements are successfully reconciled in the first round and the later $4$ distinct elements remain to be reconciled in the second round, which are hashed into $3$ distinct subset pairs (under a different hash function). $2$ remaining distinct elements are hashed into $2$ distinct subset pairs, and the other $2$ remaining distinct elements are hashed into the same subset pair. Then the former $2$ remaining distinct elements are successfully reconciled in the second round and the later $2$ remaining distinct elements remain to be reconciled in the third round, so on so force. 
%The dynamics of the number of remaining distinct elements (i.e., $10\leadsto 4\leadsto 2\leadsto \cdots$ in the example) is in nature a Markov chain, which will be elaborated and analyzed in \autoref{sec:single_markov} to derive a tight tail bound of the probability that all distinct elements are reconciled in $r$ rounds.

% Even if the ideal case does not happen, most of the distinct elements should be distributed into different subset pairs, one distinct element in each, and therefore can be successfully reconciled. So in the first round, even if PBS cannot reconcile all distinct elements, it can reconcile the majority of them.
% % (piecewise decodability mentioned in \autoref{sec:intro_oursolution})
% Based on this intuition, we generalize PBS to multi-round, so that the distinct elements that are not reconciled yet in the first round can be reconciled in later rounds.  

% Without loss of generality, we only describe the second round of multi-round PBS, the reconciliation in the later rounds are similar. Let $\hat{D}_1$ denote the set of reconciled elements in the first round. If set reconciliation is not complete in the first round (i.e., the checksum infers $A\neq B\Delta \hat{D}_1$), then multi-round PBS saves $\hat{D}_1$, which includes correctly and incorrectly reconciled elements as described in \autoref{subsec:exception_hash_partition}, and starts the second round to find (1) the remaining distinct elements; (2) the incorrectly reconciled distinct elements in the first round. In the second round, multi-round PBS reconciles $A$ and $B\Delta \hat{D}_1$ instead of $A$ and $B$ (i.e., $B\leftarrow B\Delta\hat{D}_1$) to rule out all elements that have been reconciled. {\bf It uses a hash function that is different from the one used in the first round for hash-partition, otherwise every remaining distinct element will be hashed into the same subset pair and cause the same exception (described in \autoref{subsec:exception_hash_partition}) that happened in the first round.}

% If set reconciliation is complete in the second round, the set of reconciled elements in the second round (denoted as $\hat{D}_2$) should be the union of (1) all distinct elements that have not been reconciled in the first round (i.e., $(A\Delta B)\!\setminus\!\hat{D}_1$); and (2) all incorrectly reconciled elements in the first round (i.e., $\hat{D}_1\!\setminus\!(A\Delta B)$), which is by definition the set difference between $A\Delta B$ and $\hat{D}_1$. Therefore, the overall set difference $A\Delta B$ equals to the set difference between $\hat{D}_1$ and $\hat{D}_2$; Else, multiround PBS saves $\hat{D}_2$ and starts the third round, so on so force. 

% {\bf May need this algorithm to show the dynamics, if so, the earlier algorithm needs to change accordingly.}
% \IncMargin{1em}
% \begin{algorithm}
% \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
% \Input{$A$ and $B$}
% \Input{Maximum number of rounds $r$}
% \Output{$D$}

% $\hat{D},\mbox{ complete} \leftarrow PBS(A,B)$\;

% $D \leftarrow \hat{D}$\;

% \While{!complete and $r>0$}{
	
% 	$B \leftarrow B\Delta\hat{D}$\;

% 	$\hat{D},\mbox{ complete} \leftarrow PBS(A,B)$\;

% 	$D \leftarrow D\Delta\hat{D}$\;

% 	$r \leftarrow r-1$\;
% }

% \caption{Multi-round PBS} \label{proto:multirounds}
% \end{algorithm}\DecMargin{1em}

% The idea of multi-round PBS is quite simple: In each round, we discard the reconciled distinct elements in the previous rounds and aim to find the rest distinct elements from the remaining elements. More specifically, the first round of multi-round PBS is just the same as single-round PBS in \autoref{alg:single_round_pbs}. The second round has the same procedures as the first round. One difference is, we update $B$ by $B\leftarrow B\Delta\mathcal{D}$ in the second round, so that (1) Reconciled distinct elements in $\mathcal{D}$ that were contained in $A\Delta B$ are not longer contained in $A\Delta (B\Delta\mathcal{D})$; and (2) The other distinct elements remain in $A\Delta (B\Delta\mathcal{D})$ and can be reconciled later. The other difference is, we use a different hash function for partition (\autoref{step:hash_partition}) in the second round. Later rounds update $B$ in the same way and also use different hash functions. Multi-round terminates if the check in \autoref{step:termination} is correct. The overall set difference $A\Delta B$ is simply the union of reconciled distinct elements in all rounds. 

% A straightforward approach to discard reconciled distinct elements is to remove them from both $A$ and $B$. This approach however incurs additional communication overhead to update $A$, since only Bob learns the partial set difference in \autoref{step:reconcile}. Therefore, we use the approach in \autoref{step:updateb} that only updates $B$. It has another benefit in \autoref{step:termination}, which only needs to transmit the CRC of $A$ from Alice to Bob in the first round. In the later rounds, \autoref{step:termination} can be checked locally by Bob and does not require any additional communication overhead;

% Note that the communication overhead in the first round accounts for a large percentage of the total communication overhead in multi-round PBS, since most of the distinct elements (over $95\%$ as we will show in {\bf point to the figure}) should be reconciled in the first round. Therefore, we use the same parameter $n$ in later rounds because otherwise we have to compute a new parameter that can only save tiny communication overhead, even though the number of remaining distinct elements is small and can be reconciled using smaller $n$ with high probability. {\bf Due to the same reason, we can the same expression of the communication overhead in single-round PBS to approximate the communication overhead in multi-round PBS.}

% The natural termination condition of multi-round PBS is that all distinct elements are reconciled, which could require a large number of rounds and incur large additional communication overhead (each additional round incurs $d\log n$ bits of additional communication overhead on transmitting BCH codeword). To control the amount of additional communication overhead, we set another termination condition that multi-round PBS runs for at most $r$ rounds (typically $2$ or $3$). This termination condition could cause an `early' termination when some distinct elements have not been reconciled. However, under proper parameter settings (to be discussed in \autoref{sec:parameter_settings}), we can prove that the probability of an `early' termination (i.e., set reconciliation is incomplete in $r$ round) is very small
% %, and even if an `early' termination happens, an overwhelming percentage of distinct elements should have been reconciled, which is sufficient for most applications
% . For example, when $d=5, n=255, r=2$, an `early' termination happens with probability $4.8\times 10^{-4}$ (how to compute this probability will be elaborated in \autoref{sec:tail_bound}).

% For the moment, we assume no incorrectly reconciled distinct elements appears in multi-round PBS, which happens with overwhelming probability as explained in \autoref{subsec:exception_hash_partition}. Then multi-round PBS reconciles the distinct elements gradually round by round. This is the ``piecewise decodability'' mentioned in \autoref{sec:intro_oursolution}. We use the following example to describe it in details: Given two sets $A$, $B$ with $10$ distinct elements (i.e., $d=10$), in the first round, multi-round PBS hashes them into $7$ distinct subset pairs. $6$ distinct elements are hashed into $6$ distinct subset pairs, and the other $4$ distinct elements are hashed into the same subset pair. Then the former $6$ distinct elements are successfully reconciled in the first round and the later $4$ distinct elements remain to be reconciled in the second round, which are hashed into $3$ distinct subset pairs (under a different hash function). $2$ remaining distinct elements are hashed into $2$ distinct subset pairs, and the other $2$ remaining distinct elements are hashed into the same subset pair. Then the former $2$ remaining distinct elements are successfully reconciled in the second round and the later $2$ remaining distinct elements remain to be reconciled in the third round, so on so force. The dynamics of the number of remaining distinct elements (i.e., $10\leadsto 4\leadsto 2\leadsto \cdots$ in the example) is in nature a Markov chain, which will be elaborated and analyzed in \autoref{sec:tail_bound_per_group} to derive a tail bound of success probability (i.e., all distinct elements are reconciled in $r$ rounds) for paramenter settings. 

% In most applications, a high percentage of reconciliation (e.g., $>99\%$ distinct elements are reconciled) is good enough. Therefore, we add another termination condition on the maximum number of rounds (denoted as $r$). The larger $r$ is, the higher percentage of distinct elements will be reconciled. How to set parameters based on $r$ will be elaborated in \autoref{sec:parameter_settings};

% Readers may think the communication overhead of multi-round PBS is proportional to the number of rounds. In fact, the majority of the communication overhead is spent in the first round, since most of the distinct elements (over $95\%$ as we will show in {\bf point to the figure}) are reconciled in the first round. Each additional round only incurs a small amount of additional communication overhead. For example, when $d=10, n=255, |\mathcal{U}|=2^{32}$, assume $8$ distinct elements are reconciled in the first round and the rest $2$ distinct elements are reconciled in the second round. Then the communication overhead in the first round is $432$ bits. That number of the second round is only $160$


%the communication overhead of single-round PBS of $272$ ($2d\log n+d\log |\mathcal{U}|+32$) bits, and each additional round incurs $40$ ($d\log n$) bits of additional communication overhead. 

%among the three components of the communication overhead mentioned in \autoref{sec:communication_overhead_single_PBS}, only the first component (i.e., the BCH codeword) is proportional to the number of rounds. The other two components does not depend on the number of rounds.

% The second component only depends on the total number reconciled elements, which is roughly equal to $d$. The third component, the checksum of $A$, only needs to be sent once in the first round.
%Therefore, the communication overhead of multi-round PBS is only slightly larger than that of single-round PBS when the number of rounds is small (say $3$). For example, when $d=5, n=255, |\mathcal{U}|=2^{32}$, the communication overhead of multi-round PBS of $3$ rounds is $352$ bits, which is roughly $1.3$ times of the communication overhead of single-round PBS ($272$ bits).

% Therefore, each additional round of multi-round PBS only incurs a small amount of additional communication overhead. For example, when $d=5, n=255, |\mathcal{U}|=2^{32}$, the communication overhead of single-round PBS of $272$ ($2d\log n+d\log |\mathcal{U}|+32$) bits, and each additional round incurs $40$ ($d\log n$) bits of additional communication overhead. 

% As we explained in \autoref{sec:reconcile_by_trivial}, the communication overhead in each round is proportional to the number of (remaining) distinct elements, which decreases exponentially as the number of round increase (i.e., the first round reconciles $90\%$ of distinct elements, the second round reconciles $90\%$ of the remaining $10\%$ distinct elements, etc.). So the majority of the communication overhead (i.e., $\approx 90\%$) is in the first round. Therefore, we do not bother to optimize parameters (i.e., smaller $n$) in later rounds to save tiny communication overhead, even though remaining distinct elements become fewer and can be reconciled using smaller $n$;

% The termination condition of multi-round PBS is that all distinct elements are reconciled, which may require many rounds. In most applications, a high percentage of reconciliation (e.g., $>99\%$ distinct elements are reconciled) is good enough. Therefore, we add another termination condition on the maximum number of rounds (denoted as $r$). The larger $r$ is, the higher percentage of distinct elements will be reconciled. How to set parameters based on $r$ will be elaborated in \autoref{sec:parameter_settings};

% Multi-round means multiple round-trip delays. {\bf Thanks for the piecewise decodability of PBS, in almost all practical application scenarios, this tradeoff does not lead to longer response time because the reconciliation of objects identified by the successfully decodable codewords, which constitute the vast majority of all codewords, can run in parallel with the transmissions and decodings of the rest.  In other words, the piecewise decodability effective masks the slightly larger number of communication rounds as far as the response time is concerned.}

\begin{comment}
==============================

The pseudocode of set reconciliation operations in each round is shown as follows:

\IncMargin{1em}
\begin{algorithm}
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
\Input{$A$ and $B^{(in)}$}
\Input{Set of reconciled distinct elements $D^{(in)}$}
\Output{$B^{(out)}$}
\Output{Set of reconciled distinct elements $D^{(out)}$}

% Hash-partition $A^{(in)}$, $B^{(in)}$ into $\{A^{(in)}_i\}_{i=1}^n$, $\{B^{(in)}_i\}_{i=1}^n$ (\autoref{sec:hash_partition})\label{step:hash_partition}\;

% Encode $\{A^{(in)}_i\}_{i=1}^n$, $\{B^{(in)}_i\}_{i=1}^n$ into parity bitmaps (\autoref{sec:parity_bitmap_encoding})\;


% Find those subset pairs (denoted them as $(A^{(in)}_{i_1}, B^{(in)}_{i_1}), ...,(A^{(in)}_{i_k}, B^{(in)}_{i_k})$) that parity bits differ (\autoref{sec:BCH_code})\;

Run single-round PBS on $A$ and $B^{(in)}$ to obtain the (partial) set difference $\mathcal{D}$\label{step:reconcile} \;

$D^{(out)} \leftarrow D^{(in)}\bigcup \mathcal{D}$\label{step:updated}\;

$B^{(out)} \leftarrow B^{(in)}\Delta\mathcal{D}$\label{step:updateb}\;

Check whether the set reconciliation is complete by comparing $A$ to $B^{(out)}$ (via CRC)\label{step:termination}\;

\caption{Set reconciliation operations of PBS in each round} \label{proto:multirounds}
\end{algorithm}\DecMargin{1em}

In \autoref{proto:multirounds}, the output $B^{(out)}$ in the $r^{th}$ round is the input $B^{(in)}$ in the $(r+1)^{th}$ round. $D^{(in)}$ and $D^{(out)}$ have the same relationship, and they denote the set of reconciled distinct elements before and after a round. $B^{(in)}$ and $D^{(in)}$ are initialized as $B$ and $\emptyset$ respectively. We omit the currect number of round $r$ in \autoref{proto:multirounds}, since the operations in different rounds are exactly the same. Due to the same reason, we only elaborate the operations in the first round: First, Alice and Bob reconcile $A$ and $B^{(in)}$ $(=B)$ using single-round PBS and Bob obtains the (partial) set difference $\mathcal{D}$ (\autoref{step:reconcile}); Second, Bob updates the set of reconciled distinct elements by merging it with $\mathcal{D}$ (\autoref{step:updated}); Third, Bob updates $B^{(in)}$ $(=B)$ to $B^{(out)}$ as \autoref{step:updateb} shows, such that (1) The reconciled distinct elements in $\mathcal{D}$ that are contained in $A\Delta B^{(in)}$ are not longer contained in $A\Delta B^{(out)}$; and (2) The distinct elements that are not successfully reconciled remain in $A\Delta B^{(out)}$ and can be reconciled in later rounds; Finally, we check whether all distinct elements are reconciled. Note that if it is true, $B^{(out)}$ should be the same as $A$ and multi-round PBS should terminate. We use a $32$-bit CRC (Cyclic Reduncancy Check) to check if $B^{(out)}=A$ in our evaluation. {\bf To achieve higher confidence, we can certainly use longer CRC (e.g., 64-bit). }

{\bf Remarks:}

(1) In each round, hash-partition in \autoref{sec:hash_partition} uses different hash functions, so that the remaining distinct elements from the last round will be hashed into different subset pairs with high probability;

(2) A straightforward approach to discard reconciled distinct elements is to remove them from both $A$ and $B$. This approach however incurs additional communication overhead to update $A$, since only Bob learns the partial set difference in \autoref{step:reconcile}. Therefore, we use the approach in \autoref{step:updateb} that only updates $B$. It has another benefit in \autoref{step:termination}, which only needs to transmit the CRC of $A$ from Alice to Bob in the first round. In the later rounds, \autoref{step:termination} can be checked locally by Bob and does not require any additional communication overhead;

(3) As we explained in \autoref{sec:reconcile_by_trivial}, the communication overhead in each round is proportional to the number of remaining distinct elements, which decreases exponentially as the number of round increase (i.e., the first round reconciles $90\%$ of distinct elements, the second round reconciles $90\%$ of the remaining $10\%$ distinct elements, etc.). So the majority of the communication overhead (i.e., $\approx 90\%$) is in the first round. Therefore, we do not bother to optimize parameters (i.e., smaller $n$) in later rounds to save tiny communication overhead, even though remaining distinct elements become fewer and can be reconciled using smaller $n$;

(4) One termination condition of Multi-round PBS is $B^{(out)}=A$, which refers that all distinct elements are reconciled. In most applications, a high percentage of reconciliation (e.g., $>99\%$ distinct elements are reconciled) is good enough. Therefore, we add another termination condition of the maximum number of rounds (denoted as $r$). The larger $r$ is, the higher percentage distinct elements will be reconciled, and the smaller $n$ is required. How to set parameters (e.g., $n$) based on $r$ will be elaborated in \autoref{sec:parameter_settings};

(5) Multi-round means multiple round-trip delays. {\bf Thanks for the piecewise decodability of PBS, in almost all practical application scenarios, this tradeoff does not lead to longer response time because the reconciliation of objects identified by the successfully decodable codewords, which constitute the vast majority of all codewords, can run in parallel with the transmissions and decodings of the rest.  In other words, the piecewise decodability effective masks the slightly larger number of communication rounds as far as the response time is concerned.}

==============================

\end{comment}

% (3) Readers may wonder in the later rounds, most distinct elements should be reconciled, and the rest distinct elements could be reconciled using degraded parameters (i.e., smaller $n$ and $t$). In fact, degrade parameters in later rounds cannot save much communication overhead, since the majority of it is spent in the first round (i.e., $>90\%$). Therefore, we use the same parameters (i.e., $n,t$) among all rounds in multi-rounds PBS;

% (4) The number of remaining distinct elements decreases exponentially as the number of round increase (i.e., the first round reconciles $90\%$ of distinct elements, the second round reconciles $90\%$ of the remaining $10\%$ distinct elements, etc.). 
% (4) The termination condition of Multi-rounds PBS is $B^{(out)}=A$ to reconcile all distinct elements. In some applications,  


% The output $B^{(out)}$ in the $r^{th}$ round is the input $B^{(in)}$ in the $(r+1)^{th}$ round. $D^{(in)}$ and $D^{(out)}$ are similarly defined. $B^{(in)}$ and $D^{(in)}$ are initialized as $B$ and $\emptyset$ respectively. Since and $D$ are updated in each round, so we use $B^{(in)}$ to denote the input and $B^{(out)}$ to denote the output respectively.  Specifically, in the first round, we initialize $B^{(in)}$ and $D^{(in)}$ as $B$ and $\emptyset$ respectively. we first use the single-round scheme 

% Then we run our (single-round) scheme on the updated two sets (i.e., after removing reconciled distinct elements) using a different (independent) hash-partition function from previous rounds, so that the rest distinct elements are hashed into different subset pairs (i.e., the ideal case) with high probability. At the end of each round, we check whether the set reconciliation is complete (i.e., all distinct elements are found) by computing the bitwise \code{XOR} of the remaining elements in $A$ and $B$ 
 

% This {\bf multi-rounds} scheme can significantly increase the success probability (i.e., the probability that all distinct elements are reconciled). Readers may wonder in the later rounds, most distinct elements should be reconciled, and the rest distinct elements could be reconciled using degraded parameters (i.e., smaller $n$ and $t$). In fact, degrade parameters in later rounds cannot save much communication overhead, since the majority of it is spent in the first round (i.e., $>90\%$). Therefore, we use the same parameters (i.e., $n,t$) among all rounds in our evaluation. 
% %The tradeoff between the number of rounds and the communication overhead per rounds will be elaborated in \autoref{sec:tail_bound}. In our evaluation, $r=2,3$ rounds are enough to achieve an extremely high success probability. 

% Readers may think the cost (i.e., communication overhead and the computational complexity) of this multi-rounds scheme is proportional to the number of rounds (denoted as $r$) and increases linearly with $r$. In fact, the cost of each round is roughly proportional to the number of remaining distinct elements, which decreases exponentially as $r$ increases (i.e., the first round reconciles $99\%$ of distinct elements, the second round reconciles $99\%$ of the remaining $1\%$ distinct elements, etc.). So the cost of this multi-rounds scheme is only slightly larger than that of the single-round scheme. Furthermore, as we explained in \autoref{sec:intro}, {\bf from intro thanks for the piecewise decodability of our solution, in almost all practical application scenarios, this tradeoff does not lead to longer response time because the reconciliation of objects identified by the successfully decodable codewords, which constitute the vast majority of all codewords, can run in parallel with the transmissions and decodings of the rest.  In other words, the piecewise decodability effective masks the slightly larger number of communication rounds as far as the response time is concerned.} 

\begin{comment}

\subsection{Baseline Scheme}\label{subsec:protocol1} 

Note that the set difference $A\Delta B$ can contain more than 1 elements (i.e., $d>1$), and \autoref{alg:trivial_case} cannot reconcile $A$ and $B$ directly in this case. Therefore, we propose a baseline scheme building upon~\autoref{alg:trivial_case} that also works when $d>1$: First, we partition the element universe $\mathcal{U}$ into $n$ sub-universes $\mathcal{U}_1, \mathcal{U}_2, \cdots, \mathcal{U}_n$. Denote $A_i \triangleq A\bigcap \mathcal{U}_i$ and $B_i \triangleq B\bigcap \mathcal{U}_i$ for $i=1,2,\cdots,n$. Then $\{A_i\}_{i=1}^n$ and $\{B_i\}_{i=1}^n$ are partitions of $A$ and $B$ respectively. Furthermore, $\Phi\triangleq\{A_i\Delta B_i\}_{i=1}^n$ is a partition of $A\Delta B$. 

Assume the {\bf ideal case} happens, in which each subset pair $(A_i, B_i)$ contains at most one distinct element ({\it i.e.,} $|A_i\Delta B_i|\!\leq\!1$), we use \autoref{alg:trivial_case} to reconcile each subset pair and obtain $A_i\Delta B_i$ for $i=1,2,\cdots,n$. The overall set difference $A\Delta B$ is simply their union $\bigcup_{i=1}^n \big{(}A_i\Delta B_i\big{)}$. 

In the first step of the baseline scheme, we can use a hash function $h(\cdot): \mathcal{U}\rightarrow \{1,2,\cdots,n\}$ to partition the universe $\mathcal{U}$ into $n$ sub-universes: $\mathcal{U}_i=\{s\mid s\in \mathcal{U} \mbox{ and } h(s)=i\}$ for $\forall i=1,2,\cdots,n$. And the hash function $h(\cdot)$ can be predetermined between Alice and Bob and does not require additional communication cost.

This hash-partition can be modeled as a {\it balls-into-bins problem}, in which the distinct elements are viewed as balls and the subset pairs are viewed as bins. The hash-parition basically throws (hashes) $d$ balls (distinct elements) uniformly and randomly into $n$ bins (subset pairs). The aforementioned ideal case in this context becomes, after throwing $d$ balls uniformly and randomly into $n$ bins, each bin receives at most 1 ball (i.e., $d$ nonempty bins have 1 ball in each and the rest $n-d$ bins are empty). {\bf It may remind readers about the Birthday problem. And the ideal case can be analogous to the case that no people share the same birthday.} The ideal case happens with a probability of $p=\frac{n\,!}{(n-d)\,!n^d}\!=\!\prod_{k=1}^{d - 1}(1 - \frac{k}{n})\!\approx\! e^{-\frac{d(d-1)}{2n}}$ when $d\!\ll\!n$. In other words, $n$ must be $\Omega(d^2)$ to ensure the ideal case happens with a nontrivial probability.  Note that the communication overhead of the baseline scheme is proportional to $n$, as each subset pair requires communication of a bitwise \code{XOR} in \autoref{alg:trivial_case}. So this communication overhead increases at least quadratically as $d$ increases. 

In fact, this communication overhead can be significantly reduced: In the ideal case, $n-d$ out of $n$ subset pairs are identical ones, and only $d (\ll n)$ out of $n$ subset pairs contain distinct elements (one distinct element in each of the $d$ subset pairs) and need to be reconciled. If we can identify these $d$ subset pairs (with a tiny additional communication overhead) and only reconcile them, the overall communication overhead will be significantly reduced from $\Omega(d^2)$ to $O(d)$. Based on this intuition, we propose our scheme in \autoref{sucsec:our-scheme}, which uses Parity Bitmap Sketch (PBS) and Error Correction Coding (ECC) to identify those subset pairs with a tiny additional communication overhead. 

Note that the ideal case does not always happen. However, we can ensure that the ideal case happens with high probability by properly selecting $n$ based on $d$ (i.e., $n=\Omega(d^2)$). Furthermore, as we will describe in \autoref{subsec:nonideal}, even if the ideal case does not happen (i.e., some distinct elements are hashed into the same subset pair), most of the distinct elements should be distributed into different subset pairs and therefore can be reconciled. So the baseline scheme, even cannot reconcile all of the distinct elements, can still reconcile the majority of them. Based on this property, we will extend our scheme from single-round to multi-rounds in \autoref{subsec:nonideal} to further increase the probability of reconciling all distinct elements. 

For general cases ({\it i.e.,} $t=|A\Delta B|$ is an arbitrary number), we have a straightforward strawman scheme building upon~\autoref{alg:trivial_case}, which works as follows: First, Alice and Bob choose some hash function $h(s): \mathcal{U} \rightarrow \{0,1,\cdots,2^{32}-1\}$ to partition $A$ and $B$ into $m$ subsets $A_1,A_2,\cdots,A_m$ and $B_1,B_2,\cdots,B_m$ respectively:

\begin{align}
s\in A_i & \mbox{ iff } s\in A \mbox{ and } h(s)=i\!\mod m, \nonu{}mber\\
s\in B_i & \mbox{ iff } s\in B \mbox{ and } h(s)=i\!\mod m. \nonumber
\end{align} 

{\bf call a subset pair -> partition?} Since Alice and Bob use the same hash function for partition, common elements (i.e., elements in $A\cap B$) are always hashed into the same subset pair $(A_i, B_i)$. And the set difference of each subset pair only contains distinct elements (i.e., elements in $A\Delta B$): $A_i\Delta B_i \subset A\Delta B$. In the ideal case, with a sufficient large $m$, each subset pair $(A_i, B_i)$ contains at most one distinct element ({\it i.e.,} $|A_i\Delta B_i|\!\leq\!1$). Then \autoref{alg:trivial_case} can reconcile each subset pair and obtain $A_i\Delta B_i$ for $i=1,2,\cdots,m$. The overall set difference $A\Delta B$ is simply their union $\bigcup_{i=1}^m \big{(}A_i\Delta B_i\big{)}$. The selection of hash function $h(s)$ can be predetermined between Alice and Bob and it does not require additional communication cost.

%To make sure Alice and Bob use the same hash function for partition, we let them pre-agree on some universal hash family (e.g., \code{xxHash}~\cite{Collet_xxHashExtremelyfast_}) and a common selection order, and each time they choose a hash function from the family in the same order. Note that we can also let Alice generates a hash function and send it to Bob. The hash function that Alice and Bob choose for partition can be either generated by 

This hash-partition is in nature a {\it balls-into-bins model}. We can view the distinct elements as balls and the subset pairs as bins. The hash-parition basically throws (hashes) $t$ balls (distinct elements) uniformly and randomly into $m$ bins (subset pairs). The aforementioned ideal case in this context is, with a sufficient large number of bins, each bin receives at most 1 ball. The strawman scheme works correctly if and only if the ideal case happens, which has a probability of $\frac{m\,!}{(m-t)\,!m^t}\!=\!\prod_{k=1}^{t - 1}(1 - \frac{k}{m})\!\approx\! e^{-\frac{t(t-1)}{2m}}$. In other words, to ensure the strawman scheme works correctly with a probability of $p$, it roughly requires $m \!=\!\lceil \frac{t(t-1)}{-2\ln p}\rceil$ subset pairs. 

Note that the communication overhead of this strawman scheme is proportional to the number of subset pairs $m$, as each subset pair requires communication of an \code{XOR} sum in \autoref{alg:trivial_case} during the reconciliation. When $t$ is small, a small communication cost can guarantee that the strawman scheme works correctly with high probability. For instance, when $t=5$, $m=95$ subset pairs are sufficient for the strawman scheme to work correctly with a probability of $90\%$. However, when $t$ is relatively large, it requires a huge communication cost to ensure the strawman scheme works correctly. For instance, when $t=1,000$, it requires $m=4,740,865$ subset pairs to guarantee a success probability of $90\%$. 

In fact, the majority of subset pairs are identical ones and do not need to reconcile. And only a small portion of them contain distinct elements. If we can identify those subset pairs that contain distinct elements and only reconcile them, the communication cost could be significantly reduced. Our scheme is based on this intuition and uses parity bitmap sketch and BCH code to identify the subset pairs, which we will elaborate in \autoref{sucsec:our-scheme}. 

%To distribute balls as uniformly as possible and maximize the probability of the ideal case, we choose a uniform hashing function $h$ that throws balls uniformly and randomly into bins: $$\mathbb{P}[h(s)=i]=\frac{1}{m} \mbox{ for } \forall i=1,2,\cdots,m, \forall s\in U$$.

%Note that the probability of the ideal case is $\frac{m\,!}{(m-t)\,!m^t}\!=\!\prod_{k=1}^{t - 1}(1 - \frac{k}{m})\!\approx\! e^{-\frac{t(t-1)}{2m}}$. Hence, at least $\lceil \frac{t(t-1)}{-2\ln p}\rceil$ bins are required to ensure that this probability is at least $p$. In other words, to ensure that the ideal case happens with a probability of $p$, the strawman scheme roughly requires $m \!=\!\lceil \frac{t(t-1)}{-2\ln p}\rceil$. For example, suppose $t\!=\!$\num{1000}, %and $p\!=\!0.01$, this strawman scheme roughly requires $m\!=\!$\num{720626} bins (partitions) to ensure that $|A_i\Delta B_i|\!\leq\!1$ (for any $i=1,2,\cdots,m$) holds with probability $50\%$.  

% A straightforward strawman scheme building upon~\autoref{alg:trivial_case} 
% to reconcile two sets $A$ and $B$ in general 
% ({\it i.e.,} $|A\Delta B|$ is an arbitrary number) is the following: 
% Uniformly randomly partition $A$ and $B$ into $m$ subsets ($A_1,A_2,\cdots,A_m$ 
% and $B_1,B_2,\cdots,B_m$) so that the set difference 
% $A_i\Delta B_i$ of each subset pair $(A_i, B_i)$ contains at most one element 
% ({\it i.e.,} $|A_i\Delta B_i|\!\leq\!1$) {\it w.h.p.} ({\it i.e.,} with high probability), 
% and then reconcile each subset pair with~\autoref{alg:trivial_case}. 

% Now let us analyze this strawman scheme using the {\it balls-into-bins model}. 
% Assume that sets $A$ and $B$ have $t$ elements in their set difference, {\it i.e.,} $|A\Delta B|\!=\!t$. 
% These $t$ elements can be viewed as $t$ balls and the $m$ partitions (subset pairs) can be viewed as 
% $m$ bins. The random partition process in this strawman scheme can be modeled as throwing 
% $t$ balls into $m$ bins in the following manner: Each ball goes into a 
% uniformly random bin and independently of other balls. %so that each bin contains at most one ball, {\it w.h.p.}  
% The probability that each bin contains at most one ball is  
% $\frac{m\,!}{(m-t)\,!m^t}\!=\!\prod_{k=1}^{t - 1}(1 - \frac{k}{m})\!\approx\! e^{-\frac{t(t-1)}{2m}}$. 
% Hence, at least $\lceil \frac{t(t-1)}{-2\ln p}\rceil$ bins are required 
% to ensure that this probability is at least $p$. In other words, to ensure 
% that each bin contains at most one ball with a probability of $p$, 
% the strawman scheme roughly requires $m \!=\!\lceil \frac{t(t-1)}{-2\ln p}\rceil$. 
% For example, suppose $t\!=\!$\num{1000}, %and $p\!=\!0.01$, 
% this scheme roughly requires $m\!=\!$\num{108469} bins (partitions) to 
% ensure that $|A_i\Delta B_i|\!\leq\!1$ (for any $i=1,2,\cdots,m$) holds with probability $0.01$.  

% We note that the communication overhead of this strawman scheme is proportional to 
% $m$ ($\!\gg\! t$), as each partition (subset pair) requires communication of an \code{XOR} sum during the reconciliation. 
% This communication overhead is much higher than that of the optimal scheme, which only requires 
% to exchange the elements in the set difference (assuming an oracle tells it which elements belong to 
% the set difference), {\it i.e.,} proportional to $t$. In the example above, assuming each element takes 4 bytes, 
% the communication overhead of the strawman scheme is $4m$ bytes ($\!\approx\! \num{423.71}\,$KB) to ensure 
% a success rate of only 0.01 ({\it i.e.,} with a probability of $0.0.1$, all elements in 
% the set difference are successfully reconciled), 
% which is approximately 2 orders of magnitude higher than $4t$ bytes ($\!=\!\num{3.90}\,$KB), the communication 
% overhead of the optimal scheme. 

\subsection{Our Scheme: The Preliminary Version}\label{sucsec:our-scheme}

Like the baseline scheme, our scheme also hash-partitions the two sets $A$ and $B$ into $n$ subset pairs. The difference is, instead of reconciling all subset pairs using \autoref{alg:trivial_case}, our scheme identifies the subset pairs that contains distinct elements and only reconciles them. Since the hash-partition and set reconciliation on each subset pair using \autoref{alg:trivial_case} have been described in \autoref{subsec:protocol1}, we only elaborate how to identify the subset pairs that contain distinct elements in this section. 

The general idea of identification is very simple: First, we {\bf encode} each subset into $1$ bit, such that in the ideal case, for $\forall i=1,2,\cdots,n$:

\begin{itemize}
	\item The codewords (bits) of $A_i$ and $B_i$ are different if and only if subset pair $(A_i, B_i)$ contains $1$ distinct element;
	\item The codewords (bits) of $A_i$ and $B_i$ are the same if and only if subset pair $(A_i, B_i)$ contains no distinct element;
\end{itemize}

Second, we {\bf compare} the codewords of each subset pair. And the subset pairs that contain distinct elements are the ones with different codewords (bits). We will describe the two steps in details in \autoref{sec:parity_bitmap_encoding} and \autoref{sec:BCH_code} respectively.

\subsubsection{Parity Bitmap Encoding}\label{sec:parity_bitmap_encoding}

In our scheme, we use {\it parity encoding} to encode each subset into a parity bit. More specific, it encodes a subset as ``1'' if it contains odd number of elements, and as ``0'' otherwise. And it satisfies the aforementioned requirements in the ideal case:

\begin{itemize}
	\item If subset pair $(A_i, B_i)$ contains $1$ distinct element, the corresponding two subsets $A_i$ and $B_i$ differ exactly one element, which implies that $||A_i|\!-\!|B_i||\!=\!1$. Hence, if $|A_i|$ ({\it i.e.,} number of elements in $A_i$) is odd (or even), then $|B_i|$ must be even (or odd). And the parity bits of $A_i$ and $B_i$ will be different;
	\item If subset pair $(A_i, B_i)$ contains no distinct element, the corresponding two subsets $A_i$ and $B_i$ should be the same and therefore contain the same number of elements. Hence, if $|A_i|$ is odd (or even), then $|B_i|$ must be odd (or even). And the parity bits of $A_i$ and $B_i$ will be the same;
\end{itemize}

Using parity encoding, the $n$ subsets of $A$ are encoded as a bit string $A[1..n]$ in $\{0,1\}^n$, 
where the $i$-th bit $A[i]$ in $A[1..n]$ corresponds to the parity encoding bit of $A_i$. Similarly, the $n$ subsets of $B$ are similarly 
encoded as a bit string $B[1..n]$. We call $A[1..n]$ ($B[1..n]$) the {\it parity bitmap} of $\{A_i\}_{i=1}^n$ ($\{B_i\}_{i=1}^n$). In the ideal case, $A[1..n]$ and $B[1..n]$ differ at $d$ different bit-positions, which corresponds to the $d$ subset pairs that contain distinct elements. And our scheme only reconciles those subset pairs that the parity bits are different. We will describe the nonideal case (i.e., some subset pair contains more than 1 distinct elements) in \autoref{subsec:nonideal}.

\subsubsection{Parity Bitmap Comparison Using BCH Code}\label{sec:BCH_code}

A straightforward approach to compare the parity bitmaps is to let Bob send the complete parity bitmap $B[1..n]$ to Alice, then Alice compares $A[1..n]$ with $B[1..n]$ locally. This approach has a communication overhead of $n$ bits, which is unnecessarily high. As we discussed in~\autoref{subsec:protocol0}, $d$ is usually much smaller than $n$. It means $A[1..n]$ and $B[1..n]$ differ only at a tiny portion of bits. Therefore, we can view $A[1..n]$ as a corrupted message of $B[1..n]$ with $d$ corrupted bits, and the bit-positions of the $d$ corrupted bits basically correspond to the $d$ subset pairs that contain distinct elements. The detection of corrupted bits, on the other hand, can be solved by Error-Correction Code (ECC)~\cite{Lin_ErrorControlCoding_1983}. And our scheme uses BCH code~\cite{Lint_IntroductionCodingTheory_1998} to encode the parity bitmap and detect the $d$ corrupted bits.

More specific, after the parity bitmap encoding, Bob uses a $d$-error-correcting systematic BCH code to encode $B[1..n]$ into an $n+d\log n$ codeword, in which the first $n$ bits are $B[1..n]$ (property of systematic BCH code). Then Bob sends the rest $d\log n$ bits, which we denote as {\it parity bitmap sketch (PBS)}, to Alice. Upon the received PBS and $A[1..n]$ (corrupted message), Alice uses the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} to detect the $d$ corrupted bits in $A[1..n]$. The communication overhead of this approach is $d\log n$ bits (i.e., length of PBS), which is much smaller than that of the straightforward approach ($n$ bits, when $d\!\ll\!n$). On the other hand, the computational complexity of the state-of-the-art BCH decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} is $O(d^2\log^2 n)$. 

\subsubsection{Exceptional Handling and Multi-rounds}\label{subsec:nonideal}

As we described in \autoref{subsec:protocol1}, the ideal case does not always happen, which means some subset pair may contain more than 1 distinct elements and cannot be successfully reconciled by \autoref{alg:trivial_case}. Due to the parity encoding, we can classify such subset pair into the following two scenarios:

\begin{itemize}
    \item Scenario 1: If a subset pair $(A_i, B_i)$ contains even number ($\geq 2$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be the same and our scheme will not reconcile the subset pair. Hence, the distinct elements in the subset pair will not be reconciled;
    \item Scenario 2: If a subset pair $(A_i, B_i)$ contains odd number ($\geq 3$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be different and our scheme will reconcile the subset pair using \autoref{alg:trivial_case}. However, as we described in \autoref{subsec:protocol0}, when a subset pair contains more than 1 distinct elements, \autoref{alg:trivial_case} will output the bitwise \code{XOR} of them as the `distinct element', which is not a real distinct element with high probability;
\end{itemize}

In both scenarios, the distinct elements in the subset pair cannot be reconciled. Even worse, in the second scenario, a false-positive could happen (i.e., the output of \autoref{subsec:protocol0} is not a real distinct element). However, as we will analyze in \autoref{sec:tail_bound} and show in {\bf the evaluation section}, the second scenario barely happens both theoretically and empirically. To further reduce the chance of false-positives, we add a verification step at the end of \autoref{subsec:protocol0} to check whether the output of \autoref{subsec:protocol0} $s$ is a real distinct element or not. The verification step works as follows: Given the output $s$ of subset pair $(A_i,B_i)$, if $s\in\mathcal{U}_i$ (i.e., $h(s)=i$), we consider $s$ as a real distinct element; Otherwise, we consider $s$ as an incorrect output and discard it. 

Note that if $s$ is a real distinct element of $(A_i,B_i)$, $s$ must be in sub-universe $\mathcal{U}_i$. However, if $s$ is the bitwise \code{XOR} of the distinct elements in $(A_i,B_i)$ (i.e., the second scenario happens), $s$ could be in any sub-universe other than $\mathcal{U}_i$. In fact, if we assume the hash-partition described in \autoref{subsec:protocol1} hashes the elements of $\mathcal{U}$ uniformly, independently, and randomly into $n$ sub-universes, the output $s$ in the second scenario will be in a different sub-universe $\mathcal{U}_j (j\neq i)$ with a high probability of $1-\frac{1}{n}$. Hence, this verfication step can reduce the chance of false-positives by a factor of $\frac{1}{n}$. 

Even if the ideal case does not happen, most of the distinct elements should be distributed into different subset pairs and therefore can be reconciled. So our scheme, even cannot reconcile all of the distinct elements, can still reconcile the majority of them (piecewise decodability). To reconcile the rest distinct elements, we can just run our scheme for another round under a different hash-partition function, so on so force. This {\bf multi-rounds} scheme can significantly increase the success probability (i.e., the probability that all distinct elements are reconciled). Readers may wonder in the later rounds, most distinct elements should be reconciled, and the remaining could be reconciled using degraded parameters (i.e., smaller $n$ and $t$). In fact, degrade parameters in later rounds cannot save much communication overhead, since the majority of it is spent in the first round (i.e., $>90\%$). Therefore, we use the same parameters (i.e., $n,t$) among all rounds in our evaluation.
%The tradeoff between the number of rounds and the communication overhead per rounds will be elaborated in \autoref{sec:tail_bound}. In our evaluation, $r=2,3$ rounds are enough to achieve an extremely high success probability. 

Readers may think the cost (i.e., communication overhead and the computational complexity) of this multi-rounds scheme is proportional to the number of rounds (denoted as $r$) and increases linearly with $r$. In fact, the cost of each round is roughly proportional to the number of remaining distinct elements, which decreases exponentially as $r$ increases (i.e., the first round reconciles $99\%$ of distinct elements, the second round reconciles $99\%$ of the remaining $1\%$ distinct elements, etc.). So the cost of this multi-rounds scheme is only slightly larger than that of the single-round scheme. Furthermore, as we explained in \autoref{sec:intro}, {\bf from intro thanks for the piecewise decodability of our solution, in almost all practical application scenarios, this tradeoff does not lead to longer response time because the reconciliation of objects identified by the successfully decodable codewords, which constitute the vast majority of all codewords, can run in parallel with the transmissions and decodings of the rest.  In other words, the piecewise decodability effective masks the slightly larger number of communication rounds as far as the response time is concerned.} 

\end{comment}

\section{PBS for large \texorpdfstring{\larger\boldmath\MakeLowercase{$d$}}{d}}\label{subsec:protocol2}

Note that the BCH decoding computational complexity is $O(d^2)$ of finite field operations (in GF($2^{8}$) when $n=255$) using the state-of-the-art decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019}, which is too expensive for large $d$. To overcome this drawback, we first hash-partition sets $A$ and $B$ each into $d/\delta$ subsets (which we call {\it groups} to distinguish from subsets), just like what we did in \autoref{sec:hash_partition}, for some small integer $\delta$ (say $5$), then reconcile each of the group pairs by the PBS we described in \autoref{sec:scheme}. After the partition, each group pair has $\delta$ distinct elements on average. So the BCH decoding computational complexity of each group pair is roughly $O(\delta^2)$, which can be considered as a constant, since $\delta$ is a small number. As a result, the overall computational complexity of PBS is reduced from $O(d^2)$ to $O(d)$. 

%To differentiate from the PBS described in \autoref{sec:scheme}, we refer to it as PBS-basic in this section. 
We continue to assume that the number of distinct elements $d$ is precisely known. Even so, due to the randomness of hash-partition, $\delta_i$, the number of distinct elements in the $i$-th group pair, is a Binomial random variable with mean of $\delta$ for $i=1,2,...,g$, which cannot be precisely known without a huge amount of additional communication overhead. Since $\delta_1, \delta_2, ..., \delta_g$ follows the identical Binomial distribution, there is no sense to set different parameters among the $g$ group pairs. Hence, we set two universal parameters, $t$ and $n$, for all group pairs, where $t$ is the error-correction capability of the BCH code used for reconciling each group pair, and $n$ is the number of subset pairs in each group pair.

%To deal with this randomness, we set two global parameters, denoted as $t$, that corresponds to the error-correction capability of the BCH code used for reconciling every group pair. identical no sense or additonal info

{\bf (modified based on the next paragraph from intro)} Setting $t$ properly is critical for PBS to perform well. On one hand, if $t$ is too large (say $t=10\delta$), then the communication overhead on transmitting BCH codeword for each group pair (i.e., $t\log n$) is unnecessarily large; but on the other hand, if $t$ is too small (say equal to $\delta$), then close to half of the group pairs fail to decode the BCH codeword due to the insufficient error-correction capability, which can result in hefty penalties on BCH decoding failures (to be described in \autoref{sec:BCH_exception}). In PBS, we manage to make $t$ as small as possible (so that the communication overhead on transmitting BCH codewords is kept to a minimum) yet pay negligible penalties of BCH decoding failures. 

% To ensure the error-correction capability $t$ is sufficient (i.e., $t\geq \delta_i$ for $i=1,2,...,g$) for every group pair with high probability, we set $t$ conservatively and leave a sufficient `safety margin' between $t$ and the average number of distinct elements in each group pair $\delta$. 

% Note that the `safety margin' between $t$ and $\delta$ incurs additional communication overhead on transmitting BCH codeword: In the perfect scenario (i.e., $\{d_i\}_{i=1}^g$ is precisely known), the average communication overhead on transmitting BCH codeword per group pair is $\delta\log n$; On the other hand, when we set $t$ to be the error-correction capability for each group pair, the average communication overhead becomes $t\log n$. If we set the `safety margin' to be too large (say $t=10\delta$), it will incur huge additional communication overhead. Due to this reason, we set a moderate `safety margin' that  $t$ in the range from $1.5\delta$ to $3\delta$. 

% {\bf moved from intro} The number of elements in the set difference between any group pair is in general not a constant.  Rather, it is a random variable that has roughly a Poisson distribution with mean $\delta$.  The potential issue arises from dealing with this randomness in setting a global parameter that corresponds to the error-correction capability of the BCH code used for reconciling every group pair.  This parameter, denoted as $t$ (consistent with other literatures on BCH code), is the maximum number of errors that the BCH code used by any group pair can correct, and the size of each such codeword is roughly $8t$ bits (assuming $n = 255$ as explained above). The issue is that, on one hand, if $t$ is too large (say several times larger than $\delta$), then the total size of the BCH codewords, which is the bulk of the extra communication cost, is unnecessarily large; but on the other hand, if $t$ is too small (say equal to $\delta$), then close to half of the BCH codewords cannot decode or worse decode incorrectly (unknown to Alice and Bob), which can result in hefty penalties in the latter case of incorrect decoding.   In PBS, we manage to make $t$ as small as possible (so that the total size of the BCH codewords is kept to a minimum) yet pay negligible penalties of incorrect BCH decoding.
%We will discuss the case that $d_i>t$ in \autoref{sec:BCH_exception}.

% Hence, we can no longer set the error-correction capability of the BCH code for each group pair based on the exact number of distinct element in it, as we did in \autoref{sec:scheme}. Instead, we set a conservative error-correction capability $t$ (say $2.5\delta$) for all group pairs, which is sufficient for them (i.e., $t\geq d_i$ for $i=1,2,...,g$) with high probability. We will discuss the case that $d_i>t$ in \autoref{sec:BCH_exception}.


% ===============================
% To differentiate from the PBS described in \autoref{sucsec:our-scheme}, we refer it as PBS-basic in this section. Note that the BCH decoding computational complexity is $O(d^2\log ^2 n)$, which is $\Omega(d^2\log^2 d)$ when $n=\Omega(d^2)$, with the state-of-the-art decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019}. It is too large in PBS-basic for large $d$. To overcome this drawback and generalize PBS-basic for large $d$, we partition sets $A$ and $B$ each into $d/\delta$ subsets (which we call {\it groups} to distinguish from subsets) for some small integer $\delta$ (say $5$) and reconcile the $d/\delta$ group pairs respectively using PBS-basic. After this partition, each group has $\delta$ distinct elements on average. The BCH decoding computational complexity of each group pair can be considered as $O(1)$, since $\delta$ is a small number. As a result, the overall computational complexity of PBS is reduced from $O(d^2\log ^2 n)$ to $O(d)$. 

% % To differentiate from the PBS described in \autoref{sucsec:our-scheme}, we refer it as PBS-basic in this section. PBS-basic is not suitable for large $d$ for two reasons: First, its communication overhead is asymptotically $O(d\log n)\!=\!O(d\log d)$ (since $n=\Omega(d^2)$), which is not asymptotically optimal. Second, the decoding computational complexity is proportional to $d^2$ with the state-of-the-art decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} for BCH codes, which is too high when $d$ is large. To overcome these two drawbacks, we use a simple algorithmic trick to (1) reduce the communication overhead from $O(d\log d)$ to $d\log u \!+\! O(d)$; (2) reduce the decoding computational complexity from $O(d^2)$ to $O(d)$. 

% Now, we describe the generalized PBS in details: In the first step, we hash-partition $A$ and $B$ (by some hash function $h_1(\cdot)$) into $g$ group pairs, just like what we did in \autoref{sucsec:our-scheme}. The objective of this partition is however different: In \autoref{sucsec:our-scheme}, we aim to ensure each subset pair contains at most $1$ distinct element (i.e., the ideal case) with high probability; Here we aim to make each group pair contains roughly $\delta$ distinct elements for some small constant $\delta$ (say $5$) by setting $g=d/\delta$. 
% %To differentiate the $g$ subset pairs here from those in \autoref{sec:hash_partition}, we call them the $g$ {\bf groups} in the sequel. 
% In the second step, we just apply PBS-basic (described in \autoref{sucsec:our-scheme}) to reconcile each group pair and obtain the distinct elements. 
% ================================

% To differentiate from the PBS described in \autoref{sucsec:our-scheme}, we refer it as PBS-basic in this section. When $d$ is large (more than several), we hash-partition set $A$ and $B$ into groups, such that each group pair contains $\delta$ distinct elements on average for small $\delta$ (say $5$), as described in \autoref{sec:larged}. Then each group pair can be reconciled by PBS-basic.

% When describing the PBS-basic in \autoref{sucsec:our-scheme}, we assume that the number of distinct elements is precisely known. We set the error-correction capability of the BCH code (denoted as $t$) just enough to correct $d$ errors (i.e., $t=d$). However, due to the randomness of hash-partition, $d_i$, the number of distinct elements in the $i^{th}$ group pair, is a Binomial random variable $Binomial(d,1/g)$ with expectation of $\delta$ $(=d/g)$ for $i=1,2,...,g$, which cannot be precisely known without a huge amount of additional communication overhead. Hence, we can no longer set the error-correction capability of the BCH code for each group pair based on the exact number of distinct element in it, as we did in \autoref{sucsec:our-scheme}. Instead, we set a universal error-correction capability $t$ (say $2.5\delta$) for all group pairs, which is sufficient for all group pairs (i.e., $t\geq d_i$ for $i=1,2,...,g$) with high probability. We will discuss the case that $d_i>t$ in \autoref{sec:BCH_exception}.

%This assumption in general does not hold: 
% Let $d_i$ denote the number of distinct elements in Group $i$. Due to the property of hash-partition, each $d_i$ is a Binomial random variable $Binomial(d,1/g)$ with expectation of $\delta$ $(=d/g)$. Even if $d$ is precisely known, each $d_i$ is not. To ensure the error-correction capability $t$ is sufficient for each group (i.e., $d_i\leq t$) with high probability, we leave some safety margin for the randomness of $d_i$ and conservatively set $t$ roughly $2.5\delta$ (the factor $2.5$ varies depend on other parameters, which will be discussed in \autoref{sec:parameter_settings}), so that $Pr[d_i>t]$ is tiny. We will discuss the case that $d_i>t$ in \autoref{sec:BCH_exception}.

% Note that the `safety margin' between $t$ and $\delta$ incurs additional communication overhead on transmitting BCH codeword: In the perfect scenario (i.e., $\{d_i\}_{i=1}^g$ is precisely known), the average communication overhead on transmitting BCH codeword per group pair is $\delta\log n$; On the other hand, when we set $t$ to be the error-correction capability for each group pair, the average communication overhead becomes $t\log n$. If we set the `safety margin' to be too large (say $t=10\delta$), it will incur huge additional communication overhead. Due to this reason, we set a moderate `safety margin' that  $t$ in the range from $1.5\delta$ to $3\delta$. 

%which is roughly $2.5$ times of that in the perfect scenario (when $t$ is roughly $2.5\delta$). Due to this addition
{\bf (modified)} If we have an accurate estimation of $\{\delta_i\}_{i=1}^g$, we can set $\{t_i\}_{i=1}^g$, the error-correction capabilities of the $g$ group pairs, to be very close to (slightly larger) those estimations. It can save considerate communication overhead on transmitting the BCH code. However, to estimate all the $g$ values of $\{\delta_i\}_{i=1}^g$ in high accuracy requires much larger additional communication overhead than the savings. 

% {\bf (previous)} Readers may wonder if we can reduce this additional communication overhead by using some technique to estimate $\{d_i\}_{i=1}^g$ (e.g., ToW estimator in \autoref{subsec:ToW}), so that we can set the error-correction capability of each group more wisely and save some waste on the safety margin. However, to achieve that, the estimation on $\{d_i\}_{i=1}^g$ must be in extremely high precision (since $\{d_i\}_{i=1}^g$ are small numbers with mean of $\delta$), which incurs much larger additional communication overhead than the savings. Due to the same reason (i.e., estimate $\{d_i\}_{i=1}^g$ is costly), we set the number of subset pairs for each group pair to be all equal (denoted as $n$). 
%based on $\delta$ ($n=\Omega(\delta^2)$). 

{\bf (moved from the small d case)} Although PBS runs as many rounds as to reconcile all distinct elements (in each group pair), we want PBS to successfully reconcile all distinct elements in only a few rounds (say $3$) with high probability (say $99\%$). Hence, when tuning parameters (to be discussed in \autoref{sec:parameter_settings}), we set a {\it target success probability} $p_0$ combined with a {target number of rounds} $r$ as the {\it paramenter setting requirement}, which aims to ensure that the {\it success probability}, the probability that all distinct elements are reconciled, within $r$ rounds to be larger than $p_0$. 
{\bf Normally, to achieve the same target success probability using fewer rounds (smaller $r$), PBS need more resources (e.g., larger $n$, $t$) for the ideal case happening with higher probability (fewer exceptions happen and need to be handled in later rounds), as we will explain in \autoref{sec:parameter_settings}.}
This success probability (within $r$ rounds) is also the expected value of the {\it success rate} of PBS, which is defined as the number of `successful' experiments (all distinct elements are successfully reconciled within $r$ rounds) divided by the total number of experiments. 

%The requirement above should also ensure the majority of the distinct elements are reconciled in the first round. 
% Note that PBS reconciles the distinct elements gradually round by round. The distinct elements that have been reconciled in the first round are no longer needed to be reconciled again in later rounds. This is the ``piecewise decodability'' mentioned in \autoref{sec:intro_oursolution}. The requirement above also ensures the majority of the distinct elements are reconciled in the first round, as we will show in \autoref{sec:piecewise_decodability}. Therefore, the majority of the overall communication overhead happens in the first round. In other words, the overall communication overhead of all rounds is only slightly larger than ($1.01$ to $1.07$ times of) that in the first round. Due to this reason, we use the communication overhead in the first round (described in \autoref{sec:communication_overhead_single_PBS}) to approximate the overall communication overhead of all rounds in parameter settings (to be elaborated in \autoref{sec:parameter_settings}.


% Like what we did in \autoref{sec:multi-rounds}, we set a paramenter setting requirement on the target success probability $p_0$ of $r$ rounds for all group pairs, which ensures the probability that all group pairs are completely reconciled in $r$ rounds to be larger than $p_0$. The detail about how to set $n$, $g$, and $t$ given such a success probability requirement will be elaborated in \autoref{sec:parameter_settings}. 

% we set a {\it target success probability} $p_0$ of $r$ rounds as a paramenter setting requirement, which aims to ensure the probability that all distinct elements are reconciled in $r$ rounds to be larger than $p_0$. This requirement should also ensure the majority of the distinct elements are reconciled in the first round. Use the same example ($d=5, n=255$), on average $4.81$ out of $5$ distinct elements should be reconciled in the first round. So the total communication overhead in all rounds is only slightly larger than ($1.01$ to $1.07$ times of, as we will show in \autoref{fig:per-round-con}) that in the first round. Due to this reason, we use the communication overhead in the first round (described in \autoref{sec:communication_overhead_single_PBS}) to approximate the total communication overhead of all rounds in parameter settings (to be elaborated in \autoref{sec:parameter_settings}.

% Note that this safety margin incurs additional communication overhead on transmitting BCH codeword: In the perfect scenario (i.e., $\{d_i\}_{i=1}^g$ is precisely known), the average communication overhead on transmitting BCH codeword per group is $\delta\log n$; On the other hand, when we set $t$ to be the error-correction capability for each group, then the average overhead becomes $t\log n$, which is roughly $2.5$ times of that in the perfect scenario (when $t$ is roughly $2.5\delta$). Readers may wonder if we can reduce this additional communication overhead by using some technique to estimate $\{d_i\}_{i=1}^g$ (e.g., ToW estimator in \autoref{subsec:ToW}), so that we can set the error-correction capability of each group more wisely and save some waste on the safety margin. However, to achieve that, the estimation on $\{d_i\}_{i=1}^g$ must be in high precision, which requires a much higher communication overhead than the savings.

% Although PBS may need to run many rounds to reconcile all distinct elements, the communication overhead mostly happens in the first round, since the majority of the distinct elements should be reconciled in the first round. Use the same example ($d=5, n=255$), on average $4.81$ out of $5$ distinct elements should be reconciled in the first round. So the total communication overhead in all rounds is only slightly larger than ($1.01$ to $1.07$ times of, to be shown in \autoref{fig:per-round-con}) that in the first round. Due to this reason, we use the communication overhead in the first round (described in \autoref{sec:communication_overhead_single_PBS}) to approximate the total communication overhead (all rounds) in parameter settings (to be elaborated in \autoref{sec:parameter_settings}).

%For the moment, we assume no ``fake'' distinct element in type (\RN{2}) subset pairs fails to be detected, which happens with overwhelming probability as explained in \autoref{subsec:exception_hash_partition}. Then 

% PBS reconciles the distinct elements gradually round by round. This is the ``piecewise decodability'' mentioned in \autoref{sec:intro_oursolution}. We use the following example to describe it in details: 
% Given two sets with $10$ distinct elements, in the first round, PBS tries to reconcile the $10$ distinct elements and say $6$ out of the $10$ distinct elements are successfully reconciled. Then the $6$ reconciled distinct elements are removed and PBS tries to reconcile the remaining $4$ distinct elements in the second round. Say $2$ out of the $4$ remaining distinct elements are successfully reconciled, and that leaves $2$ remaining distinct elements to be reconciled in the third round, so on so force. 
% % Given two sets $A$, $B$ with $10$ distinct elements, in the first round, PBS hashes them into $7$ distinct subset pairs. $6$ distinct elements are hashed into $6$ distinct subset pairs, and the other $4$ distinct elements are hashed into the same subset pair. Then the former $6$ distinct elements are successfully reconciled in the first round and the later $4$ distinct elements remain to be reconciled in the second round, which are hashed into $3$ distinct subset pairs (under a different hash function). $2$ remaining distinct elements are hashed into $2$ distinct subset pairs, and the other $2$ remaining distinct elements are hashed into the same subset pair. Then the former $2$ remaining distinct elements are successfully reconciled in the second round and the later $2$ remaining distinct elements remain to be reconciled in the third round, so on so force. 
% The dynamics of the number of remaining distinct elements (i.e., $10\leadsto 4\leadsto 2\leadsto \cdots$ in the example) is in nature a Markov chain, which will be elaborated and analyzed in \autoref{sec:single_markov} to derive a tight tail bound of the probability that all distinct elements are reconciled in $r$ rounds. 

%, which we will show in \autoref{subsec:mini-partition}.

% The same algorithmic trick can also be implemented in PinSketch~\cite{Dodis_PinSketch_2008} to reduce it computational complexity from $O(d^2)$ to $O(d)$. However, it will encounter the same randomness problem and have to set up a safety margin on the error-correction capability. This safety margin will incur much more communication overhead on PinSketch than on our scheme: Considering the average communication overhead per group, in our scheme, this overhead can be expressed as $t\log n+\delta\log n+\delta \log u+32$, in which $t\log n$ accounts for the BCH codeword, $\delta\log n$ accounts for the index of the subset pairs, $\delta \log u$ accounts for the bitwise \code{XOR} in \autoref{alg:trivial_case}, and $32$ accounts for the $32$-bit CRC in \autoref{proto:multirounds}. In PinSketch, this overhead increases from $O(\delta\log u)$ (optimal) to $O(t\log u)$ (PinSketch does not need to transmit bitwise \code{XOR}) if it uses the same algorithmic trick. Use the same example in \autoref{sec:intro}, when $\delta=5, n=255, u=2^{32}, t=2.5\delta$, the overhead of PinSketch using the trick is $2.5$ times of the optimal, while that of our scheme is $2.075$ times of the optimal (as we introduced in \autoref{sec:intro_oursolution}). That means our scheme has a lower communication overhead than PinSketch if they both use the algorithmic trick. Furthermore, as the signiture size $\log u$ increases, the advantage of our scheme over PinSketch becomes more significantly, which we will show in \autoref{subsec:mini-partition}.

% In PinSketch, each bit encodes only a single element in the universe, so the size of the bitmap is equal to the size of the universe.  
% For example, in the set reconciliation problem we usually assume each element is ``indexed" by a $32$-bit-long (hash) signature, so the universe contains a total of $2^{32}$ elements. In this case, the bitmap encoding for any set in PinSketch is $2^{32}$ bits long, and the Galois field involved in its BCH decoding is the ``$32$-bit-wide" $GF(2^{32})$.  In contrast, as explained earlier, in PBS 
% %since each bit encodes the oddness or evenness of the cardinality of a subset,   
% the size $n$ of a bitmap is dependent only on $d$, and not on the size of the universe or on the cardinality of the set the bitmap encodes.   For example, as shown in the example above, $n = 255$ is large enough for $d = 5$.  In this case, the BCH decoding operates in the much shorter
% ``8-bit-wide" $GF(2^{8})$.  This shorter ``width" alone in theory translates into roughly $16$ times shorter BCH decoding time, which as will be explained in~\ref{} grows quadratically with the ``width" of the underlying Galois field.  This shorter ``width" also implies four times shorter BCH codeword in PBS than in PinSketch, resulting in lower communication complexity as will be shown in~\autoref{}.

% Note that our scheme only takes 1 round trip delay to both identify the $d$ subset pairs and reconcile them: In the first half, Bob computes and sends PBS to Alice. Then Alice locally identifies the $d$ subset pairs and then initiates the reconciliation ({\it i.e.,} \autoref{alg:trivial_case}) for them, {\it i.e.,} computes the bitwise \code{XOR} of the corresponded $d$ subsets. In the second half, Alice sends the bitwise \code{XOR} of the $d$ subsets with their indexes to Bob. Then Bob can compute the set difference $A\Delta B$ locally.


% We can certainly use some communication-efficient technique to estimate $d_i$ (e.g., \autoref{subsec:ToW}). However, to obtain $d_i$ precisely will require a communication cost almost as large as to reconcile Group $i$. So instead of obtaining $d_i$ and set $c_i$ (i.e., the error-correction capability of Group $i$) equal to $d_i$, we leave the randomness of $d_i$ and set $c_i$ neither too conservative, nor too libertive in the following sense: (1) $c_i$ is not too big (conservative, i.e., $10\delta$) to make the total size of PBS unnecessarily large and incur too much extra communication overhead; (2) $c_i$ is not too small (libertive, i.e., $\delta$) to incur a high probability of insufficient decode capability, which can result in hefty penalties in the latter case of incorrect decoding (will be elaborated in \autoref{sec:BCH_exception}). In our scheme, we set $c_i$ to be $2-3$ times of $\delta$, which will be shown in \autoref{sec:tail_bound} that it is just enough to make the probability of decode failure very small. Meanwhile, we set the error-correction capability of each group ($c_1,c_2,...,c_k$) to be all equal and denote it as $c$. 

%Since the decoding capacity $t$ and the number of subset pairs for each group $n$ are both small constants independent of $d$, therefore, the communication overhead per group is $t\cdot\log n \!=\!O(1)$, which implies a total communication overhead of $O(d)$. Similarly, the total decoding computational complexity is also $O(d)$. 

% \subsection{Exception Handling}\label{sec:exceptions}

% \subsubsection{Exception Handling on Hash-Partition}\label{subsec:exception_hash_partition}

% As we have described in \autoref{sec:hash_partition}, the ideal case does not always happen, which means some subset pair may contain more than 1 distinct elements and cannot be successfully reconciled by \autoref{alg:trivial_case}. Due to the parity encoding, we can classify such subset pair into the following two scenarios:

% \begin{itemize}
%     \item Scenario 1: If a subset pair $(A_i, B_i)$ contains even number ($\geq 2$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be the same and our scheme will not reconcile the subset pair. Hence, the distinct elements in the subset pair will not be reconciled;
%     \item Scenario 2: If a subset pair $(A_i, B_i)$ contains odd number ($\geq 3$) of distinct elements, the parity bits of $A_i$ and $B_i$ will be different and our scheme will reconcile the subset pair using \autoref{alg:trivial_case}. However, as we described in \autoref{subsec:protocol0}, when a subset pair contains more than 1 distinct elements, \autoref{alg:trivial_case} will output the bitwise \code{XOR} of them as the `distinct element', which is not a real distinct element with high probability;
% \end{itemize}

% In both scenarios, the distinct elements in the subset pair cannot be reconciled. Even worse, in the second scenario, a false-positive could happen (i.e., the output of \autoref{subsec:protocol0} is not a real distinct element). For example, if subset pair $(A_i, B_i)$ contains $3$ distinct elements $s_1, s_2, s_3$, then the output of \autoref{alg:trivial_case} is $\tilde{s}_4=s_1\oplus s_2\oplus s_3$, which is normally not a distinct element. The good thing is, the probability of the false-positive is extremely small for small $d$. For instance, if $d=5$ and $n=255$, the probability of the false-positive is $7.6\times 10^{-6}$, which is very small. To further reduce the chance of false-positives, we add a verification step at the end of \autoref{subsec:protocol0} to check whether the output of \autoref{subsec:protocol0} $s$ is a real distinct element or not. The verification step works as follows: Given the output $s$ of subset pair $(A_i,B_i)$, if $s\in\mathcal{U}_i$ (i.e., $h(s)=i$), we consider $s$ as a real distinct element; Otherwise, we consider $s$ as an incorrect output and discard it. 

% Note that if $s$ is a real distinct element of $(A_i,B_i)$, $s$ must be in sub-universe $\mathcal{U}_i$. However, if $s$ is the bitwise \code{XOR} of the distinct elements in $(A_i,B_i)$ (i.e., the second scenario happens), $s$ could be in any sub-universe other than $\mathcal{U}_i$. In fact, if we assume the hash-partition described in \autoref{sec:hash_partition} hashes the elements of $\mathcal{U}$ uniformly, independently, and randomly into $n$ sub-universes, the output $s$ in the second scenario will be in a different sub-universe $\mathcal{U}_j (j\neq i)$ with a high probability of $1-\frac{1}{n}$. Hence, this verfication method can further reduce the probability of false-positives by a factor of $\frac{1}{n}$. Use the same example (i.e., $d=5$, $n=255$), the probability is reduced from $7.6\times 10^{-6}$ to $3\times 10^{-8}$ by this verification method. 

% In some super critical cases (i.e., no false-positive is allowed), we can use a more powerful verification method to completely eliminate false-positives. That is, to check if the output $s$ exists in exactly one of the two sets (i.e., $s\in A\setminus B$ or $s\in B\setminus A$). To do so, Bob transmits $s$ along with an identification bit $\mathbb{1}_{\{s\in B\}}$ to Alice, then Alice checks if $s$ . This method verification costs $d(\log u+1)$ bits of additional communication overhead. In most applications, rigorously $0\%$ probability of false-positives is unnecessary and the probability of the former verification method is small enough, so we use the former verfication method in our evaluation. Based on our observation, the false-positive does not happen even once in our evaluation using the former verfication method.

\subsection{Exception Handling on BCH Decoding}\label{sec:BCH_exception}

The exceptions that happens within PBS-basic have been discussed and handled in \autoref{subsec:exception_hash_partition} and \autoref{sec:multi-rounds}. In this section, we only discuss the exceptions that the error-correction capability $t$ is insufficient for some group $i$. More specifically, when $d_i$ (i.e., the number of distinct elements in group $i$) is larger than the error-correction capability $t$, the BCH codewords of group $i$ differ at $d_i$ bit positions in the ideal case, which exceeds the error-correction capability $t$. If so, the BCH decoder cannot decode the bit errors correctly (\autoref{step:BCH_decode} in \autoref{alg:single_round_pbs}) and report a failure. This exception happens with a small probability in each group pair: For example, when $d=1000$, and $\delta$ is set to $5$ (so that $g=d/\delta=200$), and $t$ is set to $13$, the probability that this exception happens is only $6.7\times 10^{-4}$. 

To handle this type of exceptions, we use the same algorithm trick in \autoref{subsec:protocol2} to further partition each problematic group into $3$ sub-groups and reconcile them respectively using PBS-basic. Note that $d_i$, if is not smaller, should be only slightly larger than $t$ with high probability. Hence, partitioning into $3$ sub-groups is enough to ensure each sub-group has no more than $t$ distinct elements. Then in the next round, each sub-group does not encounter this type of expections and can be reconciled by PBS-basic respectively. Use the same example above ($d=1000$, $\delta=5$, $t=13$), the probability that some sub-group has more than $t$ distinct elements is $9.5\times 10^{-10}$. More specifically, we add a termination condition of \autoref{alg:3_way_partition} after \autoref{step:BCH_decode} in \autoref{alg:single_round_pbs}.

\begin{algorithm}
\caption{Termination condition when BCH decoding fails}
\label{alg:3_way_partition}

\If{BCH decoding fails\label{step:if1}}
{Hash-partition the group into $3$ sub-groups and do PBS for each of them in the next round; Break;}\label{step:term1} 

\end{algorithm}

% Back to the \autoref{proto:multirounds}, which shows the set reconciliation operations in each round of PBS-basic, this kind of exceptions only affect \autoref{step:reconcile} in \autoref{proto:multirounds}. Now this step needs to check whether BCH decoding is successful or not: If successful, all the operations remain the same; Else, we hash-partition the group ($A$ and $B$) into $3$ sub-groups and reconcile them respectively using \autoref{proto:multirounds}. 
% {\bf I'm not sure if it is necessary to discuss this case, since PinSketch did not mention it, even it may happen in PinSketch}
% Another type of exceptions that happens when $d_i>t$ is, the BCH decoder mistakes the decoding is successful and returns $t$ incorrectly decoded bit errors (i.e., subset pairs). The probability of this type of exceptions is very small. For instance, when $d=1000, \delta=5, t=13$ $(2.5\delta)$, $d_i>t$ happens with probability roughly $6.7\times 10^{-5}$, and the probability that the BCH decoder mistakes the decoding is successful when $d_i>t$ is on the order of $10^{-7}$ \cite{kim1996undetected}. So the probability that this type of exceptions happens in each group is on the order of $10^{-12}$. On the other hand, the impact of this type of exceptions is insignificant. Assume an incorrectly decoded bit error corresponds to a random subset pair, which could contain (1) no distinct element; (2) exactly $1$ distinct element; or (3) more than $1$ distinct elements. Reconcile the subset pair using \autoref{alg:trivial_case} could (1) get nothing and waste $\log |\mathcal{U}|$ bits of communication overhead; (2) get an actual distinct elements; or (3) trigger the exceptions that were discussed and handled in \autoref{subsec:exception_hash_partition}. 

\subsection{What if PinSketch also uses partitions?}

The same algorithmic trick (i.e., hash-partition two sets each into groups) can also be implemented in PinSketch~\cite{Dodis_PinSketch_2008} to reduce it computational complexity from $O(d^2)$ (of finite field operations in GF($2^{32}$)) to $O(d)$. However, it will encounter the same randomness problem and have to set up a safety margin on the error-correction capability $t$. This safety margin will incur much more additional communication overhead on PinSketch than on our scheme: Considering the average communication overhead per group pair, the additional overhead caused by the safety margin is $(t-\delta)\log n$ in PBS and $(t-\delta)\log |\mathcal{U}|$ in PinSketch. The later is roughly $4$ times of the former under the default setting ($n=255, |\mathcal{U}|=2^{32}$). Note that the optimal communication overhead to reconcile $d$ distinct elements is $\delta\log |\mathcal{U}|$. Use the same example in \autoref{sec:intro}, when $\delta=5, n=255, |\mathcal{U}|=2^{32}, t=2.5\delta$, the overhead of PinSketch using the algorithmic trick is $2.5$ times of the optimal (i.e., $d\log |\mathcal{U}|$), while that of PBS is $2.075$ times of the optimal. It means PBS could have a lower communication overhead than PinSketch if they both use the algorithmic trick. Furthermore, as the signiture length $\log |\mathcal{U}|$ increases, the advantage of PBS over PinSketch will be more significant.

% We handle this type of exceptions by the same method (i.e., hash-partition into $3$ sub-groups) as above. To detect them, on the other hand, is simple: Note that incorrect decoded bit errors correspond to the subset pairs that do not contain distinct elements. When we reconcile those subset pairs in \autoref{sec:reconcile_by_trivial}, the output (i.e., reconciled elements) will be $\mathbf{0}$, which is abnormal (since $\mathbf{0}\notin A\bigcup B$, as we described in \autoref{subsec:protocol0}). Hence, this type of exceptions happen if and only if one of the reconciled distinct elements is $\mathbf{0}$. 
%Hence, we consider BCH decoding is successful by two criteria: (1) the BCH decoder reports a successful decode; and (2) None of the reconciled elements is $\mathbf{0}$. 
% ========================
% In fact, even if $d_i>t$, PBS-basic is still possible to reconcile group $i$ in some nonideal cases. For example, when $t=10$ and $d_i=11$, if the $11$ distinct elements are distributed in $10$ subset pairs, such that $1$ subset pair contains $2$ distinct elements and $9$ subset pairs contain $1$ distinct element in each, the two parity bitmaps differ at only $9$ bit positions. So BCH decoder is able to decode the later $9$ subset pairs and the corresponding $9$ distinct elements can be reconciled. In the second round, only $2$ distinct elements remain and BCH decoding certainly works. In this case, we do not need to partition the group into sub-groups, and this case does not trigger \autoref{alg:3_way_partition} in PBS. 
% ========================
% Instead, it will either (1) report a failure about exceeding the error-correction capability; or (2) mistake the decoding is successful and return incorrect decoded bit errors. 

% The second case happens with a very small probability (in order of $10^{-7}$ \cite{kim1996undetected}) and is very simple to detect : 

% The first case is easy to handle: We can simply adapt the same algorithmic trick to partition the group into smaller groups and reconcile them respectively. In our scheme, we set the number of smaller groups to be $3$, which is big enough because $d_i$, if not smaller, only slightly larger than $t$ with high probability. The second case on the other hand, although theoretically possible, happens with a very small probability when $d_i>t$ (in order of $10^{-7}$ \cite{kim1996undetected}). Besides, the probability of $d_i>t$ is also very small (e.g., when $t=15$ and $\delta=5$, this probability is about $2.3\times 10^{-4}$), so the overall probability of the second case, which is the multiplication of these two small numbers, is negligible (e.g., in order of $10^{-11}$).

% \subsection{Multi-rounds}

% Even if the ideal case does not happen, most of the distinct elements should be distributed into different subset pairs and therefore can be reconciled. So our scheme, even cannot reconcile all of the distinct elements, can still reconcile the majority of them (piecewise decodability). To reconcile the rest distinct elements, we can just run our scheme for multi-rounds under different hash-partition functions. For each round, our scheme works as follows: 

% \IncMargin{1em}
% \begin{algorithm}
% \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
% \Input{Two sets $A$ and $B$}
% \Input{Size of set difference $d$}
% \Input{The number of subset pairs $n$}
% \Input{BCH error-correction capability $t$}

% Hash-partition $A$ and $B$ into $n$ subset pairs $\{(A_i,B_i)\}_{i=1}^n$;

% \If{BCH decoding fails}
% 	Hash-partition $A$ and $B$ into $3$ subset pairs and reconcile them respectively in the next round\;
% \ElseIf{BCH decoding success}
	
% \Else{}

% $k \leftarrow \lceil \frac{t}{c}\rceil $\;

% Partition elements into $k$ subsets using~\autoref{alg:random-part}\;

% \For{$j = 0$ \KwTo $k-1$}{
%     Reconcile the $j$-th subset pair using the straw-man scheme with the BCH correcting capability $\tau$, number of smaller subsets $m$, and number of rounds $r$\;
% }

% \caption{PBS (per round)} \label{proto:II}
% \end{algorithm}\DecMargin{1em}

% This {\bf multi-rounds} scheme can significantly increase the success probability (i.e., the probability that all distinct elements are reconciled). Readers may wonder in the later rounds, most distinct elements should be reconciled, and the remaining could be reconciled using degraded parameters (i.e., smaller $n$ and $t$). In fact, degrade parameters in later rounds cannot save much communication overhead, since the majority of it is spent in the first round (i.e., $>90\%$). Therefore, we use the same parameters (i.e., $n,t$) among all rounds in our evaluation. 
% %The tradeoff between the number of rounds and the communication overhead per rounds will be elaborated in \autoref{sec:tail_bound}. In our evaluation, $r=2,3$ rounds are enough to achieve an extremely high success probability. 

% Readers may think the cost (i.e., communication overhead and the computational complexity) of this multi-rounds scheme is proportional to the number of rounds (denoted as $r$) and increases linearly with $r$. In fact, the cost of each round is roughly proportional to the number of remaining distinct elements, which decreases exponentially as $r$ increases (i.e., the first round reconciles $99\%$ of distinct elements, the second round reconciles $99\%$ of the remaining $1\%$ distinct elements, etc.). So the cost of this multi-rounds scheme is only slightly larger than that of the single-round scheme. Furthermore, as we explained in \autoref{sec:intro}, {\bf from intro thanks for the piecewise decodability of our solution, in almost all practical application scenarios, this tradeoff does not lead to longer response time because the reconciliation of objects identified by the successfully decodable codewords, which constitute the vast majority of all codewords, can run in parallel with the transmissions and decodings of the rest.  In other words, the piecewise decodability effective masks the slightly larger number of communication rounds as far as the response time is concerned.} 





\begin{comment}
\subsubsection{Random Partition}

\IncMargin{1em}
\begin{algorithm}
% \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
% \Input{Set $S$}
% \Input{The number of subsets $m$ for partition}
% \Output{Subsets $S_1, S_2, ..., S_m$}

% Generate hash function $h(\cdot)$ that maps each element into $\{1,2,...,m\}$;

\ForEach{$s \in S$}{
    $j \leftarrow h(s) \bmod m$\;    
    Insert $s$ into the $j$-th subset $S_j$\;
}

\caption{Partition using hash function $h(\cdot)$.} \label{alg:random-part}
\end{algorithm}\DecMargin{1em}

Like the strawman scheme, our scheme randomly partitions sets $A$ and $B$ into $m$ subsets. This random partition 
can be easily accomplished by using some hash function, $h(\cdot)$, and inserting each element $x$ into the subset 
corresponding to $h(x)$. \autoref{alg:random-part} presents the pseudo-code of this random partition using hash 
function $h(\cdot)$.  

% Unlike the strawman scheme, our scheme only reconciles those subset pairs that need to be reconciled, 
% because 



Like the strawman scheme, our scheme hash-partitions the two sets $A$ and $B$ into $m$ subset pairs $(A_i, B_i)$ for $i=1,2,\cdots,m$. 
We note that, among those $m$ bins (subset pairs), 
at most $t$ ($t\!\ll\!m$ as shown in our analysis in~\autoref{subsec:protocol1}) bins contain balls 
(elements belonging to the set difference), {\it i.e.,} requiring reconciliation.  
Motivated by this observation, we, therefore, propose to first detect those bins that 
contain balls and then only reconcile them. The detection is solved with a simple encoding approach that 
will be detailed in the next section.

\subsubsection{Detection before Reconciliation} 

In fact, identifying those non-empty bins is easy when each bin contains at most one ball. In this section, we assume that 
each bin after the random partition contains at most one ball, we will show later how to handle the cases when some 
bins contain more than one balls later in~\autoref{subsec:exceptions}. 

Given an arbitrary bin (say subset pair $(A_i, B_i)$) that contains one ball ({\it i.e.,} $A_i\Delta B_i$ contains exactly one element), 
the corresponding two subsets $A_i$ and $B_i$ differ exactly one element, which implies that 
$||A_i|\!-\!|B_i||\!=\!1$. Hence, if $|A_i|$ ({\it i.e.,} number of 
elements in $A_i$) is odd (or even), then $|B_i|$ must be even (or odd). In other words, the odevity of $|A_i|$ 
and $|B_i|$ are opposite. %differs if $|A_i\Delta B_i|\!=\!1$. 
Based on this property, we propose the {\it odevity encoding}: 
A subset is encoded as ``1'' if it contains odd number of elements, and as ``0'' otherwise. 
Using this odevity encoding, the $m$ subsets of $A$ can be encoded as a bit string $b_A$ in $\{0,1\}^m$, 
where the $i$-th bit in $b_A$ corresponds to the odevity encoding of $|A_i|$. Similarly, the $m$ subsets of $B$ can also 
be encoded as a bit string $b_B$. Clearly, $b_A$ and $b_B$ differ at $t$ different positions, or in other words, 
the Hamming distance of bit strings $b_A$ and $b_B$ is $t$. A straightforward approach is 
to let Alice send $b_A$ to Bob, and then Bob compares $b_B$ against $b_A$ to obtain those non-empty bins. 

This approach, however, has a communication overhead of $m$ bits, which is still unnecessarily high. As 
analyzed in~\autoref{subsec:protocol0}, $t$ is usually much smaller than $m$. 
That means $b_A$ and $b_B$ differ only at a tiny portion of bits. %have much more in common than differences. 
Therefore, if we view $b_B$ as a corrupted message of $b_A$ with $t$ corrupted bits, the detection of those $t$ bins can be converted to 
the detection of the positions of the $t$ corrupted bits. The latter can be solved using an Error-Correction Code (ECC)~\cite{Lin_ErrorControlCoding_1983} that can correct up to $t$ errors. In this work, we use the BCH code~\cite{Lint_IntroductionCodingTheory_1998}. 
More precisely, this ECC-based approach (with the BCH code) works as follows. 
Alice computes the parity bits for $b_A$ using a $t$-error-correcting BCH code with a block length of 
$(2^{\lceil \log m\rceil} -1)$ and sends the parity bits to Bob. Bob then decodes the positions of the $t$ corrupted bits 
using the BCH decoding algorithm with $b_B$ and those parity bits received from Alice. The communication overhead of 
this approach is roughly $t\lceil \log m\rceil$ ($=O(t\log t)$) bits. In the example above, this communication overhead is 
roughly $\num{17000}$ bits, which is approximately $6$ times lower 
than $m\!=\!\num{108469}$ bits, the communication overhead of the aforementioned straightforward approach. 

At first sight, it seems that the detection of non-empty bins and reconciliation of subsets in those bins require two rounds 
(or at least two round trip delays), {\it i.e.,} one round for detection and the other for reconciliation. In fact, 
it only requires one. After Bob receives the parity bits from Alice and decodes out those non-empty bins, it initiates 
the reconciliation ({\it i.e.,} \autoref{alg:trivial_case}) for each bin (subset pair) immediately, 
{\it i.e.,} sends the \code{XOR} sums of subsets in those bins together the indexes of those bins. 
After receiving those \code{XOR} sums and bin indexes, Alice can compute the set difference. 

% A naive way to combine the detection of non-empty bins and reconciliation of subset pairs in those bins is to first detect 
% those non-empty bins via one round of message exchanges between Alice and Bob and then to reconcile the corresponding 
% subset pairs in those bins with another round of message exchanges. This requires two rounds ({\it i.e.,} taking at least 
% two round trip delays). In fact, after Bob receives the parity bits from Alice and obtains those 

\subsubsection{Multiple Rounds}\label{sec:multiround}

{\bf This section was not clear enough. I need more time to think about and revise it.}


In the above section, we have assumed that each bin contains at most one ball. 
However, even with a sufficient large $m$, some bin might contain more than one balls though with tiny probability. 
We will show in~\autoref{subsec:exceptions}, how such rare events, {\it i.e.,} one bin contains more than one balls, 
can be easily detected.
To ensure our scheme can successfully reconcile all elements even when such rare events happen, 
we propose to use multiple rounds (of communication between Alice and Bob). More precisely, instead of 
selecting a prohibitively large $m$ to ensure that each bin contains at most one ball with a extremely high probability 
(say 0.99999), we select a reasonably large $m$ so that the communication overhead is not very high and very few bins contain 
more than one balls (or in other words, most bins contain at most one ball). Therefore, after running one round of 
our scheme, most elements in the set difference will be reconciled. Only those in the bins that contain more than one balls 
fail to be reconciled. For elements in the subsets corresponding to those bins, we run another round of our scheme. 
If some elements still fail to be reconcile, we can run one more round of our scheme. So on so forth,  
our scheme can keep running for more rounds until all elements are reconciled. 

With the same communication overhead, multiple rounds can significantly increase the success rate, 
{\it i.e.,} the probability that all elements in the set difference will be successfully reconciles, 
which will be elaborated in~\autoref{sec:tail_bound}. 

% % to be emphasized
% % say that too many rounds should be avoided (latency & communication overhead reduction is negligible when r is too large, 2 - 3 is good enough)
% % multiple rounds is not an issue when r is small

% We note that the number of rounds $r$, however, should not be large. On one hand, it results in large latency (at least $r$ round trip delays). 
% On the other hand, when $r$ is large, the reduction of communication overhead by the increase of $r$ gradually diminishes. 

We note that multiple rounds, when $r$ is small, would not really increase the ``latency'', as long as most elements in the 
set difference can be reconciled in the first rounds, since the underlying synchronization of data objects corresponding to 
those elements can start immediately after the first round of our scheme. Therefore, the actual latency is one round trip delay instead of 
$r$. 

As we mentioned, this straw-man protocol works correctly if each subset pair has at most one exclusive element (i.e., \autoref{eq:requirement_strawman} holds). On the other hand, if a subset pair has more than one exclusive elements, some of which will not be successfully reconciled:

\begin{itemize}
\item If a subset pair has even number of exclusive elements, Odevity coding will encode it as 0. Then the straw-man scheme will consider the subset pair having no exclusive element and all exclusive elements in this subset will not be reconciled;

\item If a subset pair has odd number ($\geq 3$) of exclusive elements, Odevity coding will encode it as 1 and consider the subset pair having only 1 exclusive element. Then the straw-man scheme will use \autoref{alg:trivial_case} to decode only one exclusive element and dismiss all others. Even worse, the only decoded element is probably not a real exclusive element, since the element computed by \autoref{alg:trivial_case} is the \code{XOR} sum of all exclusive elements, not one of them. 
\end{itemize}

In summary, if a subset pair has more than one exclusive elements, most of its exclusive elements cannot be reconciled, and the reconciled element is usually incorrect (i.e., false-positive). The false-positive however is easy to check, which will be elaborated in \autoref{subsec:exceptions}. The good thing is, even if not all subset pairs have at most one exclusive element and are successfully decoded, most of them will be w.h.p.. In other words, even if the straw-man protocol cannot reconcile all exclusive elements, it still can reconcile most of them. To reconcile all exclusive elements w.h.p., we can simply extend the single-round straw-man scheme to multi-round. And each round adapts the straw-man scheme to do set reconciliation using independent hashing functions $h(\cdot)$ for partition (i.e., in \autoref{alg:random-part}). This multi-round extension can significantly increase the probability of a successful reconciliation, which will be elaborated in \autoref{sec:tail_bound}. 



\subsection{Our Scheme: The Final Version}\label{subsec:protocol2}

{\bf Under revision~}

The preliminary version of our scheme suffers from two major drawbacks. 
First, its communication overhead is asymptotically 
$O(t\log m)\!=\!O(t\log t)$, which is not asymptotically optimal. 
Second, the decoding computational complexity is proportional to 
$t^2$ with the state-of-the-art decoding algorithm~\cite{Wuille_Minisketchoptimizedlibrary_2019} for BCH codes, 
which is too high when $t$ is large. 
To overcome these two drawbacks, we use a simple algorithmic trick: divide and conquer. With this algorithmic 
trick, the decoding computational complexity is reduced to $O(t)$, 
and the communication overhead is reduced to $t\cdot\frac{\log u}{8} \!+\! O(t)$ (with a small 
hidden constant roughly varying from 4 to 8) bytes which implies that 
our scheme has an additive communication overhead (compared to the optimal scheme) 
of 4 to 8 bytes per element in the 
set difference and this additive overhead is independent of the key size ({\it i.e.}, $\log u$). 
Recall that the IBF-based schemes usually have a communication overhead of roughly 6 times of the 
optimal scheme, which increases linearly as the key size. Therefore, our scheme is much more 
communication-efficient. 

Now, we describe in detail this algorithmic trick. We let Alice divide elements in $A$ into $\lceil\frac{t}{c}\rceil$ groups (subsets)  
for some small constant $c$ (say $5$) so that each group contains roughly $c$ elements from the set difference on average. We let Bob do the same operations on $B$. To ensure that any common element ({\it i.e.,} any element $x\!\in\! A\bigcup B$) goes into 
the same group ({\it i.e.,} groups at Alice and Bob with the same index), we can use the partition procedure with a hash function shown 
in~\autoref{alg:random-part}. Then, we can apply the preliminary version on each group with a constant $m$ (say $m\!=\!256$) independent of 
$t$. To ensure that each group can be reconciled with a high probability, we need to use BCH codes whose decoding capacity 
larger than $c$ (say $\tau\!=\!2c$), as exact number of elements to be reconciled could be larger than $c$. 
Since this decoding capacity $\tau$ is still a small constant independent of $t$, therefore, the communication 
overhead per group is $\tau\cdot\log m \!=\!O(1)$, which implies a total communication overhead of $O(t)$. 
Similarly, the total decoding computational complexity is also $O(t)$. 

\subsubsection{Parameter Configurations} 

Our scheme now has several parameters: $c$ (average number of elements from the set difference in each group), 
$\tau$ (the correcting capability of the BCH code), $m$ (number of bins for each group), and $r$ (maximum number of rounds). 
We note that the maximum number of rounds $r$ is usually associated with another parameter $p$ the desired success rate: With 
at most $r$ rounds, our scheme should guarantee that the success rate is at least $p$. 
%How to tune these parameters to achieve favorable performance will be detailed later in~\autoref{sec:tail_bound}. 
Here, we provide some guidances for the parameter configurations using our theoretical analysis, which gives the tail bound of 
the success probability of our scheme and will be shown in~\autoref{sec:tail_bound}. 

\noindent
{\bf Parameterizing $c$ and $r$.} The values of $c$ and $r$ are usually provided by users based on the requirements of 
applications. For the value of $c$, a larger $c$ results in a longer decoding time yet lower communication overhead.  
So if the decoding time is a big concern, then a smaller $c$ (say $c=5$) should be used; otherwise, a larger $c$ could be used. 
For the values of $r$, a larger $r$ leads to lower communication overhead and usually lower decoding time (as it allows to use 
a smaller $\tau$), however, the reduction is marginal when $r>3$. Therefore, we suggest users to configure $r$ to be $2$ or $3$. 
% The configuration of $c$ is relatively straightforward, as a larger $c$ will result in 
% a longer decoding time and a slightly lower communication overhead. The former is ..., The latter is slightly tricky. 


\noindent
{\bf Using $c$ and $r$ to parameterize other parameters.} After users specify the values for $c$ and $r$ (associated with a value for 
$p$), we can use our theoretical analysis in~\autoref{sec:tail_bound} to parameterize $\tau$ and $m$. 
Since in a BCH code, the block length is in the form of $2^q-1$, we only need to consider $m=2^q-1$. 

{\bf Liang, please revise the following algorithm!}

\begin{algorithm}
\SetKwProg{Proc}{}{}{end}
\SetKwFunction{algo}{\small Search}

\Proc{Search($c$, $r$, $p$)}{\label{search:entrance}

$\mbox{co}_{best}\leftarrow\infty$\tcc*{\small Best communication overhead}

\For{$\tau \leftarrow c\,\KwTo\, \infty$}{}



}
\end{algorithm}


% , unlike 
% the IBF-based schemes which have an multiplicative overhead of 6 
% The inspiration is from the famous 
% divide and conquer algorithm for the selection problem, in which, given an array with $n$ elements, we want to get the $k$-th largest 
% element. A straightforward idea for this problem is sorting. However, if using insertion-sorting, the complexity would be $O(n^2)$. 
% Then the famous divide and conquer trick comes. It first divides the array into $\lceil n/5\rceil$ groups so that the first 
% $\lfloor n/5\rfloor$ contains $5$ elements and at most one group contains the rest $n \mod 5$ elements, and find the median of each 
% group using the insertion-sorting and th


% This straw-man scheme still has a problem on decoding computational complexity. More specific, the complexity increases dramatically with the total number of corrupted bits $t$. Therefore, when $t$ is moderate or large, the decoding computational complexity could be very high. For instance, the decoding complexity of BCH codes~\cite{Lint_IntroductionCodingTheory_1998} is $O(t^3)$, which could be quite high for a large $t$. To keep the decoding complexity reasonably low, we design the following two-layer protocol: In the first layer, we use a hash function to partition the two sets into $\lceil\frac{t}{c}\rceil$ subsets for some small constant $c$ (say $5$), just like the first step of our straw-man scheme. The objective, which is however different from before, is to make each subset pair contains roughly $c$ exclusive elements on average. In the second layer, we use the straw-man scheme with the same configuration (number of subsets $m$, and error-correction capability $\tau$, number of rounds $r$) to reconcile each subset pair. 

% In fact, the straw-man scheme is a proper solution when $t$ is small. First, the decoding complexity will not be a problem for a small $t$; Second, we do not need an extremely large $m$ to guarantee \autoref{eq:requirement_strawman} w.h.p.. For instance, when $t=5$ and $m=1024$, \autoref{eq:requirement_strawman} holds with probability $\frac{m\,!}{(m-t)\,!m^t}\approx 99\%$. This motivates us to design the following two-layer protocol: In the first layer, we use a hash function to partition the two sets into $\lceil\frac{t}{c}\rceil$ subsets for some small constant $c$ (say $5$), just like the first step of our straw-man scheme. The objective, which is however different from before, is to make each subset pair contains roughly $c$ exclusive elements on average. In the second layer, we use the straw-man scheme with the same configuration (number of subsets $m$, and error-correction capability $\tau$) to reconcile each subset pair. 

\autoref{proto:II} shows the pseudocode of our scheme. It first uses the same hash-function based random partition algorithm as \autoref{alg:random-part} to partition elements into $k\triangleq\lceil \frac{t}{c} \rceil$ subsets. Note that the random partition only guarantees that each such subset 
contains $c$ exclusive elements on average, and the exact number is not known. Hence, our scheme uses a BCH code with a capability of 
correcting up to $\tau$ errors with $\tau > c$ to make sure that the BCH code has a high probability to decode successfully. We will describe how to deal with situation where the size of set difference exceeds $\tau$ later in~\autoref{subsec:exceptions}.

As the decoding of a $\tau$-error-correcting BCH code where $\tau$ is a small constant has a constant-time computational complexity, the decoding complexity of 
our scheme is $O(k)=O(t)$. We now have several parameters, average number of exclusive elements in each subset $c$, the correcting capability $\tau$ of BCH code, the number of smaller subsets $m$ for each subset to be divided to, and the number of rounds $r$. How to tune these parameters to achieve favorable performance will be detailed later in~\autoref{sec:tail_bound}. 

\IncMargin{1em}
\begin{algorithm}
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
\Input{Size of set difference $t$}
\Input{The number of subsets $m$ for each partition}
\Input{Average number of exclusive elements in each partition $c$}
\Input{BCH code capability $\tau$}

$k \leftarrow \lceil \frac{t}{c}\rceil $\;

Partition elements into $k$ subsets using~\autoref{alg:random-part}\;

\For{$j = 0$ \KwTo $k-1$}{
    Reconcile the $j$-th subset pair using the straw-man scheme with the BCH correcting capability $\tau$, number of smaller subsets $m$, and number of rounds $r$\;
}

\caption{Our Scheme} \label{proto:II}
\end{algorithm}\DecMargin{1em}




\subsection{Exceptional Handling}\label{subsec:exceptions}

{\bf To be revised~}

In this section, we will elaborate how to handle the following two types of exceptions that we mentioned in \autoref{sec:multiround} and \autoref{subsec:protocol2}:
\begin{itemize}
    \item Exception 1: A subset pair has odd number ($\geq 3$) of exclusive elements and causes false-positives (i.e., a decoded distinct element is not a real one);
    \item Exception 2: A subset pair contains too many exclusive elements, such that a BCH code with capability of correcting up to $\tau$ errors cannot decode it (i.e., $t>\tau$).
	\item Exception 3: A subset pair has even number ($\geq 2$) of exclusive elements and causes false-negatives(i.e., two or more distinct elements are neglected as the parity bit is 0);
\end{itemize}

To handle Exception 1, we need to check whether a computed exclusive element by \autoref{alg:trivial_case} is a real exclusive element or not. (The group index happens to come in handy if we use it as a fingerprint of the element we computed. If this element is truly an exclusive element, it should be hashed into the same group as before. Notably, We have two group indices available for this check, one is in the initial divide and conquer phase, the other is in the BCH code part) It can be easily done at the end of set reconciliation, during which two hosts exchange their exclusive elements. In fact, as we will elaborate in \autoref{sec:tail_bound}, Exception 1 hardly happens if we set parameters properly. 

On the other hand, when Exception 2 happens, the BCH decoder will report a failure about exceeding the error-correction capability. For such a subset pair, we can use the same approach as in \autoref{subsec:protocol2} to partition it into smaller subsets and use the straw-man scheme to reconcile them respectively. We set the number of small subsets to be 3. It is because, as we will elaborate in \autoref{sec:tail_bound}, the number of exclusive elements for each subset pair $t$ should be, if not smaller, only slightly larger than $\tau$ w.h.p.. Partitioning those exclusive elements into 3 small subsets is enough to guarentee that each of them has less than $\tau$ exclusive elements.

\end{comment}

==> section/theoretical_analysis.tex <==
\begin{comment}
\section{Tug-of-War Sketch}\label{sec:sketch}


In this section, we describe the {\it tug-of-war}, which was first proposed in~\cite{AlonMS99} as 
a space-efficient estimator for the second frequency moment. 
%% Copy from Infocom 2009
We briefly describe 
the plain vanilla tug-of-war sketch~\cite{AlonMS99} in the context of error estimating coding, and under the assumption
that the sketch per se is not subject to bit errors (``noiseless") during transmission.  A tug-of-war sketch of a bit array (packet) $b$
is comprised of a constant number $c$ of counters  ($c$ is determined by the desired error guarantees) that are maintained using the same update algorithm (with possibly different update values) and is sent to the receiver alongside with $b$.
After the execution of these update algorithms, each counter contains the inner product of the bit vector $\overrightarrow{b}$ (`0' converted to `-1' as discussed earlier) with a vector $\overrightarrow{s} \in \{+1, -1\}^n $  that is four-wise independent, as shown in the following algorithm.  Such four-wise independent vectors are known to exist and have computationally efficient representations (e.g., derivable from the Reed-Muller code~\cite{GilbertKMS03}).
Note the actual update algorithm is not shown here because it is not relevant to our context; Only its ``net effect" after execution is. 


\subsection{Set Reconciliation}\label{subsec:set-reconciliation}

Before we describe how to use tug-of-war for set reconciliation~\cite{Guo_SetReconciliationvia_2013,Mitzenmacher_SimpleMultiParty_2013,Eppstein_WhatsDifference?Efficient_2011}, we first give a brief 
description of set reconciliation. For two sets $A, B$ that contain elements from the same universe, $U$, the set reconciliation 
problem wants to compute the set difference $A \Delta B\triangleq (A\setminus B)\cup (B\setminus A)$. We denote $D=A\Delta B$, and 
$d=|D|$. In the context of set reconciliation, the two sets $A$ and $B$ are stored at two distinct places and the problem wants to 
compute $D$ with minimal communication overhead. 

First, we assume that $d$ is known a prior. We will show later how to use the tug-of-war sketch 
to estimate $d$, the size of 
the set difference. 
As shown in~\cite{Eppstein_WhatsDifference?Efficient_2011}, we can achieve 
$O(d)$ (with a small constant factor) 
communication overhead to compute the set difference $D$ using 
the invertible bloom filter (IBF)~\cite{Goodrich_InvertibleBloomLookup_2011,Eppstein_StragglerIdentificationRound_2011}, which is clearly (asymptotically) optimal. However, in the cases where each element is 
very large (in terms of communication requirement) such as large documents or movie chunks, it is a large communication overhead to transmit a small constant (say $2$ or $3$) times  $d$ elements. As we will show next, by using 
the tug-of-war sketch, we can reduce the communication overhead to very close to $d$ (elements) 
with a few rounds of message exchanges. 


We assume that the communication is initiated by $A$. 
Each round of communication works as follows. 
$A$ creates $m=\delta d$ buckets, $b_1,b_2,\dots,b_m$, 
where $\delta > 1$ is a constant. Each bucket $b_i$
contains a subset of elements from $A$, 
each of which is uniformly randomly selected (with properly-designed 
hash functions). 
For each bucket $b_i$, $A$ computes $c$ tug-of-war sketches, 
denoting as $z_{i,1},z_{i,2},\dots,z_{i,c}$. Note that here eahc $z_{i,j}=\sum_{a\in b_i}h(a)$, where 
$h$ is from a four-wise hash family that maps each element to $\pm 1$. 
Then, $A$ sends the $m\times c$ sketches 
to $B$. $B$ uses the same hash functions to create $m$ buckets for its elements, and then use the same hash 
functions to compute the tug-of-war sketches for each bucket, denoting those sketches as $z'_{i,j}$ for $i\in [m]$ and 
$j\in [c]$. Then, $B$ can use $\frac{1}{c}\sum_{j=1}^{c}(z_{i,j}-z'_{i,j})^2$ to estimate the size of (sub-)set difference of 
the bucket $b_i$ for any $i\in [m]$. Note that $B$ can use the median of mean approach in~\cite{AlonMS99} 
or the MLE estimator in~\cite{Hua_TowardsOptimalError_2012} to obtain 
better estimations. Then, for each bucket whose estimator is in $(0, 1.5)$ (just an example), $B$ sends the exclusive or of all the elements 
in the bucket to $B$. It is clear that if the true size of the set difference for the bucket is $1$, then $A$ can obtain the 
element belonging to $A\Delta B$ in the bucket. 

By repeating the process until all the $d$ elements are obtained, $A$ computes the set difference $D$.
\end{comment}
\begin{comment}
\medskip
\noindent
{\bf Analysis on Number of Rounds}.
Consider the whole process as a Markov chain, whose state is defined as the number of 
``hidden elements'' ({\it i.e.,} elements belonging to the set difference that are to be decoded). 
\autoref{fig:mc} presents the state transition diagram, denoting the corresponding transmission 
matrix as $P=\big{(}p_{i,j}\big{)}_{(d+1)\times (d+1)}$ where $p_{i,j}$ is the probability of moving from state $i$ to state $j$. It is complex to obtain all the elements in $P$, we 
can easily get the following probabilities, for any $k \leq d$,
\begin{align}
p_{k,0}&=\frac{\binom{m}{k}k\,!}{m^k} \\
p_{k,1}&=0 \\
p_{k,2}&=\frac{\binom{k}{2}(m-k+2)\binom{m}{k-2}(k-2)\,!}{m^k},\quad \forall k\geq 2\\
p_{k,3}&=\frac{\binom{k}{3}(m-k+3)\binom{m}{k-3}(k-3)\,!}{m^k},\quad \forall k\geq 3\\
p_{k,4}&=\frac{\big{(}\binom{k}{4}(m-k+4) + \binom{k}{2}\binom{k-2}{2}(m-k+4)(m-k+3)/2\big{)}\binom{m}{k-4}(k-4)\,!}{m^k},\quad \forall k\geq 4.
\end{align}
where $m$ is the number of buckets.

Similarly, we can calculate $p_{k,i}$ for any $k\geq i \geq 5$ but the expression gets more and more complex. 


It is not hard to check that the Markov chain described above is an absorbing Markov chain with 
a single absorbing state of $0$. By using the time to absorption theorem of Absorbing Markov Chains~\cite[Page 13]{Elizalde_LectureNotesMath_2006}, 
we can easily get the average number of rounds (steps before the chain is absorbed), which equals
the $d^{th}$ element of $(N{\bf 1})$ where the matrix 
$N=(I-Q)^{-1}$ is the fundamental matrix of $P$ (Note that $Q$ is the transition matrix for all transient states, in our case, is $P$ by removing the last row and column, {\it i.e.,} $P_{0,*}$ 
and $P_{*,0}$) and 
${\bf 1}$ is an all-one vector with length $d$. 

Denote $P^{(k)}$ as the $k$-step transition matrix, then the probability that it takes more than $n$ rounds to decode is
\begin{equation}
\mathbf{Pr}[t>n]=\sum_{k=n+1}^{\infty}p^{(k)}_{d,0},
\end{equation}
where $d$ is the initial number of elements.


\medskip
\noindent
{\bf Simplified Analysis on Number of Rounds.} In the following analysis, we assume that the number of buckets in the kth round, 
assuming remaining $d_k$ elements to be decoded, is set to be $\delta\cdot d_k$ where $\delta > 1$ is a constant. For ease of 
presentation, we drop the subscript $k$ in the following analysis\footnote{Inspired by the analysis of the number of iterations 
for PIM.}. 

Fix a bucket, the probability that it gets exactly one element belonging to the set difference that is not decoded yet is:
\begin{equation}
p = d \Big{(}\frac{1}{\delta d}\Big{)}\Big{(} 1 - \frac{1}{\delta d}\Big{)}^{d - 1} = \frac{1}{\delta}\Big{(} 1 - \frac{1}{\delta d}\Big{)}^{d - 1}\approx \frac{1}{\delta}e^{-1/\delta}.
\end{equation}

On average, there are $p$ fraction of buckets will get exact one element. Hence, on average $e^{-1/\delta}$ fraction of un-decoded 
elements will be decoded in each round. Therefore, on average, we need $\log_{\frac{1}{1- e^{-1/\delta}}}d_0$ rounds, {\it i.e.,} 
$O(\log d_0)$ rounds. 
\end{comment}

\section{Tail Bound Analysis and Parameter Settings}\label{sec:tail_bound}

In this section, we establish a tight tail bound on the {\it success probability} within $r$ rounds (defined in \autoref{subsec:protocol2}) under arbitrary parameter settings of $n$, $\delta$, and $t$. On one hand, this tail bound gives us a theoretical guarantee on the success probability under specific parameter settings. On the other hand, given a parameter setting requirement (i.e., a target success probability $p_0$ within $r$ rounds), we can use the tail bound to find all feasible parameter settings that satisfy the requirement, then select the optimal parameter settings among them that have the lowest communication overhead. {\bf This analysis also provides other theoretical results for PBS, such as the expected number (percentage) of the distinct elements would be reconciled in the each round (``piecewise decodability'', to be shown in \autoref{sec:piecewise_decodability})}%In this section, we continue to assume $d$ is precisely known. 

For simplicity, we ignore the small probability event that a type (\RN{2}) event happens and the ``fake'' distinct element is not successfully verified by \autoref{alg:verification} (mentioned in \autoref{subsec:exception_hash_partition}). As we discussed earlier, this event happens with a tiny probabilty that is in order of $10^{-7}$. Hence, ignoring these events barely compromises the accuracy of our analysis. 

% Motivated by parameter settings, we establish a strict tail bound on the {\it success probability} of PBS (i.e., all distinct elements are reconciled in $r$ rounds) as a function of parameters (i.e., $n$, $\delta$, $t$), which give us (1) a guideline on parameter settings; and (2) a theoretical guarantee about the success probability under selected parameters. 

% In this section, we still assume $d$ is precisely known. 
% For simplicity, we make the following two assumptions that hold with overwhelming probability in the analysis: First, the checksum (\autoref{step:terminate_condition} of \autoref{alg:single_round_pbs}) works perfectly on checking if the reconciliation is complete; Second, no ``fake'' distinct element fails to be checked by \autoref{alg:verification} (mentioned in \autoref{subsec:exception_hash_partition}) appears during reconciliation. 

% {\bf (to be finalized after the following subsections are finalized) We first establish a strict tail bound for a single group pair using Markov chain and Dynamic Programming in \autoref{sec:tail_bound_per_group}. Then we combine it with Times-2-Bound to get a strict tail bound for all group pairs in \autoref{sec:times2bound}. In \autoref{sec:parameter_settings}, we discuss the parameter settings using the tail bound. }

%In \autoref{sec:tail_bound_insufficient}, we remove the above BCH assumption and derive a more precise tail bound. {\bf need to decide whether to have this part or not, since we can easily set a relatively long BCH code, so that each group is decodable w.h.p.}

\subsection{Analysis of a simple case}\label{sec:single_markov}

In this section, we analyze the probability that an arbitrary group pair that contains exactly $x$ $(\leq t)$ distinct elements is completely reconciled (i.e., all distinct elements are successfully reconciled) by PBS in $r$ rounds.

As we described in \autoref{sec:multi-rounds}, in the first round of PBS, the $x$ distinct elements are hashed into $n$ subset pairs, and a distinct element is successfully reconciled if and only if it is hashed into a subset pair that contains only $1$ distinct element. 
%The successfully reconciled distinct elements in the first round are removed and the other distinct elements (i.e., the ones that have not been reconciled yet in the first round) will be hashed again in the second round using a different hash function, so on so force, until all distinct elements are successfully reconciled. 
How the $x$ distinct elements are distributed into $n$ subset pairs in the first round follows the familiar {\it balls-into-bins} probability model: Each of the $x$ balls is thrown independently and uniformly at random into one of the $n$ bins. Each successfully reconciled distinct element corresponds to a ball that ends up in a bin that receives exactly $1$ ball. We call the ball and the bin ``good'' in the sequel; each distinct element that has not been reconciled yet in the first round corresponds to a ball that ends up in a bin that receives multiple balls. We call the ball and the bin ``bad'' in the sequel. Note that balls are either ``good'' or ``bad'', but a bin could be empty besides being ``good'' and ``bad''. 

The ``bad'' balls in the first round will be the balls to be thrown in the second round. The ``bad'' balls in the second round will be the balls to be thrown in the third round, so on so force. In all rounds, how the balls are thrown into $n$ bins follows the same balls-into-bins probability model. Note that the balls are thrown using different hash functions in each round, so the number of ``bad'' balls in the $i$-th round
%(i.e., the number of balls to be thrown in the $(i+1)$-th round) 
only depends on how many balls are thrown in the $i$-th round and is independent of how these balls (``bad'' balls in the $(i-1)$-th round) are placed into the $n$ bins in the $(i-1)$-th round. Therefore, the number of balls to be thrown round after round is a Markov chain, in which each state is defined as the number of balls to be thrown. 
%Hence, the dynamics of the number of balls to be thrown in each round can be modeled as a Markov chain, in which each state is defined as the number of balls to be thrown. {\bf a little bit wordy, need advice on how to shrink it.}

In the Markov chain, a transition from state $i$ to state $j$ ($i\geq j$) means $i-j$ out of $i$ balls are ``good'' balls and the other $j$ balls are ``bad'' balls. The {\it absorbing state} of this Markov chain is state $0$, which is the ``good'' state that all balls are ``good'' (so that all distinct elements are successfully reconciled). For our analysis, the only probability that we are concerned with is $Pr[x\!\xrsquigarrow{r}\! 0]$, the probability that starting with state $x$ (initial state), the Markov chain reaches the absorbing state (i.e., state $0$) within $r$ transitions. It is also the success probability for a single group (starting with $x$ distinct elements and successfully reconciled within $r$ rounds), which can easily calculated given $M$, the $(t+1)\times (t+1)$ transition matrix of the Markov chain, as 
%, where $M(i,j)$ (i.e., the entry in the $i^{th}$ row and the $j^{th}$ column of $M$) is the probability of transition from state $i$ to state $j$ for $i,j = 0,1,...,t$
$\big{(}M^r\big{)}(x,0)$, the entry in the $x$-th row and the $0$-th column of $M^r$. Here we slightly abuse the row / column indices of a $(t+1)\times (t+1)$ matrix from $1,2,...,t+1$ to $0,1,...,t$, since the state of the Markov chain ranges from $0$ to $t$. How to compute $M$ will be elaborated in \autoref{sec:compute_M}. For the moment, we assume $M$ has been computed and therefore we can compute $Pr[x\!\xrsquigarrow{r}\! 0]$ for $x=1,2,...,t$, $r\in\mathbb{N}^+$. 

%The larger $n$ is, the larger percentage of the distinct elements will be reconciled in the first round.}
%The requirement above also ensures the majority of the distinct elements are reconciled in the first round, as we will show in \autoref{sec:piecewise_decodability}. Therefore, the majority of the overall communication overhead happens in the first round. In other words, the overall communication overhead of all rounds is only slightly larger than ($1.01$ to $1.07$ times of) that in the first round. Due to this reason, we use the communication overhead in the first round (described in \autoref{sec:communication_overhead_single_PBS}) to approximate the overall communication overhead of all rounds in parameter settings (to be elaborated in \autoref{sec:parameter_settings}.

\subsection{Tail Bound Analysis for Each Group Pair}\label{sec:tail_bound_per_group}

==========
{\bf The following may be useful in explaining why it is a Markov chain:} [Note there is no need to distinguish these four cases in calculating the ``transitioning out" probability (i.e., from state 6 to a small state say State 0), because the next round of balls-into-bins operation uses a different hash function independent of that used in the current round, and consequently how these 6 bad balls are split in the current round have no bearing on that in the next round.]  {\bf unless you have done so earlier}
==========

As we explained in \autoref{subsec:protocol2}, $\delta_1$, the number of distinct elements in group pair $1$, is a random variable that follows a Binomial distribution $Binomial(d,1/g)$. So the probability that group pair $1$ is successfully reconciled in $r$ rounds is $\sum_{x=0}^d Pr[\delta_1\!=\!x]\cdot Pr[x\!\xrsquigarrow{r}\! 0]$. 
%, where $\mathcal{B}(\cdot;d,1/g)$ is the probability mass function (PMF) of $Binomial(d,1/g)$. 
To ease computation, we slightly underestimate this probability by assuming $Pr[x\!\xrsquigarrow{r}\! 0]=0$ when $x>t$ (i.e., assume group pair $1$ cannot be reconciled if $\delta_1>t$, discussed in \autoref{sec:BCH_exception}). The loss of this underestimation is very tiny, since $Pr[\delta_1\!=\!x]$, the ``coefficient'' of $Pr[x\!\xrsquigarrow{r}\! 0]$, is very small when $x>t$. We denote this underestimated probability as $\alpha$ (i.e., $\alpha=\sum_{x=0}^t Pr[\delta_1\!=\!x]\cdot Pr[x\!\xrsquigarrow{r}\! 0]$), which is a tight tail bound of the success probability of group pair $1$. $\alpha$ is also a tight tail bound for all other group pairs, since $\delta_1,\delta_2,...,\delta_g$ follows the same distribution. $Pr[x\!\xrsquigarrow{r}\! 0]$ is a function of $n$ for given $x$ and $r$, so $\alpha=\alpha(n,t)$ is a function of $n$ and $t$ for arbitrary $d$, $r$, and $g$. 

\subsection{Tail Bound Analysis for All Group Pairs}\label{sec:times2bound}

Given $\alpha$, the tail bound of the probability that a group pair is successfully reconciled in $r$ rounds, we can easily derive a tail bound of $\alpha^g=1-(1-\alpha^g)$ for the probability that all group pairs are successfully reconciled in $r$ rounds ($1-\alpha^g$ is the failure probability, which is usually tiny), if we assume the reconciliations on group pairs are independent with each other. However, this assumption is not rigorous,
%since $d_1, d_2,...,d_g$ have a weak correlation that $\sum_{i=1}^g d_i=d$.
since $\delta_1, \delta_2,...,\delta_g$ are not strictly independent and have a relation that $\sum_{i=1}^g \delta_i=d$. 
%Fortunately, we have Times-2-Bound (Theorem 1 in \cite{hua2008rank}) to decouple the weak correlation and give us a rigorous tail bound of $1-2(1-\alpha^g)$ for the probability of all group pairs. 
However, we can use Corollary 5.11 in \cite{upfal2005probability} to
% decouple the weak correlation and 
obtain a rigorous tail bound of $1-2(1-\alpha^g)$ for the success probability of all group pairs. This rigorous tail bound is very tight and only doubles the tiny failure probability of the unrigorous tail bound: For example, if the unrigorous tail bound of the success probability of all group pairs is $0.9999$ ($0.0001$ failure probability), then the rigorous tail bound will be $0.9998$ ($0.0002$ failure probability). We use the tail bound of $1-2(1-\alpha^g)$ in parameter settings for rigorousness. 

\subsection{Parameter Settings}\label{sec:parameter_settings}

% The tail bound is based on the total number of distinct elements $d$, which is however not known precisely. The ToW Estimator introduced in \autoref{subsec:ToW} can only provide an estimation of $d$ (denoted as $\hat{d}$). Note that the tail bound of $Pr[P^{(r)}_o]$ increases as $d$ increases. So overestimate $d$ will get us a larger failure probability $Pr[P^{(r)}_o]$. To ensure a high success probability, we use an overestimated number of distinct element $\bar{d}$ $(>\hat{d})$ for parameter settings, such that $\bar{d}\geq d$ with high probability. In our evaluation, we set $\bar{d}\triangleq 1.38\hat{d}$, such that $\bar{d}\geq d$ with probability $99\%$. 

In this section, we elaborate how to set the parameters $n$, $t$, and $g$ given the target success probability $p_0$ within $r$ rounds (the probability that PBS successfully reconciles all distinct elements within $r$ rounds to be larger than $p_0$) in PBS. We continue to assume $d$ is precisely known. First, as explained in \autoref{subsec:protocol2}, $\delta$ should be a small number, so we fix $\delta=5$ and therefore $g=d/\delta$ is also fixed. 
Given the target success probability $p_0$ within $r$ rounds
%(i.e., set reconciliation is complete in $r$ rounds with probability $p_0$) 
%depend on the requirement of specific applications)
, the parameter setting problem aims to find the optimal parameter settings of $n,t$ that minimizes the overall communication overhead, under the constraint that the tail bound of the success probability of $r$ rounds is larger than $p_0$. Note that the overall communication overhead is only slightly larger than the communication overhead in the first round (to be explained in \autoref{sec:piecewise_decodability}), so we minimize the later instead of the former in the parameter setting problem. Furthermore, the later (i.e., the communication overhead in the first round) for each group pair (described in \autoref{sec:multi-rounds}) contains only two terms $t\log n+\delta\log n$ that depend on parameter settings. So we only need to minimize $t\log n+\delta\log n$ in the parameter setting problem, which can be formalized as the following optimization problem:

% \begin{equation}
% \min\limits_{n,t} t\log n+\delta\log n \quad \mbox{s.t.}\quad 1-2(1-\alpha^g(n,t))>p_0
% \end{equation}

\begin{align}
\mbox{minimize} \quad
&
t\log n+\delta\log n \nonumber
\\
\mbox{subject to} \quad 
&
1-2(1-\alpha^g(n,t))>p_0,\quad n,t\in \mathbb{N}^+ \nonumber
% \\
% &
% n,t\in \mathbb{N}^+ \label{eq:row_sum_requirement}
\end{align}

This optimization problem is not as daunting as it looks, since we can narrow down its solution space into only a few combinations and traverse all these combinations to find the optimal parameter settings as follows: First, since $n$ is the ``code length'' of BCH code, we select $n$ to be $2^m-1$ for some integer $m$ for BCH coding efficiency. Then the range of $n$ is narrowed down to $\{63,127,255,511,1023,2047\}$ (recall that $n=\Omega(\delta^2)$). Second, we select $t$ in the range from $1.5\delta$ to $3.5\delta$, since any smaller $t$ will cause a high probability of BCH decoding failure (explained in \autoref{subsec:protocol2}) and therefore a low success probability (below $50\%$), and any higher $t$ incurs significant additional communication overhead on transmitting BCH codeword (explained in \autoref{subsec:protocol2}) while barely increases the success probability.

% This optimization problem seems to be difficult to solve, since the constraint is a very comprehensive function of the parameters (remind that $\alpha=\alpha(n,t)$ is a function of $n$ and $t$ for arbitrary $r$, $d$, and $g$). However, we can narrow down the solution space into only a few combinations and traverse all these combinations to find the optimal parameter settings as follows: First, for BCH coding efficiency, we select $n$ to be $2^m-1$ for some integer $m$ and therefore narrow its range down to $\{63,127,255,511,1023\}$ (recall that $n=\Omega(\delta^2)$). Second, we select $t$ in the range from $1.5\delta$ to $3\delta$, as we suggested in \autoref{subsec:protocol2}. 

Here we use an example to show how we set parameters: Given $d=1000$ distinct elements, $r=3$ rounds, $p_0=99\%$, for each $(n,t)$ combination in $\{63,127,255,511,1023,2047\}\times \{8,9,...,16,17\}$, we compute the tail bound of the success probability under the parameter settings and obtain \autoref{tab:success_prob}.

\begin{table}[h]
\setlength{\tabcolsep}{3.2pt}
\centering
\caption{Tail bounds of the success probability under different parameter settings ($d=1000$, $r=3$)}\label{tab:success_prob}
\begin{tabular}{@{}|c|c|c|c|c|c|c|@{}}
\hline 
\diagbox{$t$}{$n$}    & $63$ & $127$ & $255$ & $511$ & $1023$ & $2047$ \\ \hline 
8   & 0 & 25.5\% & 32.7\% & 34.3\% & 34.9\% & 35.0\% \\ \hline
9   & 52.1\% & 78.0\% & 84.2\% & 85.7\% & 86.1\% & 86.2\% \\ \hline
10  & 75.1\% & 92.7\% & 96.5\% & 97.4\% & 97.6\% & 97.7\% \\ \hline
11  & 85.9\% & 96.9\% & \cellcolor{blue!25}99.1\% & \cellcolor{blue!25}99.5\% & \cellcolor{blue!25}99.6\% & \cellcolor{blue!25}99.6\% \\ \hline
12  & 91.3\% & 98.5\% & \cellcolor{blue!25}99.7\% & \cellcolor{blue!25}99.9\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% \\ \hline
13  & 93.9\% & \cellcolor{blue!60}99.1\% & \cellcolor{blue!25}99.8\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% \\ \hline
14  & 95.1\% & \cellcolor{blue!25}99.4\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% \\ \hline
15  & 95.6\% & \cellcolor{blue!25}99.5\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% \\ \hline
16  & 95.7\% & \cellcolor{blue!25}99.6\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% \\ \hline
17  & 95.8\% & \cellcolor{blue!25}99.6\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% \\ \hline
\end{tabular}
\end{table}

In \autoref{tab:success_prob}, all $(n,t)$ combinations in the highlighted cells satisfy the success probability requirement. Among them, $(127,13)$ has the lowest communication overhead (w.r.t. $t\log n+\delta\log n$). So we set $n=127, t=13$ in this case. For the case of the set difference cardinality $d$ is not precisely known, we use the scaled estimation of $d$ (described in \autoref{subsec:ToW}) for parameter settings. {\bf Note that calculating the probabilities in this table is very fast, since each entry in the table can be computed in $O(1)$ time given $M^r$, and $M^r$ for each $n\in\{63,127,255,511,1023,2047\}$ ($M$ is a function of $n$) can be precomputed in $O(t^3)$ time.}

{\bf (change r)} Note that for each possible target number of rounds $r$ (while keeping the same target success probability $p_0=99\%$), we can also compute a success probability table that is similar to \autoref{tab:success_prob} to obtain the corresponding optimal $n$ and $t$. 
%For example, when $r=1$, the optimal parameter setting is $n=524287$ and $t=16$; when $r=2$, the optimal parameter setting is $n=1023$ and $t=16$. 
The results are shown in \autoref{tab:vary_r} for $r=1,2,3,4$ ($p_0=99\%$). \autoref{tab:vary_r} also compares the {\it communication overhead per group pair} for each $r$, which accounts both the `constant' communication overhead that does not depend on the parameter settings (i.e., $\delta\log |\mathcal{U}|+32=192$ bits) and the `tunable' communication overhead that does depend on the parameter settings (i.e., the objective function $t\log n+\delta\log n$). The {\it communication overhead per distinct element}, which is simply equal to the communication overhead per group pair divided by $\delta$ (since each group pair contains $\delta$ distinct elements on average), is also compared in \autoref{tab:vary_r}. It shows that if we increase the target number of rounds $r$ while keeping the same target probability $p_0$ and therefore `loosen' the parameter setting requirement, the communication overhead (per distinct element) that is needed to achieve this requirement decreases. For instance, the communication overhead per distinct element is reduced by $32\%$ from $r=1$ to $r=2$, and that number from $r=2$ to $r=3$ and from $r=3$ to $r=4$ is $21\%$ and $10\%$ respectively. This ``saving'' on the communication overhead decreases as $r$ increases, so we set $r$ to the tune of $3$, which is a `sweet spot' that achieves the most ``saving'' on the communication overhead while not taking too many rounds to reconcile all distinct elements. 

\autoref{tab:vary_r} also shows that the optimal $n$ decreases as $r$ increases. Recall that the computational complexity per finite field operations in BCH decoding is $O(\log^2 n)$ (quadratic to the ``width" of the Galois field), which means the BCH decoding complexity also decreases as $r$ increases. Here $r=3$ is also a `sweet spot' that achieves the most `savings' on BCH decoding complexity (the complexity decreases as $O(19^2)\rightarrow O(10^2)\rightarrow O(7^2)\rightarrow O(6^2)$ when $r$ increases from $1$ to $4$). Note that the above analysis only shows that $r=3$ is a `sweet spot' when the target success probability is $p_0=99\%$. The `sweet spot' of $r$ could be different for various target success probabilities. However, we fix $r$ to be $3$ in our evaluation, since it is the `sweet spot' for the two target success probabilities to be used in our evaluation, which are $p_0=99\%$ and $p_0=99.58\%$ $(239/240)$, using the same analysis above.
%The communication overhead per group pair is $220$ bits, $210$ bits parameter settings when $r=3$ ($n=127, t=13$), this optimal parameter settings ($n=1023, t=16$) are much larger (more expensive) and incur additional communication overhead of $84$ bits per group pair. It shows that to achieve the same target success probability using fewer rounds (smaller $r$), PBS need more resources (e.g., larger $n$, $t$). Note that the optimal parameter settings when $r=1$ are even larger ($n=2047, t=15$) and incur even more additional communication overhead ($94$ bits comparing to the optimal parameter settings when $r=3$), which shows that running PBS for multiple rounds saves a considerate amount of communication overhead comparing to running PBS for only $1$ round when achieving the same target success probability.}

\begin{table}[h]
\centering
\caption{Vary $r$ ($p_0=99\%, d=1000$)}\label{tab:vary_r}
\begin{tabular}{@{}|c|c|c|c|c|@{}}
\hline 
$r$   & $1$ & $2$ & $3$ & $4$ \\ \hline 
Optimal $n$   & $524287$ & $1023$ & $127$ & $63$ \\ \hline
Optimal $t$   & $16$ & $16$ & $13$ & $11$ \\ \hline
\makecell{Objective function \\$t\log n+\delta\log n$}  & $399$ & $210$ & $126$ & $96$ \\ \hline
\makecell{Communication overhead \\per group pair (bits)}  & $591$ & $402$ & $318$ & $288$ \\ \hline
\makecell{Communication overhead \\per distinct element (bits)} & $118.2$ & $80.4$ & $63.6$ & $57.6$ \\ \hline
\end{tabular}
\end{table}

% Hidden table for d=10000
% \begin{table}[h]
% \centering
% \caption{Vary the target number of round $r$}\label{tab:vary_r}
% \begin{tabular}{@{}|c|c|c|c|@{}}
% \hline 
% $r$   & $1$ & $2$ & $3$ \\ \hline 
% Optimal $(n,t)$   & $(4096,14)$ & $(4095,17)$ & $(255,14)$ \\ \hline
% Objective function $t\log n+\delta\log n$  & $220$ & $210$ & $126$ \\ \hline
% Communication overhead per group pair (bits)  & $412$ & $402$ & $318$ \\ \hline
% Communication overhead per distinct element (bits) & $82.4$ & $80.4$ & $63.6$ \\ \hline
% \end{tabular}
% \end{table}

% {\bf (change r)} If we reduce the number of rounds $r$ from $3$ to $2$ while keeping the same target success probability $p_0=99\%$, we can also compute a success probability table that is similar to \autoref{tab:success_prob} to obtain the optimal parameter setting, which is $n=1023, t=16$. Compare to the previous optimal parameter settings when $r=3$ ($n=127, t=13$), this optimal parameter settings ($n=1023, t=16$) are much larger (more expensive) and incur additional communication overhead of $84$ bits per group pair. It shows that to achieve the same target success probability using fewer rounds (smaller $r$), PBS need more resources (e.g., larger $n$, $t$). Note that the optimal parameter settings when $r=1$ are even larger ($n=2047, t=15$) and incur even more additional communication overhead ($94$ bits comparing to the optimal parameter settings when $r=3$), which shows that running PBS for multiple rounds saves a considerate amount of communication overhead comparing to running PBS for only $1$ round when achieving the same target success probability.}

% {\bf Readers may think we can further increase $r$ (keeping the same target success probability) to reduce communication overhead. However, it could make PBS taking too many rounds to reconcile all distinct elements.} 
%Also, further increasing $r$ does not save much communication overhead. For example, if we increase $r$ from $3$ to $4$ (rounds), the optimal parameter setting becomes $n=63,t=11$, which only saves communication overhead of $30$ bits per group pair. }

\subsection{Analysis on ``Piecewise Decodability''}\label{sec:piecewise_decodability}

{\bf Note that PBS reconciles the distinct elements gradually round by round. The distinct elements that have been reconciled in the first round are no longer needed to be reconciled again and only the remaining distinct elements will be reconciled in the second round. This is the ``piecewise decodability'' mentioned in \autoref{sec:intro_oursolution}. Using the transition matrix $M$, we can theoretically analyze this ``piecewise decodability'' by computing the expected value of how many distinct elements would be reconciled in the each round as follows. 

Define $Z_i$ as the number of distinct elements that would be reconciled in the $i$-th round in an arbitrary group pair for $i=1,2,...$, and $X$ as the number of distinct elements in the group pair. $\mathbb{E}[Z_1|X=x]$, the expectation of $Z_1$ when the group pair contains exactly $x$ distinct elements, can be computed as $\sum_{y=0}^x y\cdot Pr[x\!\xrsquigarrow{1}\! y]$, where $Pr[x\!\xrsquigarrow{1}\! y]$ denotes the probability that starting with state $x$, the Markov chain reaches state $y$ in $1$ transition, which is equal to $M(x,y)$. Recall that $X$ follows the Binomial distribution $Binomial(d,1/g)$, we can compute $\mathbb{E}[Z_1]$ given $d$, $g$, and $n$. $\mathbb{E}[Z_2]$, $\mathbb{E}[Z_3]$, ..., can also be computed (e.g., $\mathbb{E}[Z_2]$ can be computed based on $\mathbb{E}[Z_1+Z_2|X=x]=\sum_{y=0}^x y\cdot Pr[x\!\xrsquigarrow{2}\! y]$ and $\mathbb{E}[Z_1]$, where $Pr[x\!\xrsquigarrow{2}\! y]=\big{(}M^2\big{)}(x,y)$). We omit the details about the computation and only show results of the expected percentage of distinct elements are reconciled in each round (i.e., $Z_1/\delta$, $Z_2/\delta$, $Z_3/\delta$, and $Z_4/\delta$) under the optimal parameter settings above when $r=3$ and $p_0=0.99$ ($d=1000$, $g=200$, $n=127$, $t=13$) in \autoref{tab:reconcile_ratio}.
} %% added by long to prevent the all-bold issue
% Using the transition matrix $M$, we can compute the expected value of how many distinct elements are reconciled in each round. 
% From the transition matrix $M$, we can theoretically analyze this ``piecewise decodability'' by computing the expected value of how many distinct elements are reconciled in the each round. 
% $\mathbb{E}[Z|X=x]=\sum_{y=0}^x y\cdot Pr[x\!\xrsquigarrow{1}\! y]=\sum_{y=0}^x y\cdot M(x,y)$
% For example, $\sum_{l=0}^x l\cdot Pr[x\!\xrsquigarrow{1}\! l]$ is the average number of the distinct elements that are reconciled in the first round (for an arbitrary group pair with $x$ distinct elements). 
% Although this expected value in any scenario (given $d$, $n$, and $t$) is computable, we only show the `general' results in \autoref{tab:reconcile_ratio}, in which we assume $\delta_1,\delta_2,...,\delta_g$ follow the Poisson distribution with mean of $\delta$ (this is a tiny approximation for relatively large $d$, since the Poisson distribution is a limiting case of the Binomial distribution with the same expectation), and $t$ is sufficiently large. }
\begin{table}[h]
\centering
\caption{The expected percentage of the distinct elements would be reconciled in each round}\label{tab:reconcile_ratio}
\begin{tabular}{@{}|c|c|c|c|@{}}
\hline 
Round $1$ & Round $2$ & Round $3$ & Round $4$ \\ \hline 
0.962 & 0.0380 & $3.61\times 10^{-4}$ & $2.86\times 10^{-6}$ \\ \hline
% $127$  & 0.961 & 0.0382 & $3.7\times 10^{-4}$ & $2.9\times 10^{-6}$ \\ \hline
% $255$  & 0.981 & 0.0193 & $8.4\times 10^{-5}$ & $3.3\times 10^{-7}$ \\ \hline
% $511$ & 0.990 & 0.00972 & $2.0\times 10^{-5}$ & $3.9\times 10^{-8}$ \\ \hline
% $1023$ & 0.995 & 0.00487 & $4.9\times 10^{-6}$ & $4.8\times 10^{-9}$ \\ \hline
% \begin{table}[h]
% \centering
% \caption{Average percentage of distinct elements are reconciled per round}\label{tab:reconcile_ratio}
% \begin{tabular}{@{}|c|c|c|c|c|@{}}
% \hline 
% $n$   & Round $1$ & Round $2$ & Round $3$ & Round $4$ \\ \hline 
% $63$   & 0.924 & 0.0746 & $1.7\times 10^{-3}$ & $2.7\times 10^{-5}$ \\ \hline
% $127$  & 0.961 & 0.0382 & $3.7\times 10^{-4}$ & $2.9\times 10^{-6}$ \\ \hline
% $255$  & 0.981 & 0.0193 & $8.4\times 10^{-5}$ & $3.3\times 10^{-7}$ \\ \hline
% $511$ & 0.990 & 0.00972 & $2.0\times 10^{-5}$ & $3.9\times 10^{-8}$ \\ \hline
% $1023$ & 0.995 & 0.00487 & $4.9\times 10^{-6}$ & $4.8\times 10^{-9}$ \\ \hline
% $63$   & 0.924 & 0.0746 & 0.00167 & 0.0000274 \\ \hline
% $127$   & 0.961 & 0.0382 & 0.000365 & 0.00000289 \\ \hline
% $255$  & 0.981 & 0.0193 & 0.0000839 & 0.000000330 \\ \hline
% $511$ & 0.990 & 0.00972 & 0.0000200 & 0.0000000392 \\ \hline
% $1023$ & 0.995 & 0.00487 & 0.00000489 & 0.00000000478 \\ \hline
% \begin{tabular}{@{}|c|c|c|c|c|c|c|@{}}
% \hline 
% \diagbox{$r$}{$n$}    & $63$ & $127$ & $255$ & $511$ & $1023$ & $2047$ \\ \hline 
% 1   & 92.4\% & 96.1\% & 98.1\% & 99.0\% & 99.5\% & 99.8\% \\ \hline
% 2   & 7.46\% & 3.82\% & 1.93\% & 0.97\% & 0.49\% & 0.24\% \\ \hline
% 3  & $1.7\times 10^{-3}$ & $3.7\times 10^{-4}$ & $8.4\times 10^{-5}$ & $2.0\times 10^{-5}$ & $4.9\times 10^{-6}$ & $1.2\times 10^{-6}$ \\ \hline
% 4  & $2.7\times 10^{-5}$ & $2.9\times 10^{-6}$ & $3.3\times 10^{-7}$ & $3.9\times 10^{-8}$ & $4.8\times 10^{-9}$ & $5.9\times 10^{-10}$ \\ \hline
\end{tabular}
\end{table}

{\bf \autoref{tab:reconcile_ratio} shows that the majority of the distinct elements ($96.2\%$) are reconciled in the first round. Therefore, the communication overhead (roughly proportional to the number of distinct elements that are reconciled) in the first round is the major part of the overall communication overhead.}  
%In other words, the overall communication overhead of all rounds is only slightly larger than that in the first round. 
Due to this reason, we use the communication overhead in the first round (described in \autoref{sec:communication_overhead_single_PBS}) to approximate the overall communication overhead of all rounds in parameter settings in \autoref{sec:parameter_settings}. {\bf \autoref{tab:reconcile_ratio} also shows that the number of remaining distinct elements (the ones that have not been reconciled) decreases exponentially round after round. }

\subsection{How to compute \texorpdfstring{\larger\boldmath{$M$}}{M}}\label{sec:compute_M}

In this section, we describe how to compute the transition matrix $M$ in details. Note that calculating an arbitrary transition probability $M(i,j)$ is not straightforward, since each state $j$ (after-transition state) with $j>3$ in the Markov chain is a {\it composite state}, which consists of a huge number of {\it atom states}. 
%The transition probability $M(i,j)$ is basically the summation of all transition probabilities from the (pre-transition) state $i$ to each of the atom states of state $j$. 

Each composite state $j$ can be broken down into atom states as follows.  Each simple state is, in combinatorics terms, {\it a permutation of a combination of $j$}, which here corresponds to how these $j$ balls are placed into the $n$ bins.  For a simple example, when $j = 4$ and $n = 7$, the vector $(2, 0, 0, 0, 0, 2, 0)$ is such a simple state, which corresponds to these $7$ bins (in a predefined order such as the natural order) have $2, 0, 0, 0, 0, 2,$ and $0$ ``bad'' balls in it respectively. The transition probability from the (pre-transition) state $i$ to any atom state of state $j$ can be directly computed, and $M(i,j)$ is basically the summation of all these transition probabilities. The problem is that the number of atom states (permutations of combinations) grow exponentially with the number of balls $j$. 
%To obtain $M(i,j)$, we have to compute all transition probabilities from the (pre-transition) state $i$ to each of the atom states of state $j$ and sum them up. 

We overcome this problem by grouping the huge number of atom states into a smaller number of coarse-grained sub-states first, then computing the transition probability from the (pre-transition) state $i$ to any sub-states of state $j$. Although each sub-state still consists of many atom states and the transition probability to a sub-state is still hard to compute directly, we discover a recurrence relation among these transition probabilities, so we can compute them using Dynamic Programming.



%as far as the calculation of the transition probability from a (larger) state $i$ $(>j)$ to $j$ is concerned. 
% To calculate the probability, we have to break the composite state $j$ down into ``atom'' states, calculate the transition probability from state $i$ to each of the ``atom'' states (which can be directly calculated), and then add them up. {\bf Note that we always view state $i$ (pre-transition state) as a {\it simple state}, since how the $i$ balls are placed into $n$ bins only depends on the hash function.}

% Each composite state $j$ can be broken down into atom states based on how these $j$ bad balls are placed into the $n$ bins. For example, state $6$ consists of $4$ atom states. The first one is $6 = 6$, where all $6$ bad balls are in the same bad bin. The second one is $6 = 2 + 4$ where, out of the $6$ bad balls, four are in one bad bin and the other two are in the other bad bin.  Similarly, the other two atom states are $6 = 3 + 3$ and $6 = 2 + 2 + 2$. The transition probability from state $i$ to any atom state can be directly calculated, but the problem is that the number of atom states grows exponentially with the number of ``bad'' balls $j$.

% We notice that we can break each composite state into a small number of coarse-grained sub-states, each of which may still contain a large number of atom states. The transition probability from a (larger) state $i$ to any sub-state is still hard to compute. However, there is a recurrence relation among them, so we can compute the transition probabilities from any state to any sub-state using Dynamic Programming. 

The sub-states of state $j$ is defined as follows: let state $(j,k)$ denote the sub-state of state $j$ that the $j$ ``bad'' balls end up to occupy exactly $k$ ``bad'' bins. Then the composite state $j$ is partitioned into state $(j,1)$, state $(j,2)$, $...$, state $(j,j)$. We slightly abuse the notation and let $M(i,j,k)$ denote the probability of transition from state $i$ to state $(j,k)$, then we have 

\begin{equation}\nonumber
    M(i,j) = \sum_{k=1}^{j} M(i,j,k)
\end{equation}

%{\bf explain the range of $k$ could be distracting, so I just leave it as it is.}
To obtain $M$, it is sufficient to compute $M(i,j,k)$ for $\forall i,j,k=0,1,...,t$. Note that the state transition resulting from throwing one ball after another is also a Markov chain, in which state $(i,j,k)$ is defined as $j$ ``bad'' balls ending up into $k$ ``bad'' bins after throwing $i$ balls into $n$ bins. In this Markov chain, throwing one more ball can transition state $(i,j,k)$ to three possible states depending on the $(i+1)$-th ball ending up in (1) a ``good'' bin; (2) a ``bad'' bin; or (3) an empty bin. The first case happens with probability $(i-j)/n$, results in $2$ additional ``bad'' balls and $1$ additional ``bad'' bin (i.e., transition to state $(i+1,j+2,k+1)$). The second and third cases transition to state $(i+1,j+1,k)$ and state $(i+1,j,k)$ respectively with probability $k/n$ and $1-(i-j+k)/n$. In the opposite direction, state $(i+1,j,k)$ can only be transitioned from (1) state $(i,j-2,k-1)$; (2) state $(i,j-1,k)$; and (3) state $(i,j,k)$, which gives us a recurrence relation that $M(i+1,j,k)$ equals to

%The second case happens with probability $k/n$ and results in state $(i+1,j+1,k)$. The third case happens with probability $1-(i-j+k)/n$ and results in state $(i+1,j,k)$. In the opposite direction, state $(i+1,j,k)$ can be transitioned from (1) state $(i,j-2,k-1)$ with probability $(i-j+2)/n$; (2) state $(i,j-1,k)$ with probability $k/n$; or (3) state $(i,j,k)$ with probability $1-(i-j+k)/n$. It gives us a recurrence relation that $P(i+1,j,k)$ equals to

\begin{equation}\nonumber
    \frac{i\!-\!j\!+\!2}{n}\cdot M(i,j\!-\!1,k\!-\!1)+\frac{k}{n}\cdot M(i,j\!-\!1,k)+(1\!-\!\frac{i\!-\!j\!+\!2}{n})\cdot M(i,j,k)
\end{equation}

The three terms in this formula corresponds to the above three possible transitions. To compute $M(i,j,k)$ for $\forall i,j,k=0,1,...,t$ via Dynamic Programming, the total computational complexity is $O(t^3)$ ($O(1)$ for $t^3$ entries), and we also need to compute the transition probabilities in the base cases as follows:  
%Combining with the following probabilities in base cases, we can compute $M(i,j,k)$ for $\forall i,j,k=0,1,...,t$ using Dynamic Programming and obtain $M$:

\begin{align}
M(0,j,k) =& \left\{ \begin{array}{ccl}
1, & \mbox{if }
 j=k=0 \\ 0, & \mbox{otherwise} 
\end{array}\right.\nonumber\\
M(i,0,k) =& \left\{ \begin{array}{ccl}
\binom{n}{i}/n^i, & \mbox{if }
 k=0 \\ 0, & \mbox{otherwise} 
\end{array}\right.\nonumber\\
M(i,j,0) =& \left\{ \begin{array}{ccl}
1, & \mbox{if }
 j=0 \\ 0, & \mbox{otherwise} 
\end{array}\right.\nonumber
\end{align}

% PBS reconciles the distinct elements gradually round by round. This is the ``piecewise decodability'' mentioned in \autoref{sec:intro_oursolution}. We use the following example to describe it in details: 
% Given two sets with $10$ distinct elements, in the first round, PBS tries to reconcile the $10$ distinct elements and say $6$ out of the $10$ distinct elements are successfully reconciled. Then the $6$ reconciled distinct elements are removed and PBS tries to reconcile the remaining $4$ distinct elements in the second round. Say $2$ out of the $4$ remaining distinct elements are successfully reconciled, and that leaves $2$ remaining distinct elements to be reconciled in the third round, so on so force. 
% % Given two sets $A$, $B$ with $10$ distinct elements, in the first round, PBS hashes them into $7$ distinct subset pairs. $6$ distinct elements are hashed into $6$ distinct subset pairs, and the other $4$ distinct elements are hashed into the same subset pair. Then the former $6$ distinct elements are successfully reconciled in the first round and the later $4$ distinct elements remain to be reconciled in the second round, which are hashed into $3$ distinct subset pairs (under a different hash function). $2$ remaining distinct elements are hashed into $2$ distinct subset pairs, and the other $2$ remaining distinct elements are hashed into the same subset pair. Then the former $2$ remaining distinct elements are successfully reconciled in the second round and the later $2$ remaining distinct elements remain to be reconciled in the third round, so on so force. 
% The dynamics of the number of remaining distinct elements (i.e., $10\leadsto 4\leadsto 2\leadsto \cdots$ in the example) is in nature a Markov chain, which will be elaborated and analyzed in \autoref{sec:single_markov} to derive a tight tail bound of the probability that all distinct elements are reconciled in $r$ rounds. 

+++++++++++

The only problem left to obtain $Pr[d\xrsquigarrow{r} 0]$ is how to compute $M$, which is not straightforward, since each state $j$ with $j>3$ in the Markov chain is a composite state as far as the calculation of the transition probability from a (larger) state $i$ $(>j)$ to $j$ (i.e., ``transitioning into'') is concerned.   {\bf You need to explain why it is not straightforward:  The reason you offer is not
the direction reason.  Instead you may say that "the transition probability between these composite states cannot be directly calculated" ...  to calculate it we have to break it down into "atom" states}

Each composite state $i$ can be broken down into atom states as follows.  Each simple state is, in combinatorics terms, {\it a permutation of a combination of $i$}, which here corresponds to 
how these $i$ balls are ``divided up" by the $n$ bins.   {\bf Liang, Read Mitzenmacher and Upfal book
for a better word for "divided up"}
For a simple example, when $i = 4$ and $n = 7$, the vector (1, 0, 1, 0, 0, 2, 0) is such a simple state, which corresponds to these 7 bins (in a predefined order such as the natural order) 
have 1, 0, 1, 0, 0, 2, and 0 balls in it respectively.   The transition probability between any two atom states can be ...    but the problem is that the number of atom states 
(permutations of combinations) grow exponentially with the number of balls $i$.

Consider two states i1 and i2 each broken down into millions of atom states.  Then the transition probability between these states is the summation of the trillions (= millions * millions) of 
transition probabilities between atom states of i1 and atom states of i2.  

The good thing is that the transition probability matrix among the (humongous number of atom states) induces a "subproblem structure ????", which leads to the recurrence relation, 
dynamic programming.   

We notice that we can break each state into a small number of coarse-grained substates, each of which may still contain a large number of atom states.  The transition probability 
between any two such substates are still hard to compute.  However, there is a recurrence relation among them ...

+++++++++++

To solve the problem, we partition the composite state into sub-states, so that the transition probability to the composite state is the summation of the transition probabilities to each of the sub-states. On the other hand, the transition probabilities to the sub-state have a recurrence relation and can be computed using Dynamic Programming. 

============================

Note that every state $j$ with $j > 3$ in the Markov chain is a composite state as far as the calculation of the transition probability from a (larger) state $i > j$ to $j$ (i.e., ``transitioning into").  For example, State 6 contains 4 different cases. The first case is $6 = 6$, where all 6 bad balls are in the same bad bin. The second case is $6 = 2 + 4$ where, out of the 6 bad balls, four are in one bad bin and the other two are in the other bad bin.  Similarly, the other two cases are $6 = 3 + 3$ and $6 = 2 + 2 + 2$. Note there is no need to distinguish these four cases in calculating the ``transitioning out" probability (i.e., from state 6 to a small state say State 0), because the next round of balls-into-bins operation uses a different hash function independent of that used in the current round, and consequently how these 6 bad balls are split in the current round have no bearing on that in the next round. 

Building on the example above, we now consider $m_{9,6}$, the transition probability from State $9$ to State $6$ (throwing 9 balls into 255 bins and ending up with 6 bad balls).  $m_{9,6}$ is simply the sum of the probabilities of these four cases, each of which has a very different formula than the others.  In general, the number of such cases, and hence the number of individual probability terms to be added up to arrive at the transition matrix element $m_{i,j}$, grows exponentially with the value of $j$. This does not however make it difficult to calculate the values of $M$, because there is a recursive structure, among the values of the matrix elements $m_{i,j}$, that can be exploited using dynamic programming, as will be elaborated shortly.

To simplify our analysis, we split each composite state into sub-composite states based on the number of nonempty bins: Let State $(j,k)$ denotes the sub-composite state with $j$ remaining distinct elements and $k$ nonempty bins, which is also a substate of State $j$. Let $m_{i,j}^{(k)}$ denote the probability of transition from State $i$ to State $(j,k)$, which is also the probability that after throwing $i$ balls uniformly and independently into $n$ bins, $i-j$ bins are ``good'' bins and $k$ bins are nonempty bins (thus $k-(i-j)$ bins are ``bad'' and $n-k$ bins are empty). The probability of transition to a composite state is simply the summation of the probabilities of the transitions to corresponding sub-composite states:

To obtain the transition matrix $M$, it is sufficient to compute $m^{(k)}_{i,j}$, which can be exploited using dynamic programming. Note that the balls-and-bins model itself can be considered as a Markov chain, in which a recursive relation exists: After throwing $i$ balls into $n$ bins, throwing one more ball randomly could be: (1) Into an empty bin and turn it to a ``good'' bin; (2) Into a ``good'' bin and turn it to a ``bad'' bin with two balls; or (3) Into a ``bad'' bin and keep it as the same. Mathematically, we have $m^{(k)}_{i+1,j}$ equals to


====================================


%{\bf (may be unnecessary) Note that both the success probability and the overall communication overhead are strictly increasing w.r.t. $n$ and $t$. Hence, instead of computing all values in the table, we could strategically compute only a few of them and obtain the optimal $(n,t)$ (e.g., find the optimal $t$ for each $n$ by binary search each column).}





\begin{comment}

As we explained in \autoref{subsec:protocol2}, $d_1$, the number of distinct elements in group pair $1$, is a random variable that follows a Binomial distribution $Binomial(d,1/g)$. So the probability that the group pair is completely reconciled in $r$ rounds is $\sum_{x=0}^d Pr[d_1=x]\cdot Pr[x\xrsquigarrow{r} 0]$.
%, where $\mathcal{B}(\cdot;d,1/g)$ is the probability mass function (PMF) of $Binomial(d,1/g)$. 
To ease computation, we slightly underestimate this probability by assuming $Pr[x\xrsquigarrow{r} 0]=0$ when $x>t$ (i.e., assume group pair $1$ cannot be reconciled if $d_i>t$, discussed in \autoref{sec:BCH_exception}). The loss of this underestimation is very tiny, since the coefficient of $Pr[x\xrsquigarrow{r} 0]$ (i.e., $Pr[d_1=x]$) is very small when $x>t$. We denote this underestimated probability as $\alpha$ (i.e., $\alpha=\sum_{x=0}^t Pr[d_1=x]\cdot Pr[x\xrsquigarrow{r} 0]$). Note that $Pr[x\xrsquigarrow{r} 0]$ is a function of $n$ and $r$ for arbitrary $x$, so $\alpha$ is a function of $n$, $r$, $t$ for arbitrary $d$ and $g$. 


\subsection{Tail Bound Analysis for Each Group Pair}\label{sec:tail_bound_per_group}

In this section, we focus on analyzing an arbitrary group pair, which we denote as $(A',B')$, and suppose their set difference $A'\Delta B'$ contains exactly $x$ elements. We only consider the case that the error-correct capability is sufficient (i.e., $x\leq t$). As we described in \autoref{sec:multi-rounds}, the $x$ distinct elements are hashed into $n$ subset pairs in the first round, and a distinct element is reconciled if and only if it is hashed into a subset pair that contains only $1$ distinct element. The distinct elements that have been reconciled in the first round are removed and the other distinct elements (i.e., the ones that have not been reconciled yet in the first round) will be hashed again in the second round using a different hash function, so on so force. 


% WLOG, we only analyze group pair $1$. {\bf Maybe say that we focus on an arbitrary group pair, which we denote as A' and B', and suppose their difference $ ... $ contains exactly $x$ elements}. 
% %The analysis for other group pairs is the same. 
% {\bf Please use x, not d}.  
% For the moment, we slightly abuse the notation and use $d$ to denote the number of distinct elements in group pair $1$ (i.e., $d_1$). In this section, we only consider the case that the error-correct capability is sufficient (i.e., $d\leq t$). As we described in \autoref{sec:multi-rounds}, the $d$ distinct elements of group pair $1$ are hashed into $n$ subset pairs in the first round, and a distinct element is reconciled if and only if it is hashed into a subset pair that contains only $1$ distinct element. The distinct elements that have been reconciled in the first round are removed and the other distinct elements (i.e., the ones that have not been reconciled yet in the first round) will be hashed again in the second round using a different hash function, so on so force. 

==========
{\bf The following may be useful in explaining why it is a Markov chain:} [Note there is no need to distinguish these four cases in calculating the ``transitioning out" probability (i.e., from state 6 to a small state say State 0), because the next round of balls-into-bins operation uses a different hash function independent of that used in the current round, and consequently how these 6 bad balls are split in the current round have no bearing on that in the next round.]  {\bf unless you have done so earlier}

{\bf we have an example at the end of multi-round PBS}
==========


As we explained in \autoref{sec:hash_partition}, how the $x$ distinct elements are distributed into $n$ subset pairs in the first round follows the familiar {\it balls-into-bins} probability model: Each of the $x$ balls are thrown independently and uniformly at random into one of the $n$ bins. Each distinct element that is reconciled in the first round corresponds to a ball that ends up in a bin that receives exactly $1$ ball. We call the ball and the bin ``good'' in the sequel; Each distinct element that has not been reconciled yet in the first round corresponds to a ball that ends up in a bin that receives multiple balls. We call the ball and the bin ``bad'' in the sequel. Note that balls are either ``good'' or ``bad'', but bins could be empty besides ``good'' and ``bad''.



The ``bad'' balls in the first round will be the balls to be thrown in the second round. The ``bad'' balls in the second round will be the balls to be thrown in the third round, so on so force. In all rounds, how the balls are thrown into $n$ bins follows the balls-into-bins model. The dynamics of the number of balls to be thrown in each round can be modeled as a Markov chain, in which each state is defined as the number of balls to be thrown. In the Markov chain, a transition from state $i$ to state $j$ ($i\geq j$) means $i-j$ out of $i$ balls are ``good'' balls and the other $j$ balls are ``bad'' balls. The {\it absorbing state} of this Markov chain is state $0$, which is the ``good'' state that means all distinct elements have been reconciled (i.e., reconciliation is complete). For our analysis, the only probability that we concerned is $Pr[x\xrsquigarrow{r} 0]$, the probability that state $x$ (initial state) reaches the absorbing state (i.e., state $0$) in $r$ transitions, which is also the probability that all distinct elements are reconciled in $r$ rounds. This probability can be easily calculated given the transition matrix of the Markov chain: Let $M$ denote the $(t+1)\times (t+1)$ transition matrix of the Markov chain.
%, where $M(i,j)$ (i.e., the entry in the $i^{th}$ row and the $j^{th}$ column of $M$) is the probability of transition from state $i$ to state $j$ for $i,j = 0,1,...,t$
$Pr[x\xrsquigarrow{r} 0]$ equals to $\big{(}M^r\big{)}(x,0)$ (i.e., the entry in the $x^{th}$ row and the $0^{th}$ column of $M^r$). Here we slightly abuse the row / column numbers of a $(t+1)\times (t+1)$ matrix from $1,2,...,t+1$ to $0,1,...,t$, since the state of the Markov chain ranges from $0$ to $t$. 

\subsubsection{How to compute \texorpdfstring{$M$}{M}}

The only problem left to obtain $Pr[x\xrsquigarrow{r} 0]$ is how to compute $M$, which is not straightforward, since each state $j$ (after-transition state) with $j>3$ in the Markov chain is a composite state as far as the calculation of the transition probability from a (larger) state $i$ $(>j)$ to $j$ is concerned. To calculate the probability, we have to break state $j$ down into ``atom'' states, calculate the transition probability from state $i$ to each of the ``atom'' states (which can be directly calculated), and then add them up. {\bf Note that we always view state $i$ (pre-transition state) as a simple state, since how the $i$ balls are placed into $n$ bins only depends on a hash function that is independent of the ones used in previous rounds.}

Each composite state $j$ can be broken down into atom states based on how these $j$ bad balls are placed into the $n$ bins. For example, state $6$ consists of $4$ atom states. The first one is $6 = 6$, where all $6$ bad balls are in the same bad bin. The second one is $6 = 2 + 4$ where, out of the $6$ bad balls, four are in one bad bin and the other two are in the other bad bin.  Similarly, the other two atom states are $6 = 3 + 3$ and $6 = 2 + 2 + 2$. The transition probability from state $i$ to any atom state can be directly calculated, but the problem is that the number of atom states grows exponentially with the number of ``bad'' balls $j$.

We notice that we can break each composite state into a small number of coarse-grained sub-states, each of which may still contain a large number of atom states. The transition probability from a (larger) state $i$ to any sub-state is still hard to compute. However, there is a recurrence relation among them, so we can compute the transition probabilities from any state to any sub-state using Dynamic Programming. 




% Each ``atom'' state is, in combinatorics terms, {\it a permutation of a combination of $j$}, which here corresponds to 
% how these $j$ ``bad'' balls are placed into the $n$ bins. 
% For a simple example, when $j = 4$ and $n = 7$, the vector $(2, 0, 0, 0, 0, 2, 0)$ is such an ``atom'' state, which corresponds to these $7$ bins (in a predefined order such as the natural order) 
% have $2$, $0$, $0$, $0$, $0$, $2$, and $0$ ``bad'' balls in it respectively. The transition probability from state $i$ to any atom state can be calculated, but the problem is that the number of atom states 
% (permutations of combinations) grow exponentially with the number of balls $j$.


+++++++++++

The only problem left to obtain $Pr[d\xrsquigarrow{r} 0]$ is how to compute $M$, which is not straightforward, since each state $j$ with $j>3$ in the Markov chain is a composite state as far as the calculation of the transition probability from a (larger) state $i$ $(>j)$ to $j$ (i.e., ``transitioning into'') is concerned.   {\bf You need to explain why it is not straightforward:  The reason you offer is not
the direction reason.  Instead you may say that "the transition probability between these composite states cannot be directly calculated" ...  to calculate it we have to break it down into "atom" states}

Each composite state $i$ can be broken down into atom states as follows.  Each simple state is, in combinatorics terms, {\it a permutation of a combination of $i$}, which here corresponds to 
how these $i$ balls are ``divided up" by the $n$ bins.   {\bf Liang, Read Mitzenmacher and Upfal book
for a better word for "divided up"}
For a simple example, when $i = 4$ and $n = 7$, the vector (1, 0, 1, 0, 0, 2, 0) is such a simple state, which corresponds to these 7 bins (in a predefined order such as the natural order) 
have 1, 0, 1, 0, 0, 2, and 0 balls in it respectively.   The transition probability between any two atom states can be ...    but the problem is that the number of atom states 
(permutations of combinations) grow exponentially with the number of balls $i$.

Consider two states i1 and i2 each broken down into millions of atom states.  Then the transition probability between these states is the summation of the trillions (= millions * millions) of 
transition probabilities between atom states of i1 and atom states of i2.  

The good thing is that the transition probability matrix among the (humongous number of atom states) induces a "subproblem structure ????", which leads to the recurrence relation, 
dynamic programming.   

We notice that we can break each state into a small number of coarse-grained substates, each of which may still contain a large number of atom states.  The transition probability 
between any two such substates are still hard to compute.  However, there is a recurrence relation among them ...

+++++++++++

To solve the problem, we partition the composite state into sub-states, so that the transition probability to the composite state is the summation of the transition probabilities to each of the sub-states. On the other hand, the transition probabilities to the sub-state have a recurrence relation and can be computed using Dynamic Programming. 

======================================

Note that every state $j$ with $j > 3$ in the Markov chain is a composite state as far as the calculation of the transition probability from a (larger) state $i > j$ to $j$ (i.e., ``transitioning into").  For example, State 6 contains 4 different cases. The first case is $6 = 6$, where all 6 bad balls are in the same bad bin. The second case is $6 = 2 + 4$ where, out of the 6 bad balls, four are in one bad bin and the other two are in the other bad bin.  Similarly, the other two cases are $6 = 3 + 3$ and $6 = 2 + 2 + 2$. Note there is no need to distinguish these four cases in calculating the ``transitioning out" probability (i.e., from state 6 to a small state say State 0), because the next round of balls-into-bins operation uses a different hash function independent of that used in the current round, and consequently how these 6 bad balls are split in the current round have no bearing on that in the next round. 

Building on the example above, we now consider $m_{9,6}$, the transition probability from State $9$ to State $6$ (throwing 9 balls into 255 bins and ending up with 6 bad balls).  $m_{9,6}$ is simply the sum of the probabilities of these four cases, each of which has a very different formula than the others.  In general, the number of such cases, and hence the number of individual probability terms to be added up to arrive at the transition matrix element $m_{i,j}$, grows exponentially with the value of $j$. This does not however make it difficult to calculate the values of $M$, because there is a recursive structure, among the values of the matrix elements $m_{i,j}$, that can be exploited using dynamic programming, as will be elaborated shortly.

To simplify our analysis, we split each composite state into sub-composite states based on the number of nonempty bins: Let State $(j,k)$ denotes the sub-composite state with $j$ remaining distinct elements and $k$ nonempty bins, which is also a substate of State $j$. Let $m_{i,j}^{(k)}$ denote the probability of transition from State $i$ to State $(j,k)$, which is also the probability that after throwing $i$ balls uniformly and independently into $n$ bins, $i-j$ bins are ``good'' bins and $k$ bins are nonempty bins (thus $k-(i-j)$ bins are ``bad'' and $n-k$ bins are empty). The probability of transition to a composite state is simply the summation of the probabilities of the transitions to corresponding sub-composite states:

To obtain the transition matrix $M$, it is sufficient to compute $m^{(k)}_{i,j}$, which can be exploited using dynamic programming. Note that the balls-and-bins model itself can be considered as a Markov chain, in which a recursive relation exists: After throwing $i$ balls into $n$ bins, throwing one more ball randomly could be: (1) Into an empty bin and turn it to a ``good'' bin; (2) Into a ``good'' bin and turn it to a ``bad'' bin with two balls; or (3) Into a ``bad'' bin and keep it as the same. Mathematically, we have $m^{(k)}_{i+1,j}$ equals to


====================================

More specifically, let state $(j,k)$ denote the sub-state of state $j$ that the $j$ ``bad'' balls end up to occupy exactly $k$ ``bad'' bins. Then the composite state $j$ is partitioned into state $(j,1)$, state $(j,2)$, $...$, state $(j,j)$. We slightly abuse the notation and let $M(i,j,k)$ denote the probability of transition from state $i$ to state $(j,k)$, then we have 

\begin{equation}
    M(i,j) = \sum_{k=1}^{j} M(i,j,k)
\end{equation}

{\bf we can use a tighter range of $k$ of $1,2,..., \lfloor j/2 \rfloor$. For cleanness, I choose a wider range of $1,2,..., j$, which is easier to understand and does not change the result}

To obtain $M$, it is sufficient to compute $M(i,j,k)$ for $\forall i,j,k=0,1,...,t$
{\bf Similarly, there is a tighter range for $i,j,k$, which seems to be unnecessary}
. Note that the state transition resulting from throwing one ball after another is also a Markov chain, in which state $(i,j,k)$ is defined as $j$ ``bad'' balls ending up into $k$ ``bad'' bins after throwing $i$ balls into $n$ bins. In this Markov chain, throwing one more ball can transition state $(i,j,k)$ to three possible states depending on the $(i+1)^{th}$ ball ending up in (1) a ``good'' bin; (2) a ``bad'' bin; or (3) an empty bin. The first case happens with probability $(i-j)/n$, results in $2$ additional ``bad'' balls and $1$ additional ``bad'' bin (i.e., transition to state $(i+1,j+2,k+1)$). The second and third cases transition to state $(i+1,j+1,k)$ and state $(i+1,j,k)$ respectively with probability $k/n$ and $1-(i-j+k)/n$. In the opposite direction, state $(i+1,j,k)$ can only be transitioned from (1) state $(i,j-2,k-1)$; (2) state $(i,j-1,k)$; and (3) state $(i,j,k)$, which gives us a recurrence relation that $M(i+1,j,k)$ equals to

%The second case happens with probability $k/n$ and results in state $(i+1,j+1,k)$. The third case happens with probability $1-(i-j+k)/n$ and results in state $(i+1,j,k)$. In the opposite direction, state $(i+1,j,k)$ can be transitioned from (1) state $(i,j-2,k-1)$ with probability $(i-j+2)/n$; (2) state $(i,j-1,k)$ with probability $k/n$; or (3) state $(i,j,k)$ with probability $1-(i-j+k)/n$. It gives us a recurrence relation that $P(i+1,j,k)$ equals to

\begin{equation}\label{eq:recursion}
    \frac{i\!-\!j\!+\!2}{n}\cdot M(i,j\!-\!1,k\!-\!1)+\frac{k}{n}\cdot M(i,j\!-\!1,k)+(1\!-\!\frac{i\!-\!j\!+\!2}{n})\cdot M(i,j,k)
\end{equation}

The three terms in \autoref{eq:recursion} corresponds to the above three possible transitions. Combining with the following probabilities in base cases, we can compute $M(i,j,k)$ for $\forall i,j,k=0,1,...,t$ using Dynamic Programming and obtain $M$:

\begin{align}
M(0,j,k) =& \left\{ \begin{array}{ccl}
1, & \mbox{if }
 j=k=0 \\ 0, & \mbox{otherwise} 
\end{array}\right.\label{eq:basic1}\\
M(i,0,k) =& \left\{ \begin{array}{ccl}
\binom{n}{i}/n^i, & \mbox{if }
 k=0 \\ 0, & \mbox{otherwise} 
\end{array}\right.\label{eq:basic2}\\
M(i,j,0) =& \left\{ \begin{array}{ccl}
1, & \mbox{if }
 j=0 \\ 0, & \mbox{otherwise} 
\end{array}\right.\label{eq:basic3}
\end{align}

%As mentioned earlier, we slightly abuse the notation `$d$' in this section to denote the number of distinct elements in group pair $1$, which is actually $d_1$ defined in \autoref{subsec:protocol2}. Now we recover the abused notation $d$ to denote the total number of distinct elements in all groups. 

As we explained in \autoref{subsec:protocol2}, $d_1$, the number of distinct elements in group pair $1$, is a random variable that follows a Binomial distribution $Binomial(d,1/g)$. So the probability that the group pair is completely reconciled in $r$ rounds is $\sum_{x=0}^d Pr[d_1=x]\cdot Pr[x\xrsquigarrow{r} 0]$.
%, where $\mathcal{B}(\cdot;d,1/g)$ is the probability mass function (PMF) of $Binomial(d,1/g)$. 
To ease computation, we slightly underestimate this probability by assuming $Pr[x\xrsquigarrow{r} 0]=0$ when $x>t$ (i.e., assume group pair $1$ cannot be reconciled if $d_i>t$, discussed in \autoref{sec:BCH_exception}). The loss of this underestimation is very tiny, since the coefficient of $Pr[x\xrsquigarrow{r} 0]$ (i.e., $Pr[d_1=x]$) is very small when $x>t$. We denote this underestimated probability as $\alpha$ (i.e., $\alpha=\sum_{x=0}^t Pr[d_1=x]\cdot Pr[x\xrsquigarrow{r} 0]$). Note that $Pr[x\xrsquigarrow{r} 0]$ is a function of $n$ and $r$ for arbitrary $x$, so $\alpha$ is a function of $n$, $r$, $t$ for arbitrary $d$ and $g$. 

\subsection{Tail Bound Analysis for all groups}\label{sec:times2bound}

Given $\alpha$, the tail bound of the probability that a group pair is successfully reconciled in $r$ rounds, we can easily derive a tail bound of $\alpha^g=1-(1-\alpha^g)$ for the probability that all group pairs are successfully reconciled in $r$ rounds, if we assume the reconciliations on group pairs are independent with each other. However, this assumption is not rigorous, since $d_1, d_2,...,d_g$ have a weak correlation that $\sum_{i=1}^g d_i=d$. 
%Fortunately, we have Times-2-Bound (Theorem 1 in \cite{hua2008rank}) to decouple the weak correlation and give us a rigorous tail bound of $1-2(1-\alpha^g)$ for the probability of all group pairs. 
To be rigorous, we use so-called Times-2-bound (Corollary 5.11 in \cite{upfal2005probability}) to decouple the weak correlation and obtain a rigorous tail bound of $1-2(1-\alpha^g)$ for the probability of all group pairs.
In \autoref{sec:parameter_settings}, we use the tail bound of $1-2(1-\alpha^g)$ in parameter settings for rigorousness. 

% More specifically, let state $(j,k)$ denote the sub-state of state $j$ that the $j$ ``bad'' balls end up to occupy exactly $k$ ``bad'' bins. Then the composite state $j$ is the union of state $(j,1)$, state $(j,2)$, $...$, state $(j,\lfloor j/2 \rfloor)$ (each ``bad'' bin receives at least $2$ ``bad'' balls, so $k\leq \lfloor j/2\rfloor$). Let $P(i,j,k)$ denote the probability of transition from state $i$ to state $(j,k)$, then we have 

% \begin{equation}
%     M(i,j) = \sum_{k=1}^{\lfloor j/2\rfloor} P(i,j,k)
% \end{equation}






% Note that each state $j$ with $j>3$ in the Markov chain is a composite state as far as the calculation of the transition probability from a (larger) state $i$ $(>j)$ to $j$ (i.e., ``transitioning into''). Such a composite state $j$ can be decomposed into sub-states based on the number of ``bad'' bins after throwing $i$ balls: Define state $(j,k)$ as the sub-state of state $j$ that the  $j$ ``bad'' balls end up to occupy exactly $k$ ``bad'' bins. Then state $j$ is the union of all states $(j,k)$ for $k=1,2,...$ (each ``bad'' bin receives at least $2$ ``bad'' balls). Let $m_{i,j}^{(k)}$ denote the probability of transition from state $i$ to state $(j,k)$
% %, which is also the probability that after throwing $i$ balls uniformly and independently into $n$ bins, $i-j$ bins are ``good'' bins and $k$ bins are nonempty bins (thus $k-(i-j)$ bins are ``bad'' and $n-k$ bins are empty)
% . The probability of transition to the composite state $j$ is simply the summation of the probabilities of the transitions to corresponding sub-states: 

% \begin{equation}
%     m_{i,j} = \sum_{k=i}^{i-j} m^{(k)}_{i,j}
% \end{equation}


% To make our description simple, we call a bin that receives exactly $1$ ball a ``good'' bin is ``good'' if and only if it receives exactly $1$ ball. We call a bin is ``bad'' if and only if it receives more than $1$ balls. The rest bins (i.e., neither ``good'' nor ``bad'') are empty. We call a ball ending up in a ``good'' bin is ``good'' if it is in a ``good bin'' Then the distinct elements that are decoded correspond to the balls that are in ``good'' bins. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Old version of 2/5
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{comment}

In this section, we only consider the cases that a group is able to be decoded by BCH code (i.e., initially contains at most $t$ set differences). Without loss of generosity, we assume the group has $d (\leq t)$ distinct elements and is partitioned into $n$ subset pairs. As we described in \autoref{sec:hash_partition}, the $d$ distinct elements are hashed into $n$ subset pairs in each round, and a distinct element is decoded if and only if it is hashed into a subset pair that contains only $1$ distinct element. As we introduced in \autoref{sec:hash_partition}, the statistical model for hashing $d$ distinct elements into $n$ subset pairs is the same as the classical balls-and-bins problem: $d$ balls are thrown independently and uniformly at random into $n$ bins. To make our description simple, we call a bin is ``good'' if and only if it receives exactly $1$ ball. And we call a bin is ``bad'' if and only if it receives more than $1$ balls. The rest bins (i.e., neither ``good'' nor ``bad'') are empty. Then the distinct elements that are decoded correspond to the balls that are in ``good'' bins. 

The decode process of each group can be considered as a Markov Chain, in which each state is defined as the number of remaining distinct elements (i.e., the distinct elements that haven't been decoded). In this Markov chain, the transition from State $i$ to State $j$ means $i-j$ out of $i$ distinct elements are decoded in this round, where $0\leq j\leq i\leq t$. Use the same analogy, the number (state) is simply the total number of balls that fall in ``bad'' bins. The transition from State $i$ to State $j$ means $i-j$ out of $i$ balls fall in ``good'' bins in this round, while the rest $j$ balls fall in ``bad'' bins. State $0$ is the {\it absorbing} state of this Markov Chain, which means all distinct elements have been reconciled. For our analysis, we only concern the probability that after $r$ rounds, the final state is state $0$ (i.e., absorbing state) when the initial state is state $i$. We denote this probability as $v^{(r)}_i(0)$.

Let $M=(m_{i,j})_{(t+1)\times (t+1)}$ denote the transition matrix of the above Markov chain, where $m_{i,j}$ is the probability of transition from State $i$ to State $j$. Given $M$, $r$, and the initial state $i$, $v^{(r)}_i(0)$ can be easily calculated. So the only problem is how to obtain $M$, which will be elaborated in the next section.

\subsubsection{Transition Matrix}\label{sec:transition_matrix}

Now we describe how to compute the transition matrix $M$ using dynamic programming in detail. Note that every State $j$ with $j > 3$ in the Markov chain is a composite state as far as the calculation of the transition probability from a (larger) state $i > j$ to $j$ (i.e., ``transitioning into").  For example, State 6 contains 4 different cases. The first case is $6 = 6$, where all 6 bad balls are in the same bad bin. The second case is $6 = 2 + 4$ where, out of the 6 bad balls, four are in one bad bin and the other two are in the other bad bin.  Similarly, the other two cases are $6 = 3 + 3$ and $6 = 2 + 2 + 2$. Note there is no need to distinguish these four cases in calculating the ``transitioning out" probability (i.e., from state 6 to a small state say State 0), because the next round of balls-into-bins operation uses a different hash function independent of that used in the current round, and consequently how these 6 bad balls are split in the current round have no bearing on that in the next round. 

Building on the example above, we now consider $m_{9,6}$, the transition probability from State $9$ to State $6$ (throwing 9 balls into 255 bins and ending up with 6 bad balls).  $m_{9,6}$ is simply the sum of the probabilities of these four cases, each of which has a very different formula than the others.  In general, the number of such cases, and hence the number of individual probability terms to be added up to arrive at the transition matrix element $m_{i,j}$, grows exponentially with the value of $j$. This does not however make it difficult to calculate the values of $M$, because there is a recursive structure, among the values of the matrix elements $m_{i,j}$, that can be exploited using dynamic programming, as will be elaborated shortly.

To simply our analysis, we split each composite state into sub-composite states based on the number of nonempty bins: Let State $(j,k)$ denotes the sub-composite state with $j$ remaining distinct elements and $k$ nonempty bins, which is also a substate of State $j$. Let $m_{i,j}^{(k)}$ denote the probability of transition from State $i$ to State $(j,k)$, which is also the probability that after throwing $i$ balls uniformly and independently into $n$ bins, $i-j$ bins are ``good'' bins and $k$ bins are nonempty bins (thus $k-(i-j)$ bins are ``bad'' and $n-k$ bins are empty). The probability of transition to a composite state is simply the summation of the probabilities of the transitions to corresponding sub-composite states:

\begin{equation}
    m_{i,j} = \sum_{k=i}^{i-j} m^{(k)}_{i,j}
\end{equation}

To obtain the transition matrix $M$, it is sufficient to compute $m^{(k)}_{i,j}$, which can be exploited using dynamic programming. Note that the balls-and-bins model itself can be considered as a Markov chain, in which a recursive relation exists: After throwing $i$ balls into $n$ bins, throwing one more ball randomly could be: (1) Into an empty bin and turn it to a ``good'' bin; (2) Into a ``good'' bin and turn it to a ``bad'' bin with two balls; or (3) Into a ``bad'' bin and keep it as the same. Mathematically, we have $m^{(k)}_{i+1,j}$ equals to

\begin{equation}\label{eq:recursion}
\frac{n-k+1}{n}\cdot m^{(k-1)}_{i,j-1} + \frac{j+1}{n}\cdot m^{(k)}_{i,j+1} + \frac{k-(i-j)}{n}\cdot m^{(k)}_{i,j} \nonumber
\end{equation}

The three terms in \autoref{eq:recursion} corresponds to the above three cases. Meanwhile, we can easily get the boundary conditions as follows:

\begin{align}
m^{(k)}_{i,0} =& \left\{ \begin{array}{ccl}
\binom{n}{i}/n^i, & \mbox{if }
 k=i \\ 0, & \mbox{otherwise} 
\end{array}\right.\label{eq:basic1}\\
m^{(k)}_{0,j} =& \left\{ \begin{array}{ccl}
1, & \mbox{if }
 k=0 \mbox{ and } j=0 \\ 0, & \mbox{otherwise} 
\end{array}\right.\label{eq:basic2}\\
m^{(0)}_{i,j} =& \left\{ \begin{array}{ccl}
1, & \mbox{if }
 i=0 \mbox{ and } j=0 \\ 0, & \mbox{otherwise} 
\end{array}\right.\label{eq:basic3}
\end{align}

Using \autoref{eq:recursion},\autoref{eq:basic1},\autoref{eq:basic2}, and \autoref{eq:basic3}, we can recursively compute $m^{(k)}_{i,j}$ and obtain $M$.


\subsection{Global Tail Bound Analysis}\label{sec:times2bound}

Consider group $1$ (other groups have the same result), the probability that all distinct elements in group $1$ are reconciled in $r$ rounds is $\sum_{i=0}^d Pr[d_1=i]v_i^{(r)}(0)\triangleq \alpha$, where $d_1$ (i.e., the number of distinct elements in group $1$) is a Binomial random variable $Binomial(d,1/g)$ as we explained in \autoref{subsec:protocol2}. To ease computation, we slightly underestimate this probability $\alpha$ by assuming $v_i^{(r)}(0)=0$ when $i>t$ (i.e., assume group $i$ cannot reconcile if $d_i>t$, discussed in \autoref{sec:BCH_exception}). The loss of this underestimation is very tiny, since the coefficient of $v_i^{(r)}(0)$ (i.e., $Pr[d_1=i]$) is very small when $i>t$.

The probability that all groups are successfully reconciled in $r$ rounds is simply $\alpha^g\triangleq \beta$, if we assume the reconciliations on groups are independent with each other. This assumption is however not rigorous, since $d_1, d_2,...,d_g$ have a weak correlation that $\sum_{i=1}^g d_i=d$. Fortunately, we have Times-2-Bound (Theorem 1 in \cite{hua2008rank}) to decouple the weak correlation and give us a rigorous bound of $2\beta-1$. In \autoref{sec:parameter_settings}, we use this rigorous bound for parameter settings. 

\end{comment}






\begin{comment}

Let $v^{(r)}_i=\big{(}{v^{(r)}_i(0), v^{(r)}_i(1),...,v^{(r)}_i(t)}\big{)}$ denote the probability vector (i.e., $\sum_{j=0}^{t}v^{(r)}_i(j) = 1$) after $r$ rounds with initial State $i$: $v^{(r)}_i(j)$ denotes the probability that the final state is State $j$ after $r$ rounds. In the probability vector, $v^{(r)}_i(0)$ is the only entry that we concern, which is the probability of the cases that all distinct elements are decoded after $r$ rounds. Given 

Note that every State $j$ with $j > 3$ in the Markov chain is a composite state as far as the calculation of the transition probability from a (larger) state $i > j$ to $j$ (i.e., ``transitioning into").  For example, State 6 contains 4 different cases. The first case is $6 = 6$, where all 6 bad balls are in the same bad bin. The second case is $6 = 2 + 4$ where, out of the 6 bad balls, four are in one bad bin and the other two are in the other bad bin.  Similarly, the other two cases are $6 = 3 + 3$ and $6 = 2 + 2 + 2$. Note there is no need to distinguish these four cases in calculating the ``transitioning out" probability (i.e., from state 6 to a small state say State 0), because the next round of balls-into-bins operation uses a different hash function independent of that used in the current round, and consequently how these 6 bad balls are split in the current round have no bearing on that in the next round. 

Building on the example above, we now consider $m_{9,6}$, the transition probability from State $9$ to State $6$ (throwing 9 balls into 255 bins and ending up with 6 bad balls).  $m_{9,6}$ is simply the sum of the probabilities of these four cases, each of which has a very different formula than the others.  In general, the number of such cases, and hence the number of individual probability terms to be added up to arrive at the transition matrix element $m_{i,j}$, grows exponentially with the value of $j$. This does not however make it difficult to calculate the values of $M$, because there is a recursive structure, among the values of the matrix elements $m_{i,j}$, that can be exploited using dynamic programming, as will be elaborated in \autoref{sec:transition_matrix}.

Let $v^{(r)}_i=\big{(}{v^{(r)}_i(0), v^{(r)}_i(1),...,v^{(r)}_i(t)}\big{)}$ denote the probability vector (i.e., $\sum_{j=0}^{t}v^{(r)}_i(j) = 1$) after $r$ rounds with initial State $i$: $v^{(r)}_i(j)$ denotes the probability that the final state is State $j$ after $r$ rounds. In the probability vector, $v^{(r)}_i(0)$ is the only ``good'' entry, which is the probability of the cases that all distinct elements are decoded after $r$ rounds. The probability of the group does not complete reconciliation is simply $1-v^{(r)}_i(0)$. 

Given the transition matrix $M$, we can easily compute the probability vector $v^{(r)}_i$ for any $r$ and $i$ as follows:
\begin{equation}
    x^{(r)}_i = e_i\cdot M^r
\end{equation}
Here $\{e_i\}_{i=0,1,2,...,t}$ denote the standard basis vectors of length $t+1$, where $e_i$ has a single nonzero value 1 at the $(i+1)^{th}$ position. So the remaining problem is how to compute $M$.

\subsubsection{Transition Matrix}\label{sec:transition_matrix}

Now we describe how to compute the transition matrix $M$ using dynamic programming in detail. As we described earlier, every State $j$ with $j > 3$ in the Markov chain is a composite state that contains many different cases. And the number of these cases increases exponentially with the value of $j$. To simply our analysis, we split each composite state into sub-composite states based on the number of nonempty bins: Let State $(j,k)$ denotes the sub-composite state with $j$ remaining distinct elements and $k$ nonempty bins, which is also a substate of State $j$. Let $m_{i,j}^{(k)}$ denote the probability of transition from State $i$ to State $(j,k)$, which is also the probability that after throwing $i$ balls uniformly and independently into $n$ bins, $i-j$ bins are ``good'' bins and $k$ bins are nonempty bins (thus $k-(i-j)$ bins are ``bad'' and $n-k$ bins are empty). The probability of transition to a composite state is simply the summation of the probabilities of the transitions to corresponding sub-composite states:

\begin{equation}
    m_{i,j} = \sum_{k=i}^{i-j} m^{(k)}_{i,j}
\end{equation}

To obtain the transition matrix $M$, it is sufficient to compute $m^{(k)}_{i,j}$, which can be exploited using dynamic programming. Note that the balls-and-bins model itself can be considered as a Markov chain, in which a recursive relation exists: After throwing $i$ balls into $n$ bins, throwing one more ball randomly could be: (1) Into an empty bin and turn it to a ``good'' bin; (2) Into a ``good'' bin and turn it to a ``bad'' bin with two balls; or (3) Into a ``bad'' bin and keep it as the same. Mathematically, we have 

\begin{align}
m^{(k)}_{i+1,j} =& \frac{n-k+1}{n}\cdot m^{(k-1)}_{i,j-1} + \frac{j+1}{n}\cdot m^{(k)}_{i,j+1} \nonumber\\
&+ \frac{k-(i-j)}{n}\cdot m^{(k)}_{i,j} \label{eq:recursion}
\end{align}

The three terms in \autoref{eq:recursion} corresponds to the above three cases. Meanwhile, we can easily get the following probabilities for basic cases:

\begin{align}
m^{(k)}_{i,0} =& \left\{ \begin{array}{ccl}
\binom{n}{i}/n^i, & \mbox{if }
 k=i \\ 0, & \mbox{otherwise} 
\end{array}\right.\label{eq:basic1}\\
m^{(k)}_{0,j} =& \left\{ \begin{array}{ccl}
1, & \mbox{if }
 k=0 \mbox{ and } j=0 \\ 0, & \mbox{otherwise} 
\end{array}\right.\label{eq:basic2}\\
m^{(0)}_{i,j} =& \left\{ \begin{array}{ccl}
1, & \mbox{if }
 i=0 \mbox{ and } j=0 \\ 0, & \mbox{otherwise} 
\end{array}\right.\label{eq:basic3}
\end{align}

Using \autoref{eq:recursion},\autoref{eq:basic1},\autoref{eq:basic2}, and \autoref{eq:basic3}, we can recursively compute $m^{(k)}_{i,j}$ and then get $v^{(r)}_i(0)$ for $\forall i=0,1,...,n$ and $r\in\mathbb{Z}$. The value of $v^{(r)}_i(0)$ will be used to compute the tail bound of $Pr[P^{(r)}_o]$ in the next section. 

\subsection{Global Tail Bound Analysis}\label{sec:times2bound}

Let random variable $X^{(d)}_i, 1\leq i\leq g$, denote the number of set differences initially allocated in the $i^{th}$ group. For an analogy, the statistical model for hashing $d$ set differences into $g$ groups is also the same as the classical balls-and-bins problem: $d$ balls are thrown independently and uniformly at random into $g$ bins. Then random variable $X^{(d)}_i$ could be translated as the number of balls ended up in the $i^{th}$ bin after $d$ balls are thrown. Therefore, $(X^{(d)}_1,...,X^{(d)}_g)$ follows the multinomial distribution. The marginal distribution for any $X^{(d)}_i$ is $Binomial(d,\frac{1}{g})$, where $Binomial(N,p)$ denotes the binomial distribution resulting from $N$ trials with success probability $p$. 

Let $f^{(r)}(x_1,x_2,...,x_g)$ denote the probability that set reconciliation does not complete (for all groups) in $r$ rounds when the $i^{th}$ group initially contains $x_i$ set differences for $i=1,2,...,g$. Define $f^{(r)}(x)$ as the probability that set reconciliation does not complete in $r$ rounds when a group initially contains $x$ set differences. Based on the result in \autoref{sec:tail_bound_per_group}, we have 

% \begin{equation}\label{eq:frx}
%     f^{(r)}(x) \leq g^{(r)}(x) \triangleq \left\{ \begin{array}{ccc}
% 1-v^{(r)}_{x}(0) & \mbox{for}
% & 0\leq x\leq c \\ 1 & \mbox{for} & x>c
% \end{array}\right.
% \end{equation}

\begin{equation}\label{eq:frx}
    f^{(r)}(x) = 1-v^{(r)}_{x}(0) \mbox{ for }  0\leq x\leq t 
\end{equation}

Since the reconciliation processes independently for each group, we have 

\begin{equation}
f^{(r)}(x_1,x_2,...,x_g) = 1-\prod_{i=1}^g \big{(}1-f^{(r)}(x_i)\big{)}
\end{equation}

Then we have 

\begin{align} 
Pr[P^{(r)}_o] 
&= E[f^{(r)}(X^{(d)}_1,X^{(d)}_2,...,X^{(d)}_g)] \label{eq:errorBound0}\\
&= 1-E[\prod_{i=1}^g \big{(}1-f^{(r)}(X^{(d)}_i)\big{)}] \label{eq:errorBound1}
\end{align}

A naive approach to calculating the probability $Pr[P^{(r)}_o]$ is to regard $X^{(d)}_i$ as mutually independent. Then we have

\begin{align} 
Pr[P^{(r)}_o] 
&= 1-\prod_{i=1}^g E[1-f^{(r)}(X^{(d)}_i)] \label{eq:errorBound2}\\
&= 1-\prod_{i=1}^g (1-E[f^{(r)}(X^{(d)}_i)]) \label{eq:errorBound3}\\
&= 1-(1-E[f^{(r)}(X^{(d)}_i)])^g \label{eq:errorBound4}
\end{align}

And the term $E[f^{(r)}(X^{(d)}_1)]$ in \autoref{eq:errorBound4} can be easily bounded by \autoref{eq:frx} as follows:

\begin{align}
& E[f^{(r)}(X^{(d)}_1)]\\
= &\sum_{k=0}^d \mathcal{B}(k;d,\frac{1}{n})f^{(r)}(k)\\
= &\sum_{k=0}^t \mathcal{B}(k;d,\frac{1}{n})f^{(r)}(k) + \sum_{k=t+1}^d \mathcal{B}(k;d,\frac{1}{n})f^{(r)}(k)\label{eq:beforeLeq}\\
\leq & \sum_{k=0}^t \mathcal{B}(k;d,\frac{1}{n})f^{(r)}(k) + \sum_{k=t+1}^d \mathcal{B}(k;d,\frac{1}{n})\label{eq:afterLeq}\\
= & \sum_{k=0}^t \mathcal{B}(k;d,\frac{1}{n})\big{(}1-v_k^{(r)}(0)\big{)}+\sum_{k=t+1}^d \mathcal{B}(k;d,\frac{1}{n})
\end{align}

Here $\mathcal{B}(k;d,\frac{1}{n})$ is the Binomial probability mass function, and how to compute $v_k^{(r)}(0)$ is discussed in \autoref{sec:tail_bound_per_group} for $\forall k=0,1,...,t$ and $r\in\mathbb{Z}$. From \autoref{eq:beforeLeq} to \autoref{eq:afterLeq}, the loss is very negligible, since $\mathcal{B}(k;d,\frac{1}{n})$ is very small when $k>t$ ($t$ is $2-3$ times of $d/n$).

However, those random variable $X^{(d)}_i$ are not totally independent since they are conditioned by $\sum_{i=1}^g X^{(d)}_i=d$. So the above bound is not rigorous. Fortunately, we have the following theorem (Times-2-Bound) to decouple the weak correlation among $(X^{(d)}_1,...,X^{(d)}_m)$ and bound $Pr[P^{(r)}_o]$ rigorously to be $2$ times of the unrigorous bound in \autoref{eq:errorBound3}. 

\textbf{Theorem 1} {\bf citation}
Let $(X^{(n)}_1,...,X^{(n)}_m)$ follows the multinomial distribution of throwing $n$ balls into $m$ bins. Let $(Y^{(n)}_1,...,Y^{(n)}_m)$ be independent and identically distributed random variables with distribution $Poission(\frac{n}{m})$. Let $f(x_1,...,x_m)$ be a nonnegative function which is increasing in each argument separately. Then
\begin{equation} \label{eq:times2bound}
E[f(X^{(n)}_1,X^{(n)}_2,...,X^{(n)}_m)] \leq 2E[f(Y^{(n)}_1,Y^{(n)}_2,...,Y^{(n)}_m)]
\end{equation}


A naive approach to calculating the probability $Pr[P^{(r)}_o]$ is to regard $X^{(d)}_i$ as mutually independent. In this case, the production in the expectation of \autoref{eq:errorBound1} can be extracted out of the expectation and hence could be easily bounded. However, those random variable $X^{(d)}_i$ are not totally independent since they are conditioned by $\sum_{i=1}^m X^{(d)}_i=d$. Fortunately, we have the following theorem to decouple the weak correlation among $(X^{(d)}_1,...,X^{(d)}_m)$ and bound our targeted probability.

\textbf{Theorem 1}
Let $(X^{(n)}_1,...,X^{(n)}_m)$ follows the multinomial distribution of throwing $n$ balls into $m$ bins. Let $(Y^{(n)}_1,...,Y^{(n)}_m)$ be independent and identically distributed random variables with distribution $Poission(\frac{n}{m})$. Let $f(x_1,...,x_m)$ be a nonnegative function which is increasing in each argument separately. Then
\begin{equation} \label{eq:times2bound}
E[f(X^{(n)}_1,X^{(n)}_2,...,X^{(n)}_m)] \leq 2E[f(Y^{(n)}_1,Y^{(n)}_2,...,Y^{(n)}_m)]
\end{equation}

Substitute \autoref{eq:times2bound} into \autoref{eq:errorBound0}, we have
\begin{align} 
Pr[P^{(r)}_o] 
&= E[f^{(r)}(X^{(d)}_1,X^{(d)}_2,...,X^{(d)}_m)] \\
&\leq 2E[f^{(r)}(Y^{(d)}_1,Y^{(d)}_2,...,Y^{(d)}_m)] \\
&= 2-2E[\prod_{i=1}^m \big{(}1-f^{(r)}(Y^{(d)}_i)\big{)}] \\
&= 2-2\prod_{i=1}^m \big{(}1-E[f^{(r)}(Y^{(d)}_i)]\big{)} \label{eq:beforeSimp}\\
&= 2-2\big{(}1-E[f^{(r)}(Y^{(d)}_1)]\big{)}^m \label{eq:afterSimp}\\
\end{align}

From \autoref{eq:beforeSimp} to \autoref{eq:afterSimp}, we use the property that $Y^{(d)}_i$, $i=1,2,...,m$ are i.i.d random variables with distribution $Poisson(\delta)$ $(\delta = \frac{d}{m})$. And the term $E[f^{(r)}(Y^{(d)}_1)]$ in \autoref{eq:afterSimp} can be easily bounded by \autoref{eq:frx} as follows:

\begin{align}
& E[f^{(r)}(Y^{(d)}_1)]\\
= &\sum_{k=0}^d p(k;\delta)f^{(r)}(k)\\
= &\sum_{k=0}^c p(k;\delta)f^{(r)}(k) + \sum_{k=c+1}^d p(k;\delta)f^{(r)}(k)\label{eq:beforeLeq}\\
\leq & \sum_{k=0}^c p(k;\delta)f^{(r)}(k) + \sum_{k=c+1}^d p(k;\delta)\label{eq:afterLeq}\\
= & \sum_{k=0}^c p(k;\delta)\big{(}1-v_k^{(r)}(0)\big{)}+\sum_{k=c+1}^d p(k;\delta)
\end{align}

Here $p(k;\delta)$ is the Poisson probability mass function, and how to compute $v_k^{(r)}(0)$ is discussed in \autoref{sec:tail_bound_per_group} for $\forall k=0,1,...,c$ and $r\in\mathbb{Z}$. From \autoref{eq:beforeLeq} to \autoref{eq:afterLeq}, the loss is very negligible, since $p(k;\delta)$ is very small when $k>c$ ($c>2\delta$).


\subsection{Parameter Settings}\label{sec:parameter_settings}

% The tail bound is based on the total number of distinct elements $d$, which is however not known precisely. The ToW Estimator introduced in \autoref{subsec:ToW} can only provide an estimation of $d$ (denoted as $\hat{d}$). Note that the tail bound of $Pr[P^{(r)}_o]$ increases as $d$ increases. So overestimate $d$ will get us a larger failure probability $Pr[P^{(r)}_o]$. To ensure a high success probability, we use an overestimated number of distinct element $\bar{d}$ $(>\hat{d})$ for parameter settings, such that $\bar{d}\geq d$ with high probability. In our evaluation, we set $\bar{d}\triangleq 1.38\hat{d}$, such that $\bar{d}\geq d$ with probability $99\%$. 

In this section, we elaborate how to set the parameters (i.e., $n$, $t$, $g$) given $d$ and the objective $(r,p_0)$ (defined in \autoref{subsec:protocol2}) in PBS. For the moment, we assume $d$ is precisely known. 
Given the objective $(r, p_0)$
%(i.e., set reconciliation is complete in $r$ rounds with probability $p_0$) 
%depend on the requirement of specific applications)
, the parameter setting problem aims to find the optimal parameter settings on $n,t,g$ that minimizes the overall communication overhead, under the constraint that the tail bound of the success probability in $r$ rounds is larger than $p_0$. As explained in \autoref{subsec:protocol2}, $\delta$ should be a small number, so we fix $\delta=5$ and therefore $g=d/\delta$ is also fixed. Note that the only two components in the communication overhead per group (described in \autoref{sec:multi-rounds}) that depend on parameter settings are $t\log n+\delta\log n$. So we can formalize the parameter setting problem as the following optimization problem:

\begin{equation}
\min\limits_{n,t} t\log n+\delta\log n \quad \mbox{s.t.}\quad 1-2(1-\alpha^g(n,t))>p_0
\end{equation}

\begin{align}
\mbox{minimize} \quad
&
t\log n+\delta\log n \label{obj:min_communication}
\\
\mbox{subject to} \quad 
&
1-2(1-\alpha^g(n,t))>p_0  \label{eq:success_rate_requirement}
\\
&
n,t\in \mathbb{N}^+ \label{eq:row_sum_requirement}
\end{align}

This optimization problem seems to be very difficult to solve, since the constraint is a very comprehensive function of the parameters (remind that $\alpha=\alpha(n,t)$ is a function of $n$ and $t$ for arbitrary $r$, $d$, and $g$). However, we can narrow down the solution space into only a few combinations and traverse all these combinations to find the optimal parameter settings as follows: First, for BCH coding efficiency, we select $n$ to be $2^m-1$ for some integer $m$ and therefore narrow its range down to $\{63,127,255,511,1023\}$ (recall that $n=\Omega(\delta^2)$). Second, we select $t$ in the range from $1.5\delta$ to $3\delta$, as we suggested in \autoref{subsec:protocol2}. 

Here we use an example to show how we set parameters: Given $d=1000$, $r=3$, $p_0=0.99\%$, for each $(n,t)$ combination in $\{63,127,255,511,1023\}\times \{8,9,...,15\}$, we compute the tail bound of the success probability under the parameter settings and obtain the following table:

\begin{table}[h]
\centering
\caption{Tail bound of success probability}\label{tab:success_prob}
\begin{tabular}{@{}|c|c|c|c|c|c|@{}}
\hline 
\diagbox{$t$}{$n$}    & $63$ & $127$ & $255$ & $511$ & $1023$ \\ \hline 
8   & 0 & 25.5\% & 32.7\% & 34.3\% & 34.9\% \\ \hline
9   & 52.1\% & 78.0\% & 84.2\% & 85.7\% & 86.1\% \\ \hline
10  & 75.1\% & 92.7\% & 96.5\% & 97.4\% & 97.6\% \\ \hline
11  & 85.9\% & 96.9\% & \cellcolor{blue!25}99.1\% & \cellcolor{blue!25}99.5\% & \cellcolor{blue!25}99.6\% \\ \hline
12  & 91.3\% & 98.5\% & \cellcolor{blue!25}99.7\% & \cellcolor{blue!25}99.9\% & \cellcolor{blue!25}$>$99.9\% \\ \hline
13  & 93.9\% & \cellcolor{blue!25}99.1\% & \cellcolor{blue!25}99.8\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% \\ \hline
14  & 95.1\% & \cellcolor{blue!25}99.4\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% \\ \hline
15  & 95.6\% & \cellcolor{blue!25}99.5\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% \\ 
\hline 
\end{tabular}
\end{table}

In the table, all $(n,t)$ combinations in the blue cells satisfy the success probability requirement. Among them, $(127,13)$ has the lowest communication overhead ({\bf measured? quantized?} by $t\log n+\delta\log n$). So we set $n=127, t=13$ in this case. {\bf (may be unnecessary) Note that both the success probability and the overall communication overhead are strictly increasing w.r.t. $n$ and $t$. Hence, instead of computing all values in the table, we could strategically compute only a few of them and obtain the optimal $(n,t)$ (e.g., find the optimal $t$ for each $n$ by binary search each column).}

\end{comment}
\begin{comment}
If not, we use the ToW estimator described in \autoref{subsec:ToW} to obtain $\hat{d}$ (i.e., the estimation of $d$). Then scale it up (e.g., $d=1.38\hat{d}$ in \autoref{sec:evaluation}) for parameter setting, as explained in \autoref{subsec:ToW}. 

Here are the $4$ parameters that need to determine: 

\begin{itemize}
	\itemsep0em
	%\item $\delta$: Average number of distinct elements per group; 
	\item $g$: Number of group pairs; 
	\item $n$: Number of subset pairs in each group pair; 
	\item $r$: Number of rounds; 
	\item $t$: BCH decode capability;
\end{itemize}

Note that the number of groups $g$ is determined after $\delta$ is determined (i.e., $g=\frac{\bar{d}}{\delta}$). Now we describe how to set the four parameters using the tail bound. First, we set $\delta$ to be some small integer (e.g., $\delta=5$), so that the computational complexity (approx $\propto \delta^2$) is small. Second, we set $r$ to be some small integer (e.g., $r=3$), so that the round-trip delay is reasonable. Third, we set an objective success probability $p$ (depend on the requirement of specific applications), and we consider a parameter combination $(n,t)$ is {\it feasible} if and only if the success probability under this parameter setting based on the tail bound is larger than $p$. Among all feasible parameter combinations $(n,t)$, we select the one that has the lowest communication overhead, which can be roughly expressed as $(\delta \log u + t\log n + \delta \log n + 32)\cdot d/\delta$, as explained in \autoref{subsec:protocol2}. Here $u$ (i.e., the size of the element universe) and $d$ (i.e., the number distinct elements) do not depend on the parameter combination. So we only need to minimize $(t+\delta) \log n$ subject to $n$ and $t$. 
\end{comment}
\begin{comment}

\autoref{fig:mc} presents an example state transition diagram with 6 states (0 - 5 ``hidden elements''), denoting the corresponding transition matrix as $P=(p_{i,j})_{6\times 6}$, where $p_{i,j}$ is the probability of moving from State $i$ to State $j$. 

For instance, $p_{5,0}$ denotes the probability that all 5 set differences are decoded, which means the 5 set differences are all hashed into separate bins. $p_{5,2}$ denotes the probability that 3 (=5-2) out of 5 set differences are decoded, which means 3 set differences are hashed into separate bins and 2 set differences are hashed into the same bin. 


Let $L_{max}$ denote the maximum number of errors that BCH code can correct. Define $g^{(r)}(s)$ as follows:

\begin{equation}
    g^{(r)}(s) = \left\{ \begin{array}{ccc}
f^{(r)}(s) & \mbox{for}
& 0\leq s\leq L_{max} \\ 1 & \mbox{for} & s>L_{max}
\end{array}\right.
\end{equation}



Assume BCH code is capable of decode $s$ set differences, then the decode process of a group can be considered as a Markov chain, in which state is defined as the number of ``hidden elements'' (i.e., elements belonging to the set differences that haven't been decoded). \autoref{fig:mc} presents an example state transition diagram with 6 states (0 - 5 ``hidden elements''), denoting the corresponding transition matrix as $P=(p_{i,j})_{6\times 6}$, where $p_{i,j}$ is the probability of moving from State $i$ to State $j$. 

For instance, $p_{5,0}$ denotes the probability that all 5 set differences are decoded, which means the 5 set differences are all hashed into separate bins. $p_{5,2}$ denotes the probability that 3 (=5-2) out of 5 set differences are decoded, which means 3 set differences are hashed into separate bins and 2 set differences are hashed into the same bin. 
% And $p_{5,4}$ denotes the probability that only 1 (=5-4) set difference are decoded. The other 4 set differences could be either hashed into the same bin, or two separate bins with 2 elements in each. 

The transition in this Markov chain basically has three properties: (1) All state transitions are either self-loops or from ``higher'' states to ``lower'' states, since decode process won't generate additional set differences; (2) No state transition to State 1, because 1 remaining difference must be in a bin by itself and is able to be decoded within the same round of transition; (3) State 0 denotes all set differences are decode, which is all the absorbing state of the Markov chain. 

In the context of the Markov chain, $f^{(r)}(k)$ equals the probability that State $k$ does not transient to State 0 (absorbing state) in $r$ rounds. Let $\{e_i\}_{i=0,1,2,...,k}$ denote the standard basis vectors of length $k+1$, where $e_i$ has a single nonzero value 1 at the $(i+1)^{th}$ position. Based on the property of Markov chain, $x^{(r)}_k\triangleq e_k\cdot P^r$ is the probability vector of states after $r$ rounds with $k$ initial set differences, and the $i^{th}$ element in $x^{(r)}_k$ denotes the probability that State $k$ transients to State $i-1$ after $r$ rounds. 

$x^{(r)}(k)=(p^{(r)}_{k,0},p^{(r)}_{k,1},...,p^{(r)}_{k,k})$ denote the probability vector of states after $r$ rounds with $k$ initial set differences, where $p^{(r)}_i$ denotes the probability . 

Given the transition matrix $P$, we can easily 

\begin{figure*}
\centering
\includegraphics[width=0.98\textwidth]{figures/set_diff_markov}
\caption{Markov chain diagram for decoding process of set difference.}\label{fig:mc}
\end{figure*}

First, we assume the length of BCH decode is sufficient to decode each group. Then the decode process of each group can be considered as a Markov chain, in which state is defined as the number of "hidden elements" (i.e., elements belonging to the set difference that are to be decoded). \autoref{fig:mc} presents the state transition diagram, denoting the corresponding transmission matrix as $P=(p_{i,j})_{(d+1)\times (d+1)}$, where $p_{i,j}$ is the probability of moving from State $i$ to State $j$. By the same anology above, considering the classical balls-into-bins problem: $i$ balls are thrown independently and uniformly at random into $m'$ bins. Then $p_{i,j}$ equals to the probability that $i-j$ out of $m'$ bins have exactly one ball in each. Let $p^{(k)}_{i,j}$ denote the probability that $i-j$ out of $m'$ bins have exactly one ball in each, and $k$ out of $m'$ bins are empty. Then we have


\medskip
\noindent
{\bf Analysis on Number of Rounds}.
Consider the whole process as a Markov chain, whose state is defined as the number of 
``hidden elements'' ({\it i.e.,} elements belonging to the set difference that are to be decoded). 
\autoref{fig:mc} presents the state transition diagram, denoting the corresponding transmission 
matrix as $P=\big{(}p_{i,j}\big{)}_{(d+1)\times (d+1)}$ where $p_{i,j}$ is the probability of moving from state $i$ to state $j$. It is complex to obtain all the elements in $P$, we 
can easily get the following probabilities, for any $k \leq d$,
\begin{align}
p_{k,0}&=\frac{\binom{m}{k}k\,!}{m^k} \\
p_{k,1}&=0 \\
p_{k,2}&=\frac{\binom{k}{2}(m-k+2)\binom{m}{k-2}(k-2)\,!}{m^k},\quad \forall k\geq 2\\
p_{k,3}&=\frac{\binom{k}{3}(m-k+3)\binom{m}{k-3}(k-3)\,!}{m^k},\quad \forall k\geq 3\\
p_{k,4}&=\frac{\big{(}\binom{k}{4}(m-k+4) + \binom{k}{2}\binom{k-2}{2}(m-k+4)(m-k+3)/2\big{)}\binom{m}{k-4}(k-4)\,!}{m^k},\quad \forall k\geq 4.
\end{align}
where $m$ is the number of buckets.

Similarly, we can calculate $p_{k,i}$ for any $k\geq i \geq 5$ but the expression gets more and more complex. 


It is not hard to check that the Markov chain described above is an absorbing Markov chain with 
a single absorbing state of $0$. By using the time to absorption theorem of Absorbing Markov Chains~\cite[Page 13]{Elizalde_LectureNotesMath_2006}, 
we can easily get the average number of rounds (steps before the chain is absorbed), which equals
the $d^{th}$ element of $(N{\bf 1})$ where the matrix 
$N=(I-Q)^{-1}$ is the fundamental matrix of $P$ (Note that $Q$ is the transition matrix for all transient states, in our case, is $P$ by removing the last row and column, {\it i.e.,} $P_{0,*}$ 
and $P_{*,0}$) and 
${\bf 1}$ is an all-one vector with length $d$. 

Denote $P^{(k)}$ as the $k$-step transition matrix, then the probability that it takes more than $n$ rounds to decode is
\begin{equation}
\mathbf{Pr}[t>n]=\sum_{k=n+1}^{\infty}p^{(k)}_{d,0},
\end{equation}
where $d$ is the initial number of elements.


\medskip
\noindent
{\bf Simplified Analysis on Number of Rounds.} In the following analysis, we assume that the number of buckets in the kth round, 
assuming remaining $d_k$ elements to be decoded, is set to be $\delta\cdot d_k$ where $\delta > 1$ is a constant. For ease of 
presentation, we drop the subscript $k$ in the following analysis\footnote{Inspired by the analysis of the number of iterations 
for PIM.}. 

Fix a bucket, the probability that it gets exactly one element belonging to the set difference that is not decoded yet is:
\begin{equation}
p = d \Big{(}\frac{1}{\delta d}\Big{)}\Big{(} 1 - \frac{1}{\delta d}\Big{)}^{d - 1} = \frac{1}{\delta}\Big{(} 1 - \frac{1}{\delta d}\Big{)}^{d - 1}\approx \frac{1}{\delta}e^{-1/\delta}.
\end{equation}

On average, there are $p$ fraction of buckets will get exact one element. Hence, on average $e^{-1/\delta}$ fraction of un-decoded 
elements will be decoded in each round. Therefore, on average, we need $\log_{\frac{1}{1- e^{-1/\delta}}}d_0$ rounds, {\it i.e.,} 
$O(\log d_0)$ rounds. 

\end{comment}



==> section/theoretical_analysis0214.tex <==
\begin{comment}
\section{Tug-of-War Sketch}\label{sec:sketch}


In this section, we describe the {\it tug-of-war}, which was first proposed in~\cite{AlonMS99} as 
a space-efficient estimator for the second frequency moment. 
%% Copy from Infocom 2009
We briefly describe 
the plain vanilla tug-of-war sketch~\cite{AlonMS99} in the context of error estimating coding, and under the assumption
that the sketch per se is not subject to bit errors (``noiseless") during transmission.  A tug-of-war sketch of a bit array (packet) $b$
is comprised of a constant number $c$ of counters  ($c$ is determined by the desired error guarantees) that are maintained using the same update algorithm (with possibly different update values) and is sent to the receiver alongside with $b$.
After the execution of these update algorithms, each counter contains the inner product of the bit vector $\overrightarrow{b}$ (`0' converted to `-1' as discussed earlier) with a vector $\overrightarrow{s} \in \{+1, -1\}^n $  that is four-wise independent, as shown in the following algorithm.  Such four-wise independent vectors are known to exist and have computationally efficient representations (e.g., derivable from the Reed-Muller code~\cite{GilbertKMS03}).
Note the actual update algorithm is not shown here because it is not relevant to our context; Only its ``net effect" after execution is. 


\subsection{Set Reconciliation}\label{subsec:set-reconciliation}

Before we describe how to use tug-of-war for set reconciliation~\cite{Guo_SetReconciliationvia_2013,Mitzenmacher_SimpleMultiParty_2013,Eppstein_WhatsDifference?Efficient_2011}, we first give a brief 
description of set reconciliation. For two sets $A, B$ that contain elements from the same universe, $U$, the set reconciliation 
problem wants to compute the set difference $A \Delta B\triangleq (A\setminus B)\cup (B\setminus A)$. We denote $D=A\Delta B$, and 
$d=|D|$. In the context of set reconciliation, the two sets $A$ and $B$ are stored at two distinct places and the problem wants to 
compute $D$ with minimal communication overhead. 

First, we assume that $d$ is known a prior. We will show later how to use the tug-of-war sketch 
to estimate $d$, the size of 
the set difference. 
As shown in~\cite{Eppstein_WhatsDifference?Efficient_2011}, we can achieve 
$O(d)$ (with a small constant factor) 
communication overhead to compute the set difference $D$ using 
the invertible bloom filter (IBF)~\cite{Goodrich_InvertibleBloomLookup_2011,Eppstein_StragglerIdentificationRound_2011}, which is clearly (asymptotically) optimal. However, in the cases where each element is 
very large (in terms of communication requirement) such as large documents or movie chunks, it is a large communication overhead to transmit a small constant (say $2$ or $3$) times  $d$ elements. As we will show next, by using 
the tug-of-war sketch, we can reduce the communication overhead to very close to $d$ (elements) 
with a few rounds of message exchanges. 


We assume that the communication is initiated by $A$. 
Each round of communication works as follows. 
$A$ creates $m=\delta d$ buckets, $b_1,b_2,\dots,b_m$, 
where $\delta > 1$ is a constant. Each bucket $b_i$
contains a subset of elements from $A$, 
each of which is uniformly randomly selected (with properly-designed 
hash functions). 
For each bucket $b_i$, $A$ computes $c$ tug-of-war sketches, 
denoting as $z_{i,1},z_{i,2},\dots,z_{i,c}$. Note that here eahc $z_{i,j}=\sum_{a\in b_i}h(a)$, where 
$h$ is from a four-wise hash family that maps each element to $\pm 1$. 
Then, $A$ sends the $m\times c$ sketches 
to $B$. $B$ uses the same hash functions to create $m$ buckets for its elements, and then use the same hash 
functions to compute the tug-of-war sketches for each bucket, denoting those sketches as $z'_{i,j}$ for $i\in [m]$ and 
$j\in [c]$. Then, $B$ can use $\frac{1}{c}\sum_{j=1}^{c}(z_{i,j}-z'_{i,j})^2$ to estimate the size of (sub-)set difference of 
the bucket $b_i$ for any $i\in [m]$. Note that $B$ can use the median of mean approach in~\cite{AlonMS99} 
or the MLE estimator in~\cite{Hua_TowardsOptimalError_2012} to obtain 
better estimations. Then, for each bucket whose estimator is in $(0, 1.5)$ (just an example), $B$ sends the exclusive or of all the elements 
in the bucket to $B$. It is clear that if the true size of the set difference for the bucket is $1$, then $A$ can obtain the 
element belonging to $A\Delta B$ in the bucket. 

By repeating the process until all the $d$ elements are obtained, $A$ computes the set difference $D$.
\end{comment}
\begin{comment}
\medskip
\noindent
{\bf Analysis on Number of Rounds}.
Consider the whole process as a Markov chain, whose state is defined as the number of 
``hidden elements'' ({\it i.e.,} elements belonging to the set difference that are to be decoded). 
\autoref{fig:mc} presents the state transition diagram, denoting the corresponding transmission 
matrix as $P=\big{(}p_{i,j}\big{)}_{(d+1)\times (d+1)}$ where $p_{i,j}$ is the probability of moving from state $i$ to state $j$. It is complex to obtain all the elements in $P$, we 
can easily get the following probabilities, for any $k \leq d$,
\begin{align}
p_{k,0}&=\frac{\binom{m}{k}k\,!}{m^k} \\
p_{k,1}&=0 \\
p_{k,2}&=\frac{\binom{k}{2}(m-k+2)\binom{m}{k-2}(k-2)\,!}{m^k},\quad \forall k\geq 2\\
p_{k,3}&=\frac{\binom{k}{3}(m-k+3)\binom{m}{k-3}(k-3)\,!}{m^k},\quad \forall k\geq 3\\
p_{k,4}&=\frac{\big{(}\binom{k}{4}(m-k+4) + \binom{k}{2}\binom{k-2}{2}(m-k+4)(m-k+3)/2\big{)}\binom{m}{k-4}(k-4)\,!}{m^k},\quad \forall k\geq 4.
\end{align}
where $m$ is the number of buckets.

Similarly, we can calculate $p_{k,i}$ for any $k\geq i \geq 5$ but the expression gets more and more complex. 


It is not hard to check that the Markov chain described above is an absorbing Markov chain with 
a single absorbing state of $0$. By using the time to absorption theorem of Absorbing Markov Chains~\cite[Page 13]{Elizalde_LectureNotesMath_2006}, 
we can easily get the average number of rounds (steps before the chain is absorbed), which equals
the $d^{th}$ element of $(N{\bf 1})$ where the matrix 
$N=(I-Q)^{-1}$ is the fundamental matrix of $P$ (Note that $Q$ is the transition matrix for all transient states, in our case, is $P$ by removing the last row and column, {\it i.e.,} $P_{0,*}$ 
and $P_{*,0}$) and 
${\bf 1}$ is an all-one vector with length $d$. 

Denote $P^{(k)}$ as the $k$-step transition matrix, then the probability that it takes more than $n$ rounds to decode is
\begin{equation}
\mathbf{Pr}[t>n]=\sum_{k=n+1}^{\infty}p^{(k)}_{d,0},
\end{equation}
where $d$ is the initial number of elements.


\medskip
\noindent
{\bf Simplified Analysis on Number of Rounds.} In the following analysis, we assume that the number of buckets in the kth round, 
assuming remaining $d_k$ elements to be decoded, is set to be $\delta\cdot d_k$ where $\delta > 1$ is a constant. For ease of 
presentation, we drop the subscript $k$ in the following analysis\footnote{Inspired by the analysis of the number of iterations 
for PIM.}. 

Fix a bucket, the probability that it gets exactly one element belonging to the set difference that is not decoded yet is:
\begin{equation}
p = d \Big{(}\frac{1}{\delta d}\Big{)}\Big{(} 1 - \frac{1}{\delta d}\Big{)}^{d - 1} = \frac{1}{\delta}\Big{(} 1 - \frac{1}{\delta d}\Big{)}^{d - 1}\approx \frac{1}{\delta}e^{-1/\delta}.
\end{equation}

On average, there are $p$ fraction of buckets will get exact one element. Hence, on average $e^{-1/\delta}$ fraction of un-decoded 
elements will be decoded in each round. Therefore, on average, we need $\log_{\frac{1}{1- e^{-1/\delta}}}d_0$ rounds, {\it i.e.,} 
$O(\log d_0)$ rounds. 
\end{comment}

\section{Tail Bound Analysis and Parameter Settings}\label{sec:tail_bound}

In this section, we establish a tight tail bound on the probability that all group pairs are completely reconciled in $r$ rounds under arbitrary parameter settings of $n$, $\delta$, and $t$. On one hand, this tail bound gives us a theoretical guarantee on the {\it success rate} (a metric for evaluation, to be defined in \autoref{subsubsec:configuration}) under specific parameter settings. On the other hand, given a target success probability of $r$ rounds, we can use the tail bound to find all feasible parameter settings that satisfy the success probability requirement, then select the optimal parameter settings among them that have the lowest communication overhead. In this section, we continue to assume $d$ is precisely known. 

%For simplicity, we ignore two types of small probability events in the analysis. The first one is, PBS mistakenly believes the set reconciliation has been completed due to an incorrect verification of the $32$-bit checksum (\autoref{step:terminate_condition} of \autoref{alg:single_round_pbs}). The second one is, a type (\RN{2}) event happens and the ``fake'' distinct element is not successfully verified by \autoref{alg:verification} (mentioned in \autoref{subsec:exception_hash_partition}). As we described earlier, the former happens with a probabilty of $2.3\times 10^{-10}$ and that of the later is in order of $10^{-7}$. Ignoring these events that happen with such tiny probabilities barely compromises the accuracy of the tail bound. 

% Motivated by parameter settings, we establish a strict tail bound on the {\it success probability} of PBS (i.e., all distinct elements are reconciled in $r$ rounds) as a function of parameters (i.e., $n$, $\delta$, $t$), which give us (1) a guideline on parameter settings; and (2) a theoretical guarantee about the success probability under selected parameters. 

% In this section, we still assume $d$ is precisely known. 
% For simplicity, we make the following two assumptions that hold with overwhelming probability in the analysis: First, the checksum (\autoref{step:terminate_condition} of \autoref{alg:single_round_pbs}) works perfectly on checking if the reconciliation is complete; Second, no ``fake'' distinct element fails to be checked by \autoref{alg:verification} (mentioned in \autoref{subsec:exception_hash_partition}) appears during reconciliation. 

{\bf (to be finalized after the following subsections are finalized) We first establish a strict tail bound for a single group pair using Markov chain and Dynamic Programming in \autoref{sec:tail_bound_per_group}. Then we combine it with Times-2-Bound to get a strict tail bound for all group pairs in \autoref{sec:times2bound}. In \autoref{sec:parameter_settings}, we discuss the parameter settings using the tail bound. }

%In \autoref{sec:tail_bound_insufficient}, we remove the above BCH assumption and derive a more precise tail bound. {\bf need to decide whether to have this part or not, since we can easily set a relatively long BCH code, so that each group is decodable w.h.p.}

\subsection{Single Group Pair Analysis}\label{sec:single_markov}

In this section, we analyze the probability that an arbitrary group pair that contains exactly $x$ $(\leq t)$ distinct elements is completely reconciled (i.e., all distinct elements are successfully reconciled) by PBS in $r$ rounds.

As we described in \autoref{sec:multi-rounds}, in the first round of PBS, the $x$ distinct elements are hashed into $n$ subset pairs, and a distinct element is successfully reconciled if and only if it is hashed into a subset pair that contains only $1$ distinct element. The successfully reconciled distinct elements in the first round are removed and the other distinct elements (i.e., the ones that have not been reconciled yet in the first round) will be hashed again in the second round using a different hash function, so on so force, until all distinct elements are successfully reconciled. 

How the $x$ distinct elements are distributed into $n$ subset pairs in the first round follows the familiar {\it balls-into-bins} probability model: Each of the $x$ balls is thrown independently and uniformly at random into one of the $n$ bins. Each successfully reconciled distinct element corresponds to a ball that ends up in a bin that receives exactly $1$ ball. We call the ball and the bin ``good'' in the sequel; each distinct element that has not been reconciled yet in the first round corresponds to a ball that ends up in a bin that receives multiple balls. We call the ball and the bin ``bad'' in the sequel. Note that balls are either ``good'' or ``bad'', but a bin could be empty besides being ``good'' and ``bad''. 

The ``bad'' balls in the first round will be the balls to be thrown in the second round. The ``bad'' balls in the second round will be the balls to be thrown in the third round, so on so force. In all rounds, how the balls are thrown into $n$ bins follows the balls-into-bins probability model. Note that the balls are thrown using independent hash functions in each round, so the number of ``bad'' balls in the $i$-th round (i.e., the number of balls to be thrown in the $(i+1)$-th round) only depends on how many balls are thrown in the $i$-th round and the {\bf underlining?} hash function. Hence, the dynamics of the number of balls to be thrown in each round can be modeled as a Markov chain, in which each state is defined as the number of balls to be thrown. {\bf a little bit wordy, need advice on how to shrink it.}

In the Markov chain, a transition from state $i$ to state $j$ ($i\geq j$) means $i-j$ out of $i$ balls are ``good'' balls and the other $j$ balls are ``bad'' balls. The {\it absorbing state} of this Markov chain is state $0$, which is the ``good'' state that corresponds to all distinct elements have been successfully reconciled. For our analysis, the only probability that we concerned is $Pr[x\xrsquigarrow{r} 0]$, the probability that state $x$ (initial state) reaches the absorbing state (i.e., state $0$) in $r$ transitions, which is also the probability that all distinct elements in this group pair are successfully reconciled in $r$ rounds. This probability can be easily calculated given $M$, the $(t+1)\times (t+1)$ transition matrix of the Markov chain, as 
%, where $M(i,j)$ (i.e., the entry in the $i^{th}$ row and the $j^{th}$ column of $M$) is the probability of transition from state $i$ to state $j$ for $i,j = 0,1,...,t$
$\big{(}M^r\big{)}(x,0)$ (i.e., the entry in the $x^{th}$ row and the $0^{th}$ column of $M^r$). Here we slightly abuse the row / column numbers of a $(t+1)\times (t+1)$ matrix from $1,2,...,t+1$ to $0,1,...,t$, since the state of the Markov chain ranges from $0$ to $t$. How to compute $M$ will be elaborated in \autoref{sec:compute_M}. For the moment, we assume $M$ has been computed and therefore we can compute $Pr[x\xrsquigarrow{r} 0]$ for $x=1,2,...,t$, $r\in\mathbb{N}^+$. 

\subsection{Tail Bound Analysis for Each Group Pair}\label{sec:tail_bound_per_group}

==========
{\bf The following may be useful in explaining why it is a Markov chain:} [Note there is no need to distinguish these four cases in calculating the ``transitioning out" probability (i.e., from state 6 to a small state say State 0), because the next round of balls-into-bins operation uses a different hash function independent of that used in the current round, and consequently how these 6 bad balls are split in the current round have no bearing on that in the next round.]  {\bf unless you have done so earlier}
==========

As we explained in \autoref{subsec:protocol2}, $d_1$, the number of distinct elements in group pair $1$, is a random variable that follows a Binomial distribution $Binomial(d,1/g)$. So the probability that group pair $1$ is completely reconciled in $r$ rounds is $\sum_{x=0}^d Pr[d_1=x]\cdot Pr[x\xrsquigarrow{r} 0]$. 
%, where $\mathcal{B}(\cdot;d,1/g)$ is the probability mass function (PMF) of $Binomial(d,1/g)$. 
To ease computation, we slightly underestimate this probability by assuming $Pr[x\xrsquigarrow{r} 0]=0$ when $x>t$ (i.e., assume group pair $1$ cannot be reconciled if $d_1>t$, discussed in \autoref{sec:BCH_exception}). The loss of this underestimation is very tiny, since the coefficient of $Pr[x\xrsquigarrow{r} 0]$ (i.e., $Pr[d_1=x]$) is very small when $x>t$. We denote this underestimated probability as $\alpha$ (i.e., $\alpha=\sum_{x=0}^t Pr[d_1=x]\cdot Pr[x\xrsquigarrow{r} 0]$), which is a tight tail bound of the success probability of group pair $1$. $\alpha$ is also a tight tail bound for all other group pairs, since $d_1,d_2,...,d_g$ follows the same distribution. Note that $Pr[x\xrsquigarrow{r} 0]$ is a function of $n$ for arbitrary $x$ and $r$, so $\alpha$ is a function of $n$ and $t$ for arbitrary $d$, $r$, and $g$. 

\subsection{Tail Bound Analysis for all groups}\label{sec:times2bound}

Given $\alpha$, the tail bound of the probability that a group pair is completely reconciled in $r$ rounds, we can easily derive a tail bound of $\alpha^g=1-(1-\alpha^g)$ for the probability that all group pairs are completely reconciled in $r$ rounds, if we assume the reconciliations on group pairs are independent with each other. However, this assumption is not rigorous, since $d_1, d_2,...,d_g$ have a weak correlation that $\sum_{i=1}^g d_i=d$. 
%Fortunately, we have Times-2-Bound (Theorem 1 in \cite{hua2008rank}) to decouple the weak correlation and give us a rigorous tail bound of $1-2(1-\alpha^g)$ for the probability of all group pairs. 
To be rigorous, we can use Corollary 5.11 in \cite{upfal2005probability} to decouple the weak correlation and obtain a rigorous tail bound of $1-2(1-\alpha^g)$ for the success probability of all group pairs. This rigorous tail bound is very tight and only doubles the failure probability of the unrigorous tail bound: For example, if the unrigorous tail bound of the success probability of all group pairs is $0.9999$ ($0.0001$ failure probability), then the rigorous tail bound will be $0.9998$ ($0.0002$ failure probability). In \autoref{sec:parameter_settings}, we use the tail bound of $1-2(1-\alpha^g)$ in parameter settings for rigorousness. 

\subsection{Parameter Settings}\label{sec:parameter_settings}

% The tail bound is based on the total number of distinct elements $d$, which is however not known precisely. The ToW Estimator introduced in \autoref{subsec:ToW} can only provide an estimation of $d$ (denoted as $\hat{d}$). Note that the tail bound of $Pr[P^{(r)}_o]$ increases as $d$ increases. So overestimate $d$ will get us a larger failure probability $Pr[P^{(r)}_o]$. To ensure a high success probability, we use an overestimated number of distinct element $\bar{d}$ $(>\hat{d})$ for parameter settings, such that $\bar{d}\geq d$ with high probability. In our evaluation, we set $\bar{d}\triangleq 1.38\hat{d}$, such that $\bar{d}\geq d$ with probability $99\%$. 

In this section, we elaborate how to set the parameters (i.e., $n$, $t$, $g$) given the target success probability $p_0$ of $r$ rounds (the probability that PBS successfully reconciles all distinct elements in $r$ rounds to be larger than $p_0$) in PBS. We continue to assume $d$ is precisely known. First, as explained in \autoref{subsec:protocol2}, $\delta$ should be a small number, so we fix $\delta=5$ and therefore $g=d/\delta$ is also fixed. 
Given the target success probability $p_0$ of $r$ rounds
%(i.e., set reconciliation is complete in $r$ rounds with probability $p_0$) 
%depend on the requirement of specific applications)
, the parameter setting problem aims to find the optimal parameter settings of $n,t$ that minimizes the overall communication overhead, under the constraint that the tail bound of the success probability of $r$ rounds is larger than $p_0$. Note that the only two components in the communication overhead per group (described in \autoref{sec:multi-rounds}) that depend on parameter settings are $t\log n+\delta\log n$. So we can formalize the parameter setting problem as the following optimization problem:

% \begin{equation}
% \min\limits_{n,t} t\log n+\delta\log n \quad \mbox{s.t.}\quad 1-2(1-\alpha^g(n,t))>p_0
% \end{equation}

\begin{align}
\mbox{minimize} \quad
&
t\log n+\delta\log n \label{obj:min_communication}
\\
\mbox{subject to} \quad 
&
1-2(1-\alpha^g(n,t))>p_0  \label{eq:success_rate_requirement}
\\
&
n,t\in \mathbb{N}^+ \label{eq:row_sum_requirement}
\end{align}

This optimization problem seems to be difficult to solve, since the constraint is a very comprehensive function of the parameters (remind that $\alpha=\alpha(n,t)$ is a function of $n$ and $t$ for arbitrary $r$, $d$, and $g$). However, we can narrow down the solution space into only a few combinations and traverse all these combinations to find the optimal parameter settings as follows: First, for BCH coding efficiency, we select $n$ to be $2^m-1$ for some integer $m$ and therefore narrow its range down to $\{63,127,255,511,1023\}$ (recall that $n=\Omega(\delta^2)$). Second, we select $t$ in the range from $1.5\delta$ to $3\delta$, as we suggested in \autoref{subsec:protocol2}. 

Here we use an example to show how we set parameters: Given $d=1000$, $r=3$, $p_0=0.99\%$, for each $(n,t)$ combination in $\{63,127,255,511,1023\}\times \{8,9,...,15\}$, we compute the tail bound of the success probability under the parameter settings and obtain the following table:

\begin{table}[h]
\centering
\caption{Tail bound of success probability}\label{tab:success_prob}
\begin{tabular}{@{}|c|c|c|c|c|c|@{}}
\hline 
\diagbox{$t$}{$n$}    & $63$ & $127$ & $255$ & $511$ & $1023$ \\ \hline 
8   & 0 & 25.5\% & 32.7\% & 34.3\% & 34.9\% \\ \hline
9   & 52.1\% & 78.0\% & 84.2\% & 85.7\% & 86.1\% \\ \hline
10  & 75.1\% & 92.7\% & 96.5\% & 97.4\% & 97.6\% \\ \hline
11  & 85.9\% & 96.9\% & \cellcolor{blue!25}99.1\% & \cellcolor{blue!25}99.5\% & \cellcolor{blue!25}99.6\% \\ \hline
12  & 91.3\% & 98.5\% & \cellcolor{blue!25}99.7\% & \cellcolor{blue!25}99.9\% & \cellcolor{blue!25}$>$99.9\% \\ \hline
13  & 93.9\% & \cellcolor{blue!60}99.1\% & \cellcolor{blue!25}99.8\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% \\ \hline
14  & 95.1\% & \cellcolor{blue!25}99.4\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% \\ \hline
15  & 95.6\% & \cellcolor{blue!25}99.5\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% \\ 
\hline 
\end{tabular}
\end{table}

In the table, all $(n,t)$ combinations in the highlighted cells satisfy the success probability requirement. Among them, $(127,13)$ has the lowest communication overhead ({\bf measured? quantized?} by $t\log n+\delta\log n$). So we set $n=127, t=13$ in this case. 

\subsection{How to compute \texorpdfstring{\larger\boldmath{$M$}}{M}}\label{sec:compute_M}

In this section, we describe how to compute the transition matrix $M$ in details. Note that calculating an arbitrary transition probability $M(i,j)$ is not straightforward, since each state $j$ (after-transition state) with $j>3$ in the Markov chain is a {\it composite state}.
%as far as the calculation of the transition probability from a (larger) state $i$ $(>j)$ to $j$ is concerned. 
To calculate the probability, we have to break the composite state $j$ down into ``atom'' states, calculate the transition probability from state $i$ to each of the ``atom'' states (which can be directly calculated), and then add them up. {\bf Note that we always view state $i$ (pre-transition state) as a {\it simple state}, since how the $i$ balls are placed into $n$ bins only depends on the hash function, which is independent of the ones used in previous rounds.}

Each composite state $j$ can be broken down into atom states based on how these $j$ bad balls are placed into the $n$ bins. For example, state $6$ consists of $4$ atom states. The first one is $6 = 6$, where all $6$ bad balls are in the same bad bin. The second one is $6 = 2 + 4$ where, out of the $6$ bad balls, four are in one bad bin and the other two are in the other bad bin.  Similarly, the other two atom states are $6 = 3 + 3$ and $6 = 2 + 2 + 2$. The transition probability from state $i$ to any atom state can be directly calculated, but the problem is that the number of atom states grows exponentially with the number of ``bad'' balls $j$.

We notice that we can break each composite state into a small number of coarse-grained sub-states, each of which may still contain a large number of atom states. The transition probability from a (larger) state $i$ to any sub-state is still hard to compute. However, there is a recurrence relation among them, so we can compute the transition probabilities from any state to any sub-state using Dynamic Programming. 

More specifically, let state $(j,k)$ denote the sub-state of state $j$ that the $j$ ``bad'' balls end up to occupy exactly $k$ ``bad'' bins. Then the composite state $j$ is partitioned into state $(j,1)$, state $(j,2)$, $...$, state $(j,j)$. We slightly abuse the notation and let $M(i,j,k)$ denote the probability of transition from state $i$ to state $(j,k)$, then we have 

\begin{equation}
    M(i,j) = \sum_{k=1}^{j} M(i,j,k)
\end{equation}

{\bf explain the range of $k$ could be distracting, so I just leave it as it is.}
To obtain $M$, it is sufficient to compute $M(i,j,k)$ for $\forall i,j,k=0,1,...,t$. Note that the state transition resulting from throwing one ball after another is also a Markov chain, in which state $(i,j,k)$ is defined as $j$ ``bad'' balls ending up into $k$ ``bad'' bins after throwing $i$ balls into $n$ bins. In this Markov chain, throwing one more ball can transition state $(i,j,k)$ to three possible states depending on the $(i+1)$-th ball ending up in (1) a ``good'' bin; (2) a ``bad'' bin; or (3) an empty bin. The first case happens with probability $(i-j)/n$, results in $2$ additional ``bad'' balls and $1$ additional ``bad'' bin (i.e., transition to state $(i+1,j+2,k+1)$). The second and third cases transition to state $(i+1,j+1,k)$ and state $(i+1,j,k)$ respectively with probability $k/n$ and $1-(i-j+k)/n$. In the opposite direction, state $(i+1,j,k)$ can only be transitioned from (1) state $(i,j-2,k-1)$; (2) state $(i,j-1,k)$; and (3) state $(i,j,k)$, which gives us a recurrence relation that $M(i+1,j,k)$ equals to

%The second case happens with probability $k/n$ and results in state $(i+1,j+1,k)$. The third case happens with probability $1-(i-j+k)/n$ and results in state $(i+1,j,k)$. In the opposite direction, state $(i+1,j,k)$ can be transitioned from (1) state $(i,j-2,k-1)$ with probability $(i-j+2)/n$; (2) state $(i,j-1,k)$ with probability $k/n$; or (3) state $(i,j,k)$ with probability $1-(i-j+k)/n$. It gives us a recurrence relation that $P(i+1,j,k)$ equals to

\begin{equation}\label{eq:recursion}
    \frac{i\!-\!j\!+\!2}{n}\cdot M(i,j\!-\!1,k\!-\!1)+\frac{k}{n}\cdot M(i,j\!-\!1,k)+(1\!-\!\frac{i\!-\!j\!+\!2}{n})\cdot M(i,j,k)
\end{equation}

The three terms in \autoref{eq:recursion} corresponds to the above three possible transitions. Combining with the following probabilities in base cases, we can compute $M(i,j,k)$ for $\forall i,j,k=0,1,...,t$ using Dynamic Programming and obtain $M$:

\begin{align}
M(0,j,k) =& \left\{ \begin{array}{ccl}
1, & \mbox{if }
 j=k=0 \\ 0, & \mbox{otherwise} 
\end{array}\right.\label{eq:basic1}\\
M(i,0,k) =& \left\{ \begin{array}{ccl}
\binom{n}{i}/n^i, & \mbox{if }
 k=0 \\ 0, & \mbox{otherwise} 
\end{array}\right.\label{eq:basic2}\\
M(i,j,0) =& \left\{ \begin{array}{ccl}
1, & \mbox{if }
 j=0 \\ 0, & \mbox{otherwise} 
\end{array}\right.\label{eq:basic3}
\end{align}

+++++++++++

The only problem left to obtain $Pr[d\xrsquigarrow{r} 0]$ is how to compute $M$, which is not straightforward, since each state $j$ with $j>3$ in the Markov chain is a composite state as far as the calculation of the transition probability from a (larger) state $i$ $(>j)$ to $j$ (i.e., ``transitioning into'') is concerned.   {\bf You need to explain why it is not straightforward:  The reason you offer is not
the direction reason.  Instead you may say that "the transition probability between these composite states cannot be directly calculated" ...  to calculate it we have to break it down into "atom" states}

Each composite state $i$ can be broken down into atom states as follows.  Each simple state is, in combinatorics terms, {\it a permutation of a combination of $i$}, which here corresponds to 
how these $i$ balls are ``divided up" by the $n$ bins.   {\bf Liang, Read Mitzenmacher and Upfal book
for a better word for "divided up"}
For a simple example, when $i = 4$ and $n = 7$, the vector (1, 0, 1, 0, 0, 2, 0) is such a simple state, which corresponds to these 7 bins (in a predefined order such as the natural order) 
have 1, 0, 1, 0, 0, 2, and 0 balls in it respectively.   The transition probability between any two atom states can be ...    but the problem is that the number of atom states 
(permutations of combinations) grow exponentially with the number of balls $i$.

Consider two states i1 and i2 each broken down into millions of atom states.  Then the transition probability between these states is the summation of the trillions (= millions * millions) of 
transition probabilities between atom states of i1 and atom states of i2.  

The good thing is that the transition probability matrix among the (humongous number of atom states) induces a "subproblem structure ????", which leads to the recurrence relation, 
dynamic programming.   

We notice that we can break each state into a small number of coarse-grained substates, each of which may still contain a large number of atom states.  The transition probability 
between any two such substates are still hard to compute.  However, there is a recurrence relation among them ...

+++++++++++

To solve the problem, we partition the composite state into sub-states, so that the transition probability to the composite state is the summation of the transition probabilities to each of the sub-states. On the other hand, the transition probabilities to the sub-state have a recurrence relation and can be computed using Dynamic Programming. 

======================================

Note that every state $j$ with $j > 3$ in the Markov chain is a composite state as far as the calculation of the transition probability from a (larger) state $i > j$ to $j$ (i.e., ``transitioning into").  For example, State 6 contains 4 different cases. The first case is $6 = 6$, where all 6 bad balls are in the same bad bin. The second case is $6 = 2 + 4$ where, out of the 6 bad balls, four are in one bad bin and the other two are in the other bad bin.  Similarly, the other two cases are $6 = 3 + 3$ and $6 = 2 + 2 + 2$. Note there is no need to distinguish these four cases in calculating the ``transitioning out" probability (i.e., from state 6 to a small state say State 0), because the next round of balls-into-bins operation uses a different hash function independent of that used in the current round, and consequently how these 6 bad balls are split in the current round have no bearing on that in the next round. 

Building on the example above, we now consider $m_{9,6}$, the transition probability from State $9$ to State $6$ (throwing 9 balls into 255 bins and ending up with 6 bad balls).  $m_{9,6}$ is simply the sum of the probabilities of these four cases, each of which has a very different formula than the others.  In general, the number of such cases, and hence the number of individual probability terms to be added up to arrive at the transition matrix element $m_{i,j}$, grows exponentially with the value of $j$. This does not however make it difficult to calculate the values of $M$, because there is a recursive structure, among the values of the matrix elements $m_{i,j}$, that can be exploited using dynamic programming, as will be elaborated shortly.

To simplify our analysis, we split each composite state into sub-composite states based on the number of nonempty bins: Let State $(j,k)$ denotes the sub-composite state with $j$ remaining distinct elements and $k$ nonempty bins, which is also a substate of State $j$. Let $m_{i,j}^{(k)}$ denote the probability of transition from State $i$ to State $(j,k)$, which is also the probability that after throwing $i$ balls uniformly and independently into $n$ bins, $i-j$ bins are ``good'' bins and $k$ bins are nonempty bins (thus $k-(i-j)$ bins are ``bad'' and $n-k$ bins are empty). The probability of transition to a composite state is simply the summation of the probabilities of the transitions to corresponding sub-composite states:

To obtain the transition matrix $M$, it is sufficient to compute $m^{(k)}_{i,j}$, which can be exploited using dynamic programming. Note that the balls-and-bins model itself can be considered as a Markov chain, in which a recursive relation exists: After throwing $i$ balls into $n$ bins, throwing one more ball randomly could be: (1) Into an empty bin and turn it to a ``good'' bin; (2) Into a ``good'' bin and turn it to a ``bad'' bin with two balls; or (3) Into a ``bad'' bin and keep it as the same. Mathematically, we have $m^{(k)}_{i+1,j}$ equals to


====================================


%{\bf (may be unnecessary) Note that both the success probability and the overall communication overhead are strictly increasing w.r.t. $n$ and $t$. Hence, instead of computing all values in the table, we could strategically compute only a few of them and obtain the optimal $(n,t)$ (e.g., find the optimal $t$ for each $n$ by binary search each column).}





\begin{comment}

As we explained in \autoref{subsec:protocol2}, $d_1$, the number of distinct elements in group pair $1$, is a random variable that follows a Binomial distribution $Binomial(d,1/g)$. So the probability that the group pair is completely reconciled in $r$ rounds is $\sum_{x=0}^d Pr[d_1=x]\cdot Pr[x\xrsquigarrow{r} 0]$.
%, where $\mathcal{B}(\cdot;d,1/g)$ is the probability mass function (PMF) of $Binomial(d,1/g)$. 
To ease computation, we slightly underestimate this probability by assuming $Pr[x\xrsquigarrow{r} 0]=0$ when $x>t$ (i.e., assume group pair $1$ cannot be reconciled if $d_i>t$, discussed in \autoref{sec:BCH_exception}). The loss of this underestimation is very tiny, since the coefficient of $Pr[x\xrsquigarrow{r} 0]$ (i.e., $Pr[d_1=x]$) is very small when $x>t$. We denote this underestimated probability as $\alpha$ (i.e., $\alpha=\sum_{x=0}^t Pr[d_1=x]\cdot Pr[x\xrsquigarrow{r} 0]$). Note that $Pr[x\xrsquigarrow{r} 0]$ is a function of $n$ and $r$ for arbitrary $x$, so $\alpha$ is a function of $n$, $r$, $t$ for arbitrary $d$ and $g$. 


\subsection{Tail Bound Analysis for Each Group Pair}\label{sec:tail_bound_per_group}

In this section, we focus on analyzing an arbitrary group pair, which we denote as $(A',B')$, and suppose their set difference $A'\Delta B'$ contains exactly $x$ elements. We only consider the case that the error-correct capability is sufficient (i.e., $x\leq t$). As we described in \autoref{sec:multi-rounds}, the $x$ distinct elements are hashed into $n$ subset pairs in the first round, and a distinct element is reconciled if and only if it is hashed into a subset pair that contains only $1$ distinct element. The distinct elements that have been reconciled in the first round are removed and the other distinct elements (i.e., the ones that have not been reconciled yet in the first round) will be hashed again in the second round using a different hash function, so on so force. 


% WLOG, we only analyze group pair $1$. {\bf Maybe say that we focus on an arbitrary group pair, which we denote as A' and B', and suppose their difference $ ... $ contains exactly $x$ elements}. 
% %The analysis for other group pairs is the same. 
% {\bf Please use x, not d}.  
% For the moment, we slightly abuse the notation and use $d$ to denote the number of distinct elements in group pair $1$ (i.e., $d_1$). In this section, we only consider the case that the error-correct capability is sufficient (i.e., $d\leq t$). As we described in \autoref{sec:multi-rounds}, the $d$ distinct elements of group pair $1$ are hashed into $n$ subset pairs in the first round, and a distinct element is reconciled if and only if it is hashed into a subset pair that contains only $1$ distinct element. The distinct elements that have been reconciled in the first round are removed and the other distinct elements (i.e., the ones that have not been reconciled yet in the first round) will be hashed again in the second round using a different hash function, so on so force. 

==========
{\bf The following may be useful in explaining why it is a Markov chain:} [Note there is no need to distinguish these four cases in calculating the ``transitioning out" probability (i.e., from state 6 to a small state say State 0), because the next round of balls-into-bins operation uses a different hash function independent of that used in the current round, and consequently how these 6 bad balls are split in the current round have no bearing on that in the next round.]  {\bf unless you have done so earlier}

{\bf we have an example at the end of multi-round PBS}
==========


As we explained in \autoref{sec:hash_partition}, how the $x$ distinct elements are distributed into $n$ subset pairs in the first round follows the familiar {\it balls-into-bins} probability model: Each of the $x$ balls are thrown independently and uniformly at random into one of the $n$ bins. Each distinct element that is reconciled in the first round corresponds to a ball that ends up in a bin that receives exactly $1$ ball. We call the ball and the bin ``good'' in the sequel; Each distinct element that has not been reconciled yet in the first round corresponds to a ball that ends up in a bin that receives multiple balls. We call the ball and the bin ``bad'' in the sequel. Note that balls are either ``good'' or ``bad'', but bins could be empty besides ``good'' and ``bad''.



The ``bad'' balls in the first round will be the balls to be thrown in the second round. The ``bad'' balls in the second round will be the balls to be thrown in the third round, so on so force. In all rounds, how the balls are thrown into $n$ bins follows the balls-into-bins model. The dynamics of the number of balls to be thrown in each round can be modeled as a Markov chain, in which each state is defined as the number of balls to be thrown. In the Markov chain, a transition from state $i$ to state $j$ ($i\geq j$) means $i-j$ out of $i$ balls are ``good'' balls and the other $j$ balls are ``bad'' balls. The {\it absorbing state} of this Markov chain is state $0$, which is the ``good'' state that means all distinct elements have been reconciled (i.e., reconciliation is complete). For our analysis, the only probability that we concerned is $Pr[x\xrsquigarrow{r} 0]$, the probability that state $x$ (initial state) reaches the absorbing state (i.e., state $0$) in $r$ transitions, which is also the probability that all distinct elements are reconciled in $r$ rounds. This probability can be easily calculated given the transition matrix of the Markov chain: Let $M$ denote the $(t+1)\times (t+1)$ transition matrix of the Markov chain.
%, where $M(i,j)$ (i.e., the entry in the $i^{th}$ row and the $j^{th}$ column of $M$) is the probability of transition from state $i$ to state $j$ for $i,j = 0,1,...,t$
$Pr[x\xrsquigarrow{r} 0]$ equals to $\big{(}M^r\big{)}(x,0)$ (i.e., the entry in the $x^{th}$ row and the $0^{th}$ column of $M^r$). Here we slightly abuse the row / column numbers of a $(t+1)\times (t+1)$ matrix from $1,2,...,t+1$ to $0,1,...,t$, since the state of the Markov chain ranges from $0$ to $t$. 

\subsubsection{How to compute \texorpdfstring{$M$}{M}}

The only problem left to obtain $Pr[x\xrsquigarrow{r} 0]$ is how to compute $M$, which is not straightforward, since each state $j$ (after-transition state) with $j>3$ in the Markov chain is a composite state as far as the calculation of the transition probability from a (larger) state $i$ $(>j)$ to $j$ is concerned. To calculate the probability, we have to break state $j$ down into ``atom'' states, calculate the transition probability from state $i$ to each of the ``atom'' states (which can be directly calculated), and then add them up. {\bf Note that we always view state $i$ (pre-transition state) as a simple state, since how the $i$ balls are placed into $n$ bins only depends on a hash function that is independent of the ones used in previous rounds.}

Each composite state $j$ can be broken down into atom states based on how these $j$ bad balls are placed into the $n$ bins. For example, state $6$ consists of $4$ atom states. The first one is $6 = 6$, where all $6$ bad balls are in the same bad bin. The second one is $6 = 2 + 4$ where, out of the $6$ bad balls, four are in one bad bin and the other two are in the other bad bin.  Similarly, the other two atom states are $6 = 3 + 3$ and $6 = 2 + 2 + 2$. The transition probability from state $i$ to any atom state can be directly calculated, but the problem is that the number of atom states grows exponentially with the number of ``bad'' balls $j$.

We notice that we can break each composite state into a small number of coarse-grained sub-states, each of which may still contain a large number of atom states. The transition probability from a (larger) state $i$ to any sub-state is still hard to compute. However, there is a recurrence relation among them, so we can compute the transition probabilities from any state to any sub-state using Dynamic Programming. 




% Each ``atom'' state is, in combinatorics terms, {\it a permutation of a combination of $j$}, which here corresponds to 
% how these $j$ ``bad'' balls are placed into the $n$ bins. 
% For a simple example, when $j = 4$ and $n = 7$, the vector $(2, 0, 0, 0, 0, 2, 0)$ is such an ``atom'' state, which corresponds to these $7$ bins (in a predefined order such as the natural order) 
% have $2$, $0$, $0$, $0$, $0$, $2$, and $0$ ``bad'' balls in it respectively. The transition probability from state $i$ to any atom state can be calculated, but the problem is that the number of atom states 
% (permutations of combinations) grow exponentially with the number of balls $j$.


+++++++++++

The only problem left to obtain $Pr[d\xrsquigarrow{r} 0]$ is how to compute $M$, which is not straightforward, since each state $j$ with $j>3$ in the Markov chain is a composite state as far as the calculation of the transition probability from a (larger) state $i$ $(>j)$ to $j$ (i.e., ``transitioning into'') is concerned.   {\bf You need to explain why it is not straightforward:  The reason you offer is not
the direction reason.  Instead you may say that "the transition probability between these composite states cannot be directly calculated" ...  to calculate it we have to break it down into "atom" states}

Each composite state $i$ can be broken down into atom states as follows.  Each simple state is, in combinatorics terms, {\it a permutation of a combination of $i$}, which here corresponds to 
how these $i$ balls are ``divided up" by the $n$ bins.   {\bf Liang, Read Mitzenmacher and Upfal book
for a better word for "divided up"}
For a simple example, when $i = 4$ and $n = 7$, the vector (1, 0, 1, 0, 0, 2, 0) is such a simple state, which corresponds to these 7 bins (in a predefined order such as the natural order) 
have 1, 0, 1, 0, 0, 2, and 0 balls in it respectively.   The transition probability between any two atom states can be ...    but the problem is that the number of atom states 
(permutations of combinations) grow exponentially with the number of balls $i$.

Consider two states i1 and i2 each broken down into millions of atom states.  Then the transition probability between these states is the summation of the trillions (= millions * millions) of 
transition probabilities between atom states of i1 and atom states of i2.  

The good thing is that the transition probability matrix among the (humongous number of atom states) induces a "subproblem structure ????", which leads to the recurrence relation, 
dynamic programming.   

We notice that we can break each state into a small number of coarse-grained substates, each of which may still contain a large number of atom states.  The transition probability 
between any two such substates are still hard to compute.  However, there is a recurrence relation among them ...

+++++++++++

To solve the problem, we partition the composite state into sub-states, so that the transition probability to the composite state is the summation of the transition probabilities to each of the sub-states. On the other hand, the transition probabilities to the sub-state have a recurrence relation and can be computed using Dynamic Programming. 

======================================

Note that every state $j$ with $j > 3$ in the Markov chain is a composite state as far as the calculation of the transition probability from a (larger) state $i > j$ to $j$ (i.e., ``transitioning into").  For example, State 6 contains 4 different cases. The first case is $6 = 6$, where all 6 bad balls are in the same bad bin. The second case is $6 = 2 + 4$ where, out of the 6 bad balls, four are in one bad bin and the other two are in the other bad bin.  Similarly, the other two cases are $6 = 3 + 3$ and $6 = 2 + 2 + 2$. Note there is no need to distinguish these four cases in calculating the ``transitioning out" probability (i.e., from state 6 to a small state say State 0), because the next round of balls-into-bins operation uses a different hash function independent of that used in the current round, and consequently how these 6 bad balls are split in the current round have no bearing on that in the next round. 

Building on the example above, we now consider $m_{9,6}$, the transition probability from State $9$ to State $6$ (throwing 9 balls into 255 bins and ending up with 6 bad balls).  $m_{9,6}$ is simply the sum of the probabilities of these four cases, each of which has a very different formula than the others.  In general, the number of such cases, and hence the number of individual probability terms to be added up to arrive at the transition matrix element $m_{i,j}$, grows exponentially with the value of $j$. This does not however make it difficult to calculate the values of $M$, because there is a recursive structure, among the values of the matrix elements $m_{i,j}$, that can be exploited using dynamic programming, as will be elaborated shortly.

To simplify our analysis, we split each composite state into sub-composite states based on the number of nonempty bins: Let State $(j,k)$ denotes the sub-composite state with $j$ remaining distinct elements and $k$ nonempty bins, which is also a substate of State $j$. Let $m_{i,j}^{(k)}$ denote the probability of transition from State $i$ to State $(j,k)$, which is also the probability that after throwing $i$ balls uniformly and independently into $n$ bins, $i-j$ bins are ``good'' bins and $k$ bins are nonempty bins (thus $k-(i-j)$ bins are ``bad'' and $n-k$ bins are empty). The probability of transition to a composite state is simply the summation of the probabilities of the transitions to corresponding sub-composite states:

To obtain the transition matrix $M$, it is sufficient to compute $m^{(k)}_{i,j}$, which can be exploited using dynamic programming. Note that the balls-and-bins model itself can be considered as a Markov chain, in which a recursive relation exists: After throwing $i$ balls into $n$ bins, throwing one more ball randomly could be: (1) Into an empty bin and turn it to a ``good'' bin; (2) Into a ``good'' bin and turn it to a ``bad'' bin with two balls; or (3) Into a ``bad'' bin and keep it as the same. Mathematically, we have $m^{(k)}_{i+1,j}$ equals to


====================================

More specifically, let state $(j,k)$ denote the sub-state of state $j$ that the $j$ ``bad'' balls end up to occupy exactly $k$ ``bad'' bins. Then the composite state $j$ is partitioned into state $(j,1)$, state $(j,2)$, $...$, state $(j,j)$. We slightly abuse the notation and let $M(i,j,k)$ denote the probability of transition from state $i$ to state $(j,k)$, then we have 

\begin{equation}
    M(i,j) = \sum_{k=1}^{j} M(i,j,k)
\end{equation}

{\bf we can use a tighter range of $k$ of $1,2,..., \lfloor j/2 \rfloor$. For cleanness, I choose a wider range of $1,2,..., j$, which is easier to understand and does not change the result}

To obtain $M$, it is sufficient to compute $M(i,j,k)$ for $\forall i,j,k=0,1,...,t$
{\bf Similarly, there is a tighter range for $i,j,k$, which seems to be unnecessary}
. Note that the state transition resulting from throwing one ball after another is also a Markov chain, in which state $(i,j,k)$ is defined as $j$ ``bad'' balls ending up into $k$ ``bad'' bins after throwing $i$ balls into $n$ bins. In this Markov chain, throwing one more ball can transition state $(i,j,k)$ to three possible states depending on the $(i+1)^{th}$ ball ending up in (1) a ``good'' bin; (2) a ``bad'' bin; or (3) an empty bin. The first case happens with probability $(i-j)/n$, results in $2$ additional ``bad'' balls and $1$ additional ``bad'' bin (i.e., transition to state $(i+1,j+2,k+1)$). The second and third cases transition to state $(i+1,j+1,k)$ and state $(i+1,j,k)$ respectively with probability $k/n$ and $1-(i-j+k)/n$. In the opposite direction, state $(i+1,j,k)$ can only be transitioned from (1) state $(i,j-2,k-1)$; (2) state $(i,j-1,k)$; and (3) state $(i,j,k)$, which gives us a recurrence relation that $M(i+1,j,k)$ equals to

%The second case happens with probability $k/n$ and results in state $(i+1,j+1,k)$. The third case happens with probability $1-(i-j+k)/n$ and results in state $(i+1,j,k)$. In the opposite direction, state $(i+1,j,k)$ can be transitioned from (1) state $(i,j-2,k-1)$ with probability $(i-j+2)/n$; (2) state $(i,j-1,k)$ with probability $k/n$; or (3) state $(i,j,k)$ with probability $1-(i-j+k)/n$. It gives us a recurrence relation that $P(i+1,j,k)$ equals to

\begin{equation}\label{eq:recursion}
    \frac{i\!-\!j\!+\!2}{n}\cdot M(i,j\!-\!1,k\!-\!1)+\frac{k}{n}\cdot M(i,j\!-\!1,k)+(1\!-\!\frac{i\!-\!j\!+\!2}{n})\cdot M(i,j,k)
\end{equation}

The three terms in \autoref{eq:recursion} corresponds to the above three possible transitions. Combining with the following probabilities in base cases, we can compute $M(i,j,k)$ for $\forall i,j,k=0,1,...,t$ using Dynamic Programming and obtain $M$:

\begin{align}
M(0,j,k) =& \left\{ \begin{array}{ccl}
1, & \mbox{if }
 j=k=0 \\ 0, & \mbox{otherwise} 
\end{array}\right.\label{eq:basic1}\\
M(i,0,k) =& \left\{ \begin{array}{ccl}
\binom{n}{i}/n^i, & \mbox{if }
 k=0 \\ 0, & \mbox{otherwise} 
\end{array}\right.\label{eq:basic2}\\
M(i,j,0) =& \left\{ \begin{array}{ccl}
1, & \mbox{if }
 j=0 \\ 0, & \mbox{otherwise} 
\end{array}\right.\label{eq:basic3}
\end{align}

%As mentioned earlier, we slightly abuse the notation `$d$' in this section to denote the number of distinct elements in group pair $1$, which is actually $d_1$ defined in \autoref{subsec:protocol2}. Now we recover the abused notation $d$ to denote the total number of distinct elements in all groups. 

As we explained in \autoref{subsec:protocol2}, $d_1$, the number of distinct elements in group pair $1$, is a random variable that follows a Binomial distribution $Binomial(d,1/g)$. So the probability that the group pair is completely reconciled in $r$ rounds is $\sum_{x=0}^d Pr[d_1=x]\cdot Pr[x\xrsquigarrow{r} 0]$.
%, where $\mathcal{B}(\cdot;d,1/g)$ is the probability mass function (PMF) of $Binomial(d,1/g)$. 
To ease computation, we slightly underestimate this probability by assuming $Pr[x\xrsquigarrow{r} 0]=0$ when $x>t$ (i.e., assume group pair $1$ cannot be reconciled if $d_i>t$, discussed in \autoref{sec:BCH_exception}). The loss of this underestimation is very tiny, since the coefficient of $Pr[x\xrsquigarrow{r} 0]$ (i.e., $Pr[d_1=x]$) is very small when $x>t$. We denote this underestimated probability as $\alpha$ (i.e., $\alpha=\sum_{x=0}^t Pr[d_1=x]\cdot Pr[x\xrsquigarrow{r} 0]$). Note that $Pr[x\xrsquigarrow{r} 0]$ is a function of $n$ and $r$ for arbitrary $x$, so $\alpha$ is a function of $n$, $r$, $t$ for arbitrary $d$ and $g$. 

\subsection{Tail Bound Analysis for all groups}\label{sec:times2bound}

Given $\alpha$, the tail bound of the probability that a group pair is successfully reconciled in $r$ rounds, we can easily derive a tail bound of $\alpha^g=1-(1-\alpha^g)$ for the probability that all group pairs are successfully reconciled in $r$ rounds, if we assume the reconciliations on group pairs are independent with each other. However, this assumption is not rigorous, since $d_1, d_2,...,d_g$ have a weak correlation that $\sum_{i=1}^g d_i=d$. 
%Fortunately, we have Times-2-Bound (Theorem 1 in \cite{hua2008rank}) to decouple the weak correlation and give us a rigorous tail bound of $1-2(1-\alpha^g)$ for the probability of all group pairs. 
To be rigorous, we use so-called Times-2-bound (Corollary 5.11 in \cite{upfal2005probability}) to decouple the weak correlation and obtain a rigorous tail bound of $1-2(1-\alpha^g)$ for the probability of all group pairs.
In \autoref{sec:parameter_settings}, we use the tail bound of $1-2(1-\alpha^g)$ in parameter settings for rigorousness. 

% More specifically, let state $(j,k)$ denote the sub-state of state $j$ that the $j$ ``bad'' balls end up to occupy exactly $k$ ``bad'' bins. Then the composite state $j$ is the union of state $(j,1)$, state $(j,2)$, $...$, state $(j,\lfloor j/2 \rfloor)$ (each ``bad'' bin receives at least $2$ ``bad'' balls, so $k\leq \lfloor j/2\rfloor$). Let $P(i,j,k)$ denote the probability of transition from state $i$ to state $(j,k)$, then we have 

% \begin{equation}
%     M(i,j) = \sum_{k=1}^{\lfloor j/2\rfloor} P(i,j,k)
% \end{equation}






% Note that each state $j$ with $j>3$ in the Markov chain is a composite state as far as the calculation of the transition probability from a (larger) state $i$ $(>j)$ to $j$ (i.e., ``transitioning into''). Such a composite state $j$ can be decomposed into sub-states based on the number of ``bad'' bins after throwing $i$ balls: Define state $(j,k)$ as the sub-state of state $j$ that the  $j$ ``bad'' balls end up to occupy exactly $k$ ``bad'' bins. Then state $j$ is the union of all states $(j,k)$ for $k=1,2,...$ (each ``bad'' bin receives at least $2$ ``bad'' balls). Let $m_{i,j}^{(k)}$ denote the probability of transition from state $i$ to state $(j,k)$
% %, which is also the probability that after throwing $i$ balls uniformly and independently into $n$ bins, $i-j$ bins are ``good'' bins and $k$ bins are nonempty bins (thus $k-(i-j)$ bins are ``bad'' and $n-k$ bins are empty)
% . The probability of transition to the composite state $j$ is simply the summation of the probabilities of the transitions to corresponding sub-states: 

% \begin{equation}
%     m_{i,j} = \sum_{k=i}^{i-j} m^{(k)}_{i,j}
% \end{equation}


% To make our description simple, we call a bin that receives exactly $1$ ball a ``good'' bin is ``good'' if and only if it receives exactly $1$ ball. We call a bin is ``bad'' if and only if it receives more than $1$ balls. The rest bins (i.e., neither ``good'' nor ``bad'') are empty. We call a ball ending up in a ``good'' bin is ``good'' if it is in a ``good bin'' Then the distinct elements that are decoded correspond to the balls that are in ``good'' bins. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Old version of 2/5
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{comment}

In this section, we only consider the cases that a group is able to be decoded by BCH code (i.e., initially contains at most $t$ set differences). Without loss of generosity, we assume the group has $d (\leq t)$ distinct elements and is partitioned into $n$ subset pairs. As we described in \autoref{sec:hash_partition}, the $d$ distinct elements are hashed into $n$ subset pairs in each round, and a distinct element is decoded if and only if it is hashed into a subset pair that contains only $1$ distinct element. As we introduced in \autoref{sec:hash_partition}, the statistical model for hashing $d$ distinct elements into $n$ subset pairs is the same as the classical balls-and-bins problem: $d$ balls are thrown independently and uniformly at random into $n$ bins. To make our description simple, we call a bin is ``good'' if and only if it receives exactly $1$ ball. And we call a bin is ``bad'' if and only if it receives more than $1$ balls. The rest bins (i.e., neither ``good'' nor ``bad'') are empty. Then the distinct elements that are decoded correspond to the balls that are in ``good'' bins. 

The decode process of each group can be considered as a Markov Chain, in which each state is defined as the number of remaining distinct elements (i.e., the distinct elements that haven't been decoded). In this Markov chain, the transition from State $i$ to State $j$ means $i-j$ out of $i$ distinct elements are decoded in this round, where $0\leq j\leq i\leq t$. Use the same analogy, the number (state) is simply the total number of balls that fall in ``bad'' bins. The transition from State $i$ to State $j$ means $i-j$ out of $i$ balls fall in ``good'' bins in this round, while the rest $j$ balls fall in ``bad'' bins. State $0$ is the {\it absorbing} state of this Markov Chain, which means all distinct elements have been reconciled. For our analysis, we only concern the probability that after $r$ rounds, the final state is state $0$ (i.e., absorbing state) when the initial state is state $i$. We denote this probability as $v^{(r)}_i(0)$.

Let $M=(m_{i,j})_{(t+1)\times (t+1)}$ denote the transition matrix of the above Markov chain, where $m_{i,j}$ is the probability of transition from State $i$ to State $j$. Given $M$, $r$, and the initial state $i$, $v^{(r)}_i(0)$ can be easily calculated. So the only problem is how to obtain $M$, which will be elaborated in the next section.

\subsubsection{Transition Matrix}\label{sec:transition_matrix}

Now we describe how to compute the transition matrix $M$ using dynamic programming in detail. Note that every State $j$ with $j > 3$ in the Markov chain is a composite state as far as the calculation of the transition probability from a (larger) state $i > j$ to $j$ (i.e., ``transitioning into").  For example, State 6 contains 4 different cases. The first case is $6 = 6$, where all 6 bad balls are in the same bad bin. The second case is $6 = 2 + 4$ where, out of the 6 bad balls, four are in one bad bin and the other two are in the other bad bin.  Similarly, the other two cases are $6 = 3 + 3$ and $6 = 2 + 2 + 2$. Note there is no need to distinguish these four cases in calculating the ``transitioning out" probability (i.e., from state 6 to a small state say State 0), because the next round of balls-into-bins operation uses a different hash function independent of that used in the current round, and consequently how these 6 bad balls are split in the current round have no bearing on that in the next round. 

Building on the example above, we now consider $m_{9,6}$, the transition probability from State $9$ to State $6$ (throwing 9 balls into 255 bins and ending up with 6 bad balls).  $m_{9,6}$ is simply the sum of the probabilities of these four cases, each of which has a very different formula than the others.  In general, the number of such cases, and hence the number of individual probability terms to be added up to arrive at the transition matrix element $m_{i,j}$, grows exponentially with the value of $j$. This does not however make it difficult to calculate the values of $M$, because there is a recursive structure, among the values of the matrix elements $m_{i,j}$, that can be exploited using dynamic programming, as will be elaborated shortly.

To simply our analysis, we split each composite state into sub-composite states based on the number of nonempty bins: Let State $(j,k)$ denotes the sub-composite state with $j$ remaining distinct elements and $k$ nonempty bins, which is also a substate of State $j$. Let $m_{i,j}^{(k)}$ denote the probability of transition from State $i$ to State $(j,k)$, which is also the probability that after throwing $i$ balls uniformly and independently into $n$ bins, $i-j$ bins are ``good'' bins and $k$ bins are nonempty bins (thus $k-(i-j)$ bins are ``bad'' and $n-k$ bins are empty). The probability of transition to a composite state is simply the summation of the probabilities of the transitions to corresponding sub-composite states:

\begin{equation}
    m_{i,j} = \sum_{k=i}^{i-j} m^{(k)}_{i,j}
\end{equation}

To obtain the transition matrix $M$, it is sufficient to compute $m^{(k)}_{i,j}$, which can be exploited using dynamic programming. Note that the balls-and-bins model itself can be considered as a Markov chain, in which a recursive relation exists: After throwing $i$ balls into $n$ bins, throwing one more ball randomly could be: (1) Into an empty bin and turn it to a ``good'' bin; (2) Into a ``good'' bin and turn it to a ``bad'' bin with two balls; or (3) Into a ``bad'' bin and keep it as the same. Mathematically, we have $m^{(k)}_{i+1,j}$ equals to

\begin{equation}\label{eq:recursion}
\frac{n-k+1}{n}\cdot m^{(k-1)}_{i,j-1} + \frac{j+1}{n}\cdot m^{(k)}_{i,j+1} + \frac{k-(i-j)}{n}\cdot m^{(k)}_{i,j} \nonumber
\end{equation}

The three terms in \autoref{eq:recursion} corresponds to the above three cases. Meanwhile, we can easily get the boundary conditions as follows:

\begin{align}
m^{(k)}_{i,0} =& \left\{ \begin{array}{ccl}
\binom{n}{i}/n^i, & \mbox{if }
 k=i \\ 0, & \mbox{otherwise} 
\end{array}\right.\label{eq:basic1}\\
m^{(k)}_{0,j} =& \left\{ \begin{array}{ccl}
1, & \mbox{if }
 k=0 \mbox{ and } j=0 \\ 0, & \mbox{otherwise} 
\end{array}\right.\label{eq:basic2}\\
m^{(0)}_{i,j} =& \left\{ \begin{array}{ccl}
1, & \mbox{if }
 i=0 \mbox{ and } j=0 \\ 0, & \mbox{otherwise} 
\end{array}\right.\label{eq:basic3}
\end{align}

Using \autoref{eq:recursion},\autoref{eq:basic1},\autoref{eq:basic2}, and \autoref{eq:basic3}, we can recursively compute $m^{(k)}_{i,j}$ and obtain $M$.


\subsection{Global Tail Bound Analysis}\label{sec:times2bound}

Consider group $1$ (other groups have the same result), the probability that all distinct elements in group $1$ are reconciled in $r$ rounds is $\sum_{i=0}^d Pr[d_1=i]v_i^{(r)}(0)\triangleq \alpha$, where $d_1$ (i.e., the number of distinct elements in group $1$) is a Binomial random variable $Binomial(d,1/g)$ as we explained in \autoref{subsec:protocol2}. To ease computation, we slightly underestimate this probability $\alpha$ by assuming $v_i^{(r)}(0)=0$ when $i>t$ (i.e., assume group $i$ cannot reconcile if $d_i>t$, discussed in \autoref{sec:BCH_exception}). The loss of this underestimation is very tiny, since the coefficient of $v_i^{(r)}(0)$ (i.e., $Pr[d_1=i]$) is very small when $i>t$.

The probability that all groups are successfully reconciled in $r$ rounds is simply $\alpha^g\triangleq \beta$, if we assume the reconciliations on groups are independent with each other. This assumption is however not rigorous, since $d_1, d_2,...,d_g$ have a weak correlation that $\sum_{i=1}^g d_i=d$. Fortunately, we have Times-2-Bound (Theorem 1 in \cite{hua2008rank}) to decouple the weak correlation and give us a rigorous bound of $2\beta-1$. In \autoref{sec:parameter_settings}, we use this rigorous bound for parameter settings. 

\end{comment}






\begin{comment}

Let $v^{(r)}_i=\big{(}{v^{(r)}_i(0), v^{(r)}_i(1),...,v^{(r)}_i(t)}\big{)}$ denote the probability vector (i.e., $\sum_{j=0}^{t}v^{(r)}_i(j) = 1$) after $r$ rounds with initial State $i$: $v^{(r)}_i(j)$ denotes the probability that the final state is State $j$ after $r$ rounds. In the probability vector, $v^{(r)}_i(0)$ is the only entry that we concern, which is the probability of the cases that all distinct elements are decoded after $r$ rounds. Given 

Note that every State $j$ with $j > 3$ in the Markov chain is a composite state as far as the calculation of the transition probability from a (larger) state $i > j$ to $j$ (i.e., ``transitioning into").  For example, State 6 contains 4 different cases. The first case is $6 = 6$, where all 6 bad balls are in the same bad bin. The second case is $6 = 2 + 4$ where, out of the 6 bad balls, four are in one bad bin and the other two are in the other bad bin.  Similarly, the other two cases are $6 = 3 + 3$ and $6 = 2 + 2 + 2$. Note there is no need to distinguish these four cases in calculating the ``transitioning out" probability (i.e., from state 6 to a small state say State 0), because the next round of balls-into-bins operation uses a different hash function independent of that used in the current round, and consequently how these 6 bad balls are split in the current round have no bearing on that in the next round. 

Building on the example above, we now consider $m_{9,6}$, the transition probability from State $9$ to State $6$ (throwing 9 balls into 255 bins and ending up with 6 bad balls).  $m_{9,6}$ is simply the sum of the probabilities of these four cases, each of which has a very different formula than the others.  In general, the number of such cases, and hence the number of individual probability terms to be added up to arrive at the transition matrix element $m_{i,j}$, grows exponentially with the value of $j$. This does not however make it difficult to calculate the values of $M$, because there is a recursive structure, among the values of the matrix elements $m_{i,j}$, that can be exploited using dynamic programming, as will be elaborated in \autoref{sec:transition_matrix}.

Let $v^{(r)}_i=\big{(}{v^{(r)}_i(0), v^{(r)}_i(1),...,v^{(r)}_i(t)}\big{)}$ denote the probability vector (i.e., $\sum_{j=0}^{t}v^{(r)}_i(j) = 1$) after $r$ rounds with initial State $i$: $v^{(r)}_i(j)$ denotes the probability that the final state is State $j$ after $r$ rounds. In the probability vector, $v^{(r)}_i(0)$ is the only ``good'' entry, which is the probability of the cases that all distinct elements are decoded after $r$ rounds. The probability of the group does not complete reconciliation is simply $1-v^{(r)}_i(0)$. 

Given the transition matrix $M$, we can easily compute the probability vector $v^{(r)}_i$ for any $r$ and $i$ as follows:
\begin{equation}
    x^{(r)}_i = e_i\cdot M^r
\end{equation}
Here $\{e_i\}_{i=0,1,2,...,t}$ denote the standard basis vectors of length $t+1$, where $e_i$ has a single nonzero value 1 at the $(i+1)^{th}$ position. So the remaining problem is how to compute $M$.

\subsubsection{Transition Matrix}\label{sec:transition_matrix}

Now we describe how to compute the transition matrix $M$ using dynamic programming in detail. As we described earlier, every State $j$ with $j > 3$ in the Markov chain is a composite state that contains many different cases. And the number of these cases increases exponentially with the value of $j$. To simply our analysis, we split each composite state into sub-composite states based on the number of nonempty bins: Let State $(j,k)$ denotes the sub-composite state with $j$ remaining distinct elements and $k$ nonempty bins, which is also a substate of State $j$. Let $m_{i,j}^{(k)}$ denote the probability of transition from State $i$ to State $(j,k)$, which is also the probability that after throwing $i$ balls uniformly and independently into $n$ bins, $i-j$ bins are ``good'' bins and $k$ bins are nonempty bins (thus $k-(i-j)$ bins are ``bad'' and $n-k$ bins are empty). The probability of transition to a composite state is simply the summation of the probabilities of the transitions to corresponding sub-composite states:

\begin{equation}
    m_{i,j} = \sum_{k=i}^{i-j} m^{(k)}_{i,j}
\end{equation}

To obtain the transition matrix $M$, it is sufficient to compute $m^{(k)}_{i,j}$, which can be exploited using dynamic programming. Note that the balls-and-bins model itself can be considered as a Markov chain, in which a recursive relation exists: After throwing $i$ balls into $n$ bins, throwing one more ball randomly could be: (1) Into an empty bin and turn it to a ``good'' bin; (2) Into a ``good'' bin and turn it to a ``bad'' bin with two balls; or (3) Into a ``bad'' bin and keep it as the same. Mathematically, we have 

\begin{align}
m^{(k)}_{i+1,j} =& \frac{n-k+1}{n}\cdot m^{(k-1)}_{i,j-1} + \frac{j+1}{n}\cdot m^{(k)}_{i,j+1} \nonumber\\
&+ \frac{k-(i-j)}{n}\cdot m^{(k)}_{i,j} \label{eq:recursion}
\end{align}

The three terms in \autoref{eq:recursion} corresponds to the above three cases. Meanwhile, we can easily get the following probabilities for basic cases:

\begin{align}
m^{(k)}_{i,0} =& \left\{ \begin{array}{ccl}
\binom{n}{i}/n^i, & \mbox{if }
 k=i \\ 0, & \mbox{otherwise} 
\end{array}\right.\label{eq:basic1}\\
m^{(k)}_{0,j} =& \left\{ \begin{array}{ccl}
1, & \mbox{if }
 k=0 \mbox{ and } j=0 \\ 0, & \mbox{otherwise} 
\end{array}\right.\label{eq:basic2}\\
m^{(0)}_{i,j} =& \left\{ \begin{array}{ccl}
1, & \mbox{if }
 i=0 \mbox{ and } j=0 \\ 0, & \mbox{otherwise} 
\end{array}\right.\label{eq:basic3}
\end{align}

Using \autoref{eq:recursion},\autoref{eq:basic1},\autoref{eq:basic2}, and \autoref{eq:basic3}, we can recursively compute $m^{(k)}_{i,j}$ and then get $v^{(r)}_i(0)$ for $\forall i=0,1,...,n$ and $r\in\mathbb{Z}$. The value of $v^{(r)}_i(0)$ will be used to compute the tail bound of $Pr[P^{(r)}_o]$ in the next section. 

\subsection{Global Tail Bound Analysis}\label{sec:times2bound}

Let random variable $X^{(d)}_i, 1\leq i\leq g$, denote the number of set differences initially allocated in the $i^{th}$ group. For an analogy, the statistical model for hashing $d$ set differences into $g$ groups is also the same as the classical balls-and-bins problem: $d$ balls are thrown independently and uniformly at random into $g$ bins. Then random variable $X^{(d)}_i$ could be translated as the number of balls ended up in the $i^{th}$ bin after $d$ balls are thrown. Therefore, $(X^{(d)}_1,...,X^{(d)}_g)$ follows the multinomial distribution. The marginal distribution for any $X^{(d)}_i$ is $Binomial(d,\frac{1}{g})$, where $Binomial(N,p)$ denotes the binomial distribution resulting from $N$ trials with success probability $p$. 

Let $f^{(r)}(x_1,x_2,...,x_g)$ denote the probability that set reconciliation does not complete (for all groups) in $r$ rounds when the $i^{th}$ group initially contains $x_i$ set differences for $i=1,2,...,g$. Define $f^{(r)}(x)$ as the probability that set reconciliation does not complete in $r$ rounds when a group initially contains $x$ set differences. Based on the result in \autoref{sec:tail_bound_per_group}, we have 

% \begin{equation}\label{eq:frx}
%     f^{(r)}(x) \leq g^{(r)}(x) \triangleq \left\{ \begin{array}{ccc}
% 1-v^{(r)}_{x}(0) & \mbox{for}
% & 0\leq x\leq c \\ 1 & \mbox{for} & x>c
% \end{array}\right.
% \end{equation}

\begin{equation}\label{eq:frx}
    f^{(r)}(x) = 1-v^{(r)}_{x}(0) \mbox{ for }  0\leq x\leq t 
\end{equation}

Since the reconciliation processes independently for each group, we have 

\begin{equation}
f^{(r)}(x_1,x_2,...,x_g) = 1-\prod_{i=1}^g \big{(}1-f^{(r)}(x_i)\big{)}
\end{equation}

Then we have 

\begin{align} 
Pr[P^{(r)}_o] 
&= E[f^{(r)}(X^{(d)}_1,X^{(d)}_2,...,X^{(d)}_g)] \label{eq:errorBound0}\\
&= 1-E[\prod_{i=1}^g \big{(}1-f^{(r)}(X^{(d)}_i)\big{)}] \label{eq:errorBound1}
\end{align}

A naive approach to calculating the probability $Pr[P^{(r)}_o]$ is to regard $X^{(d)}_i$ as mutually independent. Then we have

\begin{align} 
Pr[P^{(r)}_o] 
&= 1-\prod_{i=1}^g E[1-f^{(r)}(X^{(d)}_i)] \label{eq:errorBound2}\\
&= 1-\prod_{i=1}^g (1-E[f^{(r)}(X^{(d)}_i)]) \label{eq:errorBound3}\\
&= 1-(1-E[f^{(r)}(X^{(d)}_i)])^g \label{eq:errorBound4}
\end{align}

And the term $E[f^{(r)}(X^{(d)}_1)]$ in \autoref{eq:errorBound4} can be easily bounded by \autoref{eq:frx} as follows:

\begin{align}
& E[f^{(r)}(X^{(d)}_1)]\\
= &\sum_{k=0}^d \mathcal{B}(k;d,\frac{1}{n})f^{(r)}(k)\\
= &\sum_{k=0}^t \mathcal{B}(k;d,\frac{1}{n})f^{(r)}(k) + \sum_{k=t+1}^d \mathcal{B}(k;d,\frac{1}{n})f^{(r)}(k)\label{eq:beforeLeq}\\
\leq & \sum_{k=0}^t \mathcal{B}(k;d,\frac{1}{n})f^{(r)}(k) + \sum_{k=t+1}^d \mathcal{B}(k;d,\frac{1}{n})\label{eq:afterLeq}\\
= & \sum_{k=0}^t \mathcal{B}(k;d,\frac{1}{n})\big{(}1-v_k^{(r)}(0)\big{)}+\sum_{k=t+1}^d \mathcal{B}(k;d,\frac{1}{n})
\end{align}

Here $\mathcal{B}(k;d,\frac{1}{n})$ is the Binomial probability mass function, and how to compute $v_k^{(r)}(0)$ is discussed in \autoref{sec:tail_bound_per_group} for $\forall k=0,1,...,t$ and $r\in\mathbb{Z}$. From \autoref{eq:beforeLeq} to \autoref{eq:afterLeq}, the loss is very negligible, since $\mathcal{B}(k;d,\frac{1}{n})$ is very small when $k>t$ ($t$ is $2-3$ times of $d/n$).

However, those random variable $X^{(d)}_i$ are not totally independent since they are conditioned by $\sum_{i=1}^g X^{(d)}_i=d$. So the above bound is not rigorous. Fortunately, we have the following theorem (Times-2-Bound) to decouple the weak correlation among $(X^{(d)}_1,...,X^{(d)}_m)$ and bound $Pr[P^{(r)}_o]$ rigorously to be $2$ times of the unrigorous bound in \autoref{eq:errorBound3}. 

\textbf{Theorem 1} {\bf citation}
Let $(X^{(n)}_1,...,X^{(n)}_m)$ follows the multinomial distribution of throwing $n$ balls into $m$ bins. Let $(Y^{(n)}_1,...,Y^{(n)}_m)$ be independent and identically distributed random variables with distribution $Poission(\frac{n}{m})$. Let $f(x_1,...,x_m)$ be a nonnegative function which is increasing in each argument separately. Then
\begin{equation} \label{eq:times2bound}
E[f(X^{(n)}_1,X^{(n)}_2,...,X^{(n)}_m)] \leq 2E[f(Y^{(n)}_1,Y^{(n)}_2,...,Y^{(n)}_m)]
\end{equation}


A naive approach to calculating the probability $Pr[P^{(r)}_o]$ is to regard $X^{(d)}_i$ as mutually independent. In this case, the production in the expectation of \autoref{eq:errorBound1} can be extracted out of the expectation and hence could be easily bounded. However, those random variable $X^{(d)}_i$ are not totally independent since they are conditioned by $\sum_{i=1}^m X^{(d)}_i=d$. Fortunately, we have the following theorem to decouple the weak correlation among $(X^{(d)}_1,...,X^{(d)}_m)$ and bound our targeted probability.

\textbf{Theorem 1}
Let $(X^{(n)}_1,...,X^{(n)}_m)$ follows the multinomial distribution of throwing $n$ balls into $m$ bins. Let $(Y^{(n)}_1,...,Y^{(n)}_m)$ be independent and identically distributed random variables with distribution $Poission(\frac{n}{m})$. Let $f(x_1,...,x_m)$ be a nonnegative function which is increasing in each argument separately. Then
\begin{equation} \label{eq:times2bound}
E[f(X^{(n)}_1,X^{(n)}_2,...,X^{(n)}_m)] \leq 2E[f(Y^{(n)}_1,Y^{(n)}_2,...,Y^{(n)}_m)]
\end{equation}

Substitute \autoref{eq:times2bound} into \autoref{eq:errorBound0}, we have
\begin{align} 
Pr[P^{(r)}_o] 
&= E[f^{(r)}(X^{(d)}_1,X^{(d)}_2,...,X^{(d)}_m)] \\
&\leq 2E[f^{(r)}(Y^{(d)}_1,Y^{(d)}_2,...,Y^{(d)}_m)] \\
&= 2-2E[\prod_{i=1}^m \big{(}1-f^{(r)}(Y^{(d)}_i)\big{)}] \\
&= 2-2\prod_{i=1}^m \big{(}1-E[f^{(r)}(Y^{(d)}_i)]\big{)} \label{eq:beforeSimp}\\
&= 2-2\big{(}1-E[f^{(r)}(Y^{(d)}_1)]\big{)}^m \label{eq:afterSimp}\\
\end{align}

From \autoref{eq:beforeSimp} to \autoref{eq:afterSimp}, we use the property that $Y^{(d)}_i$, $i=1,2,...,m$ are i.i.d random variables with distribution $Poisson(\delta)$ $(\delta = \frac{d}{m})$. And the term $E[f^{(r)}(Y^{(d)}_1)]$ in \autoref{eq:afterSimp} can be easily bounded by \autoref{eq:frx} as follows:

\begin{align}
& E[f^{(r)}(Y^{(d)}_1)]\\
= &\sum_{k=0}^d p(k;\delta)f^{(r)}(k)\\
= &\sum_{k=0}^c p(k;\delta)f^{(r)}(k) + \sum_{k=c+1}^d p(k;\delta)f^{(r)}(k)\label{eq:beforeLeq}\\
\leq & \sum_{k=0}^c p(k;\delta)f^{(r)}(k) + \sum_{k=c+1}^d p(k;\delta)\label{eq:afterLeq}\\
= & \sum_{k=0}^c p(k;\delta)\big{(}1-v_k^{(r)}(0)\big{)}+\sum_{k=c+1}^d p(k;\delta)
\end{align}

Here $p(k;\delta)$ is the Poisson probability mass function, and how to compute $v_k^{(r)}(0)$ is discussed in \autoref{sec:tail_bound_per_group} for $\forall k=0,1,...,c$ and $r\in\mathbb{Z}$. From \autoref{eq:beforeLeq} to \autoref{eq:afterLeq}, the loss is very negligible, since $p(k;\delta)$ is very small when $k>c$ ($c>2\delta$).


\subsection{Parameter Settings}\label{sec:parameter_settings}

% The tail bound is based on the total number of distinct elements $d$, which is however not known precisely. The ToW Estimator introduced in \autoref{subsec:ToW} can only provide an estimation of $d$ (denoted as $\hat{d}$). Note that the tail bound of $Pr[P^{(r)}_o]$ increases as $d$ increases. So overestimate $d$ will get us a larger failure probability $Pr[P^{(r)}_o]$. To ensure a high success probability, we use an overestimated number of distinct element $\bar{d}$ $(>\hat{d})$ for parameter settings, such that $\bar{d}\geq d$ with high probability. In our evaluation, we set $\bar{d}\triangleq 1.38\hat{d}$, such that $\bar{d}\geq d$ with probability $99\%$. 

In this section, we elaborate how to set the parameters (i.e., $n$, $t$, $g$) given $d$ and the objective $(r,p_0)$ (defined in \autoref{subsec:protocol2}) in PBS. For the moment, we assume $d$ is precisely known. 
Given the objective $(r, p_0)$
%(i.e., set reconciliation is complete in $r$ rounds with probability $p_0$) 
%depend on the requirement of specific applications)
, the parameter setting problem aims to find the optimal parameter settings on $n,t,g$ that minimizes the overall communication overhead, under the constraint that the tail bound of the success probability in $r$ rounds is larger than $p_0$. As explained in \autoref{subsec:protocol2}, $\delta$ should be a small number, so we fix $\delta=5$ and therefore $g=d/\delta$ is also fixed. Note that the only two components in the communication overhead per group (described in \autoref{sec:multi-rounds}) that depend on parameter settings are $t\log n+\delta\log n$. So we can formalize the parameter setting problem as the following optimization problem:

\begin{equation}
\min\limits_{n,t} t\log n+\delta\log n \quad \mbox{s.t.}\quad 1-2(1-\alpha^g(n,t))>p_0
\end{equation}

\begin{align}
\mbox{minimize} \quad
&
t\log n+\delta\log n \label{obj:min_communication}
\\
\mbox{subject to} \quad 
&
1-2(1-\alpha^g(n,t))>p_0  \label{eq:success_rate_requirement}
\\
&
n,t\in \mathbb{N}^+ \label{eq:row_sum_requirement}
\end{align}

This optimization problem seems to be very difficult to solve, since the constraint is a very comprehensive function of the parameters (remind that $\alpha=\alpha(n,t)$ is a function of $n$ and $t$ for arbitrary $r$, $d$, and $g$). However, we can narrow down the solution space into only a few combinations and traverse all these combinations to find the optimal parameter settings as follows: First, for BCH coding efficiency, we select $n$ to be $2^m-1$ for some integer $m$ and therefore narrow its range down to $\{63,127,255,511,1023\}$ (recall that $n=\Omega(\delta^2)$). Second, we select $t$ in the range from $1.5\delta$ to $3\delta$, as we suggested in \autoref{subsec:protocol2}. 

Here we use an example to show how we set parameters: Given $d=1000$, $r=3$, $p_0=0.99\%$, for each $(n,t)$ combination in $\{63,127,255,511,1023\}\times \{8,9,...,15\}$, we compute the tail bound of the success probability under the parameter settings and obtain the following table:

\begin{table}[h]
\centering
\caption{Tail bound of success probability}\label{tab:success_prob}
\begin{tabular}{@{}|c|c|c|c|c|c|@{}}
\hline 
\diagbox{$t$}{$n$}    & $63$ & $127$ & $255$ & $511$ & $1023$ \\ \hline 
8   & 0 & 25.5\% & 32.7\% & 34.3\% & 34.9\% \\ \hline
9   & 52.1\% & 78.0\% & 84.2\% & 85.7\% & 86.1\% \\ \hline
10  & 75.1\% & 92.7\% & 96.5\% & 97.4\% & 97.6\% \\ \hline
11  & 85.9\% & 96.9\% & \cellcolor{blue!25}99.1\% & \cellcolor{blue!25}99.5\% & \cellcolor{blue!25}99.6\% \\ \hline
12  & 91.3\% & 98.5\% & \cellcolor{blue!25}99.7\% & \cellcolor{blue!25}99.9\% & \cellcolor{blue!25}$>$99.9\% \\ \hline
13  & 93.9\% & \cellcolor{blue!25}99.1\% & \cellcolor{blue!25}99.8\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% \\ \hline
14  & 95.1\% & \cellcolor{blue!25}99.4\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% \\ \hline
15  & 95.6\% & \cellcolor{blue!25}99.5\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% \\ 
\hline 
\end{tabular}
\end{table}

In the table, all $(n,t)$ combinations in the blue cells satisfy the success probability requirement. Among them, $(127,13)$ has the lowest communication overhead ({\bf measured? quantized?} by $t\log n+\delta\log n$). So we set $n=127, t=13$ in this case. {\bf (may be unnecessary) Note that both the success probability and the overall communication overhead are strictly increasing w.r.t. $n$ and $t$. Hence, instead of computing all values in the table, we could strategically compute only a few of them and obtain the optimal $(n,t)$ (e.g., find the optimal $t$ for each $n$ by binary search each column).}

\end{comment}
\begin{comment}
If not, we use the ToW estimator described in \autoref{subsec:ToW} to obtain $\hat{d}$ (i.e., the estimation of $d$). Then scale it up (e.g., $d=1.38\hat{d}$ in \autoref{sec:evaluation}) for parameter setting, as explained in \autoref{subsec:ToW}. 

Here are the $4$ parameters that need to determine: 

\begin{itemize}
	\itemsep0em
	%\item $\delta$: Average number of distinct elements per group; 
	\item $g$: Number of group pairs; 
	\item $n$: Number of subset pairs in each group pair; 
	\item $r$: Number of rounds; 
	\item $t$: BCH decode capability;
\end{itemize}

Note that the number of groups $g$ is determined after $\delta$ is determined (i.e., $g=\frac{\bar{d}}{\delta}$). Now we describe how to set the four parameters using the tail bound. First, we set $\delta$ to be some small integer (e.g., $\delta=5$), so that the computational complexity (approx $\propto \delta^2$) is small. Second, we set $r$ to be some small integer (e.g., $r=3$), so that the round-trip delay is reasonable. Third, we set an objective success probability $p$ (depend on the requirement of specific applications), and we consider a parameter combination $(n,t)$ is {\it feasible} if and only if the success probability under this parameter setting based on the tail bound is larger than $p$. Among all feasible parameter combinations $(n,t)$, we select the one that has the lowest communication overhead, which can be roughly expressed as $(\delta \log u + t\log n + \delta \log n + 32)\cdot d/\delta$, as explained in \autoref{subsec:protocol2}. Here $u$ (i.e., the size of the element universe) and $d$ (i.e., the number distinct elements) do not depend on the parameter combination. So we only need to minimize $(t+\delta) \log n$ subject to $n$ and $t$. 
\end{comment}
\begin{comment}

\autoref{fig:mc} presents an example state transition diagram with 6 states (0 - 5 ``hidden elements''), denoting the corresponding transition matrix as $P=(p_{i,j})_{6\times 6}$, where $p_{i,j}$ is the probability of moving from State $i$ to State $j$. 

For instance, $p_{5,0}$ denotes the probability that all 5 set differences are decoded, which means the 5 set differences are all hashed into separate bins. $p_{5,2}$ denotes the probability that 3 (=5-2) out of 5 set differences are decoded, which means 3 set differences are hashed into separate bins and 2 set differences are hashed into the same bin. 


Let $L_{max}$ denote the maximum number of errors that BCH code can correct. Define $g^{(r)}(s)$ as follows:

\begin{equation}
    g^{(r)}(s) = \left\{ \begin{array}{ccc}
f^{(r)}(s) & \mbox{for}
& 0\leq s\leq L_{max} \\ 1 & \mbox{for} & s>L_{max}
\end{array}\right.
\end{equation}



Assume BCH code is capable of decode $s$ set differences, then the decode process of a group can be considered as a Markov chain, in which state is defined as the number of ``hidden elements'' (i.e., elements belonging to the set differences that haven't been decoded). \autoref{fig:mc} presents an example state transition diagram with 6 states (0 - 5 ``hidden elements''), denoting the corresponding transition matrix as $P=(p_{i,j})_{6\times 6}$, where $p_{i,j}$ is the probability of moving from State $i$ to State $j$. 

For instance, $p_{5,0}$ denotes the probability that all 5 set differences are decoded, which means the 5 set differences are all hashed into separate bins. $p_{5,2}$ denotes the probability that 3 (=5-2) out of 5 set differences are decoded, which means 3 set differences are hashed into separate bins and 2 set differences are hashed into the same bin. 
% And $p_{5,4}$ denotes the probability that only 1 (=5-4) set difference are decoded. The other 4 set differences could be either hashed into the same bin, or two separate bins with 2 elements in each. 

The transition in this Markov chain basically has three properties: (1) All state transitions are either self-loops or from ``higher'' states to ``lower'' states, since decode process won't generate additional set differences; (2) No state transition to State 1, because 1 remaining difference must be in a bin by itself and is able to be decoded within the same round of transition; (3) State 0 denotes all set differences are decode, which is all the absorbing state of the Markov chain. 

In the context of the Markov chain, $f^{(r)}(k)$ equals the probability that State $k$ does not transient to State 0 (absorbing state) in $r$ rounds. Let $\{e_i\}_{i=0,1,2,...,k}$ denote the standard basis vectors of length $k+1$, where $e_i$ has a single nonzero value 1 at the $(i+1)^{th}$ position. Based on the property of Markov chain, $x^{(r)}_k\triangleq e_k\cdot P^r$ is the probability vector of states after $r$ rounds with $k$ initial set differences, and the $i^{th}$ element in $x^{(r)}_k$ denotes the probability that State $k$ transients to State $i-1$ after $r$ rounds. 

$x^{(r)}(k)=(p^{(r)}_{k,0},p^{(r)}_{k,1},...,p^{(r)}_{k,k})$ denote the probability vector of states after $r$ rounds with $k$ initial set differences, where $p^{(r)}_i$ denotes the probability . 

Given the transition matrix $P$, we can easily 

\begin{figure*}
\centering
\includegraphics[width=0.98\textwidth]{figures/set_diff_markov}
\caption{Markov chain diagram for decoding process of set difference.}\label{fig:mc}
\end{figure*}

First, we assume the length of BCH decode is sufficient to decode each group. Then the decode process of each group can be considered as a Markov chain, in which state is defined as the number of "hidden elements" (i.e., elements belonging to the set difference that are to be decoded). \autoref{fig:mc} presents the state transition diagram, denoting the corresponding transmission matrix as $P=(p_{i,j})_{(d+1)\times (d+1)}$, where $p_{i,j}$ is the probability of moving from State $i$ to State $j$. By the same anology above, considering the classical balls-into-bins problem: $i$ balls are thrown independently and uniformly at random into $m'$ bins. Then $p_{i,j}$ equals to the probability that $i-j$ out of $m'$ bins have exactly one ball in each. Let $p^{(k)}_{i,j}$ denote the probability that $i-j$ out of $m'$ bins have exactly one ball in each, and $k$ out of $m'$ bins are empty. Then we have


\medskip
\noindent
{\bf Analysis on Number of Rounds}.
Consider the whole process as a Markov chain, whose state is defined as the number of 
``hidden elements'' ({\it i.e.,} elements belonging to the set difference that are to be decoded). 
\autoref{fig:mc} presents the state transition diagram, denoting the corresponding transmission 
matrix as $P=\big{(}p_{i,j}\big{)}_{(d+1)\times (d+1)}$ where $p_{i,j}$ is the probability of moving from state $i$ to state $j$. It is complex to obtain all the elements in $P$, we 
can easily get the following probabilities, for any $k \leq d$,
\begin{align}
p_{k,0}&=\frac{\binom{m}{k}k\,!}{m^k} \\
p_{k,1}&=0 \\
p_{k,2}&=\frac{\binom{k}{2}(m-k+2)\binom{m}{k-2}(k-2)\,!}{m^k},\quad \forall k\geq 2\\
p_{k,3}&=\frac{\binom{k}{3}(m-k+3)\binom{m}{k-3}(k-3)\,!}{m^k},\quad \forall k\geq 3\\
p_{k,4}&=\frac{\big{(}\binom{k}{4}(m-k+4) + \binom{k}{2}\binom{k-2}{2}(m-k+4)(m-k+3)/2\big{)}\binom{m}{k-4}(k-4)\,!}{m^k},\quad \forall k\geq 4.
\end{align}
where $m$ is the number of buckets.

Similarly, we can calculate $p_{k,i}$ for any $k\geq i \geq 5$ but the expression gets more and more complex. 


It is not hard to check that the Markov chain described above is an absorbing Markov chain with 
a single absorbing state of $0$. By using the time to absorption theorem of Absorbing Markov Chains~\cite[Page 13]{Elizalde_LectureNotesMath_2006}, 
we can easily get the average number of rounds (steps before the chain is absorbed), which equals
the $d^{th}$ element of $(N{\bf 1})$ where the matrix 
$N=(I-Q)^{-1}$ is the fundamental matrix of $P$ (Note that $Q$ is the transition matrix for all transient states, in our case, is $P$ by removing the last row and column, {\it i.e.,} $P_{0,*}$ 
and $P_{*,0}$) and 
${\bf 1}$ is an all-one vector with length $d$. 

Denote $P^{(k)}$ as the $k$-step transition matrix, then the probability that it takes more than $n$ rounds to decode is
\begin{equation}
\mathbf{Pr}[t>n]=\sum_{k=n+1}^{\infty}p^{(k)}_{d,0},
\end{equation}
where $d$ is the initial number of elements.


\medskip
\noindent
{\bf Simplified Analysis on Number of Rounds.} In the following analysis, we assume that the number of buckets in the kth round, 
assuming remaining $d_k$ elements to be decoded, is set to be $\delta\cdot d_k$ where $\delta > 1$ is a constant. For ease of 
presentation, we drop the subscript $k$ in the following analysis\footnote{Inspired by the analysis of the number of iterations 
for PIM.}. 

Fix a bucket, the probability that it gets exactly one element belonging to the set difference that is not decoded yet is:
\begin{equation}
p = d \Big{(}\frac{1}{\delta d}\Big{)}\Big{(} 1 - \frac{1}{\delta d}\Big{)}^{d - 1} = \frac{1}{\delta}\Big{(} 1 - \frac{1}{\delta d}\Big{)}^{d - 1}\approx \frac{1}{\delta}e^{-1/\delta}.
\end{equation}

On average, there are $p$ fraction of buckets will get exact one element. Hence, on average $e^{-1/\delta}$ fraction of un-decoded 
elements will be decoded in each round. Therefore, on average, we need $\log_{\frac{1}{1- e^{-1/\delta}}}d_0$ rounds, {\it i.e.,} 
$O(\log d_0)$ rounds. 

\end{comment}



==> section/theoretical_analysis_0213.tex <==
\begin{comment}
\section{Tug-of-War Sketch}\label{sec:sketch}


In this section, we describe the {\it tug-of-war}, which was first proposed in~\cite{AlonMS99} as 
a space-efficient estimator for the second frequency moment. 
%% Copy from Infocom 2009
We briefly describe 
the plain vanilla tug-of-war sketch~\cite{AlonMS99} in the context of error estimating coding, and under the assumption
that the sketch per se is not subject to bit errors (``noiseless") during transmission.  A tug-of-war sketch of a bit array (packet) $b$
is comprised of a constant number $c$ of counters  ($c$ is determined by the desired error guarantees) that are maintained using the same update algorithm (with possibly different update values) and is sent to the receiver alongside with $b$.
After the execution of these update algorithms, each counter contains the inner product of the bit vector $\overrightarrow{b}$ (`0' converted to `-1' as discussed earlier) with a vector $\overrightarrow{s} \in \{+1, -1\}^n $  that is four-wise independent, as shown in the following algorithm.  Such four-wise independent vectors are known to exist and have computationally efficient representations (e.g., derivable from the Reed-Muller code~\cite{GilbertKMS03}).
Note the actual update algorithm is not shown here because it is not relevant to our context; Only its ``net effect" after execution is. 


\subsection{Set Reconciliation}\label{subsec:set-reconciliation}

Before we describe how to use tug-of-war for set reconciliation~\cite{Guo_SetReconciliationvia_2013,Mitzenmacher_SimpleMultiParty_2013,Eppstein_WhatsDifference?Efficient_2011}, we first give a brief 
description of set reconciliation. For two sets $A, B$ that contain elements from the same universe, $U$, the set reconciliation 
problem wants to compute the set difference $A \Delta B\triangleq (A\setminus B)\cup (B\setminus A)$. We denote $D=A\Delta B$, and 
$d=|D|$. In the context of set reconciliation, the two sets $A$ and $B$ are stored at two distinct places and the problem wants to 
compute $D$ with minimal communication overhead. 

First, we assume that $d$ is known a prior. We will show later how to use the tug-of-war sketch 
to estimate $d$, the size of 
the set difference. 
As shown in~\cite{Eppstein_WhatsDifference?Efficient_2011}, we can achieve 
$O(d)$ (with a small constant factor) 
communication overhead to compute the set difference $D$ using 
the invertible bloom filter (IBF)~\cite{Goodrich_InvertibleBloomLookup_2011,Eppstein_StragglerIdentificationRound_2011}, which is clearly (asymptotically) optimal. However, in the cases where each element is 
very large (in terms of communication requirement) such as large documents or movie chunks, it is a large communication overhead to transmit a small constant (say $2$ or $3$) times  $d$ elements. As we will show next, by using 
the tug-of-war sketch, we can reduce the communication overhead to very close to $d$ (elements) 
with a few rounds of message exchanges. 


We assume that the communication is initiated by $A$. 
Each round of communication works as follows. 
$A$ creates $m=\delta d$ buckets, $b_1,b_2,\dots,b_m$, 
where $\delta > 1$ is a constant. Each bucket $b_i$
contains a subset of elements from $A$, 
each of which is uniformly randomly selected (with properly-designed 
hash functions). 
For each bucket $b_i$, $A$ computes $c$ tug-of-war sketches, 
denoting as $z_{i,1},z_{i,2},\dots,z_{i,c}$. Note that here eahc $z_{i,j}=\sum_{a\in b_i}h(a)$, where 
$h$ is from a four-wise hash family that maps each element to $\pm 1$. 
Then, $A$ sends the $m\times c$ sketches 
to $B$. $B$ uses the same hash functions to create $m$ buckets for its elements, and then use the same hash 
functions to compute the tug-of-war sketches for each bucket, denoting those sketches as $z'_{i,j}$ for $i\in [m]$ and 
$j\in [c]$. Then, $B$ can use $\frac{1}{c}\sum_{j=1}^{c}(z_{i,j}-z'_{i,j})^2$ to estimate the size of (sub-)set difference of 
the bucket $b_i$ for any $i\in [m]$. Note that $B$ can use the median of mean approach in~\cite{AlonMS99} 
or the MLE estimator in~\cite{Hua_TowardsOptimalError_2012} to obtain 
better estimations. Then, for each bucket whose estimator is in $(0, 1.5)$ (just an example), $B$ sends the exclusive or of all the elements 
in the bucket to $B$. It is clear that if the true size of the set difference for the bucket is $1$, then $A$ can obtain the 
element belonging to $A\Delta B$ in the bucket. 

By repeating the process until all the $d$ elements are obtained, $A$ computes the set difference $D$.
\end{comment}
\begin{comment}
\medskip
\noindent
{\bf Analysis on Number of Rounds}.
Consider the whole process as a Markov chain, whose state is defined as the number of 
``hidden elements'' ({\it i.e.,} elements belonging to the set difference that are to be decoded). 
\autoref{fig:mc} presents the state transition diagram, denoting the corresponding transmission 
matrix as $P=\big{(}p_{i,j}\big{)}_{(d+1)\times (d+1)}$ where $p_{i,j}$ is the probability of moving from state $i$ to state $j$. It is complex to obtain all the elements in $P$, we 
can easily get the following probabilities, for any $k \leq d$,
\begin{align}
p_{k,0}&=\frac{\binom{m}{k}k\,!}{m^k} \\
p_{k,1}&=0 \\
p_{k,2}&=\frac{\binom{k}{2}(m-k+2)\binom{m}{k-2}(k-2)\,!}{m^k},\quad \forall k\geq 2\\
p_{k,3}&=\frac{\binom{k}{3}(m-k+3)\binom{m}{k-3}(k-3)\,!}{m^k},\quad \forall k\geq 3\\
p_{k,4}&=\frac{\big{(}\binom{k}{4}(m-k+4) + \binom{k}{2}\binom{k-2}{2}(m-k+4)(m-k+3)/2\big{)}\binom{m}{k-4}(k-4)\,!}{m^k},\quad \forall k\geq 4.
\end{align}
where $m$ is the number of buckets.

Similarly, we can calculate $p_{k,i}$ for any $k\geq i \geq 5$ but the expression gets more and more complex. 


It is not hard to check that the Markov chain described above is an absorbing Markov chain with 
a single absorbing state of $0$. By using the time to absorption theorem of Absorbing Markov Chains~\cite[Page 13]{Elizalde_LectureNotesMath_2006}, 
we can easily get the average number of rounds (steps before the chain is absorbed), which equals
the $d^{th}$ element of $(N{\bf 1})$ where the matrix 
$N=(I-Q)^{-1}$ is the fundamental matrix of $P$ (Note that $Q$ is the transition matrix for all transient states, in our case, is $P$ by removing the last row and column, {\it i.e.,} $P_{0,*}$ 
and $P_{*,0}$) and 
${\bf 1}$ is an all-one vector with length $d$. 

Denote $P^{(k)}$ as the $k$-step transition matrix, then the probability that it takes more than $n$ rounds to decode is
\begin{equation}
\mathbf{Pr}[t>n]=\sum_{k=n+1}^{\infty}p^{(k)}_{d,0},
\end{equation}
where $d$ is the initial number of elements.


\medskip
\noindent
{\bf Simplified Analysis on Number of Rounds.} In the following analysis, we assume that the number of buckets in the kth round, 
assuming remaining $d_k$ elements to be decoded, is set to be $\delta\cdot d_k$ where $\delta > 1$ is a constant. For ease of 
presentation, we drop the subscript $k$ in the following analysis\footnote{Inspired by the analysis of the number of iterations 
for PIM.}. 

Fix a bucket, the probability that it gets exactly one element belonging to the set difference that is not decoded yet is:
\begin{equation}
p = d \Big{(}\frac{1}{\delta d}\Big{)}\Big{(} 1 - \frac{1}{\delta d}\Big{)}^{d - 1} = \frac{1}{\delta}\Big{(} 1 - \frac{1}{\delta d}\Big{)}^{d - 1}\approx \frac{1}{\delta}e^{-1/\delta}.
\end{equation}

On average, there are $p$ fraction of buckets will get exact one element. Hence, on average $e^{-1/\delta}$ fraction of un-decoded 
elements will be decoded in each round. Therefore, on average, we need $\log_{\frac{1}{1- e^{-1/\delta}}}d_0$ rounds, {\it i.e.,} 
$O(\log d_0)$ rounds. 
\end{comment}

\section{Tail Bound Analysis and Parameter Settings}\label{sec:tail_bound}

In this section, we establish a strict tail bound on the probability that PBS successfully reconciles all distinct elements in $r$ rounds under arbitrary parameter settings ($n$, $\delta$, $t$)

Motivated by parameter settings, we establish a strict tail bound on the {\it success probability} of PBS (i.e., all distinct elements are reconciled in $r$ rounds) as a function of parameters (i.e., $n$, $\delta$, $t$), which give us (1) a guideline on parameter settings; and (2) a theoretical guarantee about the success probability under selected parameters. 

In this section, we still assume $d$ is precisely known. 
For simplicity, we make the following two assumptions that hold with overwhelming probability in the analysis: First, the checksum (\autoref{step:terminate_condition} of \autoref{alg:single_round_pbs}) works perfectly on checking if the reconciliation is complete; Second, no ``fake'' distinct element fails to be checked by \autoref{alg:verification} (mentioned in \autoref{subsec:exception_hash_partition}) appears during reconciliation. We first establish a strict tail bound for a single group pair using Markov chain and Dynamic Programming in \autoref{sec:tail_bound_per_group}. Then we combine it with Times-2-Bound to get a strict tail bound for all group pairs in \autoref{sec:times2bound}. In \autoref{sec:parameter_settings}, we discuss the parameter settings using the tail bound. 

%In \autoref{sec:tail_bound_insufficient}, we remove the above BCH assumption and derive a more precise tail bound. {\bf need to decide whether to have this part or not, since we can easily set a relatively long BCH code, so that each group is decodable w.h.p.}

\subsection{Tail Bound Analysis for Each Group Pair}\label{sec:tail_bound_per_group}

In this section, we focus on analyzing an arbitrary group pair, which we denote as $(A',B')$, and suppose their set difference $A'\Delta B'$ contains exactly $x$ elements. We only consider the case that the error-correct capability is sufficient (i.e., $x\leq t$). As we described in \autoref{sec:multi-rounds}, the $x$ distinct elements are hashed into $n$ subset pairs in the first round, and a distinct element is reconciled if and only if it is hashed into a subset pair that contains only $1$ distinct element. The distinct elements that have been reconciled in the first round are removed and the other distinct elements (i.e., the ones that have not been reconciled yet in the first round) will be hashed again in the second round using a different hash function, so on so force. 


% WLOG, we only analyze group pair $1$. {\bf Maybe say that we focus on an arbitrary group pair, which we denote as A' and B', and suppose their difference $ ... $ contains exactly $x$ elements}. 
% %The analysis for other group pairs is the same. 
% {\bf Please use x, not d}.  
% For the moment, we slightly abuse the notation and use $d$ to denote the number of distinct elements in group pair $1$ (i.e., $d_1$). In this section, we only consider the case that the error-correct capability is sufficient (i.e., $d\leq t$). As we described in \autoref{sec:multi-rounds}, the $d$ distinct elements of group pair $1$ are hashed into $n$ subset pairs in the first round, and a distinct element is reconciled if and only if it is hashed into a subset pair that contains only $1$ distinct element. The distinct elements that have been reconciled in the first round are removed and the other distinct elements (i.e., the ones that have not been reconciled yet in the first round) will be hashed again in the second round using a different hash function, so on so force. 

==========
{\bf The following may be useful in explaining why it is a Markov chain:} [Note there is no need to distinguish these four cases in calculating the ``transitioning out" probability (i.e., from state 6 to a small state say State 0), because the next round of balls-into-bins operation uses a different hash function independent of that used in the current round, and consequently how these 6 bad balls are split in the current round have no bearing on that in the next round.]  {\bf unless you have done so earlier}

{\bf we have an example at the end of multi-round PBS}
==========


As we explained in \autoref{sec:hash_partition}, how the $x$ distinct elements are distributed into $n$ subset pairs in the first round follows the familiar {\it balls-into-bins} probability model: Each of the $x$ balls are thrown independently and uniformly at random into one of the $n$ bins. Each distinct element that is reconciled in the first round corresponds to a ball that ends up in a bin that receives exactly $1$ ball. We call the ball and the bin ``good'' in the sequel; Each distinct element that has not been reconciled yet in the first round corresponds to a ball that ends up in a bin that receives multiple balls. We call the ball and the bin ``bad'' in the sequel. Note that balls are either ``good'' or ``bad'', but bins could be empty besides ``good'' and ``bad''.



The ``bad'' balls in the first round will be the balls to be thrown in the second round. The ``bad'' balls in the second round will be the balls to be thrown in the third round, so on so force. In all rounds, how the balls are thrown into $n$ bins follows the balls-into-bins model. The dynamics of the number of balls to be thrown in each round can be modeled as a Markov chain, in which each state is defined as the number of balls to be thrown. In the Markov chain, a transition from state $i$ to state $j$ ($i\geq j$) means $i-j$ out of $i$ balls are ``good'' balls and the other $j$ balls are ``bad'' balls. The {\it absorbing state} of this Markov chain is state $0$, which is the ``good'' state that means all distinct elements have been reconciled (i.e., reconciliation is complete). For our analysis, the only probability that we concerned is $Pr[x\xrsquigarrow{r} 0]$, the probability that state $x$ (initial state) reaches the absorbing state (i.e., state $0$) in $r$ transitions, which is also the probability that all distinct elements are reconciled in $r$ rounds. This probability can be easily calculated given the transition matrix of the Markov chain: Let $M$ denote the $(t+1)\times (t+1)$ transition matrix of the Markov chain.
%, where $M(i,j)$ (i.e., the entry in the $i^{th}$ row and the $j^{th}$ column of $M$) is the probability of transition from state $i$ to state $j$ for $i,j = 0,1,...,t$
$Pr[x\xrsquigarrow{r} 0]$ equals to $\big{(}M^r\big{)}(x,0)$ (i.e., the entry in the $x^{th}$ row and the $0^{th}$ column of $M^r$). Here we slightly abuse the row / column numbers of a $(t+1)\times (t+1)$ matrix from $1,2,...,t+1$ to $0,1,...,t$, since the state of the Markov chain ranges from $0$ to $t$. 

\subsubsection{How to compute \texorpdfstring{$M$}{M}}

The only problem left to obtain $Pr[x\xrsquigarrow{r} 0]$ is how to compute $M$, which is not straightforward, since each state $j$ (after-transition state) with $j>3$ in the Markov chain is a composite state as far as the calculation of the transition probability from a (larger) state $i$ $(>j)$ to $j$ is concerned. To calculate the probability, we have to break state $j$ down into ``atom'' states, calculate the transition probability from state $i$ to each of the ``atom'' states (which can be directly calculated), and then add them up. {\bf Note that we always view state $i$ (pre-transition state) as a simple state, since how the $i$ balls are placed into $n$ bins only depends on a hash function that is independent of the ones used in previous rounds.}

Each composite state $j$ can be broken down into atom states based on how these $j$ bad balls are placed into the $n$ bins. For example, state $6$ consists of $4$ atom states. The first one is $6 = 6$, where all $6$ bad balls are in the same bad bin. The second one is $6 = 2 + 4$ where, out of the $6$ bad balls, four are in one bad bin and the other two are in the other bad bin.  Similarly, the other two atom states are $6 = 3 + 3$ and $6 = 2 + 2 + 2$. The transition probability from state $i$ to any atom state can be directly calculated, but the problem is that the number of atom states grows exponentially with the number of ``bad'' balls $j$.

We notice that we can break each composite state into a small number of coarse-grained sub-states, each of which may still contain a large number of atom states. The transition probability from a (larger) state $i$ to any sub-state is still hard to compute. However, there is a recurrence relation among them, so we can compute the transition probabilities from any state to any sub-state using Dynamic Programming. 




% Each ``atom'' state is, in combinatorics terms, {\it a permutation of a combination of $j$}, which here corresponds to 
% how these $j$ ``bad'' balls are placed into the $n$ bins. 
% For a simple example, when $j = 4$ and $n = 7$, the vector $(2, 0, 0, 0, 0, 2, 0)$ is such an ``atom'' state, which corresponds to these $7$ bins (in a predefined order such as the natural order) 
% have $2$, $0$, $0$, $0$, $0$, $2$, and $0$ ``bad'' balls in it respectively. The transition probability from state $i$ to any atom state can be calculated, but the problem is that the number of atom states 
% (permutations of combinations) grow exponentially with the number of balls $j$.


+++++++++++

The only problem left to obtain $Pr[d\xrsquigarrow{r} 0]$ is how to compute $M$, which is not straightforward, since each state $j$ with $j>3$ in the Markov chain is a composite state as far as the calculation of the transition probability from a (larger) state $i$ $(>j)$ to $j$ (i.e., ``transitioning into'') is concerned.   {\bf You need to explain why it is not straightforward:  The reason you offer is not
the direction reason.  Instead you may say that "the transition probability between these composite states cannot be directly calculated" ...  to calculate it we have to break it down into "atom" states}

Each composite state $i$ can be broken down into atom states as follows.  Each simple state is, in combinatorics terms, {\it a permutation of a combination of $i$}, which here corresponds to 
how these $i$ balls are ``divided up" by the $n$ bins.   {\bf Liang, Read Mitzenmacher and Upfal book
for a better word for "divided up"}
For a simple example, when $i = 4$ and $n = 7$, the vector (1, 0, 1, 0, 0, 2, 0) is such a simple state, which corresponds to these 7 bins (in a predefined order such as the natural order) 
have 1, 0, 1, 0, 0, 2, and 0 balls in it respectively.   The transition probability between any two atom states can be ...    but the problem is that the number of atom states 
(permutations of combinations) grow exponentially with the number of balls $i$.

Consider two states i1 and i2 each broken down into millions of atom states.  Then the transition probability between these states is the summation of the trillions (= millions * millions) of 
transition probabilities between atom states of i1 and atom states of i2.  

The good thing is that the transition probability matrix among the (humongous number of atom states) induces a "subproblem structure ????", which leads to the recurrence relation, 
dynamic programming.   

We notice that we can break each state into a small number of coarse-grained substates, each of which may still contain a large number of atom states.  The transition probability 
between any two such substates are still hard to compute.  However, there is a recurrence relation among them ...

+++++++++++

To solve the problem, we partition the composite state into sub-states, so that the transition probability to the composite state is the summation of the transition probabilities to each of the sub-states. On the other hand, the transition probabilities to the sub-state have a recurrence relation and can be computed using Dynamic Programming. 

======================================

Note that every state $j$ with $j > 3$ in the Markov chain is a composite state as far as the calculation of the transition probability from a (larger) state $i > j$ to $j$ (i.e., ``transitioning into").  For example, State 6 contains 4 different cases. The first case is $6 = 6$, where all 6 bad balls are in the same bad bin. The second case is $6 = 2 + 4$ where, out of the 6 bad balls, four are in one bad bin and the other two are in the other bad bin.  Similarly, the other two cases are $6 = 3 + 3$ and $6 = 2 + 2 + 2$. Note there is no need to distinguish these four cases in calculating the ``transitioning out" probability (i.e., from state 6 to a small state say State 0), because the next round of balls-into-bins operation uses a different hash function independent of that used in the current round, and consequently how these 6 bad balls are split in the current round have no bearing on that in the next round. 

Building on the example above, we now consider $m_{9,6}$, the transition probability from State $9$ to State $6$ (throwing 9 balls into 255 bins and ending up with 6 bad balls).  $m_{9,6}$ is simply the sum of the probabilities of these four cases, each of which has a very different formula than the others.  In general, the number of such cases, and hence the number of individual probability terms to be added up to arrive at the transition matrix element $m_{i,j}$, grows exponentially with the value of $j$. This does not however make it difficult to calculate the values of $M$, because there is a recursive structure, among the values of the matrix elements $m_{i,j}$, that can be exploited using dynamic programming, as will be elaborated shortly.

To simplify our analysis, we split each composite state into sub-composite states based on the number of nonempty bins: Let State $(j,k)$ denotes the sub-composite state with $j$ remaining distinct elements and $k$ nonempty bins, which is also a substate of State $j$. Let $m_{i,j}^{(k)}$ denote the probability of transition from State $i$ to State $(j,k)$, which is also the probability that after throwing $i$ balls uniformly and independently into $n$ bins, $i-j$ bins are ``good'' bins and $k$ bins are nonempty bins (thus $k-(i-j)$ bins are ``bad'' and $n-k$ bins are empty). The probability of transition to a composite state is simply the summation of the probabilities of the transitions to corresponding sub-composite states:

To obtain the transition matrix $M$, it is sufficient to compute $m^{(k)}_{i,j}$, which can be exploited using dynamic programming. Note that the balls-and-bins model itself can be considered as a Markov chain, in which a recursive relation exists: After throwing $i$ balls into $n$ bins, throwing one more ball randomly could be: (1) Into an empty bin and turn it to a ``good'' bin; (2) Into a ``good'' bin and turn it to a ``bad'' bin with two balls; or (3) Into a ``bad'' bin and keep it as the same. Mathematically, we have $m^{(k)}_{i+1,j}$ equals to


====================================

More specifically, let state $(j,k)$ denote the sub-state of state $j$ that the $j$ ``bad'' balls end up to occupy exactly $k$ ``bad'' bins. Then the composite state $j$ is partitioned into state $(j,1)$, state $(j,2)$, $...$, state $(j,j)$. We slightly abuse the notation and let $M(i,j,k)$ denote the probability of transition from state $i$ to state $(j,k)$, then we have 

\begin{equation}
    M(i,j) = \sum_{k=1}^{j} M(i,j,k)
\end{equation}

{\bf we can use a tighter range of $k$ of $1,2,..., \lfloor j/2 \rfloor$. For cleanness, I choose a wider range of $1,2,..., j$, which is easier to understand and does not change the result}

To obtain $M$, it is sufficient to compute $M(i,j,k)$ for $\forall i,j,k=0,1,...,t$
{\bf Similarly, there is a tighter range for $i,j,k$, which seems to be unnecessary}
. Note that the state transition resulting from throwing one ball after another is also a Markov chain, in which state $(i,j,k)$ is defined as $j$ ``bad'' balls ending up into $k$ ``bad'' bins after throwing $i$ balls into $n$ bins. In this Markov chain, throwing one more ball can transition state $(i,j,k)$ to three possible states depending on the $(i+1)^{th}$ ball ending up in (1) a ``good'' bin; (2) a ``bad'' bin; or (3) an empty bin. The first case happens with probability $(i-j)/n$, results in $2$ additional ``bad'' balls and $1$ additional ``bad'' bin (i.e., transition to state $(i+1,j+2,k+1)$). The second and third cases transition to state $(i+1,j+1,k)$ and state $(i+1,j,k)$ respectively with probability $k/n$ and $1-(i-j+k)/n$. In the opposite direction, state $(i+1,j,k)$ can only be transitioned from (1) state $(i,j-2,k-1)$; (2) state $(i,j-1,k)$; and (3) state $(i,j,k)$, which gives us a recurrence relation that $M(i+1,j,k)$ equals to

%The second case happens with probability $k/n$ and results in state $(i+1,j+1,k)$. The third case happens with probability $1-(i-j+k)/n$ and results in state $(i+1,j,k)$. In the opposite direction, state $(i+1,j,k)$ can be transitioned from (1) state $(i,j-2,k-1)$ with probability $(i-j+2)/n$; (2) state $(i,j-1,k)$ with probability $k/n$; or (3) state $(i,j,k)$ with probability $1-(i-j+k)/n$. It gives us a recurrence relation that $P(i+1,j,k)$ equals to

\begin{equation}\label{eq:recursion}
    \frac{i\!-\!j\!+\!2}{n}\cdot M(i,j\!-\!1,k\!-\!1)+\frac{k}{n}\cdot M(i,j\!-\!1,k)+(1\!-\!\frac{i\!-\!j\!+\!2}{n})\cdot M(i,j,k)
\end{equation}

The three terms in \autoref{eq:recursion} corresponds to the above three possible transitions. Combining with the following probabilities in base cases, we can compute $M(i,j,k)$ for $\forall i,j,k=0,1,...,t$ using Dynamic Programming and obtain $M$:

\begin{align}
M(0,j,k) =& \left\{ \begin{array}{ccl}
1, & \mbox{if }
 j=k=0 \\ 0, & \mbox{otherwise} 
\end{array}\right.\label{eq:basic1}\\
M(i,0,k) =& \left\{ \begin{array}{ccl}
\binom{n}{i}/n^i, & \mbox{if }
 k=0 \\ 0, & \mbox{otherwise} 
\end{array}\right.\label{eq:basic2}\\
M(i,j,0) =& \left\{ \begin{array}{ccl}
1, & \mbox{if }
 j=0 \\ 0, & \mbox{otherwise} 
\end{array}\right.\label{eq:basic3}
\end{align}

%As mentioned earlier, we slightly abuse the notation `$d$' in this section to denote the number of distinct elements in group pair $1$, which is actually $d_1$ defined in \autoref{subsec:protocol2}. Now we recover the abused notation $d$ to denote the total number of distinct elements in all groups. 

As we explained in \autoref{subsec:protocol2}, $d_1$, the number of distinct elements in group pair $1$, is a random variable that follows a Binomial distribution $Binomial(d,1/g)$. So the probability that the group pair is completely reconciled in $r$ rounds is $\sum_{x=0}^d Pr[d_1=x]\cdot Pr[x\xrsquigarrow{r} 0]$.
%, where $\mathcal{B}(\cdot;d,1/g)$ is the probability mass function (PMF) of $Binomial(d,1/g)$. 
To ease computation, we slightly underestimate this probability by assuming $Pr[x\xrsquigarrow{r} 0]=0$ when $x>t$ (i.e., assume group pair $1$ cannot be reconciled if $d_i>t$, discussed in \autoref{sec:BCH_exception}). The loss of this underestimation is very tiny, since the coefficient of $Pr[x\xrsquigarrow{r} 0]$ (i.e., $Pr[d_1=x]$) is very small when $x>t$. We denote this underestimated probability as $\alpha$ (i.e., $\alpha=\sum_{x=0}^t Pr[d_1=x]\cdot Pr[x\xrsquigarrow{r} 0]$). Note that $Pr[x\xrsquigarrow{r} 0]$ is a function of $n$ and $r$ for arbitrary $x$, so $\alpha$ is a function of $n$, $r$, $t$ for arbitrary $d$ and $g$. 

\subsection{Tail Bound Analysis for all groups}\label{sec:times2bound}

Given $\alpha$, the tail bound of the probability that a group pair is successfully reconciled in $r$ rounds, we can easily derive a tail bound of $\alpha^g=1-(1-\alpha^g)$ for the probability that all group pairs are successfully reconciled in $r$ rounds, if we assume the reconciliations on group pairs are independent with each other. However, this assumption is not rigorous, since $d_1, d_2,...,d_g$ have a weak correlation that $\sum_{i=1}^g d_i=d$. 
%Fortunately, we have Times-2-Bound (Theorem 1 in \cite{hua2008rank}) to decouple the weak correlation and give us a rigorous tail bound of $1-2(1-\alpha^g)$ for the probability of all group pairs. 
To be rigorous, we use so-called Times-2-bound (Corollary 5.11 in \cite{upfal2005probability}) to decouple the weak correlation and obtain a rigorous tail bound of $1-2(1-\alpha^g)$ for the probability of all group pairs.
In \autoref{sec:parameter_settings}, we use the tail bound of $1-2(1-\alpha^g)$ in parameter settings for rigorousness. 

% More specifically, let state $(j,k)$ denote the sub-state of state $j$ that the $j$ ``bad'' balls end up to occupy exactly $k$ ``bad'' bins. Then the composite state $j$ is the union of state $(j,1)$, state $(j,2)$, $...$, state $(j,\lfloor j/2 \rfloor)$ (each ``bad'' bin receives at least $2$ ``bad'' balls, so $k\leq \lfloor j/2\rfloor$). Let $P(i,j,k)$ denote the probability of transition from state $i$ to state $(j,k)$, then we have 

% \begin{equation}
%     M(i,j) = \sum_{k=1}^{\lfloor j/2\rfloor} P(i,j,k)
% \end{equation}






% Note that each state $j$ with $j>3$ in the Markov chain is a composite state as far as the calculation of the transition probability from a (larger) state $i$ $(>j)$ to $j$ (i.e., ``transitioning into''). Such a composite state $j$ can be decomposed into sub-states based on the number of ``bad'' bins after throwing $i$ balls: Define state $(j,k)$ as the sub-state of state $j$ that the  $j$ ``bad'' balls end up to occupy exactly $k$ ``bad'' bins. Then state $j$ is the union of all states $(j,k)$ for $k=1,2,...$ (each ``bad'' bin receives at least $2$ ``bad'' balls). Let $m_{i,j}^{(k)}$ denote the probability of transition from state $i$ to state $(j,k)$
% %, which is also the probability that after throwing $i$ balls uniformly and independently into $n$ bins, $i-j$ bins are ``good'' bins and $k$ bins are nonempty bins (thus $k-(i-j)$ bins are ``bad'' and $n-k$ bins are empty)
% . The probability of transition to the composite state $j$ is simply the summation of the probabilities of the transitions to corresponding sub-states: 

% \begin{equation}
%     m_{i,j} = \sum_{k=i}^{i-j} m^{(k)}_{i,j}
% \end{equation}


% To make our description simple, we call a bin that receives exactly $1$ ball a ``good'' bin is ``good'' if and only if it receives exactly $1$ ball. We call a bin is ``bad'' if and only if it receives more than $1$ balls. The rest bins (i.e., neither ``good'' nor ``bad'') are empty. We call a ball ending up in a ``good'' bin is ``good'' if it is in a ``good bin'' Then the distinct elements that are decoded correspond to the balls that are in ``good'' bins. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Old version of 2/5
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{comment}

In this section, we only consider the cases that a group is able to be decoded by BCH code (i.e., initially contains at most $t$ set differences). Without loss of generosity, we assume the group has $d (\leq t)$ distinct elements and is partitioned into $n$ subset pairs. As we described in \autoref{sec:hash_partition}, the $d$ distinct elements are hashed into $n$ subset pairs in each round, and a distinct element is decoded if and only if it is hashed into a subset pair that contains only $1$ distinct element. As we introduced in \autoref{sec:hash_partition}, the statistical model for hashing $d$ distinct elements into $n$ subset pairs is the same as the classical balls-and-bins problem: $d$ balls are thrown independently and uniformly at random into $n$ bins. To make our description simple, we call a bin is ``good'' if and only if it receives exactly $1$ ball. And we call a bin is ``bad'' if and only if it receives more than $1$ balls. The rest bins (i.e., neither ``good'' nor ``bad'') are empty. Then the distinct elements that are decoded correspond to the balls that are in ``good'' bins. 

The decode process of each group can be considered as a Markov Chain, in which each state is defined as the number of remaining distinct elements (i.e., the distinct elements that haven't been decoded). In this Markov chain, the transition from State $i$ to State $j$ means $i-j$ out of $i$ distinct elements are decoded in this round, where $0\leq j\leq i\leq t$. Use the same analogy, the number (state) is simply the total number of balls that fall in ``bad'' bins. The transition from State $i$ to State $j$ means $i-j$ out of $i$ balls fall in ``good'' bins in this round, while the rest $j$ balls fall in ``bad'' bins. State $0$ is the {\it absorbing} state of this Markov Chain, which means all distinct elements have been reconciled. For our analysis, we only concern the probability that after $r$ rounds, the final state is state $0$ (i.e., absorbing state) when the initial state is state $i$. We denote this probability as $v^{(r)}_i(0)$.

Let $M=(m_{i,j})_{(t+1)\times (t+1)}$ denote the transition matrix of the above Markov chain, where $m_{i,j}$ is the probability of transition from State $i$ to State $j$. Given $M$, $r$, and the initial state $i$, $v^{(r)}_i(0)$ can be easily calculated. So the only problem is how to obtain $M$, which will be elaborated in the next section.

\subsubsection{Transition Matrix}\label{sec:transition_matrix}

Now we describe how to compute the transition matrix $M$ using dynamic programming in detail. Note that every State $j$ with $j > 3$ in the Markov chain is a composite state as far as the calculation of the transition probability from a (larger) state $i > j$ to $j$ (i.e., ``transitioning into").  For example, State 6 contains 4 different cases. The first case is $6 = 6$, where all 6 bad balls are in the same bad bin. The second case is $6 = 2 + 4$ where, out of the 6 bad balls, four are in one bad bin and the other two are in the other bad bin.  Similarly, the other two cases are $6 = 3 + 3$ and $6 = 2 + 2 + 2$. Note there is no need to distinguish these four cases in calculating the ``transitioning out" probability (i.e., from state 6 to a small state say State 0), because the next round of balls-into-bins operation uses a different hash function independent of that used in the current round, and consequently how these 6 bad balls are split in the current round have no bearing on that in the next round. 

Building on the example above, we now consider $m_{9,6}$, the transition probability from State $9$ to State $6$ (throwing 9 balls into 255 bins and ending up with 6 bad balls).  $m_{9,6}$ is simply the sum of the probabilities of these four cases, each of which has a very different formula than the others.  In general, the number of such cases, and hence the number of individual probability terms to be added up to arrive at the transition matrix element $m_{i,j}$, grows exponentially with the value of $j$. This does not however make it difficult to calculate the values of $M$, because there is a recursive structure, among the values of the matrix elements $m_{i,j}$, that can be exploited using dynamic programming, as will be elaborated shortly.

To simply our analysis, we split each composite state into sub-composite states based on the number of nonempty bins: Let State $(j,k)$ denotes the sub-composite state with $j$ remaining distinct elements and $k$ nonempty bins, which is also a substate of State $j$. Let $m_{i,j}^{(k)}$ denote the probability of transition from State $i$ to State $(j,k)$, which is also the probability that after throwing $i$ balls uniformly and independently into $n$ bins, $i-j$ bins are ``good'' bins and $k$ bins are nonempty bins (thus $k-(i-j)$ bins are ``bad'' and $n-k$ bins are empty). The probability of transition to a composite state is simply the summation of the probabilities of the transitions to corresponding sub-composite states:

\begin{equation}
    m_{i,j} = \sum_{k=i}^{i-j} m^{(k)}_{i,j}
\end{equation}

To obtain the transition matrix $M$, it is sufficient to compute $m^{(k)}_{i,j}$, which can be exploited using dynamic programming. Note that the balls-and-bins model itself can be considered as a Markov chain, in which a recursive relation exists: After throwing $i$ balls into $n$ bins, throwing one more ball randomly could be: (1) Into an empty bin and turn it to a ``good'' bin; (2) Into a ``good'' bin and turn it to a ``bad'' bin with two balls; or (3) Into a ``bad'' bin and keep it as the same. Mathematically, we have $m^{(k)}_{i+1,j}$ equals to

\begin{equation}\label{eq:recursion}
\frac{n-k+1}{n}\cdot m^{(k-1)}_{i,j-1} + \frac{j+1}{n}\cdot m^{(k)}_{i,j+1} + \frac{k-(i-j)}{n}\cdot m^{(k)}_{i,j} \nonumber
\end{equation}

The three terms in \autoref{eq:recursion} corresponds to the above three cases. Meanwhile, we can easily get the boundary conditions as follows:

\begin{align}
m^{(k)}_{i,0} =& \left\{ \begin{array}{ccl}
\binom{n}{i}/n^i, & \mbox{if }
 k=i \\ 0, & \mbox{otherwise} 
\end{array}\right.\label{eq:basic1}\\
m^{(k)}_{0,j} =& \left\{ \begin{array}{ccl}
1, & \mbox{if }
 k=0 \mbox{ and } j=0 \\ 0, & \mbox{otherwise} 
\end{array}\right.\label{eq:basic2}\\
m^{(0)}_{i,j} =& \left\{ \begin{array}{ccl}
1, & \mbox{if }
 i=0 \mbox{ and } j=0 \\ 0, & \mbox{otherwise} 
\end{array}\right.\label{eq:basic3}
\end{align}

Using \autoref{eq:recursion},\autoref{eq:basic1},\autoref{eq:basic2}, and \autoref{eq:basic3}, we can recursively compute $m^{(k)}_{i,j}$ and obtain $M$.


\subsection{Global Tail Bound Analysis}\label{sec:times2bound}

Consider group $1$ (other groups have the same result), the probability that all distinct elements in group $1$ are reconciled in $r$ rounds is $\sum_{i=0}^d Pr[d_1=i]v_i^{(r)}(0)\triangleq \alpha$, where $d_1$ (i.e., the number of distinct elements in group $1$) is a Binomial random variable $Binomial(d,1/g)$ as we explained in \autoref{subsec:protocol2}. To ease computation, we slightly underestimate this probability $\alpha$ by assuming $v_i^{(r)}(0)=0$ when $i>t$ (i.e., assume group $i$ cannot reconcile if $d_i>t$, discussed in \autoref{sec:BCH_exception}). The loss of this underestimation is very tiny, since the coefficient of $v_i^{(r)}(0)$ (i.e., $Pr[d_1=i]$) is very small when $i>t$.

The probability that all groups are successfully reconciled in $r$ rounds is simply $\alpha^g\triangleq \beta$, if we assume the reconciliations on groups are independent with each other. This assumption is however not rigorous, since $d_1, d_2,...,d_g$ have a weak correlation that $\sum_{i=1}^g d_i=d$. Fortunately, we have Times-2-Bound (Theorem 1 in \cite{hua2008rank}) to decouple the weak correlation and give us a rigorous bound of $2\beta-1$. In \autoref{sec:parameter_settings}, we use this rigorous bound for parameter settings. 

\end{comment}






\begin{comment}

Let $v^{(r)}_i=\big{(}{v^{(r)}_i(0), v^{(r)}_i(1),...,v^{(r)}_i(t)}\big{)}$ denote the probability vector (i.e., $\sum_{j=0}^{t}v^{(r)}_i(j) = 1$) after $r$ rounds with initial State $i$: $v^{(r)}_i(j)$ denotes the probability that the final state is State $j$ after $r$ rounds. In the probability vector, $v^{(r)}_i(0)$ is the only entry that we concern, which is the probability of the cases that all distinct elements are decoded after $r$ rounds. Given 

Note that every State $j$ with $j > 3$ in the Markov chain is a composite state as far as the calculation of the transition probability from a (larger) state $i > j$ to $j$ (i.e., ``transitioning into").  For example, State 6 contains 4 different cases. The first case is $6 = 6$, where all 6 bad balls are in the same bad bin. The second case is $6 = 2 + 4$ where, out of the 6 bad balls, four are in one bad bin and the other two are in the other bad bin.  Similarly, the other two cases are $6 = 3 + 3$ and $6 = 2 + 2 + 2$. Note there is no need to distinguish these four cases in calculating the ``transitioning out" probability (i.e., from state 6 to a small state say State 0), because the next round of balls-into-bins operation uses a different hash function independent of that used in the current round, and consequently how these 6 bad balls are split in the current round have no bearing on that in the next round. 

Building on the example above, we now consider $m_{9,6}$, the transition probability from State $9$ to State $6$ (throwing 9 balls into 255 bins and ending up with 6 bad balls).  $m_{9,6}$ is simply the sum of the probabilities of these four cases, each of which has a very different formula than the others.  In general, the number of such cases, and hence the number of individual probability terms to be added up to arrive at the transition matrix element $m_{i,j}$, grows exponentially with the value of $j$. This does not however make it difficult to calculate the values of $M$, because there is a recursive structure, among the values of the matrix elements $m_{i,j}$, that can be exploited using dynamic programming, as will be elaborated in \autoref{sec:transition_matrix}.

Let $v^{(r)}_i=\big{(}{v^{(r)}_i(0), v^{(r)}_i(1),...,v^{(r)}_i(t)}\big{)}$ denote the probability vector (i.e., $\sum_{j=0}^{t}v^{(r)}_i(j) = 1$) after $r$ rounds with initial State $i$: $v^{(r)}_i(j)$ denotes the probability that the final state is State $j$ after $r$ rounds. In the probability vector, $v^{(r)}_i(0)$ is the only ``good'' entry, which is the probability of the cases that all distinct elements are decoded after $r$ rounds. The probability of the group does not complete reconciliation is simply $1-v^{(r)}_i(0)$. 

Given the transition matrix $M$, we can easily compute the probability vector $v^{(r)}_i$ for any $r$ and $i$ as follows:
\begin{equation}
    x^{(r)}_i = e_i\cdot M^r
\end{equation}
Here $\{e_i\}_{i=0,1,2,...,t}$ denote the standard basis vectors of length $t+1$, where $e_i$ has a single nonzero value 1 at the $(i+1)^{th}$ position. So the remaining problem is how to compute $M$.

\subsubsection{Transition Matrix}\label{sec:transition_matrix}

Now we describe how to compute the transition matrix $M$ using dynamic programming in detail. As we described earlier, every State $j$ with $j > 3$ in the Markov chain is a composite state that contains many different cases. And the number of these cases increases exponentially with the value of $j$. To simply our analysis, we split each composite state into sub-composite states based on the number of nonempty bins: Let State $(j,k)$ denotes the sub-composite state with $j$ remaining distinct elements and $k$ nonempty bins, which is also a substate of State $j$. Let $m_{i,j}^{(k)}$ denote the probability of transition from State $i$ to State $(j,k)$, which is also the probability that after throwing $i$ balls uniformly and independently into $n$ bins, $i-j$ bins are ``good'' bins and $k$ bins are nonempty bins (thus $k-(i-j)$ bins are ``bad'' and $n-k$ bins are empty). The probability of transition to a composite state is simply the summation of the probabilities of the transitions to corresponding sub-composite states:

\begin{equation}
    m_{i,j} = \sum_{k=i}^{i-j} m^{(k)}_{i,j}
\end{equation}

To obtain the transition matrix $M$, it is sufficient to compute $m^{(k)}_{i,j}$, which can be exploited using dynamic programming. Note that the balls-and-bins model itself can be considered as a Markov chain, in which a recursive relation exists: After throwing $i$ balls into $n$ bins, throwing one more ball randomly could be: (1) Into an empty bin and turn it to a ``good'' bin; (2) Into a ``good'' bin and turn it to a ``bad'' bin with two balls; or (3) Into a ``bad'' bin and keep it as the same. Mathematically, we have 

\begin{align}
m^{(k)}_{i+1,j} =& \frac{n-k+1}{n}\cdot m^{(k-1)}_{i,j-1} + \frac{j+1}{n}\cdot m^{(k)}_{i,j+1} \nonumber\\
&+ \frac{k-(i-j)}{n}\cdot m^{(k)}_{i,j} \label{eq:recursion}
\end{align}

The three terms in \autoref{eq:recursion} corresponds to the above three cases. Meanwhile, we can easily get the following probabilities for basic cases:

\begin{align}
m^{(k)}_{i,0} =& \left\{ \begin{array}{ccl}
\binom{n}{i}/n^i, & \mbox{if }
 k=i \\ 0, & \mbox{otherwise} 
\end{array}\right.\label{eq:basic1}\\
m^{(k)}_{0,j} =& \left\{ \begin{array}{ccl}
1, & \mbox{if }
 k=0 \mbox{ and } j=0 \\ 0, & \mbox{otherwise} 
\end{array}\right.\label{eq:basic2}\\
m^{(0)}_{i,j} =& \left\{ \begin{array}{ccl}
1, & \mbox{if }
 i=0 \mbox{ and } j=0 \\ 0, & \mbox{otherwise} 
\end{array}\right.\label{eq:basic3}
\end{align}

Using \autoref{eq:recursion},\autoref{eq:basic1},\autoref{eq:basic2}, and \autoref{eq:basic3}, we can recursively compute $m^{(k)}_{i,j}$ and then get $v^{(r)}_i(0)$ for $\forall i=0,1,...,n$ and $r\in\mathbb{Z}$. The value of $v^{(r)}_i(0)$ will be used to compute the tail bound of $Pr[P^{(r)}_o]$ in the next section. 

\subsection{Global Tail Bound Analysis}\label{sec:times2bound}

Let random variable $X^{(d)}_i, 1\leq i\leq g$, denote the number of set differences initially allocated in the $i^{th}$ group. For an analogy, the statistical model for hashing $d$ set differences into $g$ groups is also the same as the classical balls-and-bins problem: $d$ balls are thrown independently and uniformly at random into $g$ bins. Then random variable $X^{(d)}_i$ could be translated as the number of balls ended up in the $i^{th}$ bin after $d$ balls are thrown. Therefore, $(X^{(d)}_1,...,X^{(d)}_g)$ follows the multinomial distribution. The marginal distribution for any $X^{(d)}_i$ is $Binomial(d,\frac{1}{g})$, where $Binomial(N,p)$ denotes the binomial distribution resulting from $N$ trials with success probability $p$. 

Let $f^{(r)}(x_1,x_2,...,x_g)$ denote the probability that set reconciliation does not complete (for all groups) in $r$ rounds when the $i^{th}$ group initially contains $x_i$ set differences for $i=1,2,...,g$. Define $f^{(r)}(x)$ as the probability that set reconciliation does not complete in $r$ rounds when a group initially contains $x$ set differences. Based on the result in \autoref{sec:tail_bound_per_group}, we have 

% \begin{equation}\label{eq:frx}
%     f^{(r)}(x) \leq g^{(r)}(x) \triangleq \left\{ \begin{array}{ccc}
% 1-v^{(r)}_{x}(0) & \mbox{for}
% & 0\leq x\leq c \\ 1 & \mbox{for} & x>c
% \end{array}\right.
% \end{equation}

\begin{equation}\label{eq:frx}
    f^{(r)}(x) = 1-v^{(r)}_{x}(0) \mbox{ for }  0\leq x\leq t 
\end{equation}

Since the reconciliation processes independently for each group, we have 

\begin{equation}
f^{(r)}(x_1,x_2,...,x_g) = 1-\prod_{i=1}^g \big{(}1-f^{(r)}(x_i)\big{)}
\end{equation}

Then we have 

\begin{align} 
Pr[P^{(r)}_o] 
&= E[f^{(r)}(X^{(d)}_1,X^{(d)}_2,...,X^{(d)}_g)] \label{eq:errorBound0}\\
&= 1-E[\prod_{i=1}^g \big{(}1-f^{(r)}(X^{(d)}_i)\big{)}] \label{eq:errorBound1}
\end{align}

A naive approach to calculating the probability $Pr[P^{(r)}_o]$ is to regard $X^{(d)}_i$ as mutually independent. Then we have

\begin{align} 
Pr[P^{(r)}_o] 
&= 1-\prod_{i=1}^g E[1-f^{(r)}(X^{(d)}_i)] \label{eq:errorBound2}\\
&= 1-\prod_{i=1}^g (1-E[f^{(r)}(X^{(d)}_i)]) \label{eq:errorBound3}\\
&= 1-(1-E[f^{(r)}(X^{(d)}_i)])^g \label{eq:errorBound4}
\end{align}

And the term $E[f^{(r)}(X^{(d)}_1)]$ in \autoref{eq:errorBound4} can be easily bounded by \autoref{eq:frx} as follows:

\begin{align}
& E[f^{(r)}(X^{(d)}_1)]\\
= &\sum_{k=0}^d \mathcal{B}(k;d,\frac{1}{n})f^{(r)}(k)\\
= &\sum_{k=0}^t \mathcal{B}(k;d,\frac{1}{n})f^{(r)}(k) + \sum_{k=t+1}^d \mathcal{B}(k;d,\frac{1}{n})f^{(r)}(k)\label{eq:beforeLeq}\\
\leq & \sum_{k=0}^t \mathcal{B}(k;d,\frac{1}{n})f^{(r)}(k) + \sum_{k=t+1}^d \mathcal{B}(k;d,\frac{1}{n})\label{eq:afterLeq}\\
= & \sum_{k=0}^t \mathcal{B}(k;d,\frac{1}{n})\big{(}1-v_k^{(r)}(0)\big{)}+\sum_{k=t+1}^d \mathcal{B}(k;d,\frac{1}{n})
\end{align}

Here $\mathcal{B}(k;d,\frac{1}{n})$ is the Binomial probability mass function, and how to compute $v_k^{(r)}(0)$ is discussed in \autoref{sec:tail_bound_per_group} for $\forall k=0,1,...,t$ and $r\in\mathbb{Z}$. From \autoref{eq:beforeLeq} to \autoref{eq:afterLeq}, the loss is very negligible, since $\mathcal{B}(k;d,\frac{1}{n})$ is very small when $k>t$ ($t$ is $2-3$ times of $d/n$).

However, those random variable $X^{(d)}_i$ are not totally independent since they are conditioned by $\sum_{i=1}^g X^{(d)}_i=d$. So the above bound is not rigorous. Fortunately, we have the following theorem (Times-2-Bound) to decouple the weak correlation among $(X^{(d)}_1,...,X^{(d)}_m)$ and bound $Pr[P^{(r)}_o]$ rigorously to be $2$ times of the unrigorous bound in \autoref{eq:errorBound3}. 

\textbf{Theorem 1} {\bf citation}
Let $(X^{(n)}_1,...,X^{(n)}_m)$ follows the multinomial distribution of throwing $n$ balls into $m$ bins. Let $(Y^{(n)}_1,...,Y^{(n)}_m)$ be independent and identically distributed random variables with distribution $Poission(\frac{n}{m})$. Let $f(x_1,...,x_m)$ be a nonnegative function which is increasing in each argument separately. Then
\begin{equation} \label{eq:times2bound}
E[f(X^{(n)}_1,X^{(n)}_2,...,X^{(n)}_m)] \leq 2E[f(Y^{(n)}_1,Y^{(n)}_2,...,Y^{(n)}_m)]
\end{equation}


A naive approach to calculating the probability $Pr[P^{(r)}_o]$ is to regard $X^{(d)}_i$ as mutually independent. In this case, the production in the expectation of \autoref{eq:errorBound1} can be extracted out of the expectation and hence could be easily bounded. However, those random variable $X^{(d)}_i$ are not totally independent since they are conditioned by $\sum_{i=1}^m X^{(d)}_i=d$. Fortunately, we have the following theorem to decouple the weak correlation among $(X^{(d)}_1,...,X^{(d)}_m)$ and bound our targeted probability.

\textbf{Theorem 1}
Let $(X^{(n)}_1,...,X^{(n)}_m)$ follows the multinomial distribution of throwing $n$ balls into $m$ bins. Let $(Y^{(n)}_1,...,Y^{(n)}_m)$ be independent and identically distributed random variables with distribution $Poission(\frac{n}{m})$. Let $f(x_1,...,x_m)$ be a nonnegative function which is increasing in each argument separately. Then
\begin{equation} \label{eq:times2bound}
E[f(X^{(n)}_1,X^{(n)}_2,...,X^{(n)}_m)] \leq 2E[f(Y^{(n)}_1,Y^{(n)}_2,...,Y^{(n)}_m)]
\end{equation}

Substitute \autoref{eq:times2bound} into \autoref{eq:errorBound0}, we have
\begin{align} 
Pr[P^{(r)}_o] 
&= E[f^{(r)}(X^{(d)}_1,X^{(d)}_2,...,X^{(d)}_m)] \\
&\leq 2E[f^{(r)}(Y^{(d)}_1,Y^{(d)}_2,...,Y^{(d)}_m)] \\
&= 2-2E[\prod_{i=1}^m \big{(}1-f^{(r)}(Y^{(d)}_i)\big{)}] \\
&= 2-2\prod_{i=1}^m \big{(}1-E[f^{(r)}(Y^{(d)}_i)]\big{)} \label{eq:beforeSimp}\\
&= 2-2\big{(}1-E[f^{(r)}(Y^{(d)}_1)]\big{)}^m \label{eq:afterSimp}\\
\end{align}

From \autoref{eq:beforeSimp} to \autoref{eq:afterSimp}, we use the property that $Y^{(d)}_i$, $i=1,2,...,m$ are i.i.d random variables with distribution $Poisson(\delta)$ $(\delta = \frac{d}{m})$. And the term $E[f^{(r)}(Y^{(d)}_1)]$ in \autoref{eq:afterSimp} can be easily bounded by \autoref{eq:frx} as follows:

\begin{align}
& E[f^{(r)}(Y^{(d)}_1)]\\
= &\sum_{k=0}^d p(k;\delta)f^{(r)}(k)\\
= &\sum_{k=0}^c p(k;\delta)f^{(r)}(k) + \sum_{k=c+1}^d p(k;\delta)f^{(r)}(k)\label{eq:beforeLeq}\\
\leq & \sum_{k=0}^c p(k;\delta)f^{(r)}(k) + \sum_{k=c+1}^d p(k;\delta)\label{eq:afterLeq}\\
= & \sum_{k=0}^c p(k;\delta)\big{(}1-v_k^{(r)}(0)\big{)}+\sum_{k=c+1}^d p(k;\delta)
\end{align}

Here $p(k;\delta)$ is the Poisson probability mass function, and how to compute $v_k^{(r)}(0)$ is discussed in \autoref{sec:tail_bound_per_group} for $\forall k=0,1,...,c$ and $r\in\mathbb{Z}$. From \autoref{eq:beforeLeq} to \autoref{eq:afterLeq}, the loss is very negligible, since $p(k;\delta)$ is very small when $k>c$ ($c>2\delta$).

\end{comment}

\subsection{Parameter Settings}\label{sec:parameter_settings}

% The tail bound is based on the total number of distinct elements $d$, which is however not known precisely. The ToW Estimator introduced in \autoref{subsec:ToW} can only provide an estimation of $d$ (denoted as $\hat{d}$). Note that the tail bound of $Pr[P^{(r)}_o]$ increases as $d$ increases. So overestimate $d$ will get us a larger failure probability $Pr[P^{(r)}_o]$. To ensure a high success probability, we use an overestimated number of distinct element $\bar{d}$ $(>\hat{d})$ for parameter settings, such that $\bar{d}\geq d$ with high probability. In our evaluation, we set $\bar{d}\triangleq 1.38\hat{d}$, such that $\bar{d}\geq d$ with probability $99\%$. 

In this section, we elaborate how to set the parameters (i.e., $n$, $t$, $g$) given $d$ and the objective $(r,p_0)$ (defined in \autoref{subsec:protocol2}) in PBS. For the moment, we assume $d$ is precisely known. 
Given the objective $(r, p_0)$
%(i.e., set reconciliation is complete in $r$ rounds with probability $p_0$) 
%depend on the requirement of specific applications)
, the parameter setting problem aims to find the optimal parameter settings on $n,t,g$ that minimizes the overall communication overhead, under the constraint that the tail bound of the success probability in $r$ rounds is larger than $p_0$. As explained in \autoref{subsec:protocol2}, $\delta$ should be a small number, so we fix $\delta=5$ and therefore $g=d/\delta$ is also fixed. Note that the only two components in the communication overhead per group (described in \autoref{sec:multi-rounds}) that depend on parameter settings are $t\log n+\delta\log n$. So we can formalize the parameter setting problem as the following optimization problem:

\begin{equation}
\min\limits_{n,t} t\log n+\delta\log n \quad \mbox{s.t.}\quad 1-2(1-\alpha^g(n,t))>p_0
\end{equation}

\begin{align}
\mbox{minimize} \quad
&
t\log n+\delta\log n \label{obj:min_communication}
\\
\mbox{subject to} \quad 
&
1-2(1-\alpha^g(n,t))>p_0  \label{eq:success_rate_requirement}
\\
&
n,t\in \mathbb{N}^+ \label{eq:row_sum_requirement}
\end{align}

This optimization problem seems to be very difficult to solve, since the constraint is a very comprehensive function of the parameters (remind that $\alpha=\alpha(n,t)$ is a function of $n$ and $t$ for arbitrary $r$, $d$, and $g$). However, we can narrow down the solution space into only a few combinations and traverse all these combinations to find the optimal parameter settings as follows: First, for BCH coding efficiency, we select $n$ to be $2^m-1$ for some integer $m$ and therefore narrow its range down to $\{63,127,255,511,1023\}$ (recall that $n=\Omega(\delta^2)$). Second, we select $t$ in the range from $1.5\delta$ to $3\delta$, as we suggested in \autoref{subsec:protocol2}. 

Here we use an example to show how we set parameters: Given $d=1000$, $r=3$, $p_0=0.99\%$, for each $(n,t)$ combination in $\{63,127,255,511,1023\}\times \{8,9,...,15\}$, we compute the tail bound of the success probability under the parameter settings and obtain the following table:

\begin{table}[h]
\centering
\caption{Tail bound of success probability}\label{tab:success_prob}
\begin{tabular}{@{}|c|c|c|c|c|c|@{}}
\hline 
\diagbox{$t$}{$n$}    & $63$ & $127$ & $255$ & $511$ & $1023$ \\ \hline 
8   & 0 & 25.5\% & 32.7\% & 34.3\% & 34.9\% \\ \hline
9   & 52.1\% & 78.0\% & 84.2\% & 85.7\% & 86.1\% \\ \hline
10  & 75.1\% & 92.7\% & 96.5\% & 97.4\% & 97.6\% \\ \hline
11  & 85.9\% & 96.9\% & \cellcolor{blue!25}99.1\% & \cellcolor{blue!25}99.5\% & \cellcolor{blue!25}99.6\% \\ \hline
12  & 91.3\% & 98.5\% & \cellcolor{blue!25}99.7\% & \cellcolor{blue!25}99.9\% & \cellcolor{blue!25}$>$99.9\% \\ \hline
13  & 93.9\% & \cellcolor{blue!25}99.1\% & \cellcolor{blue!25}99.8\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% \\ \hline
14  & 95.1\% & \cellcolor{blue!25}99.4\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% \\ \hline
15  & 95.6\% & \cellcolor{blue!25}99.5\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% \\ 
\hline 
\end{tabular}
\end{table}

In the table, all $(n,t)$ combinations in the blue cells satisfy the success probability requirement. Among them, $(127,13)$ has the lowest communication overhead ({\bf measured? quantized?} by $t\log n+\delta\log n$). So we set $n=127, t=13$ in this case. {\bf (may be unnecessary) Note that both the success probability and the overall communication overhead are strictly increasing w.r.t. $n$ and $t$. Hence, instead of computing all values in the table, we could strategically compute only a few of them and obtain the optimal $(n,t)$ (e.g., find the optimal $t$ for each $n$ by binary search each column).}

\begin{comment}
If not, we use the ToW estimator described in \autoref{subsec:ToW} to obtain $\hat{d}$ (i.e., the estimation of $d$). Then scale it up (e.g., $d=1.38\hat{d}$ in \autoref{sec:evaluation}) for parameter setting, as explained in \autoref{subsec:ToW}. 

Here are the $4$ parameters that need to determine: 

\begin{itemize}
	\itemsep0em
	%\item $\delta$: Average number of distinct elements per group; 
	\item $g$: Number of group pairs; 
	\item $n$: Number of subset pairs in each group pair; 
	\item $r$: Number of rounds; 
	\item $t$: BCH decode capability;
\end{itemize}

Note that the number of groups $g$ is determined after $\delta$ is determined (i.e., $g=\frac{\bar{d}}{\delta}$). Now we describe how to set the four parameters using the tail bound. First, we set $\delta$ to be some small integer (e.g., $\delta=5$), so that the computational complexity (approx $\propto \delta^2$) is small. Second, we set $r$ to be some small integer (e.g., $r=3$), so that the round-trip delay is reasonable. Third, we set an objective success probability $p$ (depend on the requirement of specific applications), and we consider a parameter combination $(n,t)$ is {\it feasible} if and only if the success probability under this parameter setting based on the tail bound is larger than $p$. Among all feasible parameter combinations $(n,t)$, we select the one that has the lowest communication overhead, which can be roughly expressed as $(\delta \log u + t\log n + \delta \log n + 32)\cdot d/\delta$, as explained in \autoref{subsec:protocol2}. Here $u$ (i.e., the size of the element universe) and $d$ (i.e., the number distinct elements) do not depend on the parameter combination. So we only need to minimize $(t+\delta) \log n$ subject to $n$ and $t$. 
\end{comment}
\begin{comment}

\autoref{fig:mc} presents an example state transition diagram with 6 states (0 - 5 ``hidden elements''), denoting the corresponding transition matrix as $P=(p_{i,j})_{6\times 6}$, where $p_{i,j}$ is the probability of moving from State $i$ to State $j$. 

For instance, $p_{5,0}$ denotes the probability that all 5 set differences are decoded, which means the 5 set differences are all hashed into separate bins. $p_{5,2}$ denotes the probability that 3 (=5-2) out of 5 set differences are decoded, which means 3 set differences are hashed into separate bins and 2 set differences are hashed into the same bin. 


Let $L_{max}$ denote the maximum number of errors that BCH code can correct. Define $g^{(r)}(s)$ as follows:

\begin{equation}
    g^{(r)}(s) = \left\{ \begin{array}{ccc}
f^{(r)}(s) & \mbox{for}
& 0\leq s\leq L_{max} \\ 1 & \mbox{for} & s>L_{max}
\end{array}\right.
\end{equation}



Assume BCH code is capable of decode $s$ set differences, then the decode process of a group can be considered as a Markov chain, in which state is defined as the number of ``hidden elements'' (i.e., elements belonging to the set differences that haven't been decoded). \autoref{fig:mc} presents an example state transition diagram with 6 states (0 - 5 ``hidden elements''), denoting the corresponding transition matrix as $P=(p_{i,j})_{6\times 6}$, where $p_{i,j}$ is the probability of moving from State $i$ to State $j$. 

For instance, $p_{5,0}$ denotes the probability that all 5 set differences are decoded, which means the 5 set differences are all hashed into separate bins. $p_{5,2}$ denotes the probability that 3 (=5-2) out of 5 set differences are decoded, which means 3 set differences are hashed into separate bins and 2 set differences are hashed into the same bin. 
% And $p_{5,4}$ denotes the probability that only 1 (=5-4) set difference are decoded. The other 4 set differences could be either hashed into the same bin, or two separate bins with 2 elements in each. 

The transition in this Markov chain basically has three properties: (1) All state transitions are either self-loops or from ``higher'' states to ``lower'' states, since decode process won't generate additional set differences; (2) No state transition to State 1, because 1 remaining difference must be in a bin by itself and is able to be decoded within the same round of transition; (3) State 0 denotes all set differences are decode, which is all the absorbing state of the Markov chain. 

In the context of the Markov chain, $f^{(r)}(k)$ equals the probability that State $k$ does not transient to State 0 (absorbing state) in $r$ rounds. Let $\{e_i\}_{i=0,1,2,...,k}$ denote the standard basis vectors of length $k+1$, where $e_i$ has a single nonzero value 1 at the $(i+1)^{th}$ position. Based on the property of Markov chain, $x^{(r)}_k\triangleq e_k\cdot P^r$ is the probability vector of states after $r$ rounds with $k$ initial set differences, and the $i^{th}$ element in $x^{(r)}_k$ denotes the probability that State $k$ transients to State $i-1$ after $r$ rounds. 

$x^{(r)}(k)=(p^{(r)}_{k,0},p^{(r)}_{k,1},...,p^{(r)}_{k,k})$ denote the probability vector of states after $r$ rounds with $k$ initial set differences, where $p^{(r)}_i$ denotes the probability . 

Given the transition matrix $P$, we can easily 

\begin{figure*}
\centering
\includegraphics[width=0.98\textwidth]{figures/set_diff_markov}
\caption{Markov chain diagram for decoding process of set difference.}\label{fig:mc}
\end{figure*}

First, we assume the length of BCH decode is sufficient to decode each group. Then the decode process of each group can be considered as a Markov chain, in which state is defined as the number of "hidden elements" (i.e., elements belonging to the set difference that are to be decoded). \autoref{fig:mc} presents the state transition diagram, denoting the corresponding transmission matrix as $P=(p_{i,j})_{(d+1)\times (d+1)}$, where $p_{i,j}$ is the probability of moving from State $i$ to State $j$. By the same anology above, considering the classical balls-into-bins problem: $i$ balls are thrown independently and uniformly at random into $m'$ bins. Then $p_{i,j}$ equals to the probability that $i-j$ out of $m'$ bins have exactly one ball in each. Let $p^{(k)}_{i,j}$ denote the probability that $i-j$ out of $m'$ bins have exactly one ball in each, and $k$ out of $m'$ bins are empty. Then we have


\medskip
\noindent
{\bf Analysis on Number of Rounds}.
Consider the whole process as a Markov chain, whose state is defined as the number of 
``hidden elements'' ({\it i.e.,} elements belonging to the set difference that are to be decoded). 
\autoref{fig:mc} presents the state transition diagram, denoting the corresponding transmission 
matrix as $P=\big{(}p_{i,j}\big{)}_{(d+1)\times (d+1)}$ where $p_{i,j}$ is the probability of moving from state $i$ to state $j$. It is complex to obtain all the elements in $P$, we 
can easily get the following probabilities, for any $k \leq d$,
\begin{align}
p_{k,0}&=\frac{\binom{m}{k}k\,!}{m^k} \\
p_{k,1}&=0 \\
p_{k,2}&=\frac{\binom{k}{2}(m-k+2)\binom{m}{k-2}(k-2)\,!}{m^k},\quad \forall k\geq 2\\
p_{k,3}&=\frac{\binom{k}{3}(m-k+3)\binom{m}{k-3}(k-3)\,!}{m^k},\quad \forall k\geq 3\\
p_{k,4}&=\frac{\big{(}\binom{k}{4}(m-k+4) + \binom{k}{2}\binom{k-2}{2}(m-k+4)(m-k+3)/2\big{)}\binom{m}{k-4}(k-4)\,!}{m^k},\quad \forall k\geq 4.
\end{align}
where $m$ is the number of buckets.

Similarly, we can calculate $p_{k,i}$ for any $k\geq i \geq 5$ but the expression gets more and more complex. 


It is not hard to check that the Markov chain described above is an absorbing Markov chain with 
a single absorbing state of $0$. By using the time to absorption theorem of Absorbing Markov Chains~\cite[Page 13]{Elizalde_LectureNotesMath_2006}, 
we can easily get the average number of rounds (steps before the chain is absorbed), which equals
the $d^{th}$ element of $(N{\bf 1})$ where the matrix 
$N=(I-Q)^{-1}$ is the fundamental matrix of $P$ (Note that $Q$ is the transition matrix for all transient states, in our case, is $P$ by removing the last row and column, {\it i.e.,} $P_{0,*}$ 
and $P_{*,0}$) and 
${\bf 1}$ is an all-one vector with length $d$. 

Denote $P^{(k)}$ as the $k$-step transition matrix, then the probability that it takes more than $n$ rounds to decode is
\begin{equation}
\mathbf{Pr}[t>n]=\sum_{k=n+1}^{\infty}p^{(k)}_{d,0},
\end{equation}
where $d$ is the initial number of elements.


\medskip
\noindent
{\bf Simplified Analysis on Number of Rounds.} In the following analysis, we assume that the number of buckets in the kth round, 
assuming remaining $d_k$ elements to be decoded, is set to be $\delta\cdot d_k$ where $\delta > 1$ is a constant. For ease of 
presentation, we drop the subscript $k$ in the following analysis\footnote{Inspired by the analysis of the number of iterations 
for PIM.}. 

Fix a bucket, the probability that it gets exactly one element belonging to the set difference that is not decoded yet is:
\begin{equation}
p = d \Big{(}\frac{1}{\delta d}\Big{)}\Big{(} 1 - \frac{1}{\delta d}\Big{)}^{d - 1} = \frac{1}{\delta}\Big{(} 1 - \frac{1}{\delta d}\Big{)}^{d - 1}\approx \frac{1}{\delta}e^{-1/\delta}.
\end{equation}

On average, there are $p$ fraction of buckets will get exact one element. Hence, on average $e^{-1/\delta}$ fraction of un-decoded 
elements will be decoded in each round. Therefore, on average, we need $\log_{\frac{1}{1- e^{-1/\delta}}}d_0$ rounds, {\it i.e.,} 
$O(\log d_0)$ rounds. 

\end{comment}



==> section/theoretical_analysis_OLD.tex <==
\section{Tug-of-War Sketch}\label{sec:sketch}


In this section, we describe the {\it tug-of-war}, which was first proposed in~\cite{AlonMS99} as 
a space-efficient estimator for the second frequency moment. 
%% Copy from Infocom 2009
We briefly describe 
the plain vanilla tug-of-war sketch~\cite{AlonMS99} in the context of error estimating coding, and under the assumption
that the sketch per se is not subject to bit errors (``noiseless") during transmission.  A tug-of-war sketch of a bit array (packet) $b$
is comprised of a constant number $c$ of counters  ($c$ is determined by the desired error guarantees) that are maintained using the same update algorithm (with possibly different update values) and is sent to the receiver alongside with $b$.
After the execution of these update algorithms, each counter contains the inner product of the bit vector $\overrightarrow{b}$ (`0' converted to `-1' as discussed earlier) with a vector $\overrightarrow{s} \in \{+1, -1\}^n $  that is four-wise independent, as shown in the following algorithm.  Such four-wise independent vectors are known to exist and have computationally efficient representations (e.g., derivable from the Reed-Muller code~\cite{GilbertKMS03}).
Note the actual update algorithm is not shown here because it is not relevant to our context; Only its ``net effect" after execution is. 


\subsection{Set Reconciliation}\label{subsec:set-reconciliation}

Before we describe how to use tug-of-war for set reconciliation~\cite{Guo_SetReconciliationvia_2013,Mitzenmacher_SimpleMultiParty_2013,Eppstein_WhatsDifference?Efficient_2011}, we first give a brief 
description of set reconciliation. For two sets $A, B$ that contain elements from the same universe, $U$, the set reconciliation 
problem wants to compute the set difference $A \Delta B\triangleq (A\setminus B)\cup (B\setminus A)$. We denote $D=A\Delta B$, and 
$d=|D|$. In the context of set reconciliation, the two sets $A$ and $B$ are stored at two distinct places and the problem wants to 
compute $D$ with minimal communication overhead. 

First, we assume that $d$ is known a prior. We will show later how to use the tug-of-war sketch 
to estimate $d$, the size of 
the set difference. 
As shown in~\cite{Eppstein_WhatsDifference?Efficient_2011}, we can achieve 
$O(d)$ (with a small constant factor) 
communication overhead to compute the set difference $D$ using 
the invertible bloom filter (IBF)~\cite{Goodrich_InvertibleBloomLookup_2011,Eppstein_StragglerIdentificationRound_2011}, which is clearly (asymptotically) optimal. However, in the cases where each element is 
very large (in terms of communication requirement) such as large documents or movie chunks, it is a large communication overhead to transmit a small constant (say $2$ or $3$) times  $d$ elements. As we will show next, by using 
the tug-of-war sketch, we can reduce the communication overhead to very close to $d$ (elements) 
with a few rounds of message exchanges. 


We assume that the communication is initiated by $A$. 
Each round of communication works as follows. 
$A$ creates $m=\delta d$ buckets, $b_1,b_2,\dots,b_m$, 
where $\delta > 1$ is a constant. Each bucket $b_i$
contains a subset of elements from $A$, 
each of which is uniformly randomly selected (with properly-designed 
hash functions). 
For each bucket $b_i$, $A$ computes $c$ tug-of-war sketches, 
denoting as $z_{i,1},z_{i,2},\dots,z_{i,c}$. Note that here eahc $z_{i,j}=\sum_{a\in b_i}h(a)$, where 
$h$ is from a four-wise hash family that maps each element to $\pm 1$. 
Then, $A$ sends the $m\times c$ sketches 
to $B$. $B$ uses the same hash functions to create $m$ buckets for its elements, and then use the same hash 
functions to compute the tug-of-war sketches for each bucket, denoting those sketches as $z'_{i,j}$ for $i\in [m]$ and 
$j\in [c]$. Then, $B$ can use $\frac{1}{c}\sum_{j=1}^{c}(z_{i,j}-z'_{i,j})^2$ to estimate the size of (sub-)set difference of 
the bucket $b_i$ for any $i\in [m]$. Note that $B$ can use the median of mean approach in~\cite{AlonMS99} 
or the MLE estimator in~\cite{Hua_TowardsOptimalError_2012} to obtain 
better estimations. Then, for each bucket whose estimator is in $(0, 1.5)$ (just an example), $B$ sends the exclusive or of all the elements 
in the bucket to $B$. It is clear that if the true size of the set difference for the bucket is $1$, then $A$ can obtain the 
element belonging to $A\Delta B$ in the bucket. 

By repeating the process until all the $d$ elements are obtained, $A$ computes the set difference $D$.

\begin{comment}
\medskip
\noindent
{\bf Analysis on Number of Rounds}.
Consider the whole process as a Markov chain, whose state is defined as the number of 
``hidden elements'' ({\it i.e.,} elements belonging to the set difference that are to be decoded). 
\autoref{fig:mc} presents the state transition diagram, denoting the corresponding transmission 
matrix as $P=\big{(}p_{i,j}\big{)}_{(d+1)\times (d+1)}$ where $p_{i,j}$ is the probability of moving from state $i$ to state $j$. It is complex to obtain all the elements in $P$, we 
can easily get the following probabilities, for any $k \leq d$,
\begin{align}
p_{k,0}&=\frac{\binom{m}{k}k\,!}{m^k} \\
p_{k,1}&=0 \\
p_{k,2}&=\frac{\binom{k}{2}(m-k+2)\binom{m}{k-2}(k-2)\,!}{m^k},\quad \forall k\geq 2\\
p_{k,3}&=\frac{\binom{k}{3}(m-k+3)\binom{m}{k-3}(k-3)\,!}{m^k},\quad \forall k\geq 3\\
p_{k,4}&=\frac{\big{(}\binom{k}{4}(m-k+4) + \binom{k}{2}\binom{k-2}{2}(m-k+4)(m-k+3)/2\big{)}\binom{m}{k-4}(k-4)\,!}{m^k},\quad \forall k\geq 4.
\end{align}
where $m$ is the number of buckets.

Similarly, we can calculate $p_{k,i}$ for any $k\geq i \geq 5$ but the expression gets more and more complex. 


It is not hard to check that the Markov chain described above is an absorbing Markov chain with 
a single absorbing state of $0$. By using the time to absorption theorem of Absorbing Markov Chains~\cite[Page 13]{Elizalde_LectureNotesMath_2006}, 
we can easily get the average number of rounds (steps before the chain is absorbed), which equals
the $d^{th}$ element of $(N{\bf 1})$ where the matrix 
$N=(I-Q)^{-1}$ is the fundamental matrix of $P$ (Note that $Q$ is the transition matrix for all transient states, in our case, is $P$ by removing the last row and column, {\it i.e.,} $P_{0,*}$ 
and $P_{*,0}$) and 
${\bf 1}$ is an all-one vector with length $d$. 

Denote $P^{(k)}$ as the $k$-step transition matrix, then the probability that it takes more than $n$ rounds to decode is
\begin{equation}
\mathbf{Pr}[t>n]=\sum_{k=n+1}^{\infty}p^{(k)}_{d,0},
\end{equation}
where $d$ is the initial number of elements.


\medskip
\noindent
{\bf Simplified Analysis on Number of Rounds.} In the following analysis, we assume that the number of buckets in the kth round, 
assuming remaining $d_k$ elements to be decoded, is set to be $\delta\cdot d_k$ where $\delta > 1$ is a constant. For ease of 
presentation, we drop the subscript $k$ in the following analysis\footnote{Inspired by the analysis of the number of iterations 
for PIM.}. 

Fix a bucket, the probability that it gets exactly one element belonging to the set difference that is not decoded yet is:
\begin{equation}
p = d \Big{(}\frac{1}{\delta d}\Big{)}\Big{(} 1 - \frac{1}{\delta d}\Big{)}^{d - 1} = \frac{1}{\delta}\Big{(} 1 - \frac{1}{\delta d}\Big{)}^{d - 1}\approx \frac{1}{\delta}e^{-1/\delta}.
\end{equation}

On average, there are $p$ fraction of buckets will get exact one element. Hence, on average $e^{-1/\delta}$ fraction of un-decoded 
elements will be decoded in each round. Therefore, on average, we need $\log_{\frac{1}{1- e^{-1/\delta}}}d_0$ rounds, {\it i.e.,} 
$O(\log d_0)$ rounds. 
\end{comment}

\section{Tail Bound Analysis and Parameter Settings}\label{sec:tail_bound}

In this section, we establish a strict tail bound on the probability of a successful reconciliation on all subset pairs (defined as $Pr[P^{(r)}_o]$ in this section) under our scheme. To establish the tail bound, we first establish a tail bound for each subset pair using Markov chain and dynamic programming in \autoref{sec:tail_bound_per_group}. Then in \autoref{sec:times2bound}, we derive a strict tail bound of $Pr[P^{(r)}_o]$ using Times-2-Bound. In \autoref{sec:parameter_settings}, we will discuss parameter settings using the tail bound.  

\subsection{Numerical Tail Bound for Each Subset Pair}\label{sec:tail_bound_per_group}

In this section, we only consider the case that a subset pair is BCH-decodable (i.e., contains $t\leq \tau$ exclusive elements). As we described in ..., each group hashes $i$ elements (set differences) into $c$ cells in each round, and an element is decoded if and only if it is hashed into a cell that contains only 1 element. For an analogy, the statistical model for hashing $i$ elements into $c$ cells is the same as the classical balls-and-bins problem: $i$ balls are thrown independently and uniformly at random into $c$ bins. To make our description simple, we call a bin is ``good'' if and only if it receives exactly 1 ball. And we call a bin is ``bad'' if and only if it receives at least 2 balls. The rest bins (i.e., neither ``good'' nor ``bad'') are empty. Then the elements that are decoded correspond to the balls that are in ``good'' bins. 

The decode process of each group can be considered as a Markov Chain, in which each state is defined as the number of ``hidden elements'' (i.e., the elements belonging to the set differences that haven't been decoded). And in this Markov chain, the transition from State $i$ to State $j$ means $i-j$ out of $i$ elements are decoded in this round, where $0\leq j\leq i\leq \tau$. Use the same analogy, the number (state) is simply the total number of balls that fall in ``bad'' bins. And the transition from State $i$ to State $j$ means $i-j$ out of $i$ balls fall in ``good'' bins in this round, while the rest $j$ balls fall in ``bad'' bins. 

Let $M=(m_{i,j})_{(\tau+1)\times (\tau+1)}$ denote the transition matrix of the above Markov chain, where $m_{i,j}$ is the probability of transition from State $i$ to State $j$. 
%In the analogy of balls-and-bins problem, $m_{i,j}$ equals to the probability that $i-j$ out of $i$ balls are thrown into bins with just 1 ball, or $i-j$ out of $c$ bins are ``good'' bins.

Note that every State $j$ with $j > 3$ in the Markov chain is a composite state as far as the calculation of the transition probability from a (larger) state $i > j$ to $j$ (i.e., ``transitioning into").  For example, State 6 contains 4 different cases. The first case is $6 = 6$, where all 6 bad balls are in the same bad bin. The second case is $6 = 2 + 4$ where, out of the 6 bad balls, four are in one bad bin and the other two are in the other bad bin.  Similarly, the other two cases are $6 = 3 + 3$ and $6 = 2 + 2 + 2$. Note there is no need to distinguish these four cases in calculating the ``transitioning out" probability (i.e., from state 6 to a small state say State 0), because the next round of balls-into-bins operation uses a different hash function independent of that used in the current round, and consequently how these 6 bad balls are split in the current round have no bearing on that in the next round. 

Building on the example above, we now consider $m_{9,6}$, the transition probability from State $9$ to State $6$ (throwing 9 balls into 1,023 bins and ending up with 6 bad balls).  $m_{9,6}$ is simply the sum of the probabilities of these four cases, each of which has a very different formula than the others.  In general, the number of such cases, and hence the number of individual probability terms to be added up to arrive at the transition matrix element $m_{i,j}$, grows exponentially with the value of $j$. This does not however make it difficult to calculate the values of $M$, because there is a recursive structure, among the values of the matrix elements $m_{i,j}$, that can be exploited using dynamic programming, as will be elaborated in \autoref{sec:transition_matrix}.

Let $v^{(r)}_i=\big{(}{v^{(r)}_i(0), v^{(r)}_i(1),...,v^{(r)}_i(\tau)}\big{)}$ denote the probability vector (i.e., $\sum_{j=0}^{\tau}v^{(r)}_i(j) = 1$) after $r$ rounds with initial State $i$: $v^{(r)}_i(j)$ denotes the probability that the final state is State $j$ after $r$ rounds. In the probability vector, $v^{(r)}_i(0)$ is the only ``good'' entry, which is the probability of the cases that all set differences are decoded after $r$ rounds. The probability of the group does not complete reconciliation is simply $1-v^{(r)}_i(0)$. 

Given the transition matrix $M$, we can easily compute the probability vector $v^{(r)}_i$ for any $r$ and $i$ as follows:
\begin{equation}
    x^{(r)}_i = e_i\cdot M^r
\end{equation}
Here $\{e_i\}_{i=0,1,2,...,\tau}$ denote the standard basis vectors of length $\tau+1$, where $e_i$ has a single nonzero value 1 at the $(i+1)^{th}$ position. So the remaining problem is how to compute $M$.

\subsubsection{Transition Matrix}\label{sec:transition_matrix}

Now we describe how to compute the transition matrix $M$ using dynamic programming in detail. As we described earlier, every State $j$ with $j > 3$ in the Markov chain is a composite state that contains many different cases. And the number of these cases increases exponentially with the value of $j$. To simply our analysis, we split each composite state into sub-composite states based on the number of nonempty bins: Let State $(j,k)$ denotes the sub-composite state with $j$ ``hidden elements'' and $k$ nonempty bins, which is also a substate of State $j$. Let $m_{i,j}^{(k)}$ denote the probability of transition from State $i$ to State $(j,k)$, which is also the probability that after throwing $i$ balls uniformly and independently into $c$ bins, $i-j$ bins are ``good'' bins and $k$ bins are nonempty bins (thus $k-(i-j)$ bins are ``bad'' and $c-k$ bins are empty). The probability of transition to a composite state is simply the summation of the probabilities of the transitions to corresponding sub-composite states:

\begin{equation}
    m_{i,j} = \sum_{k=i}^{i-j} m^{(k)}_{i,j}
\end{equation}

To obtain the transition matrix $M$, it is sufficient to compute $m^{(k)}_{i,j}$, which can be exploited using dynamic programming. Note that the balls-and-bins model itself can be considered as a Markov chain, in which a recursive relation exists: After throwing $i$ balls into $c$ bins, throwing one more ball randomly could be: (1) Into an empty bin and turn it to a ``good'' bin; (2) Into a ``good'' bin and turn it to a ``bad'' bin with two balls; or (3) Into a ``bad'' bin and keep it as the same. Mathematically, we have 

\begin{align}
m^{(k)}_{i+1,j} =& \frac{c-k+1}{c}\cdot m^{(k-1)}_{i,j-1} + \frac{j+1}{c}\cdot m^{(k)}_{i,j+1} \nonumber\\
&+ \frac{k-(i-j)}{c}\cdot m^{(k)}_{i,j} \label{eq:recursion}
\end{align}

The three terms in \autoref{eq:recursion} corresponds to the above three cases. Meanwhile, we can easily get the following probabilities for basic cases:

\begin{align}
m^{(k)}_{i,0} =& \left\{ \begin{array}{ccl}
\binom{c}{i}/c^i, & \mbox{if }
 k=i \\ 0, & \mbox{otherwise} 
\end{array}\right.\label{eq:basic1}\\
m^{(k)}_{0,j} =& \left\{ \begin{array}{ccl}
1, & \mbox{if }
 k=0 \mbox{ and } j=0 \\ 0, & \mbox{otherwise} 
\end{array}\right.\label{eq:basic2}\\
m^{(0)}_{i,j} =& \left\{ \begin{array}{ccl}
1, & \mbox{if }
 i=0 \mbox{ and } j=0 \\ 0, & \mbox{otherwise} 
\end{array}\right.\label{eq:basic3}
\end{align}

Using \autoref{eq:recursion},\autoref{eq:basic1},\autoref{eq:basic2}, and \autoref{eq:basic3}, we can recursively compute $m^{(k)}_{i,j}$ and then get $v^{(r)}_i(0)$ for $\forall i=0,1,...,\tau$ and $r\in\mathbb{Z}$. The value of $v^{(r)}_i(0)$ will be used to compute the tail bound of $Pr[P^{(r)}_o]$ in the next section. 

\subsection{Global Tail Bound Analysis}\label{sec:times2bound}

Let random variable $X^{(d)}_i, 1\leq i\leq m$, denote the number of set differences initially allocated in the $i^{th}$ group. For an analogy, the statistical model for hashing $d$ set differences into $m$ groups is also the same as the classical balls-and-bins problem: $d$ balls are thrown independently and uniformly at random into $m$ bins. Then random variable $X^{(d)}_i$ could be translated as the number of balls ended up in the $i^{th}$ bin after $d$ balls are thrown. Therefore, $(X^{(d)}_1,...,X^{(d)}_m)$ follows the multinomial distribution. The marginal distribution for any $X^{(d)}_i$ is $Binomial(d,\frac{1}{m})$, where $Binomial(N,p)$ denotes the binomial distribution resulting from $N$ trials with success probability $p$. 

Let $f^{(r)}(x_1,x_2,...,x_m)$ denote the probability that set reconciliation does not complete (for all groups) in $r$ rounds when the $i^{th}$ group initially contains $x_i$ set differences for $i=1,2,...,m$. Define $f^{(r)}(x)$ as the probability that set reconciliation does not complete in $r$ rounds when a group initially contains $x$ set differences. Based on the result in \autoref{sec:tail_bound_per_group}, we have 

% \begin{equation}\label{eq:frx}
%     f^{(r)}(x) \leq g^{(r)}(x) \triangleq \left\{ \begin{array}{ccc}
% 1-v^{(r)}_{x}(0) & \mbox{for}
% & 0\leq x\leq \tau \\ 1 & \mbox{for} & x>\tau
% \end{array}\right.
% \end{equation}

\begin{equation}\label{eq:frx}
    f^{(r)}(x) = 1-v^{(r)}_{x}(0) \mbox{ for }  0\leq x\leq \tau 
\end{equation}

Since the reconciliation processes independently for each group, we have 

\begin{equation}
f^{(r)}(x_1,x_2,...,x_m) = 1-\prod_{i=1}^m \big{(}1-f^{(r)}(x_i)\big{)}
\end{equation}

Then we have 

\begin{align} 
Pr[P^{(r)}_o] 
&= E[f^{(r)}(X^{(d)}_1,X^{(d)}_2,...,X^{(d)}_m)] \label{eq:errorBound0}\\
&= 1-E[\prod_{i=1}^m \big{(}1-f^{(r)}(X^{(d)}_i)\big{)}] \label{eq:errorBound1}
\end{align}

A naive approach to calculating the probability $Pr[P^{(r)}_o]$ is to regard $X^{(d)}_i$ as mutually independent. In this case, the production in the expectation of \autoref{eq:errorBound1} can be extracted out of the expectation and hence could be easily bounded. However, those random variable $X^{(d)}_i$ are not totally independent since they are conditioned by $\sum_{i=1}^m X^{(d)}_i=d$. Fortunately, we have the following theorem to decouple the weak correlation among $(X^{(d)}_1,...,X^{(d)}_m)$ and bound our targeted probability.

\textbf{Theorem 1}
Let $(X^{(n)}_1,...,X^{(n)}_m)$ follows the multinomial distribution of throwing $n$ balls into $m$ bins. Let $(Y^{(n)}_1,...,Y^{(n)}_m)$ be independent and identically distributed random variables with distribution $Poission(\frac{n}{m})$. Let $f(x_1,...,x_m)$ be a nonnegative function which is increasing in each argument separately. Then
\begin{equation} \label{eq:times2bound}
E[f(X^{(n)}_1,X^{(n)}_2,...,X^{(n)}_m)] \leq 2E[f(Y^{(n)}_1,Y^{(n)}_2,...,Y^{(n)}_m)]
\end{equation}

Substitute \autoref{eq:times2bound} into \autoref{eq:errorBound0}, we have
\begin{align} 
Pr[P^{(r)}_o] 
&= E[f^{(r)}(X^{(d)}_1,X^{(d)}_2,...,X^{(d)}_m)] \\
&\leq 2E[f^{(r)}(Y^{(d)}_1,Y^{(d)}_2,...,Y^{(d)}_m)] \\
&= 2-2E[\prod_{i=1}^m \big{(}1-f^{(r)}(Y^{(d)}_i)\big{)}] \\
&= 2-2\prod_{i=1}^m \big{(}1-E[f^{(r)}(Y^{(d)}_i)]\big{)} \label{eq:beforeSimp}\\
&= 2-2\big{(}1-E[f^{(r)}(Y^{(d)}_1)]\big{)}^m \label{eq:afterSimp}\\
\end{align}

From \autoref{eq:beforeSimp} to \autoref{eq:afterSimp}, we use the property that $Y^{(d)}_i$, $i=1,2,...,m$ are i.i.d random variables with distribution $Poisson(\frac{d}{m})$. And the term $E[f^{(r)}(Y^{(d)}_1)]$ in \autoref{eq:afterSimp} can be easily bounded by \autoref{eq:frx} as follows:

\begin{align}
& E[f^{(r)}(Y^{(d)}_1)]\\
= &\sum_{k=0}^d p(k;\frac{d}{m})f^{(r)}(k)\\
= &\sum_{k=0}^\tau p(k;\frac{d}{m})f^{(r)}(k) + \sum_{k=\tau+1}^d p(k;\frac{d}{m})f^{(r)}(k)\label{eq:beforeLeq}\\
\leq & \sum_{k=0}^\tau p(k;\frac{d}{m})f^{(r)}(k) + \sum_{k=\tau+1}^d p(k;\frac{d}{m})\label{eq:afterLeq}\\
= & \sum_{k=0}^\tau p(k;\frac{d}{m})\big{(}1-v_k^{(r)}(0)\big{)}+\sum_{k=\tau+1}^d p(k;\frac{d}{m})
\end{align}

Here $p(k;\frac{d}{m})$ is the Poisson probability mass function, and how to compute $v_k^{(r)}(0)$ is discussed in \autoref{sec:tail_bound_per_group} for $\forall k=0,1,...,\tau$ and $r\in\mathbb{Z}$. From \autoref{eq:beforeLeq} to \autoref{eq:afterLeq}, the loss is very negligible, since $p(k;\frac{d}{m})$ is very small for $k>\tau$ ($\tau>\frac{2d}{m}$).

\subsection{Parameter Settings}\label{sec:parameter_settings}

\begin{comment}

\autoref{fig:mc} presents an example state transition diagram with 6 states (0 - 5 ``hidden elements''), denoting the corresponding transition matrix as $P=(p_{i,j})_{6\times 6}$, where $p_{i,j}$ is the probability of moving from State $i$ to State $j$. 

For instance, $p_{5,0}$ denotes the probability that all 5 set differences are decoded, which means the 5 set differences are all hashed into separate bins. $p_{5,2}$ denotes the probability that 3 (=5-2) out of 5 set differences are decoded, which means 3 set differences are hashed into separate bins and 2 set differences are hashed into the same bin. 


Let $L_{max}$ denote the maximum number of errors that BCH code can correct. Define $g^{(r)}(s)$ as follows:

\begin{equation}
    g^{(r)}(s) = \left\{ \begin{array}{ccc}
f^{(r)}(s) & \mbox{for}
& 0\leq s\leq L_{max} \\ 1 & \mbox{for} & s>L_{max}
\end{array}\right.
\end{equation}



Assume BCH code is capable of decode $s$ set differences, then the decode process of a group can be considered as a Markov chain, in which state is defined as the number of ``hidden elements'' (i.e., elements belonging to the set differences that haven't been decoded). \autoref{fig:mc} presents an example state transition diagram with 6 states (0 - 5 ``hidden elements''), denoting the corresponding transition matrix as $P=(p_{i,j})_{6\times 6}$, where $p_{i,j}$ is the probability of moving from State $i$ to State $j$. 

For instance, $p_{5,0}$ denotes the probability that all 5 set differences are decoded, which means the 5 set differences are all hashed into separate bins. $p_{5,2}$ denotes the probability that 3 (=5-2) out of 5 set differences are decoded, which means 3 set differences are hashed into separate bins and 2 set differences are hashed into the same bin. 
% And $p_{5,4}$ denotes the probability that only 1 (=5-4) set difference are decoded. The other 4 set differences could be either hashed into the same bin, or two separate bins with 2 elements in each. 

The transition in this Markov chain basically has three properties: (1) All state transitions are either self-loops or from ``higher'' states to ``lower'' states, since decode process won't generate additional set differences; (2) No state transition to State 1, because 1 remaining difference must be in a bin by itself and is able to be decoded within the same round of transition; (3) State 0 denotes all set differences are decode, which is all the absorbing state of the Markov chain. 

In the context of the Markov chain, $f^{(r)}(k)$ equals the probability that State $k$ does not transient to State 0 (absorbing state) in $r$ rounds. Let $\{e_i\}_{i=0,1,2,...,k}$ denote the standard basis vectors of length $k+1$, where $e_i$ has a single nonzero value 1 at the $(i+1)^{th}$ position. Based on the property of Markov chain, $x^{(r)}_k\triangleq e_k\cdot P^r$ is the probability vector of states after $r$ rounds with $k$ initial set differences, and the $i^{th}$ element in $x^{(r)}_k$ denotes the probability that State $k$ transients to State $i-1$ after $r$ rounds. 

$x^{(r)}(k)=(p^{(r)}_{k,0},p^{(r)}_{k,1},...,p^{(r)}_{k,k})$ denote the probability vector of states after $r$ rounds with $k$ initial set differences, where $p^{(r)}_i$ denotes the probability . 

Given the transition matrix $P$, we can easily 

\begin{figure*}
\centering
\includegraphics[width=0.98\textwidth]{figures/set_diff_markov}
\caption{Markov chain diagram for decoding process of set difference.}\label{fig:mc}
\end{figure*}

First, we assume the length of BCH decode is sufficient to decode each group. Then the decode process of each group can be considered as a Markov chain, in which state is defined as the number of "hidden elements" (i.e., elements belonging to the set difference that are to be decoded). \autoref{fig:mc} presents the state transition diagram, denoting the corresponding transmission matrix as $P=(p_{i,j})_{(d+1)\times (d+1)}$, where $p_{i,j}$ is the probability of moving from State $i$ to State $j$. By the same anology above, considering the classical balls-into-bins problem: $i$ balls are thrown independently and uniformly at random into $m'$ bins. Then $p_{i,j}$ equals to the probability that $i-j$ out of $m'$ bins have exactly one ball in each. Let $p^{(k)}_{i,j}$ denote the probability that $i-j$ out of $m'$ bins have exactly one ball in each, and $k$ out of $m'$ bins are empty. Then we have


\medskip
\noindent
{\bf Analysis on Number of Rounds}.
Consider the whole process as a Markov chain, whose state is defined as the number of 
``hidden elements'' ({\it i.e.,} elements belonging to the set difference that are to be decoded). 
\autoref{fig:mc} presents the state transition diagram, denoting the corresponding transmission 
matrix as $P=\big{(}p_{i,j}\big{)}_{(d+1)\times (d+1)}$ where $p_{i,j}$ is the probability of moving from state $i$ to state $j$. It is complex to obtain all the elements in $P$, we 
can easily get the following probabilities, for any $k \leq d$,
\begin{align}
p_{k,0}&=\frac{\binom{m}{k}k\,!}{m^k} \\
p_{k,1}&=0 \\
p_{k,2}&=\frac{\binom{k}{2}(m-k+2)\binom{m}{k-2}(k-2)\,!}{m^k},\quad \forall k\geq 2\\
p_{k,3}&=\frac{\binom{k}{3}(m-k+3)\binom{m}{k-3}(k-3)\,!}{m^k},\quad \forall k\geq 3\\
p_{k,4}&=\frac{\big{(}\binom{k}{4}(m-k+4) + \binom{k}{2}\binom{k-2}{2}(m-k+4)(m-k+3)/2\big{)}\binom{m}{k-4}(k-4)\,!}{m^k},\quad \forall k\geq 4.
\end{align}
where $m$ is the number of buckets.

Similarly, we can calculate $p_{k,i}$ for any $k\geq i \geq 5$ but the expression gets more and more complex. 


It is not hard to check that the Markov chain described above is an absorbing Markov chain with 
a single absorbing state of $0$. By using the time to absorption theorem of Absorbing Markov Chains~\cite[Page 13]{Elizalde_LectureNotesMath_2006}, 
we can easily get the average number of rounds (steps before the chain is absorbed), which equals
the $d^{th}$ element of $(N{\bf 1})$ where the matrix 
$N=(I-Q)^{-1}$ is the fundamental matrix of $P$ (Note that $Q$ is the transition matrix for all transient states, in our case, is $P$ by removing the last row and column, {\it i.e.,} $P_{0,*}$ 
and $P_{*,0}$) and 
${\bf 1}$ is an all-one vector with length $d$. 

Denote $P^{(k)}$ as the $k$-step transition matrix, then the probability that it takes more than $n$ rounds to decode is
\begin{equation}
\mathbf{Pr}[t>n]=\sum_{k=n+1}^{\infty}p^{(k)}_{d,0},
\end{equation}
where $d$ is the initial number of elements.


\medskip
\noindent
{\bf Simplified Analysis on Number of Rounds.} In the following analysis, we assume that the number of buckets in the kth round, 
assuming remaining $d_k$ elements to be decoded, is set to be $\delta\cdot d_k$ where $\delta > 1$ is a constant. For ease of 
presentation, we drop the subscript $k$ in the following analysis\footnote{Inspired by the analysis of the number of iterations 
for PIM.}. 

Fix a bucket, the probability that it gets exactly one element belonging to the set difference that is not decoded yet is:
\begin{equation}
p = d \Big{(}\frac{1}{\delta d}\Big{)}\Big{(} 1 - \frac{1}{\delta d}\Big{)}^{d - 1} = \frac{1}{\delta}\Big{(} 1 - \frac{1}{\delta d}\Big{)}^{d - 1}\approx \frac{1}{\delta}e^{-1/\delta}.
\end{equation}

On average, there are $p$ fraction of buckets will get exact one element. Hence, on average $e^{-1/\delta}$ fraction of un-decoded 
elements will be decoded in each round. Therefore, on average, we need $\log_{\frac{1}{1- e^{-1/\delta}}}d_0$ rounds, {\it i.e.,} 
$O(\log d_0)$ rounds. 

\end{comment}



==> section/theoretical_analysis_seperate.bk.0719.tex <==
\section{Analytical Framework}\label{sec:tail_bound}

In this section, we derive a Markov-chain model for analyzing the aforementioned single-group-pair success probability $Pr[x\!\xrsquigarrow{r}\! 0]$.  
We will show next that, 
under this model, the initial state of the Markov chain is state $x$ (distinct elements), 
and each (set reconciliation) round triggers a state transition.  
Hence, the event $\{x\!\xrsquigarrow{r}\! 0\}$ corresponds to the Markov chain reaching the ``good" 
state $0$ (distinct elements left) within $r$ transitions.  Suppose the transition probability matrix of this Markov chain is $M$, which we will
show in \autoref{sec:compute_M} how to compute.  The formula for computing the probability of this event is simply

\begin{equation}\label{eq:single_success_prob}
Pr[x\!\xrsquigarrow{r}\! 0] = \big{(}M^r\big{)}(x, 0)
\end{equation}

Here $\big{(}M^r\big{)}(x, 0)$ is the element at the intersection of the $x^{th}$ row and the 
$0^{th}$ column in the matrix $M^r$ ($M$ to the power $r$).  Note that, 
without this Markov-chain model, $Pr[x\!\xrsquigarrow{r}\! 0]$ is hard to compute except in some
special cases such as when $r = 1$ (the probability, derived earlier in \autoref{sec:hash_partition}, for the ideal case of $x$ balls thrown ending up in $x$ distinct bins to happen).
%{\color{red}In the next four sections, we will describe the Markov-chain model and its three applications}.
%following, we describe this Markov-chain model in \autoref{sec:single_markov}.
%Its preciseness will be explained in \autoref{sec:preciseness}. %and how to compute its transitioning probability matrix $M$ in \autoref{sec:compute_M}.


%the three aforementioned research questions concerning PBS.






%This probability however 
%is hard (if not impossible) to calculate exactly, because even though the set conciliation processes of the $g$ group pairs are
%statistically independent, their parameters are not as will be explained in ???.   





%modeling of the multi-group multi-round process of PBS 

%How to appropriately parameterize PBS so that it guarantees $Pr[R\leq r] \ge p_0$ yet


%the reconciliation of to be completed.  


%So a natural optimization problem here is to minimize $R$ stochastically given a fixed communication cost cap.   This optimization problem 
%However, any optimization problem involving an order statistic such as $R$ is hard to 


%In other words, the PBS scheme needs to be appropriately parameterized to 
%guarantee that 

\begin{comment}
Our analytical model is focused on a single group pair in the case of PBS-for-large-$d$,
or the set pair in the case of PBS-for-small-$d$.
% evolves one round after another.  
As mentioned earlier in \autoref{sec:multiround_large_d}, how the number of yet unreconciled distinct elements between the pair 
decreases one round after another, and 
eventually goes down to $0$, can 
be precisely modeled as a Markov chain.   



 tradeoff leads us to study the following optimization problem.     Roughly speaking, this stipulation can be considered a stochastic lower upper bound on $R$.  

specify a stochastic upper bound on $R$ in the following form:


theoretical questions concerning this multi-group multi-round operation.  

optimization problem.
%An obvious optimization goal related to $R$ is, given the total ``budget'' of communication overhead, find the optimal parameter settings for PBS that {\it stochastically minimize} $R$. 
%Instead, we propose a more optimizable goal, which is roughly the dual of the previous goal. In this optimizable goal, 
We require that the PBS scheme guarantee a {\it target success probability} $p_0$ of reconciling all $g$ group pairs (and hence the set pair) in 
a {\it target number of rounds}.  In other words, the PBS scheme needs to be appropriately parameterized to guarantee that $Pr[R\leq r] \ge p_0$.  The optimization problem is to find the optimal 
parameter setting that guarantees $Pr[R\leq r] \ge p_0$ yet results in the smallest possible
overall communication overhead.   A motivation and application of our analytical framework, to be described in~\autoref{sec:tail_bound}, is for solving this optimization problem.   



To this end, we introduce, in the next section, 
an analytical framework that 

allows for the calculation of 

allows us to resolve, in \ref{}, this optimization question and two related questions in a principled manner.

For the moment, let us assume each element (probability value) in the matrix $M$ has been computed;  how to compute these probabilities will be described in \autoref{sec:compute_M}.   




%Let $R_i$, $i=1,2,...,g$, be the actual number of rounds for the reconciliation of group pair $i$ to be completed.  Define $R\triangleq\max(R_1,R_2,...,R_g)$.  

An immediate result from this model, to be shown in \autoref{sec:times2bound}, is a sharp lower bound on $Pr[R \!\le\! r]$, 
the success probability for the set reconciliation to complete within $r$ rounds.  This lower bound will be used in \autoref{sec:parameter_settings} to find the optimal parameter setting that
minimizes the communication overhead while guaranteeing $Pr[R \!\le\! r]\!\ge\! p_0$, the optimization problem mentioned in \autoref{sec:multiround_large_d}.

\end{comment}

% (where $p_0$ is the aforementioned target success probability).

%\input{section/motivation_analysis}

%\subsection{Analysis of a simple case}\label{sec:single_markov}
%\subsection{The Process Under PBS}\label{sec:single_markov}
%\subsection{The Markov-Chain Model}\label{sec:single_markov}

\begin{comment}
In the following modeling, we assume that the group pair 
has $x$ distinct elements before the first round starts.    For the moment, we assume $x \le t$ where $t$ is the error-correction capacity of the BCH code, 
so that we do not have to worry about the BCH decoding failure.   Using the model to be describe next, we can derive the formula for the probability that all $x$ 
distinct elements, and hence the pair, are successfully reconciled in no more than $r$ rounds.   This formula in turn serves as the basic building block for 
answering all the three aforementioned research questions concerning PBS.
\end{comment}

%Its impact on the success probability (of reconciling all distinct elements
%in $r$ rounds) analysis will be discussed in \autoref{sec:times2bound}.  

{\color{red}We now describe this Markov-chain model.}  
How the number, starting at $x$ before the first round, of yet unreconciled distinct elements between the group pair 
decreases one round after another, and 
eventually goes down to $0$, can 
be precisely modeled as a Markov chain as follows.   
As described in \autoref{sec:multi-rounds}, in the first round, each of the $x$ balls (distinct elements) is thrown uniformly and randomly (by the hash function $h$) 
into one of the $n$ bins (subset pairs).  If a ball ends up in a bin that contains no other balls, the corresponding distinct element can be 
%corresponding to a 
successfully reconciled using \autoref{alg:trivial_case}.  We call this ball a ``good'' ball, since it does not have to be thrown again in later rounds, and for the 
modeling purpose call
this bin a ``good'' bin (just for this round).  
If a ball ends up in a bin that has other balls, which corresponds to a type (\RN{1}) or type (\RN{2}) exception discussed earlier in \autoref{subsec:exception_hash_partition},
%{\bf Liang: a type ??? or ??? exception discussed earlier in ???}, 
the corresponding distinct element cannot be reconciled in this round.   We call this ball a ``bad'' ball, since it has to 
be thrown again in the second round (in the hope of making it ``good'' this time), and for the modeling purpose call this bin a ``bad'' bin (just for this round).  

As described in \autoref{sec:multi-rounds}, the ``bad'' balls (if any) that remain after the first round will be thrown again in the second round, the ``bad'' balls (if any) 
that remain in the second round will be thrown again in the third round, and so on.  
Let $B_k$, $k=1,2,\cdots$, be the number of balls 
that remain ``bad'' (yet unreconciled distinct elements) after the $k^{th}$ round.  
Let $B_0 = x$ be the number of balls to be thrown at the beginning (i.e., right before the first round).   Then $\{B_k\}_{k=0}^\infty$ is a Markov chain
for the following reason.   Since a different and mutually independent hash function is used in each round, the random variable $B_{k}$, 
which is the number of balls that remain ``bad'' after the $k^{th}$ round, depends only on $B_{k-1}$, the number of balls thrown in the $k^{th}$ round, and is conditionally (upon $B_{k-1}$) independent of the history $B_0, B_1, B_2, \cdots, B_{k-2}$. 

The states of this Markov chain are $i = 0, 1, 2, \cdots$.  Each state $i$ means that there are $i$ ``bad'' balls to be thrown at the beginning of a round.  
The (desired) termination state of this Markov chain is state $0$ (``bad'' balls remaining).
% {\bf The transition matrix of the Markov chain, denote as $M$, is an infinite matrix. For all practical matrices, however, it can be considered an $(t+1) \times (t+1)$ matrix, under the assumption $i \le t$.   
% In other words, we compute only the $(t+1) \times (t+1)$ elements in the ``upper-left corner" of $M$, and call that $M$ instead.}
%Since we assume $x \le t$, we limit the set of states to $\{0, 1, \cdots, t\}$ in the following description.   With this limitation, the transition matrix of the Markov chain is a $(t+1)\times (t+1)$ matrix, which we denote as $M$.  
For both notational convenience and confusion minimization, we shift each row/column index down by 1.  In other words, we refer to the 
first row/column as the $0^{th}$ row/column, the second as the first, and so on.   This way, the matrix element $M(i, j)$ (at the intersection of the $i^{th}$ 
row and the $j^{th}$ column under the new index numbering convention) corresponds to the probability for 
the Markov chain to move from state $i$ (``bad'' balls thrown) to state $j$ (``bad'' balls remaining).  
%In contrast, under the normal index numbering convention, $M(i, j)$ would be the transition probability from state $i\!-\!1$ to state $j\!-\!1$.  
% {\bf (new content) For any arbitrary $i$ and $j$, this probability only depends on $n$, the number of bins that the $i$ ``bad'' balls are being thrown into. Hence, every matrix element $M(i, j)$ (for $\forall i,j=0,1,\cdots,t$), or in other words, the entire transition matrix $M$, is a function of one variable that is $n$. $t$ is just the upper bound of the ``support'' of $M$. As we will ...}

{\color{red}In the interest of space, we leave out here our discussions on the preciseness of this Markov-chain model and on how the matrix $M$ is computed.
They can be found in~\autoref{sec:preciseness}.}

%Its preciseness will be explained in \autoref{sec:preciseness}. %and how to compute its transitioning probability matrix $M$ in \autoref{sec:compute_M}.






\begin{comment}

For the moment, let us assume each element (probability value) in the matrix $M$ has been computed;  how to compute these probabilities will be described in \autoref{sec:compute_M}.   Lying at the heart of all three applications (including near-optimal parameter tuning) of this Markov-chain modeling is to 
compute the probability of the following event:  There were $x$ ``bad'' balls at the beginning of the first round and there are $0$ ``bad'' balls left at the end
of the $r^{th}$ round ($r \ge 1$).  This event corresponds to all $x$ distinct elements being successfully reconciled within $r$ rounds.   
We denote this event as $\{x\!\xrsquigarrow{r}\! 0\}$.  Given the transition matrix $M$, computing this probability value $Pr[x\!\xrsquigarrow{r}\! 0]$ is
straightforward:  $Pr[x\!\xrsquigarrow{r}\! 0] = \big{(}M^r\big{)}(x, 0)$.  Here $\big{(}M^r\big{)}(x, 0)$ is the element at the intersection of the $x^{th}$ row and the 
$0^{th}$ column in the matrix $M^r$ ($M$ to the power $r$).  Note that, without this Markov-chain modeling, this probability is hard to compute except in some
special cases such as $Pr[x\!\xrsquigarrow{1}\! 0]$ (the probability, derived earlier in \autoref{sec:hash_partition}, for the ideal case of $x$ balls thrown ending up in $x$ distinct bins to happen).
%\autoref{sec:single_markov}. 

[used]
Recall from PBS-for-small-$d$, each of the $d$ balls (distinct elements) are thrown uniformly and randomly into one of the $n$ bins (subset pairs) in the first round. Each ball that ends up in a bin that receives exactly $1$ ball, corresponding to a successfully reconciled distinct element, is a ``good'' ball and will not be thrown again in later rounds. Each ball that ends up in a bin that receives multiple balls, corresponding to a distinct element that has not been reconciled yet, is a ``bad'' ball and will be thrown again in the second round to try to turn into a ``good'' one. The process of throwing ``bad'' balls round after round continues until all balls end up to be ``good''. 

[used]
In this section, we study a generic case that starting with $x$ $(\leq t)$ balls, how the number of ``bad'' balls that remain evolves round after round. This generic case arises from the set reconciliation process of each group pair in PBS. Let $B_k$ denote the number of ``bad'' balls that remain after the $k$-th round for $k=1,2,\cdots$. In the process, $B_k$ also denotes the number of balls to be thrown in the $(k+1)$-th round. Define $B_0\triangleq x$. Note that the balls are thrown using different hash functions in each round, so $B_{k}$, the number of ``bad'' balls that remain after the $k$-th round, only depends on $B_{k-1}$, the number of balls are thrown in the $k$-th round, and is independent of the history (i.e., $B_0,B_1,B_2,\cdots,B_{k-2}$). Therefore, $\{B_k\}_{k=0}^\infty$ is a Markov chain, in which each state is defined as the number of ``bad'' balls that remain. 
%, in which the distribution of $B_{k+1}$ conditioned upon $B_k$ is independent of $B_1,B_2,\cdots,B_{k-1}$. 
The ``desirable'' state of this Markov chain for PBS is state $0$ (the absorbing state), in which all balls end up to be ``good''. 



% In this section, we study a generic case that starting with $x$ $(\leq t)$ balls, how the number of balls to be thrown evolves in this process. This generic case arises from the set reconciliation process of each group pair in PBS. Let $B_k$ denote the number of balls to be thrown in the $k$-th round for $k=1,2,\cdots$, where $B_1=x$. Note that the balls are thrown using different hash functions in each round, so $B_{k+1}$, the number of ``bad'' balls that remain after the $k$-th round, only depends on $B_{k}$, the number of balls are thrown in the $k$-th round, and is independent of the history (i.e., $B_1,B_2,\cdots,B_{k-1}$). Therefore, $B_1, B_2,\cdots$ is a Markov chain, in which each state is defined as the number of balls to be thrown.
% %, in which the distribution of $B_{k+1}$ conditioned upon $B_k$ is independent of $B_1,B_2,\cdots,B_{k-1}$. 
% The ``desirable'' state of this Markov chain for PBS is state $0$ (the absorbing state), in which all balls end up to be ``good''. 

{\bf (modified)} For our analysis, the only probability that we are concerned with is $Pr[x\!\xrsquigarrow{r}\! 0]$, the probability of the event $\{x\!\xrsquigarrow{r}\! 0\}$ that the process starts with $x$ ``bad'' balls and ends up with $0$ ``bad'' ball after $r$ rounds. Note that the event $\{x\!\xrsquigarrow{1}\! 0\}$ corresponds to the ideal case in PBS-for-small-$d$. The probability of this event $Pr[x\!\xrsquigarrow{1}\! 0]$ can be easily computed as a closed-form expression. However, $Pr[x\!\xrsquigarrow{r}\! 0]$ is hard to compute when $r\geq 2$. The Markov chain modeling solves this problem by mapping the probability of the event $\{x\!\xrsquigarrow{r}\! 0\}$ to the $r$-step transition probability $\big{(}M^r\big{)}(x,0)$ of the Markov chain. 
%It is also the success probability within $r$ rounds. 
It is easy to verify that $Pr[x\!\xrsquigarrow{r}\! 0]$ is equal to $\big{(}M^r\big{)}(x,0)$, the entry in the $x$-th row and the $0$-th column of the matrix that is $M^r$. 

% Note that even without using this Markov chain modeling, $Pr[x\!\xrsquigarrow{1}\! 0]$ can be easily computed as a closed-form expression. However, $Pr[x\!\xrsquigarrow{r}\! 0]$ cannot be expressed as a closed-form expression when $r\geq 2$. 
% %In general, $Pr[d\!\xrsquigarrow{r}\! y]$ is difficult to compute when $r\geq 2$ and $y\geq 1$. 
% The Markov chain modeling solves this problem by mapping the transition probability $Pr[x\!\xrsquigarrow{r}\! 0]$ after $r$ rounds in the process to the $r$-step transition probability $\big{(}M^r\big{)}(x,0)$ of the Markov chain.

{\bf (previous)} For our analysis, the only probability that we are concerned with is $Pr[x\!\xrsquigarrow{r}\! 0]$, the probability of the event $\{x\!\xrsquigarrow{r}\! 0\}$ that the process starts with $x$ ``bad'' balls and ends up with $0$ ``bad'' ball after $r$ rounds. 
%It is also the success probability within $r$ rounds. 
$Pr[x\!\xrsquigarrow{r}\! 0]$ can be easily calculated as 
%, where $M(i,j)$ (i.e., the entry in the $i^{th}$ row and the $j^{th}$ column of $M$) is the probability of transition from state $i$ to state $j$ for $i,j = 0,1,\cdots,t$
$\big{(}M^r\big{)}(x,0)$, the entry in the $x$-th row and the $0$-th column of the matrix, that is $M^r$. Note that even without using this Markov chain modeling, $Pr[x\!\xrsquigarrow{1}\! 0]$ can be easily computed as a closed-form expression (more precisely, a multinomial formula), as we described in \autoref{sec:hash_partition}. However, $Pr[x\!\xrsquigarrow{r}\! 0]$ cannot be expressed as a closed-form as in when in \autoref{sec:hash_partition} $r\geq 2$. 
%In general, $Pr[d\!\xrsquigarrow{r}\! y]$ is difficult to compute when $r\geq 2$ and $y\geq 1$. 
The Markov chain modeling solves this problem by mapping the transition probability $Pr[x\!\xrsquigarrow{r}\! y]$ after $r$ rounds in the process to the $r$-step transition probability $\big{(}M^r\big{)}(x,y)$ of the Markov chain.

{\bf (the content of this paragraph is contained in the last paragraph, could be unnecessary)} Recall that in PBS-for-small-$d$, given two sets with $d$ distinct elements, PBS-for-small-$d$ successfully reconciles all distinct elements within $1$ round if and only if the ideal case happens. The probability for the ideal situation to occur is $Pr[d\!\xrsquigarrow{1}\! 0]$. It can be easily computed even without using this Markov chain modeling. In general, $Pr[d\!\xrsquigarrow{r}\! y]$ is difficult to compute when $r\geq 2$ and $y\geq 1$. 

% {\bf (previous)} Recall that in PBS-for-small-$d$, given two sets with $d$ distinct elements, PBS-for-small-$d$ successfully reconciles all distinct elements within $1$ round if and only if the ideal case happens. The probability for the ideal situation to occur is $Pr[d\!\xrsquigarrow{1}\! 0]$ (e.g., $0.96$ when $d = 5$ and $n=255$ as mentioned in \autoref{sec:smalld}). It can be easily computed even without using this Markov chain modeling. In general, $Pr[d\!\xrsquigarrow{r}\! y]$ is difficult to compute when $r\geq 2$ and $y\geq 1$. 

% For our analysis, the only probability that we are concerned with is $Pr[x\!\xrsquigarrow{r}\! 0]$, the probability that starting with ``bad'' balls, the process ends up with $0$ ``bad'' ball after $r$ rounds. 
% %It is also the success probability within $r$ rounds. 
% $Pr[x\!\xrsquigarrow{r}\! 0]$ can be easily calculated given $M$, the $(t+1)\times (t+1)$ transition matrix of the Markov chain, as 
% %, where $M(i,j)$ (i.e., the entry in the $i^{th}$ row and the $j^{th}$ column of $M$) is the probability of transition from state $i$ to state $j$ for $i,j = 0,1,\cdots,t$
% $\big{(}M^r\big{)}(x,0)$, the entry in the $x$-th row and the $0$-th column of the matrix, that is $M^r$.. Here we slightly abuse the row / column indices of a $(t+1)\times (t+1)$ matrix from $1,2,\cdots,t+1$ to $0,1,\cdots,t$, since the state of the Markov chain ranges from $0$ to $t$. The calculation to obtain $M$ is not trivial and will be elaborated in \autoref{sec:compute_M}. For the moment, we assume $M$ has been computed and therefore we can compute $Pr[x\!\xrsquigarrow{r}\! 0]$ for $x=1,2,\cdots,t$, $r\in\mathbb{N}^+$. 





 in which each state is defined as the number of ``bad'' balls that remain. 
%, in which the distribution of $B_{k+1}$ conditioned upon $B_k$ is independent of $B_1,B_2,\cdots,B_{k-1}$. 





In the Markov chain, a transition from state $i$ to state $j$ ($i\geq j$) means $j$ out of $i$ balls are ``bad'' balls and the other $i-j$ balls are ``good'' balls. The {\it absorbing state} of this Markov chain is state $0$, which is the ``desirable'' state that all balls are ``good'' (so that all distinct elements are successfully reconciled). 

For our analysis, the only probability that we are concerned with is $Pr[x\!\xrsquigarrow{r}\! 0]$, the probability that starting with state $x$ (initial state), the Markov chain reaches state $0$ within $r$ transitions. It is also the success probability for a single group (starting with $x$ distinct elements and successfully reconciled within $r$ rounds). $Pr[x\!\xrsquigarrow{r}\! 0]$ can easily calculated given $M$, the $(t+1)\times (t+1)$ transition matrix of the Markov chain, as 
%, where $M(i,j)$ (i.e., the entry in the $i^{th}$ row and the $j^{th}$ column of $M$) is the probability of transition from state $i$ to state $j$ for $i,j = 0,1,\cdots,t$
$\big{(}M^r\big{)}(x,0)$, the entry in the $x$-th row and the $0$-th column of $M^r$. Here we slightly abuse the row / column indices of a $(t+1)\times (t+1)$ matrix from $1,2,\cdots,t+1$ to $0,1,\cdots,t$, since the state of the Markov chain ranges from $0$ to $t$. How to compute $M$ will be elaborated in \autoref{sec:compute_M}. For the moment, we assume $M$ has been computed and therefore we can compute $Pr[x\!\xrsquigarrow{r}\! 0]$ for $x=1,2,\cdots,t$, $r\in\mathbb{N}^+$. 

For simplicity, we ignore the small probability event that a type (\RN{2}) event happens, in which the incurred ``fake'' distinct element is not successfully verified by \autoref{alg:verification} (mentioned in \autoref{subsec:exception_hash_partition}). As we discussed earlier, this event happens with a tiny probabilty that is in order of $10^{-7}$. Hence, ignoring this event barely compromises the accuracy of our analysis. 





This process will continue for a target number of rounds (i.e., $r$ round), or until the group pair is completely reconciled, which is verified by the checksum (\autoref{alg:single_round_pbs} of \autoref{step:terminate_condition}). In all rounds, how the balls are thrown into $n$ bins follows the same balls-into-bins probability model. Note that the balls are thrown using different hash functions in each round, so the number of ``bad'' balls in a round
%(i.e., the number of balls to be thrown in the $(i+1)$-th round) 
only depends on how many balls are thrown in the round and is independent of the history
 of how these balls were placed into the $n$ bins in the previous rounds. 
Therefore, the process of how the number of balls to be thrown evolves round after round 
%the number of balls to be thrown round after round 
is a Markov chain, in which each state is defined as the number of balls to be thrown. 
%Hence, the dynamics of the number of balls to be thrown in each round can be modeled as a Markov chain, in which each state is defined as the number of balls to be thrown. {\bf a little bit wordy, need advice on how to shrink it.}



%(by a different and independent hash function) 

%The process of throwing ``bad'' balls round after round continues until all balls end up to be ``good''. 


How the number of balls (yet unreconciled distinct elements) decreases one round after another can 
be precisely modeled as a Markov chain


balls, how the number of ``bad'' balls that remain evolves round after round. This generic case arises from the set reconciliation process of each group pair in PBS. Let $B_k$ denote the number of ``bad'' balls that remain after the $k$-th round for $k=1,2,\cdots$. In the process, $B_k$ also denotes the number of balls to be thrown in the $(k+1)$-th round. Define $B_0\triangleq x$. Note that the balls are thrown using different hash functions in each round, so $B_{k}$, the number of ``bad'' balls that remain after the $k$-th round, only depends on $B_{k-1}$, the number of balls are thrown in the $k$-th round, and is independent of the history (i.e., $B_0,B_1,B_2,\cdots,B_{k-2}$). Therefore, $\{B_k\}_{k=0}^\infty$ is a Markov chain, in which each state is defined as the number of ``bad'' balls that remain. 
%, in which the distribution of $B_{k+1}$ conditioned upon $B_k$ is independent of $B_1,B_2,\cdots,B_{k-1}$. 
The ``desirable'' state of this Markov chain for PBS is state $0$ (the absorbing state), in which all balls end up to be ``good''. 


and a distinct element is successfully reconciled if and only if it is hashed into a subset pair that contains no other distinct element. 


Each ball that ends up in a bin that receives exactly $1$ ball, corresponding to a successfully reconciled distinct element, is a ``good'' ball and will not be thrown again in later rounds. Each ball that ends up in a bin that receives multiple balls, corresponding to a distinct element that has not been reconciled yet, is a ``bad'' ball and will be thrown again in the second round to try to turn into a ``good'' one. The process of throwing ``bad'' balls round after round continues until all balls end up to be ``good''. 




===============================

In this section, we analyze the probability that an arbitrary group pair that contains exactly $x$ $(\leq t)$ distinct elements is {\it successfully reconciled} by PBS in $r$ rounds. Here we say a group pair is {\it successfully reconciled} within $r$ rounds if and only if all distinct elements in the group pair are successfully reconciled within $r$ rounds. 

As we described in \autoref{sec:multi-rounds}, in the first round of PBS, the $x$ distinct elements are hashed into $n$ subset pairs, and a distinct element is successfully reconciled if and only if it is hashed into a subset pair that contains only $1$ distinct element. 
%The successfully reconciled distinct elements in the first round are removed and the other distinct elements (i.e., the ones that have not been reconciled yet in the first round) will be hashed again in the second round using a different hash function, so on so force, until all distinct elements are successfully reconciled. 
How the $x$ distinct elements are distributed into $n$ subset pairs in the first round follows the familiar {\it balls-into-bins} probability model: Each of the $x$ balls is thrown independently and uniformly at random into one of the $n$ bins. Each successfully reconciled distinct element corresponds to a ball that ends up in a bin that receives exactly $1$ ball. We call both the ball and the bin ``good'' in the sequel; each distinct element that has not been reconciled yet in the first round corresponds to a ball that ends up in a bin that receives multiple balls. We call both the ball and the bin ``bad'' in the sequel. Note that balls and empty bins are either ``good'' or ``bad''.
%but a bin could be empty besides being ``good'' and ``bad''. 

The ``bad'' balls in the first round will be the balls to be thrown in the second round. The ``bad'' balls in the second round will be the balls to be thrown in the third round, and so on. This process will continue for a target number of rounds (i.e., $r$ round), or until the group pair is completely reconciled, which is verified by the checksum (\autoref{alg:single_round_pbs} of \autoref{step:terminate_condition}). In all rounds, how the balls are thrown into $n$ bins follows the same balls-into-bins probability model. Note that the balls are thrown using different hash functions in each round, so the number of ``bad'' balls in a round
%(i.e., the number of balls to be thrown in the $(i+1)$-th round) 
only depends on how many balls are thrown in the round and is independent of the history
 of how these balls were placed into the $n$ bins in the previous rounds. 
Therefore, the process of how the number of balls to be thrown evolves round after round 
%the number of balls to be thrown round after round 
is a Markov chain, in which each state is defined as the number of balls to be thrown. 
%Hence, the dynamics of the number of balls to be thrown in each round can be modeled as a Markov chain, in which each state is defined as the number of balls to be thrown. {\bf a little bit wordy, need advice on how to shrink it.}

In the Markov chain, a transition from state $i$ to state $j$ ($i\geq j$) means $j$ out of $i$ balls are ``bad'' balls and the other $i-j$ balls are ``good'' balls. The {\it absorbing state} of this Markov chain is state $0$, which is the ``desirable'' state that all balls are ``good'' (so that all distinct elements are successfully reconciled). 

For our analysis, the only probability that we are concerned with is $Pr[x\!\xrsquigarrow{r}\! 0]$, the probability that starting with state $x$ (initial state), the Markov chain reaches state $0$ within $r$ transitions. It is also the success probability for a single group (starting with $x$ distinct elements and successfully reconciled within $r$ rounds). $Pr[x\!\xrsquigarrow{r}\! 0]$ can easily calculated given $M$, the $(t+1)\times (t+1)$ transition matrix of the Markov chain, as 
%, where $M(i,j)$ (i.e., the entry in the $i^{th}$ row and the $j^{th}$ column of $M$) is the probability of transition from state $i$ to state $j$ for $i,j = 0,1,\cdots,t$
$\big{(}M^r\big{)}(x,0)$, the entry in the $x$-th row and the $0$-th column of $M^r$. Here we slightly abuse the row / column indices of a $(t+1)\times (t+1)$ matrix from $1,2,\cdots,t+1$ to $0,1,\cdots,t$, since the state of the Markov chain ranges from $0$ to $t$. How to compute $M$ will be elaborated in \autoref{sec:compute_M}. For the moment, we assume $M$ has been computed and therefore we can compute $Pr[x\!\xrsquigarrow{r}\! 0]$ for $x=1,2,\cdots,t$, $r\in\mathbb{N}^+$. 

For simplicity, we ignore the small probability event that a type (\RN{2}) event happens, in which the incurred ``fake'' distinct element is not successfully verified by \autoref{alg:verification} (mentioned in \autoref{subsec:exception_hash_partition}). As we discussed earlier, this event happens with a tiny probabilty that is in order of $10^{-7}$. Hence, ignoring this event barely compromises the accuracy of our analysis. 

===============================

\end{comment}

\begin{comment}
%% moved to appendix
\subsection{Preciseness of Markov-Chain Modeling}\label{sec:preciseness}

The Markov-chain model above precisely captures every detail of the set reconciliation process in each group pair except for one event: 
when a fake distinct element resulting from a type (\RN{2}) exception ``luckily'' (unluckily for Alice) 
passes the sub-universe verification check (\autoref{alg:verification}).  We choose to leave this event out in the modeling, because 
to incorporate it would result in a much more complicated Markov chain.   To incorporate this event is also not necessary for 
our modeling to be numerically accurate, because this event happens with a tiny probability of $O(10^{-7})$.  

%is not successfully verified by \autoref{alg:verification}. Such an element, if captured in the generic case, would increase the number of balls to be thrown in the next %round by $1$ and therefore change the transition-into state (say the transition changes from state $i\rightarrow j$ to state $i\rightarrow j+1$). 

%However, as we explained in \autoref{subsec:exception_hash_partition}, this event happens with a tiny probabilty that is in order of $10^{-7}$. Ignoring such a small %probability event barely changes the transition probability matrix $M$ of the Markov chain and therefore has negligible effect of our analysis. 

%In the Markov chain modeling above in general and the derivation of the success probability for a group pair (within $r$ rounds) in particular, 
In this model,
we assume $x\! \le\! t$, where $t$ is the error-correction capacity of the BCH code.
%only analyze the case in which the number of balls to start with is no more than the error-correction capability of the BCH code (i.e., $x\leq t$). 
To extend the Markov-chain modeling to the case of 
$x\! >\! t$ (resulting in a BCH decoding failure w.h.p.) is a daunting task, since this group pair is to 
be partitioned into $3$ sub-group-pairs as described in \autoref{sec:BCH_exception} and each sub-group-pair is to be independently reconciled. 
We also found this task unnecessary:  Assuming $Pr[x\!\xrsquigarrow{r}\! 0]\! =\! 0$ when $x\!>\!t$ in our modeling (always to our disadvantage) 
results in only a slight underestimation of ``good'' probabilities, as will be elaborated in \autoref{sec:times2bound}.
\end{comment}

%Instead of analyzing this complicated set reconciliation process, we simply `underestimate' $Pr[x\!\xrsquigarrow{r}\! 0]$ to be $0$ for $x>t$ in the following tail bound analysis. This `underestimation' incurs negligible loss on the tail bound, as we will explain shortly.


%the analysis of the set reconciliation process becomes much more complicated, since such a group pair could be partitioned into $3$ sub-group-pairs (e.g., in the ideal case) as we described in \autoref{alg:3_way_partition} and each of them will be independently reconciled. Instead of analyzing this complicated set reconciliation process, we simply `underestimate' $Pr[x\!\xrsquigarrow{r}\! 0]$ to be $0$ for $x>t$ in the following tail bound analysis. This `underestimation' incurs negligible loss on the tail bound, as we will explain shortly.

% The second event is, when the number of distinct elements in a group pair exceeds the error-correction capability $t$ then lead to a BCH decoding failure, the group pair will be partitioned into $3$ sub-group-pairs, each of which will be reconciled by PBS-for-small-$d$ in the next round, as we showed in \autoref{alg:3_way_partition}. To ease our analysis, we assume $Pr[x\!\xrsquigarrow{r}\! 0]=0$ when $x>t$. 
% % (i.e., assume group pair $1$ cannot be reconciled if $\delta_1>t$, discussed in \autoref{sec:BCH_exception}). 
% The loss of this underestimation is very tiny for the following reason: $Pr[\delta_1\!=\!x]$, the ``coefficient'' of $Pr[x\!\xrsquigarrow{r}\! 0]$, is very small when $x>t$, since $\delta_1$ is a Binomial random variable with mean of $\delta$ while $x$ is larger than $t$, which is roughly $2$ to $3$ times of $\delta$. We denote this underestimated probability as $\alpha$ (i.e., $\alpha=\sum_{x=0}^t Pr[\delta_1\!=\!x]\cdot Pr[x\!\xrsquigarrow{r}\! 0]$), which is a tight tail bound of the success probability of group pair $1$. $\alpha$ is also a tight tail bound for all other group pairs, since $\delta_1,\delta_2,\cdots,\delta_g$ follows the same distribution. 

% A ball that ends up in a bin that receives exactly $1$ ball is a ``good'' ball. In the ideal case, the $d$ balls are placed into $d$ distinct bins and the corresponding $d$ distinct elements are reconciled. In general, the ideal case may not necessarily happen. Some of the distinct elements (say $d'$ out of $d$ distinct elements) may have not been reconciled yet and will be thrown in the second round, and so on. The process of how the number of balls to be thrown evolves ($d\rightarrow d'\rightarrow \cdots$) round after round can be characterized as a Markov chain model. 






\begin{comment}

within $r$ rounds, since the set reconciliation process on group pairs are independent of each other. However, this tail bound is not rigorous, since the $g$ success probabilities of the $g$ group pairs are functions of $\delta_1, \delta_2,\cdots,\delta_g$, which are related by $\sum_{i=1}^g \delta_i=d$. Using Corollary 5.11 in \cite{upfal2005probability}, we can derive a rigorous tail bound of $1-2(1-\alpha^g)$ for the success probability of all group pairs within $r$ rounds. This rigorous tail bound is very tight and only doubles the tiny failure probability of the unrigorous tail bound (i.e., $1-\alpha^g$): For example, if the unrigorous tail bound of the success probability of all group pairs is $0.9999$ ($0.0001$ failure probability), then the rigorous tail bound will be $0.9998$ ($0.0002$ failure probability). This rigorous tail bound of $1-2(1-\alpha^g)$ will be used in parameter settings. 



Since we already know how to compute $Pr[x\!\xrsquigarrow{r}\! 0]$ for an arbitrary $x > 0$, it takes just a ``plug-in" to compute 


Since we already know how to compute 


 



{\bf (merged by the following two paragraphs)} Recall that $\delta_1,\delta_2,\cdots,\delta_g$ follows the same Binomial distribution $Binomial(d,1/g)$. The success probability $Pr[\delta_i\!\xrsquigarrow{r}\! 0]$, when fixing other parameters, only depends on the value of $x$. WLOG, we only analyze group pair $1$ among all group pairs. The success probability of group pair $1$ within $r$ rounds is $\sum_{x=0}^d Pr[\delta_1\!=\!x]\cdot Pr[x\!\xrsquigarrow{r}\! 0]$, where $Pr[x\!\xrsquigarrow{r}\! 0]=\big{(}M^r\big{)}(x,0)$ for $x=1,2,\cdots,t$. 


Recall that $\delta_1,\delta_2,\cdots,\delta_g$ follows the same distribution. The success probability $Pr[\delta_i\!\xrsquigarrow{r}\! 0]$, when fixing other parameters, only depends on the value of $x$. WLOG, we only analyze group pair $1$ among all group pairs. The success probability of group pair $1$ within $r$ rounds is $\sum_{x=0}^d Pr[\delta_1\!=\!x]\cdot Pr[x\!\xrsquigarrow{r}\! 0]$, where $Pr[x\!\xrsquigarrow{r}\! 0]=\big{(}M^r\big{)}(x,0)$ for $x=1,2,\cdots,t$. Here $\delta_1$, the number of distinct elements in group pair $1$, is a random variable that follows a Binomial distribution $Binomial(d,1/g)$. 

Recall that we underestimate $Pr[x\!\xrsquigarrow{r}\! 0]=0$ when $x>t$. The loss of this underestimation on the success probability of group pair $1$ is very tiny, since $Pr[\delta_1\!=\!x]$, the ``coefficient'' of $Pr[x\!\xrsquigarrow{r}\! 0]$, is very small when $x>t$: $\delta_1$ is a Binomial random variable with mean $\delta$ while $x$ is larger than $t$, which is roughly $2$ to $3$ times of $\delta$. We denote this underestimated probability as $\alpha$ (i.e., $\alpha=\sum_{x=0}^t Pr[\delta_1\!=\!x]\cdot Pr[x\!\xrsquigarrow{r}\! 0]$), which is a tight tail bound of the success probability for group pair $1$ and for all other group pairs. 
%$\alpha$ is also a tight tail bound for all other group pairs, since $\delta_1,\delta_2,\cdots,\delta_g$ follows the same distribution. 



===============================
To ease computation, we slightly underestimate this probability by assuming $Pr[x\!\xrsquigarrow{r}\! 0]=0$ when $x>t$. 
% (i.e., assume group pair $1$ cannot be reconciled if $\delta_1>t$, discussed in \autoref{sec:BCH_exception}). 
The loss of this underestimation is very tiny for the following reason: $Pr[\delta_1\!=\!x]$, the ``coefficient'' of $Pr[x\!\xrsquigarrow{r}\! 0]$, is very small when $x>t$, since $\delta_1$ is a Binomial random variable with mean $\delta$ while $x$ is larger than $t$, which is roughly $2$ to $3$ times of $\delta$. We denote this underestimated probability as $\alpha$ (i.e., $\alpha=\sum_{x=0}^t Pr[\delta_1\!=\!x]\cdot Pr[x\!\xrsquigarrow{r}\! 0]$), which is a tight tail bound of the success probability of group pair $1$. $\alpha$ is also a tight tail bound for all other group pairs, since $\delta_1,\delta_2,\cdots,\delta_g$ follows the same distribution. 
%group pair $i$, defined as the probability that all the distinct elements in the group pair are reconciled, within $r$ rounds, is equal to $Pr[\delta_i\!\xrsquigarrow{r}\! 0]$. 

As we explained in \autoref{subsec:protocol2}, $\delta_1$, the number of distinct elements in group pair $1$, is a random variable that follows a Binomial distribution $Binomial(d,1/g)$. So the probability that group pair $1$ is successfully reconciled in $r$ rounds is $\sum_{x=0}^d Pr[\delta_1\!=\!x]\cdot Pr[x\!\xrsquigarrow{r}\! 0]$, where $Pr[x\!\xrsquigarrow{r}\! 0]=\big{(}M^r\big{)}(x,0)$. 
%, where $\mathcal{B}(\cdot;d,1/g)$ is the probability mass function (PMF) of $Binomial(d,1/g)$. 
To ease computation, we slightly underestimate this probability by assuming $Pr[x\!\xrsquigarrow{r}\! 0]=0$ when $x>t$. 
% (i.e., assume group pair $1$ cannot be reconciled if $\delta_1>t$, discussed in \autoref{sec:BCH_exception}). 
The loss of this underestimation is very tiny for the following reason: $Pr[\delta_1\!=\!x]$, the ``coefficient'' of $Pr[x\!\xrsquigarrow{r}\! 0]$, is very small when $x>t$, since $\delta_1$ is a Binomial random variable with mean $\delta$ while $x$ is larger than $t$, which is roughly $2$ to $3$ times of $\delta$. We denote this underestimated probability as $\alpha$ (i.e., $\alpha=\sum_{x=0}^t Pr[\delta_1\!=\!x]\cdot Pr[x\!\xrsquigarrow{r}\! 0]$), which is a tight tail bound of the success probability of group pair $1$. $\alpha$ is also a tight tail bound for all other group pairs, since $\delta_1,\delta_2,\cdots,\delta_g$ follows the same distribution. 

%$Pr[x\!\xrsquigarrow{r}\! 0]$ is a function of $n$ for given $x$ and $r$, so $\alpha=\alpha(n,t)$ is a function of $n$ and $t$ for arbitrary $d$, $r$, and $g$. 

% \subsection{Tail Bound Analysis for All Group Pairs}\label{sec:times2bound}

Given $\alpha$, the tail bound of the probability that a group pair is successfully reconciled in $r$ rounds, we can easily derive a tail bound of $\alpha^g=1-(1-\alpha^g)$ for the probability that all group pairs are completely reconciled in $r$ rounds ($1-\alpha^g$ is the failure probability, which is usually tiny), since the set reconciliation process on group pairs are independent with each other. However, this tail bound is not rigorous,
%since $d_1, d_2,\cdots,d_g$ have a weak correlation that $\sum_{i=1}^g d_i=d$.
since $\delta_1, \delta_2,\cdots,\delta_g$ are not strictly independent and have a relation that $\sum_{i=1}^g \delta_i=d$. 
%Fortunately, we have Times-2-Bound (Theorem 1 in \cite{hua2008rank}) to decouple the weak correlation and give us a rigorous tail bound of $1-2(1-\alpha^g)$ for the probability of all group pairs. 
However, we can use Corollary 5.11 in \cite{upfal2005probability} to
% decouple the weak correlation and 
obtain a rigorous tail bound of $1-2(1-\alpha^g)$ for the success probability of all group pairs. This rigorous tail bound is very tight and only doubles the tiny failure probability of the unrigorous tail bound: For example, if the unrigorous tail bound of the success probability of all group pairs is $0.9999$ ($0.0001$ failure probability), then the rigorous tail bound will be $0.9998$ ($0.0002$ failure probability). This rigorous tail bound of $1-2(1-\alpha^g)$ will be used in parameter settings. 
===============================

\end{comment}

\begin{comment}
\subsection{How To Compute \texorpdfstring{\larger\boldmath{$M$}}{M}}\label{sec:compute_M}

{\color{red} This subsection is moved to appendix.}
%{\bf An optional story line: (1) Define $\tilde{M}(i,j,k)$; (2) To compute $M(i,j)$, it is sufficient to compute $\tilde{M}(i,j,k)$, since we have \cdots  (3) On the other hand, we discover a recurrence relation among $\tilde{M}(i,j,k)$, so it can be computed by dynamic programming; (From here, it is the same with the currect story line) (4) Describe slow-motion rendering and recurrence relation; (5) Base cases}



Although the transition probability matrix $M$ is in theory an infinite matrix, in this work for all practical purposes (e.g., for 
computing $Pr[x\!\xrsquigarrow{r}\! 0]$), it can be considered a $(t+1) \times (t+1)$ matrix, where $t$ is the BCH error-correction capacity.  In this section,
we describe how to compute this $(t+1) \times (t+1)$ matrix.  
To compute $M(i,j)$ is in general hard because, when $i$ and $j$ are large, there are many different ways for $j$ out of $i$ balls thrown to end up being ``bad", and each way can have 
a different probability.  
Our solution is to decompose each state $j$ into a small number of sub-states.  
Although 
there can still be many different ways for a state $i$ to transition into a sub-state of $j$, making the total transition probability hard to compute,
we discover a recurrence relation among these transition probabilities that makes them easily 
computable using dynamic programming.
% We overcome this problem by grouping the huge number of atom states into a smaller number of coarse-grained sub-states first, then computing the transition probability from the (pre-transition) state $i$ to any sub-states of state $j$. Although each sub-state still consists of many atom states and the transition probability to a sub-state is still hard to compute directly, we discover a recurrence relation among these transition probabilities, so we can compute them using Dynamic Programming.

% In this section, we describe how to compute the transition matrix $M$ in detail. For general $i,j$, $M(i,j)$ cannot be computed straightforwardly. Our solution is to decompose each state $j$ into a small number of sub-states, so that the transition probability $M(i,j)$ can be computed as the summation of the transition probabilities from state $i$ to each of the sub-states of state $j$. Although these transition probabilities also cannot be computed straightforwardly, we discover a recurrence relation among these transition probabilities that makes them easily computable using dynamic programming.

We now define these sub-states and describe the recurrence relation among the resulting transition probabilities.
Each state $j$ (``bad" balls) is decomposed into $j\!+\!1$ sub-states that we denote as $(j,0)$, $(j,1)$, $(j, 2)$, $\cdots$, $(j,j)$ respectively.
Each sub-state $(j, k)$, $k = 0, 1, 2, \cdots, j$, corresponds to the set of scenarios in which the $j$ ``bad'' balls end up occupying exactly $k$ ``bad'' bins
(those containing more than one ``bad'' balls as defined earlier in \autoref{sec:single_markov}).  Let $(i, j, k)$ denotes the event that throwing $i$ balls results in
the sub-state $(j, k)$.  Let $\tilde{M}(i,j,k)$ denote the probability of this event $(i, j, k)$.  
%The $i$ balls thrown are ttransition probability from state $i$ to 
%sub-state $(j,k)$.  
Clearly, we have $M(i,j) = \sum_{k=0}^{j} \tilde{M}(i,j,k)$ for $\forall i,j$.
% \begin{equation}\nonumber
%     M(i,j) = \sum_{k=0}^{j} \tilde{M}(i,j,k)
% \end{equation}

%corresponds to the sub-state of state $j$ in which




%{\bf explain the range of $k$ could be distracting, so I just leave it as it is.}

To obtain $M$, it suffices to compute the probabilities of $\tilde{M}(i,j,k)$ for $\forall i,j,k=0,1,\cdots,t$. 
To do so, we derive a recurrence relation for these probability values by rendering the process of throwing $i$ balls ``in slow motion'' in the following sense: We throw them one at a time.  Now consider what events happen before and after the $i^{th}$ ball is thrown.   Suppose the event $(i, j, k)$ happens after the $i^{th}$ ball is thrown.  There are only three possible events before the $i^{th}$ ball is thrown that can lead to the
event $(i, j, k)$.  Here we explain only the first event $(i\!-\!1,j\!-\!2,k\!-\!1)$ in detail, as explanations for the other two are similar.  
The event $(i\!-\!1,j\!-\!2,k\!-\!1)$ leads to the event $(i, j, k)$ if and only if the $i^{th}$ ball lands in a previously ``good'' bin 
so that the ``good'' ball 
already in the bin and the $i^{th}$ ball turn into two ``bad'' balls.  The latter happens with probability 
$(i\!-\!j\!+\!1)/n$, since $(i\!-\!1)\!-\!(j\!-\!2)$ out of $n$ bins are ``good'' at 
sub-state $(j\!-\!2,k\!-\!1)$.  
The other two events are $(i\!-\!1,j\!-\!1,k)$ and $(i\!-\!1,j,k)$, and they lead to the event $(i, j, k)$ with probability $k/n$ and $1\!-\!(i\!-\!1\!-\!j\!+\!k)/n$ respectively.
%{\bf (original) The second event is $(i\!-\!1,j\!-\!1,k)$.  It leads to the event $(i, j, k)$ when the $i^{th}$ ball lands in a ``bad'' bin, which happens with probability $k/n$.  The third event is $(i\!-\!1,j,k)$.  It leads to the event $(i, j, k)$ when the $i^{th}$ ball lands in an empty bin, which happens with probability $1\!-\!(i\!-\!1\!-\!j\!+\!k)/n$.} 
Summarizing these three cases, we can express $\tilde{M}(i,j,k)$, the probability of the event $(i, j, k)$, as the weighted sum of the probabilities of these three events
%that can possibly lead to theevent $(i,j,k)$ 
as follows:

% To obtain $M$, it suffices to compute the probabilities of $\tilde{M}(i,j,k)$ for $\forall i,j,k=0,1,\cdots,t$. 
% To do so, we derive a recurrence relation for these probability values by rendering the process of throwing $i + 1$ balls 
% ``in slow motion'' in the following sense:
% We throw them one at a time.  Now consider what events happen before and after the $(i\!+\!1)^{th}$ ball is thrown.   Suppose the event 
% $(i\!+\!1, j, k)$ happens after the $(i\!+\!1)^{th}$ ball is thrown.  There are only three possible events before the $(i\!+\!1)^{th}$ ball is thrown that can lead to the
% event $(i\!+\!1, j, k)$.  The first event is $(i,j\!-\!2,k\!-\!1)$.  It leads to the event $(i\!+\!1, j, k)$ when the $(i\!+\!1)^{th}$ ball lands in a previously ``good'' bin so that the ``good'' ball 
% already in the bin and the $(i\!+\!1)^{th}$ ball turn into two ``bad'' balls.  The probability of this ``lead-to'' transition is $(i\!-\!j\!+\!2)/n$, since $i\!-\!(j\!-\!2)$ out of $n$ bins are ``good'' at 
% sub-state $(j\!-\!2,k\!-\!1)$.  The second event is $(i,j\!-\!1,k)$.  It leads to the event $(i\!+\!1, j, k)$ when the $(i\!+\!1)^{th}$ ball lands in a ``bad'' bin, which happens with probability  $k/n$.  The third event is $(i,j,k)$.  It leads to the event $(i\!+\!1, j, k)$ when the $(i\!+\!1)^{th}$ ball lands in an empty bin, which happens with probability $1\!-\!(i\!-\!j\!+\!k)/n$. 
% Summarizing these three cases, we can express the probability $\tilde{M}(i\!+\!1,j,k)$ as the weighted sum of the probabilities of three events that can possibly lead to the
% event $(i\!+\!1,j,k)$ as follows:



% \begin{equation}\nonumber
% \tilde{M}(i+1,j,k) =     \frac{i\!-\!j\!+\!2}{n}\cdot \tilde{M}(i,j\!-\!2,k\!-\!1)+\frac{k}{n}\cdot \tilde{M}(i,j\!-\!1,k)+(1\!-\!\frac{i\!-\!j\!+\!k}{n})\cdot \tilde{M}(i,j,k)
% \end{equation}

\begin{align}
&    \frac{i\!-\!j\!+\!1}{n}\cdot \tilde{M}(i\!-\!1,j\!-\!2,k\!-\!1)+\frac{k}{n}\cdot \tilde{M}(i\!-\!1,j\!-\!1,k)\nonumber\\
&+(1\!-\!\frac{i\!-\!1\!-\!j\!+\!k}{n})\cdot \tilde{M}(i\!-\!1,j,k)\nonumber
\end{align}

% \begin{align}
% \tilde{M}(i,j,k) = &    \frac{i\!-\!j\!+\!1}{n}\cdot \tilde{M}(i\!-\!1,j\!-\!2,k\!-\!1)+\frac{k}{n}\cdot \tilde{M}(i\!-\!1,j\!-\!1,k)\nonumber\\
% &+(1\!-\!\frac{i\!-\!1\!-\!j\!+\!k}{n})\cdot \tilde{M}(i\!-\!1,j,k)\nonumber
% \end{align}

% \begin{align}
% \tilde{M}(i+1,j,k) = &    \frac{i\!-\!j\!+\!2}{n}\cdot \tilde{M}(i,j\!-\!2,k\!-\!1)+\frac{k}{n}\cdot \tilde{M}(i,j\!-\!1,k)\nonumber\\
% &+(1\!-\!\frac{i\!-\!j\!+\!k}{n})\cdot \tilde{M}(i,j,k)\nonumber
% \end{align}

%The three terms in this formula corresponds to the above three possible transitions. 
%The computational complexity for each 

Exploiting these recurrence relations (for $\forall i,j,k$), we can compute the values of all the $(t+1)^3$ $\tilde{M}(i, j, k)$ terms in $O(t^3)$ time via dynamic programming, for which the probability formulae of the three types of base cases are:

%  To do so, we need to first directly (i.e., without using the recurrence relation) compute for the following three types of base cases,
%which are clearly straightforward to do. 
% so the overall compuational complexity is $O(t^3)$ (for $t^3$ entries). To compute $M(i,j,k)$ for $\forall i,j,k=0,1,\cdots,t$ via dynamic programming, we also need to compute the transition probabilities in the base cases as follows. Here $M(i,0,0)$ contained in both the second base case and the third base case corresponds to the probability of the ideal case in PBS-for-small-$d$, which is the case that $i$ balls are thrown and all of them end up to be ``good''.
%Combining with the following probabilities in base cases, we can compute $M(i,j,k)$ for $\forall i,j,k=0,1,\cdots,t$ using Dynamic Programming and obtain $M$:

\begin{align}
\tilde{M}(0,j,k) =& \left\{ \begin{array}{ccl}
1, & \mbox{if }
 j=k=0 \\ 0, & \mbox{otherwise} 
\end{array}\right.\nonumber\\
\tilde{M}(i,0,k) =& \left\{ \begin{array}{ccl}
\binom{n}{i}/n^i, & \mbox{if }
 k=0 \\ 0, & \mbox{otherwise} 
\end{array}\right.\nonumber\\
\tilde{M}(i,j,0) =& \left\{ \begin{array}{ccl}
\binom{n}{i}/n^i, & \mbox{if }
 j=0 \\ 0, & \mbox{otherwise} 
\end{array}\right.\nonumber
\end{align}

\end{comment}

%It is clear from the three formulae above that the value of each term $\tilde{M}(i, j, k)$
%depends on only one parameter: $n$.  
%Hence, the matrix $M$ is parameterized only by $n$.  Note that $t$ is the ``support boundary", but not a parameter, of $M$.
%We will use this fact in \autoref{sec:parameter_settings}. 



% PBS reconciles the distinct elements gradually round by round. This is the ``piecewise decodability'' mentioned in \autoref{sec:intro_oursolution}. We use the following example to describe it in details: 
% Given two sets with $10$ distinct elements, in the first round, PBS tries to reconcile the $10$ distinct elements and say $6$ out of the $10$ distinct elements are successfully reconciled. Then the $6$ reconciled distinct elements are removed and PBS tries to reconcile the remaining $4$ distinct elements in the second round. Say $2$ out of the $4$ remaining distinct elements are successfully reconciled, and that leaves $2$ remaining distinct elements to be reconciled in the third round, so on so force. 
% % Given two sets $A$, $B$ with $10$ distinct elements, in the first round, PBS hashes them into $7$ distinct subset pairs. $6$ distinct elements are hashed into $6$ distinct subset pairs, and the other $4$ distinct elements are hashed into the same subset pair. Then the former $6$ distinct elements are successfully reconciled in the first round and the later $4$ distinct elements remain to be reconciled in the second round, which are hashed into $3$ distinct subset pairs (under a different hash function). $2$ remaining distinct elements are hashed into $2$ distinct subset pairs, and the other $2$ remaining distinct elements are hashed into the same subset pair. Then the former $2$ remaining distinct elements are successfully reconciled in the second round and the later $2$ remaining distinct elements remain to be reconciled in the third round, so on so force. 
% The dynamics of the number of remaining distinct elements (i.e., $10\leadsto 4\leadsto 2\leadsto \cdots$ in the example) is in nature a Markov chain, which will be elaborated and analyzed in \autoref{sec:single_markov} to derive a tight tail bound of the probability that all distinct elements are reconciled in $r$ rounds. 
\begin{comment}



In this section, we describe how to compute the transition probability matrix $M$ in detail. 
To compute $M(i,j)$ is not straightforward for the following reason.  
Each state $j$ with $j>3$ in the Markov chain is a {\it composite state} 
consisting of a large number of 
{\it atom states}.
%(defined next).  
Only the transition probability from state $i$ to any atom state (of state $j$) can be stated as a closed-form expression
%(more precisely, a multinomial formula) 
and computed straightforwardly. 
The value of $M(i,j)$ is the total of all the transition probabilities from state $i$ to each of the atom states of state $j$. 
Since the number of atom states grows exponentially with $j$, it is both complicated (as it is necessary to enumerate all atom states)
and computationally expensive to compute $M(i, j)$ this way when $j$ is large.

%the computation of $M(i,j)$ could be extremely complicated for large $j$.

Each atom state of state $j$ is, in combinatorics terms, {\it a permutation of a combination of $j$}, which here corresponds to how these $j$ balls are 
distributed in the $n$ bins (by the hash function).  For a simple example, when $j = 4$ and $n = 7$, the vector $(2, 0, 0, 0, 0, 2, 0)$ is such an atom state, which corresponds to these $7$ bins (in a predefined order such as the natural order) have $2, 0, 0, 0, 0, 2,$ and $0$ ``bad'' balls in them respectively. 
Clearly, the number of such atom states grows exponentially with $j$.

%Although the transition probability from state $i$ to each such atom state is computable, the number of atom states (permutations of combinations) grow exponentially with the number of balls $j$. 

%The transition probability from state $i$ to such an atom state is a closed-form expression and computable. The problem is that the number of atom states (permutations of combinations) grow exponentially with the number of balls $j$. 
%To obtain $M(i,j)$, we have to compute all transition probabilities from the (pre-transition) state $i$ to each of the atom states of state $j$ and sum them up. 

Our solution is to decompose each composite state $j$ into a much small number of coarse-grained sub-states, each of which may still contain a large number of atom states.  Although the transition probability from a state $i$ to any sub-state of $j$ is still a summation formula and hence hard to compute
in the ``mundane'' way as explained above, we discover a recurrence relation among these transition probabilities that makes them easily 
computable using dynamic programming.
% We overcome this problem by grouping the huge number of atom states into a smaller number of coarse-grained sub-states first, then computing the transition probability from the (pre-transition) state $i$ to any sub-states of state $j$. Although each sub-state still consists of many atom states and the transition probability to a sub-state is still hard to compute directly, we discover a recurrence relation among these transition probabilities, so we can compute them using Dynamic Programming.

% In this section, we describe how to compute the transition matrix $M$ in detail. For general $i,j$, $M(i,j)$ cannot be computed straightforwardly. Our solution is to decompose each state $j$ into a small number of sub-states, so that the transition probability $M(i,j)$ can be computed as the summation of the transition probabilities from state $i$ to each of the sub-states of state $j$. Although these transition probabilities also cannot be computed straightforwardly, we discover a recurrence relation among these transition probabilities that makes them easily computable using dynamic programming.





are defined as follows:
%The sub-states of state $j$ is defined as follows: 
let state $(j,k)$ denote the sub-state of state $j$ that the $j$ ``bad'' balls end up to occupy exactly $k$ ``bad'' bins. We call a bin ``good'' if it contains exactly $1$ (``good'') ball, and a bin ``bad'' if it contains more than $1$ (``bad'') balls. The composite state $j$ is partitioned into state $(j,1)$, state $(j,2)$, $\cdots$, state $(j,j)$. We slightly abuse the notation and let $M(i,j,k)$ denote the probability of transition from state $i$ to state $(j,k)$, then we have 


State $(i+1,j,k)$ can only be reached from three states: (1) state $(i,j-2,k-1)$ when the $(i+1)$-th ball lands in a ``good'' bin (so that the ``good'' ball in the bin and the $(i+1)$-th ball becomes two ``bad'' balls). The probability of this transition is $(i-j+2)/n$, since there are $i-(j-2)$ out of $n$ bins are ``good'' at state $(i,j-2,k-1)$; (2) state $(i,j-1,k)$ when the $(i+1)$-th ball lands in a ``bad'' bin, which happens with probability of $k/n$; and (3) state $(i,j,k)$ when the $(i+1)$-th ball lands in an empty bin, which happens with probability of $1-(i-j+2)/n$;. It induces a recurrence relation that $M(i+1,j,k)$ equals to



In the previous Markov chain, we assume the ``bad'' balls are thrown `simultaneously' into the $n$ bins. Here, we zoom into the ``throwing'' process and consider it as a ``slow motion Markov chain'', in which the ``bad'' balls are thrown one after another. In this ``slow motion Markov chain'', state $(i,j,k)$ is defined as $j$ ``bad'' balls ending up into $k$ ``bad'' bins after throwing $i$ balls.
%Note that the state transition resulting from throwing one ball after another is also a Markov chain, in which state $(i,j,k)$ is defined as $j$ ``bad'' balls ending up into $k$ ``bad'' bins after throwing $i$ balls into $n$ bins. In this Markov chain, 
%throwing one more ball can transition state $(i,j,k)$ to three possible states depending on the $(i+1)$-th ball ending up in (1) a ``good'' bin; (2) a ``bad'' bin; or (3) an empty bin. The first case happens with probability $(i-j)/n$, results in $2$ additional ``bad'' balls and $1$ additional ``bad'' bin (i.e., transition to state $(i+1,j+2,k+1)$). The second and third cases transition to state $(i+1,j+1,k)$ and state $(i+1,j,k)$ respectively with probability $k/n$ and $1-(i-j+k)/n$. In the opposite direction, 


%The second case happens with probability $k/n$ and results in state $(i+1,j+1,k)$. The third case happens with probability $1-(i-j+k)/n$ and results in state $(i+1,j,k)$. In the opposite direction, state $(i+1,j,k)$ can be transitioned from (1) state $(i,j-2,k-1)$ with probability $(i-j+2)/n$; (2) state $(i,j-1,k)$ with probability $k/n$; or (3) state $(i,j,k)$ with probability $1-(i-j+k)/n$. It gives us a recurrence relation that $P(i+1,j,k)$ equals to



In this section, we describe how to compute the transition matrix $M$ in details. 
Calculating an arbitrary transition probability $M(i,j)$ is not straightforward, since each state $j$ with $j>3$ in the Markov chain is a {\it composite state}, which consists of a huge number of {\it atom states}. Only the transition probability from state $i$ to any atom state of state $j$ can be stated as a closed-form expression (more precisely, a multinomial formula) and therefore can be computed straightforwardly. $M(i,j)$ is the summation of all the transition probabilities from state $i$ to each of the atom states of state $j$. While this may not sound like a problem, the number of atom states grow exponentially with $j$, so the computation of $M(i,j)$ could be extremely complicated for large $j$.

Each atom state of state $j$ is, in combinatorics terms, {\it a permutation of a combination of $j$}, which here corresponds to how these $j$ balls are placed into the $n$ bins.  For a simple example, when $j = 4$ and $n = 7$, the vector $(2, 0, 0, 0, 0, 2, 0)$ is such an atom state, which corresponds to these $7$ bins (in a predefined order such as the natural order) have $2, 0, 0, 0, 0, 2,$ and $0$ ``bad'' balls in it respectively. Although the transition probability from state $i$ to each such atom state is computable, the number of atom states (permutations of combinations) grow exponentially with the number of balls $j$. 

%The transition probability from state $i$ to such an atom state is a closed-form expression and computable. The problem is that the number of atom states (permutations of combinations) grow exponentially with the number of balls $j$. 
%To obtain $M(i,j)$, we have to compute all transition probabilities from the (pre-transition) state $i$ to each of the atom states of state $j$ and sum them up. 

We notice that we can break each composite state $j$ into a much small number of coarse-grained sub-states, each of which may still contain a large number of atom states. Although the transition probability from state $i$ to any sub-state is still a summation formula and hard to compute, we discover a recurrence relation among these transition probabilities that allows us to compute them using dynamic programming. 
% We overcome this problem by grouping the huge number of atom states into a smaller number of coarse-grained sub-states first, then computing the transition probability from the (pre-transition) state $i$ to any sub-states of state $j$. Although each sub-state still consists of many atom states and the transition probability to a sub-state is still hard to compute directly, we discover a recurrence relation among these transition probabilities, so we can compute them using Dynamic Programming.




%as far as the calculation of the transition probability from a (larger) state $i$ $(>j)$ to $j$ is concerned. 
% To calculate the probability, we have to break the composite state $j$ down into ``atom'' states, calculate the transition probability from state $i$ to each of the ``atom'' states (which can be directly calculated), and then add them up. {\bf Note that we always view state $i$ (pre-transition state) as a {\it simple state}, since how the $i$ balls are placed into $n$ bins only depends on the hash function.}

% Each composite state $j$ can be broken down into atom states based on how these $j$ bad balls are placed into the $n$ bins. For example, state $6$ consists of $4$ atom states. The first one is $6 = 6$, where all $6$ bad balls are in the same bad bin. The second one is $6 = 2 + 4$ where, out of the $6$ bad balls, four are in one bad bin and the other two are in the other bad bin.  Similarly, the other two atom states are $6 = 3 + 3$ and $6 = 2 + 2 + 2$. The transition probability from state $i$ to any atom state can be directly calculated, but the problem is that the number of atom states grows exponentially with the number of ``bad'' balls $j$.

% We notice that we can break each composite state into a small number of coarse-grained sub-states, each of which may still contain a large number of atom states. The transition probability from a (larger) state $i$ to any sub-state is still hard to compute. However, there is a recurrence relation among them, so we can compute the transition probabilities from any state to any sub-state using Dynamic Programming. 


+++++++++++

The only problem left to obtain $Pr[d\xrsquigarrow{r} 0]$ is how to compute $M$, which is not straightforward, since each state $j$ with $j>3$ in the Markov chain is a composite state as far as the calculation of the transition probability from a (larger) state $i$ $(>j)$ to $j$ (i.e., ``transitioning into'') is concerned.   {\bf You need to explain why it is not straightforward:  The reason you offer is not
the direction reason.  Instead you may say that "the transition probability between these composite states cannot be directly calculated" \cdots  to calculate it we have to break it down into "atom" states}

Each composite state $i$ can be broken down into atom states as follows.  Each simple state is, in combinatorics terms, {\it a permutation of a combination of $i$}, which here corresponds to 
how these $i$ balls are ``divided up" by the $n$ bins.   {\bf Liang, Read Mitzenmacher and Upfal book
for a better word for "divided up"}
For a simple example, when $i = 4$ and $n = 7$, the vector (1, 0, 1, 0, 0, 2, 0) is such a simple state, which corresponds to these 7 bins (in a predefined order such as the natural order) 
have 1, 0, 1, 0, 0, 2, and 0 balls in it respectively.   The transition probability between any two atom states can be \cdots    but the problem is that the number of atom states 
(permutations of combinations) grow exponentially with the number of balls $i$.

Consider two states i1 and i2 each broken down into millions of atom states.  Then the transition probability between these states is the summation of the trillions (= millions * millions) of 
transition probabilities between atom states of i1 and atom states of i2.  

The good thing is that the transition probability matrix among the (humongous number of atom states) induces a "subproblem structure ????", which leads to the recurrence relation, 
dynamic programming.   

We notice that we can break each state into a small number of coarse-grained substates, each of which may still contain a large number of atom states.  The transition probability 
between any two such substates are still hard to compute.  However, there is a recurrence relation among them \cdots

+++++++++++

To solve the problem, we partition the composite state into sub-states, so that the transition probability to the composite state is the summation of the transition probabilities to each of the sub-states. On the other hand, the transition probabilities to the sub-state have a recurrence relation and can be computed using Dynamic Programming. 

======================================

Note that every state $j$ with $j > 3$ in the Markov chain is a composite state as far as the calculation of the transition probability from a (larger) state $i > j$ to $j$ (i.e., ``transitioning into").  For example, State 6 contains 4 different cases. The first case is $6 = 6$, where all 6 bad balls are in the same bad bin. The second case is $6 = 2 + 4$ where, out of the 6 bad balls, four are in one bad bin and the other two are in the other bad bin.  Similarly, the other two cases are $6 = 3 + 3$ and $6 = 2 + 2 + 2$. Note there is no need to distinguish these four cases in calculating the ``transitioning out" probability (i.e., from state 6 to a small state say State 0), because the next round of balls-into-bins operation uses a different hash function independent of that used in the current round, and consequently how these 6 bad balls are split in the current round have no bearing on that in the next round. 

Building on the example above, we now consider $m_{9,6}$, the transition probability from State $9$ to State $6$ (throwing 9 balls into 255 bins and ending up with 6 bad balls).  $m_{9,6}$ is simply the sum of the probabilities of these four cases, each of which has a very different formula than the others.  In general, the number of such cases, and hence the number of individual probability terms to be added up to arrive at the transition matrix element $m_{i,j}$, grows exponentially with the value of $j$. This does not however make it difficult to calculate the values of $M$, because there is a recursive structure, among the values of the matrix elements $m_{i,j}$, that can be exploited using dynamic programming, as will be elaborated shortly.

To simplify our analysis, we split each composite state into sub-composite states based on the number of nonempty bins: Let State $(j,k)$ denotes the sub-composite state with $j$ remaining distinct elements and $k$ nonempty bins, which is also a substate of State $j$. Let $m_{i,j}^{(k)}$ denote the probability of transition from State $i$ to State $(j,k)$, which is also the probability that after throwing $i$ balls uniformly and independently into $n$ bins, $i-j$ bins are ``good'' bins and $k$ bins are nonempty bins (thus $k-(i-j)$ bins are ``bad'' and $n-k$ bins are empty). The probability of transition to a composite state is simply the summation of the probabilities of the transitions to corresponding sub-composite states:

To obtain the transition matrix $M$, it is sufficient to compute $m^{(k)}_{i,j}$, which can be exploited using dynamic programming. Note that the balls-and-bins model itself can be considered as a Markov chain, in which a recursive relation exists: After throwing $i$ balls into $n$ bins, throwing one more ball randomly could be: (1) Into an empty bin and turn it to a ``good'' bin; (2) Into a ``good'' bin and turn it to a ``bad'' bin with two balls; or (3) Into a ``bad'' bin and keep it as the same. Mathematically, we have $m^{(k)}_{i+1,j}$ equals to


====================================
\end{comment}



==> section/theoretical_analysis_seperate0222.tex <==
\section{Theoretical Analysis}\label{sec:tail_bound}

In this section, we provide a theoretical analysis (analytical framework) for PBS reconciliation process and establish a tight tail bound on the {\it success probability} within $r$ rounds (defined in \autoref{subsec:protocol2}) under arbitrary parameter settings of $n$, $\delta$, and $t$. This analytical framework has several applications on parameter settings and analyzing the properties of PBS that we will elaborate in \autoref{sec:application_analysis}.

% On one hand, this tail bound gives us a theoretical guarantee on the success probability under specific parameter settings. On the other hand, given a parameter setting requirement (i.e., a target success probability $p_0$ within $r$ rounds), we can use the tail bound to find all feasible parameter settings that satisfy the requirement, then select the optimal parameter settings among them that have the lowest communication overhead. {\bf This analysis also provides other theoretical results for PBS, such as the expected number (percentage) of the distinct elements would be reconciled in the each round (``piecewise decodability'', to be shown in \autoref{sec:piecewise_decodability})}%In this section, we continue to assume $d$ is precisely known. 

For simplicity, we ignore the small probability event that a type (\RN{2}) event happens and the incurred ``fake'' distinct element is not successfully verified by \autoref{alg:verification} (mentioned in \autoref{subsec:exception_hash_partition}). As we discussed earlier, this event happens with a tiny probabilty that is in order of $10^{-7}$. Hence, ignoring this event barely compromises the accuracy of our analysis. 

\subsection{Analysis of a simple case}\label{sec:single_markov}

In this section, we analyze the probability that an arbitrary group pair that contains exactly $x$ $(\leq t)$ distinct elements is completely reconciled (i.e., all distinct elements are successfully reconciled) by PBS in $r$ rounds.

As we described in \autoref{sec:multi-rounds}, in the first round of PBS, the $x$ distinct elements are hashed into $n$ subset pairs, and a distinct element is successfully reconciled if and only if it is hashed into a subset pair that contains only $1$ distinct element. 
%The successfully reconciled distinct elements in the first round are removed and the other distinct elements (i.e., the ones that have not been reconciled yet in the first round) will be hashed again in the second round using a different hash function, so on so force, until all distinct elements are successfully reconciled. 
How the $x$ distinct elements are distributed into $n$ subset pairs in the first round follows the familiar {\it balls-into-bins} probability model: Each of the $x$ balls is thrown independently and uniformly at random into one of the $n$ bins. Each successfully reconciled distinct element corresponds to a ball that ends up in a bin that receives exactly $1$ ball. We call the ball and the bin ``good'' in the sequel; each distinct element that has not been reconciled yet in the first round corresponds to a ball that ends up in a bin that receives multiple balls. We call the ball and the bin ``bad'' in the sequel. Note that balls are either ``good'' or ``bad'', but a bin could be empty besides being ``good'' and ``bad''. 

The ``bad'' balls in the first round will be the balls to be thrown in the second round. The ``bad'' balls in the second round will be the balls to be thrown in the third round, so on so force. In all rounds, how the balls are thrown into $n$ bins follows the same balls-into-bins probability model. Note that the balls are thrown using different hash functions in each round, so the number of ``bad'' balls in the $i$-th round
%(i.e., the number of balls to be thrown in the $(i+1)$-th round) 
only depends on how many balls are thrown in the $i$-th round and is independent of how these balls (``bad'' balls in the $(i-1)$-th round) are placed into the $n$ bins in the $(i-1)$-th round. Therefore, the number of balls to be thrown round after round is a Markov chain, in which each state is defined as the number of balls to be thrown. 
%Hence, the dynamics of the number of balls to be thrown in each round can be modeled as a Markov chain, in which each state is defined as the number of balls to be thrown. {\bf a little bit wordy, need advice on how to shrink it.}

In the Markov chain, a transition from state $i$ to state $j$ ($i\geq j$) means $i-j$ out of $i$ balls are ``good'' balls and the other $j$ balls are ``bad'' balls. The {\it absorbing state} of this Markov chain is state $0$, which is the ``good'' state that all balls are ``good'' (so that all distinct elements are successfully reconciled). For our analysis, the only probability that we are concerned with is $Pr[x\!\xrsquigarrow{r}\! 0]$, the probability that starting with state $x$ (initial state), the Markov chain reaches the absorbing state (i.e., state $0$) within $r$ transitions. It is also the success probability for a single group (starting with $x$ distinct elements and successfully reconciled within $r$ rounds), which can easily calculated given $M$, the $(t+1)\times (t+1)$ transition matrix of the Markov chain, as 
%, where $M(i,j)$ (i.e., the entry in the $i^{th}$ row and the $j^{th}$ column of $M$) is the probability of transition from state $i$ to state $j$ for $i,j = 0,1,...,t$
$\big{(}M^r\big{)}(x,0)$, the entry in the $x$-th row and the $0$-th column of $M^r$. Here we slightly abuse the row / column indices of a $(t+1)\times (t+1)$ matrix from $1,2,...,t+1$ to $0,1,...,t$, since the state of the Markov chain ranges from $0$ to $t$. How to compute $M$ will be elaborated in \autoref{sec:compute_M}. For the moment, we assume $M$ has been computed and therefore we can compute $Pr[x\!\xrsquigarrow{r}\! 0]$ for $x=1,2,...,t$, $r\in\mathbb{N}^+$. 

\subsection{Tail Bound Analysis for Each Group Pair}\label{sec:tail_bound_per_group}

% ==========
% {\bf The following may be useful in explaining why it is a Markov chain:} [Note there is no need to distinguish these four cases in calculating the ``transitioning out" probability (i.e., from state 6 to a small state say State 0), because the next round of balls-into-bins operation uses a different hash function independent of that used in the current round, and consequently how these 6 bad balls are split in the current round have no bearing on that in the next round.]  {\bf unless you have done so earlier}
% ==========

As we explained in \autoref{subsec:protocol2}, $\delta_1$, the number of distinct elements in group pair $1$, is a random variable that follows a Binomial distribution $Binomial(d,1/g)$. So the probability that group pair $1$ is successfully reconciled in $r$ rounds is $\sum_{x=0}^d Pr[\delta_1\!=\!x]\cdot Pr[x\!\xrsquigarrow{r}\! 0]$. 
%, where $\mathcal{B}(\cdot;d,1/g)$ is the probability mass function (PMF) of $Binomial(d,1/g)$. 
To ease computation, we slightly underestimate this probability by assuming $Pr[x\!\xrsquigarrow{r}\! 0]=0$ when $x>t$ (i.e., assume group pair $1$ cannot be reconciled if $\delta_1>t$, discussed in \autoref{sec:BCH_exception}). The loss of this underestimation is very tiny, since $Pr[\delta_1\!=\!x]$, the ``coefficient'' of $Pr[x\!\xrsquigarrow{r}\! 0]$, is very small when $x>t$. We denote this underestimated probability as $\alpha$ (i.e., $\alpha=\sum_{x=0}^t Pr[\delta_1\!=\!x]\cdot Pr[x\!\xrsquigarrow{r}\! 0]$), which is a tight tail bound of the success probability of group pair $1$. $\alpha$ is also a tight tail bound for all other group pairs, since $\delta_1,\delta_2,...,\delta_g$ follows the same distribution. $Pr[x\!\xrsquigarrow{r}\! 0]$ is a function of $n$ for given $x$ and $r$, so $\alpha=\alpha(n,t)$ is a function of $n$ and $t$ for arbitrary $d$, $r$, and $g$. 

\subsection{Tail Bound Analysis for All Group Pairs}\label{sec:times2bound}

Given $\alpha$, the tail bound of the probability that a group pair is successfully reconciled in $r$ rounds, we can easily derive a tail bound of $\alpha^g=1-(1-\alpha^g)$ for the probability that all group pairs are successfully reconciled in $r$ rounds ($1-\alpha^g$ is the failure probability, which is usually tiny), if we assume the reconciliations on group pairs are independent with each other. However, this assumption is not rigorous,
%since $d_1, d_2,...,d_g$ have a weak correlation that $\sum_{i=1}^g d_i=d$.
since $\delta_1, \delta_2,...,\delta_g$ are not strictly independent and have a relation that $\sum_{i=1}^g \delta_i=d$. 
%Fortunately, we have Times-2-Bound (Theorem 1 in \cite{hua2008rank}) to decouple the weak correlation and give us a rigorous tail bound of $1-2(1-\alpha^g)$ for the probability of all group pairs. 
However, we can use Corollary 5.11 in \cite{upfal2005probability} to
% decouple the weak correlation and 
obtain a rigorous tail bound of $1-2(1-\alpha^g)$ for the success probability of all group pairs. This rigorous tail bound is very tight and only doubles the tiny failure probability of the unrigorous tail bound: For example, if the unrigorous tail bound of the success probability of all group pairs is $0.9999$ ($0.0001$ failure probability), then the rigorous tail bound will be $0.9998$ ($0.0002$ failure probability). We use the tail bound of $1-2(1-\alpha^g)$ in parameter settings for rigorousness. 

\subsection{How to compute \texorpdfstring{\larger\boldmath{$M$}}{M}}\label{sec:compute_M}

In this section, we describe how to compute the transition matrix $M$ in details. Note that calculating an arbitrary transition probability $M(i,j)$ is not straightforward, since each state $j$ (after-transition state) with $j>3$ in the Markov chain is a {\it composite state}, which consists of a huge number of {\it atom states}. 
%The transition probability $M(i,j)$ is basically the summation of all transition probabilities from the (pre-transition) state $i$ to each of the atom states of state $j$. 

Each composite state $j$ can be broken down into atom states as follows.  Each simple state is, in combinatorics terms, {\it a permutation of a combination of $j$}, which here corresponds to how these $j$ balls are placed into the $n$ bins.  For a simple example, when $j = 4$ and $n = 7$, the vector $(2, 0, 0, 0, 0, 2, 0)$ is such a simple state, which corresponds to these $7$ bins (in a predefined order such as the natural order) have $2, 0, 0, 0, 0, 2,$ and $0$ ``bad'' balls in it respectively. The transition probability from the (pre-transition) state $i$ to any atom state of state $j$ can be directly computed, and $M(i,j)$ is basically the summation of all these transition probabilities. The problem is that the number of atom states (permutations of combinations) grow exponentially with the number of balls $j$. 
%To obtain $M(i,j)$, we have to compute all transition probabilities from the (pre-transition) state $i$ to each of the atom states of state $j$ and sum them up. 

We overcome this problem by grouping the huge number of atom states into a smaller number of coarse-grained sub-states first, then computing the transition probability from the (pre-transition) state $i$ to any sub-states of state $j$. Although each sub-state still consists of many atom states and the transition probability to a sub-state is still hard to compute directly, we discover a recurrence relation among these transition probabilities, so we can compute them using Dynamic Programming.



%as far as the calculation of the transition probability from a (larger) state $i$ $(>j)$ to $j$ is concerned. 
% To calculate the probability, we have to break the composite state $j$ down into ``atom'' states, calculate the transition probability from state $i$ to each of the ``atom'' states (which can be directly calculated), and then add them up. {\bf Note that we always view state $i$ (pre-transition state) as a {\it simple state}, since how the $i$ balls are placed into $n$ bins only depends on the hash function.}

% Each composite state $j$ can be broken down into atom states based on how these $j$ bad balls are placed into the $n$ bins. For example, state $6$ consists of $4$ atom states. The first one is $6 = 6$, where all $6$ bad balls are in the same bad bin. The second one is $6 = 2 + 4$ where, out of the $6$ bad balls, four are in one bad bin and the other two are in the other bad bin.  Similarly, the other two atom states are $6 = 3 + 3$ and $6 = 2 + 2 + 2$. The transition probability from state $i$ to any atom state can be directly calculated, but the problem is that the number of atom states grows exponentially with the number of ``bad'' balls $j$.

% We notice that we can break each composite state into a small number of coarse-grained sub-states, each of which may still contain a large number of atom states. The transition probability from a (larger) state $i$ to any sub-state is still hard to compute. However, there is a recurrence relation among them, so we can compute the transition probabilities from any state to any sub-state using Dynamic Programming. 

The sub-states of state $j$ is defined as follows: let state $(j,k)$ denote the sub-state of state $j$ that the $j$ ``bad'' balls end up to occupy exactly $k$ ``bad'' bins. Then the composite state $j$ is partitioned into state $(j,1)$, state $(j,2)$, $...$, state $(j,j)$. We slightly abuse the notation and let $M(i,j,k)$ denote the probability of transition from state $i$ to state $(j,k)$, then we have 

\begin{equation}\nonumber
    M(i,j) = \sum_{k=1}^{j} M(i,j,k)
\end{equation}

%{\bf explain the range of $k$ could be distracting, so I just leave it as it is.}
To obtain $M$, it is sufficient to compute $M(i,j,k)$ for $\forall i,j,k=0,1,...,t$. Note that the state transition resulting from throwing one ball after another is also a Markov chain, in which state $(i,j,k)$ is defined as $j$ ``bad'' balls ending up into $k$ ``bad'' bins after throwing $i$ balls into $n$ bins. In this Markov chain, throwing one more ball can transition state $(i,j,k)$ to three possible states depending on the $(i+1)$-th ball ending up in (1) a ``good'' bin; (2) a ``bad'' bin; or (3) an empty bin. The first case happens with probability $(i-j)/n$, results in $2$ additional ``bad'' balls and $1$ additional ``bad'' bin (i.e., transition to state $(i+1,j+2,k+1)$). The second and third cases transition to state $(i+1,j+1,k)$ and state $(i+1,j,k)$ respectively with probability $k/n$ and $1-(i-j+k)/n$. In the opposite direction, state $(i+1,j,k)$ can only be transitioned from (1) state $(i,j-2,k-1)$; (2) state $(i,j-1,k)$; and (3) state $(i,j,k)$, which gives us a recurrence relation that $M(i+1,j,k)$ equals to

%The second case happens with probability $k/n$ and results in state $(i+1,j+1,k)$. The third case happens with probability $1-(i-j+k)/n$ and results in state $(i+1,j,k)$. In the opposite direction, state $(i+1,j,k)$ can be transitioned from (1) state $(i,j-2,k-1)$ with probability $(i-j+2)/n$; (2) state $(i,j-1,k)$ with probability $k/n$; or (3) state $(i,j,k)$ with probability $1-(i-j+k)/n$. It gives us a recurrence relation that $P(i+1,j,k)$ equals to

\begin{equation}\nonumber
    \frac{i\!-\!j\!+\!2}{n}\cdot M(i,j\!-\!1,k\!-\!1)+\frac{k}{n}\cdot M(i,j\!-\!1,k)+(1\!-\!\frac{i\!-\!j\!+\!2}{n})\cdot M(i,j,k)
\end{equation}

The three terms in this formula corresponds to the above three possible transitions. To compute $M(i,j,k)$ for $\forall i,j,k=0,1,...,t$ via Dynamic Programming, the total computational complexity is $O(t^3)$ ($O(1)$ for $t^3$ entries), and we also need to compute the transition probabilities in the base cases as follows:  
%Combining with the following probabilities in base cases, we can compute $M(i,j,k)$ for $\forall i,j,k=0,1,...,t$ using Dynamic Programming and obtain $M$:

\begin{align}
M(0,j,k) =& \left\{ \begin{array}{ccl}
1, & \mbox{if }
 j=k=0 \\ 0, & \mbox{otherwise} 
\end{array}\right.\nonumber\\
M(i,0,k) =& \left\{ \begin{array}{ccl}
\binom{n}{i}/n^i, & \mbox{if }
 k=0 \\ 0, & \mbox{otherwise} 
\end{array}\right.\nonumber\\
M(i,j,0) =& \left\{ \begin{array}{ccl}
1, & \mbox{if }
 j=0 \\ 0, & \mbox{otherwise} 
\end{array}\right.\nonumber
\end{align}

% PBS reconciles the distinct elements gradually round by round. This is the ``piecewise decodability'' mentioned in \autoref{sec:intro_oursolution}. We use the following example to describe it in details: 
% Given two sets with $10$ distinct elements, in the first round, PBS tries to reconcile the $10$ distinct elements and say $6$ out of the $10$ distinct elements are successfully reconciled. Then the $6$ reconciled distinct elements are removed and PBS tries to reconcile the remaining $4$ distinct elements in the second round. Say $2$ out of the $4$ remaining distinct elements are successfully reconciled, and that leaves $2$ remaining distinct elements to be reconciled in the third round, so on so force. 
% % Given two sets $A$, $B$ with $10$ distinct elements, in the first round, PBS hashes them into $7$ distinct subset pairs. $6$ distinct elements are hashed into $6$ distinct subset pairs, and the other $4$ distinct elements are hashed into the same subset pair. Then the former $6$ distinct elements are successfully reconciled in the first round and the later $4$ distinct elements remain to be reconciled in the second round, which are hashed into $3$ distinct subset pairs (under a different hash function). $2$ remaining distinct elements are hashed into $2$ distinct subset pairs, and the other $2$ remaining distinct elements are hashed into the same subset pair. Then the former $2$ remaining distinct elements are successfully reconciled in the second round and the later $2$ remaining distinct elements remain to be reconciled in the third round, so on so force. 
% The dynamics of the number of remaining distinct elements (i.e., $10\leadsto 4\leadsto 2\leadsto \cdots$ in the example) is in nature a Markov chain, which will be elaborated and analyzed in \autoref{sec:single_markov} to derive a tight tail bound of the probability that all distinct elements are reconciled in $r$ rounds. 
\begin{comment}
+++++++++++

The only problem left to obtain $Pr[d\xrsquigarrow{r} 0]$ is how to compute $M$, which is not straightforward, since each state $j$ with $j>3$ in the Markov chain is a composite state as far as the calculation of the transition probability from a (larger) state $i$ $(>j)$ to $j$ (i.e., ``transitioning into'') is concerned.   {\bf You need to explain why it is not straightforward:  The reason you offer is not
the direction reason.  Instead you may say that "the transition probability between these composite states cannot be directly calculated" ...  to calculate it we have to break it down into "atom" states}

Each composite state $i$ can be broken down into atom states as follows.  Each simple state is, in combinatorics terms, {\it a permutation of a combination of $i$}, which here corresponds to 
how these $i$ balls are ``divided up" by the $n$ bins.   {\bf Liang, Read Mitzenmacher and Upfal book
for a better word for "divided up"}
For a simple example, when $i = 4$ and $n = 7$, the vector (1, 0, 1, 0, 0, 2, 0) is such a simple state, which corresponds to these 7 bins (in a predefined order such as the natural order) 
have 1, 0, 1, 0, 0, 2, and 0 balls in it respectively.   The transition probability between any two atom states can be ...    but the problem is that the number of atom states 
(permutations of combinations) grow exponentially with the number of balls $i$.

Consider two states i1 and i2 each broken down into millions of atom states.  Then the transition probability between these states is the summation of the trillions (= millions * millions) of 
transition probabilities between atom states of i1 and atom states of i2.  

The good thing is that the transition probability matrix among the (humongous number of atom states) induces a "subproblem structure ????", which leads to the recurrence relation, 
dynamic programming.   

We notice that we can break each state into a small number of coarse-grained substates, each of which may still contain a large number of atom states.  The transition probability 
between any two such substates are still hard to compute.  However, there is a recurrence relation among them ...

+++++++++++

To solve the problem, we partition the composite state into sub-states, so that the transition probability to the composite state is the summation of the transition probabilities to each of the sub-states. On the other hand, the transition probabilities to the sub-state have a recurrence relation and can be computed using Dynamic Programming. 

======================================

Note that every state $j$ with $j > 3$ in the Markov chain is a composite state as far as the calculation of the transition probability from a (larger) state $i > j$ to $j$ (i.e., ``transitioning into").  For example, State 6 contains 4 different cases. The first case is $6 = 6$, where all 6 bad balls are in the same bad bin. The second case is $6 = 2 + 4$ where, out of the 6 bad balls, four are in one bad bin and the other two are in the other bad bin.  Similarly, the other two cases are $6 = 3 + 3$ and $6 = 2 + 2 + 2$. Note there is no need to distinguish these four cases in calculating the ``transitioning out" probability (i.e., from state 6 to a small state say State 0), because the next round of balls-into-bins operation uses a different hash function independent of that used in the current round, and consequently how these 6 bad balls are split in the current round have no bearing on that in the next round. 

Building on the example above, we now consider $m_{9,6}$, the transition probability from State $9$ to State $6$ (throwing 9 balls into 255 bins and ending up with 6 bad balls).  $m_{9,6}$ is simply the sum of the probabilities of these four cases, each of which has a very different formula than the others.  In general, the number of such cases, and hence the number of individual probability terms to be added up to arrive at the transition matrix element $m_{i,j}$, grows exponentially with the value of $j$. This does not however make it difficult to calculate the values of $M$, because there is a recursive structure, among the values of the matrix elements $m_{i,j}$, that can be exploited using dynamic programming, as will be elaborated shortly.

To simplify our analysis, we split each composite state into sub-composite states based on the number of nonempty bins: Let State $(j,k)$ denotes the sub-composite state with $j$ remaining distinct elements and $k$ nonempty bins, which is also a substate of State $j$. Let $m_{i,j}^{(k)}$ denote the probability of transition from State $i$ to State $(j,k)$, which is also the probability that after throwing $i$ balls uniformly and independently into $n$ bins, $i-j$ bins are ``good'' bins and $k$ bins are nonempty bins (thus $k-(i-j)$ bins are ``bad'' and $n-k$ bins are empty). The probability of transition to a composite state is simply the summation of the probabilities of the transitions to corresponding sub-composite states:

To obtain the transition matrix $M$, it is sufficient to compute $m^{(k)}_{i,j}$, which can be exploited using dynamic programming. Note that the balls-and-bins model itself can be considered as a Markov chain, in which a recursive relation exists: After throwing $i$ balls into $n$ bins, throwing one more ball randomly could be: (1) Into an empty bin and turn it to a ``good'' bin; (2) Into a ``good'' bin and turn it to a ``bad'' bin with two balls; or (3) Into a ``bad'' bin and keep it as the same. Mathematically, we have $m^{(k)}_{i+1,j}$ equals to


====================================
\end{comment}



==> section/theoretical_analysis_seperate0224.tex <==
\section{Theoretical Analysis}\label{sec:tail_bound}

\subsection{Motivation}

In this section, we estabilish an analytical framework for the set reconciliation process of PBS. The motivation of it application of this analytical framework is a tight tail bound on the {\it success probability} within $r$ rounds under arbitrary parameter settings of $n$, $\delta$, and $t$.

{\bf (moved from the small d case)} Note that the set reconciliation process of the group pairs are independent with each other, and each group pair runs as many rounds of PBS-for-small-$d$ as needed to reconcile all distinct elements in it. Therefore, different group pairs may need different number of rounds to be successfully reconciled. Intuitively, we want all group pairs to be successfully reconciled in only a few rounds (say $3$) with high probability (say $99\%$). Hence, when tuning parameters (to be discussed in \autoref{sec:parameter_settings}), we set a {\it target success probability} $p_0$ combined with a {\it target number of rounds} $r$ as the {\it paramenter setting requirement}, which aims to ensure that the {\it success probability}, the probability that all distinct elements (of all group pairs) are reconciled, within $r$ rounds to be at least $p_0$. 
{\bf Normally, to achieve the same target success probability within fewer rounds (smaller $r$), PBS need more resources (e.g., larger $n$, $t$) for the ideal case happening with higher probability (fewer exceptions happen and need to be handled in later rounds), as we will explain in \autoref{sec:vary_r}.}

In this section, we provide a theoretical analysis (analytical framework) for the set reconciliation process of PBS and establish a tight tail bound on the {\it success probability} within $r$ rounds under arbitrary parameter settings of $n$, $\delta$, and $t$. This analytical framework has several applications on parameter settings and analyzing the properties of PBS that we will elaborate in \autoref{sec:application_analysis}.

% On one hand, this tail bound gives us a theoretical guarantee on the success probability under specific parameter settings. On the other hand, given a parameter setting requirement (i.e., a target success probability $p_0$ within $r$ rounds), we can use the tail bound to find all feasible parameter settings that satisfy the requirement, then select the optimal parameter settings among them that have the lowest communication overhead. {\bf This analysis also provides other theoretical results for PBS, such as the expected number (percentage) of the distinct elements would be reconciled in the each round (``piecewise decodability'', to be shown in \autoref{sec:piecewise_decodability})}%In this section, we continue to assume $d$ is precisely known. 

For simplicity, we ignore the small probability event that a type (\RN{2}) event happens, in which the incurred ``fake'' distinct element is not successfully verified by \autoref{alg:verification} (mentioned in \autoref{subsec:exception_hash_partition}). As we discussed earlier, this event happens with a tiny probabilty that is in order of $10^{-7}$. Hence, ignoring this event barely compromises the accuracy of our analysis. 

%\subsection{Analysis of a simple case}\label{sec:single_markov}
\subsection{The process under PBS}\label{sec:single_markov}

In this section, we analyze the probability that an arbitrary group pair that contains exactly $x$ $(\leq t)$ distinct elements is {\it successfully reconciled} by PBS in $r$ rounds. Here we say a group pair is {\it successfully reconciled} within $r$ rounds if and only if all distinct elements in the group pair are successfully reconciled within $r$ rounds. 

As we described in \autoref{sec:multi-rounds}, in the first round of PBS, the $x$ distinct elements are hashed into $n$ subset pairs, and a distinct element is successfully reconciled if and only if it is hashed into a subset pair that contains only $1$ distinct element. 
%The successfully reconciled distinct elements in the first round are removed and the other distinct elements (i.e., the ones that have not been reconciled yet in the first round) will be hashed again in the second round using a different hash function, so on so force, until all distinct elements are successfully reconciled. 

How the $x$ distinct elements are distributed into $n$ subset pairs in the first round follows the familiar {\it balls-into-bins} probability model: Each of the $x$ balls is thrown independently and uniformly at random into one of the $n$ bins. Each successfully reconciled distinct element corresponds to a ball that ends up in a bin that receives exactly $1$ ball. We call both the ball and the bin ``good'' in the sequel; each distinct element that has not been reconciled yet in the first round corresponds to a ball that ends up in a bin that receives multiple balls. We call both the ball and the bin ``bad'' in the sequel. %Note that balls and empty bins are either ``good'' or ``bad''.
%but a bin could be empty besides being ``good'' and ``bad''. 

The ``bad'' balls in the first round will be the balls to be thrown again in the second round. The ``bad'' balls in the second round will be the balls to be thrown in the third round, and so on. This process will continue for a target number of rounds (i.e., $r$ round), or until the group pair is completely reconciled, which is verifiable by the checksum (\autoref{alg:single_round_pbs} of \autoref{step:terminate_condition}). In all rounds, how the balls are thrown into $n$ bins follows the same balls-into-bins probability model. Note that the balls are thrown using a different hash function in each round, so the number of ``bad'' balls in a round
%(i.e., the number of balls to be thrown in the $(i+1)$-th round) 
only depends on the number of ``bad'' balls to start with in the round and is independent of the history
 of how these balls were placed into the $n$ bins in the previous rounds. 
Therefore, the process of how the number of balls to be thrown evolves round after round 
%the number of balls to be thrown round after round 
is a Markov chain, in which each state is defined as the number of balls to be thrown. 
%Hence, the dynamics of the number of balls to be thrown in each round can be modeled as a Markov chain, in which each state is defined as the number of balls to be thrown. {\bf a little bit wordy, need advice on how to shrink it.}

In the Markov chain, a transition from state $i$ to state $j$ ($i\geq j$) means $j$ out of $i$ balls are ``bad'' balls (the other $i-j$ balls are ``good'' balls). The ``desirable state'' for PBS is state $0$, the {\it absorbing state} in this Markov chain, which is the state that all distinct elements are successfully reconciled. For our analysis, the only probability that we are concerned with is $Pr[x\!\xrsquigarrow{r}\! 0]$, the probability that starting with $x$ ``bad'' balls, the process ends up with $0$ ``bad'' ball after $r$ rounds.
% reaches the absorbing state (i.e., state $0$) within $r$ transitions. 
It is also the success probability for a single group (starting with $x$ distinct elements and successfully reconciled within $r$ rounds). $Pr[x\!\xrsquigarrow{r}\! 0]$ can easily calculated given $M$, the $(t+1)\times (t+1)$ transition matrix of the Markov chain, as 
%, where $M(i,j)$ (i.e., the entry in the $i^{th}$ row and the $j^{th}$ column of $M$) is the probability of transition from state $i$ to state $j$ for $i,j = 0,1,...,t$
$\big{(}M^r\big{)}(x,0)$, the entry in the $x$-th row and the $0$-th column of the matrix, that is $M^r$. Here we slightly abuse the row / column indices of a $(t+1)\times (t+1)$ matrix from $1,2,...,t+1$ to $0,1,...,t$, since the state of the Markov chain ranges from $0$ to $t$. The calculation to obtain $M$ is not trivial and will be elaborated in \autoref{sec:compute_M}. For the moment, we assume $M$ has been computed and therefore we can compute $Pr[x\!\xrsquigarrow{r}\! 0]$ for $x=1,2,...,t$, $r\in\mathbb{N}^+$. 

\subsection{Tail Bound Analysis for Each Group Pair}\label{sec:tail_bound_per_group}

% ==========
% {\bf The following may be useful in explaining why it is a Markov chain:} [Note there is no need to distinguish these four cases in calculating the ``transitioning out" probability (i.e., from state 6 to a small state say State 0), because the next round of balls-into-bins operation uses a different hash function independent of that used in the current round, and consequently how these 6 bad balls are split in the current round have no bearing on that in the next round.]  {\bf unless you have done so earlier}
% ==========

The tail bound analysis of each group pair 
As we explained in \autoref{subsec:protocol2}, $\delta_1$, the number of distinct elements in group pair $1$, is a random variable that follows a Binomial distribution $Binomial(d,1/g)$. So the probability that group pair $1$ is successfully reconciled in $r$ rounds is $\sum_{x=0}^d Pr[\delta_1\!=\!x]\cdot Pr[x\!\xrsquigarrow{r}\! 0]$, where $Pr[x\!\xrsquigarrow{r}\! 0]=\big{(}M^r\big{)}(x,0)$. 
%, where $\mathcal{B}(\cdot;d,1/g)$ is the probability mass function (PMF) of $Binomial(d,1/g)$. 
To ease computation, we slightly underestimate this probability by assuming $Pr[x\!\xrsquigarrow{r}\! 0]=0$ when $x>t$. 
% (i.e., assume group pair $1$ cannot be reconciled if $\delta_1>t$, discussed in \autoref{sec:BCH_exception}). 
The loss of this underestimation is very tiny for the following reason: $Pr[\delta_1\!=\!x]$, the ``coefficient'' of $Pr[x\!\xrsquigarrow{r}\! 0]$, is very small when $x>t$, since $\delta_1$ is a Binomial random variable with mean of $\delta$ while $x$ is larger than $t$, which is roughly $2$ to $3$ times of $\delta$. We denote this underestimated probability as $\alpha$ (i.e., $\alpha=\sum_{x=0}^t Pr[\delta_1\!=\!x]\cdot Pr[x\!\xrsquigarrow{r}\! 0]$), which is a tight tail bound of the success probability of group pair $1$. $\alpha$ is also a tight tail bound for all other group pairs, since $\delta_1,\delta_2,...,\delta_g$ follows the same distribution. 

%$Pr[x\!\xrsquigarrow{r}\! 0]$ is a function of $n$ for given $x$ and $r$, so $\alpha=\alpha(n,t)$ is a function of $n$ and $t$ for arbitrary $d$, $r$, and $g$. 

\subsection{Tail Bound Analysis for All Group Pairs}\label{sec:times2bound}

Given $\alpha$, the tail bound of the probability that a group pair is successfully reconciled in $r$ rounds, we can easily derive a tail bound of $\alpha^g=1-(1-\alpha^g)$ for the probability that all group pairs are completely reconciled in $r$ rounds ($1-\alpha^g$ is the failure probability, which is usually tiny), since the set reconciliation process on group pairs are independent with each other. However, this tail bound is not rigorous,
%since $d_1, d_2,...,d_g$ have a weak correlation that $\sum_{i=1}^g d_i=d$.
since $\delta_1, \delta_2,...,\delta_g$ are not strictly independent and have a relation that $\sum_{i=1}^g \delta_i=d$. 
%Fortunately, we have Times-2-Bound (Theorem 1 in \cite{hua2008rank}) to decouple the weak correlation and give us a rigorous tail bound of $1-2(1-\alpha^g)$ for the probability of all group pairs. 
However, we can use Corollary 5.11 in \cite{upfal2005probability} to
% decouple the weak correlation and 
obtain a rigorous tail bound of $1-2(1-\alpha^g)$ for the success probability of all group pairs. This rigorous tail bound is very tight and only doubles the tiny failure probability of the unrigorous tail bound: For example, if the unrigorous tail bound of the success probability of all group pairs is $0.9999$ ($0.0001$ failure probability), then the rigorous tail bound will be $0.9998$ ($0.0002$ failure probability). This rigorous tail bound of $1-2(1-\alpha^g)$ will be used in parameter settings. 

\subsection{How to compute \texorpdfstring{\larger\boldmath{$M$}}{M}}\label{sec:compute_M}

In this section, we describe how to compute the transition matrix $M$ in details. Note that calculating an arbitrary transition probability $M(i,j)$ is not straightforward, since each state $j$ (after-transition state) with $j>3$ in the Markov chain is a {\it composite state}, which consists of a huge number of {\it atom states}. Only the transition probability from state $i$ to any atom state of state $j$ can be directly computed. $M(i,j)$ is basically the summation of all the transition probabilities from state $i$ to each of the atom states of state $j$. 

Each atom state of state $j$ is, in combinatorics terms, {\it a permutation of a combination of $j$}, which here corresponds to how these $j$ balls are placed into the $n$ bins.  For a simple example, when $j = 4$ and $n = 7$, the vector $(2, 0, 0, 0, 0, 2, 0)$ is such an atom state, which corresponds to these $7$ bins (in a predefined order such as the natural order) have $2, 0, 0, 0, 0, 2,$ and $0$ ``bad'' balls in it respectively. The transition probability from state $i$ to such an atom state can be directly computed. The problem is that the number of atom states (permutations of combinations) grow exponentially with the number of balls $j$. 
%To obtain $M(i,j)$, we have to compute all transition probabilities from the (pre-transition) state $i$ to each of the atom states of state $j$ and sum them up. 

We notice that we can break each composite state into a much small number of coarse-grained sub-states, each of which may still contain a large number of atom states. Although the transition probability from state $i$ to any sub-state is still a summation formula and hard to compute, we discover a recurrence relation among these transition probabilities, so we can compute them using dynamic programming. 
% We overcome this problem by grouping the huge number of atom states into a smaller number of coarse-grained sub-states first, then computing the transition probability from the (pre-transition) state $i$ to any sub-states of state $j$. Although each sub-state still consists of many atom states and the transition probability to a sub-state is still hard to compute directly, we discover a recurrence relation among these transition probabilities, so we can compute them using Dynamic Programming.



%as far as the calculation of the transition probability from a (larger) state $i$ $(>j)$ to $j$ is concerned. 
% To calculate the probability, we have to break the composite state $j$ down into ``atom'' states, calculate the transition probability from state $i$ to each of the ``atom'' states (which can be directly calculated), and then add them up. {\bf Note that we always view state $i$ (pre-transition state) as a {\it simple state}, since how the $i$ balls are placed into $n$ bins only depends on the hash function.}

% Each composite state $j$ can be broken down into atom states based on how these $j$ bad balls are placed into the $n$ bins. For example, state $6$ consists of $4$ atom states. The first one is $6 = 6$, where all $6$ bad balls are in the same bad bin. The second one is $6 = 2 + 4$ where, out of the $6$ bad balls, four are in one bad bin and the other two are in the other bad bin.  Similarly, the other two atom states are $6 = 3 + 3$ and $6 = 2 + 2 + 2$. The transition probability from state $i$ to any atom state can be directly calculated, but the problem is that the number of atom states grows exponentially with the number of ``bad'' balls $j$.

% We notice that we can break each composite state into a small number of coarse-grained sub-states, each of which may still contain a large number of atom states. The transition probability from a (larger) state $i$ to any sub-state is still hard to compute. However, there is a recurrence relation among them, so we can compute the transition probabilities from any state to any sub-state using Dynamic Programming. 

State $j$ is broken down into at most $j$ sub-states, which are defined as follows:
%The sub-states of state $j$ is defined as follows: 
let state $(j,k)$ denote the sub-state of state $j$ that the $j$ ``bad'' balls end up to occupy exactly $k$ ``bad'' bins. Then the composite state $j$ is partitioned into state $(j,1)$, state $(j,2)$, $...$, state $(j,j)$. We slightly abuse the notation and let $M(i,j,k)$ denote the probability of transition from state $i$ to state $(j,k)$, then we have 

\begin{equation}\nonumber
    M(i,j) = \sum_{k=1}^{j} M(i,j,k)
\end{equation}

%{\bf explain the range of $k$ could be distracting, so I just leave it as it is.}
To obtain $M$, it is sufficient to compute $M(i,j,k)$ for $\forall i,j,k=0,1,...,t$. Note that the state transition resulting from throwing one ball after another is also a Markov chain, in which state $(i,j,k)$ is defined as $j$ ``bad'' balls ending up into $k$ ``bad'' bins after throwing $i$ balls into $n$ bins. In this Markov chain, 
%throwing one more ball can transition state $(i,j,k)$ to three possible states depending on the $(i+1)$-th ball ending up in (1) a ``good'' bin; (2) a ``bad'' bin; or (3) an empty bin. The first case happens with probability $(i-j)/n$, results in $2$ additional ``bad'' balls and $1$ additional ``bad'' bin (i.e., transition to state $(i+1,j+2,k+1)$). The second and third cases transition to state $(i+1,j+1,k)$ and state $(i+1,j,k)$ respectively with probability $k/n$ and $1-(i-j+k)/n$. In the opposite direction, 
state $(i+1,j,k)$ can only be transitioned from (1) state $(i,j-2,k-1)$ when the $(i+1)$-th ball lands in a ``good'' bin; (2) state $(i,j-1,k)$ when the $(i+1)$-th ball lands in a ``bad'' bin; and (3) state $(i,j,k)$ when the $(i+1)$-th ball lands in an empty bin. It gives us a recurrence relation that $M(i+1,j,k)$ equals to

%The second case happens with probability $k/n$ and results in state $(i+1,j+1,k)$. The third case happens with probability $1-(i-j+k)/n$ and results in state $(i+1,j,k)$. In the opposite direction, state $(i+1,j,k)$ can be transitioned from (1) state $(i,j-2,k-1)$ with probability $(i-j+2)/n$; (2) state $(i,j-1,k)$ with probability $k/n$; or (3) state $(i,j,k)$ with probability $1-(i-j+k)/n$. It gives us a recurrence relation that $P(i+1,j,k)$ equals to

\begin{equation}\nonumber
    \frac{i\!-\!j\!+\!2}{n}\cdot M(i,j\!-\!2,k\!-\!1)+\frac{k}{n}\cdot M(i,j\!-\!1,k)+(1\!-\!\frac{i\!-\!j\!+\!2}{n})\cdot M(i,j,k)
\end{equation}

The three terms in this formula corresponds to the above three possible transitions. The computational complexity for each $M(i,j,k)$ is $O(1)$ via dynamic programming, so the overall compuational complexity is $O(t^3)$ (for $t^3$ entries). To compute $M(i,j,k)$ for $\forall i,j,k=0,1,...,t$ via dynamic programming, we also need to compute the transition probabilities in the base cases as follows:  
%Combining with the following probabilities in base cases, we can compute $M(i,j,k)$ for $\forall i,j,k=0,1,...,t$ using Dynamic Programming and obtain $M$:

\begin{align}
M(0,j,k) =& \left\{ \begin{array}{ccl}
1, & \mbox{if }
 j=k=0 \\ 0, & \mbox{otherwise} 
\end{array}\right.\nonumber\\
M(i,0,k) =& \left\{ \begin{array}{ccl}
\binom{n}{i}/n^i, & \mbox{if }
 k=0 \\ 0, & \mbox{otherwise} 
\end{array}\right.\nonumber\\
M(i,j,0) =& \left\{ \begin{array}{ccl}
1, & \mbox{if }
 j=0 \\ 0, & \mbox{otherwise} 
\end{array}\right.\nonumber
\end{align}

% PBS reconciles the distinct elements gradually round by round. This is the ``piecewise decodability'' mentioned in \autoref{sec:intro_oursolution}. We use the following example to describe it in details: 
% Given two sets with $10$ distinct elements, in the first round, PBS tries to reconcile the $10$ distinct elements and say $6$ out of the $10$ distinct elements are successfully reconciled. Then the $6$ reconciled distinct elements are removed and PBS tries to reconcile the remaining $4$ distinct elements in the second round. Say $2$ out of the $4$ remaining distinct elements are successfully reconciled, and that leaves $2$ remaining distinct elements to be reconciled in the third round, so on so force. 
% % Given two sets $A$, $B$ with $10$ distinct elements, in the first round, PBS hashes them into $7$ distinct subset pairs. $6$ distinct elements are hashed into $6$ distinct subset pairs, and the other $4$ distinct elements are hashed into the same subset pair. Then the former $6$ distinct elements are successfully reconciled in the first round and the later $4$ distinct elements remain to be reconciled in the second round, which are hashed into $3$ distinct subset pairs (under a different hash function). $2$ remaining distinct elements are hashed into $2$ distinct subset pairs, and the other $2$ remaining distinct elements are hashed into the same subset pair. Then the former $2$ remaining distinct elements are successfully reconciled in the second round and the later $2$ remaining distinct elements remain to be reconciled in the third round, so on so force. 
% The dynamics of the number of remaining distinct elements (i.e., $10\leadsto 4\leadsto 2\leadsto \cdots$ in the example) is in nature a Markov chain, which will be elaborated and analyzed in \autoref{sec:single_markov} to derive a tight tail bound of the probability that all distinct elements are reconciled in $r$ rounds. 
\begin{comment}
+++++++++++

The only problem left to obtain $Pr[d\xrsquigarrow{r} 0]$ is how to compute $M$, which is not straightforward, since each state $j$ with $j>3$ in the Markov chain is a composite state as far as the calculation of the transition probability from a (larger) state $i$ $(>j)$ to $j$ (i.e., ``transitioning into'') is concerned.   {\bf You need to explain why it is not straightforward:  The reason you offer is not
the direction reason.  Instead you may say that "the transition probability between these composite states cannot be directly calculated" ...  to calculate it we have to break it down into "atom" states}

Each composite state $i$ can be broken down into atom states as follows.  Each simple state is, in combinatorics terms, {\it a permutation of a combination of $i$}, which here corresponds to 
how these $i$ balls are ``divided up" by the $n$ bins.   {\bf Liang, Read Mitzenmacher and Upfal book
for a better word for "divided up"}
For a simple example, when $i = 4$ and $n = 7$, the vector (1, 0, 1, 0, 0, 2, 0) is such a simple state, which corresponds to these 7 bins (in a predefined order such as the natural order) 
have 1, 0, 1, 0, 0, 2, and 0 balls in it respectively.   The transition probability between any two atom states can be ...    but the problem is that the number of atom states 
(permutations of combinations) grow exponentially with the number of balls $i$.

Consider two states i1 and i2 each broken down into millions of atom states.  Then the transition probability between these states is the summation of the trillions (= millions * millions) of 
transition probabilities between atom states of i1 and atom states of i2.  

The good thing is that the transition probability matrix among the (humongous number of atom states) induces a "subproblem structure ????", which leads to the recurrence relation, 
dynamic programming.   

We notice that we can break each state into a small number of coarse-grained substates, each of which may still contain a large number of atom states.  The transition probability 
between any two such substates are still hard to compute.  However, there is a recurrence relation among them ...

+++++++++++

To solve the problem, we partition the composite state into sub-states, so that the transition probability to the composite state is the summation of the transition probabilities to each of the sub-states. On the other hand, the transition probabilities to the sub-state have a recurrence relation and can be computed using Dynamic Programming. 

======================================

Note that every state $j$ with $j > 3$ in the Markov chain is a composite state as far as the calculation of the transition probability from a (larger) state $i > j$ to $j$ (i.e., ``transitioning into").  For example, State 6 contains 4 different cases. The first case is $6 = 6$, where all 6 bad balls are in the same bad bin. The second case is $6 = 2 + 4$ where, out of the 6 bad balls, four are in one bad bin and the other two are in the other bad bin.  Similarly, the other two cases are $6 = 3 + 3$ and $6 = 2 + 2 + 2$. Note there is no need to distinguish these four cases in calculating the ``transitioning out" probability (i.e., from state 6 to a small state say State 0), because the next round of balls-into-bins operation uses a different hash function independent of that used in the current round, and consequently how these 6 bad balls are split in the current round have no bearing on that in the next round. 

Building on the example above, we now consider $m_{9,6}$, the transition probability from State $9$ to State $6$ (throwing 9 balls into 255 bins and ending up with 6 bad balls).  $m_{9,6}$ is simply the sum of the probabilities of these four cases, each of which has a very different formula than the others.  In general, the number of such cases, and hence the number of individual probability terms to be added up to arrive at the transition matrix element $m_{i,j}$, grows exponentially with the value of $j$. This does not however make it difficult to calculate the values of $M$, because there is a recursive structure, among the values of the matrix elements $m_{i,j}$, that can be exploited using dynamic programming, as will be elaborated shortly.

To simplify our analysis, we split each composite state into sub-composite states based on the number of nonempty bins: Let State $(j,k)$ denotes the sub-composite state with $j$ remaining distinct elements and $k$ nonempty bins, which is also a substate of State $j$. Let $m_{i,j}^{(k)}$ denote the probability of transition from State $i$ to State $(j,k)$, which is also the probability that after throwing $i$ balls uniformly and independently into $n$ bins, $i-j$ bins are ``good'' bins and $k$ bins are nonempty bins (thus $k-(i-j)$ bins are ``bad'' and $n-k$ bins are empty). The probability of transition to a composite state is simply the summation of the probabilities of the transitions to corresponding sub-composite states:

To obtain the transition matrix $M$, it is sufficient to compute $m^{(k)}_{i,j}$, which can be exploited using dynamic programming. Note that the balls-and-bins model itself can be considered as a Markov chain, in which a recursive relation exists: After throwing $i$ balls into $n$ bins, throwing one more ball randomly could be: (1) Into an empty bin and turn it to a ``good'' bin; (2) Into a ``good'' bin and turn it to a ``bad'' bin with two balls; or (3) Into a ``bad'' bin and keep it as the same. Mathematically, we have $m^{(k)}_{i+1,j}$ equals to


====================================
\end{comment}



==> section/theoretical_analysis_seperate0227.tex <==
\section{Theoretical Analysis}\label{sec:tail_bound}

\subsection{Motivation (new section)}\label{sec:motivation_theoretical_analysis}

In PBS, the set reconciliation process of the group pairs are independent with each other, and each group pair runs as many rounds of PBS-for-small-$d$ as needed to reconcile all distinct elements in it. Therefore, different group pairs may take different number of rounds to be successfully reconciled. The total number of rounds to reconcile all group pairs, denoted as $R$, is their maximum.
An obvious goal related to $R$ is, given the total ``budget'' of communication overhead, find the optimal parameter settings for PBS that {\it stochastically minimize} $R$. 

This optimization is hard to achieve if not possible. Instead, we propose a more optimizable goal, which is roughly the dual of the previous optimization problem, as follows: Given a {\it target success probability} $p_0$ and a {\it target number of rounds} $r$, find the optimal parameter settings that minimize the overall communication overhead under the constraint that the {\it success probability}, the probability that all distinct elements are reconciled, within $r$ rounds is at least $p_0$. 

Towards this optimizable goal, we propose an analytical framework for the set reconciliation process of PBS. From this framework, we can obtain a fairly accurate estimation of the success probability within an arbitrary number of rounds under any given parameter settings. Based on it, we can reach the optimizable goal, as we will elaborate in \autoref{sec:parameter_settings}. This analytical framework also enables us to analyze other performance metrics of PBS, as we will show in \autoref{sec:vary_r} and \autoref{sec:piecewise_decodability}.



% In this section, we provide a theoretical analysis (analytical framework) for the set reconciliation process of PBS and establish a tight tail bound on the {\it success probability} within $r$ rounds under arbitrary parameter settings of $n$, $\delta$, and $t$. This analytical framework has several applications on parameter settings and analyzing the properties of PBS that we will elaborate in \autoref{sec:application_analysis}.

% Note that the set reconciliation process of the group pairs are independent with each other, and each group pair runs as many rounds of PBS-for-small-$d$ as needed to reconcile all distinct elements in it. Therefore, different group pairs may need different number of rounds to be successfully reconciled. Intuitively, we want all group pairs to be successfully reconciled in only a few rounds (say $3$) with high probability (say $99\%$). Hence, when tuning parameters (to be discussed in \autoref{sec:parameter_settings}), we set a {\it target success probability} $p_0$ combined with a {\it target number of rounds} $r$ as the {\it paramenter setting requirement}, which aims to ensure that the {\it success probability}, the probability that all distinct elements (of all group pairs) are reconciled, within $r$ rounds to be at least $p_0$. 

% {\bf Normally, to achieve the same target success probability within fewer rounds (smaller $r$), PBS need more resources (e.g., larger $n$, $t$) for the ideal case happening with higher probability (fewer exceptions happen and need to be handled in later rounds), as we will explain in \autoref{sec:vary_r}.}

% On one hand, this tail bound gives us a theoretical guarantee on the success probability under specific parameter settings. On the other hand, given a parameter setting requirement (i.e., a target success probability $p_0$ within $r$ rounds), we can use the tail bound to find all feasible parameter settings that satisfy the requirement, then select the optimal parameter settings among them that have the lowest communication overhead. {\bf This analysis also provides other theoretical results for PBS, such as the expected number (percentage) of the distinct elements would be reconciled in the each round (``piecewise decodability'', to be shown in \autoref{sec:piecewise_decodability})}%In this section, we continue to assume $d$ is precisely known. 

% For simplicity, we ignore the small probability event that a type (\RN{2}) event happens, in which the incurred ``fake'' distinct element is not successfully verified by \autoref{alg:verification} (mentioned in \autoref{subsec:exception_hash_partition}). As we discussed earlier, this event happens with a tiny probabilty that is in order of $10^{-7}$. Hence, ignoring this event barely compromises the accuracy of our analysis. 

%\subsection{Analysis of a simple case}\label{sec:single_markov}
%\subsection{The Process Under PBS}\label{sec:single_markov}
\subsection{Markov Chain Modeling of Multi-round PBS Process}\label{sec:single_markov}

Recall from PBS-for-small-$d$, each of the $d$ balls (distinct elements) are thrown uniformly and randomly into one of the $n$ bins (subset pairs) in the first round. Each ball that ends up in a bin that receives exactly $1$ ball, corresponding to a successfully reconciled distinct element, is a ``good'' ball and will not be thrown again in latter rounds. Each ball that ends up in a bin that receives multiple balls, corresponding to a distinct element that has not been reconciled yet, is a ``bad'' ball and will be thrown again in the second round to try to turn into a ``good'' one. The process of throwing ``bad'' balls round after round continues until all balls end up to be ``good''. 

In this section, we study a generic case that starting with $x$ $(\leq t)$ balls, how the number of ``bad'' balls that remain evolves round after round. This generic case arises from the set reconciliation process of each group pair in PBS. Let $B_k$ denote the number of ``bad'' balls that remain after the $k$-th round for $k=1,2,...$. In the process, $B_k$ also denotes the number of balls to be thrown in the $(k+1)$-th round. Define $B_0\triangleq x$. Note that the balls are thrown using different hash functions in each round, so $B_{k}$, the number of ``bad'' balls that remain after the $k$-th round, only depends on $B_{k-1}$, the number of balls are thrown in the $k$-th round, and is independent of the history (i.e., $B_0,B_1,B_2,...,B_{k-1}$). Therefore, $\{B_k\}_{k=0}^\infty$ is a Markov chain, in which each state is defined as the number of ``bad'' balls that remain. 
%, in which the distribution of $B_{k+1}$ conditioned upon $B_k$ is independent of $B_1,B_2,...,B_{k-1}$. 
The ``desirable'' state of this Markov chain for PBS is state $0$ (the absorbing state), in which all balls end up to be ``good''. 

Let $M$ denote the $(t+1)\times (t+1)$ transition matrix of the Markov chain. Here we slightly abuse the row / column indices of a $(t+1)\times (t+1)$ matrix from $1,2,...,t+1$ to $0,1,...,t$, since the state of the Markov chain ranges from $0$ to $t$. The calculation to obtain $M$ is not trivial and will be elaborated in \autoref{sec:compute_M}. For the moment, we assume $M$ has been computed.

% In this section, we study a generic case that starting with $x$ $(\leq t)$ balls, how the number of balls to be thrown evolves in this process. This generic case arises from the set reconciliation process of each group pair in PBS. Let $B_k$ denote the number of balls to be thrown in the $k$-th round for $k=1,2,...$, where $B_1=x$. Note that the balls are thrown using different hash functions in each round, so $B_{k+1}$, the number of ``bad'' balls that remain after the $k$-th round, only depends on $B_{k}$, the number of balls are thrown in the $k$-th round, and is independent of the history (i.e., $B_1,B_2,...,B_{k-1}$). Therefore, $B_1, B_2,...$ is a Markov chain, in which each state is defined as the number of balls to be thrown.
% %, in which the distribution of $B_{k+1}$ conditioned upon $B_k$ is independent of $B_1,B_2,...,B_{k-1}$. 
% The ``desirable'' state of this Markov chain for PBS is state $0$ (the absorbing state), in which all balls end up to be ``good''. 

For our analysis, the only probability that we are concerned with is $Pr[x\!\xrsquigarrow{r}\! 0]$, the probability that starting with $x$ ``bad'' balls, the process ends up with $0$ ``bad'' ball after $r$ rounds. 
%It is also the success probability within $r$ rounds. 
$Pr[x\!\xrsquigarrow{r}\! 0]$ can be easily calculated as 
%, where $M(i,j)$ (i.e., the entry in the $i^{th}$ row and the $j^{th}$ column of $M$) is the probability of transition from state $i$ to state $j$ for $i,j = 0,1,...,t$
$\big{(}M^r\big{)}(x,0)$, the entry in the $x$-th row and the $0$-th column of the matrix, that is $M^r$. Note that even without using this Markov chain modeling, $Pr[x\!\xrsquigarrow{1}\! 0]$ can be easily computed as a closed-form expression, as we described in \autoref{sec:hash_partition}. However, $Pr[x\!\xrsquigarrow{r}\! 0]$ cannot be expressed as a closed-form as in when in \autoref{sec:hash_partition} $r\geq 2$. 
%In general, $Pr[d\!\xrsquigarrow{r}\! y]$ is difficult to compute when $r\geq 2$ and $y\geq 1$. 
The Markov chain modeling solves this problem by mapping the transition probability $Pr[x\!\xrsquigarrow{r}\! y]$ after $r$ rounds in the process to the $r$-step transition probability $\big{(}M^r\big{)}(x,y)$ of the Markov chain.

Recall that in PBS-for-small-$d$, given two sets with $d$ distinct elements, PBS-for-small-$d$ successfully reconciles all distinct elements within $1$ round if and only if the ideal case happens. The probability for the ideal situation to occur is $Pr[d\!\xrsquigarrow{1}\! 0]$ (e.g., $0.96$ when $d = 5$ and $n=255$ as mentioned in \autoref{sec:smalld}). It can be easily computed even without using this Markov chain modeling. In general, $Pr[d\!\xrsquigarrow{r}\! y]$ is difficult to compute when $r\geq 2$ and $y\geq 1$. 

% For our analysis, the only probability that we are concerned with is $Pr[x\!\xrsquigarrow{r}\! 0]$, the probability that starting with ``bad'' balls, the process ends up with $0$ ``bad'' ball after $r$ rounds. 
% %It is also the success probability within $r$ rounds. 
% $Pr[x\!\xrsquigarrow{r}\! 0]$ can be easily calculated given $M$, the $(t+1)\times (t+1)$ transition matrix of the Markov chain, as 
% %, where $M(i,j)$ (i.e., the entry in the $i^{th}$ row and the $j^{th}$ column of $M$) is the probability of transition from state $i$ to state $j$ for $i,j = 0,1,...,t$
% $\big{(}M^r\big{)}(x,0)$, the entry in the $x$-th row and the $0$-th column of the matrix, that is $M^r$.. Here we slightly abuse the row / column indices of a $(t+1)\times (t+1)$ matrix from $1,2,...,t+1$ to $0,1,...,t$, since the state of the Markov chain ranges from $0$ to $t$. The calculation to obtain $M$ is not trivial and will be elaborated in \autoref{sec:compute_M}. For the moment, we assume $M$ has been computed and therefore we can compute $Pr[x\!\xrsquigarrow{r}\! 0]$ for $x=1,2,...,t$, $r\in\mathbb{N}^+$. 
\subsection{Preciseness of Markov Chain Modeling}

This Markov chain captures all the details about the set reconciliation process of PBS in each group pair except for one event, that is, the ``fake'' distinct element incurred from a type (\RN{2}) event is not successfully verified by \autoref{alg:verification}. Such an element, if captured in the generic case, would increase the number of balls to be thrown in the next round by $1$ and therefore change the transition-into state (say the transition changes from state $i\rightarrow j$ to state $i\rightarrow j+1$). However, as we explained in \autoref{subsec:exception_hash_partition}, this event happens with a tiny probabilty that is in order of $10^{-7}$. Ignoring such a small probability event barely changes the transition probability matrix $M$ of the Markov chain and therefore has negligible effect of our analysis. 

In the Markov chain, we only analyze the case in which the number of balls to start with is no more than the error-correction capability of the BCH code (i.e., $x\leq t$). For the case where $x>t$, the analysis of the set reconciliation process becomes much more complicated, since such a group pair could be partitioned into $3$ sub-group-pairs (e.g., in the ideal case) as we described in \autoref{alg:3_way_partition} and each of them will be independently reconciled. Instead of analyzing this complicated set reconciliation process, we simply `underestimate' $Pr[x\!\xrsquigarrow{r}\! 0]$ to be $0$ for $x>t$ in the following tail bound analysis. This `underestimation' incurs negligible loss on the tail bound, as we will explain shortly.

% The second event is, when the number of distinct elements in a group pair exceeds the error-correction capability $t$ then lead to a BCH decoding failure, the group pair will be partitioned into $3$ sub-group-pairs, each of which will be reconciled by PBS-for-small-$d$ in the next round, as we showed in \autoref{alg:3_way_partition}. To ease our analysis, we assume $Pr[x\!\xrsquigarrow{r}\! 0]=0$ when $x>t$. 
% % (i.e., assume group pair $1$ cannot be reconciled if $\delta_1>t$, discussed in \autoref{sec:BCH_exception}). 
% The loss of this underestimation is very tiny for the following reason: $Pr[\delta_1\!=\!x]$, the ``coefficient'' of $Pr[x\!\xrsquigarrow{r}\! 0]$, is very small when $x>t$, since $\delta_1$ is a Binomial random variable with mean of $\delta$ while $x$ is larger than $t$, which is roughly $2$ to $3$ times of $\delta$. We denote this underestimated probability as $\alpha$ (i.e., $\alpha=\sum_{x=0}^t Pr[\delta_1\!=\!x]\cdot Pr[x\!\xrsquigarrow{r}\! 0]$), which is a tight tail bound of the success probability of group pair $1$. $\alpha$ is also a tight tail bound for all other group pairs, since $\delta_1,\delta_2,...,\delta_g$ follows the same distribution. 

% A ball that ends up in a bin that receives exactly $1$ ball is a ``good'' ball. In the ideal case, the $d$ balls are placed into $d$ distinct bins and the corresponding $d$ distinct elements are reconciled. In general, the ideal case may not necessarily happen. Some of the distinct elements (say $d'$ out of $d$ distinct elements) may have not been reconciled yet and will be thrown in the second round, and so on. The process of how the number of balls to be thrown evolves ($d\rightarrow d'\rightarrow \cdots$) round after round can be characterized as a Markov chain model. 
===============================

In this section, we analyze the probability that an arbitrary group pair that contains exactly $x$ $(\leq t)$ distinct elements is {\it successfully reconciled} by PBS in $r$ rounds. Here we say a group pair is {\it successfully reconciled} within $r$ rounds if and only if all distinct elements in the group pair are successfully reconciled within $r$ rounds. 

As we described in \autoref{sec:multi-rounds}, in the first round of PBS, the $x$ distinct elements are hashed into $n$ subset pairs, and a distinct element is successfully reconciled if and only if it is hashed into a subset pair that contains only $1$ distinct element. 
%The successfully reconciled distinct elements in the first round are removed and the other distinct elements (i.e., the ones that have not been reconciled yet in the first round) will be hashed again in the second round using a different hash function, so on so force, until all distinct elements are successfully reconciled. 
How the $x$ distinct elements are distributed into $n$ subset pairs in the first round follows the familiar {\it balls-into-bins} probability model: Each of the $x$ balls is thrown independently and uniformly at random into one of the $n$ bins. Each successfully reconciled distinct element corresponds to a ball that ends up in a bin that receives exactly $1$ ball. We call both the ball and the bin ``good'' in the sequel; each distinct element that has not been reconciled yet in the first round corresponds to a ball that ends up in a bin that receives multiple balls. We call both the ball and the bin ``bad'' in the sequel. Note that balls and empty bins are either ``good'' or ``bad''.
%but a bin could be empty besides being ``good'' and ``bad''. 

The ``bad'' balls in the first round will be the balls to be thrown in the second round. The ``bad'' balls in the second round will be the balls to be thrown in the third round, and so on. This process will continue for a target number of rounds (i.e., $r$ round), or until the group pair is completely reconciled, which is verified by the checksum (\autoref{alg:single_round_pbs} of \autoref{step:terminate_condition}). In all rounds, how the balls are thrown into $n$ bins follows the same balls-into-bins probability model. Note that the balls are thrown using different hash functions in each round, so the number of ``bad'' balls in a round
%(i.e., the number of balls to be thrown in the $(i+1)$-th round) 
only depends on how many balls are thrown in the round and is independent of the history
 of how these balls were placed into the $n$ bins in the previous rounds. 
Therefore, the process of how the number of balls to be thrown evolves round after round 
%the number of balls to be thrown round after round 
is a Markov chain, in which each state is defined as the number of balls to be thrown. 
%Hence, the dynamics of the number of balls to be thrown in each round can be modeled as a Markov chain, in which each state is defined as the number of balls to be thrown. {\bf a little bit wordy, need advice on how to shrink it.}

In the Markov chain, a transition from state $i$ to state $j$ ($i\geq j$) means $j$ out of $i$ balls are ``bad'' balls and the other $i-j$ balls are ``good'' balls. The {\it absorbing state} of this Markov chain is state $0$, which is the ``desirable'' state that all balls are ``good'' (so that all distinct elements are successfully reconciled). 

For our analysis, the only probability that we are concerned with is $Pr[x\!\xrsquigarrow{r}\! 0]$, the probability that starting with state $x$ (initial state), the Markov chain reaches state $0$ within $r$ transitions. It is also the success probability for a single group (starting with $x$ distinct elements and successfully reconciled within $r$ rounds). $Pr[x\!\xrsquigarrow{r}\! 0]$ can easily calculated given $M$, the $(t+1)\times (t+1)$ transition matrix of the Markov chain, as 
%, where $M(i,j)$ (i.e., the entry in the $i^{th}$ row and the $j^{th}$ column of $M$) is the probability of transition from state $i$ to state $j$ for $i,j = 0,1,...,t$
$\big{(}M^r\big{)}(x,0)$, the entry in the $x$-th row and the $0$-th column of $M^r$. Here we slightly abuse the row / column indices of a $(t+1)\times (t+1)$ matrix from $1,2,...,t+1$ to $0,1,...,t$, since the state of the Markov chain ranges from $0$ to $t$. How to compute $M$ will be elaborated in \autoref{sec:compute_M}. For the moment, we assume $M$ has been computed and therefore we can compute $Pr[x\!\xrsquigarrow{r}\! 0]$ for $x=1,2,...,t$, $r\in\mathbb{N}^+$. 

For simplicity, we ignore the small probability event that a type (\RN{2}) event happens, in which the incurred ``fake'' distinct element is not successfully verified by \autoref{alg:verification} (mentioned in \autoref{subsec:exception_hash_partition}). As we discussed earlier, this event happens with a tiny probabilty that is in order of $10^{-7}$. Hence, ignoring this event barely compromises the accuracy of our analysis. 

===============================

\subsection{Tail Bound Analysis}\label{sec:times2bound}

% ==========
% {\bf The following may be useful in explaining why it is a Markov chain:} [Note there is no need to distinguish these four cases in calculating the ``transitioning out" probability (i.e., from state 6 to a small state say State 0), because the next round of balls-into-bins operation uses a different hash function independent of that used in the current round, and consequently how these 6 bad balls are split in the current round have no bearing on that in the next round.]  {\bf unless you have done so earlier}
% ==========

Recall that $\delta_1,\delta_2,...,\delta_g$ follows the same distribution. The success probability $Pr[\delta_i\!\xrsquigarrow{r}\! 0]$, when fixing other parameters, only depends on the value of $x$. WLOG, we only analyze group pair $1$ among all group pairs. The success probability of group pair $1$ within $r$ rounds is $\sum_{x=0}^d Pr[\delta_1\!=\!x]\cdot Pr[x\!\xrsquigarrow{r}\! 0]$, where $Pr[x\!\xrsquigarrow{r}\! 0]=\big{(}M^r\big{)}(x,0)$ for $x=1,2,...,t$. Here $\delta_1$, the number of distinct elements in group pair $1$, is a random variable that follows a Binomial distribution $Binomial(d,1/g)$. 

Recall that we underestimate $Pr[x\!\xrsquigarrow{r}\! 0]=0$ when $x>t$. The loss of this underestimation on the success probability of group pair $1$ is very tiny, since $Pr[\delta_1\!=\!x]$, the ``coefficient'' of $Pr[x\!\xrsquigarrow{r}\! 0]$, is very small when $x>t$: $\delta_1$ is a Binomial random variable with mean of $\delta$ while $x$ is larger than $t$, which is roughly $2$ to $3$ times of $\delta$. We denote this underestimated probability as $\alpha$ (i.e., $\alpha=\sum_{x=0}^t Pr[\delta_1\!=\!x]\cdot Pr[x\!\xrsquigarrow{r}\! 0]$), which is a tight tail bound of the success probability for group pair $1$ and for all other group pairs. 
%$\alpha$ is also a tight tail bound for all other group pairs, since $\delta_1,\delta_2,...,\delta_g$ follows the same distribution. 

We can easily derive a tail bound of $\alpha^g$ for the success probability of all group pairs within $r$ rounds, since the set reconciliation process on group pairs are independent with each other. However, this tail bound is not rigorous, since the $g$ success probabilities of the $g$ group pairs are functions of $\delta_1, \delta_2,...,\delta_g$, which are related by $\sum_{i=1}^g \delta_i=d$. Using Corollary 5.11 in \cite{upfal2005probability}, we can derive a rigorous tail bound of $1-2(1-\alpha^g)$ for the success probability of all group pairs within $r$ rounds. This rigorous tail bound is very tight and only doubles the tiny failure probability of the unrigorous tail bound (i.e., $1-\alpha^g$): For example, if the unrigorous tail bound of the success probability of all group pairs is $0.9999$ ($0.0001$ failure probability), then the rigorous tail bound will be $0.9998$ ($0.0002$ failure probability). This rigorous tail bound of $1-2(1-\alpha^g)$ will be used in parameter settings. 


===============================
To ease computation, we slightly underestimate this probability by assuming $Pr[x\!\xrsquigarrow{r}\! 0]=0$ when $x>t$. 
% (i.e., assume group pair $1$ cannot be reconciled if $\delta_1>t$, discussed in \autoref{sec:BCH_exception}). 
The loss of this underestimation is very tiny for the following reason: $Pr[\delta_1\!=\!x]$, the ``coefficient'' of $Pr[x\!\xrsquigarrow{r}\! 0]$, is very small when $x>t$, since $\delta_1$ is a Binomial random variable with mean of $\delta$ while $x$ is larger than $t$, which is roughly $2$ to $3$ times of $\delta$. We denote this underestimated probability as $\alpha$ (i.e., $\alpha=\sum_{x=0}^t Pr[\delta_1\!=\!x]\cdot Pr[x\!\xrsquigarrow{r}\! 0]$), which is a tight tail bound of the success probability of group pair $1$. $\alpha$ is also a tight tail bound for all other group pairs, since $\delta_1,\delta_2,...,\delta_g$ follows the same distribution. 
%group pair $i$, defined as the probability that all the distinct elements in the group pair are reconciled, within $r$ rounds, is equal to $Pr[\delta_i\!\xrsquigarrow{r}\! 0]$. 

As we explained in \autoref{subsec:protocol2}, $\delta_1$, the number of distinct elements in group pair $1$, is a random variable that follows a Binomial distribution $Binomial(d,1/g)$. So the probability that group pair $1$ is successfully reconciled in $r$ rounds is $\sum_{x=0}^d Pr[\delta_1\!=\!x]\cdot Pr[x\!\xrsquigarrow{r}\! 0]$, where $Pr[x\!\xrsquigarrow{r}\! 0]=\big{(}M^r\big{)}(x,0)$. 
%, where $\mathcal{B}(\cdot;d,1/g)$ is the probability mass function (PMF) of $Binomial(d,1/g)$. 
To ease computation, we slightly underestimate this probability by assuming $Pr[x\!\xrsquigarrow{r}\! 0]=0$ when $x>t$. 
% (i.e., assume group pair $1$ cannot be reconciled if $\delta_1>t$, discussed in \autoref{sec:BCH_exception}). 
The loss of this underestimation is very tiny for the following reason: $Pr[\delta_1\!=\!x]$, the ``coefficient'' of $Pr[x\!\xrsquigarrow{r}\! 0]$, is very small when $x>t$, since $\delta_1$ is a Binomial random variable with mean of $\delta$ while $x$ is larger than $t$, which is roughly $2$ to $3$ times of $\delta$. We denote this underestimated probability as $\alpha$ (i.e., $\alpha=\sum_{x=0}^t Pr[\delta_1\!=\!x]\cdot Pr[x\!\xrsquigarrow{r}\! 0]$), which is a tight tail bound of the success probability of group pair $1$. $\alpha$ is also a tight tail bound for all other group pairs, since $\delta_1,\delta_2,...,\delta_g$ follows the same distribution. 

%$Pr[x\!\xrsquigarrow{r}\! 0]$ is a function of $n$ for given $x$ and $r$, so $\alpha=\alpha(n,t)$ is a function of $n$ and $t$ for arbitrary $d$, $r$, and $g$. 

% \subsection{Tail Bound Analysis for All Group Pairs}\label{sec:times2bound}

Given $\alpha$, the tail bound of the probability that a group pair is successfully reconciled in $r$ rounds, we can easily derive a tail bound of $\alpha^g=1-(1-\alpha^g)$ for the probability that all group pairs are completely reconciled in $r$ rounds ($1-\alpha^g$ is the failure probability, which is usually tiny), since the set reconciliation process on group pairs are independent with each other. However, this tail bound is not rigorous,
%since $d_1, d_2,...,d_g$ have a weak correlation that $\sum_{i=1}^g d_i=d$.
since $\delta_1, \delta_2,...,\delta_g$ are not strictly independent and have a relation that $\sum_{i=1}^g \delta_i=d$. 
%Fortunately, we have Times-2-Bound (Theorem 1 in \cite{hua2008rank}) to decouple the weak correlation and give us a rigorous tail bound of $1-2(1-\alpha^g)$ for the probability of all group pairs. 
However, we can use Corollary 5.11 in \cite{upfal2005probability} to
% decouple the weak correlation and 
obtain a rigorous tail bound of $1-2(1-\alpha^g)$ for the success probability of all group pairs. This rigorous tail bound is very tight and only doubles the tiny failure probability of the unrigorous tail bound: For example, if the unrigorous tail bound of the success probability of all group pairs is $0.9999$ ($0.0001$ failure probability), then the rigorous tail bound will be $0.9998$ ($0.0002$ failure probability). This rigorous tail bound of $1-2(1-\alpha^g)$ will be used in parameter settings. 
===============================

\subsection{How To Compute \texorpdfstring{\larger\boldmath{$M$}}{M}}\label{sec:compute_M}

In this section, we describe how to compute the transition matrix $M$ in details. Note that calculating an arbitrary transition probability $M(i,j)$ is not straightforward, since each state $j$ with $j>3$ in the Markov chain is a {\it composite state}, which consists of a huge number of {\it atom states}. Only the transition probability from state $i$ to any atom state of state $j$ can be stated as a closed-form expression (more precisely, a multinomial formula) and therefore can be computed straightforwardly. $M(i,j)$ is the summation of all the transition probabilities from state $i$ to each of the atom states of state $j$. While this may not sound like a problem, the number of atom states grow exponentially with $j$, so the computation of $M(i,j)$ could be extremely complicated for large $j$.

Each atom state of state $j$ is, in combinatorics terms, {\it a permutation of a combination of $j$}, which here corresponds to how these $j$ balls are placed into the $n$ bins.  For a simple example, when $j = 4$ and $n = 7$, the vector $(2, 0, 0, 0, 0, 2, 0)$ is such an atom state, which corresponds to these $7$ bins (in a predefined order such as the natural order) have $2, 0, 0, 0, 0, 2,$ and $0$ ``bad'' balls in it respectively. Although the transition probability from state $i$ to each such atom state is computable, the number of atom states (permutations of combinations) grow exponentially with the number of balls $j$. 

%The transition probability from state $i$ to such an atom state is a closed-form expression and computable. The problem is that the number of atom states (permutations of combinations) grow exponentially with the number of balls $j$. 
%To obtain $M(i,j)$, we have to compute all transition probabilities from the (pre-transition) state $i$ to each of the atom states of state $j$ and sum them up. 

We notice that we can break each composite state $j$ into a much small number of coarse-grained sub-states, each of which may still contain a large number of atom states. Although the transition probability from state $i$ to any sub-state is still a summation formula and hard to compute, we discover a recurrence relation among these transition probabilities that allows us to compute them using dynamic programming. 
% We overcome this problem by grouping the huge number of atom states into a smaller number of coarse-grained sub-states first, then computing the transition probability from the (pre-transition) state $i$ to any sub-states of state $j$. Although each sub-state still consists of many atom states and the transition probability to a sub-state is still hard to compute directly, we discover a recurrence relation among these transition probabilities, so we can compute them using Dynamic Programming.



%as far as the calculation of the transition probability from a (larger) state $i$ $(>j)$ to $j$ is concerned. 
% To calculate the probability, we have to break the composite state $j$ down into ``atom'' states, calculate the transition probability from state $i$ to each of the ``atom'' states (which can be directly calculated), and then add them up. {\bf Note that we always view state $i$ (pre-transition state) as a {\it simple state}, since how the $i$ balls are placed into $n$ bins only depends on the hash function.}

% Each composite state $j$ can be broken down into atom states based on how these $j$ bad balls are placed into the $n$ bins. For example, state $6$ consists of $4$ atom states. The first one is $6 = 6$, where all $6$ bad balls are in the same bad bin. The second one is $6 = 2 + 4$ where, out of the $6$ bad balls, four are in one bad bin and the other two are in the other bad bin.  Similarly, the other two atom states are $6 = 3 + 3$ and $6 = 2 + 2 + 2$. The transition probability from state $i$ to any atom state can be directly calculated, but the problem is that the number of atom states grows exponentially with the number of ``bad'' balls $j$.

% We notice that we can break each composite state into a small number of coarse-grained sub-states, each of which may still contain a large number of atom states. The transition probability from a (larger) state $i$ to any sub-state is still hard to compute. However, there is a recurrence relation among them, so we can compute the transition probabilities from any state to any sub-state using Dynamic Programming. 

State $j$ is broken down into at most $j$ sub-states, which are defined as follows:
%The sub-states of state $j$ is defined as follows: 
let state $(j,k)$ denote the sub-state of state $j$ that the $j$ ``bad'' balls end up to occupy exactly $k$ ``bad'' bins. We call a bin ``good'' if it contains exactly $1$ (``good'') ball, and a bin ``bad'' if it contains more than $1$ (``bad'') balls. The composite state $j$ is partitioned into state $(j,1)$, state $(j,2)$, $...$, state $(j,j)$. We slightly abuse the notation and let $M(i,j,k)$ denote the probability of transition from state $i$ to state $(j,k)$, then we have 

\begin{equation}\nonumber
    M(i,j) = \sum_{k=1}^{j} M(i,j,k)
\end{equation}

%{\bf explain the range of $k$ could be distracting, so I just leave it as it is.}
To obtain $M$, it is sufficient to compute $M(i,j,k)$ for $\forall i,j,k=0,1,...,t$. 
In the previous Markov chain, we assume the ``bad'' balls are thrown `simultaneously' into the $n$ bins. Here, we zoom into the ``throwing'' process and consider it as a ``slow motion Markov chain'', in which the ``bad'' balls are thrown one after another. In this ``slow motion Markov chain'', state $(i,j,k)$ is defined as $j$ ``bad'' balls ending up into $k$ ``bad'' bins after throwing $i$ balls.
%Note that the state transition resulting from throwing one ball after another is also a Markov chain, in which state $(i,j,k)$ is defined as $j$ ``bad'' balls ending up into $k$ ``bad'' bins after throwing $i$ balls into $n$ bins. In this Markov chain, 
%throwing one more ball can transition state $(i,j,k)$ to three possible states depending on the $(i+1)$-th ball ending up in (1) a ``good'' bin; (2) a ``bad'' bin; or (3) an empty bin. The first case happens with probability $(i-j)/n$, results in $2$ additional ``bad'' balls and $1$ additional ``bad'' bin (i.e., transition to state $(i+1,j+2,k+1)$). The second and third cases transition to state $(i+1,j+1,k)$ and state $(i+1,j,k)$ respectively with probability $k/n$ and $1-(i-j+k)/n$. In the opposite direction, 

State $(i+1,j,k)$ can only be reached from three states: (1) state $(i,j-2,k-1)$ when the $(i+1)$-th ball lands in a ``good'' bin (so that the ``good'' ball in the bin and the $(i+1)$-th ball becomes two ``bad'' balls). The probability of this transition is $(i-j+2)/n$, since there are $i-(j-2)$ out of $n$ bins are ``good'' at state $(i,j-2,k-1)$; (2) state $(i,j-1,k)$ when the $(i+1)$-th ball lands in a ``bad'' bin, which happens with probability of $k/n$; and (3) state $(i,j,k)$ when the $(i+1)$-th ball lands in an empty bin, which happens with probability of $1-(i-j+2)/n$;. It induces a recurrence relation that $M(i+1,j,k)$ equals to

%The second case happens with probability $k/n$ and results in state $(i+1,j+1,k)$. The third case happens with probability $1-(i-j+k)/n$ and results in state $(i+1,j,k)$. In the opposite direction, state $(i+1,j,k)$ can be transitioned from (1) state $(i,j-2,k-1)$ with probability $(i-j+2)/n$; (2) state $(i,j-1,k)$ with probability $k/n$; or (3) state $(i,j,k)$ with probability $1-(i-j+k)/n$. It gives us a recurrence relation that $P(i+1,j,k)$ equals to

\begin{equation}\nonumber
    \frac{i\!-\!j\!+\!2}{n}\cdot M(i,j\!-\!2,k\!-\!1)+\frac{k}{n}\cdot M(i,j\!-\!1,k)+(1\!-\!\frac{i\!-\!j\!+\!2}{n})\cdot M(i,j,k)
\end{equation}

%The three terms in this formula corresponds to the above three possible transitions. 
The computational complexity for each $M(i,j,k)$ is $O(1)$ via dynamic programming, so the overall compuational complexity is $O(t^3)$ (for $t^3$ entries). To compute $M(i,j,k)$ for $\forall i,j,k=0,1,...,t$ via dynamic programming, we also need to compute the transition probabilities in the base cases as follows:  
%Combining with the following probabilities in base cases, we can compute $M(i,j,k)$ for $\forall i,j,k=0,1,...,t$ using Dynamic Programming and obtain $M$:

\begin{align}
M(0,j,k) =& \left\{ \begin{array}{ccl}
1, & \mbox{if }
 j=k=0 \\ 0, & \mbox{otherwise} 
\end{array}\right.\nonumber\\
M(i,0,k) =& \left\{ \begin{array}{ccl}
\binom{n}{i}/n^i, & \mbox{if }
 k=0 \\ 0, & \mbox{otherwise} 
\end{array}\right.\nonumber\\
M(i,j,0) =& \left\{ \begin{array}{ccl}
1, & \mbox{if }
 j=0 \\ 0, & \mbox{otherwise} 
\end{array}\right.\nonumber
\end{align}

% PBS reconciles the distinct elements gradually round by round. This is the ``piecewise decodability'' mentioned in \autoref{sec:intro_oursolution}. We use the following example to describe it in details: 
% Given two sets with $10$ distinct elements, in the first round, PBS tries to reconcile the $10$ distinct elements and say $6$ out of the $10$ distinct elements are successfully reconciled. Then the $6$ reconciled distinct elements are removed and PBS tries to reconcile the remaining $4$ distinct elements in the second round. Say $2$ out of the $4$ remaining distinct elements are successfully reconciled, and that leaves $2$ remaining distinct elements to be reconciled in the third round, so on so force. 
% % Given two sets $A$, $B$ with $10$ distinct elements, in the first round, PBS hashes them into $7$ distinct subset pairs. $6$ distinct elements are hashed into $6$ distinct subset pairs, and the other $4$ distinct elements are hashed into the same subset pair. Then the former $6$ distinct elements are successfully reconciled in the first round and the later $4$ distinct elements remain to be reconciled in the second round, which are hashed into $3$ distinct subset pairs (under a different hash function). $2$ remaining distinct elements are hashed into $2$ distinct subset pairs, and the other $2$ remaining distinct elements are hashed into the same subset pair. Then the former $2$ remaining distinct elements are successfully reconciled in the second round and the later $2$ remaining distinct elements remain to be reconciled in the third round, so on so force. 
% The dynamics of the number of remaining distinct elements (i.e., $10\leadsto 4\leadsto 2\leadsto \cdots$ in the example) is in nature a Markov chain, which will be elaborated and analyzed in \autoref{sec:single_markov} to derive a tight tail bound of the probability that all distinct elements are reconciled in $r$ rounds. 
\begin{comment}
+++++++++++

The only problem left to obtain $Pr[d\xrsquigarrow{r} 0]$ is how to compute $M$, which is not straightforward, since each state $j$ with $j>3$ in the Markov chain is a composite state as far as the calculation of the transition probability from a (larger) state $i$ $(>j)$ to $j$ (i.e., ``transitioning into'') is concerned.   {\bf You need to explain why it is not straightforward:  The reason you offer is not
the direction reason.  Instead you may say that "the transition probability between these composite states cannot be directly calculated" ...  to calculate it we have to break it down into "atom" states}

Each composite state $i$ can be broken down into atom states as follows.  Each simple state is, in combinatorics terms, {\it a permutation of a combination of $i$}, which here corresponds to 
how these $i$ balls are ``divided up" by the $n$ bins.   {\bf Liang, Read Mitzenmacher and Upfal book
for a better word for "divided up"}
For a simple example, when $i = 4$ and $n = 7$, the vector (1, 0, 1, 0, 0, 2, 0) is such a simple state, which corresponds to these 7 bins (in a predefined order such as the natural order) 
have 1, 0, 1, 0, 0, 2, and 0 balls in it respectively.   The transition probability between any two atom states can be ...    but the problem is that the number of atom states 
(permutations of combinations) grow exponentially with the number of balls $i$.

Consider two states i1 and i2 each broken down into millions of atom states.  Then the transition probability between these states is the summation of the trillions (= millions * millions) of 
transition probabilities between atom states of i1 and atom states of i2.  

The good thing is that the transition probability matrix among the (humongous number of atom states) induces a "subproblem structure ????", which leads to the recurrence relation, 
dynamic programming.   

We notice that we can break each state into a small number of coarse-grained substates, each of which may still contain a large number of atom states.  The transition probability 
between any two such substates are still hard to compute.  However, there is a recurrence relation among them ...

+++++++++++

To solve the problem, we partition the composite state into sub-states, so that the transition probability to the composite state is the summation of the transition probabilities to each of the sub-states. On the other hand, the transition probabilities to the sub-state have a recurrence relation and can be computed using Dynamic Programming. 

======================================

Note that every state $j$ with $j > 3$ in the Markov chain is a composite state as far as the calculation of the transition probability from a (larger) state $i > j$ to $j$ (i.e., ``transitioning into").  For example, State 6 contains 4 different cases. The first case is $6 = 6$, where all 6 bad balls are in the same bad bin. The second case is $6 = 2 + 4$ where, out of the 6 bad balls, four are in one bad bin and the other two are in the other bad bin.  Similarly, the other two cases are $6 = 3 + 3$ and $6 = 2 + 2 + 2$. Note there is no need to distinguish these four cases in calculating the ``transitioning out" probability (i.e., from state 6 to a small state say State 0), because the next round of balls-into-bins operation uses a different hash function independent of that used in the current round, and consequently how these 6 bad balls are split in the current round have no bearing on that in the next round. 

Building on the example above, we now consider $m_{9,6}$, the transition probability from State $9$ to State $6$ (throwing 9 balls into 255 bins and ending up with 6 bad balls).  $m_{9,6}$ is simply the sum of the probabilities of these four cases, each of which has a very different formula than the others.  In general, the number of such cases, and hence the number of individual probability terms to be added up to arrive at the transition matrix element $m_{i,j}$, grows exponentially with the value of $j$. This does not however make it difficult to calculate the values of $M$, because there is a recursive structure, among the values of the matrix elements $m_{i,j}$, that can be exploited using dynamic programming, as will be elaborated shortly.

To simplify our analysis, we split each composite state into sub-composite states based on the number of nonempty bins: Let State $(j,k)$ denotes the sub-composite state with $j$ remaining distinct elements and $k$ nonempty bins, which is also a substate of State $j$. Let $m_{i,j}^{(k)}$ denote the probability of transition from State $i$ to State $(j,k)$, which is also the probability that after throwing $i$ balls uniformly and independently into $n$ bins, $i-j$ bins are ``good'' bins and $k$ bins are nonempty bins (thus $k-(i-j)$ bins are ``bad'' and $n-k$ bins are empty). The probability of transition to a composite state is simply the summation of the probabilities of the transitions to corresponding sub-composite states:

To obtain the transition matrix $M$, it is sufficient to compute $m^{(k)}_{i,j}$, which can be exploited using dynamic programming. Note that the balls-and-bins model itself can be considered as a Markov chain, in which a recursive relation exists: After throwing $i$ balls into $n$ bins, throwing one more ball randomly could be: (1) Into an empty bin and turn it to a ``good'' bin; (2) Into a ``good'' bin and turn it to a ``bad'' bin with two balls; or (3) Into a ``bad'' bin and keep it as the same. Mathematically, we have $m^{(k)}_{i+1,j}$ equals to


====================================
\end{comment}



==> section/theoretical_analysis_without_comments.tex <==
\begin{comment}
\section{Tug-of-War Sketch}\label{sec:sketch}


In this section, we describe the {\it tug-of-war}, which was first proposed in~\cite{AlonMS99} as 
a space-efficient estimator for the second frequency moment. 
%% Copy from Infocom 2009
We briefly describe 
the plain vanilla tug-of-war sketch~\cite{AlonMS99} in the context of error estimating coding, and under the assumption
that the sketch per se is not subject to bit errors (``noiseless") during transmission.  A tug-of-war sketch of a bit array (packet) $b$
is comprised of a constant number $c$ of counters  ($c$ is determined by the desired error guarantees) that are maintained using the same update algorithm (with possibly different update values) and is sent to the receiver alongside with $b$.
After the execution of these update algorithms, each counter contains the inner product of the bit vector $\overrightarrow{b}$ (`0' converted to `-1' as discussed earlier) with a vector $\overrightarrow{s} \in \{+1, -1\}^n $  that is four-wise independent, as shown in the following algorithm.  Such four-wise independent vectors are known to exist and have computationally efficient representations (e.g., derivable from the Reed-Muller code~\cite{GilbertKMS03}).
Note the actual update algorithm is not shown here because it is not relevant to our context; Only its ``net effect" after execution is. 


\subsection{Set Reconciliation}\label{subsec:set-reconciliation}

Before we describe how to use tug-of-war for set reconciliation~\cite{Guo_SetReconciliationvia_2013,Mitzenmacher_SimpleMultiParty_2013,Eppstein_WhatsDifference?Efficient_2011}, we first give a brief 
description of set reconciliation. For two sets $A, B$ that contain elements from the same universe, $U$, the set reconciliation 
problem wants to compute the set difference $A \Delta B\triangleq (A\setminus B)\cup (B\setminus A)$. We denote $D=A\Delta B$, and 
$d=|D|$. In the context of set reconciliation, the two sets $A$ and $B$ are stored at two distinct places and the problem wants to 
compute $D$ with minimal communication overhead. 

First, we assume that $d$ is known a prior. We will show later how to use the tug-of-war sketch 
to estimate $d$, the size of 
the set difference. 
As shown in~\cite{Eppstein_WhatsDifference?Efficient_2011}, we can achieve 
$O(d)$ (with a small constant factor) 
communication overhead to compute the set difference $D$ using 
the invertible bloom filter (IBF)~\cite{Goodrich_InvertibleBloomLookup_2011,Eppstein_StragglerIdentificationRound_2011}, which is clearly (asymptotically) optimal. However, in the cases where each element is 
very large (in terms of communication requirement) such as large documents or movie chunks, it is a large communication overhead to transmit a small constant (say $2$ or $3$) times  $d$ elements. As we will show next, by using 
the tug-of-war sketch, we can reduce the communication overhead to very close to $d$ (elements) 
with a few rounds of message exchanges. 


We assume that the communication is initiated by $A$. 
Each round of communication works as follows. 
$A$ creates $m=\delta d$ buckets, $b_1,b_2,\dots,b_m$, 
where $\delta > 1$ is a constant. Each bucket $b_i$
contains a subset of elements from $A$, 
each of which is uniformly randomly selected (with properly-designed 
hash functions). 
For each bucket $b_i$, $A$ computes $c$ tug-of-war sketches, 
denoting as $z_{i,1},z_{i,2},\dots,z_{i,c}$. Note that here eahc $z_{i,j}=\sum_{a\in b_i}h(a)$, where 
$h$ is from a four-wise hash family that maps each element to $\pm 1$. 
Then, $A$ sends the $m\times c$ sketches 
to $B$. $B$ uses the same hash functions to create $m$ buckets for its elements, and then use the same hash 
functions to compute the tug-of-war sketches for each bucket, denoting those sketches as $z'_{i,j}$ for $i\in [m]$ and 
$j\in [c]$. Then, $B$ can use $\frac{1}{c}\sum_{j=1}^{c}(z_{i,j}-z'_{i,j})^2$ to estimate the size of (sub-)set difference of 
the bucket $b_i$ for any $i\in [m]$. Note that $B$ can use the median of mean approach in~\cite{AlonMS99} 
or the MLE estimator in~\cite{Hua_TowardsOptimalError_2012} to obtain 
better estimations. Then, for each bucket whose estimator is in $(0, 1.5)$ (just an example), $B$ sends the exclusive or of all the elements 
in the bucket to $B$. It is clear that if the true size of the set difference for the bucket is $1$, then $A$ can obtain the 
element belonging to $A\Delta B$ in the bucket. 

By repeating the process until all the $d$ elements are obtained, $A$ computes the set difference $D$.
\end{comment}
\begin{comment}
\medskip
\noindent
{\bf Analysis on Number of Rounds}.
Consider the whole process as a Markov chain, whose state is defined as the number of 
``hidden elements'' ({\it i.e.,} elements belonging to the set difference that are to be decoded). 
\autoref{fig:mc} presents the state transition diagram, denoting the corresponding transmission 
matrix as $P=\big{(}p_{i,j}\big{)}_{(d+1)\times (d+1)}$ where $p_{i,j}$ is the probability of moving from state $i$ to state $j$. It is complex to obtain all the elements in $P$, we 
can easily get the following probabilities, for any $k \leq d$,
\begin{align}
p_{k,0}&=\frac{\binom{m}{k}k\,!}{m^k} \\
p_{k,1}&=0 \\
p_{k,2}&=\frac{\binom{k}{2}(m-k+2)\binom{m}{k-2}(k-2)\,!}{m^k},\quad \forall k\geq 2\\
p_{k,3}&=\frac{\binom{k}{3}(m-k+3)\binom{m}{k-3}(k-3)\,!}{m^k},\quad \forall k\geq 3\\
p_{k,4}&=\frac{\big{(}\binom{k}{4}(m-k+4) + \binom{k}{2}\binom{k-2}{2}(m-k+4)(m-k+3)/2\big{)}\binom{m}{k-4}(k-4)\,!}{m^k},\quad \forall k\geq 4.
\end{align}
where $m$ is the number of buckets.

Similarly, we can calculate $p_{k,i}$ for any $k\geq i \geq 5$ but the expression gets more and more complex. 


It is not hard to check that the Markov chain described above is an absorbing Markov chain with 
a single absorbing state of $0$. By using the time to absorption theorem of Absorbing Markov Chains~\cite[Page 13]{Elizalde_LectureNotesMath_2006}, 
we can easily get the average number of rounds (steps before the chain is absorbed), which equals
the $d^{th}$ element of $(N{\bf 1})$ where the matrix 
$N=(I-Q)^{-1}$ is the fundamental matrix of $P$ (Note that $Q$ is the transition matrix for all transient states, in our case, is $P$ by removing the last row and column, {\it i.e.,} $P_{0,*}$ 
and $P_{*,0}$) and 
${\bf 1}$ is an all-one vector with length $d$. 

Denote $P^{(k)}$ as the $k$-step transition matrix, then the probability that it takes more than $n$ rounds to decode is
\begin{equation}
\mathbf{Pr}[t>n]=\sum_{k=n+1}^{\infty}p^{(k)}_{d,0},
\end{equation}
where $d$ is the initial number of elements.


\medskip
\noindent
{\bf Simplified Analysis on Number of Rounds.} In the following analysis, we assume that the number of buckets in the kth round, 
assuming remaining $d_k$ elements to be decoded, is set to be $\delta\cdot d_k$ where $\delta > 1$ is a constant. For ease of 
presentation, we drop the subscript $k$ in the following analysis\footnote{Inspired by the analysis of the number of iterations 
for PIM.}. 

Fix a bucket, the probability that it gets exactly one element belonging to the set difference that is not decoded yet is:
\begin{equation}
p = d \Big{(}\frac{1}{\delta d}\Big{)}\Big{(} 1 - \frac{1}{\delta d}\Big{)}^{d - 1} = \frac{1}{\delta}\Big{(} 1 - \frac{1}{\delta d}\Big{)}^{d - 1}\approx \frac{1}{\delta}e^{-1/\delta}.
\end{equation}

On average, there are $p$ fraction of buckets will get exact one element. Hence, on average $e^{-1/\delta}$ fraction of un-decoded 
elements will be decoded in each round. Therefore, on average, we need $\log_{\frac{1}{1- e^{-1/\delta}}}d_0$ rounds, {\it i.e.,} 
$O(\log d_0)$ rounds. 
\end{comment}

\section{Tail Bound Analysis and Parameter Settings}\label{sec:tail_bound}

In this section, we establish a tight tail bound on the {\it success probability} within $r$ rounds (defined in \autoref{subsec:protocol2}) under arbitrary parameter settings of $n$, $\delta$, and $t$. On one hand, this tail bound gives us a theoretical guarantee on the success probability under specific parameter settings. On the other hand, given a parameter setting requirement (i.e., a target success probability $p_0$ within $r$ rounds), we can use the tail bound to find all feasible parameter settings that satisfy the requirement, then select the optimal parameter settings among them that have the lowest communication overhead. {\bf This analysis also provides other theoretical results for PBS, such as the expected number of distinct elements will be reconciled in the each round (``Piecewise Decodability'', to be shown in \autoref{sec:piecewise_decodability})}%In this section, we continue to assume $d$ is precisely known. 

%For simplicity, we ignore two types of small probability events in the analysis. The first one is, PBS mistakenly believes the set reconciliation has been completed due to an incorrect verification of the $32$-bit checksum (\autoref{step:terminate_condition} of \autoref{alg:single_round_pbs}). The second one is, a type (\RN{2}) event happens and the ``fake'' distinct element is not successfully verified by \autoref{alg:verification} (mentioned in \autoref{subsec:exception_hash_partition}). As we described earlier, the former happens with a probabilty of $2.3\times 10^{-10}$ and that of the later is in order of $10^{-7}$. Ignoring these events that happen with such tiny probabilities barely compromises the accuracy of the tail bound. 

% Motivated by parameter settings, we establish a strict tail bound on the {\it success probability} of PBS (i.e., all distinct elements are reconciled in $r$ rounds) as a function of parameters (i.e., $n$, $\delta$, $t$), which give us (1) a guideline on parameter settings; and (2) a theoretical guarantee about the success probability under selected parameters. 

% In this section, we still assume $d$ is precisely known. 
% For simplicity, we make the following two assumptions that hold with overwhelming probability in the analysis: First, the checksum (\autoref{step:terminate_condition} of \autoref{alg:single_round_pbs}) works perfectly on checking if the reconciliation is complete; Second, no ``fake'' distinct element fails to be checked by \autoref{alg:verification} (mentioned in \autoref{subsec:exception_hash_partition}) appears during reconciliation. 

% {\bf (to be finalized after the following subsections are finalized) We first establish a strict tail bound for a single group pair using Markov chain and Dynamic Programming in \autoref{sec:tail_bound_per_group}. Then we combine it with Times-2-Bound to get a strict tail bound for all group pairs in \autoref{sec:times2bound}. In \autoref{sec:parameter_settings}, we discuss the parameter settings using the tail bound. }

%In \autoref{sec:tail_bound_insufficient}, we remove the above BCH assumption and derive a more precise tail bound. {\bf need to decide whether to have this part or not, since we can easily set a relatively long BCH code, so that each group is decodable w.h.p.}

\subsection{Analysis of a simple case}\label{sec:single_markov}

In this section, we analyze the probability that an arbitrary group pair that contains exactly $x$ $(\leq t)$ distinct elements is completely reconciled (i.e., all distinct elements are successfully reconciled) by PBS in $r$ rounds.

As we described in \autoref{sec:multi-rounds}, in the first round of PBS, the $x$ distinct elements are hashed into $n$ subset pairs, and a distinct element is successfully reconciled if and only if it is hashed into a subset pair that contains only $1$ distinct element. 
%The successfully reconciled distinct elements in the first round are removed and the other distinct elements (i.e., the ones that have not been reconciled yet in the first round) will be hashed again in the second round using a different hash function, so on so force, until all distinct elements are successfully reconciled. 
How the $x$ distinct elements are distributed into $n$ subset pairs in the first round follows the familiar {\it balls-into-bins} probability model: Each of the $x$ balls is thrown independently and uniformly at random into one of the $n$ bins. Each successfully reconciled distinct element corresponds to a ball that ends up in a bin that receives exactly $1$ ball. We call the ball and the bin ``good'' in the sequel; each distinct element that has not been reconciled yet in the first round corresponds to a ball that ends up in a bin that receives multiple balls. We call the ball and the bin ``bad'' in the sequel. Note that balls are either ``good'' or ``bad'', but a bin could be empty besides being ``good'' and ``bad''. 

The ``bad'' balls in the first round will be the balls to be thrown in the second round. The ``bad'' balls in the second round will be the balls to be thrown in the third round, so on so force. In all rounds, how the balls are thrown into $n$ bins follows the same balls-into-bins probability model. Note that the balls are thrown using different hash functions in each round, so the number of ``bad'' balls in the $i$-th round
%(i.e., the number of balls to be thrown in the $(i+1)$-th round) 
only depends on how many balls are thrown in the $i$-th round and is independent of how these balls (``bad'' balls in the $(i-1)$-th round) are placed into the $n$ bins in the $(i-1)$-th round. Therefore, the number of balls to be thrown round after round is a Markov chain, in which each state is defined as the number of balls to be thrown. 
%Hence, the dynamics of the number of balls to be thrown in each round can be modeled as a Markov chain, in which each state is defined as the number of balls to be thrown. {\bf a little bit wordy, need advice on how to shrink it.}

In the Markov chain, a transition from state $i$ to state $j$ ($i\geq j$) means $i-j$ out of $i$ balls are ``good'' balls and the other $j$ balls are ``bad'' balls. The {\it absorbing state} of this Markov chain is state $0$, which is the ``good'' state that all balls are ``good'' (so that all distinct elements are successfully reconciled). For our analysis, the only probability that we are concerned with is $Pr[x\!\xrsquigarrow{r}\! 0]$, the probability that starting with state $x$ (initial state), the Markov chain reaches the absorbing state (i.e., state $0$) within $r$ transitions. It is also the success probability for a single group (starting with $x$ distinct elements and successfully reconciled within $r$ rounds), which can easily calculated given $M$, the $(t+1)\times (t+1)$ transition matrix of the Markov chain, as 
%, where $M(i,j)$ (i.e., the entry in the $i^{th}$ row and the $j^{th}$ column of $M$) is the probability of transition from state $i$ to state $j$ for $i,j = 0,1,...,t$
$\big{(}M^r\big{)}(x,0)$, the entry in the $x$-th row and the $0$-th column of $M^r$. Here we slightly abuse the row / column indices of a $(t+1)\times (t+1)$ matrix from $1,2,...,t+1$ to $0,1,...,t$, since the state of the Markov chain ranges from $0$ to $t$. How to compute $M$ will be elaborated in \autoref{sec:compute_M}. For the moment, we assume $M$ has been computed and therefore we can compute $Pr[x\!\xrsquigarrow{r}\! 0]$ for $x=1,2,...,t$, $r\in\mathbb{N}^+$. 

\subsection{Analysis on ``Piecewise Decodability''}\label{sec:piecewise_decodability}

{\bf Note that PBS reconciles the distinct elements gradually round by round. The distinct elements that have been reconciled in the first round are no longer needed to be reconciled again in the second round. This is the ``piecewise decodability'' mentioned in \autoref{sec:intro_oursolution}. From the transition matrix $M$, we can theoretically analyze this ``piecewise decodability'' by computing the expected value of how many distinct elements are reconciled in the each round. 
%For example, $\sum_{l=0}^x l\cdot Pr[x\!\xrsquigarrow{1}\! l]$ is the average number of the distinct elements that are reconciled in the first round (for an arbitrary group pair with $x$ distinct elements). 
Although this expected value in any scenario (given $d$, $n$, and $t$) is computable, we only show the `general' results in \autoref{tab:reconcile_ratio}, in which we assume $\delta_1,\delta_2,...,\delta_g$ follow the Poisson distribution with mean of $\delta$ (this is a tiny approximation for relatively large $d$, since the Poisson distribution is a limiting case of the Binomial distribution with the same expectation), and $t$ is sufficiently large. }

\begin{table}[h]
\centering
\caption{Average percentage of distinct elements are reconciled per round}\label{tab:reconcile_ratio}
\begin{tabular}{@{}|c|c|c|c|c|@{}}
\hline 
$n$   & Round $1$ & Round $2$ & Round $3$ & Round $4$ \\ \hline 
$63$   & 92.4\% & 7.46\% & $1.7\times 10^{-3}$ & $2.7\times 10^{-5}$ \\ \hline
$127$   & 96.1\% & 3.82\% & $3.7\times 10^{-4}$ & $2.9\times 10^{-6}$ \\ \hline
$255$  & 98.1\% & 1.93\% & $8.4\times 10^{-5}$ & $3.3\times 10^{-7}$ \\ \hline
$511$ & 99.0\% & 0.97\% & $2.0\times 10^{-5}$ & $3.9\times 10^{-8}$ \\ \hline
$1023$ & 99.5\% & 0.49\% & $4.9\times 10^{-6}$ & $4.8\times 10^{-9}$ \\ \hline
% \begin{tabular}{@{}|c|c|c|c|c|c|c|@{}}
% \hline 
% \diagbox{$r$}{$n$}    & $63$ & $127$ & $255$ & $511$ & $1023$ & $2047$ \\ \hline 
% 1   & 92.4\% & 96.1\% & 98.1\% & 99.0\% & 99.5\% & 99.8\% \\ \hline
% 2   & 7.46\% & 3.82\% & 1.93\% & 0.97\% & 0.49\% & 0.24\% \\ \hline
% 3  & $1.7\times 10^{-3}$ & $3.7\times 10^{-4}$ & $8.4\times 10^{-5}$ & $2.0\times 10^{-5}$ & $4.9\times 10^{-6}$ & $1.2\times 10^{-6}$ \\ \hline
% 4  & $2.7\times 10^{-5}$ & $2.9\times 10^{-6}$ & $3.3\times 10^{-7}$ & $3.9\times 10^{-8}$ & $4.8\times 10^{-9}$ & $5.9\times 10^{-10}$ \\ \hline
\end{tabular}
\end{table}

{\bf \autoref{tab:reconcile_ratio} shows that the majority of the distinct elements are reconciled in the first round. Therefore, the communication overhead (roughly proportional to the number of distinct elements that are reconciled) in the first round is the major part of the overall communication overhead. 
%In other words, the overall communication overhead of all rounds is only slightly larger than that in the first round. 
Due to this reason, we use the communication overhead in the first round (described in \autoref{sec:communication_overhead_single_PBS}) to approximate the overall communication overhead of all rounds in parameter settings (to be elaborated in \autoref{sec:parameter_settings}. {\bf \autoref{tab:reconcile_ratio} also shows that the number of remaining distinct elements (the ones that have not been reconciled) decreases exponentially round after round. 
%The larger $n$ is, the larger percentage of the distinct elements will be reconciled in the first round.}
%The requirement above also ensures the majority of the distinct elements are reconciled in the first round, as we will show in \autoref{sec:piecewise_decodability}. Therefore, the majority of the overall communication overhead happens in the first round. In other words, the overall communication overhead of all rounds is only slightly larger than ($1.01$ to $1.07$ times of) that in the first round. Due to this reason, we use the communication overhead in the first round (described in \autoref{sec:communication_overhead_single_PBS}) to approximate the overall communication overhead of all rounds in parameter settings (to be elaborated in \autoref{sec:parameter_settings}.

\subsection{Tail Bound Analysis for Each Group Pair}\label{sec:tail_bound_per_group}

% ==========
% {\bf The following may be useful in explaining why it is a Markov chain:} [Note there is no need to distinguish these four cases in calculating the ``transitioning out" probability (i.e., from state 6 to a small state say State 0), because the next round of balls-into-bins operation uses a different hash function independent of that used in the current round, and consequently how these 6 bad balls are split in the current round have no bearing on that in the next round.]  {\bf unless you have done so earlier}
% ==========

As we explained in \autoref{subsec:protocol2}, $\delta_1$, the number of distinct elements in group pair $1$, is a random variable that follows a Binomial distribution $Binomial(d,1/g)$. So the probability that group pair $1$ is successfully reconciled in $r$ rounds is $\sum_{x=0}^d Pr[\delta_1\!=\!x]\cdot Pr[x\!\xrsquigarrow{r}\! 0]$. 
%, where $\mathcal{B}(\cdot;d,1/g)$ is the probability mass function (PMF) of $Binomial(d,1/g)$. 
To ease computation, we slightly underestimate this probability by assuming $Pr[x\!\xrsquigarrow{r}\! 0]=0$ when $x>t$ (i.e., assume group pair $1$ cannot be reconciled if $\delta_1>t$, discussed in \autoref{sec:BCH_exception}). The loss of this underestimation is very tiny, since $Pr[\delta_1\!=\!x]$, the ``coefficient'' of $Pr[x\!\xrsquigarrow{r}\! 0]$, is very small when $x>t$. We denote this underestimated probability as $\alpha$ (i.e., $\alpha=\sum_{x=0}^t Pr[\delta_1\!=\!x]\cdot Pr[x\!\xrsquigarrow{r}\! 0]$), which is a tight tail bound of the success probability of group pair $1$. $\alpha$ is also a tight tail bound for all other group pairs, since $\delta_1,\delta_2,...,\delta_g$ follows the same distribution. $Pr[x\!\xrsquigarrow{r}\! 0]$ is a function of $n$ for given $x$ and $r$, so $\alpha=\alpha(n,t)$ is a function of $n$ and $t$ for arbitrary $d$, $r$, and $g$. 

\subsection{Tail Bound Analysis for All Group Pairs}\label{sec:times2bound}

Given $\alpha$, the tail bound of the probability that a group pair is successfully reconciled in $r$ rounds, we can easily derive a tail bound of $\alpha^g=1-(1-\alpha^g)$ for the probability that all group pairs are successfully reconciled in $r$ rounds ($1-\alpha^g$ is the failure probability, which is usually tiny), if we assume the reconciliations on group pairs are independent with each other. However, this assumption is not rigorous,
%since $d_1, d_2,...,d_g$ have a weak correlation that $\sum_{i=1}^g d_i=d$.
since $\delta_1, \delta_2,...,\delta_g$ are not strictly independent and have a relation that $\sum_{i=1}^g \delta_i=d$. 
%Fortunately, we have Times-2-Bound (Theorem 1 in \cite{hua2008rank}) to decouple the weak correlation and give us a rigorous tail bound of $1-2(1-\alpha^g)$ for the probability of all group pairs. 
However, we can use Corollary 5.11 in \cite{upfal2005probability} to
% decouple the weak correlation and 
obtain a rigorous tail bound of $1-2(1-\alpha^g)$ for the success probability of all group pairs. This rigorous tail bound is very tight and only doubles the tiny failure probability of the unrigorous tail bound: For example, if the unrigorous tail bound of the success probability of all group pairs is $0.9999$ ($0.0001$ failure probability), then the rigorous tail bound will be $0.9998$ ($0.0002$ failure probability). We use the tail bound of $1-2(1-\alpha^g)$ in parameter settings for rigorousness. 

\subsection{Parameter Settings}\label{sec:parameter_settings}

% The tail bound is based on the total number of distinct elements $d$, which is however not known precisely. The ToW Estimator introduced in \autoref{subsec:ToW} can only provide an estimation of $d$ (denoted as $\hat{d}$). Note that the tail bound of $Pr[P^{(r)}_o]$ increases as $d$ increases. So overestimate $d$ will get us a larger failure probability $Pr[P^{(r)}_o]$. To ensure a high success probability, we use an overestimated number of distinct element $\bar{d}$ $(>\hat{d})$ for parameter settings, such that $\bar{d}\geq d$ with high probability. In our evaluation, we set $\bar{d}\triangleq 1.38\hat{d}$, such that $\bar{d}\geq d$ with probability $99\%$. 

In this section, we elaborate how to set the parameters $n$, $t$, and $g$ given the target success probability $p_0$ within $r$ rounds (the probability that PBS successfully reconciles all distinct elements within $r$ rounds to be larger than $p_0$) in PBS. We continue to assume $d$ is precisely known. First, as explained in \autoref{subsec:protocol2}, $\delta$ should be a small number, so we fix $\delta=5$ and therefore $g=d/\delta$ is also fixed. 
Given the target success probability $p_0$ within $r$ rounds
%(i.e., set reconciliation is complete in $r$ rounds with probability $p_0$) 
%depend on the requirement of specific applications)
, the parameter setting problem aims to find the optimal parameter settings of $n,t$ that minimizes the overall communication overhead, under the constraint that the tail bound of the success probability of $r$ rounds is larger than $p_0$. Note that the only two components in the communication overhead per group pair (described in \autoref{sec:multi-rounds}) that depend on parameter settings are $t\log n+\delta\log n$. So we can formalize the parameter setting problem as the following optimization problem:

% \begin{equation}
% \min\limits_{n,t} t\log n+\delta\log n \quad \mbox{s.t.}\quad 1-2(1-\alpha^g(n,t))>p_0
% \end{equation}

\begin{align}
\mbox{minimize} \quad
&
t\log n+\delta\log n \nonumber
\\
\mbox{subject to} \quad 
&
1-2(1-\alpha^g(n,t))>p_0,\quad n,t\in \mathbb{N}^+ \nonumber
% \\
% &
% n,t\in \mathbb{N}^+ \label{eq:row_sum_requirement}
\end{align}

This optimization problem is not as daunting as it looks, since we can narrow down its solution space into only a few combinations and traverse all these combinations to find the optimal parameter settings as follows: First, since $n$ is the ``code length'' of BCH code, we select $n$ to be $2^m-1$ for some integer $m$ for BCH coding efficiency. Then the range of $n$ is narrowed down to $\{63,127,255,511,1023\}$ (recall that $n=\Omega(\delta^2)$). Second, we select $t$ in the range from $1.5\delta$ to $3.5\delta$, since any smaller $t$ will cause a high probability of BCH decoding failure (explained in \autoref{subsec:protocol2}) and therefore a low success probability (below $50\%$), and any higher $t$ incurs significant additional communication overhead on transmitting BCH codeword (explained in \autoref{subsec:protocol2}) while barely increases the success probability.

% This optimization problem seems to be difficult to solve, since the constraint is a very comprehensive function of the parameters (remind that $\alpha=\alpha(n,t)$ is a function of $n$ and $t$ for arbitrary $r$, $d$, and $g$). However, we can narrow down the solution space into only a few combinations and traverse all these combinations to find the optimal parameter settings as follows: First, for BCH coding efficiency, we select $n$ to be $2^m-1$ for some integer $m$ and therefore narrow its range down to $\{63,127,255,511,1023\}$ (recall that $n=\Omega(\delta^2)$). Second, we select $t$ in the range from $1.5\delta$ to $3\delta$, as we suggested in \autoref{subsec:protocol2}. 

Here we use an example to show how we set parameters: Given $d=1000$ distinct elements, $r=3$ rounds, $p_0=99\%$, for each $(n,t)$ combination in $\{63,127,255,511,1023\}\times \{8,9,...,16,17\}$, we compute the tail bound of the success probability under the parameter settings and obtain \autoref{tab:success_prob}.

\begin{table}[h]
\centering
\caption{Tail bound of success probability}\label{tab:success_prob}
\begin{tabular}{@{}|c|c|c|c|c|c|@{}}
\hline 
\diagbox{$t$}{$n$}    & $63$ & $127$ & $255$ & $511$ & $1023$ \\ \hline 
8   & 0 & 25.5\% & 32.7\% & 34.3\% & 34.9\% \\ \hline
9   & 52.1\% & 78.0\% & 84.2\% & 85.7\% & 86.1\% \\ \hline
10  & 75.1\% & 92.7\% & 96.5\% & 97.4\% & 97.6\% \\ \hline
11  & 85.9\% & 96.9\% & \cellcolor{blue!25}99.1\% & \cellcolor{blue!25}99.5\% & \cellcolor{blue!25}99.6\% \\ \hline
12  & 91.3\% & 98.5\% & \cellcolor{blue!25}99.7\% & \cellcolor{blue!25}99.9\% & \cellcolor{blue!25}$>$99.9\% \\ \hline
13  & 93.9\% & \cellcolor{blue!60}99.1\% & \cellcolor{blue!25}99.8\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% \\ \hline
14  & 95.1\% & \cellcolor{blue!25}99.4\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% \\ \hline
15  & 95.6\% & \cellcolor{blue!25}99.5\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% \\ \hline
16  & 95.7\% & \cellcolor{blue!25}99.6\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% \\ \hline
17  & 95.8\% & \cellcolor{blue!25}99.6\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% \\ \hline
\end{tabular}
\end{table}

In \autoref{tab:success_prob}, all $(n,t)$ combinations in the highlighted cells satisfy the success probability requirement. Among them, $(127,13)$ has the lowest communication overhead (w.r.t. $t\log n+\delta\log n$). So we set $n=127, t=13$ in this case. For the case of the set difference cardinality $d$ is not precisely known, we use the scaled estimation of $d$ (described in \autoref{subsec:ToW}) for parameter settings. {\bf Note that calculating the probabilities in this table is very fast, since each entry in the table can be computed in $O(1)$ time given $M^r$, and $M^r$ for each $n\in\{63,127,255,511,1023\}$ ($M$ is a function of $n$) can be precomputed in $O(t^3)$ time.}

{\bf (change r)} If we reduce the number of rounds $r$ from $3$ to $2$ while keeping the same target success probability $p_0=99\%$, we can also compute a success probability table that is similar to \autoref{tab:success_prob} to obtain the optimal parameter setting, which is $n=1023, t=16$. Compare to the previous optimal parameter settings when $r=3$ ($n=127, t=13$), this optimal parameter settings ($n=1023, t=16$) is much larger (more expensive) and incur additional communication overhead of $84$ bits per group pair. It shows that to achieve the same target success probability using fewer rounds (smaller $r$), PBS need more resources (e.g., larger $n$, $t$). Readers may think we can further increase $r$ (keeping the same target success probability) to reduce communication overhead. However, it could make PBS taking too many rounds to reconcile all distinct elements. Also, further increasing $r$ does not save much communication overhead. For example, if we increase $r$ from $3$ to $4$ (rounds), the optimal parameter setting becomes $n=63,t=11$, which only saves communication overhead of $30$ bits per group pair. }

\subsection{How to compute \texorpdfstring{\larger\boldmath{$M$}}{M}}\label{sec:compute_M}

In this section, we describe how to compute the transition matrix $M$ in details. Note that calculating an arbitrary transition probability $M(i,j)$ is not straightforward, since each state $j$ (after-transition state) with $j>3$ in the Markov chain is a {\it composite state}, which consists of a huge number of {\it atom states}. 
%The transition probability $M(i,j)$ is basically the summation of all transition probabilities from the (pre-transition) state $i$ to each of the atom states of state $j$. 

Each composite state $j$ can be broken down into atom states as follows.  Each simple state is, in combinatorics terms, {\it a permutation of a combination of $j$}, which here corresponds to how these $j$ balls are placed into the $n$ bins.  For a simple example, when $j = 4$ and $n = 7$, the vector $(2, 0, 0, 0, 0, 2, 0)$ is such a simple state, which corresponds to these $7$ bins (in a predefined order such as the natural order) have $2, 0, 0, 0, 0, 2,$ and $0$ balls in it respectively. The transition probability from the (pre-transition) state $i$ to any atom state of state $j$ can be directly computed, and $M(i,j)$ is basically the summation of all these transition probabilities. The problem is that the number of atom states (permutations of combinations) grow exponentially with the number of balls $j$. 
%To obtain $M(i,j)$, we have to compute all transition probabilities from the (pre-transition) state $i$ to each of the atom states of state $j$ and sum them up. 

We overcome this problem by grouping the huge number of atom states into a smaller number of coarse-grained sub-states first, then computing the transition probability from the (pre-transition) state $i$ to any sub-states of state $j$. Although each sub-state still consists of many atom states and the transition probability to a sub-state is still hard to compute directly, we discover a recurrence relation among these transition probabilities, so we can compute them using Dynamic Programming.



%as far as the calculation of the transition probability from a (larger) state $i$ $(>j)$ to $j$ is concerned. 
% To calculate the probability, we have to break the composite state $j$ down into ``atom'' states, calculate the transition probability from state $i$ to each of the ``atom'' states (which can be directly calculated), and then add them up. {\bf Note that we always view state $i$ (pre-transition state) as a {\it simple state}, since how the $i$ balls are placed into $n$ bins only depends on the hash function.}

% Each composite state $j$ can be broken down into atom states based on how these $j$ bad balls are placed into the $n$ bins. For example, state $6$ consists of $4$ atom states. The first one is $6 = 6$, where all $6$ bad balls are in the same bad bin. The second one is $6 = 2 + 4$ where, out of the $6$ bad balls, four are in one bad bin and the other two are in the other bad bin.  Similarly, the other two atom states are $6 = 3 + 3$ and $6 = 2 + 2 + 2$. The transition probability from state $i$ to any atom state can be directly calculated, but the problem is that the number of atom states grows exponentially with the number of ``bad'' balls $j$.

% We notice that we can break each composite state into a small number of coarse-grained sub-states, each of which may still contain a large number of atom states. The transition probability from a (larger) state $i$ to any sub-state is still hard to compute. However, there is a recurrence relation among them, so we can compute the transition probabilities from any state to any sub-state using Dynamic Programming. 

The sub-states of state $j$ is defined as follows: let state $(j,k)$ denote the sub-state of state $j$ that the $j$ ``bad'' balls end up to occupy exactly $k$ ``bad'' bins. Then the composite state $j$ is partitioned into state $(j,1)$, state $(j,2)$, $...$, state $(j,j)$. We slightly abuse the notation and let $M(i,j,k)$ denote the probability of transition from state $i$ to state $(j,k)$, then we have 

\begin{equation}
    M(i,j) = \sum_{k=1}^{j} M(i,j,k)
\end{equation}

%{\bf explain the range of $k$ could be distracting, so I just leave it as it is.}
To obtain $M$, it is sufficient to compute $M(i,j,k)$ for $\forall i,j,k=0,1,...,t$. Note that the state transition resulting from throwing one ball after another is also a Markov chain, in which state $(i,j,k)$ is defined as $j$ ``bad'' balls ending up into $k$ ``bad'' bins after throwing $i$ balls into $n$ bins. In this Markov chain, throwing one more ball can transition state $(i,j,k)$ to three possible states depending on the $(i+1)$-th ball ending up in (1) a ``good'' bin; (2) a ``bad'' bin; or (3) an empty bin. The first case happens with probability $(i-j)/n$, results in $2$ additional ``bad'' balls and $1$ additional ``bad'' bin (i.e., transition to state $(i+1,j+2,k+1)$). The second and third cases transition to state $(i+1,j+1,k)$ and state $(i+1,j,k)$ respectively with probability $k/n$ and $1-(i-j+k)/n$. In the opposite direction, state $(i+1,j,k)$ can only be transitioned from (1) state $(i,j-2,k-1)$; (2) state $(i,j-1,k)$; and (3) state $(i,j,k)$, which gives us a recurrence relation that $M(i+1,j,k)$ equals to

%The second case happens with probability $k/n$ and results in state $(i+1,j+1,k)$. The third case happens with probability $1-(i-j+k)/n$ and results in state $(i+1,j,k)$. In the opposite direction, state $(i+1,j,k)$ can be transitioned from (1) state $(i,j-2,k-1)$ with probability $(i-j+2)/n$; (2) state $(i,j-1,k)$ with probability $k/n$; or (3) state $(i,j,k)$ with probability $1-(i-j+k)/n$. It gives us a recurrence relation that $P(i+1,j,k)$ equals to

\begin{equation}\label{eq:recursion}
    \frac{i\!-\!j\!+\!2}{n}\cdot M(i,j\!-\!1,k\!-\!1)+\frac{k}{n}\cdot M(i,j\!-\!1,k)+(1\!-\!\frac{i\!-\!j\!+\!2}{n})\cdot M(i,j,k)
\end{equation}

The three terms in \autoref{eq:recursion} corresponds to the above three possible transitions. To compute $M(i,j,k)$ for $\forall i,j,k=0,1,...,t$ via Dynamic Programming, the total computational complexity is $O(t^3)$ ($O(1)$ for $t^3$ entries), and we also need to compute the transition probabilities in the base cases as follows:  
%Combining with the following probabilities in base cases, we can compute $M(i,j,k)$ for $\forall i,j,k=0,1,...,t$ using Dynamic Programming and obtain $M$:

\begin{align}
M(0,j,k) =& \left\{ \begin{array}{ccl}
1, & \mbox{if }
 j=k=0 \\ 0, & \mbox{otherwise} 
\end{array}\right.\label{eq:basic1}\\
M(i,0,k) =& \left\{ \begin{array}{ccl}
\binom{n}{i}/n^i, & \mbox{if }
 k=0 \\ 0, & \mbox{otherwise} 
\end{array}\right.\label{eq:basic2}\\
M(i,j,0) =& \left\{ \begin{array}{ccl}
1, & \mbox{if }
 j=0 \\ 0, & \mbox{otherwise} 
\end{array}\right.\label{eq:basic3}
\end{align}

% PBS reconciles the distinct elements gradually round by round. This is the ``piecewise decodability'' mentioned in \autoref{sec:intro_oursolution}. We use the following example to describe it in details: 
% Given two sets with $10$ distinct elements, in the first round, PBS tries to reconcile the $10$ distinct elements and say $6$ out of the $10$ distinct elements are successfully reconciled. Then the $6$ reconciled distinct elements are removed and PBS tries to reconcile the remaining $4$ distinct elements in the second round. Say $2$ out of the $4$ remaining distinct elements are successfully reconciled, and that leaves $2$ remaining distinct elements to be reconciled in the third round, so on so force. 
% % Given two sets $A$, $B$ with $10$ distinct elements, in the first round, PBS hashes them into $7$ distinct subset pairs. $6$ distinct elements are hashed into $6$ distinct subset pairs, and the other $4$ distinct elements are hashed into the same subset pair. Then the former $6$ distinct elements are successfully reconciled in the first round and the later $4$ distinct elements remain to be reconciled in the second round, which are hashed into $3$ distinct subset pairs (under a different hash function). $2$ remaining distinct elements are hashed into $2$ distinct subset pairs, and the other $2$ remaining distinct elements are hashed into the same subset pair. Then the former $2$ remaining distinct elements are successfully reconciled in the second round and the later $2$ remaining distinct elements remain to be reconciled in the third round, so on so force. 
% The dynamics of the number of remaining distinct elements (i.e., $10\leadsto 4\leadsto 2\leadsto \cdots$ in the example) is in nature a Markov chain, which will be elaborated and analyzed in \autoref{sec:single_markov} to derive a tight tail bound of the probability that all distinct elements are reconciled in $r$ rounds. 

\begin{comment}
+++++++++++

The only problem left to obtain $Pr[d\xrsquigarrow{r} 0]$ is how to compute $M$, which is not straightforward, since each state $j$ with $j>3$ in the Markov chain is a composite state as far as the calculation of the transition probability from a (larger) state $i$ $(>j)$ to $j$ (i.e., ``transitioning into'') is concerned.   {\bf You need to explain why it is not straightforward:  The reason you offer is not
the direction reason.  Instead you may say that "the transition probability between these composite states cannot be directly calculated" ...  to calculate it we have to break it down into "atom" states}

Each composite state $i$ can be broken down into atom states as follows.  Each simple state is, in combinatorics terms, {\it a permutation of a combination of $i$}, which here corresponds to 
how these $i$ balls are ``divided up" by the $n$ bins.   {\bf Liang, Read Mitzenmacher and Upfal book
for a better word for "divided up"}
For a simple example, when $i = 4$ and $n = 7$, the vector (1, 0, 1, 0, 0, 2, 0) is such a simple state, which corresponds to these 7 bins (in a predefined order such as the natural order) 
have 1, 0, 1, 0, 0, 2, and 0 balls in it respectively.   The transition probability between any two atom states can be ...    but the problem is that the number of atom states 
(permutations of combinations) grow exponentially with the number of balls $i$.

Consider two states i1 and i2 each broken down into millions of atom states.  Then the transition probability between these states is the summation of the trillions (= millions * millions) of 
transition probabilities between atom states of i1 and atom states of i2.  

The good thing is that the transition probability matrix among the (humongous number of atom states) induces a "subproblem structure ????", which leads to the recurrence relation, 
dynamic programming.   

We notice that we can break each state into a small number of coarse-grained substates, each of which may still contain a large number of atom states.  The transition probability 
between any two such substates are still hard to compute.  However, there is a recurrence relation among them ...

+++++++++++

To solve the problem, we partition the composite state into sub-states, so that the transition probability to the composite state is the summation of the transition probabilities to each of the sub-states. On the other hand, the transition probabilities to the sub-state have a recurrence relation and can be computed using Dynamic Programming. 

======================================

Note that every state $j$ with $j > 3$ in the Markov chain is a composite state as far as the calculation of the transition probability from a (larger) state $i > j$ to $j$ (i.e., ``transitioning into").  For example, State 6 contains 4 different cases. The first case is $6 = 6$, where all 6 bad balls are in the same bad bin. The second case is $6 = 2 + 4$ where, out of the 6 bad balls, four are in one bad bin and the other two are in the other bad bin.  Similarly, the other two cases are $6 = 3 + 3$ and $6 = 2 + 2 + 2$. Note there is no need to distinguish these four cases in calculating the ``transitioning out" probability (i.e., from state 6 to a small state say State 0), because the next round of balls-into-bins operation uses a different hash function independent of that used in the current round, and consequently how these 6 bad balls are split in the current round have no bearing on that in the next round. 

Building on the example above, we now consider $m_{9,6}$, the transition probability from State $9$ to State $6$ (throwing 9 balls into 255 bins and ending up with 6 bad balls).  $m_{9,6}$ is simply the sum of the probabilities of these four cases, each of which has a very different formula than the others.  In general, the number of such cases, and hence the number of individual probability terms to be added up to arrive at the transition matrix element $m_{i,j}$, grows exponentially with the value of $j$. This does not however make it difficult to calculate the values of $M$, because there is a recursive structure, among the values of the matrix elements $m_{i,j}$, that can be exploited using dynamic programming, as will be elaborated shortly.

To simplify our analysis, we split each composite state into sub-composite states based on the number of nonempty bins: Let State $(j,k)$ denotes the sub-composite state with $j$ remaining distinct elements and $k$ nonempty bins, which is also a substate of State $j$. Let $m_{i,j}^{(k)}$ denote the probability of transition from State $i$ to State $(j,k)$, which is also the probability that after throwing $i$ balls uniformly and independently into $n$ bins, $i-j$ bins are ``good'' bins and $k$ bins are nonempty bins (thus $k-(i-j)$ bins are ``bad'' and $n-k$ bins are empty). The probability of transition to a composite state is simply the summation of the probabilities of the transitions to corresponding sub-composite states:

To obtain the transition matrix $M$, it is sufficient to compute $m^{(k)}_{i,j}$, which can be exploited using dynamic programming. Note that the balls-and-bins model itself can be considered as a Markov chain, in which a recursive relation exists: After throwing $i$ balls into $n$ bins, throwing one more ball randomly could be: (1) Into an empty bin and turn it to a ``good'' bin; (2) Into a ``good'' bin and turn it to a ``bad'' bin with two balls; or (3) Into a ``bad'' bin and keep it as the same. Mathematically, we have $m^{(k)}_{i+1,j}$ equals to


====================================


%{\bf (may be unnecessary) Note that both the success probability and the overall communication overhead are strictly increasing w.r.t. $n$ and $t$. Hence, instead of computing all values in the table, we could strategically compute only a few of them and obtain the optimal $(n,t)$ (e.g., find the optimal $t$ for each $n$ by binary search each column).}







As we explained in \autoref{subsec:protocol2}, $d_1$, the number of distinct elements in group pair $1$, is a random variable that follows a Binomial distribution $Binomial(d,1/g)$. So the probability that the group pair is completely reconciled in $r$ rounds is $\sum_{x=0}^d Pr[d_1=x]\cdot Pr[x\xrsquigarrow{r} 0]$.
%, where $\mathcal{B}(\cdot;d,1/g)$ is the probability mass function (PMF) of $Binomial(d,1/g)$. 
To ease computation, we slightly underestimate this probability by assuming $Pr[x\xrsquigarrow{r} 0]=0$ when $x>t$ (i.e., assume group pair $1$ cannot be reconciled if $d_i>t$, discussed in \autoref{sec:BCH_exception}). The loss of this underestimation is very tiny, since the coefficient of $Pr[x\xrsquigarrow{r} 0]$ (i.e., $Pr[d_1=x]$) is very small when $x>t$. We denote this underestimated probability as $\alpha$ (i.e., $\alpha=\sum_{x=0}^t Pr[d_1=x]\cdot Pr[x\xrsquigarrow{r} 0]$). Note that $Pr[x\xrsquigarrow{r} 0]$ is a function of $n$ and $r$ for arbitrary $x$, so $\alpha$ is a function of $n$, $r$, $t$ for arbitrary $d$ and $g$. 


\subsection{Tail Bound Analysis for Each Group Pair}\label{sec:tail_bound_per_group}

In this section, we focus on analyzing an arbitrary group pair, which we denote as $(A',B')$, and suppose their set difference $A'\Delta B'$ contains exactly $x$ elements. We only consider the case that the error-correct capability is sufficient (i.e., $x\leq t$). As we described in \autoref{sec:multi-rounds}, the $x$ distinct elements are hashed into $n$ subset pairs in the first round, and a distinct element is reconciled if and only if it is hashed into a subset pair that contains only $1$ distinct element. The distinct elements that have been reconciled in the first round are removed and the other distinct elements (i.e., the ones that have not been reconciled yet in the first round) will be hashed again in the second round using a different hash function, so on so force. 


% WLOG, we only analyze group pair $1$. {\bf Maybe say that we focus on an arbitrary group pair, which we denote as A' and B', and suppose their difference $ ... $ contains exactly $x$ elements}. 
% %The analysis for other group pairs is the same. 
% {\bf Please use x, not d}.  
% For the moment, we slightly abuse the notation and use $d$ to denote the number of distinct elements in group pair $1$ (i.e., $d_1$). In this section, we only consider the case that the error-correct capability is sufficient (i.e., $d\leq t$). As we described in \autoref{sec:multi-rounds}, the $d$ distinct elements of group pair $1$ are hashed into $n$ subset pairs in the first round, and a distinct element is reconciled if and only if it is hashed into a subset pair that contains only $1$ distinct element. The distinct elements that have been reconciled in the first round are removed and the other distinct elements (i.e., the ones that have not been reconciled yet in the first round) will be hashed again in the second round using a different hash function, so on so force. 

==========
{\bf The following may be useful in explaining why it is a Markov chain:} [Note there is no need to distinguish these four cases in calculating the ``transitioning out" probability (i.e., from state 6 to a small state say State 0), because the next round of balls-into-bins operation uses a different hash function independent of that used in the current round, and consequently how these 6 bad balls are split in the current round have no bearing on that in the next round.]  {\bf unless you have done so earlier}

{\bf we have an example at the end of multi-round PBS}
==========


As we explained in \autoref{sec:hash_partition}, how the $x$ distinct elements are distributed into $n$ subset pairs in the first round follows the familiar {\it balls-into-bins} probability model: Each of the $x$ balls are thrown independently and uniformly at random into one of the $n$ bins. Each distinct element that is reconciled in the first round corresponds to a ball that ends up in a bin that receives exactly $1$ ball. We call the ball and the bin ``good'' in the sequel; Each distinct element that has not been reconciled yet in the first round corresponds to a ball that ends up in a bin that receives multiple balls. We call the ball and the bin ``bad'' in the sequel. Note that balls are either ``good'' or ``bad'', but bins could be empty besides ``good'' and ``bad''.



The ``bad'' balls in the first round will be the balls to be thrown in the second round. The ``bad'' balls in the second round will be the balls to be thrown in the third round, so on so force. In all rounds, how the balls are thrown into $n$ bins follows the balls-into-bins model. The dynamics of the number of balls to be thrown in each round can be modeled as a Markov chain, in which each state is defined as the number of balls to be thrown. In the Markov chain, a transition from state $i$ to state $j$ ($i\geq j$) means $i-j$ out of $i$ balls are ``good'' balls and the other $j$ balls are ``bad'' balls. The {\it absorbing state} of this Markov chain is state $0$, which is the ``good'' state that means all distinct elements have been reconciled (i.e., reconciliation is complete). For our analysis, the only probability that we concerned is $Pr[x\xrsquigarrow{r} 0]$, the probability that state $x$ (initial state) reaches the absorbing state (i.e., state $0$) in $r$ transitions, which is also the probability that all distinct elements are reconciled in $r$ rounds. This probability can be easily calculated given the transition matrix of the Markov chain: Let $M$ denote the $(t+1)\times (t+1)$ transition matrix of the Markov chain.
%, where $M(i,j)$ (i.e., the entry in the $i^{th}$ row and the $j^{th}$ column of $M$) is the probability of transition from state $i$ to state $j$ for $i,j = 0,1,...,t$
$Pr[x\xrsquigarrow{r} 0]$ equals to $\big{(}M^r\big{)}(x,0)$ (i.e., the entry in the $x^{th}$ row and the $0^{th}$ column of $M^r$). Here we slightly abuse the row / column numbers of a $(t+1)\times (t+1)$ matrix from $1,2,...,t+1$ to $0,1,...,t$, since the state of the Markov chain ranges from $0$ to $t$. 

\subsubsection{How to compute \texorpdfstring{$M$}{M}}

The only problem left to obtain $Pr[x\xrsquigarrow{r} 0]$ is how to compute $M$, which is not straightforward, since each state $j$ (after-transition state) with $j>3$ in the Markov chain is a composite state as far as the calculation of the transition probability from a (larger) state $i$ $(>j)$ to $j$ is concerned. To calculate the probability, we have to break state $j$ down into ``atom'' states, calculate the transition probability from state $i$ to each of the ``atom'' states (which can be directly calculated), and then add them up. {\bf Note that we always view state $i$ (pre-transition state) as a simple state, since how the $i$ balls are placed into $n$ bins only depends on a hash function that is independent of the ones used in previous rounds.}

Each composite state $j$ can be broken down into atom states based on how these $j$ bad balls are placed into the $n$ bins. For example, state $6$ consists of $4$ atom states. The first one is $6 = 6$, where all $6$ bad balls are in the same bad bin. The second one is $6 = 2 + 4$ where, out of the $6$ bad balls, four are in one bad bin and the other two are in the other bad bin.  Similarly, the other two atom states are $6 = 3 + 3$ and $6 = 2 + 2 + 2$. The transition probability from state $i$ to any atom state can be directly calculated, but the problem is that the number of atom states grows exponentially with the number of ``bad'' balls $j$.

We notice that we can break each composite state into a small number of coarse-grained sub-states, each of which may still contain a large number of atom states. The transition probability from a (larger) state $i$ to any sub-state is still hard to compute. However, there is a recurrence relation among them, so we can compute the transition probabilities from any state to any sub-state using Dynamic Programming. 




% Each ``atom'' state is, in combinatorics terms, {\it a permutation of a combination of $j$}, which here corresponds to 
% how these $j$ ``bad'' balls are placed into the $n$ bins. 
% For a simple example, when $j = 4$ and $n = 7$, the vector $(2, 0, 0, 0, 0, 2, 0)$ is such an ``atom'' state, which corresponds to these $7$ bins (in a predefined order such as the natural order) 
% have $2$, $0$, $0$, $0$, $0$, $2$, and $0$ ``bad'' balls in it respectively. The transition probability from state $i$ to any atom state can be calculated, but the problem is that the number of atom states 
% (permutations of combinations) grow exponentially with the number of balls $j$.


+++++++++++

The only problem left to obtain $Pr[d\xrsquigarrow{r} 0]$ is how to compute $M$, which is not straightforward, since each state $j$ with $j>3$ in the Markov chain is a composite state as far as the calculation of the transition probability from a (larger) state $i$ $(>j)$ to $j$ (i.e., ``transitioning into'') is concerned.   {\bf You need to explain why it is not straightforward:  The reason you offer is not
the direction reason.  Instead you may say that "the transition probability between these composite states cannot be directly calculated" ...  to calculate it we have to break it down into "atom" states}

Each composite state $i$ can be broken down into atom states as follows.  Each simple state is, in combinatorics terms, {\it a permutation of a combination of $i$}, which here corresponds to 
how these $i$ balls are ``divided up" by the $n$ bins.   {\bf Liang, Read Mitzenmacher and Upfal book
for a better word for "divided up"}
For a simple example, when $i = 4$ and $n = 7$, the vector (1, 0, 1, 0, 0, 2, 0) is such a simple state, which corresponds to these 7 bins (in a predefined order such as the natural order) 
have 1, 0, 1, 0, 0, 2, and 0 balls in it respectively.   The transition probability between any two atom states can be ...    but the problem is that the number of atom states 
(permutations of combinations) grow exponentially with the number of balls $i$.

Consider two states i1 and i2 each broken down into millions of atom states.  Then the transition probability between these states is the summation of the trillions (= millions * millions) of 
transition probabilities between atom states of i1 and atom states of i2.  

The good thing is that the transition probability matrix among the (humongous number of atom states) induces a "subproblem structure ????", which leads to the recurrence relation, 
dynamic programming.   

We notice that we can break each state into a small number of coarse-grained substates, each of which may still contain a large number of atom states.  The transition probability 
between any two such substates are still hard to compute.  However, there is a recurrence relation among them ...

+++++++++++

To solve the problem, we partition the composite state into sub-states, so that the transition probability to the composite state is the summation of the transition probabilities to each of the sub-states. On the other hand, the transition probabilities to the sub-state have a recurrence relation and can be computed using Dynamic Programming. 

======================================

Note that every state $j$ with $j > 3$ in the Markov chain is a composite state as far as the calculation of the transition probability from a (larger) state $i > j$ to $j$ (i.e., ``transitioning into").  For example, State 6 contains 4 different cases. The first case is $6 = 6$, where all 6 bad balls are in the same bad bin. The second case is $6 = 2 + 4$ where, out of the 6 bad balls, four are in one bad bin and the other two are in the other bad bin.  Similarly, the other two cases are $6 = 3 + 3$ and $6 = 2 + 2 + 2$. Note there is no need to distinguish these four cases in calculating the ``transitioning out" probability (i.e., from state 6 to a small state say State 0), because the next round of balls-into-bins operation uses a different hash function independent of that used in the current round, and consequently how these 6 bad balls are split in the current round have no bearing on that in the next round. 

Building on the example above, we now consider $m_{9,6}$, the transition probability from State $9$ to State $6$ (throwing 9 balls into 255 bins and ending up with 6 bad balls).  $m_{9,6}$ is simply the sum of the probabilities of these four cases, each of which has a very different formula than the others.  In general, the number of such cases, and hence the number of individual probability terms to be added up to arrive at the transition matrix element $m_{i,j}$, grows exponentially with the value of $j$. This does not however make it difficult to calculate the values of $M$, because there is a recursive structure, among the values of the matrix elements $m_{i,j}$, that can be exploited using dynamic programming, as will be elaborated shortly.

To simplify our analysis, we split each composite state into sub-composite states based on the number of nonempty bins: Let State $(j,k)$ denotes the sub-composite state with $j$ remaining distinct elements and $k$ nonempty bins, which is also a substate of State $j$. Let $m_{i,j}^{(k)}$ denote the probability of transition from State $i$ to State $(j,k)$, which is also the probability that after throwing $i$ balls uniformly and independently into $n$ bins, $i-j$ bins are ``good'' bins and $k$ bins are nonempty bins (thus $k-(i-j)$ bins are ``bad'' and $n-k$ bins are empty). The probability of transition to a composite state is simply the summation of the probabilities of the transitions to corresponding sub-composite states:

To obtain the transition matrix $M$, it is sufficient to compute $m^{(k)}_{i,j}$, which can be exploited using dynamic programming. Note that the balls-and-bins model itself can be considered as a Markov chain, in which a recursive relation exists: After throwing $i$ balls into $n$ bins, throwing one more ball randomly could be: (1) Into an empty bin and turn it to a ``good'' bin; (2) Into a ``good'' bin and turn it to a ``bad'' bin with two balls; or (3) Into a ``bad'' bin and keep it as the same. Mathematically, we have $m^{(k)}_{i+1,j}$ equals to


====================================

More specifically, let state $(j,k)$ denote the sub-state of state $j$ that the $j$ ``bad'' balls end up to occupy exactly $k$ ``bad'' bins. Then the composite state $j$ is partitioned into state $(j,1)$, state $(j,2)$, $...$, state $(j,j)$. We slightly abuse the notation and let $M(i,j,k)$ denote the probability of transition from state $i$ to state $(j,k)$, then we have 

\begin{equation}
    M(i,j) = \sum_{k=1}^{j} M(i,j,k)
\end{equation}

{\bf we can use a tighter range of $k$ of $1,2,..., \lfloor j/2 \rfloor$. For cleanness, I choose a wider range of $1,2,..., j$, which is easier to understand and does not change the result}

To obtain $M$, it is sufficient to compute $M(i,j,k)$ for $\forall i,j,k=0,1,...,t$
{\bf Similarly, there is a tighter range for $i,j,k$, which seems to be unnecessary}
. Note that the state transition resulting from throwing one ball after another is also a Markov chain, in which state $(i,j,k)$ is defined as $j$ ``bad'' balls ending up into $k$ ``bad'' bins after throwing $i$ balls into $n$ bins. In this Markov chain, throwing one more ball can transition state $(i,j,k)$ to three possible states depending on the $(i+1)^{th}$ ball ending up in (1) a ``good'' bin; (2) a ``bad'' bin; or (3) an empty bin. The first case happens with probability $(i-j)/n$, results in $2$ additional ``bad'' balls and $1$ additional ``bad'' bin (i.e., transition to state $(i+1,j+2,k+1)$). The second and third cases transition to state $(i+1,j+1,k)$ and state $(i+1,j,k)$ respectively with probability $k/n$ and $1-(i-j+k)/n$. In the opposite direction, state $(i+1,j,k)$ can only be transitioned from (1) state $(i,j-2,k-1)$; (2) state $(i,j-1,k)$; and (3) state $(i,j,k)$, which gives us a recurrence relation that $M(i+1,j,k)$ equals to

%The second case happens with probability $k/n$ and results in state $(i+1,j+1,k)$. The third case happens with probability $1-(i-j+k)/n$ and results in state $(i+1,j,k)$. In the opposite direction, state $(i+1,j,k)$ can be transitioned from (1) state $(i,j-2,k-1)$ with probability $(i-j+2)/n$; (2) state $(i,j-1,k)$ with probability $k/n$; or (3) state $(i,j,k)$ with probability $1-(i-j+k)/n$. It gives us a recurrence relation that $P(i+1,j,k)$ equals to

\begin{equation}\label{eq:recursion}
    \frac{i\!-\!j\!+\!2}{n}\cdot M(i,j\!-\!1,k\!-\!1)+\frac{k}{n}\cdot M(i,j\!-\!1,k)+(1\!-\!\frac{i\!-\!j\!+\!2}{n})\cdot M(i,j,k)
\end{equation}

The three terms in \autoref{eq:recursion} corresponds to the above three possible transitions. Combining with the following probabilities in base cases, we can compute $M(i,j,k)$ for $\forall i,j,k=0,1,...,t$ using Dynamic Programming and obtain $M$:

\begin{align}
M(0,j,k) =& \left\{ \begin{array}{ccl}
1, & \mbox{if }
 j=k=0 \\ 0, & \mbox{otherwise} 
\end{array}\right.\label{eq:basic1}\\
M(i,0,k) =& \left\{ \begin{array}{ccl}
\binom{n}{i}/n^i, & \mbox{if }
 k=0 \\ 0, & \mbox{otherwise} 
\end{array}\right.\label{eq:basic2}\\
M(i,j,0) =& \left\{ \begin{array}{ccl}
1, & \mbox{if }
 j=0 \\ 0, & \mbox{otherwise} 
\end{array}\right.\label{eq:basic3}
\end{align}

%As mentioned earlier, we slightly abuse the notation `$d$' in this section to denote the number of distinct elements in group pair $1$, which is actually $d_1$ defined in \autoref{subsec:protocol2}. Now we recover the abused notation $d$ to denote the total number of distinct elements in all groups. 

As we explained in \autoref{subsec:protocol2}, $d_1$, the number of distinct elements in group pair $1$, is a random variable that follows a Binomial distribution $Binomial(d,1/g)$. So the probability that the group pair is completely reconciled in $r$ rounds is $\sum_{x=0}^d Pr[d_1=x]\cdot Pr[x\xrsquigarrow{r} 0]$.
%, where $\mathcal{B}(\cdot;d,1/g)$ is the probability mass function (PMF) of $Binomial(d,1/g)$. 
To ease computation, we slightly underestimate this probability by assuming $Pr[x\xrsquigarrow{r} 0]=0$ when $x>t$ (i.e., assume group pair $1$ cannot be reconciled if $d_i>t$, discussed in \autoref{sec:BCH_exception}). The loss of this underestimation is very tiny, since the coefficient of $Pr[x\xrsquigarrow{r} 0]$ (i.e., $Pr[d_1=x]$) is very small when $x>t$. We denote this underestimated probability as $\alpha$ (i.e., $\alpha=\sum_{x=0}^t Pr[d_1=x]\cdot Pr[x\xrsquigarrow{r} 0]$). Note that $Pr[x\xrsquigarrow{r} 0]$ is a function of $n$ and $r$ for arbitrary $x$, so $\alpha$ is a function of $n$, $r$, $t$ for arbitrary $d$ and $g$. 

\subsection{Tail Bound Analysis for all groups}\label{sec:times2bound}

Given $\alpha$, the tail bound of the probability that a group pair is successfully reconciled in $r$ rounds, we can easily derive a tail bound of $\alpha^g=1-(1-\alpha^g)$ for the probability that all group pairs are successfully reconciled in $r$ rounds, if we assume the reconciliations on group pairs are independent with each other. However, this assumption is not rigorous, since $d_1, d_2,...,d_g$ have a weak correlation that $\sum_{i=1}^g d_i=d$. 
%Fortunately, we have Times-2-Bound (Theorem 1 in \cite{hua2008rank}) to decouple the weak correlation and give us a rigorous tail bound of $1-2(1-\alpha^g)$ for the probability of all group pairs. 
To be rigorous, we use so-called Times-2-bound (Corollary 5.11 in \cite{upfal2005probability}) to decouple the weak correlation and obtain a rigorous tail bound of $1-2(1-\alpha^g)$ for the probability of all group pairs.
In \autoref{sec:parameter_settings}, we use the tail bound of $1-2(1-\alpha^g)$ in parameter settings for rigorousness. 

% More specifically, let state $(j,k)$ denote the sub-state of state $j$ that the $j$ ``bad'' balls end up to occupy exactly $k$ ``bad'' bins. Then the composite state $j$ is the union of state $(j,1)$, state $(j,2)$, $...$, state $(j,\lfloor j/2 \rfloor)$ (each ``bad'' bin receives at least $2$ ``bad'' balls, so $k\leq \lfloor j/2\rfloor$). Let $P(i,j,k)$ denote the probability of transition from state $i$ to state $(j,k)$, then we have 

% \begin{equation}
%     M(i,j) = \sum_{k=1}^{\lfloor j/2\rfloor} P(i,j,k)
% \end{equation}






% Note that each state $j$ with $j>3$ in the Markov chain is a composite state as far as the calculation of the transition probability from a (larger) state $i$ $(>j)$ to $j$ (i.e., ``transitioning into''). Such a composite state $j$ can be decomposed into sub-states based on the number of ``bad'' bins after throwing $i$ balls: Define state $(j,k)$ as the sub-state of state $j$ that the  $j$ ``bad'' balls end up to occupy exactly $k$ ``bad'' bins. Then state $j$ is the union of all states $(j,k)$ for $k=1,2,...$ (each ``bad'' bin receives at least $2$ ``bad'' balls). Let $m_{i,j}^{(k)}$ denote the probability of transition from state $i$ to state $(j,k)$
% %, which is also the probability that after throwing $i$ balls uniformly and independently into $n$ bins, $i-j$ bins are ``good'' bins and $k$ bins are nonempty bins (thus $k-(i-j)$ bins are ``bad'' and $n-k$ bins are empty)
% . The probability of transition to the composite state $j$ is simply the summation of the probabilities of the transitions to corresponding sub-states: 

% \begin{equation}
%     m_{i,j} = \sum_{k=i}^{i-j} m^{(k)}_{i,j}
% \end{equation}


% To make our description simple, we call a bin that receives exactly $1$ ball a ``good'' bin is ``good'' if and only if it receives exactly $1$ ball. We call a bin is ``bad'' if and only if it receives more than $1$ balls. The rest bins (i.e., neither ``good'' nor ``bad'') are empty. We call a ball ending up in a ``good'' bin is ``good'' if it is in a ``good bin'' Then the distinct elements that are decoded correspond to the balls that are in ``good'' bins. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Old version of 2/5
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{comment}

In this section, we only consider the cases that a group is able to be decoded by BCH code (i.e., initially contains at most $t$ set differences). Without loss of generosity, we assume the group has $d (\leq t)$ distinct elements and is partitioned into $n$ subset pairs. As we described in \autoref{sec:hash_partition}, the $d$ distinct elements are hashed into $n$ subset pairs in each round, and a distinct element is decoded if and only if it is hashed into a subset pair that contains only $1$ distinct element. As we introduced in \autoref{sec:hash_partition}, the statistical model for hashing $d$ distinct elements into $n$ subset pairs is the same as the classical balls-and-bins problem: $d$ balls are thrown independently and uniformly at random into $n$ bins. To make our description simple, we call a bin is ``good'' if and only if it receives exactly $1$ ball. And we call a bin is ``bad'' if and only if it receives more than $1$ balls. The rest bins (i.e., neither ``good'' nor ``bad'') are empty. Then the distinct elements that are decoded correspond to the balls that are in ``good'' bins. 

The decode process of each group can be considered as a Markov Chain, in which each state is defined as the number of remaining distinct elements (i.e., the distinct elements that haven't been decoded). In this Markov chain, the transition from State $i$ to State $j$ means $i-j$ out of $i$ distinct elements are decoded in this round, where $0\leq j\leq i\leq t$. Use the same analogy, the number (state) is simply the total number of balls that fall in ``bad'' bins. The transition from State $i$ to State $j$ means $i-j$ out of $i$ balls fall in ``good'' bins in this round, while the rest $j$ balls fall in ``bad'' bins. State $0$ is the {\it absorbing} state of this Markov Chain, which means all distinct elements have been reconciled. For our analysis, we only concern the probability that after $r$ rounds, the final state is state $0$ (i.e., absorbing state) when the initial state is state $i$. We denote this probability as $v^{(r)}_i(0)$.

Let $M=(m_{i,j})_{(t+1)\times (t+1)}$ denote the transition matrix of the above Markov chain, where $m_{i,j}$ is the probability of transition from State $i$ to State $j$. Given $M$, $r$, and the initial state $i$, $v^{(r)}_i(0)$ can be easily calculated. So the only problem is how to obtain $M$, which will be elaborated in the next section.

\subsubsection{Transition Matrix}\label{sec:transition_matrix}

Now we describe how to compute the transition matrix $M$ using dynamic programming in detail. Note that every State $j$ with $j > 3$ in the Markov chain is a composite state as far as the calculation of the transition probability from a (larger) state $i > j$ to $j$ (i.e., ``transitioning into").  For example, State 6 contains 4 different cases. The first case is $6 = 6$, where all 6 bad balls are in the same bad bin. The second case is $6 = 2 + 4$ where, out of the 6 bad balls, four are in one bad bin and the other two are in the other bad bin.  Similarly, the other two cases are $6 = 3 + 3$ and $6 = 2 + 2 + 2$. Note there is no need to distinguish these four cases in calculating the ``transitioning out" probability (i.e., from state 6 to a small state say State 0), because the next round of balls-into-bins operation uses a different hash function independent of that used in the current round, and consequently how these 6 bad balls are split in the current round have no bearing on that in the next round. 

Building on the example above, we now consider $m_{9,6}$, the transition probability from State $9$ to State $6$ (throwing 9 balls into 255 bins and ending up with 6 bad balls).  $m_{9,6}$ is simply the sum of the probabilities of these four cases, each of which has a very different formula than the others.  In general, the number of such cases, and hence the number of individual probability terms to be added up to arrive at the transition matrix element $m_{i,j}$, grows exponentially with the value of $j$. This does not however make it difficult to calculate the values of $M$, because there is a recursive structure, among the values of the matrix elements $m_{i,j}$, that can be exploited using dynamic programming, as will be elaborated shortly.

To simply our analysis, we split each composite state into sub-composite states based on the number of nonempty bins: Let State $(j,k)$ denotes the sub-composite state with $j$ remaining distinct elements and $k$ nonempty bins, which is also a substate of State $j$. Let $m_{i,j}^{(k)}$ denote the probability of transition from State $i$ to State $(j,k)$, which is also the probability that after throwing $i$ balls uniformly and independently into $n$ bins, $i-j$ bins are ``good'' bins and $k$ bins are nonempty bins (thus $k-(i-j)$ bins are ``bad'' and $n-k$ bins are empty). The probability of transition to a composite state is simply the summation of the probabilities of the transitions to corresponding sub-composite states:

\begin{equation}
    m_{i,j} = \sum_{k=i}^{i-j} m^{(k)}_{i,j}
\end{equation}

To obtain the transition matrix $M$, it is sufficient to compute $m^{(k)}_{i,j}$, which can be exploited using dynamic programming. Note that the balls-and-bins model itself can be considered as a Markov chain, in which a recursive relation exists: After throwing $i$ balls into $n$ bins, throwing one more ball randomly could be: (1) Into an empty bin and turn it to a ``good'' bin; (2) Into a ``good'' bin and turn it to a ``bad'' bin with two balls; or (3) Into a ``bad'' bin and keep it as the same. Mathematically, we have $m^{(k)}_{i+1,j}$ equals to

\begin{equation}\label{eq:recursion}
\frac{n-k+1}{n}\cdot m^{(k-1)}_{i,j-1} + \frac{j+1}{n}\cdot m^{(k)}_{i,j+1} + \frac{k-(i-j)}{n}\cdot m^{(k)}_{i,j} \nonumber
\end{equation}

The three terms in \autoref{eq:recursion} corresponds to the above three cases. Meanwhile, we can easily get the boundary conditions as follows:

\begin{align}
m^{(k)}_{i,0} =& \left\{ \begin{array}{ccl}
\binom{n}{i}/n^i, & \mbox{if }
 k=i \\ 0, & \mbox{otherwise} 
\end{array}\right.\label{eq:basic1}\\
m^{(k)}_{0,j} =& \left\{ \begin{array}{ccl}
1, & \mbox{if }
 k=0 \mbox{ and } j=0 \\ 0, & \mbox{otherwise} 
\end{array}\right.\label{eq:basic2}\\
m^{(0)}_{i,j} =& \left\{ \begin{array}{ccl}
1, & \mbox{if }
 i=0 \mbox{ and } j=0 \\ 0, & \mbox{otherwise} 
\end{array}\right.\label{eq:basic3}
\end{align}

Using \autoref{eq:recursion},\autoref{eq:basic1},\autoref{eq:basic2}, and \autoref{eq:basic3}, we can recursively compute $m^{(k)}_{i,j}$ and obtain $M$.


\subsection{Global Tail Bound Analysis}\label{sec:times2bound}

Consider group $1$ (other groups have the same result), the probability that all distinct elements in group $1$ are reconciled in $r$ rounds is $\sum_{i=0}^d Pr[d_1=i]v_i^{(r)}(0)\triangleq \alpha$, where $d_1$ (i.e., the number of distinct elements in group $1$) is a Binomial random variable $Binomial(d,1/g)$ as we explained in \autoref{subsec:protocol2}. To ease computation, we slightly underestimate this probability $\alpha$ by assuming $v_i^{(r)}(0)=0$ when $i>t$ (i.e., assume group $i$ cannot reconcile if $d_i>t$, discussed in \autoref{sec:BCH_exception}). The loss of this underestimation is very tiny, since the coefficient of $v_i^{(r)}(0)$ (i.e., $Pr[d_1=i]$) is very small when $i>t$.

The probability that all groups are successfully reconciled in $r$ rounds is simply $\alpha^g\triangleq \beta$, if we assume the reconciliations on groups are independent with each other. This assumption is however not rigorous, since $d_1, d_2,...,d_g$ have a weak correlation that $\sum_{i=1}^g d_i=d$. Fortunately, we have Times-2-Bound (Theorem 1 in \cite{hua2008rank}) to decouple the weak correlation and give us a rigorous bound of $2\beta-1$. In \autoref{sec:parameter_settings}, we use this rigorous bound for parameter settings. 

\end{comment}






\begin{comment}

Let $v^{(r)}_i=\big{(}{v^{(r)}_i(0), v^{(r)}_i(1),...,v^{(r)}_i(t)}\big{)}$ denote the probability vector (i.e., $\sum_{j=0}^{t}v^{(r)}_i(j) = 1$) after $r$ rounds with initial State $i$: $v^{(r)}_i(j)$ denotes the probability that the final state is State $j$ after $r$ rounds. In the probability vector, $v^{(r)}_i(0)$ is the only entry that we concern, which is the probability of the cases that all distinct elements are decoded after $r$ rounds. Given 

Note that every State $j$ with $j > 3$ in the Markov chain is a composite state as far as the calculation of the transition probability from a (larger) state $i > j$ to $j$ (i.e., ``transitioning into").  For example, State 6 contains 4 different cases. The first case is $6 = 6$, where all 6 bad balls are in the same bad bin. The second case is $6 = 2 + 4$ where, out of the 6 bad balls, four are in one bad bin and the other two are in the other bad bin.  Similarly, the other two cases are $6 = 3 + 3$ and $6 = 2 + 2 + 2$. Note there is no need to distinguish these four cases in calculating the ``transitioning out" probability (i.e., from state 6 to a small state say State 0), because the next round of balls-into-bins operation uses a different hash function independent of that used in the current round, and consequently how these 6 bad balls are split in the current round have no bearing on that in the next round. 

Building on the example above, we now consider $m_{9,6}$, the transition probability from State $9$ to State $6$ (throwing 9 balls into 255 bins and ending up with 6 bad balls).  $m_{9,6}$ is simply the sum of the probabilities of these four cases, each of which has a very different formula than the others.  In general, the number of such cases, and hence the number of individual probability terms to be added up to arrive at the transition matrix element $m_{i,j}$, grows exponentially with the value of $j$. This does not however make it difficult to calculate the values of $M$, because there is a recursive structure, among the values of the matrix elements $m_{i,j}$, that can be exploited using dynamic programming, as will be elaborated in \autoref{sec:transition_matrix}.

Let $v^{(r)}_i=\big{(}{v^{(r)}_i(0), v^{(r)}_i(1),...,v^{(r)}_i(t)}\big{)}$ denote the probability vector (i.e., $\sum_{j=0}^{t}v^{(r)}_i(j) = 1$) after $r$ rounds with initial State $i$: $v^{(r)}_i(j)$ denotes the probability that the final state is State $j$ after $r$ rounds. In the probability vector, $v^{(r)}_i(0)$ is the only ``good'' entry, which is the probability of the cases that all distinct elements are decoded after $r$ rounds. The probability of the group does not complete reconciliation is simply $1-v^{(r)}_i(0)$. 

Given the transition matrix $M$, we can easily compute the probability vector $v^{(r)}_i$ for any $r$ and $i$ as follows:
\begin{equation}
    x^{(r)}_i = e_i\cdot M^r
\end{equation}
Here $\{e_i\}_{i=0,1,2,...,t}$ denote the standard basis vectors of length $t+1$, where $e_i$ has a single nonzero value 1 at the $(i+1)^{th}$ position. So the remaining problem is how to compute $M$.

\subsubsection{Transition Matrix}\label{sec:transition_matrix}

Now we describe how to compute the transition matrix $M$ using dynamic programming in detail. As we described earlier, every State $j$ with $j > 3$ in the Markov chain is a composite state that contains many different cases. And the number of these cases increases exponentially with the value of $j$. To simply our analysis, we split each composite state into sub-composite states based on the number of nonempty bins: Let State $(j,k)$ denotes the sub-composite state with $j$ remaining distinct elements and $k$ nonempty bins, which is also a substate of State $j$. Let $m_{i,j}^{(k)}$ denote the probability of transition from State $i$ to State $(j,k)$, which is also the probability that after throwing $i$ balls uniformly and independently into $n$ bins, $i-j$ bins are ``good'' bins and $k$ bins are nonempty bins (thus $k-(i-j)$ bins are ``bad'' and $n-k$ bins are empty). The probability of transition to a composite state is simply the summation of the probabilities of the transitions to corresponding sub-composite states:

\begin{equation}
    m_{i,j} = \sum_{k=i}^{i-j} m^{(k)}_{i,j}
\end{equation}

To obtain the transition matrix $M$, it is sufficient to compute $m^{(k)}_{i,j}$, which can be exploited using dynamic programming. Note that the balls-and-bins model itself can be considered as a Markov chain, in which a recursive relation exists: After throwing $i$ balls into $n$ bins, throwing one more ball randomly could be: (1) Into an empty bin and turn it to a ``good'' bin; (2) Into a ``good'' bin and turn it to a ``bad'' bin with two balls; or (3) Into a ``bad'' bin and keep it as the same. Mathematically, we have 

\begin{align}
m^{(k)}_{i+1,j} =& \frac{n-k+1}{n}\cdot m^{(k-1)}_{i,j-1} + \frac{j+1}{n}\cdot m^{(k)}_{i,j+1} \nonumber\\
&+ \frac{k-(i-j)}{n}\cdot m^{(k)}_{i,j} \label{eq:recursion}
\end{align}

The three terms in \autoref{eq:recursion} corresponds to the above three cases. Meanwhile, we can easily get the following probabilities for basic cases:

\begin{align}
m^{(k)}_{i,0} =& \left\{ \begin{array}{ccl}
\binom{n}{i}/n^i, & \mbox{if }
 k=i \\ 0, & \mbox{otherwise} 
\end{array}\right.\label{eq:basic1}\\
m^{(k)}_{0,j} =& \left\{ \begin{array}{ccl}
1, & \mbox{if }
 k=0 \mbox{ and } j=0 \\ 0, & \mbox{otherwise} 
\end{array}\right.\label{eq:basic2}\\
m^{(0)}_{i,j} =& \left\{ \begin{array}{ccl}
1, & \mbox{if }
 i=0 \mbox{ and } j=0 \\ 0, & \mbox{otherwise} 
\end{array}\right.\label{eq:basic3}
\end{align}

Using \autoref{eq:recursion},\autoref{eq:basic1},\autoref{eq:basic2}, and \autoref{eq:basic3}, we can recursively compute $m^{(k)}_{i,j}$ and then get $v^{(r)}_i(0)$ for $\forall i=0,1,...,n$ and $r\in\mathbb{Z}$. The value of $v^{(r)}_i(0)$ will be used to compute the tail bound of $Pr[P^{(r)}_o]$ in the next section. 

\subsection{Global Tail Bound Analysis}\label{sec:times2bound}

Let random variable $X^{(d)}_i, 1\leq i\leq g$, denote the number of set differences initially allocated in the $i^{th}$ group. For an analogy, the statistical model for hashing $d$ set differences into $g$ groups is also the same as the classical balls-and-bins problem: $d$ balls are thrown independently and uniformly at random into $g$ bins. Then random variable $X^{(d)}_i$ could be translated as the number of balls ended up in the $i^{th}$ bin after $d$ balls are thrown. Therefore, $(X^{(d)}_1,...,X^{(d)}_g)$ follows the multinomial distribution. The marginal distribution for any $X^{(d)}_i$ is $Binomial(d,\frac{1}{g})$, where $Binomial(N,p)$ denotes the binomial distribution resulting from $N$ trials with success probability $p$. 

Let $f^{(r)}(x_1,x_2,...,x_g)$ denote the probability that set reconciliation does not complete (for all groups) in $r$ rounds when the $i^{th}$ group initially contains $x_i$ set differences for $i=1,2,...,g$. Define $f^{(r)}(x)$ as the probability that set reconciliation does not complete in $r$ rounds when a group initially contains $x$ set differences. Based on the result in \autoref{sec:tail_bound_per_group}, we have 

% \begin{equation}\label{eq:frx}
%     f^{(r)}(x) \leq g^{(r)}(x) \triangleq \left\{ \begin{array}{ccc}
% 1-v^{(r)}_{x}(0) & \mbox{for}
% & 0\leq x\leq c \\ 1 & \mbox{for} & x>c
% \end{array}\right.
% \end{equation}

\begin{equation}\label{eq:frx}
    f^{(r)}(x) = 1-v^{(r)}_{x}(0) \mbox{ for }  0\leq x\leq t 
\end{equation}

Since the reconciliation processes independently for each group, we have 

\begin{equation}
f^{(r)}(x_1,x_2,...,x_g) = 1-\prod_{i=1}^g \big{(}1-f^{(r)}(x_i)\big{)}
\end{equation}

Then we have 

\begin{align} 
Pr[P^{(r)}_o] 
&= E[f^{(r)}(X^{(d)}_1,X^{(d)}_2,...,X^{(d)}_g)] \label{eq:errorBound0}\\
&= 1-E[\prod_{i=1}^g \big{(}1-f^{(r)}(X^{(d)}_i)\big{)}] \label{eq:errorBound1}
\end{align}

A naive approach to calculating the probability $Pr[P^{(r)}_o]$ is to regard $X^{(d)}_i$ as mutually independent. Then we have

\begin{align} 
Pr[P^{(r)}_o] 
&= 1-\prod_{i=1}^g E[1-f^{(r)}(X^{(d)}_i)] \label{eq:errorBound2}\\
&= 1-\prod_{i=1}^g (1-E[f^{(r)}(X^{(d)}_i)]) \label{eq:errorBound3}\\
&= 1-(1-E[f^{(r)}(X^{(d)}_i)])^g \label{eq:errorBound4}
\end{align}

And the term $E[f^{(r)}(X^{(d)}_1)]$ in \autoref{eq:errorBound4} can be easily bounded by \autoref{eq:frx} as follows:

\begin{align}
& E[f^{(r)}(X^{(d)}_1)]\\
= &\sum_{k=0}^d \mathcal{B}(k;d,\frac{1}{n})f^{(r)}(k)\\
= &\sum_{k=0}^t \mathcal{B}(k;d,\frac{1}{n})f^{(r)}(k) + \sum_{k=t+1}^d \mathcal{B}(k;d,\frac{1}{n})f^{(r)}(k)\label{eq:beforeLeq}\\
\leq & \sum_{k=0}^t \mathcal{B}(k;d,\frac{1}{n})f^{(r)}(k) + \sum_{k=t+1}^d \mathcal{B}(k;d,\frac{1}{n})\label{eq:afterLeq}\\
= & \sum_{k=0}^t \mathcal{B}(k;d,\frac{1}{n})\big{(}1-v_k^{(r)}(0)\big{)}+\sum_{k=t+1}^d \mathcal{B}(k;d,\frac{1}{n})
\end{align}

Here $\mathcal{B}(k;d,\frac{1}{n})$ is the Binomial probability mass function, and how to compute $v_k^{(r)}(0)$ is discussed in \autoref{sec:tail_bound_per_group} for $\forall k=0,1,...,t$ and $r\in\mathbb{Z}$. From \autoref{eq:beforeLeq} to \autoref{eq:afterLeq}, the loss is very negligible, since $\mathcal{B}(k;d,\frac{1}{n})$ is very small when $k>t$ ($t$ is $2-3$ times of $d/n$).

However, those random variable $X^{(d)}_i$ are not totally independent since they are conditioned by $\sum_{i=1}^g X^{(d)}_i=d$. So the above bound is not rigorous. Fortunately, we have the following theorem (Times-2-Bound) to decouple the weak correlation among $(X^{(d)}_1,...,X^{(d)}_m)$ and bound $Pr[P^{(r)}_o]$ rigorously to be $2$ times of the unrigorous bound in \autoref{eq:errorBound3}. 

\textbf{Theorem 1} {\bf citation}
Let $(X^{(n)}_1,...,X^{(n)}_m)$ follows the multinomial distribution of throwing $n$ balls into $m$ bins. Let $(Y^{(n)}_1,...,Y^{(n)}_m)$ be independent and identically distributed random variables with distribution $Poission(\frac{n}{m})$. Let $f(x_1,...,x_m)$ be a nonnegative function which is increasing in each argument separately. Then
\begin{equation} \label{eq:times2bound}
E[f(X^{(n)}_1,X^{(n)}_2,...,X^{(n)}_m)] \leq 2E[f(Y^{(n)}_1,Y^{(n)}_2,...,Y^{(n)}_m)]
\end{equation}


A naive approach to calculating the probability $Pr[P^{(r)}_o]$ is to regard $X^{(d)}_i$ as mutually independent. In this case, the production in the expectation of \autoref{eq:errorBound1} can be extracted out of the expectation and hence could be easily bounded. However, those random variable $X^{(d)}_i$ are not totally independent since they are conditioned by $\sum_{i=1}^m X^{(d)}_i=d$. Fortunately, we have the following theorem to decouple the weak correlation among $(X^{(d)}_1,...,X^{(d)}_m)$ and bound our targeted probability.

\textbf{Theorem 1}
Let $(X^{(n)}_1,...,X^{(n)}_m)$ follows the multinomial distribution of throwing $n$ balls into $m$ bins. Let $(Y^{(n)}_1,...,Y^{(n)}_m)$ be independent and identically distributed random variables with distribution $Poission(\frac{n}{m})$. Let $f(x_1,...,x_m)$ be a nonnegative function which is increasing in each argument separately. Then
\begin{equation} \label{eq:times2bound}
E[f(X^{(n)}_1,X^{(n)}_2,...,X^{(n)}_m)] \leq 2E[f(Y^{(n)}_1,Y^{(n)}_2,...,Y^{(n)}_m)]
\end{equation}

Substitute \autoref{eq:times2bound} into \autoref{eq:errorBound0}, we have
\begin{align} 
Pr[P^{(r)}_o] 
&= E[f^{(r)}(X^{(d)}_1,X^{(d)}_2,...,X^{(d)}_m)] \\
&\leq 2E[f^{(r)}(Y^{(d)}_1,Y^{(d)}_2,...,Y^{(d)}_m)] \\
&= 2-2E[\prod_{i=1}^m \big{(}1-f^{(r)}(Y^{(d)}_i)\big{)}] \\
&= 2-2\prod_{i=1}^m \big{(}1-E[f^{(r)}(Y^{(d)}_i)]\big{)} \label{eq:beforeSimp}\\
&= 2-2\big{(}1-E[f^{(r)}(Y^{(d)}_1)]\big{)}^m \label{eq:afterSimp}\\
\end{align}

From \autoref{eq:beforeSimp} to \autoref{eq:afterSimp}, we use the property that $Y^{(d)}_i$, $i=1,2,...,m$ are i.i.d random variables with distribution $Poisson(\delta)$ $(\delta = \frac{d}{m})$. And the term $E[f^{(r)}(Y^{(d)}_1)]$ in \autoref{eq:afterSimp} can be easily bounded by \autoref{eq:frx} as follows:

\begin{align}
& E[f^{(r)}(Y^{(d)}_1)]\\
= &\sum_{k=0}^d p(k;\delta)f^{(r)}(k)\\
= &\sum_{k=0}^c p(k;\delta)f^{(r)}(k) + \sum_{k=c+1}^d p(k;\delta)f^{(r)}(k)\label{eq:beforeLeq}\\
\leq & \sum_{k=0}^c p(k;\delta)f^{(r)}(k) + \sum_{k=c+1}^d p(k;\delta)\label{eq:afterLeq}\\
= & \sum_{k=0}^c p(k;\delta)\big{(}1-v_k^{(r)}(0)\big{)}+\sum_{k=c+1}^d p(k;\delta)
\end{align}

Here $p(k;\delta)$ is the Poisson probability mass function, and how to compute $v_k^{(r)}(0)$ is discussed in \autoref{sec:tail_bound_per_group} for $\forall k=0,1,...,c$ and $r\in\mathbb{Z}$. From \autoref{eq:beforeLeq} to \autoref{eq:afterLeq}, the loss is very negligible, since $p(k;\delta)$ is very small when $k>c$ ($c>2\delta$).


\subsection{Parameter Settings}\label{sec:parameter_settings}

% The tail bound is based on the total number of distinct elements $d$, which is however not known precisely. The ToW Estimator introduced in \autoref{subsec:ToW} can only provide an estimation of $d$ (denoted as $\hat{d}$). Note that the tail bound of $Pr[P^{(r)}_o]$ increases as $d$ increases. So overestimate $d$ will get us a larger failure probability $Pr[P^{(r)}_o]$. To ensure a high success probability, we use an overestimated number of distinct element $\bar{d}$ $(>\hat{d})$ for parameter settings, such that $\bar{d}\geq d$ with high probability. In our evaluation, we set $\bar{d}\triangleq 1.38\hat{d}$, such that $\bar{d}\geq d$ with probability $99\%$. 

In this section, we elaborate how to set the parameters (i.e., $n$, $t$, $g$) given $d$ and the objective $(r,p_0)$ (defined in \autoref{subsec:protocol2}) in PBS. For the moment, we assume $d$ is precisely known. 
Given the objective $(r, p_0)$
%(i.e., set reconciliation is complete in $r$ rounds with probability $p_0$) 
%depend on the requirement of specific applications)
, the parameter setting problem aims to find the optimal parameter settings on $n,t,g$ that minimizes the overall communication overhead, under the constraint that the tail bound of the success probability in $r$ rounds is larger than $p_0$. As explained in \autoref{subsec:protocol2}, $\delta$ should be a small number, so we fix $\delta=5$ and therefore $g=d/\delta$ is also fixed. Note that the only two components in the communication overhead per group (described in \autoref{sec:multi-rounds}) that depend on parameter settings are $t\log n+\delta\log n$. So we can formalize the parameter setting problem as the following optimization problem:

\begin{equation}
\min\limits_{n,t} t\log n+\delta\log n \quad \mbox{s.t.}\quad 1-2(1-\alpha^g(n,t))>p_0
\end{equation}

\begin{align}
\mbox{minimize} \quad
&
t\log n+\delta\log n \label{obj:min_communication}
\\
\mbox{subject to} \quad 
&
1-2(1-\alpha^g(n,t))>p_0  \label{eq:success_rate_requirement}
\\
&
n,t\in \mathbb{N}^+ \label{eq:row_sum_requirement}
\end{align}

This optimization problem seems to be very difficult to solve, since the constraint is a very comprehensive function of the parameters (remind that $\alpha=\alpha(n,t)$ is a function of $n$ and $t$ for arbitrary $r$, $d$, and $g$). However, we can narrow down the solution space into only a few combinations and traverse all these combinations to find the optimal parameter settings as follows: First, for BCH coding efficiency, we select $n$ to be $2^m-1$ for some integer $m$ and therefore narrow its range down to $\{63,127,255,511,1023\}$ (recall that $n=\Omega(\delta^2)$). Second, we select $t$ in the range from $1.5\delta$ to $3\delta$, as we suggested in \autoref{subsec:protocol2}. 

Here we use an example to show how we set parameters: Given $d=1000$, $r=3$, $p_0=0.99\%$, for each $(n,t)$ combination in $\{63,127,255,511,1023\}\times \{8,9,...,15\}$, we compute the tail bound of the success probability under the parameter settings and obtain the following table:

\begin{table}[h]
\centering
\caption{Tail bound of success probability}\label{tab:success_prob}
\begin{tabular}{@{}|c|c|c|c|c|c|@{}}
\hline 
\diagbox{$t$}{$n$}    & $63$ & $127$ & $255$ & $511$ & $1023$ \\ \hline 
8   & 0 & 25.5\% & 32.7\% & 34.3\% & 34.9\% \\ \hline
9   & 52.1\% & 78.0\% & 84.2\% & 85.7\% & 86.1\% \\ \hline
10  & 75.1\% & 92.7\% & 96.5\% & 97.4\% & 97.6\% \\ \hline
11  & 85.9\% & 96.9\% & \cellcolor{blue!25}99.1\% & \cellcolor{blue!25}99.5\% & \cellcolor{blue!25}99.6\% \\ \hline
12  & 91.3\% & 98.5\% & \cellcolor{blue!25}99.7\% & \cellcolor{blue!25}99.9\% & \cellcolor{blue!25}$>$99.9\% \\ \hline
13  & 93.9\% & \cellcolor{blue!25}99.1\% & \cellcolor{blue!25}99.8\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% \\ \hline
14  & 95.1\% & \cellcolor{blue!25}99.4\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% \\ \hline
15  & 95.6\% & \cellcolor{blue!25}99.5\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% & \cellcolor{blue!25}$>$99.9\% \\ 
\hline 
\end{tabular}
\end{table}

In the table, all $(n,t)$ combinations in the blue cells satisfy the success probability requirement. Among them, $(127,13)$ has the lowest communication overhead ({\bf measured? quantized?} by $t\log n+\delta\log n$). So we set $n=127, t=13$ in this case. {\bf (may be unnecessary) Note that both the success probability and the overall communication overhead are strictly increasing w.r.t. $n$ and $t$. Hence, instead of computing all values in the table, we could strategically compute only a few of them and obtain the optimal $(n,t)$ (e.g., find the optimal $t$ for each $n$ by binary search each column).}

\end{comment}
\begin{comment}
If not, we use the ToW estimator described in \autoref{subsec:ToW} to obtain $\hat{d}$ (i.e., the estimation of $d$). Then scale it up (e.g., $d=1.38\hat{d}$ in \autoref{sec:evaluation}) for parameter setting, as explained in \autoref{subsec:ToW}. 

Here are the $4$ parameters that need to determine: 

\begin{itemize}
	\itemsep0em
	%\item $\delta$: Average number of distinct elements per group; 
	\item $g$: Number of group pairs; 
	\item $n$: Number of subset pairs in each group pair; 
	\item $r$: Number of rounds; 
	\item $t$: BCH decode capability;
\end{itemize}

Note that the number of groups $g$ is determined after $\delta$ is determined (i.e., $g=\frac{\bar{d}}{\delta}$). Now we describe how to set the four parameters using the tail bound. First, we set $\delta$ to be some small integer (e.g., $\delta=5$), so that the computational complexity (approx $\propto \delta^2$) is small. Second, we set $r$ to be some small integer (e.g., $r=3$), so that the round-trip delay is reasonable. Third, we set an objective success probability $p$ (depend on the requirement of specific applications), and we consider a parameter combination $(n,t)$ is {\it feasible} if and only if the success probability under this parameter setting based on the tail bound is larger than $p$. Among all feasible parameter combinations $(n,t)$, we select the one that has the lowest communication overhead, which can be roughly expressed as $(\delta \log u + t\log n + \delta \log n + 32)\cdot d/\delta$, as explained in \autoref{subsec:protocol2}. Here $u$ (i.e., the size of the element universe) and $d$ (i.e., the number distinct elements) do not depend on the parameter combination. So we only need to minimize $(t+\delta) \log n$ subject to $n$ and $t$. 
\end{comment}
\begin{comment}

\autoref{fig:mc} presents an example state transition diagram with 6 states (0 - 5 ``hidden elements''), denoting the corresponding transition matrix as $P=(p_{i,j})_{6\times 6}$, where $p_{i,j}$ is the probability of moving from State $i$ to State $j$. 

For instance, $p_{5,0}$ denotes the probability that all 5 set differences are decoded, which means the 5 set differences are all hashed into separate bins. $p_{5,2}$ denotes the probability that 3 (=5-2) out of 5 set differences are decoded, which means 3 set differences are hashed into separate bins and 2 set differences are hashed into the same bin. 


Let $L_{max}$ denote the maximum number of errors that BCH code can correct. Define $g^{(r)}(s)$ as follows:

\begin{equation}
    g^{(r)}(s) = \left\{ \begin{array}{ccc}
f^{(r)}(s) & \mbox{for}
& 0\leq s\leq L_{max} \\ 1 & \mbox{for} & s>L_{max}
\end{array}\right.
\end{equation}



Assume BCH code is capable of decode $s$ set differences, then the decode process of a group can be considered as a Markov chain, in which state is defined as the number of ``hidden elements'' (i.e., elements belonging to the set differences that haven't been decoded). \autoref{fig:mc} presents an example state transition diagram with 6 states (0 - 5 ``hidden elements''), denoting the corresponding transition matrix as $P=(p_{i,j})_{6\times 6}$, where $p_{i,j}$ is the probability of moving from State $i$ to State $j$. 

For instance, $p_{5,0}$ denotes the probability that all 5 set differences are decoded, which means the 5 set differences are all hashed into separate bins. $p_{5,2}$ denotes the probability that 3 (=5-2) out of 5 set differences are decoded, which means 3 set differences are hashed into separate bins and 2 set differences are hashed into the same bin. 
% And $p_{5,4}$ denotes the probability that only 1 (=5-4) set difference are decoded. The other 4 set differences could be either hashed into the same bin, or two separate bins with 2 elements in each. 

The transition in this Markov chain basically has three properties: (1) All state transitions are either self-loops or from ``higher'' states to ``lower'' states, since decode process won't generate additional set differences; (2) No state transition to State 1, because 1 remaining difference must be in a bin by itself and is able to be decoded within the same round of transition; (3) State 0 denotes all set differences are decode, which is all the absorbing state of the Markov chain. 

In the context of the Markov chain, $f^{(r)}(k)$ equals the probability that State $k$ does not transient to State 0 (absorbing state) in $r$ rounds. Let $\{e_i\}_{i=0,1,2,...,k}$ denote the standard basis vectors of length $k+1$, where $e_i$ has a single nonzero value 1 at the $(i+1)^{th}$ position. Based on the property of Markov chain, $x^{(r)}_k\triangleq e_k\cdot P^r$ is the probability vector of states after $r$ rounds with $k$ initial set differences, and the $i^{th}$ element in $x^{(r)}_k$ denotes the probability that State $k$ transients to State $i-1$ after $r$ rounds. 

$x^{(r)}(k)=(p^{(r)}_{k,0},p^{(r)}_{k,1},...,p^{(r)}_{k,k})$ denote the probability vector of states after $r$ rounds with $k$ initial set differences, where $p^{(r)}_i$ denotes the probability . 

Given the transition matrix $P$, we can easily 

\begin{figure*}
\centering
\includegraphics[width=0.98\textwidth]{figures/set_diff_markov}
\caption{Markov chain diagram for decoding process of set difference.}\label{fig:mc}
\end{figure*}

First, we assume the length of BCH decode is sufficient to decode each group. Then the decode process of each group can be considered as a Markov chain, in which state is defined as the number of "hidden elements" (i.e., elements belonging to the set difference that are to be decoded). \autoref{fig:mc} presents the state transition diagram, denoting the corresponding transmission matrix as $P=(p_{i,j})_{(d+1)\times (d+1)}$, where $p_{i,j}$ is the probability of moving from State $i$ to State $j$. By the same anology above, considering the classical balls-into-bins problem: $i$ balls are thrown independently and uniformly at random into $m'$ bins. Then $p_{i,j}$ equals to the probability that $i-j$ out of $m'$ bins have exactly one ball in each. Let $p^{(k)}_{i,j}$ denote the probability that $i-j$ out of $m'$ bins have exactly one ball in each, and $k$ out of $m'$ bins are empty. Then we have


\medskip
\noindent
{\bf Analysis on Number of Rounds}.
Consider the whole process as a Markov chain, whose state is defined as the number of 
``hidden elements'' ({\it i.e.,} elements belonging to the set difference that are to be decoded). 
\autoref{fig:mc} presents the state transition diagram, denoting the corresponding transmission 
matrix as $P=\big{(}p_{i,j}\big{)}_{(d+1)\times (d+1)}$ where $p_{i,j}$ is the probability of moving from state $i$ to state $j$. It is complex to obtain all the elements in $P$, we 
can easily get the following probabilities, for any $k \leq d$,
\begin{align}
p_{k,0}&=\frac{\binom{m}{k}k\,!}{m^k} \\
p_{k,1}&=0 \\
p_{k,2}&=\frac{\binom{k}{2}(m-k+2)\binom{m}{k-2}(k-2)\,!}{m^k},\quad \forall k\geq 2\\
p_{k,3}&=\frac{\binom{k}{3}(m-k+3)\binom{m}{k-3}(k-3)\,!}{m^k},\quad \forall k\geq 3\\
p_{k,4}&=\frac{\big{(}\binom{k}{4}(m-k+4) + \binom{k}{2}\binom{k-2}{2}(m-k+4)(m-k+3)/2\big{)}\binom{m}{k-4}(k-4)\,!}{m^k},\quad \forall k\geq 4.
\end{align}
where $m$ is the number of buckets.

Similarly, we can calculate $p_{k,i}$ for any $k\geq i \geq 5$ but the expression gets more and more complex. 


It is not hard to check that the Markov chain described above is an absorbing Markov chain with 
a single absorbing state of $0$. By using the time to absorption theorem of Absorbing Markov Chains~\cite[Page 13]{Elizalde_LectureNotesMath_2006}, 
we can easily get the average number of rounds (steps before the chain is absorbed), which equals
the $d^{th}$ element of $(N{\bf 1})$ where the matrix 
$N=(I-Q)^{-1}$ is the fundamental matrix of $P$ (Note that $Q$ is the transition matrix for all transient states, in our case, is $P$ by removing the last row and column, {\it i.e.,} $P_{0,*}$ 
and $P_{*,0}$) and 
${\bf 1}$ is an all-one vector with length $d$. 

Denote $P^{(k)}$ as the $k$-step transition matrix, then the probability that it takes more than $n$ rounds to decode is
\begin{equation}
\mathbf{Pr}[t>n]=\sum_{k=n+1}^{\infty}p^{(k)}_{d,0},
\end{equation}
where $d$ is the initial number of elements.


\medskip
\noindent
{\bf Simplified Analysis on Number of Rounds.} In the following analysis, we assume that the number of buckets in the kth round, 
assuming remaining $d_k$ elements to be decoded, is set to be $\delta\cdot d_k$ where $\delta > 1$ is a constant. For ease of 
presentation, we drop the subscript $k$ in the following analysis\footnote{Inspired by the analysis of the number of iterations 
for PIM.}. 

Fix a bucket, the probability that it gets exactly one element belonging to the set difference that is not decoded yet is:
\begin{equation}
p = d \Big{(}\frac{1}{\delta d}\Big{)}\Big{(} 1 - \frac{1}{\delta d}\Big{)}^{d - 1} = \frac{1}{\delta}\Big{(} 1 - \frac{1}{\delta d}\Big{)}^{d - 1}\approx \frac{1}{\delta}e^{-1/\delta}.
\end{equation}

On average, there are $p$ fraction of buckets will get exact one element. Hence, on average $e^{-1/\delta}$ fraction of un-decoded 
elements will be decoded in each round. Therefore, on average, we need $\log_{\frac{1}{1- e^{-1/\delta}}}d_0$ rounds, {\it i.e.,} 
$O(\log d_0)$ rounds. 

\end{comment}


